A Lyapunov analysis of Korpelevich's extragradient method with fast and flexible extensions

We develop a Lyapunov-based analysis of Korpelevich's extragradient method and show that it achieves an $o(1/k)$ last-iterate convergence rate of the constructed Lyapunov function. This Lyapunov function simultaneously upper bounds several standard measures of optimality, which allows our analysis to sharpen existing last-iterate convergence guarantees for these measures. Moreover, the same analysis enables the design of a class of flexible extensions of the extragradient method in which extragradient steps are adaptively blended with user-specified directions via a Lyapunov-guided line-search procedure. These extensions retain global convergence under practical assumptions and can attain superlinear rates when the directions are chosen appropriately. Numerical experiments confirm the simplicity and efficiency of the proposed framework.

==> TeX/Algs/Prox-I-FLEX.tex <==
%!TEX root = ../../main.tex
\begin{algorithm}[t]
    \caption{\ProxIFLEX{} (Proximal-\texttt{I-FLEX})} 
    \label{alg:Prox-I-FLEX}
    \begin{algorithmic}[1]
        \INITIALIZE  \(z^{0}\in\calH\), \(\gamma\in\p{0,1/L_{F}}\), \(\p{\sigma,\beta} \in \p{0,1}^{}\)
        \REQUIRE Lyapunov function \(\V\) as in \eqref{eq:V} and algorithmic operators \(T_1^{\gamma}, T_2^{\gamma}\) as in \eqref{eq:T1T2}
        \For{\(k = 0, 1, 2, \ldots\)}
            \State \(\bar{z}^{k} = T_1^\gamma(z^k)\) \label{State:Prox-I-FLEX:EG:1}   \hfill {\footnotesize\gray  \( = \prox_{\gamma g} \big(z^{k} - \gamma F\p{z^{k}}\big) \)}
            \State \(w^{k} = T_2^\gamma(z^k)\)
            \hfill {\footnotesize\gray  \(= \prox_{\gamma g} \big(z^{k} - \gamma F\p{\bar{z}^{k}}\big)\)}
            \State\label{State:Prox-I-FLEX:dk}Compute a direction \(d^{k}\in\calH\) at \(z^{k}\)
            \If{\(\norm{w^{k}-\bar{z}^{k}} = 0\)} \label{State:Prox-I-FLEX:contraction}
                \Return $z^{k}$
            \Else
                \State \label{State:Prox-I-FLEX:LS} 
                \begin{tabular}[t]{@{}r@{}l@{}}
                Set \(z^{k+1} = \p{1-\tau_{k}} w^{k} + \tau_{k} (z^{k} + d^{k})\) where \(\tau_{k}\) is the largest number in 
                \\
                \(\set{ \beta^{i} \mid i\in\naturals }\) such that \hfill\hfill
                \end{tabular}
                \begin{align}\label{eq:Prox-I-FLEX:descent}
                     ~~~~~~~~~\mathcal{V}(z^{k+1}, T_1^\gamma(z^{k+1}), T_2^\gamma(z^{k+1})) \leq \mathcal{V}(z^k, \bar z^k, w^{k}) - \sigma\p{1-\gamma^{2}L_{F}^{2}} \norm{w^{k}-\bar{z}^{k}}^{2}
                \end{align}
            \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm}

==> extragradient/TeX/Algs/Cournot_Nash_data_generation.tex <==
\begin{customalgorithm}{Datagen}[H]
    \begin{algorithmic}[1] 
        \INPUT \(n \in \mathbb{N}\) 
        \OUTPUT \(\p{\p{T_{i}, a_{i}, b_{i}, m_{i}, d_{i}}}_{i=1}^{n}\) 
        \Repeat 
            \State For each \(i \in \llbracket1,n\rrbracket\), sample \(m_{i}\) uniformly from \([150, 250]\) 
            \State For each \(i \in \llbracket1,n\rrbracket\), sample \(b_{i}\) uniformly from \([30, 50]\) 
            \State For each \(i \in \llbracket1,n\rrbracket\), sample \(T_{i}\) uniformly from \([3, 7]\) 
            \State For each \(i \in \llbracket1,n\rrbracket\), sample \(d_{i}\) uniformly from \([5, 20]\) 
            \State Sort \(\p{d_{i}}_{i=1}^{n}\) in increasing order 
            \State For each \(i \in \llbracket1,n\rrbracket\), sample \(u_{i}\) uniformly from \([-10, -5]\) 
            \State For each \(i \in \llbracket1,n\rrbracket\), compute \(a_{i} = d_{i} / u_{i}\) 
            \State Sort \(\p{a_{i}}_{i=1}^{n}\) in decreasing order 
            \State \(\text{valid} \leftarrow \texttt{True}\) 
            \For{\(i \in \llbracket1,n\rrbracket\)} 
                \If{\(b_{i} < -2 a_{i} T_{i}\) \textbf{or} \(m_{i} \leq b_{i}\) \textbf{or} \(d_{i} \leq - a_{i}\) } 
                    \State \(\text{valid} \leftarrow \texttt{False}\) 
                    \State \textbf{break} 
                \EndIf 
            \EndFor 
        \Until{\(\text{valid}\) is \texttt{True}} 
    \end{algorithmic}
\end{customalgorithm}

==> extragradient/TeX/Algs/FLEX.tex <==
%!TEX root = ../../main.tex
\begin{algorithm}[t]
    \caption{\FLEX~(Fast Line-search EXtragradient)}
    \label{alg:FLEX}
    \begin{algorithmic}[1]
        \INITIALIZE  \(z^{0}\in\calH\), \(\gamma\in\p{0,{1}/{L_{F}}}\), \(\p{\rho,\sigma,\beta} \in \p{0,1}^{3}\), \(M\in\mathbb{N}_{0}\)
        \For{\(k = 0, 1, 2, \ldots\)}
            \State \label{State:FLEX:dk} Compute a direction \(d^{k}\in\calH\) at \(z^{k}\)
            \If{\(\norm{F\p{z^{k} + d^{k} }} \leq \rho\norm{F\p{z^{k}}}\)} \label{State:FLEX:contraction}
                \State \label{State:FLEX:full} \(z^{k+1} = z^{k} + d^{k}\)
            \Else
                \State \label{State:FLEX:EG} \(\bar{z}^{k} =  z^{k} - \gamma F\p{z^{k}}\); \(w^{k} = z^{k} - \gamma F\p{\bar{z}^{k}}\)
                \State \label{State:FLEX:LS} 
                \begin{tabular}[t]{@{}r@{}l@{}}
                     Set \(z^{k+1} = \p{1-\tau_{k}} w^{k} + \tau_{k} (z^{k} + d^{k})\) where \(\tau_{k}\) is the largest number in
                    \\
                     \(\set{ \beta^{i} \mid i \in \llbracket 1 , M \rrbracket}\cup\set{0}\) such that \hfill\hfill
                    \end{tabular}
                \begin{align}\label{eq:FLEX:descent}
                    \norm{F\p{z^{k+1}}}^{2} \leq \norm{F\p{z^{k}}}^{2} - \sigma\p{1-\gamma^{2}L_{F}^{2}} \norm{F\p{z^{k}}-F\p{\bar{z}^{k}}}^{2}
                \end{align}    
            \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm}

==> extragradient/TeX/Algs/I-FLEX.tex <==
%!TEX root = ../../main.tex
\begin{algorithm}[t]
    \caption{\IFLEX{} (Injective-\texttt{FLEX})}
    \label{alg:I-FLEX}
    \begin{algorithmic}[1]
        \INITIALIZE  \(z^{0}\in\calH\), \(\gamma\in\p{0,{1}/{L_{F}}}\), \(\p{\sigma,\beta} \in \p{0,1}^{2}\)
        \For{\(k = 0, 1, 2, \ldots\)}
        \State \label{State:I-FLEX:dk} Compute a direction \(d^{k}\in\calH\) at \(z^{k}\)
        \State \label{State:I-FLEX:EG} \(\bar{z}^{k} =  z^{k} - \gamma F\p{z^{k}}\); \(w^{k} = z^{k} - \gamma F\p{\bar{z}^{k}}\)
        \State \label{State:I-FLEX:LS} 
            \begin{tabular}[t]{@{}r@{}l@{}}
                     Set \(z^{k+1} = \p{1-\tau_{k}} w^{k} + \tau_{k} (z^{k} + d^{k})\) where \(\tau_{k}\) is the largest number in 
                    \\
                     \(\set{ \beta^{i} \mid i \in \naturals}\) such that \hfill\hfill
            \end{tabular}
            \begin{align}\label{eq:I-FLEX:descent}
                \norm{F\p{z^{k+1}}}^{2} \leq \norm{F\p{z^{k}}}^{2} - \sigma\p{1-\gamma^{2}L_{F}^{2}} \norm{F\p{z^{k}}-F\p{\bar{z}^{k}}}^{2}
            \end{align}    
        \EndFor
    \end{algorithmic}
\end{algorithm}

==> extragradient/TeX/Algs/Prox-FLEX.tex <==
%!TEX root = ../../main.tex
\begin{algorithm}[t]
    \caption{\ProxFLEX{} (Proximal-\texttt{FLEX})} 
    \label{alg:Prox-FLEX}
    \begin{algorithmic}[1]
        \INITIALIZE  \(z^{0}\in\calH\), \(\gamma\in\p{0,1/L_{F}}\), \(\p{\rho,\sigma,\beta} \in \p{0,1}^{3}\), \(M\in\mathbb{N}_{0}\)
        \REQUIRE Lyapunov function \(\V\) as in~\eqref{eq:V} and algorithmic operators \(T_1^{\gamma}, T_2^{\gamma}\) as in~\eqref{eq:T1T2}
        \For{\(k = 0, 1, 2, \ldots\)}
            \State\label{State:Prox-FLEX:dk}Compute a direction \(d^{k}\in\calH\) at \(z^{k}\)
            \State \(\bar{z}^{k} = T_1^\gamma(z^k)\) \label{State:Prox-FLEX:EG:1} \hfill {\footnotesize\gray  \( = \prox_{\gamma g} \big(z^{k} - \gamma F\p{z^{k}}\big) \)}
            \State \(w^{k} = T_2^\gamma(z^k)\)
            \hfill {\footnotesize\gray  \(= \prox_{\gamma g} \big(z^{k} - \gamma F\p{\bar{z}^{k}}\big)\)}
            \If{\(\mathcal{V}(z^{k} + d^{k}, T_1^\gamma(z^{k} + d^{k}), T_2^\gamma(z^{k} + d^{k})) \leq \rho^2 \mathcal{V}(z^k, \bar z^k, w^{k}) \)} \label{State:Prox-FLEX:contraction}
                \State \label{State:Prox-FLEX:full} \(z^{k+1} = z^{k} + d^{k}\)
            \Else
                \State \label{State:Prox-FLEX:LS} 
                \begin{tabular}[t]{@{}r@{}l@{}}
                Set \(z^{k+1} = \p{1-\tau_{k}} w^{k} + \tau_{k} (z^{k} + d^{k})\) where \(\tau_{k}\) is the largest number in 
                \\
                \(\set{ \beta^{i} \mid i \in \llbracket 1 , M \rrbracket}\cup\set{0}\) such that \hfill\hfill
                \end{tabular}
                \begin{align}\label{eq:Prox-FLEX:descent}
                     ~~~~~~~~~\mathcal{V}(z^{k+1}, T_1^\gamma(z^{k+1}), T_2^\gamma(z^{k+1})) \leq \mathcal{V}(z^k, \bar z^k, w^{k}) - \sigma\p{1-\gamma^{2}L_{F}^{2}}\gamma^{-2} \norm{w^{k}-\bar{z}^{k}}^{2}
                \end{align}
            \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm}

==> extragradient/TeX/Algs/Prox-I-FLEX.tex <==
%!TEX root = ../../main.tex
\begin{algorithm}[t]
    \caption{\ProxIFLEX{} (Proximal-\texttt{I-FLEX})} 
    \label{alg:Prox-I-FLEX}
    \begin{algorithmic}[1]
        \INITIALIZE  \(z^{0}\in\calH\), \(\gamma\in\p{0,1/L_{F}}\), \(\p{\sigma,\beta} \in \p{0,1}^{}\)
        \REQUIRE Lyapunov function \(\V\) as in \eqref{eq:V} and algorithmic operators \(T_1^{\gamma}, T_2^{\gamma}\) as in \eqref{eq:T1T2}
        \For{\(k = 0, 1, 2, \ldots\)}
            \State \(\bar{z}^{k} = T_1^\gamma(z^k)\) \label{State:Prox-I-FLEX:EG:1}   \hfill {\footnotesize\gray  \( = \prox_{\gamma g} \big(z^{k} - \gamma F\p{z^{k}}\big) \)}
            \State \(w^{k} = T_2^\gamma(z^k)\)
            \hfill {\footnotesize\gray  \(= \prox_{\gamma g} \big(z^{k} - \gamma F\p{\bar{z}^{k}}\big)\)}
            \State\label{State:Prox-I-FLEX:dk}Compute a direction \(d^{k}\in\calH\) at \(z^{k}\)
            \If{\(\norm{w^{k}-\bar{z}^{k}} = 0\)} \label{State:Prox-I-FLEX:contraction}
                \Return $z^{k}$
            \Else
                \State \label{State:Prox-I-FLEX:LS} 
                \begin{tabular}[t]{@{}r@{}l@{}}
                Set \(z^{k+1} = \p{1-\tau_{k}} w^{k} + \tau_{k} (z^{k} + d^{k})\) where \(\tau_{k}\) is the largest number in 
                \\
                \(\set{ \beta^{i} \mid i\in\naturals }\) such that \hfill\hfill
                \end{tabular}
                \begin{align}\label{eq:Prox-I-FLEX:descent}
                     ~~~~~~~~~\mathcal{V}(z^{k+1}, T_1^\gamma(z^{k+1}), T_2^\gamma(z^{k+1})) \leq \mathcal{V}(z^k, \bar z^k, w^{k}) - \sigma\p{1-\gamma^{2}L_{F}^{2}} \norm{w^{k}-\bar{z}^{k}}^{2}
                \end{align}
            \EndIf
        \EndFor
    \end{algorithmic}
\end{algorithm}

==> extragradient/TeX/Algs/minimax_data_generation.tex <==
\begin{customalgorithm}{Datagen}[H]
    \begin{algorithmic}[1]
        \INPUT \(\QuadMinMaxParam \in \reals_{+}\) and \(n \in \mathbb{N}\)
        \OUTPUT \(x^{\star},\,y^{\star} \in \reals^{n}\), \(A,\, B \in \sym^{n}_{+}\) and \(C \in \reals^{n \times n}\)
        \State Let \(x^{\star},\,y^{\star} \in \reals^{n}\) such that \(x_{i}^{\star},\,y_{i}^{\star}\sim \mathcal{N}(0, 1)\) for each \(i\in\llbracket1,n\rrbracket\)
        \State Let \(S \in \mathbb{R}^{n \times n}\) such that \([S]_{i,j} \sim \mathcal{N}(0, 1/\sqrt{n})\) for each \(i,j\in\llbracket1,n\rrbracket\)
        \State \(S \leftarrow \p{S + S^\top}/2\)
        \State \(S \leftarrow S + \p{\abs{\lambda_{\min}(S)} + 1} I\)
        \State \(A \leftarrow \QuadMinMaxParam S\)
        \State Repeat steps 2-4 with a different random seed and let \(B \leftarrow \QuadMinMaxParam S\)
        \State Repeat step 2 with a different random seed and let \(C \leftarrow S\)
    \end{algorithmic}
\end{customalgorithm}

==> extragradient/TeX/Text/Lyapunov.tex <==
%!TEX root = main.tex
\section{A new Lyapunov analysis}\label{sec:Lyapunov}
Classical convergence analyses of Korpelevich’s extragradient method~\eqref{alg:EG} typically rely on Fejér-type arguments, as discussed in \Cref{app:background}. In this section, we introduce a complementary Lyapunov inequality that not only leads to a last-iterate result but also forms the basis of the new algorithms presented in \Cref{sec:algs}. Throughout this work, we investigate~\eqref{eq:the_inclusion_problem} under the following assumption.

\begin{assumption}\label{ass:main} 
    The following hold in problem~\eqref{eq:the_inclusion_problem}.
    \begin{enumeratass} 
        \item \label{ass:F} \(F:\calH\to\calH\) is monotone and \(L_{F}\)-Lipschitz continuous for some \(L_{F}\in\reals_{++}\).
        \item \label{ass:g}\(g:\calH\to \reals \cup \{+\infty\}\) is proper, convex and lower semicontinuous. 
    \end{enumeratass}
\end{assumption}

Our analysis is centered around the Lyapunov function \(\mathcal{V}:\calH^{3}\to\reals\) given by
\begin{equation}\label{eq:V}
    \mathcal{V}(z, \bar z, z^{+}) = 2\gamma^{-1}\inner{z - z^{+}}{F\p{z} - F\p{\bar{z}}} + \gamma^{-2}\norm{z^{+} - \bar{z}}^{2} + \gamma^{-2}\norm{z - z^{+}}^{2} 
\end{equation}
for each \(\p{z, \bar z, z^{+}} \in \calH^{3}\). \Cref{prop:V_performance_measure} establishes that \(\mathcal{V}\) is generally a valid optimality measure for the inclusion problem in~\eqref{eq:the_inclusion_problem}. For notational convenience, we define the algorithmic operators \(T_{1}^{\gamma}, T_{2}^{\gamma} : \calH \to \calH\) by 
\begin{equation}\label{eq:T1T2}
    T_{1}^{\gamma} = \prox_{\gamma g} \circ (\Id - \gamma F) 
    \quad \text{and} \quad
    T_{2}^{\gamma} = \prox_{\gamma g} \circ (\Id - \gamma F \circ T_{1}^{\gamma}),
\end{equation}
where \(\gamma \in \reals_{++}\) is the step-size parameter. With this notation, the iterates of~\eqref{alg:EG} can be written compactly as \(\bar{z}^k = T_{1}^{\gamma}(z^k)\) and \(z^{k+1} = T_2^{\gamma}(z^k)\).

\input{TeX/Text/Results/V_optimality_measure}

The following result shows that \(\mathcal{V}\) is, in fact, a suitable Lyapunov function for the extragradient method~\eqref{alg:EG}, i.e., it fulfills a descent inequality. Moreover, the descent inequality neither contains a solution of~\eqref{eq:the_inclusion_problem} nor assumes the existence of a solution. 

\input{TeX/Text/Results/dual_Vk_inequality}

Next, we present \Cref{cor:EG:new_Lyapunov_w.o._sol:g_zero}, which follows immediately from \Cref{thm:EG:new_Lyapunov_w.o._sol} by letting \(g=0\). \new{Observe that \Cref{cor:EG:new_Lyapunov_w.o._sol:g_zero} recovers known results, e.g., see~\cite[Lemma 3.2 and Theorem 3.3]{gorbunov2022extragradientmethodo1/k},~\cite[Theorem 1]{cai2022tightlastiterateconvergenceextragradient}, and~\cite[Remark 2.1]{bot2024extragradientmethod}.}

\input{TeX/Text/Results/last_iterate_g_zero}

The following result shows that \(\V_k\), when scaled by a nonnegative constant, equals the residual of a Fej\'er-type inequality. As a direct consequence, this gives a \(o(1/k)\) last-iterate convergence result in terms of \(\V_k\) as presented in \Cref{cor:lastiter:T}. 

\input{TeX/Text/Results/primal_Vk_inequality}

\input{TeX/Text/Results/last_iterate_Vk}

\new{
\begin{remark}\label{rmk:cyclically_monotone}
    A close review of the proofs of \Cref{thm:EG:new_Lyapunov_w.o._sol,thm:EG:primal_descent_for_V} (and therefore also \Cref{cor:lastiter:T}) shows that the arguments remain valid when \(\partial g\) in \eqref{eq:the_inclusion_problem} is replaced with a maximally monotone and 3-cyclically monotone operator \(T:\calH\to\calH\) (see \cite[Definition 22.13]{bauschke2017convexanalysismonotone}) and the proximal operators \(\prox_{\gamma g}\) in \eqref{alg:EG} with the resolvent \(\p{\Id + \gamma T}^{-1}\); the only change is to use cyclic-monotonicity inequalities in place of the subgradient inequalities. We nonetheless choose to present the slightly more restrictive subdifferential‐based formulation, as it avoids the added abstraction of cyclic monotonicity and is likely more immediately accessible to a broader audience.
\end{remark}
}

==> extragradient/TeX/Text/Results/V_optimality_measure.tex <==
%!TEX root = ../../../main.tex
\begin{proposition}\label{prop:V_performance_measure}
    Suppose that \Cref{ass:main} holds. Let  \(\gamma \in (0, 1/L_F)\), \(z\in \calH\), \(\bar z = T_{1}^{\gamma}(z)\) and \(z^+ = T_{2}^{\gamma}(z)\) where \(T_{1}^{\gamma}\) and \(T_{2}^{\gamma}\) are the algorithmic operators defined in~\eqref{eq:T1T2}, and \(\mathcal{V}\) the Lyapunov function defined in~\eqref{eq:V}. Then the following hold.
    \begin{propenumerate}
        \item \(\mathcal{V}\p{z, \bar z, z^+}  \geq  \p{1- \gamma \LF}\gamma^{-2} \p{\norm{{z}^{+}-\bar{z}}^{2} + \norm{{z}^{+}-{z}}^{2} } \geq 0\).
        \label{prop:V_performance_measure:lower_bound}
        \item \(\mathcal{V}\p{z, \bar z, z^+} = 0\) if and only if \(z = \bar z = z^+ \in \zer\p{F + \partial g }\).\label{prop:V_performance_measure:zero_iff}
    \end{propenumerate}
    \begin{proof}\textit{ }
    \begin{itemize}
            \item[\ref{prop:V_performance_measure:lower_bound}:] 
            The inner product in the definition of \(\V\) can be written as 
            {\begin{allowdisplaybreaks}
            \begin{align*}
                \inner{ {z}-{z}^{+}}{F\p{z}-F\p{\bar{z}}}
                ={}&
                 \inner{ {z}-{z}^{+}}{F\p{z}-F\p{z^{+}}}
                 + 
                 \inner{ {z}-{z}^{+}}{F\p{z^{+}}-F\p{\bar{z}}}
                 \\
                 \geq{}& 
                 \inner{ {z}-{z}^{+}}{F\p{z^{+}}-F\p{\bar{z}}}
                 \\
                 \geq{}&
                 -\norm{{z}-{z}^{+}}\norm{F\p{z^{+}}-F\p{\bar{z}}}
                 \\
                 \geq{}& 
                 - \LF\norm{{z}-{z}^{+}}\norm{{z}^{+}-\bar{z}} \\
                 \geq{}&
                 -\tfrac{\LF}{2} \p{\norm{{z}-{z}^{+}}^{2} + \norm{{z}^{+}-\bar{z}}^{2} },
            \end{align*}
            \end{allowdisplaybreaks}}%
            where monotonicity of \(F\) is used in the first inequality, the Cauchy--Schwarz inequality is used in the second inequality, Lipschitz continuity of \(F\) is used in the third inequality, and Young's inequality for products is used in the fourth inequality. The lower bound of \(\mathcal{V}\) follows from using this inequality in~\eqref{eq:V} and the assumption \(\gamma\LF \in (0,1)\).
            \item[\ref{prop:V_performance_measure:zero_iff}:] Suppose that \(\mathcal{V}\p{z, \bar z, z^+} = 0\). Then \Cref{prop:V_performance_measure:lower_bound} and \Cref{prop:EG:fixed_point:fixed_points_are_solutions} imply that \(z = \bar z = z^+ \in \zer\p{F + \partial g }\). Conversely, suppose that \(z = \bar z = z^+ \in \zer\p{F + \partial g }\). Then it is clear from~\eqref{eq:V} that \(\mathcal{V}\p{z, \bar z, z^+} = 0\). \qedhere
        \end{itemize}
    \end{proof}
\end{proposition} 


==> extragradient/TeX/Text/Results/dual_Vk_inequality.tex <==
\begin{theorem}\label{thm:EG:new_Lyapunov_w.o._sol}
    Suppose that \Cref{ass:main} holds and the sequence \(\p{\p{z^{k},\bar{z}^{k}}}_{k\in\naturals}\) is generated by~\eqref{alg:EG} with initial point \(z^0\in \calH\) and step-size parameter \(\gamma \in \reals_{++}\). Then
    \begin{align}\label{eq:EG:new_Lyapunov_w.o._sol}
        \mathcal{V}_{k+1} \leq \mathcal{V}_{k} - \p{1-\gamma^{2}L_{F}^{2}} \gamma^{-2}\norm{z^{k+1}-\bar{z}^{k}}^{2}
    \end{align}
    for each \(k\in \naturals\), where \(\V_k =\mathcal{V}(z^k, \bar z^k, z^{k+1})\) for the Lyapunov function \(\mathcal V\) defined in~\eqref{eq:V}.

    \begin{proof}
        Note that the first and second proximal steps in~\eqref{alg:EG} can equivalently be written via their subgradient characterization as
        \begin{equation}\label{eq:subgrad:char}
            \gamma^{-1}\p{z^{k}-\bar{z}^{k}}-F(z^{k}) \in \partial g(\bar z^k) \quad \text{ and } \quad 
         \gamma^{-1}\p{z^{k}-z^{k+1}}-F(\bar{z}^{k}) \in \partial g(z^{k+1}),
        \end{equation}
        respectively. Using the subgradient inequality at the points \(z^{k+1}\), \(z^{k+2}\) and \(\bar{z}^{k+1}\), with the particular subgradients given in~\eqref{eq:subgrad:char}, it follows that
        \begin{subequations}
            \begin{align}\label{eq:EG:prox_implicit:k1}
            0 &\geq g\p{z^{k+1}} - g\p{z} + \inner{\gamma^{-1}\p{z^{k} - z^{k+1}} - F\p{\bar{z}^{k}}}{z-z^{k+1}},
            \\ \label{eq:EG:prox_implicit:k2}
            0 &\geq g\p{z^{k+2}} - g\p{z} + \inner{\gamma^{-1}\p{z^{k+1} - z^{k+2}} - F\p{\bar{z}^{k+1}}}{z-z^{k+2}},
            \\ \label{eq:EG:prox_implicit:kbar1}
            0 &\geq g\p{\bar{z}^{k+1}} - g\p{z} + \inner{\gamma^{-1}\p{z^{k+1} - \bar{z}^{k+1}} - F\p{z^{k+1}}}{z-\bar{z}^{k+1}}.
        \end{align}
        \end{subequations}
        holds for any \(z \in \calH\), respectively. Picking \(z = \bar{z}^{k+1}\) in~\eqref{eq:EG:prox_implicit:k1}, \(z = z^{k+1}\) in~\eqref{eq:EG:prox_implicit:k2}, \(z = z^{k+2}\) in~\eqref{eq:EG:prox_implicit:kbar1}, summing the resulting inequalities, and multiplying by \(2\gamma^{-1}\) gives 
        {\begin{allowdisplaybreaks}
        \begin{align} \notag
            0 
            \geq{}& 
            2\gamma^{-2}\inner{ z^{k} - z^{k+1} }{\bar{z}^{k+1}-z^{k+1}}   - 2 \gamma^{-1} \inner{F\p{\bar{z}^{k}} }{\bar{z}^{k+1}-z^{k+1}}  
            \nonumber
            \\
            &{}+ 
            2\gamma^{-2}\norm{ z^{k+1} - z^{k+2} }^{2}  - 2\gamma^{-1}\inner{ F\p{\bar{z}^{k+1}} }{z^{k+1}-z^{k+2}} 
            \nonumber
            \\
            &{}+ 
            2\gamma^{-2}\inner{ z^{k+1} - \bar{z}^{k+1}}{z^{k+2}-\bar{z}^{k+1}} - 2\gamma^{-1} \inner{ F\p{z^{k+1}} }{z^{k+2}-\bar{z}^{k+1}}.
                \label{eq:ApB}
        \end{align}
        \end{allowdisplaybreaks}}%
        The first two inner products in~\eqref{eq:ApB} can be simplified as  
        {\begin{allowdisplaybreaks}
        \begin{align*}
            A_k & =  2\gamma^{-2}\inner{ z^{k} - z^{k+1} }{\bar{z}^{k+1}-z^{k+1}}   - 2 \gamma^{-1} \inner{F\p{\bar{z}^{k}} }{\bar{z}^{k+1}-z^{k+1}} \\
            &= \gamma^{-2}\norm{z^{k} - z^{k+1}}^2 + \gamma^{-2}\norm{ \bar{z}^{k+1}-z^{k+1} }^2 - \gamma^{-2}\norm{z^{k} - \bar{z}^{k+1} }^2  - 2 \gamma^{-1} \inner{F\p{\bar{z}^{k}} }{\bar{z}^{k+1}-z^{k+1}},
        \end{align*}
        \end{allowdisplaybreaks}}%
        where the identity \(2\inner{x}{y} = \norm{x}^2 + \norm{y}^2 - \norm{x-y}^2\) for each \(x,y\in \calH\) is used in the second equality, while the remaining four terms in~\eqref{eq:ApB} can be simplified as 
        {\begin{allowdisplaybreaks}
        \begin{align*}
            B_k &  =  
            \begin{aligned}[t]
                & 2\gamma^{-2}\norm{ z^{k+1} - z^{k+2} }^{2}  - 2\gamma^{-1}\inner{ F\p{\bar{z}^{k+1}} }{z^{k+1}-z^{k+2}} \\
                & + 2\gamma^{-2}\inner{ z^{k+1} - \bar{z}^{k+1}}{z^{k+2}-\bar{z}^{k+1}} -  2\gamma^{-1} \inner{ F\p{z^{k+1}} }{z^{k+2}-\bar{z}^{k+1}} 
            \end{aligned}\\
            & = 
            \begin{aligned}[t]
                & 2\gamma^{-1}\inner{z^{k+1} - z^{k+2}}{F\p{z^{k+1}} - F\p{\bar{z}^{k+1}}} + \gamma^{-2}\norm{z^{k+2} - \bar{z}^{k+1}}^{2} + \gamma^{-2}\norm{z^{k+1} - z^{k+2}}^{2}  \\
                & + \gamma^{-2}\norm{z^{k+1} - \bar{z}^{k+1}}^2 - 2\gamma^{-1} \inner{ F\p{z^{k+1}} }{z^{k+1}-\bar{z}^{k+1}} 
            \end{aligned}\\
            &= \mathcal{V}_{k+1} + \gamma^{-2}\norm{z^{k+1} - \bar{z}^{k+1}}^2 - 2\gamma^{-1} \inner{ F\p{z^{k+1}} }{z^{k+1}-\bar{z}^{k+1}},
        \end{align*}
        \end{allowdisplaybreaks}}%
        where the identity \(2\inner{x}{y} = \norm{x}^2 + \norm{y}^2 - \norm{x-y}^2\) for each \(x,y\in \calH\) is used in the second equality, and the explicit expression for \(\V_{k+1} =\mathcal{V}(z^{k+1}, \bar z^{k+1}, z^{k+2})\) is used in the third equality. Therefore, the inequality \(A_k + B_k \leq 0\) in~\eqref{eq:ApB} can be rearranged as  
        \begin{equation}\label{eq:V+:ub}
            \mathcal{V}_{k+1}  
            \leq{}
            \begin{aligned}[t]
                &\gamma^{-2}\norm{z^{k} - \bar{z}^{k+1}}^2  - \gamma^{-2}\norm{z^{k} - z^{k+1}}^2 - 2\gamma^{-2}\norm{ \bar{z}^{k+1}-z^{k+1} }^2 \\
                & + 2\gamma^{-1} \smash{\underbracket{\inner{F\p{\bar{z}^{k}} - F\p{z^{k+1}} }{\bar z^{k+1}-{z}^{k+1}}%
                }_{=C_k}}.
            \end{aligned}
        \end{equation}
        We can upper bound the term \(C_k\) as
            \begin{align}
            C_k
            ={}&
            \inner{F\p{{z}^{k}} - F\p{z^{k+1}} }{z^{k+1} - z^k} 
            + 
            \inner{F\p{\bar{z}^{k}} - F\p{z^{k}} }{z^{k+1} - z^k} 
            \nonumber \\
            &{}
            + \inner{F\p{\bar{z}^{k}} - F\p{z^{k+1}} }{\bar{z}^{k+1} + z^k - 2z^{k+1}}
            \nonumber
            \\
            \leq{}&
            \inner{F\p{\bar{z}^{k}} - F\p{z^{k}} }{z^{k+1} - z^k}
            \nonumber \\
            &{}
            + \tfrac{\gamma}{2}\norm{F\p{\bar{z}^{k}} - F\p{z^{k+1}}}^{2} + \tfrac1{2\gamma}\norm{\bar{z}^{k+1}-2z^{k+1} + z^{k}}^{2}
            \nonumber 
            \\
            \leq{}&
            \inner{F\p{\bar{z}^{k}} - F\p{z^{k}} }{z^{k+1} - z^k}
            {}
            + \tfrac{\gamma L_F^2}{2}\norm{{\bar{z}^{k}} - {z^{k+1}}}^{2} 
            \nonumber \\
            &{}
            + \tfrac1{2\gamma}
            (%
            2\norm{z^{k} - z^{k+1}}^2 + 2\norm{ \bar{z}^{k+1}-z^{k+1} }^2
            -\norm{z^{k} - \bar{z}^{k+1}}^2 
            )
            \label{eq:innerprod:vk+:ub}
        \end{align}
        where monotonicity of \(F\) and Young's inequality is used in the first inequality, and Lipschitz continuity of \(F\) along with the identity \(\norm{x+y}^{2} + \norm{x-y}^{2} = 2\norm{x}^{2} + 2\norm{y}^{2}\) for each \(x,y\in\calH\) is used in the last inequality. 

        Combining~\eqref{eq:V+:ub} and~\eqref{eq:innerprod:vk+:ub}, and using \(\mathcal{V}_{k}= 2\gamma^{-1}\inner{z^{k} - z^{k+1}}{F\p{z^{k}} - F\p{\bar{z}^{k}}} + \gamma^{-2}\norm{z^{k+1} - \bar{z}^{k}}^{2}  + \gamma^{-2}\norm{z^{k} - z^{k+1}}^{2}\) gives 
        \begin{align*}
            \V_{k+1} - \V_k 
            \leq{}&
            2\gamma^{-1}\inner{z^{k+1} - z^k}{F\p{\bar{z}^{k}} - F\p{z^{k}} }
            {}
            + { L_F^2}\norm{{\bar{z}^{k}} - {z^{k+1}}}^{2} 
            \\
            &{}
            +\gamma^{-2}\norm{z^{k} - z^{k+1}}^2 
            - \V_k
            \\
            = {}&
            - (1- \gamma^2 L_F^2)\gamma^{-2}\norm{{\bar{z}^{k}} - {z^{k+1}}}^{2},
        \end{align*}
        as claimed. 
    \end{proof}
\end{theorem}

==> extragradient/TeX/Text/Results/last_iterate_Vk.tex <==
\begin{corollary}\label{cor:lastiter:T}
    Suppose that \Cref{ass:main} and \(\zer\p{F + \partial g}\neq \emptyset\) hold, and the sequence \(\p{\p{z^{k},\bar{z}^{k}}}_{k\in\naturals}\) is generated by~\eqref{alg:EG} with initial point \(z^0\in \calH\) and step-size parameter \(\gamma\in(0,1/L_{F})\). \new{Then,
    \begin{align}\label{eq:Vk:last_iterate:little-o}
        \V_{k} \in o\p{1/k} \text{ as } k \to \infty,
    \end{align}
    and for any \(k\in\naturals\) and \(z^{\star}\in\zer\p{F + \partial g}\) it holds that  
    \begin{align}\label{eq:Vk:last_iterate}
        \V_{k} \leq \frac{\norm{z^{0} - z^{\star} }^{2} }{ \alpha\p{ \gamma, L_{F}} \p{k+1} },
    \end{align}
    where \(\alpha\p{ \gamma, L_{F}}>0\) is defined in~\eqref{eq:EG:primal_descent_for_V:alpha} and \(\V_k =\mathcal{V}(z^k, \bar z^k, z^{k+1})\) for the Lyapunov function \(\V\) defined in~\eqref{eq:V}.}
    \begin{proof}
        \new{The last-iterate convergence results in \eqref{eq:Vk:last_iterate:little-o} and \eqref{eq:Vk:last_iterate} follows by inductively summing~\eqref{eq:EG:primal_descent_for_V}, rearranging, dividing by \(\alpha\p{ \gamma, L_{F}}\), and using monotonicity of \(\p{\V_k}_{k\in\naturals}\) as shown in~\eqref{eq:EG:new_Lyapunov_w.o._sol}.} 
    \end{proof}
\end{corollary}

==> extragradient/TeX/Text/Results/last_iterate_g_zero.tex <==
\begin{corollary}\label{cor:EG:new_Lyapunov_w.o._sol:g_zero}
    Suppose that \Cref{ass:F} holds and the sequence \(\p{\p{z^{k},\bar{z}^{k}}}_{k\in\naturals}\) is generated by 
    \begin{subequations}%\label{alg:EG:g_zero}
            \begin{align*}
                \bar{z}^{k} &=z^{k} - \gamma F\p{z^{k}}, \\
                z^{k+1}     &=z^{k} - \gamma F\p{\bar{z}^{k}}
            \end{align*}
    \end{subequations}
    for each \(k\in\naturals\), with initial point \(z^0\in \calH\) and step-size parameter \(\gamma \in \reals_{++}\). Then, 
    \begin{align}\label{eq:EG:new_Lyapunov_w.o._sol:g_zero}
        \norm{F\p{z^{k+1}}}^{2} \leq \norm{F\p{z^{k}}}^{2} - \p{1-\gamma^{2}L_{F}^{2}} \norm{F\p{z^{k}}-F\p{\bar{z}^{k}}}^{2}
    \end{align}
    for each \(k\in \naturals\). \new{Moreover, if \(\gamma\in\p{0,1/L_{F}}\) and \(\zer\p{F} \neq \emptyset\), then
    \begin{align}\label{eq:EG:g_zero:little-o}
        \norm{F\p{z^{k}}}^{2} \in o\p{1/k} \text{ as }  k \to \infty,
    \end{align}
    and for any \(k\in\naturals\) and \(z^{\star} \in \zer\p{F}\) it holds that
    \begin{align}\label{eq:EG:g_zero:last_iterate_rate}
        \norm{F\p{z^{k}}}^{2} \leq \frac{\norm{z^{0}-z^{\star}}^{2} }{\gamma^{2}\p{1-\gamma^{2} L_{F}^{2}}\p{k+1}}.
    \end{align}}
    
    \begin{proof}
        Letting \(g=0\) in \Cref{thm:EG:new_Lyapunov_w.o._sol} gives~\eqref{eq:EG:new_Lyapunov_w.o._sol:g_zero}. Using \(g=0\),~\eqref{eq:EG:Lyapunov_with_solution} in \Cref{prop:EG:primal_descent} gives
        \begin{equation}\label{eq:EG:Lyapunov_with_solution:g_zero_and_relaxed}
            \norm{z^{i+1}-z^{\star}}^{2} \leq \norm{z^{i}-z^{\star}}^{2} 
            - \gamma^{2}\p{1-\gamma^{2} L_{F}^{2}}\norm{F\p{z^{i}}}^{2}.        
        \end{equation}
        for each \(i\in\naturals\). Inductively summing~\eqref{eq:EG:Lyapunov_with_solution:g_zero_and_relaxed} from \(i=0\) to \(i=k\), rearranging, and dividing by \(\gamma^{2}\p{1-\gamma^{2} L_{F}^{2}}\) gives that
        {\begin{allowdisplaybreaks}
        \begin{align*}
            \sum_{i=0}^{k} \norm{F\p{z^{i}}}^{2} 
            &\leq \frac{\sum_{i=0}^{k}\p{\norm{z^{i}-z^{\star}}^{2} - \norm{z^{i+1}-z^{\star}}^{2}}}{\gamma^{2}\p{1-\gamma^{2} L_{F}^{2}}} \\
            &\leq \frac{\norm{z^{0}-z^{\star}}^{2} }{\gamma^{2}\p{1-\gamma^{2} L_{F}^{2}}} 
        \end{align*}
        \end{allowdisplaybreaks}}%
        for each \(k\in\naturals\). Now \eqref{eq:EG:g_zero:little-o} and \eqref{eq:EG:g_zero:last_iterate_rate} follow from the monotonicity of \(\p{\norm{F\p{z^{i}}}}_{i\in\naturals}\), i.e., \eqref{eq:EG:new_Lyapunov_w.o._sol:g_zero}. 
    \end{proof}
\end{corollary}

==> extragradient/TeX/Text/Results/primal_Vk_inequality.tex <==
%!TEX root = ../../../main.tex
\begin{theorem}\label{thm:EG:primal_descent_for_V}
    Suppose that \Cref{ass:main} holds, the sequence \(\p{\p{z^{k},\bar{z}^{k}}}_{k\in\naturals}\) is generated by~\eqref{alg:EG} with initial point \(z^0\in \calH\) and step-size parameter \(\gamma\in(0,1/L_{F}]\), and the sequence \(\p{\mathcal{V}_{k}}_{k\in\naturals}\) is given by \(\V_k =\mathcal{V}(z^k, \bar z^k, z^{k+1})\) for each \(k\in \naturals\) and the Lyapunov function \(\V\) defined in~\eqref{eq:V}. Then, for any \(k\in\naturals\) and \(z^{\star}\in\zer\p{F + \partial g}\) it holds that
    \begin{equation}\label{eq:EG:primal_descent_for_V}
        \norm{z^{k+1}-z^{\star}}^{2} \leq \norm{z^{k}-z^{\star}}^{2} 
        - \alpha\p{\gamma, L_F} \V_k,
    \end{equation}
    where
    \begin{align}\label{eq:EG:primal_descent_for_V:alpha}
        \alpha\p{\gamma, L_F} = \tfrac{\gamma^{2}}{2}\p{\sqrt{5-4\gamma^2 L_{F}^2 } - 1} \geq 0.
    \end{align}
    \begin{proof}
         Note that~\eqref{eq:subgrad:char} and \(-F\p{z^{\star}} \in \partial g\p{z^{\star}}\) can equivalently be characterized by
        \begin{subequations}
            \begin{align}\label{eq:primal_descent_for_V:subdiff:1}
                0&\leq g\p{z} -  g\p{\bar{z}^{k}} - \inner{ \gamma^{-1} \p{ z^{k} - \bar{z}^{k} } - F\p{z^{k}}}{z - \bar{z}^{k} }, \\\label{eq:primal_descent_for_V:subdiff:2}
                0&\leq  g(z) - g\p{z^{k+1}} - \inner{ \gamma^{-1} \p{ z^{k} - z^{k+1} } - F\p{\bar{z}^{k}}}{z - z^{k+1} },\\\label{eq:primal_descent_for_V:subdiff:3}
                0&\leq g\p{z} - g(z^{\star}) - \inner{ - F\p{z^{\star}}}{z - z^{\star} }
            \end{align}
        \end{subequations}
        for each \(z\in\calH\). Picking \(z = z^{k+1}\) in~\eqref{eq:primal_descent_for_V:subdiff:1}, \(z = z^{\star}\) in~\eqref{eq:primal_descent_for_V:subdiff:2}, \(z = \bar{z}^{k}\) in~\eqref{eq:primal_descent_for_V:subdiff:3}, summing the resulting inequalities, and multiplying by \(2\gamma\) gives  
        {\begin{allowdisplaybreaks}
        \begin{align}
            0 &\leq 
            \begin{aligned}[t] 
                & - 2\inner{ z^{k} - \bar{z}^{k}}{z^{k+1} - \bar{z}^{k} } + 2\gamma\inner{  F\p{z^{k}}}{z^{k+1} - \bar{z}^{k} } \\
                & - 2\inner{ z^{k} - z^{k+1}}{z^{\star} - z^{k+1} }  +  2\gamma\inner{ F\p{\bar{z}^{k}}}{z^{\star} - z^{k+1} } \\ 
                & - 2\gamma\inner{F\p{\bar{z}^{k}} - F\p{z^{\star}}}{\bar{z}^{k} - z^{\star} } + 2\gamma\inner{F\p{\bar{z}^{k}}}{\bar{z}^{k} - z^{\star} } 
            \end{aligned}\notag\\
            &\leq 
            \begin{aligned}[t] 
                & \norm{z^{k} -z^{k+1}}^{2} - \norm{z^{k} - \bar{z}^{k}}^{2} - \norm{z^{k+1} - \bar{z}^{k}}^{2} + 2\gamma\inner{  F\p{z^{k}}}{z^{k+1} - \bar{z}^{k} } \\
                & + \norm{z^{k} - z^{\star}}^{2} - \norm{z^{k} - z^{k+1}}^{2} - \norm{z^{\star} - z^{k+1}}^{2}  +  2\gamma\inner{ F\p{\bar{z}^{k}}}{z^{\star} - z^{k+1} } \\ 
                &+ 2\gamma\inner{F\p{\bar{z}^{k}}}{\bar{z}^{k} - z^{\star} } 
            \end{aligned}\notag\\
            &= 
            \begin{aligned}[t] 
                & \norm{z^{k} - z^{\star}}^{2} - \norm{z^{\star} - z^{k+1}}^{2} - \norm{z^{k} - \bar{z}^{k}}^{2} - \norm{z^{k+1} - \bar{z}^{k}}^{2} \\ 
                &- 2\gamma\inner{  F\p{z^{k}} - F\p{\bar{z}^{k}}}{ \bar{z}^{k} - z^{k+1} },
            \end{aligned} \label{eq:V:primal_ineq:sub_ineq_1}
        \end{align}
        \end{allowdisplaybreaks}}%
        where the identity \(-2\inner{x}{y} = \norm{x-y}^2 - \norm{x}^2 - \norm{y}^2\) for each \(x,y\in \calH\) and monotonicity of \(F\) is used in the second inequality. Picking \(z = z^{k+1}\) in~\eqref{eq:primal_descent_for_V:subdiff:1}, \(z = \bar{z}^{k}\) in~\eqref{eq:primal_descent_for_V:subdiff:2},  and summing the resulting inequalities gives
        {\begin{allowdisplaybreaks}
        \begin{align}
            0 &\leq 
            \begin{aligned}[t]
                & g\p{z^{k+1}} - g\p{\bar{z}^{k}} - \inner{ \gamma^{-1} \p{ z^{k} - \bar{z}^{k} } - F\p{z^{k}}}{z^{k+1} - \bar{z}^{k} } \\
                & + g\p{\bar{z}^{k}} - g\p{z^{k+1}} - \inner{\gamma^{-1} \p{ z^{k} - z^{k+1} } - F\p{\bar{z}^{k}}}{\bar{z}^{k}-z^{k+1}}
            \end{aligned} \notag \\
            &=  - \inner{ F\p{z^{k}} - F\p{\bar{z}^{k}}  }{ \bar{z}^{k} - z^{k+1} }  -  \gamma^{-1}\norm{ \bar{z}^{k} - z^{k+1}  }^{2}. \label{eq:V:primal_ineq:sub_ineq_2}
        \end{align}
        \end{allowdisplaybreaks}}%
        For notational simplicity, we let \(\alpha = \alpha\p{\gamma, L_{F}}\) for \(\alpha\p{\gamma, L_{F}}\) as in~\eqref{eq:EG:primal_descent_for_V:alpha}, where simple algebra shows that \(\alpha \geq 0\) if and only if \(\gamma L_{F} \leq 1\). Multiplying~\eqref{eq:V:primal_ineq:sub_ineq_2} with \(2 \alpha\gamma^{-1}\), and adding the result to~\eqref{eq:V:primal_ineq:sub_ineq_1} gives 
        {\begin{allowdisplaybreaks}
        \begin{align*}
            0 &\leq 
            \begin{aligned}[t] 
                &\norm{z^{k} - z^{\star} }^{2} - \norm{z^{k+1} - z^{\star}}^{2} - \norm{z^{k} - \bar{z}^{k}}^{2} - (1+2\alpha\gamma^{-2}) \norm{z^{k+1} - \bar{z}^{k}}^{2} \\
                &  - 2\gamma(1+\alpha\gamma^{-2}) \inner{  F\p{z^{k}} - F\p{\bar{z}^{k}}}{\bar{z}^{k} - z^{k+1} } 
                \end{aligned} \\
            &= \norm{z^{k} - z^{\star}}^{2} - \norm{z^{k+1} - z^{\star}}^{2}  -  \alpha\V_k + A_k,
        \end{align*}
        \end{allowdisplaybreaks}}%
        where
        \begin{align}
            A_k 
            ={}&
             - \norm{z^{k} - \bar{z}^{k}}^{2}  - \p{1+ 2\alpha\gamma^{-2}} \norm{z^{k+1} - \bar{z}^{k}}^{2} - 2\gamma\p{1+ \alpha\gamma^{-2}} \inner{  F\p{z^{k}} - F\p{\bar{z}^{k}}}{\bar{z}^{k} - z^{k+1} } 
             \nonumber\\  
            &{} + \alpha\V_k 
            \nonumber\\
            ={}& - \norm{z^{k} - \bar{z}^{k}}^{2}  - \p{1+ \alpha\gamma^{-2}} \norm{z^{k+1} - \bar{z}^{k}}^{2} 
                +
                 \alpha\gamma^{-2}\norm{z^{k} - z^{k+1}}^{2} 
            \nonumber\\  
            &{}
            +
            2\gamma
            \smash{\underbracket{\inner{%
            \alpha\gamma^{-2}\p{z^{k} - z^{k+1}} 
            - 
            (1+\alpha\gamma^{-2})\p{\bar z^k - z^{k+1}}
            }{F\p{z^{k}} - F\p{\bar{z}^{k}}}}_{= B_k}}, 
            \label{eq:Ak:thm:tight}
        \end{align}
        where we substituted \(\V_k\).
        
        To complete the proof, it is enough to show that \(A_k \leq 0\). The last inner product in~\eqref{eq:Ak:thm:tight} can be upper bounded using Young's inequality as
        \begin{align} \notag
            B_k \leq {}&
            \tfrac{\gamma}{2}
            \norm{F\p{z^{k}} - F\p{\bar{z}^{k}}}^2 
            + \tfrac{1}{2\gamma}
            \norm{\alpha\gamma^{-2}\p{z^{k} - z^{k+1}} - (1+\alpha\gamma^{-2})\p{\bar z^k - z^{k+1}}}^2 \\\notag
            \leq{}&
            \tfrac{\gamma L_F^2}{2}
            \norm{z^{k} - \bar{z}^{k}}^2 \\ \label{eq:Bk:thm:tight}
            &{} + 
            \tfrac{1}{2\gamma} 
            \p{            
            \p{1+\alpha\gamma^{-2}}\norm{\bar{z}^k - z^{k+1}}^2 
            + \alpha\gamma^{-2}\p{1+\alpha\gamma^{-2}} \norm{z^{k} - \bar{z}^k}^2
            - \alpha\gamma^{-2}\norm{z^{k} - z^{k+1}}^2  
            },
        \end{align}
        where Lipschitz continuity of \(F\) and the identity 
        \(\norm{\beta x - \p{1+\beta}y}^2 = \p{1+\beta}\norm{y}^2 + \beta(1+\beta)\norm{x-y}^2 - \beta\norm{x}^2\)
        for each \(x,y\in\calH\) and each \(\beta\in\reals\) {\cite[Corollary 2.15]{bauschke2017convexanalysismonotone}} are used in the second inequality. Substituting~\eqref{eq:Bk:thm:tight} in~\eqref{eq:Ak:thm:tight} gives 
        \begin{equation}
            A_k \leq{} - \p{1- \gamma^2 L_F^2 - \alpha\gamma^{-2}\p{1+\alpha\gamma^{-2}}} \norm{z^{k} - \bar{z}^{k}}^{2}  = 0,
       \end{equation}
       where the last equality follows from simple algebra after substituting \(\alpha = \alpha\p{\gamma, L_F}\) as in~\eqref{eq:EG:primal_descent_for_V:alpha}. 
    \end{proof}
\end{theorem}

==> extragradient/TeX/Text/abstract.tex <==
\noindent
\new{We develop a Lyapunov-based analysis of Korpelevich’s extragradient method and show that it achieves an \(o(1/k)\) last-iterate convergence rate of the constructed Lyapunov function. This Lyapunov function simultaneously upper bounds several standard measures of optimality, which allows our analysis to sharpen existing last-iterate convergence guarantees for these measures. Moreover, the same analysis enables the design of a class of flexible extensions of the extragradient method in which extragradient steps are adaptively blended with user-specified directions via a Lyapunov-guided line-search procedure. These extensions retain global convergence under practical assumptions and can attain superlinear rates when the directions are chosen appropriately. Numerical experiments confirm the simplicity and efficiency of the proposed framework.}

==> extragradient/TeX/Text/acknowledgments.tex <==
M. Upadhyaya and P. Giselsson acknowledge support from the ELLIIT Strategic Research Area and the Wallenberg AI, Autonomous Systems, and Software Program (WASP), funded by the Knut and Alice Wallenberg Foundation. Additionally, P. Giselsson acknowledges support from the Swedish Research Council. P. Latafat is a member of the Gruppo Nazionale per l'Analisi Matematica, la Probabilit\`a e le loro Applicazioni (GNAMPA - National Group for Mathematical Analysis, Probability and their Applications) of the Istituto Nazionale di Alta Matematica (INdAM - National Institute of Higher Mathematics). We thank Yurong Chen for highlighting some details in~\Cref{sec:equilibrium}. \new{We also thank Max Nilsson, Sebastian Banert, and the anonymous reviewers for providing valuable comments and suggestions for a previous version of this work.}

==> extragradient/TeX/Text/algs.tex <==
%!TEX root = ../../main.tex
\section{Algorithms for monotone inclusions}\label{sec:algs}
In light of the descent property established in \Cref{thm:EG:new_Lyapunov_w.o._sol}, we propose line-search extensions of the extragradient method that combine the nominal steps of~\eqref{alg:EG} with user-specified directions. This section focuses on identifying appropriate conditions to guarantee global convergence, with detailed proofs deferred to \Cref{sec:global}. We deliberately leave the choice of directions open at this stage and postpone the superlinear convergence analysis to \Cref{sec:superlinear}. This abstraction offers flexibility in choosing methods---such as (inexact) (quasi-)Newton approaches, Anderson acceleration, or other suitable algorithms---for computing the directions.

In the first subsection, we consider the classical extragradient setting where \(g = 0\) and introduce a line search based on \(\|F(z^k)\|^2\) and its descent inequality in~\eqref{eq:EG:new_Lyapunov_w.o._sol:g_zero}. We then extend our approach in \Cref{sec:ProxFLEX} to the more general setting of~\eqref{eq:the_inclusion_problem}. Separating the analysis in this way reflects the stronger convergence results available when \(g = 0\), as well as the fact that, in this case, the line search is more computationally efficient.

\subsection{Fast line-search extragradient}\label{sec:FLEX}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{TeX/Text/flex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proximal fast line-search extragradient}
\label{sec:ProxFLEX}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{TeX/Text/proxflex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> extragradient/TeX/Text/background.tex <==
\section{Background on Korpelevich's extragradient method}\label{app:background}
In the original paper~\cite{korpelevich1976extragradientmethodfinding}, the extragradient method~\eqref{alg:EG} was analyzed under the assumption that \(g\) is the indicator function of a nonempty, closed, and convex set, making the proximal operator reduce to the projection onto that set. However, as noted in~\cite{monteiro2011complexityvariantstsengs}, the extragradient method extends to the more general setting~\eqref{eq:the_inclusion_problem}. The remainder of this section presents results in this more general context, with proofs included for completeness.

\begin{definition}%[\normalfont{Fixed point}]
    Suppose that \Cref{ass:main} holds and let \(\gamma\in\reals_{++}\). A point \(z\in\calH\) is said to be a fixed point of the extragradient method~\eqref{alg:EG} if
    \begin{subequations}\label{eq:EG:fixed_point}
        \begin{align}\label{eq:EG:fixed_point:1}
            \bar{z} &= \prox_{\gamma g}\p{z - \gamma F\p{z}}, \\ \label{eq:EG:fixed_point:2}
            z &=\prox_{\gamma g}\p{z - \gamma F\p{\bar{z} }}.
        \end{align}
    \end{subequations}
\end{definition}

\begin{proposition}%[\normalfont{Fixed-point encoding property}]
\label{prop:EG:fixed_point}
    Suppose that \Cref{ass:main} holds and let \(\gamma\in\reals_{++}\). Then, the following hold:
    \begin{propenumerate}
        \item If \(z\in \zer\p{F + \partial g}\), then \(z\) is a fixed point of the extragradient method, i.e.,~\eqref{eq:EG:fixed_point} holds, and \(z = \bar{z}\). \label{prop:EG:fixed_point:solutions_are_fixed_points}
        \item If \(\gamma \in (0,1/L_{F})\), \(z\) is a fixed point of the extragradient method, and \(\bar{z}\) is defined as in~\eqref{eq:EG:fixed_point:1}, then \(z=\bar{z} \in \zer\p{F + \partial g}\). \label{prop:EG:fixed_point:fixed_points_are_solutions}
    \end{propenumerate}
    \begin{proof}
        The proximal evaluations in~\eqref{eq:EG:fixed_point:1} and~\eqref{eq:EG:fixed_point:2} can equivalently be written via their subgradient characterization as
        \begin{subequations}\label{eq:EG:fixed_point:implicit_prox}
            \begin{align}\label{eq:EG:fixed_point:implicit_prox:1}
                \gamma^{-1}\p{z  - \bar{z}} -  F\p{z} &\in \partial g\p{\bar{z}}, \\\label{eq:EG:fixed_point:implicit_prox:2}
                -F\p{\bar{z}} &\in \partial g\p{z},
            \end{align}
        \end{subequations}
        respectively.
        \begin{itemize}
            \item[\ref{prop:EG:fixed_point:solutions_are_fixed_points}:] Note that \(z\in \zer\p{F + \partial g}\) and~\eqref{eq:EG:fixed_point:1} is equivalent to \(-F\p{z}\in \partial g \p{z}\) and~\eqref{eq:EG:fixed_point:implicit_prox:1}, respectively. Using monotonicity of \(\partial g\)~\cite[Theorem 20.48]{bauschke2017convexanalysismonotone},  we get that 
            \begin{align*}
                0   &\leq \inner{\gamma^{-1}\p{z  - \bar{z}} -  F\p{z} + F\p{z}}{\bar{z} - z } \\
                    &= - \gamma^{-1} \norm{z-\bar{z}}^{2} \leq 0,
            \end{align*}
            since \(\gamma\in\reals_{++}\). We conclude that \(z = \bar{z}\) and that~\eqref{eq:EG:fixed_point} holds.
            \item[\ref{prop:EG:fixed_point:fixed_points_are_solutions}:] By using monotonicity of \(\partial g\) at the points \(\bar{z}\) and  \(z\), and the corresponding subgradients in~\eqref{eq:EG:fixed_point:implicit_prox}, we get that 
            {\begin{allowdisplaybreaks}
            \begin{align}
                0   &\leq \inner{\gamma^{-1}\p{z  - \bar{z}} -  F\p{z} + F\p{\bar{z}}}{\bar{z} - z } \notag\\
                    &= - \gamma^{-1} \norm{z-\bar{z}}^{2} + \inner{F\p{\bar{z}} - F\p{z}}{\bar{z} - z} \notag\\
                    &\leq - \gamma^{-1} \norm{z-\bar{z}}^{2} + \norm{F\p{\bar{z}} - F\p{z}}\norm{\bar{z} - z} \notag\\
                    &\leq \p{L_{F}- \gamma^{-1}} \norm{z-\bar{z}}^{2}, \label{eq:EG:fixed_point:ineq}
            \end{align}
            \end{allowdisplaybreaks}}%
            where the Cauchy–Schwarz inequality is used in the second inequality, and Lipschitz continuity of \(F\) in the third inequality. Since \(L_{F}- \gamma^{-1}<0\), we conclude from~\eqref{eq:EG:fixed_point:ineq} that \(z = \bar{z}\). That \(z=\bar{z} \in \zer\p{F + \partial g}\) now follows from~\eqref{eq:EG:fixed_point:implicit_prox:1} or~\eqref{eq:EG:fixed_point:implicit_prox:2}. \qedhere
        \end{itemize}
    \end{proof}
\end{proposition}

\begin{proposition}%[\normalfont{A Lyapunov inequality and sequence convergence}]
    \label{prop:EG:primal_descent}
    Suppose that \Cref{ass:main} holds, the sequence \(\p{\p{z^{k},\bar{z}^{k}}}_{k\in\naturals}\) is generated by~\eqref{alg:EG} with initial point \(z^0\in \calH\) and step-size parameter \(\gamma\in\reals_{++}    \), and \(z^{\star}\in\zer\p{F + \partial g}\). Then
    \begin{equation}\label{eq:EG:Lyapunov_with_solution}
        \norm{z^{k+1}-z^{\star}}^{2} \leq \norm{z^{k}-z^{\star}}^{2} 
        - \p{1-\gamma^{2} L_{F}^{2}}\norm{\bar{z}^{k}-z^{k}}^{2} 
    \end{equation}
    for each \(k\in\naturals\). Moreover, if \(\gamma\in\p{0,1/L_{F}}\), then \(\p{z^{k}}_{k\in\naturals}\) converges weakly to a point in \(\zer\p{F + \partial g}\).
    \begin{proof}
        Note that the first and second proximal evaluations in~\eqref{alg:EG} are equivalent to 
        \begin{align}\label{alg:EG:1:rewritten}
            0\leq g\p{z} - g\p{\bar{z}^{k}} - \inner{\gamma^{-1}\p{z^{k} - \bar{z}^{k}} - F\p{z^{k}}}{ z - \bar{z}^{k} } \text{ for each } z \in \calH,
        \end{align}
        and
        \begin{align}\label{alg:EG:2:rewritten}
            0\leq g\p{z} - g\p{z^{k+1}} - \inner{\gamma^{-1}\p{z^{k} - z^{k+1}} - F\p{\bar{z}^{k}}}{z - z^{k+1} } \text{ for each } z \in \calH,
        \end{align}
        respectively, and the assumption \(z^{\star}\in\zer\p{F + \partial g}\) is equivalent to
        \begin{align}\label{ass:Korpelevic:main:solution_exists:rewritten}
            0 \leq g\p{z} - g(z^{\star}) - \inner{ -F\p{z^{\star}}}{z - z^{\star} } \text{ for each } z \in \calH.
        \end{align}
        Picking \(z = z^{k+1}\) in~\eqref{alg:EG:1:rewritten}, \(z = z^{\star}\) in~\eqref{alg:EG:2:rewritten}, \(z = \bar{z}^{k}\) in~\eqref{ass:Korpelevic:main:solution_exists:rewritten}, summing the resulting inequalities, and multiplying by \(2\gamma\) gives 
        {\begin{allowdisplaybreaks}
        \begin{align*}
            0 &\leq
            \begin{aligned}[t]
                & 2\gamma g\p{z^{k+1}} - 2\gamma g\p{\bar{z}^{k}} - 2\inner{ z^{k} - \bar{z}^{k} - \gamma F\p{z^{k}}}{z^{k+1} - \bar{z}^{k} } \\
                & + 2\gamma g(z^{\star}) - 2\gamma g\p{z^{k+1}} - 2\inner{ z^{k} - z^{k+1} - \gamma F\p{\bar{z}^{k}}}{z^{\star} - z^{k+1} } \\
                & + 2\gamma g\p{\bar{z}^{k}} - 2\gamma g(z^{\star}) - 2\inner{ -\gamma F\p{z^{\star}}}{\bar{z}^{k} - z^{\star} } 
            \end{aligned}\\
            &= A_k + B_k,
        \end{align*} 
        \end{allowdisplaybreaks}}%
        where
        {\begin{allowdisplaybreaks}
        \begin{align*}
            A_k {}={}& - 2\inner{ z^{k} - \bar{z}^{k}}{z^{k+1} - \bar{z}^{k}}  - 2\inner{ z^{k} - z^{k+1}}{z^{\star} - z^{k+1} } \\
            {}={}& \norm{z^{k} -z^{k+1}}^{2} - \norm{z^{k} - \bar{z}^{k}}^{2} - \norm{z^{k+1} - \bar{z}^{k}}^{2} + \norm{z^{k} - z^{\star}}^{2} - \norm{z^{k} - z^{k+1}}^{2} \\
            {}{}&- \norm{z^{\star} - z^{k+1}}^{2} \\
            {}={}&  \norm{z^{k} - z^{\star}}^{2} - \norm{z^{\star} - z^{k+1}}^{2} - \norm{z^{k} - \bar{z}^{k}}^{2} - \norm{z^{k+1} - \bar{z}^{k}}^{2},
        \end{align*} 
        \end{allowdisplaybreaks}}%
        and 
        {\begin{allowdisplaybreaks}
        \begin{align*}
            B_k &= 2\gamma\inner{  F\p{z^{k}}}{z^{k+1} - \bar{z}^{k} } +  2\gamma\inner{ F\p{\bar{z}^{k}}}{z^{\star} - z^{k+1} }  - 2\gamma\inner{ - F\p{z^{\star}}}{\bar{z}^{k} - z^{\star} } \\
            &= 
            \begin{aligned}[t]
                & 2\gamma\inner{  F\p{z^{k}}}{z^{k+1} - \bar{z}^{k} } +  2\gamma\inner{ F\p{\bar{z}^{k}}}{z^{\star} - z^{k+1} } + 2\gamma\inner{F\p{\bar{z}^{k}}}{\bar{z}^{k} - z^{\star}} \\
                & - 2\gamma\inner{F\p{\bar{z}^{k}} - F\p{z^{\star}}}{\bar{z}^{k} - z^{\star} }
            \end{aligned}\\
            & \leq 2\gamma\inner{  F\p{z^{k}}}{z^{k+1} - \bar{z}^{k} } +  2\gamma\inner{ F\p{\bar{z}^{k}}}{z^{\star} - z^{k+1} } + 2\gamma\inner{F\p{\bar{z}^{k}}}{\bar{z}^{k} - z^{\star}} \\
            & = 2\gamma\inner{  F\p{z^{k}} - F\p{\bar{z}^{k}}}{z^{k+1} - \bar{z}^{k} } \\
            &\leq \gamma^{2}\norm{F\p{z^{k}} - F\p{\bar{z}^{k}}}^{2} + \norm{z^{k+1} - \bar{z}^{k}}^{2} \\
            &\leq \gamma^2L_{F}^{2}\norm{z^{k} - \bar{z}^{k}}^{2}  + \norm{z^{k+1} - \bar{z}^{k}}^{2},
        \end{align*} 
        \end{allowdisplaybreaks}}%
        where monotonicity of \(F\) is used in the first inequality, Young's inequality is used in the second inequality, and Lipschitz continuity of \(F\) in the third inequality. We conclude that 
        \begin{align*}
            0   &\leq A_k + B_k \leq  \norm{z^{k} - z^{\star}}^{2} - \norm{z^{\star} - z^{k+1}}^{2} - \p{1 - \gamma^{2}L_{F}^{2} } \norm{z^{k} - \bar{z}^{k}}^{2},
        \end{align*}
        which proves~\eqref{eq:EG:Lyapunov_with_solution}.
    
        Next, note that~\eqref{eq:EG:Lyapunov_with_solution} gives that \(\p{\norm{z^{k} - z^{\star}}}_{k\in\naturals}\) converges. Thus, \(\p{z^{k}}_{k\in\naturals}\) is bounded and there exists a subsequence \(\p{z^{k}}_{k\in K}\rightharpoonup z^{\infty}\) for some \(z^{\infty} \in \calH\)~\cite[Lemma 2.45]{bauschke2017convexanalysismonotone}. Moreover,~\eqref{eq:EG:Lyapunov_with_solution} and the requirement \(\gamma\in\p{0, 1/L_{F}}\) give that \(\p{\norm{\bar{z}^{k}-z^{k}}^{2}}_{k\in\naturals}\) is summable, and therefore, \(\p{\bar{z}^{k}}_{k\in K}\rightharpoonup z^{\infty}\). The first proximal evaluation in~\eqref{alg:EG} can equivalently be written as 
        \begin{align}\label{alg:EG:1:rewritten:seq}
            \gamma^{-1}\p{z^{k}- \bar{z}^{k} } - F\p{z^{k}} + F\p{\bar{z}^{k}} \in \p{F + \partial g}\p{\bar{z}^{k}}.
        \end{align}
        The left-hand side of~\eqref{alg:EG:1:rewritten:seq} converges strongly to zero since \(F\) is continuous and \((\norm{z^{k}-\bar{z}^{k}})_{k\in\naturals}\) converges to zero. Moreover, the operator \(F + \partial g\) is maximally monotone, since \(F\) is maximally monotone (by continuity and monotonicity~\cite[Corollary 20.28]{bauschke2017convexanalysismonotone}), \(\partial g\) is maximally monotone~\cite[Theorem 20.48]{bauschke2017convexanalysismonotone}, and \(F\) has full domain~\cite[Corollary 25.5]{bauschke2017convexanalysismonotone}. Thus,~\cite[Proposition 20.38]{bauschke2017convexanalysismonotone} gives that \(z^{\infty} \in \zer\p{F + \partial g}\), and by~\cite[Lemma 2.47]{bauschke2017convexanalysismonotone} we conclude that \(\p{z^{k}}_{k\in\naturals}\) converges weakly to a point in \(\zer\p{F + \partial g}\), as claimed. 
    \end{proof}
\end{proposition}

\new{
\begin{remark}
    Similar to \Cref{rmk:cyclically_monotone}, the results in this section remain valid when \(\partial g\) in \eqref{eq:the_inclusion_problem} is replaced with a maximally monotone and 3-cyclically monotone operator \(T:\calH\to\calH\) and the proximal operators \(\prox_{\gamma g}\) in \eqref{alg:EG} with the resolvent \(\p{\Id + \gamma T}^{-1}\).
\end{remark}
}

==> extragradient/TeX/Text/bilinear.tex <==
Consider the bilinear zero-sum game with simplex constraints given by
\begin{align}\label{eq:bilinear}
    \minimize_{x \in \Delta^n}\; \maximize_{y \in \Delta^n}\; x^{\top} A y
\end{align}
where \(A\in\reals^{n\times n}\) is the payoff matrix and \(\Delta^{n}=\set{w\in\reals_{+}^n\mid w^{\top}\mathbf{1} = 1 }\) is the probability simplex in \(\reals^n\), which is equivalent to finding a saddle point \(\p{x^{\star},y^{\star}}\in\Delta^{n}\times\Delta^{n}\) (which is guaranteed to exist), i.e.,
\begin{align*}
     \p{x^{\star}}^{\top} A y \leq \p{x^{\star}}^{\top} A y^{\star} \leq x^{\top} A y^{\star} 
\end{align*}
for each \(\p{x,y} \in \Delta^{n}\times\Delta^{n}\). This, in turn, is equivalent to solving~\eqref{eq:the_inclusion_problem} by letting \(\calH=\reals^{2n}\) with the inner product set to the dot product, \(g=\delta_{\Delta^{n}\times\Delta^{n}}\), and \(F: \reals^{2n}\to\reals^{2n}\) as the monotone and \(L_F\)-Lipschitz continuous operator given by
\begin{align*}
    F(z) = 
    \begin{bmatrix}
        Ay \\
        - A^{\top}x
    \end{bmatrix}
\end{align*}
for each \(z = (x,y)\in \reals^{n} \times \reals^{n}\), where
\begin{align*}
    L_{F} = 
    \left\lVert 
    \begin{bmatrix}
        0 &  A \\
        - A^{\top} & 0
    \end{bmatrix}
    \right\rVert.
\end{align*}

We generate \(A = S - S^{\top}\) for a random matrix \(S\in\reals^{n\times n}\) such that \([S]_{i,j} \sim \mathcal{N}(0, 1)\) for each \(i,j \in \llbracket 1, n \rrbracket\), resulting in a skew-symmetric matrix \(A\). The results of the numerical experiments are presented in \Cref{fig:bmg}. We see that using \texttt{AA-II} directions in~\ProxFLEX{} gives good performance.

\input{plots/bilinear.tex}

==> extragradient/TeX/Text/comparison.tex <==
%!TEX root = ../../main_arxiv.tex
\new{%
\section{Comparison to standard optimality measures}\label{sec:comparison}
This section presents some standard optimality measures for \eqref{eq:the_inclusion_problem} and compares them to \(\V_k = \V\p{z^{k},\bar{z}^{k},z^{k+1}}\) for the Lyapunov function \(\V\) defined in~\eqref{eq:V} and iterates \(\seq{\p{z^{k},\bar{z}^{k}}}\) generated by the extragradient method~\eqref{alg:EG}. It also includes a comparison to recent last-iterate convergence results for the extragradient method.

\begin{definition}\label{def:performance_measures}
    Suppose that \Cref{ass:main} holds.
    \begin{enumerate}[label=(\roman*)]
        \item The \emph{natural residual} is defined as
        \begin{align*}
            \norm{z - \prox_{g}(z - F(z))}
        \end{align*}
        for each \(z\in \calH\).
        \item The \emph{tangent residual} is defined as
        \begin{align*}
            \inf_{\xi \in \partial g(z)} \norm{F(z)+ \xi}
        \end{align*}
        for each \(z\in \calH\).
        \item Suppose that \(z^{0}\in\calH\), \(z^{\star} \in \mathrm{zer}(F + \partial g)\) and \(\delta = \|z^0 - z^{\star}\|>0\). Then the restricted gap function \(\textup{\texttt{Gap}}:\calH\to\reals\cup\set{+\infty}\) is defined as
        \begin{align}\label{eq:gap_functions}
            \textup{\texttt{Gap}}(z) = \sup_{w \in \mathrm{dom}\,\partial g \cap \mathbb{B}(z^{\star};\delta)} \left(\inner{F(w)}{z-w} + g(z) - g(w)\right)
        \end{align}
        for each \(z\in \calH\), where \(\mathbb{B}(z^{\star};\delta) = \{ z \in\mathcal{H} : \|z - z^{\star}\| \leq \delta \} \).
    \end{enumerate}
\end{definition}

\begin{remark}
    In this remark, we establish that the measures in \Cref{def:performance_measures} are indeed optimality measures for \eqref{eq:the_inclusion_problem}.
    \begin{enumerate}[label=(\roman*)]
        \item The natural residual is nonnegative and zero if and only if \(z\in\zer\p{F + \partial g}\), since 
        \begin{align*}
            \norm{z - \prox_{g}(z - F(z))} = 0 \; \iff \; z = \prox_{g}(z - F(z)) \; \iff \; -F(z) \in \partial g(z),
        \end{align*}
        where the last equivalence follows from the subgradient characterization of the proximal operator. 
        \item The tangent residual is nonnegative and zero if and only if \(z\in\zer\p{F + \partial g}\), since the tangent residual upper bounds the natural residual by \Cref{prop:natres_upper_tanres}.
        \item  It is well-known that (e.g., see \cite[Lemma 1]{nesterov2006dualextrapolationits} and \cite[Lemma 3]{malitsky2020goldenratioalgorithms})
        \begin{itemize}
            \item \(\textup{\texttt{Gap}}(z) \geq 0\) for each \(z\in\mathcal{H}\), 
            \item if \(z\in\mathrm{zer}(F + \partial g)\cap \mathbb{B}(z^{\star};\delta)\), then \(\textup{\texttt{Gap}}(z) = 0\), and
            \item if $z \in \mathrm{dom}\,\partial g \cap \mathbb{B}(z^{\star};\tilde{\delta})$ for some \(\tilde{\delta} \in (0,\delta)\), then \(\textup{\texttt{Gap}}(z) = 0\) implies that \(z\in\mathrm{zer}(F + \partial g)\).
        \end{itemize}
    \end{enumerate}
\end{remark}

Note that the second proximal step in~\eqref{alg:EG} can equivalently be written via its subgradient characterization as
\begin{equation}\label{eq:comparison:subgradient}
     \underbracket{\gamma^{-1}\p{z^{k}-z^{k+1}}-F(\bar{z}^{k})}_{=\xi^{k+1}} \in \partial g(z^{k+1})
\end{equation}
for each \(k\in\naturals\). This notation allows us to introduce another standard optimality measure, namely \(\p{\norm{F(z^{k}) + \xi^{k}}}_{k\in\mathbb{N}}\). It is clear that this measure upper bounds the tangent residual, i.e.,
\begin{align}\label{eq:tanres_upper_tseng_res}
    \inf_{\xi \in \partial g(z^{k})} \|F(z^{k})+ \xi\| \leq \norm{F(z^{k}) + \xi^{k}}
\end{align}
for each \(k\in\mathbb{N}\).

Next, we present a result that, when combined with \eqref{eq:tanres_upper_tseng_res}, shows that \(\V_k\) upper bounds all the squared optimality measures considered above, except the squared restricted gap function, which is upper bounded up to a positive constant. 

\begin{proposition}\label{prop:comp:bounds}
    Suppose that \Cref{ass:main} holds, the sequence \(\p{\p{z^{k},\bar{z}^{k}}}_{k\in\naturals}\) is generated by~\eqref{alg:EG} with initial point \(z^0\in \calH\) and step-size parameter \(\gamma\in(0,1/L_{F})\), the sequence \(\p{\mathcal{V}_{k}}_{k\in\naturals}\) is given by \(\V_k =\mathcal{V}(z^k, \bar z^k, z^{k+1})\) for each \(k\in \naturals\) and the Lyapunov function \(\V\) defined in~\eqref{eq:V}, and the sequence \(\p{\xi^{k}}_{k\in\mathbb{N}}\) is given by \eqref{eq:comparison:subgradient}. Then,
    \begin{propenumerate}
        \item \label{prop:tsengres_upper_V}\(\norm{F(z^{k+1}) + \xi^{k+1}}^2 \leq \V_{k}\) for each \(k \in \naturals\), 
        \item \label{prop:natres_upper_tanres} \(\norm{z - \prox_{g}(z - F(z))} \leq \inf_{\xi \in \partial g(z)} \norm{F(z)+ \xi}\) for each \(z \in \calH\), 
        \item \label{prop:gap_upper_tanres} \(\textup{\texttt{Gap}}(z)\leq\p{\delta + \norm{z-z^{\star}}}\inf_{\xi \in \partial g(z)} \norm{F(z)+ \xi}\) for each \(z \in \calH\), and in particular, \(\textup{\texttt{Gap}}(z^{k})\leq2\delta \inf_{\xi \in \partial g(z^{k})} \norm{F(z^{k})+ \xi}\) for each \(k\in\mathbb{N}\), where \(\textup{\texttt{Gap}}\) is defined in \eqref{eq:gap_functions}.
    \end{propenumerate}
\end{proposition}
\begin{proof}
    The proofs of \Cref{prop:natres_upper_tanres,prop:gap_upper_tanres} are simple generalizations of corresponding results found in \cite{sedlmayer2023fastoptimistic}, which we include for completeness. 
    \begin{itemize}
        \item[\ref{prop:tsengres_upper_V}]
        Note that 
        \begin{align*}
             & \|F(z^{k+1})+ \xi^{k+1}\|^2  \\
             & = \|\tfrac{1}{\gamma}\big(z^{k}-z^{k+1}\big)+F(z^{k+1})-F(\bar{z}^{k})\|^{2}
             \\ 
             & =
             \|F(z^{k+1})-F(\bar{z}^{k})\|^{2}+\tfrac{1}{\gamma^{2}}\|z^{k}-z^{k+1}\|^{2}+\tfrac{2}{\gamma}\langle F(z^{k+1})-F(\bar{z}^{k}),z^{k}-z^{k+1}\rangle
             \\ 
             & \leq
             L_{F}^{2}\|z^{k+1}-\bar{z}^{k}\|^{2}+\tfrac{1}{\gamma^{2}}\|z^{k}-z^{k+1}\|^{2}+\tfrac{2}{\gamma}\langle F(z^{k+1})-F(\bar{z}^{k}),z^{k}-z^{k+1}\rangle
             \\ 
             & \leq
             \tfrac1{\gamma^{2}}\|z^{k+1}-\bar{z}^{k}\|^{2}+\tfrac{1}{\gamma^{2}}\|z^{k}-z^{k+1}\|^{2}+\tfrac{2}{\gamma}\langle F(z^{k})-F(\bar{z}^{k}),z^{k}-z^{k+1}\rangle
             \\ 
             & = \mathcal V_k
        \end{align*} 
        where Lipschitz continuity of \(F\) was used in the first inequality,  and \(\gamma L_{F} \leq 1\) and monotonicity of \(F\) was used in the second inequality.
        \item[\ref{prop:natres_upper_tanres}]
        We claim that the natural residual is upper bounded by the tangent residual, i.e., 
        \begin{align}\label{eq:natural_leq_tangent}
            \|z - \mathrm{prox}_{g}(z - F(z))\| \leq \inf_{\xi \in \partial g(z)} \|F(z)+ \xi\|
        \end{align}
        for each \(z\in\calH\).
        When \(z \notin \mathrm{dom}\,\partial g\), then \eqref{eq:natural_leq_tangent} holds trivially. Thus, suppose that \(z \in \mathrm{dom}\,\partial g\) and let \(\xi \in \partial g (z)\). The latter inclusion holds if and only if \(z = \mathrm{prox}_{g}(z + \xi)\). Therefore, 
        \begin{align*}
            \|z - \mathrm{prox}_{g}(z - F(z))\| 
            = \| \mathrm{prox}_{g}(z + \xi) - \mathrm{prox}_{g}(z - F(z))\| 
            \leq \|F(z) + \xi \|
        \end{align*}
        where the inequality follows from the nonexpansivity of the proximal operator \cite[Proposition 12.28]{bauschke2017convexanalysismonotone}. 
        However, since \(\xi \in \partial g (z)\) is arbitrary, \eqref{eq:natural_leq_tangent} follows. 
        \item[\ref{prop:gap_upper_tanres}]
        We claim that the restricted gap function is upper bounded by the tangent residual up to a positive quantity, i.e., 
        \begin{align}\label{eq:restricted_gap_function_leq_tangent_residual}
            \texttt{Gap}(z) \leq \p{\delta + \norm{z-z^{\star}}} \inf_{\xi \in \partial g(z)} \|F(z)+ \xi\|
        \end{align}
        for each \(z\in\calH\), and therefore,
        \begin{align}\label{eq:restricted_gap_function_leq_tangent_residual:k}
            \textup{\texttt{Gap}}(z^{k}) \leq 2\delta \inf_{\xi \in \partial g(z^{k})} \|F(z^{k})+ \xi\|
        \end{align}
        for each \(k\in \mathbb{N}\), by \Cref{prop:EG:primal_descent}.
        Let us prove \eqref{eq:restricted_gap_function_leq_tangent_residual}. If $z \notin \mathrm{dom}\,\partial g$, then \eqref{eq:restricted_gap_function_leq_tangent_residual} holds trivially. Thus, assume that $z \in \mathrm{dom}\,\partial g$, and let \(\xi \in \partial g(z)\) and \(w\in \mathrm{dom}\,\partial g \cap \mathbb{B}(z^{\star};\delta) \). Then we have that 
        \begin{align}
            &\inner{F(w)}{z-w} + g(z) - g(w) \nonumber\\
            & = \underbracket{\inner{F(w) - F(z)}{z-w}}_{\leq 0} + \inner{F(z)}{z-w} + \underbracket{g(z) - g(w)}_{\leq \inner{\xi}{z - w}} \nonumber\\
            &\leq \inner{F(z)+\xi}{z-z^{\star}} + \inner{F(z)+\xi}{z^{\star}-w} \nonumber\\
            &\leq \norm{F(z)+\xi}\norm{{z-z^{\star}}} + \norm{F(z)+\xi}\underbracket{\norm{z^{\star}-w}}_{\leq \delta} \nonumber\\
            &\leq \p{\delta + \norm{z-z^{\star}}} \|F(z)+ \xi\|
            \label{eq:restricted_gap_function_leq_tangent_residual:helper},
        \end{align}
        % or
        % \begin{align}\label{eq:restricted_gap_function_leq_tangent_residual:helper}
        %     \inner{F(w)}{z-w} + g(z) - g(w) \leq \p{\delta + \norm{z-z^{\star}}} \|F(z)+ \xi\|.
        % \end{align}
        Maximizing over \(w\in \mathrm{dom}\,\partial g \cap \mathbb{B}(z^{\star};\delta) \) and minimizing over \(\xi \in \partial g(z)\) in \eqref{eq:restricted_gap_function_leq_tangent_residual:helper} gives \eqref{eq:restricted_gap_function_leq_tangent_residual}, as claimed. \qedhere
    \end{itemize}
\end{proof}

\begin{corollary}\label{cor:rates_standard_measures}
    Suppose that \Cref{ass:main} and \(\zer\p{F + \partial g}\neq \emptyset\) hold, the sequence \(\p{\p{z^{k},\bar{z}^{k}}}_{k\in\naturals}\) is generated by~\eqref{alg:EG} with initial point \(z^0\in \calH\) and step-size parameter \(\gamma\in(0,1/L_{F})\), and the sequence \(\p{\xi^{k}}_{k\in\mathbb{N}}\) is given by \eqref{eq:comparison:subgradient}. Then,
    \begin{align*}
        \norm{F(z^{k}) + \xi^{k}} & \in o\p{1/\sqrt{k}} \text{ as } k \to \infty,\\
        \inf_{\xi \in \partial g(z^{k})} \|F(z^{k})+ \xi\| & \in o\p{1/\sqrt{k}} \text{ as } k \to \infty, \\
        \norm{z^k - \prox_{g}(z - F(z^k))} & \in o\p{1/\sqrt{k}} \text{ as } k \to \infty, \\
        \textup{\texttt{Gap}}(z^{k}) & \in o\p{1/\sqrt{k}} \text{ as } k \to \infty,
    \end{align*}
    and for any \(k\in\mathbb{N}\) and \(z^{\star}\in\zer\p{F + \partial g}\) it holds that  
    \begin{gather*}
        \norm{z^k - \prox_{g}(z - F(z^k))} 
        \leq 
        \inf_{\xi \in \partial g(z^{k})} \|F(z^{k})+ \xi\| 
        \leq 
        \norm{F(z^{k}) + \xi^{k}} 
        \leq 
        \frac{\norm{z^{0} - z^{\star} } }{ \sqrt{\alpha\p{ \gamma, L_{F}} k} }, \\
        \textup{\texttt{Gap}}(z^{k})
        \leq 
        \frac{2\delta\norm{z^{0} - z^{\star} } }{ \sqrt{\alpha\p{ \gamma, L_{F}} k} },
    \end{gather*}
    where \(\alpha\p{ \gamma, L_{F}}=\tfrac{\gamma^{2}}{2}\p{\sqrt{5-4\gamma^2 L_{F}^2 } - 1}>0\) and \(\textup{\texttt{Gap}}\) is defined in \eqref{eq:gap_functions}.
    \begin{proof}
        Follows immediately from \eqref{eq:tanres_upper_tseng_res}, \Cref{prop:comp:bounds}, and \Cref{cor:lastiter:T}.
    \end{proof}
\end{corollary}

\begin{remark}\label{rmk:last-iterate_rates}
    In the items listed below, we compare the recent last-iterate rates in \cite[Theorem 3]{cai2022tightlastiterateconvergenceextragradient} and \cite[Corollary 4.1(b)]{trandinh2024revisitingextragradienttype} with \Cref{cor:rates_standard_measures}. In the following, assume that \Cref{ass:main} holds, the sequence \(\p{\p{z^{k},\bar{z}^{k}}}_{k\in\naturals}\) is generated by~\eqref{alg:EG} with initial point \(z^0\in \calH\) and step-size parameter \(\gamma\in(0,1/L_{F})\), and the sequence \(\p{\xi^{k}}_{k\in\mathbb{N}}\) is given by \eqref{eq:comparison:subgradient}.
    \begin{enumerate}
        \item \cite[Theorem 3]{cai2022tightlastiterateconvergenceextragradient} proves that 
        \begin{align}\label{eq:rate_cai}
            \inf_{\xi \in \partial g(z^{k})} \|F(z^{k})+ \xi\| \leq \frac{3 \norm{z^{0} - z^{\star} } }{ \gamma \sqrt{\p{1-\gamma^{} L_{F}^{2}} k }  }
        \end{align}
        for each \(k\in\mathbb{N}\) and \(z^{\star}\in\zer\p{F + \partial g}\), in the particular case when \(g\) is the indicator function of a closed, convex, and nonempty set. Simple computation shows that the corresponding rate in \Cref{cor:rates_standard_measures} sharpens \eqref{eq:rate_cai}, i.e.,
        \begin{align}\label{eq:rate_cai:comparison}
            \frac{1 }{ \sqrt{\alpha\p{ \gamma, L_{F}}} } < \frac{3}{ \gamma \sqrt{1-\gamma^{2} L_{F}^{2} }  }
        \end{align}
        for any \(\gamma \in (0,1/L_{F})\). For convenience, we plot the quotient 
        \begin{align}\label{eq:rate_cai:comparison:quotient}
            \left.\frac{1 }{ \sqrt{\alpha\p{ \gamma, L_{F}}} } \middle/  \frac{3}{ \gamma \sqrt{1-\gamma^{2} L_{F}^{2}}} \right.
        \end{align}
        in \Cref{fig:rate_quotient:a}, proving \eqref{eq:rate_cai:comparison} graphically.

        \item \cite[Corollary 4.1(b)]{trandinh2024revisitingextragradienttype} proves that 
        \begin{align}\label{eq:rate_trandinh}
            \|F(z^{k})+ \xi^{k}\| \leq \frac{\sqrt{3+2\gamma^2L_{F}^{2}} \norm{z^{0} - z^{\star} } }{ \gamma \sqrt{\p{1-\gamma L_{F}} k }  }
        \end{align}
        for each \(k\in\mathbb{N}\) and \(z^{\star}\in\zer\p{F + \partial g}\). Simple computation shows that the corresponding rate in \Cref{cor:rates_standard_measures} sharpens \eqref{eq:rate_trandinh}, i.e.,
        \begin{align}\label{eq:rate_trandinh:comparison}
            \frac{1 }{ \sqrt{\alpha\p{ \gamma, L_{F}}} } < \frac{\sqrt{3+2\gamma^2L_{F}^{2}} }{ \gamma \sqrt{1-\gamma L_{F}}}
        \end{align}
        for any \(\gamma \in (0,1/L_{F})\). For convenience, we plot the quotient 
        \begin{align}\label{eq:rate_trandinh:comparison:quotient}
            \left.\frac{1 }{ \sqrt{\alpha\p{ \gamma, L_{F}}} } \middle/  \frac{\sqrt{3+2\gamma^2L_{F}^{2}} }{ \gamma \sqrt{1-\gamma L_{F}  }   } \right.
        \end{align}
        in \Cref{fig:rate_quotient:b}, proving \eqref{eq:rate_trandinh:comparison} graphically.
    \end{enumerate}

\end{remark}

\begin{figure}[!t]
  \centering

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % (a) Quotient plot (top) -- no y=1 reference line
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.99\linewidth}
    \centering
    \begin{tikzpicture}
      % x = \gamma L_F
      \pgfmathdeclarefunction{q}{1}{%
        \pgfmathparse{(1.0/3.0)*sqrt( 2*(1 - #1*#1) / (sqrt(5 - 4*#1*#1) - 1) )}%
      }

      \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        domain=0.001:0.999,            % avoid endpoints/singularities
        xmin=0, xmax=1,                % show full axis 0..1
        ymin=0.3, ymax=0.5, 
        samples=1200,
        ymode=log,
        log ticks with fixed point,
        axis lines=left,
        xlabel={$\gamma L_F$},
        ylabel={},
        tick align=outside,
        tick style={black},
        xtick={0,0.1,...,1},
        minor x tick num=9,
        grid=both,
        grid style={dashed,black!35},
        minor grid style={dotted,black!25},
        legend style={
          draw=none,
          fill=white, fill opacity=0.9, text opacity=1,
          font=\small,
          at={(0.98,0.98)}, anchor=north east,
          row sep=8pt, inner sep=8pt,
          cells={anchor=west}
        },
        legend image post style={xscale=1.8},
        every axis plot/.append style={color=black, mark=none, line cap=round, line join=round},
        clip=false
      ]

        % Quotient curve: (1/sqrt(alpha)) / (3/(gamma*sqrt(1-gamma^2 L_F^2)))
        \addplot[ultra thick, restrict x to domain=0.001:0.999] ({x}, {q(x)});
        \addlegendentry{$\displaystyle
          \left.\frac{1}{\sqrt{\alpha(\gamma,L_F)}} \middle/ \frac{3}{\gamma\sqrt{1-\gamma^{2}L_F^{2}}}\right.
          \;=\; \frac{1}{3}\sqrt{\frac{2\bigl(1-\gamma^{2} L_F^{2}\bigr)}{\sqrt{5-4\gamma^{2} L_F^{2}}-1}}$}

      \end{axis}
    \end{tikzpicture}
    \caption{
    The ratio between the coefficients of the last-iterate rate in \Cref{cor:rates_standard_measures} and that of \cite[Theorem 3]{cai2022tightlastiterateconvergenceextragradient}.
    %Graphical verification that $\tfrac{1}{\sqrt{\alpha(\gamma,L_F)}} < \tfrac{3}{\gamma\sqrt{1-\gamma^{2}L_F^{2}}}$ for $\gamma\in(0,1/L_F)$ via the quotient \eqref{eq:rate_cai:comparison:quotient} being $<1$.
    }
    \label{fig:rate_quotient:a}
  \end{subfigure}

  \vspace{0.6em}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % (b) Trandinh comparison 
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{subfigure}{0.99\linewidth}
    \centering
    \begin{tikzpicture}
      % x = \gamma L_F
      \pgfmathdeclarefunction{qb}{1}{%
        \pgfmathparse{ sqrt( 2*(1-#1) / ((sqrt(5-4*#1*#1)-1)*(3+2*#1*#1)) ) }%
      }

      \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        domain=0.001:0.999,            % avoid endpoints/singularities
        xmin=0, xmax=1,                % show full axis 0..1
        ymin=0.2, ymax=1.3,
        samples=1200,
        ymode=log,
        log ticks with fixed point,
        axis lines=left,
        xlabel={$\gamma L_F$},
        ylabel={},
        tick align=outside,
        tick style={black},
        xtick={0,0.1,...,1},
        minor x tick num=9,
        grid=both,
        grid style={dashed,black!35},
        minor grid style={dotted,black!25},
        legend style={
          draw=none,
          fill=white, fill opacity=0.9, text opacity=1,
          font=\small,
          at={(0.98,0.98)}, anchor=north east,
          row sep=8pt, inner sep=8pt,
          cells={anchor=west}
        },
        legend image post style={xscale=1.8},
        every axis plot/.append style={color=black, mark=none, line cap=round, line join=round},
        clip=false
      ]

        % Quotient curve: (1/sqrt(alpha)) / ( sqrt(3+2 x^2) / (gamma*sqrt(1-x)) )
        \addplot[ultra thick, restrict x to domain=0.001:0.999] ({x}, {qb(x)});
        \addlegendentry{$\displaystyle
          \left.\frac{1}{\sqrt{\alpha(\gamma,L_F)}} \middle/ \frac{\sqrt{3+2\gamma^{2}L_F^{2}}}{\gamma\sqrt{1-\gamma L_F}}\right.
          \;=\; \sqrt{\frac{2\bigl(1-\gamma L_F\bigr)}{\bigl(\sqrt{5-4\gamma^{2} L_F^{2}}-1\bigr)\,\bigl(3+2\gamma^{2} L_F^{2}\bigr)}}$}

      \end{axis}
    \end{tikzpicture}
    \caption{
    The ratio between the coefficients of the last-iterate rate in \Cref{cor:rates_standard_measures} and that of \cite[Corollary 4.1(b)]{trandinh2024revisitingextragradienttype}.
    %Graphical verification that $\tfrac{1}{\sqrt{\alpha(\gamma,L_F)}} < \tfrac{\sqrt{3+2\gamma^2L_F^{2}}}{\gamma\sqrt{1-\gamma L_{F}}}$ for $\gamma\in(0,1/L_F)$ via the quotient \eqref{eq:rate_trandinh:comparison:quotient} being $<1$.
    }
    \label{fig:rate_quotient:b}
  \end{subfigure}

  \caption{}
  \label{fig:rate_quotients}
\end{figure}




\begin{remark}
    Similar to \Cref{rmk:cyclically_monotone}, the results in this section remain valid (except the ones involving the restricted gap function \(\textup{\texttt{Gap}}\)) when \(\partial g\) in \eqref{eq:the_inclusion_problem} is replaced with a maximally monotone and 3-cyclically monotone operator \(T:\calH\to\calH\) and the proximal operators \(\prox_{\gamma g}\) in \eqref{alg:EG} with the resolvent \(\p{\Id + \gamma T}^{-1}\).
\end{remark}
}%

==> extragradient/TeX/Text/conclusions.tex <==
%!TEX root = ../../main.tex
\section{Conclusions}\label{sec:conclusions}
This paper investigated algorithms for solving inclusion problems involving the sum of a monotone and Lipschitz continuous operator and the subdifferential of a proper, convex, and lower semicontinuous function. We proposed a new Lyapunov function for Korpelevich’s extragradient method and established a last-iterate convergence result. Departing from the standard Fej\'er-type analysis, this Lyapunov-based optimality measure did not rely on a known solution to the inclusion problem. It underpinned three novel algorithms that extend the extragradient method. These algorithms balanced user-specified directions and standard extragradient steps, guided by carefully designed line search steps based on the new Lyapunov analysis. In addition to providing global convergence results under various assumptions, we showed that when the directions are superlinear, no backtracking is triggered, leading to superlinear convergence.

\new{Future research directions include developing solution-independent Lyapunov functions for other related methods. In particular, the forward-reflected-backward method of Malitsky and Tam~\cite{malitsky2020forwardbackwardsplitting} is a relevant case. Relatedly, a solution-independent Lyapunov function is already available for Malitsky’s projected reflected gradient method~\cite{malitsky2015projectedreflectedgradient} in \cite[Section~D]{cai2023accelerated}}. Another promising direction is to broaden the scope of the analysis beyond the monotone setting to include cohypomonotone operators~\cite{pennanen2002localconvergenceproximal}, and the more general class of problems characterized by the weak Minty condition~\cite{diakonikolas2021efficient,lee2021fast,pethick2022escaping}. Additionally, further exploration is warranted to adapt the approach to the mirror prox framework~\cite{nemirovski2004proxmethodrate}.



==> extragradient/TeX/Text/counterexamples.tex <==
\section{Counterexamples}\label{app:counterexamples}
\begin{example}\label{ex:counterexample:tseng}
    Let \(\V_k = \V\p{z^{k},\bar{z}^{k},z^{k+1}}\) for the Lyapunov function \(\V\) defined in~\eqref{eq:V} and iterates \(\seq{\p{z^{k},\bar{z}^{k}}}\) generated by Tseng's method~\eqref{alg:Tseng}. This example contains a particular instance of the inclusion problem~\eqref{eq:the_inclusion_problem}, initial point \(z^{0}\in\calH\), and step size \(\gamma\in\p{0,1/L_F}\) for which \(\V_k\) increases between the first two consecutive iterations, thereby establishing that \(\V_k\) has no (one-step) descent inequality in this case. In particular, consider \(\calH=\reals^4\), \(F:\reals^4 \to \reals^4\), and \(g:\reals^4\to\reals\cup \{+\infty\}\) such that 
    \begin{align*}
        F(z) {}={} 
        \begin{bmatrix}
            A x \\
            - A^{\top} y
        \end{bmatrix}
        \quad 
        \text{ and }
        \quad
        g(z) {}={}
        \begin{cases}
            0 & \text{if } x \in [-7,6]^2 \text{ and } y \in [1,8]^2,\\
            +\infty & \text{otherwise}
        \end{cases}
    \end{align*}
    for each \(z = \p{x,y} \in \reals^2 \times \reals^2\), respectively, where   
    \begin{align*}
        A {}={}
        \begin{bmatrix}
            7 & 6 \\
            1 & 0
        \end{bmatrix}.
    \end{align*}
    It is straightforward to verify that \Cref{ass:main} holds with\footnote{The matrix norm is taken as the spectral norm.} 
    \begin{align*}
        L_{F} {}={} 
        \left\lVert 
        \begin{bmatrix}
            0 &  A \\
            - A^{\top} & 0
        \end{bmatrix}
        \right\rVert \approx 9.25091.
    \end{align*}
    By letting \(z^{0} = \p{-1, -7, -1, 7} \) and \(\gamma = {1}/{10}\), Tseng's method gives that 
    {\begin{allowdisplaybreaks}
    \begin{align*}
        \bar{z}^{0} &{}={} \left(-\frac{9}{2}, - \frac{69}{10}, 1, \frac{32}{5}\right), \\ %= \p{-4.5, -6.9, 1, 6.4}, \\
        z^{1} &{}={} \left(-\frac{277}{50}, -\frac{71}{10}, -\frac{36}{25}, \frac{43}{10}\right), \\ %= \p{-5.54, -7.1, -1.44, 4.3 },\\
        \bar{z}^{1} &{}={} \left(-7,-\frac{1739}{250}, 1, 1\right), %= \p{-7,-6.956, 1, 1},
    \end{align*}
    \end{allowdisplaybreaks}}%
    and therefore
    \begin{align*}
        \V_0 {}={} 1662 \quad \text{ and }\quad
        \V_1 {}={} \frac{1187246}{625} {}={} 1899.5936,
    \end{align*}
    establishing the claim.\footnote{Code to reproduce this example can be found at \url{https://github.com/ManuUpadhyaya/flex/blob/main/Counterexample_B1.ipynb}.} \qed
\end{example}

\begin{example}\label{ex:counterexample:full_eg}
    Consider the inclusion problem
    \begin{align*}
        \text{find}\  z\in\calH\ \text{ such that }\ 0 \in F(z) + T(z)
    \end{align*}
    where \(F:\calH\to\calH\) satisfies \Cref{ass:F} and \(T:\calH\to2^\calH\) is a maximally monotone operator. Let
    \begin{align}\label{alg:full_eg}
        \begin{split}
          \bar{z}^{k}
          &= \p{\Id+\gamma T}^{-1}\p{z^{k} - \gamma F(z^{k})}, 
          \\
          z^{k+1} 
          &= \p{\Id+\gamma T}^{-1}\p{z^{k} - \gamma F(\bar{z}^{k})},
        \end{split}
    \end{align}
    and \(\V_k = \V\p{z^{k},\bar{z}^{k},z^{k+1}}\) for the Lyapunov function \(\V\) defined in~\eqref{eq:V}. This example contains a particular problem instance for which \(\seq{z^{k}}\) diverges and \(\V_k\) increases between the first two consecutive iterations. In particular, consider \(\calH = \reals^2\), \(z^0 = (10, 10)\), \(\gamma = 1/10\), and \(F,T:\reals^2 \to \reals^2\) such that
    \begin{align*}
        F(z) {}={} 
        \underbracket{
        \begin{bmatrix}
            0 & 9 \\
            -9 & 0 
        \end{bmatrix}
        }_{=A}
        \begin{bmatrix}
            x \\
            y
        \end{bmatrix}
        \quad \text{ and } \quad
        T(z) {}={}
        \underbracket{
        \begin{bmatrix}
            0 & -4 \\
            4 & 0 
        \end{bmatrix}
        }_{=B}
        \begin{bmatrix}
            x \\
            y
        \end{bmatrix}
    \end{align*}
    for each \(z = \p{x,y} \in \reals\times\reals\), where \(L_F = 9\). Note that~\eqref{alg:full_eg} reduces to
    \begin{align*}
        z^{k+1} = \underbracket{\left(I+\gamma B\right)^{-1}\left(I - \gamma A \left( \left(I+\gamma B\right)^{-1} \left( I - \gamma A\right) \right) \right)}_{=C} z^{k},
    \end{align*}
    where \(C\in\reals^{2\times 2}\)  has full rank and spectral radius \(\approx 1.132596\), which is greater than one. Therefore, we can conclude that \(\seq{z^{k}}\) diverges. Moreover,~\eqref{alg:full_eg} gives that
    {\begin{allowdisplaybreaks}
    \begin{align*}
        \bar{z}^0 &{}={} \left(\frac{215}{29}, \frac{465}{29}\right), \\
        z^1 &{}={} \left(\frac{3245}{1682}, \frac{26745}{1682}\right), \\
        \bar{z}^1 &{}={} \left(-\frac{447965}{97556}, \frac{1899785}{97556}\right), \\
        z^2 &{}={} \left(-\frac{53118995}{5658248}, \frac{87834005}{5658248}\right),
    \end{align*}
    \end{allowdisplaybreaks}}%
    and therefore
    {\begin{allowdisplaybreaks}
    \begin{align*}
        \V_0 &{}={} \frac{5875000}{841} {}\approx{} 6985.73127229489, \\
        \V_1 &{}={} \frac{12676046875}{1414562} {}\approx{} 8961.11084208398,
    \end{align*}
    \end{allowdisplaybreaks}}%
    establishing the second claim.\footnote{Code to reproduce this example can be found at \url{https://github.com/ManuUpadhyaya/flex/blob/main/Counterexample_B2.ipynb}.} \qed
\end{example}


==> extragradient/TeX/Text/equilibrium.tex <==
Consider a noncooperative game with \(n\in\mathbb{N}\) players, in which each player \(i \in \llbracket1,n\rrbracket\) has to pick a strategy \(z_{i}\) that lies in \(\mathcal{Z}_{i}\), a subset of a real Hilbert space \(\calH_i\), and has an associated loss function \(\varphi_{i}:\calH \to \reals\), where \(\calH=\prod_{j=1}^{n}\calH_j\).  In this case, a pure strategy Nash equilibrium is a strategy profile \(z = \p{z_{1},\ldots, z_{n}}\in\calH\) that solves the problem
\begin{align}\label{eq:Nash}
    \text{find}\  z\in\calH\ \text{ such that }\ z_{i} \in \Argmin_{x \in \mathcal{Z}_{i}} \varphi_{i}\p{x;z_{\smallsetminus i}} \ \text{ for each }\ i \in \llbracket1,n\rrbracket,
\end{align}
where we have used the notation \(\p{x;z_{\smallsetminus i}} = \p{z_{1},\ldots, z_{i-1}, x, z_{i+1},\ldots,z_{n}}\) for each \(x\in\calH_{i}\) and \(i \in \llbracket1,n\rrbracket\). In particular, assume that, for each \(i \in \llbracket1,n\rrbracket\), the function \(\varphi_{i}(\,\cdot\,;z_{\smallsetminus i}):\calH_{i} \to \reals\) is convex for each \(z\in\calH\), the gradient \(\nabla_{z_{i}}\varphi_{i}:\calH \to \calH_{i}\) exists and is Lipschitz continuous, and the set \(\mathcal{Z}_{i}\subseteq\calH_{i}\) is nonempty, closed and convex. Then~\eqref{eq:Nash} can equivalently be written as~\eqref{eq:the_inclusion_problem} by letting \(F:\calH \to \calH : z \mapsto \p{\nabla_{z_{i}}\varphi_{i}\p{z}}_{i=1}^{n}\) and \(g=\delta_{\mathcal{Z}}\), where \(\mathcal{Z} = \prod_{i=1}^{n}\mathcal{Z}_{i}\), and it is straightforward to verify that \Cref{ass:main} holds.


Let us further specialize the model to the Cournot--Nash equilibrium problem for oligopolistic markets with concave-quadratic cost functions and a differentiated commodity, as presented in~\cite{Bigi_Passacantando_2017}. Such models are useful for policymakers and economists in analyzing market outcomes, assessing welfare effects, and evaluating the impact of various market interventions~\cite{Bonanno_1990,fudenberg1986dynamic,von_Mouche_Quartieri_2016,Muu2008,Okuguchi_Szidarovszky_1999,Vives_1989}. In particular, in the model of~\cite{Bigi_Passacantando_2017}, each producer \(i\in\llbracket1,n\rrbracket\) chooses to produce and supply a quantity \(z_{i} \in [0,T_{i}]\) of a differentiated commodity at a cost \(c_{i}:\reals\to\reals\) such that 
\begin{align*}
    c_{i}\p{z_{i}} = a_{i} z_{i}^{2} + b_{i} z_{i},
\end{align*}
for each \(z_{i}\in \reals\), where \(T_{i}>0\) denotes the maximum capacity of production, and \(a_{i}<0\) and \(b_{i}>0\) are numbers such that \(b_{i} \geq -2T_{i}a_{i}\), ensuring that \(c_{i}\) is increasing on \([0,T_{i}]\). Moreover, each producer \(i\in\llbracket1,n\rrbracket\) has a price per produced unit of the differentiated commodity\footnote{Also known as the inverse demand function.}, denoted by \(p_{i}:\reals^{n}\to\reals\), that also depends on the other producers' supply, and is modeled by 
\begin{align*}
    p_{i}\p{z} = m_{i} - d_{i} \sum_{j=1}^{n}z_{j}
\end{align*}
for each \(z = \p{z_{1},\ldots,z_{n}}\in\reals^{n}\), for some \(m_{i} > b_{i}\) and \(d_{i}> - a_{i}\), where the last two assumptions guarantee a positive profit in a monopolistic setting, i.e., when \(n=1\). Thus, given that the goal of each producer is to maximize profit, or equivalently minimize losses, an equilibrium state where no producer has any incentive to deviate unidirectionally from its production plan can be modeled by~\eqref{eq:Nash}, with  \(\mathcal{Z}_{i} = [0, T_{i}]\), \(\calH_{i} = \reals\), and
\begin{align*}
    \varphi_{i}\p{z} &= c_{i}\p{z_{i}} - z_{i} p\p{z} %= \p{a_{i} + d_{i} } z_{i}^{2} + \p{b_{i} - m_{i} + d_{i} \sum_{\substack{j=1 \\ j\neq i}}^{n}z_{j}} z_{i} \\
    %\nabla_{z_{i}} \varphi_{i}\p{z} & = 2 \p{a_{i} + d_{i} }z_{i} + d_{i} \sum_{\substack{j=1 \\ j\neq i}}^{n}z_{j} + b_{i} - m_{i}
\end{align*}
for each \(z = \p{z_{1},\ldots,z_{n}}\in\reals^{n}\) and \(i\in\llbracket1,n\rrbracket\), which fulfill the assumptions in the first paragraph of this section. We identify \(F\) as 
\begin{align*}
    F\p{z} = 
    \underbracket{
    \begin{bmatrix}
        2\p{a_{1} + d_{1}}  & d_{1}             & d_{1}     & \cdots & d_{1} \\ 
        d_{2}               & 2\p{a_{2} + d_{2}}& d_{2} & \cdots & d_{2} \\
        d_{3} & d_{3} & 2\p{a_{3} + d_{3}} & \cdots & d_{3} \\
        \vdots & \vdots & \vdots & \ddots & \vdots \\
        d_{n} & d_{n} & d_{n} & \cdots & 2\p{a_{n} + d_{n}}
    \end{bmatrix} 
    }_{= A}
    z 
    +
    \begin{bmatrix}
        b_{1} - m_{1} \\
        \vdots \\
        b_{n} - m_{n} 
    \end{bmatrix} 
\end{align*}
with Lipschitz constant \(L_{F} = \norm{A}\). We also note that~\cite{Rosen_1965} provides the existence of a solution in this case. We generate the data similar to the approach in~\cite[Section 4.1]{Bigi_Passacantando_2017}, as outlined below. The results of the numerical experiments are presented in \Cref{fig:nash}. Although \(n=100\) in \Cref{fig:nash:100} is not representative of a real oligopolistic market, we include this larger problem size to evaluate the performance and scalability of the algorithms. We observe that~\ProxFLEX{} has a superlinear drop-off in both cases and that \texttt{EG-AA} and \texttt{aGRAAL} scale well for this particular problem.  

\input{TeX/Algs/Cournot_Nash_data_generation}

\input{plots/Cournot_Nash.tex}

==> extragradient/TeX/Text/flex.tex <==
%!TEX root = ../../main.tex
In this subsection, we focus on the case \(g = 0\) in~\eqref{eq:the_inclusion_problem}, where the Lyapunov inequality~\eqref{eq:EG:new_Lyapunov_w.o._sol} simplifies to~\eqref{eq:EG:new_Lyapunov_w.o._sol:g_zero}. The first algorithm introduced here is~\refFLEX, which can be viewed as a hybrid scheme in the same spirit as \cite[Algorithm 5.16]{izmailov2014newtontypemethods}. At each iteration, it computes a suitable direction \(d^k\) (see \Cref{sec:superlinear}) and performs the updates \(z^{k+1} = z^k + d^k\) whenever the contraction condition in \Cref{State:FLEX:contraction} holds. Otherwise, it conducts a line search based on the descent inequality~\eqref{eq:EG:new_Lyapunov_w.o._sol:g_zero}, serving as a \emph{performance safeguard}.

Before we present the convergence results for~\FLEX{}, we offer some observations on the line-search procedure.

\begin{remark}
    \label{rem:FLEX:LS} 
   The line-search interpolation strategy in~\FLEX{} is designed to ensure global convergence while infusing local update directions in the algorithm. It differs from standard line-search procedures in some respects. 
    \begin{enumerate}
        \item\label{rem:FLEX:LS:bad_case}%
        After a finite number of backtracks, the method defaults to \(\tau_k = 0\), at which point~\eqref{eq:FLEX:descent} is satisfied due to~\eqref{eq:EG:new_Lyapunov_w.o._sol:g_zero} in \Cref{cor:EG:new_Lyapunov_w.o._sol:g_zero}. 
        Taking the nominal step after a finite number of trials is not just a practical consideration but is also theoretically grounded. Without additional assumptions, it is possible that \(\|F(z^k) - F(\bar{z}^k)\| = 0\) even when no solution has been found, and~\eqref{eq:FLEX:descent} is not satisfied by any \(\tau_k > 0\) for some ill-chosen user-specified direction \(d^k\). Therefore, additional assumptions are required for such edge cases if an infinite backtracking strategy with known finite termination is to be employed. This is further explored in \Cref{sec:IFLEX}.
        
        \item 
        Enforcing a descent inequality as in~\eqref{eq:FLEX:descent} of \Cref{State:FLEX:LS} can be viewed as a performance safeguarding. 
        As it is shown in \Cref{thm:FLEX:dk_summable} below, the convergence of~\FLEX{} can be guaranteed provided that \(\seq{d^k} \in \ell^{1}(\naturals;\,\calH)\). Therefore, the descent inequality within the line-search procedure ensures that the directions contribute effectively to the convergence, preventing arbitrarily poor performance.  
    \end{enumerate}  
\end{remark}
The next theorem establishes global convergence of~\FLEX{} under the assumption that the directions are summable, a setting that will be revisited in \Cref{sec:superlinear}, see also \Cref{thm:suplin:summable}.
Alternatively, if \(F\) is uniformly monotone, the summability assumption is dropped, as shown in \Cref{thm:FLEX:F_unifrom}. Moreover, when \(F\) is \(\mu_F\)-strongly monotone, as in \Cref{thm:FLEX:F_strongly}, a linear convergence rate is achieved.

\input{TeX/Algs/FLEX}

\begin{theorem}\label{thm:FLEX}
    Suppose that \Cref{ass:F} holds,  \(\zer \p{F}\neq \emptyset\), and the sequence \(\p{z^{k}}_{k\in\naturals}\) is generated by~\refFLEX. Then, the following hold.
    \begin{thmenumerate}

        \item \label{thm:FLEX:dk_summable} If \(\seq{d^k}\in\ell^{1}(\naturals;\,\calH)\), then \(\seq{z^k}\) converges weakly to some point in \(\zer \p{F}\). 

        \item \label{thm:FLEX:F_unifrom} If \(F\) is uniformly monotone, then \(\seq{z^k}\) converges weakly to some point in \(\zer \p{F}\).
    
        \item \label{thm:FLEX:F_strongly} If there exists \(0<\mu_F\leq L_F\) such that \(\mu_F \norm{x - y}\leq\norm{F\p{x}- F\p{y}}\) for each \(x,y\in \calH\), then \(\seq{z^k}\) converges strongly to some point in \(\zer \p{F}\) and
        \begin{align}\label{eq:FLEX:F_strongly:linear}
                \norm{F(z^{k+1})}^2 \leq 
                \smash{\underbracket{
                \max\p{ \rho^2, 1- \sigma\gamma^{2}\mu_{F}^{2}\p{1-\gamma^{2}L_{F}^{2}} }
                }_{\in(0,1)}}
                \norm{F(z^{k})}^2
            \end{align} 
        for each \(k\in\naturals\).
    \end{thmenumerate}
\end{theorem}




\subsubsection{Variant of \texttt{FLEX} under injectivity}\label{sec:IFLEX}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{TeX/Text/iflex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> extragradient/TeX/Text/global.tex <==
\section{Global convergence}\label{sec:global}
This section provides detailed proofs of the results presented in \Cref{sec:algs}. We start by providing two useful lemmas. The first lemma establishes that the iterates generated by~\FLEX,~\IFLEX, and~\ProxFLEX{} are quasi-Fej\'er monotone with respect to the solution set, which is an important tool in establishing global convergence. The second lemma contains some auxiliary results. 

\begin{lemma}\label{lem:zk_quasi_fejer}
    Suppose that \Cref{ass:main} holds, \(z^{\star}\in\zer \p{F + \partial g}\), \(\seq{d^k}\in\ell^{1}(\naturals;\,\calH)\), \(T_1^{\gamma}\) and \(T_2^{\gamma}\) are the algorithmic operators defined in~\eqref{eq:T1T2}, and \(\V\) is the Lyapunov function given in~\eqref{eq:V}. Let \(\p{z^{k}}_{k\in\naturals}\in\calH^{\naturals}\) such that \(z^{k+1} = (1-\tau_k)w^{k} + \tau_{k}(z^{k} + d^{k})\), where \(\tau_k \in [0,1]\) and \(w^{k} = T_2^\gamma(z^k)\) for each \(k\in\naturals\). Then there exists a sequence \(\seq{\varepsilon_k}\in\ell^{1}\p{\naturals;\,\reals_{+}}\) such that
    \begin{align}\label{eq:zk_quasi_fejer}
        \norm{z^{k+1}-z^\star}^2 \leq \norm{z^k-z^\star}^2 + \varepsilon_k - (1- \tau_k)\alpha\p{\gamma, L_F}\V_k,
    \end{align}
    where \(\alpha\p{\gamma, L_F}\) is defined in~\eqref{eq:EG:primal_descent_for_V:alpha}, \(\V_{k} = \V(z^k, \bar z^k, w^{k})\), and \(\bar z^k = T_1^{\gamma}(z^k)\) for each \(k\in\naturals\).
    \begin{proof}
        Note that \Cref{prop:V_performance_measure:lower_bound} gives that \(\V_{k}\geq 0\) for each \(k\in\naturals\). Using the identity 
        \begin{align*}
            \norm{\tau x+\p{1-\tau}y}^2 = \tau\norm{x}^2 + \p{1-\tau}\norm{y}^2 - \tau\p{1-\tau}\norm{x-y}^2
        \end{align*}
        for each \(x,y\in\calH\) and \(\tau\in\reals\) {\cite[Corollary 2.15]{bauschke2017convexanalysismonotone}}, and \(z^{k+1} - z^{\star} = \tau_{k} (z^{k} + d^{k} - z^{\star}) + (1-\tau_{k}) (w^{k} - z^{\star}) \) for each \(k\in\naturals\), we get that
        {\begin{allowdisplaybreaks}
        \begin{align} \nonumber
            & \norm{z^{k+1} - z^\star}^2 \\ \nonumber
            & \quad =
            \tau_k\norm{z^{k}+ d^k - z^\star}^2 
            + (1- \tau_k)\norm{w^k-z^\star}^2 
            - \tau_k(1- \tau_k)\norm{z^{k} + d^{k} - w^k}^2 \\ \nonumber
            & \quad \leq 
            \tau_k\norm{z^{k} + d^k- z^\star}^2 
            + (1- \tau_k)\norm{z^k-z^\star}^2  
            - (1- \tau_k)\alpha\p{\gamma, L_F} \V_k \\ \nonumber
            & \quad \leq 
            \tau_k\p{\norm{z^{k}- z^\star}+\norm{d^k}}^2 + (1- \tau_k)\norm{z^k-z^\star}^2  - (1- \tau_k)\alpha\p{\gamma, L_F} \V_k  \\ \label{eq:zk_quasi_fejer_}
            & \quad \leq
            \norm{z^k-z^\star}^2 
            + 2\norm{z^{k}- z^\star}\norm{d^k}
            + \norm{d^k}^2 - (1- \tau_k)\alpha\p{\gamma, L_F} \V_k \\ \label{eq:zk_bounded_}
            & \quad  \leq \p{\norm{z^k-z^\star} + \norm{d^k}}^2
        \end{align}
        \end{allowdisplaybreaks}}%
        for each \(k\in\naturals\), where~\eqref{eq:EG:primal_descent_for_V}  and \(\tau_k(1-\tau_k)\geq 0\) is used in the first inequality, the triangle inequality is used in the second inequality, \(\tau_{k} \leq 1\) is used in the third inequality, and \( (1- \tau_k)\alpha\p{\gamma, L_F} \geq 0\) is used in the last inequality. Taking the square root of~\eqref{eq:zk_bounded_} and inductively applying the resulting inequality gives that 
        \begin{align}\label{eq:zk_bounded}
            \norm{z^k-z^\star} \leq \norm{z^0-z^\star} + \textstyle\sum_{i=0}^{k-1} \norm{d^{i}} \leq \underbracket{\norm{z^0-z^\star} + \textstyle\sum_{i=0}^{\infty} \norm{d^{i}}}_{=E} < \infty
        \end{align}
        for each \(k\in\naturals\), where the empty sum is interpreted as zero and \(E\) is finite since \(\seq{d^k}\in\ell^{1}(\naturals;\,\calH)\). Therefore,~\eqref{eq:zk_quasi_fejer_} and~\eqref{eq:zk_bounded} imply that 
        \begin{align*}
            \norm{z^{k+1}-z^\star}^2 {}\leq{}& \norm{z^k-z^\star}^2  + \underbracket{2E \norm{d^k} +\norm{d^k}^2}_{=\varepsilon_k} - (1- \tau_k)\alpha\p{\gamma, L_F} \V_k
        \end{align*}
        for each \(k\in\naturals\), where summability of \(\seq{\varepsilon_k}\) follows from \(\seq{d^k}\in\ell^{1}(\naturals;\,\calH)\). 
    \end{proof}
\end{lemma}

\begin{lemma}\label{lem:(Prox)(I)FLEX}
    Suppose that \Cref{ass:main} holds, the sequences \(\p{z^{k}}_{k\in\naturals}\), \(\p{\bar{z}^{k}}_{k\in\naturals}\) and \(\p{w^{k}}_{k\in\naturals}\) are generated by either~\refFLEX{},~\refIFLEX, or~\refProxFLEX, and \(\V\) is the Lyapunov function given in~\eqref{eq:V}. Then, the following hold.
    \begin{enumeratlem}
    
        \item \label{lem:(Prox)(I)FLEX:norm_F_or_V_convergent} 
        \(\seq{\V\p{z^{k},\bar{z}^{k},w^{k}}}\) is convergent, which for~\FLEX{} and~\IFLEX{} reduces to \(\seq{F\p{z^{k}}}\) being convergent.
        
        \item \label{lem:(Prox)(I)FLEX:residual_summable} \(\seq{\norm{w^{k}-\bar{z}^{k}}^{2}}\in\ell^{1}\p{\naturals;\,\reals_{+}}\), which for~\FLEX{} and~\IFLEX{} can be written as \(\seq{\norm{F\p{z^{k}}-F\p{\bar{z}^{k}}}^{2}}\in\ell^{1}\p{\naturals;\,\reals_{+}}\).

        \item \label{lem:(Prox)(I)FLEX:uniformly} If \(F\) is uniformly monotone, then \(\seq{\norm{F( z^{k})}}\) converges to zero for~\FLEX{} and~\IFLEX.
    \end{enumeratlem}
    \begin{proof}

        First, we establish for~\ProxFLEX{} that 
        \begin{align}\notag
            \V\p{z^{k+1},\bar{z}^{k+1},w^{k+1}} \leq{}& \V\p{z^{k},\bar{z}^{k},w^{k}} \\ \label{eq:ProxFLEX:has_dual_descent}
            &{}- \min(\p{1- \gamma \LF}\p{1-\rho^{2}},\sigma\p{1-\gamma^{2}L_{F}^{2}}) \gamma^{-2}\norm{w^{k}-\bar{z}^{k}}^{2} 
        \end{align}
        for each \(k\in\naturals\). Note that \Cref{State:Prox-FLEX:contraction} in~\ProxFLEX{} implies that
        {\begin{allowdisplaybreaks}
        \begin{align*}
            \V\p{z^{k+1},\bar{z}^{k+1},w^{k+1}} 
            \leq{} & \rho^{2}\V\p{z^{k},\bar{z}^{k},w^{k}} \\
            ={} & \V\p{z^{k},\bar{z}^{k},w^{k}} - \p{1-\rho^{2}}\V\p{z^{k},\bar{z}^{k},w^{k}} \\
            \leq{} & \V\p{z^{k},\bar{z}^{k},w^{k}} - \p{1- \gamma \LF}\p{1-\rho^{2}}\gamma^{-2}\norm{w^{k}-\bar{z}^{k}}^{2} 
        \end{align*}
        \end{allowdisplaybreaks}}%
        for each iteration \(k\) when the condition in \Cref{State:Prox-FLEX:contraction} of~\ProxFLEX{} is true, where \Cref{prop:V_performance_measure:lower_bound} is used in the last inequality. This combined with~\eqref{eq:Prox-FLEX:descent} in~\ProxFLEX{} gives~\eqref{eq:ProxFLEX:has_dual_descent}.

        Second, since~\ProxFLEX{} reduced to~\FLEX{} when \(g=0\),~\eqref{eq:ProxFLEX:has_dual_descent} implies that
        \begin{align}\label{eq:FLEX:has_dual_descent}
            \norm{F\p{z^{k+1}}}^{2} \leq{}& \norm{F\p{z^{k}}}^{2} - \min(\p{1- \gamma \LF}\p{1-\rho^{2}},\sigma\p{1-\gamma^{2}L_{F}^{2}}) \norm{F\p{z^{k}}-F\p{\bar{z}^{k}}}^{2}
        \end{align}
        for each \(k\in\naturals\), for~\FLEX.
        
        \begin{itemize}%[left=1.2cm]

            \item[\ref{lem:(Prox)(I)FLEX:norm_F_or_V_convergent}:] Follows from~\eqref{eq:FLEX:has_dual_descent} for~\FLEX{},~\eqref{eq:I-FLEX:descent} for~\IFLEX, and~\eqref{eq:ProxFLEX:has_dual_descent} for~\ProxFLEX, combined with the monotone convergence theorem.
            
            \item[\ref{lem:(Prox)(I)FLEX:residual_summable}:] Note that \(\seq{\norm{w^{k}-\bar{z}^{k}}^{2}} = \seq{ \gamma^{2} \norm{F\p{z^{k}}-F\p{\bar{z}^{k}}}^{2} } \) for~\FLEX{} and~\IFLEX. The statement follows from~\eqref{eq:FLEX:has_dual_descent} for~\FLEX{},~\eqref{eq:I-FLEX:descent} for~\IFLEX, and~\eqref{eq:ProxFLEX:has_dual_descent} for~\ProxFLEX, combined with a telescoping summation argument. 

            \item[\ref{lem:(Prox)(I)FLEX:uniformly}:] Suppose that \(F\) is uniformly monotone, i.e., there exists an increasing function \(\phi : \reals_{+} \to \reals_{+}\), that vanishes only at \(0\),  such that 
            \begin{align*}
                \phi\left(\norm{x-y}\right) \leq \langle x - y , F(x) - F(y) \rangle
            \end{align*}
            for each \(x,y\in \calH\). Note that
            {\begin{allowdisplaybreaks}
            \begin{align*}
                \phi\left(\gamma\norm{F\p{z^{k}}}\right) 
                    &= \phi\left(\norm{z^{k} - \bar{z}^{k}}\right) \\
                    &\leq \langle z^{k} - \bar{z}^{k} , F\p{z^{k}} - F\p{\bar{z}^{k}} \rangle \\
                    &\leq \norm{ z^{k} - \bar{z}^{k}} \norm{ F\p{z^{k}} - F\p{\bar{z}^{k}} } \\
                    &= \gamma \norm{ F\p{z^{k}} } \norm{ F\p{z^{k}} - F\p{\bar{z}^{k}} } \xrightarrow[k\rightarrow \infty]{} 0, 
            \end{align*}
            \end{allowdisplaybreaks}}%
            where \(\bar{z}^{k} = z^{k} - \gamma F(z^{k})\) is used in the first equality, the Cauchy--Schwarz inequality is used in the second inequality, \(\bar{z}^{k} = z^{k} - \gamma F(z^{k})\) is used in the last equality, and the convergence to zero in the last line follows from \Cref{lem:(Prox)(I)FLEX:norm_F_or_V_convergent} and \Cref{lem:(Prox)(I)FLEX:residual_summable}. This proves the claim. \qedhere
        \end{itemize}
    \end{proof}
\end{lemma}


\iffalse
\begin{remark}
    Note that~\ProxFLEX{} is not discussed in \Cref{lem:(Prox)(I)FLEX:uniformly}. However, similar to \Cref{rem:strength:proxflex}, if \(F\) is uniformly monotone, it is possible to strengthen the linear search condition~\eqref{eq:Prox-FLEX:descent} in~\ProxFLEX{} to take the uniform monotonicity into account, and then conclude that \(\seq{\V\p{z^{k},\bar{z}^{k},w^{k}}}\) converges to zero. Since the resulting line-search condition is not actionable for many practical problems, we choose not to consider this case further. 
\end{remark}
\fi


\subsection{Proofs regarding~\FLEX}

\begin{proof}[Proof of \Cref{thm:FLEX:dk_summable}.]
    This follows from \Cref{thm:ProxFLEX}, since~\refProxFLEX{} reduces to~\refFLEX{} when \(g=0\). 
\end{proof}

\begin{proof}[Proof of \Cref{thm:FLEX:F_unifrom}.]
    See \Cref{lem:(Prox)(I)FLEX:uniformly}. 
\end{proof}

\begin{proof}[Proof of \Cref{thm:FLEX:F_strongly}.]
    Note that~\eqref{eq:FLEX:descent} gives that
    {\begin{allowdisplaybreaks}
    \begin{align}\notag
        \norm{F\p{z^{k+1}}}^2 
        \leq &  \norm{F\p{z^{k}}}^2 -  \sigma\p{1-\gamma^{2}L_{F}^{2}} \norm{F\p{z^{k}} - F\p{\bar{z}^{k}}}^2 \\\notag
        \leq &  \norm{F\p{z^{k}}}^2  - \sigma\mu_{F}^{2}\p{1-\gamma^{2}L_{F}^{2}} \norm{z^{k} - \bar{z}^{k}}^{2}  \\\label{eq:FLEX:dual_descent_plus_strong_give_contraction}
        = & \p{1 - \sigma\gamma^{2}\mu_{F}^{2}\p{1-\gamma^{2}L_{F}^{2}}  } \norm{F\p{z^{k}}}^2
    \end{align}
    \end{allowdisplaybreaks}}%
    for each iteration \(k\) such that the condition in \Cref{State:FLEX:contraction} in~\FLEX{} is false, where \Cref{State:FLEX:EG} in~\FLEX{} is used in the last equality. Combining~\eqref{eq:FLEX:dual_descent_plus_strong_give_contraction} and \Cref{State:FLEX:contraction} in~\FLEX{} gives~\eqref{eq:FLEX:F_strongly:linear}. Moreover, \(\seq{\norm{F(z^k)}}\) converges to zero since \( \max(\rho^2, 1- \sigma\gamma^{2}\mu_{F}^{2}\p{1-\gamma^{2}L_{F}^{2}} ) \in (0,1)\). Since
    \begin{align*}
        \norm{z^{k} - z^{\star}} \leq \mu_{F}^{-1} \norm{F(z^{k}) - F(z^{\star})} = \mu_{F}^{-1} \norm{F(z^{k})}
    \end{align*}
    for each \(k\in\naturals\), \(\seq{z^k}\) converges strongly to \(z^{\star}\in \zer(F)\). 
\end{proof}

\subsection{Proofs regarding~\IFLEX}

\begin{proof}[Proof of \Cref{thm:I-FLEX:injective}.]
    Suppose that \(\seq{z^{k}}[k\in K]\rightharpoonup z^\infty\). Weak continuity of \(F\) and \(\bar{z}^{k} = z^{k} - \gamma F\p{z^{k}}\) give that \(\seq{\bar{z}^{k}}[k\in K] \rightharpoonup \bar{z}^\infty = z^\infty - \gamma F(z^\infty)\). On the other hand, it follows from  \Cref{lem:(Prox)(I)FLEX:residual_summable} and weak continuity of \(F\) that \(F(z^\infty) = F(\bar z^\infty)\), which in view of the injectivity assumption of \(F\), implies \(z^\infty = \bar z^\infty = z^\infty - \gamma F(z^\infty)\). Therefore, \(z^\infty \in \zer\p{F}\), as claimed. 
\end{proof}

\begin{proof}[Proof of \Cref{thm:I-FLEX:dk_bounded}.]
    Note that \Cref{thm:I-FLEX:injective} gives that each weak sequential cluster point of  \(\seq{z^k}\) is in \(\zer \p{F}\). Moreover,~\cite[Lemma 5.31]{bauschke2017convexanalysismonotone} and~\eqref{eq:zk_quasi_fejer} in \Cref{lem:zk_quasi_fejer} give that \(\seq{\norm{z^k-z^\star}}\) converges. Thus,~\cite[Lemma 2.47]{bauschke2017convexanalysismonotone} gives that \(\seq{z^k}\) converges weakly to some point in \(\zer \p{F}\), as claimed. 
\end{proof}

\begin{proof}[Proof of \Cref{thm:I-FLEX:F_unifrom}.]
    See \Cref{lem:(Prox)(I)FLEX:uniformly}. 
\end{proof}

\begin{proof}[Proof of \Cref{thm:I-FLEX:F_strongly}.]
    Note that~\eqref{eq:I-FLEX:descent} gives that
    {\begin{allowdisplaybreaks}
    \begin{align*}
        \norm{F\p{z^{k+1}}}^2 
        \leq &  \norm{F\p{z^{k}}}^2 -  \sigma\p{1-\gamma^{2}L_{F}^{2}} \norm{F\p{z^{k}} - F\p{\bar{z}^{k}}}^2 \\
        \leq &  \norm{F\p{z^{k}}}^2  - \sigma\mu_{F}^{2}\p{1-\gamma^{2}L_{F}^{2}} \norm{z^{k} - \bar{z}^{k}}^{2}  \\
        = & \p{1 - \sigma\gamma^{2}\mu_{F}^{2}\p{1-\gamma^{2}L_{F}^{2}}  } \norm{F\p{z^{k}}}^2
    \end{align*}
    \end{allowdisplaybreaks}}%
    for each \(k\in\naturals\), where \Cref{State:I-FLEX:EG} in~\IFLEX{} is used in the last equality. Therefore, \(\seq{\norm{F(z^k)}}\) converges to zero since \( 1 - \sigma\gamma^{2}\mu_{F}^{2}\p{1-\gamma^{2}L_{F}^{2}}  \in (0,1)\). Since
    \begin{align*}
        \norm{z^{k} - z^{\star}} \leq \mu_{F}^{-1} \norm{F(z^{k}) - F(z^{\star})} = \mu_{F}^{-1} \norm{F(z^{k})}
    \end{align*}
    for each \(k\in\naturals\), \(\seq{z^k}\) converges strongly to \(z^{\star}\in \zer(F)\). 
\end{proof}

\subsection{Proofs regarding~\ProxFLEX}

\begin{proof}[Proof of \Cref{thm:ProxFLEX}.]
    Set \(\tau_{k} = 1\) for the iterations when the condition in \Cref{State:Prox-FLEX:contraction} in~\ProxFLEX{} is true and let \(z^{\star}\in\zer \p{F + \partial g}\). Then~\eqref{eq:zk_quasi_fejer} in \Cref{lem:zk_quasi_fejer} and {\cite[Lemma 5.31]{bauschke2017convexanalysismonotone}} imply that \(\seq{\norm{z^k-z^\star}}\) converges. Thus, the proof is complete if we can show that weak sequential cluster points of \(\seq{z^{k}}\) belong to \(\zer\p{F+\partial g}\), due to {\cite[Lemma 2.47]{bauschke2017convexanalysismonotone}}. 
    
    For this, it suffices to show that \(\seq{\norm{\bar{z}^{k}-z^{k}}}\) converges to zero. Indeed, suppose that \(\p{z^{k}}_{k\in K}\rightharpoonup z^{\infty}\) for some \(z^{\infty} \in \calH\) and \(\seq{\norm{\bar{z}^{k}-z^{k}}}\) converges to zero. Then \(\p{\bar{z}^{k}}_{k\in K}\rightharpoonup z^{\infty}\). Moreover, the proximal evaluation in \Cref{State:Prox-FLEX:EG:1} in~\ProxFLEX{} can equivalently be written as 
    \begin{align}\label{Prox-FLEX:EG:1:rewritten}
        \gamma^{-1}\p{z^{k}- \bar{z}^{k} } - F\p{z^{k}} + F\p{\bar{z}^{k}} \in \p{F + \partial g}\p{\bar{z}^{k}}.
    \end{align}
    The left-hand side of~\eqref{Prox-FLEX:EG:1:rewritten} converges strongly to zero since \(F\) is continuous and \((\norm{z^{k}-\bar{z}^{k}})_{k\in\naturals}\) converges to zero. Moreover, the operator \(F + \partial g\) is maximally monotone, since \(F\) is maximally monotone (by continuity and monotonicity~\cite[Corollary 20.28]{bauschke2017convexanalysismonotone}), \(\partial g\) is maximally monotone~\cite[Theorem 20.48]{bauschke2017convexanalysismonotone}, and \(F\) has full domain~\cite[Corollary 25.5]{bauschke2017convexanalysismonotone}. Thus,~\cite[Proposition 20.38]{bauschke2017convexanalysismonotone} gives that \(z^{\infty} \in \zer\p{F + \partial g}\), and by~\cite[Lemma 2.47]{bauschke2017convexanalysismonotone} we conclude that \(\p{z^{k}}_{k\in\naturals}\) converges weakly to a point in \(\zer\p{F + \partial g}\).

    It remains to show that \(\seq{\norm{\bar{z}^{k}-z^{k}}}\) converges to zero, which we do by showing that \(\seq{\mathcal{V}_{k}}\) converges to zero and applying \Cref{prop:V_performance_measure:lower_bound}. Let  \(K_{<1} = \set{k\in \naturals \mid \tau_k < 1} \). Suppose that \(\abs{K_{<1}} < \infty\). Then \(\V_{k+1} \leq \rho^{2}\V_{k}\) for each \(k \in \naturals\) such that \(k > \max K_{<1}\), and \(\seq{\V_{k}}\) converges to zero since \(\rho \in (0,1)\). On the contrary, suppose that \(\abs{K_{<1}} = \infty\). Let \(\Gamma : K_{<1} \to K_{<1}\) such that \(\Gamma(k) = \min\set{i \in K_{<1} \mid k < i } \) for each \(k\in K_{<1}\). Let \(k\in K_{<1}\), and notice that \(\tau_k \leq \bar{\tau}\) for any such index, where \(\bar{\tau} = \max \set{ \beta^{i} \mid i \in \llbracket 1 , M \rrbracket}\cup\set{0}<1\). Inductively summing~\eqref{eq:zk_quasi_fejer} in \Cref{lem:zk_quasi_fejer} from \(k\) to \(\Gamma(k)-1\) gives
    \begin{align}\label{eq:Prox-FLEX:zk_quasi_fejer:sum}
        \norm{z^{\Gamma(k)} - z^\star}^2 
        \leq& 
        \norm{z^k-z^\star}^2
        - (1- \bar{\tau})\alpha\p{\gamma, L_F} \V_k +  \sum_{i=k}^{\Gamma(k)-1}\varepsilon_i, 
    \end{align}
    where we used the fact that \(\tau_i = 1\) for any \(i \in K_{1}\). Inductively summing over all \(k \in K_{<1}\) in~\eqref{eq:Prox-FLEX:zk_quasi_fejer:sum}, rearranging, and dividing by \((1- \bar{\tau})\alpha\p{\gamma, L_F}>0\) gives 
    {\begin{allowdisplaybreaks}
    \begin{align} \notag
        \sum_{k\in K_{<1}}  \V_{k} \leq{}&
        \frac{\sum_{k\in K_{<1}} \p{ \norm{z^k-z^\star}^2 - \norm{z^{\Gamma(k)} - z^\star}^2 +  \sum_{i=k}^{\Gamma(k)-1}\varepsilon_i  } }{(1- \bar{\tau})\alpha\p{\gamma, L_F}} \\ \label{eq:Prox-FLEX:partial_F_sum_bounded}
        \leq{}&
        \frac{\norm{z^{\min(K_{<1}) }-z^\star}^2 + \sum_{k=0}^{\infty} \varepsilon_k  }{(1- \bar{\tau})\alpha\p{\gamma, L_F}} < \infty,
    \end{align}
    \end{allowdisplaybreaks}}%
    where summability of \(\seq{\varepsilon_k}\) is used in the last inequality. Note that 
    {\begin{allowdisplaybreaks}
    \begin{align*}
        \sum_{k=0}^{\infty} \V_{k} 
        &= \sum_{k\in K_{<1}} \sum_{i=k}^{\Gamma(k)-1} \V_{i} \\
        & \leq\sum_{k\in K_{<1}} \sum_{i=k}^{\Gamma(k)-1} \rho^{2(i - k)}\V_{k} \\
        & \leq \frac1{1-\rho^{2}}\sum_{k\in K_{<1}}  \V_{k}
        < \infty,
    \end{align*}
    \end{allowdisplaybreaks}}%
    where \Cref{State:Prox-FLEX:contraction} in~\ProxFLEX{} is used in the first inequality, the expression for the geometric series is used in the second inequality, and~\eqref{eq:Prox-FLEX:partial_F_sum_bounded} is used in the last inequality. This completes the proof. 
\end{proof}

==> extragradient/TeX/Text/iflex.tex <==
As highlighted in \Cref{rem:FLEX:LS:bad_case}, since \(\|F(z^k) - F(\bar{z}^k)\| = 0\) can occur without reaching a solution, special considerations are necessary. In~\FLEX, this is addressed by employing an explicit finite termination in the line-search procedure and assuming that the directions \(d^{k}\) are summable. However, when the operator \(F\) is injective, it is possible to exploit the Lyapunov inequality in~\eqref{eq:EG:new_Lyapunov_w.o._sol:g_zero} directly to establish convergence results without additional assumptions. To this end, we introduce~\IFLEX{}, which incorporates a more traditional line-search procedure similar to that used in~\cite[Algorithm \texttt{PANOC}]{stella2017simpleefficientalgorithm}. However, the \texttt{PANOC} algorithm is developed for minimization problems and utilizes a fundamentally different Lyapunov function. Importantly,~\IFLEX{} uses an infinite backtracking strategy with guaranteed finite termination since injectivity ensures that \(\|F(z^k) - F(\bar{z}^k)\| = 0\) only when a solution has been found. Moreover,~\IFLEX{} has two fewer parameters than~\FLEX, simplifying its implementation. \new{Note that the computation of \(w^{k}\) in \Cref{State:I-FLEX:EG} in~\IFLEX{} can be deferred to the case in which \(\tau_{k}=1\) in \eqref{eq:I-FLEX:descent} fails, saving some computations.}

\input{TeX/Algs/I-FLEX}

\begin{proposition}\label{prop:IFLEX:well_defined}
    Suppose that \Cref{ass:F} holds and \(F\) is injective. Then, independent of the choice of the direction \(d^{k}\) in \Cref{State:I-FLEX:dk} of~\refIFLEX{}, either there exists an iteration \(k\in\naturals\) such that \(z^{k}\in\zer\p{F}\) or the line search in \Cref{State:I-FLEX:LS} is well-defined for each iteration \(k\in\naturals\).
    \begin{proof}
        Follows from \(\sigma \in (0,1)\),~\eqref{eq:EG:new_Lyapunov_w.o._sol:g_zero}, continuity of \(F\), and that \(\norm{F\p{z^{k}}-F\p{\bar{z}^{k}}}\neq 0\) if and only if \(z^{k} \notin \zer\p{F}\).  
    \end{proof}
\end{proposition}

\begin{theorem}\label{thm:IFLEX}
    Suppose that \Cref{ass:F} holds,  \(\zer \p{F}\neq \emptyset\), and the sequence \(\p{z^{k}}_{k\in\naturals}\) is generated by~\refIFLEX. 
    \begin{thmenumerate}

        \item \label{thm:I-FLEX:injective} If \(F\) is injective and weakly continuous, then each weak sequential cluster point of  \(\seq{z^k}\) is in \(\zer \p{F}\). 

        \item \label{thm:I-FLEX:dk_bounded} If \(F\) is injective and weakly continuous, and \(\seq{d^k}\in\ell^{1}(\naturals;\,\calH)\), then \(\seq{z^k}\) converges weakly to some point in \(\zer \p{F}\). 

        \item \label{thm:I-FLEX:F_unifrom} If \(F\) is uniformly monotone, then \(\seq{z^k}\) converges weakly to some point in \(\zer \p{F}\).
        
        \item \label{thm:I-FLEX:F_strongly} If there exists \(0<\mu_F\leq L_F\) such that \(\mu_F \norm{x - y}\leq\norm{F\p{x}- F\p{y}}\) for each \(x,y\in \calH\), then \(\seq{z^k}\) converges strongly to some point in \(\zer \p{F}\) and
        \begin{align}\label{eq:IFLEX:F_strongly:linear}
            \norm{F(z^{k+1})}^2 \leq 
            \smash{\underbracket{
            \p{1-\sigma\gamma^{2}\mu_{F}^{2}\p{1-\gamma^{2}L_{F}^{2}}} 
            }_{\in(0,1)}}
            \norm{F(z^{k})}^2
        \end{align}
        for each \(k\in\naturals\).
    \end{thmenumerate}
\end{theorem}



==> extragradient/TeX/Text/introduction.tex <==
%!TEX root = ../../main_arxiv.tex
\section{Introduction}\label{sec:introduction}
In this work, we consider the inclusion problem
\begin{align}\label{eq:the_inclusion_problem}
\text{find}\  z\in\calH\ \text{ such that }\ 0 \in F(z) + \partial g(z),
\end{align}
where \(F:\calH\to\calH\) is monotone and \(L_{F}\)-Lipschitz continuous for some \(L_{F}\in\reals_{++}\), \(g:\calH\to \reals \cup \{+\infty\}\) is a proper, convex, and lower semicontinuous function, and \((\calH,\inner{\cdot}{\cdot})\) is a real Hilbert space. Inclusion problems of the form~\eqref{eq:the_inclusion_problem} are known as \emph{hemivariational inequalities}~\cite{monteiro2011complexityvariantstsengs} or \emph{(mixed) variational inequalities}~\cite{malitsky2020goldenratioalgorithms,noor1990mixedvariationalinequalities}, and frequently arise in fundamental mathematical programming problems—either directly or through reformulation—including minimization, saddle-point, complementarity, Nash equilibrium, and fixed-point problems~\cite{bauschke2017convexanalysismonotone,facchinei2004finitedimensionalvariationalI}. The most common methods for solving~\eqref{eq:the_inclusion_problem} belong to the large class of extragradient-type methods~\cite{korpelevich1976extragradientmethodfinding,popov1980modificationarrowhurwicz,tseng2000modifiedforwardbackward}. For a recent review, see~\cite{trandinh2024revisitingextragradienttype,trandinh2025acceleratedextragradienttype}. Among these methods, the first and most widely recognized is Korpelevich's extragradient method~\cite{korpelevich1976extragradientmethodfinding}. Although originally proposed for the constrained case in which \(g\) is the indicator function of a nonempty, closed, and convex set, the method also applies to the more general setting in~\eqref{eq:the_inclusion_problem}. Specifically, given an initial point \(z^0\in \calH\) and a step-size parameter \(\gamma \in (0,1/L_{F})\), its iterations are given by
\begin{subequations}\label{alg:EG}
    \begin{align}\label{alg:EG:1}
        \bar{z}^{k}
        ={}&
        \prox_{\gamma g}\left(z^{k} - \gamma F(z^{k})\right), 
        \\ \label{alg:EG:2}
        z^{k+1} 
        ={}& \prox_{\gamma g}\left(z^{k} - \gamma F(\bar{z}^{k})\right)
    \end{align}
\end{subequations}
for each \(k\in\naturals\). A popular alternative is Tseng's forward-backward-forward method~\cite{tseng2000modifiedforwardbackward}, given by
\begin{subequations}\label{alg:Tseng}
    \begin{align}
        \bar{z}^{k} {} = {} \prox_{\gamma g}\left(z^{k} - \gamma F(z^{k})\right), \\
        z^{k+1} {} = {} \bar{z}^{k} + \gamma \p{ F\p{z^{k} } -F\p{\bar{z}^{k}} }
    \end{align}
\end{subequations}
for each \(k\in\naturals\), that requires one less evaluation of the proximal operator \(\prox_{\gamma g}\) per iteration. Classically, the convergence analyses of these methods rely on Fej\'er-type arguments~\cite{korpelevich1976extragradientmethodfinding, tseng2000modifiedforwardbackward}.

In this work, we propose an analysis centered around the Lyapunov function
\begin{align*}      
    \V\p{z^{k},\bar{z}^{k},z^{k+1}} 
    = 2\gamma^{-1}\inner{z^{k} - z^{k+1}}{F\p{z^{k}} - F\p{\bar{z}^{k}}}
    + \gamma^{-2}\norm{z^{k+1} - \bar{z}^{k}}^{2}
    + \gamma^{-2}\norm{z^{k} - z^{k+1}}^{2}.
\end{align*}
For the extragradient method, \(\V_k\) serves as a nonnegative optimality measure for the inclusion problem~\eqref{eq:the_inclusion_problem} as shown in \Cref{prop:V_performance_measure}. \new{Likewise, \(\V_k\) is a nonnegative optimality measure for Tseng's method, since the Lyapunov function reduces to \(\V_k = \gamma^{-2}\norm{z^{k} - \bar{z}^{k}}^{2}\) in this case.} In the particular case when \(g = 0\), both methods are identical, and the Lyapunov function reduces to \(\V_k=\|F(z^k)\|^2\).

Besides being an optimality measure, we show in \Cref{thm:EG:new_Lyapunov_w.o._sol} that \(\V_k\) satisfies a descent inequality for the extragradient method. Moreover, \new{for the extragradient method}, we show a Fejér-type inequality in which \(\V_k\) appears as the residual term (see \Cref{thm:EG:primal_descent_for_V}). \new{By combining this result with the descent property, we establish a \(o(1/k)\) last-iterate convergence rate for \(\V_k\) for the extragradient method, as shown in \Cref{cor:lastiter:T}.} \new{In \Cref{sec:comparison}, we show that \(\V_k\) upper bounds some common optimality measures used to judge the quality of approximate solutions for \eqref{eq:the_inclusion_problem}; hence, together with \Cref{cor:lastiter:T}, the same last-iterate convergence result automatically holds for each of those measures as well. Taken together, the results we obtain for $\V_k$ enable us to recover and, in some cases, extend recent last-iterate convergence-rate results for the extragradient method (cf. \cite[Theorem 3.3]{gorbunov2022extragradientmethodo1/k}, \cite[Theorem 3]{cai2022tightlastiterateconvergenceextragradient}, and \cite[Corollary 4.1]{trandinh2024revisitingextragradienttype}).}

\new{Interestingly, \Cref{thm:EG:new_Lyapunov_w.o._sol} is particular to Korpelevich's extragradient method.} We demonstrate through a simple counterexample in \Cref{ex:counterexample:tseng} that the descent inequality in terms of \(\V_k\) fails for Tseng's method. Moreover, even for the extragradient method, it is crucial to leverage the specific structure of~\eqref{eq:the_inclusion_problem}. Indeed, the claimed descent inequality fails, and even the convergence of the method does not hold if we replace \(\partial g\) with a maximally monotone operator \(T:\calH\to 2^{\calH}\) and correspondingly the proximal operators \(\prox_{\gamma g}\) in~\eqref{alg:EG} with the resolvent \(\p{\Id + \gamma T}^{-1}\). This broader setting is ruled out by a counterexample presented in \Cref{ex:counterexample:full_eg}. \new{However, if \(T\) is also  3-cyclically monotone (see \cite[Definition 22.13]{bauschke2017convexanalysismonotone}), then \Cref{thm:EG:new_Lyapunov_w.o._sol,thm:EG:primal_descent_for_V} (and therefore also \Cref{cor:lastiter:T}) remain valid; see \Cref{rmk:cyclically_monotone} for details.}





The second objective of this work is to develop flexible extragradient-type schemes that accommodate fast local directions while maintaining global convergence. In this regard, the seminal work \cite{solodov1998globallyconvergentinexact} 
\new{proposes a hybrid method for solving monotone equations, i.e., when \(g=0\) in \eqref{eq:the_inclusion_problem}. Their scheme achieves global convergence by blending an inexact regularized Newton step with the hyperplane projection framework from \cite{solodov1999hybridapproximateextragradient}. At each iteration, a search direction is computed based on an inexact regularized Newton step. A line search is then performed along this direction, not to decrease a merit function, but to identify a hyperplane separating the current iterate from the solution set. The algorithm then proceeds by projecting the iterate onto this hyperplane. While this approach incorporates a line search, the convergence analysis still fundamentally} relies on Fej\'er-type monotonicity arguments.
 In practice, however, the projection step can undermine the effectiveness of the Newtonian directions, resulting in slower convergence.



% The second objective of this work is to develop flexible extragradient-type schemes that accommodate fast local directions while maintaining global convergence. In this regard, the seminal work~\cite{solodov1998globallyconvergentinexact} introduced an inexact regularized Newton method for solving monotone equations, i.e., when \(g=0\) in~\eqref{eq:the_inclusion_problem}. Global convergence in~\cite{solodov1998globallyconvergentinexact} is achieved through a scheme that relies on the hyperplane projection idea from~\cite{solodov1999hybridapproximateextragradient}. Specifically, an intricate line search is used to identify a hyperplane separating the current iterate from the solution set, and the method then projects onto this hyperplane to ensure global convergence. Consequently, even though a line search is performed, the convergence analysis still relies on Fejér-type techniques. In practice, however, the projection step can undermine the effectiveness of the Newtonian directions, resulting in slower convergence.

Another related work to ours is~\cite{themelis2019supermannsuperlinearlyconvergent}, which addresses the problem of finding fixed points of averaged operators. They propose a hybrid scheme accelerating many numerical algorithms under the Krasnosel'ski\u{\i}--Mann framework. Similar to~\cite{solodov1998globallyconvergentinexact}, their scheme incorporates a hyperplane projection step and achieves superlinear convergence under suitable assumptions. In addition, it allows for a general class of local directions, including quasi-Newton-type directions, providing greater flexibility in practice.

In contrast to the approaches mentioned earlier that use a line search to identify a separating hyperplane onto which the iterates are projected (see~\cite{solodov1998globallyconvergentinexact, themelis2019supermannsuperlinearlyconvergent}), our proposed schemes incorporate line search procedures grounded in our new Lyapunov analysis, directly aiming to reduce \(\V_k\).  
We introduce three flexible algorithms tailored to specific instances of problem~\eqref{eq:the_inclusion_problem}.~\refFLEX{} is introduced for finding zeros of \(F\),~\refIFLEX{} is applicable when \(F\) is injective, and~\refProxFLEX{} addresses problem~\eqref{eq:the_inclusion_problem} in its full generality. All three algorithms share the same guiding principle: at each iteration, one performs a convex combination of a standard extragradient step~\eqref{alg:EG} and a step based on a user-specified direction. The specific weighting for this convex combination is determined by the line-search procedure, ensuring sufficient descent of the optimality measure \(\V_k\). Similar to~\cite{themelis2019supermannsuperlinearlyconvergent}, our schemes accommodate a wide range of user-chosen directions, including quasi-Newton-type directions. A key feature enabling this approach is that \(\V_k\) depends solely on values computed at each iteration and does not involve a solution to~\eqref{eq:the_inclusion_problem}. This design ensures high flexibility while guaranteeing global (see \Cref{sec:algs}) and superlinear convergence (see \Cref{sec:superlinear}) when choosing suitable directions. 

Our preliminary numerical experiments indicate that using quasi-Newton directions in our proposed algorithms yields favorable performance. In particular, limited-memory type-I and type-II Anderson acceleration exhibit promising results (see \Cref{sec:numerical}). In related work,~\cite{zhang2020globallyconvergenttype} studies Anderson acceleration for finding fixed points of averaged operators, proposing a globalization strategy based on a stabilization and safeguarding mechanism—rather than a line search—that reverts to a nominal Krasnosel’ski\u{\i}–Mann step whenever the Anderson acceleration step fails to sufficiently reduce the forward residual. More recently,~\cite{qu2024extragradientanderson} introduced an extragradient-based scheme with memory-one Anderson acceleration, which reduces overhead and allows for simple, explicit updates of the directions. Furthermore,~\cite{asl2024jsymmetricquasi} presents a quasi-Newton method tailored to minimax problems. Our theory offers a direct globalization strategy for such directions, applicable in the uniformly monotone and injective settings (see \Cref{thm:IFLEX}), or whenever the resulting directions are summable (see \Cref{thm:FLEX:dk_summable}).

\subsection{Organization}\label{sec:organization}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{TeX/Text/organization.tex}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Notation and preliminaries}\label{sec:notation}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{TeX/Text/notation.tex}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> extragradient/TeX/Text/logistic.tex <==
Consider the sparse logistic regression problem
\begin{align}\label{eq:logistic_01_label}
    \minimize_{x\in\mathbb{R}^{n}}\; \sum_{i=1}^m \log\left(1 + \exp\left({-b_i a_i^{\top}x}\right)\right) + \lambda \norm{x}_{1}
\end{align}
where \((a_i,b_i) \in \mathbb{R}^n\times \{\pm 1\}\) for each \(i = 1,\dots,m\). The minimization problem~\eqref{eq:logistic_01_label} can equivalently be written as the inclusion problem \eqref{eq:the_inclusion_problem} by letting \(\calH=\reals^{n}\) with the inner product set to the dot product, \(F:\mathbb{R}^{n}\to\mathbb{R}^{n}\) such that \(F(x)=K^{\top} \sigma(Kx)\) for each \(x\in\reals^{n}\)
where
\begin{align*}
    \sigma:\mathbb{R}^{m}\to\mathbb{R}^{m}:
    \begin{bmatrix} u_1 \\ \vdots \\ u_m \end{bmatrix} 
    \mapsto 
    \begin{bmatrix} \frac{\exp(u_1)}{1+\exp(u_1)} \\ \vdots \\ \frac{\exp(u_m)}{1+\exp(u_m)} \end{bmatrix},  \quad K = 
    \begin{bmatrix}
        - b_1 a_1^{\top} \\
        \vdots  \\
        - b_m a_m^{\top} 
    \end{bmatrix}
    \in \mathbb{R}^{m\times n},
\end{align*}
and \(g = \lambda \norm{\cdot}_{1} \). Moreover, note that \Cref{ass:main} holds with \(L_F=(1/4)\norm{K}^2\). The results of the numerical experiments are presented in \Cref{fig:logistic}. Although not designed specifically for minimization problems, we observe that~\ProxFLEX{} with \texttt{AA-II} directions performs at the top in all but one problem.

\input{plots/logistic.tex}

==> extragradient/TeX/Text/notation.tex <==
Let \(\naturals\) denote the set of nonnegative integers, \(\mathbb{N}\) the set of positive integers, \(\mathbb{Z}\) the set of integers, \(\llbracket n,m \rrbracket = \set{l \in \mathbb{Z} \xmiddle| n \leq l \leq m}\) the set of integers inclusively between the integers \(n\) and \(m\),  \(\reals\) the set of real numbers, \(\reals_+\) the set of nonnegative real numbers, \(\reals_{++}\) the set of positive real numbers, \(\reals^n\) the set of all \(n\)-tuples of elements of \(\reals\), \(\reals^{m\times n}\) the set of real-valued matrices of size \(m\times n\), if \(M\in\reals^{m\times n}\) then \([M]_{i,j}\) the \(i,j\)-th element of \(M\), \(\sym^{n}\) the set of symmetric real-valued matrices of size \(n\times n\), and \(\sym_+^n\subseteq \sym^{n}\) the set of positive semidefinite real-valued matrices of size \(n\times n\). Suppose that \( 1 \leq p < +\infty \), \(K\subseteq\naturals\), and \(\mathcal{U} \subseteq \mathcal{W} \), where \(\mathcal{W}\) is a normed space. Then we define the space \( \ell^{p}\p{K;\,\mathcal{U}} = \{(u^{k})_{k\in K} \in \mathcal{U}^{K} \mid \sum_{k\in K} \norm{u^{k}}^{p} < +\infty \} \).

Throughout this paper, \((\calH,\inner{\cdot}{\cdot})\) will denote a real Hilbert space and \(\norm{\cdot}\) the canonical norm, which will be clear from the context. Let \(F:\calH\to\calH\) be an operator. Suppose that \(L_{F}\geq0\). The operator \(F\) is said to be \emph{\(L_{F}\)-Lipschitz continuous} if \(\norm{F\p{x} - F\p{y}} \leq L_{F} \norm{x-y}\) for each \(x,y\in\calH\). The operator \(F\) is said to be \emph{monotone} if \(0\leq \inner{F\p{x} - F\p{y}}{x-y}\) for each \(x,y\in\calH\). Suppose that \(\mu_{F}\geq0\). The operator \(F\) is said to be \emph{\(\mu_{F}\)-strongly monotone} if \(\mu_{F}\norm{x-y}^{2}\leq \inner{F\p{x} - F\p{y}}{x-y}\) for each \(x,y\in\calH\). Moreover, \(F\) is said to be \emph{uniformly monotone with modulus} \(\phi:\reals_{+}\to \reals_{+}\) if \(\phi\) is increasing, vanishes only at \(0\), and \(\phi\p{\norm{x-y}}\leq \inner{F\p{x} - F\p{y}}{x-y}\) for each \(x,y\in\calH\). For a general set-valued operator \(T:\calH \to 2^{\calH}\), the set of \emph{zeros} is denoted by \(\zer\p{T}=\set{x\in\calH \xmiddle| 0 \in T\p{x} }\). The Cauchy–Schwarz inequality states that \(\abs{\inner{x}{y}}\leq\norm{x}\norm{y}\) for each \(x,y\in\calH\) and Young's inequality that \(2\inner{x}{y} \leq \alpha\norm{x}^{2} + \alpha^{-1}\norm{y}^{2}\) for each \(x,y\in\calH\) and \(\alpha>0\).


Given a function \(g:\calH\rightarrow\reals\cup\{+\infty\}\), the \emph{effective domain} of \(g\) is the set \(\dom g = \{x\in\calH \mid g\p{x}<+\infty\}\). The function \(g\) is said to be \emph{proper} if \(\dom g \neq \emptyset\). The \emph{subdifferential} of a proper function \(g\) is the set-valued operator \(\partial g:\calH \rightarrow 2^{\calH}\) defined as the mapping \(x \mapsto \{u \in \calH \mid \forall y \in \calH,\, g\p{y} \geq g\p{x} + \inner{u}{y-x} \}\). The function \(g\) is said to be \emph{convex} if \(g\p{\p{1 - \lambda} x + \lambda y} \leq \p{1 - \lambda} g\p{x} + \lambda g\p{y}\) for each \(x, y \in \calH\) and \(0 \leq \lambda \leq 1\). The function \(g\) is said to be \emph{lower semicontinuous} if \(\liminf_{y\to x} g\p{y} \geq g\p{x}\) for each \(x\in\calH\). If \(C\subseteq\calH\), the \emph{indicator function of \(C\)}, denoted \(\delta_{C}:\calH \to \reals\cup\set{+\infty}\), is defined as \(\delta_{C}(x) = 0\) if \(x\in C\) and \(\delta_{C}(x) = +\infty\) if \(x\in \calH\setminus C\).

Let \(g:\calH\to \reals \cup \{+\infty\}\) be proper, convex and lower semicontinuous, and let \(\gamma>0\). Then the \emph{proximal operator} \(\prox_{\gamma g} : \calH \to \calH \) is defined as the single-valued operator given by
\begin{align*}
    \prox_{\gamma g}\p{x} = \argmin_{z\in\calH}\left(g(z) + \tfrac{1}{2\gamma}\norm{x-z}^2\right) 
\end{align*}
for each \(x\in\calH\)~\cite[Proposition 12.15]{bauschke2017convexanalysismonotone}. If \(x,p\in\calH\), then \(p = \prox_{\gamma g}\p{x}\) \(\Leftrightarrow\) \(\gamma^{-1}\p{x-p} \in \partial g\p{p}\) \(\Leftrightarrow\) \(0 \leq g\p{y} - g\p{p} - \inner{\gamma^{-1}\p{x-p}}{y-p}\) for each \(y\in\calH\)~\cite[Proposition 16.44, Proposition 16.6]{bauschke2017convexanalysismonotone}. 



==> extragradient/TeX/Text/numerical.tex <==
\section{Numerical experiments}\label{sec:numerical}
In this section, we assess the performance of the proposed algorithms in \Cref{sec:algs} through a series of simulations on standard problems using both synthetic and real-world datasets. Code to replicate the experiments is made available online.\footnote{\url{https://github.com/manuupadhyaya/flex}} \Cref{tab:algorithms} contains a description of the algorithms used. 

\begin{table}[h]
    \centering
    \caption{Algorithms used in the numerical simulations (when applicable).}
    \label{tab:algorithms}
    \begin{tabular}{@{}l p{0.7\textwidth}@{}}
        \toprule
        \textbf{Method} & \textbf{Description} \\
        \midrule
        {\algnamefont EG}      
            & Extragradient method~\eqref{alg:EG} with \(\gamma = 0.9/L_{F}\). \\
        {\algnamefont EAG-C}   
            & Extra anchored gradient with constant step size \(\alpha = 1/(8L_{F})\)~\cite[Section 2.1]{yoon2021accelerated}. \\
        {\algnamefont GRAAL}   
            & Golden ratio algorithm with \(\phi = 2\) and \(\alpha = 0.999/L_{F}\)~\cite[Algorithm 2]{alacaoglu2023beyond},~\cite{malitsky2020goldenratioalgorithms}. \\
        {\algnamefont aGRAAL}  
            & Adaptive golden ratio algorithm with \(\phi = (2 + \sqrt{5})/2 \), \(\gamma = 1 / \phi + 1 /\phi^2\) and \(\alpha_0 = 0.1\)~\cite[Algorithm 1]{alacaoglu2023beyond},~\cite{malitsky2020goldenratioalgorithms}. \\
        {\algnamefont EG-AA}   
            & An extragradient-type method with type-II Anderson acceleration with memory \(m = 1\)~\cite[Algorithm 1]{qu2024extragradientanderson} using the parameter values described in~\cite[Section 4]{qu2024extragradientanderson}. \\
        {\algnamefont FISTA}   
            & Fast iterative shrinkage-thresholding algorithm with constant step size~\cite[Section 4]{Beck_2009}. \\
        \FLEX
            &\Cref{alg:FLEX} with \(\gamma = 0.9/L_F\), \(\beta = 0.3\), \(\sigma = 0.1\), \(\rho = 0.99\), and \(M=2\). \\
        \IFLEX
            &\Cref{alg:I-FLEX} with \(\beta = 0.01\) and \(\sigma = 0.1\). \\
        \ProxFLEX
            &\Cref{alg:Prox-FLEX} with \(\gamma = 0.9/L_F\), \(\beta = 0.3\), \(\sigma = 0.1\), \(\rho = 0.99\), and \(M=2\). \\
        \bottomrule
    \end{tabular}
\end{table}

In the numerical experiments for~\FLEX{},~\IFLEX{}, and~\ProxFLEX{}, we use directions \(\seq{d^{k}}\) based on 
quasi-Newton directions. 

\paragraph{Anderson acceleration.} 

The first set of quasi-Newton directions we use are the standard limited-memory type-I and type-II Anderson acceleration methods~\cite{Anderson1965, fang2009multisecant}. These directions are computed via~\eqref{eq:direction:Rgam}, i.e., \(d^k = - H_{k} R_\gamma(z^k)\), where \(H_{k}\) differs between the type-I and type-II variants. Both methods employ a memory parameter \(m \in \mathbb{N}\) and define \(m_k = \min\{m, k\}\). They also maintain two buffer matrices:
\[
Y_k = \begin{bmatrix}
y^{k - m_k}  & \cdots & y^{k-1}
\end{bmatrix}
\quad\text{and}\quad
S_k = \begin{bmatrix}
s^{k - m_k}  & \cdots & s^{k-1}
\end{bmatrix},
\]
where \(y^i = R_\gamma(z^{i+1}) - R_\gamma(z^i)\) and \(s^i = z^{i+1} - z^i\). For type-I Anderson acceleration (denoted {\algnamefont AA-I}), we have
\[
H_k = I + (S_k - Y_k)\,(S_k^{\top}Y_k)^{-1}\,S_k^{\top},
\]
whereas for type-II Anderson acceleration (denoted {\algnamefont AA-II}), we have
\[
H_k = I + (S_k - Y_k)\,(Y_k^{\top}Y_k)^{-1}\,Y_k^{\top}.
\]
Additional discussion can be found in~\cite{zhang2020globallyconvergenttype}.

\paragraph{J-symmetric directions.} 

We also incorporate directions derived from the J-symmetric quasi-Newton approach proposed in~\cite{asl2024jsymmetricquasi}, which is developed for unconstrained minimax problems. This method exploits the so-called J-symmetric structure of the Hessian in such problems, allowing a rank-2 update of the (inverse) Hessian estimate that naturally generalizes the classic Powell's symmetric Broyden method from standard minimization to minimax optimization. The formula for updating \(H_k\) in~\eqref{eq:direction:Rgam} can be found in~\cite[Proposition 2.2]{asl2024jsymmetricquasi}. We refer to this method as {\algnamefont J-sym}.

\subsection{Quadratic minimax problem}\label{sec:quadratic_minimax}
\input{TeX/Text/quadratic_minimax}

\subsection{Bilinear zero-sum game with simplex constraints}\label{sec:bilinear}
\input{TeX/Text/bilinear}

\subsection{Cournot--Nash equilibrium problem}\label{sec:equilibrium}
\input{TeX/Text/equilibrium}

\subsection{Sparse logistic regression}\label{sec:logistic}
\input{TeX/Text/logistic}



==> extragradient/TeX/Text/organization.tex <==
In \Cref{sec:Lyapunov}, we formally introduce the new Lyapunov analysis for Korpelevich’s extragradient method. Building on this framework, we present the three new algorithms in \Cref{sec:algs} and establish their global convergence under suitable assumptions. In \Cref{sec:global}, we provide detailed proofs of the results from the preceding section. Next, \Cref{sec:superlinear} focuses on superlinear convergence, including corresponding proofs for the proposed algorithms. Numerical experiments appear in \Cref{sec:numerical}, and we conclude in \Cref{sec:conclusions} with a summary of key findings and directions for future research. \new{Finally, \Cref{app:background} offers background material on Korpelevich’s extragradient method, \Cref{app:counterexamples} presents the counterexamples mentioned earlier, and \Cref{sec:comparison} contains a comparison to recent last-iterate convergence results for the extragradient method.}

==> extragradient/TeX/Text/proxflex.tex <==
A direct generalization of~\refFLEX{} in \Cref{sec:FLEX} is provided in~\refProxFLEX{} for the case when \( g \) in~\eqref{eq:the_inclusion_problem} is nonzero. Here, the Lyapunov inequality~\eqref{eq:EG:new_Lyapunov_w.o._sol} from \Cref{thm:EG:new_Lyapunov_w.o._sol} is used to modify the standard extragradient method in~\eqref{alg:EG}; otherwise, the underlying approach remains the same. However, there is one important difference between~\FLEX{} and~\ProxFLEX{} in terms of computations required per line-search trial. The condition~\eqref{eq:FLEX:descent} in~\FLEX{} requires only one additional \(F\) evaluation per trial while condition~\eqref{eq:Prox-FLEX:descent} in~\ProxFLEX{} requires two additional \(F\) evaluations and two additional \(\prox_{\gamma g}\) evaluations per trial. Next, we present a convergence result of~\ProxFLEX.

\begin{theorem}\label{thm:ProxFLEX}
    Suppose that \Cref{ass:main} holds, \(\zer \p{F + \partial g}\neq \emptyset\), the sequence \(\p{z^{k}}_{k\in\naturals}\) is generated by~\refProxFLEX, and \(\seq{d^k}\in\ell^{1}(\naturals;\,\calH)\). Then \(\seq{z^k}\) converges weakly to some point in \(\zer \p{F+ \partial g}\).
\end{theorem}

\input{TeX/Algs/Prox-FLEX}

\begin{remark}
    \begin{enumerate}
        \item \label{rem:strength:proxflex} If \(F\) is \(\mu_{F}\)-strongly monotone, then the Lyapunov inequality~\eqref{eq:EG:new_Lyapunov_w.o._sol} in \Cref{thm:EG:new_Lyapunov_w.o._sol} can be strengthened to include the additional term \(-2\gamma^{-1}\mu_{F}\norm{z^{k+1} - z^{k} }^2\) in the right-hand side; this follows from using strong monotonicity of \(F\) instead of monotonicity of \(F\) in the first inequality in~\eqref{eq:innerprod:vk+:ub}. This observation suggests that the line-search condition~\eqref{eq:Prox-FLEX:descent} in~\ProxFLEX{} can be replaced by
        \begin{align}\notag
            \V(z^{k+1}, \bar{z}^{k+1}, w^{k+1}) 
            \leq{}& \V(z^k, \bar z^k, w^{k}) - \sigma\p{1-\gamma^{2}L_{F}^{2}}\gamma^{-2} \norm{w^{k}-\bar{z}^{k}}^{2} \\\label{eq:Prox-FLEX:descent:strongly}
            &{}-2\gamma^{-1}\sigma\mu_{F}\norm{w^{k} - z^{k} }^2.
        \end{align}
        Note that using Young's inequality, we get 
        \begin{align}\label{eq:V:upper_bound}
            \V(z^k, \bar z^k, w^{k}) \leq \p{2\gamma^{-1} + \gamma^{-1} L_{F} + \gamma^{-2}}\norm{w^{k} - z^{k}}^{2} + \p{\gamma^{-1} L_{F} + \gamma^{-2}}\norm{w^{k} - \bar{z}^{k}}^{2}.
        \end{align}
        Combining~\eqref{eq:Prox-FLEX:descent:strongly},~\eqref{eq:V:upper_bound} and \Cref{State:Prox-FLEX:contraction} in~\ProxFLEX{} gives 
        \begin{align*}
            \V(z^{k+1}, \bar{z}^{k+1}, w^{k+1}) \leq{}& 
            \underbracket{
             \max\left(\rho^2 ,1 - \frac{\sigma \min\p{(1-\gamma^{2}L_{F}^{2}) , 2\gamma\mu_{F}}}{2\gamma + \gamma L_{F} + 1} \right)
             }_{\in(0,1)}
             \V(z^k, \bar z^k, w^{k})
        \end{align*}
        for each \(k\in\naturals\), i.e. \(\seq{\V(z^k, \bar z^k, w^{k})}\) converges at least \(Q\)-linearly to zero. However, the resulting line-search condition is not always actionable since \(\mu_{F}\) may not be known in many practical problems. Therefore, we have chosen not to consider the strongly monotone case further. 
        
        \item Similar to~\IFLEX{},~\ProxFLEX{} can be modified to perform infinite backtracking on~\eqref{eq:Prox-FLEX:descent} with guaranteed finite termination, even without the strengthened line-search condition described above in \Cref{rem:strength:proxflex}. 
        This modification requires \(\norm{w^k-\bar{z}^k}\) to be an optimality measure, which holds when both \(F\) and \(\prox_{\gamma g}\) are injective. However, since \(\prox_{\gamma g}\) is rarely injective in practical applications, we omit this modification from our analysis.
    \end{enumerate}
\end{remark}


==> extragradient/TeX/Text/quadratic_minimax.tex <==
Consider the quadratic convex-concave minimax problem 
\begin{align}\label{eq:quadratic_minimax}
    \minimize_{x \in \reals^n}\; \maximize_{y \in \reals^n}\; \mathcal{L}\p{x,y}
\end{align}
for the saddle function \(\mathcal{L}:\reals^{n}\times\reals^{n}\to\reals\) such that 
\begin{align*}
    \mathcal{L}\p{x,y} = \tfrac{1}{2}\p{x - x^{\star}}^{\top} A \p{x - x^{\star}} + \p{x - x^{\star}}^{\top} C \p{y - y^{\star}} - \tfrac{1}{2}\p{y - y^{\star}}^{\top} B \p{y - y^{\star}}
\end{align*}
for each \(\p{x,y} \in \reals^{n}\times\reals^{n}\), where \(x^{\star},\,y^{\star} \in \reals^{n}\), \(A,\, B \in \sym_{+}^{n}\), and \(C\in\reals^{n\times n}\). A solution to the minimax problem~\eqref{eq:quadratic_minimax} can be obtained by solving an associated saddle point problem, which in turn can equivalently be written as~\eqref{eq:the_inclusion_problem} by letting \(\calH=\reals^{2n}\) with the inner product set to the dot product, \(g=0\), and \(F: \reals^{2n}\to\reals^{2n}\) as the monotone and \(L_F\)-Lipschitz continuous operator given by
\begin{align}\label{eq:quadratic_minimax:F}
    F(z) = 
    \begin{bmatrix}
        \nabla_{x} \mathcal{L}\p{x,y} \\
        -\nabla_{y} \mathcal{L}\p{x,y} 
    \end{bmatrix}
    =
    \begin{bmatrix}
        A \p{x - x^{\star}} + C\p{y - y^{\star}} \\
        B \p{y - y^{\star}} - C^{\top}\p{x - x^{\star}}
    \end{bmatrix}
\end{align}
for each \(z = (x,y)\in \reals^{n} \times \reals^{n}\), where\footnote{The matrix norm is taken as the spectral norm.}
\begin{align*}
    L_{F} = 
    \left\lVert 
    \begin{bmatrix}
        A &  C \\
        - C^{\top} & B
    \end{bmatrix}
    \right\rVert.
\end{align*}
We generate problem data as in \cite[Section 5.1]{asl2024jsymmetricquasi}, which is outlined below. The results of the numerical experiments are presented in \Cref{fig:qmp}. We see that~\FLEX{} and~\IFLEX{} do very well for small problems, while larger ones are more challenging. Nevertheless, the use of \texttt{AA-II} directions in our algorithms systematically performs at the top.

\input{TeX/Algs/minimax_data_generation}

\input{plots/quadratic_minimax}


==> extragradient/TeX/Text/superlinear.tex <==
%!TEX root = ../../main_arxiv.tex
\section{Superlinear convergence}\label{sec:superlinear}
The convergence analyses presented so far have been blind to the choice of directions \(\seq{d^k}\); nevertheless, attaining a fast convergence rate relies on their precise choice. This section presents a minimal set of assumptions on the directions that ensure superlinear convergence. Our main focus will be on quasi-Newton-type directions that are computed as 
\begin{equation}\label{eq:direction:Rgam}
    d^k = - H_{k} R_\gamma(z^k),\quad \text{where} \quad R_\gamma  = \tfrac1{\gamma} \p{\Id - \prox_{\gamma g} \circ \p{\Id - \gamma F} },
\end{equation}
\(\gamma\in\reals_{++}\), \(H_{k}:\calH\to\calH\) is a linear operator encapsulating information of the geometry of the residual mapping \(R_\gamma\) at \(z^k\), and \(F\) and \(g\) satisfy \Cref{ass:main}. The specific way \(H_k\) is computed determines the underlying quasi-Newton method (see \Cref{sec:numerical} for details). Notice that the zeros of \(R_\gamma\) coincide with the set of solutions of~\eqref{eq:the_inclusion_problem}. Moreover, when \(g = 0\), \(R_\gamma\) reduces to \(F\), and the directions are given by \(d^k = - H_{k} F(z^k)\). The following assumption on the directions \(\seq{d^k}\) can be seen as a boundedness assumption on the linear operators \(\seq{H_k}\). However, note that the assumption applies to directions beyond the ones given in~\eqref{eq:direction:Rgam}. 

\begin{assumption}\label{ass:dk:bound}%
    The sequence of directions \(\seq{d^k}\) used in~\FLEX{},~\IFLEX{}, or~\ProxFLEX{} satisfies \( \norm{d^k} \leq D \norm{R_\gamma(z^k)} \) for each \(k\in\naturals\) such that \(k \geq K\), for some constants \(D \geq 0\) and \(K \in \naturals\), where \(R_\gamma\) denotes the residual operator as defined in~\eqref{eq:direction:Rgam} (the function \(g\) is set to zero in the particular cases of~\FLEX{} and~\IFLEX).
\end{assumption}

\Cref{ass:dk:bound} is a natural assumption for directions defined in~\eqref{eq:direction:Rgam}. For example, under suitable regularity conditions for regularized Newton directions—specifically when \(g=0\)—we demonstrate this in \Cref{prop:dk_Newton}. Note that in \Cref{prop:dk_Newton}, we assume that \(F\) is continuously Fréchet differentiable; however, this assumption is made solely for illustrative purposes and is not required elsewhere in the paper. \Cref{ass:dk:bound} has also been utilized in the context of minimization and in finding zeros of nonexpansive maps, as seen in~\cite[Theorem 5.7.A3]{ahookhosh2021bregmanforwardbackward} and~\cite[Assumption 2]{themelis2019supermannsuperlinearlyconvergent}, respectively.

\begin{proposition}\label{prop:dk_Newton}  
    Let \(F:\calH\to \calH\) be monotone and continuously Fr\'echet differentiable, and suppose that the Fr\'echet derivative \(\mathsf{D} F\) at \(z^\star \in \zer\p{F}\) is left invertible. 
    Suppose that \(\seq{z^k},\seq{d^k}\in\calH^{\naturals}\) are such that
    \begin{equation}\label{eq:reg_Newton_dir}
        \p{r_k\Id + \mathsf{D} F(z^k)}d^k = - F(z^k)
    \end{equation}
    for some sequence \(\seq{r_k} \in \reals_{++}^{\naturals}\), and that \(\seq{z^k}\) converges strongly to \(z^\star\). Then, \Cref{ass:dk:bound} is satisfied with \(g =0\). 
    \begin{proof}
        Let \(t>0\) and note that
        \begin{align}\label{eq:DF:monotone}
            0 \leq \frac{\inner{ F(z + t v) - F(z)}{ z + t v - z } }{t^2} \xrightarrow[t	\downarrow 0]{} \inner{ \mathsf{D} F(z)v}{ v }
        \end{align}
        for any \(v\in \calH\) and for any \(z \in \calH\), by monotonicity of \(F\). This implies that the bounded linear operator  \(r_k\Id + \mathsf{D} F(z^k)\) is \(r_k\)-strongly monotone, and therefore invertible for each \(k \in \naturals\). This, in turn, ensures that the regularized Newton update~\eqref{eq:reg_Newton_dir} is well-defined, i.e., \(d^{k}\) is uniquely defined at each iteration.
        
        Moreover, since \(\mathsf{D} F(z^\star)\) is left invertible, there exists \(c_1>0\) such that \(\norm{\textstyle\mathsf{D} F(z^\star) v} \geq c_1\norm{v}\) for any \(v\in \calH\)~\cite[Proposition 10.29]{axler2020measureintegration}. This observation combined with \(z^k \to z^\star\) and continuity of \(\mathsf{D} F(\cdot)\) implies that there exists \(c_2 >0\) and \(K\in\naturals\) such that \(\norm{\mathsf{D} F(z^k) v} \geq c_2\norm{v}\) for any \(v\in \calH\) and for any \(k\geq K\). Therefore, 
        {\begin{allowdisplaybreaks}
        \begin{align*}
           \norm{F(z^k)}^{2} {}={}&  \norm{r_k\Id + \mathsf{D} F(z^k)d^k}^2 \\
           {}={}& \norm{r_k d^k}^2 + 2r_k \inner{ \mathsf{D} F(z^k)d^k}{ d^k} + \norm{\mathsf{D} F(z^k)d^k}^2 \\
            {}\geq{}& \norm{\mathsf{D} F(z^k)d^k}^2 \\
            {}\geq{}& c_2^2\norm{d^k}^2
        \end{align*}
        \end{allowdisplaybreaks}}%
        for each \(k\geq K\), where the first inequality follows from~\eqref{eq:DF:monotone} and \(r_k>0\). This establishes that \Cref{ass:dk:bound} is satisfied with \(D = 1/c_2\), when \(g=0\). 
    \end{proof}        
\end{proposition}

\begin{remark}
    In the case of~\FLEX, when the operator is strongly monotone, the sequence \(\seq{\norm{F(z^k)}}\) converges \(Q\)-linearly to zero, as established in \Cref{thm:FLEX:F_strongly}. This observation, combined with \Cref{ass:dk:bound} is sufficient to conclude that \(\seq{d^k} \in \ell^1(\naturals;\,\calH)\), thereby yielding global convergence as demonstrated in \Cref{thm:FLEX:dk_summable}. An analogous argument extends to~\ProxFLEX{} after incorporating the strengthening discussed in \Cref{rem:strength:proxflex}.
\end{remark}

We proceed to quantify the quality of the directions used in the algorithms that guarantee fast convergence. The classical condition of~\cite[Chapter 7.5]{facchinei2004finitedimensionalvariationalII} for Newton-type methods identifies a sequence of directions \(\seq{d^k}\) relative to a sequence \(\seq{z^k}\) converging to \(z^\star\) as superlinear if 
\begin{equation}\label{eq:Suplin:Facchinei}
        \lim_{k\to \infty} \frac{\norm{z^k + d^k - z^\star}}{\norm{z^k - z^\star}} = 0.
\end{equation}
This notion a priori assumes the convergence of the sequence \(\seq{z^k}\). Here, we use a slightly refined notion and define superlinear directions similar to~\cite[Definition VI.2]{themelis2019supermannsuperlinearlyconvergent}. 
\begin{definition}\label{def:superlin}%
    Suppose that \(\gamma\in\reals_{++}\), \((z^k)_{k\in\N}, (d^k)_{k\in\N} \in \calH^{\naturals}\), \Cref{ass:main} holds, \(T_1^{\gamma}\) and \(T_2^{\gamma}\) are the algorithmic operators defined in~\eqref{eq:T1T2}, and \(\V\) is the Lyapunov function given in~\eqref{eq:V}. Then we say that the sequence of directions \((d^k)_{k\in\N}\) is \emph{superlinear relative to} \((z^k)_{k\in\N}\) if 
    \begin{equation}\label{eq:dir:superlin}
        \lim_{k\to\infty}\frac{\V(z^k+d^k, T_1^\gamma(z^k+d^k), T_2^\gamma(z^k+d^k))}{\V(z^k, T_1^\gamma(z^k), T_2^\gamma(z^k))} = 0.
    \end{equation}
\end{definition}

In the case of solving monotone equations where \(g = 0\), addressed by~\FLEX{} and~\IFLEX{},~\eqref{eq:dir:superlin} reduces to 
\begin{equation}\label{def:eq:dir:superlin:F}
    \lim_{k\to\infty}{\frac{\norm{F(z^k + d^k)}}{\norm{F(z^k)}}} = 0.
\end{equation}
\new{This condition is closely related to the classical Dennis-Mor\'e assumption \cite{dennis1977quasinewtonmethods}. Specifically, when \(F\) is strictly differentiable at its zeros, the Dennis-Mor\'e assumption implies \eqref{def:eq:dir:superlin:F}, as shown in \cite[Theorem VI.7]{themelis2019supermannsuperlinearlyconvergent}. In particular, the condition is satisfied by Broyden’s method under mild regularity assumptions at the limit points \cite[Theorem VI.8]{themelis2019supermannsuperlinearlyconvergent}. 
}

 \begin{remark}\label{rem:superlin:DM}
     The superlinear convergence results presented in \Cref{thm:suplin} also hold under~\eqref{eq:Suplin:Facchinei} of~\cite{facchinei2004finitedimensionalvariationalII} since it implies the notion in \Cref{def:superlin}. Indeed, by \Cref{ass:dk:bound}
     {\begin{allowdisplaybreaks}
    \begin{align*}
        \norm{d^k}^2 
        \leq{}&
        D^2 \left(\norm{z^k - T_2^\gamma(z^k)} + \norm{T_2^\gamma(z^k) - T_1^\gamma(z^k)} \right)^2
        \\
        \leq{}&
        2D^2 \left(\norm{z^k - T_2^\gamma(z^k)}^2 + \norm{T_2^\gamma(z^k) - T_1^\gamma(z^k)}^2 \right) \\
        \leq{}& \frac{2\gamma^2D^2}{1-\gamma L_F} \V(z^k, T_1^\gamma(z^k), T_2^\gamma(z^k))
    \end{align*}
    \end{allowdisplaybreaks}}%
    for each \(k\in\naturals\) such that \(k \geq K\), where the triangle inequality is used in the first inequality and \Cref{prop:V_performance_measure:lower_bound} is used in the last inequality. Hence
    \begin{align}\label{eq:superlinear:ineq}
        \frac{\V(z^k+d^k, T_1^\gamma(z^k+d^k), T_2^\gamma(z^k+d^k))}{\V(z^k, T_1^\gamma(z^k), T_2^\gamma(z^k))}
        {}\leq{}  
        \frac{2\gamma^2D^2}{(1-\gamma L_F)\alpha\p{\gamma, \LF}}
        \frac{\norm{z^k+d^k - z^\star}^2}{\norm{d^k}},
    \end{align}
    for each \(k\in\naturals\) such that \(k \geq K\), where 
    \(\V(z^k+d^k, T_1^\gamma(z^k+d^k), T_2^\gamma(z^k+d^k)) \leq \norm{z^k+d^k - z^\star}^2/ \alpha\p{\gamma, L_F} \) is used (see \Cref{thm:EG:primal_descent_for_V}). Combining~\eqref{eq:superlinear:ineq} with~\eqref{eq:Suplin:Facchinei} and the fact that \(\lim_{k \to \infty} \norm{z^k - z^\star}/\norm{d^k} = 1\) (see~\cite[Lemmma 7.5.7]{facchinei2004finitedimensionalvariationalII}) shows that the ratio on the left-hand-side of~\eqref{eq:superlinear:ineq} vanishes. Therefore,~\eqref{eq:dir:superlin} is a weaker condition than~\eqref{eq:Suplin:Facchinei} under \Cref{ass:dk:bound}. We also refer the reader to~\cite{facchinei2004finitedimensionalvariationalII} for further details.
 \end{remark}

\new{As shown below in \Cref{thm:suplin:summable}, \Cref{def:superlin} in conjunction with \Cref{ass:dk:bound} is sufficient to conclude \(\seq{d^k}\in\ell^{1}(\naturals;\,\calH)\), establishing global weak sequential convergence by \Cref{thm:ProxFLEX}. See also \Cref{thm:FLEX:dk_summable,thm:I-FLEX:dk_bounded} for~\FLEX{} and~\IFLEX, respectively.}

\begin{theorem}\label{thm:suplin}
Suppose that \Cref{ass:main} and \Cref{ass:dk:bound} hold, \(\zer\p{F + \partial g }\neq \emptyset\),  \(T_1^{\gamma}\) and \(T_2^{\gamma}\) are the algorithmic operators defined in~\eqref{eq:T1T2}, \(\V\) is the Lyapunov function given in~\eqref{eq:V}, and \(\seq{d^k}\) is superlinear relative to the sequence \(\seq{z^k}\) generated by either~\refFLEX{},~\refIFLEX{}, or~\refProxFLEX{}. 
Then, the following hold. 
\begin{thmenumerate}
      \item \label{thm:suplin:full_accepted}  \(z^{k+1} = z^k + d^k\) for all \(k\in\naturals\) sufficiently large. 
      \item \label{thm:suplin:Q_superlinear} \(\seq{\V(z^k, T_1^\gamma(z^k), T_2^\gamma(z^k))}\) converges to zero at least \(Q\)-superlinearly.  
      \item \label{thm:suplin:summable} \(\seq{d^k}\in\ell^{1}(\naturals;\,\calH)\) with \(\seq{d^k}\) converging to zero at least \(R\)-superlinearly.  
      \item \label{thm:suplin:R_superlinear} If \(\dim \calH < \infty\), then \(\seq{z^k}\) converges to some point \(z^\star \in \zer\p{F + \partial g }\) at least \(R\)-superlinearly.
  \end{thmenumerate}  
\end{theorem}

\begin{proof}
    The proof is presented for~\ProxFLEX{}, with the necessary adjustments for~\FLEX{} and~\IFLEX{} outlined at the end of the proof. 
    \begin{itemize}
        \item[\ref{thm:suplin:full_accepted}] Follows from~\eqref{eq:dir:superlin} since \Cref{State:Prox-FLEX:contraction} in~\ProxFLEX{} is true for all \(k\in\naturals\) sufficiently large.
        \item[\ref{thm:suplin:Q_superlinear}] Follows from~\ref{thm:suplin:full_accepted} and~\eqref{eq:dir:superlin}.
        \item[\ref{thm:suplin:summable}] Note that \Cref{ass:dk:bound} and \Cref{prop:V_performance_measure:lower_bound} give that 
        \begin{align*}
            \norm{d^k} \leq \frac{D}{\gamma}\norm{z^{k} - T_1^\gamma(z^k)} \leq \frac{2D}{\sqrt{1-\gamma L_F}}  \sqrt{\V(z^{k}, T_1^\gamma(z^k), T_2^\gamma(z^k))}
        \end{align*}
        for each \(k\in\naturals\) such that \(k\geq K\). The claim now follows from~\ref{thm:suplin:Q_superlinear}.
        \item[\ref{thm:suplin:R_superlinear}] \Cref{thm:ProxFLEX} and~\ref{thm:suplin:summable} imply that the sequence \(\seq{z^k}\) converges to some point \(z^\star\in \zer \p{F + \partial g }\). Since \(z^{k+1}-z^{k} = d^{k}\) for all \(k\in\naturals\) sufficiently large,~\ref{thm:suplin:summable} implies that \(\seq{z^{k+1} - z^k}\) converges to zero at least \(R\)-(super)linearly. In particular, there exists \(\kappa \in \reals_{++}\) and \(\seq{c_k} \in \reals_{++}^{\naturals}\) such that \(\lim_{k\to\infty}c_{k} = 0\) and 
        \begin{align}\label{eq:superlinear:diff_R_linear}
            \norm{z^{k+1} - z^k} \leq \kappa \prod_{i=1}^{k} c_i
        \end{align}
        for each \(k\in\naturals\). Let \(k,j\in\naturals\) such that \(j>k\). The triangle inequality and~\eqref{eq:superlinear:diff_R_linear} give that
        \begin{align*}
            \norm{z^k - z^\star} \xleftarrow[j \rightarrow \infty]{} \norm{z^k - z^j} \leq \sum_{\ell=k}^{j-1} \norm{z^{\ell}- z^{\ell+1}} \leq \kappa \sum_{\ell=k}^{j-1} \prod_{i=1}^{\ell} c_i \xrightarrow[j \rightarrow \infty]{} \kappa \sum_{\ell=k}^{\infty} \prod_{i=1}^{\ell} c_i = \mu_k.
        \end{align*}
        The sequence \(\seq{\mu_k}\in\reals_{++}^{\naturals}\) converges to zero at least \(Q\)-superlinearly since 
        \begin{align*}
            \frac{\mu_k}{\mu_{k-1}}
            =
            \frac{\sum_{\ell=k}^{\infty} \prod_{i=1}^{\ell} c_i}{\sum_{\ell=k-1}^{\infty} \prod_{i=1}^{\ell} c_i}
            =
            \frac{%
                \big(%
                    \prod_{i=1}^{k-1} c_i
                \big)
                \big(%
                    \sum_{\ell=k}^{\infty} \prod_{i=k}^{\ell} c_i
                \big)
            }{%
                \big(%
                    \prod_{i=1}^{k-1} c_i
                \big)%
                \big(%
                    1 + \sum_{\ell=k}^{\infty} \prod_{i=k}^{\ell} c_i
                \big)%
                }    
             =
             \frac{%
                \big(%
                    \sum_{\ell=k}^{\infty} \prod_{i=k}^{\ell} c_i
                \big)
            }{%
                \big(%
                    1 + \sum_{\ell=k}^{\infty} \prod_{i=k}^{\ell} c_i
                \big)%
                }
                \to 0    
        \end{align*}
        and \(\lim_{k\to\infty}\sum_{\ell=k}^{\infty} \prod_{i=k}^{\ell} c_i = 0\). Thus, \(\seq{z^k}\) converges to \(z^{\star}\) at least \(R\)-superlinearly, as claimed.
    \end{itemize}
    The assertions for~\FLEX{} follow directly, as setting 
    \(g=0\) reduces~\ProxFLEX{} and its underlying assumptions to those of~\FLEX{}. For~\IFLEX{}, the only distinction is that, for sufficiently large \(k\), \(\tau_k = 1\) is always accepted in \Cref{State:I-FLEX:LS} of~\IFLEX{}, due to~\eqref{def:eq:dir:superlin:F}. All other arguments remain unchanged. \qedhere
\end{proof}


==> extragradient/TeX/commands.tex <==
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\lVert#1\rVert}
\newcommand\inner[2]{\langle #1, #2 \rangle}
\newcommand\p[1]{\mathord{( #1 )}}
\newcommand\set[1]{\mathord{\left\{ #1 \right\}}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\Rbar}{\overline{\mathbf{R}}}
\newcommand{\N}{\mathbf{N}}
\newcommand{\naturals}{\mathbb{N}_0}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\Or}{\mathbf{O}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\Sym}{\mathbf{S}}
\newcommand{\sym}{\mathbb{S}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\Pro}[1]{\mathbf{P}\left[#1\right]}
\newcommand{\Var}[1]{\mathbf{Var}\left[#1\right]}
\newcommand{\Cov}[1]{\mathbf{Cov}\left[#1\right]}
\newcommand{\tr}[1]{\operatorname{tr}\left(#1\right)}
\newcommand{\trace}{{\mathrm{trace}}}
\newcommand{\E}[1]{\mathbf{E}\left[#1\right]}
\newcommand\Fix{\operatorname{Fix}}
\newcommand\epi{\operatorname{epi}}
\newcommand\diag{\operatorname{diag}}
\newcommand\rank{\operatorname{rank}}
\newcommand\sgn{\operatorname{sgn}}
\newcommand\Prox{\operatorname{Prox}}
\newcommand{\prox}{{\mathrm{prox}}}
\newcommand{\kron}{\otimes}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\Argmin}{Argmin}
\DeclareMathOperator*{\adj}{adj}
\DeclareMathOperator*{\gra}{gra}
\DeclareMathOperator*{\ran}{ran}
\DeclareMathOperator*{\zer}{zer}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\Id}{Id}
\DeclareMathOperator*{\Ker}{Ker}
\DeclareMathOperator*{\Ima}{Im}
\DeclareMathOperator*{\Cl}{cl}
\DeclareMathOperator*{\Int}{int}
\DeclareMathOperator*{\Conv}{conv}

\newcommand{\xmiddle}[1]{\;\middle#1\;}

\renewcommand{\N}{\mathbb{N}_{0}}%                       naturals
\newcommand{\V}{\mathcal V}

\DeclareMathOperator*{\jac}{Jac}
\newcommand{\I}{{\rm I}}%
\newcommand{\LF}{L_F}

\newcommand{\QuadMinMaxParam}{\omega}

\newcommandx{\seq}[3][{2=k\in\naturals},{3={}}]{(#1)_{#2}^{#3}}

% Revision and comments =======================================================
% Comment command
\newcommand{\note}[1]{{\Red\sffamily\footnotesize(#1\unskip)}}


    \newif\ifshowold\showoldtrue
    \newif\ifshownew\shownewtrue

    \colorlet{newcolor}{black}
    \colorlet{oldcolor}{black!30}
    \newcommand{\disablecolorlinks}{\def\HyColor@UseColor##1{}}
    \newcommand{\parsymbol}{\P}

    \newcommand{\old}[1]{{%
        \ifshowold
            \disablecolorlinks
            \color{oldcolor}{}%
            #1%
        \fi
    }}
    \newcommand{\new}[2][]{{%
        \ifshownew
            \disablecolorlinks
            \color{newcolor}{}#2%
        \fi
    }}
    \newcommand{\oldnew}[2]{\old{#1}\new{#2}}


\makeatother


==> extragradient/TeX/preamble.tex <==
\usepackage[top=25mm,bottom=25mm,right=30mm,left=30mm]{geometry}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{mathptmx,lmodern,mathrsfs,amsthm,amsmath,graphicx,graphics, float,cases,xfrac,amssymb,bm,bbm,mathtools,gensymb,subcaption,tocloft,listings,pgffor,lipsum,microtype,titling,mathrsfs,proof,sectsty,fancyhdr,longtable,lscape,emptypage,parskip,booktabs,bm,stmaryrd,enumerate,autobreak,enumitem}
%\usepackage[dvipsnames]{xcolor}
\usepackage[labelfont={bf,sf}]{caption}
% \usepackage[
% maxnames=20, 
% giveninits=true,% abbreviate first names
% isbn=false,%do not print ISBN or ISSN
% %url=false,
% %doi=true
% ]{biblatex}
% \addbibresource{TeX/mybib.bib}

%%% tikz stuff %%%
\usepackage{tikz}
\usetikzlibrary{positioning}
\usetikzlibrary{plotmarks}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.7}

\definecolor{color1}{RGB}{68,119,170}   % Blue
\definecolor{color2}{RGB}{102,204,238}  % Cyan
\definecolor{color3}{RGB}{34,136,51}    % Teal
\definecolor{color4}{RGB}{17,119,51}    % Green
\definecolor{color5}{RGB}{204,187,68}   % Olive
\definecolor{color6}{RGB}{221,204,119}  % Sand
\definecolor{color7}{RGB}{204,102,119}  % Rose
\definecolor{color8}{RGB}{136,34,85}    % Wine
\definecolor{color9}{RGB}{170,51,119}   % Purple
\definecolor{color10}{RGB}{102,102,102} % Grey
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{xargs}
\usepackage{units}

\input{TeX/commands}

% Give chapters, subsections, etc. in document desired font ---------
\allsectionsfont{\normalfont\sffamily\bfseries}  
\renewcommand{\abstractname}{\normalfont\sffamily\bfseries Abstract}

% newtheorem environment -------------------------
\makeatletter
\def\th@plain{
  \thm@headfont{\normalfont\sffamily\bfseries}
  \itshape 
}

\def\th@definition{
  \thm@headfont{\normalfont\sffamily\bfseries}
  \thm@notefont{\normalfont\sffamily\bfseries}
  %\itshape 
}

\newtheoremstyle{myStyle1}
  {0.3cm}% space before
  {0.3cm}% space after
  {\itshape}% body font
  {}% indent
  {\normalfont\sffamily\bfseries}% header font
  {:}% punctuation
  {.5em}% after theorem header
  {}% header specification (empty for default)


\newtheoremstyle{myStyle2}
  {0.3cm}% space before
  {0.3cm}% space after
  {}% body font
  {}% indent
  {\normalfont\sffamily\bfseries}% header font
  {:}% punctuation
  {.5em}% after theorem header
  {}% header specification (empty for default)

\makeatother

% Keywords command
\providecommand{\keywords}[1]
{\textbf{\textsf{Keywords.}} #1}

% AMS  subject classification command
\providecommand{\MSC}[1]
{\textbf{\textsf{Mathematics subject classification 2020.}} #1}

% https://tex.stackexchange.com/questions/100139/prevent-equation-labeling-to-change-sizes
\makeatletter
\def\maketag@@@#1{\hbox{\m@th\normalfont\normalsize#1}}
\makeatother


% https://tex.stackexchange.com/questions/83509/hfill-in-math-mode
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{hyperref}
\hypersetup{%
    hidelinks,
    hypertexnames = true,
    plainpages    = false,
    colorlinks = true,
    urlcolor   = MidnightBlue,
    linkcolor  = MidnightBlue,
    citecolor  = ForestGreen,
  }

\usepackage[capitalize,nameinlink]{cleveref}
% \PassOptionsToPackage{nameinlink,capitalize}{cleveref}
% \crefname{equation}{}{} % removes "eq." in front of equation references
\crefname{assumption}{assumption}{assumptions}
% Customize cleveref for enumerate (to add assumption number + enumerate)
\crefname{enumi}{Assumption}{Assumptions}  % Use "Assumption" for enumi references
\creflabelformat{enumi}{#2\theassumption.(\roman{enumi})#3}  % Format reference as "Assumption 1.(i)"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{myStyle1}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}[theorem]{Definition}
%\newtheorem{definition}{Definition}[section]

\theoremstyle{myStyle2}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
%\newtheorem{remark}{Remark}[section]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Algorithms
\usepackage{algorithm}
\captionsetup[algorithm]{labelsep=colon}
\usepackage{algpseudocode}
% \usepackage{etoolbox}
% Algorithm commands
\newcommand{\INITIALIZE}{\item[\textbf{Initialize:}]}
\newcommand{\REQUIRE}{\item[\textbf{Require:}]}
\newcommand{\INPUT}{\item[\textbf{Input:}]}
\newcommand{\OUTPUT}{\item[\textbf{Output:}]}

% Change cref names
\crefname{ALG@line}{Step}{Steps}
\Crefname{ALG@line}{Step}{Steps}
\renewcommand{\thealgorithm}{\arabic{algorithm}}

% Algorithmic line referencing fix
\makeatletter
\newcounter{algorithmicH}% New algorithmic-like hyperref counter
\let\OLDalgorithmic\algorithmic
\def\fixalgref{%
  \phantomsection
  \addtocounter{ALG@line}{-1}%
  \refstepcounter{ALG@line}%
}
\let\OLDState\State  \renewcommand{\State}{\OLDState\fixalgref}
\let\OLDIf\If        \renewcommand{\If}[1]{\OLDIf{#1}\fixalgref}
\let\OLDFor\For      \renewcommand{\For}[1]{\OLDFor{#1}\fixalgref}
\let\OLDElse\Else    \renewcommand{\Else}{\OLDElse\fixalgref}
\let\OLDElsIf\ElsIf  \renewcommand{\ElsIf}[1]{\OLDElsIf{#1}\fixalgref}
\let\OLDWhile\While  \renewcommand{\While}[1]{\OLDWhile{#1}\fixalgref}
\renewcommand{\algorithmic}{%
  \setcounter{ALG@line}{0}%
  \stepcounter{algorithmicH}%
  \OLDalgorithmic%
}
\renewcommand{\theHALG@line}{\thealgorithm.\arabic{ALG@line}}



%% Algorithm references
  \newcommand{\algnamefont}{\ttfamily} % Font for algorithm names
  \newcommand{\FLEX}{{\hyperref[alg:FLEX]{\algnamefont FLEX}}}
  \newcommand{\refFLEX}{\FLEX\ (\Cref{alg:FLEX})}  

  \newcommand{\IFLEX}{{\hyperref[alg:I-FLEX]{\algnamefont I-FLEX}}}
  \newcommand{\refIFLEX}{\IFLEX\ (\Cref{alg:I-FLEX})}

  \newcommand{\ProxFLEX}{{\hyperref[alg:Prox-FLEX]{\algnamefont Prox-FLEX}}}
  \newcommand{\refProxFLEX}{\ProxFLEX\ (\Cref{alg:Prox-FLEX})}  

  \newcommand{\ProxIFLEX}{{\hyperref[alg:Prox-I-FLEX]{\algnamefont Prox-I-FLEX}}}
  \newcommand{\refProxIFLEX}{\ProxIFLEX\ (\Cref{alg:Prox-I-FLEX})}  
  


\makeatother

% Define our custom algorithm environment
\newenvironment{customalgorithm}[1]{
    % Switch to 'plain' style so the top rule disappears:
    \floatstyle{plain}
    \restylefloat{algorithm}
    %
    \floatname{algorithm}{#1}        % Set custom caption title, e.g. "Datagen"
    \renewcommand{\thealgorithm}{}   % Disable numbering
    \begin{algorithm}
}{
    \end{algorithm}
    \addtocounter{algorithm}{-1} % Prevent incrementing the counter
    %
    % Restore the default 'ruled' style, so other algorithms are unaffected:
    \floatstyle{ruled}
    \restylefloat{algorithm}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% extra commands-PL  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\definecolor{Red}{rgb}{1, 0, 0}
\definecolor{BlueIMT}{RGB}{0,42,72}
\definecolor{ForestGreen}{rgb}{0.13, 0.55, 0.13}
\definecolor{Gray}{rgb}{0.66, 0.66, 0.66}
\definecolor{Green}{rgb}{0.0, 0.5, 0.0}
\definecolor{MidnightBlue}{rgb}{0.098, 0.098, 0.439}
\definecolor{Orange}{rgb}{0.93, 0.53, 0.18}


\foreach \x/\y/\z in {gray/Gray/gray, blue/Blue/MidnightBlue, orange/Orange/orange, red/Red/red, black/Black/black, green/Green/ForestGreen} {%
    \edef\temp{%
      \noexpand\expandafter\noexpand\gdef\noexpand\csname\x\noexpand\endcsname{\noexpand\color{\z}}%
      \noexpand\expandafter\noexpand\gdef\noexpand\csname\y\noexpand\endcsname{\noexpand\bfseries\noexpand\csname\x\noexpand\endcsname}%
    }\temp
  }

%%% cref related and numbering
\theoremstyle{myStyle1}
\newtheorem{assumption}{Assumption}

\renewcommand\theassumption{\Roman{assumption}}

\newlist{enumeratass}{enumerate}{1} 
\setlist[enumeratass]{label={(\roman*)}, ref=\theassumption.{(\roman*)}}
\crefname{enumeratassi}{Assumption}{Assumptions}

\newlist{enumeratlem}{enumerate}{1} 
\setlist[enumeratlem]{label={(\roman*)}, ref=\thelemma.{(\roman*)}}
\crefname{enumeratlemi}{Lemma}{Lemmas}

\newlist{thmenumerate}{enumerate}{1}
\setlist[thmenumerate]{label={(\roman*)}, ref=\thetheorem.{(\roman*)}}
\crefalias{thmenumeratei}{theorem}

\newlist{propenumerate}{enumerate}{1}
\setlist[propenumerate]{label={(\roman*)}, ref=\theproposition.{(\roman*)}}
\crefalias{propenumeratei}{proposition}

\Crefname{remark}{Remark}{Remarks}
%\Crefname{corollary}{Corollary}{Corollaries}
%\Crefname{proposition}{Proposition}{Propositions}

\numberwithin{equation}{section}


%% == Lists ================================================================

  \setlist[itemize,1]{label=\textbullet,wide,labelwidth=!,labelindent=0pt}
  % automatic widest <https://tex.stackexchange.com/a/547398/21001>
  \SetEnumitemKey{widestL}{
    labelwidth=\eqboxwidth{listlabel@\EnumitemId},
    leftmargin=!,
    format=\mylistlabel,
  }
  \newcommand\mylistlabel[2][l]{\eqmakebox[listlabel@\EnumitemId][#1]{#2}}

  \setlist[enumerate,1]{
    % widestL,
    label=\text{\it(\roman*)},
    ref=\text{(\roman*)},
  }

  % to create theorem-compatible enumerate lists
  \newcommand{\createthmlists}[1]{%
    \newlist{#1enumerate}{enumerate}{1}%
    \setlist[#1enumerate,1]{%
      % widestL,
      label = \upshape{(\roman*)},%
      ref = \thetheorem(\roman*),%
    }%
    \crefalias{#1enumeratei}{#1}%
    %
    \AtBeginEnvironment{#1}{%
      \expandafter\let\expandafter\enumerate\csname #1enumerate\endcsname
      \expandafter\let\expandafter\endenumerate\csname end#1enumerate\endcsname
    }{}{}%
  }%

  \createthmlists{assumption}
  \createthmlists{corollary}
  \createthmlists{example}
  \createthmlists{fact}
  \createthmlists{lemma}
  \createthmlists{remark}
  \createthmlists{theorem}



==> extragradient/plot_data/bilinear_matrix_game_n250/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007281303405761719,2.0175302852282635
200,201,200,401,0.0959312915802002,0.04349679025208781
400,401,400,801,0.18608999252319336,0.01463313080366676
601,602,601,1203,0.26926732063293457,0.008383382119091624
801,802,801,1603,0.35022425651550293,0.005308128436778398
1001,1002,1001,2003,0.43725109100341797,0.003611737845149916
1201,1202,1201,2403,0.5174431800842285,0.0024998306769794553
1401,1402,1401,2803,0.5994551181793213,0.0019129109684775767
1602,1603,1602,3205,0.6778171062469482,0.001517403112843079
1802,1803,1802,3605,0.8061790466308594,0.0010801183065014036
2002,2003,2002,4005,0.8882951736450195,0.00084483215213907
2202,2203,2202,4405,0.9704623222351074,0.0006737009382688204
2402,2403,2402,4805,1.0517749786376953,0.0006006934794445092
2603,2604,2603,5207,1.1305081844329834,0.0005524341654471254
2803,2804,2803,5607,1.2131781578063965,0.0005203715067254704
3003,3004,3003,6007,1.2967259883880615,0.0004938357892155201
3203,3204,3203,6407,1.3826229572296143,0.00047381790976371306
3403,3404,3403,6807,1.4719600677490234,0.0004562055350135338
3604,3605,3604,7209,1.5571630001068115,0.0004405816327960734
3804,3805,3804,7609,1.6411750316619873,0.00042684807770256423
4004,4005,4004,8009,1.7317380905151367,0.0004144581307523731
4204,4205,4204,8409,1.8344430923461914,0.00038701197829392155
4404,4405,4404,8809,1.9236962795257568,0.0003589698467677532
4605,4606,4605,9211,2.0135202407836914,0.0003389567700187074
4805,4806,4805,9611,2.0992672443389893,0.00032438123433770473
5005,5006,5005,10011,2.18808913230896,0.00031323731496694224
5205,5206,5205,10411,2.277238130569458,0.00030312153139750776
5405,5406,5405,10811,2.365588426589966,0.0002951313295900683
5606,5607,5606,11213,2.454519033432007,0.0002868730286204068
5806,5807,5806,11613,2.5455241203308105,0.0002796332694694478
6006,6007,6006,12013,2.637850284576416,0.0002726067510085043
6206,6207,6206,12413,2.7258191108703613,0.0002662437298906885
6406,6407,6406,12813,2.817854404449463,0.0002606660196780025
6607,6608,6607,13215,2.907839059829712,0.00025464941279198096
6807,6808,6807,13615,3.000429153442383,0.0002492815683777871
7007,7008,7007,14015,3.0906150341033936,0.00024396338135374693
7207,7208,7207,14415,3.182464122772217,0.0002388132550460753
7407,7408,7407,14815,3.2756950855255127,0.0002338609486167385
7608,7609,7608,15217,3.3696093559265137,0.00022920305099681287
7808,7809,7808,15617,3.4653522968292236,0.0002245584023920893
8008,8009,8008,16017,3.554715156555176,0.00022025811900593448
8208,8209,8208,16417,3.6455612182617188,0.00021579995562336568
8408,8409,8408,16817,3.738467216491699,0.0002117638984231238
8609,8610,8609,17219,3.824047088623047,0.00020765253453355168
8809,8810,8809,17619,3.9229352474212646,0.000203800244734095
9009,9010,9009,18019,4.02763819694519,0.00020007474747131315
9209,9210,9209,18419,4.115026235580444,0.00019642733860085837
9409,9410,9409,18819,4.203932285308838,0.00019277617511714317
9610,9611,9610,19221,4.2919652462005615,0.00018910103929544058
9810,9811,9810,19621,4.380505084991455,0.00018559030195585525
10010,10011,10010,20021,4.470429182052612,0.00018217491027878736
10210,10211,10210,20421,4.5800042152404785,0.00017912284445985077
10410,10411,10410,20821,4.6981422901153564,0.0001760786239302967
10611,10612,10611,21223,4.811402082443237,0.00017298073175407749
10811,10812,10811,21623,4.920499324798584,0.00017016636966793168
11011,11012,11011,22023,5.029935121536255,0.00016737462008611416
11211,11212,11211,22423,5.132140159606934,0.00016464480556627341
11411,11412,11411,22823,5.234155178070068,0.00016197874359082196
11612,11613,11612,23225,5.338236331939697,0.00015923884347311177
11812,11813,11812,23625,5.438040256500244,0.00015662353894798823
12012,12013,12012,24025,5.539370059967041,0.00015415289946156186
12212,12213,12212,24425,5.637982368469238,0.00015162225637175758
12412,12413,12412,24825,5.7329981327056885,0.00014936172321451153
12613,12614,12613,25227,5.82281231880188,0.00014701752975775564
12813,12814,12813,25627,5.909841299057007,0.00014481711209930154
13013,13014,13013,26027,6.0059521198272705,0.00014272320071532593
13213,13214,13213,26427,6.120509386062622,0.0001405836563330132
13413,13414,13413,26827,6.210010290145874,0.00013853138183307168
13614,13615,13614,27229,6.303691148757935,0.00013641277160255833
13814,13815,13814,27629,6.3946921825408936,0.00013437125727317872
14014,14015,14014,28029,6.489281177520752,0.00013243351483812772
14214,14215,14214,28429,6.585764169692993,0.00013061002723731207
14414,14415,14414,28829,6.682311296463013,0.0001288618374643721
14615,14616,14615,29231,6.782353162765503,0.00012700312591845954
14815,14816,14815,29631,6.887568235397339,0.00012533549026164323
15015,15016,15015,30031,6.986952304840088,0.0001237316292711887
15215,15216,15215,30431,7.07727313041687,0.00012210328503496048
15415,15416,15415,30831,7.174143075942993,0.00012051037294022716
15616,15617,15616,31233,7.268860340118408,0.00011892206660066964
15816,15817,15816,31633,7.35948634147644,0.00011735141627086584
16016,16017,16016,32033,7.448448181152344,0.00011582617945084914
16216,16217,16216,32433,7.536229133605957,0.00011438478665953952
16416,16417,16416,32833,7.631782293319702,0.0001130040587119364
16617,16618,16617,33235,7.735324144363403,0.00011159045898095159
16817,16818,16817,33635,7.836766242980957,0.00011027016872333847
17017,17018,17017,34035,7.929502248764038,0.00010901316527982595
17217,17218,17217,34435,8.022398233413696,0.00010772137193150168
17417,17418,17417,34835,8.114703178405762,0.00010648026163911816
17618,17619,17618,35237,8.224632263183594,0.00010520697983787658
17818,17819,17818,35637,8.323623180389404,0.00010399621761891964
18018,18019,18018,36037,8.411773204803467,0.00010284042235574151
18218,18219,18218,36437,8.517847061157227,0.00010170143365575595
18418,18419,18418,36837,8.624557256698608,0.00010056456640249463
18619,18620,18619,37239,8.729220151901245,9.944541358835505e-05
18819,18820,18819,37639,8.836987257003784,9.839306022937163e-05
19019,19020,19019,38039,8.937278985977173,9.738862420113625e-05
19219,19220,19219,38439,9.031203269958496,9.639341303068005e-05
19419,19420,19419,38839,9.12900710105896,9.538202453546805e-05
19620,19621,19620,39241,9.27678918838501,9.4363304220243e-05
19820,19821,19820,39641,9.431886196136475,9.340180684196344e-05
20020,20021,20020,40041,9.564775228500366,9.243656539940447e-05
20220,20221,20220,40441,9.686647176742554,9.15572172742962e-05
20420,20421,20420,40841,9.809267282485962,9.065229658907348e-05
20621,20622,20621,41243,9.929938316345215,8.977120777822201e-05
20821,20822,20821,41643,10.022725105285645,8.892907706479929e-05
21021,21022,21021,42043,10.11018419265747,8.812551845793952e-05
21221,21222,21221,42443,10.196634292602539,8.730915054718582e-05
21421,21422,21421,42843,10.285643100738525,8.649798321388793e-05
21622,21623,21622,43245,10.388175249099731,8.567629477582349e-05
21822,21823,21822,43645,10.483395099639893,8.487925320532365e-05
22022,22023,22022,44045,10.570648193359375,8.40986245948514e-05
22222,22223,22222,44445,10.658637046813965,8.33526239707654e-05
22422,22423,22422,44845,10.74113416671753,8.262284079297658e-05
22623,22624,22623,45247,10.826329231262207,8.187989195743251e-05
22823,22824,22823,45647,10.909593105316162,8.119464191111391e-05
23023,23024,23023,46047,10.994264125823975,8.052384466515087e-05
23223,23224,23223,46447,11.077093124389648,7.984401896895232e-05
23423,23424,23423,46847,11.156476259231567,7.918024523915324e-05
23624,23625,23624,47249,11.239704132080078,7.84837687200331e-05
23824,23825,23824,47649,11.323280334472656,7.782481633673095e-05
24024,24025,24024,48049,11.402717351913452,7.719433726700041e-05
24224,24225,24224,48449,11.494933128356934,7.657328989244122e-05
24424,24425,24424,48849,11.57755708694458,7.594551450031627e-05
24625,24626,24625,49251,11.656225204467773,7.531904821314078e-05
24825,24826,24825,49651,11.73757529258728,7.473586971830085e-05
25025,25026,25025,50051,11.817572116851807,7.416603701640299e-05
25225,25226,25225,50451,11.899257183074951,7.359763946756605e-05
25425,25426,25425,50851,11.98238730430603,7.304486610845149e-05
25626,25627,25626,51253,12.069847106933594,7.245258116200675e-05
25826,25827,25826,51653,12.156044006347656,7.187416202223475e-05
26026,26027,26026,52053,12.236670970916748,7.133977069260418e-05
26226,26227,26226,52453,12.318674325942993,7.081460010485274e-05
26426,26427,26426,52853,12.405185222625732,7.026964256451874e-05
26627,26628,26627,53255,12.508796215057373,6.973241909225221e-05
26827,26828,26827,53655,12.598721027374268,6.923029817992534e-05
27027,27028,27027,54055,12.685818195343018,6.875023710613176e-05
27227,27228,27227,54455,12.777579069137573,6.824743391150301e-05
27427,27428,27427,54855,12.864879131317139,6.774479328299629e-05
27628,27629,27628,55257,12.95504117012024,6.724269230360465e-05
27828,27829,27828,55657,13.043668270111084,6.676429741580756e-05
28028,28029,28028,56057,13.129280090332031,6.63060719300869e-05
28228,28229,28228,56457,13.21379828453064,6.583518619066744e-05
28428,28429,28428,56857,13.30055022239685,6.537685298370303e-05
28629,28630,28629,57259,13.388512134552002,6.491668355074883e-05
28829,28830,28829,57659,13.471657276153564,6.448072388554719e-05
29029,29030,29029,58059,13.560417175292969,6.405672803483145e-05
29229,29230,29229,58459,13.646382093429565,6.361382713284362e-05
29429,29430,29429,58859,13.733050107955933,6.31888947632797e-05
29630,29631,29630,59261,13.818182229995728,6.274900507254005e-05
29830,29831,29830,59661,13.902440309524536,6.232775681204577e-05
30030,30031,30030,60061,13.996052265167236,6.191535312863151e-05
30230,30231,30230,60461,14.081595182418823,6.150523032318522e-05
30430,30431,30430,60861,14.168079137802124,6.109476700765481e-05
30631,30632,30631,61263,14.25273323059082,6.069076591888799e-05
30831,30832,30831,61663,14.33932113647461,6.031392572042342e-05
31031,31032,31031,62063,14.425340175628662,5.9924358648023766e-05
31231,31232,31231,62463,14.511688232421875,5.955666867858864e-05
31431,31432,31431,62863,14.614310264587402,5.9155968409256884e-05
31632,31633,31632,63265,14.710103034973145,5.877554694422264e-05
31832,31833,31832,63665,14.798553228378296,5.839570861606201e-05
32032,32033,32032,64065,14.887530088424683,5.803407125043927e-05
32232,32233,32232,64465,14.981438398361206,5.766553082290742e-05
32432,32433,32432,64865,15.07377004623413,5.728559856767123e-05
32633,32634,32633,65267,15.169085264205933,5.6922519498144956e-05
32833,32834,32833,65667,15.263267278671265,5.657271025306751e-05
33033,33034,33033,66067,15.349680185317993,5.6226674498752885e-05
33233,33234,33233,66467,15.442358016967773,5.5880773115064576e-05
33433,33434,33433,66867,15.530570983886719,5.552197816727787e-05
33634,33635,33634,67269,15.615693092346191,5.516561988359456e-05
33834,33835,33834,67669,15.70409607887268,5.483004777874078e-05
34034,34035,34034,68069,15.792055130004883,5.449542895384602e-05
34234,34235,34234,68469,15.878031253814697,5.414930042640301e-05
34434,34435,34434,68869,15.974096298217773,5.3813721934697497e-05
34635,34636,34635,69271,16.076503038406372,5.3480548749246844e-05
34835,34836,34835,69671,16.167524099349976,5.316271007961268e-05
35035,35036,35035,70071,16.25555920600891,5.284537795893794e-05
35235,35236,35235,70471,16.34127116203308,5.25210258070886e-05
35435,35436,35435,70871,16.443947076797485,5.219307813928155e-05
35636,35637,35636,71273,16.533640384674072,5.187487251807022e-05
35836,35837,35836,71673,16.620553970336914,5.156750595635992e-05
36036,36037,36036,72073,16.715681076049805,5.126633912635567e-05
36236,36237,36236,72473,16.819322109222412,5.0953583616013344e-05
36436,36437,36436,72873,16.905238151550293,5.06364164037916e-05
36637,36638,36637,73275,16.994919300079346,5.033224679889726e-05
36837,36838,36837,73675,17.086060047149658,5.003721734554995e-05
37037,37038,37037,74075,17.178019046783447,4.9741082168717235e-05
37237,37238,37237,74475,17.266119241714478,4.944104546404938e-05
37437,37438,37437,74875,17.352636337280273,4.9139840639682104e-05
37638,37639,37638,75277,17.440890312194824,4.885057992917566e-05
37838,37839,37838,75677,17.526872158050537,4.85575752231326e-05
38038,38039,38038,76077,17.61354923248291,4.827473332435137e-05
38238,38239,38238,76477,17.697108268737793,4.7980470467051044e-05
38438,38439,38438,76877,17.785032272338867,4.7692428596902716e-05
38639,38640,38639,77279,17.87205410003662,4.7408535184029144e-05
38839,38840,38839,77679,17.963057279586792,4.713660351074352e-05
39039,39040,39039,78079,18.04795813560486,4.686073608735103e-05
39239,39240,39239,78479,18.135825157165527,4.6582040221635385e-05
39439,39440,39439,78879,18.219581365585327,4.6300431451159644e-05
39640,39641,39640,79281,18.305496215820312,4.602805926680519e-05
39840,39841,39840,79681,18.393071174621582,4.576611665363842e-05
40040,40041,40040,80081,18.484689235687256,4.55030706163161e-05
40240,40241,40240,80481,18.569539070129395,4.5229626912537586e-05
40440,40441,40440,80881,18.655269145965576,4.495617216004105e-05
40641,40642,40641,81283,18.741225957870483,4.469361414303455e-05
40841,40842,40841,81683,18.832993030548096,4.443907725495218e-05
41041,41042,41041,82083,18.94217610359192,4.418266302272347e-05
41241,41242,41241,82483,19.031660079956055,4.3923346657347656e-05
41441,41442,41441,82883,19.119991064071655,4.3661149519129555e-05
41642,41643,41642,83285,19.205779314041138,4.340203533190099e-05
41842,41843,41842,83685,19.29512619972229,4.315515969837136e-05
42042,42043,42042,84085,19.3821382522583,4.290805443483866e-05
42242,42243,42242,84485,19.476263284683228,4.2654259017404e-05
42442,42443,42442,84885,19.5628080368042,4.240127396810882e-05
42643,42644,42643,85287,19.65214514732361,4.2158107159545125e-05
42843,42844,42843,85687,19.738636016845703,4.1918176335549746e-05
43043,43044,43043,86087,19.826378107070923,4.168443320234073e-05
43243,43244,43243,86487,19.917054414749146,4.1432271363523665e-05
43443,43444,43443,86887,20.00820827484131,4.1189617959602924e-05
43644,43645,43644,87289,20.095766067504883,4.094897669748808e-05
43844,43845,43844,87689,20.181411266326904,4.0722031790799655e-05
44044,44045,44044,88089,20.26870822906494,4.048807391286977e-05
44244,44245,44244,88489,20.353931188583374,4.024834902875708e-05
44444,44445,44444,88889,20.4399151802063,4.002200765569792e-05
44645,44646,44645,89291,20.530725240707397,3.979216703043228e-05
44845,44846,44845,89691,20.617687225341797,3.9573382357795005e-05
45045,45046,45045,90091,20.70560932159424,3.935498479010369e-05
45245,45246,45245,90491,20.79341220855713,3.911584928846526e-05
45445,45446,45445,90891,20.8846652507782,3.8885417425241024e-05
45646,45647,45646,91293,20.984723329544067,3.866250353869032e-05
45846,45847,45846,91693,21.08818221092224,3.84441429876271e-05
46046,46047,46046,92093,21.17937731742859,3.8223162140471584e-05
46246,46247,46246,92493,21.267199993133545,3.800206366730713e-05
46446,46447,46446,92893,21.35773015022278,3.777199618817935e-05
46647,46648,46647,93295,21.44730806350708,3.756278377254041e-05
46847,46848,46847,93695,21.53773522377014,3.7346762305204784e-05
47047,47048,47047,94095,21.62648916244507,3.712812633548001e-05
47247,47248,47247,94495,21.712921142578125,3.690899975869172e-05
47447,47448,47447,94895,21.8012752532959,3.669440941879532e-05
47648,47649,47648,95297,21.886057376861572,3.649059687226073e-05
47848,47849,47848,95697,21.972025156021118,3.629093444915889e-05
48048,48049,48048,96097,22.053450107574463,3.607905216132611e-05
48248,48249,48248,96497,22.133105278015137,3.5866872854294585e-05
48448,48449,48448,96897,22.212169408798218,3.566114855347171e-05
48649,48650,48649,97299,22.29220414161682,3.5464307067232614e-05
48849,48850,48849,97699,22.373934268951416,3.5260934826246345e-05
49049,49050,49049,98099,22.458714246749878,3.5058303816099254e-05
49249,49250,49249,98499,22.54260516166687,3.485677672621492e-05
49449,49450,49449,98899,22.63002109527588,3.465229051577856e-05
49650,49651,49650,99301,22.71369218826294,3.446204642760552e-05
49850,49851,49850,99701,22.797407150268555,3.426979772366392e-05
50050,50051,50050,100101,22.87967324256897,3.407187424216444e-05
50250,50251,50250,100501,22.967891216278076,3.387398383225383e-05
50450,50451,50450,100901,23.051912307739258,3.3679433436960105e-05
50651,50652,50651,101303,23.14886713027954,3.348877979673868e-05
50851,50852,50851,101703,23.241708040237427,3.3297045777433164e-05
51051,51052,51051,102103,23.324677228927612,3.310325505168251e-05
51251,51252,51251,102503,23.409648180007935,3.2908020179998376e-05
51451,51452,51451,102903,23.496121168136597,3.271969423756346e-05
51652,51653,51652,103305,23.581294059753418,3.254145881685616e-05
51852,51853,51852,103705,23.66253638267517,3.2363333636571314e-05
52052,52053,52052,104105,23.743874073028564,3.218078029110317e-05
52252,52253,52252,104505,23.82852029800415,3.199345322738687e-05
52452,52453,52452,104905,23.91178011894226,3.1808958844089716e-05
52653,52654,52653,105307,23.997891187667847,3.16296981168475e-05
52853,52854,52853,105707,24.080198287963867,3.145343828161283e-05
53053,53054,53053,106107,24.161572217941284,3.1272107881341055e-05
53253,53254,53253,106507,24.242918252944946,3.108836469116431e-05
53453,53454,53453,106907,24.322376251220703,3.0909774845599655e-05
53654,53655,53654,107309,24.407057285308838,3.073469595710666e-05
53854,53855,53854,107709,24.492629051208496,3.056027578407177e-05
54054,54055,54054,108109,24.574190139770508,3.038100894217561e-05
54254,54255,54254,108509,24.656105995178223,3.0203118740216653e-05
54454,54455,54454,108909,24.738986015319824,3.0030033428673074e-05
54655,54656,54655,109311,24.8208429813385,2.98647824054099e-05
54855,54856,54855,109711,24.903655290603638,2.9697277166727948e-05
55055,55056,55055,110111,24.992390155792236,2.952720305410415e-05
55255,55256,55255,110511,25.07669234275818,2.9356086829694833e-05
55455,55456,55455,110911,25.162471294403076,2.918587659355347e-05
55656,55657,55656,111313,25.25596809387207,2.902127739964588e-05
55856,55857,55856,111713,25.35647225379944,2.8854875181490635e-05
56056,56057,56056,112113,25.43930721282959,2.8688969036073803e-05
56256,56257,56256,112513,25.52698016166687,2.8519344336321652e-05
56456,56457,56456,112913,25.61405324935913,2.8362085893505203e-05
56657,56658,56657,113315,25.700395107269287,2.8208489059329487e-05
56857,56858,56857,113715,25.785850286483765,2.805028514924895e-05
57057,57058,57057,114115,25.86933922767639,2.789225266345393e-05
57257,57258,57257,114515,25.960916996002197,2.7730269917025014e-05
57457,57458,57457,114915,26.048280239105225,2.7576539585561855e-05
57658,57659,57658,115317,26.13961434364319,2.7422879010784986e-05
57858,57859,57858,115717,26.231770277023315,2.7270934028296223e-05
58058,58059,58058,116117,26.32039499282837,2.71116464066292e-05
58258,58259,58258,116517,26.409600019454956,2.6958623057787118e-05
58458,58459,58458,116917,26.503130197525024,2.6806296062578798e-05
58659,58660,58659,117319,26.591439247131348,2.6654732163003354e-05
58859,58860,58859,117719,26.680423259735107,2.6504644921813096e-05
59059,59060,59059,118119,26.76919412612915,2.6353382897758466e-05
59259,59260,59259,118519,26.857580184936523,2.6209521400123258e-05
59459,59460,59459,118919,26.947571992874146,2.605103973363189e-05
59660,59661,59660,119321,27.044185161590576,2.5908216042562068e-05
59860,59861,59860,119721,27.131198406219482,2.5758696896866847e-05
60060,60061,60060,120121,27.215150117874146,2.5609108228294194e-05
60260,60261,60260,120521,27.301974058151245,2.5458114950506286e-05
60460,60461,60460,120921,27.395907163619995,2.5313059922511282e-05
60661,60662,60661,121323,27.500123262405396,2.5173770542197303e-05
60861,60862,60861,121723,27.58786630630493,2.5031268591886076e-05
61061,61062,61061,122123,27.67835807800293,2.4885463431454354e-05
61261,61262,61261,122523,27.7620952129364,2.47408479227083e-05
61461,61462,61461,122923,27.847088098526,2.4605641264016896e-05
61662,61663,61662,123325,27.93605136871338,2.4468448103554395e-05
61862,61863,61862,123725,28.023831129074097,2.4330026607709257e-05
62062,62063,62062,124125,28.109291076660156,2.4184956760315136e-05
62262,62263,62262,124525,28.193724155426025,2.4047497090560827e-05
62462,62463,62462,124925,28.285835027694702,2.3909342168140502e-05
62663,62664,62663,125327,28.37330937385559,2.3777020478215538e-05
62863,62864,62863,125727,28.460122108459473,2.3642438244826853e-05
63063,63064,63063,126127,28.54674220085144,2.3510426749577215e-05
63263,63264,63263,126527,28.634721040725708,2.3373624985522568e-05
63463,63464,63463,126927,28.71939516067505,2.3241726833500494e-05
63664,63665,63664,127329,28.804619073867798,2.3110620054245152e-05
63864,63865,63864,127729,28.89165425300598,2.2978669536567172e-05
64064,64065,64064,128129,28.980464220046997,2.284442418077898e-05
64264,64265,64264,128529,29.073018312454224,2.2713707140117137e-05
64464,64465,64464,128929,29.156590223312378,2.2584849821385144e-05
64665,64666,64665,129331,29.24294137954712,2.2458991312388633e-05
64865,64866,64865,129731,29.328445196151733,2.2331154158446256e-05
65065,65066,65065,130131,29.414799213409424,2.220309375251141e-05
65265,65266,65265,130531,29.511436223983765,2.2075911381711464e-05
65465,65466,65465,130931,29.620408058166504,2.1948898272173608e-05
65666,65667,65666,131333,29.70530414581299,2.1826364675657413e-05
65866,65867,65866,131733,29.790765047073364,2.170112154996743e-05
66066,66067,66066,132133,29.876289129257202,2.15737448610592e-05
66266,66267,66266,132533,29.965140342712402,2.1449877968642182e-05
66466,66467,66466,132933,30.050936222076416,2.132837537995066e-05
66667,66668,66667,133335,30.135828971862793,2.120706404296143e-05
66867,66868,66867,133735,30.219041109085083,2.1087404115954594e-05
67067,67068,67067,134135,30.30274200439453,2.0967753027169325e-05
67267,67268,67267,134535,30.38755202293396,2.0847117874275213e-05
67467,67468,67467,134935,30.476243257522583,2.073328887901093e-05
67668,67669,67668,135337,30.562254190444946,2.0615851924748196e-05
67868,67869,67868,135737,30.64954113960266,2.049701664325926e-05
68068,68069,68068,136137,30.73502016067505,2.037283772410546e-05
68268,68269,68268,136537,30.819689989089966,2.0254139543673416e-05
68468,68469,68468,136937,30.910118341445923,2.014272231499512e-05
68669,68670,68669,137339,31.000458002090454,2.0032141631323935e-05
68869,68870,68869,137739,31.08446431159973,1.9915547674094848e-05
69069,69070,69069,138139,31.172425270080566,1.980543503806041e-05
69269,69270,69269,138539,31.256185293197632,1.9689311784544486e-05
69469,69470,69469,138939,31.344226121902466,1.957909782685141e-05
69670,69671,69670,139341,31.432355165481567,1.946957057844719e-05
69870,69871,69870,139741,31.52322220802307,1.936034205208686e-05
70070,70071,70070,140141,31.609008312225342,1.9248035024627546e-05
70270,70271,70270,140541,31.71252417564392,1.9137475047250834e-05
70470,70471,70470,140941,31.8079891204834,1.9032495567941314e-05
70671,70672,70671,141343,31.89241123199463,1.8925067225835913e-05
70871,70872,70871,141743,31.979313135147095,1.8816859701573948e-05
71071,71072,71071,142143,32.06584811210632,1.871317163277767e-05
71271,71272,71271,142543,32.150076150894165,1.8602829039216538e-05
71471,71472,71471,142943,32.23574924468994,1.849854790345044e-05
71672,71673,71672,143345,32.321300983428955,1.8393355147318334e-05
71872,71873,71872,143745,32.40733814239502,1.8288877257039196e-05
72072,72073,72072,144145,32.49301505088806,1.8182668416874208e-05
72272,72273,72272,144545,32.57851314544678,1.8078682742004895e-05
72472,72473,72472,144945,32.669490337371826,1.797781604599285e-05
72673,72674,72673,145347,32.75463318824768,1.7877559608407162e-05
72873,72874,72873,145747,32.84002113342285,1.7774621973660255e-05
73073,73074,73073,146147,32.92782020568848,1.7671610821187407e-05
73273,73274,73273,146547,33.015589237213135,1.756973935132372e-05
73473,73474,73473,146947,33.101744174957275,1.747329327111986e-05
73674,73675,73674,147349,33.190232038497925,1.7374525672091756e-05
73874,73875,73874,147749,33.27490711212158,1.7275369901994712e-05
74074,74075,74074,148149,33.3624210357666,1.717358237177867e-05
74274,74275,74274,148549,33.4491183757782,1.7077728116492744e-05
74474,74475,74474,148949,33.53477120399475,1.6984968192025977e-05
74675,74676,74675,149351,33.626697301864624,1.6888433011821516e-05
74875,74876,74875,149751,33.72048997879028,1.6789067229618358e-05
75075,75076,75075,150151,33.82384014129639,1.6694372616519443e-05
75275,75276,75275,150551,33.92210936546326,1.6599683191183772e-05
75475,75476,75475,150951,34.01589608192444,1.6507158233319994e-05
75676,75677,75676,151353,34.1069540977478,1.641388719841217e-05
75876,75877,75876,151753,34.193522214889526,1.6318430792519853e-05
76076,76077,76076,152153,34.28123211860657,1.622664920892012e-05
76276,76277,76276,152553,34.36935019493103,1.613263647306398e-05
76476,76477,76476,152953,34.45884919166565,1.6042642537678262e-05
76677,76678,76677,153355,34.54640531539917,1.595332275702541e-05
76877,76878,76877,153755,34.63629412651062,1.5861364616726558e-05
77077,77078,77077,154155,34.72506618499756,1.5771308142881872e-05
77277,77278,77277,154555,34.8109712600708,1.567945437052457e-05
77477,77478,77477,154955,34.89591908454895,1.5592383651183548e-05
77678,77679,77678,155357,34.987088203430176,1.550500368071316e-05
77878,77879,77878,155757,35.07900619506836,1.541514508955842e-05
78078,78079,78078,156157,35.169002056121826,1.532726187204755e-05
78278,78279,78278,156557,35.25713014602661,1.5239189362436148e-05
78478,78479,78478,156957,35.34570908546448,1.5155070081383821e-05
78679,78680,78679,157359,35.42943525314331,1.5068687944061798e-05
78879,78880,78879,157759,35.51671504974365,1.498359297659093e-05
79079,79080,79079,158159,35.598002195358276,1.4896729783120503e-05
79279,79280,79279,158559,35.68087029457092,1.4813475747881937e-05
79479,79480,79479,158959,35.76240420341492,1.4730560494425782e-05
79680,79681,79680,159361,35.844667196273804,1.4646996890496018e-05
79880,79881,79880,159761,35.93958806991577,1.4560002145798024e-05
80080,80081,80080,160161,36.03884816169739,1.4476186589892849e-05
80280,80281,80280,160561,36.12272310256958,1.4395097411046645e-05
80480,80481,80480,160961,36.206061124801636,1.4315172193088612e-05
80681,80682,80681,161363,36.289852142333984,1.4236856002886425e-05
80881,80882,80881,161763,36.37353825569153,1.4150203928221278e-05
81081,81082,81081,162163,36.46173810958862,1.4067153841413783e-05
81281,81282,81281,162563,36.571128129959106,1.3990612108117471e-05
81481,81482,81481,162963,36.663679122924805,1.3913492084054254e-05
81682,81683,81682,163365,36.74499320983887,1.3833593305324456e-05
81882,81883,81882,163765,36.825958251953125,1.3753436174266995e-05
82082,82083,82082,164165,36.907679080963135,1.3673504656062576e-05
82282,82283,82282,164565,36.99503827095032,1.3597546959275085e-05
82482,82483,82482,164965,37.07935905456543,1.3523344221911589e-05
82683,82684,82683,165367,37.1655490398407,1.3445790494248331e-05
82883,82884,82883,165767,37.24769115447998,1.3366168963109555e-05
83083,83084,83083,166167,37.332786321640015,1.3290207252721693e-05
83283,83284,83283,166567,37.417065382003784,1.3217145131435926e-05
83483,83484,83483,166967,37.503191232681274,1.3144771373967242e-05
83684,83685,83684,167369,37.58613038063049,1.3068561346953922e-05
83884,83885,83884,167769,37.66823410987854,1.2993877510351008e-05
84084,84085,84084,168169,37.76060223579407,1.2918538839732042e-05
84284,84285,84284,168569,37.87095808982849,1.284635403925718e-05
84484,84485,84484,168969,37.977957248687744,1.2775084182800254e-05
84685,84686,84685,169371,38.091347217559814,1.2703089080745518e-05
84885,84886,84885,169771,38.19183111190796,1.2627186356168554e-05
85085,85086,85085,170171,38.28093910217285,1.2553614886837949e-05
85285,85286,85285,170571,38.371111154556274,1.2482807758333311e-05
85485,85486,85485,170971,38.46280813217163,1.2412574522608132e-05
85686,85687,85686,171373,38.55041837692261,1.2341653257175407e-05
85886,85887,85886,171773,38.64422821998596,1.2268011364632383e-05
86086,86087,86086,172173,38.73240613937378,1.2198067277010739e-05
86286,86287,86286,172573,38.822418212890625,1.2130567663723096e-05
86486,86487,86486,172973,38.913533210754395,1.2063519989761432e-05
86687,86688,86687,173375,39.00458025932312,1.1994782350828172e-05
86887,86888,86887,173775,39.09005117416382,1.1926540938979378e-05
87087,87088,87087,174175,39.177168130874634,1.1859056114325685e-05
87287,87288,87287,174575,39.26691937446594,1.1792963164654534e-05
87487,87488,87487,174975,39.36198616027832,1.1728072346173193e-05
87688,87689,87688,175377,39.45076131820679,1.1661055000865613e-05
87888,87889,87888,175777,39.53821015357971,1.1591635581218765e-05
88088,88089,88088,176177,39.625449419021606,1.1524971141301988e-05
88288,88289,88288,176577,39.71242427825928,1.1462061148892754e-05
88488,88489,88488,176977,39.79675912857056,1.1397996884956163e-05
88689,88690,88689,177379,39.90486931800842,1.1331194879032195e-05
88889,88890,88889,177779,40.001904249191284,1.1264734713039969e-05
89089,89090,89089,178179,40.09389901161194,1.1201278905969727e-05
89289,89290,89289,178579,40.19308638572693,1.1138286682471249e-05
89489,89490,89489,178979,40.32176208496094,1.1076275055199093e-05
89690,89691,89690,179381,40.42419219017029,1.1011625595230796e-05
89890,89891,89890,179781,40.51807904243469,1.0946218733063632e-05
90090,90091,90090,180181,40.610016107559204,1.0883652978229117e-05
90290,90291,90290,180581,40.71813416481018,1.082407796913197e-05
90490,90491,90490,180981,40.81458520889282,1.0762841532907455e-05
90691,90692,90691,181383,40.90506720542908,1.069995362685662e-05
90891,90892,90891,181783,40.99842119216919,1.0637989688755233e-05
91091,91092,91091,182183,41.08807325363159,1.0576978793842233e-05
91291,91292,91291,182583,41.17828035354614,1.0519428315203072e-05
91491,91492,91491,182983,41.273818254470825,1.0460205544327225e-05
91692,91693,91692,183385,41.373125314712524,1.0399279010932019e-05
91892,91893,91892,183785,41.46453809738159,1.0338077800684421e-05
92092,92093,92092,184185,41.55148434638977,1.0279236108530647e-05
92292,92293,92292,184585,41.63846826553345,1.0222595426219058e-05
92492,92493,92492,184985,41.729570150375366,1.0165476590759664e-05
92693,92694,92693,185387,41.82087826728821,1.0106965946968143e-05
92893,92894,92893,185787,41.91093301773071,1.0047979093423436e-05
93093,93094,93093,186187,42.01155924797058,9.992029115818428e-06
93293,93294,93293,186587,42.11090421676636,9.936188686266707e-06
93493,93494,93493,186987,42.20409917831421,9.888179843250737e-06
93694,93695,93694,187389,42.29166221618652,9.822220005432028e-06
93894,93895,93894,187789,42.39812135696411,9.766523145870332e-06
94094,94095,94094,188189,42.493778228759766,9.711209007788484e-06
94294,94295,94294,188589,42.592668294906616,9.656566854886302e-06
94494,94495,94494,188989,42.69567322731018,9.601785480860508e-06
94695,94696,94695,189391,42.79308319091797,9.545181432049737e-06
94895,94896,94895,189791,42.883384227752686,9.491006241791224e-06
95095,95096,95095,190191,42.97774839401245,9.437170162256242e-06
95295,95296,95295,190591,43.07686519622803,9.385722909177113e-06
95495,95496,95495,190991,43.17552423477173,9.331982594350384e-06
95696,95697,95696,191393,43.27419710159302,9.276436018378357e-06
95896,95897,95896,191793,43.371798038482666,9.22380359591023e-06
96096,96097,96096,192193,43.46268630027771,9.173311425034029e-06
96296,96297,96296,192593,43.564003229141235,9.12304677342077e-06
96496,96497,96496,192993,43.663639068603516,9.076016934642456e-06
96697,96698,96697,193395,43.76241993904114,9.017977783387326e-06
96897,96898,96897,193795,43.85579538345337,8.964977245746173e-06
97097,97098,97097,194195,43.946585178375244,8.915509818162027e-06
97297,97298,97297,194595,44.03918528556824,8.865499485225698e-06
97497,97498,97497,194995,44.135743141174316,8.815651035134451e-06
97698,97699,97698,195397,44.22439503669739,8.763548882829001e-06
97898,97899,97898,195797,44.31154727935791,8.714078811968866e-06
98098,98099,98098,196197,44.397473096847534,8.664748059073114e-06
98298,98299,98298,196597,44.50200414657593,8.617950007077424e-06
98498,98499,98498,196997,44.602713108062744,8.569490594598892e-06
98699,98700,98699,197399,44.6940233707428,8.519496449041145e-06
98899,98900,98899,197799,44.81284022331238,8.469081446068534e-06
99099,99100,99099,198199,44.91015124320984,8.421919303452898e-06
99299,99300,99299,198599,45.0010712146759,8.375832936988574e-06
99499,99500,99499,198999,45.08664131164551,8.327289277030876e-06
99700,99701,99700,199401,45.17001438140869,8.279740604673074e-06
99900,99901,99900,199801,45.254982233047485,8.232556299703297e-06
100100,100101,100100,200201,45.33551001548767,8.187861662788702e-06
100300,100301,100300,200601,45.4224750995636,8.143090911955738e-06
100501,100502,100501,201003,45.50975012779236,8.096226425652079e-06
100701,100702,100701,201403,45.593329191207886,8.047851563498193e-06
100901,100902,100901,201803,45.67242217063904,8.001506353776e-06
101101,101102,101101,202203,45.753419160842896,7.957957067868442e-06
101301,101302,101301,202603,45.83167314529419,7.914362998011838e-06
101502,101503,101502,203005,45.91275906562805,7.868267750736862e-06
101702,101703,101702,203405,45.99980711936951,7.822778572526234e-06
101902,101903,101902,203805,46.08198928833008,7.777997477156777e-06
102102,102103,102102,204205,46.16177725791931,7.735105682221598e-06
102302,102303,102302,204605,46.242027044296265,7.69140113834208e-06
102503,102504,102503,205007,46.32365012168884,7.647265836262396e-06
102703,102704,102703,205407,46.41679835319519,7.6024128769950155e-06
102903,102904,102903,205807,46.50459027290344,7.558557999868285e-06
103103,103104,103103,206207,46.594165086746216,7.5172329858954946e-06
103303,103304,103303,206607,46.695430278778076,7.475667689075542e-06
103504,103505,103504,207009,46.777791023254395,7.433316207017866e-06
103704,103705,103704,207409,46.86339211463928,7.3904607216209005e-06
103904,103905,103904,207809,46.94918608665466,7.3487793982693055e-06
104104,104105,104104,208209,47.0341522693634,7.308695653046114e-06
104304,104305,104304,208609,47.11628532409668,7.267843087453281e-06
104505,104506,104505,209011,47.19780611991882,7.225187486675726e-06
104705,104706,104705,209411,47.28155517578125,7.1847829705377135e-06
104905,104906,104905,209811,47.360255002975464,7.1425970162026215e-06
105105,105106,105105,210211,47.440399169921875,7.102740645568939e-06
105305,105306,105305,210611,47.52539110183716,7.063664662893853e-06
105506,105507,105506,211013,47.60515522956848,7.022931594858061e-06
105706,105707,105706,211413,47.68693828582764,6.983007970698289e-06
105906,105907,105906,211813,47.76656222343445,6.942851370848088e-06
106106,106107,106106,212213,47.84989905357361,6.904054188906401e-06
106306,106307,106306,212613,47.93008732795715,6.866024858623425e-06
106507,106508,106507,213015,48.01617407798767,6.831161309195722e-06
106707,106708,106707,213415,48.09770917892456,6.786716736019232e-06
106907,106908,106907,213815,48.17917013168335,6.747085679167501e-06
107107,107108,107107,214215,48.259138107299805,6.710457176493548e-06
107307,107308,107307,214615,48.34131622314453,6.673894731775271e-06
107508,107509,107508,215017,48.423524141311646,6.634596728957456e-06
107708,107709,107708,215417,48.51013422012329,6.596333389429583e-06
107908,107909,107908,215817,48.591888189315796,6.55875567330477e-06
108108,108109,108108,216217,48.67230796813965,6.521709778577157e-06
108308,108309,108308,216617,48.768097162246704,6.48475646096923e-06
108509,108510,108509,217019,48.86126637458801,6.446957563705855e-06
108709,108710,108709,217419,48.94289422035217,6.410124675273209e-06
108909,108910,108909,217819,49.02840614318848,6.3735047949777245e-06
109109,109110,109109,218219,49.110273122787476,6.3387100395728065e-06
109309,109310,109309,218619,49.18974804878235,6.303264507839649e-06
109510,109511,109510,219021,49.27346730232239,6.26594156040476e-06
109710,109711,109710,219421,49.356210231781006,6.230114679577024e-06
109910,109911,109910,219821,49.44166707992554,6.195392964836623e-06
110110,110111,110110,220221,49.526987075805664,6.160919111543487e-06
110310,110311,110310,220621,49.612834215164185,6.126547435417245e-06
110511,110512,110511,221023,49.6968731880188,6.090908389723805e-06
110711,110712,110711,221423,49.782581090927124,6.056373075441068e-06
110911,110912,110911,221823,49.86642813682556,6.022046526245351e-06
111111,111112,111111,222223,49.953198194503784,5.989234963475322e-06
111311,111312,111311,222623,50.03725004196167,5.9546821462155175e-06
111512,111513,111512,223025,50.121598958969116,5.919971932242254e-06
111712,111713,111712,223425,50.20906329154968,5.885588224794241e-06
111912,111913,111912,223825,50.29168510437012,5.852521556349666e-06
112112,112113,112112,224225,50.37882423400879,5.819652453995612e-06
112312,112313,112312,224625,50.469651222229004,5.786986589682616e-06
112513,112514,112513,225027,50.55397129058838,5.761303188026167e-06
112713,112714,112713,225427,50.64255905151367,5.7209883144942705e-06
112913,112914,112913,225827,50.72891902923584,5.689392897735931e-06
113113,113114,113113,226227,50.827126026153564,5.658430138208078e-06
113313,113314,113313,226627,50.93534517288208,5.626163438732719e-06
113514,113515,113514,227029,51.0314781665802,5.59329222763666e-06
113714,113715,113714,227429,51.11634111404419,5.560483086520448e-06
113914,113915,113914,227829,51.207160234451294,5.529595917532374e-06
114114,114115,114114,228229,51.29783320426941,5.498878527221582e-06
114314,114315,114314,228629,51.38554120063782,5.467604774574579e-06
114515,114516,114515,229031,51.48664927482605,5.436039426810836e-06
114715,114716,114715,229431,51.57849717140198,5.404885074361433e-06
114915,114916,114915,229831,51.68083620071411,5.37465957030492e-06
115115,115116,115115,230231,51.822256326675415,5.344551722224886e-06
115315,115316,115315,230631,51.924217224121094,5.3139674276703164e-06
115516,115517,115516,231033,52.03352117538452,5.282484136343555e-06
115716,115717,115716,231433,52.12432932853699,5.252167052581579e-06
115916,115917,115916,231833,52.22235631942749,5.2225895859792976e-06
116116,116117,116116,232233,52.31183838844299,5.193619933992208e-06
116316,116317,116316,232633,52.40067410469055,5.163634391351634e-06
116517,116518,116517,233035,52.49454426765442,5.133862547879912e-06
116717,116718,116717,233435,52.586546182632446,5.104173935153621e-06
116917,116918,116917,233835,52.676539182662964,5.075048980562166e-06
117117,117118,117117,234235,52.765629291534424,5.0469882079925365e-06
117317,117318,117317,234635,52.85749316215515,5.018754647973475e-06
117518,117519,117518,235037,52.9489221572876,4.989883322961416e-06
117718,117719,117718,235437,53.052213191986084,4.960454651475315e-06
117918,117919,117918,235837,53.15244126319885,4.9333725433021495e-06
118118,118119,118118,236237,53.239437103271484,4.906215436775493e-06
118318,118319,118318,236637,53.33315300941467,4.878549755850128e-06
118519,118520,118519,237039,53.438016176223755,4.849999058121794e-06
118719,118720,118719,237439,53.53287220001221,4.8222777819013e-06
118919,118920,118919,237839,53.6273992061615,4.795527613240651e-06
119119,119120,119119,238239,53.7214732170105,4.769372596404722e-06
119319,119320,119319,238639,53.81100630760193,4.7420195749754784e-06
119520,119521,119520,239041,53.89844512939453,4.714145423391133e-06
119720,119721,119720,239441,53.993834018707275,4.68744748784577e-06
119920,119921,119920,239841,54.08727812767029,4.661452050644872e-06
120120,120121,120120,240241,54.178460359573364,4.635832608636287e-06
120320,120321,120320,240641,54.26636624336243,4.608816707570432e-06
120521,120522,120521,241043,54.35849714279175,4.582145810216974e-06
120721,120722,120721,241443,54.45196533203125,4.557121301219853e-06
120921,120922,120921,241843,54.54093813896179,4.53207321944241e-06
121121,121122,121121,242243,54.633501291275024,4.506712853053064e-06
121321,121322,121321,242643,54.73170518875122,4.480349117063416e-06
121522,121523,121522,243045,54.828819274902344,4.4554788836808854e-06
121722,121723,121722,243445,54.91991710662842,4.429815612875676e-06
121922,121923,121922,243845,55.01193809509277,4.404986312075987e-06
122122,122123,122122,244245,55.10078001022339,4.3807255256023425e-06
122322,122323,122322,244645,55.21037721633911,4.355918356725533e-06
122523,122524,122523,245047,55.30659317970276,4.330151175773273e-06
122723,122724,122723,245447,55.40895915031433,4.305382257365376e-06
122923,122924,122923,245847,55.4962272644043,4.281954035529351e-06
123123,123124,123123,246247,55.581159353256226,4.258066003107592e-06
123323,123324,123323,246647,55.671040058135986,4.234807829512278e-06
123524,123525,123524,247049,55.755115032196045,4.209306584459531e-06
123724,123725,123724,247449,55.84262228012085,4.1850994300822315e-06
123924,123925,123924,247849,55.9251503944397,4.162027353551061e-06
124124,124125,124124,248249,56.016584396362305,4.138511605945008e-06
124324,124325,124324,248649,56.10177421569824,4.1142411309897794e-06
124525,124526,124525,249051,56.18327021598816,4.090216506405872e-06
124725,124726,124725,249451,56.26347327232361,4.0672064586146996e-06
124925,124926,124925,249851,56.347331047058105,4.044312350661372e-06
125125,125126,125125,250251,56.42869305610657,4.021473262463542e-06
125325,125326,125325,250651,56.51269316673279,3.998615972002192e-06
125526,125527,125526,251053,56.597246408462524,3.974866067594163e-06
125726,125727,125726,251453,56.679646253585815,3.952386089389956e-06
125926,125927,125926,251853,56.75952625274658,3.930279568985189e-06
126126,126127,126126,252253,56.840665102005005,3.908425677116255e-06
126326,126327,126326,252653,56.92083215713501,3.8853745473425175e-06
126527,126528,126527,253055,57.01153206825256,3.862763463840644e-06
126727,126728,126727,253455,57.09730815887451,3.841000728521865e-06
126927,126928,126927,253855,57.17815828323364,3.819576216189526e-06
127127,127128,127127,254255,57.26222324371338,3.798158847496963e-06
127327,127328,127327,254655,57.361873149871826,3.7774076703632913e-06
127528,127529,127528,255057,57.44834518432617,3.75443117023806e-06
127728,127729,127728,255457,57.530511140823364,3.7329396374982485e-06
127928,127929,127928,255857,57.61095333099365,3.7123139046352756e-06
128128,128129,128128,256257,57.692867279052734,3.6913673064958397e-06
128328,128329,128328,256657,57.77237915992737,3.6703484167712795e-06
128529,128530,128529,257059,57.853761196136475,3.64871700757102e-06
128729,128730,128729,257459,57.936909198760986,3.6282191666943833e-06
128929,128930,128929,257859,58.02786922454834,3.608326582631187e-06
129129,129130,129129,258259,58.10923218727112,3.587862519135937e-06
129329,129330,129329,258659,58.188711166381836,3.567497511752732e-06
129530,129531,129530,259061,58.268033027648926,3.5463680175267706e-06
129730,129731,129730,259461,58.35261631011963,3.526806613637431e-06
129930,129931,129930,259861,58.43675112724304,3.507040998849397e-06
130130,130131,130130,260261,58.51893711090088,3.4873589432489304e-06
130330,130331,130330,260661,58.603127241134644,3.467121896273956e-06
130531,130532,130531,261063,58.68762016296387,3.4471028983850092e-06
130731,130732,130731,261463,58.768731117248535,3.4272218749924875e-06
130931,130932,130931,261863,58.849626302719116,3.408373109611838e-06
131131,131132,131131,262263,58.93136429786682,3.3888258036825796e-06
131331,131332,131331,262663,59.019240379333496,3.370022053174968e-06
131532,131533,131532,263065,59.10644721984863,3.349740448428859e-06
131732,131733,131732,263465,59.18827700614929,3.3311533741821176e-06
131932,131933,131932,263865,59.269222259521484,3.3123546732014664e-06
132132,132133,132132,264265,59.35318398475647,3.294216828231353e-06
132332,132333,132332,264665,59.45107936859131,3.2746188997900226e-06
132533,132534,132533,265067,59.544440269470215,3.2564814371836964e-06
132733,132734,132733,265467,59.6243052482605,3.2381577745146836e-06
132933,132934,132933,265867,59.70670533180237,3.2202873466823e-06
133133,133134,133133,266267,59.78807020187378,3.2020437662962715e-06
133333,133334,133333,266667,59.868343114852905,3.1833013017315015e-06
133534,133535,133534,267069,59.95253825187683,3.165538512896137e-06
133734,133735,133734,267469,60.03793931007385,3.147936966649231e-06
133934,133935,133934,267869,60.1218900680542,3.130525836772855e-06
134134,134135,134134,268269,60.20272731781006,3.1128261226792207e-06
134334,134335,134334,268669,60.2862069606781,3.094539206919594e-06
134535,134536,134535,269071,60.368030309677124,3.0764632467627773e-06
134735,134736,134735,269471,60.45102524757385,3.0591994206220575e-06
134935,134936,134935,269871,60.533467292785645,3.042267653097232e-06
135135,135136,135135,270271,60.614479303359985,3.029664901103961e-06
135335,135336,135335,270671,60.69613003730774,3.0071122277653154e-06
135536,135537,135536,271073,60.77813124656677,2.990187523948622e-06
135736,135737,135736,271473,60.859251976013184,2.9733484074857267e-06
135936,135937,135936,271873,60.94271731376648,2.9573306186851967e-06
136136,136137,136136,272273,61.03611636161804,2.9402991867878705e-06
136336,136337,136336,272673,61.12214517593384,2.9232189941024096e-06
136537,136538,136537,273075,61.20425820350647,2.9062591299551176e-06
136737,136738,136737,273475,61.28866934776306,2.8899228612593216e-06
136937,136938,136937,273875,61.37317609786987,2.8740198165689633e-06
137137,137138,137137,274275,61.457863330841064,2.857682139417256e-06
137337,137338,137337,274675,61.55189228057861,2.8414319596705668e-06
137538,137539,137538,275077,61.65402817726135,2.825357813276045e-06
137738,137739,137738,275477,61.73937940597534,2.809807840002144e-06
137938,137939,137938,275877,61.82424330711365,2.794254403054702e-06
138138,138139,138138,276277,61.90872120857239,2.7780723454245834e-06
138338,138339,138338,276677,62.000731229782104,2.7617434256517622e-06
138539,138540,138539,277079,62.087000131607056,2.745888935792973e-06
138739,138740,138739,277479,62.17082333564758,2.7306118650300285e-06
138939,138940,138939,277879,62.254353284835815,2.7152552841518053e-06
139139,139140,139139,278279,62.33811712265015,2.6995980824671166e-06
139339,139340,139339,278679,62.421884298324585,2.683903841784815e-06
139540,139541,139540,279081,62.51154017448425,2.6689224115844418e-06
139740,139741,139740,279481,62.596100091934204,2.6541026301367727e-06
139940,139941,139940,279881,62.684070348739624,2.639522105128327e-06
140140,140141,140140,280281,62.77025008201599,2.624119251892004e-06
140340,140341,140340,280681,62.855215311050415,2.6089059476600566e-06
140541,140542,140541,281083,62.94090914726257,2.593948506390809e-06
140741,140742,140741,281483,63.02745819091797,2.5793133367035224e-06
140941,140942,140941,281883,63.112969398498535,2.564484466064733e-06
141141,141142,141141,282283,63.19780707359314,2.5498298422342615e-06
141341,141342,141341,282683,63.281222343444824,2.5349893659549536e-06
141542,141543,141542,283085,63.36606526374817,2.5205360191464064e-06
141742,141743,141742,283485,63.45773005485535,2.5066106262036886e-06
141942,141943,141942,283885,63.544188261032104,2.492891297211928e-06
142142,142143,142142,284285,63.62878632545471,2.478543662518289e-06
142342,142343,142342,284685,63.73173713684082,2.4642758108044606e-06
142543,142544,142543,285087,63.82488012313843,2.4503111080130504e-06
142743,142744,142743,285487,63.91644024848938,2.436495898988028e-06
142943,142944,142943,285887,64.0080304145813,2.4231776927164623e-06
143143,143144,143143,286287,64.093985080719,2.4090391102364873e-06
143343,143344,143343,286687,64.18219327926636,2.3946855322819923e-06
143544,143545,143544,287089,64.26683211326599,2.3809877820546917e-06
143744,143745,143744,287489,64.35139107704163,2.368134433118297e-06
143944,143945,143944,287889,64.43585419654846,2.3548396166942888e-06
144144,144145,144144,288289,64.52274417877197,2.341095060031355e-06
144344,144345,144344,288689,64.6108672618866,2.3272029171049934e-06
144545,144546,144545,289091,64.71733713150024,2.313839348283859e-06
144745,144746,144745,289491,64.81882810592651,2.3012678548074625e-06
144945,144946,144945,289891,64.91929030418396,2.288486671191682e-06
145145,145146,145145,290291,65.02398729324341,2.275624022035547e-06
145345,145346,145345,290691,65.12602615356445,2.261827355641338e-06
145546,145547,145546,291093,65.22216701507568,2.24938029762909e-06
145746,145747,145746,291493,65.3068790435791,2.236829167762275e-06
145946,145947,145946,291893,65.39177322387695,2.2242327706517435e-06
146146,146147,146146,292293,65.47965908050537,2.2112506418933274e-06
146346,146347,146346,292693,65.57010006904602,2.1985453376863777e-06
146547,146548,146547,293095,65.65482020378113,2.1860274161723088e-06
146747,146748,146747,293495,65.73876023292542,2.1737610464866753e-06
146947,146948,146947,293895,65.83322525024414,2.1616262951522927e-06
147147,147148,147147,294295,65.9346091747284,2.151126929646245e-06
147347,147348,147347,294695,66.024405002594,2.137008947122713e-06
147548,147549,147548,295097,66.11118006706238,2.124881452027083e-06
147748,147749,147748,295497,66.19579124450684,2.113039070017792e-06
147948,147949,147948,295897,66.27935838699341,2.100782219713635e-06
148148,148149,148148,296297,66.36417818069458,2.088748825141724e-06
148348,148349,148348,296697,66.45030307769775,2.076502686374212e-06
148549,148550,148549,297099,66.53940415382385,2.064735336122421e-06
148749,148750,148749,297499,66.62313604354858,2.0534550687387436e-06
148949,148950,148949,297899,66.70881938934326,2.041851633126925e-06
149149,149150,149149,298299,66.79395198822021,2.030002240236783e-06
149349,149350,149349,298699,66.88272428512573,2.018232044194471e-06
149550,149551,149550,299101,66.97243118286133,2.006900430778905e-06
149750,149751,149750,299501,67.05919528007507,1.9955816065548074e-06
149950,149951,149950,299901,67.14407134056091,1.98423750763542e-06
150150,150151,150150,300301,67.22739315032959,1.972789115227807e-06
150350,150351,150350,300701,67.3109622001648,1.961795532936832e-06
150551,150552,150551,301103,67.39764523506165,1.951381433041126e-06
150751,150752,150751,301503,67.48822617530823,1.9401783392959634e-06
150951,150952,150951,301903,67.57386922836304,1.929333276496591e-06
151151,151152,151151,302303,67.65852427482605,1.9178842374624006e-06
151351,151352,151351,302703,67.7481632232666,1.9070490234917765e-06
151552,151553,151552,303105,67.83478808403015,1.896089291746204e-06
151752,151753,151752,303505,67.91557216644287,1.8856985384355935e-06
151952,151953,151952,303905,68.01843619346619,1.8749630877464356e-06
152152,152153,152152,304305,68.10704922676086,1.8641227771494844e-06
152352,152353,152352,304705,68.19049119949341,1.8532767979950097e-06
152553,152554,152553,305107,68.27241921424866,1.8426994246499879e-06
152753,152754,152753,305507,68.3529462814331,1.8322641373658785e-06
152953,152954,152953,305907,68.43296122550964,1.8219125865047145e-06
153153,153154,153153,306307,68.52345323562622,1.8116113653022025e-06
153353,153354,153353,306707,68.6076431274414,1.8008863212770262e-06
153554,153555,153554,307109,68.69192218780518,1.7909098501926035e-06
153754,153755,153754,307509,68.77533912658691,1.7811143640887083e-06
153954,153955,153954,307909,68.85911417007446,1.7706995870076275e-06
154154,154155,154154,308309,68.94375705718994,1.7602966536502565e-06
154354,154355,154354,308709,69.02685213088989,1.750393814074423e-06
154555,154556,154555,309111,69.10880422592163,1.7405935095661445e-06
154755,154756,154755,309511,69.2007691860199,1.7309545365512805e-06
154955,154956,154955,309911,69.2832441329956,1.7207723281600438e-06
155155,155156,155155,310311,69.36306405067444,1.71095335116057e-06
155355,155356,155355,310711,69.4468641281128,1.7012836024144258e-06
155556,155557,155556,311113,69.53017115592957,1.6918905935332747e-06
155756,155757,155756,311513,69.61179637908936,1.6825843005794104e-06
155956,155957,155956,311913,69.69340324401855,1.6729058890094791e-06
156156,156157,156156,312313,69.77425527572632,1.6636194524444971e-06
156356,156357,156356,312713,69.85610604286194,1.653711939253074e-06
156557,156558,156557,313115,69.94010019302368,1.6444939302208409e-06
156757,156758,156757,313515,70.02695322036743,1.6352911800215729e-06
156957,156958,156957,313915,70.12745809555054,1.6258284698317766e-06
157157,157158,157157,314315,70.21875619888306,1.618368740586243e-06
157357,157358,157357,314715,70.30283808708191,1.6067393543857386e-06
157558,157559,157558,315117,70.38761234283447,1.5977250476711676e-06
157758,157759,157758,315517,70.47188830375671,1.5888757827668538e-06
157958,157959,157958,315917,70.55356311798096,1.5795913004581145e-06
158158,158159,158158,316317,70.63537120819092,1.570608810350478e-06
158358,158359,158358,316717,70.71579122543335,1.5617110188569635e-06
158559,158560,158559,317119,70.79988408088684,1.5528794429914128e-06
158759,158760,158759,317519,70.88253021240234,1.5441675464706106e-06
158959,158960,158959,317919,70.96916818618774,1.535305644798588e-06
159159,159160,159159,318319,71.05104613304138,1.5263321360950432e-06
159359,159360,159359,318719,71.13193917274475,1.5177715565740298e-06
159560,159561,159560,319121,71.21447014808655,1.509384229492866e-06
159760,159761,159760,319521,71.29808735847473,1.5008620845155104e-06
159960,159961,159960,319921,71.38238739967346,1.492269599551294e-06
160160,160161,160160,320321,71.46986222267151,1.4834707498540984e-06
160360,160361,160360,320721,71.55293416976929,1.4749946879052687e-06
160561,160562,160561,321123,71.63887310028076,1.4669138871960282e-06
160761,160762,160761,321523,71.72281122207642,1.458729283316187e-06
160961,160962,160961,321923,71.80681419372559,1.4502849325085294e-06
161161,161162,161161,322323,71.88667011260986,1.4417152147817524e-06
161361,161362,161361,322723,71.97321820259094,1.433496262834744e-06
161562,161563,161562,323125,72.05464720726013,1.4253392282509135e-06
161762,161763,161762,323525,72.13727021217346,1.4171773543585026e-06
161962,161963,161962,323925,72.2316381931305,1.4090352163833686e-06
162162,162163,162162,324325,72.3301842212677,1.4007608036353105e-06
162362,162363,162362,324725,72.41723108291626,1.3930191069323943e-06
162563,162564,162563,325127,72.50107622146606,1.385408610647173e-06
162763,162764,162763,325527,72.58217024803162,1.3776391935560298e-06
162963,162964,162963,325927,72.6654942035675,1.3695410927058486e-06
163163,163164,163163,326327,72.74903130531311,1.361705671488435e-06
163363,163364,163363,326727,72.83518123626709,1.3541468337733352e-06
163564,163565,163564,327129,72.92025423049927,1.3466406455584843e-06
163764,163765,163764,327529,73.01315021514893,1.3396506712546759e-06
163964,163965,163964,327929,73.0967812538147,1.3310884658048107e-06
164164,164165,164164,328329,73.18311929702759,1.323705287918419e-06
164364,164365,164364,328729,73.26453232765198,1.3160237064158271e-06
164565,164566,164565,329131,73.35499334335327,1.3087070040440991e-06
164765,164766,164765,329531,73.4385621547699,1.3013563882263244e-06
164965,164966,164965,329931,73.52450513839722,1.293682160063805e-06
165165,165166,165165,330331,73.60887122154236,1.2863540017328635e-06
165365,165366,165365,330731,73.693852186203,1.2790972851853344e-06
165566,165567,165566,331133,73.7794680595398,1.2720229469069562e-06
165766,165767,165766,331533,73.86330604553223,1.2645975261853332e-06
165966,165967,165966,331933,73.9543821811676,1.2574254102904896e-06
166166,166167,166166,332333,74.03971219062805,1.2502970852412562e-06
166366,166367,166366,332733,74.12403321266174,1.243201792165125e-06
166567,166568,166567,333135,74.20994019508362,1.2362991437277558e-06
166767,166768,166767,333535,74.29239821434021,1.229181530098369e-06
166967,166968,166967,333935,74.39245319366455,1.2220104192229843e-06
167167,167168,167167,334335,74.49317717552185,1.215107685643783e-06
167367,167368,167367,334735,74.5774872303009,1.2084285586683026e-06
167568,167569,167568,335137,74.66306209564209,1.2016796159513486e-06
167768,167769,167768,335537,74.7453281879425,1.194753447166928e-06
167968,167969,167968,335937,74.83089828491211,1.1879011243063643e-06
168168,168169,168168,336337,74.9145781993866,1.1811101859234309e-06
168368,168369,168368,336737,75.00385618209839,1.1743978693841215e-06
168569,168570,168569,337139,75.09056997299194,1.1677525890106903e-06
168769,168770,168769,337539,75.17265725135803,1.1609821434926218e-06
168969,168970,168969,337939,75.25789523124695,1.1545172614384433e-06
169169,169170,169169,338339,75.34411597251892,1.1478393542035605e-06
169369,169370,169369,338739,75.4303343296051,1.1413134343205205e-06
169570,169571,169570,339141,75.51909613609314,1.1348085554437323e-06
169770,169771,169770,339541,75.60366916656494,1.1283247118979894e-06
169970,169971,169970,339941,75.68957114219666,1.1216969098350833e-06
170170,170171,170170,340341,75.77269911766052,1.1154101765609897e-06
170370,170371,170370,340741,75.8593909740448,1.1091514981415845e-06
170571,170572,170571,341143,75.95056319236755,1.1030735539157273e-06
170771,170772,170771,341543,76.04130029678345,1.0969246157260208e-06
170971,170972,170971,341943,76.13083910942078,1.0903969783507227e-06
171171,171172,171171,342343,76.22507524490356,1.084074278344191e-06
171371,171372,171371,342743,76.3136613368988,1.0781296401053813e-06
171572,171573,171572,343145,76.41091322898865,1.0721365407258387e-06
171772,171773,171772,343545,76.51547908782959,1.0660123391442508e-06
171972,171973,171972,343945,76.61334133148193,1.0597118778765552e-06
172172,172173,172172,344345,76.69817018508911,1.0537316470694623e-06
172372,172373,172372,344745,76.78634810447693,1.0479812427289459e-06
172573,172574,172573,345147,76.87309622764587,1.0420043751657023e-06
172773,172774,172773,345547,76.96471619606018,1.0359569363089506e-06
172973,172974,172973,345947,77.05447506904602,1.0300347057521302e-06
173173,173174,173173,346347,77.14677715301514,1.0240676695724767e-06
173373,173374,173373,346747,77.23544025421143,1.018367613584667e-06
173574,173575,173574,347149,77.32656121253967,1.0126565989746515e-06
173774,173775,173774,347549,77.41710019111633,1.0069378287980792e-06
173974,173975,173974,347949,77.51365399360657,1.0009584897469769e-06
174174,174175,174174,348349,77.60151505470276,9.9526863722283e-07
174374,174375,174374,348749,77.69118738174438,9.896905560489258e-07
174575,174576,174575,349151,77.7815523147583,9.841965770004544e-07
174775,174776,174775,349551,77.86895632743835,9.785847893980665e-07
174975,174976,174975,349951,77.95851922035217,9.729713271939889e-07
175175,175176,175175,350351,78.04887914657593,9.67434579833167e-07
175375,175376,175375,350751,78.14032530784607,9.621580873898784e-07
175576,175577,175576,351153,78.22319626808167,9.567406696831976e-07
175776,175777,175776,351553,78.30948209762573,9.514092090496734e-07
175976,175977,175976,351953,78.39351320266724,9.458702194952806e-07
176176,176177,176176,352353,78.48345422744751,9.404131409160448e-07
176376,176377,176376,352753,78.56807398796082,9.351040730747422e-07
176577,176578,176577,353155,78.67342615127563,9.297711726256543e-07
176777,176778,176777,353555,78.76823234558105,9.244347252873792e-07
176977,176978,176977,353955,78.85048127174377,9.189835080894896e-07
177177,177178,177177,354355,78.93354225158691,9.137048423938579e-07
177377,177378,177377,354755,79.02119517326355,9.087381221152103e-07
177578,177579,177578,355157,79.10580205917358,9.035499664885918e-07
177778,177779,177778,355557,79.18887519836426,8.988208864982556e-07
177978,177979,177978,355957,79.27180218696594,8.931433401258064e-07
178178,178179,178178,356357,79.35419917106628,8.88217220107514e-07
178378,178379,178378,356757,79.44062328338623,8.833870022013993e-07
178579,178580,178579,357159,79.52743029594421,8.783014637941094e-07
178779,178780,178779,357559,79.61257028579712,8.731778758467085e-07
178979,178980,178979,357959,79.69666814804077,8.682153073103946e-07
179179,179180,179179,358359,79.77777814865112,8.632622826504102e-07
179379,179380,179379,358759,79.85971403121948,8.585086205329206e-07
179580,179581,179580,359161,79.94281721115112,8.535715903474609e-07
179780,179781,179780,359561,80.0290641784668,8.488045755539175e-07
179980,179981,179980,359961,80.11285305023193,8.43735664859004e-07
180180,180181,180180,360361,80.19827508926392,8.390635844414143e-07
180380,180381,180380,360761,80.28178215026855,8.343654711936556e-07
180581,180582,180581,361163,80.3748049736023,8.295917085084299e-07
180781,180782,180781,361563,80.45827031135559,8.247359812657187e-07
180981,180982,180981,361963,80.5426230430603,8.199624027656454e-07
181181,181182,181181,362363,80.63252711296082,8.152774409615655e-07
181381,181382,181381,362763,80.71852707862854,8.10818265342465e-07
181582,181583,181582,363165,80.82114100456238,8.061483218654954e-07
181782,181783,181782,363565,80.90704822540283,8.014186109194501e-07
181982,181983,181982,363965,80.99162697792053,7.966942973198168e-07
182182,182183,182182,364365,81.08420825004578,7.923019482382126e-07
182382,182383,182382,364765,81.1715440750122,7.878994990193921e-07
182583,182584,182583,365167,81.25319719314575,7.833626112886265e-07
182783,182784,182783,365567,81.33611226081848,7.790971272303747e-07
182983,182984,182983,365967,81.41890406608582,7.743870722857946e-07
183183,183184,183183,366367,81.50921130180359,7.700228492843724e-07
183383,183384,183383,366767,81.59558033943176,7.656999658276006e-07
183584,183585,183584,367169,81.68667912483215,7.613295380249383e-07
183784,183785,183784,367569,81.78168320655823,7.568606673573515e-07
183984,183985,183984,367969,81.86837816238403,7.52433361813907e-07
184184,184185,184184,368369,81.9528021812439,7.482265273240532e-07
184384,184385,184384,368769,82.03949809074402,7.440239782120753e-07
184585,184586,184585,369171,82.12498617172241,7.398498631444622e-07
184785,184786,184785,369571,82.210125207901,7.35694108615847e-07
184985,184986,184985,369971,82.29050421714783,7.313266299648924e-07
185185,185186,185185,370371,82.37285304069519,7.272369133182928e-07
185385,185386,185385,370771,82.45696115493774,7.231025316213001e-07
185586,185587,185586,371173,82.54091715812683,7.190787341995408e-07
185786,185787,185786,371573,82.62648010253906,7.148656406098845e-07
185986,185987,185986,371973,82.7092490196228,7.107791952803422e-07
186186,186187,186186,372373,82.79500126838684,7.067740523380568e-07
186386,186387,186386,372773,82.88611721992493,7.028546932199119e-07
186587,186588,186587,373175,82.9913432598114,6.994423345264101e-07
186787,186788,186787,373575,83.07317018508911,6.94835256838561e-07
186987,186988,186987,373975,83.15543341636658,6.90798797463085e-07
187187,187188,187187,374375,83.23738598823547,6.868985106011215e-07
187387,187388,187387,374775,83.31937408447266,6.83150056231658e-07
187588,187589,187588,375177,83.40254521369934,6.791958547894463e-07
187788,187789,187788,375577,83.4896183013916,6.752142021811029e-07
187988,187989,187988,375977,83.57182216644287,6.712707412703946e-07
188188,188189,188188,376377,83.65272331237793,6.676213378443125e-07
188388,188389,188388,376777,83.73511719703674,6.63861842528099e-07
188589,188590,188589,377179,83.81949639320374,6.599675066056163e-07
188789,188790,188789,377579,83.90352511405945,6.561611078041058e-07
188989,188990,188989,377979,83.98798727989197,6.525168518915859e-07
189189,189190,189189,378379,84.07259631156921,6.489438035948672e-07
189389,189390,189389,378779,84.15499210357666,6.452057207741219e-07
189590,189591,189590,379181,84.23464822769165,6.414828022347998e-07
189790,189791,189790,379581,84.31692004203796,6.379218627081438e-07
189990,189991,189990,379981,84.39945030212402,6.341534624299936e-07
190190,190191,190190,380381,84.48668217658997,6.305996198821383e-07
190390,190391,190390,380781,84.5701732635498,6.270795524012682e-07
190591,190592,190591,381183,84.65944814682007,6.235004520639838e-07
190791,190792,190791,381583,84.74176216125488,6.19802914747599e-07
190991,190992,190991,381983,84.82805728912354,6.16311345231977e-07
191191,191192,191191,382383,84.91150307655334,6.12930597550132e-07
191391,191392,191391,382783,85.00691413879395,6.094311973779521e-07
191592,191593,191592,383185,85.11287331581116,6.059591644938298e-07
191792,191793,191792,383585,85.19695115089417,6.023656603796567e-07
191992,191993,191992,383985,85.28079223632812,5.989395263239582e-07
192192,192193,192192,384385,85.36564016342163,5.956833716031137e-07
192392,192393,192392,384785,85.45174407958984,5.924392465923274e-07
192593,192594,192593,385187,85.53754806518555,5.889510172922747e-07
192793,192794,192793,385587,85.62152028083801,5.855765487780605e-07
192993,192994,192993,385987,85.705313205719,5.822954106317591e-07
193193,193194,193193,386387,85.78813004493713,5.791414083868989e-07
193393,193394,193393,386787,85.87448906898499,5.759362043870781e-07
193594,193595,193594,387189,85.96216917037964,5.72539815660154e-07
193794,193795,193794,387589,86.04885125160217,5.693783562355431e-07
193994,193995,193994,387989,86.13573503494263,5.661114582370183e-07
194194,194195,194194,388389,86.22248220443726,5.630425224663886e-07
194394,194395,194394,388789,86.30280923843384,5.599084046997841e-07
194595,194596,194595,389191,86.3889410495758,5.566337895315287e-07
194795,194796,194795,389591,86.4788122177124,5.534270201112066e-07
194995,194996,194995,389991,86.56181716918945,5.503048952815871e-07
195195,195196,195195,390391,86.64605331420898,5.473687590676287e-07
195395,195396,195395,390791,86.72925329208374,5.44254787735938e-07
195596,195597,195596,391193,86.8123242855072,5.410624280695706e-07
195796,195797,195796,391593,86.89521217346191,5.379968787457807e-07
195996,195997,195996,391993,86.9868233203888,5.349279576888236e-07
196196,196197,196196,392393,87.07024931907654,5.319565892269288e-07
196396,196397,196396,392793,87.16988706588745,5.289533801549177e-07
196597,196598,196597,393195,87.27372908592224,5.258412149092268e-07
196797,196798,196797,393595,87.36277914047241,5.228466904680187e-07
196997,196998,196997,393995,87.45530605316162,5.198050756252843e-07
197197,197198,197197,394395,87.54201436042786,5.169894968839095e-07
197397,197398,197397,394795,87.63115429878235,5.14023018605938e-07
197598,197599,197598,395197,87.72147727012634,5.1098066775506e-07
197798,197799,197798,395597,87.80976819992065,5.081093523268522e-07
197998,197999,197998,395997,87.89838719367981,5.052262276137409e-07
198198,198199,198198,396397,87.98861122131348,5.024005016115388e-07
198398,198399,198398,396797,88.07749819755554,4.995611789583819e-07
198599,198600,198599,397199,88.17024111747742,4.965828284980772e-07
198799,198800,198799,397599,88.25665616989136,4.936393280495487e-07
198999,199000,198999,397999,88.34202814102173,4.909466866543911e-07
199199,199200,199199,398399,88.42644810676575,4.881870538851842e-07
199399,199400,199399,398799,88.51781725883484,4.853742564905798e-07
199600,199601,199600,399201,88.60183715820312,4.8251840039751e-07
199800,199801,199800,399601,88.6873950958252,4.797568227500172e-07
200000,200001,200000,400001,88.77694797515869,4.77107858322766e-07


==> extragradient/plot_data/bilinear_matrix_game_n250/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00047588348388671875,2.0175302852282635
100,201,200,401,0.07272672653198242,0.03870059256068895
200,401,400,801,0.1674938201904297,0.0179642168274124
300,601,600,1201,0.2631378173828125,0.010215612352113134
400,801,800,1601,0.3383307456970215,0.006414884987572114
501,1003,1002,2005,0.401430606842041,0.004292887866686561
601,1203,1202,2405,0.4629027843475342,0.0031981848552840673
701,1403,1402,2805,0.5230207443237305,0.0023495755858960704
801,1603,1602,3205,0.5862510204315186,0.0017642014700653555
901,1803,1802,3605,0.6527140140533447,0.0013107140383380224
1001,2003,2002,4005,0.7124638557434082,0.0010771361342336561
1101,2203,2202,4405,0.773129940032959,0.0008891647471929582
1201,2403,2402,4805,0.8368008136749268,0.0007896238285358858
1301,2603,2602,5205,0.897061824798584,0.0007243730865874144
1401,2803,2802,5605,0.9626357555389404,0.000648621889859143
1502,3005,3004,6009,1.0246357917785645,0.000605342378155228
1602,3205,3204,6409,1.0892417430877686,0.0005733026994351765
1702,3405,3404,6809,1.1666560173034668,0.0005447368428944139
1802,3605,3604,7209,1.2288289070129395,0.00048258186702094223
1902,3805,3804,7609,1.294442892074585,0.00043623502306099424
2002,4005,4004,8009,1.3591816425323486,0.0004039543762459166
2102,4205,4204,8409,1.425360918045044,0.00037891678446560513
2202,4405,4404,8809,1.4932479858398438,0.00035856970156738626
2302,4605,4604,9209,1.5671398639678955,0.00034167885404962273
2402,4805,4804,9609,1.6504325866699219,0.000327471216222133
2503,5007,5006,10013,1.7211709022521973,0.00031528514633575623
2603,5207,5206,10413,1.7851316928863525,0.00030494059155017047
2703,5407,5406,10813,1.8479349613189697,0.0002959793336833732
2803,5607,5606,11213,1.912571907043457,0.0002881403091160926
2903,5807,5806,11613,1.9763097763061523,0.000281214281208699
3003,6007,6006,12013,2.042221784591675,0.0002750331765274161
3103,6207,6206,12413,2.113581657409668,0.00026946189858635845
3203,6407,6406,12813,2.179924964904785,0.00026439183980072673
3303,6607,6606,13213,2.2421817779541016,0.00025973566986274647
3403,6807,6806,13613,2.3085358142852783,0.000255423132572343
3504,7009,7008,14017,2.3710098266601562,0.0002513586896688166
3604,7209,7208,14417,2.4370386600494385,0.0002475768793537788
3704,7409,7408,14817,2.5008208751678467,0.00024399934675541638
3804,7609,7608,15217,2.565274715423584,0.00024059633077260883
3904,7809,7808,15617,2.629607915878296,0.00023734367502605227
4004,8009,8008,16017,2.6918137073516846,0.00023422171215643902
4104,8209,8208,16417,2.756436824798584,0.00023121437386540734
4204,8409,8408,16817,2.8209075927734375,0.00022830848122147552
4304,8609,8608,17217,2.883953809738159,0.0002254931786417318
4404,8809,8808,17617,2.9494547843933105,0.00022275948222810613
4505,9011,9010,18021,3.015483856201172,0.0002200736757568169
4605,9211,9210,18421,3.0785017013549805,0.00021748264631160484
4705,9411,9410,18821,3.148026704788208,0.00021495419299109208
4805,9611,9610,19221,3.212247848510742,0.00021248387115568304
4905,9811,9810,19621,3.2781167030334473,0.0002100678928804713
5005,10011,10010,20021,3.341017723083496,0.00020770300764981782
5105,10211,10210,20421,3.4063117504119873,0.00020538640619713179
5205,10411,10410,20821,3.469348907470703,0.0002031156428412569
5305,10611,10610,21221,3.533604860305786,0.00020088857263204926
5405,10811,10810,21621,3.6030948162078857,0.0001987033003656253
5506,11013,11012,22025,3.6710116863250732,0.00019653688483370254
5606,11213,11212,22425,3.7486836910247803,0.00019443070110695764
5706,11413,11412,22825,3.8196768760681152,0.0001923617375405541
5806,11613,11612,23225,3.8810906410217285,0.0001903287540892684
5906,11813,11812,23625,3.941903829574585,0.00018833061625778637
6006,12013,12012,24025,4.002641916275024,0.00018636627982224012
6106,12213,12212,24425,4.0656418800354,0.00018443477820151422
6206,12413,12412,24825,4.13269567489624,0.00018253521198341002
6306,12613,12612,25225,4.195744752883911,0.00018066674020936473
6406,12813,12812,25625,4.255319833755493,0.00017882857309627258
6507,13015,13014,26029,4.320741891860962,0.0001770020267232668
6607,13215,13214,26429,4.382824897766113,0.00017522255984983156
6707,13415,13414,26829,4.44559383392334,0.0001734712724405494
6807,13615,13614,27229,4.511922836303711,0.0001717475275193629
6907,13815,13814,27629,4.592723846435547,0.00017005071684054419
7007,14015,14014,28029,4.674487829208374,0.00016838025819878897
7107,14215,14214,28429,4.7548627853393555,0.00016673559311093918
7207,14415,14414,28829,4.8321616649627686,0.00016511618481099277
7307,14615,14614,29229,4.9103429317474365,0.000163521516504671
7407,14815,14814,29629,4.985045909881592,0.00016195108984464797
7508,15017,15016,30033,5.062867879867554,0.0001603890753312936
7608,15217,15216,30433,5.1423118114471436,0.0001588659348191652
7708,15417,15416,30833,5.217313766479492,0.00015736563452041881
7808,15617,15616,31233,5.288184881210327,0.00015588773806327232
7908,15817,15816,31633,5.359011888504028,0.00015443182216535014
8008,16017,16016,32033,5.428246021270752,0.0001529974758801278
8108,16217,16216,32433,5.505482912063599,0.00015158429991368803
8208,16417,16416,32833,5.577248811721802,0.00015019190600647155
8308,16617,16616,33233,5.655069828033447,0.00014881991636835176
8408,16817,16816,33633,5.72034478187561,0.00014746796316294591
8509,17019,17018,34037,5.783164978027344,0.00014612246346770548
8609,17219,17218,34437,5.862015962600708,0.00014480970865508907
8709,17419,17418,34837,5.938431978225708,0.0001435159385685191
8809,17619,17618,35237,6.001131057739258,0.00014224082088285596
8909,17819,17818,35637,6.074168682098389,0.0001409840311898774
9009,18019,18018,36037,6.145569801330566,0.00013974525267497582
9109,18219,18218,36437,6.208853006362915,0.00013852417581637554
9209,18419,18418,36837,6.2771687507629395,0.00013732049810336562
9309,18619,18618,37237,6.345607757568359,0.00013613392377165485
9409,18819,18818,37637,6.411422967910767,0.0001349641635563538
9510,19021,19020,38041,6.475384712219238,0.00013379948470752128
9610,19221,19220,38441,6.539919853210449,0.00013266267093725852
9710,19421,19420,38841,6.6088478565216064,0.0001315418375357308
9810,19621,19620,39241,6.679074764251709,0.00013043671908828831
9910,19821,19820,39641,6.750177621841431,0.00012934705563775144
10010,20021,20020,40041,6.822494983673096,0.00012827259250720958
10110,20221,20220,40441,6.901018857955933,0.0001272130801360416
10210,20421,20420,40841,6.977330923080444,0.0001261682739210451
10310,20621,20620,41241,7.046806812286377,0.00012513793406670548
10410,20821,20820,41641,7.117313623428345,0.00012412182544308851
10511,21023,21022,42045,7.181934833526611,0.00012310976630411754
10611,21223,21222,42445,7.253396987915039,0.00012212156935771686
10711,21423,21422,42845,7.322274684906006,0.00012114692271993615
10811,21623,21622,43245,7.386224746704102,0.000120185608667928
10911,21823,21822,43645,7.451824903488159,0.00011923741352364664
11011,22023,22022,44045,7.514302968978882,0.00011830212754717816
11111,22223,22222,44445,7.577594757080078,0.00011737954483300902
11211,22423,22422,44845,7.649980783462524,0.00011646946321229426
11311,22623,22622,45245,7.7232208251953125,0.00011557168415702394
11411,22823,22822,45645,7.80270791053772,0.00011468601269024659
11512,23025,23024,46049,7.872832775115967,0.00011380357928193565
11612,23225,23224,46449,7.945671796798706,0.00011294166817294914
11712,23425,23424,46849,8.025213956832886,0.00011209129834021222
11812,23625,23624,47249,8.10024881362915,0.00011125228820360766
11912,23825,23824,47649,8.164610862731934,0.00011042445932999713
12012,24025,24024,48049,8.229391813278198,0.0001096076363612358
12112,24225,24224,48449,8.295880794525146,0.00010880164694508419
12212,24425,24424,48849,8.371251821517944,0.00010800632166848759
12312,24625,24624,49249,8.445003032684326,0.00010722149399299883
12412,24825,24824,49649,8.50806975364685,0.00010644700019297531
12513,25027,25026,50053,8.574897766113281,0.00010567508692150307
12613,25227,25226,50453,8.651501655578613,0.00010492088000252017
12713,25427,25426,50853,8.729159832000732,0.00010417653052252305
12813,25627,25626,51253,8.804819822311401,0.00010344188545014195
12913,25827,25826,51653,8.875765800476074,0.00010271679428441283
13013,26027,26026,52053,8.959142923355103,0.0001020011090041051
13113,26227,26226,52453,9.0274658203125,0.00010129468401762708
13213,26427,26426,52853,9.090668678283691,0.00010059737611571367
13313,26627,26626,53253,9.155654907226562,9.990904442504029e-05
13413,26827,26826,53653,9.218154907226562,9.922955036211032e-05
13514,27029,27028,54057,9.30608081817627,9.855209314758345e-05
13614,27229,27228,54457,9.400410890579224,9.788995253410103e-05
13714,27429,27428,54857,9.498633861541748,9.723624579831776e-05
13814,27629,27628,55257,9.611552715301514,9.659084311227403e-05
13914,27829,27828,55657,9.701282739639282,9.595361673015083e-05
14014,28029,28028,56057,9.787440776824951,9.532444095068601e-05
14114,28229,28228,56457,9.876288652420044,9.470319207907087e-05
14214,28429,28428,56857,9.96551775932312,9.408974839206253e-05
14314,28629,28628,57257,10.055198907852173,9.348399010080046e-05
14414,28829,28828,57657,10.140354633331299,9.28857993179508e-05
14515,29031,29030,58061,10.21906590461731,9.228918987302865e-05
14615,29231,29230,58461,10.284523725509644,9.170586068479885e-05
14715,29431,29430,58861,10.353298902511597,9.112975530307399e-05
14815,29631,29630,59261,10.420745849609375,9.056076313423452e-05
14915,29831,29830,59661,10.487427711486816,8.99987753263165e-05
15015,30031,30030,60061,10.55381989479065,8.94436847378516e-05
15115,30231,30230,60461,10.626414775848389,8.889538590984509e-05
15215,30431,30430,60861,10.692333698272705,8.835377503693193e-05
15315,30631,30630,61261,10.760651588439941,8.78187499394078e-05
15415,30831,30830,61661,10.825255870819092,8.729021003659379e-05
15516,31033,31032,62065,10.89151382446289,8.676286670204717e-05
15616,31233,31232,62465,10.961732864379883,8.624706410975493e-05
15716,31433,31432,62865,11.02937388420105,8.57374533479452e-05
15816,31633,31632,63265,11.09963870048523,8.523393998619012e-05
15916,31833,31832,63665,11.165775775909424,8.473643106529019e-05
16016,32033,32032,64065,11.232435941696167,8.424483507322058e-05
16116,32233,32232,64465,11.299577713012695,8.375906192201825e-05
16216,32433,32432,64865,11.367831707000732,8.327902292558504e-05
16316,32633,32632,65265,11.430197715759277,8.280463077566314e-05
16416,32833,32832,65665,11.496893882751465,8.233579952114378e-05
16517,33035,33034,66069,11.560484886169434,8.186783836882488e-05
16617,33235,33234,66469,11.631219863891602,8.140992988516565e-05
16717,33435,33434,66869,11.698361873626709,8.095733155701019e-05
16817,33635,33634,67269,11.761122703552246,8.050996266081315e-05
16917,33835,33834,67669,11.822941780090332,8.006774372664463e-05
17017,34035,34034,68069,11.886918783187866,7.963059651706329e-05
17117,34235,34234,68469,11.947406768798828,7.919844400880142e-05
17217,34435,34434,68869,12.009092807769775,7.877121037323326e-05
17317,34635,34634,69269,12.068854808807373,7.834882095884943e-05
17417,34835,34834,69669,12.131845712661743,7.793120227196671e-05
17518,35037,35036,70073,12.191683769226074,7.751417624099244e-05
17618,35237,35236,70473,12.264989852905273,7.710592898752043e-05
17718,35437,35436,70873,12.341523885726929,7.670223805725681e-05
17818,35637,35636,71273,12.400407791137695,7.630303442478913e-05
17918,35837,35836,71673,12.46053671836853,7.590825013610193e-05
18018,36037,36036,72073,12.520835876464844,7.551781829324232e-05
18118,36237,36236,72473,12.58266282081604,7.513167303666393e-05
18218,36437,36436,72873,12.648432731628418,7.474974953090994e-05
18318,36637,36636,73273,12.70765495300293,7.437198394798899e-05
18418,36837,36836,73673,12.769538640975952,7.399831345240632e-05
18519,37039,37038,74077,12.831421852111816,7.362499997502704e-05
18619,37239,37238,74477,12.892984867095947,7.325937446272465e-05
18719,37439,37438,74877,12.952471733093262,7.289766074269952e-05
18819,37639,37638,75277,13.012419700622559,7.253979981131108e-05
18919,37839,37838,75677,13.072731733322144,7.2185733583804e-05
19019,38039,38038,76077,13.133089780807495,7.183540488073206e-05
19119,38239,38238,76477,13.19375491142273,7.148875741550155e-05
19219,38439,38438,76877,13.254408836364746,7.114573577934091e-05
19319,38639,38638,77277,13.314326763153076,7.080628542869801e-05
19419,38839,38838,77677,13.373690843582153,7.047035267272691e-05
19520,39041,39040,78081,13.434013843536377,7.013457729963545e-05
19620,39241,39240,78481,13.494062662124634,6.980555587168995e-05
19720,39441,39440,78881,13.557009935379028,6.947989544303976e-05
19820,39641,39640,79281,13.625906944274902,6.915754561282357e-05
19920,39841,39840,79681,13.685525894165039,6.88384567705233e-05
20020,40041,40040,80081,13.746004819869995,6.852258008345205e-05
20120,40241,40240,80481,13.80783987045288,6.820986748509168e-05
20220,40441,40440,80881,13.87239670753479,6.790027166386641e-05
20320,40641,40640,81281,13.932830810546875,6.759374605147888e-05
20420,40841,40840,81681,13.99358582496643,6.729024481193715e-05
20521,41043,41042,82085,14.0553138256073,6.698673250509319e-05
20621,41243,41242,82485,14.11851692199707,6.668917450416247e-05
20721,41443,41442,82885,14.178155660629272,6.639450721864771e-05
20821,41643,41642,83285,14.23722767829895,6.610268763956923e-05
20921,41843,41842,83685,14.296689748764038,6.581367343690462e-05
21021,42043,42042,84085,14.361608982086182,6.552742294888833e-05
21121,42243,42242,84485,14.437617778778076,6.524389517202788e-05
21221,42443,42442,84885,14.505149841308594,6.496304975121927e-05
21321,42643,42642,85285,14.565720796585083,6.468484696983597e-05
21421,42843,42842,85685,14.633960962295532,6.440924774014854e-05
21522,43045,43044,86089,14.695036888122559,6.41334960777934e-05
21622,43245,43244,86489,14.75614881515503,6.38630142401576e-05
21722,43445,43444,86889,14.817907810211182,6.359502200085604e-05
21822,43645,43644,87289,14.879477739334106,6.332948269971798e-05
21922,43845,43844,87689,14.940345764160156,6.30663602598269e-05
22022,44045,44044,88089,15.00441288948059,6.280561917716129e-05
22122,44245,44244,88489,15.064349889755249,6.254722451316279e-05
22222,44445,44444,88889,15.127297639846802,6.229114188589911e-05
22322,44645,44644,89289,15.188875675201416,6.203733746082567e-05
22422,44845,44844,89689,15.252185821533203,6.17857779432218e-05
22523,45047,45046,90093,15.317328929901123,6.15339481577865e-05
22623,45247,45246,90493,15.376502752304077,6.128680232625892e-05
22723,45447,45446,90893,15.435687780380249,6.104180435902917e-05
22823,45647,45646,91293,15.498583793640137,6.0798923043198106e-05
22923,45847,45846,91693,15.559515953063965,6.0558127666077395e-05
23023,46047,46046,92093,15.623236894607544,6.0319388005680966e-05
23123,46247,46246,92493,15.684305906295776,6.008267432479922e-05
23223,46447,46446,92893,15.744663715362549,5.984795736310033e-05
23323,46647,46646,93293,15.805034875869751,5.96152083296387e-05
23423,46847,46846,93693,15.865962982177734,5.938439889501202e-05
23524,47049,47048,94097,15.927655935287476,5.915322176959705e-05
23624,47249,47248,94497,15.987140893936157,5.892622706563186e-05
23724,47449,47448,94897,16.050443649291992,5.870108940807669e-05
23824,47649,47648,95297,16.11430287361145,5.847778225090531e-05
23924,47849,47848,95697,16.17697787284851,5.825627947499746e-05
24024,48049,48048,96097,16.23909878730774,5.803655538210418e-05
24124,48249,48248,96497,16.299139738082886,5.781858468792967e-05
24224,48449,48448,96897,16.361562728881836,5.760234251642121e-05
24324,48649,48648,97297,16.42176079750061,5.7387804392374776e-05
24424,48849,48848,97697,16.489569664001465,5.717494623594152e-05
24525,49051,49050,98101,16.568176746368408,5.696164062245334e-05
24625,49251,49250,98501,16.648170948028564,5.675208792416326e-05
24725,49451,49450,98901,16.709577798843384,5.6544145035742415e-05
24825,49651,49650,99301,16.771440744400024,5.633778939997808e-05
24925,49851,49850,99701,16.834394693374634,5.613299882503801e-05
25025,50051,50050,100101,16.895659685134888,5.592975147842594e-05
25125,50251,50250,100501,16.956289768218994,5.5728025881110405e-05
25225,50451,50450,100901,17.020992040634155,5.552780090197602e-05
25325,50651,50650,101301,17.083465814590454,5.532905575236193e-05
25425,50851,50850,101701,17.14965581893921,5.5131769980631085e-05
25526,51053,51052,102105,17.211790800094604,5.493397220296787e-05
25626,51253,51252,102505,17.27417278289795,5.473955924971031e-05
25726,51453,51452,102905,17.3357937335968,5.454654609613513e-05
25826,51653,51652,103305,17.396607875823975,5.435491358867113e-05
25926,51853,51852,103705,17.458869695663452,5.416464288595694e-05
26026,52053,52052,104105,17.521105766296387,5.3975715451758205e-05
26126,52253,52252,104505,17.584826707839966,5.378811305171785e-05
26226,52453,52452,104905,17.652232885360718,5.360181774731357e-05
26326,52653,52652,105305,17.714491844177246,5.34168118919679e-05
26426,52853,52852,105705,17.779160737991333,5.323307812581171e-05
26527,53055,53054,106109,17.842590808868408,5.304878086415723e-05
26627,53255,53254,106509,17.90602397918701,5.2867552619982375e-05
26727,53455,53454,106909,17.968557834625244,5.2687545897219964e-05
26827,53655,53654,107309,18.031638622283936,5.250874444120578e-05
26927,53855,53854,107709,18.097718715667725,5.2331132261406814e-05
27027,54055,54054,108109,18.163861989974976,5.215469362782098e-05
27127,54255,54254,108509,18.226041793823242,5.197941306635809e-05
27227,54455,54454,108909,18.288907766342163,5.1805275354476744e-05
27327,54655,54654,109309,18.352965831756592,5.1632265517846414e-05
27427,54855,54854,109709,18.417703866958618,5.1460368825518695e-05
27528,55057,55056,110113,18.48016881942749,5.1287868306265416e-05
27628,55257,55256,110513,18.54567575454712,5.111816543831433e-05
27728,55457,55456,110913,18.618793964385986,5.09495328064174e-05
27828,55657,55656,111313,18.697121620178223,5.078195661803489e-05
27928,55857,55856,111713,18.766775846481323,5.0615423305065665e-05
28028,56057,56056,112113,18.831172704696655,5.0449919519951715e-05
28128,56257,56256,112513,18.895862817764282,5.028543213283578e-05
28228,56457,56456,112913,18.958630800247192,5.012194822687067e-05
28328,56657,56656,113313,19.0207040309906,4.995945509631485e-05
28428,56857,56856,113713,19.084012746810913,4.9797940240634196e-05
28529,57059,57058,114117,19.148635864257812,4.9635790712233653e-05
28629,57259,57258,114517,19.21101689338684,4.947620519613613e-05
28729,57459,57458,114917,19.27271580696106,4.931756154448826e-05
28829,57659,57658,115317,19.338337659835815,4.915984805257059e-05
28929,57859,57858,115717,19.401904821395874,4.9003053205780613e-05
29029,58059,58058,116117,19.466214895248413,4.8847165676960624e-05
29129,58259,58258,116517,19.529254913330078,4.86921743226596e-05
29229,58459,58458,116917,19.593536615371704,4.853806817981771e-05
29329,58659,58658,117317,19.658894777297974,4.838483646400338e-05
29429,58859,58858,117717,19.71975564956665,4.823246856530781e-05
29530,59061,59060,118121,19.789920806884766,4.807944317543942e-05
29630,59261,59260,118521,19.853489875793457,4.7928780146489794e-05
29730,59461,59460,118921,19.91538977622986,4.77789500257163e-05
29830,59661,59660,119321,19.978328704833984,4.762994287589807e-05
29930,59861,59860,119721,20.04066777229309,4.74817489207553e-05
30030,60061,60060,120121,20.110052824020386,4.7334358542261396e-05
30130,60261,60260,120521,20.17225670814514,4.7187762277395645e-05
30230,60461,60460,120921,20.234437704086304,4.704195081676821e-05
30330,60661,60660,121321,20.297086000442505,4.689691500079174e-05
30430,60861,60860,121721,20.35811686515808,4.6752645817759055e-05
30531,61063,61062,122125,20.420567750930786,4.66077030845435e-05
30631,61263,61262,122525,20.48275876045227,4.6464948158740704e-05
30731,61463,61462,122925,20.544649839401245,4.632293360830165e-05
30831,61663,61662,123325,20.60789680480957,4.6181650990126026e-05
30931,61863,61862,123725,20.670949935913086,4.604109199664402e-05
31031,62063,62062,124125,20.736583948135376,4.590124845406999e-05
31131,62263,62262,124525,20.81710171699524,4.576211231931207e-05
31231,62463,62462,124925,20.890580892562866,4.5623675679175676e-05
31331,62663,62662,125325,20.954001903533936,4.5485930746875977e-05
31431,62863,62862,125725,21.016719818115234,4.534886986040284e-05
31532,63065,63064,126129,21.080803871154785,4.521112502764261e-05
31632,63265,63264,126529,21.15177869796753,4.5075416389486785e-05
31732,63465,63464,126929,21.215779781341553,4.494036946647604e-05
31832,63665,63664,127329,21.279448747634888,4.480597707620194e-05
31932,63865,63864,127729,21.34489870071411,4.467223215084162e-05
32032,64065,64064,128129,21.4071307182312,4.453912773524867e-05
32132,64265,64264,128529,21.471852779388428,4.440665698460036e-05
32232,64465,64464,128929,21.53396463394165,4.4274813163455194e-05
32332,64665,64664,129329,21.59962272644043,4.414358964266024e-05
32432,64865,64864,129729,21.666780948638916,4.4012979898811586e-05
32533,65067,65066,130133,21.73043203353882,4.388168053371468e-05
32633,65267,65266,130533,21.795270919799805,4.3752285163802853e-05
32733,65467,65466,130933,21.85829186439514,4.362348455197484e-05
32833,65667,65666,131333,21.92271375656128,4.349527257846508e-05
32933,65867,65866,131733,21.98644185066223,4.336764322057305e-05
33033,66067,66066,132133,22.05093479156494,4.324059055024682e-05
33133,66267,66266,132533,22.12180185317993,4.3114108732870426e-05
33233,66467,66466,132933,22.183629751205444,4.2988192024788874e-05
33333,66667,66666,133333,22.248013734817505,4.286283477379785e-05
33433,66867,66866,133733,22.317211866378784,4.273803141498402e-05
33534,67069,67068,134137,22.380308866500854,4.2612536673078805e-05
33634,67269,67268,134537,22.443177938461304,4.248883015614444e-05
33734,67469,67468,134937,22.50528883934021,4.23656613025213e-05
33834,67669,67668,135337,22.566770792007446,4.224302488806544e-05
33934,67869,67868,135737,22.633603811264038,4.212091576986844e-05
34034,68069,68068,136137,22.697070837020874,4.199932888547904e-05
34134,68269,68268,136537,22.763086795806885,4.187825925009619e-05
34234,68469,68468,136937,22.82633876800537,4.175770195691165e-05
34334,68669,68668,137337,22.897483825683594,4.1637652174587665e-05
34434,68869,68868,137737,22.976841926574707,4.151810514622675e-05
34535,69071,69070,138141,23.04711079597473,4.139786819858964e-05
34635,69271,69270,138541,23.115595817565918,4.1279317611775465e-05
34735,69471,69470,138941,23.181025743484497,4.116125589861157e-05
34835,69671,69670,139341,23.24330496788025,4.104367858893266e-05
34935,69871,69870,139741,23.306303024291992,4.0926581280700996e-05
35035,70071,70070,140141,23.366692781448364,4.080995963938163e-05
35135,70271,70270,140541,23.426178693771362,4.069380939636397e-05
35235,70471,70470,140941,23.486709594726562,4.057812634818032e-05
35335,70671,70670,141341,23.548614740371704,4.0462906354930845e-05
35435,70871,70870,141741,23.609497785568237,4.034814533943403e-05
35536,71073,71072,142145,23.673510789871216,4.023269851009812e-05
35636,71273,71272,142545,23.733162879943848,4.0118847955303736e-05
35736,71473,71472,142945,23.793778896331787,4.0005444474302674e-05
35836,71673,71672,143345,23.85513973236084,3.989248423133194e-05
35936,71873,71872,143745,23.914684772491455,3.977996344779066e-05
36036,72073,72072,144145,23.97638177871704,3.966787840167345e-05
36136,72273,72272,144545,24.03983163833618,3.9556225426652794e-05
36236,72473,72472,144945,24.105119943618774,3.944500091107113e-05
36336,72673,72672,145345,24.16535186767578,3.9334201296940535e-05
36436,72873,72872,145745,24.226430892944336,3.922382307882055e-05
36537,73075,73074,146149,24.285569667816162,3.911276530013233e-05
36637,73275,73274,146549,24.347455978393555,3.9003223693911626e-05
36737,73475,73474,146949,24.40735697746277,3.889409324269979e-05
36837,73675,73674,147349,24.468113899230957,3.878537064403034e-05
36937,73875,73874,147749,24.52676773071289,3.867705264373247e-05
37037,74075,74074,148149,24.587738752365112,3.8569136035575155e-05
37137,74275,74274,148549,24.65071988105774,3.846161765936627e-05
37237,74475,74474,148949,24.708622694015503,3.8354494401890974e-05
37337,74675,74674,149349,24.766830682754517,3.824776319413055e-05
37437,74875,74874,149749,24.83012366294861,3.814142101205568e-05
37538,75077,75076,150153,24.89115285873413,3.803440725340683e-05
37638,75277,75276,150553,24.950530767440796,3.79288380403949e-05
37738,75477,75476,150953,25.012677907943726,3.782364901093012e-05
37838,75677,75676,151353,25.090811729431152,3.7718837310885584e-05
37938,75877,75876,151753,25.161483764648438,3.7614400127851394e-05
38038,76077,76076,152153,25.219861030578613,3.751033468881929e-05
38138,76277,76276,152553,25.280463695526123,3.740663826028056e-05
38238,76477,76476,152953,25.342641830444336,3.730330814739174e-05
38338,76677,76676,153353,25.4044828414917,3.720034169323855e-05
38438,76877,76876,153753,25.465162992477417,3.709773627867321e-05
38539,77079,77078,154157,25.523655891418457,3.699446865294886e-05
38639,77279,77278,154557,25.583855867385864,3.6892581151433304e-05
38739,77479,77478,154957,25.652617931365967,3.679104702434905e-05
38839,77679,77678,155357,25.71157670021057,3.668986379534003e-05
38939,77879,77878,155757,25.771318674087524,3.6589029022979676e-05
39039,78079,78078,156157,25.833792686462402,3.648854029927933e-05
39139,78279,78278,156557,25.896007776260376,3.638839524956265e-05
39239,78479,78478,156957,25.95579481124878,3.6288591531761835e-05
39339,78679,78678,157357,26.01594591140747,3.61891268352783e-05
39439,78879,78878,157757,26.076109647750854,3.608999888182181e-05
39540,79081,79080,158161,26.139468669891357,3.5990219170194606e-05
39640,79281,79280,158561,26.199374675750732,3.589176130081737e-05
39740,79481,79480,158961,26.259541988372803,3.579363349966635e-05
39840,79681,79680,159361,26.320567846298218,3.569583360914854e-05
39940,79881,79880,159761,26.378925800323486,3.559835949977883e-05
40040,80081,80080,160161,26.43829870223999,3.5501209071416535e-05
40140,80281,80280,160561,26.497519731521606,3.5404380251281975e-05
40240,80481,80480,160961,26.556930780410767,3.5307870994029904e-05
40340,80681,80680,161361,26.619699954986572,3.5211679281427e-05
40440,80881,80880,161761,26.679641723632812,3.511580312144049e-05
40541,81083,81082,162165,26.738422632217407,3.5019286499979554e-05
40641,81283,81282,162565,26.800447940826416,3.492403868100052e-05
40741,81483,81482,162965,26.859991788864136,3.4829100574807754e-05
40841,81683,81682,163365,26.92001485824585,3.4734470291890646e-05
40941,81883,81882,163765,26.978901863098145,3.464014596647524e-05
41041,82083,82082,164165,27.039376735687256,3.45461257568566e-05
41141,82283,82282,164565,27.104881763458252,3.445240784510626e-05
41241,82483,82482,164965,27.174027681350708,3.435899043634538e-05
41341,82683,82682,165365,27.250688791275024,3.426587175791585e-05
41441,82883,82882,165765,27.316126823425293,3.4173050060040944e-05
41542,83085,83084,166169,27.377529859542847,3.4079599835957025e-05
41642,83285,83284,166569,27.43725895881653,3.3987369864515485e-05
41742,83485,83484,166969,27.49760890007019,3.3895431737749304e-05
41842,83685,83684,167369,27.557403802871704,3.380378379178892e-05
41942,83885,83884,167769,27.623613834381104,3.3712424383170477e-05
42042,84085,84084,168169,27.6836040019989,3.3621351888860514e-05
42142,84285,84284,168569,27.742475748062134,3.3530564705567713e-05
42242,84485,84484,168969,27.80174684524536,3.344006124921282e-05
42342,84685,84684,169369,27.861262798309326,3.3349839955396146e-05
42442,84885,84884,169769,27.924989938735962,3.325989927833864e-05
42543,85087,85086,170173,27.98733377456665,3.316934247953814e-05
42643,85287,85286,170573,28.050837993621826,3.307996124134588e-05
42743,85487,85486,170973,28.116127014160156,3.2990856078097836e-05
42843,85687,85686,171373,28.180689811706543,3.2902025516997306e-05
42943,85887,85886,171773,28.242631912231445,3.2813468102134975e-05
43043,86087,86086,172173,28.305933713912964,3.2725182394760776e-05
43143,86287,86286,172573,28.370012760162354,3.2637166973119995e-05
43243,86487,86486,172973,28.43040370941162,3.2549420431910284e-05
43343,86687,86686,173373,28.492596864700317,3.246194138205185e-05
43443,86887,86886,173773,28.55423593521118,3.2374728450169683e-05
43544,87089,87088,174177,28.623234748840332,3.2286912129785224e-05
43644,87289,87288,174577,28.686349868774414,3.220023000499881e-05
43744,87489,87488,174977,28.751685857772827,3.211380995897561e-05
43844,87689,87688,175377,28.815334796905518,3.2027650679817884e-05
43944,87889,87888,175777,28.87765884399414,3.194175087097991e-05
44044,88089,88088,176177,28.940574884414673,3.185610924959775e-05
44144,88289,88288,176577,29.00537395477295,3.177072454766679e-05
44244,88489,88488,176977,29.0709388256073,3.1685595510624095e-05
44344,88689,88688,177377,29.138222694396973,3.1600720897995835e-05
44444,88889,88888,177777,29.20726990699768,3.151609948276434e-05
44545,89091,89090,178181,29.27113676071167,3.14308876253352e-05
44645,89291,89290,178581,29.351338863372803,3.134677147855145e-05
44745,89491,89490,178981,29.427680015563965,3.12629049154091e-05
44845,89691,89690,179381,29.49190664291382,3.117928676108141e-05
44945,89891,89890,179781,29.554945707321167,3.109591585283589e-05
45045,90091,90090,180181,29.62382984161377,3.101279104053156e-05
45145,90291,90290,180581,29.688154697418213,3.092991118627236e-05
45245,90491,90490,180981,29.755613803863525,3.0847275163573484e-05
45345,90691,90690,181381,29.82003092765808,3.076488185817855e-05
45445,90891,90890,181781,29.88526678085327,3.068273016674983e-05
45546,91093,91092,182185,29.949141025543213,3.060000109696152e-05
45646,91293,91292,182585,30.014394760131836,3.051833175864916e-05
45746,91493,91492,182985,30.07803964614868,3.0436900781789743e-05
45846,91693,91692,183385,30.14532995223999,3.035570710759452e-05
45946,91893,91892,183785,30.208630800247192,3.0274749687879228e-05
46046,92093,92092,184185,30.27203679084778,3.019402748502417e-05
46146,92293,92292,184585,30.340221881866455,3.0113539471342186e-05
46246,92493,92492,184985,30.40301275253296,3.0033284629731675e-05
46346,92693,92692,185385,30.46654486656189,2.9953261952689638e-05
46446,92893,92892,185785,30.530184984207153,2.9873470442305168e-05
46547,93095,93094,186189,30.596466779708862,2.97931146568962e-05
46647,93295,93294,186589,30.66164994239807,2.9713784813298593e-05
46747,93495,93494,186989,30.72463369369507,2.9634683191163725e-05
46847,93695,93694,187389,30.79154372215271,2.9555808830914836e-05
46947,93895,93894,187789,30.85551166534424,2.947716078132438e-05
47047,94095,94094,188189,30.92010498046875,2.9398738100701532e-05
47147,94295,94294,188589,30.985195636749268,2.9320539855758794e-05
47247,94495,94494,188989,31.048735857009888,2.9242565122036886e-05
47347,94695,94694,189389,31.116156816482544,2.9164812983457692e-05
47447,94895,94894,189789,31.18205690383911,2.9087282532179822e-05
47548,95097,95096,190193,31.24878478050232,2.9009200884041206e-05
47648,95297,95296,190593,31.31783175468445,2.8932113311716377e-05
47748,95497,95496,190993,31.382730960845947,2.8855244743650734e-05
47848,95697,95696,191393,31.462570905685425,2.877859430446245e-05
47948,95897,95896,191793,31.54263401031494,2.8702161126272125e-05
48048,96097,96096,192193,31.60734486579895,2.862594434899295e-05
48148,96297,96296,192593,31.67253088951111,2.8549943120269324e-05
48248,96497,96496,192993,31.73583984375,2.8474156594495263e-05
48348,96697,96696,193393,31.802209615707397,2.8398583933947197e-05
48448,96897,96896,193793,31.865108966827393,2.8323224307540278e-05
48549,97099,97098,194197,31.93009376525879,2.8247326486691827e-05
48649,97299,97298,194597,31.99338388442993,2.817239257455151e-05
48749,97499,97498,194997,32.05857181549072,2.8097669238021834e-05
48849,97699,97698,195397,32.127349615097046,2.8023155674178978e-05
48949,97899,97898,195797,32.19183278083801,2.7948851086527247e-05
49049,98099,98098,196197,32.255483865737915,2.7874754684591886e-05
49149,98299,98298,196597,32.32176470756531,2.780086568570416e-05
49249,98499,98498,196997,32.390267848968506,2.7727183311740008e-05
49349,98699,98698,197397,32.45708680152893,2.7653706792183907e-05
49449,98899,98898,197797,32.52044701576233,2.758043536234747e-05
49550,99101,99100,198201,32.584118604660034,2.7506638621631794e-05
49650,99301,99300,198601,32.653728008270264,2.7433777132734744e-05
49750,99501,99500,199001,32.71680164337158,2.7361118467608967e-05
49850,99701,99700,199401,32.780311822891235,2.7288661885254508e-05
49950,99901,99900,199801,32.8449547290802,2.7216406650517186e-05
50050,100101,100100,200201,32.910966634750366,2.7144352033615213e-05
50150,100301,100300,200601,32.973827838897705,2.7072497310831866e-05
50250,100501,100500,201001,33.040363788604736,2.7000841762909114e-05
50350,100701,100700,201401,33.10841774940491,2.6929384677127086e-05
50450,100901,100900,201801,33.17995285987854,2.6858125345551605e-05
50551,101103,101102,202205,33.24387264251709,2.6786353435153334e-05
50651,101303,101302,202605,33.309685707092285,2.6715489468926942e-05
50751,101503,101502,203005,33.37795686721802,2.664482115731684e-05
50851,101703,101702,203405,33.44026494026184,2.6574347812971902e-05
50951,101903,101902,203805,33.506608724594116,2.6504068753598124e-05
51051,102103,102102,204205,33.58182668685913,2.6433983301478658e-05
51151,102303,102302,204605,33.664233922958374,2.6364090784217187e-05
51251,102503,102502,205005,33.72711396217346,2.6294390533643692e-05
51351,102703,102702,205405,33.78829884529114,2.622488188663606e-05
51451,102903,102902,205805,33.8530969619751,2.615556418426677e-05
51552,103105,103104,206209,33.91295266151428,2.6085746457375544e-05
51652,103305,103304,206609,33.9733829498291,2.6016810580009973e-05
51752,103505,103504,207009,34.03633689880371,2.5948063691814663e-05
51852,103705,103704,207409,34.102829694747925,2.587950515238442e-05
51952,103905,103904,207809,34.16466999053955,2.5811134324963e-05
52052,104105,104104,208209,34.22405481338501,2.5742950577323302e-05
52152,104305,104304,208609,34.28350472450256,2.567495328149912e-05
52252,104505,104504,209009,34.34286880493164,2.560714181311486e-05
52352,104705,104704,209409,34.4020516872406,2.5539515552817387e-05
52452,104905,104904,209809,34.46197462081909,2.5472073884457064e-05
52553,105107,105106,210213,34.5233678817749,2.5404144546321363e-05
52653,105307,105306,210613,34.58318591117859,2.533707206083591e-05
52753,105507,105506,211013,34.647419929504395,2.5270182337160887e-05
52853,105707,105706,211413,34.70920777320862,2.520347477521847e-05
52953,105907,105906,211813,34.76962876319885,2.5136948778363798e-05
53053,106107,106106,212213,34.83373284339905,2.5070603753709034e-05
53153,106307,106306,212613,34.8931667804718,2.500443911217596e-05
53253,106507,106506,213013,34.95272088050842,2.4938454268183675e-05
53353,106707,106706,213413,35.013731718063354,2.48726486398525e-05
53453,106907,106906,213813,35.07195687294006,2.4807021648456734e-05
53554,107109,107108,214217,35.13920783996582,2.4740919127460702e-05
53654,107309,107308,214617,35.199403047561646,2.4675649460674334e-05
53754,107509,107508,215017,35.25947189331055,2.461055671077888e-05
53854,107709,107708,215417,35.31996393203735,2.4545640312633613e-05
53954,107909,107908,215817,35.37937688827515,2.4480899704857497e-05
54054,108109,108108,216217,35.440008878707886,2.441633432916529e-05
54154,108309,108308,216617,35.500051975250244,2.4351943630693313e-05
54254,108509,108508,217017,35.56007981300354,2.4287727057213384e-05
54354,108709,108708,217417,35.62243676185608,2.422368406037015e-05
54454,108909,108908,217817,35.68525290489197,2.4159814094366667e-05
54555,109111,109110,218221,35.7649028301239,2.4095480511209837e-05
54655,109311,109310,218621,35.838013887405396,2.403195669900347e-05
54755,109511,109510,219021,35.89842486381531,2.396860429375416e-05
54855,109711,109710,219421,35.96056389808655,2.390542276187011e-05
54955,109911,109910,219821,36.020386695861816,2.3842411572404317e-05
55055,110111,110110,220221,36.08207368850708,2.377957019812172e-05
55155,110311,110310,220621,36.15934181213379,2.3716898113502782e-05
55255,110511,110510,221021,36.220353841781616,2.3654394796708936e-05
55355,110711,110710,221421,36.28086566925049,2.3592059728499633e-05
55455,110911,110910,221821,36.342429876327515,2.352989239212878e-05
55556,111113,111112,222225,36.403488636016846,2.3467273115073354e-05
55656,111313,111312,222625,36.466869592666626,2.3405441367879728e-05
55756,111513,111512,223025,36.52736282348633,2.3343775813775845e-05
55856,111713,111712,223425,36.590242862701416,2.3282275946711545e-05
55956,111913,111912,223825,36.652925968170166,2.322094126385062e-05
56056,112113,112112,224225,36.71377182006836,2.3159771263642842e-05
56156,112313,112312,224625,36.77490472793579,2.3098765448635443e-05
56256,112513,112512,225025,36.83595871925354,2.3037923322603186e-05
56356,112713,112712,225425,36.90648865699768,2.2977244392556e-05
56456,112913,112912,225825,36.9749538898468,2.2916728167328615e-05
56557,113115,113114,226229,37.04696559906006,2.285577143627992e-05
56657,113315,113314,226629,37.11756086349487,2.2795580773450657e-05
56757,113515,113514,227029,37.19169878959656,2.2735551352643295e-05
56857,113715,113714,227429,37.26145267486572,2.2675682692531344e-05
56957,113915,113914,227829,37.33019495010376,2.2615974314403126e-05
57057,114115,114114,228229,37.40320062637329,2.2556425741619783e-05
57157,114315,114314,228629,37.46857666969299,2.2497036499421136e-05
57257,114515,114514,229029,37.52863788604736,2.2437806115965838e-05
57357,114715,114714,229429,37.5961217880249,2.2378734121140846e-05
57457,114915,114914,229829,37.658761978149414,2.23198200471003e-05
57558,115117,115116,230233,37.7204008102417,2.2260476655638483e-05
57658,115317,115316,230633,37.78886389732361,2.220187859615511e-05
57758,115517,115516,231033,37.859503746032715,2.2143437062694848e-05
57858,115717,115716,231433,37.93786382675171,2.208515159585446e-05
57958,115917,115916,231833,38.00258469581604,2.2027021738412768e-05
58058,116117,116116,232233,38.063939809799194,2.196904703531825e-05
58158,116317,116316,232633,38.12898778915405,2.1911227033862122e-05
58258,116517,116516,233033,38.18970775604248,2.1853561282433104e-05
58358,116717,116716,233433,38.249839782714844,2.179604933237747e-05
58458,116917,116916,233833,38.313055992126465,2.1738690736792868e-05
58559,117119,117118,234237,38.37541079521179,2.1680913764197943e-05
58659,117319,117318,234637,38.43527293205261,2.16238620660385e-05
58759,117519,117518,235037,38.497769832611084,2.1566962388363205e-05
58859,117719,117718,235437,38.56167197227478,2.1510214291852315e-05
58959,117919,117918,235837,38.62746977806091,2.145361733882728e-05
59059,118119,118118,236237,38.68745279312134,2.1397171093987558e-05
59159,118319,118318,236637,38.7475106716156,2.1340875123504925e-05
59259,118519,118518,237037,38.80898380279541,2.1284728995255595e-05
59359,118719,118718,237437,38.871450901031494,2.1228732279424487e-05
59459,118919,118918,237837,38.934820890426636,2.1172884547671173e-05
59560,119121,119120,238241,38.997742891311646,2.1116629130278112e-05
59660,119321,119320,238641,39.058573722839355,2.1061079567991885e-05
59760,119521,119520,239041,39.12334990501404,2.1005677711233096e-05
59860,119721,119720,239441,39.18463587760925,2.0950423138432683e-05
59960,119921,119920,239841,39.247824907302856,2.0895315430546292e-05
60060,120121,120120,240241,39.315417766571045,2.084035416953603e-05
60160,120321,120320,240641,39.383118867874146,2.0785538939042277e-05
60260,120521,120520,241041,39.4451117515564,2.0730869324710094e-05
60360,120721,120720,241441,39.50621175765991,2.0676344913662552e-05
60460,120921,120920,241841,39.56856560707092,2.0621965294468176e-05
60561,121123,121122,242245,39.63962483406067,2.0567188433262498e-05
60661,121323,121322,242645,39.7005558013916,2.051309860880756e-05
60761,121523,121522,243045,39.7645959854126,2.0459152348164386e-05
60861,121723,121722,243445,39.82689881324768,2.040534924679027e-05
60961,121923,121922,243845,39.88857078552246,2.035168890128138e-05
61061,122123,122122,244245,39.95306968688965,2.0298170909973146e-05
61161,122323,122322,244645,40.03318667411804,2.0244794872959396e-05
61261,122523,122522,245045,40.106661796569824,2.0191560391286615e-05
61361,122723,122722,245445,40.16896367073059,2.013846706802766e-05
61461,122923,122922,245845,40.2325656414032,2.0085514507503593e-05
61562,123125,123124,246249,40.294004917144775,2.0032174901477545e-05
61662,123325,123324,246649,40.35611176490784,1.9979504083596258e-05
61762,123525,123524,247049,40.42210268974304,1.9926972846823785e-05
61862,123725,123724,247449,40.48480677604675,1.9874580801212154e-05
61962,123925,123924,247849,40.54647493362427,1.982232755876665e-05
62062,124125,124124,248249,40.613316774368286,1.977021273223869e-05
62162,124325,124324,248649,40.67843770980835,1.9718235937093582e-05
62262,124525,124524,249049,40.73909783363342,1.9666396788647028e-05
62362,124725,124724,249449,40.800609827041626,1.9614694904457984e-05
62462,124925,124924,249849,40.86293077468872,1.9563129903492418e-05
62563,125127,125126,250253,40.927931785583496,1.95111878088456e-05
62663,125327,125326,250653,40.98856782913208,1.9459896795404316e-05
62763,125527,125526,251053,41.05214285850525,1.9408741525726247e-05
62863,125727,125726,251453,41.11838173866272,1.9357721624437273e-05
62963,125927,125926,251853,41.182180881500244,1.9306836717067964e-05
63063,126127,126126,252253,41.24813961982727,1.9256086430376436e-05
63163,126327,126326,252653,41.311903953552246,1.9205470392660153e-05
63263,126527,126526,253053,41.37296485900879,1.9154988233616504e-05
63363,126727,126726,253453,41.43518590927124,1.9104639584039083e-05
63463,126927,126926,253853,41.49732303619385,1.905442407592919e-05
63564,127129,127128,254257,41.56132197380066,1.900384118471068e-05
63664,127329,127328,254657,41.62863492965698,1.8953892183638294e-05
63764,127529,127528,255057,41.69296073913574,1.890407522448166e-05
63864,127729,127728,255457,41.75541877746582,1.8854389944565315e-05
63964,127929,127928,255857,41.818063735961914,1.8804835982245097e-05
64064,128129,128128,256257,41.88010382652283,1.8755412977338632e-05
64164,128329,128328,256657,41.94575476646423,1.8706120570740475e-05
64264,128529,128528,257057,42.010913610458374,1.865695840461242e-05
64364,128729,128728,257457,42.07405376434326,1.860792612203922e-05
64464,128929,128928,257857,42.1563138961792,1.855902336819472e-05
64565,129131,129130,258261,42.23398971557617,1.850976270343003e-05
64665,129331,129330,258661,42.29843783378601,1.8461119230959207e-05
64765,129531,129530,259061,42.3647255897522,1.841260422389944e-05
64865,129731,129730,259461,42.42790198326111,1.836421733186464e-05
64965,129931,129930,259861,42.48987698554993,1.8315958205267807e-05
65065,130131,130130,260261,42.55211877822876,1.8267826495468693e-05
65165,130331,130330,260661,42.62112879753113,1.8219821855713516e-05
65265,130531,130530,261061,42.683899879455566,1.8171943939394313e-05
65365,130731,130730,261461,42.74708366394043,1.8124192401890763e-05
65465,130931,130930,261861,42.81195282936096,1.807656689920891e-05
65566,131133,131132,262265,42.87499499320984,1.802859272401759e-05
65666,131333,131332,262665,42.93743896484375,1.7981219515825615e-05
65766,131533,131532,263065,43.00391888618469,1.7933971314153006e-05
65866,131733,131732,263465,43.0698618888855,1.7886847779718556e-05
65966,131933,131932,263865,43.139283895492554,1.7839848574542793e-05
66066,132133,132132,264265,43.20223879814148,1.7792973360984327e-05
66166,132333,132332,264665,43.26378870010376,1.774622180305548e-05
66266,132533,132532,265065,43.32903504371643,1.7699593565845852e-05
66366,132733,132732,265465,43.391610860824585,1.765308831498967e-05
66466,132933,132932,265865,43.45572090148926,1.7606705718167207e-05
66567,133135,133134,266269,43.51843786239624,1.755998345668219e-05
66667,133335,133334,266669,43.582661867141724,1.7513846390966255e-05
66767,133535,133534,267069,43.64826488494873,1.7467830982985047e-05
66867,133735,133734,267469,43.714876890182495,1.742193690438056e-05
66967,133935,133934,267869,43.78171968460083,1.7376163827261714e-05
67067,134135,134134,268269,43.85039782524109,1.733051142500303e-05
67167,134335,134334,268669,43.9307918548584,1.7284979372039063e-05
67267,134535,134534,269069,44.006051778793335,1.7239567343650374e-05
67367,134735,134734,269469,44.06965184211731,1.7194275015922567e-05
67467,134935,134934,269869,44.13825988769531,1.714910206677827e-05
67568,135137,135136,270273,44.204345703125,1.7103598235798575e-05
67668,135337,135336,270673,44.280171632766724,1.7058664265164614e-05
67768,135537,135536,271073,44.35967183113098,1.7013848707814715e-05
67868,135737,135736,271473,44.42330288887024,1.6969151245040448e-05
67968,135937,135936,271873,44.4865927696228,1.692457155918788e-05
68068,136137,136136,272273,44.55309081077576,1.6880109333620768e-05
68168,136337,136336,272673,44.62365388870239,1.683576425243439e-05
68268,136537,136536,273073,44.68789291381836,1.6791536000936082e-05
68368,136737,136736,273473,44.75003695487976,1.6747424265589038e-05
68468,136937,136936,273873,44.81188893318176,1.670342873304796e-05
68569,137139,137138,274277,44.87170886993408,1.665911087932783e-05
68669,137339,137338,274677,44.93295884132385,1.6615347972363444e-05
68769,137539,137538,275077,44.994489669799805,1.6571700332197553e-05
68869,137739,137738,275477,45.05829358100891,1.6528167649959238e-05
68969,137939,137938,275877,45.121466875076294,1.6484749617580144e-05
69069,138139,138138,276277,45.183440923690796,1.6441445927369382e-05
69169,138339,138338,276677,45.243870973587036,1.639825627356887e-05
69269,138539,138538,277077,45.304391860961914,1.635518035047111e-05
69369,138739,138738,277477,45.36407780647278,1.6312217853410014e-05
69469,138939,138938,277877,45.42367887496948,1.6269368479208947e-05
69570,139141,139140,278281,45.484657764434814,1.6226205128021875e-05
69670,139341,139340,278681,45.545018911361694,1.618358221545783e-05
69770,139541,139540,279081,45.607767820358276,1.6141071517023545e-05
69870,139741,139740,279481,45.66744565963745,1.6098672732901098e-05
69970,139941,139940,279881,45.725178718566895,1.6056385563722527e-05
70070,140141,140140,280281,45.79205584526062,1.601420971158354e-05
70170,140341,140340,280681,45.85235095024109,1.597214487904291e-05
70270,140541,140540,281081,45.914833784103394,1.5930190769403622e-05
70370,140741,140740,281481,45.97655177116394,1.5888347086828253e-05
70470,140941,140940,281881,46.04197669029236,1.5846613537293226e-05
70571,141143,141142,282285,46.11008381843567,1.5804574142821485e-05
70671,141343,141342,282685,46.17034697532654,1.5763061071677336e-05
70771,141543,141542,283085,46.231791734695435,1.572165725098083e-05
70871,141743,141742,283485,46.292701959609985,1.568036238932342e-05
70971,141943,141942,283885,46.35278391838074,1.563917619661719e-05
71071,142143,142142,284285,46.4298198223114,1.5598098383079944e-05
71171,142343,142342,284685,46.50633502006531,1.5557128659879805e-05
71271,142543,142542,285085,46.57215690612793,1.551626673904173e-05
71371,142743,142742,285485,46.6460497379303,1.5475512333340215e-05
71471,142943,142942,285885,46.70930576324463,1.543486515664381e-05
71572,143145,143144,286289,46.7738037109375,1.5393920059972016e-05
71672,143345,143344,286689,46.83751082420349,1.535348755058224e-05
71772,143545,143544,287089,46.89985466003418,1.531316141333044e-05
71872,143745,143744,287489,46.96201181411743,1.5272941365183232e-05
71972,143945,143944,287889,47.022955656051636,1.523282712384033e-05
72072,144145,144144,288289,47.08926177024841,1.5192818407997424e-05
72172,144345,144344,288689,47.15054988861084,1.5152914936847771e-05
72272,144545,144544,289089,47.2124707698822,1.5113116430789984e-05
72372,144745,144744,289489,47.272623777389526,1.5073422610793069e-05
72472,144945,144944,289889,47.33659291267395,1.5033833198687016e-05
72573,145147,145146,290293,47.399831771850586,1.4993953589126237e-05
72673,145347,145346,290693,47.4590117931366,1.4954573198261597e-05
72773,145547,145546,291093,47.52144980430603,1.4915296382650158e-05
72873,145747,145746,291493,47.583388805389404,1.4876122867020013e-05
72973,145947,145946,291893,47.64910697937012,1.4837052377335046e-05
73073,146147,146146,292293,47.7104377746582,1.4798084639996012e-05
73173,146347,146346,292693,47.77579593658447,1.4759219382225475e-05
73273,146547,146546,293093,47.841179847717285,1.4720456332134343e-05
73373,146747,146746,293493,47.90208983421326,1.4681795218396131e-05
73473,146947,146946,293893,47.96236968040466,1.464323577088099e-05
73574,147149,147148,294297,48.027838945388794,1.4604393650022224e-05
73674,147349,147348,294697,48.09632062911987,1.4566037736105774e-05
73774,147549,147548,295097,48.1641149520874,1.4527782678803756e-05
73874,147749,147748,295497,48.22772574424744,1.4489628210470056e-05
73974,147949,147948,295897,48.29231286048889,1.4451574064646674e-05
74074,148149,148148,296297,48.357097864151,1.4413619975729352e-05
74174,148349,148348,296697,48.41983389854431,1.4375765677929323e-05
74274,148549,148548,297097,48.482542753219604,1.4338010907430697e-05
74374,148749,148748,297497,48.56151485443115,1.4300355400015598e-05
74474,148949,148948,297897,48.638797760009766,1.4262798893241198e-05
74575,149151,149150,298301,48.70144987106323,1.4224967044582713e-05
74675,149351,149350,298701,48.76380491256714,1.4187608735879116e-05
74775,149551,149550,299101,48.827343702316284,1.4150348640633926e-05
74875,149751,149750,299501,48.88867783546448,1.411318649859706e-05
74975,149951,149950,299901,48.95222783088684,1.4076122050697859e-05
75075,150151,150150,300301,49.015859842300415,1.4039155038217177e-05
75175,150351,150350,300701,49.07669281959534,1.4002285203044059e-05
75275,150551,150550,301101,49.14351487159729,1.396551228814974e-05
75375,150751,150750,301501,49.203664779663086,1.3928836037334154e-05
75475,150951,150950,301901,49.26411485671997,1.3892256194644411e-05
75576,151153,151152,302305,49.32530999183655,1.3855408152760232e-05
75676,151353,151352,302705,49.39313364028931,1.3819021319724948e-05
75776,151553,151552,303105,49.45714473724365,1.378273012937316e-05
75876,151753,151752,303505,49.52260875701904,1.37465343287313e-05
75976,151953,151952,303905,49.593164682388306,1.3710433665364345e-05
76076,152153,152152,304305,49.662842750549316,1.3674427888222097e-05
76176,152353,152352,304705,49.72659373283386,1.3638516746108737e-05
76276,152553,152552,305105,49.78871488571167,1.3602699989017592e-05
76376,152753,152752,305505,49.855841636657715,1.3566977367307783e-05
76476,152953,152952,305905,49.91856575012207,1.3531348632291498e-05
76577,153155,153154,306309,49.98172879219055,1.3495458657206668e-05
76677,153355,153354,306709,50.04346179962158,1.3460017884723614e-05
76777,153555,153554,307109,50.1093168258667,1.3424670254234672e-05
76877,153755,153754,307509,50.17098069190979,1.3389415520023877e-05
76977,153955,153954,307909,50.23222279548645,1.3354253435917976e-05
77077,154155,154154,308309,50.29608869552612,1.331918375795346e-05
77177,154355,154354,308709,50.35841369628906,1.3284206241693176e-05
77277,154555,154554,309109,50.419339656829834,1.3249320643883574e-05
77377,154755,154754,309509,50.48069787025452,1.321452672189924e-05
77477,154955,154954,309909,50.54465675354004,1.3179824233379296e-05
77578,155157,155156,310313,50.612870931625366,1.3144867284058924e-05
77678,155357,155356,310713,50.68724298477173,1.3110347847813236e-05
77778,155557,155556,311113,50.765379667282104,1.3075919120364645e-05
77878,155757,155756,311513,50.83086895942688,1.3041580862856384e-05
77978,155957,155956,311913,50.89207077026367,1.3007332836114578e-05
78078,156157,156156,312313,50.9590847492218,1.2973174802116794e-05
78178,156357,156356,312713,51.021283864974976,1.2939106523417998e-05
78278,156557,156556,313113,51.087806940078735,1.2905127763163407e-05
78378,156757,156756,313513,51.155457735061646,1.2871238285231564e-05
78478,156957,156956,313913,51.21731781959534,1.2837437853971156e-05
78579,157159,157158,314317,51.28267979621887,1.2803389565780477e-05
78679,157359,157358,314717,51.3445258140564,1.2769767408582331e-05
78779,157559,157558,315117,51.40675091743469,1.2736233592828765e-05
78879,157759,157758,315517,51.46991991996765,1.2702787885569308e-05
78979,157959,157958,315917,51.533527851104736,1.266943005464994e-05
79079,158159,158158,316317,51.59865069389343,1.263615986810437e-05
79179,158359,158358,316717,51.662890911102295,1.2602977095002604e-05
79279,158559,158558,317117,51.72475075721741,1.2569881504720002e-05
79379,158759,158758,317517,51.787813901901245,1.253687286739442e-05
79479,158959,158958,317917,51.852107763290405,1.2503950953878767e-05
79580,159161,159160,318321,51.91646885871887,1.2470787617383913e-05
79680,159361,159360,318721,51.97757887840271,1.2438039327649303e-05
79780,159561,159560,319121,52.04013681411743,1.240537707547421e-05
79880,159761,159760,319521,52.10605072975159,1.237280063375178e-05
79980,159961,159960,319921,52.169761657714844,1.2340309776876111e-05
80080,160161,160160,320321,52.23467183113098,1.2307904278813797e-05
80180,160361,160360,320721,52.30017590522766,1.2275583914711291e-05
80280,160561,160560,321121,52.36604595184326,1.2243348460431628e-05
80380,160761,160760,321521,52.429768800735474,1.221119769218869e-05
80480,160961,160960,321921,52.491896867752075,1.2179131386483536e-05
80581,161163,161162,322325,52.55766677856445,1.2146829925215369e-05
80681,161363,161362,322725,52.62608575820923,1.2114932717436678e-05
80781,161563,161562,323125,52.68730878829956,1.2083119304311862e-05
80881,161763,161762,323525,52.751253843307495,1.205138946520942e-05
80981,161963,161962,323925,52.83150267601013,1.2019742980131977e-05
81081,162163,162162,324325,52.909152030944824,1.1988179629343102e-05
81181,162363,162362,324725,52.97776675224304,1.1956699193857707e-05
81281,162563,162562,325125,53.04440665245056,1.1925301455426336e-05
81381,162763,162762,325525,53.110718965530396,1.1893986196231848e-05
81481,162963,162962,325925,53.173091888427734,1.1862753198888453e-05
81582,163165,163164,326329,53.23634672164917,1.1831291150946348e-05
81682,163365,163364,326729,53.299784898757935,1.1800222845606567e-05
81782,163565,163564,327129,53.36803579330444,1.1769236151740224e-05
81882,163765,163764,327529,53.434117794036865,1.1738330854899474e-05
81982,163965,163964,327929,53.49762678146362,1.1707506740377812e-05
82082,164165,164164,328329,53.560675859451294,1.1676763594383616e-05
82182,164365,164364,328729,53.626788854599,1.1646101204224468e-05
82282,164565,164564,329129,53.69016671180725,1.161551935693326e-05
82382,164765,164764,329529,53.75265574455261,1.1585017840624047e-05
82482,164965,164964,329929,53.815067768096924,1.1554596443897515e-05
82583,165167,165166,330333,53.878150939941406,1.1523951943227812e-05
82683,165367,165366,330733,53.94112181663513,1.1493690949118079e-05
82783,165567,165566,331133,54.004857778549194,1.1463509441390283e-05
82883,165767,165766,331533,54.06805777549744,1.1433407210656454e-05
82983,165967,165966,331933,54.13514280319214,1.1403384048218123e-05
83083,166167,166166,332333,54.19924974441528,1.1373439746596062e-05
83183,166367,166366,332733,54.26348066329956,1.1343574097645675e-05
83283,166567,166566,333133,54.32720375061035,1.131378689441373e-05
83383,166767,166766,333533,54.3893518447876,1.1284077930830338e-05
83483,166967,166966,333933,54.45244789123535,1.1254447000641382e-05
83584,167169,167168,334337,54.51708173751831,1.1224598760195044e-05
83684,167369,167368,334737,54.58513689041138,1.11951240568669e-05
83784,167569,167568,335137,54.654451847076416,1.1165726770648461e-05
83884,167769,167768,335537,54.72075271606445,1.1136406698171625e-05
83984,167969,167968,335937,54.78343391418457,1.1107163635669422e-05
84084,168169,168168,336337,54.845852851867676,1.1077997381037363e-05
84184,168369,168368,336737,54.916547775268555,1.1048907731975638e-05
84284,168569,168568,337137,54.995606660842896,1.1019894487093157e-05
84384,168769,168768,337537,55.06654977798462,1.0990957445159922e-05
84484,168969,168968,337937,55.139970779418945,1.0962096405986309e-05
84585,169171,169170,338341,55.207175970077515,1.0933023699233323e-05
84685,169371,169370,338741,55.27115488052368,1.0904314820877476e-05
84785,169571,169570,339141,55.333653926849365,1.0875681345230212e-05
84885,169771,169770,339541,55.398563861846924,1.0847123073347615e-05
84985,169971,169970,339941,55.46084189414978,1.0818639808014849e-05
85085,170171,170170,340341,55.523459672927856,1.0790231351637085e-05
85185,170371,170370,340741,55.590152978897095,1.0761897507666352e-05
85285,170571,170570,341141,55.65738272666931,1.0733638079534253e-05
85385,170771,170770,341541,55.718788862228394,1.0705452871767683e-05
85485,170971,170970,341941,55.78410482406616,1.067734168925997e-05
85586,171173,171172,342345,55.84885787963867,1.064902433568676e-05
85686,171373,171372,342745,55.91477084159851,1.0621061355043744e-05
85786,171573,171572,343145,55.98222494125366,1.059317181518744e-05
85886,171773,171772,343545,56.044158935546875,1.0565355523073603e-05
85986,171973,171972,343945,56.11265778541565,1.0537612285765303e-05
86086,172173,172172,344345,56.17842483520508,1.0509941911292575e-05
86186,172373,172372,344745,56.24048376083374,1.0482344208128958e-05
86286,172573,172572,345145,56.303576707839966,1.0454818985153182e-05
86386,172773,172772,345545,56.36762595176697,1.0427366051932911e-05
86486,172973,172972,345945,56.43075680732727,1.0399985217957848e-05
86587,173175,173174,346349,56.49749994277954,1.0372403567356618e-05
86687,173375,173374,346749,56.560948848724365,1.0345167080779708e-05
86787,173575,173574,347149,56.62744975090027,1.0318002124323727e-05
86887,173775,173774,347549,56.6940758228302,1.0290908510408078e-05
86987,173975,173974,347949,56.7755069732666,1.0263886051489661e-05
87087,174175,174174,348349,56.83990287780762,1.023693456009163e-05
87187,174375,174374,348749,56.90011692047119,1.0210053849828041e-05
87287,174575,174574,349149,56.96192169189453,1.0183243734818245e-05
87387,174775,174774,349549,57.022228956222534,1.0156504029432973e-05
87487,174975,174974,349949,57.097779989242554,1.0129834548314839e-05
87588,175177,175176,350353,57.172900676727295,1.0102969465708931e-05
87688,175377,175376,350753,57.236249685287476,1.0076440577754233e-05
87788,175577,175576,351153,57.2980580329895,1.0049981359889729e-05
87888,175777,175776,351553,57.35730791091919,1.0023591629317674e-05
87988,175977,175976,351953,57.41666793823242,9.997271203206732e-06
88088,176177,176176,352353,57.477030754089355,9.971019899275373e-06
88188,176377,176376,352753,57.5373158454895,9.944837536108938e-06
88288,176577,176576,353153,57.60360288619995,9.918723932113912e-06
88388,176777,176776,353553,57.66580772399902,9.892678906949668e-06
88488,176977,176976,353953,57.726704835891724,9.86670228002259e-06
88589,177179,177178,354357,57.78657364845276,9.840535131651284e-06
88689,177379,177378,354757,57.85005283355713,9.814695442258035e-06
88789,177579,177578,355157,57.90976881980896,9.788923611639064e-06
88889,177779,177778,355557,57.96827173233032,9.763219461283837e-06
88989,177979,177978,355957,58.032957792282104,9.737582813622028e-06
89089,178179,178178,356357,58.09718465805054,9.71201349078275e-06
89189,178379,178378,356757,58.15884804725647,9.686511316281724e-06
89289,178579,178578,357157,58.219987869262695,9.661076113395552e-06
89389,178779,178778,357557,58.28227376937866,9.635707706140528e-06
89489,178979,178978,357957,58.34099888801575,9.610405919055778e-06
89590,179181,179180,358361,58.40276098251343,9.584918558584647e-06
89690,179381,179380,358761,58.46356773376465,9.559750148907463e-06
89790,179581,179580,359161,58.52334475517273,9.534647833836196e-06
89890,179781,179780,359561,58.58604693412781,9.509611439370758e-06
89990,179981,179980,359961,58.64669179916382,9.484640792811653e-06
90090,180181,180180,360361,58.707385778427124,9.459735720964691e-06
90190,180381,180380,360761,58.76913094520569,9.434896051772496e-06
90290,180581,180580,361161,58.83020877838135,9.41012161331594e-06
90390,180781,180780,361561,58.88839888572693,9.385412234062858e-06
90490,180981,180980,361961,58.94734573364258,9.360767743141195e-06
90591,181183,181182,362365,59.00803780555725,9.335942498442284e-06
90691,181383,181382,362765,59.06842494010925,9.311427917734878e-06
90791,181583,181582,363165,59.13674592971802,9.286977713627531e-06
90891,181783,181782,363565,59.204509973526,9.262591716663786e-06
90991,181983,181982,363965,59.28204584121704,9.238269758334862e-06
91091,182183,182182,364365,59.35250473022461,9.214011670239104e-06
91191,182383,182382,364765,59.414482831954956,9.189817284931266e-06
91291,182583,182582,365165,59.47769284248352,9.165686434584442e-06
91391,182783,182782,365565,59.537710666656494,9.141618952547733e-06
91491,182983,182982,365965,59.607956886291504,9.117614672312289e-06
91592,183185,183184,366369,59.67258286476135,9.093434332876992e-06
91692,183385,183384,366769,59.736228704452515,9.069556586098724e-06
91792,183585,183584,367169,59.807148694992065,9.045741542650036e-06
91892,183785,183784,367569,59.870224714279175,9.021989037697424e-06
91992,183985,183984,367969,59.937676668167114,8.998298906767125e-06
92092,184185,184184,368369,60.00594472885132,8.974670986220466e-06
92192,184385,184384,368769,60.068989992141724,8.951105112489225e-06
92292,184585,184584,369169,60.134809732437134,8.927601122714584e-06
92392,184785,184784,369569,60.20256686210632,8.904158854121014e-06
92492,184985,184984,369969,60.266865968704224,8.880778144547698e-06
92593,185187,185186,370373,60.33127188682556,8.857225948945374e-06
92693,185387,185386,370773,60.3946008682251,8.833968484521094e-06
92793,185587,185586,371173,60.46256685256958,8.810772093657265e-06
92893,185787,185786,371573,60.52518582344055,8.787636616030929e-06
92993,185987,185986,371973,60.586747884750366,8.76456189144025e-06
93093,186187,186186,372373,60.65077090263367,8.74154776047529e-06
93193,186387,186386,372773,60.71414566040039,8.718594063931502e-06
93293,186587,186586,373173,60.774542808532715,8.69570064296409e-06
93393,186787,186786,373573,60.83701181411743,8.672867339118376e-06
93493,186987,186986,373973,60.89744472503662,8.650093994644548e-06
93594,187189,187188,374377,60.95997977256775,8.627153618231377e-06
93694,187389,187388,374777,61.01917290687561,8.604500315880699e-06
93794,187589,187588,375177,61.079434871673584,8.581906500167287e-06
93894,187789,187788,375577,61.143789768218994,8.559372014568675e-06
93994,187989,187988,375977,61.20530080795288,8.536896703382973e-06
94094,188189,188188,376377,61.26762390136719,8.51448041113686e-06
94194,188389,188388,376777,61.3402099609375,8.492122982742851e-06
94294,188589,188588,377177,61.418150901794434,8.469824263595075e-06
94394,188789,188788,377577,61.48151397705078,8.447584099478365e-06
94494,188989,188988,377977,61.541154861450195,8.425402336658989e-06
94595,189191,189190,378381,61.60847282409668,8.403057880107026e-06
94695,189391,189390,378781,61.66924977302551,8.380993040051644e-06
94795,189591,189590,379181,61.729530811309814,8.358986140706932e-06
94895,189791,189790,379581,61.79324173927307,8.337037029693978e-06
94995,189991,189990,379981,61.85584473609924,8.315145555526873e-06
95095,190191,190190,380381,61.918139934539795,8.293311566688538e-06
95195,190391,190390,380781,61.982097864151,8.271534912131095e-06
95295,190591,190590,381181,62.04397487640381,8.249815441257319e-06
95395,190791,190790,381581,62.108863830566406,8.228153003993022e-06
95495,190991,190990,381981,62.1702516078949,8.20654745034469e-06
95596,191193,191192,382385,62.234365940093994,8.18478342861278e-06
95696,191393,191392,382785,62.30076599121094,8.163291759574838e-06
95796,191593,191592,383185,62.3842077255249,8.141856525790952e-06
95896,191793,191792,383585,62.46625280380249,8.120477578772226e-06
95996,191993,191992,383985,62.53123474121094,8.099154771029846e-06
96096,192193,192192,384385,62.60042190551758,8.077887954753892e-06
96196,192393,192392,384785,62.6646249294281,8.056676983023173e-06
96296,192593,192592,385185,62.72741079330444,8.035521709281445e-06
96396,192793,192792,385585,62.790751934051514,8.01442198711689e-06
96496,192993,192992,385985,62.8533399105072,7.993377670530982e-06
96597,193195,193194,386389,62.915512800216675,7.972179002151493e-06
96697,193395,193394,386789,62.979718923568726,7.951245611324585e-06
96797,193595,193594,387189,63.04375076293945,7.930367189221866e-06
96897,193795,193794,387589,63.10781383514404,7.909543591465406e-06
96997,193995,193994,387989,63.17216682434082,7.888774674113965e-06
97097,194195,194194,388389,63.23477387428284,7.868060293792467e-06
97197,194395,194394,388789,63.30028796195984,7.847400306949162e-06
97297,194595,194594,389189,63.36410188674927,7.82679457074163e-06
97397,194795,194794,389589,63.428107023239136,7.806242942921378e-06
97497,194995,194994,389989,63.50613284111023,7.785745281091523e-06
97598,195197,195196,390393,63.584152698516846,7.765097276632814e-06
97698,195397,195396,390793,63.65177869796753,7.744707658473797e-06
97798,195597,195596,391193,63.7145049571991,7.724371580820378e-06
97898,195797,195796,391593,63.77921104431152,7.704088903287185e-06
97998,195997,195996,391993,63.84142279624939,7.683859485397779e-06
98098,196197,196196,392393,63.9047737121582,7.66368318755156e-06
98198,196397,196396,392793,63.96815490722656,7.643559869844438e-06
98298,196597,196596,393193,64.03508567810059,7.623489393519238e-06
98398,196797,196796,393593,64.10143899917603,7.603471619576296e-06
98498,196997,196996,393993,64.16545176506042,7.583506409682425e-06
98599,197199,197198,394397,64.22760677337646,7.563394762203865e-06
98699,197399,197398,394797,64.29047298431396,7.543534788658607e-06
98799,197599,197598,395197,64.35208988189697,7.5237269649544795e-06
98899,197799,197798,395597,64.41716885566711,7.5039711537993115e-06
98999,197999,197998,395997,64.48248672485352,7.484267218548834e-06
99099,198199,198198,396397,64.54431176185608,7.464615023158375e-06
99199,198399,198398,396797,64.60906767845154,7.445014431702537e-06
99299,198599,198598,397197,64.67135286331177,7.425465308523278e-06
99399,198799,198798,397597,64.73917484283447,7.405967518857829e-06
99499,198999,198998,397997,64.80042481422424,7.386520927231448e-06
99600,199201,199200,398401,64.86484575271606,7.366931701973265e-06
99700,199401,199400,398801,64.92686080932617,7.3475876126997645e-06
99800,199601,199600,399201,64.99025583267212,7.3282943183382445e-06
99900,199801,199800,399601,65.05600571632385,7.309051685286365e-06
100000,200001,200000,400001,65.12728381156921,7.289859580783329e-06


==> extragradient/plot_data/bilinear_matrix_game_n250/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00047588348388671875,2.0175302852282635
100,201,200,401,0.07343316078186035,0.03870059256068895
200,401,400,801,0.1350259780883789,0.0179642168274124
300,601,600,1201,0.21738910675048828,0.010215612352113134
400,801,800,1601,0.3028271198272705,0.006414884987572114
501,1003,1002,2005,0.38286495208740234,0.004292887866686561
601,1203,1202,2405,0.4563760757446289,0.0031981848552840673
701,1403,1402,2805,0.5311760902404785,0.0023495755858960704
801,1603,1602,3205,0.606680154800415,0.0017642014700653555
901,1803,1802,3605,0.6794161796569824,0.0013107140383380224
1001,2003,2002,4005,0.754554033279419,0.0010771361342336561
1101,2203,2202,4405,0.821796178817749,0.0008891647471929582
1201,2403,2402,4805,0.8943130970001221,0.0007896238285358858
1301,2603,2602,5205,0.9764370918273926,0.0007243730865874144
1401,2803,2802,5605,1.0550200939178467,0.000648621889859143
1502,3005,3004,6009,1.1196181774139404,0.000605342378155228
1602,3205,3204,6409,1.1941471099853516,0.0005733026994351765
1702,3405,3404,6809,1.2673139572143555,0.0005447368428944139
1802,3605,3604,7209,1.4162800312042236,0.00048258186702094223
1902,3805,3804,7609,1.5148448944091797,0.00043623502306099424
2002,4005,4004,8009,1.5982789993286133,0.0004039543762459166
2102,4205,4204,8409,1.6816120147705078,0.00037891678446560513
2202,4405,4404,8809,1.7489171028137207,0.00035856970156738626
2302,4605,4604,9209,1.8173861503601074,0.00034167885404962273
2402,4805,4804,9609,1.8881070613861084,0.000327471216222133
2503,5007,5006,10013,1.9650418758392334,0.00031528514633575623
2603,5207,5206,10413,2.035529136657715,0.00030494059155017047
2703,5407,5406,10813,2.1040210723876953,0.0002959793336833732
2803,5607,5606,11213,2.1681830883026123,0.0002881403091160926
2903,5807,5806,11613,2.231938123703003,0.000281214281208699
3003,6007,6006,12013,2.3091230392456055,0.0002750331765274161
3103,6207,6206,12413,2.400527238845825,0.00026946189858635845
3203,6407,6406,12813,2.4808499813079834,0.00026439183980072673
3303,6607,6606,13213,2.547389030456543,0.00025973566986274647
3403,6807,6806,13613,2.618852138519287,0.000255423132572343
3504,7009,7008,14017,2.7045681476593018,0.0002513586896688166
3604,7209,7208,14417,2.79475998878479,0.0002475768793537788
3704,7409,7408,14817,2.8882720470428467,0.00024399934675541638
3804,7609,7608,15217,2.964362144470215,0.00024059633077260883
3904,7809,7808,15617,3.0376369953155518,0.00023734367502605227
4004,8009,8008,16017,3.1161391735076904,0.00023422171215643902
4104,8209,8208,16417,3.2095940113067627,0.00023121437386540734
4204,8409,8408,16817,3.2963531017303467,0.00022830848122147552
4304,8609,8608,17217,3.383721113204956,0.0002254931786417318
4404,8809,8808,17617,3.479944944381714,0.00022275948222810613
4505,9011,9010,18021,3.5598201751708984,0.0002200736757568169
4605,9211,9210,18421,3.6319000720977783,0.00021748264631160484
4705,9411,9410,18821,3.698601007461548,0.00021495419299109208
4805,9611,9610,19221,3.777956962585449,0.00021248387115568304
4905,9811,9810,19621,3.870835065841675,0.0002100678928804713
5005,10011,10010,20021,3.968748092651367,0.00020770300764981782
5105,10211,10210,20421,4.083566188812256,0.00020538640619713179
5205,10411,10410,20821,4.1821582317352295,0.0002031156428412569
5305,10611,10610,21221,4.277889013290405,0.00020088857263204926
5405,10811,10810,21621,4.38100004196167,0.0001987033003656253
5506,11013,11012,22025,4.483083009719849,0.00019653688483370254
5606,11213,11212,22425,4.592471122741699,0.00019443070110695764
5706,11413,11412,22825,4.675595045089722,0.0001923617375405541
5806,11613,11612,23225,4.754606246948242,0.0001903287540892684
5906,11813,11812,23625,4.830786228179932,0.00018833061625778637
6006,12013,12012,24025,4.916647911071777,0.00018636627982224012
6106,12213,12212,24425,4.998574256896973,0.00018443477820151422
6206,12413,12412,24825,5.078344106674194,0.00018253521198341002
6306,12613,12612,25225,5.151682138442993,0.00018066674020936473
6406,12813,12812,25625,5.2225470542907715,0.00017882857309627258
6507,13015,13014,26029,5.29066014289856,0.0001770020267232668
6607,13215,13214,26429,5.359029054641724,0.00017522255984983156
6707,13415,13414,26829,5.423156023025513,0.0001734712724405494
6807,13615,13614,27229,5.489932060241699,0.0001717475275193629
6907,13815,13814,27629,5.555908918380737,0.00017005071684054419
7007,14015,14014,28029,5.621159076690674,0.00016838025819878897
7107,14215,14214,28429,5.6914591789245605,0.00016673559311093918
7207,14415,14414,28829,5.75805401802063,0.00016511618481099277
7307,14615,14614,29229,5.82707405090332,0.000163521516504671
7407,14815,14814,29629,5.896754026412964,0.00016195108984464797
7508,15017,15016,30033,5.963438987731934,0.0001603890753312936
7608,15217,15216,30433,6.033016204833984,0.0001588659348191652
7708,15417,15416,30833,6.100348949432373,0.00015736563452041881
7808,15617,15616,31233,6.168921947479248,0.00015588773806327232
7908,15817,15816,31633,6.249572992324829,0.00015443182216535014
8008,16017,16016,32033,6.3154072761535645,0.0001529974758801278
8108,16217,16216,32433,6.382838010787964,0.00015158429991368803
8208,16417,16416,32833,6.450484037399292,0.00015019190600647155
8308,16617,16616,33233,6.524154901504517,0.00014881991636835176
8408,16817,16816,33633,6.586607933044434,0.00014746796316294591
8509,17019,17018,34037,6.660737037658691,0.00014612246346770548
8609,17219,17218,34437,6.739203214645386,0.00014480970865508907
8709,17419,17418,34837,6.804547071456909,0.0001435159385685191
8809,17619,17618,35237,6.870097875595093,0.00014224082088285596
8909,17819,17818,35637,6.935740947723389,0.0001409840311898774
9009,18019,18018,36037,7.002842903137207,0.00013974525267497582
9109,18219,18218,36437,7.070187091827393,0.00013852417581637554
9209,18419,18418,36837,7.132735013961792,0.00013732049810336562
9309,18619,18618,37237,7.197118043899536,0.00013613392377165485
9409,18819,18818,37637,7.25817084312439,0.0001349641635563538
9510,19021,19020,38041,7.323210000991821,0.00013379948470752128
9610,19221,19220,38441,7.3848700523376465,0.00013266267093725852
9710,19421,19420,38841,7.4489359855651855,0.0001315418375357308
9810,19621,19620,39241,7.516002178192139,0.00013043671908828831
9910,19821,19820,39641,7.577508211135864,0.00012934705563775144
10010,20021,20020,40041,7.645086050033569,0.00012827259250720958
10110,20221,20220,40441,7.711074113845825,0.0001272130801360416
10210,20421,20420,40841,7.773271083831787,0.0001261682739210451
10310,20621,20620,41241,7.833543062210083,0.00012513793406670548
10410,20821,20820,41641,7.892524003982544,0.00012412182544308851
10511,21023,21022,42045,7.955588102340698,0.00012310976630411754
10611,21223,21222,42445,8.026118993759155,0.00012212156935771686
10711,21423,21422,42845,8.090049028396606,0.00012114692271993615
10811,21623,21622,43245,8.15012001991272,0.000120185608667928
10911,21823,21822,43645,8.209603071212769,0.00011923741352364664
11011,22023,22022,44045,8.270666122436523,0.00011830212754717816
11111,22223,22222,44445,8.33216905593872,0.00011737954483300902
11211,22423,22422,44845,8.391311168670654,0.00011646946321229426
11311,22623,22622,45245,8.456070899963379,0.00011557168415702394
11411,22823,22822,45645,8.524376153945923,0.00011468601269024659
11512,23025,23024,46049,8.585857152938843,0.00011380357928193565
11612,23225,23224,46449,8.646278858184814,0.00011294166817294914
11712,23425,23424,46849,8.706762075424194,0.00011209129834021222
11812,23625,23624,47249,8.773117065429688,0.00011125228820360766
11912,23825,23824,47649,8.849900007247925,0.00011042445932999713
12012,24025,24024,48049,8.920488119125366,0.0001096076363612358
12112,24225,24224,48449,8.986858129501343,0.00010880164694508419
12212,24425,24424,48849,9.055395126342773,0.00010800632166848759
12312,24625,24624,49249,9.124843120574951,0.00010722149399299883
12412,24825,24824,49649,9.190991163253784,0.00010644700019297531
12513,25027,25026,50053,9.255736112594604,0.00010567508692150307
12613,25227,25226,50453,9.323813915252686,0.00010492088000252017
12713,25427,25426,50853,9.412030935287476,0.00010417653052252305
12813,25627,25626,51253,9.493982076644897,0.00010344188545014195
12913,25827,25826,51653,9.562824010848999,0.00010271679428441283
13013,26027,26026,52053,9.630218982696533,0.0001020011090041051
13113,26227,26226,52453,9.693585872650146,0.00010129468401762708
13213,26427,26426,52853,9.75853705406189,0.00010059737611571367
13313,26627,26626,53253,9.822446823120117,9.990904442504029e-05
13413,26827,26826,53653,9.884482145309448,9.922955036211032e-05
13514,27029,27028,54057,9.974233865737915,9.855209314758345e-05
13614,27229,27228,54457,10.076505184173584,9.788995253410103e-05
13714,27429,27428,54857,10.16294813156128,9.723624579831776e-05
13814,27629,27628,55257,10.247828006744385,9.659084311227403e-05
13914,27829,27828,55657,10.311815977096558,9.595361673015083e-05
14014,28029,28028,56057,10.372221946716309,9.532444095068601e-05
14114,28229,28228,56457,10.435741901397705,9.470319207907087e-05
14214,28429,28428,56857,10.50788402557373,9.408974839206253e-05
14314,28629,28628,57257,10.57536792755127,9.348399010080046e-05
14414,28829,28828,57657,10.641330003738403,9.28857993179508e-05
14515,29031,29030,58061,10.701415061950684,9.228918987302865e-05
14615,29231,29230,58461,10.76329493522644,9.170586068479885e-05
14715,29431,29430,58861,10.823459148406982,9.112975530307399e-05
14815,29631,29630,59261,10.883630990982056,9.056076313423452e-05
14915,29831,29830,59661,10.959683179855347,8.99987753263165e-05
15015,30031,30030,60061,11.034543991088867,8.94436847378516e-05
15115,30231,30230,60461,11.09489893913269,8.889538590984509e-05
15215,30431,30430,60861,11.153671026229858,8.835377503693193e-05
15315,30631,30630,61261,11.215556144714355,8.78187499394078e-05
15415,30831,30830,61661,11.278244256973267,8.729021003659379e-05
15516,31033,31032,62065,11.340703010559082,8.676286670204717e-05
15616,31233,31232,62465,11.506344079971313,8.624706410975493e-05
15716,31433,31432,62865,11.588660955429077,8.57374533479452e-05
15816,31633,31632,63265,11.669956922531128,8.523393998619012e-05
15916,31833,31832,63665,11.739082098007202,8.473643106529019e-05
16016,32033,32032,64065,11.800426959991455,8.424483507322058e-05
16116,32233,32232,64465,11.860701084136963,8.375906192201825e-05
16216,32433,32432,64865,11.92795205116272,8.327902292558504e-05
16316,32633,32632,65265,11.994153022766113,8.280463077566314e-05
16416,32833,32832,65665,12.056287050247192,8.233579952114378e-05
16517,33035,33034,66069,12.11782193183899,8.186783836882488e-05
16617,33235,33234,66469,12.177124977111816,8.140992988516565e-05
16717,33435,33434,66869,12.23940896987915,8.095733155701019e-05
16817,33635,33634,67269,12.299065828323364,8.050996266081315e-05
16917,33835,33834,67669,12.358952045440674,8.006774372664463e-05
17017,34035,34034,68069,12.4217050075531,7.963059651706329e-05
17117,34235,34234,68469,12.485789060592651,7.919844400880142e-05
17217,34435,34434,68869,12.548320055007935,7.877121037323326e-05
17317,34635,34634,69269,12.608582973480225,7.834882095884943e-05
17417,34835,34834,69669,12.668835163116455,7.793120227196671e-05
17518,35037,35036,70073,12.734426975250244,7.751417624099244e-05
17618,35237,35236,70473,12.794718980789185,7.710592898752043e-05
17718,35437,35436,70873,12.854438066482544,7.670223805725681e-05
17818,35637,35636,71273,12.914785146713257,7.630303442478913e-05
17918,35837,35836,71673,12.976360082626343,7.590825013610193e-05
18018,36037,36036,72073,13.05699110031128,7.551781829324232e-05
18118,36237,36236,72473,13.134474039077759,7.513167303666393e-05
18218,36437,36436,72873,13.20080304145813,7.474974953090994e-05
18318,36637,36636,73273,13.26089096069336,7.437198394798899e-05
18418,36837,36836,73673,13.322571039199829,7.399831345240632e-05
18519,37039,37038,74077,13.383954048156738,7.362499997502704e-05
18619,37239,37238,74477,13.44687795639038,7.325937446272465e-05
18719,37439,37438,74877,13.512434959411621,7.289766074269952e-05
18819,37639,37638,75277,13.576700925827026,7.253979981131108e-05
18919,37839,37838,75677,13.637963056564331,7.2185733583804e-05
19019,38039,38038,76077,13.702265977859497,7.183540488073206e-05
19119,38239,38238,76477,13.763113975524902,7.148875741550155e-05
19219,38439,38438,76877,13.826855897903442,7.114573577934091e-05
19319,38639,38638,77277,13.88791823387146,7.080628542869801e-05
19419,38839,38838,77677,13.95231008529663,7.047035267272691e-05
19520,39041,39040,78081,14.019391059875488,7.013457729963545e-05
19620,39241,39240,78481,14.080207824707031,6.980555587168995e-05
19720,39441,39440,78881,14.144328117370605,6.947989544303976e-05
19820,39641,39640,79281,14.210116147994995,6.915754561282357e-05
19920,39841,39840,79681,14.271610975265503,6.88384567705233e-05
20020,40041,40040,80081,14.336351156234741,6.852258008345205e-05
20120,40241,40240,80481,14.401312112808228,6.820986748509168e-05
20220,40441,40440,80881,14.462592124938965,6.790027166386641e-05
20320,40641,40640,81281,14.52526307106018,6.759374605147888e-05
20420,40841,40840,81681,14.586520195007324,6.729024481193715e-05
20521,41043,41042,82085,14.650897026062012,6.698673250509319e-05
20621,41243,41242,82485,14.712496995925903,6.668917450416247e-05
20721,41443,41442,82885,14.774214029312134,6.639450721864771e-05
20821,41643,41642,83285,14.837050914764404,6.610268763956923e-05
20921,41843,41842,83685,14.89735198020935,6.581367343690462e-05
21021,42043,42042,84085,14.960206031799316,6.552742294888833e-05
21121,42243,42242,84485,15.031552076339722,6.524389517202788e-05
21221,42443,42442,84885,15.10669493675232,6.496304975121927e-05
21321,42643,42642,85285,15.180561065673828,6.468484696983597e-05
21421,42843,42842,85685,15.26571798324585,6.440924774014854e-05
21522,43045,43044,86089,15.338438987731934,6.41334960777934e-05
21622,43245,43244,86489,15.401171922683716,6.38630142401576e-05
21722,43445,43444,86889,15.4708731174469,6.359502200085604e-05
21822,43645,43644,87289,15.554537057876587,6.332948269971798e-05
21922,43845,43844,87689,15.656753063201904,6.30663602598269e-05
22022,44045,44044,88089,15.742815971374512,6.280561917716129e-05
22122,44245,44244,88489,15.826184034347534,6.254722451316279e-05
22222,44445,44444,88889,15.896483182907104,6.229114188589911e-05
22322,44645,44644,89289,15.959712982177734,6.203733746082567e-05
22422,44845,44844,89689,16.028170108795166,6.17857779432218e-05
22523,45047,45046,90093,16.095652103424072,6.15339481577865e-05
22623,45247,45246,90493,16.16066598892212,6.128680232625892e-05
22723,45447,45446,90893,16.22472906112671,6.104180435902917e-05
22823,45647,45646,91293,16.28817892074585,6.0798923043198106e-05
22923,45847,45846,91693,16.352083921432495,6.0558127666077395e-05
23023,46047,46046,92093,16.4148428440094,6.0319388005680966e-05
23123,46247,46246,92493,16.48942494392395,6.008267432479922e-05
23223,46447,46446,92893,16.576825857162476,5.984795736310033e-05
23323,46647,46646,93293,16.654251098632812,5.96152083296387e-05
23423,46847,46846,93693,16.726219177246094,5.938439889501202e-05
23524,47049,47048,94097,16.797863006591797,5.915322176959705e-05
23624,47249,47248,94497,16.86500310897827,5.892622706563186e-05
23724,47449,47448,94897,16.93070697784424,5.870108940807669e-05
23824,47649,47648,95297,17.00060200691223,5.847778225090531e-05
23924,47849,47848,95697,17.07359004020691,5.825627947499746e-05
24024,48049,48048,96097,17.14391803741455,5.803655538210418e-05
24124,48249,48248,96497,17.209400177001953,5.781858468792967e-05
24224,48449,48448,96897,17.28093385696411,5.760234251642121e-05
24324,48649,48648,97297,17.36248517036438,5.7387804392374776e-05
24424,48849,48848,97697,17.436079025268555,5.717494623594152e-05
24525,49051,49050,98101,17.50133991241455,5.696164062245334e-05
24625,49251,49250,98501,17.566242218017578,5.675208792416326e-05
24725,49451,49450,98901,17.626689195632935,5.6544145035742415e-05
24825,49651,49650,99301,17.687072038650513,5.633778939997808e-05
24925,49851,49850,99701,17.747967958450317,5.613299882503801e-05
25025,50051,50050,100101,17.808813095092773,5.592975147842594e-05
25125,50251,50250,100501,17.87018609046936,5.5728025881110405e-05
25225,50451,50450,100901,17.93022894859314,5.552780090197602e-05
25325,50651,50650,101301,17.997947931289673,5.532905575236193e-05
25425,50851,50850,101701,18.058608055114746,5.5131769980631085e-05
25526,51053,51052,102105,18.122747898101807,5.493397220296787e-05
25626,51253,51252,102505,18.184081077575684,5.473955924971031e-05
25726,51453,51452,102905,18.246819019317627,5.454654609613513e-05
25826,51653,51652,103305,18.30887198448181,5.435491358867113e-05
25926,51853,51852,103705,18.368821144104004,5.416464288595694e-05
26026,52053,52052,104105,18.427808046340942,5.3975715451758205e-05
26126,52253,52252,104505,18.489118099212646,5.378811305171785e-05
26226,52453,52452,104905,18.554276943206787,5.360181774731357e-05
26326,52653,52652,105305,18.61440896987915,5.34168118919679e-05
26426,52853,52852,105705,18.673380851745605,5.323307812581171e-05
26527,53055,53054,106109,18.73564600944519,5.304878086415723e-05
26627,53255,53254,106509,18.80081009864807,5.2867552619982375e-05
26727,53455,53454,106909,18.86258316040039,5.2687545897219964e-05
26827,53655,53654,107309,18.923017024993896,5.250874444120578e-05
26927,53855,53854,107709,18.986143112182617,5.2331132261406814e-05
27027,54055,54054,108109,19.048579216003418,5.215469362782098e-05
27127,54255,54254,108509,19.109400033950806,5.197941306635809e-05
27227,54455,54454,108909,19.17191195487976,5.1805275354476744e-05
27327,54655,54654,109309,19.232340097427368,5.1632265517846414e-05
27427,54855,54854,109709,19.29310703277588,5.1460368825518695e-05
27528,55057,55056,110113,19.356661081314087,5.1287868306265416e-05
27628,55257,55256,110513,19.416484832763672,5.111816543831433e-05
27728,55457,55456,110913,19.494091033935547,5.09495328064174e-05
27828,55657,55656,111313,19.570528984069824,5.078195661803489e-05
27928,55857,55856,111713,19.63014006614685,5.0615423305065665e-05
28028,56057,56056,112113,19.69282102584839,5.0449919519951715e-05
28128,56257,56256,112513,19.75321912765503,5.028543213283578e-05
28228,56457,56456,112913,19.812342166900635,5.012194822687067e-05
28328,56657,56656,113313,19.871321201324463,4.995945509631485e-05
28428,56857,56856,113713,19.93083119392395,4.9797940240634196e-05
28529,57059,57058,114117,19.995983839035034,4.9635790712233653e-05
28629,57259,57258,114517,20.057284116744995,4.947620519613613e-05
28729,57459,57458,114917,20.119473934173584,4.931756154448826e-05
28829,57659,57658,115317,20.179906129837036,4.915984805257059e-05
28929,57859,57858,115717,20.241369247436523,4.9003053205780613e-05
29029,58059,58058,116117,20.30073094367981,4.8847165676960624e-05
29129,58259,58258,116517,20.361204147338867,4.86921743226596e-05
29229,58459,58458,116917,20.42389416694641,4.853806817981771e-05
29329,58659,58658,117317,20.489437103271484,4.838483646400338e-05
29429,58859,58858,117717,20.552964210510254,4.823246856530781e-05
29530,59061,59060,118121,20.614126205444336,4.807944317543942e-05
29630,59261,59260,118521,20.675737142562866,4.7928780146489794e-05
29730,59461,59460,118921,20.734943151474,4.77789500257163e-05
29830,59661,59660,119321,20.793910026550293,4.762994287589807e-05
29930,59861,59860,119721,20.86021399497986,4.74817489207553e-05
30030,60061,60060,120121,20.92821192741394,4.7334358542261396e-05
30130,60261,60260,120521,21.000325918197632,4.7187762277395645e-05
30230,60461,60460,120921,21.059906005859375,4.704195081676821e-05
30330,60661,60660,121321,21.11972212791443,4.689691500079174e-05
30430,60861,60860,121721,21.179396152496338,4.6752645817759055e-05
30531,61063,61062,122125,21.240628957748413,4.66077030845435e-05
30631,61263,61262,122525,21.300339937210083,4.6464948158740704e-05
30731,61463,61462,122925,21.360275983810425,4.632293360830165e-05
30831,61663,61662,123325,21.4247989654541,4.6181650990126026e-05
30931,61863,61862,123725,21.489184141159058,4.604109199664402e-05
31031,62063,62062,124125,21.549930095672607,4.590124845406999e-05
31131,62263,62262,124525,21.626277923583984,4.576211231931207e-05
31231,62463,62462,124925,21.70211410522461,4.5623675679175676e-05
31331,62663,62662,125325,21.764585971832275,4.5485930746875977e-05
31431,62863,62862,125725,21.823428869247437,4.534886986040284e-05
31532,63065,63064,126129,21.884209871292114,4.521112502764261e-05
31632,63265,63264,126529,21.945003032684326,4.5075416389486785e-05
31732,63465,63464,126929,22.009697198867798,4.494036946647604e-05
31832,63665,63664,127329,22.07280993461609,4.480597707620194e-05
31932,63865,63864,127729,22.133182048797607,4.467223215084162e-05
32032,64065,64064,128129,22.196921825408936,4.453912773524867e-05
32132,64265,64264,128529,22.25826406478882,4.440665698460036e-05
32232,64465,64464,128929,22.318892002105713,4.4274813163455194e-05
32332,64665,64664,129329,22.382190227508545,4.414358964266024e-05
32432,64865,64864,129729,22.442739963531494,4.4012979898811586e-05
32533,65067,65066,130133,22.507764101028442,4.388168053371468e-05
32633,65267,65266,130533,22.56766390800476,4.3752285163802853e-05
32733,65467,65466,130933,22.62724208831787,4.362348455197484e-05
32833,65667,65666,131333,22.68734383583069,4.349527257846508e-05
32933,65867,65866,131733,22.754194974899292,4.336764322057305e-05
33033,66067,66066,132133,22.817228078842163,4.324059055024682e-05
33133,66267,66266,132533,22.87998390197754,4.3114108732870426e-05
33233,66467,66466,132933,22.941440105438232,4.2988192024788874e-05
33333,66667,66666,133333,23.004770040512085,4.286283477379785e-05
33433,66867,66866,133733,23.065598011016846,4.273803141498402e-05
33534,67069,67068,134137,23.12633204460144,4.2612536673078805e-05
33634,67269,67268,134537,23.187089920043945,4.248883015614444e-05
33734,67469,67468,134937,23.24946117401123,4.23656613025213e-05
33834,67669,67668,135337,23.315654039382935,4.224302488806544e-05
33934,67869,67868,135737,23.375306129455566,4.212091576986844e-05
34034,68069,68068,136137,23.435209035873413,4.199932888547904e-05
34134,68269,68268,136537,23.501359939575195,4.187825925009619e-05
34234,68469,68468,136937,23.561525106430054,4.175770195691165e-05
34334,68669,68668,137337,23.62149405479431,4.1637652174587665e-05
34434,68869,68868,137737,23.685164213180542,4.151810514622675e-05
34535,69071,69070,138141,23.762242078781128,4.139786819858964e-05
34635,69271,69270,138541,23.837980031967163,4.1279317611775465e-05
34735,69471,69470,138941,23.900025129318237,4.116125589861157e-05
34835,69671,69670,139341,23.96117091178894,4.104367858893266e-05
34935,69871,69870,139741,24.024566173553467,4.0926581280700996e-05
35035,70071,70070,140141,24.086927890777588,4.080995963938163e-05
35135,70271,70270,140541,24.1510910987854,4.069380939636397e-05
35235,70471,70470,140941,24.21554684638977,4.057812634818032e-05
35335,70671,70670,141341,24.275197982788086,4.0462906354930845e-05
35435,70871,70870,141741,24.336708068847656,4.034814533943403e-05
35536,71073,71072,142145,24.400001049041748,4.023269851009812e-05
35636,71273,71272,142545,24.465681076049805,4.0118847955303736e-05
35736,71473,71472,142945,24.529128074645996,4.0005444474302674e-05
35836,71673,71672,143345,24.591012239456177,3.989248423133194e-05
35936,71873,71872,143745,24.650862216949463,3.977996344779066e-05
36036,72073,72072,144145,24.710915088653564,3.966787840167345e-05
36136,72273,72272,144545,24.771440982818604,3.9556225426652794e-05
36236,72473,72472,144945,24.835297107696533,3.944500091107113e-05
36336,72673,72672,145345,24.898639917373657,3.9334201296940535e-05
36436,72873,72872,145745,24.958641052246094,3.922382307882055e-05
36537,73075,73074,146149,25.02669405937195,3.911276530013233e-05
36637,73275,73274,146549,25.086930990219116,3.9003223693911626e-05
36737,73475,73474,146949,25.146661043167114,3.889409324269979e-05
36837,73675,73674,147349,25.20660400390625,3.878537064403034e-05
36937,73875,73874,147749,25.265960931777954,3.867705264373247e-05
37037,74075,74074,148149,25.326695919036865,3.8569136035575155e-05
37137,74275,74274,148549,25.386808156967163,3.846161765936627e-05
37237,74475,74474,148949,25.448529958724976,3.8354494401890974e-05
37337,74675,74674,149349,25.516902923583984,3.824776319413055e-05
37437,74875,74874,149749,25.578537940979004,3.814142101205568e-05
37538,75077,75076,150153,25.640088081359863,3.803440725340683e-05
37638,75277,75276,150553,25.70636010169983,3.79288380403949e-05
37738,75477,75476,150953,25.768594980239868,3.782364901093012e-05
37838,75677,75676,151353,25.829385995864868,3.7718837310885584e-05
37938,75877,75876,151753,25.906239986419678,3.7614400127851394e-05
38038,76077,76076,152153,25.98167395591736,3.751033468881929e-05
38138,76277,76276,152553,26.044738054275513,3.740663826028056e-05
38238,76477,76476,152953,26.108609199523926,3.730330814739174e-05
38338,76677,76676,153353,26.169402837753296,3.720034169323855e-05
38438,76877,76876,153753,26.23012113571167,3.709773627867321e-05
38539,77079,77078,154157,26.29254984855652,3.699446865294886e-05
38639,77279,77278,154557,26.356276988983154,3.6892581151433304e-05
38739,77479,77478,154957,26.419641971588135,3.679104702434905e-05
38839,77679,77678,155357,26.486824989318848,3.668986379534003e-05
38939,77879,77878,155757,26.550708055496216,3.6589029022979676e-05
39039,78079,78078,156157,26.614723205566406,3.648854029927933e-05
39139,78279,78278,156557,26.678500175476074,3.638839524956265e-05
39239,78479,78478,156957,26.741147994995117,3.6288591531761835e-05
39339,78679,78678,157357,26.805557012557983,3.61891268352783e-05
39439,78879,78878,157757,26.86624312400818,3.608999888182181e-05
39540,79081,79080,158161,26.925209045410156,3.5990219170194606e-05
39640,79281,79280,158561,26.988821983337402,3.589176130081737e-05
39740,79481,79480,158961,27.054599046707153,3.579363349966635e-05
39840,79681,79680,159361,27.11619806289673,3.569583360914854e-05
39940,79881,79880,159761,27.176886081695557,3.559835949977883e-05
40040,80081,80080,160161,27.23843216896057,3.5501209071416535e-05
40140,80281,80280,160561,27.30005717277527,3.5404380251281975e-05
40240,80481,80480,160961,27.359698057174683,3.5307870994029904e-05
40340,80681,80680,161361,27.425312042236328,3.5211679281427e-05
40440,80881,80880,161761,27.490803003311157,3.511580312144049e-05
40541,81083,81082,162165,27.553033113479614,3.5019286499979554e-05
40641,81283,81282,162565,27.611776113510132,3.492403868100052e-05
40741,81483,81482,162965,27.671313047409058,3.4829100574807754e-05
40841,81683,81682,163365,27.733587980270386,3.4734470291890646e-05
40941,81883,81882,163765,27.796478033065796,3.464014596647524e-05
41041,82083,82082,164165,27.85707402229309,3.45461257568566e-05
41141,82283,82282,164565,27.919551134109497,3.445240784510626e-05
41241,82483,82482,164965,27.98361301422119,3.435899043634538e-05
41341,82683,82682,165365,28.064504146575928,3.426587175791585e-05
41441,82883,82882,165765,28.13604211807251,3.4173050060040944e-05
41542,83085,83084,166169,28.19820809364319,3.4079599835957025e-05
41642,83285,83284,166569,28.258728981018066,3.3987369864515485e-05
41742,83485,83484,166969,28.32262396812439,3.3895431737749304e-05
41842,83685,83684,167369,28.3836190700531,3.380378379178892e-05
41942,83885,83884,167769,28.447817087173462,3.3712424383170477e-05
42042,84085,84084,168169,28.51190710067749,3.3621351888860514e-05
42142,84285,84284,168569,28.572402000427246,3.3530564705567713e-05
42242,84485,84484,168969,28.634758949279785,3.344006124921282e-05
42342,84685,84684,169369,28.69732689857483,3.3349839955396146e-05
42442,84885,84884,169769,28.757309913635254,3.325989927833864e-05
42543,85087,85086,170173,28.817710161209106,3.316934247953814e-05
42643,85287,85286,170573,28.878966093063354,3.307996124134588e-05
42743,85487,85486,170973,28.938889026641846,3.2990856078097836e-05
42843,85687,85686,171373,29.004228115081787,3.2902025516997306e-05
42943,85887,85886,171773,29.067846059799194,3.2813468102134975e-05
43043,86087,86086,172173,29.12875008583069,3.2725182394760776e-05
43143,86287,86286,172573,29.189945936203003,3.2637166973119995e-05
43243,86487,86486,172973,29.249550104141235,3.2549420431910284e-05
43343,86687,86686,173373,29.314621925354004,3.246194138205185e-05
43443,86887,86886,173773,29.374917030334473,3.2374728450169683e-05
43544,87089,87088,174177,29.437520027160645,3.2286912129785224e-05
43644,87289,87288,174577,29.502690076828003,3.220023000499881e-05
43744,87489,87488,174977,29.564358949661255,3.211380995897561e-05
43844,87689,87688,175377,29.625138998031616,3.2027650679817884e-05
43944,87889,87888,175777,29.687814950942993,3.194175087097991e-05
44044,88089,88088,176177,29.748260974884033,3.185610924959775e-05
44144,88289,88288,176577,29.81150507926941,3.177072454766679e-05
44244,88489,88488,176977,29.87224292755127,3.1685595510624095e-05
44344,88689,88688,177377,29.935152053833008,3.1600720897995835e-05
44444,88889,88888,177777,29.99995493888855,3.151609948276434e-05
44545,89091,89090,178181,30.06231999397278,3.14308876253352e-05
44645,89291,89290,178581,30.127152919769287,3.134677147855145e-05
44745,89491,89490,178981,30.206428050994873,3.12629049154091e-05
44845,89691,89690,179381,30.277119159698486,3.117928676108141e-05
44945,89891,89890,179781,30.33815884590149,3.109591585283589e-05
45045,90091,90090,180181,30.40171194076538,3.101279104053156e-05
45145,90291,90290,180581,30.463276147842407,3.092991118627236e-05
45245,90491,90490,180981,30.52742099761963,3.0847275163573484e-05
45345,90691,90690,181381,30.586591958999634,3.076488185817855e-05
45445,90891,90890,181781,30.64703893661499,3.068273016674983e-05
45546,91093,91092,182185,30.70935821533203,3.060000109696152e-05
45646,91293,91292,182585,30.769718170166016,3.051833175864916e-05
45746,91493,91492,182985,30.830543994903564,3.0436900781789743e-05
45846,91693,91692,183385,30.889766931533813,3.035570710759452e-05
45946,91893,91892,183785,30.949860095977783,3.0274749687879228e-05
46046,92093,92092,184185,31.014179229736328,3.019402748502417e-05
46146,92293,92292,184585,31.07537317276001,3.0113539471342186e-05
46246,92493,92492,184985,31.134984970092773,3.0033284629731675e-05
46346,92693,92692,185385,31.194934129714966,2.9953261952689638e-05
46446,92893,92892,185785,31.253893852233887,2.9873470442305168e-05
46547,93095,93094,186189,31.315081119537354,2.97931146568962e-05
46647,93295,93294,186589,31.37522602081299,2.9713784813298593e-05
46747,93495,93494,186989,31.437015056610107,2.9634683191163725e-05
46847,93695,93694,187389,31.504925966262817,2.9555808830914836e-05
46947,93895,93894,187789,31.565916061401367,2.947716078132438e-05
47047,94095,94094,188189,31.626742124557495,2.9398738100701532e-05
47147,94295,94294,188589,31.6867778301239,2.9320539855758794e-05
47247,94495,94494,188989,31.74597716331482,2.9242565122036886e-05
47347,94695,94694,189389,31.80498504638672,2.9164812983457692e-05
47447,94895,94894,189789,31.866416931152344,2.9087282532179822e-05
47548,95097,95096,190193,31.926162004470825,2.9009200884041206e-05
47648,95297,95296,190593,31.98571491241455,2.8932113311716377e-05
47748,95497,95496,190993,32.046512842178345,2.8855244743650734e-05
47848,95697,95696,191393,32.10714411735535,2.877859430446245e-05
47948,95897,95896,191793,32.16607904434204,2.8702161126272125e-05
48048,96097,96096,192193,32.227293968200684,2.862594434899295e-05
48148,96297,96296,192593,32.29750108718872,2.8549943120269324e-05
48248,96497,96496,192993,32.37343215942383,2.8474156594495263e-05
48348,96697,96696,193393,32.435569047927856,2.8398583933947197e-05
48448,96897,96896,193793,32.50310516357422,2.8323224307540278e-05
48549,97099,97098,194197,32.56303906440735,2.8247326486691827e-05
48649,97299,97298,194597,32.622446060180664,2.817239257455151e-05
48749,97499,97498,194997,32.68220806121826,2.8097669238021834e-05
48849,97699,97698,195397,32.742225885391235,2.8023155674178978e-05
48949,97899,97898,195797,32.79985809326172,2.7948851086527247e-05
49049,98099,98098,196197,32.86019992828369,2.7874754684591886e-05
49149,98299,98298,196597,32.91786289215088,2.780086568570416e-05
49249,98499,98498,196997,32.97821593284607,2.7727183311740008e-05
49349,98699,98698,197397,33.04173707962036,2.7653706792183907e-05
49449,98899,98898,197797,33.1019721031189,2.758043536234747e-05
49550,99101,99100,198201,33.16315698623657,2.7506638621631794e-05
49650,99301,99300,198601,33.226613998413086,2.7433777132734744e-05
49750,99501,99500,199001,33.28790092468262,2.7361118467608967e-05
49850,99701,99700,199401,33.34882211685181,2.7288661885254508e-05
49950,99901,99900,199801,33.41244912147522,2.7216406650517186e-05
50050,100101,100100,200201,33.474843978881836,2.7144352033615213e-05
50150,100301,100300,200601,33.53719210624695,2.7072497310831866e-05
50250,100501,100500,201001,33.598244190216064,2.7000841762909114e-05
50350,100701,100700,201401,33.658616065979004,2.6929384677127086e-05
50450,100901,100900,201801,33.718199014663696,2.6858125345551605e-05
50551,101103,101102,202205,33.77887010574341,2.6786353435153334e-05
50651,101303,101302,202605,33.83878207206726,2.6715489468926942e-05
50751,101503,101502,203005,33.90007305145264,2.664482115731684e-05
50851,101703,101702,203405,33.96159315109253,2.6574347812971902e-05
50951,101903,101902,203805,34.026583194732666,2.6504068753598124e-05
51051,102103,102102,204205,34.08673691749573,2.6433983301478658e-05
51151,102303,102302,204605,34.145323038101196,2.6364090784217187e-05
51251,102503,102502,205005,34.20225787162781,2.6294390533643692e-05
51351,102703,102702,205405,34.25861096382141,2.622488188663606e-05
51451,102903,102902,205805,34.31529092788696,2.615556418426677e-05
51552,103105,103104,206209,34.37206411361694,2.6085746457375544e-05
51652,103305,103304,206609,34.444064140319824,2.6016810580009973e-05
51752,103505,103504,207009,34.51768708229065,2.5948063691814663e-05
51852,103705,103704,207409,34.57418608665466,2.587950515238442e-05
51952,103905,103904,207809,34.631526947021484,2.5811134324963e-05
52052,104105,104104,208209,34.691428899765015,2.5742950577323302e-05
52152,104305,104304,208609,34.75179195404053,2.567495328149912e-05
52252,104505,104504,209009,34.81348204612732,2.560714181311486e-05
52352,104705,104704,209409,34.87326002120972,2.5539515552817387e-05
52452,104905,104904,209809,34.933434009552,2.5472073884457064e-05
52553,105107,105106,210213,34.99685883522034,2.5404144546321363e-05
52653,105307,105306,210613,35.05789017677307,2.533707206083591e-05
52753,105507,105506,211013,35.116515159606934,2.5270182337160887e-05
52853,105707,105706,211413,35.176865100860596,2.520347477521847e-05
52953,105907,105906,211813,35.23504996299744,2.5136948778363798e-05
53053,106107,106106,212213,35.294333934783936,2.5070603753709034e-05
53153,106307,106306,212613,35.35459303855896,2.500443911217596e-05
53253,106507,106506,213013,35.41207003593445,2.4938454268183675e-05
53353,106707,106706,213413,35.46925902366638,2.48726486398525e-05
53453,106907,106906,213813,35.530752182006836,2.4807021648456734e-05
53554,107109,107108,214217,35.589913845062256,2.4740919127460702e-05
53654,107309,107308,214617,35.64864420890808,2.4675649460674334e-05
53754,107509,107508,215017,35.71019005775452,2.461055671077888e-05
53854,107709,107708,215417,35.76896905899048,2.4545640312633613e-05
53954,107909,107908,215817,35.82634496688843,2.4480899704857497e-05
54054,108109,108108,216217,35.884624004364014,2.441633432916529e-05
54154,108309,108308,216617,35.94183611869812,2.4351943630693313e-05
54254,108509,108508,217017,36.004230976104736,2.4287727057213384e-05
54354,108709,108708,217417,36.06269598007202,2.422368406037015e-05
54454,108909,108908,217817,36.1186089515686,2.4159814094366667e-05
54555,109111,109110,218221,36.17714786529541,2.4095480511209837e-05
54655,109311,109310,218621,36.234050035476685,2.403195669900347e-05
54755,109511,109510,219021,36.291516065597534,2.396860429375416e-05
54855,109711,109710,219421,36.34851789474487,2.390542276187011e-05
54955,109911,109910,219821,36.409252882003784,2.3842411572404317e-05
55055,110111,110110,220221,36.468438148498535,2.377957019812172e-05
55155,110311,110310,220621,36.53349995613098,2.3716898113502782e-05
55255,110511,110510,221021,36.60826921463013,2.3654394796708936e-05
55355,110711,110710,221421,36.678497076034546,2.3592059728499633e-05
55455,110911,110910,221821,36.736088037490845,2.352989239212878e-05
55556,111113,111112,222225,36.79369306564331,2.3467273115073354e-05
55656,111313,111312,222625,36.85337495803833,2.3405441367879728e-05
55756,111513,111512,223025,36.911197900772095,2.3343775813775845e-05
55856,111713,111712,223425,36.97515797615051,2.3282275946711545e-05
55956,111913,111912,223825,37.048951148986816,2.322094126385062e-05
56056,112113,112112,224225,37.11321187019348,2.3159771263642842e-05
56156,112313,112312,224625,37.1738440990448,2.3098765448635443e-05
56256,112513,112512,225025,37.234411001205444,2.3037923322603186e-05
56356,112713,112712,225425,37.2939510345459,2.2977244392556e-05
56456,112913,112912,225825,37.354856967926025,2.2916728167328615e-05
56557,113115,113114,226229,37.41774106025696,2.285577143627992e-05
56657,113315,113314,226629,37.47979497909546,2.2795580773450657e-05
56757,113515,113514,227029,37.541768074035645,2.2735551352643295e-05
56857,113715,113714,227429,37.60663414001465,2.2675682692531344e-05
56957,113915,113914,227829,37.66718506813049,2.2615974314403126e-05
57057,114115,114114,228229,37.72553300857544,2.2556425741619783e-05
57157,114315,114314,228629,37.784953117370605,2.2497036499421136e-05
57257,114515,114514,229029,37.844940185546875,2.2437806115965838e-05
57357,114715,114714,229429,37.90478014945984,2.2378734121140846e-05
57457,114915,114914,229829,37.96525812149048,2.23198200471003e-05
57558,115117,115116,230233,38.030476093292236,2.2260476655638483e-05
57658,115317,115316,230633,38.09724187850952,2.220187859615511e-05
57758,115517,115516,231033,38.17395806312561,2.2143437062694848e-05
57858,115717,115716,231433,38.27467393875122,2.208515159585446e-05
57958,115917,115916,231833,38.37975811958313,2.2027021738412768e-05
58058,116117,116116,232233,38.45366406440735,2.196904703531825e-05
58158,116317,116316,232633,38.53201413154602,2.1911227033862122e-05
58258,116517,116516,233033,38.603452920913696,2.1853561282433104e-05
58358,116717,116716,233433,38.67583203315735,2.179604933237747e-05
58458,116917,116916,233833,38.814563035964966,2.1738690736792868e-05
58559,117119,117118,234237,38.91707706451416,2.1680913764197943e-05
58659,117319,117318,234637,38.99020600318909,2.16238620660385e-05
58759,117519,117518,235037,39.05570101737976,2.1566962388363205e-05
58859,117719,117718,235437,39.121212005615234,2.1510214291852315e-05
58959,117919,117918,235837,39.194600105285645,2.145361733882728e-05
59059,118119,118118,236237,39.26524019241333,2.1397171093987558e-05
59159,118319,118318,236637,39.33371710777283,2.1340875123504925e-05
59259,118519,118518,237037,39.40707993507385,2.1284728995255595e-05
59359,118719,118718,237437,39.47681403160095,2.1228732279424487e-05
59459,118919,118918,237837,39.5463330745697,2.1172884547671173e-05
59560,119121,119120,238241,39.622212171554565,2.1116629130278112e-05
59660,119321,119320,238641,39.70764708518982,2.1061079567991885e-05
59760,119521,119520,239041,39.79366207122803,2.1005677711233096e-05
59860,119721,119720,239441,39.86970496177673,2.0950423138432683e-05
59960,119921,119920,239841,39.944485902786255,2.0895315430546292e-05
60060,120121,120120,240241,40.02109217643738,2.084035416953603e-05
60160,120321,120320,240641,40.085602045059204,2.0785538939042277e-05
60260,120521,120520,241041,40.154300928115845,2.0730869324710094e-05
60360,120721,120720,241441,40.22001004219055,2.0676344913662552e-05
60460,120921,120920,241841,40.28709411621094,2.0621965294468176e-05
60561,121123,121122,242245,40.36570596694946,2.0567188433262498e-05
60661,121323,121322,242645,40.46163892745972,2.051309860880756e-05
60761,121523,121522,243045,40.59351086616516,2.0459152348164386e-05
60861,121723,121722,243445,40.68087100982666,2.040534924679027e-05
60961,121923,121922,243845,40.761879205703735,2.035168890128138e-05
61061,122123,122122,244245,40.84949994087219,2.0298170909973146e-05
61161,122323,122322,244645,40.93617010116577,2.0244794872959396e-05
61261,122523,122522,245045,41.00992488861084,2.0191560391286615e-05
61361,122723,122722,245445,41.075340032577515,2.013846706802766e-05
61461,122923,122922,245845,41.140610218048096,2.0085514507503593e-05
61562,123125,123124,246249,41.20603799819946,2.0032174901477545e-05
61662,123325,123324,246649,41.26913905143738,1.9979504083596258e-05
61762,123525,123524,247049,41.33357501029968,1.9926972846823785e-05
61862,123725,123724,247449,41.4020721912384,1.9874580801212154e-05
61962,123925,123924,247849,41.46933722496033,1.982232755876665e-05
62062,124125,124124,248249,41.53588318824768,1.977021273223869e-05
62162,124325,124324,248649,41.61472797393799,1.9718235937093582e-05
62262,124525,124524,249049,41.67889213562012,1.9666396788647028e-05
62362,124725,124724,249449,41.74444603919983,1.9614694904457984e-05
62462,124925,124924,249849,41.81407904624939,1.9563129903492418e-05
62563,125127,125126,250253,41.897539138793945,1.95111878088456e-05
62663,125327,125326,250653,41.971031188964844,1.9459896795404316e-05
62763,125527,125526,251053,42.052191972732544,1.9408741525726247e-05
62863,125727,125726,251453,42.143413066864014,1.9357721624437273e-05
62963,125927,125926,251853,42.214234828948975,1.9306836717067964e-05
63063,126127,126126,252253,42.283514976501465,1.9256086430376436e-05
63163,126327,126326,252653,42.355140924453735,1.9205470392660153e-05
63263,126527,126526,253053,42.424036264419556,1.9154988233616504e-05
63363,126727,126726,253453,42.49950385093689,1.9104639584039083e-05
63463,126927,126926,253853,42.571844816207886,1.905442407592919e-05
63564,127129,127128,254257,42.65924406051636,1.900384118471068e-05
63664,127329,127328,254657,42.73374700546265,1.8953892183638294e-05
63764,127529,127528,255057,42.80725407600403,1.890407522448166e-05
63864,127729,127728,255457,42.8773980140686,1.8854389944565315e-05
63964,127929,127928,255857,42.94754910469055,1.8804835982245097e-05
64064,128129,128128,256257,43.02516007423401,1.8755412977338632e-05
64164,128329,128328,256657,43.12477898597717,1.8706120570740475e-05
64264,128529,128528,257057,43.20882201194763,1.865695840461242e-05
64364,128729,128728,257457,43.28218102455139,1.860792612203922e-05
64464,128929,128928,257857,43.35149693489075,1.855902336819472e-05
64565,129131,129130,258261,43.43532919883728,1.850976270343003e-05
64665,129331,129330,258661,43.55033206939697,1.8461119230959207e-05
64765,129531,129530,259061,43.64145112037659,1.841260422389944e-05
64865,129731,129730,259461,43.72235608100891,1.836421733186464e-05
64965,129931,129930,259861,43.79960107803345,1.8315958205267807e-05
65065,130131,130130,260261,43.8638129234314,1.8267826495468693e-05
65165,130331,130330,260661,43.93085598945618,1.8219821855713516e-05
65265,130531,130530,261061,44.007577896118164,1.8171943939394313e-05
65365,130731,130730,261461,44.07643914222717,1.8124192401890763e-05
65465,130931,130930,261861,44.15638709068298,1.807656689920891e-05
65566,131133,131132,262265,44.2262659072876,1.802859272401759e-05
65666,131333,131332,262665,44.30878806114197,1.7981219515825615e-05
65766,131533,131532,263065,44.37558102607727,1.7933971314153006e-05
65866,131733,131732,263465,44.44200921058655,1.7886847779718556e-05
65966,131933,131932,263865,44.508220911026,1.7839848574542793e-05
66066,132133,132132,264265,44.57316207885742,1.7792973360984327e-05
66166,132333,132332,264665,44.645423889160156,1.774622180305548e-05
66266,132533,132532,265065,44.71285796165466,1.7699593565845852e-05
66366,132733,132732,265465,44.77874422073364,1.765308831498967e-05
66466,132933,132932,265865,44.85220503807068,1.7606705718167207e-05
66567,133135,133134,266269,44.921720027923584,1.755998345668219e-05
66667,133335,133334,266669,45.00990700721741,1.7513846390966255e-05
66767,133535,133534,267069,45.08195114135742,1.7467830982985047e-05
66867,133735,133734,267469,45.165651082992554,1.742193690438056e-05
66967,133935,133934,267869,45.24304413795471,1.7376163827261714e-05
67067,134135,134134,268269,45.30722403526306,1.733051142500303e-05
67167,134335,134334,268669,45.37396216392517,1.7284979372039063e-05
67267,134535,134534,269069,45.43927884101868,1.7239567343650374e-05
67367,134735,134734,269469,45.51144599914551,1.7194275015922567e-05
67467,134935,134934,269869,45.58039402961731,1.714910206677827e-05
67568,135137,135136,270273,45.65519309043884,1.7103598235798575e-05
67668,135337,135336,270673,45.72137808799744,1.7058664265164614e-05
67768,135537,135536,271073,45.786109924316406,1.7013848707814715e-05
67868,135737,135736,271473,45.849003076553345,1.6969151245040448e-05
67968,135937,135936,271873,45.91118907928467,1.692457155918788e-05
68068,136137,136136,272273,45.98314094543457,1.6880109333620768e-05
68168,136337,136336,272673,46.06321406364441,1.683576425243439e-05
68268,136537,136536,273073,46.1374249458313,1.6791536000936082e-05
68368,136737,136736,273473,46.21761894226074,1.6747424265589038e-05
68468,136937,136936,273873,46.28481411933899,1.670342873304796e-05
68569,137139,137138,274277,46.350478172302246,1.665911087932783e-05
68669,137339,137338,274677,46.42668604850769,1.6615347972363444e-05
68769,137539,137538,275077,46.54464912414551,1.6571700332197553e-05
68869,137739,137738,275477,46.623708963394165,1.6528167649959238e-05
68969,137939,137938,275877,46.70111894607544,1.6484749617580144e-05
69069,138139,138138,276277,46.76961803436279,1.6441445927369382e-05
69169,138339,138338,276677,46.8310170173645,1.639825627356887e-05
69269,138539,138538,277077,46.89963912963867,1.635518035047111e-05
69369,138739,138738,277477,46.9647171497345,1.6312217853410014e-05
69469,138939,138938,277877,47.034991979599,1.6269368479208947e-05
69570,139141,139140,278281,47.09899187088013,1.6226205128021875e-05
69670,139341,139340,278681,47.15993595123291,1.618358221545783e-05
69770,139541,139540,279081,47.22236394882202,1.6141071517023545e-05
69870,139741,139740,279481,47.29422116279602,1.6098672732901098e-05
69970,139941,139940,279881,47.36868095397949,1.6056385563722527e-05
70070,140141,140140,280281,47.42943000793457,1.601420971158354e-05
70170,140341,140340,280681,47.491909980773926,1.597214487904291e-05
70270,140541,140540,281081,47.55337405204773,1.5930190769403622e-05
70370,140741,140740,281481,47.61780309677124,1.5888347086828253e-05
70470,140941,140940,281881,47.67964005470276,1.5846613537293226e-05
70571,141143,141142,282285,47.73950386047363,1.5804574142821485e-05
70671,141343,141342,282685,47.80331087112427,1.5763061071677336e-05
70771,141543,141542,283085,47.86467003822327,1.572165725098083e-05
70871,141743,141742,283485,47.92683506011963,1.568036238932342e-05
70971,141943,141942,283885,47.99285316467285,1.563917619661719e-05
71071,142143,142142,284285,48.0574312210083,1.5598098383079944e-05
71171,142343,142342,284685,48.122058153152466,1.5557128659879805e-05
71271,142543,142542,285085,48.182312965393066,1.551626673904173e-05
71371,142743,142742,285485,48.2444748878479,1.5475512333340215e-05
71471,142943,142942,285885,48.302847146987915,1.543486515664381e-05
71572,143145,143144,286289,48.36166191101074,1.5393920059972016e-05
71672,143345,143344,286689,48.421552896499634,1.535348755058224e-05
71772,143545,143544,287089,48.483402967453,1.531316141333044e-05
71872,143745,143744,287489,48.544431924819946,1.5272941365183232e-05
71972,143945,143944,287889,48.60335898399353,1.523282712384033e-05
72072,144145,144144,288289,48.66177201271057,1.5192818407997424e-05
72172,144345,144344,288689,48.721412897109985,1.5152914936847771e-05
72272,144545,144544,289089,48.7825448513031,1.5113116430789984e-05
72372,144745,144744,289489,48.84299612045288,1.5073422610793069e-05
72472,144945,144944,289889,48.904239892959595,1.5033833198687016e-05
72573,145147,145146,290293,48.96405792236328,1.4993953589126237e-05
72673,145347,145346,290693,49.02584910392761,1.4954573198261597e-05
72773,145547,145546,291093,49.08558106422424,1.4915296382650158e-05
72873,145747,145746,291493,49.143707036972046,1.4876122867020013e-05
72973,145947,145946,291893,49.2022762298584,1.4837052377335046e-05
73073,146147,146146,292293,49.26285696029663,1.4798084639996012e-05
73173,146347,146346,292693,49.32313299179077,1.4759219382225475e-05
73273,146547,146546,293093,49.387080907821655,1.4720456332134343e-05
73373,146747,146746,293493,49.462162017822266,1.4681795218396131e-05
73473,146947,146946,293893,49.531558990478516,1.464323577088099e-05
73574,147149,147148,294297,49.59518003463745,1.4604393650022224e-05
73674,147349,147348,294697,49.65400719642639,1.4566037736105774e-05
73774,147549,147548,295097,49.712162017822266,1.4527782678803756e-05
73874,147749,147748,295497,49.77154207229614,1.4489628210470056e-05
73974,147949,147948,295897,49.829899072647095,1.4451574064646674e-05
74074,148149,148148,296297,49.89012002944946,1.4413619975729352e-05
74174,148349,148348,296697,49.950109004974365,1.4375765677929323e-05
74274,148549,148548,297097,50.01958990097046,1.4338010907430697e-05
74374,148749,148748,297497,50.09098696708679,1.4300355400015598e-05
74474,148949,148948,297897,50.16384792327881,1.4262798893241198e-05
74575,149151,149150,298301,50.23714208602905,1.4224967044582713e-05
74675,149351,149350,298701,50.3080689907074,1.4187608735879116e-05
74775,149551,149550,299101,50.38009190559387,1.4150348640633926e-05
74875,149751,149750,299501,50.453068017959595,1.411318649859706e-05
74975,149951,149950,299901,50.526692152023315,1.4076122050697859e-05
75075,150151,150150,300301,50.59930920600891,1.4039155038217177e-05
75175,150351,150350,300701,50.67139005661011,1.4002285203044059e-05
75275,150551,150550,301101,50.742648124694824,1.396551228814974e-05
75375,150751,150750,301501,50.813210010528564,1.3928836037334154e-05
75475,150951,150950,301901,50.88388800621033,1.3892256194644411e-05
75576,151153,151152,302305,50.96641707420349,1.3855408152760232e-05
75676,151353,151352,302705,51.04253387451172,1.3819021319724948e-05
75776,151553,151552,303105,51.10890293121338,1.378273012937316e-05
75876,151753,151752,303505,51.17459297180176,1.37465343287313e-05
75976,151953,151952,303905,51.23417091369629,1.3710433665364345e-05
76076,152153,152152,304305,51.29582214355469,1.3674427888222097e-05
76176,152353,152352,304705,51.357146978378296,1.3638516746108737e-05
76276,152553,152552,305105,51.41727590560913,1.3602699989017592e-05
76376,152753,152752,305505,51.47824311256409,1.3566977367307783e-05
76476,152953,152952,305905,51.549875020980835,1.3531348632291498e-05
76577,153155,153154,306309,51.62541699409485,1.3495458657206668e-05
76677,153355,153354,306709,51.6894690990448,1.3460017884723614e-05
76777,153555,153554,307109,51.75234889984131,1.3424670254234672e-05
76877,153755,153754,307509,51.810774087905884,1.3389415520023877e-05
76977,153955,153954,307909,51.87255883216858,1.3354253435917976e-05
77077,154155,154154,308309,51.93256616592407,1.331918375795346e-05
77177,154355,154354,308709,51.999232053756714,1.3284206241693176e-05
77277,154555,154554,309109,52.061965227127075,1.3249320643883574e-05
77377,154755,154754,309509,52.121992111206055,1.321452672189924e-05
77477,154955,154954,309909,52.18409514427185,1.3179824233379296e-05
77578,155157,155156,310313,52.26201510429382,1.3144867284058924e-05
77678,155357,155356,310713,52.364274978637695,1.3110347847813236e-05
77778,155557,155556,311113,52.434406995773315,1.3075919120364645e-05
77878,155757,155756,311513,52.49760699272156,1.3041580862856384e-05
77978,155957,155956,311913,52.56014704704285,1.3007332836114578e-05
78078,156157,156156,312313,52.61971092224121,1.2973174802116794e-05
78178,156357,156356,312713,52.681859254837036,1.2939106523417998e-05
78278,156557,156556,313113,52.743342876434326,1.2905127763163407e-05
78378,156757,156756,313513,52.804682970047,1.2871238285231564e-05
78478,156957,156956,313913,52.872211933135986,1.2837437853971156e-05
78579,157159,157158,314317,52.945780992507935,1.2803389565780477e-05
78679,157359,157358,314717,53.015170097351074,1.2769767408582331e-05
78779,157559,157558,315117,53.07935118675232,1.2736233592828765e-05
78879,157759,157758,315517,53.14018702507019,1.2702787885569308e-05
78979,157959,157958,315917,53.2009539604187,1.266943005464994e-05
79079,158159,158158,316317,53.26300406455994,1.263615986810437e-05
79179,158359,158358,316717,53.32847499847412,1.2602977095002604e-05
79279,158559,158558,317117,53.39084506034851,1.2569881504720002e-05
79379,158759,158758,317517,53.450828075408936,1.253687286739442e-05
79479,158959,158958,317917,53.516319036483765,1.2503950953878767e-05
79580,159161,159160,318321,53.57790017127991,1.2470787617383913e-05
79680,159361,159360,318721,53.63758587837219,1.2438039327649303e-05
79780,159561,159560,319121,53.71590518951416,1.240537707547421e-05
79880,159761,159760,319521,53.788382053375244,1.237280063375178e-05
79980,159961,159960,319921,53.84899401664734,1.2340309776876111e-05
80080,160161,160160,320321,53.90836715698242,1.2307904278813797e-05
80180,160361,160360,320721,53.97010803222656,1.2275583914711291e-05
80280,160561,160560,321121,54.036465883255005,1.2243348460431628e-05
80380,160761,160760,321521,54.10026407241821,1.221119769218869e-05
80480,160961,160960,321921,54.16195511817932,1.2179131386483536e-05
80581,161163,161162,322325,54.222883224487305,1.2146829925215369e-05
80681,161363,161362,322725,54.28583908081055,1.2114932717436678e-05
80781,161563,161562,323125,54.34552812576294,1.2083119304311862e-05
80881,161763,161762,323525,54.40606498718262,1.205138946520942e-05
80981,161963,161962,323925,54.46708297729492,1.2019742980131977e-05
81081,162163,162162,324325,54.53352499008179,1.1988179629343102e-05
81181,162363,162362,324725,54.5942862033844,1.1956699193857707e-05
81281,162563,162562,325125,54.6559271812439,1.1925301455426336e-05
81381,162763,162762,325525,54.71763205528259,1.1893986196231848e-05
81481,162963,162962,325925,54.78127121925354,1.1862753198888453e-05
81582,163165,163164,326329,54.843661069869995,1.1831291150946348e-05
81682,163365,163364,326729,54.90649700164795,1.1800222845606567e-05
81782,163565,163564,327129,54.97090697288513,1.1769236151740224e-05
81882,163765,163764,327529,55.03459620475769,1.1738330854899474e-05
81982,163965,163964,327929,55.098690032958984,1.1707506740377812e-05
82082,164165,164164,328329,55.16075611114502,1.1676763594383616e-05
82182,164365,164364,328729,55.22142791748047,1.1646101204224468e-05
82282,164565,164564,329129,55.284862995147705,1.161551935693326e-05
82382,164765,164764,329529,55.34860706329346,1.1585017840624047e-05
82482,164965,164964,329929,55.410505056381226,1.1554596443897515e-05
82583,165167,165166,330333,55.477620124816895,1.1523951943227812e-05
82683,165367,165366,330733,55.539631843566895,1.1493690949118079e-05
82783,165567,165566,331133,55.60016894340515,1.1463509441390283e-05
82883,165767,165766,331533,55.66121697425842,1.1433407210656454e-05
82983,165967,165966,331933,55.733959913253784,1.1403384048218123e-05
83083,166167,166166,332333,55.81354594230652,1.1373439746596062e-05
83183,166367,166366,332733,55.90067195892334,1.1343574097645675e-05
83283,166567,166566,333133,55.971961975097656,1.131378689441373e-05
83383,166767,166766,333533,56.06272220611572,1.1284077930830338e-05
83483,166967,166966,333933,56.13110399246216,1.1254447000641382e-05
83584,167169,167168,334337,56.2074408531189,1.1224598760195044e-05
83684,167369,167368,334737,56.27086400985718,1.11951240568669e-05
83784,167569,167568,335137,56.33277606964111,1.1165726770648461e-05
83884,167769,167768,335537,56.398136138916016,1.1136406698171625e-05
83984,167969,167968,335937,56.46111798286438,1.1107163635669422e-05
84084,168169,168168,336337,56.52499008178711,1.1077997381037363e-05
84184,168369,168368,336737,56.592005014419556,1.1048907731975638e-05
84284,168569,168568,337137,56.6559739112854,1.1019894487093157e-05
84384,168769,168768,337537,56.71983313560486,1.0990957445159922e-05
84484,168969,168968,337937,56.782668113708496,1.0962096405986309e-05
84585,169171,169170,338341,56.85440015792847,1.0933023699233323e-05
84685,169371,169370,338741,56.918915033340454,1.0904314820877476e-05
84785,169571,169570,339141,56.98477816581726,1.0875681345230212e-05
84885,169771,169770,339541,57.054137229919434,1.0847123073347615e-05
84985,169971,169970,339941,57.12385416030884,1.0818639808014849e-05
85085,170171,170170,340341,57.223886251449585,1.0790231351637085e-05
85185,170371,170370,340741,57.34209203720093,1.0761897507666352e-05
85285,170571,170570,341141,57.41559982299805,1.0733638079534253e-05
85385,170771,170770,341541,57.48238706588745,1.0705452871767683e-05
85485,170971,170970,341941,57.55517601966858,1.067734168925997e-05
85586,171173,171172,342345,57.6290819644928,1.064902433568676e-05
85686,171373,171372,342745,57.70120406150818,1.0621061355043744e-05
85786,171573,171572,343145,57.76696705818176,1.059317181518744e-05
85886,171773,171772,343545,57.834681034088135,1.0565355523073603e-05
85986,171973,171972,343945,57.9016489982605,1.0537612285765303e-05
86086,172173,172172,344345,57.98109221458435,1.0509941911292575e-05
86186,172373,172372,344745,58.06200194358826,1.0482344208128958e-05
86286,172573,172572,345145,58.12554097175598,1.0454818985153182e-05
86386,172773,172772,345545,58.19473910331726,1.0427366051932911e-05
86486,172973,172972,345945,58.25661110877991,1.0399985217957848e-05
86587,173175,173174,346349,58.321529150009155,1.0372403567356618e-05
86687,173375,173374,346749,58.383257150650024,1.0345167080779708e-05
86787,173575,173574,347149,58.453930139541626,1.0318002124323727e-05
86887,173775,173774,347549,58.52028799057007,1.0290908510408078e-05
86987,173975,173974,347949,58.58262896537781,1.0263886051489661e-05
87087,174175,174174,348349,58.654279947280884,1.023693456009163e-05
87187,174375,174374,348749,58.74740719795227,1.0210053849828041e-05
87287,174575,174574,349149,58.82279706001282,1.0183243734818245e-05
87387,174775,174774,349549,58.886335134506226,1.0156504029432973e-05
87487,174975,174974,349949,58.95944809913635,1.0129834548314839e-05
87588,175177,175176,350353,59.03487801551819,1.0102969465708931e-05
87688,175377,175376,350753,59.10231614112854,1.0076440577754233e-05
87788,175577,175576,351153,59.17583394050598,1.0049981359889729e-05
87888,175777,175776,351553,59.27949905395508,1.0023591629317674e-05
87988,175977,175976,351953,59.38219404220581,9.997271203206732e-06
88088,176177,176176,352353,59.46260905265808,9.971019899275373e-06
88188,176377,176376,352753,59.52503991127014,9.944837536108938e-06
88288,176577,176576,353153,59.58541393280029,9.918723932113912e-06
88388,176777,176776,353553,59.66006088256836,9.892678906949668e-06
88488,176977,176976,353953,59.72267198562622,9.86670228002259e-06
88589,177179,177178,354357,59.80564522743225,9.840535131651284e-06
88689,177379,177378,354757,59.895848989486694,9.814695442258035e-06
88789,177579,177578,355157,59.965404987335205,9.788923611639064e-06
88889,177779,177778,355557,60.02500295639038,9.763219461283837e-06
88989,177979,177978,355957,60.09770917892456,9.737582813622028e-06
89089,178179,178178,356357,60.169198989868164,9.71201349078275e-06
89189,178379,178378,356757,60.22980213165283,9.686511316281724e-06
89289,178579,178578,357157,60.28949785232544,9.661076113395552e-06
89389,178779,178778,357557,60.346922159194946,9.635707706140528e-06
89489,178979,178978,357957,60.40296912193298,9.610405919055778e-06
89590,179181,179180,358361,60.463566064834595,9.584918558584647e-06
89690,179381,179380,358761,60.52304410934448,9.559750148907463e-06
89790,179581,179580,359161,60.58046913146973,9.534647833836196e-06
89890,179781,179780,359561,60.64058709144592,9.509611439370758e-06
89990,179981,179980,359961,60.69972801208496,9.484640792811653e-06
90090,180181,180180,360361,60.7566180229187,9.459735720964691e-06
90190,180381,180380,360761,60.81454014778137,9.434896051772496e-06
90290,180581,180580,361161,60.871915102005005,9.41012161331594e-06
90390,180781,180780,361561,60.92906904220581,9.385412234062858e-06
90490,180981,180980,361961,60.991580963134766,9.360767743141195e-06
90591,181183,181182,362365,61.05205798149109,9.335942498442284e-06
90691,181383,181382,362765,61.10981798171997,9.311427917734878e-06
90791,181583,181582,363165,61.173251152038574,9.286977713627531e-06
90891,181783,181782,363565,61.23197293281555,9.262591716663786e-06
90991,181983,181982,363965,61.291651248931885,9.238269758334862e-06
91091,182183,182182,364365,61.34740400314331,9.214011670239104e-06
91191,182383,182382,364765,61.40494108200073,9.189817284931266e-06
91291,182583,182582,365165,61.46318221092224,9.165686434584442e-06
91391,182783,182782,365565,61.51978397369385,9.141618952547733e-06
91491,182983,182982,365965,61.57594299316406,9.117614672312289e-06
91592,183185,183184,366369,61.63368511199951,9.093434332876992e-06
91692,183385,183384,366769,61.69197392463684,9.069556586098724e-06
91792,183585,183584,367169,61.749796867370605,9.045741542650036e-06
91892,183785,183784,367569,61.80956697463989,9.021989037697424e-06
91992,183985,183984,367969,61.867374897003174,8.998298906767125e-06
92092,184185,184184,368369,61.92514705657959,8.974670986220466e-06
92192,184385,184384,368769,61.98847484588623,8.951105112489225e-06
92292,184585,184584,369169,62.04955816268921,8.927601122714584e-06
92392,184785,184784,369569,62.1106071472168,8.904158854121014e-06
92492,184985,184984,369969,62.172420263290405,8.880778144547698e-06
92593,185187,185186,370373,62.249412059783936,8.857225948945374e-06
92693,185387,185386,370773,62.32385206222534,8.833968484521094e-06
92793,185587,185586,371173,62.38503408432007,8.810772093657265e-06
92893,185787,185786,371573,62.44967818260193,8.787636616030929e-06
92993,185987,185986,371973,62.51503801345825,8.76456189144025e-06
93093,186187,186186,372373,62.57600688934326,8.74154776047529e-06
93193,186387,186386,372773,62.63807392120361,8.718594063931502e-06
93293,186587,186586,373173,62.70024085044861,8.69570064296409e-06
93393,186787,186786,373573,62.75999402999878,8.672867339118376e-06
93493,186987,186986,373973,62.82198190689087,8.650093994644548e-06
93594,187189,187188,374377,62.88219404220581,8.627153618231377e-06
93694,187389,187388,374777,62.94294619560242,8.604500315880699e-06
93794,187589,187588,375177,63.007352113723755,8.581906500167287e-06
93894,187789,187788,375577,63.068793058395386,8.559372014568675e-06
93994,187989,187988,375977,63.129430055618286,8.536896703382973e-06
94094,188189,188188,376377,63.192564964294434,8.51448041113686e-06
94194,188389,188388,376777,63.253337144851685,8.492122982742851e-06
94294,188589,188588,377177,63.3152379989624,8.469824263595075e-06
94394,188789,188788,377577,63.3754780292511,8.447584099478365e-06
94494,188989,188988,377977,63.43884015083313,8.425402336658989e-06
94595,189191,189190,378381,63.50341987609863,8.403057880107026e-06
94695,189391,189390,378781,63.567315101623535,8.380993040051644e-06
94795,189591,189590,379181,63.629010915756226,8.358986140706932e-06
94895,189791,189790,379581,63.68923592567444,8.337037029693978e-06
94995,189991,189990,379981,63.75510501861572,8.315145555526873e-06
95095,190191,190190,380381,63.816511154174805,8.293311566688538e-06
95195,190391,190390,380781,63.87701416015625,8.271534912131095e-06
95295,190591,190590,381181,63.93740105628967,8.249815441257319e-06
95395,190791,190790,381581,64.00578308105469,8.228153003993022e-06
95495,190991,190990,381981,64.07020401954651,8.20654745034469e-06
95596,191193,191192,382385,64.1295530796051,8.18478342861278e-06
95696,191393,191392,382785,64.20947313308716,8.163291759574838e-06
95796,191593,191592,383185,64.30380201339722,8.141856525790952e-06
95896,191793,191792,383585,64.38137602806091,8.120477578772226e-06
95996,191993,191992,383985,64.45665216445923,8.099154771029846e-06
96096,192193,192192,384385,64.52126121520996,8.077887954753892e-06
96196,192393,192392,384785,64.58236289024353,8.056676983023173e-06
96296,192593,192592,385185,64.64344310760498,8.035521709281445e-06
96396,192793,192792,385585,64.70583295822144,8.01442198711689e-06
96496,192993,192992,385985,64.77690815925598,7.993377670530982e-06
96597,193195,193194,386389,64.87492203712463,7.972179002151493e-06
96697,193395,193394,386789,64.9681601524353,7.951245611324585e-06
96797,193595,193594,387189,65.0380539894104,7.930367189221866e-06
96897,193795,193794,387589,65.10066103935242,7.909543591465406e-06
96997,193995,193994,387989,65.16144490242004,7.888774674113965e-06
97097,194195,194194,388389,65.22143006324768,7.868060293792467e-06
97197,194395,194394,388789,65.28319811820984,7.847400306949162e-06
97297,194595,194594,389189,65.34560585021973,7.82679457074163e-06
97397,194795,194794,389589,65.43794202804565,7.806242942921378e-06
97497,194995,194994,389989,65.53986597061157,7.785745281091523e-06
97598,195197,195196,390393,65.61782884597778,7.765097276632814e-06
97698,195397,195396,390793,65.68192100524902,7.744707658473797e-06
97798,195597,195596,391193,65.74933505058289,7.724371580820378e-06
97898,195797,195796,391593,65.81123518943787,7.704088903287185e-06
97998,195997,195996,391993,65.87289309501648,7.683859485397779e-06
98098,196197,196196,392393,65.93844103813171,7.66368318755156e-06
98198,196397,196396,392793,66.00352120399475,7.643559869844438e-06
98298,196597,196596,393193,66.06980109214783,7.623489393519238e-06
98398,196797,196796,393593,66.16812109947205,7.603471619576296e-06
98498,196997,196996,393993,66.2714250087738,7.583506409682425e-06
98599,197199,197198,394397,66.34382605552673,7.563394762203865e-06
98699,197399,197398,394797,66.40471720695496,7.543534788658607e-06
98799,197599,197598,395197,66.47266888618469,7.5237269649544795e-06
98899,197799,197798,395597,66.54924607276917,7.5039711537993115e-06
98999,197999,197998,395997,66.6159610748291,7.484267218548834e-06
99099,198199,198198,396397,66.71374607086182,7.464615023158375e-06
99199,198399,198398,396797,66.81213283538818,7.445014431702537e-06
99299,198599,198598,397197,66.90341520309448,7.425465308523278e-06
99399,198799,198798,397597,66.97349214553833,7.405967518857829e-06
99499,198999,198998,397997,67.04444599151611,7.386520927231448e-06
99600,199201,199200,398401,67.10474300384521,7.366931701973265e-06
99700,199401,199400,398801,67.16728806495667,7.3475876126997645e-06
99800,199601,199600,399201,67.23281407356262,7.3282943183382445e-06
99900,199801,199800,399601,67.32581615447998,7.309051685286365e-06
100000,200001,200000,400001,67.43154215812683,7.289859580783329e-06


==> extragradient/plot_data/bilinear_matrix_game_n250/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0008831024169921875,2.0175302852282635
200,201,200,401,0.12049603462219238,0.04478652689802895
400,401,400,801,0.20284509658813477,0.01876849959713967
601,602,601,1203,0.2959010601043701,0.010727747668166946
801,802,801,1603,0.4237070083618164,0.006834670046924187
1001,1002,1001,2003,0.5958869457244873,0.0046996607619437004
1201,1202,1201,2403,0.750946044921875,0.003564882185873673
1401,1402,1401,2803,0.876762866973877,0.0027081890851968246
1602,1603,1602,3205,0.9743978977203369,0.001855631651017109
1802,1803,1802,3605,1.0715441703796387,0.0014061223319154967
2002,2003,2002,4005,1.1632349491119385,0.0010943812851285626
2202,2203,2202,4405,1.2528870105743408,0.0009419078130188925
2402,2403,2402,4805,1.3943300247192383,0.0008516517817800815
2603,2604,2603,5207,1.5030009746551514,0.0007836220906947915
2803,2804,2803,5607,1.5856258869171143,0.0007337162996024967
3003,3004,3003,6007,1.6683039665222168,0.0006843837934935394
3203,3204,3203,6407,1.7451019287109375,0.000621430620659287
3403,3404,3403,6807,1.8288710117340088,0.0005738291089869442
3604,3605,3604,7209,1.9163148403167725,0.0005386157069433298
3804,3805,3804,7609,1.9980790615081787,0.0005102432591415502
4004,4005,4004,8009,2.08270001411438,0.0004859931252849459
4204,4205,4204,8409,2.16211199760437,0.0004647943297305488
4404,4405,4404,8809,2.245716094970703,0.0004460128472459026
4605,4606,4605,9211,2.378455877304077,0.0004291432956780943
4805,4806,4805,9611,2.500087022781372,0.00041404377633446406
5005,5006,5005,10011,2.6060659885406494,0.0004003897550704579
5205,5206,5205,10411,2.692835807800293,0.00038799322043170777
5405,5406,5405,10811,2.7805190086364746,0.0003766997750865513
5606,5607,5606,11213,2.877800941467285,0.0003663304164950251
5806,5807,5806,11613,2.9619860649108887,0.00035687721271075555
6006,6007,6006,12013,3.075845956802368,0.0003481906656339682
6206,6207,6206,12413,3.183511972427368,0.00034018745892135376
6406,6407,6406,12813,3.3075931072235107,0.0003327945029156792
6607,6608,6607,13215,3.4310169219970703,0.000325914425714135
6807,6808,6807,13615,3.5302951335906982,0.00031955852168277804
7007,7008,7007,14015,3.611382007598877,0.00031364081882276855
7207,7208,7207,14415,3.6889679431915283,0.0003081165565063809
7407,7408,7407,14815,3.7686169147491455,0.00030294595791825675
7608,7609,7608,15217,3.8599209785461426,0.0002980701275253528
7808,7809,7808,15617,4.004011154174805,0.0002935059691853229
8008,8009,8008,16017,4.111639976501465,0.0002892004304440692
8208,8209,8208,16417,4.216598987579346,0.0002851285393824211
8408,8409,8408,16817,4.307560920715332,0.00028126803576462617
8609,8610,8609,17219,4.39081883430481,0.00027758117322436584
8809,8810,8809,17619,4.529435873031616,0.00027408685490339953
9009,9010,9009,18019,4.703139781951904,0.0002707504714707638
9209,9210,9209,18419,4.801892995834351,0.0002675579071072609
9409,9410,9409,18819,4.908695936203003,0.0002644965460433607
9610,9611,9610,19221,5.035598993301392,0.00026154068254627383
9810,9811,9810,19621,5.14483904838562,0.0002587095917783479
10010,10011,10010,20021,5.2472779750823975,0.0002559792390777811
10210,10211,10210,20421,5.417272090911865,0.00025334152331706045
10410,10411,10410,20821,5.535682201385498,0.00025078917689414995
10611,10612,10611,21223,5.65929388999939,0.00024830349446085443
10811,10812,10811,21623,5.764245986938477,0.000245903320786389
11011,11012,11011,22023,5.841943025588989,0.00024357082283191648
11211,11212,11211,22423,5.921584844589233,0.0002413012497644246
11411,11412,11411,22823,6.005275011062622,0.0002390903176070361
11612,11613,11612,23225,6.084932804107666,0.00023692350957163374
11812,11813,11812,23625,6.163479804992676,0.000234818876188913
12012,12013,12012,24025,6.274410009384155,0.00023276234079066868
12212,12213,12212,24425,6.4124720096588135,0.00023075103695135703
12412,12413,12412,24825,6.522176027297974,0.0002287823631151437
12613,12614,12613,25227,6.597858190536499,0.0002268444101240626
12813,12814,12813,25627,6.675458192825317,0.0002249543001830085
13013,13014,13013,26027,6.750562906265259,0.00022310033153375412
13213,13214,13213,26427,6.829948902130127,0.00022128071310333408
13413,13414,13413,26827,6.919861078262329,0.00021949380670303125
13614,13615,13614,27229,7.059284925460815,0.00021772940904341104
13814,13815,13814,27629,7.1755030155181885,0.00021600369343878668
14014,14015,14014,28029,7.25197696685791,0.00021430653915116896
14214,14215,14214,28429,7.325778007507324,0.00021263678034784885
14414,14415,14414,28829,7.399510145187378,0.0002109933413399964
14615,14616,14615,29231,7.494488954544067,0.00020936719927568728
14815,14816,14815,29631,7.605759143829346,0.0002077736101569283
15015,15016,15015,30031,7.699090003967285,0.00020620356714784883
15215,15216,15215,30431,7.777405023574829,0.00020465627632769098
15415,15416,15415,30831,7.859264135360718,0.000203130998293746
15616,15617,15616,31233,7.940685987472534,0.00020161957581777
15816,15817,15816,31633,8.017739057540894,0.0002001364003753276
16016,16017,16016,32033,8.092456102371216,0.00019867329583096713
16216,16217,16216,32433,8.171181917190552,0.00019722969554983585
16416,16417,16416,32833,8.246679782867432,0.00019580506686676602
16617,16618,16617,33235,8.324879884719849,0.00019439192294999017
16817,16818,16817,33635,8.399815082550049,0.00019300384976726458
17017,17018,17017,34035,8.475190162658691,0.00019163332384738367
17217,17218,17217,34435,8.548149108886719,0.00019027992188536436
17417,17418,17417,34835,8.625688791275024,0.00018894324247093898
17618,17619,17618,35237,8.706074953079224,0.00018761634308815523
17818,17819,17818,35637,8.780152797698975,0.00018631206254184643
18018,18019,18018,36037,8.854882001876831,0.00018502341330576148
18218,18219,18218,36437,8.931019067764282,0.00018375006570833902
18418,18419,18418,36837,9.01211404800415,0.0001824917047254518
18619,18620,18619,37239,9.085239171981812,0.00018124184694090495
18819,18820,18819,37639,9.161256074905396,0.00018001263874275233
19019,19020,19019,38039,9.255383968353271,0.00017879754841943784
19219,19220,19219,38439,9.339904069900513,0.00017759630984320028
19419,19420,19419,38839,9.418071031570435,0.0001764086670745427
19620,19621,19620,39241,9.497464895248413,0.000175228535364549
19820,19821,19820,39641,9.573375940322876,0.00017406741883776853
20020,20021,20020,40041,9.648216962814331,0.00017291918390125387
20220,20221,20220,40441,9.722985982894897,0.00017178360927004832
20420,20421,20420,40841,9.802890062332153,0.00017066048102396057
20621,20622,20621,41243,9.882990837097168,0.00016954406814495123
20821,20822,20821,41643,9.968230962753296,0.00016844527794923606
21021,21022,21021,42043,10.049038887023926,0.0001673583314685384
21221,21222,21221,42443,10.12700605392456,0.0001662830402869128
21421,21422,21421,42843,10.208755016326904,0.00016521922150953457
21622,21623,21622,43245,10.288034915924072,0.0001641614629402783
21822,21823,21822,43645,10.36751389503479,0.00016312011613611507
22022,22023,22022,44045,10.44872498512268,0.0001620897225734824
22222,22223,22222,44445,10.536749839782715,0.0001610701187869821
22422,22423,22422,44845,10.643959999084473,0.00016006114558607382
22623,22624,22623,45247,10.781828880310059,0.000159057681431108
22823,22824,22823,45647,10.911773920059204,0.00015806955919467862
23023,23024,23023,46047,11.035829067230225,0.00015709161296936859
23223,23224,23223,46447,11.120351076126099,0.00015612369882119328
23423,23424,23423,46847,11.200459003448486,0.00015516567621955306
23624,23625,23624,47249,11.281244039535522,0.00015421269083493608
23824,23825,23824,47649,11.383264064788818,0.00015327409041627737
24024,24025,24024,48049,11.531846046447754,0.00015234497834770155
24224,24225,24224,48449,11.663513898849487,0.00015142522639086814
24424,24425,24424,48849,11.76941180229187,0.00015051470908089608
24625,24626,24625,49251,11.883808135986328,0.00014960881928547922
24825,24826,24825,49651,11.997035026550293,0.0001487164501126954
25025,25026,25025,50051,12.10321307182312,0.00014783295423499924
25225,25226,25225,50451,12.23271894454956,0.00014695821630477903
25425,25426,25425,50851,12.340255975723267,0.00014609212327915575
25626,25627,25626,51253,12.47423005104065,0.00014523029780489532
25826,25827,25826,51653,12.601628065109253,0.000144381206144761
26026,26027,26026,52053,12.728004932403564,0.0001435404327899102
26226,26227,26226,52453,12.882900953292847,0.00014270787317310877
26426,26427,26426,52853,13.02777099609375,0.00014188342467383932
26627,26628,26627,53255,13.160400867462158,0.00014106292432481763
26827,26828,26827,53655,13.296576976776123,0.00014025443699057426
27027,27028,27027,54055,13.437337875366211,0.0001394537635074081
27227,27228,27227,54455,13.55974793434143,0.00013866080846049175
27427,27428,27427,54855,13.649142980575562,0.00013787547810154065
27628,27629,27628,55257,13.728205919265747,0.00013709381008254016
27828,27829,27828,55657,13.807626962661743,0.00013632349125976612
28028,28029,28028,56057,13.890321016311646,0.000135560524954989
28228,28229,28228,56457,13.9719979763031,0.00013480482362331078
28428,28429,28428,56857,14.054435968399048,0.00013405630116166174
28629,28630,28629,57259,14.142336130142212,0.0001333111834121381
28829,28830,28829,57659,14.246279954910278,0.00013257680080252073
29029,29030,29029,58059,14.329503059387207,0.00013184934661522748
29229,29230,29229,58459,14.40976595878601,0.00013112874014536353
29429,29430,29429,58859,14.491132974624634,0.00013041490194906852
29630,29631,29630,59261,14.573677062988281,0.00012970423474908816
29830,29831,29830,59661,14.65652585029602,0.00012900373252629438
30030,30031,30030,60061,14.736051082611084,0.00012830976712002569
30230,30231,30230,60461,14.820665836334229,0.0001276222638275209
30430,30431,30430,60861,14.94722318649292,0.00012694114905889648
30631,30632,30631,61263,15.037583827972412,0.0001262629920642769
30831,30832,30831,61663,15.115169048309326,0.00012559446893549512
31031,31032,31031,62063,15.189738035202026,0.00012493211962466455
31231,31232,31231,62463,15.269076108932495,0.0001242758747413995
31431,31432,31431,62863,15.352334976196289,0.00012362566588363646
31632,31633,31632,63265,15.43562388420105,0.00012297821930005854
31832,31833,31832,63665,15.508949995040894,0.00012233991048153504
32032,32033,32032,64065,15.584118127822876,0.00012170743787703473
32232,32233,32232,64465,15.673862934112549,0.00012108073683266719
32432,32433,32432,64865,15.760732889175415,0.00012045974358089348
32633,32634,32633,65267,15.837193965911865,0.00011984133255828426
32833,32834,32833,65667,15.947982788085938,0.00011923159480041812
33033,33034,33033,66067,16.086374044418335,0.0001186273783612972
33233,33234,33233,66467,16.216865062713623,0.00011802862284136297
33433,33434,33433,66867,16.30769109725952,0.00011743526863959277
33634,33635,33634,67269,16.38527202606201,0.00011684433020463652
33834,33835,33834,67669,16.457973957061768,0.00011626162923078444
34034,34035,34034,68069,16.535773038864136,0.0001156841551247771
34234,34235,34234,68469,16.628818035125732,0.00011511185133113707
34434,34435,34434,68869,16.72135901451111,0.00011454466201889047
34635,34636,34635,69271,16.80422306060791,0.00011397973403805185
34835,34836,34835,69671,16.889918088912964,0.00011342263391541219
35035,35036,35035,70071,16.9703209400177,0.0001128704847270032
35235,35236,35235,70471,17.05233907699585,0.00011232323341223033
35435,35436,35435,70871,17.128280878067017,0.00011178082757014295
35636,35637,35636,71273,17.21573519706726,0.0001112405393460803
35836,35837,35836,71673,17.3018000125885,0.00011070769341683268
36036,36037,36036,72073,17.381528854370117,0.00011017953935532546
36236,36237,36236,72473,17.4526150226593,0.00010965602729298843
36436,36437,36436,72873,17.52601718902588,0.0001091371079663427
36637,36638,36637,73275,17.598998069763184,0.00010862017216672441
36837,36838,36837,73675,17.674810886383057,0.00010811031525171424
37037,37038,37037,74075,17.751288175582886,0.00010760490657805096
37237,37238,37237,74475,17.84167981147766,0.0001071038992072625
37437,37438,37437,74875,17.920642137527466,0.00010660724675889057
37638,37639,37638,75277,17.997591972351074,0.00010611245243394272
37838,37839,37838,75677,18.082210779190063,0.00010562439407843234
38038,38039,38038,76077,18.179426908493042,0.00010514055453646331
38238,38239,38238,76477,18.318520069122314,0.00010466088957114157
38438,38439,38438,76877,18.444578170776367,0.00010418535546241655
38639,38640,38639,77279,18.544833183288574,0.00010371156196181448
38839,38840,38839,77679,18.635758876800537,0.00010324418054166516
39039,39040,39039,78079,18.77023482322693,0.0001027808016175643
39239,39240,39239,78479,18.931095123291016,0.00010232138345445304
39439,39440,39439,78879,19.039772987365723,0.00010186588479476518
39640,39641,39640,79281,19.141204118728638,0.00010141201642939574
39840,39841,39840,79681,19.23035192489624,0.00010096425397197347
40040,40041,40040,80081,19.32494282722473,0.00010052028984418028
40240,40241,40240,80481,19.42292594909668,0.00010008008463429918
40440,40441,40440,80881,19.532476902008057,9.964359937337433e-05
40641,40642,40641,81283,19.62502098083496,9.920864069779614e-05
40841,40842,40841,81683,19.717000007629395,9.877949829929947e-05
41041,41042,41041,82083,19.809156894683838,9.835396136279923e-05
41241,41242,41241,82483,19.903674840927124,9.793199263978274e-05
41441,41442,41441,82883,20.00769805908203,9.751355529516753e-05
41642,41643,41642,83285,20.098005056381226,9.709654691218016e-05
41842,41843,41842,83685,20.181541919708252,9.668508065671065e-05
42042,42043,42042,84085,20.263671159744263,9.62770375316916e-05
42242,42243,42242,84485,20.343008041381836,9.587238230831156e-05
42442,42443,42442,84885,20.420871019363403,9.547108014633218e-05
42643,42644,42643,85287,20.507550954818726,9.507111494994549e-05
42843,42844,42843,85687,20.58618402481079,9.46764322514415e-05
43043,43044,43043,86087,20.666361808776855,9.428500020119824e-05
43243,43244,43243,86487,20.747601985931396,9.389678546250573e-05
43443,43444,43443,86887,20.82712411880493,9.351175506177486e-05
43644,43645,43644,87289,20.906795978546143,9.312797485581297e-05
43844,43845,43844,87689,20.99163508415222,9.274923115939283e-05
44044,44045,44044,88089,21.075260877609253,9.237357485832367e-05
44244,44245,44244,88489,21.155706882476807,9.200097439029355e-05
44444,44445,44444,88889,21.239439964294434,9.163139853442863e-05
44645,44646,44645,89291,21.327847003936768,9.126299096701417e-05
44845,44846,44845,89691,21.409576892852783,9.089938675815504e-05
45045,45046,45045,90091,21.49201798439026,9.053871535572686e-05
45245,45246,45245,90491,21.570523023605347,9.018094686580128e-05
45445,45446,45445,90891,21.64850115776062,8.982605171536e-05
45646,45647,45646,91293,21.72933316230774,8.947224748965964e-05
45846,45847,45846,91693,21.810827016830444,8.912302556724162e-05
46046,46047,46046,92093,21.890777826309204,8.877659001126892e-05
46246,46247,46246,92493,21.97556781768799,8.843291249752094e-05
46446,46447,46446,92893,22.06977391242981,8.809196500370597e-05
46647,46648,46647,93295,22.163414001464844,8.775203532486355e-05
46847,46848,46847,93695,22.249400854110718,8.741647830476478e-05
47047,47048,47047,94095,22.331507921218872,8.708356888522966e-05
47247,47248,47247,94495,22.41346788406372,8.67532802213865e-05
47447,47448,47447,94895,22.494573831558228,8.642558575382821e-05
47648,47649,47648,95297,22.57612180709839,8.609883998114885e-05
47848,47849,47848,95697,22.658337116241455,8.577626799914256e-05
48048,48049,48048,96097,22.739909887313843,8.545621208802587e-05
48248,48249,48248,96497,22.822602033615112,8.513864679971089e-05
48448,48449,48448,96897,22.902847051620483,8.482354695528796e-05
48649,48650,48649,97299,22.98941707611084,8.450933043627853e-05
48849,48850,48849,97699,23.069077014923096,8.419909902464256e-05
49049,49050,49049,98099,23.149054050445557,8.389125898630491e-05
49249,49250,49249,98499,23.228686809539795,8.358578619249559e-05
49449,49450,49449,98899,23.312968015670776,8.328265676829103e-05
49650,49651,49650,99301,23.395845890045166,8.298034883202131e-05
49850,49851,49850,99701,23.480364084243774,8.26818469527207e-05
50050,50051,50050,100101,23.560869932174683,8.238561820525842e-05
50250,50251,50250,100501,23.643989086151123,8.209163970748663e-05
50450,50451,50450,100901,23.723180055618286,8.179988881806894e-05
50651,50652,50651,101303,23.800158977508545,8.150890090921825e-05
50851,50852,50851,101703,23.89248275756836,8.122154912387039e-05
51051,51052,51051,102103,23.986531972885132,8.093635833399582e-05
51251,51252,51251,102503,24.07516598701477,8.065330683722813e-05
51451,51452,51451,102903,24.162660837173462,8.037237315940119e-05
51652,51653,51652,103305,24.267250061035156,8.009214709870085e-05
51852,51853,51852,103705,24.351770877838135,7.98153958614352e-05
52052,52053,52052,104105,24.435747861862183,7.954069926096685e-05
52252,52253,52252,104505,24.52430009841919,7.92680367120229e-05
52452,52453,52452,104905,24.603420972824097,7.899738784538442e-05
52653,52654,52653,105307,24.6835720539093,7.872739420379245e-05
52853,52854,52853,105707,24.76341676712036,7.846072226447492e-05
53053,53054,53053,106107,24.846208095550537,7.819600407440881e-05
53253,53254,53253,106507,24.92695188522339,7.793322010616023e-05
53453,53454,53453,106907,25.012013912200928,7.767235103745557e-05
53654,53655,53654,107309,25.093711853027344,7.741208761281565e-05
53854,53855,53854,107709,25.173446893692017,7.715500052003898e-05
54054,54055,54054,108109,25.254040956497192,7.689977147197986e-05
54254,54255,54254,108509,25.334940910339355,7.664638194434872e-05
54454,54455,54454,108909,25.41624093055725,7.639481360610304e-05
54655,54656,54655,109311,25.503758907318115,7.61438039924113e-05
54855,54856,54855,109711,25.582852840423584,7.589583268786947e-05
55055,55056,55055,110111,25.663201093673706,7.564962863625688e-05
55255,55256,55255,110511,25.74322009086609,7.540517426344573e-05
55455,55456,55455,110911,25.821986198425293,7.516245217910972e-05
55656,55657,55656,111313,25.902826070785522,7.492024442034343e-05
55856,55857,55856,111713,25.99095392227173,7.468094391609287e-05
56056,56057,56056,112113,26.071812868118286,7.444332453028067e-05
56256,56257,56256,112513,26.152323961257935,7.42073695898061e-05
56456,56457,56456,112913,26.233736038208008,7.397306259647093e-05
56657,56658,56657,113315,26.324461221694946,7.373922791978346e-05
56857,56858,56857,113715,26.418071031570435,7.350817605088851e-05
57057,57058,57057,114115,26.498764038085938,7.327872358259517e-05
57257,57258,57257,114515,26.577029943466187,7.305085469714894e-05
57457,57458,57457,114915,26.65278697013855,7.282455374198466e-05
57658,57659,57658,115317,26.73037815093994,7.25986853602794e-05
57858,57859,57858,115717,26.807143926620483,7.237548160855203e-05
58058,58059,58058,116117,26.884843111038208,7.215379972950237e-05
58258,58259,58258,116517,26.963917016983032,7.193362471635184e-05
58458,58459,58458,116917,27.04108190536499,7.171494171926677e-05
58659,58660,58659,117319,27.11909008026123,7.149665370228072e-05
58859,58860,58859,117719,27.1958270072937,7.12809180841927e-05
59059,59060,59059,118119,27.271045923233032,7.106663078614305e-05
59259,59260,59259,118519,27.35154414176941,7.085377757066214e-05
59459,59460,59459,118919,27.43084192276001,7.064234434913386e-05
59660,59661,59660,119321,27.50988507270813,7.04312705540779e-05
59860,59861,59860,119721,27.586936950683594,7.022264257005662e-05
60060,60061,60060,120121,27.664318084716797,7.001539312474726e-05
60260,60261,60260,120521,27.740385055541992,6.980950871115826e-05
60460,60461,60460,120921,27.82063388824463,6.960497596325298e-05
60661,60662,60661,121323,27.899882078170776,6.940076902442114e-05
60861,60862,60861,121723,27.9793758392334,6.91989066624089e-05
61061,61062,61061,122123,28.055932998657227,6.899835663758004e-05
61261,61262,61261,122523,28.13402509689331,6.879910613550458e-05
61461,61462,61461,122923,28.209588050842285,6.860114247641028e-05
61662,61663,61662,123325,28.289003133773804,6.840347284622901e-05
61862,61863,61862,123725,28.368034839630127,6.820805164001644e-05
62062,62063,62062,124125,28.454330921173096,6.801387996602056e-05
62262,62263,62262,124525,28.54748797416687,6.782094566770763e-05
62462,62463,62462,124925,28.624649047851562,6.762923671586997e-05
62663,62664,62663,125327,28.703840970993042,6.743779175831863e-05
62863,62864,62863,125727,28.781768083572388,6.72485038930965e-05
63063,63064,63063,126127,28.856557846069336,6.706040597897114e-05
63263,63264,63263,126527,28.932852029800415,6.687348648372273e-05
63463,63464,63463,126927,29.01355504989624,6.668773399591672e-05
63664,63665,63664,127329,29.091745138168335,6.650221712455504e-05
63864,63865,63864,127729,29.168794870376587,6.631877058890159e-05
64064,64065,64064,128129,29.24690318107605,6.61364574834492e-05
64264,64265,64264,128529,29.324352025985718,6.59552668681437e-05
64464,64465,64464,128929,29.40546488761902,6.577518791799872e-05
64665,64666,64665,129331,29.486733198165894,6.559531777946051e-05
64865,64866,64865,129731,29.565805912017822,6.54174355616983e-05
65065,65066,65065,130131,29.645183086395264,6.524063315732268e-05
65265,65266,65265,130531,29.72502899169922,6.506490018873243e-05
65465,65466,65465,130931,29.79925799369812,6.489022638686707e-05
65666,65667,65666,131333,29.877559185028076,6.471573608532318e-05
65866,65867,65866,131733,29.954976081848145,6.454315541007359e-05
66066,66067,66066,132133,30.03234100341797,6.437160368764693e-05
66266,66267,66266,132533,30.107356071472168,6.420107107375229e-05
66466,66467,66466,132933,30.186134099960327,6.403154782756372e-05
66667,66668,66667,133335,30.264997005462646,6.386218418921362e-05
66867,66868,66867,133735,30.342664003372192,6.369465579189391e-05
67067,67068,67067,134135,30.42068576812744,6.35281081026798e-05
67267,67268,67267,134535,30.503714084625244,6.336253178358987e-05
67467,67468,67467,134935,30.593995094299316,6.319791759543655e-05
67668,67669,67668,135337,30.68472719192505,6.303344046842269e-05
67868,67869,67868,135737,30.761645078659058,6.287072790733236e-05
68068,68069,68068,136137,30.837589979171753,6.27089502918304e-05
68268,68269,68268,136537,30.913481950759888,6.254809876510694e-05
68468,68469,68468,136937,30.99388098716736,6.238816456301334e-05
68669,68670,68669,137339,31.074273109436035,6.222834615446276e-05
68869,68870,68869,137739,31.15427303314209,6.207022515635127e-05
69069,69070,69069,138139,31.2361159324646,6.191299569727916e-05
69269,69270,69269,138539,31.31629180908203,6.175664937664303e-05
69469,69470,69469,138939,31.394287824630737,6.16011778815979e-05
69670,69671,69670,139341,31.478402853012085,6.144580212597409e-05
69870,69871,69870,139741,31.55917501449585,6.129205996493087e-05
70070,70071,70070,140141,31.638890027999878,6.113916817214204e-05
70270,70271,70270,140541,31.71678900718689,6.098711877923536e-05
70470,70471,70470,140941,31.798381805419922,6.083590390207905e-05
70671,70672,70671,141343,31.87745213508606,6.0684765862157374e-05
70871,70872,70871,141743,31.964252948760986,6.053520076929896e-05
71071,71072,71071,142143,32.04550886154175,6.038644699480457e-05
71271,71272,71271,142543,32.12396192550659,6.023849698105509e-05
71471,71472,71471,142943,32.20651698112488,6.0091343249464345e-05
71672,71673,71672,143345,32.28747200965881,5.994424854685157e-05
71872,71873,71872,143745,32.36630892753601,5.979866914962293e-05
72072,72073,72072,144145,32.44901990890503,5.965386403302622e-05
72272,72273,72272,144545,32.532268047332764,5.950982602909717e-05
72472,72473,72472,144945,32.61255192756653,5.9366548045045374e-05
72673,72674,72673,145347,32.69681215286255,5.922331231836823e-05
72873,72874,72873,145747,32.79669785499573,5.90815371070149e-05
73073,73074,73073,146147,32.880292892456055,5.8940501047744434e-05
73273,73274,73273,146547,32.96521306037903,5.880019734245497e-05
73473,73474,73473,146947,33.05357599258423,5.866061926368029e-05
73674,73675,73674,147349,33.134254932403564,5.852106765516473e-05
73874,73875,73874,147749,33.21486496925354,5.8382924476626055e-05
74074,74075,74074,148149,33.29492783546448,5.8245487132798064e-05
74274,74275,74274,148549,33.37486290931702,5.810874917559272e-05
74474,74475,74474,148949,33.45612287521362,5.7972704225169004e-05
74675,74676,74675,149351,33.5372748374939,5.783667089169477e-05
74875,74876,74875,149751,33.61662006378174,5.770199646834424e-05
75075,75076,75075,150151,33.6955509185791,5.7567996279863634e-05
75275,75276,75275,150551,33.77832102775574,5.743466421089161e-05
75475,75476,75475,150951,33.8564031124115,5.73019942102215e-05
75676,75677,75676,151353,33.936882972717285,5.716932185897792e-05
75876,75877,75876,151753,34.020718812942505,5.7037961330809366e-05
76076,76077,76076,152153,34.0984411239624,5.690724506755854e-05
76276,76277,76276,152553,34.17979979515076,5.677716726815116e-05
76476,76477,76476,152953,34.25961709022522,5.664772219367532e-05
76677,76678,76677,153355,34.340604066848755,5.6518261641105676e-05
76877,76878,76877,153755,34.424769163131714,5.63900681324997e-05
77077,77078,77077,154155,34.509692907333374,5.626249046277443e-05
77277,77278,77277,154555,34.59125900268555,5.613552313081021e-05
77477,77478,77477,154955,34.673171043395996,5.600916069291289e-05
77678,77679,77678,155357,34.75337100028992,5.588277044546666e-05
77878,77879,77878,155757,34.84217596054077,5.575760465119703e-05
78078,78079,78078,156157,34.94300198554993,5.563302773534676e-05
78278,78279,78278,156557,35.03144598007202,5.550903448005872e-05
78478,78479,78478,156957,35.11827802658081,5.538561972235338e-05
78679,78680,78679,157359,35.19811701774597,5.526216557873743e-05
78879,78880,78879,157759,35.279863119125366,5.513989537255256e-05
79079,79080,79079,158159,35.36023187637329,5.5018188473490145e-05
79279,79280,79279,158559,35.445720911026,5.489703993204642e-05
79479,79480,79479,158959,35.528383016586304,5.477644485141013e-05
79680,79681,79680,159361,35.614418029785156,5.465579952392235e-05
79880,79881,79880,159761,35.70518898963928,5.453629958596505e-05
80080,80081,80080,160161,35.78712821006775,5.441733870051712e-05
80280,80281,80280,160561,35.86912202835083,5.429891217312706e-05
80480,80481,80480,160961,35.950814962387085,5.418101535887664e-05
80681,80682,80681,161363,36.03790903091431,5.4063058114779584e-05
80881,80882,80881,161763,36.11598181724548,5.394620957790516e-05
81081,81082,81081,162163,36.19698476791382,5.382987708743884e-05
81281,81282,81281,162563,36.27899408340454,5.3714056190593805e-05
81481,81482,81481,162963,36.35883402824402,5.359874248125065e-05
81682,81683,81682,163365,36.44224691390991,5.3483358801464176e-05
81882,81883,81882,163765,36.52805209159851,5.336904891532779e-05
82082,82083,82082,164165,36.60699915885925,5.325523325306986e-05
82282,82283,82282,164565,36.687411069869995,5.314190759032265e-05
82482,82483,82482,164965,36.76889610290527,5.302906774833565e-05
82683,82684,82683,165367,36.84950518608093,5.291614900333781e-05
82883,82884,82883,165767,36.93309020996094,5.2804270815807494e-05
83083,83084,83083,166167,37.03491401672363,5.269286615101121e-05
83283,83284,83283,166567,37.12440204620361,5.2581931001994976e-05
83483,83484,83483,166967,37.204638957977295,5.247146140387234e-05
83684,83685,83684,167369,37.282936811447144,5.2360904546793865e-05
83884,83885,83884,167769,37.36454510688782,5.225135660081314e-05
84084,84085,84084,168169,37.44671106338501,5.2142262539445014e-05
84284,84285,84284,168569,37.53071999549866,5.203361856143172e-05
84484,84485,84484,168969,37.6095609664917,5.192542090537031e-05
84685,84686,84685,169371,37.69192099571228,5.181712817989302e-05
84885,84886,84885,169771,37.771737813949585,5.1709814226058195e-05
85085,85086,85085,170171,37.852418184280396,5.1602935526182555e-05
85285,85286,85285,170571,37.93754601478577,5.149648847405787e-05
85485,85486,85485,170971,38.03316402435303,5.1390469500802935e-05
85686,85687,85686,171373,38.110337018966675,5.128434816386314e-05
85886,85887,85886,171773,38.187089920043945,5.117917688809456e-05
86086,86087,86086,172173,38.26246190071106,5.1074423190192124e-05
86286,86287,86286,172573,38.33917188644409,5.097008364846747e-05
86486,86487,86486,172973,38.413886070251465,5.08661548770032e-05
86687,86688,86687,173375,38.49755096435547,5.0762116936507874e-05
86887,86888,86887,173775,38.57399606704712,5.0659001700684e-05
87087,87088,87087,174175,38.65196919441223,5.0556287271015e-05
87287,87288,87287,174575,38.72747182846069,5.045397040122372e-05
87487,87488,87487,174975,38.804770946502686,5.0352047877948285e-05
87688,87689,87688,175377,38.88428020477295,5.0250009842411725e-05
87888,87889,87888,175777,38.96459603309631,5.014886843963249e-05
88088,88089,88088,176177,39.043445110321045,5.00481119280004e-05
88288,88289,88288,176577,39.133360862731934,4.994773722723566e-05
88488,88489,88488,176977,39.22648000717163,4.9847741287811807e-05
88689,88690,88689,177379,39.30248188972473,4.974762393134118e-05
88889,88890,88889,177779,39.378626108169556,4.964837835114046e-05
89089,89090,89089,178179,39.46527600288391,4.954950255986683e-05
89289,89290,89289,178579,39.541452169418335,4.945099363336175e-05
89489,89490,89489,178979,39.61946988105774,4.935284867797949e-05
89690,89691,89690,179381,39.69503593444824,4.925457681335154e-05
89890,89891,89890,179781,39.77126097679138,4.9157153023239795e-05
90090,90091,90090,180181,39.846813917160034,4.906008468798891e-05
90290,90291,90290,180581,39.921870946884155,4.896336903265644e-05
90490,90491,90490,180981,40.00406312942505,4.886700331024598e-05
90691,90692,90691,181383,40.08094000816345,4.877050557829593e-05
90891,90892,90891,181783,40.161118030548096,4.8674833311830626e-05
91091,91092,91091,182183,40.244093894958496,4.857950289529335e-05
91291,91292,91291,182583,40.32598614692688,4.848451169400805e-05
91491,91492,91491,182983,40.40557599067688,4.8389857100470086e-05
91692,91693,91692,183385,40.4888379573822,4.829506576708527e-05
91892,91893,91892,183785,40.57007098197937,4.820107832665457e-05
92092,92093,92092,184185,40.6472430229187,4.810741982061989e-05
92292,92293,92292,184585,40.72266602516174,4.8014087747849376e-05
92492,92493,92492,184985,40.79735517501831,4.7921079633238715e-05
92693,92694,92693,185387,40.87606501579285,4.78279303978405e-05
92893,92894,92893,185787,40.95604419708252,4.773556446505198e-05
93093,93094,93093,186187,41.03342604637146,4.764351520490155e-05
93293,93294,93293,186587,41.115866899490356,4.755178024267786e-05
93493,93494,93493,186987,41.19392800331116,4.746035722810253e-05
93694,93695,93694,187389,41.29188895225525,4.736878904256728e-05
93894,93895,93894,187789,41.38224911689758,4.7277984500203896e-05
94094,94095,94094,188189,41.466525077819824,4.718748498762865e-05
94294,94295,94294,188589,41.544636964797974,4.709728824991651e-05
94494,94495,94494,188989,41.621017932891846,4.700739205520845e-05
94695,94696,94695,189391,41.69918608665466,4.6917346951021994e-05
94895,94896,94895,189791,41.774725914001465,4.682804671365096e-05
95095,95096,95095,190191,41.851755142211914,4.6739040449231476e-05
95295,95296,95295,190591,41.93176507949829,4.6650326016469764e-05
95495,95496,95495,190991,42.01332902908325,4.65619012955308e-05
95696,95697,95696,191393,42.09184908866882,4.647332422196686e-05
95896,95897,95896,191793,42.17249393463135,4.638547407461628e-05
96096,96097,96096,192193,42.25408601760864,4.62979073989207e-05
96296,96297,96296,192593,42.32894492149353,4.6210622160562225e-05
96496,96497,96496,192993,42.40735220909119,4.6123616346403906e-05
96697,96698,96697,193395,42.492279052734375,4.603645501466148e-05
96897,96898,96897,193795,42.56978988647461,4.595000346169595e-05
97097,97098,97097,194195,42.65055012702942,4.5863825404706794e-05
97297,97298,97297,194595,42.728776931762695,4.5777918910961394e-05
97497,97498,97497,194995,42.81455993652344,4.569228206742184e-05
97698,97699,97698,195397,42.90494894981384,4.5606486804786894e-05
97898,97899,97898,195797,42.99353504180908,4.552138492516394e-05
98098,98099,98098,196197,43.07409596443176,4.5436547063727276e-05
98298,98299,98298,196597,43.15143084526062,4.535197138353022e-05
98498,98499,98498,196997,43.230798959732056,4.526765606715384e-05
98699,98700,98699,197399,43.31730580329895,4.518317967796968e-05
98899,98900,98899,197799,43.40867495536804,4.509938098880208e-05
99099,99100,99099,198199,43.50590896606445,4.501583731072681e-05
99299,99300,99299,198599,43.58467888832092,4.4932546898934345e-05
99499,99500,99499,198999,43.668943881988525,4.4849508025442464e-05
99700,99701,99700,199401,43.74657201766968,4.476630565986469e-05
99900,99901,99900,199801,43.82656788825989,4.468376598651652e-05
100100,100101,100100,200201,43.91165804862976,4.460147276404328e-05
100300,100301,100300,200601,43.99417304992676,4.4519424333958804e-05
100501,100502,100501,201003,44.074317932128906,4.4437210635475236e-05
100701,100702,100701,201403,44.15537214279175,4.4355648082676674e-05
100901,100902,100901,201803,44.23448896408081,4.427432543655744e-05
101101,101102,101101,202203,44.31381893157959,4.4193241104020573e-05
101301,101302,101301,202603,44.39270997047424,4.411239350782217e-05
101502,101503,101502,203005,44.478676080703735,4.403137861250175e-05
101702,101703,101702,203405,44.557607889175415,4.3951000984366675e-05
101902,101903,101902,203805,44.63611078262329,4.387085544702319e-05
102102,102103,102102,204205,44.71394395828247,4.379094048596792e-05
102302,102303,102302,204605,44.79495882987976,4.371125460109813e-05
102503,102504,102503,205007,44.87564396858215,4.363139958517778e-05
102703,102704,102703,205407,44.95785713195801,4.355216853968124e-05
102903,102904,102903,205807,45.04213881492615,4.347316215269364e-05
103103,103104,103103,206207,45.121954917907715,4.339437898297778e-05
103303,103304,103303,206607,45.20370101928711,4.3315817604432367e-05
103504,103505,103504,207009,45.28641319274902,4.3237085450637275e-05
103704,103705,103704,207409,45.36842393875122,4.31589645219411e-05
103904,103905,103904,207809,45.45476698875427,4.308106118189421e-05
104104,104105,104104,208209,45.54423999786377,4.300337405977073e-05
104304,104305,104304,208609,45.64161705970764,4.292590179788452e-05
104505,104506,104505,209011,45.72373700141907,4.284825729345846e-05
104705,104706,104705,209411,45.803914070129395,4.2771211792207505e-05
104905,104906,104905,209811,45.8831729888916,4.2694377153060974e-05
105105,105106,105105,210211,45.96348690986633,4.2617752071961553e-05
105305,105306,105305,210611,46.04665184020996,4.2541335256941415e-05
105506,105507,105506,211013,46.13040113449097,4.246474489785581e-05
105706,105707,105706,211413,46.212258100509644,4.238874181677754e-05
105906,105907,105906,211813,46.293575048446655,4.23129431963783e-05
106106,106107,106106,212213,46.37206196784973,4.223734779535781e-05
106306,106307,106306,212613,46.45710492134094,4.21619543842812e-05
106507,106508,106507,213015,46.538617849349976,4.208638628516038e-05
106707,106708,106707,213415,46.61709499359131,4.2011394208758133e-05
106907,106908,106907,213815,46.695218086242676,4.193660049983342e-05
107107,107108,107107,214215,46.775821924209595,4.186200397677679e-05
107307,107308,107307,214615,46.85411477088928,4.178760346839654e-05
107508,107509,107508,215017,46.93628191947937,4.171302727544776e-05
107708,107709,107708,215417,47.01962184906006,4.163901629685916e-05
107908,107909,107908,215817,47.09853005409241,4.1565197883957355e-05
108108,108109,108108,216217,47.181257009506226,4.1491570911192283e-05
108308,108309,108308,216617,47.264363050460815,4.141813426371686e-05
108509,108510,108509,217019,47.34454679489136,4.134452107380839e-05
108709,108710,108709,217419,47.42446494102478,4.127146271369822e-05
108909,108910,108909,217819,47.509562969207764,4.119859139323062e-05
109109,109110,109109,218219,47.59292697906494,4.112590604067391e-05
109309,109310,109309,218619,47.686015129089355,4.105340559358115e-05
109510,109511,109510,219021,47.78118681907654,4.098072787766297e-05
109710,109711,109710,219421,47.86658596992493,4.090859500833572e-05
109910,109911,109910,219821,47.949278116226196,4.08366439143689e-05
110110,110111,110110,220221,48.03438115119934,4.076487357428793e-05
110310,110311,110310,220621,48.11350393295288,4.069328297583729e-05
110511,110512,110511,221023,48.19527792930603,4.06215145052255e-05
110711,110712,110711,221423,48.27540111541748,4.0550281279324136e-05
110911,110912,110911,221823,48.35679388046265,4.047922481193626e-05
111111,111112,111111,222223,48.43810200691223,4.0408344129327434e-05
111311,111312,111311,222623,48.51961088180542,4.033763826678008e-05
111512,111513,111512,223025,48.60093283653259,4.026675404407288e-05
111712,111713,111712,223425,48.68097376823425,4.0196395826437246e-05
111912,111913,111912,223825,48.76327395439148,4.012620958492055e-05
112112,112113,112112,224225,48.846166133880615,4.005619439092852e-05
112312,112313,112312,224625,48.92725205421448,3.9986349324519967e-05
112513,112514,112513,225027,49.01716685295105,3.991632551894718e-05
112713,112714,112713,225427,49.09960889816284,3.984681882233775e-05
112913,112914,112913,225827,49.1836371421814,3.977747954114498e-05
113113,113114,113113,226227,49.26512002944946,3.9708306789901046e-05
113313,113314,113313,226627,49.350492000579834,3.963929969087814e-05
113514,113515,113514,227029,49.43362498283386,3.957011357645754e-05
113714,113715,113714,227429,49.515828132629395,3.950143600047526e-05
113914,113915,113914,227829,49.59797692298889,3.943292148971854e-05
114114,114115,114114,228229,49.679116010665894,3.936456919881085e-05
114314,114315,114314,228629,49.76152205467224,3.929637829092299e-05
114515,114516,114515,229031,49.862327098846436,3.922800818680446e-05
114715,114716,114715,229431,49.94787001609802,3.91601383607746e-05
114915,114916,114915,229831,50.03011417388916,3.909242744835706e-05
115115,115116,115115,230231,50.1070830821991,3.902487464335613e-05
115315,115316,115315,230631,50.1849639415741,3.895747914627273e-05
115516,115517,115516,231033,50.26413917541504,3.888990436266954e-05
115716,115717,115716,231433,50.34012293815613,3.8822821890638963e-05
115916,115917,115916,231833,50.421066999435425,3.8755894369682186e-05
116116,116117,116116,232233,50.503714084625244,3.8689121029266045e-05
116316,116317,116316,232633,50.581632137298584,3.8622501106821576e-05
116517,116518,116517,233035,50.65706396102905,3.8555701891965155e-05
116717,116718,116717,233435,50.73379111289978,3.8489387301604596e-05
116917,116918,116917,233835,50.80900597572327,3.842322387769995e-05
117117,117118,117117,234235,50.88679003715515,3.8357210885008294e-05
117317,117318,117317,234635,50.96498107910156,3.829134759437342e-05
117518,117519,117518,235037,51.044734954833984,3.822530508543405e-05
117718,117719,117718,235437,51.12202596664429,3.815973977851581e-05
117918,117919,117918,235837,51.203428983688354,3.8094322023284365e-05
118118,118119,118118,236237,51.284037828445435,3.8029051116542725e-05
118318,118319,118318,236637,51.36483311653137,3.7963926362210494e-05
118519,118520,118519,237039,51.4428391456604,3.789862253742803e-05
118719,118720,118719,237439,51.526309967041016,3.783378874488906e-05
118919,118920,118919,237839,51.60740399360657,3.7769099048986214e-05
119119,119120,119119,238239,51.68603181838989,3.770455277765697e-05
119319,119320,119319,238639,51.766318798065186,3.764014926536829e-05
119520,119521,119520,239041,51.84431791305542,3.7575566900848915e-05
119720,119721,119720,239441,51.92880582809448,3.751144763786003e-05
119920,119921,119920,239841,52.026668071746826,3.744746916831129e-05
120120,120121,120120,240241,52.109638929367065,3.738363084998344e-05
120320,120321,120320,240641,52.18917798995972,3.7319932045600794e-05
120521,120522,120521,241043,52.26630902290344,3.7256054672370245e-05
120721,120722,120721,241443,52.34456515312195,3.71926336979702e-05
120921,120922,120921,241843,52.420315980911255,3.712935035773095e-05
121121,121122,121121,242243,52.4990758895874,3.706620403679001e-05
121321,121322,121321,242643,52.57432413101196,3.7003194126042957e-05
121522,121523,121522,243045,52.65137696266174,3.694000599102525e-05
121722,121723,121722,243445,52.72774600982666,3.687726776829454e-05
121922,121923,121922,243845,52.803921937942505,3.681466415666744e-05
122122,122123,122122,244245,52.88351106643677,3.675219456746879e-05
122322,122323,122322,244645,52.96416997909546,3.668985841792255e-05
122523,122524,122523,245047,53.04464602470398,3.662734444588582e-05
122723,122724,122723,245447,53.12048602104187,3.656527410556934e-05
122923,122924,122923,245847,53.19624400138855,3.650333548221747e-05
123123,123124,123123,246247,53.273268938064575,3.644152801252862e-05
123323,123324,123323,246647,53.34997296333313,3.637985113779499e-05
123524,123525,123524,247049,53.42550086975098,3.631799689617622e-05
123724,123725,123724,247449,53.5063259601593,3.6256580201276516e-05
123924,123925,123924,247849,53.58531308174133,3.6195292451558116e-05
124124,124125,124124,248249,53.664392948150635,3.61341331075647e-05
124324,124325,124324,248649,53.74486780166626,3.6073101634029336e-05
124525,124526,124525,249051,53.820728063583374,3.601189329879468e-05
124725,124726,124725,249451,53.89958691596985,3.595111661170688e-05
124925,124926,124925,249851,53.982946157455444,3.589046621418496e-05
125125,125126,125125,250251,54.07029414176941,3.582994158898002e-05
125325,125326,125325,250651,54.16751503944397,3.576954222295726e-05
125526,125527,125526,251053,54.24735903739929,3.5708966547326677e-05
125726,125727,125726,251453,54.32513689994812,3.5648816798425745e-05
125926,125927,125926,251853,54.405335903167725,3.5588790793452624e-05
126126,126127,126126,252253,54.491832971572876,3.552888803582781e-05
126326,126327,126326,252653,54.57054805755615,3.546910803420644e-05
126527,126528,126527,253055,54.65074801445007,3.54091523182087e-05
126727,126728,126727,253455,54.73316502571106,3.534961697648097e-05
126927,126928,126927,253855,54.81295585632324,3.529020293667073e-05
127127,127128,127127,254255,54.89159393310547,3.5230909723080626e-05
127327,127328,127327,254655,54.97502112388611,3.517173686366934e-05
127528,127529,127528,255057,55.05451703071594,3.5112388926087264e-05
127728,127729,127728,255457,55.13575291633606,3.5053455970777626e-05
127928,127929,127928,255857,55.21449613571167,3.499464197430056e-05
128128,128129,128128,256257,55.29251194000244,3.493594648039009e-05
128328,128329,128328,256657,55.372421979904175,3.4877369035759516e-05
128529,128530,128529,257059,55.45490217208862,3.481861718652739e-05
128729,128730,128729,257459,55.53842496871948,3.476027508052361e-05
128929,128930,128929,257859,55.61725187301636,3.470204968447367e-05
129129,129130,129129,258259,55.69550704956055,3.464394055939638e-05
129329,129330,129329,258659,55.776094913482666,3.458594727052638e-05
129530,129531,129530,259061,55.858604192733765,3.452778028585888e-05
129730,129731,129730,259461,55.93754696846008,3.447001795149704e-05
129930,129931,129930,259861,56.02201199531555,3.441237016624485e-05
130130,130131,130130,260261,56.10311198234558,3.4354836508896e-05
130330,130331,130330,260661,56.18953204154968,3.429741656130051e-05
130531,130532,130531,261063,56.28816604614258,3.4239823659516414e-05
130731,130732,130731,261463,56.36943006515503,3.418263045364034e-05
130931,130932,130931,261863,56.450993061065674,3.412554972080765e-05
131131,131132,131131,262263,56.533968925476074,3.406858105580677e-05
131331,131332,131331,262663,56.61682891845703,3.401172405665122e-05
131532,131533,131532,263065,56.6952760219574,3.395469487482563e-05
131732,131733,131732,263465,56.77333998680115,3.3898060567339216e-05
131932,131933,131932,263865,56.85051202774048,3.3841536736675074e-05
132132,132133,132132,264265,56.929431200027466,3.3785122992633076e-05
132332,132333,132332,264665,57.01650905609131,3.3728818948922185e-05
132533,132534,132533,265067,57.09825801849365,3.3672343522096916e-05
132733,132734,132733,265467,57.179256200790405,3.361625827438868e-05
132933,132934,132933,265867,57.26089596748352,3.3560281582751796e-05
133133,133134,133133,266267,57.34064602851868,3.3504413071810436e-05
133333,133334,133333,266667,57.41987490653992,3.3448652369900155e-05
133534,133535,133534,267069,57.50400900840759,3.339272111034821e-05
133734,133735,133734,267469,57.58537411689758,3.333717545501748e-05
133934,133935,133934,267869,57.6638867855072,3.328173650691955e-05
134134,134135,134134,268269,57.74568510055542,3.3226403905068906e-05
134334,134335,134334,268669,57.823628187179565,3.317117729093063e-05
134535,134536,134535,269071,57.90759992599487,3.311578096867486e-05
134735,134736,134735,269471,57.99188780784607,3.306076579105177e-05
134935,134936,134935,269871,58.07089376449585,3.300585554015017e-05
135135,135136,135135,270271,58.15035605430603,3.29510498680178e-05
135335,135336,135335,270671,58.22900581359863,3.289634842950437e-05
135536,135537,135536,271073,58.31248688697815,3.284147815433303e-05
135736,135737,135736,271473,58.413609981536865,3.2786984673873046e-05
135936,135937,135936,271873,58.5001118183136,3.273259440441426e-05
136136,136137,136136,272273,58.583348989486694,3.26783070105449e-05
136336,136337,136336,272673,58.66291785240173,3.262412215948365e-05
136537,136538,136537,273075,58.74141812324524,3.256976936384509e-05
136737,136738,136737,273475,58.82089805603027,3.251578911756609e-05
136937,136938,136937,273875,58.90895104408264,3.246191042815115e-05
137137,137138,137137,274275,58.996533155441284,3.2408132972123315e-05
137337,137338,137337,274675,59.12900400161743,3.2354456428208e-05
137538,137539,137538,275077,59.23639106750488,3.2300612849941055e-05
137738,137739,137738,275477,59.32491707801819,3.2247137676755736e-05
137938,137939,137938,275877,59.41680097579956,3.219376246431049e-05
138138,138139,138138,276277,59.512840032577515,3.21404869005079e-05
138338,138339,138338,276677,59.650712966918945,3.2087310675677356e-05
138539,138540,138539,277079,59.75735402107239,3.2033968343968456e-05
138739,138740,138739,277479,59.840436935424805,3.198099036833098e-05
138939,138940,138939,277879,59.924654960632324,3.1928110813003945e-05
139139,139140,139139,278279,60.02080798149109,3.187532937664559e-05
139339,139340,139339,278679,60.11024498939514,3.182264576006815e-05
139540,139541,139540,279081,60.2020947933197,3.176979697987561e-05
139740,139741,139740,279481,60.287895917892456,3.171730859837285e-05
139940,139941,139940,279881,60.37164902687073,3.166491714939388e-05
140140,140141,140140,280281,60.47385811805725,3.1612622341890724e-05
140340,140341,140340,280681,60.63343286514282,3.156042388655909e-05
140541,140542,140541,281083,60.75730800628662,3.1508061225090445e-05
140741,140742,140741,281483,60.853440046310425,3.1456055092394756e-05
140941,140942,140941,281883,60.9466598033905,3.140414445468293e-05
141141,141142,141141,282283,61.115293979644775,3.1352329030188275e-05
141341,141342,141341,282683,61.22227907180786,3.130060853944777e-05
141542,141543,141542,283085,61.30240797996521,3.124872481293569e-05
141742,141743,141742,283485,61.39384698867798,3.119719382931265e-05
141942,141943,141942,283885,61.48024106025696,3.114575695049307e-05
142142,142143,142142,284285,61.56629204750061,3.109441390386984e-05
142342,142343,142342,284685,61.64851093292236,3.104316441907263e-05
142543,142544,142543,285087,61.72599720954895,3.0991752680304946e-05
142743,142744,142743,285487,61.80568194389343,3.094068997928876e-05
142943,142944,142943,285887,61.881242990493774,3.088972003759656e-05
143143,143144,143143,286287,61.96367120742798,3.0838842592008134e-05
143343,143344,143343,286687,62.0442099571228,3.078805738069055e-05
143544,143545,143544,287089,62.12278985977173,3.0737110907847793e-05
143744,143745,143744,287489,62.20016598701477,3.0686509843999976e-05
143944,143945,143944,287889,62.279021978378296,3.063600023778612e-05
144144,144145,144144,288289,62.357348918914795,3.0585581833750395e-05
144344,144345,144344,288689,62.43450307846069,3.0535254378489374e-05
144545,144546,144545,289091,62.51990604400635,3.0484766663359365e-05
144745,144746,144745,289491,62.606056928634644,3.043462080276711e-05
144945,144946,144945,289891,62.7058482170105,3.0384565138386286e-05
145145,145146,145145,290291,62.799638986587524,3.0334599422977208e-05
145345,145346,145345,290691,62.88571500778198,3.0284723410669133e-05
145546,145547,145546,291093,62.97048997879028,3.0234688149085694e-05
145746,145747,145746,291493,63.050812005996704,3.0184991257592242e-05
145946,145947,145946,291893,63.142739057540894,3.013538334007429e-05
146146,146147,146146,292293,63.260359048843384,3.008586415646252e-05
146346,146347,146346,292693,63.37720823287964,3.003643346912084e-05
146547,146548,146547,293095,63.46417307853699,2.9986844549692967e-05
146747,146748,146747,293495,63.544156074523926,2.993759058442196e-05
146947,146948,146947,293895,63.620667934417725,2.9888424407463857e-05
147147,147148,147147,294295,63.699203968048096,2.9839345786595368e-05
147347,147348,147347,294695,63.77456998825073,2.97903544902232e-05
147548,147549,147548,295097,63.851314067840576,2.9741205986444744e-05
147748,147749,147748,295497,63.93123197555542,2.9692389085414498e-05
147948,147949,147948,295897,64.01650595664978,2.9643658822735838e-05
148148,148149,148148,296297,64.09740710258484,2.9595014972604923e-05
148348,148349,148348,296697,64.17262601852417,2.9546457310445976e-05
148549,148550,148549,297099,64.25500702857971,2.94977434705667e-05
148749,148750,148749,297499,64.33599400520325,2.944935794508017e-05
148949,148950,148949,297899,64.42420792579651,2.9401057940915373e-05
149149,149150,149149,298299,64.51295900344849,2.9352843239262764e-05
149349,149350,149349,298699,64.60090494155884,2.9304713621886748e-05
149550,149551,149550,299101,64.68781805038452,2.9256428861240055e-05
149750,149751,149750,299501,64.78203392028809,2.9208469186524026e-05
149950,149951,149950,299901,64.88598608970642,2.9160593948292362e-05
150150,150151,150150,300301,64.97136211395264,2.9112802934132927e-05
150350,150351,150350,300701,65.05492901802063,2.9065095931660782e-05
150551,150552,150551,301103,65.13524794578552,2.9017234824598267e-05
150751,150752,150751,301503,65.21284508705139,2.8969695632407664e-05
150951,150952,150951,301903,65.29227089881897,2.8922239822920026e-05
151151,151152,151151,302303,65.37263488769531,2.8874867188456232e-05
151351,151352,151351,302703,65.45100402832031,2.8827577523143312e-05
151552,151553,151552,303105,65.53881812095642,2.8780134795310163e-05
151752,151753,151752,303505,65.62929010391235,2.873301086728754e-05
151952,151953,151952,303905,65.71251201629639,2.8685969296261616e-05
152152,152153,152152,304305,65.7923309803009,2.863900988055603e-05
152352,152353,152352,304705,65.87299799919128,2.8592132419901223e-05
152553,152554,152553,305107,65.95416498184204,2.854510294121894e-05
152753,152754,152753,305507,66.03378009796143,2.8498389200783686e-05
152953,152954,152953,305907,66.11412310600281,2.8451756819195488e-05
153153,153154,153153,306307,66.19321608543396,2.8405205600672602e-05
153353,153354,153353,306707,66.27086901664734,2.835873534986366e-05
153554,153555,153554,307109,66.34968495368958,2.8312114127950125e-05
153754,153755,153754,307509,66.43026995658875,2.8265805633858505e-05
153954,153955,153954,307909,66.51378893852234,2.8219577527341483e-05
154154,154155,154154,308309,66.59417200088501,2.8173429617296937e-05
154354,154355,154354,308709,66.67005181312561,2.8127361713733652e-05
154555,154556,154555,309111,66.74963998794556,2.808114388731143e-05
154755,154756,154755,309511,66.82511115074158,2.8035235827740164e-05
154955,154956,154955,309911,66.90601086616516,2.798940720963267e-05
155155,155156,155155,310311,67.00175595283508,2.7943657846335562e-05
155355,155356,155355,310711,67.08723592758179,2.7897987552790368e-05
155556,155557,155556,311113,67.16258311271667,2.7852168385338706e-05
155756,155757,155756,311513,67.24588298797607,2.7806656072274796e-05
155956,155957,155956,311913,67.32316493988037,2.776122227784372e-05
156156,156157,156156,312313,67.4009428024292,2.7715866820602497e-05
156356,156357,156356,312713,67.48641300201416,2.767058951975651e-05
156557,156558,156557,313115,67.56510901451111,2.7625164394857523e-05
156757,156758,156757,313515,67.64877009391785,2.7580043257270633e-05
156957,156958,156957,313915,67.72689580917358,2.7534999738770038e-05
157157,157158,157157,314315,67.80661988258362,2.7490033662440043e-05
157357,157358,157357,314715,67.8848888874054,2.744514485171511e-05
157558,157559,157558,315117,67.97049307823181,2.7400109266054946e-05
157758,157759,157758,315517,68.05316090583801,2.73553748458076e-05
157958,157959,157958,315917,68.13464403152466,2.7310717166699878e-05
158158,158159,158158,316317,68.21304821968079,2.726613605625704e-05
158358,158359,158358,316717,68.29418182373047,2.7221631342149742e-05
158559,158560,158559,317119,68.37260293960571,2.7176980902198065e-05
158759,158760,158759,317519,68.45442485809326,2.7132628848051296e-05
158959,158960,158959,317919,68.53934597969055,2.7088352678290366e-05
159159,159160,159159,318319,68.62397599220276,2.7044152224168055e-05
159359,159360,159359,318719,68.70588397979736,2.700002731772764e-05
159560,159561,159560,319121,68.78680300712585,2.695575773311357e-05
159760,159761,159760,319521,68.86467599868774,2.6911783796723035e-05
159960,159961,159960,319921,68.94763708114624,2.6867884907825417e-05
160160,160161,160160,320321,69.0287868976593,2.6824060901366357e-05
160360,160361,160360,320721,69.12804698944092,2.6780311613273723e-05
160561,160562,160561,321123,69.2211651802063,2.6736418693567236e-05
160761,160762,160761,321523,69.2997100353241,2.669281872431606e-05
160961,160962,160961,321923,69.38189387321472,2.6649292984668876e-05
161161,161162,161161,322323,69.46844911575317,2.6605841313346673e-05
161361,161362,161361,322723,69.54917788505554,2.656246354986753e-05
161562,161563,161562,323125,69.63123989105225,2.6518943199524403e-05
161762,161763,161762,323525,69.7119529247284,2.6475713140751926e-05
161962,161963,161962,323925,69.79346489906311,2.643255651172769e-05
162162,162163,162162,324325,69.874342918396,2.6389473155239724e-05
162362,162363,162362,324725,69.96125912666321,2.6346462913894484e-05
162563,162564,162563,325127,70.04554605484009,2.6303311128111402e-05
162763,162764,162763,325527,70.12514686584473,2.626044701272213e-05
162963,162964,162963,325927,70.20838403701782,2.6217655545066073e-05
163163,163164,163163,326327,70.29753708839417,2.6174936570835707e-05
163363,163364,163363,326727,70.37494993209839,2.613228993624304e-05
163564,163565,163564,327129,70.46351385116577,2.6089502797447043e-05
163764,163765,163764,327529,70.54457807540894,2.60470007442656e-05
163964,163965,163964,327929,70.62369203567505,2.6004570573183797e-05
164164,164165,164164,328329,70.70361185073853,2.59622121331005e-05
164364,164365,164364,328729,70.78573703765869,2.591992527400661e-05
164565,164566,164565,329131,70.86762809753418,2.5877498948005026e-05
164765,164766,164765,329531,70.95184707641602,2.583535515765484e-05
164965,164966,164965,329931,71.03708386421204,2.579328250024782e-05
165165,165166,165165,330331,71.12117791175842,2.575128082717377e-05
165365,165366,165365,330731,71.20958280563354,2.5709349991992775e-05
165566,165567,165566,331133,71.31035089492798,2.566728072405003e-05
165766,165767,165766,331533,71.39327907562256,2.5625491476525075e-05
165966,165967,165966,331933,71.47820591926575,2.5583772627428496e-05
166166,166167,166166,332333,71.55819511413574,2.5542124031821056e-05
166366,166367,166366,332733,71.64023494720459,2.5500545545581572e-05
166567,166568,166567,333135,71.72308588027954,2.5458829657697984e-05
166767,166768,166767,333535,71.80168795585632,2.5417391307826607e-05
166967,166968,166967,333935,71.88214778900146,2.5376022637118338e-05
167167,167168,167167,334335,71.96519613265991,2.533472350322284e-05
167367,167368,167367,334735,72.04813814163208,2.5293493764724562e-05
167568,167569,167568,335137,72.12994694709778,2.5252127652204736e-05
167768,167769,167768,335537,72.23067498207092,2.5211036627615562e-05
167968,167969,167968,335937,72.37901020050049,2.517001457651908e-05
168168,168169,168168,336337,72.48583984375,2.5129061359817475e-05
168368,168369,168368,336737,72.58683395385742,2.5088176838883764e-05
168569,168570,168569,337139,72.67611908912659,2.504715696707863e-05
168769,168770,168769,337539,72.75958895683289,2.5006409764613043e-05
168969,168970,168969,337939,72.85273098945618,2.4965730843957197e-05
169169,169170,169169,338339,72.95363688468933,2.492512006818308e-05
169369,169370,169369,338739,73.03515601158142,2.4884577301458747e-05
169570,169571,169570,339141,73.11619687080383,2.4843900203789654e-05
169770,169771,169770,339541,73.19726014137268,2.4803493386753263e-05
169970,169971,169970,339941,73.27739191055298,2.476315417274965e-05
170170,170171,170170,340341,73.37172198295593,2.4722882427436343e-05
170370,170371,170370,340741,73.4651780128479,2.4682678017042692e-05
170571,170572,170571,341143,73.5430281162262,2.464234029133234e-05
170771,170772,170771,341543,73.61900281906128,2.4602270487442722e-05
170971,170972,170971,341943,73.69428300857544,2.4562267619795407e-05
171171,171172,171171,342343,73.77080702781677,2.4522331557166596e-05
171371,171372,171371,342743,73.8505449295044,2.44824621681199e-05
171572,171573,171572,343145,73.93052387237549,2.444246047446521e-05
171772,171773,171772,343545,74.01479005813599,2.440272437249855e-05
171972,171973,171972,343945,74.10432291030884,2.4363054552510238e-05
172172,172173,172172,344345,74.18094301223755,2.432345088527498e-05
172372,172373,172372,344745,74.25656199455261,2.4283913241877487e-05
172573,172574,172573,345147,74.33667588233948,2.424424430063261e-05
172773,172774,172773,345547,74.41180300712585,2.4204838648445188e-05
172973,172974,172973,345947,74.49563908576965,2.416549863573101e-05
173173,173174,173173,346347,74.57271194458008,2.4126224135012666e-05
173373,173374,173373,346747,74.64954996109009,2.408701501978019e-05
173574,173575,173574,347149,74.72903776168823,2.4047675608390944e-05
173774,173775,173774,347549,74.80734300613403,2.4008597211097718e-05
173974,173975,173974,347949,74.8836760520935,2.3969583821460713e-05
174174,174175,174174,348349,74.96640276908875,2.393063531418105e-05
174374,174375,174374,348749,75.04356002807617,2.3891751565157153e-05
174575,174576,174575,349151,75.12446188926697,2.3852738516664782e-05
174775,174776,174775,349551,75.20208096504211,2.381398423381695e-05
174975,174976,174975,349951,75.27801990509033,2.377529433750164e-05
175175,175176,175175,350351,75.35660600662231,2.3736668704880963e-05
175375,175376,175375,350751,75.43533897399902,2.369810721313198e-05
175576,175577,175576,351153,75.5359570980072,2.365941741395211e-05
175776,175777,175776,351553,75.62187504768372,2.362098415806257e-05
175976,175977,175976,351953,75.69964504241943,2.358261467762799e-05
176176,176177,176176,352353,75.77583694458008,2.3544308852217578e-05
176376,176377,176376,352753,75.85486698150635,2.3506066560952518e-05
176577,176578,176577,353155,75.9324791431427,2.346769694891448e-05
176777,176778,176777,353555,76.01628589630127,2.3429581682828507e-05
176977,176978,176977,353955,76.09648394584656,2.3391529591373932e-05
177177,177178,177177,354355,76.17445302009583,2.335354055597404e-05
177377,177378,177377,354755,76.2517352104187,2.331561445777261e-05
177578,177579,177578,355157,76.33051705360413,2.327756202008536e-05
177778,177779,177778,355557,76.4132969379425,2.3239761755813876e-05
177978,177979,177978,355957,76.49679112434387,2.3202024074966632e-05
178178,178179,178178,356357,76.57534003257751,2.3164348860408362e-05
178378,178379,178378,356757,76.65414619445801,2.3126735995848277e-05
178579,178580,178579,357159,76.73327112197876,2.30889977676818e-05
178779,178780,178779,357559,76.81040287017822,2.3051509564292444e-05
178979,178980,178979,357959,76.88769316673279,2.3014083362342935e-05
179179,179180,179179,358359,76.96696710586548,2.2976719046527596e-05
179379,179380,179379,358759,77.04788517951965,2.2939416502165614e-05
179580,179581,179580,359161,77.12526178359985,2.290198956470806e-05
179780,179781,179780,359561,77.20362901687622,2.2864810527063875e-05
179980,179981,179980,359961,77.28173398971558,2.2827692917542094e-05
180180,180181,180180,360361,77.3619978427887,2.279063662294794e-05
180380,180381,180380,360761,77.43956112861633,2.275364152996231e-05
180581,180582,180581,361163,77.52642703056335,2.2716523009035234e-05
180781,180782,180781,361563,77.61226916313171,2.2679650285878982e-05
180981,180982,180981,361963,77.70938086509705,2.2642838426256483e-05
181181,181182,181181,362363,77.78803992271423,2.2606087318521188e-05
181381,181382,181381,362763,77.8656358718872,2.2569396851381405e-05
181582,181583,181582,363165,77.94710087776184,2.2532583915660897e-05
181782,181783,181782,363565,78.03105688095093,2.2496014698016048e-05
181982,181983,181982,363965,78.10898113250732,2.2459505787817227e-05
182182,182183,182182,364365,78.18795084953308,2.2423057074984687e-05
182382,182383,182382,364765,78.27460503578186,2.238666844956508e-05
182583,182584,182583,365167,78.35239887237549,2.23501583093598e-05
182783,182784,182783,365567,78.43050694465637,2.231388982964097e-05
182983,182984,182983,365967,78.51196599006653,2.2277681109248998e-05
183183,183184,183183,366367,78.59074378013611,2.2241532039375165e-05
183383,183384,183383,366767,78.66966104507446,2.2205442512081338e-05
183584,183585,183584,367169,78.75222206115723,2.216923241788285e-05
183784,183785,183784,367569,78.8373351097107,2.213326194814222e-05
183984,183985,183984,367969,78.91518998146057,2.209735069722583e-05
184184,184185,184184,368369,78.9989321231842,2.206149855818492e-05
184384,184385,184384,368769,79.08092093467712,2.2025705424122853e-05
184585,184586,184585,369171,79.16448378562927,2.1989792665458342e-05
184785,184786,184785,369571,79.24175596237183,2.195411751612526e-05
184985,184986,184985,369971,79.32132697105408,2.1918501052878556e-05
185185,185186,185185,370371,79.40154099464417,2.188294317003418e-05
185385,185386,185385,370771,79.48456192016602,2.184744376233669e-05
185586,185587,185586,371173,79.56626415252686,2.1811825666163558e-05
185786,185787,185786,371573,79.65042686462402,2.1776443184989083e-05
185986,185987,185986,371973,79.7382800579071,2.1741118864522782e-05
186186,186187,186186,372373,79.83636212348938,2.170585260020651e-05
186386,186387,186386,372773,79.91850090026855,2.1670644288367613e-05
186587,186588,186587,373175,80.00304794311523,2.1635318218169804e-05
186787,186788,186787,373575,80.0810980796814,2.1600225789428827e-05
186987,186988,186987,373975,80.16105389595032,2.156519100240126e-05
187187,187188,187187,374375,80.24417901039124,2.1530213754814547e-05
187387,187388,187387,374775,80.32584500312805,2.1495293943770525e-05
187588,187589,187588,375177,80.40543293952942,2.146025729886453e-05
187788,187789,187788,375577,80.4919319152832,2.142545234100725e-05
187988,187989,187988,375977,80.5713460445404,2.139070451345724e-05
188188,188189,188188,376377,80.65219497680664,2.1356013714720305e-05
188388,188389,188388,376777,80.73476696014404,2.1321379844114263e-05
188589,188590,188589,377179,80.81750798225403,2.1286630057780718e-05
188789,188790,188789,377579,80.89874005317688,2.1252110023521814e-05
188989,188990,188989,377979,80.98782396316528,2.1217646614955024e-05
189189,189190,189189,378379,81.07085180282593,2.1183239731677537e-05
189389,189390,189389,378779,81.15163707733154,2.1148889273751914e-05
189590,189591,189590,379181,81.22996520996094,2.1114423812671987e-05
189790,189791,189790,379581,81.31006908416748,2.108018618819083e-05
189990,189991,189990,379981,81.39129877090454,2.1046004690758173e-05
190190,190191,190190,380381,81.47272086143494,2.1011879221415873e-05
190390,190391,190390,380781,81.555184841156,2.0977809681550047e-05
190591,190592,190591,381183,81.63444900512695,2.0943626044549757e-05
190791,190792,190791,381583,81.7119870185852,2.0909668347591e-05
190991,190992,190991,381983,81.7903881072998,2.08757662853754e-05
191191,191192,191191,382383,81.87673091888428,2.0841919760578568e-05
191391,191392,191391,382783,81.97823810577393,2.0808128675370656e-05
191592,191593,191592,383185,82.05850601196289,2.0774224393076465e-05
191792,191793,191792,383585,82.13778114318848,2.0740544172617413e-05
191992,191993,191992,383985,82.21685791015625,2.0706919100714405e-05
192192,192193,192192,384385,82.2965259552002,2.067334908140701e-05
192392,192393,192392,384785,82.37558507919312,2.0639834017932536e-05
192593,192594,192593,385187,82.46506190299988,2.0606206651676476e-05
192793,192794,192793,385587,82.54411196708679,2.0572801486660452e-05
192993,192994,192993,385987,82.623281955719,2.053945099044336e-05
193193,193194,193193,386387,82.70281982421875,2.0506155067475658e-05
193393,193394,193393,386787,82.7836549282074,2.0472913622900712e-05
193594,193595,193594,387189,82.8673779964447,2.0439560763288755e-05
193794,193795,193794,387589,82.95098805427551,2.0406428262576952e-05
193994,193995,193994,387989,83.03341388702393,2.0373349956217545e-05
194194,194195,194194,388389,83.11208987236023,2.034032575001734e-05
194394,194395,194394,388789,83.19315481185913,2.030735555027573e-05
194595,194596,194595,389191,83.27531385421753,2.0274274816786687e-05
194795,194796,194795,389591,83.35463309288025,2.0241412617790692e-05
194995,194996,194995,389991,83.43343806266785,2.0208604144447255e-05
195195,195196,195195,390391,83.51981496810913,2.0175849303462362e-05
195395,195396,195395,390791,83.59795475006104,2.0143148002623625e-05
195596,195597,195596,391193,83.68014597892761,2.0110337043753115e-05
195796,195797,195796,391593,83.7615418434143,2.0077742811394474e-05
195996,195997,195996,391993,83.84008002281189,2.004520184155823e-05
196196,196197,196196,392393,83.92409801483154,2.0012714042127814e-05
196396,196397,196396,392793,84.01330304145813,1.9980279321454077e-05
196597,196598,196597,393195,84.11510515213013,1.9947735812606565e-05
196797,196798,196797,393595,84.19420099258423,1.991540723970521e-05
196997,196998,196997,393995,84.27405500411987,1.9883131471160428e-05
197197,197198,197197,394395,84.35312390327454,1.9850908416439607e-05
197397,197398,197397,394795,84.43261075019836,1.981873798463001e-05
197598,197599,197598,395197,84.51691603660583,1.9786459627906017e-05
197798,197799,197798,395597,84.59809112548828,1.975439443307053e-05
197998,197999,197998,395997,84.67818999290466,1.972238159024842e-05
198198,198199,198198,396397,84.75963807106018,1.9690421009510514e-05
198398,198399,198398,396797,84.84417009353638,1.9658512601123204e-05
198599,198600,198599,397199,84.92877507209778,1.9626497124947146e-05
198799,198800,198799,397599,85.0115659236908,1.959469305310981e-05
198999,199000,198999,397999,85.09134292602539,1.9562940885766075e-05
199199,199200,199199,398399,85.16927599906921,1.9531240534026683e-05
199399,199400,199399,398799,85.2428948879242,1.9499591909158424e-05
199600,199601,199600,399201,85.3191339969635,1.9467837067431413e-05
199800,199801,199800,399601,85.39420914649963,1.9436291888846276e-05
200000,200001,200000,400001,85.47471189498901,1.940479817205344e-05


==> extragradient/plot_data/bilinear_matrix_game_n250/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0022521018981933594,2.0175302852282635
27,140,140,280,0.11786293983459473,0.13386604132059543
53,324,324,648,0.23158597946166992,0.05239901804132782
80,524,524,1048,0.321026086807251,0.025483537201023237
106,722,722,1444,0.4019429683685303,0.014797314834664448
133,926,926,1852,0.4670898914337158,0.010422851966899497
159,1128,1128,2256,0.5397119522094727,0.00823981414556747
186,1334,1334,2668,0.6062941551208496,0.005949829350939559
212,1538,1538,3076,0.6630330085754395,0.004895687120914551
239,1748,1748,3496,0.7195460796356201,0.0039387324137672795
265,1948,1948,3896,0.7773702144622803,0.0031334824091006626
292,2150,2150,4300,0.8646221160888672,0.002151612155160017
318,2354,2354,4708,0.9531641006469727,0.0018311447514661934
345,2570,2570,5140,1.022481918334961,0.0018042080287622372
371,2778,2778,5556,1.1024482250213623,0.00179021331690119
398,2994,2994,5988,1.206083059310913,0.0017788398911990659
425,3210,3210,6420,1.2930150032043457,0.0017437804703963203
451,3412,3412,6824,1.371291160583496,0.0014807552790521632
478,3628,3628,7256,1.4577879905700684,0.0014119864217351996
504,3836,3836,7672,1.5337810516357422,0.0014024814049348523
531,4042,4042,8084,1.6428380012512207,0.001070835919770597
557,4244,4244,8488,1.7207098007202148,0.0008657670844045979
584,4456,4456,8912,1.7912940979003906,0.0007541440144498692
610,4664,4664,9328,1.8709361553192139,0.0007214237513235053
637,4878,4878,9756,1.964846134185791,0.0006679622953102352
663,5082,5082,10164,2.063000202178955,0.0005805290268225688
690,5298,5298,10596,2.2186429500579834,0.0005699182526091067
716,5506,5506,11012,2.3672990798950195,0.0005591325622961148
743,5720,5720,11440,2.6216681003570557,0.0005519075003482119
769,5926,5926,11852,2.7312090396881104,0.0004844202086686495
796,6140,6140,12280,2.821415901184082,0.0004508791766902869
822,6348,6348,12696,2.920520067214966,0.00043709173602084396
849,6550,6550,13100,3.0005390644073486,0.00030231464991499723
876,6766,6766,13532,3.066215991973877,0.00028836861154595797
902,6974,6974,13948,3.1498939990997314,0.00028429351895218924
929,7190,7190,14380,3.2088701725006104,0.0002812130174537038
955,7398,7398,14796,3.2707982063293457,0.00027728577118186153
982,7612,7612,15224,3.3387489318847656,0.00027441835396858287
1008,7812,7812,15624,3.4027981758117676,0.0002135443685586855
1035,8028,8028,16056,3.4842381477355957,0.00020930359686738954
1061,8236,8236,16472,3.6295440196990967,0.00020747106041227239
1088,8452,8452,16904,3.6934080123901367,0.00020601837043941735
1114,8660,8660,17320,3.746070146560669,0.0002048442213182238
1141,8870,8870,17740,3.7994518280029297,0.0001711968704143183
1167,9078,9078,18156,3.8500568866729736,0.00016787962445776085
1194,9294,9294,18588,3.9119009971618652,0.00016685197067492708
1220,9502,9502,19004,3.9665799140930176,0.00016608140305148398
1247,9718,9718,19436,4.0265491008758545,0.00016540632347586423
1274,9924,9924,19848,4.094965934753418,0.00015505071678485066
1300,10132,10132,20264,4.150645971298218,0.00015163264462378788
1327,10348,10348,20696,4.201340913772583,0.0001505610595880387
1353,10556,10556,21112,4.252288103103638,0.00014991846436712182
1380,10772,10772,21544,4.302511215209961,0.00014938322943022553
1406,10980,10980,21960,4.364464998245239,0.0001489416491123278
1433,11196,11196,22392,4.43955397605896,0.00014853780425029808
1459,11404,11404,22808,4.515912055969238,0.0001481893063254073
1486,11620,11620,23240,4.590045928955078,0.00014786032917005562
1512,11826,11826,23652,4.654447078704834,0.000141631966840428
1539,12042,12042,24084,4.753337144851685,0.00013795986233394698
1565,12250,12250,24500,4.890406847000122,0.00013662932758002464
1592,12466,12466,24932,5.016093969345093,0.00013583443566834609
1618,12674,12674,25348,5.083708047866821,0.00013530970582852612
1645,12890,12890,25780,5.151303052902222,0.00013490204202589863
1671,13098,13098,26196,5.254472017288208,0.0001345911142012028
1698,13312,13312,26624,5.361530065536499,0.00013279247106082716
1725,13526,13526,27052,5.45979118347168,0.0001214775156834342
1751,13734,13734,27468,5.518681049346924,0.00011860912868665622
1778,13950,13950,27900,5.5772950649261475,0.0001169647997291521
1804,14158,14158,28316,5.628485202789307,0.00011593111834342874
1831,14368,14368,28736,5.679145097732544,0.00011516660359808975
1857,14576,14576,29152,5.732731103897095,0.00011461444399115416
1884,14792,14792,29584,5.786726951599121,0.00011416722114314834
1910,15000,15000,30000,5.843304872512817,0.00011382098870405677
1937,15216,15216,30432,5.905013084411621,0.00011352414149890013
1963,15424,15424,30848,5.968358993530273,0.00011328275836235257
1990,15638,15638,31276,6.059362173080444,0.0001084823543773074
2016,15846,15846,31692,6.166356086730957,0.00010561959785485005
2043,16062,16062,32124,6.251826047897339,0.00010450006180903445
2069,16270,16270,32540,6.311590909957886,0.00010395809268762762
2096,16486,16486,32972,6.374425172805786,0.00010360430410391714
2123,16702,16702,33404,6.451365232467651,0.0001033515789537631
2149,16906,16906,33812,6.598901033401489,9.371785491371214e-05
2176,17122,17122,34244,6.707133054733276,9.068926478384993e-05
2202,17330,17330,34660,6.796364068984985,8.931322542185274e-05
2229,17546,17546,35092,6.867257118225098,8.848928190346306e-05
2255,17754,17754,35508,6.924974203109741,8.797005645963781e-05
2282,17970,17970,35940,7.000967979431152,8.758228905676102e-05
2308,18178,18178,36356,7.133243083953857,8.729446211838591e-05
2335,18394,18394,36788,7.213040113449097,8.705094863479934e-05
2361,18602,18602,37204,7.279374122619629,8.685171389426975e-05
2388,18816,18816,37632,7.350128889083862,8.499979333457976e-05
2414,19024,19024,38048,7.4133710861206055,8.241750845332826e-05
2441,19240,19240,38480,7.467947006225586,8.139918447999447e-05
2467,19448,19448,38896,7.524602174758911,8.085605297882907e-05
2494,19664,19664,39328,7.584980010986328,8.046589846610135e-05
2520,19872,19872,39744,7.650965929031372,8.017867258280167e-05
2547,20088,20088,40176,7.711814880371094,7.993825011628805e-05
2574,20302,20302,40604,7.777748107910156,7.830088300152179e-05
2600,20510,20510,41020,7.8478310108184814,7.532593076527558e-05
2627,20726,20726,41452,7.928389072418213,7.421244247688861e-05
2653,20934,20934,41868,7.99311900138855,7.3672105715229e-05
2680,21144,21144,42288,8.063168048858643,7.33175064950595e-05
2706,21352,21352,42704,8.125668048858643,7.307387538284401e-05
2733,21568,21568,43136,8.191911935806274,7.287968218194353e-05
2759,21776,21776,43552,8.249104976654053,7.27292381899256e-05
2786,21990,21990,43980,8.309134006500244,6.885302509422136e-05
2812,22198,22198,44396,8.369533061981201,6.765233804292725e-05
2839,22408,22408,44816,8.425894975662231,6.711511825580034e-05
2865,22616,22616,45232,8.489995002746582,6.681415240167379e-05
2892,22832,22832,45664,8.554644107818604,6.65996395543345e-05
2918,23034,23034,46068,8.60841703414917,6.644485180737433e-05
2945,23250,23250,46500,8.665284156799316,6.631702726622706e-05
2972,23466,23466,46932,8.722867012023926,6.621114171973429e-05
2998,23666,23666,47332,8.771969079971313,6.493623635808064e-05
3025,23882,23882,47764,8.82278823852539,6.167459296993791e-05
3051,24090,24090,48180,8.884504079818726,6.09284669044297e-05
3078,24306,24306,48612,8.948414087295532,6.0638890985231244e-05
3104,24514,24514,49028,9.007719039916992,6.048030200274136e-05
3131,24722,24722,49444,9.128625869750977,5.784700683514006e-05
3157,24930,24930,49860,9.20567512512207,5.6444100339231787e-05
3184,25146,25146,50292,9.278661251068115,5.59664365878355e-05
3210,25354,25354,50708,9.34933614730835,5.5725894259415703e-05
3237,25570,25570,51140,9.426176071166992,5.555623134898498e-05
3263,25778,25778,51556,9.489758968353271,5.5431253877137254e-05
3290,25994,25994,51988,9.560914039611816,5.5325091267556734e-05
3316,26196,26196,52392,9.623784065246582,5.523774797174259e-05
3343,26412,26412,52824,9.692344188690186,5.515769194501938e-05
3370,26622,26622,53244,9.768681049346924,5.5085423533469376e-05
3396,26824,26824,53648,9.817859172821045,4.77378914207915e-05
3423,27040,27040,54080,9.86974310874939,4.587565317309067e-05
3449,27248,27248,54496,9.920037269592285,4.481493991377205e-05
3476,27464,27464,54928,9.969804048538208,4.4087665282734094e-05
3502,27672,27672,55344,10.021512031555176,4.359386612887478e-05
3529,27888,27888,55776,10.073235988616943,4.32123476541333e-05
3555,28090,28090,56180,10.11982011795044,4.292730302694882e-05
3582,28304,28304,56608,10.169533014297485,4.188928992277808e-05
3608,28512,28512,57024,10.219257116317749,4.155762719988694e-05
3635,28728,28728,57456,10.27060604095459,4.132716867357425e-05
3661,28928,28928,57856,10.318481922149658,3.99200863214391e-05
3688,29144,29144,58288,10.373099088668823,3.883659594322249e-05
3714,29352,29352,58704,10.422804117202759,3.844886526348497e-05
3741,29568,29568,59136,10.474486112594604,3.823961130631038e-05
3767,29776,29776,59552,10.523056268692017,3.8109007228984274e-05
3794,29992,29992,59984,10.573950052261353,3.800889598681757e-05
3821,30208,30208,60416,10.62541913986206,3.792945648535132e-05
3847,30416,30416,60832,10.674789190292358,3.786523955975681e-05
3874,30632,30632,61264,10.726577997207642,3.7807064376290335e-05
3900,30840,30840,61680,10.781315088272095,3.775676618346048e-05
3927,31056,31056,62112,10.837064981460571,3.770879755003675e-05
3953,31264,31264,62528,10.885648250579834,3.766564847956498e-05
3980,31478,31478,62956,10.941834926605225,3.565839830206878e-05
4006,31686,31686,63372,10.991253137588501,3.490356320384085e-05
4033,31902,31902,63804,11.04212999343872,3.455567826805344e-05
4059,32110,32110,64220,11.090188026428223,3.437115130505264e-05
4086,32326,32326,64652,11.14206600189209,3.4248044691080096e-05
4112,32534,32534,65068,11.191554069519043,3.416417852874644e-05
4139,32748,32748,65496,11.242393016815186,3.2376515824540745e-05
4165,32956,32956,65912,11.29013991355896,3.173951492471495e-05
4192,33172,33172,66344,11.340918064117432,3.1520683885889836e-05
4219,33388,33388,66776,11.39651107788086,3.1414201525974064e-05
4245,33596,33596,67192,11.445641040802002,3.134651026886788e-05
4272,33812,33812,67624,11.495362997055054,3.129216955226211e-05
4298,34020,34020,68040,11.545071125030518,3.1248263894868376e-05
4325,34236,34236,68472,11.595269918441772,3.120805880591474e-05
4351,34444,34444,68888,11.6429922580719,3.117280971466993e-05
4378,34658,34658,69316,11.694154024124146,2.9362450330697884e-05
4404,34866,34866,69732,11.742655992507935,2.8933755483151436e-05
4431,35082,35082,70164,11.793884038925171,2.8748797062197033e-05
4457,35290,35290,70580,11.842998027801514,2.8647936584784465e-05
4484,35506,35506,71012,11.892839908599854,2.8576082075314087e-05
4510,35712,35712,71424,11.939726114273071,2.8568455042885183e-05
4537,35928,35928,71856,11.990597248077393,2.715819267937776e-05
4563,36136,36136,72272,12.038399934768677,2.670528045573686e-05
4590,36352,36352,72704,12.089936971664429,2.6473089793050608e-05
4616,36560,36560,73120,12.138375997543335,2.63387849570088e-05
4643,36776,36776,73552,12.196505069732666,2.6243867578324844e-05
4670,36992,36992,73984,12.24733591079712,2.6174070523914213e-05
4696,37200,37200,74400,12.300095081329346,2.6121169946479188e-05
4723,37416,37416,74832,12.35162901878357,2.607574838686311e-05
4749,37622,37622,75244,12.404536008834839,2.5574920831748935e-05
4776,37838,37838,75676,12.45529294013977,2.457924163327967e-05
4802,38046,38046,76092,12.509525060653687,2.4290358135247928e-05
4829,38262,38262,76524,12.561557054519653,2.4146412692876718e-05
4855,38470,38470,76940,12.613218069076538,2.4058879542196876e-05
4882,38680,38680,77360,12.664427042007446,2.399323040849407e-05
4908,38882,38882,77764,12.714942932128906,2.3944248149366882e-05
4935,39096,39096,78192,12.771934986114502,2.286871783005853e-05
4961,39304,39304,78608,12.824717044830322,2.2396852967113035e-05
4988,39520,39520,79040,12.886391162872314,2.2207487795219564e-05
5014,39728,39728,79456,12.93936800956726,2.211009749324525e-05
5041,39944,39944,79888,12.989595890045166,2.2043070382135523e-05
5068,40154,40154,80308,13.03895616531372,2.19930901749752e-05
5094,40362,40362,80724,13.088166236877441,2.1954199869933548e-05
5121,40578,40578,81156,13.137755155563354,2.1919912084014755e-05
5147,40786,40786,81572,13.192728042602539,2.1890896399747784e-05
5174,41000,41000,82000,13.243595123291016,2.113632699190753e-05
5200,41208,41208,82416,13.29367208480835,2.065579783253509e-05
5227,41424,41424,82848,13.344955205917358,2.0478518890918242e-05
5253,41632,41632,83264,13.395933866500854,2.0388961644178854e-05
5280,41848,41848,83696,13.447001218795776,2.0328052613951203e-05
5306,42056,42056,84112,13.496336936950684,2.0284809415658133e-05
5333,42272,42272,84544,13.547231912612915,2.024914636759447e-05
5359,42478,42478,84956,13.596578121185303,1.9164465123797088e-05
5386,42694,42694,85388,13.646286010742188,1.886180952885167e-05
5412,42902,42902,85804,13.694293022155762,1.8746056849765743e-05
5439,43118,43118,86236,13.746047019958496,1.8676226845042725e-05
5465,43320,43320,86640,13.798388957977295,1.8628755979689576e-05
5492,43536,43536,87072,13.848267078399658,1.8590259759957193e-05
5519,43752,43752,87504,13.904207229614258,1.8558483609209513e-05
5545,43960,43960,87920,13.953518152236938,1.8532081433165425e-05
5572,44174,44174,88348,14.003972053527832,1.767721978794513e-05
5598,44382,44382,88764,14.055486917495728,1.7389935439783714e-05
5625,44598,44598,89196,14.105928897857666,1.7276129137474404e-05
5651,44806,44806,89612,14.154624938964844,1.7213037357547875e-05
5678,45022,45022,90044,14.204571962356567,1.716696847020796e-05
5704,45228,45228,90456,14.253201961517334,1.6186359514089838e-05
5731,45444,45444,90888,14.303974866867065,1.5982886028568674e-05
5757,45652,45652,91304,14.352151155471802,1.589167484100302e-05
5784,45868,45868,91736,14.404288053512573,1.583112628223609e-05
5810,46076,46076,92152,14.452955961227417,1.5788194825316296e-05
5837,46292,46292,92584,14.50324296951294,1.5752546291371434e-05
5863,46500,46500,93000,14.552881002426147,1.5723608572896556e-05
5890,46716,46716,93432,14.602864265441895,1.5697301367058494e-05
5917,46932,46932,93864,14.652223110198975,1.567368645439576e-05
5943,47140,47140,94280,14.701200246810913,1.5652818882483105e-05
5970,47356,47356,94712,14.75200891494751,1.5632632524878597e-05
5996,47564,47564,95128,14.800342082977295,1.561432099992208e-05
6023,47778,47778,95556,14.851035833358765,1.4833382146013845e-05
6049,47986,47986,95972,14.904275894165039,1.4740859336284681e-05
6076,48202,48202,96404,14.962889909744263,1.4690054270272048e-05
6102,48410,48410,96820,15.023020029067993,1.4657230486153633e-05
6129,48626,48626,97252,15.078128814697266,1.4631399466933933e-05
6155,48834,48834,97668,15.129851818084717,1.4611021257114592e-05
6182,49050,49050,98100,15.185184955596924,1.4592725805484992e-05
6208,49256,49256,98512,15.238086938858032,1.385770588114784e-05
6235,49472,49472,98944,15.29203724861145,1.3573134293083075e-05
6261,49680,49680,99360,15.342271089553833,1.3476653544717966e-05
6288,49896,49896,99792,15.396870851516724,1.3422781397062628e-05
6315,50112,50112,100224,15.451764106750488,1.3386889368457435e-05
6341,50320,50320,100640,15.500114917755127,1.3360765867466923e-05
6368,50534,50534,101068,15.550987958908081,1.2698403827586001e-05
6394,50742,50742,101484,15.599744081497192,1.2521258501181357e-05
6421,50958,50958,101916,15.64988112449646,1.2450217423193459e-05
6447,51166,51166,102332,15.698907136917114,1.240840802423431e-05
6474,51382,51382,102764,15.749876976013184,1.2376396963969564e-05
6500,51590,51590,103180,15.798398971557617,1.2351684303538062e-05
6527,51806,51806,103612,15.848531007766724,1.2330029388741112e-05
6553,52014,52014,104028,15.901179075241089,1.231180578199364e-05
6580,52230,52230,104460,15.950672149658203,1.2294817618689408e-05
6606,52438,52438,104876,15.998822927474976,1.2279832288967316e-05
6633,52654,52654,105308,16.052660942077637,1.2265347795433905e-05
6659,52862,52862,105724,16.100779056549072,1.2252205896324105e-05
6686,53078,53078,106156,16.15157723426819,1.2239222188055422e-05
6712,53286,53286,106572,16.200420141220093,1.2227238107172625e-05
6739,53502,53502,107004,16.250648021697998,1.2215237525064696e-05
6766,53718,53718,107436,16.30125594139099,1.2203616917566838e-05
6792,53926,53926,107852,16.350656032562256,1.2192732465262935e-05
6819,54120,54120,108240,16.39771604537964,6.482293554408768e-06
6845,54314,54314,108628,16.44376802444458,3.3639300084132412e-06
6872,54518,54518,109036,16.49209713935852,2.270950508417078e-06
6898,54726,54726,109452,16.541006088256836,2.2116137144652923e-06
6925,54942,54942,109884,16.59039306640625,2.186084970010495e-06
6951,55150,55150,110300,16.64016318321228,2.168025181538764e-06
6978,55366,55366,110732,16.689915895462036,2.1524448853865892e-06
7004,55574,55574,111148,16.738728046417236,2.139294690385555e-06
7031,55790,55790,111580,16.789462089538574,2.1269952429169403e-06
7057,55998,55998,111996,16.836831092834473,2.1161749091863977e-06
7084,56214,56214,112428,16.89032816886902,2.1058222042766963e-06
7110,56414,56414,112828,16.94182300567627,1.98294391508423e-06
7137,56630,56630,113260,16.991131067276,1.9792618539584646e-06
7164,56846,56846,113692,17.047528982162476,1.9762809987192465e-06
7190,57046,57046,114092,17.10164713859558,1.9087559147450525e-06
7217,57262,57262,114524,17.15247893333435,1.8643889327961766e-06
7243,57470,57470,114940,17.201712131500244,1.8458751871396735e-06
7270,57686,57686,115372,17.252121210098267,1.8356146779659014e-06
7296,57894,57894,115788,17.301172018051147,1.8293256503856762e-06
7323,58110,58110,116220,17.35158920288086,1.8245883139306753e-06
7349,58318,58318,116636,17.402512073516846,1.8209902102157538e-06
7376,58534,58534,117068,17.452580213546753,1.817868278983619e-06
7402,58742,58742,117484,17.500495195388794,1.8152533241548102e-06
7429,58958,58958,117916,17.549904108047485,1.8128177782991241e-06
7455,59166,59166,118332,17.59753108024597,1.8106655668664043e-06
7482,59382,59382,118764,17.64752507209778,1.8085778966767408e-06
7508,59590,59590,119180,17.695736169815063,1.8066750183025746e-06
7535,59806,59806,119612,17.746268033981323,1.8047854498155256e-06
7561,60014,60014,120028,17.794738054275513,1.8030322804317549e-06
7588,60230,60230,120460,17.844583988189697,1.801267860115637e-06
7615,60446,60446,120892,17.896639108657837,1.7995511348484285e-06
7641,60654,60654,121308,17.944512128829956,1.7979363100339613e-06
7668,60870,60870,121740,17.995028972625732,1.7962938086400112e-06
7694,61078,61078,122156,18.04370903968811,1.7947413116437452e-06
7721,61270,61270,122540,18.089659214019775,9.801651153810561e-07
7747,61470,61470,122940,18.1358060836792,7.781729287710595e-07
7774,61686,61686,123372,18.186150074005127,7.503228693316351e-07
7800,61894,61894,123788,18.234426259994507,7.418855873121678e-07
7827,62110,62110,124220,18.284271240234375,7.365605839453741e-07
7853,62318,62318,124636,18.332539081573486,7.328164468601248e-07
7880,62534,62534,125068,18.38431215286255,7.29654143769554e-07
7906,62742,62742,125484,18.431912899017334,7.270154935204601e-07
7933,62958,62958,125916,18.48183012008667,7.245492044228381e-07
7959,63166,63166,126332,18.530248880386353,7.223636358777695e-07
7986,63382,63382,126764,18.580140113830566,7.20245787112376e-07
8013,63598,63598,127196,18.63086485862732,7.182543787362395e-07
8039,63806,63806,127612,18.67930507659912,7.164385431988053e-07
8066,64022,64022,128044,18.729897022247314,7.146456933932975e-07
8092,64230,64230,128460,18.777682065963745,7.129994931471628e-07
8119,64446,64446,128892,18.827536821365356,7.113657977680619e-07
8145,64654,64654,129308,18.87870502471924,7.098598008838166e-07
8172,64870,64870,129740,18.92972207069397,7.083604933061446e-07
8198,65076,65076,130152,18.97933006286621,6.756001307624728e-07
8225,65292,65292,130584,19.029873847961426,6.729801542818347e-07
8251,65500,65500,131000,19.079803228378296,6.714996219268264e-07
8278,65716,65716,131432,19.13465189933777,6.702772168642425e-07
8304,65924,65924,131848,19.19125199317932,6.692491455597113e-07
8331,66140,66140,132280,19.242733001708984,6.682719202926963e-07
8357,66348,66348,132696,19.290716886520386,6.673892975390276e-07
8384,66564,66564,133128,19.342061042785645,6.66517638233652e-07
8410,66772,66772,133544,19.3908851146698,6.657128630435071e-07
8437,66988,66988,133976,19.442065000534058,6.649072711239891e-07
8464,67204,67204,134408,19.49208402633667,6.641282907642649e-07
8490,67412,67412,134824,19.540704011917114,6.634004194547181e-07
8517,67628,67628,135256,19.59184217453003,6.626652972668231e-07
8543,67836,67836,135672,19.639536142349243,6.619755233032762e-07
8570,68052,68052,136104,19.689499139785767,6.612763863520846e-07
8596,68258,68258,136516,19.73823595046997,6.286452096010413e-07
8623,68474,68474,136948,19.78730010986328,6.251089808166837e-07
8649,68682,68682,137364,19.835302114486694,6.230268121186324e-07
8676,68898,68898,137796,19.889683961868286,6.215168058506068e-07
8702,69106,69106,138212,19.939322233200073,6.203976927035464e-07
8729,69322,69322,138644,19.989410161972046,6.194328866853801e-07
8755,69530,69530,139060,20.037353992462158,6.186206863532935e-07
8782,69746,69746,139492,20.08672523498535,6.178571688906542e-07
8808,69954,69954,139908,20.13473892211914,6.171764181573655e-07
8835,70170,70170,140340,20.184968948364258,6.165116706574259e-07
8862,70386,70386,140772,20.234918117523193,6.158803963944961e-07
8888,70594,70594,141188,20.281707048416138,6.152979172811688e-07
8915,70810,70810,141620,20.33037304878235,6.147147281486978e-07
8941,71018,71018,142036,20.378523111343384,6.141706301989394e-07
8968,71234,71234,142468,20.433488130569458,6.136209648111344e-07
8994,71442,71442,142884,20.488720178604126,6.1310430710107e-07
9021,71654,71654,143308,20.549326181411743,5.620021354457368e-07
9047,71848,71848,143696,20.60204315185547,3.723914763882819e-07
9074,72050,72050,144100,20.658984899520874,2.4833383964094253e-07
9100,72248,72248,144496,20.717812061309814,1.8466403470263716e-07
9127,72464,72464,144928,20.779590845108032,1.7420796618528976e-07
9153,72672,72672,145344,20.835480213165283,1.7292155133234222e-07
9180,72888,72888,145776,20.89610505104065,1.7207727437454413e-07
9206,73096,73096,146192,20.950842142105103,1.7140184167528777e-07
9233,73312,73312,146624,21.005342960357666,1.707717564810728e-07
9260,73528,73528,147056,21.059011220932007,1.701886737779958e-07
9286,73736,73736,147472,21.111257076263428,1.6966064848449172e-07
9313,73946,73946,147892,21.16248917579651,1.69141043085831e-07
9339,74152,74152,148304,21.217949867248535,1.5947512978053335e-07
9366,74368,74368,148736,21.27544403076172,1.5919279360662965e-07
9392,74576,74576,149152,21.324481964111328,1.5898597842920977e-07
9419,74792,74792,149584,21.37867283821106,1.5880803491966152e-07
9445,75000,75000,150000,21.430424213409424,1.5865685862431035e-07
9472,75216,75216,150432,21.482807159423828,1.585121223568774e-07
9498,75424,75424,150848,21.532416105270386,1.5837994682162644e-07
9525,75630,75630,151260,21.581794023513794,1.1965190799828172e-07
9551,75836,75836,151672,21.630789041519165,1.0592199434159446e-07
9578,76052,76052,152104,21.68128514289856,1.0449529241836949e-07
9604,76260,76260,152520,21.73021411895752,1.0354478427472251e-07
9631,76476,76476,152952,21.78104019165039,1.0276150971058099e-07
9657,76676,76676,153352,21.827311038970947,9.86717853306269e-08
9684,76892,76892,153784,21.877404928207397,9.780045947312819e-08
9711,77108,77108,154216,21.927419185638428,9.724207223556604e-08
9737,77316,77316,154632,21.977187156677246,9.68623231874329e-08
9764,77532,77532,155064,22.02715492248535,9.656059279363799e-08
9790,77740,77740,155480,22.075666904449463,9.632317302782461e-08
9817,77956,77956,155912,22.1256160736084,9.611076050759287e-08
9843,78164,78164,156328,22.17411994934082,9.59276015170029e-08
9870,78380,78380,156760,22.22452211380005,9.575243317811626e-08
9896,78588,78588,157176,22.272881984710693,9.559405765308704e-08
9923,78802,78802,157604,22.324765920639038,9.227767550154768e-08
9949,79010,79010,158020,22.38255214691162,9.200554586484151e-08
9976,79226,79226,158452,22.43379306793213,9.181538367428163e-08
10002,79434,79434,158868,22.482731103897095,9.166570102827042e-08
10029,79650,79650,159300,22.532649993896484,9.153007157506743e-08
10055,79858,79858,159716,22.581478118896484,9.14116503851238e-08
10082,80074,80074,160148,22.632692098617554,9.129713068686918e-08
10109,80290,80290,160580,22.68545627593994,9.118858925198865e-08
10135,80498,80498,160996,22.733687162399292,9.108811488150926e-08
10162,80712,80712,161424,22.789479970932007,8.667864439282008e-08
10188,80920,80920,161840,22.8406081199646,8.642929024252174e-08
10215,81136,81136,162272,22.89767813682556,8.629158749435724e-08
10241,81344,81344,162688,22.948019981384277,8.618882748105997e-08
10268,81560,81560,163120,22.998101949691772,8.609557781321453e-08
10294,81768,81768,163536,23.047685861587524,8.601268011064987e-08
10321,81984,81984,163968,23.098492860794067,8.593082352599343e-08
10347,82192,82192,164384,23.14786195755005,8.585461479682454e-08
10374,82408,82408,164816,23.200469970703125,8.577731566606505e-08
10400,82614,82614,165228,23.25110101699829,8.17988332361502e-08
10427,82830,82830,165660,23.305029153823853,8.157275877362854e-08
10453,83038,83038,166076,23.364810943603516,8.146733951408776e-08
10480,83254,83254,166508,23.419806957244873,8.137651748780843e-08
10506,83462,83462,166924,23.468239068984985,8.129732007146897e-08
10533,83678,83678,167356,23.518683195114136,8.122024007359589e-08
10560,83894,83894,167788,23.570927143096924,8.114670475157896e-08
10586,84100,84100,168200,23.62405300140381,7.833127836595647e-08
10613,84316,84316,168632,23.676099061965942,7.764364776059635e-08
10639,84524,84524,169048,23.725605249404907,7.745628663066036e-08
10666,84740,84740,169480,23.778044939041138,7.733738485397787e-08
10692,84948,84948,169896,23.831854104995728,7.724683071272162e-08
10719,85164,85164,170328,23.886877059936523,7.716440351294449e-08
10745,85372,85372,170744,23.935550928115845,7.709154477897092e-08
10772,85588,85588,171176,23.986334085464478,7.702030129864721e-08
10798,85796,85796,171592,24.03543496131897,7.695469488341327e-08
10825,86004,86004,172008,24.084764003753662,6.316672723335424e-08
10851,86212,86212,172424,24.134387016296387,5.813363702737362e-08
10878,86428,86428,172856,24.184941053390503,5.618370974052356e-08
10904,86636,86636,173272,24.23318910598755,5.518371329034335e-08
10931,86852,86852,173704,24.283013820648193,5.454329638168174e-08
10958,87068,87068,174136,24.332093000411987,5.4115837639667745e-08
10984,87276,87276,174552,24.383673191070557,5.3821811535306644e-08
11011,87492,87492,174984,24.44175910949707,5.3592728675997555e-08
11037,87700,87700,175400,24.491987943649292,5.342022788966661e-08
11064,87916,87916,175832,24.542477130889893,5.3274701286936864e-08
11090,88124,88124,176248,24.592432260513306,5.3157070179074445e-08
11117,88340,88340,176680,24.64319109916687,5.305152701628783e-08
11143,88548,88548,177096,24.692174196243286,5.296160751452458e-08
11170,88764,88764,177528,24.743088245391846,5.2877327217727946e-08
11196,88970,88970,177940,24.79142189025879,4.9783385491705415e-08
11223,89186,89186,178372,24.840841054916382,4.945330673917523e-08
11249,89394,89394,178788,24.890552043914795,4.9271480786476946e-08
11276,89610,89610,179220,24.940301179885864,4.914475998891065e-08
11302,89818,89818,179636,24.990463972091675,4.905379858482024e-08
11329,90034,90034,180068,25.040336847305298,4.897759757382978e-08
11355,90242,90242,180484,25.090471982955933,4.891505234113249e-08
11382,90458,90458,180916,25.14059591293335,4.885744841418883e-08
11409,90674,90674,181348,25.190388917922974,4.8804993642807103e-08
11435,90882,90882,181764,25.238043069839478,4.875796069146215e-08
11462,91096,91096,182192,25.288090229034424,4.575166839789606e-08
11488,91304,91304,182608,25.336988925933838,4.55688873928656e-08
11515,91520,91520,183040,25.39331889152527,4.5458319221530755e-08
11541,91728,91728,183456,25.450122117996216,4.538090126222209e-08
11568,91944,91944,183888,25.504317045211792,4.5316655701045794e-08
11594,92152,92152,184304,25.552917003631592,4.52641516814563e-08
11621,92368,92368,184736,25.603116989135742,4.521582090614254e-08
11647,92576,92576,185152,25.653565883636475,4.5173269128871444e-08
11674,92792,92792,185584,25.704499006271362,4.513192945893812e-08
11700,92998,92998,185996,25.753700017929077,4.163714744965339e-08
11727,93214,93214,186428,25.803696155548096,4.144332863243436e-08
11753,93422,93422,186844,25.851476907730103,4.134266753725041e-08
11780,93638,93638,187276,25.907927989959717,4.127226566162487e-08
11807,93854,93854,187708,25.958820104599,4.1217338384369516e-08
11833,94062,94062,188124,26.008170127868652,4.117186465101644e-08
11860,94278,94278,188556,26.058440923690796,4.1129090114746646e-08
11886,94486,94486,188972,26.106034994125366,4.109066062612021e-08
11913,94702,94702,189404,26.156266927719116,4.105273767226845e-08
11939,94910,94910,189820,26.204665184020996,4.1017621737603926e-08
11966,95126,95126,190252,26.2553391456604,4.098226375312266e-08
11992,95332,95332,190664,26.305809020996094,3.83847210881023e-08
12019,95548,95548,191096,26.362330198287964,3.8051233488664596e-08
12045,95756,95756,191512,26.416726112365723,3.791001716447089e-08
12072,95972,95972,191944,26.469808101654053,3.7829467808583773e-08
12098,96180,96180,192360,26.517718076705933,3.777775298966859e-08
12125,96396,96396,192792,26.569414854049683,3.7735703347069324e-08
12151,96604,96604,193208,26.62083888053894,3.770062140112706e-08
12178,96818,96818,193636,26.674744129180908,3.4902535742452574e-08
12205,97034,97034,194068,26.72801685333252,3.465925042674646e-08
12231,97242,97242,194484,26.77686309814453,3.454366353881045e-08
12258,97458,97458,194916,26.827497005462646,3.446773901955822e-08
12284,97666,97666,195332,26.876457929611206,3.441327483601478e-08
12311,97882,97882,195764,26.926454067230225,3.436641193091832e-08
12337,98090,98090,196180,26.975163221359253,3.432662959794648e-08
12364,98306,98306,196612,27.02936816215515,3.4288814981487295e-08
12390,98514,98514,197028,27.08163809776306,3.425470944099852e-08
12417,98730,98730,197460,27.146308183670044,3.422102724832726e-08
12443,98938,98938,197876,27.204560041427612,3.418986217681712e-08
12470,99154,99154,198308,27.261170864105225,3.4158532898019955e-08
12496,99362,99362,198724,27.314191102981567,3.412917072387689e-08
12523,99576,99576,199152,27.370328187942505,3.194309532705665e-08
12549,99784,99784,199568,27.42475700378418,3.1315165970127556e-08
12576,100000,100000,200000,27.4806489944458,3.1044566147961335e-08
12602,100208,100208,200416,27.543943881988525,3.090317425505134e-08
12629,100424,100424,200848,27.604400873184204,3.081174422222816e-08
12656,100640,100640,201280,27.6634361743927,3.074823991389183e-08
12682,100848,100848,201696,27.715656042099,3.070120081788147e-08
12709,101064,101064,202128,27.771205186843872,3.066082275194959e-08
12735,101272,101272,202544,27.823642253875732,3.062702181098593e-08
12762,101486,101486,202972,27.880073070526123,2.9307676128613264e-08
12788,101694,101694,203388,27.934751987457275,2.9096734719838536e-08
12815,101910,101910,203820,27.994017124176025,2.898005122135084e-08
12841,102118,102118,204236,28.047703981399536,2.8902928859335093e-08
12868,102334,102334,204668,28.103469133377075,2.8842142406016128e-08
12894,102542,102542,205084,28.155792236328125,2.8795023281197162e-08
12921,102758,102758,205516,28.20711922645569,2.8753917271565133e-08
12947,102966,102966,205932,28.273011922836304,2.8719556187250218e-08
12974,103182,103182,206364,28.357230186462402,2.86877131792045e-08
13000,103390,103390,206780,28.418761014938354,2.8659724584423115e-08
13027,103604,103604,207208,28.474779844284058,2.659026505587146e-08
13054,103820,103820,207640,28.53519105911255,2.636255937348481e-08
13080,104028,104028,208056,28.585851907730103,2.6256863352299592e-08
13107,104244,104244,208488,28.63621997833252,2.6190476352213853e-08
13133,104452,104452,208904,28.68430495262146,2.6144825070483548e-08
13160,104668,104668,209336,28.734463930130005,2.6107006968988892e-08
13186,104876,104876,209752,28.783596992492676,2.6075972671658692e-08
13213,105092,105092,210184,28.833627939224243,2.6047317571927962e-08
13239,105300,105300,210600,28.882442951202393,2.6022079397370064e-08
13266,105514,105514,211028,28.933040142059326,2.497332232133732e-08
13292,105722,105722,211444,28.981913089752197,2.4859480227465657e-08
13319,105938,105938,211876,29.032305002212524,2.4790877569155815e-08
13345,106146,106146,212292,29.080727100372314,2.4743813792967105e-08
13372,106362,106362,212724,29.130887985229492,2.470558568156012e-08
13398,106570,106570,213140,29.181886911392212,2.4675066808632903e-08
13425,106778,106778,213556,29.232605934143066,2.1045778916679627e-08
13451,106976,106976,213952,29.2795672416687,1.4553750854105837e-08
13478,107188,107188,214376,29.32932209968567,1.236392872331942e-08
13505,107404,107404,214808,29.383002042770386,1.2247491512100302e-08
13531,107612,107612,215224,29.431856870651245,1.2179613449260736e-08
13558,107828,107828,215656,29.482610940933228,1.2123073861701939e-08
13584,108036,108036,216072,29.537065982818604,1.2076613183021443e-08
13611,108252,108252,216504,29.5905442237854,1.2034137452234584e-08
13637,108460,108460,216920,29.645643949508667,1.1997461293452776e-08
13664,108676,108676,217352,29.6995689868927,1.196287106476073e-08
13690,108884,108884,217768,29.747686862945557,1.1932340287563358e-08
13717,109100,109100,218200,29.798168182373047,1.190306446652295e-08
13743,109308,109308,218616,29.847097158432007,1.1876880233006802e-08
13770,109524,109524,219048,29.897136211395264,1.18514976923426e-08
13796,109732,109732,219464,29.945804119110107,1.182858446365172e-08
13823,109948,109948,219896,29.996986150741577,1.180619397618999e-08
13849,110156,110156,220312,30.04659104347229,1.1785837205279528e-08
13876,110372,110372,220744,30.097466230392456,1.176581678821107e-08
13903,110588,110588,221176,30.146849155426025,1.1746821356667623e-08
13929,110796,110796,221592,30.19627022743225,1.172940310007071e-08
13956,111012,111012,222024,30.246073007583618,1.1712135716461398e-08
13982,111220,111220,222440,30.294625997543335,1.1696225662091161e-08
14009,111436,111436,222872,30.344796895980835,1.1680381510232621e-08
14035,111644,111644,223288,30.39616584777832,1.1665719284864168e-08
14062,111860,111860,223720,30.44754195213318,1.1651056692459972e-08
14088,112068,112068,224136,30.49672293663025,1.163743376032991e-08
14115,112284,112284,224568,30.54746389389038,1.1623758594755423e-08
14141,112492,112492,224984,30.59538197517395,1.1611006123656809e-08
14168,112708,112708,225416,30.645906925201416,1.159815956643294e-08
14194,112916,112916,225832,30.695049047470093,1.1586139538087852e-08
14221,113132,113132,226264,30.74705195426941,1.1573991347201891e-08
14247,113340,113340,226680,30.79545497894287,1.1562589571373698e-08
14274,113556,113556,227112,30.852461099624634,1.155103199665218e-08
14300,113762,113762,227524,30.90613293647766,1.0982508411257378e-08
14327,113978,113978,227956,30.959094047546387,1.090987165721981e-08
14354,114194,114194,228388,31.01079821586609,1.088336695132162e-08
14380,114402,114402,228804,31.05874514579773,1.0863512732264081e-08
14407,114618,114618,229236,31.108379125595093,1.0845882574431997e-08
14433,114826,114826,229652,31.158926010131836,1.0830851153903378e-08
14460,115042,115042,230084,31.21569514274597,1.0816724192029043e-08
14486,115250,115250,230500,31.26387310028076,1.080421660512175e-08
14513,115466,115466,230932,31.313596963882446,1.0792120988216546e-08
14539,115674,115674,231348,31.366277933120728,1.0781161809274484e-08
14566,115890,115890,231780,31.4201819896698,1.0770360356367054e-08
14592,116098,116098,232196,31.472080945968628,1.0760416493944473e-08
14619,116314,116314,232628,31.525202989578247,1.0750483415794483e-08
14645,116522,116522,233044,31.576033115386963,1.0741234573542822e-08
14672,116738,116738,233476,31.63325595855713,1.0731905754956147e-08
14698,116946,116946,233892,31.689652919769287,1.0723147314237343e-08
14725,117160,117160,234320,31.751626014709473,1.0374589811499138e-08
14752,117374,117374,234748,31.80627202987671,9.320273746872426e-09
14778,117582,117582,235164,31.85559606552124,9.260128457516207e-09
14805,117798,117798,235596,31.91099214553833,9.215131147704734e-09
14831,118006,118006,236012,31.96307611465454,9.181827817177534e-09
14858,118222,118222,236444,32.01792788505554,9.154425713617178e-09
14884,118430,118430,236860,32.0681049823761,9.133005829606647e-09
14911,118646,118646,237292,32.12005805969238,9.114513777369648e-09
14937,118854,118854,237708,32.18181920051575,9.099373503176047e-09
14964,119070,119070,238140,32.266319036483765,9.085705376534355e-09
14990,119278,119278,238556,32.32625699043274,9.074028506686815e-09
15017,119494,119494,238988,32.39094090461731,9.063064704379459e-09
15043,119702,119702,239404,32.447272062301636,9.053360651992557e-09
15070,119918,119918,239836,32.49844813346863,9.043962507617825e-09
15096,120126,120126,240252,32.54803800582886,9.03541975109878e-09
15123,120342,120342,240684,32.59802508354187,9.026959939626707e-09
15150,120558,120558,241116,32.6484010219574,9.018830723275011e-09
15176,120766,120766,241532,32.69691014289856,9.011251569502171e-09
15203,120982,120982,241964,32.747188091278076,9.003588985830203e-09
15229,121190,121190,242380,32.79479908943176,8.996374215236541e-09
15256,121404,121404,242808,32.84459710121155,8.715461560364205e-09
15282,121612,121612,243224,32.89502215385437,8.610825268513496e-09
15309,121828,121828,243656,32.94524598121643,8.59607336829992e-09
15335,122036,122036,244072,32.99638605117798,8.586479355359625e-09
15362,122252,122252,244504,33.054309129714966,8.577900022289505e-09
15388,122460,122460,244920,33.10907793045044,8.570296918568652e-09
15415,122676,122676,245352,33.16472911834717,8.562816165330635e-09
15441,122884,122884,245768,33.218985080718994,8.555884437056221e-09
15468,123100,123100,246200,33.279412031173706,8.548889867276195e-09
15494,123306,123306,246612,33.33303189277649,8.233370725752458e-09
15521,123522,123522,247044,33.38973808288574,8.211566194343423e-09
15547,123730,123730,247460,33.44302487373352,8.198681646946204e-09
15574,123946,123946,247892,33.494619846343994,8.188283438579382e-09
15601,124162,124162,248324,33.5453839302063,8.179475718755337e-09
15627,124370,124370,248740,33.59361791610718,8.17190438034602e-09
15654,124580,124580,249160,33.67481303215027,7.195085328884555e-09
15680,124784,124784,249568,33.73996901512146,5.925531959866341e-09
15707,125000,125000,250000,33.80896306037903,5.691676408991624e-09
15733,125208,125208,250416,33.874415159225464,5.5560109956803855e-09
15760,125424,125424,250848,33.930258989334106,5.4592591957152336e-09
15786,125632,125632,251264,33.98092317581177,5.391567091981272e-09
15813,125848,125848,251696,34.033231019973755,5.3385185938728485e-09
15839,126056,126056,252112,34.082342863082886,5.298886310054247e-09
15866,126272,126272,252544,34.13430094718933,5.266179172146452e-09
15892,126480,126480,252960,34.18434715270996,5.2406463343738636e-09
15919,126696,126696,253392,34.23627710342407,5.218754435385755e-09
15945,126904,126904,253808,34.28565311431885,5.201072979909106e-09
15972,127120,127120,254240,34.3376669883728,5.185443091330974e-09
15999,127336,127336,254672,34.393638134002686,5.171997311307352e-09
16025,127544,127544,255088,34.44420409202576,5.160689319570114e-09
16052,127760,127760,255520,34.493520975112915,5.1503127437608225e-09
16078,127968,127968,255936,34.54524326324463,5.1413886712758564e-09
16105,128184,128184,256368,34.60092115402222,5.133026363909419e-09
16131,128392,128392,256784,34.65673494338989,5.125691344672317e-09
16158,128608,128608,257216,34.71256184577942,5.118689537511902e-09
16184,128816,128816,257632,34.767301082611084,5.1124402862707104e-09
16211,129032,129032,258064,34.822365045547485,5.106377769025786e-09
16237,129240,129240,258480,34.87619090080261,5.1008850375156776e-09
16264,129456,129456,258912,34.93346619606018,5.095482561902372e-09
16290,129664,129664,259328,34.98952388763428,5.090525392073564e-09
16317,129880,129880,259760,35.048032999038696,5.08559331970645e-09
16343,130084,130084,260168,35.09870791435242,4.618778577597207e-09
16370,130300,130300,260600,35.149214029312134,4.554179139759402e-09
16396,130508,130508,261016,35.19755005836487,4.521653940727291e-09
16423,130724,130724,261448,35.24903607368469,4.497917475463576e-09
16450,130940,130940,261880,35.29940986633301,4.4799388424928055e-09
16476,131148,131148,262296,35.34702801704407,4.466201780216034e-09
16503,131364,131364,262728,35.40149188041687,4.454545987175855e-09
16529,131572,131572,263144,35.45062208175659,4.445156950781284e-09
16556,131788,131788,263576,35.591886043548584,4.436821940854117e-09
16582,131996,131996,263992,35.646016120910645,4.42982591298641e-09
16609,132212,132212,264424,35.70308804512024,4.42337660043316e-09
16635,132420,132420,264840,35.76995396614075,4.417773109351732e-09
16662,132636,132636,265272,35.8276801109314,4.4124441200368086e-09
16688,132844,132844,265688,35.88564109802246,4.407683415478625e-09
16715,133060,133060,266120,35.94725823402405,4.403044677890086e-09
16741,133268,133268,266536,36.00890898704529,4.398812521389773e-09
16768,133484,133484,266968,36.0633909702301,4.394613678109437e-09
16794,133692,133692,267384,36.11515402793884,4.390724021084872e-09
16821,133908,133908,267816,36.1669659614563,4.3868152453647095e-09
16848,134124,134124,268248,36.21695899963379,4.383015999669431e-09
16874,134332,134332,268664,36.26975417137146,4.379443491810952e-09
16901,134548,134548,269096,36.32217502593994,4.375808526586297e-09
16927,134756,134756,269512,36.374449014663696,4.372369220312512e-09
16954,134972,134972,269944,36.42697501182556,4.368851517729395e-09
16980,135180,135180,270360,36.479249000549316,4.365508707869389e-09
17007,135396,135396,270792,36.532305002212524,4.36207736293431e-09
17033,135604,135604,271208,36.58330702781677,4.358806734886172e-09
17060,135820,135820,271640,36.636688232421875,4.355440800389815e-09
17086,136022,136022,272044,36.68683218955994,3.9408908228585145e-09
17113,136236,136236,272472,36.73975706100464,3.3767703592315993e-09
17139,136444,136444,272888,36.79060506820679,3.3286268534980642e-09
17166,136660,136660,273320,36.842817068099976,3.294793623118673e-09
17192,136868,136868,273736,36.894779205322266,3.2693279413006996e-09
17219,137084,137084,274168,36.948055028915405,3.24788356801964e-09
17245,137292,137292,274584,36.99920415878296,3.2307504188389805e-09
17272,137508,137508,275016,37.05271291732788,3.215700319554067e-09
17299,137724,137724,275448,37.10410404205322,3.202792623548526e-09
17325,137932,137932,275864,37.15147590637207,3.191939876005199e-09
17352,138148,138148,276296,37.20134615898132,3.1819628701729116e-09
17378,138356,138356,276712,37.24997806549072,3.1733533191032393e-09
17405,138572,138572,277144,37.299586057662964,3.165250856427533e-09
17431,138780,138780,277560,37.34944701194763,3.158109884443869e-09
17458,138996,138996,277992,37.40211796760559,3.151261752483314e-09
17484,139204,139204,278408,37.45095205307007,3.1451252913683666e-09
17511,139420,139420,278840,37.50161623954773,3.1391535714073467e-09
17537,139628,139628,279256,37.54983305931091,3.1337332640965935e-09
17564,139844,139844,279688,37.59930491447449,3.128399474120118e-09
17590,140052,140052,280104,37.647162199020386,3.123510293729514e-09
17617,140268,140268,280536,37.697954177856445,3.118658431715808e-09
17643,140476,140476,280952,37.7463219165802,3.1141779322513166e-09
17670,140692,140692,281384,37.796600103378296,3.1097024640190265e-09
17697,140908,140908,281816,37.84666705131531,3.1053890385944543e-09
17723,141116,141116,282232,37.89457416534424,3.1013734504982132e-09
17750,141332,141332,282664,37.94523811340332,3.0973338166260963e-09
17776,141540,141540,283080,37.99736499786377,3.093558130701936e-09
17803,141756,141756,283512,38.05302405357361,3.089746298581286e-09
17829,141964,141964,283928,38.108344078063965,3.0861723338235445e-09
17856,142180,142180,284360,38.15922784805298,3.082553401273512e-09
17882,142388,142388,284776,38.20794701576233,3.079151361544254e-09
17909,142604,142604,285208,38.25897693634033,3.0756980568011367e-09
17935,142812,142812,285624,38.306660175323486,3.072444263803485e-09
17962,143028,143028,286056,38.35919523239136,3.069134768265108e-09
17988,143236,143236,286472,38.413970947265625,3.0660104697680355e-09
18015,143452,143452,286904,38.46690106391907,3.0628264067277634e-09
18041,143660,143660,287320,38.51557922363281,3.059815441631472e-09
18068,143876,143876,287752,38.566279888153076,3.0567421645807584e-09
18095,144092,144092,288184,38.61624717712402,3.0537202160345224e-09
18121,144300,144300,288600,38.66462802886963,3.0508558870224063e-09
18148,144516,144516,289032,38.71491503715515,3.047926053028114e-09
18174,144724,144724,289448,38.76386094093323,3.0451454077027916e-09
18201,144940,144940,289880,38.81441617012024,3.0422975550416937e-09
18227,145148,145148,290296,38.863539934158325,3.0395913072104352e-09
18254,145364,145364,290728,38.91473412513733,3.036816638105382e-09
18280,145572,145572,291144,38.96329712867737,3.0341770284884322e-09
18307,145788,145788,291576,39.01370286941528,3.0314679338448213e-09
18333,145994,145994,291988,39.062337160110474,2.754252837536229e-09
18360,146202,146202,292404,39.11026406288147,2.0385898557429877e-09
18386,146410,146410,292820,39.16187810897827,1.994119999287948e-09
18413,146626,146626,293252,39.21202611923218,1.9689333183023516e-09
18439,146834,146834,293668,39.26063513755798,1.94946048619299e-09
18466,147050,147050,294100,39.310267210006714,1.9320310663570594e-09
18492,147258,147258,294516,39.35938620567322,1.9172353792188698e-09
18519,147474,147474,294948,39.41061997413635,1.903546985391276e-09
18546,147690,147690,295380,39.461026191711426,1.8912952474175665e-09
18572,147898,147898,295796,39.50906801223755,1.880657267277363e-09
18599,148114,148114,296228,39.56003212928772,1.87064784046831e-09
18625,148322,148322,296644,39.60789394378662,1.8618766874425667e-09
18652,148538,148538,297076,39.65808320045471,1.8535526557777876e-09
18678,148746,148746,297492,39.70688199996948,1.8461984424988483e-09
18705,148962,148962,297924,39.75739502906799,1.8391645374626117e-09
18731,149170,149170,298340,39.805976152420044,1.8329036073810948e-09
18758,149386,149386,298772,39.85540294647217,1.8268727248974085e-09
18784,149594,149594,299188,39.90574502944946,1.8214680092133865e-09
18811,149810,149810,299620,39.95647597312927,1.816227898930003e-09
18837,150018,150018,300036,40.00419521331787,1.811502758740886e-09
18864,150234,150234,300468,40.05579900741577,1.8068944865605773e-09
18890,150442,150442,300884,40.11220622062683,1.8027157062273497e-09
18917,150658,150658,301316,40.16665697097778,1.798618323113457e-09
18944,150874,150874,301748,40.21639704704285,1.7947438998676322e-09
18970,151082,151082,302164,40.26375412940979,1.791203560375327e-09
18997,151298,151298,302596,40.31379508972168,1.787706818681249e-09
19023,151506,151506,303012,40.363829135894775,1.7844972644032896e-09
19050,151722,151722,303444,40.41533017158508,1.7813138038489333e-09
19076,151930,151930,303860,40.4635808467865,1.7783793946203e-09
19103,152146,152146,304292,40.51330900192261,1.7754569847436415e-09
19129,152354,152354,304708,40.56448006629944,1.7727529949171123e-09
19156,152570,152570,305140,40.61795711517334,1.7700502400856208e-09
19182,152778,152778,305556,40.67138886451721,1.7675404771983607e-09
19209,152994,152994,305988,40.72121286392212,1.7650234207386447e-09
19235,153202,153202,306404,40.769288063049316,1.7626784918939504e-09
19262,153418,153418,306836,40.81903409957886,1.760318991122382e-09
19288,153626,153626,307252,40.86920094490051,1.7581142619101856e-09
19315,153842,153842,307684,40.91988205909729,1.755889456913624e-09
19341,154050,154050,308100,40.968666076660156,1.7538050795431167e-09
19368,154266,154266,308532,41.01831603050232,1.7516958916735193e-09
19395,154482,154482,308964,41.068275928497314,1.749639227652956e-09
19421,154690,154690,309380,41.11373710632324,1.7477050430222987e-09
19448,154906,154906,309812,41.16303992271423,1.7457409079203432e-09
19474,155114,155114,310228,41.211714029312134,1.7438894927433297e-09
19501,155330,155330,310660,41.262624979019165,1.7420053845551068e-09
19527,155538,155538,311076,41.31103706359863,1.7402259108605262e-09
19554,155754,155754,311508,41.3635950088501,1.7384114851983098e-09
19580,155962,155962,311924,41.413496017456055,1.7366943934731455e-09
19607,156178,156178,312356,41.46401619911194,1.7349409196723484e-09
19633,156382,156382,312764,41.511337995529175,1.5271291634042704e-09
19660,156598,156598,313196,41.56156015396118,1.5107854313440196e-09
19686,156806,156806,313612,41.61032700538635,1.5063144709264903e-09
19713,157022,157022,314044,41.66008400917053,1.5023580174463173e-09
19739,157230,157230,314460,41.70968294143677,1.4989523914854085e-09
19766,157446,157446,314892,41.760266065597534,1.495739571395177e-09
19793,157662,157662,315324,41.80885910987854,1.4927953241883967e-09
19819,157870,157870,315740,41.85632300376892,1.4901728782336183e-09
19846,158086,158086,316172,41.906113147735596,1.4876374188690583e-09
19872,158294,158294,316588,41.953927993774414,1.48535196312125e-09
19899,158510,158510,317020,42.003265142440796,1.4831195738439229e-09
19925,158718,158718,317436,42.050785064697266,1.4810882622377115e-09
19952,158934,158934,317868,42.10026693344116,1.4790869402255657e-09
19978,159142,159142,318284,42.148316860198975,1.4772517546337678e-09
20005,159358,159358,318716,42.20439600944519,1.4754301305217451e-09
20031,159566,159566,319132,42.25797986984253,1.4737483298424897e-09
20058,159782,159782,319564,42.30746603012085,1.4720683691759985e-09
20084,159990,159990,319980,42.35733604431152,1.4705078418469971e-09
20111,160206,160206,320412,42.41067290306091,1.4689407973703804e-09
20137,160414,160414,320828,42.459264039993286,1.4674777571693796e-09
20164,160630,160630,321260,42.508147954940796,1.4660012941902235e-09
20190,160838,160838,321676,42.55618405342102,1.4646166261070144e-09
20217,161054,161054,322108,42.6059730052948,1.4632135678752492e-09
20244,161270,161270,322540,42.65536093711853,1.4618425866091364e-09
20270,161478,161478,322956,42.7034649848938,1.4605498275857863e-09
20297,161694,161694,323388,42.751118183135986,1.459232956523294e-09
20323,161902,161902,323804,42.799540996551514,1.4579876885932895e-09
20350,162118,162118,324236,42.849205017089844,1.4567156565489237e-09
20376,162326,162326,324652,42.89849591255188,1.455509666668491e-09
20403,162538,162538,325076,42.947962045669556,1.179102050742756e-09
20429,162746,162746,325492,42.99640512466431,1.1390709678442723e-09
20456,162962,162962,325924,43.04764795303345,1.1257066842355735e-09
20482,163170,163170,326340,43.095707178115845,1.1155812259139533e-09
20509,163386,163386,326772,43.14640998840332,1.1067823363195112e-09
20535,163594,163594,327188,43.1945641040802,1.099579377230038e-09
20562,163810,163810,327620,43.24473714828491,1.0931606629145279e-09
20588,164018,164018,328036,43.29170513153076,1.087818871216318e-09
20615,164234,164234,328468,43.34189224243164,1.0829922457087006e-09
20642,164450,164450,328900,43.395617961883545,1.0787757260483052e-09
20668,164658,164658,329316,43.44254803657532,1.0751966132634088e-09
20695,164874,164874,329748,43.491848945617676,1.071897836376734e-09
20721,165082,165082,330164,43.53982424736023,1.069060172424087e-09
20748,165298,165298,330596,43.59014916419983,1.0664094919796405e-09
20774,165506,165506,331012,43.63978815078735,1.0640979707329833e-09
20801,165722,165722,331444,43.688326835632324,1.0619089266474604e-09
20827,165930,165930,331860,43.73467493057251,1.0599741079869308e-09
20854,166146,166146,332292,43.78403997421265,1.058117451883689e-09
20880,166354,166354,332708,43.8307580947876,1.0564548056545894e-09
20907,166570,166570,333140,43.880250215530396,1.0548398821956905e-09
20933,166778,166778,333556,43.92948603630066,1.0533766202824056e-09
20960,166994,166994,333988,43.97951102256775,1.0519391929385193e-09
20986,167202,167202,334404,44.02803301811218,1.0506230640110168e-09
21013,167418,167418,334836,44.07764196395874,1.0493173293545792e-09
21040,167634,167634,335268,44.12799787521362,1.0480657591650542e-09
21066,167842,167842,335684,44.176109075546265,1.0469049775528515e-09
21093,168058,168058,336116,44.22671604156494,1.0457394618823047e-09
21119,168266,168266,336532,44.27908396720886,1.0446512508308197e-09
21146,168482,168482,336964,44.335633993148804,1.0435521564261377e-09
21172,168690,168690,337380,44.386996030807495,1.042519945284346e-09
21199,168906,168906,337812,44.437451124191284,1.041472344239033e-09
21225,169114,169114,338228,44.485151052474976,1.0404840467892877e-09
21252,169330,169330,338660,44.53593111038208,1.0394771214630908e-09
21278,169536,169536,339072,44.58394813537598,9.85951547272177e-10
21305,169752,169752,339504,44.63376212120056,9.806214212964366e-10
21331,169960,169960,339920,44.682072162628174,9.791686172317546e-10
21358,170176,170176,340352,44.73316311836243,9.779500594461906e-10
21384,170384,170384,340768,44.78151297569275,9.76897393553761e-10
21411,170600,170600,341200,44.83208918571472,9.758840346599972e-10
21437,170808,170808,341616,44.88229513168335,9.749646569216198e-10
21464,171024,171024,342048,44.93991804122925,9.740556010145501e-10
21491,171240,171240,342480,44.99752402305603,9.73183896046032e-10
21517,171448,171448,342896,45.04885506629944,9.723729775214853e-10
21544,171664,171664,343328,45.098711013793945,9.715550831735025e-10
21570,171872,171872,343744,45.14943528175354,9.707867863540409e-10
21597,172082,172082,344164,45.2012140750885,8.144034550928322e-10
21623,172274,172274,344548,45.25033402442932,4.91373409501672e-10
21650,172486,172486,344972,45.303022146224976,4.151602240871747e-10
21676,172694,172694,345388,45.36006712913513,4.089318433278169e-10
21703,172910,172910,345820,45.41794991493225,4.0424539430372127e-10
21729,173118,173118,346236,45.4698600769043,4.0051025587859924e-10
21756,173334,173334,346668,45.52254009246826,3.9716101279593727e-10
21782,173542,173542,347084,45.57394504547119,3.9429861477611267e-10
21809,173758,173758,347516,45.62411904335022,3.9160602463260497e-10
21835,173966,173966,347932,45.672693967819214,3.8922170833469605e-10
21862,174182,174182,348364,45.72289681434631,3.8691812204300453e-10
21889,174398,174398,348796,45.773431062698364,3.847578417165901e-10
21915,174606,174606,349212,45.82149291038513,3.8279057883641406e-10
21942,174822,174822,349644,45.87265992164612,3.808474253846863e-10
21968,175030,175030,350060,45.92610216140747,3.7905935832982983e-10
21995,175246,175246,350492,45.97993016242981,3.772780742340626e-10
22021,175454,175454,350908,46.0289421081543,3.756274153721434e-10
22048,175670,175670,351340,46.08059000968933,3.739729566793404e-10
22074,175878,175878,351756,46.13281202316284,3.7243241030792595e-10
22101,176094,176094,352188,46.201526165008545,3.708817024726051e-10
22127,176302,176302,352604,46.433205127716064,3.694322765200313e-10
22154,176518,176518,353036,46.5122811794281,3.679686797219304e-10
22180,176726,176726,353452,46.57299995422363,3.665967902204963e-10
22207,176942,176942,353884,46.634032249450684,3.6520840678293177e-10
22233,177150,177150,354300,46.688392877578735,3.6390427245535956e-10
22260,177366,177366,354732,46.742916107177734,3.62581831325577e-10
22286,177574,177574,355148,46.79462003707886,3.613375323508887e-10
22313,177790,177790,355580,46.85002112388611,3.600742922086493e-10
22340,178006,178006,356012,46.91052603721619,3.588385583389832e-10
22366,178214,178214,356428,46.96736216545105,3.57673780904062e-10
22393,178430,178430,356860,47.02373194694519,3.564891261163934e-10
22419,178638,178638,357276,47.08161401748657,3.553710791742343e-10
22446,178854,178854,357708,47.14038705825806,3.5423326766026594e-10
22472,179062,179062,358124,47.19464302062988,3.531585623849731e-10
22499,179278,179278,358556,47.250508069992065,3.520639728326588e-10
22525,179486,179486,358972,47.305821895599365,3.510296692180383e-10
22552,179702,179702,359404,47.36448788642883,3.499754408001583e-10
22578,179910,179910,359820,47.41852807998657,3.489786885579964e-10
22605,180126,180126,360252,47.47511291503906,3.479621882505795e-10
22631,180332,180332,360664,47.531249046325684,3.372985312260888e-10
22658,180548,180548,361096,47.58519506454468,3.349943576993715e-10
22684,180756,180756,361512,47.63615584373474,3.340261717232244e-10
22711,180972,180972,361944,47.68972206115723,3.331545820719997e-10
22738,181188,181188,362376,47.741945028305054,3.3233303359875036e-10
22764,181396,181396,362792,47.79337406158447,3.3157035223510595e-10
22791,181612,181612,363224,47.8465940952301,3.3080094617036596e-10
22817,181820,181820,363640,48.01314997673035,3.300783797116761e-10
22844,182036,182036,364072,48.10572385787964,3.293448168522896e-10
22870,182244,182244,364488,48.167989015579224,3.286532540158866e-10
22897,182460,182460,364920,48.224138021469116,3.2794961160922876e-10
22923,182668,182668,365336,48.27978301048279,3.2728451747842774e-10
22950,182884,182884,365768,48.337449073791504,3.2660672519701e-10
22976,183092,183092,366184,48.39833402633667,3.259654950650672e-10
23003,183308,183308,366616,48.46144199371338,3.2531099937784675e-10
23029,183516,183516,367032,48.53028702735901,3.2469142870405665e-10
23056,183732,183732,367464,48.5925509929657,3.240582797929899e-10
23082,183940,183940,367880,48.646435022354126,3.2345846325716325e-10
23109,184156,184156,368312,48.70228099822998,3.228452382641829e-10
23135,184364,184364,368728,48.75724005699158,3.2226393113846105e-10
23162,184580,184580,369160,48.8148980140686,3.216691830649567e-10
23189,184796,184796,369592,48.872533082962036,3.210835517590475e-10
23215,185004,185004,370008,48.95948791503906,3.2052789224622424e-10
23242,185220,185220,370440,49.04325819015503,3.1995905758328193e-10
23268,185428,185428,370856,49.10331392288208,3.1941904058920797e-10
23295,185644,185644,371288,49.159088134765625,3.1886624561335006e-10
23321,185852,185852,371704,49.21566414833069,3.183412055992943e-10
23348,186068,186068,372136,49.27568507194519,3.178034182194054e-10
23374,186276,186276,372552,49.32619595527649,3.1729240962248493e-10
23401,186490,186490,372980,49.3791720867157,3.0530152661866424e-10
23427,186698,186698,373396,49.428208112716675,3.026541214832442e-10
23454,186914,186914,373828,49.477944135665894,3.015588263408091e-10
23480,187122,187122,374244,49.52731800079346,3.0068046583234935e-10
23507,187338,187338,374676,49.57732820510864,2.99858525945102e-10
23533,187546,187546,375092,49.626708984375,2.9913065675582827e-10
23560,187762,187762,375524,49.676762104034424,2.984288771599595e-10
23587,187978,187978,375956,49.72454810142517,2.977730559748071e-10
23613,188186,188186,376372,49.77243208885193,2.971789807749287e-10
23640,188402,188402,376804,49.82179307937622,2.965954522969727e-10
23666,188610,188610,377220,49.87063026428223,2.960615318807665e-10
23693,188826,188826,377652,49.921021938323975,2.95532623334152e-10
23719,189034,189034,378068,49.96988105773926,2.950450356696166e-10
23746,189250,189250,378500,50.01989817619324,2.9455880112838426e-10
23772,189458,189458,378916,50.0680410861969,2.9410769399342475e-10
23799,189674,189674,379348,50.117936849594116,2.936551390984652e-10
23825,189882,189882,379764,50.16493105888367,2.9323287124275506e-10
23852,190098,190098,380196,50.213963985443115,2.9280733656749874e-10
23878,190306,190306,380612,50.261582136154175,2.9240884040700086e-10
23905,190522,190522,381044,50.31189513206482,2.920054985676106e-10
23931,190728,190728,381456,50.36308002471924,2.764757535985974e-10
23958,190944,190944,381888,50.424888134002686,2.75019409149424e-10
23985,191160,191160,382320,50.48118805885315,2.742673918304457e-10
24011,191368,191368,382736,50.53324913978577,2.736733691457546e-10
24038,191584,191584,383168,50.589115142822266,2.7313598421803856e-10
24064,191792,191792,383584,50.65294599533081,2.72675247316346e-10
24091,192008,192008,384016,50.7140531539917,2.72242663789203e-10
24117,192216,192216,384432,50.7633159160614,2.7186190157023346e-10
24144,192432,192432,384864,50.81506299972534,2.7149633099463814e-10
24170,192640,192640,385280,50.86906385421753,2.711683434603649e-10
24197,192856,192856,385712,50.92184090614319,2.7084816479115085e-10
24223,193064,193064,386128,50.974138259887695,2.705563842312856e-10
24250,193280,193280,386560,51.02688694000244,2.7026776109276255e-10
24276,193488,193488,386976,51.076475858688354,2.7000171108317374e-10
24303,193704,193704,387408,51.12950801849365,2.697355919207224e-10
24329,193910,193910,387820,51.1793270111084,2.51197061008475e-10
24356,194126,194126,388252,51.22966814041138,2.4948526649906596e-10
24382,194334,194334,388668,51.28073811531067,2.4856049268641e-10
24409,194550,194550,389100,51.329750061035156,2.478319107630578e-10
24436,194766,194766,389532,51.46214509010315,2.472559942439297e-10
24462,194974,194974,389948,51.557279109954834,2.4680272610039083e-10
24489,195190,195190,390380,51.62726187705994,2.464078164441183e-10
24515,195398,195398,390796,51.68726706504822,2.4608061948413327e-10
24542,195614,195614,391228,51.742311000823975,2.457816392280499e-10
24568,195822,195822,391644,51.79316210746765,2.455227221292621e-10
24595,196038,196038,392076,51.848499059677124,2.452761209437787e-10
24621,196246,196246,392492,51.91196322441101,2.450548226777264e-10
24648,196460,196460,392920,51.977618932724,2.3184524360877893e-10
24674,196668,196668,393336,52.03176712989807,2.3071528818318698e-10
24701,196884,196884,393768,52.08821511268616,2.3018514060955262e-10
24727,197092,197092,394184,52.145694971084595,2.297981789716863e-10
24754,197308,197308,394616,52.20365905761719,2.2947042395000194e-10
24780,197516,197516,395032,52.262699127197266,2.292018815455303e-10
24807,197732,197732,395464,52.3239848613739,2.2895626521423914e-10
24834,197948,197948,395896,52.38589596748352,2.287340467471147e-10
24860,198156,198156,396312,52.441981077194214,2.2853573522102568e-10
24887,198372,198372,396744,52.49801707267761,2.2834120983843012e-10
24913,198580,198580,397160,52.560901165008545,2.281620402062767e-10
24940,198788,198788,397576,52.62107706069946,1.8664037791155965e-10
24966,198994,198994,397988,52.67828416824341,1.6921718553620175e-10
24993,199210,199210,398420,52.746273040771484,1.6745932904801618e-10
25019,199418,199418,398836,52.80449104309082,1.6615345443744904e-10
25046,199634,199634,399268,52.861563205718994,1.6501616591359448e-10
25072,199842,199842,399684,52.917208194732666,1.6408808246868233e-10
25099,200058,200058,400116,52.97368025779724,1.6326450791424247e-10
25125,200266,200266,400532,53.02777695655823,1.6258164390160714e-10
25152,200482,200482,400964,53.08713698387146,1.6196647090713364e-10
25178,200690,200690,401380,53.13739490509033,1.614490443734176e-10
25205,200906,200906,401812,53.188210010528564,1.609760618625813e-10
25231,201114,201114,402228,53.23671007156372,1.6057249504759005e-10
25258,201330,201330,402660,53.28749704360962,1.60198429283347e-10
25285,201546,201546,403092,53.33724308013916,1.5986280665855122e-10
25311,201754,201754,403508,53.391940116882324,1.5957012248533634e-10
25338,201970,201970,403940,53.44289684295654,1.5929328771591507e-10
25364,202178,202178,404356,53.49325895309448,1.5904832705736028e-10
25391,202394,202394,404788,53.54532814025879,1.588132855664465e-10
25417,202602,202602,405204,53.594155073165894,1.5860284566900567e-10
25444,202818,202818,405636,53.64402413368225,1.5839806351008877e-10
25470,203026,203026,406052,53.692129135131836,1.5821261464190592e-10
25497,203242,203242,406484,53.74271583557129,1.5803028341640335e-10
25523,203450,203450,406900,53.79029202461243,1.578631701083756e-10
25550,203666,203666,407332,53.84007811546326,1.5769728480112235e-10
25576,203870,203870,407740,53.89224910736084,1.5245853057992653e-10
25603,204086,204086,408172,53.94326615333557,1.4092609366995786e-10
25629,204294,204294,408588,53.99314093589783,1.3979883411964305e-10
25656,204510,204510,409020,54.04377198219299,1.3902037013007854e-10
25683,204726,204726,409452,54.09384799003601,1.383980737874464e-10
25709,204934,204934,409868,54.14091897010803,1.378964560781229e-10
25736,205150,205150,410300,54.1910080909729,1.3745180089560851e-10
25762,205358,205358,410716,54.238534927368164,1.3708114222350224e-10
25789,205574,205574,411148,54.29546117782593,1.3674394292109498e-10
25815,205782,205782,411564,54.343636989593506,1.3645627157082882e-10
25842,205998,205998,411996,54.39477825164795,1.361889049236478e-10
25868,206206,206206,412412,54.44349122047424,1.3595599102728846e-10
25895,206422,206422,412844,54.49519896507263,1.3573536424741303e-10
25921,206628,206628,413256,54.542702198028564,1.31872879804505e-10
25948,206844,206844,413688,54.599608182907104,1.3111476100081764e-10
25974,207052,207052,414104,54.65060091018677,1.3084286963275665e-10
26001,207268,207268,414536,54.701329946517944,1.3063601127100293e-10
26027,207476,207476,414952,54.74926996231079,1.3047123891059795e-10
26054,207692,207692,415384,54.80565309524536,1.3032222727162313e-10
26080,207900,207900,415800,54.86499094963074,1.3019299785447032e-10
26107,208116,208116,416232,54.9215202331543,1.3006923690540625e-10
26134,208332,208332,416664,54.982614040374756,1.2995326136556266e-10
26160,208540,208540,417080,55.03372001647949,1.2984691878187716e-10
26187,208756,208756,417512,55.08434987068176,1.2974053495429668e-10
26213,208962,208962,417924,55.13338112831116,1.2352845442102827e-10
26240,209178,209178,418356,55.18900108337402,1.2302212162922477e-10
26266,209386,209386,418772,55.237189054489136,1.2282604295118663e-10
26293,209602,209602,419204,55.28784704208374,1.226691835073487e-10
26319,209810,209810,419620,55.33585524559021,1.2254077163732595e-10
26346,210026,210026,420052,55.387797117233276,1.2242140618741984e-10
26372,210234,210234,420468,55.43795418739319,1.2231523737579488e-10
26399,210450,210450,420900,55.49569606781006,1.2221100473591906e-10
26425,210658,210658,421316,55.546751976013184,1.221149796028102e-10
26452,210874,210874,421748,55.597557067871094,1.220184615135572e-10
26478,211082,211082,422164,55.64609408378601,1.2192764039242257e-10
26505,211288,211288,422576,55.69403910636902,9.941933474411593e-11


==> extragradient/plot_data/bilinear_matrix_game_n250/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0003790855407714844,2.0175302852282635
19,40,40,80,0.026957035064697266,0.3228983898673162
38,80,80,160,0.050685882568359375,0.1498185508703752
57,130,130,260,0.0745401382446289,0.07567792005333666
77,188,188,376,0.0974888801574707,0.047935423211501516
96,244,244,488,0.1203761100769043,0.03468826647884769
115,306,306,612,0.14422607421875,0.021315318614970064
134,362,362,724,0.16945195198059082,0.012393377357513611
153,422,422,844,0.1971898078918457,0.00904687651286605
172,488,488,976,0.22531986236572266,0.00790227561050279
191,552,552,1104,0.25109410285949707,0.006616396449975184
211,622,622,1244,0.28113317489624023,0.005758668913051867
230,696,696,1392,0.30570507049560547,0.0052543449605302476
249,770,770,1540,0.3308119773864746,0.004877799310625684
268,844,844,1688,0.356564998626709,0.004563773813828424
287,920,920,1840,0.381619930267334,0.004350350316512475
306,994,994,1988,0.40740299224853516,0.003920567854838844
325,1056,1056,2112,0.43190813064575195,0.0032199106975918123
344,1124,1124,2248,0.4560708999633789,0.00277529093157287
364,1188,1188,2376,0.4808781147003174,0.002247813917176663
383,1250,1250,2500,0.5061471462249756,0.0018446853257633592
402,1310,1310,2620,0.5354061126708984,0.0015033045682312609
421,1378,1378,2756,0.5662579536437988,0.0013371149219795504
440,1454,1454,2908,0.596473217010498,0.001275307295872697
459,1530,1530,3060,0.6321010589599609,0.0012343664472471046
478,1606,1606,3212,0.6614789962768555,0.0011965732408387435
498,1686,1686,3372,0.6949372291564941,0.0011281633539907418
517,1762,1762,3524,0.7263100147247314,0.001085102855492376
536,1838,1838,3676,0.7521259784698486,0.0010496653714075828
555,1906,1906,3812,0.7785861492156982,0.0009437854330096502
574,1974,1974,3948,0.8033668994903564,0.0008243170722245169
593,2050,2050,4100,0.8307540416717529,0.0007869330262073819
612,2124,2124,4248,0.8547570705413818,0.0007277305486597394
632,2204,2204,4408,0.8813331127166748,0.0006980571443961036
651,2280,2280,4560,0.9120020866394043,0.0006758961171027778
670,2356,2356,4712,0.9408042430877686,0.0006319804069390513
689,2424,2424,4848,0.9664700031280518,0.0005719965397465796
708,2498,2498,4996,0.9931230545043945,0.0005221820932372291
727,2574,2574,5148,1.0192110538482666,0.0004944556593075173
746,2650,2650,5300,1.0456230640411377,0.00047183985509187984
766,2730,2730,5460,1.0771620273590088,0.00044586596650082966
785,2806,2806,5612,1.1154282093048096,0.0004266742517845743
804,2882,2882,5764,1.1542441844940186,0.0004158061867951996
823,2958,2958,5916,1.1803710460662842,0.00040502523948225065
842,3034,3034,6068,1.2049989700317383,0.0003902062946982429
861,3110,3110,6220,1.229449987411499,0.0003798301666891546
880,3186,3186,6372,1.2550389766693115,0.00037213346826118614
899,3262,3262,6524,1.2804019451141357,0.0003616023883668246
919,3342,3342,6684,1.3086190223693848,0.00034995879904334656
938,3418,3418,6836,1.3338391780853271,0.00034359202544205367
957,3494,3494,6988,1.3584380149841309,0.0003362633431563166
976,3570,3570,7140,1.38466215133667,0.00032460583203786943
995,3646,3646,7292,1.4108669757843018,0.0003175934433178128
1014,3722,3722,7444,1.4354429244995117,0.0003132409457599409
1033,3798,3798,7596,1.4623780250549316,0.0003058335334654909
1053,3878,3878,7756,1.488158941268921,0.00029763316389054003
1072,3954,3954,7908,1.5122339725494385,0.0002929620516876683
1091,4030,4030,8060,1.5373451709747314,0.00028820108926604754
1110,4106,4106,8212,1.5630221366882324,0.0002824243588623943
1129,4182,4182,8364,1.5890181064605713,0.0002748999519585629
1148,4258,4258,8516,1.6145339012145996,0.00026629110443704684
1167,4334,4334,8668,1.639772891998291,0.0002577173337108483
1187,4414,4414,8828,1.6664190292358398,0.00025064183733689623
1206,4490,4490,8980,1.6908988952636719,0.0002442832836223381
1225,4566,4566,9132,1.7172322273254395,0.00024075221396476922
1244,4642,4642,9284,1.7433719635009766,0.0002382113555391448
1263,4718,4718,9436,1.7682318687438965,0.0002340770507126394
1282,4794,4794,9588,1.7925629615783691,0.0002299217961040375
1301,4870,4870,9740,1.817093849182129,0.00022694855707144438
1321,4950,4950,9900,1.8433499336242676,0.0002229478616984248
1340,5026,5026,10052,1.8678889274597168,0.00021624442529538077
1359,5102,5102,10204,1.894714117050171,0.00021017667813369816
1378,5178,5178,10356,1.9212191104888916,0.00020712358713058005
1397,5254,5254,10508,1.9479460716247559,0.0002039336518822789
1416,5330,5330,10660,1.9723079204559326,0.00020003928831681554
1435,5406,5406,10812,1.9978089332580566,0.0001968146653664996
1454,5482,5482,10964,2.0233700275421143,0.00019450209352442693
1474,5562,5562,11124,2.0520241260528564,0.0001915093835953259
1493,5638,5638,11276,2.0796642303466797,0.0001886627954276121
1512,5714,5714,11428,2.1064939498901367,0.0001867693905431896
1531,5790,5790,11580,2.131575107574463,0.00018435148693195903
1550,5866,5866,11732,2.156757116317749,0.00018102213408817945
1569,5942,5942,11884,2.1828019618988037,0.0001791548917834186
1588,6018,6018,12036,2.207545042037964,0.0001771828615709225
1608,6098,6098,12196,2.2339892387390137,0.00017382644742640097
1627,6174,6174,12348,2.2588090896606445,0.00017049842908553126
1646,6250,6250,12500,2.284738063812256,0.00016840930460057052
1665,6326,6326,12652,2.3118221759796143,0.0001660527419139597
1684,6402,6402,12804,2.3400540351867676,0.0001645412092055474
1703,6478,6478,12956,2.3681750297546387,0.00015896536239880964
1722,6554,6554,13108,2.3966519832611084,0.00015605039238803057
1742,6634,6634,13268,2.4287731647491455,0.0001513606131050411
1761,6710,6710,13420,2.4548869132995605,0.00014834515177159025
1780,6786,6786,13572,2.4814419746398926,0.000146467621824141
1799,6862,6862,13724,2.5074081420898438,0.00014509283641646513
1818,6938,6938,13876,2.5346081256866455,0.00014351646571388347
1837,7014,7014,14028,2.5647361278533936,0.000142128756557581
1856,7090,7090,14180,2.5928120613098145,0.00014071508702683344
1876,7170,7170,14340,2.620434045791626,0.00013911691550149983
1895,7246,7246,14492,2.646843910217285,0.00013793153627629149
1914,7322,7322,14644,2.6730899810791016,0.00013662023472092545
1933,7398,7398,14796,2.6989340782165527,0.00013496877550316365
1952,7474,7474,14948,2.7248129844665527,0.0001335604483672822
1971,7550,7550,15100,2.752716064453125,0.00013273541653023525
1990,7626,7626,15252,2.7784690856933594,0.00013132430460411642
2010,7706,7706,15412,2.805528163909912,0.000129257945327756
2029,7782,7782,15564,2.831674098968506,0.00012814285438100532
2048,7858,7858,15716,2.859205961227417,0.0001271577424605461
2067,7934,7934,15868,2.890321969985962,0.00012604024060895497
2086,8010,8010,16020,2.9204559326171875,0.0001243859699381058
2105,8086,8086,16172,2.9502971172332764,0.00012330640981205346
2124,8162,8162,16324,2.979663133621216,0.00012233795103569554
2143,8238,8238,16476,3.008358955383301,0.00012106127321824741
2163,8318,8318,16636,3.03757381439209,0.00012010498381069365
2182,8394,8394,16788,3.0647380352020264,0.0001192938040322467
2201,8470,8470,16940,3.092024087905884,0.00011831396432527017
2220,8546,8546,17092,3.118865966796875,0.00011586356343898263
2239,8622,8622,17244,3.149451971054077,0.00011351976544594829
2258,8698,8698,17396,3.1854000091552734,0.00011255385794139954
2277,8774,8774,17548,3.225482940673828,0.00011184627726385472
2297,8854,8854,17708,3.3193259239196777,0.00011086266829920093
2316,8930,8930,17860,3.347707986831665,0.00010963648056806331
2335,9006,9006,18012,3.3766069412231445,0.00010868888633007279
2354,9082,9082,18164,3.4061460494995117,0.00010715105335647734
2373,9158,9158,18316,3.439253091812134,0.00010561337277398657
2392,9234,9234,18468,3.468890905380249,0.00010403891235306137
2411,9310,9310,18620,3.498802900314331,0.00010261846495541443
2431,9390,9390,18780,3.5289950370788574,0.00010020972137794654
2450,9466,9466,18932,3.5609710216522217,9.786547645216975e-05
2469,9542,9542,19084,3.589478015899658,9.638504899789277e-05
2488,9618,9618,19236,3.616136074066162,9.56012120210361e-05
2507,9694,9694,19388,3.642595052719116,9.481236407775397e-05
2526,9770,9770,19540,3.669398069381714,9.383340913667569e-05
2545,9846,9846,19692,3.6958820819854736,9.296829058552138e-05
2565,9926,9926,19852,3.72444486618042,9.212571885911171e-05
2584,10002,10002,20004,3.752812147140503,9.128349320076944e-05
2603,10078,10078,20156,3.7814579010009766,9.055274668584026e-05
2622,10154,10154,20308,3.810621976852417,8.980703370628129e-05
2641,10230,10230,20460,3.842036008834839,8.891076954627032e-05
2660,10306,10306,20612,3.8751020431518555,8.811408259271204e-05
2679,10382,10382,20764,3.9101200103759766,8.755511650838224e-05
2698,10458,10458,20916,3.946599006652832,8.690116982072477e-05
2718,10538,10538,21076,3.987758159637451,8.582519026426493e-05
2737,10614,10614,21228,4.036738157272339,8.503863403446941e-05
2756,10690,10690,21380,4.0894951820373535,8.457992914014676e-05
2775,10766,10766,21532,4.145998001098633,8.356271687918801e-05
2794,10842,10842,21684,4.1949639320373535,8.135291665542812e-05
2813,10918,10918,21836,4.229257106781006,8.005579998767833e-05
2832,10994,10994,21988,4.268249034881592,7.952411845655962e-05
2852,11074,11074,22148,4.306529998779297,7.79474844626115e-05
2871,11150,11150,22300,4.341532945632935,7.643533687821026e-05
2890,11226,11226,22452,4.381439924240112,7.553307757988387e-05
2909,11302,11302,22604,4.425256967544556,7.488076913396961e-05
2928,11378,11378,22756,4.469105958938599,7.421578130876301e-05
2947,11454,11454,22908,4.5150909423828125,7.355911107631924e-05
2966,11530,11530,23060,4.558912992477417,7.288728433894157e-05
2986,11610,11610,23220,4.603184223175049,7.22609762145224e-05
3005,11686,11686,23372,4.645240068435669,7.161870269669543e-05
3024,11762,11762,23524,4.698071002960205,7.106684155981786e-05
3043,11838,11838,23676,4.7502851486206055,7.033588252684922e-05
3062,11914,11914,23828,4.791490077972412,6.937888236506033e-05
3081,11990,11990,23980,4.82598614692688,6.893494493967078e-05
3100,12066,12066,24132,4.856105089187622,6.804722355891129e-05
3120,12146,12146,24292,4.88659405708313,6.578440682041257e-05
3139,12222,12222,24444,4.916157960891724,6.307723235721876e-05
3158,12296,12296,24592,4.945683002471924,6.021205552201465e-05
3177,12372,12372,24744,4.9755470752716064,5.795120851422954e-05
3196,12448,12448,24896,5.0049920082092285,5.732128475736447e-05
3215,12524,12524,25048,5.034170150756836,5.590741606836574e-05
3234,12600,12600,25200,5.063931941986084,5.400223795973229e-05
3253,12676,12676,25352,5.093800067901611,5.165025904912568e-05
3273,12756,12756,25512,5.123060941696167,4.9570595262097536e-05
3292,12832,12832,25664,5.153572082519531,4.8194689693770004e-05
3311,12908,12908,25816,5.182197093963623,4.741321118979061e-05
3330,12984,12984,25968,5.2109949588775635,4.692610422824808e-05
3349,13060,13060,26120,5.242654085159302,4.644564256145297e-05
3368,13136,13136,26272,5.271162033081055,4.606318914889834e-05
3387,13212,13212,26424,5.299745082855225,4.5742581835810526e-05
3407,13292,13292,26584,5.3291709423065186,4.527591880127348e-05
3426,13368,13368,26736,5.361296892166138,4.488139912671564e-05
3445,13444,13444,26888,5.393439054489136,4.457390962479894e-05
3464,13520,13520,27040,5.424391984939575,4.423927000811646e-05
3483,13596,13596,27192,5.4509499073028564,4.375773407595282e-05
3502,13672,13672,27344,5.47686505317688,4.330183136405989e-05
3521,13748,13748,27496,5.503280878067017,4.302709776070579e-05
3541,13828,13828,27656,5.531553030014038,4.268599074368539e-05
3560,13904,13904,27808,5.558804035186768,4.229938237535625e-05
3579,13980,13980,27960,5.586022853851318,4.2006623713820904e-05
3598,14056,14056,28112,5.617470979690552,4.176970224883301e-05
3617,14132,14132,28264,5.651376247406006,4.141619672053851e-05
3636,14208,14208,28416,5.680170059204102,4.1084677141792353e-05
3655,14284,14284,28568,5.709174156188965,4.081822563690908e-05
3675,14364,14364,28728,5.751659154891968,4.047901297456077e-05
3694,14440,14440,28880,5.799084186553955,4.019118274025782e-05
3713,14516,14516,29032,5.841543912887573,3.9684358005713136e-05
3732,14592,14592,29184,5.879024982452393,3.879144950608753e-05
3751,14668,14668,29336,5.916637897491455,3.808316819036218e-05
3770,14744,14744,29488,5.955078840255737,3.757838963198868e-05
3789,14820,14820,29640,5.993396043777466,3.7022674368797836e-05
3808,14896,14896,29792,6.026766061782837,3.658984833942952e-05
3828,14976,14976,29952,6.06911301612854,3.627441390342288e-05
3847,15052,15052,30104,6.097218036651611,3.5952312007025993e-05
3866,15128,15128,30256,6.127371072769165,3.560526780103887e-05
3885,15204,15204,30408,6.1633570194244385,3.528676011310906e-05
3904,15280,15280,30560,6.194199085235596,3.499545593781946e-05
3923,15356,15356,30712,6.220769166946411,3.462461205094376e-05
3942,15432,15432,30864,6.248703956604004,3.4327965018842924e-05
3962,15512,15512,31024,6.278416872024536,3.4057005602285226e-05
3981,15588,15588,31176,6.306085824966431,3.3674403375194456e-05
4000,15664,15664,31328,6.334196090698242,3.319528994498697e-05
4019,15740,15740,31480,6.3617260456085205,3.292224144872073e-05
4038,15816,15816,31632,6.389644145965576,3.191643996136267e-05
4057,15892,15892,31784,6.417590141296387,3.0491031214857217e-05
4076,15968,15968,31936,6.484866142272949,2.9268930051656906e-05
4096,16048,16048,32096,6.519949197769165,2.882013242207161e-05
4115,16124,16124,32248,6.546706914901733,2.8581032195988534e-05
4134,16200,16200,32400,6.574974060058594,2.8268107550317493e-05
4153,16276,16276,32552,6.6014180183410645,2.7978660640506512e-05
4172,16352,16352,32704,6.62758207321167,2.7689649212646687e-05
4191,16428,16428,32856,6.653665065765381,2.7396542755456227e-05
4210,16504,16504,33008,6.682292938232422,2.712474391712649e-05
4230,16584,16584,33168,6.710263013839722,2.6877003112486187e-05
4249,16660,16660,33320,6.736721992492676,2.6636678750493646e-05
4268,16736,16736,33472,6.766211032867432,2.6365956948824394e-05
4287,16812,16812,33624,6.812191963195801,2.6166705001180993e-05
4306,16888,16888,33776,6.852997064590454,2.5919221553792704e-05
4325,16964,16964,33928,6.887853145599365,2.5541522428796416e-05
4344,17040,17040,34080,6.918400049209595,2.5379146186538e-05
4363,17116,17116,34232,6.947848081588745,2.4794957761500124e-05
4383,17196,17196,34392,6.978410959243774,2.3718837800267234e-05
4402,17270,17270,34540,7.006395101547241,2.2032440966393797e-05
4421,17332,17332,34664,7.0346879959106445,1.8882627820101763e-05
4440,17396,17396,34792,7.067112922668457,1.5774138095846622e-05
4459,17466,17466,34932,7.096421957015991,1.4623852273810803e-05
4478,17542,17542,35084,7.1235949993133545,1.4443365509139972e-05
4497,17618,17618,35236,7.150317192077637,1.4217279523931072e-05
4517,17698,17698,35396,7.178293943405151,1.39558276029802e-05
4536,17774,17774,35548,7.205086946487427,1.3787816119299687e-05
4555,17850,17850,35700,7.231328010559082,1.3635817303894182e-05
4574,17926,17926,35852,7.257399082183838,1.3418305818083003e-05
4593,18002,18002,36004,7.283522129058838,1.2933618636456774e-05
4612,18078,18078,36156,7.312929153442383,1.2678758115919515e-05
4631,18154,18154,36308,7.340739011764526,1.2487083240216316e-05
4651,18234,18234,36468,7.368335247039795,1.2371561556111374e-05
4670,18310,18310,36620,7.394979000091553,1.2172122804113603e-05
4689,18386,18386,36772,7.421003103256226,1.1795182363995153e-05
4708,18462,18462,36924,7.450648069381714,1.1585080779926392e-05
4727,18538,18538,37076,7.478063106536865,1.1428128858104445e-05
4746,18614,18614,37228,7.506853103637695,1.1205827103580563e-05
4765,18690,18690,37380,7.535181045532227,1.1030039059068808e-05
4785,18770,18770,37540,7.566465139389038,1.0867004863850638e-05
4804,18846,18846,37692,7.593012094497681,1.0711690929714693e-05
4823,18922,18922,37844,7.61938214302063,1.0524350147417501e-05
4842,18998,18998,37996,7.646093130111694,1.0233908031212052e-05
4861,19074,19074,38148,7.671919107437134,1.0029140664952466e-05
4880,19150,19150,38300,7.697947978973389,9.955455756736647e-06
4899,19226,19226,38452,7.72607421875,9.87731326430738e-06
4919,19306,19306,38612,7.755829095840454,9.767042139018196e-06
4938,19382,19382,38764,7.785372972488403,9.6691718152243e-06
4957,19458,19458,38916,7.814738035202026,9.562124346426962e-06
4976,19534,19534,39068,7.8462138175964355,9.480276981256454e-06
4995,19610,19610,39220,7.878848075866699,9.413521195767384e-06
5014,19686,19686,39372,7.911349058151245,9.317608318871124e-06
5033,19762,19762,39524,7.943127155303955,9.199527535808796e-06
5052,19838,19838,39676,7.972332000732422,9.131233783016483e-06
5072,19918,19918,39836,8.005044937133789,9.057482673364713e-06
5091,19994,19994,39988,8.036698818206787,8.911471537343377e-06
5110,20070,20070,40140,8.068739175796509,8.783893046852182e-06
5129,20146,20146,40292,8.097573041915894,8.732868946907649e-06
5148,20222,20222,40444,8.12598991394043,8.651224804525217e-06
5167,20298,20298,40596,8.15427303314209,8.534454089388488e-06
5186,20374,20374,40748,8.182738065719604,8.419684360601436e-06
5206,20454,20454,40908,8.216098070144653,8.35201198511418e-06
5225,20530,20530,41060,8.246889114379883,8.248815870551312e-06
5244,20606,20606,41212,8.27763295173645,8.138664822136965e-06
5263,20682,20682,41364,8.307248830795288,8.076509540604217e-06
5282,20758,20758,41516,8.337262153625488,8.001420659445664e-06
5301,20834,20834,41668,8.366353988647461,7.931461754421474e-06
5320,20910,20910,41820,8.395130157470703,7.850103710170154e-06
5340,20990,20990,41980,8.426184892654419,7.795291669885273e-06
5359,21066,21066,42132,8.455661058425903,7.734642487373119e-06
5378,21142,21142,42284,8.48528504371643,7.638071438165847e-06
5397,21218,21218,42436,8.51448917388916,7.583591776029057e-06
5416,21294,21294,42588,8.544440031051636,7.533178204119876e-06
5435,21370,21370,42740,8.573814153671265,7.490145543716813e-06
5454,21446,21446,42892,8.602313995361328,7.397027384516808e-06
5474,21526,21526,43052,8.631715059280396,7.246735189879488e-06
5493,21602,21602,43204,8.658172845840454,7.185079328607147e-06
5512,21678,21678,43356,8.684613227844238,7.109307967846526e-06
5531,21754,21754,43508,8.710710048675537,6.956408714921932e-06
5550,21830,21830,43660,8.737122058868408,6.7021809875714556e-06
5569,21906,21906,43812,8.763216257095337,6.317604564395027e-06
5588,21982,21982,43964,8.791587114334106,5.959115454395556e-06
5607,22058,22058,44116,8.818197011947632,5.693638047240866e-06
5627,22138,22138,44276,8.8454110622406,5.576854392857891e-06
5646,22214,22214,44428,8.871029138565063,5.5225787205363135e-06
5665,22290,22290,44580,8.89635705947876,5.481763998446739e-06
5684,22366,22366,44732,8.921659231185913,5.444859340701007e-06
5703,22442,22442,44884,8.94754409790039,5.402164237758666e-06
5722,22518,22518,45036,8.97198486328125,5.351635124742235e-06
5741,22594,22594,45188,8.997323989868164,5.301801599208546e-06
5761,22674,22674,45348,9.023997068405151,5.263026681270247e-06
5780,22750,22750,45500,9.05042314529419,5.221597769256241e-06
5799,22826,22826,45652,9.076350927352905,5.167609611285496e-06
5818,22902,22902,45804,9.101033926010132,5.132317022212822e-06
5837,22978,22978,45956,9.125395059585571,5.096642730999931e-06
5856,23054,23054,46108,9.150218963623047,5.037207850083691e-06
5875,23130,23130,46260,9.174800872802734,4.977997987051101e-06
5895,23210,23210,46420,9.20045018196106,4.9417707696311285e-06
5914,23286,23286,46572,9.224855184555054,4.905580382367852e-06
5933,23362,23362,46724,9.249639987945557,4.840735199854986e-06
5952,23438,23438,46876,9.274018049240112,4.7866609678381914e-06
5971,23514,23514,47028,9.298496007919312,4.755882592923055e-06
5990,23590,23590,47180,9.322615146636963,4.723709543582555e-06
6009,23666,23666,47332,9.347473859786987,4.67261982746689e-06
6029,23746,23746,47492,9.373452186584473,4.589726027762183e-06
6048,23822,23822,47644,9.397841930389404,4.543996124419403e-06
6067,23898,23898,47796,9.422840118408203,4.498670936917222e-06
6086,23974,23974,47948,9.448178052902222,4.439266949294305e-06
6105,24050,24050,48100,9.472994089126587,4.355922186869912e-06
6124,24126,24126,48252,9.49767804145813,4.283160033115196e-06
6143,24202,24202,48404,9.522348165512085,4.254599731543941e-06
6162,24278,24278,48556,9.550740003585815,4.221380838975599e-06
6182,24358,24358,48716,9.581774234771729,4.187034811156217e-06
6201,24434,24434,48868,9.61033296585083,4.011753799927059e-06
6220,24510,24510,49020,9.636044025421143,3.8055816356736127e-06
6239,24586,24586,49172,9.660312175750732,3.6771641326223698e-06
6258,24662,24662,49324,9.684700965881348,3.603485630677282e-06
6277,24738,24738,49476,9.70939016342163,3.526942985030453e-06
6296,24814,24814,49628,9.733482122421265,3.483765775429887e-06
6316,24894,24894,49788,9.758648157119751,3.453918498708187e-06
6335,24970,24970,49940,9.782518148422241,3.4118112868932765e-06
6354,25046,25046,50092,9.806745052337646,3.3842179509393666e-06
6373,25122,25122,50244,9.831516027450562,3.3599560762845403e-06
6392,25198,25198,50396,9.856032133102417,3.3319203279805948e-06
6411,25274,25274,50548,9.880819082260132,3.304103833517798e-06
6430,25350,25350,50700,9.904863119125366,3.241404276123197e-06
6450,25430,25430,50860,9.930340051651001,3.1517705515953465e-06
6469,25506,25506,51012,9.954345941543579,3.1268214608582474e-06
6488,25582,25582,51164,9.978240013122559,3.0919917200668193e-06
6507,25658,25658,51316,10.002202987670898,3.035157515303282e-06
6526,25734,25734,51468,10.026133060455322,2.9236935085843403e-06
6545,25810,25810,51620,10.051343202590942,2.8315219154830204e-06
6564,25886,25886,51772,10.08141803741455,2.7885504081731686e-06
6584,25966,25966,51932,10.107025861740112,2.7594825026002794e-06
6603,26042,26042,52084,10.1318359375,2.7342947650547863e-06
6622,26118,26118,52236,10.156451225280762,2.707066941993117e-06
6641,26194,26194,52388,10.181274175643921,2.665822075985095e-06
6660,26270,26270,52540,10.205770015716553,2.6407470912791272e-06
6679,26346,26346,52692,10.23079800605774,2.6220070212616786e-06
6698,26422,26422,52844,10.255729913711548,2.593138226963386e-06
6717,26498,26498,52996,10.280765056610107,2.569152620315324e-06
6737,26578,26578,53156,10.30739712715149,2.5500116604193708e-06
6756,26654,26654,53308,10.333456993103027,2.5276724732056612e-06
6775,26730,26730,53460,10.358617067337036,2.508272315734266e-06
6794,26806,26806,53612,10.383882999420166,2.4895636525010773e-06
6813,26882,26882,53764,10.408481121063232,2.470578191057554e-06
6832,26958,26958,53916,10.432662010192871,2.4520064853922513e-06
6851,27034,27034,54068,10.457028150558472,2.433916969986658e-06
6871,27114,27114,54228,10.483246088027954,2.4134602006838295e-06
6890,27190,27190,54380,10.50813913345337,2.362317917931276e-06
6909,27266,27266,54532,10.53307294845581,2.2949093412734173e-06
6928,27342,27342,54684,10.560023069381714,2.207313618484793e-06
6947,27418,27418,54836,10.585673093795776,2.1692325092001153e-06
6966,27494,27494,54988,10.610832929611206,2.1560010234056612e-06
6985,27570,27570,55140,10.636698246002197,2.1343048462727146e-06
7005,27650,27650,55300,10.662121057510376,2.1117182901250213e-06
7024,27726,27726,55452,10.687103033065796,2.077438273309809e-06
7043,27802,27802,55604,10.711971044540405,2.0158281541566885e-06
7062,27878,27878,55756,10.736912250518799,1.999632441443173e-06
7081,27954,27954,55908,10.76433515548706,1.981933422381867e-06
7100,28030,28030,56060,10.789093971252441,1.95445923682678e-06
7119,28106,28106,56212,10.813328981399536,1.935950674172215e-06
7139,28186,28186,56372,10.839141130447388,1.8935752595571038e-06
7158,28262,28262,56524,10.864253997802734,1.831519343380959e-06
7177,28338,28338,56676,10.88936710357666,1.7450026183774698e-06
7196,28414,28414,56828,10.913105964660645,1.6110154119972297e-06
7215,28490,28490,56980,10.937128067016602,1.5585673289733337e-06
7234,28566,28566,57132,10.960785865783691,1.5290605926164126e-06
7253,28642,28642,57284,10.985352993011475,1.5117507251575947e-06
7272,28718,28718,57436,11.009511947631836,1.500249720445125e-06
7292,28798,28798,57596,11.034367084503174,1.4779482119705333e-06
7311,28874,28874,57748,11.058810234069824,1.440333671925266e-06
7330,28950,28950,57900,11.083434104919434,1.4175347855775186e-06
7349,29026,29026,58052,11.10721206665039,1.4080680947557514e-06
7368,29102,29102,58204,11.131974935531616,1.3931998426297632e-06
7387,29178,29178,58356,11.155387163162231,1.3790529066834568e-06
7406,29254,29254,58508,11.179323196411133,1.368205270582583e-06
7426,29334,29334,58668,11.208964109420776,1.3552788545740731e-06
7445,29410,29410,58820,11.235111951828003,1.3423661905752576e-06
7464,29486,29486,58972,11.265936851501465,1.3333464719288878e-06
7483,29562,29562,59124,11.296030044555664,1.3157528319071315e-06
7502,29638,29638,59276,11.322327136993408,1.2897957035246862e-06
7521,29714,29714,59428,11.34875226020813,1.2740536580779728e-06
7540,29790,29790,59580,11.375422954559326,1.2530287573315032e-06
7560,29870,29870,59740,11.402992963790894,1.2050424514845937e-06
7579,29946,29946,59892,11.429331064224243,1.1778794734178375e-06
7598,30022,30022,60044,11.456024169921875,1.1676046174544041e-06
7617,30098,30098,60196,11.48409390449524,1.151347567282193e-06
7636,30174,30174,60348,11.509093046188354,1.1123234275409094e-06
7655,30250,30250,60500,11.534292936325073,1.0841338456171113e-06
7674,30326,30326,60652,11.560685157775879,1.0751897112760152e-06
7694,30406,30406,60812,11.588526010513306,1.0556826316110598e-06
7713,30482,30482,60964,11.615571975708008,1.0352007908785669e-06
7732,30558,30558,61116,11.645836114883423,1.0244207170074395e-06
7751,30634,30634,61268,11.674925088882446,1.0136184370027393e-06
7770,30710,30710,61420,11.70596718788147,9.973701546178073e-07
7789,30786,30786,61572,11.734520196914673,9.813954344970281e-07
7808,30862,30862,61724,11.760701894760132,9.726207871547228e-07
7827,30938,30938,61876,11.786956071853638,9.600410227689745e-07
7847,31018,31018,62036,11.81591510772705,9.434895835779149e-07
7866,31094,31094,62188,11.842435121536255,9.355706998631097e-07
7885,31170,31170,62340,11.86868405342102,9.274837619349303e-07
7904,31246,31246,62492,11.893836975097656,9.122220229543149e-07
7923,31322,31322,62644,11.91868281364441,8.940976588099979e-07
7942,31398,31398,62796,11.9441499710083,8.811070195231093e-07
7961,31474,31474,62948,11.9689199924469,8.718049136884984e-07
7981,31554,31554,63108,11.99581503868103,8.56215153610875e-07
8000,31630,31630,63260,12.022788047790527,8.260926986246417e-07
8019,31706,31706,63412,12.054189205169678,7.989490343047128e-07
8038,31782,31782,63564,12.082665920257568,7.862950556563411e-07
8057,31858,31858,63716,12.108533143997192,7.802668614680248e-07
8076,31934,31934,63868,12.133764028549194,7.710721036334104e-07
8095,32010,32010,64020,12.158136129379272,7.59329831878912e-07
8115,32090,32090,64180,12.182712078094482,7.524358267928398e-07
8134,32166,32166,64332,12.207520961761475,7.43355612549941e-07
8153,32242,32242,64484,12.232397079467773,7.212732013206015e-07
8172,32318,32318,64636,12.257026195526123,7.03799256084607e-07
8191,32394,32394,64788,12.281772136688232,6.939583780735346e-07
8210,32470,32470,64940,12.306210041046143,6.825770338642899e-07
8229,32546,32546,65092,12.33043098449707,6.602711568446025e-07
8249,32626,32626,65252,12.358731985092163,6.209605318886539e-07
8268,32702,32702,65404,12.385037183761597,6.080455307022952e-07
8287,32778,32778,65556,12.410980224609375,6.027204149838272e-07
8306,32854,32854,65708,12.436062097549438,5.97625470141118e-07
8325,32930,32930,65860,12.461453199386597,5.913449063784614e-07
8344,33006,33006,66012,12.485249996185303,5.847655762485115e-07
8363,33082,33082,66164,12.509046077728271,5.793653526715182e-07
8383,33162,33162,66324,12.534357070922852,5.741525244382481e-07
8402,33238,33238,66476,12.561439990997314,5.69965893918156e-07
8421,33314,33314,66628,12.611098051071167,5.651154677480464e-07
8440,33390,33390,66780,12.766846895217896,5.598689013297229e-07
8459,33466,33466,66932,12.809402227401733,5.559138992655764e-07
8478,33542,33542,67084,12.846740007400513,5.516813107003708e-07
8497,33618,33618,67236,12.879951238632202,5.453449050040802e-07
8516,33694,33694,67388,12.923732995986938,5.411422034416186e-07
8536,33774,33774,67548,12.962069988250732,5.376564890975951e-07
8555,33850,33850,67700,12.997495174407959,5.302425697114291e-07
8574,33926,33926,67852,13.026316165924072,5.174899715505873e-07
8593,34002,34002,68004,13.054663896560669,5.099102581790435e-07
8612,34078,34078,68156,13.084453105926514,5.06574691094215e-07
8631,34154,34154,68308,13.11216115951538,5.018648040399332e-07
8650,34230,34230,68460,13.13844108581543,4.974503536995299e-07
8670,34310,34310,68620,13.167108058929443,4.935036004837861e-07
8689,34386,34386,68772,13.195137023925781,4.881754228071711e-07
8708,34462,34462,68924,13.222979068756104,4.7451310661866373e-07
8727,34538,34538,69076,13.25071096420288,4.6783534847266625e-07
8746,34614,34614,69228,13.276937007904053,4.6287318352817366e-07
8765,34690,34690,69380,13.300904989242554,4.55750170739361e-07
8784,34766,34766,69532,13.326061010360718,4.5302208268773146e-07
8804,34846,34846,69692,13.352832078933716,4.4711290781700213e-07
8823,34922,34922,69844,13.37833023071289,4.3429766642223075e-07
8842,34998,34998,69996,13.403923988342285,4.1611046082325325e-07
8861,35074,35074,70148,13.431636095046997,3.9741735258566415e-07
8880,35150,35150,70300,13.458368062973022,3.9194543150725093e-07
8899,35226,35226,70452,13.48373818397522,3.889991449630418e-07
8918,35302,35302,70604,13.509011030197144,3.785311884956437e-07
8938,35382,35382,70764,13.535524129867554,3.6378378745650414e-07
8957,35458,35458,70916,13.568986177444458,3.5123649034412205e-07
8976,35534,35534,71068,13.605443000793457,3.447947189620574e-07
8995,35610,35610,71220,13.692230939865112,3.4061186525849e-07
9014,35686,35686,71372,13.72465205192566,3.375161045442387e-07
9033,35762,35762,71524,13.752233028411865,3.346435269070403e-07
9052,35838,35838,71676,13.778929948806763,3.3175799537398096e-07
9071,35914,35914,71828,13.805958986282349,3.292196894357558e-07
9091,35994,35994,71988,13.831500053405762,3.265503667055457e-07
9110,36070,36070,72140,13.85689401626587,3.2389345647333023e-07
9129,36146,36146,72292,13.884162187576294,3.205981632226604e-07
9148,36222,36222,72444,13.912928104400635,3.179494506344113e-07
9167,36298,36298,72596,13.941829204559326,3.1573575429152433e-07
9186,36374,36374,72748,13.968487024307251,3.1213442619960426e-07
9205,36450,36450,72900,13.994053840637207,3.093915023410332e-07
9225,36530,36530,73060,14.022724151611328,3.0740607341750224e-07
9244,36606,36606,73212,14.050166130065918,3.0483754452877795e-07
9263,36682,36682,73364,14.077791929244995,3.0237868666657844e-07
9282,36758,36758,73516,14.102512836456299,3.00303660443521e-07
9301,36834,36834,73668,14.130005121231079,2.981581620705105e-07
9320,36910,36910,73820,14.15619707107544,2.9548313926399296e-07
9339,36986,36986,73972,14.181957960128784,2.929178950361286e-07
9359,37066,37066,74132,14.209655046463013,2.9067845831274635e-07
9378,37142,37142,74284,14.235656023025513,2.88347557575493e-07
9397,37218,37218,74436,14.262666940689087,2.8607971378914433e-07
9416,37294,37294,74588,14.291990041732788,2.8396924080150304e-07
9435,37370,37370,74740,14.319348096847534,2.821087068396243e-07
9454,37446,37446,74892,14.349593162536621,2.7985492532826463e-07
9473,37522,37522,75044,14.378445148468018,2.779958466811596e-07
9493,37602,37602,75204,14.40720510482788,2.755694139110002e-07
9512,37678,37678,75356,14.432760000228882,2.7243764552870145e-07
9531,37754,37754,75508,14.459985971450806,2.705532798123168e-07
9550,37830,37830,75660,14.48703408241272,2.683375913377821e-07
9569,37906,37906,75812,14.514256954193115,2.652100968778569e-07
9588,37982,37982,75964,14.54234504699707,2.6093421602270614e-07
9607,38058,38058,76116,14.575109243392944,2.568822990932386e-07
9626,38134,38134,76268,14.60202693939209,2.5430118976032596e-07
9646,38214,38214,76428,14.631672143936157,2.499206723462347e-07
9665,38290,38290,76580,14.662761926651001,2.477328396629314e-07
9684,38366,38366,76732,14.690956115722656,2.447502672990802e-07
9703,38442,38442,76884,14.716705083847046,2.4057305458779137e-07
9722,38518,38518,77036,14.743281841278076,2.3643615699498853e-07
9741,38594,38594,77188,14.768900156021118,2.3381307774859543e-07
9760,38670,38670,77340,14.796441078186035,2.32033568111576e-07
9780,38750,38750,77500,14.82541012763977,2.3011507673275918e-07
9799,38826,38826,77652,14.855026006698608,2.2835015234850787e-07
9818,38902,38902,77804,14.890378952026367,2.2457544676555165e-07
9837,38978,38978,77956,14.93654203414917,2.2223952001638764e-07
9856,39054,39054,78108,15.052608966827393,2.2047633931829834e-07
9875,39130,39130,78260,15.096871852874756,2.171301512132511e-07
9894,39206,39206,78412,15.131529092788696,2.1314495527086599e-07
9914,39286,39286,78572,15.165858030319214,2.0582183418004533e-07
9933,39362,39362,78724,15.199959993362427,2.0334770718352096e-07
9952,39438,39438,78876,15.22857403755188,2.0037930564110314e-07
9971,39514,39514,79028,15.25667405128479,1.9554135210614035e-07
9990,39590,39590,79180,15.284349918365479,1.903937399746747e-07
10009,39666,39666,79332,15.311885118484497,1.8714323745317418e-07
10028,39742,39742,79484,15.339740991592407,1.8543294327779848e-07
10048,39822,39822,79644,15.367172241210938,1.834821960125647e-07
10067,39898,39898,79796,15.393383979797363,1.8146789663677985e-07
10086,39974,39974,79948,15.418936014175415,1.798810029473968e-07
10105,40050,40050,80100,15.447163105010986,1.783224731646988e-07
10124,40126,40126,80252,15.474684953689575,1.765459484861123e-07
10143,40202,40202,80404,15.50234603881836,1.7527730147138863e-07
10162,40278,40278,80556,15.529587984085083,1.7400996434055474e-07
10181,40354,40354,80708,15.55888319015503,1.7193746932483943e-07
10201,40434,40434,80868,15.586235284805298,1.703124938203353e-07
10220,40510,40510,81020,15.612246990203857,1.6922004922507634e-07
10239,40586,40586,81172,15.638092041015625,1.6716758895756044e-07
10258,40662,40662,81324,15.663267135620117,1.6541146231430715e-07
10277,40738,40738,81476,15.689232110977173,1.6433640565858102e-07
10296,40814,40814,81628,15.714364051818848,1.626092871699249e-07
10315,40890,40890,81780,15.740207195281982,1.6156809542811833e-07
10335,40970,40970,81940,15.766525030136108,1.5932896225627154e-07
10354,41046,41046,82092,15.792968034744263,1.5602263087513647e-07
10373,41122,41122,82244,15.822848081588745,1.5036045595095985e-07
10392,41198,41198,82396,15.851722002029419,1.490616425297635e-07
10411,41274,41274,82548,15.879408121109009,1.467604041308098e-07
10430,41350,41350,82700,15.907189130783081,1.452898381852695e-07
10449,41426,41426,82852,15.935664892196655,1.4248040571390264e-07
10469,41506,41506,83012,15.96613097190857,1.3906813821127356e-07
10488,41582,41582,83164,15.993690967559814,1.3734712334356317e-07
10507,41658,41658,83316,16.0206139087677,1.3643125585341458e-07
10526,41734,41734,83468,16.047213077545166,1.353919987452578e-07
10545,41810,41810,83620,16.072776079177856,1.342552438397828e-07
10564,41886,41886,83772,16.097162008285522,1.333793980341655e-07
10583,41962,41962,83924,16.121732234954834,1.3248853645048653e-07
10603,42042,42042,84084,16.14785408973694,1.3136770745709364e-07
10622,42118,42118,84236,16.174192905426025,1.3078583677589325e-07
10641,42194,42194,84388,16.203289031982422,1.294836779665041e-07
10660,42270,42270,84540,16.23114800453186,1.2765406813883796e-07
10679,42346,42346,84692,16.256903886795044,1.2661200773217276e-07
10698,42422,42422,84844,16.28210997581482,1.2451857269641833e-07
10717,42498,42498,84996,16.30671000480652,1.228787309051713e-07
10736,42574,42574,85148,16.331077098846436,1.1941211370582445e-07
10756,42654,42654,85308,16.35714626312256,1.1539681273720418e-07
10775,42730,42730,85460,16.38165807723999,1.1319466207637223e-07
10794,42806,42806,85612,16.405846118927002,1.1206918815042183e-07
10813,42882,42882,85764,16.432907104492188,1.1116315576231877e-07
10832,42958,42958,85916,16.457698106765747,1.1007449486322114e-07
10851,43034,43034,86068,16.48449683189392,1.0863532497829951e-07
10870,43110,43110,86220,16.51062822341919,1.0710833728671388e-07
10890,43190,43190,86380,16.537646055221558,1.0636661997475458e-07
10909,43266,43266,86532,16.566116094589233,1.04378423078976e-07
10928,43342,43342,86684,16.594385862350464,1.0230941643384394e-07
10947,43418,43418,86836,16.619384050369263,1.0077586975164321e-07
10966,43494,43494,86988,16.644987106323242,9.922996548361543e-08
10985,43570,43570,87140,16.670547008514404,9.80504474497917e-08
11004,43646,43646,87292,16.69814705848694,9.639680917186724e-08
11024,43726,43726,87452,16.725208044052124,9.525863962656455e-08
11043,43802,43802,87604,16.750366926193237,9.437903930934381e-08
11062,43878,43878,87756,16.77602195739746,9.152921853629519e-08
11081,43954,43954,87908,16.801659107208252,8.613133070435472e-08
11100,44030,44030,88060,16.827577114105225,8.28887606167079e-08
11119,44106,44106,88212,16.85318088531494,8.220020341728871e-08
11138,44182,44182,88364,16.878688097000122,8.14266951748913e-08
11158,44262,44262,88524,16.905583143234253,8.03004470565211e-08
11177,44338,44338,88676,16.932199954986572,7.926527328491887e-08
11196,44414,44414,88828,16.9580659866333,7.87347906903955e-08
11215,44490,44490,88980,16.98328399658203,7.804371736830008e-08
11234,44566,44566,89132,17.00841498374939,7.718987120182144e-08
11253,44642,44642,89284,17.035311222076416,7.663572500721359e-08
11272,44718,44718,89436,17.062573194503784,7.613700357286634e-08
11292,44798,44798,89596,17.08958911895752,7.55220256494139e-08
11311,44874,44874,89748,17.115426063537598,7.485840157545957e-08
11330,44950,44950,89900,17.141327142715454,7.429261349684688e-08
11349,45026,45026,90052,17.178310871124268,7.352446497136087e-08
11368,45102,45102,90204,17.22393798828125,7.261232550234918e-08
11387,45178,45178,90356,17.254556894302368,7.203394487918418e-08
11406,45254,45254,90508,17.283421993255615,7.153128227189651e-08
11425,45330,45330,90660,17.311129093170166,7.082453843694383e-08
11445,45410,45410,90820,17.34017515182495,7.008463788670893e-08
11464,45486,45486,90972,17.370420932769775,6.960561459622244e-08
11483,45562,45562,91124,17.400132179260254,6.826978265575268e-08
11502,45638,45638,91276,17.446876049041748,6.708180482131434e-08
11521,45714,45714,91428,17.480773210525513,6.623140740594348e-08
11540,45790,45790,91580,17.511696100234985,6.514612542690798e-08
11559,45866,45866,91732,17.542321920394897,6.429618758320467e-08
11579,45946,45946,91892,17.571887254714966,6.292442753367921e-08
11598,46022,46022,92044,17.598891973495483,6.237467574885127e-08
11617,46098,46098,92196,17.628303050994873,6.203994998861795e-08
11636,46174,46174,92348,17.65620994567871,6.06723844649361e-08
11655,46250,46250,92500,17.68679189682007,5.962044658678671e-08
11674,46326,46326,92652,17.71674919128418,5.756481246918268e-08
11693,46402,46402,92804,17.744165182113647,5.5269100723158e-08
11713,46482,46482,92964,17.776113986968994,5.435300333938948e-08
11732,46558,46558,93116,17.817289113998413,5.385426686415536e-08
11751,46634,46634,93268,17.851790189743042,5.3005970913211766e-08
11770,46710,46710,93420,17.887528896331787,5.2012999063250154e-08
11789,46786,46786,93572,17.92059302330017,5.14757802967535e-08
11808,46862,46862,93724,17.95544695854187,5.092183268325296e-08
11827,46938,46938,93876,17.99309206008911,5.0164443983467764e-08
11847,47018,47018,94036,18.025179862976074,4.956040758386796e-08
11866,47094,47094,94188,18.053953170776367,4.905158275055611e-08
11885,47170,47170,94340,18.084779024124146,4.834703563188641e-08
11904,47246,47246,94492,18.110996961593628,4.782384268889288e-08
11923,47322,47322,94644,18.136863946914673,4.746382679774443e-08
11942,47398,47398,94796,18.163305044174194,4.690189574102989e-08
11961,47474,47474,94948,18.188519954681396,4.6108059009858624e-08
11980,47550,47550,95100,18.21442198753357,4.577148427257149e-08
12000,47630,47630,95260,18.2417049407959,4.521576711649911e-08
12019,47706,47706,95412,18.267162084579468,4.4303786385103095e-08
12038,47782,47782,95564,18.29547905921936,4.3742201009727945e-08
12057,47858,47858,95716,18.324143171310425,4.3340960985999195e-08
12076,47934,47934,95868,18.35058307647705,4.285208349278467e-08
12095,48010,48010,96020,18.381335020065308,4.2273113439207584e-08
12114,48086,48086,96172,18.408878087997437,4.136451415018338e-08
12134,48166,48166,96332,18.44019603729248,4.0834046989516206e-08
12153,48242,48242,96484,18.465620040893555,4.05533244421094e-08
12172,48318,48318,96636,18.49207615852356,4.0188707911261066e-08
12191,48394,48394,96788,18.51746106147766,3.9771194148525164e-08
12210,48470,48470,96940,18.544207096099854,3.9430902927330194e-08
12229,48546,48546,97092,18.571299076080322,3.908226144672192e-08
12248,48622,48622,97244,18.596714973449707,3.872825483203991e-08
12268,48702,48702,97404,18.62300395965576,3.842332567917799e-08
12287,48778,48778,97556,18.648802042007446,3.802273466070255e-08
12306,48854,48854,97708,18.674302101135254,3.742358778201812e-08
12325,48930,48930,97860,18.699306964874268,3.712112396059052e-08
12344,49006,49006,98012,18.72503399848938,3.680728988205042e-08
12363,49082,49082,98164,18.750949144363403,3.6508233472414696e-08
12382,49158,49158,98316,18.77713418006897,3.609026520610402e-08
12402,49238,49238,98476,18.807897090911865,3.5646950405196314e-08
12421,49314,49314,98628,18.837902069091797,3.5087763004437536e-08
12440,49390,49390,98780,18.86698293685913,3.419738698491668e-08
12459,49466,49466,98932,18.898840188980103,3.293617564021175e-08
12478,49542,49542,99084,18.92722201347351,3.220088758119591e-08
12497,49618,49618,99236,18.954775094985962,3.198535670093827e-08
12516,49694,49694,99388,18.980458974838257,3.174425905521725e-08
12535,49770,49770,99540,19.00676417350769,3.1278323900449814e-08
12555,49850,49850,99700,19.038851022720337,3.094713634239555e-08
12574,49926,49926,99852,19.069332122802734,3.0656984719254595e-08
12593,50002,50002,100004,19.100543975830078,3.0370965049691386e-08
12612,50078,50078,100156,19.1286940574646,2.9931745842312414e-08
12631,50154,50154,100308,19.156656980514526,2.9567151872611242e-08
12650,50230,50230,100460,19.189263105392456,2.9338065875312828e-08
12669,50306,50306,100612,19.220784187316895,2.910833443667019e-08
12689,50386,50386,100772,19.24981713294983,2.8809562254474463e-08
12708,50462,50462,100924,19.276596069335938,2.8544346781246448e-08
12727,50538,50538,101076,19.302640914916992,2.8329820922438343e-08
12746,50614,50614,101228,19.32818603515625,2.8108058712547013e-08
12765,50690,50690,101380,19.356178998947144,2.781172820706738e-08
12784,50766,50766,101532,19.381484985351562,2.7569268962602605e-08
12803,50842,50842,101684,19.40780997276306,2.7403705072005963e-08
12823,50922,50922,101844,19.43644690513611,2.7102183362925178e-08
12842,50998,50998,101996,19.46336603164673,2.6617674759643852e-08
12861,51074,51074,102148,19.490128993988037,2.635827089888049e-08
12880,51150,51150,102300,19.515534162521362,2.6052127278680988e-08
12899,51226,51226,102452,19.542320251464844,2.521645020054392e-08
12918,51302,51302,102604,19.57611107826233,2.4480762863674434e-08
12937,51378,51378,102756,19.604961156845093,2.3875240811483564e-08
12957,51458,51458,102916,19.638500213623047,2.3461218626185518e-08
12976,51534,51534,103068,19.66926407814026,2.32511191018955e-08
12995,51610,51610,103220,19.699434995651245,2.305189348008416e-08
13014,51686,51686,103372,19.7344331741333,2.2819765008412288e-08
13033,51762,51762,103524,19.769891023635864,2.2620316126344e-08
13052,51838,51838,103676,19.80080795288086,2.2478643849878555e-08
13071,51914,51914,103828,19.837918043136597,2.224002044059171e-08
13090,51990,51990,103980,19.875622034072876,2.1872775304893167e-08
13110,52070,52070,104140,19.914303064346313,2.1598785722460005e-08
13129,52146,52146,104292,19.952255964279175,2.145199344823116e-08
13148,52222,52222,104444,19.983999967575073,2.128200393051849e-08
13167,52298,52298,104596,20.014212131500244,2.1073799194517552e-08
13186,52374,52374,104748,20.054739952087402,2.0883053847765038e-08
13205,52450,52450,104900,20.091917037963867,2.0539680978449223e-08
13224,52526,52526,105052,20.133827209472656,2.0353937993944897e-08
13244,52606,52606,105212,20.166420936584473,1.9974214919746477e-08
13263,52682,52682,105364,20.202155113220215,1.9532123022011546e-08
13282,52758,52758,105516,20.240148067474365,1.9205504996158316e-08
13301,52834,52834,105668,20.27207088470459,1.8996476217379524e-08
13320,52910,52910,105820,20.303479194641113,1.884026084702916e-08
13339,52986,52986,105972,20.337518215179443,1.862664286725609e-08
13358,53062,53062,106124,20.369264841079712,1.8313526235750087e-08
13378,53142,53142,106284,20.39704918861389,1.8172453217176777e-08
13397,53218,53218,106436,20.42494010925293,1.7889372206632495e-08
13416,53294,53294,106588,20.451431035995483,1.710811678949239e-08
13435,53370,53370,106740,20.477365016937256,1.59626433781478e-08
13454,53446,53446,106892,20.503448009490967,1.5023434987331274e-08
13473,53522,53522,107044,20.530899047851562,1.460127761690278e-08
13492,53598,53598,107196,20.557648181915283,1.4376273853425856e-08
13512,53678,53678,107356,20.586645126342773,1.4265809362926662e-08
13531,53754,53754,107508,20.61333703994751,1.4136164020827228e-08
13550,53830,53830,107660,20.638476133346558,1.3906536239601473e-08
13569,53906,53906,107812,20.66358208656311,1.3714372958383737e-08
13588,53982,53982,107964,20.690030097961426,1.3625767822016242e-08
13607,54058,54058,108116,20.714564085006714,1.3502674711396301e-08
13626,54134,54134,108268,20.740104913711548,1.336708558087578e-08
13645,54210,54210,108420,20.76555299758911,1.3256282100844254e-08
13665,54290,54290,108580,20.792160034179688,1.3011817718915725e-08
13684,54366,54366,108732,20.818401098251343,1.2743801754883238e-08
13703,54442,54442,108884,20.844671964645386,1.2409518352877433e-08
13722,54518,54518,109036,20.86987018585205,1.2048252820271863e-08
13741,54594,54594,109188,20.895036935806274,1.186939263102265e-08
13760,54670,54670,109340,20.921975135803223,1.1765067033988007e-08
13779,54746,54746,109492,20.947720050811768,1.1668938178209883e-08
13799,54826,54826,109652,20.974747896194458,1.1578595563725505e-08
13818,54902,54902,109804,20.9998459815979,1.147224408656984e-08
13837,54978,54978,109956,21.024891138076782,1.130777189511324e-08
13856,55054,55054,110108,21.052191972732544,1.1196421390651567e-08
13875,55130,55130,110260,21.078976154327393,1.1102222454630661e-08
13894,55206,55206,110412,21.104248046875,1.1001089189905664e-08
13913,55282,55282,110564,21.129817008972168,1.0924119455184525e-08
13933,55362,55362,110724,21.15647315979004,1.0710802230565706e-08
13952,55438,55438,110876,21.18314814567566,9.953948563288455e-09
13971,55510,55510,111020,21.207717895507812,9.046966807312428e-09
13990,55586,55586,111172,21.233038187026978,8.807033689508296e-09
14009,55662,55662,111324,21.258736848831177,8.732002360333906e-09
14028,55738,55738,111476,21.28340196609497,8.661324625413237e-09
14047,55814,55814,111628,21.308868169784546,8.489329710600225e-09
14067,55894,55894,111788,21.338631868362427,8.225255285686635e-09
14086,55970,55970,111940,21.36849617958069,7.957833505337916e-09
14105,56046,56046,112092,21.39926505088806,7.77237852315203e-09
14124,56122,56122,112244,21.429857969284058,7.698747615675068e-09
14143,56198,56198,112396,21.45979118347168,7.629789592456136e-09
14162,56274,56274,112548,21.487033128738403,7.554411510311557e-09
14181,56350,56350,112700,21.51193404197693,7.494573993600703e-09
14200,56426,56426,112852,21.53653311729431,7.429759150543498e-09
14220,56506,56506,113012,21.564496994018555,7.358662724805082e-09
14239,56582,56582,113164,21.589723825454712,7.31441431397731e-09
14258,56658,56658,113316,21.614251136779785,7.2465251889643505e-09
14277,56734,56734,113468,21.639193058013916,7.143396894992209e-09
14296,56810,56810,113620,21.66386318206787,7.081438150058934e-09
14315,56886,56886,113772,21.68853497505188,7.035803280073274e-09
14334,56962,56962,113924,21.713171005249023,6.971033167183084e-09
14354,57042,57042,114084,21.739301204681396,6.827824795945569e-09
14373,57118,57118,114236,21.763997077941895,6.779724566281315e-09
14392,57194,57194,114388,21.788469076156616,6.710962759521894e-09
14411,57270,57270,114540,21.81301712989807,6.607702686012319e-09
14430,57346,57346,114692,21.837477207183838,6.41563006374133e-09
14449,57422,57422,114844,21.861430168151855,6.2751906978431865e-09
14468,57498,57498,114996,21.886117935180664,6.218471493041952e-09
14488,57578,57578,115156,21.91265892982483,6.173585089602788e-09
14507,57654,57654,115308,21.938267946243286,6.116244663357851e-09
14526,57730,57730,115460,21.9632089138031,6.056513087598996e-09
14545,57806,57806,115612,21.987877130508423,6.0047031933896634e-09
14564,57882,57882,115764,22.012383937835693,5.947467025964566e-09
14583,57958,57958,115916,22.036932229995728,5.899674751282645e-09
14602,58034,58034,116068,22.062705039978027,5.857347979369291e-09
14622,58114,58114,116228,22.08937406539917,5.796594372437242e-09
14641,58190,58190,116380,22.11614418029785,5.723993675963049e-09
14660,58266,58266,116532,22.14287495613098,5.687236605615658e-09
14679,58342,58342,116684,22.175206899642944,5.632594036877115e-09
14698,58418,58418,116836,22.20447301864624,5.58485209553809e-09
14717,58494,58494,116988,22.23661494255066,5.456684723445231e-09
14736,58570,58570,117140,22.266350030899048,5.3352255127176995e-09
14756,58650,58650,117300,22.299707889556885,5.265558175385488e-09
14775,58726,58726,117452,22.331329107284546,5.21471524041096e-09
14794,58802,58802,117604,22.35961604118347,5.178613136046546e-09
14813,58878,58878,117756,22.387087106704712,5.126938084640616e-09
14832,58954,58954,117908,22.414546966552734,5.079386971614159e-09
14851,59030,59030,118060,22.442858934402466,5.032279233620644e-09
14870,59106,59106,118212,22.475855112075806,4.994117079540176e-09
14889,59182,59182,118364,22.511600971221924,4.957440670392196e-09
14909,59262,59262,118524,22.546441078186035,4.9162165379768474e-09
14928,59338,59338,118676,22.579818964004517,4.871066336175836e-09
14947,59414,59414,118828,22.610738039016724,4.834691213783057e-09
14966,59490,59490,118980,22.63909912109375,4.794398269408208e-09
14985,59566,59566,119132,22.665178060531616,4.750295543892221e-09
15004,59642,59642,119284,22.69313406944275,4.717535766502281e-09
15023,59718,59718,119436,22.720208883285522,4.679684128428746e-09
15043,59798,59798,119596,22.74909496307373,4.62683593131303e-09
15062,59874,59874,119748,22.775799989700317,4.585855019417694e-09
15081,59950,59950,119900,22.802706956863403,4.559409181859359e-09
15100,60026,60026,120052,22.829843044281006,4.504520856841202e-09
15119,60102,60102,120204,22.85798406600952,4.447791119540012e-09
15138,60178,60178,120356,22.88503098487854,4.419731292548446e-09
15157,60254,60254,120508,22.913203954696655,4.392908876626748e-09
15177,60334,60334,120668,22.94500708580017,4.328456640129379e-09
15196,60410,60410,120820,22.973496198654175,4.241293823541063e-09
15215,60486,60486,120972,23.004456043243408,4.184262728050918e-09
15234,60562,60562,121124,23.0329270362854,4.1477104332184e-09
15253,60638,60638,121276,23.06614398956299,4.118635810244612e-09
15272,60714,60714,121428,23.098018169403076,4.085550326278136e-09
15291,60790,60790,121580,23.12842607498169,4.060752972149538e-09
15311,60870,60870,121740,23.158611059188843,4.024140777674009e-09
15330,60946,60946,121892,23.187745094299316,3.984110707636406e-09
15349,61022,61022,122044,23.2174870967865,3.928976205680765e-09
15368,61098,61098,122196,23.246134042739868,3.886319404566696e-09
15387,61174,61174,122348,23.273933172225952,3.733897158465928e-09
15406,61244,61244,122488,23.299370050430298,3.3483812511925777e-09
15425,61310,61310,122620,23.32446002960205,2.9213246302534777e-09
15444,61378,61378,122756,23.349406957626343,2.5810472852808924e-09
15464,61452,61452,122904,23.375810146331787,2.275707589626283e-09
15483,61528,61528,123056,23.399932861328125,2.223720824270411e-09
15502,61604,61604,123208,23.42788815498352,2.1982644128753292e-09
15521,61680,61680,123360,23.454318046569824,2.170412395040682e-09
15540,61756,61756,123512,23.480674028396606,2.1466320215925137e-09
15559,61832,61832,123664,23.50648593902588,2.1228344806090236e-09
15578,61908,61908,123816,23.531836986541748,2.1022461436760196e-09
15598,61988,61988,123976,23.562047958374023,2.085318189085071e-09
15617,62064,62064,124128,23.58856511116028,2.0634587143495304e-09
15636,62140,62140,124280,23.61261796951294,2.0341360437134478e-09
15655,62216,62216,124432,23.63728094100952,2.0192576203252032e-09
15674,62292,62292,124584,23.661618947982788,2.0035396580267694e-09
15693,62368,62368,124736,23.6856791973114,1.973795726678738e-09
15712,62444,62444,124888,23.71014404296875,1.9551951197469996e-09
15732,62524,62524,125048,23.7361159324646,1.935857558870567e-09
15751,62600,62600,125200,23.762032985687256,1.902752774981094e-09
15770,62676,62676,125352,23.78807306289673,1.8680085565059616e-09
15789,62752,62752,125504,23.813552856445312,1.8238775237025082e-09
15808,62828,62828,125656,23.84126114845276,1.8001931727876243e-09
15827,62904,62904,125808,23.86847686767578,1.7855701551765708e-09
15846,62980,62980,125960,23.89510703086853,1.7711919323540194e-09
15866,63060,63060,126120,23.92740511894226,1.7511952873461403e-09
15885,63136,63136,126272,23.95202112197876,1.7353567788081513e-09
15904,63212,63212,126424,23.97657012939453,1.7073502716006043e-09
15923,63288,63288,126576,24.001206159591675,1.6857148497623019e-09
15942,63364,63364,126728,24.027429819107056,1.6723384027898227e-09
15961,63440,63440,126880,24.05290389060974,1.6583424916635487e-09
15980,63516,63516,127032,24.077797889709473,1.6363000624760596e-09
15999,63592,63592,127184,24.10322618484497,1.6098418618316493e-09
16019,63672,63672,127344,24.128662109375,1.5869368786853441e-09
16038,63748,63748,127496,24.153409004211426,1.5709884472125336e-09
16057,63824,63824,127648,24.17794418334961,1.5589515371929474e-09
16076,63900,63900,127800,24.20340394973755,1.545006620068925e-09
16095,63976,63976,127952,24.230334043502808,1.5319774725545616e-09
16114,64052,64052,128104,24.258990049362183,1.5210883404948956e-09
16133,64128,64128,128256,24.287755012512207,1.5081337720631577e-09
16153,64208,64208,128416,24.317482948303223,1.4920488649088993e-09
16172,64284,64284,128568,24.343717098236084,1.481311294386571e-09
16191,64360,64360,128720,24.368292093276978,1.4719675012336963e-09
16210,64436,64436,128872,24.39462399482727,1.4532175690441475e-09
16229,64512,64512,129024,24.421308040618896,1.4318254608261732e-09
16248,64588,64588,129176,24.449968814849854,1.4225303927854775e-09
16267,64664,64664,129328,24.476052045822144,1.4073100822321958e-09
16287,64744,64744,129488,24.503509998321533,1.3868273462771134e-09
16306,64820,64820,129640,24.531996965408325,1.3652255572961767e-09
16325,64896,64896,129792,24.5622341632843,1.3530869408444316e-09
16344,64972,64972,129944,24.589495182037354,1.3396075148202928e-09
16363,65048,65048,130096,24.614530086517334,1.3139059516622554e-09
16382,65124,65124,130248,24.63958191871643,1.2963475527986686e-09
16401,65200,65200,130400,24.66420006752014,1.28764056764663e-09
16421,65280,65280,130560,24.690353870391846,1.2762497654164924e-09
16440,65356,65356,130712,24.715497970581055,1.262761382903009e-09
16459,65432,65432,130864,24.740423917770386,1.2515352637381206e-09
16478,65508,65508,131016,24.766206979751587,1.241614235412984e-09
16497,65584,65584,131168,24.79283905029297,1.229212928420058e-09
16516,65660,65660,131320,24.81837797164917,1.218120783311026e-09
16535,65736,65736,131472,24.843941926956177,1.2078757470815185e-09
16554,65812,65812,131624,24.8694109916687,1.197117922511142e-09
16574,65892,65892,131784,24.898255109786987,1.1881228961333235e-09
16593,65968,65968,131936,24.92452621459961,1.1799127666144108e-09
16612,66044,66044,132088,24.94835901260376,1.16756972590051e-09
16631,66120,66120,132240,24.971972227096558,1.1569508947677734e-09
16650,66196,66196,132392,24.99577021598816,1.1505589278484708e-09
16669,66272,66272,132544,25.019239902496338,1.1398355732043759e-09
16688,66348,66348,132696,25.043873071670532,1.1264046715669374e-09
16708,66428,66428,132856,25.071117162704468,1.1176053879273786e-09
16727,66504,66504,133008,25.095194101333618,1.1039203955447988e-09
16746,66580,66580,133160,25.119140148162842,1.0938900975326181e-09
16765,66656,66656,133312,25.142646074295044,1.0611769999889544e-09
16784,66732,66732,133464,25.167458057403564,1.0194796603254013e-09
16803,66808,66808,133616,25.19381809234619,9.877263144647557e-10
16822,66884,66884,133768,25.219995975494385,9.752369374436238e-10
16842,66964,66964,133928,25.24647307395935,9.66801154249689e-10
16861,67040,67040,134080,25.272258043289185,9.573342694336994e-10
16880,67116,67116,134232,25.297441005706787,9.48837818496589e-10
16899,67192,67192,134384,25.32215404510498,9.413270922720891e-10
16918,67268,67268,134536,25.34718418121338,9.307755481330474e-10
16937,67344,67344,134688,25.37030005455017,9.212440554438018e-10
16956,67420,67420,134840,25.39429497718811,9.158193687675185e-10
16976,67500,67500,135000,25.419332027435303,9.051490282818979e-10
16995,67576,67576,135152,25.442479133605957,8.887680768021845e-10
17014,67652,67652,135304,25.465861082077026,8.76106652433935e-10
17033,67728,67728,135456,25.489616870880127,8.701036779796625e-10
17052,67804,67804,135608,25.513070106506348,8.574267028403075e-10
17071,67880,67880,135760,25.536871910095215,8.416678963185764e-10
17090,67956,67956,135912,25.56094002723694,8.179859417401469e-10
17109,68032,68032,136064,25.58483624458313,8.052911780635141e-10
17129,68112,68112,136224,25.60987114906311,7.928851577860093e-10
17148,68188,68188,136376,25.633785009384155,7.838534724515638e-10
17167,68264,68264,136528,25.65716314315796,7.75296007586155e-10
17186,68340,68340,136680,25.680902004241943,7.643403922332503e-10
17205,68416,68416,136832,25.704787015914917,7.58752830876068e-10
17224,68492,68492,136984,25.728559255599976,7.518518381676017e-10
17243,68568,68568,137136,25.75176501274109,7.380297171955318e-10
17263,68648,68648,137296,25.77695107460022,7.320604649370911e-10
17282,68724,68724,137448,25.800689935684204,7.227062470863463e-10
17301,68800,68800,137600,25.824765920639038,7.105280014395129e-10
17320,68876,68876,137752,25.848124027252197,7.049475824515699e-10
17339,68952,68952,137904,25.872055053710938,6.969587585366719e-10
17358,69028,69028,138056,25.895820140838623,6.91612373159959e-10
17377,69104,69104,138208,25.92080807685852,6.838518990841614e-10
17397,69184,69184,138368,25.94605588912964,6.766796652273205e-10
17416,69260,69260,138520,25.969949960708618,6.663102842676656e-10
17435,69336,69336,138672,25.99382495880127,6.561007648853108e-10
17454,69412,69412,138824,26.0175359249115,6.504014490438953e-10
17473,69488,69488,138976,26.04222011566162,6.448250342260688e-10
17492,69564,69564,139128,26.069313049316406,6.370950253945585e-10
17511,69640,69640,139280,26.09277606010437,6.306104803075918e-10
17531,69720,69720,139440,26.117543935775757,6.259115795761608e-10
17550,69796,69796,139592,26.141451120376587,6.196689823480773e-10
17569,69872,69872,139744,26.16507387161255,6.128522100662818e-10
17588,69948,69948,139896,26.1885929107666,6.079587127589242e-10
17607,70024,70024,140048,26.212785005569458,6.026753195768273e-10
17626,70100,70100,140200,26.236598014831543,5.962004441002043e-10
17645,70176,70176,140352,26.26033902168274,5.901400529783045e-10
17665,70256,70256,140512,26.285095930099487,5.845259625933176e-10
17684,70332,70332,140664,26.30851101875305,5.798120617504628e-10
17703,70408,70408,140816,26.332787036895752,5.761370410063161e-10
17722,70484,70484,140968,26.359230041503906,5.696000080992084e-10
17741,70560,70560,141120,26.385215997695923,5.592921094640386e-10
17760,70636,70636,141272,26.411333084106445,5.524250575626027e-10
17779,70712,70712,141424,26.43647313117981,5.490640869662535e-10
17798,70788,70788,141576,26.45988416671753,5.442377683075396e-10
17818,70868,70868,141736,26.484950065612793,5.369573413789578e-10
17837,70944,70944,141888,26.50940704345703,5.249036268647372e-10
17856,71020,71020,142040,26.533493995666504,5.197879922076542e-10
17875,71096,71096,142192,26.564078092575073,5.132242635708938e-10
17894,71172,71172,142344,26.588722944259644,5.079003912039374e-10
17913,71248,71248,142496,26.614331245422363,4.986674861073562e-10
17932,71324,71324,142648,26.639650106430054,4.866442160356789e-10
17952,71404,71404,142808,26.66384792327881,4.747814302098987e-10
17971,71480,71480,142960,26.68720507621765,4.699420616178839e-10
17990,71556,71556,143112,26.711788177490234,4.661195528920667e-10
18009,71632,71632,143264,26.737231254577637,4.630115157649221e-10
18028,71708,71708,143416,26.76443910598755,4.5915036786552945e-10
18047,71784,71784,143568,26.79813003540039,4.55982292121083e-10
18066,71860,71860,143720,26.849870204925537,4.506809700951012e-10
18086,71940,71940,143880,26.912731885910034,4.431081927447979e-10
18105,72016,72016,144032,26.961239099502563,4.376850221335132e-10
18124,72092,72092,144184,26.997541904449463,4.320434053336853e-10
18143,72168,72168,144336,27.030189037322998,4.29070678969461e-10
18162,72244,72244,144488,27.063432931900024,4.251792086886737e-10
18181,72320,72320,144640,27.091354846954346,4.1800194579248575e-10
18200,72396,72396,144792,27.12053608894348,4.091192732573801e-10
18220,72476,72476,144952,27.15315294265747,3.95401452302434e-10
18239,72552,72552,145104,27.181907892227173,3.844910906608798e-10
18258,72628,72628,145256,27.208603858947754,3.801957904114449e-10
18277,72704,72704,145408,27.237773180007935,3.7666058893890575e-10
18296,72780,72780,145560,27.266159057617188,3.7278539210155233e-10
18315,72856,72856,145712,27.291892051696777,3.689679735102998e-10
18334,72932,72932,145864,27.325093269348145,3.6517758603199857e-10
18353,73008,73008,146016,27.387096166610718,3.619719029481995e-10
18373,73088,73088,146176,27.43195104598999,3.590060192817644e-10
18392,73164,73164,146328,27.465683937072754,3.5530660140719954e-10
18411,73240,73240,146480,27.50155210494995,3.522429304826888e-10
18430,73316,73316,146632,27.530094146728516,3.4981409921987823e-10
18449,73392,73392,146784,27.559324026107788,3.4532714904418516e-10
18468,73468,73468,146936,27.590464115142822,3.411843834227715e-10
18487,73544,73544,147088,27.615143060684204,3.3906315271995637e-10
18507,73624,73624,147248,27.642755031585693,3.348959868880364e-10
18526,73700,73700,147400,27.667388916015625,3.280892048665021e-10
18545,73776,73776,147552,27.696571826934814,3.2529178891575464e-10
18564,73852,73852,147704,27.724413871765137,3.2248877001579904e-10
18583,73928,73928,147856,27.75141191482544,3.185247349460129e-10
18602,74004,74004,148008,27.776385068893433,3.1233384234389396e-10
18621,74080,74080,148160,27.80099606513977,3.029792203954347e-10
18641,74160,74160,148320,27.827747106552124,2.9625503774718513e-10
18660,74236,74236,148472,27.853914976119995,2.9302102302452344e-10
18679,74312,74312,148624,27.88144588470459,2.9072008718383656e-10
18698,74388,74388,148776,27.90752100944519,2.8853838051364027e-10
18717,74464,74464,148928,27.935101985931396,2.8616435820479453e-10
18736,74540,74540,149080,27.959824085235596,2.832716654650673e-10
18755,74616,74616,149232,27.988905906677246,2.8015206236480673e-10
18775,74696,74696,149392,28.020753860473633,2.7615049324464034e-10
18794,74772,74772,149544,28.060487985610962,2.726038611167965e-10
18813,74848,74848,149696,28.09604811668396,2.706533853401499e-10
18832,74922,74922,149844,28.12948989868164,2.6128484250726064e-10
18851,74998,74998,149996,28.163044214248657,2.4912643758534363e-10
18870,75074,75074,150148,28.193723917007446,2.4039648052014673e-10
18889,75150,75150,150300,28.221823930740356,2.3243961237380164e-10
18908,75226,75226,150452,28.250991106033325,2.2698172966114265e-10
18928,75306,75306,150612,28.2793869972229,2.2446775824877319e-10
18947,75382,75382,150764,28.31003499031067,2.2045462848712608e-10
18966,75458,75458,150916,28.341698169708252,2.160167347342216e-10
18985,75534,75534,151068,28.370162963867188,2.1302009395340623e-10
19004,75610,75610,151220,28.396483182907104,2.1131947092692786e-10
19023,75686,75686,151372,28.42569088935852,2.0855921304135283e-10
19042,75762,75762,151524,28.45758318901062,2.035279097064256e-10
19062,75842,75842,151684,28.492834091186523,1.9545620023190134e-10
19081,75906,75906,151812,28.564209938049316,1.7057430094828486e-10
19100,75966,75966,151932,28.609542846679688,1.2679405409216228e-10
19119,76028,76028,152056,28.653594970703125,9.938571835454203e-11


==> extragradient/plot_data/bilinear_matrix_game_n500/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0006918907165527344,2.018959020339561
200,201,200,401,0.1296858787536621,0.04076116011065535
400,401,400,801,0.26802611351013184,0.013980634384136865
601,602,601,1203,0.3660888671875,0.007478912404918883
801,802,801,1603,0.4648020267486572,0.004753673888981912
1001,1002,1001,2003,0.5659382343292236,0.0034486820656248356
1201,1202,1201,2403,0.6663830280303955,0.002503810172570822
1401,1402,1401,2803,0.7686519622802734,0.001967307432897608
1602,1603,1602,3205,0.8746190071105957,0.0016086456926083137
1802,1803,1802,3605,0.9693329334259033,0.001346028185622625
2002,2003,2002,4005,1.0699031352996826,0.0011547644415371076
2202,2203,2202,4405,1.1716101169586182,0.0010113283795863633
2402,2403,2402,4805,1.2654519081115723,0.0008764012526336981
2603,2604,2603,5207,1.3598101139068604,0.0007885591955443794
2803,2804,2803,5607,1.452869176864624,0.0007122684974326582
3003,3004,3003,6007,1.5454058647155762,0.0006497270049117522
3203,3204,3203,6407,1.6400229930877686,0.0005899921784646016
3403,3404,3403,6807,1.7330100536346436,0.0005401320849306003
3604,3605,3604,7209,1.8269810676574707,0.00048778459359689
3804,3805,3804,7609,1.9202721118927002,0.0004349041072029605
4004,4005,4004,8009,2.0117061138153076,0.00038847113218683465
4204,4205,4204,8409,2.1071619987487793,0.00034649996662180084
4404,4405,4404,8809,2.201352834701538,0.0003201086977566544
4605,4606,4605,9211,2.29284405708313,0.0002976451494178679
4805,4806,4805,9611,2.388306140899658,0.0002787488048750214
5005,5006,5005,10011,2.4809839725494385,0.0002616834252635549
5205,5206,5205,10411,2.573606014251709,0.00024784174446748375
5405,5406,5405,10811,2.673776149749756,0.0002358932581286411
5606,5607,5606,11213,2.7657270431518555,0.00022222057465141908
5806,5807,5806,11613,2.8600728511810303,0.00021096911391128278
6006,6007,6006,12013,2.958130121231079,0.00020129223980205993
6206,6207,6206,12413,3.0504298210144043,0.00019273585909174623
6406,6407,6406,12813,3.1431519985198975,0.00018480935625377168
6607,6608,6607,13215,3.2350680828094482,0.00017803357936582126
6807,6808,6807,13615,3.3298280239105225,0.0001711143671780811
7007,7008,7007,14015,3.4230520725250244,0.00016481564381359934
7207,7208,7207,14415,3.5168471336364746,0.00015805629373417124
7407,7408,7407,14815,3.611877202987671,0.00015149638458837136
7608,7609,7608,15217,3.7040019035339355,0.0001457797693524913
7808,7809,7808,15617,3.7940468788146973,0.00014069619698805783
8008,8009,8008,16017,3.8849031925201416,0.0001359878556802032
8208,8209,8208,16417,3.98093581199646,0.0001315320310631447
8408,8409,8408,16817,4.078026056289673,0.00012704728798727748
8609,8610,8609,17219,4.177298069000244,0.0001228685672485282
8809,8810,8809,17619,4.2906410694122314,0.00011888091126387573
9009,9010,9009,18019,4.400728940963745,0.00011504608407371523
9209,9210,9209,18419,4.506505012512207,0.00011138986323499458
9409,9410,9409,18819,4.624882936477661,0.00010790003027536749
9610,9611,9610,19221,4.739508867263794,0.00010454200480419918
9810,9811,9810,19621,4.8490800857543945,0.00010140520053005085
10010,10011,10010,20021,4.967380046844482,9.822756870887653e-05
10210,10211,10210,20421,5.2764060497283936,9.541139505465662e-05
10410,10411,10410,20821,5.399012088775635,9.248817336717906e-05
10611,10612,10611,21223,5.503271818161011,8.995358236946512e-05
10811,10812,10811,21623,5.6055450439453125,8.734485968815005e-05
11011,11012,11011,22023,5.704674959182739,8.48791956616179e-05
11211,11212,11211,22423,5.800329923629761,8.245861582703645e-05
11411,11412,11411,22823,5.894937038421631,8.010144426179838e-05
11612,11613,11612,23225,5.998507976531982,7.797391654826677e-05
11812,11813,11812,23625,6.112811088562012,7.583731772200379e-05
12012,12013,12012,24025,6.217639207839966,7.386174880433945e-05
12212,12213,12212,24425,6.31752610206604,7.20418939795912e-05
12412,12413,12412,24825,6.4215521812438965,7.028027063577944e-05
12613,12614,12613,25227,6.525040149688721,6.85981658108995e-05
12813,12814,12813,25627,6.628347158432007,6.659217145937226e-05
13013,13014,13013,26027,6.736782073974609,6.470267677953778e-05
13213,13214,13213,26427,6.8364951610565186,6.310141366150047e-05
13413,13414,13413,26827,6.937504053115845,6.161135450139276e-05
13614,13615,13614,27229,7.043515205383301,6.020157899221332e-05
13814,13815,13814,27629,7.149831056594849,5.8815072055932136e-05
14014,14015,14014,28029,7.265031814575195,5.7547747299027675e-05
14214,14215,14214,28429,7.367095947265625,5.614420156885427e-05
14414,14415,14414,28829,7.471224069595337,5.486335234982929e-05
14615,14616,14615,29231,7.578567028045654,5.322820019981047e-05
14815,14816,14815,29631,7.691308975219727,5.202449048620488e-05
15015,15016,15015,30031,7.799606084823608,5.086413902761968e-05
15215,15216,15215,30431,7.904677152633667,4.982837480104092e-05
15415,15416,15415,30831,8.005128860473633,4.890273196719915e-05
15616,15617,15616,31233,8.114667892456055,4.79454249621053e-05
15816,15817,15816,31633,8.21501898765564,4.706167708545054e-05
16016,16017,16016,32033,8.313063144683838,4.62281166999516e-05
16216,16217,16216,32433,8.41104793548584,4.538942964559918e-05
16416,16417,16416,32833,8.514524221420288,4.4590360490614544e-05
16617,16618,16617,33235,8.61496901512146,4.353209502387373e-05
16817,16818,16817,33635,8.714219093322754,4.263773141728704e-05
17017,17018,17017,34035,8.814344882965088,4.183191531420544e-05
17217,17218,17217,34435,8.912204027175903,4.1101143869169994e-05
17417,17418,17417,34835,9.015105962753296,4.0360256985905896e-05
17618,17619,17618,35237,9.113395929336548,3.906652236937047e-05
17818,17819,17818,35637,9.207871913909912,3.790749927061513e-05
18018,18019,18018,36037,9.30925989151001,3.69682448243175e-05
18218,18219,18218,36437,9.41080117225647,3.565240984025893e-05
18418,18419,18418,36837,9.50629711151123,3.464829804257318e-05
18619,18620,18619,37239,9.603679895401001,3.3696335798690846e-05
18819,18820,18819,37639,9.699116945266724,3.283983530912163e-05
19019,19020,19019,38039,9.795572996139526,3.207373520938785e-05
19219,19220,19219,38439,9.896644115447998,3.137846258035208e-05
19419,19420,19419,38839,9.992188215255737,3.071992072208155e-05
19620,19621,19620,39241,10.087995052337646,3.0082033730808437e-05
19820,19821,19820,39641,10.183105945587158,2.9510012025143946e-05
20020,20021,20020,40041,10.27529501914978,2.896615470596412e-05
20220,20221,20220,40441,10.368828058242798,2.8434583872974098e-05
20420,20421,20420,40841,10.469096899032593,2.793860337033127e-05
20621,20622,20621,41243,10.569383144378662,2.7490957086516356e-05
20821,20822,20821,41643,10.672912120819092,2.703876168167222e-05
21021,21022,21021,42043,10.766280889511108,2.658779938271546e-05
21221,21222,21221,42443,10.859131097793579,2.615450272457967e-05
21421,21422,21421,42843,10.954699993133545,2.5738748388132668e-05
21622,21623,21622,43245,11.060182094573975,2.5334905800384553e-05
21822,21823,21822,43645,11.20461893081665,2.4959294441267445e-05
22022,22023,22022,44045,11.353259086608887,2.459701794802076e-05
22222,22223,22222,44445,11.491460084915161,2.426120923799731e-05
22422,22423,22422,44845,11.610867023468018,2.3922797641951904e-05
22623,22624,22623,45247,11.737671136856079,2.358720458996452e-05
22823,22824,22823,45647,11.854620218276978,2.3275211369388992e-05
23023,23024,23023,46047,11.9806649684906,2.2973512579643727e-05
23223,23224,23223,46447,12.074445009231567,2.2665489990414793e-05
23423,23424,23423,46847,12.167971134185791,2.2368521492252474e-05
23624,23625,23624,47249,12.264154195785522,2.2072263160185305e-05
23824,23825,23824,47649,12.360112190246582,2.1792185038854662e-05
24024,24025,24024,48049,12.45248293876648,2.1525360890788575e-05
24224,24225,24224,48449,12.544377088546753,2.125398993827494e-05
24424,24425,24424,48849,12.639373064041138,2.0998476168699493e-05
24625,24626,24625,49251,12.73472785949707,2.0753234444392037e-05
24825,24826,24825,49651,12.83138394355774,2.050499326246106e-05
25025,25026,25025,50051,12.928743124008179,2.0263779114669623e-05
25225,25226,25225,50451,13.023812055587769,2.002763713607128e-05
25425,25426,25425,50851,13.118359088897705,1.9805233570316335e-05
25626,25627,25626,51253,13.215132236480713,1.957580440117947e-05
25826,25827,25826,51653,13.314393043518066,1.9354726886901396e-05
26026,26027,26026,52053,13.412336111068726,1.9139851551286825e-05
26226,26227,26226,52453,13.516237020492554,1.892443046324196e-05
26426,26427,26426,52853,13.614874124526978,1.870746277251029e-05
26627,26628,26627,53255,13.711395025253296,1.849366920421552e-05
26827,26828,26827,53655,13.806719064712524,1.82954772494338e-05
27027,27028,27027,54055,13.901834964752197,1.80982210178185e-05
27227,27228,27227,54455,13.99579405784607,1.7894585600168836e-05
27427,27428,27427,54855,14.091858148574829,1.7709397908678323e-05
27628,27629,27628,55257,14.186588048934937,1.7515650693615462e-05
27828,27829,27828,55657,14.28153395652771,1.732427641359571e-05
28028,28029,28028,56057,14.376243829727173,1.7147237054429712e-05
28228,28229,28228,56457,14.473362922668457,1.6972500600055034e-05
28428,28429,28428,56857,14.56869387626648,1.679195799284979e-05
28629,28630,28629,57259,14.669846057891846,1.6607256050936346e-05
28829,28830,28829,57659,14.76469087600708,1.642869071927071e-05
29029,29030,29029,58059,14.86123013496399,1.6231257726122935e-05
29229,29230,29229,58459,14.956342935562134,1.6024972866530433e-05
29429,29430,29429,58859,15.051623106002808,1.5853808018765536e-05
29630,29631,29630,59261,15.148389101028442,1.569204420032237e-05
29830,29831,29830,59661,15.244492053985596,1.5532286416476243e-05
30030,30031,30030,60061,15.339235067367554,1.5368048729864727e-05
30230,30231,30230,60461,15.433658123016357,1.52144092700436e-05
30430,30431,30430,60861,15.528075933456421,1.5064718214837631e-05
30631,30632,30631,61263,15.634865045547485,1.4918452637393357e-05
30831,30832,30831,61663,15.731381893157959,1.4761723748896858e-05
31031,31032,31031,62063,15.825240135192871,1.4608026991756164e-05
31231,31232,31231,62463,15.918967962265015,1.445938620784927e-05
31431,31432,31431,62863,16.019155025482178,1.4309819524528183e-05
31632,31633,31632,63265,16.11668610572815,1.4165565403782295e-05
31832,31833,31832,63665,16.211090087890625,1.4026286746972872e-05
32032,32033,32032,64065,16.307175874710083,1.3891845552646173e-05
32232,32233,32232,64465,16.4012930393219,1.3759353011761771e-05
32432,32433,32432,64865,16.49498200416565,1.3627393518862995e-05
32633,32634,32633,65267,16.590874195098877,1.3493330216095803e-05
32833,32834,32833,65667,16.686962127685547,1.336472730427581e-05
33033,33034,33033,66067,16.783434867858887,1.3237456413725868e-05
33233,33234,33233,66467,16.877807140350342,1.3104077921619519e-05
33433,33434,33433,66867,16.972100019454956,1.2971952307878424e-05
33634,33635,33634,67269,17.06850004196167,1.2849211294540985e-05
33834,33835,33834,67669,17.16551113128662,1.27304845762743e-05
34034,34035,34034,68069,17.261146068572998,1.2610698323242823e-05
34234,34235,34234,68469,17.356317043304443,1.2494558653915198e-05
34434,34435,34434,68869,17.45000696182251,1.2380092999855784e-05
34635,34636,34635,69271,17.545637130737305,1.2261217945080221e-05
34835,34836,34835,69671,17.646136045455933,1.2139834880251609e-05
35035,35036,35035,70071,17.746479988098145,1.2026607430768636e-05
35235,35236,35235,70471,17.839752912521362,1.191297555905526e-05
35435,35436,35435,70871,17.933840036392212,1.1802104176124104e-05
35636,35637,35636,71273,18.02974510192871,1.1697859209508473e-05
35836,35837,35836,71673,18.127595901489258,1.1593350938515641e-05
36036,36037,36036,72073,18.222767114639282,1.1484846965917414e-05
36236,36237,36236,72473,18.316753149032593,1.137616652938302e-05
36436,36437,36436,72873,18.41055679321289,1.1274540752686246e-05
36637,36638,36637,73275,18.505696058273315,1.1169779568499476e-05
36837,36838,36837,73675,18.60184383392334,1.1065977902943369e-05
37037,37038,37037,74075,18.697523832321167,1.0964628542114361e-05
37237,37238,37237,74475,18.79206609725952,1.0865536874384976e-05
37437,37438,37437,74875,18.886479139328003,1.076698146593839e-05
37638,37639,37638,75277,18.980812072753906,1.0669147761633347e-05
37838,37839,37838,75677,19.08000612258911,1.0577326056653098e-05
38038,38039,38038,76077,19.175289154052734,1.0489528596715121e-05
38238,38239,38238,76477,19.269999980926514,1.039699018425426e-05
38438,38439,38438,76877,19.366328954696655,1.0300859837930527e-05
38639,38640,38639,77279,19.462563037872314,1.0206423717576803e-05
38839,38840,38839,77679,19.558115005493164,1.01168692783896e-05
39039,39040,39039,78079,19.65616202354431,1.0027431114998991e-05
39239,39240,39239,78479,19.756765842437744,9.936632068242417e-06
39439,39440,39439,78879,19.85674500465393,9.849268237464279e-06
39640,39641,39640,79281,19.95108389854431,9.764672465319682e-06
39840,39841,39840,79681,20.042896032333374,9.681609859551707e-06
40040,40041,40040,80081,20.13780403137207,9.597575790342973e-06
40240,40241,40240,80481,20.230418920516968,9.518647301155423e-06
40440,40441,40440,80881,20.32302212715149,9.4410621490745e-06
40641,40642,40641,81283,20.416075944900513,9.363718544451202e-06
40841,40842,40841,81683,20.507107973098755,9.280907336570204e-06
41041,41042,41041,82083,20.600291967391968,9.199697595519134e-06
41241,41242,41241,82483,20.719552040100098,9.121410873527956e-06
41441,41442,41441,82883,20.832530975341797,9.045341672050303e-06
41642,41643,41642,83285,20.940994024276733,8.972881324353301e-06
41842,41843,41842,83685,21.04140591621399,8.90221492046207e-06
42042,42043,42042,84085,21.14841914176941,8.83213764554076e-06
42242,42243,42242,84485,21.24477791786194,8.760057655293868e-06
42442,42443,42442,84885,21.343119144439697,8.685254751873719e-06
42643,42644,42643,85287,21.441895246505737,8.61612623864594e-06
42843,42844,42843,85687,21.538846969604492,8.545982217779857e-06
43043,43044,43043,86087,21.638636112213135,8.474467565874431e-06
43243,43244,43243,86487,21.738508939743042,8.403897586724643e-06
43443,43444,43443,86887,21.84026002883911,8.336935516667862e-06
43644,43645,43644,87289,21.943989992141724,8.27007569037697e-06
43844,43845,43844,87689,22.042582035064697,8.206592746369263e-06
44044,44045,44044,88089,22.143998861312866,8.146718725239161e-06
44244,44245,44244,88489,22.241874933242798,8.084758748804204e-06
44444,44445,44444,88889,22.33720111846924,8.019859794305835e-06
44645,44646,44645,89291,22.437224864959717,7.954726309405252e-06
44845,44846,44845,89691,22.53642201423645,7.891127928376821e-06
45045,45046,45045,90091,22.635721921920776,7.830402212055003e-06
45245,45246,45245,90491,22.73248600959778,7.770226660958626e-06
45445,45446,45445,90891,22.829209089279175,7.713394005620631e-06
45646,45647,45646,91293,22.929249048233032,7.656807957493565e-06
45846,45847,45846,91693,23.032167196273804,7.597628530126564e-06
46046,46047,46046,92093,23.136861085891724,7.5399833159383375e-06
46246,46247,46246,92493,23.242263078689575,7.484794376567849e-06
46446,46447,46446,92893,23.343194007873535,7.431001207166474e-06
46647,46648,46647,93295,23.446534156799316,7.375298460765313e-06
46847,46848,46847,93695,23.54470920562744,7.3179891854175204e-06
47047,47048,47047,94095,23.6479651927948,7.2643933610587996e-06
47247,47248,47247,94495,23.751644134521484,7.210976018832241e-06
47447,47448,47447,94895,23.85156512260437,7.157167250338387e-06
47648,47649,47648,95297,23.960018157958984,7.106481508665893e-06
47848,47849,47848,95697,24.065216064453125,7.058426206645073e-06
48048,48049,48048,96097,24.169049978256226,7.011757297099145e-06
48248,48249,48248,96497,24.271368980407715,6.96287273060307e-06
48448,48449,48448,96897,24.37349009513855,6.914040790896323e-06
48649,48650,48649,97299,24.47553515434265,6.864688381152165e-06
48849,48850,48849,97699,24.57674217224121,6.817333096090463e-06
49049,49050,49049,98099,24.680713891983032,6.76971622479867e-06
49249,49250,49249,98499,24.782012224197388,6.722371397200465e-06
49449,49450,49449,98899,24.883830070495605,6.676677912066424e-06
49650,49651,49650,99301,24.98781704902649,6.633045644389544e-06
49850,49851,49850,99701,25.09436798095703,6.590913145902961e-06
50050,50051,50050,100101,25.196091175079346,6.549847249049841e-06
50250,50251,50250,100501,25.29758310317993,6.509289614765456e-06
50450,50451,50450,100901,25.397894144058228,6.467316660525181e-06
50651,50652,50651,101303,25.49740695953369,6.423400223265311e-06
50851,50852,50851,101703,25.599399089813232,6.38011207953982e-06
51051,51052,51051,102103,25.698559999465942,6.339115387005411e-06
51251,51252,51251,102503,25.79839515686035,6.299527201620974e-06
51451,51452,51451,102903,25.89651393890381,6.261892104954493e-06
51652,51653,51652,103305,25.997303009033203,6.2254929303293284e-06
51852,51853,51852,103705,26.106410026550293,6.188056806975595e-06
52052,52053,52052,104105,26.20594882965088,6.149521534613314e-06
52252,52253,52252,104505,26.30411696434021,6.112217875909116e-06
52452,52453,52452,104905,26.40741205215454,6.0755667616829965e-06
52653,52654,52653,105307,26.51087212562561,6.037966831298695e-06
52853,52854,52853,105707,26.613919019699097,6.000595396202917e-06
53053,53054,53053,106107,26.721017122268677,5.964719897248612e-06
53253,53254,53253,106507,26.824865102767944,5.929290757505344e-06
53453,53454,53453,106907,26.929698944091797,5.8930219972410895e-06
53654,53655,53654,107309,27.03413200378418,5.860179437535335e-06
53854,53855,53854,107709,27.14177107810974,5.82905388092337e-06
54054,54055,54054,108109,27.248713970184326,5.797622797539256e-06
54254,54255,54254,108509,27.354344844818115,5.764513518132299e-06
54454,54455,54454,108909,27.460352897644043,5.73207691718837e-06
54655,54656,54655,109311,27.565953969955444,5.700153188091916e-06
54855,54856,54855,109711,27.68617606163025,5.669208311318425e-06
55055,55056,55055,110111,27.789266109466553,5.636970540443322e-06
55255,55256,55255,110511,27.892818927764893,5.606782221634632e-06
55455,55456,55455,110911,27.995154857635498,5.576470004151609e-06
55656,55657,55656,111313,28.105796098709106,5.547153176124909e-06
55856,55857,55856,111713,28.2175190448761,5.518532269959701e-06
56056,56057,56056,112113,28.337097883224487,5.490115285505996e-06
56256,56257,56256,112513,28.438060998916626,5.4635662726641095e-06
56456,56457,56456,112913,28.540628910064697,5.436879659221792e-06
56657,56658,56657,113315,28.643023014068604,5.408584772660401e-06
56857,56858,56857,113715,28.74557113647461,5.380623637182365e-06
57057,57058,57057,114115,28.84782886505127,5.352979434197074e-06
57257,57258,57257,114515,28.951789140701294,5.3267180316268536e-06
57457,57458,57457,114915,29.05465292930603,5.301241596314342e-06
57658,57659,57658,115317,29.15745997428894,5.27710711255904e-06
57858,57859,57858,115717,29.25677514076233,5.254068373673773e-06
58058,58059,58058,116117,29.354795932769775,5.230000029364922e-06
58258,58259,58258,116517,29.45415186882019,5.205039121357084e-06
58458,58459,58458,116917,29.553133964538574,5.180943469472777e-06
58659,58660,58659,117319,29.656657218933105,5.157011645011207e-06
58859,58860,58859,117719,29.753202199935913,5.132910296991532e-06
59059,59060,59059,118119,29.8489990234375,5.109750031148203e-06
59259,59260,59259,118519,29.94454288482666,5.087007908396386e-06
59459,59460,59459,118919,30.039232969284058,5.0648453998596624e-06
59660,59661,59660,119321,30.13569712638855,5.0433900557700875e-06
59860,59861,59860,119721,30.234748125076294,5.023202304706336e-06
60060,60061,60060,120121,30.333423137664795,5.003052869498259e-06
60260,60261,60260,120521,30.428997039794922,4.9825495787796475e-06
60460,60461,60460,120921,30.524867057800293,4.960494591596389e-06
60661,60662,60661,121323,30.621906995773315,4.9393012891353374e-06
60861,60862,60861,121723,30.717531204223633,4.918420123380644e-06
61061,61062,61061,122123,30.81237506866455,4.8985283671483695e-06
61261,61262,61261,122523,30.9104220867157,4.879252320801058e-06
61461,61462,61461,122923,31.00460410118103,4.860985096003401e-06
61662,61663,61662,123325,31.102582931518555,4.84254485608748e-06
61862,61863,61862,123725,31.19775414466858,4.823939417995177e-06
62062,62063,62062,124125,31.292733907699585,4.805359624821139e-06
62262,62263,62262,124525,31.387348890304565,4.7876716781659345e-06
62462,62463,62462,124925,31.47947096824646,4.770333724815941e-06
62663,62664,62663,125327,31.573507070541382,4.751917075696197e-06
62863,62864,62863,125727,31.665882110595703,4.734497071727218e-06
63063,63064,63063,126127,31.75905990600586,4.716981144593251e-06
63263,63264,63263,126527,31.850483894348145,4.699738393525728e-06
63463,63464,63463,126927,31.942511081695557,4.68302970087913e-06
63664,63665,63664,127329,32.03462290763855,4.667474086693693e-06
63864,63865,63864,127729,32.13322901725769,4.652468759595238e-06
64064,64065,64064,128129,32.26862621307373,4.6374707246470715e-06
64264,64265,64264,128529,32.45208120346069,4.622366835618746e-06
64464,64465,64464,128929,32.56269598007202,4.607134866975447e-06
64665,64666,64665,129331,32.671852111816406,4.591599882665121e-06
64865,64866,64865,129731,32.8482460975647,4.576496106197752e-06
65065,65066,65065,130131,33.010972023010254,4.561101505619987e-06
65265,65266,65265,130531,33.107089042663574,4.546860134347892e-06
65465,65466,65465,130931,33.20658802986145,4.532842824405755e-06
65666,65667,65666,131333,33.30677604675293,4.519075480989607e-06
65866,65867,65866,131733,33.40000891685486,4.505964376744404e-06
66066,66067,66066,132133,33.4933500289917,4.493110169566521e-06
66266,66267,66266,132533,33.58946204185486,4.480415647204266e-06
66466,66467,66466,132933,33.68166899681091,4.467205847928215e-06
66667,66668,66667,133335,33.77987289428711,4.4536148780169356e-06
66867,66868,66867,133735,33.8745059967041,4.440545853833456e-06
67067,67068,67067,134135,33.968589067459106,4.4281484209915045e-06
67267,67268,67267,134535,34.06047010421753,4.415453849927751e-06
67467,67468,67467,134935,34.158344984054565,4.4037673371999596e-06
67668,67669,67668,135337,34.25226402282715,4.39236225021195e-06
67868,67869,67868,135737,34.351333141326904,4.3810901735621005e-06
68068,68069,68068,136137,34.45274591445923,4.369691234486843e-06
68268,68269,68268,136537,34.551236152648926,4.358164543030429e-06
68468,68469,68468,136937,34.65007710456848,4.346713176592339e-06
68669,68670,68669,137339,34.74675393104553,4.335463344571485e-06
68869,68870,68869,137739,34.84600281715393,4.324737368158083e-06
69069,69070,69069,138139,34.94595503807068,4.313903768047646e-06
69269,69270,69269,138539,35.04680109024048,4.30313423285168e-06
69469,69470,69469,138939,35.14942502975464,4.292781123240539e-06
69670,69671,69670,139341,35.248818159103394,4.282688677953163e-06
69870,69871,69870,139741,35.348260164260864,4.273067794852501e-06
70070,70071,70070,140141,35.44508695602417,4.2636157067140405e-06
70270,70271,70270,140541,35.541301012039185,4.253838947828608e-06
70470,70471,70470,140941,35.640661001205444,4.243846625576968e-06
70671,70672,70671,141343,35.73720908164978,4.234177267318673e-06
70871,70872,70871,141743,35.83641505241394,4.224645396643351e-06
71071,71072,71071,142143,35.92889213562012,4.215049202222403e-06
71271,71272,71271,142543,36.021042823791504,4.205948448742238e-06
71471,71472,71471,142943,36.111812114715576,4.197279939738672e-06
71672,71673,71672,143345,36.205511808395386,4.188786196939538e-06
71872,71873,71872,143745,36.30340600013733,4.180408358976297e-06
72072,72073,72072,144145,36.45951294898987,4.17190893009907e-06
72272,72273,72272,144545,36.554157972335815,4.163786463602608e-06
72472,72473,72472,144945,36.64809322357178,4.155652908468142e-06
72673,72674,72673,145347,36.73644804954529,4.147242216025874e-06
72873,72874,72873,145747,36.83294987678528,4.139013513304246e-06
73073,73074,73073,146147,36.92401099205017,4.130919640312966e-06
73273,73274,73273,146547,37.01356792449951,4.123127015327734e-06
73473,73474,73473,146947,37.10783791542053,4.115585418812253e-06
73674,73675,73674,147349,37.1999568939209,4.108381735321472e-06
73874,73875,73874,147749,37.29207491874695,4.1012675465273464e-06
74074,74075,74074,148149,37.38387393951416,4.094248224277239e-06
74274,74275,74274,148549,37.47462606430054,4.0870923060152975e-06
74474,74475,74474,148949,37.56565713882446,4.079693746196919e-06
74675,74676,74675,149351,37.65762400627136,4.0727133283119276e-06
74875,74876,74875,149751,37.74791121482849,4.065826301944098e-06
75075,75076,75075,150151,37.84222412109375,4.059006507320213e-06
75275,75276,75275,150551,37.93434500694275,4.0521906697351686e-06
75475,75476,75475,150951,38.02464509010315,4.045674576685878e-06
75676,75677,75676,151353,38.11622405052185,4.0393336016755366e-06
75876,75877,75876,151753,38.20697498321533,4.033333273628305e-06
76076,76077,76076,152153,38.3018901348114,4.027298543636594e-06
76276,76277,76276,152553,38.39377999305725,4.021193192440547e-06
76476,76477,76476,152953,38.4865038394928,4.0149576661416324e-06
76677,76678,76677,153355,38.58054804801941,4.008895581939894e-06
76877,76878,76877,153755,38.67763710021973,4.002774638468063e-06
77077,77078,77077,154155,38.77093696594238,3.9969923587777165e-06
77277,77278,77277,154555,38.86297011375427,3.991401466563471e-06
77477,77478,77477,154955,38.95234704017639,3.985886879839035e-06
77678,77679,77678,155357,39.04276204109192,3.980451839208984e-06
77878,77879,77878,155757,39.13620901107788,3.975126866825627e-06
78078,78079,78078,156157,39.228610038757324,3.969799667592655e-06
78278,78279,78278,156557,39.321882009506226,3.964469089178127e-06
78478,78479,78478,156957,39.41318917274475,3.959272054995678e-06
78679,78680,78679,157359,39.504117012023926,3.954077470783236e-06
78879,78880,78879,157759,39.595104932785034,3.94898050721214e-06
79079,79080,79079,158159,39.68644189834595,3.943673356239752e-06
79279,79280,79279,158559,39.78028416633606,3.9386541712250405e-06
79479,79480,79479,158959,39.8751380443573,3.933803650520798e-06
79680,79681,79680,159361,39.96749401092529,3.929140761824007e-06
79880,79881,79880,159761,40.057514905929565,3.924539350390322e-06
80080,80081,80080,160161,40.14920496940613,3.920094688821877e-06
80280,80281,80280,160561,40.24252796173096,3.915453915360784e-06
80480,80481,80480,160961,40.33435797691345,3.910767291848993e-06
80681,80682,80681,161363,40.43546199798584,3.906111333251841e-06
80881,80882,80881,161763,40.62334418296814,3.901714516713664e-06
81081,81082,81081,162163,40.71922993659973,3.897214431136008e-06
81281,81282,81281,162563,40.83222699165344,3.892946791404614e-06
81481,81482,81481,162963,41.02259802818298,3.888896912543337e-06
81682,81683,81682,163365,41.13066101074219,3.884563437801456e-06
81882,81883,81882,163765,41.303099155426025,3.8805551465020765e-06
82082,82083,82082,164165,41.424992084503174,3.876599629082436e-06
82282,82283,82282,164565,41.53570914268494,3.872625858505034e-06
82482,82483,82482,164965,41.64863991737366,3.868763556883427e-06
82683,82684,82683,165367,41.75031113624573,3.864558697265752e-06
82883,82884,82883,165767,41.84966707229614,3.860634353469451e-06
83083,83084,83083,166167,41.94989013671875,3.85684809239632e-06
83283,83284,83283,166567,42.05026412010193,3.85308683509126e-06
83483,83484,83483,166967,42.150813817977905,3.849526720554424e-06
83684,83685,83684,167369,42.25664710998535,3.846000914369786e-06
83884,83885,83884,167769,42.35644602775574,3.842559418722024e-06
84084,84085,84084,168169,42.455684185028076,3.839121728038319e-06
84284,84285,84284,168569,42.55196785926819,3.8356570707362545e-06
84484,84485,84484,168969,42.65697407722473,3.8321670359823925e-06
84685,84686,84685,169371,42.762418031692505,3.8287586140416584e-06
84885,84886,84885,169771,42.873571157455444,3.825344477799412e-06
85085,85086,85085,170171,42.996302127838135,3.822200867033416e-06
85285,85286,85285,170571,43.1283860206604,3.818747085077099e-06
85485,85486,85485,170971,43.2457070350647,3.815519354451327e-06
85686,85687,85686,171373,43.356924057006836,3.8124183993943223e-06
85886,85887,85886,171773,43.452800035476685,3.8094628980598518e-06
86086,86087,86086,172173,43.55099701881409,3.806435672493939e-06
86286,86287,86286,172573,43.65881705284119,3.8034591493704346e-06
86486,86487,86486,172973,43.75982093811035,3.800325027549511e-06
86687,86688,86687,173375,43.863672971725464,3.7973266881858254e-06
86887,86888,86887,173775,43.96985220909119,3.7945347980899444e-06
87087,87088,87087,174175,44.08529615402222,3.791435936185064e-06
87287,87288,87287,174575,44.195558071136475,3.7886118597548922e-06
87487,87488,87487,174975,44.33368802070618,3.785796509879588e-06
87688,87689,87688,175377,44.5316321849823,3.78303453246106e-06
87888,87889,87888,175777,44.64543414115906,3.780385938384853e-06
88088,88089,88088,176177,44.74361205101013,3.777667771943591e-06
88288,88289,88288,176577,44.83990406990051,3.7750884264033755e-06
88488,88489,88488,176977,44.94275999069214,3.772397819825494e-06
88689,88690,88689,177379,45.06967115402222,3.769863306207296e-06
88889,88890,88889,177779,45.2270929813385,3.7671615873099728e-06
89089,89090,89089,178179,45.36690878868103,3.7645308834472864e-06
89289,89290,89289,178579,45.49857711791992,3.7620974500934466e-06
89489,89490,89489,178979,45.61096501350403,3.759614833835517e-06
89690,89691,89690,179381,45.83793807029724,3.7572130715827153e-06
89890,89891,89890,179781,46.02369499206543,3.754864221432682e-06
90090,90091,90090,180181,46.139047145843506,3.7525294408557296e-06
90290,90291,90290,180581,46.24462699890137,3.7501803552079395e-06
90490,90491,90490,180981,46.388453006744385,3.7477842998475575e-06
90691,90692,90691,181383,46.526610136032104,3.7454945656799693e-06
90891,90892,90891,181783,46.64155912399292,3.7432000227649795e-06
91091,91092,91091,182183,46.73408102989197,3.7409134530419383e-06
91291,91292,91291,182583,46.8275671005249,3.738683795275269e-06
91491,91492,91491,182983,46.92595195770264,3.7365222446340325e-06
91692,91693,91692,183385,47.04710078239441,3.7343767569591324e-06
91892,91893,91892,183785,47.149458169937134,3.7323154290629394e-06
92092,92093,92092,184185,47.239197969436646,3.7301716297545393e-06
92292,92293,92292,184585,47.32997918128967,3.7281863854228945e-06
92492,92493,92492,184985,47.420137882232666,3.726067592104909e-06
92693,92694,92693,185387,47.508331060409546,3.724183839862485e-06
92893,92894,92893,185787,47.59714984893799,3.721825316935096e-06
93093,93094,93093,186187,47.684956073760986,3.71972810444048e-06
93293,93294,93293,186587,47.7758629322052,3.7177701170806563e-06
93493,93494,93493,186987,47.86515808105469,3.7158223947371162e-06
93694,93695,93694,187389,47.95587921142578,3.7138827485621074e-06
93894,93895,93894,187789,48.04366993904114,3.712019497988328e-06
94094,94095,94094,188189,48.13531684875488,3.710109732879412e-06
94294,94295,94294,188589,48.225646018981934,3.70820806248976e-06
94494,94495,94494,188989,48.319069147109985,3.706328687912312e-06
94695,94696,94695,189391,48.409878969192505,3.7048368386704402e-06
94895,94896,94895,189791,48.50325083732605,3.702601561340612e-06
95095,95096,95095,190191,48.61845302581787,3.700848325617244e-06
95295,95296,95295,190591,48.70965504646301,3.6990599923859866e-06
95495,95496,95495,190991,48.80339980125427,3.6972888686868124e-06
95696,95697,95696,191393,48.89261507987976,3.6955438880176505e-06
95896,95897,95896,191793,49.001646995544434,3.6938752363480025e-06
96096,96097,96096,192193,49.1314799785614,3.6923681691613874e-06
96296,96297,96296,192593,49.231239795684814,3.6906668149503246e-06
96496,96497,96496,192993,49.3258171081543,3.6888131307535134e-06
96697,96698,96697,193395,49.42498707771301,3.6871557762478547e-06
96897,96898,96897,193795,49.53670287132263,3.6856869824557805e-06
97097,97098,97097,194195,49.63691997528076,3.684000212393828e-06
97297,97298,97297,194595,49.73324489593506,3.6821924860130233e-06
97497,97498,97497,194995,49.82456398010254,3.680807010521433e-06
97698,97699,97698,195397,49.91615414619446,3.6790336353535507e-06
97898,97899,97898,195797,50.01034998893738,3.677536949066528e-06
98098,98099,98098,196197,50.10253691673279,3.675993762552712e-06
98298,98299,98298,196597,50.195690870285034,3.674504717919146e-06
98498,98499,98498,196997,50.29033899307251,3.6729623017245877e-06
98699,98700,98699,197399,50.38551998138428,3.6714088305943873e-06
98899,98900,98899,197799,50.47486686706543,3.6698918742390845e-06
99099,99100,99099,198199,50.56640601158142,3.6684024894023545e-06
99299,99300,99299,198599,50.65923309326172,3.6669233787449315e-06
99499,99500,99499,198999,50.75168299674988,3.665470817937386e-06
99700,99701,99700,199401,50.850322246551514,3.6640486061728827e-06
99900,99901,99900,199801,50.952394008636475,3.6625962913386964e-06
100100,100101,100100,200201,51.04625415802002,3.661321063926394e-06
100300,100301,100300,200601,51.14597702026367,3.659934498220359e-06
100501,100502,100501,201003,51.2496280670166,3.6583940046432007e-06
100701,100702,100701,201403,51.34889483451843,3.6570459840609714e-06
100901,100902,100901,201803,51.4476420879364,3.6555778345557384e-06
101101,101102,101101,202203,51.53963899612427,3.65425530159682e-06
101301,101302,101301,202603,51.63260793685913,3.6529769183013395e-06
101502,101503,101502,203005,51.72717595100403,3.651588252692143e-06
101702,101703,101702,203405,51.82353615760803,3.650338155017774e-06
101902,101903,101902,203805,51.91591691970825,3.6490016715319337e-06
102102,102103,102102,204205,52.010631799697876,3.6476743822881173e-06
102302,102303,102302,204605,52.11590003967285,3.6464075866002488e-06
102503,102504,102503,205007,52.2110378742218,3.645163129078619e-06
102703,102704,102703,205407,52.30600595474243,3.643813897321237e-06
102903,102904,102903,205807,52.39948797225952,3.6425627628613955e-06
103103,103104,103103,206207,52.49227809906006,3.6412924832709977e-06
103303,103304,103303,206607,52.58258509635925,3.6400597933845685e-06
103504,103505,103504,207009,52.68566703796387,3.6389025693785554e-06
103704,103705,103704,207409,52.77837896347046,3.637688045649134e-06
103904,103905,103904,207809,52.86756086349487,3.636410691344211e-06
104104,104105,104104,208209,52.95899319648743,3.6351880889918814e-06
104304,104305,104304,208609,53.04885292053223,3.63400220949961e-06
104505,104506,104505,209011,53.14626502990723,3.632792721563805e-06
104705,104706,104705,209411,53.2363121509552,3.631566200796507e-06
104905,104906,104905,209811,53.333500146865845,3.6304514597641224e-06
105105,105106,105105,210211,53.427687883377075,3.6292143445833866e-06
105305,105306,105305,210611,53.5181941986084,3.6280599779825227e-06
105506,105507,105506,211013,53.6130211353302,3.626989157960634e-06
105706,105707,105706,211413,53.70371413230896,3.6258268346509264e-06
105906,105907,105906,211813,53.795125007629395,3.6246556145840978e-06
106106,106107,106106,212213,53.88651490211487,3.623549306803784e-06
106306,106307,106306,212613,53.980369091033936,3.622456921551003e-06
106507,106508,106507,213015,54.074939012527466,3.6213720110268776e-06
106707,106708,106707,213415,54.16955900192261,3.62016283014433e-06
106907,106908,106907,213815,54.26261806488037,3.6190779435693513e-06
107107,107108,107107,214215,54.359132051467896,3.6180257979024736e-06
107307,107308,107307,214615,54.45151901245117,3.6169510374423863e-06
107508,107509,107508,215017,54.54325008392334,3.615847792170557e-06
107708,107709,107708,215417,54.634669065475464,3.614804081416602e-06
107908,107909,107908,215817,54.72487497329712,3.613776195877722e-06
108108,108109,108108,216217,54.82055115699768,3.6127350462912375e-06
108308,108309,108308,216617,54.913492918014526,3.6116533175993466e-06
108509,108510,108509,217019,55.00493407249451,3.61066190820256e-06
108709,108710,108709,217419,55.10102605819702,3.60959283690523e-06
108909,108910,108909,217819,55.19363808631897,3.6085558839492688e-06
109109,109110,109109,218219,55.289167165756226,3.6074692116373004e-06
109309,109310,109309,218619,55.385814905166626,3.6064728761455927e-06
109510,109511,109510,219021,55.487919092178345,3.605416999944293e-06
109710,109711,109710,219421,55.579545974731445,3.604413560242234e-06
109910,109911,109910,219821,55.67207908630371,3.603418617273633e-06
110110,110111,110110,220221,55.76504397392273,3.602393225901843e-06
110310,110311,110310,220621,55.856667041778564,3.6014218381734103e-06
110511,110512,110511,221023,55.94851303100586,3.600700056428718e-06
110711,110712,110711,221423,56.04057812690735,3.5993842837907464e-06
110911,110912,110911,221823,56.13319110870361,3.5984143936985385e-06
111111,111112,111111,222223,56.22398400306702,3.5974722266238937e-06
111311,111312,111311,222623,56.31700086593628,3.5967595894486207e-06
111512,111513,111512,223025,56.40873384475708,3.5955721846205844e-06
111712,111713,111712,223425,56.499176025390625,3.5945584812528503e-06
111912,111913,111912,223825,56.59226584434509,3.5936665258617684e-06
112112,112113,112112,224225,56.6836211681366,3.592655565972945e-06
112312,112313,112312,224625,56.777273178100586,3.591718297376623e-06
112513,112514,112513,225027,56.8686408996582,3.590736554979234e-06
112713,112714,112713,225427,56.96247601509094,3.5898088141995905e-06
112913,112914,112913,225827,57.05435585975647,3.5888654697869555e-06
113113,113114,113113,226227,57.148947954177856,3.5879380170002856e-06
113313,113314,113313,226627,57.24056100845337,3.5870165408366276e-06
113514,113515,113514,227029,57.333438873291016,3.586075454086718e-06
113714,113715,113714,227429,57.42562818527222,3.5851665726852584e-06
113914,113915,113914,227829,57.524746894836426,3.584284045528196e-06
114114,114115,114114,228229,57.61766600608826,3.5834424465347335e-06
114314,114315,114314,228629,57.71021509170532,3.582460661770281e-06
114515,114516,114515,229031,57.80681586265564,3.581598190738723e-06
114715,114716,114715,229431,57.89836597442627,3.580646366523325e-06
114915,114916,114915,229831,57.99176383018494,3.5797398065941318e-06
115115,115116,115115,230231,58.08562707901001,3.578802918227916e-06
115315,115316,115315,230631,58.177494049072266,3.5780069642737337e-06
115516,115517,115516,231033,58.26969790458679,3.5770515803358267e-06
115716,115717,115716,231433,58.36274003982544,3.5761837770838292e-06
115916,115917,115916,231833,58.453558921813965,3.5753204374720326e-06
116116,116117,116116,232233,58.544723987579346,3.5744395190576685e-06
116316,116317,116316,232633,58.63681888580322,3.5735904507546236e-06
116517,116518,116517,233035,58.7299702167511,3.5727045747248425e-06
116717,116718,116717,233435,58.822696924209595,3.571820613667159e-06
116917,116918,116917,233835,58.915359020233154,3.5710219655410136e-06
117117,117118,117117,234235,59.007988929748535,3.570291537889936e-06
117317,117318,117317,234635,59.10262703895569,3.5693396183529e-06
117518,117519,117518,235037,59.19489097595215,3.5684107862366385e-06
117718,117719,117718,235437,59.288946866989136,3.5676647279645713e-06
117918,117919,117918,235837,59.38119912147522,3.566792582555437e-06
118118,118119,118118,236237,59.473016023635864,3.5659263881836753e-06
118318,118319,118318,236637,59.56638312339783,3.5650234293002642e-06
118519,118520,118519,237039,59.667826890945435,3.5641751314567284e-06
118719,118720,118719,237439,59.76055121421814,3.563336753411786e-06
118919,118920,118919,237839,59.85114502906799,3.5624700222558714e-06
119119,119120,119119,238239,59.94211983680725,3.561674513359251e-06
119319,119320,119319,238639,60.032907009124756,3.5608745990155976e-06
119520,119521,119520,239041,60.12494897842407,3.560022096479922e-06
119720,119721,119720,239441,60.218767166137695,3.5593898354947857e-06
119920,119921,119920,239841,60.31383800506592,3.5584745937809444e-06
120120,120121,120120,240241,60.40705609321594,3.557593676248367e-06
120320,120321,120320,240641,60.4993531703949,3.5567668282299495e-06
120521,120522,120521,241043,60.59048104286194,3.555901939431318e-06
120721,120722,120721,241443,60.679245948791504,3.555086751142809e-06
120921,120922,120921,241843,60.77135109901428,3.5542912867220536e-06
121121,121122,121121,242243,60.86029505729675,3.5535031376142156e-06
121321,121322,121321,242643,60.947548151016235,3.5526661675162146e-06
121522,121523,121522,243045,61.03523087501526,3.551905502602422e-06
121722,121723,121722,243445,61.12284207344055,3.551087652116537e-06
121922,121923,121922,243845,61.21103096008301,3.5503198156791884e-06
122122,122123,122122,244245,61.30056691169739,3.5495609295052415e-06
122322,122323,122322,244645,61.39022612571716,3.5488026772929757e-06
122523,122524,122523,245047,61.478424072265625,3.5480119796001534e-06
122723,122724,122723,245447,61.565768003463745,3.547192604328507e-06
122923,122924,122923,245847,61.6547429561615,3.546387736032759e-06
123123,123124,123123,246247,61.74920916557312,3.5456493717712528e-06
123323,123324,123323,246647,61.838299036026,3.5448293149937176e-06
123524,123525,123524,247049,61.92569708824158,3.5440487908477966e-06
123724,123725,123724,247449,62.014272928237915,3.543368191925474e-06
123924,123925,123924,247849,62.102782011032104,3.542509218553008e-06
124124,124125,124124,248249,62.18991994857788,3.541721528580885e-06
124324,124325,124324,248649,62.27818489074707,3.541039301986417e-06
124525,124526,124525,249051,62.36692190170288,3.54014850858092e-06
124725,124726,124725,249451,62.45385003089905,3.5394631372012827e-06
124925,124926,124925,249851,62.541561126708984,3.5386925317015138e-06
125125,125126,125125,250251,62.63221096992493,3.5378831737959678e-06
125325,125326,125325,250651,62.720191955566406,3.537152504250966e-06
125526,125527,125526,251053,62.81426191329956,3.5362994818281e-06
125726,125727,125726,251453,62.904847145080566,3.535572000413214e-06
125926,125927,125926,251853,62.99170804023743,3.5347763929844403e-06
126126,126127,126126,252253,63.07954406738281,3.5340457596137737e-06
126326,126327,126326,252653,63.16828894615173,3.5332964728934487e-06
126527,126528,126527,253055,63.256393909454346,3.5326429391150837e-06
126727,126728,126727,253455,63.34591197967529,3.531792719119011e-06
126927,126928,126927,253855,63.43310904502869,3.5309849233837294e-06
127127,127128,127127,254255,63.52011322975159,3.530228588921692e-06
127327,127328,127327,254655,63.60719895362854,3.529431473946044e-06
127528,127529,127528,255057,63.695026874542236,3.5287003386970187e-06
127728,127729,127728,255457,63.79266715049744,3.5280125268634974e-06
127928,127929,127928,255857,63.885565996170044,3.5272725083081323e-06
128128,128129,128128,256257,63.97267508506775,3.526477265727934e-06
128328,128329,128328,256657,64.06014204025269,3.525748812844922e-06
128529,128530,128529,257059,64.15022110939026,3.5250033809509174e-06
128729,128730,128729,257459,64.23729300498962,3.524285184961569e-06
128929,128930,128929,257859,64.32784509658813,3.5238308557443216e-06
129129,129130,129129,258259,64.41509699821472,3.522803299949979e-06
129329,129330,129329,258659,64.50192999839783,3.522017013481699e-06
129530,129531,129530,259061,64.59017014503479,3.521299064603755e-06
129730,129731,129730,259461,64.67738914489746,3.5205674263314605e-06
129930,129931,129930,259861,64.76944303512573,3.5199178235738453e-06
130130,130131,130130,260261,64.86010789871216,3.5190710069940486e-06
130330,130331,130330,260661,64.95252394676208,3.5183700257661206e-06
130531,130532,130531,261063,65.04340291023254,3.5176945673851214e-06
130731,130732,130731,261463,65.13491106033325,3.5168878186808805e-06
130931,130932,130931,261863,65.22514986991882,3.5161579184222357e-06
131131,131132,131131,262263,65.31656503677368,3.5153908100359487e-06
131331,131332,131331,262663,65.4070680141449,3.514866690626913e-06
131532,131533,131532,263065,65.49560284614563,3.5139532039472525e-06
131732,131733,131732,263465,65.5883309841156,3.513289123403636e-06
131932,131933,131932,263865,65.67851209640503,3.5126876714394535e-06
132132,132133,132132,264265,65.77021598815918,3.5117701315830934e-06
132332,132333,132332,264665,65.86473202705383,3.511095852865735e-06
132533,132534,132533,265067,65.96084094047546,3.5103706977963687e-06
132733,132734,132733,265467,66.05109596252441,3.5096067222499512e-06
132933,132934,132933,265867,66.1447081565857,3.5088774444739407e-06
133133,133134,133133,266267,66.23631715774536,3.5081648227961693e-06
133333,133334,133333,266667,66.32828307151794,3.5075501746365935e-06
133534,133535,133534,267069,66.41893005371094,3.5067376452936556e-06
133734,133735,133734,267469,66.50920915603638,3.5060937908496315e-06
133934,133935,133934,267869,66.59984517097473,3.505328131593079e-06
134134,134135,134134,268269,66.69040608406067,3.504697321649805e-06
134334,134335,134334,268669,66.78409218788147,3.503972505804664e-06
134535,134536,134535,269071,66.87404799461365,3.503345646086937e-06
134735,134736,134735,269471,66.96305823326111,3.5024778995242773e-06
134935,134936,134935,269871,67.05193996429443,3.5019223167713573e-06
135135,135136,135135,270271,67.14177203178406,3.501066388453343e-06
135335,135336,135335,270671,67.23007202148438,3.500394387875641e-06
135536,135537,135536,271073,67.32238793373108,3.499689949140648e-06
135736,135737,135736,271473,67.41466212272644,3.4989808787122177e-06
135936,135937,135936,271873,67.505117893219,3.4981894468716895e-06
136136,136137,136136,272273,67.59568786621094,3.4974832107236417e-06
136336,136337,136336,272673,67.68640995025635,3.4967907541811196e-06
136537,136538,136537,273075,67.77853107452393,3.4960577457299842e-06
136737,136738,136737,273475,67.86736416816711,3.495398869756492e-06
136937,136938,136937,273875,67.96443486213684,3.494647282419294e-06
137137,137138,137137,274275,68.06065106391907,3.493932986909508e-06
137337,137338,137337,274675,68.15153503417969,3.493244886974424e-06
137538,137539,137538,275077,68.24282789230347,3.4925112060764606e-06
137738,137739,137738,275477,68.33789896965027,3.49191744435819e-06
137938,137939,137938,275877,68.4299430847168,3.4911165184422223e-06
138138,138139,138138,276277,68.52151393890381,3.490540132402268e-06
138338,138339,138338,276677,68.61695504188538,3.4897026097470855e-06
138539,138540,138539,277079,68.71215987205505,3.4890305090634606e-06
138739,138740,138739,277479,68.80822610855103,3.4883105292270884e-06
138939,138940,138939,277879,68.98308491706848,3.4876273836291153e-06
139139,139140,139139,278279,69.12741494178772,3.486919837310448e-06
139339,139340,139339,278679,69.23948216438293,3.4861955815432036e-06
139540,139541,139540,279081,69.3427619934082,3.4854673297202553e-06
139740,139741,139740,279481,69.50762391090393,3.48484303689197e-06
139940,139941,139940,279881,69.63860297203064,3.4840711036439993e-06
140140,140141,140140,280281,69.73347091674805,3.483416872278094e-06
140340,140341,140340,280681,69.82700300216675,3.4826981322866945e-06
140541,140542,140541,281083,69.92115497589111,3.4819924884594537e-06
140741,140742,140741,281483,70.01010990142822,3.4816334047995833e-06
140941,140942,140941,281883,70.11327004432678,3.4805962912100866e-06
141141,141142,141141,282283,70.20310711860657,3.479925762186245e-06
141341,141342,141341,282683,70.29368495941162,3.479219174555366e-06
141542,141543,141542,283085,70.38299584388733,3.4785308432079906e-06
141742,141743,141742,283485,70.47344994544983,3.477831626322073e-06
141942,141943,141942,283885,70.5667769908905,3.4771412674857387e-06
142142,142143,142142,284285,70.65889811515808,3.4764415266969835e-06
142342,142343,142342,284685,70.74912405014038,3.4758578626966332e-06
142543,142544,142543,285087,70.83870315551758,3.4751026507959646e-06
142743,142744,142743,285487,70.93199706077576,3.4743682537944623e-06
142943,142944,142943,285887,71.02158904075623,3.4737682532478783e-06
143143,143144,143143,286287,71.11590099334717,3.473027417084298e-06
143343,143344,143343,286687,71.2061722278595,3.472318797698662e-06
143544,143545,143544,287089,71.29559588432312,3.471789361445389e-06
143744,143745,143744,287489,71.38512706756592,3.470935760410887e-06
143944,143945,143944,287889,71.47452807426453,3.4703682123404705e-06
144144,144145,144144,288289,71.56584000587463,3.469566040773638e-06
144344,144345,144344,288689,71.65932703018188,3.4689274390683853e-06
144545,144546,144545,289091,71.74756813049316,3.46819572027044e-06
144745,144746,144745,289491,71.83584499359131,3.467510667838851e-06
144945,144946,144945,289891,71.92568492889404,3.46697663083158e-06
145145,145146,145145,290291,72.01532316207886,3.4661892726735403e-06
145345,145346,145345,290691,72.10860705375671,3.46546081689497e-06
145546,145547,145546,291093,72.20680212974548,3.464950685002346e-06
145746,145747,145746,291493,72.29694414138794,3.464207398085972e-06
145946,145947,145946,291893,72.38726902008057,3.463449659072743e-06
146146,146147,146146,292293,72.47705221176147,3.462777777466818e-06
146346,146347,146346,292693,72.56691408157349,3.462106263862404e-06
146547,146548,146547,293095,72.65774011611938,3.4614232802677062e-06
146747,146748,146747,293495,72.7487359046936,3.46078491646456e-06
146947,146948,146947,293895,72.83910298347473,3.4600821704532618e-06
147147,147148,147147,294295,72.9296510219574,3.4593711530446307e-06
147347,147348,147347,294695,73.02011799812317,3.4588003775604815e-06
147548,147549,147548,295097,73.11458921432495,3.458024191135792e-06
147748,147749,147748,295497,73.20909786224365,3.457344878006345e-06
147948,147949,147948,295897,73.30163288116455,3.4566604769453155e-06
148148,148149,148148,296297,73.45096015930176,3.455988225477692e-06
148348,148349,148348,296697,73.58246397972107,3.4553322855737114e-06
148549,148550,148549,297099,73.68294405937195,3.454642903832826e-06
148749,148750,148749,297499,73.78631496429443,3.4539444481618764e-06
148949,148950,148949,297899,73.88309097290039,3.453271672964887e-06
149149,149150,149149,298299,74.05168890953064,3.452575770284382e-06
149349,149350,149349,298699,74.15095114707947,3.451926121333366e-06
149550,149551,149550,299101,74.25214004516602,3.451228768828515e-06
149750,149751,149750,299501,74.3514051437378,3.4506536374759687e-06
149950,149951,149950,299901,74.44615125656128,3.450097155564441e-06
150150,150151,150150,300301,74.54742193222046,3.44924778743016e-06
150350,150351,150350,300701,74.65680718421936,3.448705982265692e-06
150551,150552,150551,301103,74.76267600059509,3.448076620390334e-06
150751,150752,150751,301503,74.85411405563354,3.4471931590768103e-06
150951,150952,150951,301903,74.94694089889526,3.446629173176605e-06
151151,151152,151151,302303,75.03963899612427,3.4458867574480568e-06
151351,151352,151351,302703,75.13047122955322,3.4454103991922682e-06
151552,151553,151552,303105,75.22581815719604,3.444519252877284e-06
151752,151753,151752,303505,75.31673288345337,3.4439563862612033e-06
151952,151953,151952,303905,75.40548920631409,3.4431652800843435e-06
152152,152153,152152,304305,75.4962990283966,3.442520922807105e-06
152352,152353,152352,304705,75.5882978439331,3.4420042070252237e-06
152553,152554,152553,305107,75.75744724273682,3.4411280171572528e-06
152753,152754,152753,305507,75.89748811721802,3.440526233403317e-06
152953,152954,152953,305907,76.01344299316406,3.4397724821426077e-06
153153,153154,153153,306307,76.1408360004425,3.439178079967985e-06
153353,153354,153353,306707,76.24802994728088,3.438604152072623e-06
153554,153555,153554,307109,76.37207913398743,3.4378544233462346e-06
153754,153755,153754,307509,76.50334405899048,3.437129355774005e-06
153954,153955,153954,307909,76.7069640159607,3.436441927624496e-06
154154,154155,154154,308309,76.87808513641357,3.435817628689162e-06
154354,154355,154354,308709,77.00418210029602,3.4351241098725588e-06
154555,154556,154555,309111,77.11921715736389,3.4344584106569338e-06
154755,154756,154755,309511,77.23233103752136,3.4337817002090034e-06
154955,154956,154955,309911,77.40522313117981,3.43322308805101e-06
155155,155156,155155,310311,77.50960993766785,3.4324670872371094e-06
155355,155356,155355,310711,77.63313412666321,3.4319358885620312e-06
155556,155557,155556,311113,77.74723196029663,3.431184867085261e-06
155756,155757,155756,311513,77.87779402732849,3.4304567587841552e-06
155956,155957,155956,311913,78.00778484344482,3.429770336676518e-06
156156,156157,156156,312313,78.20791602134705,3.429166330153163e-06
156356,156357,156356,312713,78.31961107254028,3.428443927604507e-06
156557,156558,156557,313115,78.4688229560852,3.4278053905641005e-06
156757,156758,156757,313515,78.56340098381042,3.4271514408267063e-06
156957,156958,156957,313915,78.67934679985046,3.4264759326647524e-06
157157,157158,157157,314315,78.77258801460266,3.4257553646262294e-06
157357,157358,157357,314715,78.86126399040222,3.425140726683123e-06
157558,157559,157558,315117,79.29195404052734,3.424503995448006e-06
157758,157759,157758,315517,79.41204810142517,3.4237592836184784e-06
157958,157959,157958,315917,79.56829309463501,3.4232632918188655e-06
158158,158159,158158,316317,79.73529601097107,3.4224184305079447e-06
158358,158359,158358,316717,79.86795592308044,3.4217951124150534e-06
158559,158560,158559,317119,79.96277713775635,3.4211278757330945e-06
158759,158760,158759,317519,80.11604714393616,3.4205666996138646e-06
158959,158960,158959,317919,80.26785516738892,3.419816390514421e-06
159159,159160,159159,318319,80.43250513076782,3.4192576775609206e-06
159359,159360,159359,318719,80.63040208816528,3.4185710765626936e-06
159560,159561,159560,319121,80.7477879524231,3.417930451283167e-06
159760,159761,159760,319521,80.86276412010193,3.4171622995098387e-06
159960,159961,159960,319921,81.0679018497467,3.4165339290644833e-06
160160,160161,160160,320321,81.21168613433838,3.4159499058822118e-06
160360,160361,160360,320721,81.31885099411011,3.415184119116376e-06
160561,160562,160561,321123,81.4782178401947,3.414617612269566e-06
160761,160762,160761,321523,81.58495092391968,3.413897615677291e-06
160961,160962,160961,321923,81.67347979545593,3.4132468791163803e-06
161161,161162,161161,322323,81.76309490203857,3.412644737022177e-06
161361,161362,161361,322723,81.92263507843018,3.4119157942788337e-06
161562,161563,161562,323125,82.04798197746277,3.4112562859757845e-06
161762,161763,161762,323525,82.14724087715149,3.4106295803551933e-06
161962,161963,161962,323925,82.24423384666443,3.409976142059682e-06
162162,162163,162162,324325,82.35847592353821,3.409303331091664e-06
162362,162363,162362,324725,82.50785899162292,3.408683645185493e-06
162563,162564,162563,325127,82.59557914733887,3.408024208394193e-06
162763,162764,162763,325527,82.68590688705444,3.4073412021995734e-06
162963,162964,162963,325927,82.78439283370972,3.4066787874865304e-06
163163,163164,163163,326327,82.88073015213013,3.4060242750313874e-06
163363,163364,163363,326727,83.01500415802002,3.4054648573308787e-06
163564,163565,163564,327129,83.13153982162476,3.4047021201642704e-06
163764,163765,163764,327529,83.24413204193115,3.404092126762162e-06
163964,163965,163964,327929,83.34336304664612,3.4034196099975267e-06
164164,164165,164164,328329,83.45004200935364,3.4027616254540074e-06
164364,164365,164364,328729,83.59796500205994,3.4021199457661598e-06
164565,164566,164565,329131,83.68722414970398,3.401434743711699e-06
164765,164766,164765,329531,83.78665208816528,3.400796263594804e-06
164965,164966,164965,329931,83.91025304794312,3.4002003638651694e-06
165165,165166,165165,330331,84.00670504570007,3.39944032626465e-06
165365,165366,165365,330731,84.10822701454163,3.3987961480092597e-06
165566,165567,165566,331133,84.2057409286499,3.3981523763085232e-06
165766,165767,165766,331533,84.31247901916504,3.397519158592078e-06
165966,165967,165966,331933,84.52383303642273,3.3969279719757815e-06
166166,166167,166166,332333,84.61318612098694,3.396430521283752e-06
166366,166367,166366,332733,84.70151591300964,3.395568324944846e-06
166567,166568,166567,333135,84.79836702346802,3.394907248876583e-06
166767,166768,166767,333535,84.89627599716187,3.3942424082397956e-06
166967,166968,166967,333935,84.98455500602722,3.3936537878528283e-06
167167,167168,167167,334335,85.06939911842346,3.392969036862157e-06
167367,167368,167367,334735,85.15993595123291,3.392276909574587e-06
167568,167569,167568,335137,85.24653697013855,3.3916397940340583e-06
167768,167769,167768,335537,85.33594393730164,3.390953520046819e-06
167968,167969,167968,335937,85.42914915084839,3.3903391600834536e-06
168168,168169,168168,336337,85.51950097084045,3.3896361395323865e-06
168368,168369,168368,336737,85.68872594833374,3.389047473624733e-06
168569,168570,168569,337139,85.82596611976624,3.388346064336822e-06
168769,168770,168769,337539,85.9300971031189,3.387695292678486e-06
168969,168970,168969,337939,86.02599596977234,3.3870536001885914e-06
169169,169170,169169,338339,86.18377590179443,3.3864051699603985e-06
169369,169370,169369,338739,86.31375789642334,3.3858812051130585e-06
169570,169571,169570,339141,86.40387296676636,3.385137217178538e-06
169770,169771,169770,339541,86.49593806266785,3.384422155807015e-06
169970,169971,169970,339941,86.58613395690918,3.3838229293431887e-06
170170,170171,170170,340341,86.70032620429993,3.3831706604989417e-06
170370,170371,170370,340741,86.79628586769104,3.3825618317817883e-06
170571,170572,170571,341143,86.89981698989868,3.3818671842808877e-06
170771,170772,170771,341543,87.03592300415039,3.381204478871493e-06
170971,170972,170971,341943,87.14048886299133,3.3806274435162043e-06
171171,171172,171171,342343,87.25238800048828,3.379989852001807e-06
171371,171372,171371,342743,87.36700797080994,3.3793206599910786e-06
171572,171573,171572,343145,87.54483914375305,3.3786743658935063e-06
171772,171773,171772,343545,87.65336894989014,3.3779683176251157e-06
171972,171973,171972,343945,87.74472904205322,3.3773347349614195e-06
172172,172173,172172,344345,87.83460307121277,3.376685123170381e-06
172372,172373,172372,344745,87.9234230518341,3.3760701628044765e-06
172573,172574,172573,345147,88.01237916946411,3.3754093398700396e-06
172773,172774,172773,345547,88.12131714820862,3.3747875571274564e-06
172973,172974,172973,345947,88.21407103538513,3.374100107905853e-06
173173,173174,173173,346347,88.3344419002533,3.37352526932218e-06
173373,173374,173373,346747,88.46120500564575,3.372819970962153e-06
173574,173575,173574,347149,88.5717089176178,3.3721750902713298e-06
173774,173775,173774,347549,88.68049001693726,3.3714706506108707e-06
173974,173975,173974,347949,88.83451104164124,3.370860532882936e-06
174174,174175,174174,348349,88.95465016365051,3.370212253199084e-06
174374,174375,174374,348749,89.08841109275818,3.3695445575166e-06
174575,174576,174575,349151,89.19369006156921,3.368887968672079e-06
174775,174776,174775,349551,89.30470490455627,3.3682047008774316e-06
174975,174976,174975,349951,89.42561411857605,3.367564154279671e-06
175175,175176,175175,350351,89.56946396827698,3.3669485454626686e-06
175375,175376,175375,350751,89.72860789299011,3.366281638626052e-06
175576,175577,175576,351153,89.83069801330566,3.3656151729741273e-06
175776,175777,175776,351553,89.92696905136108,3.3650546492546464e-06
175976,175977,175976,351953,90.01978492736816,3.3643535442588354e-06
176176,176177,176176,352353,90.11235809326172,3.3637086342624873e-06
176376,176377,176376,352753,90.22169017791748,3.363109537758372e-06
176577,176578,176577,353155,90.31638693809509,3.3624978655769054e-06
176777,176778,176777,353555,90.41806197166443,3.3617900914369723e-06
176977,176978,176977,353955,90.51583504676819,3.3611699055292966e-06
177177,177178,177177,354355,90.61724996566772,3.360552755127972e-06
177377,177378,177377,354755,90.74362111091614,3.3599091827120814e-06
177578,177579,177578,355157,90.87839317321777,3.3592230072068913e-06
177778,177779,177778,355557,91.01897311210632,3.358540831131648e-06
177978,177979,177978,355957,91.15695786476135,3.3579036857553855e-06
178178,178179,178178,356357,91.2556369304657,3.357255515194151e-06
178378,178379,178378,356757,91.36409997940063,3.3565629603326405e-06
178579,178580,178579,357159,91.50692820549011,3.356044927325285e-06
178779,178780,178779,357559,91.65913605690002,3.3552906279575177e-06
178979,178980,178979,357959,91.7627329826355,3.354654590387562e-06
179179,179180,179179,358359,91.86067199707031,3.3540145671172687e-06
179379,179380,179379,358759,91.9573540687561,3.3534061305991415e-06
179580,179581,179580,359161,92.05357098579407,3.3527393655184977e-06
179780,179781,179780,359561,92.15118622779846,3.3521298543957716e-06
179980,179981,179980,359961,92.24879884719849,3.3515517004098762e-06
180180,180181,180180,360361,92.34737706184387,3.350844153883206e-06
180380,180381,180380,360761,92.44541907310486,3.350250965202778e-06
180581,180582,180581,361163,92.6175742149353,3.349539123676289e-06
180781,180782,180781,361563,92.79039883613586,3.3488541884208035e-06
180981,180982,180981,361963,93.02943992614746,3.348261176514396e-06
181181,181182,181181,362363,93.25762104988098,3.347579497542345e-06
181381,181382,181381,362763,93.46082305908203,3.3469339322649455e-06
181582,181583,181582,363165,93.68392491340637,3.346320720681804e-06
181782,181783,181782,363565,93.88377499580383,3.345695141641126e-06
181982,181983,181982,363965,94.10338187217712,3.345031785873872e-06
182182,182183,182182,364365,94.26099300384521,3.3444012427202306e-06
182382,182383,182382,364765,94.47114586830139,3.3437329965697242e-06
182583,182584,182583,365167,94.63372302055359,3.3432315057821984e-06
182783,182784,182783,365567,94.7783579826355,3.3424697200203775e-06
182983,182984,182983,365967,94.91957712173462,3.3418072335729596e-06
183183,183184,183183,366367,95.0609860420227,3.3412012115310623e-06
183383,183384,183383,366767,95.19886517524719,3.340525883947471e-06
183584,183585,183584,367169,95.3376088142395,3.3399139620384896e-06
183784,183785,183784,367569,95.48006916046143,3.339290543959559e-06
183984,183985,183984,367969,95.6169068813324,3.3386055654649744e-06
184184,184185,184184,368369,95.75215601921082,3.3380268300804425e-06
184384,184385,184384,368769,95.88416719436646,3.3373190201738643e-06
184585,184586,184585,369171,96.0176329612732,3.336809403604226e-06
184785,184786,184785,369571,96.15019488334656,3.3360265989773456e-06
184985,184986,184985,369971,96.28283905982971,3.3354472901500613e-06
185185,185186,185185,370371,96.41452598571777,3.3347707424439878e-06
185385,185386,185385,370771,96.54717206954956,3.334286188686744e-06
185586,185587,185586,371173,96.67994117736816,3.3336551860262184e-06
185786,185787,185786,371573,96.81164479255676,3.332894296914425e-06
185986,185987,185986,371973,96.94526696205139,3.332280134855741e-06
186186,186187,186186,372373,97.07758402824402,3.3315978112037023e-06
186386,186387,186386,372773,97.20597815513611,3.330934864024138e-06
186587,186588,186587,373175,97.33349084854126,3.3302963769696974e-06
186787,186788,186787,373575,97.46547102928162,3.329680423230011e-06
186987,186988,186987,373975,97.6000440120697,3.3290100396817725e-06
187187,187188,187187,374375,97.72885394096375,3.3284266386005066e-06
187387,187388,187387,374775,97.85769319534302,3.3277224848510946e-06
187588,187589,187588,375177,97.98953914642334,3.327182233113577e-06
187788,187789,187788,375577,98.11994218826294,3.32649268491151e-06
187988,187989,187988,375977,98.2512149810791,3.3258127152538236e-06
188188,188189,188188,376377,98.3833909034729,3.325171560250952e-06
188388,188389,188388,376777,98.51320290565491,3.3246988841601044e-06
188589,188590,188589,377179,98.64458012580872,3.3239022829689867e-06
188789,188790,188789,377579,98.77505898475647,3.3233112026639262e-06
188989,188990,188989,377979,98.90650606155396,3.3226153634903792e-06
189189,189190,189189,378379,99.03715395927429,3.3219782722871176e-06
189389,189390,189389,378779,99.1705892086029,3.3215512432829327e-06
189590,189591,189590,379181,99.30200815200806,3.3207039505051247e-06
189790,189791,189790,379581,99.43993282318115,3.320065171092034e-06
189990,189991,189990,379981,99.5920250415802,3.319457993469332e-06
190190,190191,190190,380381,99.73626112937927,3.318869819007809e-06
190390,190391,190390,380781,99.88042211532593,3.3181900806196383e-06
190591,190592,190591,381183,100.0255401134491,3.3175315945672974e-06
190791,190792,190791,381583,100.2519862651825,3.3168980669266286e-06
190991,190992,190991,381983,100.47894501686096,3.3162627023978704e-06
191191,191192,191191,382383,100.64531302452087,3.3156389721718295e-06
191391,191392,191391,382783,100.8662462234497,3.3150104793049094e-06
191592,191593,191592,383185,101.01458716392517,3.314355621055969e-06
191792,191793,191792,383585,101.17182612419128,3.3137832187968524e-06
191992,191993,191992,383985,101.33043909072876,3.3131101559246675e-06
192192,192193,192192,384385,101.47556805610657,3.3124726124379095e-06
192392,192393,192392,384785,101.6245949268341,3.3118468889391635e-06
192593,192594,192593,385187,101.77484583854675,3.3112598741459983e-06
192793,192794,192793,385587,101.91741418838501,3.310589778153652e-06
192993,192994,192993,385987,102.06255602836609,3.3099617171187286e-06
193193,193194,193193,386387,102.2122311592102,3.309325277507578e-06
193393,193394,193393,386787,102.35639119148254,3.308688425381222e-06
193594,193595,193594,387189,102.50137710571289,3.3081905701703216e-06
193794,193795,193794,387589,102.64424705505371,3.307494560084455e-06
193994,193995,193994,387989,102.78581094741821,3.3068319216605577e-06
194194,194195,194194,388389,102.92579102516174,3.3061964692855746e-06
194394,194395,194394,388789,103.06817102432251,3.3055793426945365e-06
194595,194596,194595,389191,103.21387100219727,3.3050041782001423e-06
194795,194796,194795,389591,103.3535668849945,3.3042669867422242e-06
194995,194996,194995,389991,103.49243688583374,3.303642429415485e-06
195195,195196,195195,390391,103.62884092330933,3.3029945056986474e-06
195395,195396,195395,390791,103.7712790966034,3.3023578143166874e-06
195596,195597,195596,391193,103.90990614891052,3.301709350255027e-06
195796,195797,195796,391593,104.04524993896484,3.301125447554811e-06
195996,195997,195996,391993,104.18705296516418,3.300442308385055e-06
196196,196197,196196,392393,104.32571482658386,3.2998402298932846e-06
196396,196397,196396,392793,104.4634599685669,3.2992563449047137e-06
196597,196598,196597,393195,104.60139584541321,3.2986100697137956e-06
196797,196798,196797,393595,104.73679614067078,3.2979295409922413e-06
196997,196998,196997,393995,104.87557291984558,3.297295796262986e-06
197197,197198,197197,394395,105.02048707008362,3.296665564859316e-06
197397,197398,197397,394795,105.15401315689087,3.296059796886112e-06
197598,197599,197598,395197,105.29481792449951,3.295385729088287e-06
197798,197799,197798,395597,105.43347597122192,3.2947669303936944e-06
197998,197999,197998,395997,105.58395481109619,3.2941387721313485e-06
198198,198199,198198,396397,105.71854400634766,3.293536489326479e-06
198398,198399,198398,396797,105.8626868724823,3.2929934109579766e-06
198599,198600,198599,397199,106.00780010223389,3.2923666886425277e-06
198799,198800,198799,397599,106.14717888832092,3.2916220904989886e-06
198999,199000,198999,397999,106.28946495056152,3.2909945986226353e-06
199199,199200,199199,398399,106.42613387107849,3.2903488078438487e-06
199399,199400,199399,398799,106.56055402755737,3.289723177103505e-06
199600,199601,199600,399201,106.74682593345642,3.2890853061528397e-06
199800,199801,199800,399601,107.0596330165863,3.288488741848778e-06
200000,200001,200000,400001,107.24130702018738,3.287916130847992e-06


==> extragradient/plot_data/bilinear_matrix_game_n500/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.001096963882446289,2.018959020339561
100,201,200,401,0.12761402130126953,0.04084193889187754
200,401,400,801,0.24407100677490234,0.01555572904704933
300,601,600,1201,0.3618738651275635,0.008941559671892264
400,801,800,1601,0.5734660625457764,0.005957710393872965
501,1003,1002,2005,0.7021570205688477,0.004080388626738635
601,1203,1202,2405,0.8251359462738037,0.003044183482286378
701,1403,1402,2805,0.9428930282592773,0.00247078219342337
801,1603,1602,3205,1.071336030960083,0.002022425653118514
901,1803,1802,3605,1.2060868740081787,0.0017090990324214828
1001,2003,2002,4005,1.3234241008758545,0.0014375084752964995
1101,2203,2202,4405,1.4424350261688232,0.0012047380988628406
1201,2403,2402,4805,1.5759758949279785,0.001000692926912849
1301,2603,2602,5205,1.6909470558166504,0.0008161398070111659
1401,2803,2802,5605,1.817399024963379,0.0007105240339073027
1502,3005,3004,6009,1.9883739948272705,0.0006406047458752685
1602,3205,3204,6409,2.113914966583252,0.0005873580809235912
1702,3405,3404,6809,2.2286458015441895,0.0005382536666146199
1802,3605,3604,7209,2.34254789352417,0.0004953501567577407
1902,3805,3804,7609,2.462355852127075,0.00046283265676205554
2002,4005,4004,8009,2.5771610736846924,0.0004308549629022895
2102,4205,4204,8409,2.6892149448394775,0.0003999154365291184
2202,4405,4404,8809,2.8060190677642822,0.00037725255875169743
2302,4605,4604,9209,2.9175941944122314,0.0003527435669886361
2402,4805,4804,9609,3.033135175704956,0.0003335273689751663
2503,5007,5006,10013,3.145364999771118,0.00031945940005734464
2603,5207,5206,10413,3.2616031169891357,0.00030878973556726564
2703,5407,5406,10813,3.381549119949341,0.0003000156905100278
2803,5607,5606,11213,3.507230043411255,0.00029252572517975546
2903,5807,5806,11613,3.635338068008423,0.00028541420036607454
3003,6007,6006,12013,3.7633018493652344,0.0002780152490870146
3103,6207,6206,12413,3.8923110961914062,0.00027195002345469855
3203,6407,6406,12813,4.032411813735962,0.00026673775102073016
3303,6607,6606,13213,4.160904884338379,0.00026209269718888097
3403,6807,6806,13613,4.288547992706299,0.00025787167822761395
3504,7009,7008,14017,4.412109136581421,0.00025394578198297755
3604,7209,7208,14417,4.537891149520874,0.00025011718889721537
3704,7409,7408,14817,4.669328927993774,0.0002467056013739032
3804,7609,7608,15217,4.807438135147095,0.00024351263461413038
3904,7809,7808,15617,4.935776948928833,0.00024048591179458707
4004,8009,8008,16017,5.0740790367126465,0.00023752401694437778
4104,8209,8208,16417,5.213096857070923,0.00023457721923087589
4204,8409,8408,16817,5.316133975982666,0.00023189293501112748
4304,8609,8608,17217,5.406888961791992,0.00022910798042041975
4404,8809,8808,17617,5.49542498588562,0.00022619918421695374
4505,9011,9010,18021,5.580489873886108,0.0002230343272817675
4605,9211,9210,18421,5.669863939285278,0.00022034767502957447
4705,9411,9410,18821,5.756553888320923,0.0002178537931555071
4805,9611,9610,19221,5.8356359004974365,0.00021549280886485868
4905,9811,9810,19621,5.918337106704712,0.00021323705999951907
5005,10011,10010,20021,6.002753973007202,0.00021107038667084828
5105,10211,10210,20421,6.103009939193726,0.00020898191834835915
5205,10411,10410,20821,6.193850994110107,0.0002069636366998869
5305,10611,10610,21221,6.277092933654785,0.00020500924417355266
5405,10811,10810,21621,6.358474016189575,0.00020311357261230275
5506,11013,11012,22025,6.441426992416382,0.00020125409421659746
5606,11213,11212,22425,6.52184796333313,0.000199463812585603
5706,11413,11412,22825,6.608471155166626,0.00019772072266799426
5806,11613,11612,23225,6.698142051696777,0.00019602185970323322
5906,11813,11812,23625,6.781621932983398,0.00019436456045111267
6006,12013,12012,24025,6.869600057601929,0.00019226895881548032
6106,12213,12212,24425,6.955971002578735,0.00018981336384564818
6206,12413,12412,24825,7.039137125015259,0.00018778452212550104
6306,12613,12612,25225,7.1226561069488525,0.00018589168393157325
6406,12813,12812,25625,7.205045938491821,0.00018405691086032967
6507,13015,13014,26029,7.289658784866333,0.00018229450115027232
6607,13215,13214,26429,7.376216173171997,0.00018061323138483316
6707,13415,13414,26829,7.46609902381897,0.00017896837070119164
6807,13615,13614,27229,7.558402061462402,0.00017670539366986823
6907,13815,13814,27629,7.649850845336914,0.00017394478665026857
7007,14015,14014,28029,7.731376886367798,0.00017182380289514751
7107,14215,14214,28429,7.814044952392578,0.00016995140199686445
7207,14415,14414,28829,7.89528489112854,0.00016822996598922252
7307,14615,14614,29229,7.977820873260498,0.00016600502050577174
7407,14815,14814,29629,8.066671133041382,0.00016417365369737495
7508,15017,15016,30033,8.16715383529663,0.00016248289306673215
7608,15217,15216,30433,8.261332988739014,0.00016090886540011637
7708,15417,15416,30833,8.347661972045898,0.0001588388697985169
7808,15617,15616,31233,8.440347909927368,0.00015716504752308173
7908,15817,15816,31633,8.525253057479858,0.00015560807575707016
8008,16017,16016,32033,8.60353398323059,0.0001528670951392979
8108,16217,16216,32433,8.677960872650146,0.0001508824226984641
8208,16417,16416,32833,8.75490403175354,0.00014869762396062543
8308,16617,16616,33233,8.831784963607788,0.00014660531424563205
8408,16817,16816,33633,8.907333850860596,0.00014472799576799907
8509,17019,17018,34037,8.987329006195068,0.00014295922339428892
8609,17219,17218,34437,9.066649198532104,0.0001412736273534982
8709,17419,17418,34837,9.146150827407837,0.0001396714101891978
8809,17619,17618,35237,9.220611095428467,0.00013813795600318
8909,17819,17818,35637,9.300578117370605,0.00013538373808574897
9009,18019,18018,36037,9.381643056869507,0.00013331524081584936
9109,18219,18218,36437,9.46270203590393,0.0001315176266269928
9209,18419,18418,36837,9.53578805923462,0.00012838146992159456
9309,18619,18618,37237,9.61345100402832,0.0001260062401086033
9409,18819,18818,37637,9.691370964050293,0.000123989736577564
9510,19021,19020,38041,9.76991319656372,0.0001221400303066318
9610,19221,19220,38441,9.845095872879028,0.0001204386966298002
9710,19421,19420,38841,9.917457818984985,0.00011847239407814625
9810,19621,19620,39241,9.993470907211304,0.00011669918825553777
9910,19821,19820,39641,10.07895302772522,0.00011274641903217324
10010,20021,20020,40041,10.155710935592651,0.00011039424919270669
10110,20221,20220,40441,10.230703830718994,0.00010842101331861896
10210,20421,20420,40841,10.312434911727905,0.0001056460432049642
10310,20621,20620,41241,10.391633987426758,0.0001034347785040179
10410,20821,20820,41641,10.471705198287964,0.00010121426707386297
10511,21023,21022,42045,10.551375150680542,9.88379844340756e-05
10611,21223,21222,42445,10.623746156692505,9.691614316935306e-05
10711,21423,21422,42845,10.695191144943237,9.51729702356169e-05
10811,21623,21622,43245,10.768929958343506,9.355874460556968e-05
10911,21823,21822,43645,10.838359117507935,9.195903659656644e-05
11011,22023,22022,44045,10.9112389087677,9.044062572871737e-05
11111,22223,22222,44445,10.9878249168396,8.760072395653058e-05
11211,22423,22422,44845,11.063947916030884,8.501766878337613e-05
11311,22623,22622,45245,11.14454197883606,8.292729869838731e-05
11411,22823,22822,45645,11.220165967941284,8.10564411007725e-05
11512,23025,23024,46049,11.293896913528442,7.89596690741875e-05
11612,23225,23224,46449,11.370150804519653,7.709389597231927e-05
11712,23425,23424,46849,11.45893406867981,7.544918173016605e-05
11812,23625,23624,47249,11.55593490600586,7.397387281337675e-05
11912,23825,23824,47649,11.664345026016235,7.25963281164493e-05
12012,24025,24024,48049,11.774802923202515,7.129342706426366e-05
12112,24225,24224,48449,11.88359808921814,6.997551128540555e-05
12212,24425,24424,48849,11.99154782295227,6.870086322848533e-05
12312,24625,24624,49249,12.089431047439575,6.749927088782142e-05
12412,24825,24824,49649,12.19192910194397,6.532043439414624e-05
12513,25027,25026,50053,12.31520700454712,6.377417764162247e-05
12613,25227,25226,50453,12.4426429271698,6.241931681348971e-05
12713,25427,25426,50853,12.590233087539673,6.117000796872597e-05
12813,25627,25626,51253,12.708111763000488,5.9999357950401774e-05
12913,25827,25826,51653,12.784279108047485,5.8892075906161434e-05
13013,26027,26026,52053,12.860136985778809,5.783806989101728e-05
13113,26227,26226,52453,12.934285163879395,5.683013725086848e-05
13213,26427,26426,52853,13.010757207870483,5.586287849136061e-05
13313,26627,26626,53253,13.08290410041809,5.493210368684028e-05
13413,26827,26826,53653,13.154614925384521,5.40344745752552e-05
13514,27029,27028,54057,13.226295948028564,5.315874701548238e-05
13614,27229,27228,54457,13.297316789627075,5.231999088587542e-05
13714,27429,27428,54857,13.367642164230347,5.150748953360285e-05
13814,27629,27628,55257,13.440670013427734,5.071961773190266e-05
13914,27829,27828,55657,13.511812210083008,4.9954964822641746e-05
14014,28029,28028,56057,13.587191104888916,4.9212291176279406e-05
14114,28229,28228,56457,13.666639804840088,4.8490495271269185e-05
14214,28429,28428,56857,13.87378191947937,4.778858852014829e-05
14314,28629,28628,57257,13.972169876098633,4.710567581298244e-05
14414,28829,28828,57657,14.052112817764282,4.6440940328542634e-05
14515,29031,29030,58061,14.130964994430542,4.5787244079736674e-05
14615,29231,29230,58461,14.214099884033203,4.515683226577822e-05
14715,29431,29430,58861,14.293139934539795,4.454250253990974e-05
14815,29631,29630,59261,14.368993997573853,4.394365350429401e-05
14915,29831,29830,59661,14.445281028747559,4.335972145555563e-05
15015,30031,30030,60061,14.53045392036438,4.279017615475833e-05
15115,30231,30230,60461,14.612350940704346,4.2234517292302766e-05
15215,30431,30430,60861,14.690605163574219,4.169227150309635e-05
15315,30631,30630,61261,14.767595052719116,4.116298982875498e-05
15415,30831,30830,61661,14.84438705444336,4.064624553921866e-05
15516,31033,31032,62065,14.920983076095581,4.013664605096901e-05
15616,31233,31232,62465,14.998863935470581,3.96438916138613e-05
15716,31433,31432,62865,15.075066089630127,3.916250645932755e-05
15816,31633,31632,63265,15.149865865707397,3.8692136325430465e-05
15916,31833,31832,63665,15.223530054092407,3.823244181240052e-05
16016,32033,32032,64065,15.296606063842773,3.778309738033774e-05
16116,32233,32232,64465,15.370474100112915,3.7343790450688504e-05
16216,32433,32432,64865,15.449031829833984,3.69142205982145e-05
16316,32633,32632,65265,15.528342008590698,3.6494098819374294e-05
16416,32833,32832,65665,15.601690769195557,3.6083146870131576e-05
16517,33035,33034,66069,15.675189971923828,3.5677120231280035e-05
16617,33235,33234,66469,15.749475002288818,3.528379843960052e-05
16717,33435,33434,66869,15.828022003173828,3.4898868073149153e-05
16817,33635,33634,67269,15.908409118652344,3.452208846989514e-05
16917,33835,33834,67669,16.004122972488403,3.4153227173809356e-05
17017,34035,34034,68069,16.09199094772339,3.379205954143965e-05
17117,34235,34234,68469,16.17581009864807,3.3438368377594996e-05
17217,34435,34434,68869,16.25357484817505,3.309194359746961e-05
17317,34635,34634,69269,16.334832906723022,3.2752581913295634e-05
17417,34835,34834,69669,16.415905952453613,3.242008654192568e-05
17518,35037,35036,70073,16.49494194984436,3.2091041818962486e-05
17618,35237,35236,70473,16.572021007537842,3.177177739504206e-05
17718,35437,35436,70873,16.65629482269287,3.145882356187534e-05
17818,35637,35636,71273,16.733814001083374,3.115200705127862e-05
17918,35837,35836,71673,16.807672023773193,3.085115989694329e-05
18018,36037,36036,72073,16.882555961608887,3.055611923573243e-05
18118,36237,36236,72473,16.95915198326111,3.0266727121420946e-05
18218,36437,36436,72873,17.033157110214233,2.998283034703666e-05
18318,36637,36636,73273,17.106882095336914,2.9704280278715254e-05
18418,36837,36836,73673,17.18053889274597,2.9430932697111267e-05
18519,37039,37038,74077,17.252413034439087,2.9159989898597117e-05
18619,37239,37238,74477,17.325382947921753,2.8896680138948832e-05
18719,37439,37438,74877,17.397274017333984,2.8638163927325157e-05
18819,37639,37638,75277,17.469266891479492,2.838431330815558e-05
18919,37839,37838,75677,17.54068088531494,2.8135004055142335e-05
19019,38039,38038,76077,17.610975980758667,2.7890115554991762e-05
19119,38239,38238,76477,17.68160104751587,2.7649530692710136e-05
19219,38439,38438,76877,17.756972074508667,2.7413135744249717e-05
19319,38639,38638,77277,17.82768201828003,2.7180820271181197e-05
19419,38839,38838,77677,17.89791488647461,2.6952477022695076e-05
19520,39041,39040,78081,17.97134304046631,2.6725776274959876e-05
19620,39241,39240,78481,18.043089866638184,2.6505105158808064e-05
19720,39441,39440,78881,18.113878965377808,2.6288101721943395e-05
19820,39641,39640,79281,18.189677000045776,2.60746705615014e-05
19920,39841,39840,79681,18.27058696746826,2.5864719015414138e-05
20020,40041,40040,80081,18.34655213356018,2.5658157080510214e-05
20120,40241,40240,80481,18.43445611000061,2.5454897336755517e-05
20220,40441,40440,80881,18.519476890563965,2.5254854872420898e-05
20320,40641,40640,81281,18.604310035705566,2.5057947211617455e-05
20420,40841,40840,81681,18.6878559589386,2.4864094243831293e-05
20521,41043,41042,82085,18.77606511116028,2.4671324172818473e-05
20621,41243,41242,82485,18.850317001342773,2.4483378027808908e-05
20721,41443,41442,82885,18.923684120178223,2.429825905215031e-05
20821,41643,41642,83285,18.999311208724976,2.411589596343249e-05
20921,41843,41842,83685,19.072793006896973,2.3936219526962322e-05
21021,42043,42042,84085,19.146358966827393,2.375916249582231e-05
21121,42243,42242,84485,19.221683979034424,2.358465955640318e-05
21221,42443,42442,84885,19.295365810394287,2.3412647271865886e-05
21321,42643,42642,85285,19.36719012260437,2.3243064029661924e-05
21421,42843,42842,85685,19.43897294998169,2.307584999029077e-05
21522,43045,43044,86089,19.511658906936646,2.290930948446167e-05
21622,43245,43244,86489,19.583112001419067,2.274668343669633e-05
21722,43445,43444,86889,19.65372586250305,2.2586256669867326e-05
21822,43645,43644,87289,19.725353956222534,2.2427975960148327e-05
21922,43845,43844,87689,19.79776406288147,2.2271789617417764e-05
22022,44045,44044,88089,19.86985492706299,2.2117647441859577e-05
22122,44245,44244,88489,19.95303511619568,2.1965500681564148e-05
22222,44445,44444,88889,20.042757987976074,2.1815301990555972e-05
22322,44645,44644,89289,20.14317488670349,2.1667005389170224e-05
22422,44845,44844,89689,20.22169589996338,2.1520566223945708e-05
22523,45047,45046,90093,20.298234939575195,2.137450389743613e-05
22623,45247,45246,90493,20.37393307685852,2.1231668274742093e-05
22723,45447,45446,90893,20.450881004333496,2.109056331098932e-05
22823,45647,45646,91293,20.523797035217285,2.095114930112278e-05
22923,45847,45846,91693,20.59470009803772,2.0813387685584392e-05
23023,46047,46046,92093,20.666278839111328,2.067724101748545e-05
23123,46247,46246,92493,20.739521026611328,2.054267293063988e-05
23223,46447,46446,92893,20.835583925247192,2.040964810749064e-05
23323,46647,46646,93293,20.90951919555664,2.0278132248572443e-05
23423,46847,46846,93693,20.9794180393219,2.014809204346726e-05
23524,47049,47048,94097,21.048605918884277,2.0018216353502114e-05
23624,47249,47248,94497,21.117487907409668,1.989104529704416e-05
23724,47449,47448,94897,21.187855005264282,1.9765255307275363e-05
23824,47649,47648,95297,21.256896018981934,1.9640816754702152e-05
23924,47849,47848,95697,21.323410034179688,1.9517700861296387e-05
24024,48049,48048,96097,21.393530130386353,1.9395879674889236e-05
24124,48249,48248,96497,21.478386878967285,1.9275326045535996e-05
24224,48449,48448,96897,21.5487859249115,1.9156013600908175e-05
24324,48649,48648,97297,21.618031978607178,1.9037916723550638e-05
24424,48849,48848,97697,21.68618607521057,1.8921010528517207e-05
24525,49051,49050,98101,21.755781888961792,1.8804119255199948e-05
24625,49251,49250,98501,21.82394003868103,1.8689533904571334e-05
24725,49451,49450,98901,21.892395973205566,1.857606853538815e-05
24825,49651,49650,99301,21.964552879333496,1.846370098658152e-05
24925,49851,49850,99701,22.032359838485718,1.835240972575939e-05
25025,50051,50050,100101,22.100332021713257,1.8242173830892025e-05
25125,50251,50250,100501,22.16816997528076,1.8132972971845767e-05
25225,50451,50450,100901,22.235920906066895,1.8024787392688152e-05
25325,50651,50650,101301,22.304487943649292,1.791759789366019e-05
25425,50851,50850,101701,22.378192901611328,1.7811385815375412e-05
25526,51053,51052,102105,22.466506958007812,1.7705085278162808e-05
25626,51253,51252,102505,22.541590929031372,1.7600783470369335e-05
25726,51453,51452,102905,22.61687183380127,1.749740601403757e-05
25826,51653,51652,103305,22.688760995864868,1.7394936255609e-05
25926,51853,51852,103705,22.7609920501709,1.729335800409566e-05
26026,52053,52052,104105,22.83814287185669,1.7192655517201312e-05
26126,52253,52252,104505,22.915133953094482,1.7092813487563866e-05
26226,52453,52452,104905,22.989957094192505,1.6993817030214183e-05
26326,52653,52652,105305,23.05929398536682,1.68956516684544e-05
26426,52853,52852,105705,23.127636909484863,1.6798303322708575e-05
26527,53055,53054,106109,23.200187921524048,1.670079685866953e-05
26627,53255,53254,106509,23.271903038024902,1.660504966524333e-05
26727,53455,53454,106909,23.34390878677368,1.6510079380238825e-05
26827,53655,53654,107309,23.415092945098877,1.641587339620174e-05
26927,53855,53854,107709,23.488311052322388,1.6322419444874413e-05
27027,54055,54054,108109,23.559279203414917,1.622970558720964e-05
27127,54255,54254,108509,23.6304829120636,1.6137720202917003e-05
27227,54455,54454,108909,23.709583044052124,1.604645198133419e-05
27327,54655,54654,109309,23.786777019500732,1.5955889911033592e-05
27427,54855,54854,109709,23.861466884613037,1.5866023271890535e-05
27528,55057,55056,110113,23.934846878051758,1.5775953233158783e-05
27628,55257,55256,110513,24.008338928222656,1.568745311075853e-05
27728,55457,55456,110913,24.08047890663147,1.559961781625362e-05
27828,55657,55656,111313,24.150479793548584,1.5512437707874757e-05
27928,55857,55856,111713,24.221068143844604,1.5425903392593543e-05
28028,56057,56056,112113,24.29201102256775,1.5340005718320964e-05
28128,56257,56256,112513,24.362289905548096,1.525473576666453e-05
28228,56457,56456,112913,24.433223962783813,1.5170084845910363e-05
28328,56657,56656,113313,24.503427028656006,1.5086044483851001e-05
28428,56857,56856,113713,24.575226068496704,1.5002606421231444e-05
28529,57059,57058,114117,24.64724612236023,1.4918937141126023e-05
28629,57259,57258,114517,24.717171907424927,1.4836685543758747e-05
28729,57459,57458,114917,24.786906003952026,1.4755012605720003e-05
28829,57659,57658,115317,24.861464023590088,1.4673910858305012e-05
28929,57859,57858,115717,24.93104314804077,1.4593373014588697e-05
29029,58059,58058,116117,25.00850796699524,1.4513391965261338e-05
29129,58259,58258,116517,25.08350110054016,1.4433960771370196e-05
29229,58459,58458,116917,25.153981924057007,1.4355072660792616e-05
29329,58659,58658,117317,25.224217176437378,1.4276721022064467e-05
29429,58859,58858,117717,25.29456901550293,1.4198899400570339e-05
29530,59061,59060,118121,25.36618185043335,1.412083113709544e-05
29630,59261,59260,118521,25.438392162322998,1.4044055930350786e-05
29730,59461,59460,118921,25.508455991744995,1.3967792206863045e-05
29830,59661,59660,119321,25.57916808128357,1.3892034091469082e-05
29930,59861,59860,119721,25.667461156845093,1.3816775843772175e-05
30030,60061,60060,120121,25.825155019760132,1.3742011852258061e-05
30130,60261,60260,120521,25.90750479698181,1.3667736632245829e-05
30230,60461,60460,120921,25.981377124786377,1.3593944821175885e-05
30330,60661,60660,121321,26.053498029708862,1.3520631174841028e-05
30430,60861,60860,121721,26.123279809951782,1.3447790563785466e-05
30531,61063,61062,122125,26.195186853408813,1.3374696591499395e-05
30631,61263,61262,122525,26.26737403869629,1.3302791713261758e-05
30731,61463,61462,122925,26.338029146194458,1.323134509156123e-05
30831,61663,61662,123325,26.409916877746582,1.3160352024723339e-05
30931,61863,61862,123725,26.48111891746521,1.3089807910219068e-05
31031,62063,62062,124125,26.55295491218567,1.3019708241126746e-05
31131,62263,62262,124525,26.62286901473999,1.2950048603807798e-05
31231,62463,62462,124925,26.693433046340942,1.2880824674895394e-05
31331,62663,62662,125325,26.7625789642334,1.2812032218859102e-05
31431,62863,62862,125725,26.834033966064453,1.2743667084967246e-05
31532,63065,63064,126129,26.909325122833252,1.2675047910385669e-05
31632,63265,63264,126529,26.98162293434143,1.2607529470036943e-05
31732,63465,63464,126929,27.05293107032776,1.2540426347793953e-05
31832,63665,63664,127329,27.141531944274902,1.2473734709913572e-05
31932,63865,63864,127729,27.22516393661499,1.2407450796598108e-05
32032,64065,64064,128129,27.30821704864502,1.2341570918836015e-05
32132,64265,64264,128529,27.383866786956787,1.2276091457306583e-05
32232,64465,64464,128929,27.455891847610474,1.2211008859601882e-05
32332,64665,64664,129329,27.52599287033081,1.2146319638728943e-05
32432,64865,64864,129729,27.59622097015381,1.2082020371446252e-05
32533,65067,65066,130133,27.667299032211304,1.2017470510092746e-05
32633,65267,65266,130533,27.7378990650177,1.1953944940703191e-05
32733,65467,65466,130933,27.82461380958557,1.1890799385439199e-05
32833,65667,65666,131333,27.971014976501465,1.1828030657689164e-05
32933,65867,65866,131733,28.041895866394043,1.1765635626103807e-05
33033,66067,66066,132133,28.11245322227478,1.1703611212723357e-05
33133,66267,66266,132533,28.194426774978638,1.1641954391581306e-05
33233,66467,66466,132933,28.26665997505188,1.1580662187235834e-05
33333,66667,66666,133333,28.337690830230713,1.151973167320635e-05
33433,66867,66866,133733,28.40821409225464,1.145915997127233e-05
33534,67069,67068,134137,28.481445789337158,1.1398343880375843e-05
33634,67269,67268,134537,28.561541080474854,1.1338484869761771e-05
33734,67469,67468,134937,28.650254011154175,1.1278976282498303e-05
33834,67669,67668,135337,28.730575799942017,1.1219815419291802e-05
33934,67869,67868,135737,28.803237915039062,1.1160999622212621e-05
34034,68069,68068,136137,28.886374950408936,1.1102526274125163e-05
34134,68269,68268,136537,28.958348989486694,1.1044392797122087e-05
34234,68469,68468,136937,29.02831196784973,1.0986596652116044e-05
34334,68669,68668,137337,29.108270168304443,1.092913533714529e-05
34434,68869,68868,137737,29.214366912841797,1.087200638689396e-05
34535,69071,69070,138141,29.353482007980347,1.0814641039152443e-05
34635,69271,69270,138541,29.424020051956177,1.0758172826412265e-05
34735,69471,69470,138941,29.4968159198761,1.0702029768192477e-05
34835,69671,69670,139341,29.566255807876587,1.0646209535832354e-05
34935,69871,69870,139741,29.634788751602173,1.0590709832984052e-05
35035,70071,70070,140141,29.70313596725464,1.0535528394461525e-05
35135,70271,70270,140541,29.77219796180725,1.0480662985438994e-05
35235,70471,70470,140941,29.851051092147827,1.0426111400662178e-05
35335,70671,70670,141341,29.928076028823853,1.0371871463733768e-05
35435,70871,70870,141741,29.99859881401062,1.0317941026897855e-05
35536,71073,71072,142145,30.068323135375977,1.0263783283944533e-05
35636,71273,71272,142545,30.13632297515869,1.0210468554471236e-05
35736,71473,71472,142945,30.205604791641235,1.0157457022502795e-05
35836,71673,71672,143345,30.27677011489868,1.0104746646564005e-05
35936,71873,71872,143745,30.34517812728882,1.0052335410015979e-05
36036,72073,72072,144145,30.41482186317444,1.0000221320252732e-05
36136,72273,72272,144545,30.49792790412903,9.948402408870986e-06
36236,72473,72472,144945,30.566853046417236,9.896876730314829e-06
36336,72673,72672,145345,30.633946180343628,9.845642362438357e-06
36436,72873,72872,145745,30.714571952819824,9.794697404628907e-06
36537,73075,73074,146149,30.785908937454224,9.74353484946901e-06
36637,73275,73274,146549,30.854099988937378,9.693165944138935e-06
36737,73475,73474,146949,30.922213792800903,9.643080857668941e-06
36837,73675,73674,147349,30.99303102493286,9.593277773582359e-06
36937,73875,73874,147749,31.06166100502014,9.543754895089129e-06
37037,74075,74074,148149,31.129328966140747,9.494510445563372e-06
37137,74275,74274,148549,31.197998046875,9.445542666678655e-06
37237,74475,74474,148949,31.26694917678833,9.39684981854373e-06
37337,74675,74674,149349,31.338430881500244,9.348430179943802e-06
37437,74875,74874,149749,31.41509509086609,9.300282047109628e-06
37538,75077,75076,150153,31.485002040863037,9.251926307497324e-06
37638,75277,75276,150553,31.553173065185547,9.204318817428131e-06
37738,75477,75476,150953,31.632922887802124,9.156977808712949e-06
37838,75677,75676,151353,31.708256006240845,9.109901645389194e-06
37938,75877,75876,151753,31.77719497680664,9.06308870710001e-06
38038,76077,76076,152153,31.846298933029175,9.016537389877662e-06
38138,76277,76276,152553,31.914397954940796,8.97024610490771e-06
38238,76477,76476,152953,31.986521005630493,8.924213278269528e-06
38338,76677,76676,153353,32.05594491958618,8.878437350907728e-06
38438,76877,76876,153753,32.12362194061279,8.83291677849829e-06
38539,77079,77078,154157,32.19227194786072,8.787198639970328e-06
38639,77279,77278,154557,32.266266107559204,8.742186716186681e-06
38739,77479,77478,154957,32.3398699760437,8.69742558348526e-06
38839,77679,77678,155357,32.41372108459473,8.652913752906591e-06
38939,77879,77878,155757,32.48853302001953,8.608649748757887e-06
39039,78079,78078,156157,32.55872988700867,8.564632108607513e-06
39139,78279,78278,156557,32.62793493270874,8.520859381960493e-06
39239,78479,78478,156957,32.6964647769928,8.477330131968392e-06
39339,78679,78678,157357,32.76560401916504,8.434042933128069e-06
39439,78879,78878,157757,32.83546280860901,8.390996372740759e-06
39540,79081,79080,158161,32.90314078330994,8.347762179717916e-06
39640,79281,79280,158561,32.97943902015686,8.305195075779838e-06
39740,79481,79480,158961,33.05616998672485,8.262864427904646e-06
39840,79681,79680,159361,33.13908410072327,8.220768869818147e-06
39940,79881,79880,159761,33.2110059261322,8.178907046014787e-06
40040,80081,80080,160161,33.28960990905762,8.13727761196053e-06
40140,80281,80280,160561,33.38313603401184,8.095879234201466e-06
40240,80481,80480,160961,33.48282599449158,8.054710589422994e-06
40340,80681,80680,161361,33.560083866119385,8.013770365173272e-06
40440,80881,80880,161761,33.632901191711426,7.973057259006582e-06
40541,81083,81082,162165,33.71219778060913,7.93216624198212e-06
40641,81283,81282,162565,33.78965997695923,7.891905744237378e-06
40741,81483,81482,162965,33.863577127456665,7.85186850499992e-06
40841,81683,81682,163365,33.938737869262695,7.812053261607058e-06
40941,81883,81882,163765,34.01409196853638,7.772458760678725e-06
41041,82083,82082,164165,34.107768058776855,7.733083758506741e-06
41141,82283,82282,164565,34.30961585044861,7.693927020716855e-06
41241,82483,82482,164965,34.41290998458862,7.654987321654853e-06
41341,82683,82682,165365,34.49614906311035,7.616263445389694e-06
41441,82883,82882,165765,34.57344889640808,7.577754183968579e-06
41542,83085,83084,166169,34.6516637802124,7.539076454204235e-06
41642,83285,83284,166569,34.72819209098816,7.500994951635613e-06
41742,83485,83484,166969,34.87647008895874,7.4631244818936705e-06
41842,83685,83684,167369,34.98021101951599,7.425463871914123e-06
41942,83885,83884,167769,35.063727140426636,7.388011956974788e-06
42042,84085,84084,168169,35.13854908943176,7.35076758060331e-06
42142,84285,84284,168569,35.211276054382324,7.313729594061847e-06
42242,84485,84484,168969,35.283100843429565,7.2768968571314685e-06
42342,84685,84684,169369,35.35355806350708,7.24026823721206e-06
42442,84885,84884,169769,35.42340087890625,7.203842609448843e-06
42543,85087,85086,170173,35.49665594100952,7.16725763496288e-06
42643,85287,85286,170573,35.57561492919922,7.131236650136116e-06
42743,85487,85486,170973,35.6498339176178,7.095415318007942e-06
42843,85687,85686,171373,35.729480028152466,7.059792544354096e-06
42943,85887,85886,171773,35.80146312713623,7.0243672419622075e-06
43043,86087,86086,172173,35.87255907058716,6.989138331090712e-06
43143,86287,86286,172573,35.94755506515503,6.954104739154548e-06
43243,86487,86486,172973,36.017701864242554,6.9192654006023495e-06
43343,86687,86686,173373,36.08926701545715,6.884619256872231e-06
43443,86887,86886,173773,36.15984010696411,6.850165256685627e-06
43544,87089,87088,174177,36.23258399963379,6.815560687752278e-06
43644,87289,87288,174577,36.31043982505798,6.781489742640136e-06
43744,87489,87488,174977,36.38764500617981,6.747607816964063e-06
43844,87689,87688,175377,36.45941877365112,6.7139138864022474e-06
43944,87889,87888,175777,36.53039312362671,6.680406933143287e-06
44044,88089,88088,176177,36.60039496421814,6.647085946019172e-06
44144,88289,88288,176577,36.67127299308777,6.613949920010182e-06
44244,88489,88488,176977,36.74121022224426,6.58099785674499e-06
44344,88689,88688,177377,36.812865018844604,6.5482287641530055e-06
44444,88889,88888,177777,36.885605812072754,6.515641656444835e-06
44545,89091,89090,178181,36.95863199234009,6.482912403623686e-06
44645,89291,89290,178581,37.029573917388916,6.450688128178052e-06
44745,89491,89490,178981,37.0997200012207,6.4186429074786614e-06
44845,89691,89690,179381,37.17013502120972,6.386775780018332e-06
44945,89891,89890,179781,37.239691972732544,6.355085790635725e-06
45045,90091,90090,180181,37.309996128082275,6.323571989721938e-06
45145,90291,90290,180581,37.380481004714966,6.292233433956981e-06
45245,90491,90490,180981,37.46369791030884,6.261069185429767e-06
45345,90691,90690,181381,37.54446887969971,6.230078312059861e-06
45445,90891,90890,181781,37.6224639415741,6.199259887835986e-06
45546,91093,91092,182185,37.701570987701416,6.168307385898487e-06
45646,91293,91292,182585,37.77109885215759,6.137832804711906e-06
45746,91493,91492,182985,37.842074155807495,6.1075279183302e-06
45846,91693,91692,183385,37.91293692588806,6.077391822975231e-06
45946,91893,91892,183785,37.983055114746094,6.047423619766005e-06
46046,92093,92092,184185,38.05249905586243,6.017622416051659e-06
46146,92293,92292,184585,38.125706911087036,5.987987324065617e-06
46246,92493,92492,184985,38.201038122177124,5.958517461319691e-06
46346,92693,92692,185385,38.27179789543152,5.929211950894008e-06
46446,92893,92892,185785,38.34473180770874,5.900069920885861e-06
46547,93095,93094,186189,38.41503405570984,5.870801528813013e-06
46647,93295,93294,186589,38.490373849868774,5.841985478237522e-06
46747,93495,93494,186989,38.56064987182617,5.813330314928808e-06
46847,93695,93694,187389,38.63480186462402,5.784835187868471e-06
46947,93895,93894,187789,38.703763008117676,5.756499250526048e-06
47047,94095,94094,188189,38.77419400215149,5.7283216620927856e-06
47147,94295,94294,188589,38.844074964523315,5.7003015858583396e-06
47247,94495,94494,188989,38.9144549369812,5.672438190651915e-06
47347,94695,94694,189389,38.98704481124878,5.6447306499422615e-06
47447,94895,94894,189789,39.05746793746948,5.61717814195004e-06
47548,95097,95096,190193,39.12756395339966,5.589506643035452e-06
47648,95297,95296,190593,39.19454908370972,5.562263284700671e-06
47748,95497,95496,190993,39.26336193084717,5.535172514797879e-06
47848,95697,95696,191393,39.33214497566223,5.50823353060782e-06
47948,95897,95896,191793,39.400306940078735,5.48144553394883e-06
48048,96097,96096,192193,39.46723985671997,5.454807731632171e-06
48148,96297,96296,192593,39.53531789779663,5.428319334839365e-06
48248,96497,96496,192993,39.60313391685486,5.401979559216118e-06
48348,96697,96696,193393,39.66940116882324,5.375787625232161e-06
48448,96897,96896,193793,39.744767904281616,5.349742757503943e-06
48549,97099,97098,194197,39.816986083984375,5.323585935685384e-06
48649,97299,97298,194597,39.88421392440796,5.297834343902858e-06
48749,97499,97498,194997,39.95539712905884,5.272227511842524e-06
48849,97699,97698,195397,40.02338004112244,5.246764681542395e-06
48949,97899,97898,195797,40.09161901473999,5.22144510013245e-06
49049,98099,98098,196197,40.16041088104248,5.196268018480843e-06
49149,98299,98298,196597,40.22707200050354,5.171232691703259e-06
49249,98499,98498,196997,40.294589042663574,5.146338379849339e-06
49349,98699,98698,197397,40.364161014556885,5.121584346210965e-06
49449,98899,98898,197797,40.434096813201904,5.096969858858035e-06
49550,99101,99100,198201,40.50340509414673,5.072250131919366e-06
49650,99301,99300,198601,40.57938003540039,5.047913935088097e-06
49750,99501,99500,199001,40.65838003158569,5.023715105716969e-06
49850,99701,99700,199401,40.74133086204529,4.999652928508329e-06
49950,99901,99900,199801,40.81439208984375,4.975726691870215e-06
50050,100101,100100,200201,40.88902807235718,4.951935688293543e-06
50150,100301,100300,200601,40.96863794326782,4.928279214059409e-06
50250,100501,100500,201001,41.06242513656616,4.904756569533034e-06
50350,100701,100700,201401,41.1516318321228,4.881367059087401e-06
50450,100901,100900,201801,41.22422194480896,4.858109990902602e-06
50551,101103,101102,202205,41.302666902542114,4.834754087025463e-06
50651,101303,101302,202605,41.379855155944824,4.811761150684866e-06
50751,101503,101502,203005,41.45747518539429,4.788898597468498e-06
50851,101703,101702,203405,41.531347036361694,4.7661657510782e-06
50951,101903,101902,203805,41.602821826934814,4.7435619388122915e-06
51051,102103,102102,204205,41.67313885688782,4.721086491744434e-06
51151,102303,102302,204605,41.74377083778381,4.698738744567397e-06
51251,102503,102502,205005,41.821946144104004,4.67651803588588e-06
51351,102703,102702,205405,41.8944251537323,4.65442370798411e-06
51451,102903,102902,205805,41.964563846588135,4.632455106646605e-06
51552,103105,103104,206209,42.03250503540039,4.6103937754140965e-06
51652,103305,103304,206609,42.101747035980225,4.588675919869479e-06
51752,103505,103504,207009,42.16954493522644,4.56708184364518e-06
51852,103705,103704,207409,42.238028049468994,4.5456109068755234e-06
51952,103905,103904,207809,42.30637502670288,4.524262473038207e-06
52052,104105,104104,208209,42.377718925476074,4.50303590985631e-06
52152,104305,104304,208609,42.46031212806702,4.481930587629535e-06
52252,104505,104504,209009,42.5433669090271,4.4609458807438155e-06
52352,104705,104704,209409,42.617496967315674,4.44008116686596e-06
52452,104905,104904,209809,42.687257051467896,4.419335826924423e-06
52553,105107,105106,210213,42.759377002716064,4.398503576999496e-06
52653,105307,105306,210613,42.830195903778076,4.377996319994162e-06
52753,105507,105506,211013,42.9013090133667,4.357606594234406e-06
52853,105707,105706,211413,42.97286081314087,4.337333794270907e-06
52953,105907,105906,211813,43.043484926223755,4.317177317871906e-06
53053,106107,106106,212213,43.115062952041626,4.297136566234023e-06
53153,106307,106306,212613,43.1864697933197,4.277210943642991e-06
53253,106507,106506,213013,43.25796604156494,4.257399857657006e-06
53353,106707,106706,213413,43.32678198814392,4.237702719258374e-06
53453,106907,106906,213813,43.39454197883606,4.218118942136207e-06
53554,107109,107108,214217,43.469626903533936,4.198453801489868e-06
53654,107309,107308,214617,43.54593801498413,4.1790961215606555e-06
53754,107509,107508,215017,43.63023400306702,4.159850058205327e-06
53854,107709,107708,215417,43.70662498474121,4.140715038374712e-06
53954,107909,107908,215817,43.78087592124939,4.12169049185086e-06
54054,108109,108108,216217,43.85509991645813,4.102775851226692e-06
54154,108309,108308,216617,43.9396858215332,4.083970552582838e-06
54254,108509,108508,217017,44.01490783691406,4.065274034718134e-06
54354,108709,108708,217417,44.086764097213745,4.046685739693659e-06
54454,108909,108908,217817,44.15858197212219,4.028205112167068e-06
54555,109111,109110,218221,44.234851121902466,4.009648404477159e-06
54655,109311,109310,218621,44.31241488456726,3.991382522047146e-06
54755,109511,109510,219021,44.3857479095459,3.9732226543964645e-06
54855,109711,109710,219421,44.45734190940857,3.95516825846744e-06
54955,109911,109910,219821,44.52795100212097,3.937218793731326e-06
55055,110111,110110,220221,44.59768080711365,3.9193737228706324e-06
55155,110311,110310,220621,44.6673641204834,3.901632511197682e-06
55255,110511,110510,221021,44.74003195762634,3.883994627014341e-06
55355,110711,110710,221421,44.81431698799133,3.866459541242284e-06
55455,110911,110910,221821,44.88526201248169,3.849026727987626e-06
55556,111113,111112,222225,44.963114976882935,3.831522865416961e-06
55656,111313,111312,222625,45.033313035964966,3.814294039421805e-06
55756,111513,111512,223025,45.104944944381714,3.7971659193340194e-06
55856,111713,111712,223425,45.17578196525574,3.7801379897162253e-06
55956,111913,111912,223825,45.24748706817627,3.7632097383087628e-06
56056,112113,112112,224225,45.322311878204346,3.746380655818998e-06
56156,112313,112312,224625,45.39608097076416,3.7296502350543283e-06
56256,112513,112512,225025,45.47146916389465,3.7130179717656068e-06
56356,112713,112712,225425,45.54185199737549,3.6964833643197807e-06
56456,112913,112912,225825,45.610896825790405,3.680045913899004e-06
56557,113115,113114,226229,45.684041023254395,3.6635422025605246e-06
56657,113315,113314,226629,45.76325297355652,3.6472985387737856e-06
56757,113515,113514,227029,45.8371148109436,3.631150545658939e-06
56857,113715,113714,227429,45.90832996368408,3.6150977346360793e-06
56957,113915,113914,227829,45.98531794548035,3.5991396197010377e-06
57057,114115,114114,228229,46.06306004524231,3.5832757172888128e-06
57157,114315,114314,228629,46.13350987434387,3.5675055463678695e-06
57257,114515,114514,229029,46.20726704597473,3.5518286286233473e-06
57357,114715,114714,229429,46.27881097793579,3.5362444877194963e-06
57457,114915,114914,229829,46.35221290588379,3.520752650323909e-06
57558,115117,115116,230233,46.42676091194153,3.5051991071690087e-06
57658,115317,115316,230633,46.498636960983276,3.4898913768323703e-06
57758,115517,115516,231033,46.57248902320862,3.474674539149808e-06
57858,115717,115716,231433,46.64836883544922,3.4595481300296076e-06
57958,115917,115916,231833,46.72419309616089,3.444511688451795e-06
58058,116117,116116,232233,46.80020093917847,3.4295647549437967e-06
58158,116317,116316,232633,46.87156105041504,3.414706872755212e-06
58258,116517,116516,233033,46.94558596611023,3.3999375876989694e-06
58358,116717,116716,233433,47.02105712890625,3.3852564473989437e-06
58458,116917,116916,233833,47.09240913391113,3.370663002187943e-06
58559,117119,117118,234237,47.163968086242676,3.3560121814881122e-06
58659,117319,117318,234637,47.233680963516235,3.341593651901923e-06
58759,117519,117518,235037,47.30398201942444,3.327261477001474e-06
58859,117719,117718,235437,47.373003005981445,3.313015216356852e-06
58959,117919,117918,235837,47.445063829422,3.29885443130374e-06
59059,118119,118118,236237,47.51489782333374,3.2847786855520033e-06
59159,118319,118318,236637,47.587085008621216,3.270787545082869e-06
59259,118519,118518,237037,47.65963006019592,3.2568805777448162e-06
59359,118719,118718,237437,47.7319438457489,3.243057354221872e-06
59459,118919,118918,237837,47.80570101737976,3.229317446507438e-06
59560,119121,119120,238241,47.8811981678009,3.2155242764601247e-06
59660,119321,119320,238641,47.95652890205383,3.2019505491993925e-06
59760,119521,119520,239041,48.046530961990356,3.188458863532566e-06
59860,119721,119720,239441,48.14667892456055,3.1750488005229006e-06
59960,119921,119920,239841,48.22349214553833,3.1617199431699828e-06
60060,120121,120120,240241,48.29840898513794,3.148471876535181e-06
60160,120321,120320,240641,48.37248206138611,3.1353041875904403e-06
60260,120521,120520,241041,48.44804787635803,3.12221646560781e-06
60360,120721,120720,241441,48.522977113723755,3.109208301734977e-06
60460,120921,120920,241841,48.59606981277466,3.096279288879458e-06
60561,121123,121122,242245,48.673168897628784,3.0833009160880306e-06
60661,121323,121322,242645,48.74701905250549,3.0705297745346636e-06
60761,121523,121522,243045,48.82254481315613,3.057836571767367e-06
60861,121723,121722,243445,48.89572191238403,3.0452209085410903e-06
60961,121923,121922,243845,48.969276905059814,3.0326823878801493e-06
61061,122123,122122,244245,49.04455089569092,3.0202206151558014e-06
61161,122323,122322,244645,49.11736607551575,3.0078351968175384e-06
61261,122523,122522,245045,49.188942193984985,2.995525741793433e-06
61361,122723,122722,245445,49.260936975479126,2.983291860656169e-06
61461,122923,122922,245845,49.33193492889404,2.9711331660294383e-06
61562,123125,123124,246249,49.40277719497681,2.9589288098924783e-06
61662,123325,123324,246649,49.472355127334595,2.9469200756642875e-06
61762,123525,123524,247049,49.54762005805969,2.934985372665422e-06
61862,123725,123724,247449,49.62604284286499,2.9231243211627506e-06
61962,123925,123924,247849,49.698084115982056,2.9113365428115323e-06
62062,124125,124124,248249,49.77164912223816,2.8996216609782116e-06
62162,124325,124324,248649,49.84279918670654,2.8879793009363483e-06
62262,124525,124524,249049,49.91619396209717,2.876409090102088e-06
62362,124725,124724,249449,49.99341702461243,2.864910657114372e-06
62462,124925,124924,249849,50.06777501106262,2.853483632643486e-06
62563,125127,125126,250253,50.143357038497925,2.8420144466557163e-06
62663,125327,125326,250653,50.23497009277344,2.830729842905204e-06
62763,125527,125526,251053,50.3152859210968,2.819515546092488e-06
62863,125727,125726,251453,50.39330196380615,2.8083711939183947e-06
62963,125927,125926,251853,50.46758818626404,2.797296425574582e-06
63063,126127,126126,252253,50.53906512260437,2.7862908817192455e-06
63163,126327,126326,252653,50.6185040473938,2.775354205192744e-06
63263,126527,126526,253053,50.694839000701904,2.7644860399032016e-06
63363,126727,126726,253453,50.76990795135498,2.7536860318430737e-06
63463,126927,126926,253853,50.8443489074707,2.7429538284824577e-06
63564,127129,127128,254257,50.91617679595947,2.7321827708355152e-06
63664,127329,127328,254657,50.990731954574585,2.721585794767247e-06
63764,127529,127528,255057,51.062554121017456,2.711055572255011e-06
63864,127729,127728,255457,51.13549304008484,2.700591756681407e-06
63964,127929,127928,255857,51.206661224365234,2.6901940038882488e-06
64064,128129,128128,256257,51.2767870426178,2.6798619706745087e-06
64164,128329,128328,256657,51.347057819366455,2.6695953156258623e-06
64264,128529,128528,257057,51.41762614250183,2.659393699021787e-06
64364,128729,128728,257457,51.48976492881775,2.649256782559759e-06
64464,128929,128928,257857,51.55862307548523,2.639184229190856e-06
64565,129131,129130,258261,51.62944412231445,2.6290759409266197e-06
64665,129331,129330,258661,51.70014309883118,2.6191317449486765e-06
64765,129531,129530,259061,51.768963098526,2.6092509074161096e-06
64865,129731,129730,259461,51.83746790885925,2.5994330977607984e-06
64965,129931,129930,259861,51.906309843063354,2.589677986323251e-06
65065,130131,130130,260261,51.97751593589783,2.5799852454567913e-06
65165,130331,130330,260661,52.04592299461365,2.5703545484942893e-06
65265,130531,130530,261061,52.11480402946472,2.5607855706475568e-06
65365,130731,130730,261461,52.18163204193115,2.5512779882598767e-06
65465,130931,130930,261861,52.24852395057678,2.5418314792641497e-06
65566,131133,131132,262265,52.32625985145569,2.5323521709510194e-06
65666,131333,131332,262665,52.3963258266449,2.523027450649723e-06
65766,131533,131532,263065,52.47155785560608,2.5137628423610064e-06
65866,131733,131732,263465,52.54235100746155,2.5045580298119715e-06
65966,131933,131932,263865,52.62768793106079,2.4954126978385856e-06
66066,132133,132132,264265,52.70843505859375,2.4863265324961008e-06
66166,132333,132332,264665,52.78497314453125,2.4772992213185746e-06
66266,132533,132532,265065,52.87507104873657,2.468330453227136e-06
66366,132733,132732,265465,52.97519493103027,2.4594199184772105e-06
66466,132933,132932,265865,53.04699397087097,2.4505673088944696e-06
66567,133135,133134,266269,53.1208930015564,2.4416846569844214e-06
66667,133335,133334,266669,53.19413495063782,2.4329475486101967e-06
66767,133535,133534,267069,53.26772499084473,2.424267444997775e-06
66867,133735,133734,267469,53.339343786239624,2.415644042512235e-06
66967,133935,133934,267869,53.41228103637695,2.407077039411883e-06
67067,134135,134134,268269,53.4872100353241,2.398566135092775e-06
67167,134335,134334,268669,53.56065106391907,2.3901110302742894e-06
67267,134535,134534,269069,53.63433909416199,2.3817114267139655e-06
67367,134735,134734,269469,53.707239866256714,2.373367027660072e-06
67467,134935,134934,269869,53.78173804283142,2.3650775374344425e-06
67568,135137,135136,270273,53.853919982910156,2.3567605878678364e-06
67668,135337,135336,270673,53.925498962402344,2.3485805752968476e-06
67768,135537,135536,271073,53.998778104782104,2.3404545891950986e-06
67868,135737,135736,271473,54.07103991508484,2.3323823390859886e-06
67968,135937,135936,271873,54.1431097984314,2.324363535425193e-06
68068,136137,136136,272273,54.2176718711853,2.3163978898000402e-06
68168,136337,136336,272673,54.28940391540527,2.3084851152131723e-06
68268,136537,136536,273073,54.36292886734009,2.3006249257527494e-06
68368,136737,136736,273473,54.4419219493866,2.292817036715171e-06
68468,136937,136936,273873,54.51297307014465,2.28506116463904e-06
68569,137139,137138,274277,54.58465313911438,2.277280245826642e-06
68669,137339,137338,274677,54.65662217140198,2.269628074550235e-06
68769,137539,137538,275077,54.72842288017273,2.262027073533906e-06
68869,137739,137738,275477,54.79981207847595,2.2544769639386698e-06
68969,137939,137938,275877,54.86952090263367,2.246977468094862e-06
69069,138139,138138,276277,54.94379186630249,2.239528309248918e-06
69169,138339,138338,276677,55.01922607421875,2.232129211675099e-06
69269,138539,138538,277077,55.09207201004028,2.224779901255263e-06
69369,138739,138738,277477,55.16268587112427,2.217480104439679e-06
69469,138939,138938,277877,55.23352909088135,2.210229549177222e-06
69570,139141,139140,278281,55.30650281906128,2.2029561950037375e-06
69670,139341,139340,278681,55.37718892097473,2.195803796210658e-06
69770,139541,139540,279081,55.4523389339447,2.188699826214872e-06
69870,139741,139740,279481,55.526089906692505,2.1816440171058295e-06
69970,139941,139940,279881,55.60014486312866,2.1746361021918227e-06
70070,140141,140140,280281,55.67289400100708,2.1676758158810486e-06
70170,140341,140340,280681,55.74444603919983,2.160762893294456e-06
70270,140541,140540,281081,55.81593704223633,2.153897071094307e-06
70370,140741,140740,281481,55.88795495033264,2.1470780865682e-06
70470,140941,140940,281881,55.96220588684082,2.1403056783586055e-06
70571,141143,141142,282285,56.036673069000244,2.1335125582210985e-06
70671,141343,141342,282685,56.11044406890869,2.126832981776931e-06
70771,141543,141542,283085,56.18540000915527,2.1201992007846804e-06
70871,141743,141742,283485,56.26055288314819,2.1136109580559547e-06
70971,141943,141942,283885,56.33446979522705,2.1070679973443883e-06
71071,142143,142142,284285,56.4070200920105,2.100570063260819e-06
71171,142343,142342,284685,56.48858118057251,2.094116901446059e-06
71271,142543,142542,285085,56.567424058914185,2.087708259066037e-06
71371,142743,142742,285485,56.647247076034546,2.0813438834648194e-06
71471,142943,142942,285885,56.72894597053528,2.0750235232705427e-06
71572,143145,143144,286289,56.81772708892822,2.0686843828919825e-06
71672,143345,143344,286689,56.969274044036865,2.0624517383600515e-06
71772,143545,143544,287089,57.16792917251587,2.056262359115471e-06
71872,143745,143744,287489,57.25225496292114,2.050115997800982e-06
71972,143945,143944,287889,57.33186888694763,2.0440124083681556e-06
72072,144145,144144,288289,57.44246816635132,2.0379513453490074e-06
72172,144345,144344,288689,57.55598211288452,2.0319325641643383e-06
72272,144545,144544,289089,57.65483283996582,2.0259558216145032e-06
72372,144745,144744,289489,57.759860038757324,2.0200208753586987e-06
72472,144945,144944,289889,57.8575119972229,2.0141274837413022e-06
72573,145147,145146,290293,57.986648082733154,2.008217093332123e-06
72673,145347,145346,290693,58.10359811782837,2.002406499793463e-06
72773,145547,145546,291093,58.220020055770874,1.996636739963973e-06
72873,145747,145746,291493,58.37285304069519,1.9909075760700736e-06
72973,145947,145946,291893,58.51882004737854,1.985218771099692e-06
73073,146147,146146,292293,58.616738080978394,1.979570089524111e-06
73173,146347,146346,292693,58.70088601112366,1.9739612963998257e-06
73273,146547,146546,293093,58.78315997123718,1.9683921578082133e-06
73373,146747,146746,293493,58.86001801490784,1.9628624408575366e-06
73473,146947,146946,293893,58.945537090301514,1.9573719130255463e-06
73574,147149,147148,294297,59.03167009353638,1.951866023886824e-06
73674,147349,147348,294697,59.11124515533447,1.946453568571144e-06
73774,147549,147548,295097,59.18671989440918,1.9410796095815656e-06
73874,147749,147748,295497,59.26131296157837,1.9357439186554453e-06
73974,147949,147948,295897,59.33521509170532,1.930446268220333e-06
74074,148149,148148,296297,59.41333293914795,1.9251864315266883e-06
74174,148349,148348,296697,59.493890047073364,1.919964183130938e-06
74274,148549,148548,297097,59.56971192359924,1.9147792981028865e-06
74374,148749,148748,297497,59.65098285675049,1.9096315527452103e-06
74474,148949,148948,297897,59.733636140823364,1.904520723824285e-06
74575,149151,149150,298301,59.81791400909424,1.8993960326464324e-06
74675,149351,149350,298701,59.8901948928833,1.8943587350300446e-06
74775,149551,149550,299101,59.96285581588745,1.8893576883488883e-06
74875,149751,149750,299501,60.03399085998535,1.884392672963078e-06
74975,149951,149950,299901,60.10562610626221,1.879463470399839e-06
75075,150151,150150,300301,60.18236494064331,1.8745698629375028e-06
75175,150351,150350,300701,60.254727840423584,1.8697116340249785e-06
75275,150551,150550,301101,60.32468104362488,1.8648885677041297e-06
75375,150751,150750,301501,60.39591693878174,1.860100448892799e-06
75475,150951,150950,301901,60.4701669216156,1.8553470635185739e-06
75576,151153,151152,302305,60.57488203048706,1.850581183229221e-06
75676,151353,151352,302705,60.65757203102112,1.8458969680701343e-06
75776,151553,151552,303105,60.73555088043213,1.841246847050018e-06
75876,151753,151752,303505,60.80660700798035,1.836630609614162e-06
75976,151953,151952,303905,60.88055396080017,1.832048046098284e-06
76076,152153,152152,304305,60.956743001937866,1.8274989473565958e-06
76176,152353,152352,304705,61.035258769989014,1.8229831058025645e-06
76276,152553,152552,305105,61.12924909591675,1.818500313879528e-06
76376,152753,152752,305505,61.21458196640015,1.8140503654104226e-06
76476,152953,152952,305905,61.29322600364685,1.8096330548917877e-06
76577,153155,153154,306309,61.367249965667725,1.8052044924095253e-06
76677,153355,153354,306709,61.441890001297,1.8008521664431159e-06
76777,153555,153554,307109,61.514612913131714,1.7965318653049106e-06
76877,153755,153754,307509,61.5899920463562,1.7922433870349087e-06
76977,153955,153954,307909,61.66326093673706,1.7879865303773963e-06
77077,154155,154154,308309,61.73578596115112,1.7837610951737734e-06
77177,154355,154354,308709,61.80779194831848,1.7795668817952114e-06
77277,154555,154554,309109,61.88446807861328,1.775403691839618e-06
77377,154755,154754,309509,61.961199045181274,1.7712713274828856e-06
77477,154955,154954,309909,62.03153419494629,1.7671695917911344e-06
77578,155157,155156,310313,62.11247801780701,1.763057728629924e-06
77678,155357,155356,310713,62.19210076332092,1.759016964202382e-06
77778,155557,155556,311113,62.271831035614014,1.755006240998e-06
77878,155757,155756,311513,62.3539559841156,1.7510253653561124e-06
77978,155957,155956,311913,62.455573081970215,1.7470741444808845e-06
78078,156157,156156,312313,62.53610014915466,1.7431523867505794e-06
78178,156357,156356,312713,62.61177396774292,1.739259901037415e-06
78278,156557,156556,313113,62.685948848724365,1.7353964971853342e-06
78378,156757,156756,313513,62.76630091667175,1.7315619860625706e-06
78478,156957,156956,313913,62.84904599189758,1.7277561789569766e-06
78579,157159,157158,314317,62.924530029296875,1.7239412587906194e-06
78679,157359,157358,314717,63.00164198875427,1.7201925799825884e-06
78779,157559,157558,315117,63.07585692405701,1.7164720431074261e-06
78879,157759,157758,315517,63.1503050327301,1.7127794629624441e-06
78979,157959,157958,315917,63.22413396835327,1.7091146549861194e-06
79079,158159,158158,316317,63.29810094833374,1.7054774360387703e-06
79179,158359,158358,316717,63.37608814239502,1.7018676233897183e-06
79279,158559,158558,317117,63.45469284057617,1.698285035077022e-06
79379,158759,158758,317517,63.53827500343323,1.6947294902313227e-06
79479,158959,158958,317917,63.61941885948181,1.6912008087318635e-06
79580,159161,159160,318321,63.698418855667114,1.6876639254544311e-06
79680,159361,159360,318721,63.77352595329285,1.684188697519512e-06
79780,159561,159560,319121,63.85061717033386,1.6807397956576483e-06
79880,159761,159760,319521,63.92747902870178,1.6773170429601805e-06
79980,159961,159960,319921,64.00474905967712,1.6739202634554277e-06
80080,160161,160160,320321,64.08145999908447,1.6705492819888668e-06
80180,160361,160360,320721,64.1577820777893,1.6672039242535504e-06
80280,160561,160560,321121,64.2343499660492,1.6638840163777806e-06
80380,160761,160760,321521,64.31194996833801,1.660589385918047e-06
80480,160961,160960,321921,64.38817310333252,1.6573198610569068e-06
80581,161163,161162,322325,64.46783900260925,1.6540429497962114e-06
80681,161363,161362,322725,64.54290199279785,1.6508233700928283e-06
80781,161563,161562,323125,64.61773014068604,1.6476283833373464e-06
80881,161763,161762,323525,64.69210290908813,1.6444578209271493e-06
80981,161963,161962,323925,64.76538014411926,1.6413115151153036e-06
81081,162163,162162,324325,64.84190702438354,1.6381892988558482e-06
81181,162363,162362,324725,64.92215490341187,1.6350910059707293e-06
81281,162563,162562,325125,65.01429986953735,1.6320164711392937e-06
81381,162763,162762,325525,65.10189008712769,1.6289655296477216e-06
81481,162963,162962,325925,65.19637989997864,1.6259380180947523e-06
81582,163165,163164,326329,65.34731698036194,1.6229038476649173e-06
81682,163365,163364,326729,65.45349407196045,1.619922937826256e-06
81782,163565,163564,327129,65.53290486335754,1.6169649696847463e-06
81882,163765,163764,327529,65.60747385025024,1.614029782964095e-06
81982,163965,163964,327929,65.690425157547,1.6111172178562461e-06
82082,164165,164164,328329,65.77483010292053,1.608227115614968e-06
82182,164365,164364,328729,65.8751540184021,1.6053593179189702e-06
82282,164565,164564,329129,65.9681568145752,1.6025136679114424e-06
82382,164765,164764,329529,66.05261206626892,1.599690008754685e-06
82482,164965,164964,329929,66.15925288200378,1.5968881850724742e-06
82583,165167,165166,330333,66.28485822677612,1.594080349363094e-06
82683,165367,165366,330733,66.40743613243103,1.5913219471252603e-06
82783,165567,165566,331133,66.49222803115845,1.588584916599724e-06
82883,165767,165766,331533,66.57049489021301,1.5858691054244984e-06
82983,165967,165966,331933,66.65568399429321,1.5831743617700876e-06
83083,166167,166166,332333,66.73676204681396,1.5805005350361195e-06
83183,166367,166366,332733,66.81768703460693,1.5778474748757486e-06
83283,166567,166566,333133,66.96390199661255,1.5752150326098378e-06
83383,166767,166766,333533,67.04806613922119,1.572603059155467e-06
83483,166967,166966,333933,67.12381601333618,1.5700114072136505e-06
83584,167169,167168,334337,67.19931101799011,1.5674143163533773e-06
83684,167369,167368,334737,67.2751739025116,1.5648630669727027e-06
83784,167569,167568,335137,67.34995102882385,1.5623316993091795e-06
83884,167769,167768,335537,67.43186616897583,1.5598200690349098e-06
83984,167969,167968,335937,67.5145320892334,1.5573280321679621e-06
84084,168169,168168,336337,67.5947048664093,1.5548554459424362e-06
84184,168369,168368,336737,67.67700409889221,1.5524021681994328e-06
84284,168569,168568,337137,67.74986505508423,1.5499680578256143e-06
84384,168769,168768,337537,67.81996011734009,1.5475529739526512e-06
84484,168969,168968,337937,67.88930606842041,1.5451567769376212e-06
84585,169171,169170,338341,67.96084785461426,1.5427556474698198e-06
84685,169371,169370,338741,68.0351140499115,1.5403969933505532e-06
84785,169571,169570,339141,68.11504197120667,1.5380568098468841e-06
84885,169771,169770,339541,68.18636202812195,1.535734960562266e-06
84985,169971,169970,339941,68.26095199584961,1.5334313094921342e-06
85085,170171,170170,340341,68.33754396438599,1.5311457214689604e-06
85185,170371,170370,340741,68.41568517684937,1.5288780623743324e-06
85285,170571,170570,341141,68.4911060333252,1.526628198387049e-06
85385,170771,170770,341541,68.5607259273529,1.5243959968526471e-06
85485,170971,170970,341941,68.63015508651733,1.5221813256097273e-06
85586,171173,171172,342345,68.70061302185059,1.5199621680827842e-06
85686,171373,171372,342745,68.77140784263611,1.5177823365159705e-06
85786,171573,171572,343145,68.84421896934509,1.5156196423009276e-06
85886,171773,171772,343545,68.92285895347595,1.5134739568266023e-06
85986,171973,171972,343945,68.99951887130737,1.5113451514983241e-06
86086,172173,172172,344345,69.08006811141968,1.5092330991083433e-06
86186,172373,172372,344745,69.1626181602478,1.5071376727685602e-06
86286,172573,172572,345145,69.24062299728394,1.5050587465666602e-06
86386,172773,172772,345545,69.32267808914185,1.502996195389828e-06
86486,172973,172972,345945,69.40260195732117,1.5009498945678348e-06
86587,173175,173174,346349,69.48088812828064,1.4988994999018596e-06
86687,173375,173374,346749,69.55895400047302,1.4968854890651688e-06
86787,173575,173574,347149,69.63507509231567,1.494887358749664e-06
86887,173775,173774,347549,69.7116129398346,1.4929049870984796e-06
86987,173975,173974,347949,69.78380489349365,1.4909382537904246e-06
87087,174175,174174,348349,69.88013696670532,1.4889870386305271e-06
87187,174375,174374,348749,69.96298289299011,1.4870512223823873e-06
87287,174575,174574,349149,70.04795002937317,1.4851306864376108e-06
87387,174775,174774,349549,70.13316893577576,1.4832253130428921e-06
87487,174975,174974,349949,70.21263003349304,1.4813349852828165e-06
87588,175177,175176,350353,70.29317998886108,1.479440907684181e-06
87688,175377,175376,350753,70.3679449558258,1.4775804702262628e-06
87788,175577,175576,351153,70.44201588630676,1.4757347303277195e-06
87888,175777,175776,351553,70.51570892333984,1.4739035738584341e-06
87988,175977,175976,351953,70.59650206565857,1.472086887270369e-06
88088,176177,176176,352353,70.67098999023438,1.4702845579719397e-06
88188,176377,176376,352753,70.74478888511658,1.4684964739474555e-06
88288,176577,176576,353153,70.8189160823822,1.4667225239311733e-06
88388,176777,176776,353553,70.89260387420654,1.4649625973142203e-06
88488,176977,176976,353953,70.96290612220764,1.4632165841767938e-06
88589,177179,177178,354357,71.03498077392578,1.4614671226851623e-06
88689,177379,177378,354757,71.10689210891724,1.4597487462110185e-06
88789,177579,177578,355157,71.18229699134827,1.4580439569882368e-06
88889,177779,177778,355557,71.25433015823364,1.4563526476187764e-06
88989,177979,177978,355957,71.32851600646973,1.4546747120474548e-06
89089,178179,178178,356357,71.40420603752136,1.4530100443197464e-06
89189,178379,178378,356757,71.47553586959839,1.4513585399173698e-06
89289,178579,178578,357157,71.58033680915833,1.449720094158862e-06
89389,178779,178778,357557,71.65662479400635,1.4480946036842707e-06
89489,178979,178978,357957,71.72971606254578,1.4464819654288502e-06
89590,179181,179180,358361,71.82574200630188,1.4448661425046581e-06
89690,179381,179380,358761,71.9017128944397,1.443279028929558e-06
89790,179581,179580,359161,71.99795293807983,1.4417044619077524e-06
89890,179781,179780,359561,72.07052493095398,1.4401423414844319e-06
89990,179981,179980,359961,72.16034412384033,1.4385925681442626e-06
90090,180181,180180,360361,72.23221611976624,1.437055042820718e-06
90190,180381,180380,360761,72.30706691741943,1.4355296675786023e-06
90290,180581,180580,361161,72.38331484794617,1.4340163447196163e-06
90390,180781,180780,361561,72.45414900779724,1.432514977630394e-06
90490,180981,180980,361961,72.52265000343323,1.4310254699660522e-06
90591,181183,181182,362365,72.59627485275269,1.4295330079215403e-06
90691,181383,181382,362765,72.6646101474762,1.4280670495519363e-06
90791,181583,181582,363165,72.73372602462769,1.4266126651034025e-06
90891,181783,181782,363565,72.80232501029968,1.4251697609257057e-06
90991,181983,181982,363965,72.87524890899658,1.4237382443122814e-06
91091,182183,182182,364365,72.94749116897583,1.4223180227652558e-06
91191,182383,182382,364765,73.01836585998535,1.4209090048431104e-06
91291,182583,182582,365165,73.09382700920105,1.4195110994672459e-06
91391,182783,182782,365565,73.16676712036133,1.4181242161469805e-06
91491,182983,182982,365965,73.238028049469,1.4167482654553145e-06
91592,183185,183184,366369,73.3213198184967,1.4153695613472516e-06
91692,183385,183384,366769,73.4268319606781,1.4140153160225222e-06
91792,183585,183584,367169,73.51969695091248,1.4126717368033945e-06
91892,183785,183784,367569,73.60921597480774,1.4113387365096943e-06
91992,183985,183984,367969,73.68926692008972,1.4100162286344663e-06
92092,184185,184184,368369,73.76327300071716,1.4087041271765727e-06
92192,184385,184384,368769,73.83497405052185,1.4074023466679913e-06
92292,184585,184584,369169,73.90830993652344,1.4061108024713637e-06
92392,184785,184784,369569,74.02981805801392,1.4048294103705945e-06
92492,184985,184984,369969,74.10685110092163,1.4035580868439076e-06
92593,185187,185186,370373,74.17940306663513,1.402284185577777e-06
92693,185387,185386,370773,74.25293016433716,1.4010328495400257e-06
92793,185587,185586,371173,74.32350492477417,1.3997913341642846e-06
92893,185787,185786,371573,74.39193487167358,1.3985595584414396e-06
92993,185987,185986,371973,74.47486209869385,1.3973374416603614e-06
93093,186187,186186,372373,74.5578920841217,1.3961249039379972e-06
93193,186387,186386,372773,74.62818789482117,1.3949218657123098e-06
93293,186587,186586,373173,74.69855093955994,1.3937282484210587e-06
93393,186787,186786,373573,74.7751259803772,1.3925439736077279e-06
93493,186987,186986,373973,74.8539628982544,1.3913689637980936e-06
93594,187189,187188,374377,74.92611193656921,1.3901915296867567e-06
93694,187389,187388,374777,75.00283288955688,1.3890349098432154e-06
93794,187589,187588,375177,75.07335186004639,1.3878873246357019e-06
93894,187789,187788,375577,75.14713597297668,1.3867486985945261e-06
93994,187989,187988,375977,75.21955108642578,1.3856189570908606e-06
94094,188189,188188,376377,75.30344700813293,1.38449802570958e-06
94194,188389,188388,376777,75.3826801776886,1.3833858307656064e-06
94294,188589,188588,377177,75.46144318580627,1.3822822991316638e-06
94394,188789,188788,377577,75.53371381759644,1.3811873582845045e-06
94494,188989,188988,377977,75.60540008544922,1.380100935891496e-06
94595,189191,189190,378381,75.67790102958679,1.3790122236024353e-06
94695,189391,189390,378781,75.75213599205017,1.3779427080479144e-06
94795,189591,189590,379181,75.83418488502502,1.376881497565118e-06
94895,189791,189790,379581,75.90955400466919,1.3758285222432733e-06
94995,189991,189990,379981,75.984610080719,1.374783712646331e-06
95095,190191,190190,380381,76.06032800674438,1.3737469999185782e-06
95195,190391,190390,380781,76.13598012924194,1.3727183158601186e-06
95295,190591,190590,381181,76.21611905097961,1.3716975926498783e-06
95395,190791,190790,381581,76.29199314117432,1.3706847629116834e-06
95495,190991,190990,381981,76.37700986862183,1.3696797599346017e-06
95596,191193,191192,382385,76.46512579917908,1.368672584022339e-06
95696,191393,191392,382785,76.55124187469482,1.367683112962588e-06
95796,191593,191592,383185,76.6246588230133,1.3667012708478613e-06
95896,191793,191792,383585,76.70560884475708,1.3657269930463281e-06
95996,191993,191992,383985,76.78116297721863,1.3647602150997397e-06
96096,192193,192192,384385,76.85214376449585,1.3638008733392518e-06
96196,192393,192392,384785,76.93126702308655,1.3628489047718675e-06
96296,192593,192592,385185,77.05319499969482,1.3619042464747929e-06
96396,192793,192792,385585,77.16177988052368,1.3609668361281709e-06
96496,192993,192992,385985,77.28858184814453,1.360036612080165e-06
96597,193195,193194,386389,77.3745129108429,1.3591043179385103e-06
96697,193395,193394,386789,77.48634696006775,1.358188353514031e-06
96797,193595,193594,387189,77.61352705955505,1.3572793923773275e-06
96897,193795,193794,387589,77.69308996200562,1.3563773748001648e-06
96997,193995,193994,387989,77.78841018676758,1.3554822410965038e-06
97097,194195,194194,388389,77.89498901367188,1.35459393284761e-06
97197,194395,194394,388789,77.97774004936218,1.3537123913264018e-06
97297,194595,194594,389189,78.07344198226929,1.3528375585785545e-06
97397,194795,194794,389589,78.15262579917908,1.3519693771399977e-06
97497,194995,194994,389989,78.23534202575684,1.351107789933584e-06
97598,195197,195196,390393,78.3273069858551,1.3502442227272008e-06
97698,195397,195396,390793,78.46989583969116,1.349395719271456e-06
97798,195597,195596,391193,78.57799196243286,1.348553640899381e-06
97898,195797,195796,391593,78.65797305107117,1.3477179327329728e-06
97998,195997,195996,391993,78.74201011657715,1.3468885396055964e-06
98098,196197,196196,392393,78.84986186027527,1.3460654073491742e-06
98198,196397,196396,392793,78.93418097496033,1.3452484819625905e-06
98298,196597,196596,393193,79.0104410648346,1.3444377100831858e-06
98398,196797,196796,393593,79.14340090751648,1.3436330384876309e-06
98498,196997,196996,393993,79.22752094268799,1.3428344145000124e-06
98599,197199,197198,394397,79.30831694602966,1.3420338897748264e-06
98699,197399,197398,394797,79.38493204116821,1.3412472640671224e-06
98799,197599,197598,395197,79.46774101257324,1.3404665303278835e-06
98899,197799,197798,395597,79.56147503852844,1.3396916374270527e-06
98999,197999,197998,395997,79.65011501312256,1.338922534672346e-06
99099,198199,198198,396397,79.72694897651672,1.3381591725322445e-06
99199,198399,198398,396797,79.81008577346802,1.3374015005807464e-06
99299,198599,198598,397197,79.88635015487671,1.3366494697956206e-06
99399,198799,198798,397597,79.96523690223694,1.335903031252909e-06
99499,198999,198998,397997,80.04846477508545,1.3351621364456628e-06
99600,199201,199200,398401,80.13039588928223,1.3344194110065009e-06
99700,199401,199400,398801,80.20455503463745,1.3336895139686216e-06
99800,199601,199600,399201,80.27845811843872,1.3329650172670143e-06
99900,199801,199800,399601,80.35852789878845,1.332245873735849e-06
100000,200001,200000,400001,80.44037985801697,1.3315320367501845e-06


==> extragradient/plot_data/bilinear_matrix_game_n500/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0009160041809082031,2.018959020339561
100,201,200,401,0.07715821266174316,0.04084193889187754
200,401,400,801,0.16120600700378418,0.01555572904704933
300,601,600,1201,0.24944210052490234,0.008941559671892264
400,801,800,1601,0.3368391990661621,0.005957710393872965
501,1003,1002,2005,0.46764707565307617,0.004080388626738635
601,1203,1202,2405,0.5416932106018066,0.003044183482286378
701,1403,1402,2805,0.621251106262207,0.00247078219342337
801,1603,1602,3205,0.7011713981628418,0.002022425653118514
901,1803,1802,3605,0.7767093181610107,0.0017090990324214828
1001,2003,2002,4005,0.8524861335754395,0.0014375084752964995
1101,2203,2202,4405,0.9366452693939209,0.0012047380988628406
1201,2403,2402,4805,1.019376277923584,0.001000692926912849
1301,2603,2602,5205,1.1019251346588135,0.0008161398070111659
1401,2803,2802,5605,1.1924023628234863,0.0007105240339073027
1502,3005,3004,6009,1.2840192317962646,0.0006406047458752685
1602,3205,3204,6409,1.3672723770141602,0.0005873580809235912
1702,3405,3404,6809,1.4364511966705322,0.0005382536666146199
1802,3605,3604,7209,1.510073184967041,0.0004953501567577407
1902,3805,3804,7609,1.5858969688415527,0.00046283265676205554
2002,4005,4004,8009,1.7175931930541992,0.0004308549629022895
2102,4205,4204,8409,1.8151521682739258,0.0003999154365291184
2202,4405,4404,8809,1.9494280815124512,0.00037725255875169743
2302,4605,4604,9209,2.157297134399414,0.0003527435669886361
2402,4805,4804,9609,2.242280960083008,0.0003335273689751663
2503,5007,5006,10013,2.4526331424713135,0.00031945940005734464
2603,5207,5206,10413,2.590062141418457,0.00030878973556726564
2703,5407,5406,10813,2.7304251194000244,0.0003000156905100278
2803,5607,5606,11213,2.823237180709839,0.00029252572517975546
2903,5807,5806,11613,2.897221326828003,0.00028541420036607454
3003,6007,6006,12013,2.973459005355835,0.0002780152490870146
3103,6207,6206,12413,3.0520529747009277,0.00027195002345469855
3203,6407,6406,12813,3.1366500854492188,0.00026673775102073016
3303,6607,6606,13213,3.2105050086975098,0.00026209269718888097
3403,6807,6806,13613,3.284858226776123,0.00025787167822761395
3504,7009,7008,14017,3.3663980960845947,0.00025394578198297755
3604,7209,7208,14417,3.44762921333313,0.00025011718889721537
3704,7409,7408,14817,3.5469560623168945,0.0002467056013739032
3804,7609,7608,15217,3.635627031326294,0.00024351263461413038
3904,7809,7808,15617,3.7246532440185547,0.00024048591179458707
4004,8009,8008,16017,3.8213601112365723,0.00023752401694437778
4104,8209,8208,16417,3.9039900302886963,0.00023457721923087589
4204,8409,8408,16817,3.9846279621124268,0.00023189293501112748
4304,8609,8608,17217,4.058801174163818,0.00022910798042041975
4404,8809,8808,17617,4.136341094970703,0.00022619918421695374
4505,9011,9010,18021,4.219438076019287,0.0002230343272817675
4605,9211,9210,18421,4.296112298965454,0.00022034767502957447
4705,9411,9410,18821,4.372629165649414,0.0002178537931555071
4805,9611,9610,19221,4.449649333953857,0.00021549280886485868
4905,9811,9810,19621,4.52517032623291,0.00021323705999951907
5005,10011,10010,20021,4.602029085159302,0.00021107038667084828
5105,10211,10210,20421,4.686842203140259,0.00020898191834835915
5205,10411,10410,20821,4.759340047836304,0.0002069636366998869
5305,10611,10610,21221,4.832656145095825,0.00020500924417355266
5405,10811,10810,21621,4.916287183761597,0.00020311357261230275
5506,11013,11012,22025,5.001103162765503,0.00020125409421659746
5606,11213,11212,22425,5.0937652587890625,0.000199463812585603
5706,11413,11412,22825,5.196096181869507,0.00019772072266799426
5806,11613,11612,23225,5.292882919311523,0.00019602185970323322
5906,11813,11812,23625,5.397942066192627,0.00019436456045111267
6006,12013,12012,24025,5.526998043060303,0.00019226895881548032
6106,12213,12212,24425,5.664118051528931,0.00018981336384564818
6206,12413,12412,24825,5.77864408493042,0.00018778452212550104
6306,12613,12612,25225,5.865795135498047,0.00018589168393157325
6406,12813,12812,25625,5.958546161651611,0.00018405691086032967
6507,13015,13014,26029,6.034569978713989,0.00018229450115027232
6607,13215,13214,26429,6.1109912395477295,0.00018061323138483316
6707,13415,13414,26829,6.1928770542144775,0.00017896837070119164
6807,13615,13614,27229,6.32046103477478,0.00017670539366986823
6907,13815,13814,27629,6.4215381145477295,0.00017394478665026857
7007,14015,14014,28029,6.527940273284912,0.00017182380289514751
7107,14215,14214,28429,6.661684989929199,0.00016995140199686445
7207,14415,14414,28829,6.759672164916992,0.00016822996598922252
7307,14615,14614,29229,6.865925312042236,0.00016600502050577174
7407,14815,14814,29629,6.957630157470703,0.00016417365369737495
7508,15017,15016,30033,7.026482343673706,0.00016248289306673215
7608,15217,15216,30433,7.097146272659302,0.00016090886540011637
7708,15417,15416,30833,7.173899173736572,0.0001588388697985169
7808,15617,15616,31233,7.319712162017822,0.00015716504752308173
7908,15817,15816,31633,7.410336017608643,0.00015560807575707016
8008,16017,16016,32033,7.489384174346924,0.0001528670951392979
8108,16217,16216,32433,7.6832640171051025,0.0001508824226984641
8208,16417,16416,32833,7.777975082397461,0.00014869762396062543
8308,16617,16616,33233,7.868849277496338,0.00014660531424563205
8408,16817,16816,33633,7.978354215621948,0.00014472799576799907
8509,17019,17018,34037,8.067054271697998,0.00014295922339428892
8609,17219,17218,34437,8.14896011352539,0.0001412736273534982
8709,17419,17418,34837,8.225372314453125,0.0001396714101891978
8809,17619,17618,35237,8.297926187515259,0.00013813795600318
8909,17819,17818,35637,8.376390218734741,0.00013538373808574897
9009,18019,18018,36037,8.449045181274414,0.00013331524081584936
9109,18219,18218,36437,8.540098190307617,0.0001315176266269928
9209,18419,18418,36837,8.61720609664917,0.00012838146992159456
9309,18619,18618,37237,8.692612171173096,0.0001260062401086033
9409,18819,18818,37637,8.776901245117188,0.000123989736577564
9510,19021,19020,38041,8.883724212646484,0.0001221400303066318
9610,19221,19220,38441,8.994230031967163,0.0001204386966298002
9710,19421,19420,38841,9.079511165618896,0.00011847239407814625
9810,19621,19620,39241,9.16598916053772,0.00011669918825553777
9910,19821,19820,39641,9.239830017089844,0.00011274641903217324
10010,20021,20020,40041,9.312960147857666,0.00011039424919270669
10110,20221,20220,40441,9.384573221206665,0.00010842101331861896
10210,20421,20420,40841,9.455811262130737,0.0001056460432049642
10310,20621,20620,41241,9.530109167098999,0.0001034347785040179
10410,20821,20820,41641,9.606977224349976,0.00010121426707386297
10511,21023,21022,42045,9.682388067245483,9.88379844340756e-05
10611,21223,21222,42445,9.77069902420044,9.691614316935306e-05
10711,21423,21422,42845,9.861533164978027,9.51729702356169e-05
10811,21623,21622,43245,9.959519147872925,9.355874460556968e-05
10911,21823,21822,43645,10.04480528831482,9.195903659656644e-05
11011,22023,22022,44045,10.126850128173828,9.044062572871737e-05
11111,22223,22222,44445,10.207280158996582,8.760072395653058e-05
11211,22423,22422,44845,10.281220197677612,8.501766878337613e-05
11311,22623,22622,45245,10.35869812965393,8.292729869838731e-05
11411,22823,22822,45645,10.43043303489685,8.10564411007725e-05
11512,23025,23024,46049,10.50618028640747,7.89596690741875e-05
11612,23225,23224,46449,10.581852197647095,7.709389597231927e-05
11712,23425,23424,46849,10.666245222091675,7.544918173016605e-05
11812,23625,23624,47249,10.742191076278687,7.397387281337675e-05
11912,23825,23824,47649,10.818507194519043,7.25963281164493e-05
12012,24025,24024,48049,10.893757343292236,7.129342706426366e-05
12112,24225,24224,48449,10.969269037246704,6.997551128540555e-05
12212,24425,24424,48849,11.04262924194336,6.870086322848533e-05
12312,24625,24624,49249,11.118250131607056,6.749927088782142e-05
12412,24825,24824,49649,11.193716049194336,6.532043439414624e-05
12513,25027,25026,50053,11.27043104171753,6.377417764162247e-05
12613,25227,25226,50453,11.342777252197266,6.241931681348971e-05
12713,25427,25426,50853,11.416340112686157,6.117000796872597e-05
12813,25627,25626,51253,11.490470170974731,5.9999357950401774e-05
12913,25827,25826,51653,11.563889265060425,5.8892075906161434e-05
13013,26027,26026,52053,11.642538070678711,5.783806989101728e-05
13113,26227,26226,52453,11.718331336975098,5.683013725086848e-05
13213,26427,26426,52853,11.796934127807617,5.586287849136061e-05
13313,26627,26626,53253,11.879348039627075,5.493210368684028e-05
13413,26827,26826,53653,11.960280179977417,5.40344745752552e-05
13514,27029,27028,54057,12.07690715789795,5.315874701548238e-05
13614,27229,27228,54457,12.19296407699585,5.231999088587542e-05
13714,27429,27428,54857,12.297738075256348,5.150748953360285e-05
13814,27629,27628,55257,12.398382186889648,5.071961773190266e-05
13914,27829,27828,55657,12.518952369689941,4.9954964822641746e-05
14014,28029,28028,56057,12.624227046966553,4.9212291176279406e-05
14114,28229,28228,56457,12.736079216003418,4.8490495271269185e-05
14214,28429,28428,56857,12.840842008590698,4.778858852014829e-05
14314,28629,28628,57257,12.95626711845398,4.710567581298244e-05
14414,28829,28828,57657,13.069595336914062,4.6440940328542634e-05
14515,29031,29030,58061,13.185526132583618,4.5787244079736674e-05
14615,29231,29230,58461,13.307294130325317,4.515683226577822e-05
14715,29431,29430,58861,13.416558265686035,4.454250253990974e-05
14815,29631,29630,59261,13.522042274475098,4.394365350429401e-05
14915,29831,29830,59661,13.626391172409058,4.335972145555563e-05
15015,30031,30030,60061,13.739590167999268,4.279017615475833e-05
15115,30231,30230,60461,13.847413063049316,4.2234517292302766e-05
15215,30431,30430,60861,13.967111349105835,4.169227150309635e-05
15315,30631,30630,61261,14.086551189422607,4.116298982875498e-05
15415,30831,30830,61661,14.20417833328247,4.064624553921866e-05
15516,31033,31032,62065,14.321059226989746,4.013664605096901e-05
15616,31233,31232,62465,14.437446117401123,3.96438916138613e-05
15716,31433,31432,62865,14.556769132614136,3.916250645932755e-05
15816,31633,31632,63265,14.66842007637024,3.8692136325430465e-05
15916,31833,31832,63665,14.771836280822754,3.823244181240052e-05
16016,32033,32032,64065,14.90726613998413,3.778309738033774e-05
16116,32233,32232,64465,15.068897008895874,3.7343790450688504e-05
16216,32433,32432,64865,15.21175503730774,3.69142205982145e-05
16316,32633,32632,65265,15.357553243637085,3.6494098819374294e-05
16416,32833,32832,65665,15.496569156646729,3.6083146870131576e-05
16517,33035,33034,66069,15.640648365020752,3.5677120231280035e-05
16617,33235,33234,66469,15.748964071273804,3.528379843960052e-05
16717,33435,33434,66869,15.851580142974854,3.4898868073149153e-05
16817,33635,33634,67269,15.959979057312012,3.452208846989514e-05
16917,33835,33834,67669,16.06515622138977,3.4153227173809356e-05
17017,34035,34034,68069,16.18707013130188,3.379205954143965e-05
17117,34235,34234,68469,16.288823127746582,3.3438368377594996e-05
17217,34435,34434,68869,16.3892822265625,3.309194359746961e-05
17317,34635,34634,69269,16.490548133850098,3.2752581913295634e-05
17417,34835,34834,69669,16.594680070877075,3.242008654192568e-05
17518,35037,35036,70073,16.75674605369568,3.2091041818962486e-05
17618,35237,35236,70473,16.855870008468628,3.177177739504206e-05
17718,35437,35436,70873,16.956817150115967,3.145882356187534e-05
17818,35637,35636,71273,17.06025719642639,3.115200705127862e-05
17918,35837,35836,71673,17.17358112335205,3.085115989694329e-05
18018,36037,36036,72073,17.276860237121582,3.055611923573243e-05
18118,36237,36236,72473,17.426112174987793,3.0266727121420946e-05
18218,36437,36436,72873,17.526703119277954,2.998283034703666e-05
18318,36637,36636,73273,17.63402223587036,2.9704280278715254e-05
18418,36837,36836,73673,17.74004626274109,2.9430932697111267e-05
18519,37039,37038,74077,17.84474015235901,2.9159989898597117e-05
18619,37239,37238,74477,17.944088220596313,2.8896680138948832e-05
18719,37439,37438,74877,18.045551300048828,2.8638163927325157e-05
18819,37639,37638,75277,18.148414134979248,2.838431330815558e-05
18919,37839,37838,75677,18.264541387557983,2.8135004055142335e-05
19019,38039,38038,76077,18.376450061798096,2.7890115554991762e-05
19119,38239,38238,76477,18.478642225265503,2.7649530692710136e-05
19219,38439,38438,76877,18.584816217422485,2.7413135744249717e-05
19319,38639,38638,77277,18.69430136680603,2.7180820271181197e-05
19419,38839,38838,77677,18.798993349075317,2.6952477022695076e-05
19520,39041,39040,78081,18.90667223930359,2.6725776274959876e-05
19620,39241,39240,78481,19.028571128845215,2.6505105158808064e-05
19720,39441,39440,78881,19.135950088500977,2.6288101721943395e-05
19820,39641,39640,79281,19.242622137069702,2.60746705615014e-05
19920,39841,39840,79681,19.34536123275757,2.5864719015414138e-05
20020,40041,40040,80081,19.4580180644989,2.5658157080510214e-05
20120,40241,40240,80481,19.56177306175232,2.5454897336755517e-05
20220,40441,40440,80881,19.683651208877563,2.5254854872420898e-05
20320,40641,40640,81281,19.793426990509033,2.5057947211617455e-05
20420,40841,40840,81681,19.899259328842163,2.4864094243831293e-05
20521,41043,41042,82085,19.999800205230713,2.4671324172818473e-05
20621,41243,41242,82485,20.10373306274414,2.4483378027808908e-05
20721,41443,41442,82885,20.209615230560303,2.429825905215031e-05
20821,41643,41642,83285,20.310593128204346,2.411589596343249e-05
20921,41843,41842,83685,20.426883220672607,2.3936219526962322e-05
21021,42043,42042,84085,20.528851985931396,2.375916249582231e-05
21121,42243,42242,84485,20.627896070480347,2.358465955640318e-05
21221,42443,42442,84885,20.735274076461792,2.3412647271865886e-05
21321,42643,42642,85285,20.842782974243164,2.3243064029661924e-05
21421,42843,42842,85685,20.9623122215271,2.307584999029077e-05
21522,43045,43044,86089,21.10989212989807,2.290930948446167e-05
21622,43245,43244,86489,21.254266262054443,2.274668343669633e-05
21722,43445,43444,86889,21.404250144958496,2.2586256669867326e-05
21822,43645,43644,87289,21.612995147705078,2.2427975960148327e-05
21922,43845,43844,87689,21.752506256103516,2.2271789617417764e-05
22022,44045,44044,88089,21.870522260665894,2.2117647441859577e-05
22122,44245,44244,88489,21.99016499519348,2.1965500681564148e-05
22222,44445,44444,88889,22.099338054656982,2.1815301990555972e-05
22322,44645,44644,89289,22.232834100723267,2.1667005389170224e-05
22422,44845,44844,89689,22.351218223571777,2.1520566223945708e-05
22523,45047,45046,90093,22.45926308631897,2.137450389743613e-05
22623,45247,45246,90493,22.58220911026001,2.1231668274742093e-05
22723,45447,45446,90893,22.70063328742981,2.109056331098932e-05
22823,45647,45646,91293,22.825556993484497,2.095114930112278e-05
22923,45847,45846,91693,22.93882131576538,2.0813387685584392e-05
23023,46047,46046,92093,23.06244206428528,2.067724101748545e-05
23123,46247,46246,92493,23.180089235305786,2.054267293063988e-05
23223,46447,46446,92893,23.283591270446777,2.040964810749064e-05
23323,46647,46646,93293,23.387843132019043,2.0278132248572443e-05
23423,46847,46846,93693,23.48790192604065,2.014809204346726e-05
23524,47049,47048,94097,23.593610048294067,2.0018216353502114e-05
23624,47249,47248,94497,23.701472997665405,1.989104529704416e-05
23724,47449,47448,94897,23.80323100090027,1.9765255307275363e-05
23824,47649,47648,95297,23.90330219268799,1.9640816754702152e-05
23924,47849,47848,95697,24.00944995880127,1.9517700861296387e-05
24024,48049,48048,96097,24.110535144805908,1.9395879674889236e-05
24124,48249,48248,96497,24.214813947677612,1.9275326045535996e-05
24224,48449,48448,96897,24.31739115715027,1.9156013600908175e-05
24324,48649,48648,97297,24.41633105278015,1.9037916723550638e-05
24424,48849,48848,97697,24.51978325843811,1.8921010528517207e-05
24525,49051,49050,98101,24.63312005996704,1.8804119255199948e-05
24625,49251,49250,98501,24.75270915031433,1.8689533904571334e-05
24725,49451,49450,98901,24.853676080703735,1.857606853538815e-05
24825,49651,49650,99301,24.95366621017456,1.846370098658152e-05
24925,49851,49850,99701,25.052947998046875,1.835240972575939e-05
25025,50051,50050,100101,25.156164169311523,1.8242173830892025e-05
25125,50251,50250,100501,25.25630807876587,1.8132972971845767e-05
25225,50451,50450,100901,25.359933376312256,1.8024787392688152e-05
25325,50651,50650,101301,25.460934162139893,1.791759789366019e-05
25425,50851,50850,101701,25.564114332199097,1.7811385815375412e-05
25526,51053,51052,102105,25.66991114616394,1.7705085278162808e-05
25626,51253,51252,102505,25.769639253616333,1.7600783470369335e-05
25726,51453,51452,102905,25.86827325820923,1.749740601403757e-05
25826,51653,51652,103305,25.968862056732178,1.7394936255609e-05
25926,51853,51852,103705,26.070621967315674,1.729335800409566e-05
26026,52053,52052,104105,26.172730207443237,1.7192655517201312e-05
26126,52253,52252,104505,26.277496099472046,1.7092813487563866e-05
26226,52453,52452,104905,26.377682209014893,1.6993817030214183e-05
26326,52653,52652,105305,26.4779691696167,1.68956516684544e-05
26426,52853,52852,105705,26.580912113189697,1.6798303322708575e-05
26527,53055,53054,106109,26.68442440032959,1.670079685866953e-05
26627,53255,53254,106509,26.79988932609558,1.660504966524333e-05
26727,53455,53454,106909,26.91183614730835,1.6510079380238825e-05
26827,53655,53654,107309,27.014228105545044,1.641587339620174e-05
26927,53855,53854,107709,27.118714094161987,1.6322419444874413e-05
27027,54055,54054,108109,27.22154211997986,1.622970558720964e-05
27127,54255,54254,108509,27.327182054519653,1.6137720202917003e-05
27227,54455,54454,108909,27.424816131591797,1.604645198133419e-05
27327,54655,54654,109309,27.529564142227173,1.5955889911033592e-05
27427,54855,54854,109709,27.635689973831177,1.5866023271890535e-05
27528,55057,55056,110113,27.735810041427612,1.5775953233158783e-05
27628,55257,55256,110513,27.837635278701782,1.568745311075853e-05
27728,55457,55456,110913,27.940760135650635,1.559961781625362e-05
27828,55657,55656,111313,28.044401168823242,1.5512437707874757e-05
27928,55857,55856,111713,28.152737140655518,1.5425903392593543e-05
28028,56057,56056,112113,28.252470016479492,1.5340005718320964e-05
28128,56257,56256,112513,28.35704016685486,1.525473576666453e-05
28228,56457,56456,112913,28.45846128463745,1.5170084845910363e-05
28328,56657,56656,113313,28.562904119491577,1.5086044483851001e-05
28428,56857,56856,113713,28.66449522972107,1.5002606421231444e-05
28529,57059,57058,114117,28.765266180038452,1.4918937141126023e-05
28629,57259,57258,114517,28.870808124542236,1.4836685543758747e-05
28729,57459,57458,114917,28.98716115951538,1.4755012605720003e-05
28829,57659,57658,115317,29.086259365081787,1.4673910858305012e-05
28929,57859,57858,115717,29.187304258346558,1.4593373014588697e-05
29029,58059,58058,116117,29.29400396347046,1.4513391965261338e-05
29129,58259,58258,116517,29.396027326583862,1.4433960771370196e-05
29229,58459,58458,116917,29.49954628944397,1.4355072660792616e-05
29329,58659,58658,117317,29.605151176452637,1.4276721022064467e-05
29429,58859,58858,117717,29.713823080062866,1.4198899400570339e-05
29530,59061,59060,118121,29.822351217269897,1.412083113709544e-05
29630,59261,59260,118521,29.924923181533813,1.4044055930350786e-05
29730,59461,59460,118921,30.027302265167236,1.3967792206863045e-05
29830,59661,59660,119321,30.133381128311157,1.3892034091469082e-05
29930,59861,59860,119721,30.239591360092163,1.3816775843772175e-05
30030,60061,60060,120121,30.347352266311646,1.3742011852258061e-05
30130,60261,60260,120521,30.450016021728516,1.3667736632245829e-05
30230,60461,60460,120921,30.550556182861328,1.3593944821175885e-05
30330,60661,60660,121321,30.653573274612427,1.3520631174841028e-05
30430,60861,60860,121721,30.753499269485474,1.3447790563785466e-05
30531,61063,61062,122125,30.85486912727356,1.3374696591499395e-05
30631,61263,61262,122525,30.95430612564087,1.3302791713261758e-05
30731,61463,61462,122925,31.06964421272278,1.323134509156123e-05
30831,61663,61662,123325,31.182352304458618,1.3160352024723339e-05
30931,61863,61862,123725,31.292527198791504,1.3089807910219068e-05
31031,62063,62062,124125,31.405327081680298,1.3019708241126746e-05
31131,62263,62262,124525,31.507395267486572,1.2950048603807798e-05
31231,62463,62462,124925,31.612488985061646,1.2880824674895394e-05
31331,62663,62662,125325,31.71368908882141,1.2812032218859102e-05
31431,62863,62862,125725,31.817703247070312,1.2743667084967246e-05
31532,63065,63064,126129,31.92434310913086,1.2675047910385669e-05
31632,63265,63264,126529,32.03887724876404,1.2607529470036943e-05
31732,63465,63464,126929,32.144713163375854,1.2540426347793953e-05
31832,63665,63664,127329,32.246196031570435,1.2473734709913572e-05
31932,63865,63864,127729,32.34967613220215,1.2407450796598108e-05
32032,64065,64064,128129,32.449201345443726,1.2341570918836015e-05
32132,64265,64264,128529,32.54858422279358,1.2276091457306583e-05
32232,64465,64464,128929,32.66675114631653,1.2211008859601882e-05
32332,64665,64664,129329,32.76741623878479,1.2146319638728943e-05
32432,64865,64864,129729,32.869649171829224,1.2082020371446252e-05
32533,65067,65066,130133,32.97638416290283,1.2017470510092746e-05
32633,65267,65266,130533,33.07767915725708,1.1953944940703191e-05
32733,65467,65466,130933,33.189101219177246,1.1890799385439199e-05
32833,65667,65666,131333,33.30017113685608,1.1828030657689164e-05
32933,65867,65866,131733,33.40964412689209,1.1765635626103807e-05
33033,66067,66066,132133,33.51306223869324,1.1703611212723357e-05
33133,66267,66266,132533,33.611897230148315,1.1641954391581306e-05
33233,66467,66466,132933,33.713993072509766,1.1580662187235834e-05
33333,66667,66666,133333,33.81589722633362,1.151973167320635e-05
33433,66867,66866,133733,33.91670513153076,1.145915997127233e-05
33534,67069,67068,134137,34.020872354507446,1.1398343880375843e-05
33634,67269,67268,134537,34.122106313705444,1.1338484869761771e-05
33734,67469,67468,134937,34.225759983062744,1.1278976282498303e-05
33834,67669,67668,135337,34.32770323753357,1.1219815419291802e-05
33934,67869,67868,135737,34.430339097976685,1.1160999622212621e-05
34034,68069,68068,136137,34.527913093566895,1.1102526274125163e-05
34134,68269,68268,136537,34.62800312042236,1.1044392797122087e-05
34234,68469,68468,136937,34.73245811462402,1.0986596652116044e-05
34334,68669,68668,137337,34.83179211616516,1.092913533714529e-05
34434,68869,68868,137737,34.93324613571167,1.087200638689396e-05
34535,69071,69070,138141,35.04060912132263,1.0814641039152443e-05
34635,69271,69270,138541,35.1400990486145,1.0758172826412265e-05
34735,69471,69470,138941,35.239885091781616,1.0702029768192477e-05
34835,69671,69670,139341,35.35705494880676,1.0646209535832354e-05
34935,69871,69870,139741,35.463709354400635,1.0590709832984052e-05
35035,70071,70070,140141,35.56255531311035,1.0535528394461525e-05
35135,70271,70270,140541,35.66658616065979,1.0480662985438994e-05
35235,70471,70470,140941,35.76502823829651,1.0426111400662178e-05
35335,70671,70670,141341,35.86672019958496,1.0371871463733768e-05
35435,70871,70870,141741,35.96499824523926,1.0317941026897855e-05
35536,71073,71072,142145,36.0654993057251,1.0263783283944533e-05
35636,71273,71272,142545,36.166359186172485,1.0210468554471236e-05
35736,71473,71472,142945,36.26771521568298,1.0157457022502795e-05
35836,71673,71672,143345,36.368667125701904,1.0104746646564005e-05
35936,71873,71872,143745,36.46716594696045,1.0052335410015979e-05
36036,72073,72072,144145,36.5653293132782,1.0000221320252732e-05
36136,72273,72272,144545,36.67101693153381,9.948402408870986e-06
36236,72473,72472,144945,36.7737090587616,9.896876730314829e-06
36336,72673,72672,145345,36.873839139938354,9.845642362438357e-06
36436,72873,72872,145745,36.977638244628906,9.794697404628907e-06
36537,73075,73074,146149,37.083521127700806,9.74353484946901e-06
36637,73275,73274,146549,37.21228313446045,9.693165944138935e-06
36737,73475,73474,146949,37.33172607421875,9.643080857668941e-06
36837,73675,73674,147349,37.44846320152283,9.593277773582359e-06
36937,73875,73874,147749,37.56352210044861,9.543754895089129e-06
37037,74075,74074,148149,37.67926502227783,9.494510445563372e-06
37137,74275,74274,148549,37.78353214263916,9.445542666678655e-06
37237,74475,74474,148949,37.890079975128174,9.39684981854373e-06
37337,74675,74674,149349,37.9896981716156,9.348430179943802e-06
37437,74875,74874,149749,38.0910861492157,9.300282047109628e-06
37538,75077,75076,150153,38.19508934020996,9.251926307497324e-06
37638,75277,75276,150553,38.2969172000885,9.204318817428131e-06
37738,75477,75476,150953,38.398585081100464,9.156977808712949e-06
37838,75677,75676,151353,38.50137495994568,9.109901645389194e-06
37938,75877,75876,151753,38.60097098350525,9.06308870710001e-06
38038,76077,76076,152153,38.71761107444763,9.016537389877662e-06
38138,76277,76276,152553,38.85112714767456,8.97024610490771e-06
38238,76477,76476,152953,39.005346059799194,8.924213278269528e-06
38338,76677,76676,153353,39.14303421974182,8.878437350907728e-06
38438,76877,76876,153753,39.25026822090149,8.83291677849829e-06
38539,77079,77078,154157,39.354480266571045,8.787198639970328e-06
38639,77279,77278,154557,39.4545202255249,8.742186716186681e-06
38739,77479,77478,154957,39.564836263656616,8.69742558348526e-06
38839,77679,77678,155357,39.68078327178955,8.652913752906591e-06
38939,77879,77878,155757,39.82592225074768,8.608649748757887e-06
39039,78079,78078,156157,39.98680233955383,8.564632108607513e-06
39139,78279,78278,156557,40.163650035858154,8.520859381960493e-06
39239,78479,78478,156957,40.37507104873657,8.477330131968392e-06
39339,78679,78678,157357,40.47745203971863,8.434042933128069e-06
39439,78879,78878,157757,40.65609407424927,8.390996372740759e-06
39540,79081,79080,158161,40.874149322509766,8.347762179717916e-06
39640,79281,79280,158561,40.982991218566895,8.305195075779838e-06
39740,79481,79480,158961,41.08484625816345,8.262864427904646e-06
39840,79681,79680,159361,41.19215226173401,8.220768869818147e-06
39940,79881,79880,159761,41.301215171813965,8.178907046014787e-06
40040,80081,80080,160161,41.40928411483765,8.13727761196053e-06
40140,80281,80280,160561,41.5113160610199,8.095879234201466e-06
40240,80481,80480,160961,41.620946168899536,8.054710589422994e-06
40340,80681,80680,161361,41.83861303329468,8.013770365173272e-06
40440,80881,80880,161761,42.017919063568115,7.973057259006582e-06
40541,81083,81082,162165,42.247716188430786,7.93216624198212e-06
40641,81283,81282,162565,42.44263505935669,7.891905744237378e-06
40741,81483,81482,162965,42.543612241744995,7.85186850499992e-06
40841,81683,81682,163365,42.72900724411011,7.812053261607058e-06
40941,81883,81882,163765,42.85758018493652,7.772458760678725e-06
41041,82083,82082,164165,42.96165204048157,7.733083758506741e-06
41141,82283,82282,164565,43.06507706642151,7.693927020716855e-06
41241,82483,82482,164965,43.169800996780396,7.654987321654853e-06
41341,82683,82682,165365,43.275665283203125,7.616263445389694e-06
41441,82883,82882,165765,43.38475704193115,7.577754183968579e-06
41542,83085,83084,166169,43.490100145339966,7.539076454204235e-06
41642,83285,83284,166569,43.599133253097534,7.500994951635613e-06
41742,83485,83484,166969,43.70434927940369,7.4631244818936705e-06
41842,83685,83684,167369,43.80776500701904,7.425463871914123e-06
41942,83885,83884,167769,43.99910521507263,7.388011956974788e-06
42042,84085,84084,168169,44.17692232131958,7.35076758060331e-06
42142,84285,84284,168569,44.37733316421509,7.313729594061847e-06
42242,84485,84484,168969,44.48134207725525,7.2768968571314685e-06
42342,84685,84684,169369,44.584593296051025,7.24026823721206e-06
42442,84885,84884,169769,44.69068717956543,7.203842609448843e-06
42543,85087,85086,170173,44.79387331008911,7.16725763496288e-06
42643,85287,85286,170573,44.90286898612976,7.131236650136116e-06
42743,85487,85486,170973,45.002530097961426,7.095415318007942e-06
42843,85687,85686,171373,45.10636019706726,7.059792544354096e-06
42943,85887,85886,171773,45.21059727668762,7.0243672419622075e-06
43043,86087,86086,172173,45.312313079833984,6.989138331090712e-06
43143,86287,86286,172573,45.41354322433472,6.954104739154548e-06
43243,86487,86486,172973,45.52088499069214,6.9192654006023495e-06
43343,86687,86686,173373,45.622828006744385,6.884619256872231e-06
43443,86887,86886,173773,45.73828101158142,6.850165256685627e-06
43544,87089,87088,174177,45.94174528121948,6.815560687752278e-06
43644,87289,87288,174577,46.110809087753296,6.781489742640136e-06
43744,87489,87488,174977,46.27103328704834,6.747607816964063e-06
43844,87689,87688,175377,46.37400221824646,6.7139138864022474e-06
43944,87889,87888,175777,46.47498607635498,6.680406933143287e-06
44044,88089,88088,176177,46.58612608909607,6.647085946019172e-06
44144,88289,88288,176577,46.703660011291504,6.613949920010182e-06
44244,88489,88488,176977,46.819880962371826,6.58099785674499e-06
44344,88689,88688,177377,46.99234628677368,6.5482287641530055e-06
44444,88889,88888,177777,47.22457814216614,6.515641656444835e-06
44545,89091,89090,178181,47.43951916694641,6.482912403623686e-06
44645,89291,89290,178581,47.60617804527283,6.450688128178052e-06
44745,89491,89490,178981,47.70934724807739,6.4186429074786614e-06
44845,89691,89690,179381,47.83062124252319,6.386775780018332e-06
44945,89891,89890,179781,48.031583070755005,6.355085790635725e-06
45045,90091,90090,180181,48.13915801048279,6.323571989721938e-06
45145,90291,90290,180581,48.253451108932495,6.292233433956981e-06
45245,90491,90490,180981,48.365581035614014,6.261069185429767e-06
45345,90691,90690,181381,48.46831226348877,6.230078312059861e-06
45445,90891,90890,181781,48.56904220581055,6.199259887835986e-06
45546,91093,91092,182185,48.67323613166809,6.168307385898487e-06
45646,91293,91292,182585,48.777981996536255,6.137832804711906e-06
45746,91493,91492,182985,48.8846001625061,6.1075279183302e-06
45846,91693,91692,183385,48.9891562461853,6.077391822975231e-06
45946,91893,91892,183785,49.09219717979431,6.047423619766005e-06
46046,92093,92092,184185,49.194677114486694,6.017622416051659e-06
46146,92293,92292,184585,49.29855513572693,5.987987324065617e-06
46246,92493,92492,184985,49.40027904510498,5.958517461319691e-06
46346,92693,92692,185385,49.501004219055176,5.929211950894008e-06
46446,92893,92892,185785,49.60478734970093,5.900069920885861e-06
46547,93095,93094,186189,49.71181321144104,5.870801528813013e-06
46647,93295,93294,186589,49.814640283584595,5.841985478237522e-06
46747,93495,93494,186989,49.915300130844116,5.813330314928808e-06
46847,93695,93694,187389,50.0175621509552,5.784835187868471e-06
46947,93895,93894,187789,50.11969304084778,5.756499250526048e-06
47047,94095,94094,188189,50.22571611404419,5.7283216620927856e-06
47147,94295,94294,188589,50.32874417304993,5.7003015858583396e-06
47247,94495,94494,188989,50.447163343429565,5.672438190651915e-06
47347,94695,94694,189389,50.54650115966797,5.6447306499422615e-06
47447,94895,94894,189789,50.6466600894928,5.61717814195004e-06
47548,95097,95096,190193,50.74992823600769,5.589506643035452e-06
47648,95297,95296,190593,50.84984016418457,5.562263284700671e-06
47748,95497,95496,190993,50.94977521896362,5.535172514797879e-06
47848,95697,95696,191393,51.05258226394653,5.50823353060782e-06
47948,95897,95896,191793,51.15896224975586,5.48144553394883e-06
48048,96097,96096,192193,51.26131510734558,5.454807731632171e-06
48148,96297,96296,192593,51.3629412651062,5.428319334839365e-06
48248,96497,96496,192993,51.46465826034546,5.401979559216118e-06
48348,96697,96696,193393,51.5663480758667,5.375787625232161e-06
48448,96897,96896,193793,51.67214918136597,5.349742757503943e-06
48549,97099,97098,194197,51.77845025062561,5.323585935685384e-06
48649,97299,97298,194597,51.88401818275452,5.297834343902858e-06
48749,97499,97498,194997,51.986568212509155,5.272227511842524e-06
48849,97699,97698,195397,52.08934807777405,5.246764681542395e-06
48949,97899,97898,195797,52.19312834739685,5.22144510013245e-06
49049,98099,98098,196197,52.29562711715698,5.196268018480843e-06
49149,98299,98298,196597,52.39695429801941,5.171232691703259e-06
49249,98499,98498,196997,52.51057410240173,5.146338379849339e-06
49349,98699,98698,197397,52.62275409698486,5.121584346210965e-06
49449,98899,98898,197797,52.73303031921387,5.096969858858035e-06
49550,99101,99100,198201,52.837470054626465,5.072250131919366e-06
49650,99301,99300,198601,52.940104246139526,5.047913935088097e-06
49750,99501,99500,199001,53.04196810722351,5.023715105716969e-06
49850,99701,99700,199401,53.14535713195801,4.999652928508329e-06
49950,99901,99900,199801,53.2530403137207,4.975726691870215e-06
50050,100101,100100,200201,53.3644642829895,4.951935688293543e-06
50150,100301,100300,200601,53.468767166137695,4.928279214059409e-06
50250,100501,100500,201001,53.56981825828552,4.904756569533034e-06
50350,100701,100700,201401,53.6709303855896,4.881367059087401e-06
50450,100901,100900,201801,53.77235007286072,4.858109990902602e-06
50551,101103,101102,202205,53.87683415412903,4.834754087025463e-06
50651,101303,101302,202605,53.9776291847229,4.811761150684866e-06
50751,101503,101502,203005,54.0791802406311,4.788898597468498e-06
50851,101703,101702,203405,54.18799901008606,4.7661657510782e-06
50951,101903,101902,203805,54.287660121917725,4.7435619388122915e-06
51051,102103,102102,204205,54.386139154434204,4.721086491744434e-06
51151,102303,102302,204605,54.48935413360596,4.698738744567397e-06
51251,102503,102502,205005,54.595059394836426,4.67651803588588e-06
51351,102703,102702,205405,54.716997146606445,4.65442370798411e-06
51451,102903,102902,205805,54.820436000823975,4.632455106646605e-06
51552,103105,103104,206209,54.92305827140808,4.6103937754140965e-06
51652,103305,103304,206609,55.0226571559906,4.588675919869479e-06
51752,103505,103504,207009,55.12048530578613,4.56708184364518e-06
51852,103705,103704,207409,55.239176988601685,4.5456109068755234e-06
51952,103905,103904,207809,55.37847924232483,4.524262473038207e-06
52052,104105,104104,208209,55.533244132995605,4.50303590985631e-06
52152,104305,104304,208609,55.633039236068726,4.481930587629535e-06
52252,104505,104504,209009,55.73797917366028,4.4609458807438155e-06
52352,104705,104704,209409,55.84005403518677,4.44008116686596e-06
52452,104905,104904,209809,55.94533133506775,4.419335826924423e-06
52553,105107,105106,210213,56.04826331138611,4.398503576999496e-06
52653,105307,105306,210613,56.153748989105225,4.377996319994162e-06
52753,105507,105506,211013,56.277130126953125,4.357606594234406e-06
52853,105707,105706,211413,56.44590210914612,4.337333794270907e-06
52953,105907,105906,211813,56.58954215049744,4.317177317871906e-06
53053,106107,106106,212213,56.71138405799866,4.297136566234023e-06
53153,106307,106306,212613,56.828797340393066,4.277210943642991e-06
53253,106507,106506,213013,56.93524932861328,4.257399857657006e-06
53353,106707,106706,213413,57.03900218009949,4.237702719258374e-06
53453,106907,106906,213813,57.14194631576538,4.218118942136207e-06
53554,107109,107108,214217,57.245851278305054,4.198453801489868e-06
53654,107309,107308,214617,57.34871220588684,4.1790961215606555e-06
53754,107509,107508,215017,57.448331117630005,4.159850058205327e-06
53854,107709,107708,215417,57.547160148620605,4.140715038374712e-06
53954,107909,107908,215817,57.64982724189758,4.12169049185086e-06
54054,108109,108108,216217,57.78003215789795,4.102775851226692e-06
54154,108309,108308,216617,57.95662808418274,4.083970552582838e-06
54254,108509,108508,217017,58.08343815803528,4.065274034718134e-06
54354,108709,108708,217417,58.232728242874146,4.046685739693659e-06
54454,108909,108908,217817,58.34463906288147,4.028205112167068e-06
54555,109111,109110,218221,58.444677114486694,4.009648404477159e-06
54655,109311,109310,218621,58.543519020080566,3.991382522047146e-06
54755,109511,109510,219021,58.64771914482117,3.9732226543964645e-06
54855,109711,109710,219421,58.74995517730713,3.95516825846744e-06
54955,109911,109910,219821,58.85095024108887,3.937218793731326e-06
55055,110111,110110,220221,58.97096014022827,3.9193737228706324e-06
55155,110311,110310,220621,59.07712531089783,3.901632511197682e-06
55255,110511,110510,221021,59.17912030220032,3.883994627014341e-06
55355,110711,110710,221421,59.27898812294006,3.866459541242284e-06
55455,110911,110910,221821,59.38111615180969,3.849026727987626e-06
55556,111113,111112,222225,59.48685121536255,3.831522865416961e-06
55656,111313,111312,222625,59.5897159576416,3.814294039421805e-06
55756,111513,111512,223025,59.69114923477173,3.7971659193340194e-06
55856,111713,111712,223425,59.78925323486328,3.7801379897162253e-06
55956,111913,111912,223825,59.88989210128784,3.7632097383087628e-06
56056,112113,112112,224225,59.98958420753479,3.746380655818998e-06
56156,112313,112312,224625,60.11167120933533,3.7296502350543283e-06
56256,112513,112512,225025,60.23150014877319,3.7130179717656068e-06
56356,112713,112712,225425,60.34554719924927,3.6964833643197807e-06
56456,112913,112912,225825,60.458627223968506,3.680045913899004e-06
56557,113115,113114,226229,60.573596239089966,3.6635422025605246e-06
56657,113315,113314,226629,60.68550205230713,3.6472985387737856e-06
56757,113515,113514,227029,60.8016791343689,3.631150545658939e-06
56857,113715,113714,227429,60.91537308692932,3.6150977346360793e-06
56957,113915,113914,227829,61.0342321395874,3.5991396197010377e-06
57057,114115,114114,228229,61.15578317642212,3.5832757172888128e-06
57157,114315,114314,228629,61.26014423370361,3.5675055463678695e-06
57257,114515,114514,229029,61.36601495742798,3.5518286286233473e-06
57357,114715,114714,229429,61.47215914726257,3.5362444877194963e-06
57457,114915,114914,229829,61.579395055770874,3.520752650323909e-06
57558,115117,115116,230233,61.68844699859619,3.5051991071690087e-06
57658,115317,115316,230633,61.791574001312256,3.4898913768323703e-06
57758,115517,115516,231033,61.896756172180176,3.474674539149808e-06
57858,115717,115716,231433,62.00423717498779,3.4595481300296076e-06
57958,115917,115916,231833,62.112807273864746,3.444511688451795e-06
58058,116117,116116,232233,62.22048830986023,3.4295647549437967e-06
58158,116317,116316,232633,62.33106517791748,3.414706872755212e-06
58258,116517,116516,233033,62.43858623504639,3.3999375876989694e-06
58358,116717,116716,233433,62.54180097579956,3.3852564473989437e-06
58458,116917,116916,233833,62.65843725204468,3.370663002187943e-06
58559,117119,117118,234237,62.778656005859375,3.3560121814881122e-06
58659,117319,117318,234637,62.89924216270447,3.341593651901923e-06
58759,117519,117518,235037,63.00933623313904,3.327261477001474e-06
58859,117719,117718,235437,63.11628603935242,3.313015216356852e-06
58959,117919,117918,235837,63.283374071121216,3.29885443130374e-06
59059,118119,118118,236237,63.44907808303833,3.2847786855520033e-06
59159,118319,118318,236637,63.60206317901611,3.270787545082869e-06
59259,118519,118518,237037,63.73354434967041,3.2568805777448162e-06
59359,118719,118718,237437,63.90878915786743,3.243057354221872e-06
59459,118919,118918,237837,64.10689115524292,3.229317446507438e-06
59560,119121,119120,238241,64.28118515014648,3.2155242764601247e-06
59660,119321,119320,238641,64.62930727005005,3.2019505491993925e-06
59760,119521,119520,239041,64.84549927711487,3.188458863532566e-06
59860,119721,119720,239441,65.09259128570557,3.1750488005229006e-06
59960,119921,119920,239841,65.29561805725098,3.1617199431699828e-06
60060,120121,120120,240241,65.45650815963745,3.148471876535181e-06
60160,120321,120320,240641,65.764484167099,3.1353041875904403e-06
60260,120521,120520,241041,65.94493699073792,3.12221646560781e-06
60360,120721,120720,241441,66.07479119300842,3.109208301734977e-06
60460,120921,120920,241841,66.19477415084839,3.096279288879458e-06
60561,121123,121122,242245,66.30953598022461,3.0833009160880306e-06
60661,121323,121322,242645,66.42448616027832,3.0705297745346636e-06
60761,121523,121522,243045,66.54067516326904,3.057836571767367e-06
60861,121723,121722,243445,66.65636825561523,3.0452209085410903e-06
60961,121923,121922,243845,66.77815818786621,3.0326823878801493e-06
61061,122123,122122,244245,66.8913562297821,3.0202206151558014e-06
61161,122323,122322,244645,67.00161409378052,3.0078351968175384e-06
61261,122523,122522,245045,67.11826729774475,2.995525741793433e-06
61361,122723,122722,245445,67.2259521484375,2.983291860656169e-06
61461,122923,122922,245845,67.33637809753418,2.9711331660294383e-06
61562,123125,123124,246249,67.44893908500671,2.9589288098924783e-06
61662,123325,123324,246649,67.5767571926117,2.9469200756642875e-06
61762,123525,123524,247049,67.6853392124176,2.934985372665422e-06
61862,123725,123724,247449,67.79008316993713,2.9231243211627506e-06
61962,123925,123924,247849,67.89725518226624,2.9113365428115323e-06
62062,124125,124124,248249,68.01188921928406,2.8996216609782116e-06
62162,124325,124324,248649,68.15599918365479,2.8879793009363483e-06
62262,124525,124524,249049,68.30095219612122,2.876409090102088e-06
62362,124725,124724,249449,68.40800213813782,2.864910657114372e-06
62462,124925,124924,249849,68.50756025314331,2.853483632643486e-06
62563,125127,125126,250253,68.60940313339233,2.8420144466557163e-06
62663,125327,125326,250653,68.70946717262268,2.830729842905204e-06
62763,125527,125526,251053,68.80888605117798,2.819515546092488e-06
62863,125727,125726,251453,68.90914916992188,2.8083711939183947e-06
62963,125927,125926,251853,69.01304602622986,2.797296425574582e-06
63063,126127,126126,252253,69.11284303665161,2.7862908817192455e-06
63163,126327,126326,252653,69.21514010429382,2.775354205192744e-06
63263,126527,126526,253053,69.31524419784546,2.7644860399032016e-06
63363,126727,126726,253453,69.41325807571411,2.7536860318430737e-06
63463,126927,126926,253853,69.5091462135315,2.7429538284824577e-06
63564,127129,127128,254257,69.61159706115723,2.7321827708355152e-06
63664,127329,127328,254657,69.72320103645325,2.721585794767247e-06
63764,127529,127528,255057,69.8349711894989,2.711055572255011e-06
63864,127729,127728,255457,70.00159811973572,2.700591756681407e-06
63964,127929,127928,255857,70.1339361667633,2.6901940038882488e-06
64064,128129,128128,256257,70.23588299751282,2.6798619706745087e-06
64164,128329,128328,256657,70.33814716339111,2.6695953156258623e-06
64264,128529,128528,257057,70.46089816093445,2.659393699021787e-06
64364,128729,128728,257457,70.62414693832397,2.649256782559759e-06
64464,128929,128928,257857,70.77940917015076,2.639184229190856e-06
64565,129131,129130,258261,70.89299511909485,2.6290759409266197e-06
64665,129331,129330,258661,70.9902720451355,2.6191317449486765e-06
64765,129531,129530,259061,71.10234498977661,2.6092509074161096e-06
64865,129731,129730,259461,71.22846531867981,2.5994330977607984e-06
64965,129931,129930,259861,71.33300924301147,2.589677986323251e-06
65065,130131,130130,260261,71.4307131767273,2.5799852454567913e-06
65165,130331,130330,260661,71.52759623527527,2.5703545484942893e-06
65265,130531,130530,261061,71.62449836730957,2.5607855706475568e-06
65365,130731,130730,261461,71.72826218605042,2.5512779882598767e-06
65465,130931,130930,261861,71.84188532829285,2.5418314792641497e-06
65566,131133,131132,262265,71.94398427009583,2.5323521709510194e-06
65666,131333,131332,262665,72.04446816444397,2.523027450649723e-06
65766,131533,131532,263065,72.143470287323,2.5137628423610064e-06
65866,131733,131732,263465,72.24342608451843,2.5045580298119715e-06
65966,131933,131932,263865,72.3437283039093,2.4954126978385856e-06
66066,132133,132132,264265,72.44011116027832,2.4863265324961008e-06
66166,132333,132332,264665,72.53612613677979,2.4772992213185746e-06
66266,132533,132532,265065,72.63615322113037,2.468330453227136e-06
66366,132733,132732,265465,72.73270034790039,2.4594199184772105e-06
66466,132933,132932,265865,72.82887411117554,2.4505673088944696e-06
66567,133135,133134,266269,72.92542719841003,2.4416846569844214e-06
66667,133335,133334,266669,73.02438521385193,2.4329475486101967e-06
66767,133535,133534,267069,73.12055611610413,2.424267444997775e-06
66867,133735,133734,267469,73.2204282283783,2.415644042512235e-06
66967,133935,133934,267869,73.32311725616455,2.407077039411883e-06
67067,134135,134134,268269,73.42170596122742,2.398566135092775e-06
67167,134335,134334,268669,73.52293038368225,2.3901110302742894e-06
67267,134535,134534,269069,73.61944723129272,2.3817114267139655e-06
67367,134735,134734,269469,73.71494507789612,2.373367027660072e-06
67467,134935,134934,269869,73.81232523918152,2.3650775374344425e-06
67568,135137,135136,270273,73.9314432144165,2.3567605878678364e-06
67668,135337,135336,270673,74.03434324264526,2.3485805752968476e-06
67768,135537,135536,271073,74.13284730911255,2.3404545891950986e-06
67868,135737,135736,271473,74.22797012329102,2.3323823390859886e-06
67968,135937,135936,271873,74.32362914085388,2.324363535425193e-06
68068,136137,136136,272273,74.41878724098206,2.3163978898000402e-06
68168,136337,136336,272673,74.51795625686646,2.3084851152131723e-06
68268,136537,136536,273073,74.61405110359192,2.3006249257527494e-06
68368,136737,136736,273473,74.7115273475647,2.292817036715171e-06
68468,136937,136936,273873,74.80643010139465,2.28506116463904e-06
68569,137139,137138,274277,74.90263414382935,2.277280245826642e-06
68669,137339,137338,274677,75.00094103813171,2.269628074550235e-06
68769,137539,137538,275077,75.09928226470947,2.262027073533906e-06
68869,137739,137738,275477,75.2052092552185,2.2544769639386698e-06
68969,137939,137938,275877,75.31380105018616,2.246977468094862e-06
69069,138139,138138,276277,75.41963124275208,2.239528309248918e-06
69169,138339,138338,276677,75.51684021949768,2.232129211675099e-06
69269,138539,138538,277077,75.61428713798523,2.224779901255263e-06
69369,138739,138738,277477,75.71352410316467,2.217480104439679e-06
69469,138939,138938,277877,75.81177926063538,2.210229549177222e-06
69570,139141,139140,278281,75.91126132011414,2.2029561950037375e-06
69670,139341,139340,278681,76.02415418624878,2.195803796210658e-06
69770,139541,139540,279081,76.136057138443,2.188699826214872e-06
69870,139741,139740,279481,76.23487734794617,2.1816440171058295e-06
69970,139941,139940,279881,76.33326816558838,2.1746361021918227e-06
70070,140141,140140,280281,76.43243217468262,2.1676758158810486e-06
70170,140341,140340,280681,76.5362823009491,2.160762893294456e-06
70270,140541,140540,281081,76.63513922691345,2.153897071094307e-06
70370,140741,140740,281481,76.7354941368103,2.1470780865682e-06
70470,140941,140940,281881,76.83453917503357,2.1403056783586055e-06
70571,141143,141142,282285,76.93393421173096,2.1335125582210985e-06
70671,141343,141342,282685,77.0343542098999,2.126832981776931e-06
70771,141543,141542,283085,77.13158822059631,2.1201992007846804e-06
70871,141743,141742,283485,77.23248624801636,2.1136109580559547e-06
70971,141943,141942,283885,77.33168816566467,2.1070679973443883e-06
71071,142143,142142,284285,77.43060302734375,2.100570063260819e-06
71171,142343,142342,284685,77.52851915359497,2.094116901446059e-06
71271,142543,142542,285085,77.62760019302368,2.087708259066037e-06
71371,142743,142742,285485,77.72929000854492,2.0813438834648194e-06
71471,142943,142942,285885,77.82766222953796,2.0750235232705427e-06
71572,143145,143144,286289,77.9301540851593,2.0686843828919825e-06
71672,143345,143344,286689,78.02818727493286,2.0624517383600515e-06
71772,143545,143544,287089,78.14102911949158,2.056262359115471e-06
71872,143745,143744,287489,78.25385928153992,2.050115997800982e-06
71972,143945,143944,287889,78.3537962436676,2.0440124083681556e-06
72072,144145,144144,288289,78.4560010433197,2.0379513453490074e-06
72172,144345,144344,288689,78.55420231819153,2.0319325641643383e-06
72272,144545,144544,289089,78.66750812530518,2.0259558216145032e-06
72372,144745,144744,289489,78.88346028327942,2.0200208753586987e-06
72472,144945,144944,289889,79.01966214179993,2.0141274837413022e-06
72573,145147,145146,290293,79.14887714385986,2.008217093332123e-06
72673,145347,145346,290693,79.30927801132202,2.002406499793463e-06
72773,145547,145546,291093,79.42158794403076,1.996636739963973e-06
72873,145747,145746,291493,79.55884003639221,1.9909075760700736e-06
72973,145947,145946,291893,79.71916913986206,1.985218771099692e-06
73073,146147,146146,292293,79.86513113975525,1.979570089524111e-06
73173,146347,146346,292693,79.9888813495636,1.9739612963998257e-06
73273,146547,146546,293093,80.1880111694336,1.9683921578082133e-06
73373,146747,146746,293493,80.33305597305298,1.9628624408575366e-06
73473,146947,146946,293893,80.45786499977112,1.9573719130255463e-06
73574,147149,147148,294297,80.58053922653198,1.951866023886824e-06
73674,147349,147348,294697,80.71064019203186,1.946453568571144e-06
73774,147549,147548,295097,80.85702419281006,1.9410796095815656e-06
73874,147749,147748,295497,80.98993015289307,1.9357439186554453e-06
73974,147949,147948,295897,81.133798122406,1.930446268220333e-06
74074,148149,148148,296297,81.2742862701416,1.9251864315266883e-06
74174,148349,148348,296697,81.39790916442871,1.919964183130938e-06
74274,148549,148548,297097,81.51293802261353,1.9147792981028865e-06
74374,148749,148748,297497,81.6778461933136,1.9096315527452103e-06
74474,148949,148948,297897,81.82833409309387,1.904520723824285e-06
74575,149151,149150,298301,81.96236538887024,1.8993960326464324e-06
74675,149351,149350,298701,82.07087731361389,1.8943587350300446e-06
74775,149551,149550,299101,82.18559908866882,1.8893576883488883e-06
74875,149751,149750,299501,82.29206013679504,1.884392672963078e-06
74975,149951,149950,299901,82.41211700439453,1.879463470399839e-06
75075,150151,150150,300301,82.5331220626831,1.8745698629375028e-06
75175,150351,150350,300701,82.64353895187378,1.8697116340249785e-06
75275,150551,150550,301101,82.79541301727295,1.8648885677041297e-06
75375,150751,150750,301501,82.9594361782074,1.860100448892799e-06
75475,150951,150950,301901,83.09409427642822,1.8553470635185739e-06
75576,151153,151152,302305,83.23633933067322,1.850581183229221e-06
75676,151353,151352,302705,83.44004416465759,1.8458969680701343e-06
75776,151553,151552,303105,83.59899497032166,1.841246847050018e-06
75876,151753,151752,303505,83.74046897888184,1.836630609614162e-06
75976,151953,151952,303905,83.87303519248962,1.832048046098284e-06
76076,152153,152152,304305,84.02393126487732,1.8274989473565958e-06
76176,152353,152352,304705,84.22670221328735,1.8229831058025645e-06
76276,152553,152552,305105,84.40283608436584,1.818500313879528e-06
76376,152753,152752,305505,84.54468512535095,1.8140503654104226e-06
76476,152953,152952,305905,84.73232007026672,1.8096330548917877e-06
76577,153155,153154,306309,84.87966799736023,1.8052044924095253e-06
76677,153355,153354,306709,85.05643320083618,1.8008521664431159e-06
76777,153555,153554,307109,85.27463126182556,1.7965318653049106e-06
76877,153755,153754,307509,85.39880013465881,1.7922433870349087e-06
76977,153955,153954,307909,85.51560616493225,1.7879865303773963e-06
77077,154155,154154,308309,85.62580418586731,1.7837610951737734e-06
77177,154355,154354,308709,85.75929403305054,1.7795668817952114e-06
77277,154555,154554,309109,85.87474822998047,1.775403691839618e-06
77377,154755,154754,309509,85.98389029502869,1.7712713274828856e-06
77477,154955,154954,309909,86.08848309516907,1.7671695917911344e-06
77578,155157,155156,310313,86.20611214637756,1.763057728629924e-06
77678,155357,155356,310713,86.35916423797607,1.759016964202382e-06
77778,155557,155556,311113,86.51732611656189,1.755006240998e-06
77878,155757,155756,311513,86.73001909255981,1.7510253653561124e-06
77978,155957,155956,311913,86.87972521781921,1.7470741444808845e-06
78078,156157,156156,312313,87.0017831325531,1.7431523867505794e-06
78178,156357,156356,312713,87.17805218696594,1.739259901037415e-06
78278,156557,156556,313113,87.32341194152832,1.7353964971853342e-06
78378,156757,156756,313513,87.43999528884888,1.7315619860625706e-06
78478,156957,156956,313913,87.5625159740448,1.7277561789569766e-06
78579,157159,157158,314317,87.68316221237183,1.7239412587906194e-06
78679,157359,157358,314717,87.80998826026917,1.7201925799825884e-06
78779,157559,157558,315117,87.92280602455139,1.7164720431074261e-06
78879,157759,157758,315517,88.03131127357483,1.7127794629624441e-06
78979,157959,157958,315917,88.13860416412354,1.7091146549861194e-06
79079,158159,158158,316317,88.26107335090637,1.7054774360387703e-06
79179,158359,158358,316717,88.4091432094574,1.7018676233897183e-06
79279,158559,158558,317117,88.51409316062927,1.698285035077022e-06
79379,158759,158758,317517,88.61962914466858,1.6947294902313227e-06
79479,158959,158958,317917,88.72694420814514,1.6912008087318635e-06
79580,159161,159160,318321,88.85969734191895,1.6876639254544311e-06
79680,159361,159360,318721,88.97842311859131,1.684188697519512e-06
79780,159561,159560,319121,89.07598423957825,1.6807397956576483e-06
79880,159761,159760,319521,89.18444609642029,1.6773170429601805e-06
79980,159961,159960,319921,89.30364608764648,1.6739202634554277e-06
80080,160161,160160,320321,89.40490818023682,1.6705492819888668e-06
80180,160361,160360,320721,89.55618715286255,1.6672039242535504e-06
80280,160561,160560,321121,89.71426820755005,1.6638840163777806e-06
80380,160761,160760,321521,89.835764169693,1.660589385918047e-06
80480,160961,160960,321921,89.97450232505798,1.6573198610569068e-06
80581,161163,161162,322325,90.09926724433899,1.6540429497962114e-06
80681,161363,161362,322725,90.2290141582489,1.6508233700928283e-06
80781,161563,161562,323125,90.36642217636108,1.6476283833373464e-06
80881,161763,161762,323525,90.60947513580322,1.6444578209271493e-06
80981,161963,161962,323925,90.72151613235474,1.6413115151153036e-06
81081,162163,162162,324325,90.83162808418274,1.6381892988558482e-06
81181,162363,162362,324725,90.94294810295105,1.6350910059707293e-06
81281,162563,162562,325125,91.0874490737915,1.6320164711392937e-06
81381,162763,162762,325525,91.20136022567749,1.6289655296477216e-06
81481,162963,162962,325925,91.30678820610046,1.6259380180947523e-06
81582,163165,163164,326329,91.41367721557617,1.6229038476649173e-06
81682,163365,163364,326729,91.51982116699219,1.619922937826256e-06
81782,163565,163564,327129,91.62342619895935,1.6169649696847463e-06
81882,163765,163764,327529,91.73388123512268,1.614029782964095e-06
81982,163965,163964,327929,91.86147713661194,1.6111172178562461e-06
82082,164165,164164,328329,91.98789715766907,1.608227115614968e-06
82182,164365,164364,328729,92.09929704666138,1.6053593179189702e-06
82282,164565,164564,329129,92.20586705207825,1.6025136679114424e-06
82382,164765,164764,329529,92.30565214157104,1.599690008754685e-06
82482,164965,164964,329929,92.41766500473022,1.5968881850724742e-06
82583,165167,165166,330333,92.53006410598755,1.594080349363094e-06
82683,165367,165366,330733,92.9722511768341,1.5913219471252603e-06
82783,165567,165566,331133,93.081866979599,1.588584916599724e-06
82883,165767,165766,331533,93.19315934181213,1.5858691054244984e-06
82983,165967,165966,331933,93.29824829101562,1.5831743617700876e-06
83083,166167,166166,332333,93.41257500648499,1.5805005350361195e-06
83183,166367,166366,332733,93.52518200874329,1.5778474748757486e-06
83283,166567,166566,333133,93.64514517784119,1.5752150326098378e-06
83383,166767,166766,333533,93.75449514389038,1.572603059155467e-06
83483,166967,166966,333933,93.86165809631348,1.5700114072136505e-06
83584,167169,167168,334337,93.97964024543762,1.5674143163533773e-06
83684,167369,167368,334737,94.10658717155457,1.5648630669727027e-06
83784,167569,167568,335137,94.21281838417053,1.5623316993091795e-06
83884,167769,167768,335537,94.32114720344543,1.5598200690349098e-06
83984,167969,167968,335937,94.43762516975403,1.5573280321679621e-06
84084,168169,168168,336337,94.56369614601135,1.5548554459424362e-06
84184,168369,168368,336737,94.68600010871887,1.5524021681994328e-06
84284,168569,168568,337137,94.79502415657043,1.5499680578256143e-06
84384,168769,168768,337537,94.9050281047821,1.5475529739526512e-06
84484,168969,168968,337937,95.00996112823486,1.5451567769376212e-06
84585,169171,169170,338341,95.11934113502502,1.5427556474698198e-06
84685,169371,169370,338741,95.2494101524353,1.5403969933505532e-06
84785,169571,169570,339141,95.35683917999268,1.5380568098468841e-06
84885,169771,169770,339541,95.45274424552917,1.535734960562266e-06
84985,169971,169970,339941,95.55066227912903,1.5334313094921342e-06
85085,170171,170170,340341,95.64839720726013,1.5311457214689604e-06
85185,170371,170370,340741,95.74668216705322,1.5288780623743324e-06
85285,170571,170570,341141,95.86059904098511,1.526628198387049e-06
85385,170771,170770,341541,95.98376607894897,1.5243959968526471e-06
85485,170971,170970,341941,96.11770820617676,1.5221813256097273e-06
85586,171173,171172,342345,96.23578596115112,1.5199621680827842e-06
85686,171373,171372,342745,96.33239030838013,1.5177823365159705e-06
85786,171573,171572,343145,96.43331933021545,1.5156196423009276e-06
85886,171773,171772,343545,96.5825469493866,1.5134739568266023e-06
85986,171973,171972,343945,96.75318717956543,1.5113451514983241e-06
86086,172173,172172,344345,96.85284924507141,1.5092330991083433e-06
86186,172373,172372,344745,96.9531421661377,1.5071376727685602e-06
86286,172573,172572,345145,97.05555629730225,1.5050587465666602e-06
86386,172773,172772,345545,97.15552735328674,1.502996195389828e-06
86486,172973,172972,345945,97.27389025688171,1.5009498945678348e-06
86587,173175,173174,346349,97.48162627220154,1.4988994999018596e-06
86687,173375,173374,346749,97.59139513969421,1.4968854890651688e-06
86787,173575,173574,347149,97.72366714477539,1.494887358749664e-06
86887,173775,173774,347549,97.83290123939514,1.4929049870984796e-06
86987,173975,173974,347949,97.93794107437134,1.4909382537904246e-06
87087,174175,174174,348349,98.0398530960083,1.4889870386305271e-06
87187,174375,174374,348749,98.14783310890198,1.4870512223823873e-06
87287,174575,174574,349149,98.24815917015076,1.4851306864376108e-06
87387,174775,174774,349549,98.35274600982666,1.4832253130428921e-06
87487,174975,174974,349949,98.45888113975525,1.4813349852828165e-06
87588,175177,175176,350353,98.5620322227478,1.479440907684181e-06
87688,175377,175376,350753,98.66804313659668,1.4775804702262628e-06
87788,175577,175576,351153,98.78160119056702,1.4757347303277195e-06
87888,175777,175776,351553,98.97549104690552,1.4739035738584341e-06
87988,175977,175976,351953,99.13419532775879,1.472086887270369e-06
88088,176177,176176,352353,99.27405118942261,1.4702845579719397e-06
88188,176377,176376,352753,99.43142294883728,1.4684964739474555e-06
88288,176577,176576,353153,99.57987403869629,1.4667225239311733e-06
88388,176777,176776,353553,99.78443312644958,1.4649625973142203e-06
88488,176977,176976,353953,99.91965126991272,1.4632165841767938e-06
88589,177179,177178,354357,100.0458812713623,1.4614671226851623e-06
88689,177379,177378,354757,100.19044423103333,1.4597487462110185e-06
88789,177579,177578,355157,100.35189199447632,1.4580439569882368e-06
88889,177779,177778,355557,100.48634505271912,1.4563526476187764e-06
88989,177979,177978,355957,100.61389803886414,1.4546747120474548e-06
89089,178179,178178,356357,100.73774313926697,1.4530100443197464e-06
89189,178379,178378,356757,100.85363411903381,1.4513585399173698e-06
89289,178579,178578,357157,100.96205425262451,1.449720094158862e-06
89389,178779,178778,357557,101.06928014755249,1.4480946036842707e-06
89489,178979,178978,357957,101.17774105072021,1.4464819654288502e-06
89590,179181,179180,358361,101.30249333381653,1.4448661425046581e-06
89690,179381,179380,358761,101.42164301872253,1.443279028929558e-06
89790,179581,179580,359161,101.53781723976135,1.4417044619077524e-06
89890,179781,179780,359561,101.65390801429749,1.4401423414844319e-06
89990,179981,179980,359961,101.77976608276367,1.4385925681442626e-06
90090,180181,180180,360361,101.8983039855957,1.437055042820718e-06
90190,180381,180380,360761,102.01084613800049,1.4355296675786023e-06
90290,180581,180580,361161,102.12431526184082,1.4340163447196163e-06
90390,180781,180780,361561,102.23787522315979,1.432514977630394e-06
90490,180981,180980,361961,102.34231519699097,1.4310254699660522e-06
90591,181183,181182,362365,102.46240615844727,1.4295330079215403e-06
90691,181383,181382,362765,102.57666826248169,1.4280670495519363e-06
90791,181583,181582,363165,102.69147515296936,1.4266126651034025e-06
90891,181783,181782,363565,102.79964113235474,1.4251697609257057e-06
90991,181983,181982,363965,102.90350413322449,1.4237382443122814e-06
91091,182183,182182,364365,103.03303408622742,1.4223180227652558e-06
91191,182383,182382,364765,103.20101809501648,1.4209090048431104e-06
91291,182583,182582,365165,103.31295204162598,1.4195110994672459e-06
91391,182783,182782,365565,103.42662715911865,1.4181242161469805e-06
91491,182983,182982,365965,103.5311541557312,1.4167482654553145e-06
91592,183185,183184,366369,103.64447736740112,1.4153695613472516e-06
91692,183385,183384,366769,103.80086016654968,1.4140153160225222e-06
91792,183585,183584,367169,103.94320893287659,1.4126717368033945e-06
91892,183785,183784,367569,104.08269119262695,1.4113387365096943e-06
91992,183985,183984,367969,104.25820112228394,1.4100162286344663e-06
92092,184185,184184,368369,104.42326617240906,1.4087041271765727e-06
92192,184385,184384,368769,104.56827807426453,1.4074023466679913e-06
92292,184585,184584,369169,104.82582521438599,1.4061108024713637e-06
92392,184785,184784,369569,105.03728222846985,1.4048294103705945e-06
92492,184985,184984,369969,105.26979303359985,1.4035580868439076e-06
92593,185187,185186,370373,105.52982926368713,1.402284185577777e-06
92693,185387,185386,370773,105.74928307533264,1.4010328495400257e-06
92793,185587,185586,371173,105.93291902542114,1.3997913341642846e-06
92893,185787,185786,371573,106.14074420928955,1.3985595584414396e-06
92993,185987,185986,371973,106.31491422653198,1.3973374416603614e-06
93093,186187,186186,372373,106.42064619064331,1.3961249039379972e-06
93193,186387,186386,372773,106.55228114128113,1.3949218657123098e-06
93293,186587,186586,373173,106.73558306694031,1.3937282484210587e-06
93393,186787,186786,373573,106.87419509887695,1.3925439736077279e-06
93493,186987,186986,373973,106.98887228965759,1.3913689637980936e-06
93594,187189,187188,374377,107.1040723323822,1.3901915296867567e-06
93694,187389,187388,374777,107.26602506637573,1.3890349098432154e-06
93794,187589,187588,375177,107.45153522491455,1.3878873246357019e-06
93894,187789,187788,375577,107.5809690952301,1.3867486985945261e-06
93994,187989,187988,375977,107.6941351890564,1.3856189570908606e-06
94094,188189,188188,376377,107.84236311912537,1.38449802570958e-06
94194,188389,188388,376777,108.03728818893433,1.3833858307656064e-06
94294,188589,188588,377177,108.15611219406128,1.3822822991316638e-06
94394,188789,188788,377577,108.28355002403259,1.3811873582845045e-06
94494,188989,188988,377977,108.39712715148926,1.380100935891496e-06
94595,189191,189190,378381,108.50991415977478,1.3790122236024353e-06
94695,189391,189390,378781,108.650071144104,1.3779427080479144e-06
94795,189591,189590,379181,108.81130337715149,1.376881497565118e-06
94895,189791,189790,379581,109.03955721855164,1.3758285222432733e-06
94995,189991,189990,379981,109.2151780128479,1.374783712646331e-06
95095,190191,190190,380381,109.3678891658783,1.3737469999185782e-06
95195,190391,190390,380781,109.56848621368408,1.3727183158601186e-06
95295,190591,190590,381181,109.86159110069275,1.3716975926498783e-06
95395,190791,190790,381581,110.04809403419495,1.3706847629116834e-06
95495,190991,190990,381981,110.25134801864624,1.3696797599346017e-06
95596,191193,191192,382385,110.38564419746399,1.368672584022339e-06
95696,191393,191392,382785,110.58093118667603,1.367683112962588e-06
95796,191593,191592,383185,110.73061513900757,1.3667012708478613e-06
95896,191793,191792,383585,110.82876229286194,1.3657269930463281e-06
95996,191993,191992,383985,110.9324791431427,1.3647602150997397e-06
96096,192193,192192,384385,111.0347592830658,1.3638008733392518e-06
96196,192393,192392,384785,111.13786911964417,1.3628489047718675e-06
96296,192593,192592,385185,111.23613429069519,1.3619042464747929e-06
96396,192793,192792,385585,111.3360960483551,1.3609668361281709e-06
96496,192993,192992,385985,111.44344401359558,1.360036612080165e-06
96597,193195,193194,386389,111.54480528831482,1.3591043179385103e-06
96697,193395,193394,386789,111.66218709945679,1.358188353514031e-06
96797,193595,193594,387189,111.78188800811768,1.3572793923773275e-06
96897,193795,193794,387589,111.89626812934875,1.3563773748001648e-06
96997,193995,193994,387989,112.03595519065857,1.3554822410965038e-06
97097,194195,194194,388389,112.14686799049377,1.35459393284761e-06
97197,194395,194394,388789,112.29300832748413,1.3537123913264018e-06
97297,194595,194594,389189,112.4224591255188,1.3528375585785545e-06
97397,194795,194794,389589,112.55034232139587,1.3519693771399977e-06
97497,194995,194994,389989,112.65154314041138,1.351107789933584e-06
97598,195197,195196,390393,112.86236333847046,1.3502442227272008e-06
97698,195397,195396,390793,113.00616216659546,1.349395719271456e-06
97798,195597,195596,391193,113.11509108543396,1.348553640899381e-06
97898,195797,195796,391593,113.2205183506012,1.3477179327329728e-06
97998,195997,195996,391993,113.3239471912384,1.3468885396055964e-06
98098,196197,196196,392393,113.46361708641052,1.3460654073491742e-06
98198,196397,196396,392793,113.58850312232971,1.3452484819625905e-06
98298,196597,196596,393193,113.73002600669861,1.3444377100831858e-06
98398,196797,196796,393593,113.86904120445251,1.3436330384876309e-06
98498,196997,196996,393993,114.04113006591797,1.3428344145000124e-06
98599,197199,197198,394397,114.27629709243774,1.3420338897748264e-06
98699,197399,197398,394797,114.46716022491455,1.3412472640671224e-06
98799,197599,197598,395197,114.59969997406006,1.3404665303278835e-06
98899,197799,197798,395597,114.73124814033508,1.3396916374270527e-06
98999,197999,197998,395997,114.84335613250732,1.338922534672346e-06
99099,198199,198198,396397,114.95711421966553,1.3381591725322445e-06
99199,198399,198398,396797,115.08629727363586,1.3374015005807464e-06
99299,198599,198598,397197,115.19669818878174,1.3366494697956206e-06
99399,198799,198798,397597,115.30324411392212,1.335903031252909e-06
99499,198999,198998,397997,115.41541409492493,1.3351621364456628e-06
99600,199201,199200,398401,115.55123710632324,1.3344194110065009e-06
99700,199401,199400,398801,115.67147922515869,1.3336895139686216e-06
99800,199601,199600,399201,115.78401732444763,1.3329650172670143e-06
99900,199801,199800,399601,115.89904737472534,1.332245873735849e-06
100000,200001,200000,400001,116.01496505737305,1.3315320367501845e-06


==> extragradient/plot_data/bilinear_matrix_game_n500/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012600421905517578,2.018959020339561
200,201,200,401,0.14514613151550293,0.046482251948234084
400,401,400,801,0.2978670597076416,0.01712120879549692
601,602,601,1203,0.43784022331237793,0.010238352144301867
801,802,801,1603,0.5829730033874512,0.006553442772398745
1001,1002,1001,2003,0.7231240272521973,0.004385682950619011
1201,1202,1201,2403,0.8626072406768799,0.003197778950946866
1401,1402,1401,2803,1.0024261474609375,0.002496321008503863
1602,1603,1602,3205,1.163182258605957,0.002144660757615812
1802,1803,1802,3605,1.29364013671875,0.001762637810262336
2002,2003,2002,4005,1.4332520961761475,0.0015091980552559801
2202,2203,2202,4405,1.6063041687011719,0.0012087647514370439
2402,2403,2402,4805,1.7513999938964844,0.0010289858283729944
2603,2604,2603,5207,1.8973362445831299,0.0008925435566486958
2803,2804,2803,5607,2.0444180965423584,0.0008015520107389197
3003,3004,3003,6007,2.1909031867980957,0.0007289576997704426
3203,3204,3203,6407,2.3724770545959473,0.0006617447243810016
3403,3404,3403,6807,2.5353879928588867,0.0006131100527668779
3604,3605,3604,7209,2.6904311180114746,0.0005680655402142006
3804,3805,3804,7609,2.863551139831543,0.00048022264511595044
4004,4005,4004,8009,3.0355851650238037,0.00043212050886599706
4204,4205,4204,8409,3.1889290809631348,0.000393116042656765
4404,4405,4404,8809,3.331102132797241,0.0003666199428392579
4605,4606,4605,9211,3.4773762226104736,0.0003451532971075256
4805,4806,4805,9611,3.6228091716766357,0.00032846386195348946
5005,5006,5005,10011,3.7640531063079834,0.0003145392112841674
5205,5206,5205,10411,3.9029722213745117,0.00030251142235609215
5405,5406,5405,10811,4.054957151412964,0.00028821983850401523
5606,5607,5606,11213,4.198130130767822,0.0002738558083393277
5806,5807,5806,11613,4.33680534362793,0.0002636576222328156
6006,6007,6006,12013,4.494132995605469,0.0002550453263141989
6206,6207,6206,12413,4.657612085342407,0.0002475459908481011
6406,6407,6406,12813,4.796328067779541,0.0002409047627142882
6607,6608,6607,13215,4.9418933391571045,0.0002346104783932992
6807,6808,6807,13615,5.152656316757202,0.00022923018703085668
7007,7008,7007,14015,5.427306175231934,0.0002243568267627466
7207,7208,7207,14415,5.687941312789917,0.00021990372138149208
7407,7408,7407,14815,5.9810802936553955,0.0002158119315476405
7608,7609,7608,15217,6.259033203125,0.00021201712334363766
7808,7809,7808,15617,6.506990194320679,0.00020810533579128433
8008,8009,8008,16017,6.742325067520142,0.00020462043559535262
8208,8209,8208,16417,6.897526025772095,0.00019918143092702428
8408,8409,8408,16817,7.043233156204224,0.0001953078143870299
8609,8610,8609,17219,7.217888116836548,0.00019186561505209513
8809,8810,8809,17619,7.3665242195129395,0.00018874806386831746
9009,9010,9009,18019,7.521957159042358,0.0001858670233743703
9209,9210,9209,18419,7.663906097412109,0.000183179331511306
9409,9410,9409,18819,7.807445049285889,0.00018065534051514326
9610,9611,9610,19221,7.941411256790161,0.00017826164346721222
9810,9811,9810,19621,8.074471950531006,0.000176005145036593
10010,10011,10010,20021,8.223432064056396,0.00017194113344987783
10210,10211,10210,20421,8.354803085327148,0.00016743146783829504
10410,10411,10410,20821,8.486855030059814,0.00016424816011725076
10611,10612,10611,21223,8.630044937133789,0.0001615453071910808
10811,10812,10811,21623,8.790509223937988,0.00015915931460213953
11011,11012,11011,22023,8.933178186416626,0.000156494203539692
11211,11212,11211,22423,9.059962272644043,0.00015407193762690633
11411,11412,11411,22823,9.192383050918579,0.00015197881750619153
11612,11613,11612,23225,9.324392080307007,0.00014998039132118108
11812,11813,11812,23625,9.46609902381897,0.0001482286014210995
12012,12013,12012,24025,9.60834002494812,0.00014662753605077162
12212,12213,12212,24425,9.78330397605896,0.00014349315766923722
12412,12413,12412,24825,10.010026216506958,0.00014067479182094144
12613,12614,12613,25227,10.209289073944092,0.0001383935801344753
12813,12814,12813,25627,10.541073322296143,0.00013641820828361962
13013,13014,13013,26027,10.813481092453003,0.00013463503462371373
13213,13214,13213,26427,11.136569261550903,0.00013267099402021105
13413,13414,13413,26827,11.356925010681152,0.00013066436936772606
13614,13615,13614,27229,11.572815179824829,0.0001289509776855378
13814,13815,13814,27629,11.770438194274902,0.00012695764619518967
14014,14015,14014,28029,11.959854125976562,0.00012553852777686178
14214,14215,14214,28429,12.176806926727295,0.0001242966564725052
14414,14415,14414,28829,12.374903202056885,0.0001226691610167531
14615,14616,14615,29231,12.560961246490479,0.00012114326492845113
14815,14816,14815,29631,12.694914102554321,0.00011992373667054951
15015,15016,15015,30031,12.829683065414429,0.00011883437251330645
15215,15216,15215,30431,12.961914300918579,0.00011746116004514385
15415,15416,15415,30831,13.122225999832153,0.00011627365810361616
15616,15617,15616,31233,13.292293310165405,0.00011494202133355959
15816,15817,15816,31633,13.423165082931519,0.00011380136928453277
16016,16017,16016,32033,13.563583135604858,0.00011278886354251818
16216,16217,16216,32433,13.70481014251709,0.0001108625525811567
16416,16417,16416,32833,13.840825319290161,0.00010936533325807899
16617,16618,16617,33235,13.976957082748413,0.0001078360624225857
16817,16818,16817,33635,14.1309072971344,0.00010646863722811088
17017,17018,17017,34035,14.272335290908813,0.0001052815822331466
17217,17218,17217,34435,14.402703285217285,0.00010419081065635188
17417,17418,17417,34835,14.537955284118652,0.00010304917243215209
17618,17619,17618,35237,14.67287302017212,0.00010196966675974209
17818,17819,17818,35637,14.809681177139282,9.993263786335589e-05
18018,18019,18018,36037,14.946874141693115,9.778462010637506e-05
18218,18219,18218,36437,15.08458399772644,9.622565445469146e-05
18418,18419,18418,36837,15.223376274108887,9.48686193257932e-05
18619,18620,18619,37239,15.368772268295288,9.290515410830554e-05
18819,18820,18819,37639,15.516224145889282,9.132968286909853e-05
19019,19020,19019,38039,15.65610408782959,8.998369516507806e-05
19219,19220,19219,38439,15.795960187911987,8.879849428756358e-05
19419,19420,19419,38839,15.933882236480713,8.771036141256288e-05
19620,19621,19620,39241,16.092019081115723,8.668888609940676e-05
19820,19821,19820,39641,16.228254079818726,8.547475690231487e-05
20020,20021,20020,40041,16.363744020462036,8.443869200609595e-05
20220,20221,20220,40441,16.506999254226685,8.246313013584528e-05
20420,20421,20420,40841,16.655288219451904,8.11581658930375e-05
20621,20622,20621,41243,16.80072522163391,7.999595753313809e-05
20821,20822,20821,41643,16.938998222351074,7.892685657496265e-05
21021,21022,21021,42043,17.082861185073853,7.792137960650144e-05
21221,21222,21221,42443,17.223963260650635,7.696662023583319e-05
21421,21422,21421,42843,17.37539529800415,7.6054167456929e-05
21622,21623,21622,43245,17.538817167282104,7.517372130089341e-05
21822,21823,21822,43645,17.681883335113525,7.43294998575266e-05
22022,22023,22022,44045,17.825006246566772,7.351349938882748e-05
22222,22223,22222,44445,17.9719340801239,7.272287927894987e-05
22422,22423,22422,44845,18.120655298233032,7.195531307062059e-05
22623,22624,22623,45247,18.259881019592285,7.120518396725883e-05
22823,22824,22823,45647,18.400633096694946,7.04783205571956e-05
23023,23024,23023,46047,18.558226108551025,6.97695541350563e-05
23223,23224,23223,46447,18.69919228553772,6.907769470916285e-05
23423,23424,23423,46847,18.839216232299805,6.840171157892528e-05
23624,23625,23624,47249,18.989493131637573,6.77374363123991e-05
23824,23825,23824,47649,19.1439311504364,6.709068453065306e-05
24024,24025,24024,48049,19.28413414955139,6.645741470020184e-05
24224,24225,24224,48449,19.42569136619568,6.583700291778728e-05
24424,24425,24424,48849,19.593454122543335,6.522888947237478e-05
24625,24626,24625,49251,19.745521306991577,6.46296163617347e-05
24825,24826,24825,49651,19.88302230834961,6.404468590260554e-05
25025,25026,25025,50051,20.03135323524475,6.347066876523294e-05
25225,25226,25225,50451,20.177649974822998,6.290718042680914e-05
25425,25426,25425,50851,20.325681924819946,6.235386603456538e-05
25626,25627,25626,51253,20.46769618988037,6.180770341956507e-05
25826,25827,25826,51653,20.617171049118042,6.127381936011798e-05
26026,26027,26026,52053,20.756291151046753,6.074918578479355e-05
26226,26227,26226,52453,20.90580916404724,6.023353373562771e-05
26426,26427,26426,52853,21.05268931388855,5.972660983966785e-05
26627,26628,26627,53255,21.197460174560547,5.9225703408486985e-05
26827,26828,26827,53655,21.338621139526367,5.8735570708512064e-05
27027,27028,27027,54055,21.492202043533325,5.825348300766713e-05
27227,27228,27227,54455,21.64440131187439,5.7779234883752995e-05
27427,27428,27427,54855,21.804235219955444,5.731263021530778e-05
27628,27629,27628,55257,21.950355052947998,5.6851204073482e-05
27828,27829,27828,55657,22.103323221206665,5.6399367235227945e-05
28028,28029,28028,56057,22.234316110610962,5.595463301104026e-05
28228,28229,28228,56457,22.347458124160767,5.551683552126061e-05
28428,28429,28428,56857,22.469223022460938,5.508581508604093e-05
28629,28630,28629,57259,22.602074146270752,5.465931220875329e-05
28829,28830,28829,57659,22.71276617050171,5.424142159615184e-05
29029,29030,29029,58059,22.820433378219604,5.38298615098952e-05
29229,29230,29229,58459,22.934701204299927,5.342449331001834e-05
29429,29430,29429,58859,23.04284906387329,5.302518284603325e-05
29630,29631,29630,59261,23.206806182861328,5.262984797572304e-05
29830,29831,29830,59661,23.372571229934692,5.2242295969390406e-05
30030,30031,30030,60061,23.492276191711426,5.186042320499224e-05
30230,30231,30230,60461,23.63127613067627,5.148411122937319e-05
30430,30431,30430,60861,23.90234112739563,5.111324503012289e-05
30631,30632,30631,61263,24.00805926322937,5.074589843226193e-05
30831,30832,30831,61663,24.123696327209473,5.038561757739843e-05
31031,31032,31031,62063,24.248091220855713,5.0030456031216506e-05
31231,31232,31231,62463,24.356842041015625,4.968031105798552e-05
31431,31432,31431,62863,24.454406261444092,4.9335082662645556e-05
31632,31633,31632,63265,24.554129362106323,4.899298337974067e-05
31832,31833,31832,63665,24.673924207687378,4.865732194860279e-05
32032,32033,32032,64065,24.783249378204346,4.832629200612741e-05
32232,32233,32232,64465,24.87970519065857,4.799980347295473e-05
32432,32433,32432,64865,24.974018096923828,4.767776851191872e-05
32633,32634,32633,65267,25.064289093017578,4.7358523943857555e-05
32833,32834,32833,65667,25.15842914581299,4.704516239229665e-05
33033,33034,33033,66067,25.248825311660767,4.673600315045491e-05
33233,33234,33233,66467,25.34378218650818,4.643096657848961e-05
33433,33434,33433,66867,25.44339418411255,4.612997490931848e-05
33634,33635,33634,67269,25.54515314102173,4.5831476917467705e-05
33834,33835,33834,67669,25.647933959960938,4.5538368218799185e-05
34034,34035,34034,68069,25.759108304977417,4.5249081382821374e-05
34234,34235,34234,68469,25.88338613510132,4.496354554183562e-05
34434,34435,34434,68869,25.992146015167236,4.468169141584407e-05
34635,34636,34635,69271,26.090628147125244,4.440206903210665e-05
34835,34836,34835,69671,26.18622326850891,4.412739418180952e-05
35035,35036,35035,70071,26.28350591659546,4.385620193721823e-05
35235,35236,35235,70471,26.38726305961609,4.3588428910829274e-05
35435,35436,35435,70871,26.50752329826355,4.33240130799537e-05
35636,35637,35636,71273,26.63034224510193,4.306159633349643e-05
35836,35837,35836,71673,26.740304231643677,4.280373013053059e-05
36036,36037,36036,72073,26.858155012130737,4.254904257590863e-05
36236,36237,36236,72473,26.99963116645813,4.2297476739904984e-05
36436,36437,36436,72873,27.164287090301514,4.204897687910038e-05
36637,36638,36637,73275,27.37017822265625,4.18022684376533e-05
36837,36838,36837,73675,27.54705309867859,4.155975254162307e-05
37037,37038,37037,74075,27.69939613342285,4.1320141939070216e-05
37237,37238,37237,74475,27.874901056289673,4.108338533348318e-05
37437,37438,37437,74875,28.05324125289917,4.084943246946974e-05
37638,37639,37638,75277,28.23068404197693,4.0617084952938246e-05
37838,37839,37838,75677,28.356577157974243,4.038860624924723e-05
38038,38039,38038,76077,28.490979194641113,4.0162786274017004e-05
38238,38239,38238,76477,28.60239315032959,3.9939578688379176e-05
38438,38439,38438,76877,28.707544088363647,3.971893807343628e-05
38639,38640,38639,77279,29.145904302597046,3.94997355814331e-05
38839,38840,38839,77679,29.340537309646606,3.928410850827424e-05
39039,39040,39039,78079,29.51750421524048,3.907091724329487e-05
39239,39240,39239,78479,29.645483016967773,3.886011984195347e-05
39439,39440,39439,78879,29.75278902053833,3.865167517799471e-05
39640,39641,39640,79281,29.842135190963745,3.844451800765205e-05
39840,39841,39840,79681,29.93302822113037,3.824066988993605e-05
40040,40041,40040,80081,30.01878809928894,3.8039055670061645e-05
40240,40241,40240,80481,30.120408296585083,3.783963732244478e-05
40440,40441,40440,80881,30.256263971328735,3.764237755311526e-05
40641,40642,40641,81283,30.374924182891846,3.744626936738244e-05
40841,40842,40841,81683,30.48551034927368,3.7253228066234705e-05
41041,41042,41041,82083,30.592182159423828,3.706223752687029e-05
41241,41242,41241,82483,30.696604013442993,3.687326323452506e-05
41441,41442,41441,82883,30.798938274383545,3.66862713328702e-05
41642,41643,41642,83285,30.902891159057617,3.650030823855181e-05
41842,41843,41842,83685,31.006432056427002,3.631719161467735e-05
42042,42043,42042,84085,31.119814157485962,3.613595946621684e-05
42242,42243,42242,84485,31.21942710876465,3.595658043798982e-05
42442,42443,42442,84885,31.324332237243652,3.57790237678335e-05
42643,42644,42643,85287,31.431270360946655,3.560238490501452e-05
42843,42844,42843,85687,31.52005624771118,3.542839171642989e-05
43043,43044,43043,86087,31.6076340675354,3.525613189535699e-05
43243,43244,43243,86487,31.69571304321289,3.508557693744426e-05
43443,43444,43443,86887,31.78084421157837,3.491669887425543e-05
43644,43645,43644,87289,31.869376182556152,3.474863821856932e-05
43844,43845,43844,87689,31.954997062683105,3.458304017664543e-05
44044,44045,44044,88089,32.042142152786255,3.441903810443876e-05
44244,44245,44244,88489,32.12962627410889,3.425660607625741e-05
44444,44445,44444,88889,32.215885162353516,3.409571865172703e-05
44645,44646,44645,89291,32.30864691734314,3.393555780413881e-05
44845,44846,44845,89691,32.399174213409424,3.377769257492962e-05
45045,45046,45045,90091,32.48354911804199,3.36212983279557e-05
45245,45246,45245,90491,32.57027220726013,3.346635147388814e-05
45445,45446,45445,90891,32.66498613357544,3.33128288637691e-05
45646,45647,45646,91293,32.75137114524841,3.315995065859952e-05
45846,45847,45846,91693,32.837600231170654,3.300921564869888e-05
46046,46047,46046,92093,32.92296314239502,3.285983788453062e-05
46246,46247,46246,92493,33.00935411453247,3.271179589688412e-05
46446,46447,46446,92893,33.09670829772949,3.25650686163105e-05
46647,46648,46647,93295,33.18457913398743,3.24189114156641e-05
46847,46848,46847,93695,33.27504205703735,3.2274758218588145e-05
47047,47048,47047,94095,33.37079930305481,3.213185874309639e-05
47247,47248,47247,94495,33.45638918876648,3.199019344500518e-05
47447,47448,47447,94895,33.53927707672119,3.184974314316998e-05
47648,47649,47648,95297,33.62557816505432,3.1709795716324703e-05
47848,47849,47848,95697,33.71322822570801,3.157172512443075e-05
48048,48049,48048,96097,33.79749321937561,3.1434814005624235e-05
48248,48249,48248,96497,33.8827862739563,3.129904456531931e-05
48448,48449,48448,96897,33.973188161849976,3.1164399338385454e-05
48649,48650,48649,97299,34.059046268463135,3.103019624625016e-05
48849,48850,48849,97699,34.14633131027222,3.089775374975954e-05
49049,49050,49049,98099,34.236040115356445,3.07663849082937e-05
49249,49250,49249,98499,34.32284331321716,3.063607351682905e-05
49449,49450,49449,98899,34.44578719139099,3.0506803670608126e-05
49650,49651,49650,99301,34.55240201950073,3.0377921091134972e-05
49850,49851,49850,99701,34.648935079574585,3.0250692807107405e-05
50050,50051,50050,100101,34.75107407569885,3.012446002254187e-05
50250,50251,50250,100501,34.84409499168396,2.9999207978304106e-05
50450,50451,50450,100901,34.935460329055786,2.9874922187545127e-05
50651,50652,50651,101303,35.02441716194153,2.9750974131023067e-05
50851,50852,50851,101703,35.11425423622131,2.96285831081996e-05
51051,51052,51051,102103,35.20168399810791,2.9507116396292626e-05
51251,51252,51251,102503,35.28807616233826,2.938656055009835e-05
51451,51452,51451,102903,35.367393255233765,2.926690237216241e-05
51652,51653,51652,103305,35.44815015792847,2.914753724253906e-05
51852,51853,51852,103705,35.53099012374878,2.902964010587454e-05
52052,52053,52052,104105,35.625288009643555,2.8912602424620825e-05
52252,52253,52252,104505,35.72148013114929,2.8796411948261192e-05
52452,52453,52452,104905,35.81532025337219,2.86810566513841e-05
52653,52654,52653,105307,35.90273904800415,2.8565954119412308e-05
52853,52854,52853,105707,35.9942672252655,2.845223801586405e-05
53053,53054,53053,106107,36.086045026779175,2.833932226940535e-05
53253,53254,53253,106507,36.194252252578735,2.8227195714919036e-05
53453,53454,53453,106907,36.30929112434387,2.811584739238264e-05
53654,53655,53654,107309,36.44191002845764,2.800471554887439e-05
53854,53855,53854,107709,36.55337309837341,2.7894895368070214e-05
54054,54055,54054,108109,36.65229320526123,2.7785821677693187e-05
54254,54255,54254,108509,36.74607229232788,2.7677484299499778e-05
54454,54455,54454,108909,36.831539154052734,2.7569873241230218e-05
54655,54656,54655,109311,36.91353917121887,2.7462446004623772e-05
54855,54856,54855,109711,36.99459910392761,2.7356261846727034e-05
55055,55056,55055,110111,37.07502818107605,2.725077506653154e-05
55255,55256,55255,110511,37.15795111656189,2.714597638234907e-05
55455,55456,55455,110911,37.23895215988159,2.704185668086908e-05
55656,55657,55656,111313,37.32210731506348,2.6937891435424704e-05
55856,55857,55856,111713,37.40258717536926,2.6835106305327283e-05
56056,56057,56056,112113,37.482553243637085,2.6732973758590242e-05
56256,56257,56256,112513,37.563844203948975,2.663148532741533e-05
56456,56457,56456,112913,37.646361112594604,2.6530632697336934e-05
56657,56658,56657,113315,37.726529121398926,2.6429908142948734e-05
56857,56858,56857,113715,37.80669903755188,2.633030584940144e-05
57057,57058,57057,114115,37.887105226516724,2.623131526670404e-05
57257,57258,57257,114515,37.967199087142944,2.613292866583915e-05
57457,57458,57457,114915,38.048078298568726,2.6035138457738e-05
57658,57659,57658,115317,38.13300323486328,2.593745265072798e-05
57858,57859,57858,115717,38.2145631313324,2.584083589395524e-05
58058,58059,58058,116117,38.295165061950684,2.5744793535738902e-05
58258,58259,58258,116517,38.37734627723694,2.5649318518629235e-05
58458,58459,58458,116917,38.45971202850342,2.5554403911189596e-05
58659,58660,58659,117319,38.54290318489075,2.5459572481065633e-05
58859,58860,58859,117719,38.63540005683899,2.5365761111430925e-05
59059,59060,59059,118119,38.71957302093506,2.5272490060190403e-05
59259,59260,59259,118519,38.801727056503296,2.517975287871068e-05
59459,59460,59459,118919,38.884151220321655,2.5087543233125403e-05
59660,59661,59660,119321,38.97304606437683,2.4995397759972512e-05
59860,59861,59860,119721,39.055641174316406,2.490422719334325e-05
60060,60061,60060,120121,39.1409752368927,2.4813565798024234e-05
60260,60261,60260,120521,39.22315716743469,2.4723407677749496e-05
60460,60461,60460,120921,39.309699296951294,2.4633747040773896e-05
60661,60662,60661,121323,39.392553091049194,2.4544133578804296e-05
60861,60862,60861,121723,39.475656032562256,2.445545335596371e-05
61061,61062,61061,122123,39.56047606468201,2.4367253818083246e-05
61261,61262,61261,122523,39.64517617225647,2.4279529570473223e-05
61461,61462,61461,122923,39.72691893577576,2.419227531280689e-05
61662,61663,61662,123325,39.80868220329285,2.4105053049282856e-05
61862,61863,61862,123725,39.89128136634827,2.4018725524974882e-05
62062,62063,62062,124125,39.97302317619324,2.393285261366525e-05
62262,62263,62262,124525,40.05393314361572,2.3847429375221576e-05
62462,62463,62462,124925,40.13815212249756,2.3762450955219734e-05
62663,62664,62663,125327,40.22333908081055,2.367749098917859e-05
62863,62864,62863,125727,40.30549216270447,2.3593390142712952e-05
63063,63064,63063,126127,40.38931107521057,2.3509720026446284e-05
63263,63264,63263,126527,40.4712290763855,2.3426476112930486e-05
63463,63464,63463,126927,40.552550315856934,2.3343653952199534e-05
63664,63665,63664,127329,40.640188217163086,2.3260838188049547e-05
63864,63865,63864,127729,40.73017716407776,2.3178848541311665e-05
64064,64065,64064,128129,40.81672191619873,2.3097267727812514e-05
64264,64265,64264,128529,40.90213918685913,2.301609159425178e-05
64464,64465,64464,128929,40.98490905761719,2.2935316057600474e-05
64665,64666,64665,129331,41.0671010017395,2.285453619857201e-05
64865,64866,64865,129731,41.15092992782593,2.2774551834489358e-05
65065,65066,65065,130131,41.23350214958191,2.2694956207966895e-05
65265,65266,65265,130531,41.316845178604126,2.261574550445783e-05
65465,65466,65465,130931,41.39958715438843,2.2536915973737697e-05
65666,65667,65666,131333,41.48357915878296,2.2458072609819874e-05
65866,65867,65866,131733,41.56598615646362,2.2379996282607706e-05
66066,66067,66066,132133,41.64959001541138,2.2302290230041918e-05
66266,66267,66266,132533,41.732869148254395,2.2224950945359918e-05
66466,66467,66466,132933,41.81506896018982,2.214797497965102e-05
66667,66668,66667,133335,41.89903020858765,2.2070976759758464e-05
66867,66868,66867,133735,41.98053002357483,2.1994719086430073e-05
67067,67068,67067,134135,42.063552141189575,2.1918814706062988e-05
67267,67268,67267,134535,42.150269985198975,2.184326039062006e-05
67467,67468,67467,134935,42.23257613182068,2.176805296494671e-05
67668,67669,67668,135337,42.31943917274475,2.1692815845554933e-05
67868,67869,67868,135737,42.40129208564758,2.1618294574471988e-05
68068,68069,68068,136137,42.48292112350464,2.1544110957735844e-05
68268,68269,68268,136537,42.567588329315186,2.1470262020018156e-05
68468,68469,68468,136937,42.64931011199951,2.1396744834767492e-05
68669,68670,68669,137339,42.73258399963379,2.1323191401157828e-05
68869,68870,68869,137739,42.82264018058777,2.1250330747897147e-05
69069,69070,69069,138139,42.907435178756714,2.117779332844724e-05
69269,69270,69269,138539,42.99036502838135,2.1105576397422385e-05
69469,69470,69469,138939,43.07250213623047,2.103367725270873e-05
69670,69671,69670,139341,43.158547163009644,2.0961736101926563e-05
69870,69871,69870,139741,43.240233182907104,2.0890466148643186e-05
70070,70071,70070,140141,43.322426319122314,2.081950611376842e-05
70270,70271,70270,140541,43.405068159103394,2.0748853460282683e-05
70470,70471,70470,140941,43.48699927330017,2.067850569045603e-05
70671,70672,70671,141343,43.57007908821106,2.0608110873715858e-05
70871,70872,70871,141743,43.653810024261475,2.0538367024535718e-05
71071,71072,71071,142143,43.735849142074585,2.0468920781284533e-05
71271,71272,71271,142543,43.819966077804565,2.039976979595512e-05
71471,71472,71471,142943,43.903003215789795,2.0330911755908095e-05
71672,71673,71672,143345,43.98634219169617,2.0262002273157513e-05
71872,71873,71872,143745,44.06945514678955,2.019372476173676e-05
72072,72073,72072,144145,44.15385293960571,2.0125733453889435e-05
72272,72273,72272,144545,44.23960828781128,2.0058026172939623e-05
72472,72473,72472,144945,44.325000047683716,1.9990600774481392e-05
72673,72674,72673,145347,44.40813326835632,1.9923120117651816e-05
72873,72874,72873,145747,44.48855018615723,1.985625356098274e-05
73073,73074,73073,146147,44.570730209350586,1.9789662631901633e-05
73273,73274,73273,146547,44.65583515167236,1.972334530909264e-05
73473,73474,73473,146947,44.73605728149414,1.965729960122765e-05
73674,73675,73674,147349,44.815953969955444,1.9591195339295265e-05
73874,73875,73874,147749,44.90125107765198,1.9525688334960787e-05
74074,74075,74074,148149,44.98626732826233,1.9460447131892794e-05
74274,74275,74274,148549,45.06622815132141,1.9395469850748335e-05
74474,74475,74474,148949,45.14847421646118,1.9330754638791675e-05
74675,74676,74675,149351,45.22895908355713,1.9265978045387693e-05
74875,74876,74875,149751,45.307910203933716,1.9201782805228185e-05
75075,75076,75075,150151,45.38691735267639,1.913784422237462e-05
75275,75276,75275,150551,45.467788219451904,1.9074160545524843e-05
75475,75476,75475,150951,45.54771304130554,1.9010730048309565e-05
75676,75677,75676,151353,45.63355112075806,1.8947235761531615e-05
75876,75877,75876,151753,45.714914083480835,1.8884307782907123e-05
76076,76077,76076,152153,45.794103145599365,1.882162793661646e-05
76276,76277,76276,152553,45.873279094696045,1.8759194588663902e-05
76476,76477,76476,152953,45.95307397842407,1.869700612725142e-05
76677,76678,76677,153355,46.03263211250305,1.8634751844596676e-05
76877,76878,76877,153755,46.11339616775513,1.857304961089388e-05
77077,77078,77077,154155,46.19196128845215,1.851158754835832e-05
77277,77278,77277,154555,46.27171325683594,1.8450364129109865e-05
77477,77478,77477,154955,46.35158610343933,1.8389377845871568e-05
77678,77679,77678,155357,46.432382106781006,1.832832404689695e-05
77878,77879,77878,155757,46.511687994003296,1.826780875814684e-05
78078,78079,78078,156157,46.59302020072937,1.820752619194463e-05
78278,78279,78278,156557,46.675095081329346,1.814747491725869e-05
78478,78479,78478,156957,46.754526138305664,1.8087653521743525e-05
78679,78680,78679,157359,46.834689140319824,1.8027763217743672e-05
78879,78880,78879,157759,46.91481018066406,1.7968398546087996e-05
79079,79080,79079,158159,47.002111196517944,1.790925961531048e-05
79279,79280,79279,158559,47.086590051651,1.7850345082594146e-05
79479,79480,79479,158959,47.16901922225952,1.77916536220726e-05
79680,79681,79680,159361,47.24979901313782,1.7732892130257014e-05
79880,79881,79880,159761,47.33171200752258,1.767464399981772e-05
80080,80081,80080,160161,47.411569356918335,1.7616615053687694e-05
80280,80281,80280,160561,47.49116921424866,1.7558804029918216e-05
80480,80481,80480,160961,47.57131505012512,1.7501209680881247e-05
80681,80682,80681,161363,47.65248227119446,1.7443544419424363e-05
80881,80882,80881,161763,47.73202204704285,1.7386380806455728e-05
81081,81082,81081,162163,47.810752153396606,1.732943020950099e-05
81281,81282,81281,162563,47.891120195388794,1.727269143931636e-05
81481,81482,81481,162963,47.97016930580139,1.721616332099927e-05
81682,81683,81682,163365,48.04989314079285,1.7159563624247025e-05
81882,81883,81882,163765,48.130043268203735,1.7103454376987176e-05
82082,82083,82082,164165,48.20962309837341,1.704755233113992e-05
82282,82283,82282,164565,48.290152072906494,1.6991856364663583e-05
82482,82483,82482,164965,48.37482023239136,1.6936365368107678e-05
82683,82684,82683,165367,48.45788908004761,1.6880802319181295e-05
82883,82884,82883,165767,48.539708375930786,1.68257189948937e-05
83083,83084,83083,166167,48.625216007232666,1.6770837380892027e-05
83283,83284,83283,166567,48.707961320877075,1.671615641601582e-05
83483,83484,83483,166967,48.79037117958069,1.6661675051111054e-05
83684,83685,83684,167369,48.87225127220154,1.660712133124954e-05
83884,83885,83884,167769,48.95408320426941,1.6553037048599732e-05
84084,84085,84084,168169,49.03753709793091,1.6499149280554046e-05
84284,84285,84284,168569,49.12951421737671,1.6445457022070205e-05
84484,84485,84484,168969,49.21263313293457,1.639195927880118e-05
84685,84686,84685,169371,49.295525312423706,1.6338389030361827e-05
84885,84886,84885,169771,49.37850022315979,1.6285278336546473e-05
85085,85086,85085,170171,49.46029496192932,1.6232359232065325e-05
85285,85286,85285,170571,49.542994022369385,1.617963076332526e-05
85485,85486,85485,170971,49.62920022010803,1.6127091986225298e-05
85686,85687,85686,171373,49.712876081466675,1.607448068914669e-05
85886,85887,85886,171773,49.79535698890686,1.6022319438823913e-05
86086,86087,86086,172173,49.87778615951538,1.5970345100562545e-05
86286,86287,86286,172573,49.95950698852539,1.59185567678154e-05
86486,86487,86486,172973,50.03991198539734,1.5866953542714857e-05
86687,86688,86687,173375,50.12251925468445,1.5815277902837814e-05
86887,86888,86887,173775,50.20437526702881,1.5764043149488323e-05
87087,87088,87087,174175,50.28575801849365,1.5712990858523172e-05
87287,87288,87287,174575,50.36725211143494,1.5662120166279346e-05
87487,87488,87487,174975,50.448121309280396,1.561143021732443e-05
87688,87689,87688,175377,50.53107404708862,1.556066806512898e-05
87888,87889,87888,175777,50.617125272750854,1.551033796261631e-05
88088,88089,88088,176177,50.70149827003479,1.546018608140113e-05
88288,88289,88288,176577,50.783332109451294,1.541021159757741e-05
88488,88489,88488,176977,50.865468978881836,1.5360413694842413e-05
88689,88690,88689,177379,50.948644161224365,1.5310543893950142e-05
88889,88890,88889,177779,51.03002905845642,1.5261097607059525e-05
89089,89090,89089,178179,51.11573624610901,1.5211825492432295e-05
89289,89290,89289,178579,51.207757234573364,1.5162726762667496e-05
89489,89490,89489,178979,51.28935623168945,1.5113800637662409e-05
89690,89691,89690,179381,51.371663331985474,1.5064803002550323e-05
89890,89891,89890,179781,51.45304298400879,1.5016220626173443e-05
90090,90091,90090,180181,51.536499977111816,1.496780854995849e-05
90290,90291,90290,180581,51.622777223587036,1.4919566020356012e-05
90490,90491,90490,180981,51.70666027069092,1.4871492290022668e-05
90691,90692,90691,181383,51.7896683216095,1.482334751064452e-05
90891,90892,90891,181783,51.87171411514282,1.4775609996959472e-05
91091,91092,91091,182183,51.954761028289795,1.4728039074650312e-05
91291,91292,91291,182583,52.03614592552185,1.4680634020818699e-05
91491,91492,91491,182983,52.11994218826294,1.4633394119198879e-05
91692,91693,91692,183385,52.20252513885498,1.4586083693257845e-05
91892,91893,91892,183785,52.302470207214355,1.4539172785598242e-05
92092,92093,92092,184185,52.38480615615845,1.449242491083937e-05
92292,92293,92292,184585,52.46718430519104,1.4445839375256317e-05
92492,92493,92492,184985,52.549750089645386,1.4399415490292629e-05
92693,92694,92693,185387,52.63514018058777,1.4352921661750194e-05
92893,92894,92893,185787,52.718037128448486,1.4306819834244368e-05
93093,93094,93093,186187,52.80059504508972,1.4260877620885504e-05
93293,93294,93293,186587,52.88272523880005,1.421509435426674e-05
93493,93494,93493,186987,52.983479261398315,1.416946937231629e-05
93694,93695,93694,187389,53.065057039260864,1.4123775075896307e-05
93894,93895,93894,187789,53.14977431297302,1.407846547956422e-05
94094,94095,94094,188189,53.23535108566284,1.403331220762613e-05
94294,94295,94294,188589,53.32433223724365,1.3988314617509197e-05
94494,94495,94494,188989,53.406904220581055,1.3943472071226609e-05
94695,94696,94695,189391,53.490148305892944,1.3898560881576206e-05
94895,94896,94895,189791,53.57285928726196,1.3854027294927159e-05
95095,95096,95095,190191,53.65824913978577,1.3809646862917044e-05
95295,95296,95295,190591,53.739262104034424,1.37654189656538e-05
95495,95496,95495,190991,53.82012605667114,1.3721342987907271e-05
95696,95697,95696,191393,53.90365123748779,1.3677199074409121e-05
95896,95897,95896,191793,53.984935998916626,1.3633425858836057e-05
96096,96097,96096,192193,54.067047119140625,1.3589802739206199e-05
96296,96297,96296,192593,54.1490421295166,1.35463291176933e-05
96496,96497,96496,192993,54.23257303237915,1.3503004399434766e-05
96697,96698,96697,193395,54.3149311542511,1.3459612484043863e-05
96897,96898,96897,193795,54.39736604690552,1.3416584543123717e-05
97097,97098,97097,194195,54.479088306427,1.3373703743705375e-05
97297,97298,97297,194595,54.56222701072693,1.3330969507415631e-05
97497,97498,97497,194995,54.64604115486145,1.3288381259472336e-05
97698,97699,97698,195397,54.729719161987305,1.3245726579234039e-05
97898,97899,97898,195797,54.81182813644409,1.3203429321934942e-05
98098,98099,98098,196197,54.89386224746704,1.3161276348606287e-05
98298,98299,98298,196597,54.97547507286072,1.311926709916427e-05
98498,98499,98498,196997,55.05808901786804,1.3077401017313403e-05
98699,98700,98699,197399,55.14601135253906,1.3035469290422872e-05
98899,98900,98899,197799,55.23300099372864,1.2993888597849217e-05
99099,99100,99099,198199,55.319483280181885,1.295244942193559e-05
99299,99300,99299,198599,55.40947914123535,1.2911151220506686e-05
99499,99500,99499,198999,55.49622297286987,1.286999345406011e-05
99700,99701,99700,199401,55.58433532714844,1.2828770847985822e-05
99900,99901,99900,199801,55.671189069747925,1.2787893042801397e-05
100100,100101,100100,200201,55.759101152420044,1.2747154072082138e-05
100300,100301,100300,200601,55.847018003463745,1.2706553409680154e-05
100501,100502,100501,201003,55.93038320541382,1.2665888563453976e-05
100701,100702,100701,201403,56.01234722137451,1.2625563636433892e-05
100901,100902,100901,201803,56.09601902961731,1.2585375455221049e-05
101101,101102,101101,202203,56.17913818359375,1.2545323505865218e-05
101301,101302,101301,202603,56.261112213134766,1.2505407277379385e-05
101502,101503,101502,203005,56.34305214881897,1.246542769567226e-05
101702,101703,101702,203405,56.425682067871094,1.242578206043349e-05
101902,101903,101902,203805,56.50773620605469,1.2386270628372378e-05
102102,102103,102102,204205,56.592748165130615,1.2346892900642486e-05
102302,102303,102302,204605,56.677401304244995,1.2307648380173032e-05
102503,102504,102503,205007,56.760523080825806,1.226834134718589e-05
102703,102704,102703,205407,56.843353271484375,1.2229362423342488e-05
102903,102904,102903,205807,56.92632818222046,1.21905152316598e-05
103103,103104,103103,206207,57.00939130783081,1.2151799286759989e-05
103303,103304,103303,206607,57.090880155563354,1.211321410573703e-05
103504,103505,103504,207009,57.17375707626343,1.2074567260251462e-05
103704,103705,103704,207409,57.25677013397217,1.2036242816293373e-05
103904,103905,103904,207809,57.339313983917236,1.1998047700984065e-05
104104,104105,104104,208209,57.42503523826599,1.1959981441548137e-05
104304,104305,104304,208609,57.51032614707947,1.1922043567960165e-05
104505,104506,104505,209011,57.59447622299194,1.1884044883636587e-05
104705,104706,104705,209411,57.68574333190918,1.1846363017727352e-05
104905,104906,104905,209811,57.7726571559906,1.1808808140174205e-05
105105,105106,105105,210211,57.860472202301025,1.1771379790578626e-05
105305,105306,105305,210611,57.94793915748596,1.173407751130435e-05
105506,105507,105506,211013,58.034064292907715,1.1696715278194096e-05
105706,105707,105706,211413,58.12151503562927,1.1659664399754602e-05
105906,105907,105906,211813,58.20805311203003,1.1622738229691517e-05
106106,106107,106106,212213,58.295690059661865,1.1585936319549328e-05
106306,106307,106306,212613,58.37905216217041,1.1549258222760815e-05
106507,106508,106507,213015,58.46277832984924,1.1512521031012849e-05
106707,106708,106707,213415,58.545199155807495,1.1476089844787305e-05
106907,106908,106907,213815,58.629393339157104,1.1439781144320975e-05
107107,107108,107107,214215,58.71263527870178,1.1403594491893309e-05
107307,107308,107307,214615,58.795422077178955,1.1367529452242465e-05
107508,107509,107508,215017,58.88515520095825,1.1331406176650323e-05
107708,107709,107708,215417,58.9714560508728,1.129558366783659e-05
107908,107909,107908,215817,59.05280113220215,1.1259881476273338e-05
108108,108109,108108,216217,59.133827209472656,1.1224299174926978e-05
108308,108309,108308,216617,59.21881604194641,1.118883633898473e-05
108509,108510,108509,217019,59.30098819732666,1.115331612505416e-05
108709,108710,108709,217419,59.382495164871216,1.1118091545471364e-05
108909,108910,108909,217819,59.46509122848511,1.1082985166328097e-05
109109,109110,109109,218219,59.55757212638855,1.1047996571136456e-05
109309,109310,109309,218619,59.64228415489197,1.101312534450629e-05
109510,109511,109510,219021,59.724966287612915,1.0978197595520242e-05
109710,109711,109710,219421,59.80658006668091,1.0943560450911147e-05
109910,109911,109910,219821,59.886285066604614,1.0909039439771724e-05
110110,110111,110110,220221,59.97186613082886,1.0874634154690197e-05
110310,110311,110310,220621,60.05821418762207,1.0840344190103891e-05
110511,110512,110511,221023,60.1472430229187,1.0805998555340542e-05
110711,110712,110711,221423,60.23111605644226,1.0771938594496827e-05
110911,110912,110911,221823,60.31340718269348,1.0737992747055034e-05
111111,111112,111111,222223,60.39606523513794,1.0704160614568677e-05
111311,111312,111311,222623,60.47836494445801,1.067044180086801e-05
111512,111513,111512,223025,60.56355834007263,1.063666816496293e-05
111712,111713,111712,223425,60.652015209198,1.060317536842048e-05
111912,111913,111912,223825,60.73712420463562,1.0569794710229288e-05
112112,112113,112112,224225,60.82260012626648,1.0536525800915557e-05
112312,112313,112312,224625,60.90695810317993,1.0503368252932648e-05
112513,112514,112513,225027,60.990076303482056,1.0470156725601657e-05
112713,112714,112713,225427,61.074737310409546,1.0437221296023998e-05
112913,112914,112913,225827,61.157536029815674,1.0404396073128646e-05
113113,113114,113113,226227,61.241475105285645,1.037168067598162e-05
113313,113314,113313,226627,61.322914123535156,1.0339074725084136e-05
113514,113515,113514,227029,61.40246105194092,1.0306415632052334e-05
113714,113715,113714,227429,61.481754302978516,1.0274027985320975e-05
113914,113915,113914,227829,61.56212306022644,1.0241748655058571e-05
114114,114115,114114,228229,61.65098714828491,1.0209577268509251e-05
114314,114315,114314,228629,61.7320830821991,1.0177513454397468e-05
114515,114516,114515,229031,61.81203818321228,1.0145397328777266e-05
114715,114716,114715,229431,61.89190196990967,1.0113548085397391e-05
114915,114916,114915,229831,61.969919204711914,1.0081805308292804e-05
115115,115116,115115,230231,62.04933309555054,1.0050168632586782e-05
115315,115316,115315,230631,62.13101506233215,1.0018637694797622e-05
115516,115517,115516,231033,62.21102333068848,9.987055269208646e-06
115716,115717,115716,231433,62.29133319854736,9.955735246800352e-06
115916,115917,115916,231833,62.3699471950531,9.92451987894531e-06
116116,116117,116116,232233,62.448580265045166,9.893408808518569e-06
116316,116317,116316,232633,62.528685092926025,9.862401678996708e-06
116517,116518,116517,233035,62.611998081207275,9.831343878126327e-06
116717,116718,116717,233435,62.69117498397827,9.800544084108416e-06
116917,116918,116917,233835,62.77099132537842,9.769847170287656e-06
117117,117118,117117,234235,62.851256132125854,9.739252786091199e-06
117317,117318,117317,234635,62.93094515800476,9.708760583111614e-06
117518,117519,117518,235037,63.011595010757446,9.678218517043588e-06
117718,117719,117718,235437,63.09220814704895,9.64793014194564e-06
117918,117919,117918,235837,63.171974182128906,9.617742908107303e-06
118118,118119,118118,236237,63.25153613090515,9.587656472445572e-06
118318,118319,118318,236637,63.33178114891052,9.557670492909305e-06
118519,118520,118519,237039,63.4126501083374,9.52763545108183e-06
118719,118720,118719,237439,63.49139904975891,9.497849862176717e-06
118919,118920,118919,237839,63.572394132614136,9.468163710447886e-06
119119,119120,119119,238239,63.65534424781799,9.438576659636312e-06
119319,119320,119319,238639,63.74105715751648,9.409088374268713e-06
119520,119521,119520,239041,63.820749282836914,9.379551818509335e-06
119720,119721,119720,239441,63.89986205101013,9.350260554350756e-06
119920,119921,119920,239841,63.9797682762146,9.321067056833196e-06
120120,120121,120120,240241,64.05941200256348,9.29197099608622e-06
120320,120321,120320,240641,64.14099621772766,9.262972043598616e-06
120521,120522,120521,241043,64.22175526618958,9.233925603618453e-06
120721,120722,120721,241443,64.30166506767273,9.205120368296e-06
120921,120922,120921,241843,64.38187336921692,9.17641126156657e-06
121121,121122,121121,242243,64.46089029312134,9.147797959813484e-06
121321,121322,121321,242643,64.54038405418396,9.119280140789257e-06
121522,121523,121522,243045,64.6213493347168,9.090715608890595e-06
121722,121723,121722,243445,64.70330023765564,9.062388267207441e-06
121922,121923,121922,243845,64.78582620620728,9.034155447263861e-06
122122,122123,122122,244245,64.86826825141907,9.006016832067756e-06
122322,122323,122322,244645,64.95072412490845,8.977972105350256e-06
122523,122524,122523,245047,65.03344321250916,8.949881431041437e-06
122723,122724,122723,245447,65.11611318588257,8.922024003229597e-06
122923,122924,122923,245847,65.19912624359131,8.894259521458041e-06
123123,123124,123123,246247,65.28164720535278,8.866587673950486e-06
123323,123324,123323,246647,65.36757731437683,8.83900815125399e-06
123524,123525,123524,247049,65.44757413864136,8.811383437088735e-06
123724,123725,123724,247449,65.52745127677917,8.783988095040832e-06
123924,123925,123924,247849,65.61439514160156,8.756684152684236e-06
124124,124125,124124,248249,65.69609212875366,8.729471304443888e-06
124324,124325,124324,248649,65.7847352027893,8.702349245869233e-06
124525,124526,124525,249051,65.87060403823853,8.675182742870968e-06
124725,124726,124725,249451,65.95205521583557,8.648241805597124e-06
124925,124926,124925,249851,66.03696322441101,8.62139075050072e-06
125125,125126,125125,250251,66.1193060874939,8.594629277698607e-06
125325,125326,125325,250651,66.20284223556519,8.567957088477786e-06
125526,125527,125526,251053,66.28498315811157,8.54124119258651e-06
125726,125727,125726,251453,66.3669912815094,8.514747121879422e-06
125926,125927,125926,251853,66.44849634170532,8.48834144398622e-06
126126,126127,126126,252253,66.53056621551514,8.462023864807587e-06
126326,126327,126326,252653,66.61522316932678,8.435794090847101e-06
126527,126528,126527,253055,66.69977498054504,8.409521338462826e-06
126727,126728,126727,253455,66.7852771282196,8.38346673558935e-06
126927,126928,126927,253855,66.86958599090576,8.357499063731341e-06
127127,127128,127127,254255,66.95108723640442,8.331618033921907e-06
127327,127328,127327,254655,67.03261613845825,8.30582335838185e-06
127528,127529,127528,255057,67.11662006378174,8.279986422925265e-06
127728,127729,127728,255457,67.19920706748962,8.254364025002071e-06
127928,127929,127928,255857,67.28080105781555,8.228827122700622e-06
128128,128129,128128,256257,67.36298704147339,8.203375432618442e-06
128328,128329,128328,256657,67.44664025306702,8.178008672136299e-06
128529,128530,128529,257059,67.52905201911926,8.15260036121952e-06
128729,128730,128729,257459,67.61581707000732,8.127403037376114e-06
128929,128930,128929,257859,67.69750714302063,8.102289800305277e-06
129129,129130,129129,258259,67.7787721157074,8.077260371112561e-06
129329,129330,129329,258659,67.86357307434082,8.05231447263009e-06
129530,129531,129530,259061,67.95147013664246,8.027327724085965e-06
129730,129731,129730,259461,68.03400135040283,8.002548472907759e-06
129930,129931,129930,259861,68.11838817596436,7.977851924540117e-06
130130,130131,130130,260261,68.20078611373901,7.953237805721846e-06
130330,130331,130330,260661,68.28298807144165,7.928705843924688e-06
130531,130532,130531,261063,68.36508917808533,7.904133722467289e-06
130731,130732,130731,261463,68.44769716262817,7.879765668388104e-06
130931,130932,130931,261863,68.52838516235352,7.855478958332093e-06
131131,131132,131131,262263,68.61180329322815,7.831273323906519e-06
131331,131332,131331,262663,68.69618320465088,7.80714849714627e-06
131532,131533,131532,263065,68.77891421318054,7.782984192247002e-06
131732,131733,131732,263465,68.86512327194214,7.759020582952624e-06
131932,131933,131932,263865,68.9474949836731,7.735136983153761e-06
132132,132133,132132,264265,69.0284571647644,7.711333128961429e-06
132332,132333,132332,264665,69.11035132408142,7.687608757569467e-06
132533,132534,132533,265067,69.19677710533142,7.663845579966502e-06
132733,132734,132733,265467,69.28165936470032,7.64027978354873e-06
132933,132934,132933,265867,69.37582325935364,7.616792685465662e-06
133133,133134,133133,266267,69.65532493591309,7.59338402694937e-06
133333,133334,133333,266667,70.18477129936218,7.570053549732815e-06
133534,133535,133534,267069,70.39662003517151,7.546684928873255e-06
133734,133735,133734,267469,70.49111104011536,7.5235104308046415e-06
133934,133935,133934,267869,70.5857002735138,7.500413343511995e-06
134134,134135,134134,268269,70.67993307113647,7.477393412523349e-06
134334,134335,134334,268669,70.78225111961365,7.454450384212125e-06
134535,134536,134535,269071,70.8787100315094,7.431469865915137e-06
134735,134736,134735,269471,70.97583413124084,7.408680266896116e-06
134935,134936,134935,269871,71.06534814834595,7.385966813593818e-06
135135,135136,135135,270271,71.15178918838501,7.3633292561568134e-06
135335,135336,135335,270671,71.23639297485352,7.340767345116454e-06
135536,135537,135536,271073,71.31830525398254,7.3181685889755275e-06
135736,135737,135736,271473,71.40337324142456,7.295757602098325e-06
135936,135937,135936,271873,71.49139618873596,7.2734215183694e-06
136136,136137,136136,272273,71.5752022266388,7.251160091890145e-06
136336,136337,136336,272673,71.65918326377869,7.228973077821536e-06
136537,136538,136537,273075,71.74149823188782,7.206749854210524e-06
136737,136738,136737,273475,71.82965421676636,7.184711303109882e-06
136937,136938,136937,273875,71.92425417900085,7.162746434143544e-06
137137,137138,137137,274275,72.00585198402405,7.140855005631626e-06
137337,137338,137337,274675,72.0938241481781,7.119036777113917e-06
137538,137539,137538,275077,72.19051599502563,7.097182965459542e-06
137738,137739,137738,275477,72.28550100326538,7.0755107816114285e-06
137938,137939,137938,275877,72.37241315841675,7.0539110800218686e-06
138138,138139,138138,276277,72.45609927177429,7.032383623238822e-06
138338,138339,138338,276677,72.5475401878357,7.010928175214588e-06
138539,138540,138539,277079,72.64508390426636,6.989437761847133e-06
138739,138740,138739,277479,72.72696208953857,6.968125982219415e-06
138939,138940,138939,277879,72.80712914466858,6.94688550594555e-06
139139,139140,139139,278279,72.89026713371277,6.9257160998572495e-06
139339,139340,139339,278679,72.97753405570984,6.9046175317472975e-06
139540,139541,139540,279081,73.07275414466858,6.883484607254361e-06
139740,139741,139740,279481,73.16079211235046,6.862527372744858e-06
139940,139941,139940,279881,73.24163913726807,6.8416402829467025e-06
140140,140141,140140,280281,73.32342100143433,6.820823108963178e-06
140340,140341,140340,280681,73.40516304969788,6.800075622496457e-06
140541,140542,140541,281083,73.48748111724854,6.779294380109529e-06
140741,140742,140741,281483,73.57267308235168,6.75868593274596e-06
140941,140942,140941,281883,73.66525602340698,6.738146491706433e-06
141141,141142,141141,282283,73.75500321388245,6.717675832176795e-06
141341,141342,141341,282683,73.84777617454529,6.697273729440451e-06
141542,141543,141542,283085,73.9300811290741,6.676838462741711e-06
141742,141743,141742,283485,74.01140999794006,6.656573144298918e-06
141942,141943,141942,283885,74.09667015075684,6.636375713416838e-06
142142,142143,142142,284285,74.18892502784729,6.616245948960334e-06
142342,142343,142342,284685,74.29210233688354,6.596183630459056e-06
142543,142544,142543,285087,74.38144207000732,6.576088731472025e-06
142743,142744,142743,285487,74.46471214294434,6.556160981244117e-06
142943,142944,142943,285887,74.55007004737854,6.536300019031881e-06
143143,143144,143143,286287,74.64809012413025,6.516505627667735e-06
143343,143344,143343,286687,74.74036407470703,6.496777590244595e-06
143544,143545,143544,287089,74.82950711250305,6.477017547417035e-06
143744,143745,143744,287489,74.91263628005981,6.457421900283139e-06
143944,143945,143944,287889,74.99823522567749,6.437891960801721e-06
144144,144145,144144,288289,75.0924642086029,6.4184275151688715e-06
144344,144345,144344,288689,75.18819522857666,6.399028350372062e-06
144545,144546,144545,289091,75.28292608261108,6.379597746888274e-06
144745,144746,144745,289491,75.37040424346924,6.36032883183998e-06
144945,144946,144945,289891,75.45894622802734,6.341124562219437e-06
145145,145146,145145,290291,75.54470920562744,6.321984728138481e-06
145345,145346,145345,290691,75.62730813026428,6.302909120228026e-06
145546,145547,145546,291093,75.71021604537964,6.2838026324741395e-06
145746,145747,145746,291493,75.79186820983887,6.264855170358031e-06
145946,145947,145946,291893,75.87667512893677,6.245971309952342e-06
146146,146147,146146,292293,75.96036005020142,6.227150844507652e-06
146346,146347,146346,292693,76.04610514640808,6.208393568735078e-06
146547,146548,146547,293095,76.13376808166504,6.189605963924979e-06
146747,146748,146747,293495,76.21604323387146,6.170974766069455e-06
146947,146948,146947,293895,76.30161619186401,6.152406143804706e-06
147147,147148,147147,294295,76.39349412918091,6.133899894440153e-06
147347,147348,147347,294695,76.47602820396423,6.115455815292239e-06
147548,147549,147548,295097,76.5607750415802,6.096981950148837e-06
147748,147749,147748,295497,76.64663910865784,6.0786619166569175e-06
147948,147949,147948,295897,76.73002123832703,6.060403450161269e-06
148148,148149,148148,296297,76.8124611377716,6.0422063514438506e-06
148348,148349,148348,296697,76.89551019668579,6.024070421392554e-06
148549,148550,148549,297099,76.97915410995483,6.005905240359498e-06
148749,148750,148749,297499,77.06420612335205,5.9878913581281e-06
148949,148950,148949,297899,77.14962720870972,5.969938051646227e-06
149149,149150,149149,298299,77.23365521430969,5.952045124915494e-06
149349,149350,149349,298699,77.317312002182,5.934212382477478e-06
149550,149551,149550,299101,77.4003803730011,5.916350916448263e-06
149750,149751,149750,299501,77.48380398750305,5.898638257874787e-06
149950,149951,149950,299901,77.56787109375,5.880985200618706e-06
150150,150151,150150,300301,77.65407705307007,5.863391552095641e-06
150350,150351,150350,300701,77.73729515075684,5.845857120064781e-06
150551,150552,150551,301103,77.8217101097107,5.8282944842517344e-06
150751,150752,150751,301503,77.9050931930542,5.810878205637926e-06
150951,150952,150951,301903,77.98876404762268,5.793520570547523e-06
151151,151152,151151,302303,78.07310128211975,5.776221389484622e-06
151351,151352,151351,302703,78.15638518333435,5.758980473760684e-06
151552,151553,151552,303105,78.24030208587646,5.7417118665296125e-06
151752,151753,151752,303505,78.32296299934387,5.7245872065216314e-06
151952,151953,151952,303905,78.41066217422485,5.707520248421549e-06
152152,152153,152152,304305,78.50056719779968,5.690510806009137e-06
152352,152353,152352,304705,78.5856761932373,5.673558693701847e-06
152553,152554,152553,305107,78.67054414749146,5.656579395014361e-06
152753,152754,152753,305507,78.75332307815552,5.6397416732233425e-06
152953,152954,152953,305907,78.83580327033997,5.622960727485643e-06
153153,153154,153153,306307,78.91842103004456,5.60623637512853e-06
153353,153354,153353,306707,79.00165915489197,5.589568433535449e-06
153554,153555,153554,307109,79.08798432350159,5.572873803292435e-06
153754,153755,153754,307509,79.17192816734314,5.556318418328363e-06
153954,153955,153954,307909,79.25389814376831,5.53981889963583e-06
154154,154155,154154,308309,79.33682107925415,5.523375067476945e-06
154354,154355,154354,308709,79.42008829116821,5.506986742267757e-06
154555,154556,154555,309111,79.50329613685608,5.490572219075588e-06
154755,154756,154755,309511,79.59057116508484,5.474294647870861e-06
154955,154956,154955,309911,79.6765022277832,5.458072048367161e-06
155155,155156,155155,310311,79.75979328155518,5.441904243861847e-06
155355,155356,155355,310711,79.84225797653198,5.425791057964205e-06
155556,155557,155556,311113,79.92532205581665,5.409652157798915e-06
155756,155757,155756,311513,80.00808024406433,5.393647953517257e-06
155956,155957,155956,311913,80.09406614303589,5.377697841658157e-06
156156,156157,156156,312313,80.17740511894226,5.361801648365874e-06
156356,156357,156356,312713,80.26141428947449,5.345959200183234e-06
156557,156558,156557,313115,80.3458480834961,5.330091514488206e-06
156757,156758,156757,313515,80.42912697792053,5.314356305722761e-06
156957,156958,156957,313915,80.5181040763855,5.298674324951923e-06
157157,157158,157157,314315,80.60876226425171,5.283045401037381e-06
157357,157358,157357,314715,80.6929280757904,5.267469363605866e-06
157558,157559,157558,315117,80.77761626243591,5.251868558504785e-06
157758,157759,157758,315517,80.86196303367615,5.236398047709231e-06
157958,157959,157958,315917,80.9455292224884,5.220979914787411e-06
158158,158159,158158,316317,81.02847123146057,5.20561399170804e-06
158358,158359,158358,316717,81.11386227607727,5.190300110980987e-06
158559,158560,158559,317119,81.1976752281189,5.17496192570724e-06
158759,158760,158759,317519,81.28125214576721,5.159751887560836e-06
158959,158960,158959,317919,81.36353898048401,5.144593391857393e-06
159159,159160,159159,318319,81.44860219955444,5.12948627310576e-06
159359,159360,159359,318719,81.53195714950562,5.114430366742394e-06
159560,159561,159560,319121,81.61807608604431,5.099350612312682e-06
159760,159761,159760,319521,81.70053720474243,5.084396892996728e-06
159960,159961,159960,319921,81.78380703926086,5.069493894353015e-06
160160,160161,160160,320321,81.86683392524719,5.054641454197632e-06
160360,160361,160360,320721,81.94985604286194,5.039839410504112e-06
160561,160562,160561,321123,82.03676128387451,5.0250139685924725e-06
160761,160762,160761,321523,82.12274217605591,5.010312483961548e-06
160961,160962,160961,321923,82.20556426048279,4.995660912460998e-06
161161,161162,161161,322323,82.28741002082825,4.981059094358693e-06
161361,161362,161361,322723,82.3715672492981,4.966506870434838e-06
161562,161563,161562,323125,82.45309805870056,4.951931691979661e-06
161762,161763,161762,323525,82.53753519058228,4.937478426846193e-06
161962,161963,161962,323925,82.63427114486694,4.923074280748261e-06
162162,162163,162162,324325,82.71947121620178,4.908719096604075e-06
162362,162363,162362,324725,82.8032820224762,4.8944127178173414e-06
162563,162564,162563,325127,82.88685917854309,4.880083821849876e-06
162763,162764,162763,325527,82.96958422660828,4.865874828457729e-06
162963,162964,162963,325927,83.05414032936096,4.85171417324227e-06
163163,163164,163163,326327,83.13734722137451,4.837601701773514e-06
163363,163364,163363,326727,83.22019004821777,4.823537260273935e-06
163564,163565,163564,327129,83.30385899543762,4.809450732482969e-06
163764,163765,163764,327529,83.38437724113464,4.795482129261541e-06
163964,163965,163964,327929,83.46392297744751,4.7815610965890805e-06
164164,164165,164164,328329,83.54588413238525,4.767687482577345e-06
164364,164365,164364,328729,83.6284191608429,4.753861135957325e-06
164565,164566,164565,329131,83.70778298377991,4.7400131277851735e-06
164765,164766,164765,329531,83.78936123847961,4.7262810984038405e-06
164965,164966,164965,329931,83.87116599082947,4.712595884574897e-06
165165,165166,165165,330331,83.95205116271973,4.698957337224422e-06
165365,165366,165365,330731,84.03083395957947,4.685365307538176e-06
165566,165567,165566,331133,84.11362409591675,4.671752035158019e-06
165766,165767,165766,331533,84.19334197044373,4.658252826979034e-06
165966,165967,165966,331933,84.27852606773376,4.644799692376063e-06
166166,166167,166166,332333,84.35987210273743,4.631392484494098e-06
166366,166367,166366,332733,84.44255113601685,4.618031056900356e-06
166567,166568,166567,333135,84.5227541923523,4.604648799540899e-06
166767,166768,166767,333535,84.60620617866516,4.591378723030828e-06
166967,166968,166967,333935,84.69136810302734,4.5781539903311905e-06
167167,167168,167167,334335,84.77600693702698,4.564974456861088e-06
167367,167368,167367,334735,84.85540103912354,4.5518399790590344e-06
167568,167569,167568,335137,84.93938732147217,4.538685078197147e-06
167768,167769,167768,335537,85.04242515563965,4.525640505249132e-06
167968,167969,167968,335937,85.22534823417664,4.512640558597665e-06
168168,168169,168168,336337,85.35312700271606,4.499685096210891e-06
168368,168369,168368,336737,85.46996927261353,4.486773976566787e-06
168569,168570,168569,337139,85.62969517707825,4.473842834837155e-06
168769,168770,168769,337539,85.7568621635437,4.461020198219809e-06
168969,168970,168969,337939,85.85062408447266,4.448241482146131e-06
169169,169170,169169,338339,85.94550609588623,4.435506547144565e-06
169369,169370,169369,338739,86.03550601005554,4.422815253946041e-06
169570,169571,169570,339141,86.12473607063293,4.410104334204606e-06
169770,169771,169770,339541,86.21001601219177,4.397500125925452e-06
169970,169971,169970,339941,86.29458904266357,4.384939144325197e-06
170170,170171,170170,340341,86.39054322242737,4.3724212521793095e-06
170370,170371,170370,340741,86.47238612174988,4.35994631292614e-06
170571,170572,170571,341143,86.5525860786438,4.347452136560655e-06
170771,170772,170771,341543,86.63819599151611,4.335062907228532e-06
170971,170972,170971,341943,86.73045992851257,4.322716222189959e-06
171171,171172,171171,342343,86.83357119560242,4.310411946732527e-06
171371,171372,171371,342743,86.91714906692505,4.298149946170563e-06
171572,171573,171572,343145,87.00003099441528,4.285869092836647e-06
171772,171773,171772,343545,87.08158016204834,4.273691450262132e-06
171972,171973,171972,343945,87.16664028167725,4.261555681150889e-06
172172,172173,172172,344345,87.24870920181274,4.249461652809163e-06
172372,172373,172372,344745,87.33037424087524,4.2374092329218775e-06
172573,172574,172573,345147,87.41122102737427,4.225338339002142e-06
172773,172774,172773,345547,87.49238419532776,4.213368947507302e-06
172973,172974,172973,345947,87.57524108886719,4.201440769678948e-06
173173,173174,173173,346347,87.66237020492554,4.189553674950268e-06
173373,173374,173373,346747,87.74525022506714,4.177707533306873e-06
173574,173575,173574,347149,87.83526039123535,4.1658432907343624e-06
173774,173775,173774,347549,87.95246815681458,4.154078869982883e-06
173974,173975,173974,347949,88.06980514526367,4.142355013982203e-06
174174,174175,174174,348349,88.1721441745758,4.130671594444888e-06
174374,174375,174374,348749,88.27610397338867,4.119028483341975e-06
174575,174576,174575,349151,88.38093423843384,4.107367639356372e-06
174775,174776,174775,349551,88.55289220809937,4.095804963243175e-06
174975,174976,174975,349951,88.67004704475403,4.08428221362813e-06
175175,175176,175175,350351,88.75565695762634,4.07279926471679e-06
175375,175376,175375,350751,88.87589526176453,4.061355990216689e-06
175576,175577,175576,351153,89.08825612068176,4.049895345413593e-06
175776,175777,175776,351553,89.21320033073425,4.038531241383466e-06
175976,175977,175976,351953,89.31206822395325,4.027206436351518e-06
176176,176177,176176,352353,89.45635509490967,4.0159208061340195e-06
176376,176377,176376,352753,89.54749417304993,4.004674227189648e-06
176577,176578,176577,353155,89.63443422317505,3.993410635410604e-06
176777,176778,176777,353555,89.72042918205261,3.982241982920431e-06
176977,176978,176977,353955,89.80315232276917,3.971112012351288e-06
177177,177178,177177,354355,89.89599919319153,3.960020601547578e-06
177377,177378,177377,354755,89.99499011039734,3.948967628741191e-06
177578,177579,177578,355157,90.08924126625061,3.93789799552895e-06
177778,177779,177778,355557,90.18333697319031,3.926921725920134e-06
177978,177979,177978,355957,90.27276110649109,3.915983531108525e-06
178178,178179,178178,356357,90.35851216316223,3.905083291013593e-06
178378,178379,178378,356757,90.44582319259644,3.894220885888012e-06
178579,178580,178579,357159,90.53684210777283,3.883342167592487e-06
178779,178780,178779,357559,90.6274561882019,3.8725552626467974e-06
178979,178980,178979,357959,90.71124625205994,3.861805835294575e-06
179179,179180,179179,358359,90.79846811294556,3.851093767523302e-06
179379,179380,179379,358759,90.88042497634888,3.840418941583324e-06
179580,179581,179580,359161,90.97934126853943,3.829728144689203e-06
179780,179781,179780,359561,91.07939314842224,3.819127635572895e-06
179980,179981,179980,359961,91.16667222976685,3.8085640167242036e-06
180180,180181,180180,360361,91.25168704986572,3.798037172209107e-06
180380,180381,180380,360761,91.33764004707336,3.78754698582098e-06
180581,180582,180581,361163,91.43054604530334,3.7770411660805533e-06
180781,180782,180781,361563,91.51832413673401,3.766624132485261e-06
180981,180982,180981,361963,91.61066222190857,3.7562434117344197e-06
181181,181182,181181,362363,91.69976925849915,3.7458988894226225e-06
181381,181382,181381,362763,91.7863712310791,3.735590451487756e-06
181582,181583,181582,363165,91.87139511108398,3.725266712420481e-06
181782,181783,181782,363565,91.95488810539246,3.7150302823397906e-06
181982,181983,181982,363965,92.03960704803467,3.7048295966063823e-06
182182,182183,182182,364365,92.12823295593262,3.694664543184869e-06
182382,182383,182382,364765,92.21705722808838,3.6845350093777956e-06
182583,182584,182583,365167,92.30245923995972,3.674390502331316e-06
182783,182784,182783,365567,92.44869303703308,3.6643318500779676e-06
182983,182984,182983,365967,92.55951428413391,3.6543083833884026e-06
183183,183184,183183,366367,92.66052412986755,3.6443199917770276e-06
183383,183384,183383,366767,92.75522303581238,3.6343665645754896e-06
183584,183585,183584,367169,92.84922122955322,3.6243984866895515e-06
183784,183785,183784,367569,92.94401621818542,3.6145148331475004e-06
183984,183985,183984,367969,93.03875517845154,3.604665815118484e-06
184184,184185,184184,368369,93.13649106025696,3.594851323842784e-06
184384,184385,184384,368769,93.23334503173828,3.585071251068171e-06
184585,184586,184585,369171,93.32234311103821,3.5752768455795214e-06
184785,184786,184785,369571,93.43902111053467,3.5655654562939783e-06
184985,184986,184985,369971,93.54184913635254,3.555888161526495e-06
185185,185186,185185,370371,93.64711213111877,3.546244854486385e-06
185385,185386,185385,370771,93.74704813957214,3.5366354282192133e-06
185586,185587,185586,371173,93.84707713127136,3.5270119830807915e-06
185786,185787,185786,371573,93.94477319717407,3.5174701681373214e-06
185986,185987,185986,371973,94.04428720474243,3.5079619156391466e-06
186186,186187,186186,372373,94.14524602890015,3.4984871202307283e-06
186386,186387,186386,372773,94.24584603309631,3.489045676859773e-06
186587,186588,186587,373175,94.33968114852905,3.4795905234501075e-06
186787,186788,186787,373575,94.47994804382324,3.4702156363848467e-06
186987,186988,186987,373975,94.60863423347473,3.4608737880986954e-06
187187,187188,187187,374375,94.71200919151306,3.4515648749836343e-06
187387,187388,187387,374775,94.80528903007507,3.442288793944027e-06
187588,187589,187588,375177,94.90378499031067,3.432999306950669e-06
187788,187789,187788,375577,95.00267910957336,3.4237887440570193e-06
187988,187989,187988,375977,95.10134410858154,3.4146107047527672e-06
188188,188189,188188,376377,95.2101731300354,3.4054650870217814e-06
188388,188389,188388,376777,95.31319308280945,3.3963517894367473e-06
188589,188590,188589,377179,95.40930509567261,3.3872253859145233e-06
188789,188790,188789,377579,95.51400399208069,3.378176585100577e-06
188989,188990,188989,377979,95.61129713058472,3.3691598010748837e-06
189189,189190,189189,378379,95.71116232872009,3.360174933378381e-06
189389,189390,189389,378779,95.80019903182983,3.3512218820301922e-06
189590,189591,189590,379181,95.89053010940552,3.3422560202512777e-06
189790,189791,189790,379581,95.98109126091003,3.333366460839072e-06
189990,189991,189990,379981,96.0824122428894,3.3245084193059867e-06
190190,190191,190190,380381,96.1750180721283,3.3156817968977727e-06
190390,190391,190390,380781,96.2740581035614,3.3068864953261105e-06
190591,190592,190591,381183,96.36535811424255,3.2980786741537125e-06
190791,190792,190791,381583,96.4585211277008,3.2893458755720514e-06
190991,190992,190991,381983,96.55125403404236,3.2806441039922677e-06
191191,191192,191191,382383,96.64191317558289,3.271973262189206e-06
191391,191392,191391,382783,96.7356550693512,3.2633332534198247e-06
191592,191593,191592,383185,96.82852506637573,3.2546810119418195e-06
191792,191793,191792,383585,96.91915822029114,3.246102533030569e-06
191992,191993,191992,383985,97.02435898780823,3.2375545979473857e-06
192192,192193,192192,384385,97.1788592338562,3.229037111300812e-06
192392,192393,192392,384785,97.28403425216675,3.2205499777021097e-06
192593,192594,192593,385187,97.40208530426025,3.2120508937044906e-06
192793,192794,192793,385587,97.51149010658264,3.203624332187115e-06
192993,192994,192993,385987,97.68711829185486,3.1952278391694564e-06
193193,193194,193193,386387,97.82531714439392,3.18686132047068e-06
193393,193394,193393,386787,97.93581318855286,3.1785246828576896e-06
193594,193595,193594,387189,98.04452323913574,3.1701763724487542e-06
193794,193795,193794,387589,98.15052008628845,3.161899364064116e-06
193994,193995,193994,387989,98.2971830368042,3.153651956277848e-06
194194,194195,194194,388389,98.41300320625305,3.1454340564722e-06
194394,194395,194394,388789,98.52772212028503,3.1372455723753427e-06
194595,194596,194595,389191,98.6321370601654,3.1290456898217e-06
194795,194796,194795,389591,98.73207712173462,3.120915907429245e-06
194995,194996,194995,389991,98.83217430114746,3.1128152649873918e-06
195195,195196,195195,390391,98.93304705619812,3.1047436716530736e-06
195395,195396,195395,390791,99.04259729385376,3.096701036413431e-06
195596,195597,195596,391193,99.14281702041626,3.0886472721443106e-06
195796,195797,195796,391593,99.24699020385742,3.0806624253621303e-06
195996,195997,195996,391993,99.3459861278534,3.0727062652486203e-06
196196,196197,196196,392393,99.456707239151,3.0647787021755737e-06
196396,196397,196396,392793,99.63131618499756,3.0568796467545124e-06
196597,196598,196597,393195,99.73147392272949,3.0489697279017453e-06
196797,196798,196797,393595,99.82690906524658,3.041127561739402e-06
196997,196998,196997,393995,99.92197608947754,3.0333136362707805e-06
197197,197198,197197,394395,100.08301210403442,3.0255278630411608e-06
197397,197398,197397,394795,100.22543597221375,3.0177701539259605e-06
197598,197599,197598,395197,100.33053421974182,3.0100018425907908e-06
197798,197799,197798,395597,100.42784023284912,3.0023001379631036e-06
197998,197999,197998,395997,100.57458305358887,2.99462623443086e-06
198198,198199,198198,396397,100.73203611373901,2.9869800453218034e-06
198398,198399,198398,396797,100.84103512763977,2.9793614836000283e-06
198599,198600,198599,397199,100.95713806152344,2.9717325770115906e-06
198799,198800,198799,397599,101.0737202167511,2.964169148538521e-06
198999,199000,198999,397999,101.19772219657898,2.9566330888374547e-06
199199,199200,199199,398399,101.36313724517822,2.9491243120777195e-06
199399,199400,199399,398799,101.4587972164154,2.9416427331583467e-06
199600,199601,199600,399201,101.6027102470398,2.934151062541536e-06
199800,199801,199800,399601,101.77419400215149,2.926723758749551e-06
200000,200001,200000,400001,101.9226770401001,2.9193233981248053e-06


==> extragradient/plot_data/bilinear_matrix_game_n500/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0008990764617919922,2.018959020339561
100,630,630,1260,0.7926907539367676,0.016955538903785962
200,1408,1408,2816,1.9575417041778564,0.00509124984935892
300,2194,2194,4388,2.821923017501831,0.0029190791169841366
400,2988,2988,5976,3.999485731124878,0.0019769291918388643
501,3788,3788,7576,4.753366947174072,0.001386850821596553
601,4578,4578,9156,5.501091003417969,0.0009261398725110851
701,5368,5368,10736,6.4988720417022705,0.0006371851507888394
801,6160,6160,12320,7.2532737255096436,0.00045484893904930196
901,6960,6960,13920,8.152987718582153,0.0004287061386675959
1001,7758,7758,15516,8.962201833724976,0.0003616089715194565
1101,8552,8552,17104,9.955989837646484,0.00028162733682044773
1201,9348,9348,18696,10.838840007781982,0.00024026955667390244
1301,10148,10148,20296,11.558543682098389,0.00023407537823526932
1401,10940,10940,21880,12.324745893478394,0.00017539558177249575
1502,11748,11748,23496,13.085269927978516,0.00017056819096984547
1602,12544,12544,25088,13.846674919128418,0.00014760133033107917
1702,13344,13344,26688,14.746678829193115,0.00014341869917563582
1802,14140,14140,28280,15.644820928573608,0.0001210621447322439
1902,14936,14936,29872,16.603880882263184,0.00010682822637046061
2002,15736,15736,31472,17.556581735610962,0.0001009986259508994
2102,16532,16532,33064,18.52286982536316,9.02976930312845e-05
2202,17332,17332,34664,19.873430967330933,8.448992177688343e-05
2302,18114,18114,36228,20.83201289176941,4.646700913824585e-05
2402,18914,18914,37828,21.978569984436035,4.22413395307836e-05
2503,19722,19722,39444,23.02886986732483,4.148860509170336e-05
2603,20522,20522,41044,24.078049898147583,4.1000273598608064e-05
2703,21316,21316,42632,25.140458822250366,3.239542001884659e-05
2803,22110,22110,44220,26.042916774749756,2.6661849554904908e-05
2903,22900,22900,45800,27.07267665863037,1.7326274576708128e-05
3003,23700,23700,47400,28.019145965576172,1.713009128439785e-05
3103,24496,24496,48992,29.041709899902344,1.4906355248503622e-05
3203,25296,25296,50592,30.39768075942993,1.4668108882325533e-05
3303,26096,26096,52192,31.57872772216797,1.4605272127657383e-05
3403,26896,26896,53792,32.56172490119934,1.4550957029235648e-05
3504,27694,27694,55388,33.59352087974548,1.0517257699384487e-05
3604,28494,28494,56988,34.594701051712036,1.0276429266699877e-05
3704,29294,29294,58588,35.55801177024841,1.0165989403438173e-05
3804,30094,30094,60188,36.523990869522095,1.0094068642342995e-05
3904,30894,30894,61788,37.59448170661926,1.0042615494573434e-05
4004,31692,31692,63384,38.588966846466064,9.662160914747742e-06
4104,32488,32488,64976,39.558127880096436,8.297329399426618e-06
4204,33288,33288,66576,40.49451684951782,8.167730381531815e-06
4304,34088,34088,68176,41.78272294998169,8.081141659904289e-06
4404,34888,34888,69776,42.905396938323975,8.01243396686031e-06
4505,35696,35696,71392,44.094162940979004,7.954645482219052e-06
4605,36496,36496,72992,45.21505689620972,7.905875249941169e-06
4705,37296,37296,74592,46.378437757492065,7.863640478012805e-06
4805,38096,38096,76192,47.41506886482239,7.826650289335817e-06
4905,38896,38896,77792,48.41278672218323,7.793952952282462e-06
5005,39696,39696,79392,49.449824810028076,7.764819611501512e-06
5105,40494,40494,80988,50.34048366546631,7.166402662396179e-06
5205,41294,41294,82588,51.24671196937561,7.047236425733933e-06
5305,42094,42094,84188,52.107511043548584,6.990741772512877e-06
5405,42894,42894,85788,52.984118938446045,6.9537677374474735e-06
5506,43702,43702,87404,53.8645658493042,6.925716947904835e-06
5606,44502,44502,89004,54.91956400871277,6.903215712920718e-06
5706,45302,45302,90604,55.76042985916138,6.884226767241571e-06
5806,46098,46098,92196,56.637136697769165,6.327974417755719e-06
5906,46898,46898,93796,57.5794198513031,6.208366959417366e-06
6006,47698,47698,95396,58.43850064277649,6.136007466258612e-06
6106,48498,48498,96996,59.393412828445435,6.084044217559392e-06
6206,49298,49298,98596,60.231329917907715,6.044335784100266e-06
6306,50098,50098,100196,61.10032367706299,6.01283857894685e-06
6406,50898,50898,101796,61.9570198059082,5.987261697908394e-06
6507,51706,51706,103412,62.80311870574951,5.965972732795764e-06
6607,52506,52506,105012,63.81721901893616,5.9484040330547516e-06
6707,53306,53306,106612,64.66270089149475,5.933614986659097e-06
6807,54106,54106,108212,65.51485896110535,5.92106982596861e-06
6907,54906,54906,109812,66.34856796264648,5.910352400037816e-06
7007,55706,55706,111412,67.19943881034851,5.901133338181961e-06
7107,56506,56506,113012,68.11392188072205,5.893148619359206e-06
7207,57306,57306,114612,69.03902983665466,5.886184733560652e-06
7307,58106,58106,116212,69.89641070365906,5.880067919030899e-06
7407,58906,58906,117812,70.80985498428345,5.874656086411362e-06
7508,59714,59714,119428,71.67700600624084,5.869787002670731e-06
7608,60514,60514,121028,72.55386996269226,5.8654603424681444e-06
7708,61314,61314,122628,73.49285769462585,5.861546002901846e-06
7808,62114,62114,124228,74.4341549873352,5.857978493310768e-06
7908,62914,62914,125828,75.3052008152008,5.854703492354356e-06
8008,63714,63714,127428,76.2234480381012,5.8516758491434274e-06
8108,64514,64514,129028,77.18024802207947,5.8488579589917724e-06
8208,65314,65314,130628,78.14422082901001,5.8462184416253495e-06
8308,66114,66114,132228,79.00415897369385,5.843731060338492e-06
8408,66914,66914,133828,79.85006284713745,5.841373837443945e-06
8509,67722,67722,135444,80.70301675796509,5.839106382327398e-06
8609,68522,68522,137044,81.70879673957825,5.836957968985265e-06
8709,69322,69322,138644,82.74072289466858,5.809443370042186e-06
8809,70122,70122,140244,83.72970986366272,5.793271603385568e-06
8909,70922,70922,141844,84.81722593307495,5.780556087621354e-06
9009,71722,71722,143444,86.0396568775177,5.769409677235646e-06
9109,72522,72522,145044,87.08651781082153,5.759252189389179e-06
9209,73322,73322,146644,88.03691792488098,5.749798073419194e-06
9309,74122,74122,148244,88.96929478645325,5.74087728462336e-06
9409,74922,74922,149844,89.91716074943542,5.7323778165870145e-06
9510,75730,75730,151460,90.85673475265503,5.724141135486942e-06
9610,76530,76530,153060,91.81113696098328,5.716272632508954e-06
9710,77330,77330,154660,92.76479887962341,5.708646194882714e-06
9810,78130,78130,156260,93.71330285072327,5.701228817024818e-06
9910,78930,78930,157860,94.63588285446167,5.693994694010253e-06
10010,79730,79730,159460,95.58167791366577,5.686923346424502e-06
10110,80530,80530,161060,96.505441904068,5.679998300698835e-06
10210,81330,81330,162660,97.44689989089966,5.67320613726925e-06
10310,82130,82130,164260,98.38244771957397,5.666535794335813e-06
10410,82930,82930,165860,99.29994988441467,5.659978047952543e-06
10511,83738,83738,167476,100.24005079269409,5.653461099630956e-06
10611,84538,84538,169076,101.17765402793884,5.6471073237840765e-06
10711,85338,85338,170676,102.33229184150696,5.640845993031622e-06
10811,86138,86138,172276,103.40878486633301,5.634672163954087e-06
10911,86938,86938,173876,104.35806894302368,5.628581503665035e-06
11011,87738,87738,175476,105.30638003349304,5.6225701828768e-06
11111,88538,88538,177076,106.22948884963989,5.616634791473215e-06
11211,89338,89338,178676,107.16312170028687,5.610772270460315e-06
11311,90136,90136,180272,108.18980884552002,5.433366258963905e-06
11411,90936,90936,181872,109.23143482208252,5.403292853218072e-06
11512,91744,91744,183488,110.34522795677185,5.389959419218816e-06
11612,92544,92544,185088,111.36492681503296,5.379030745130811e-06
11712,93344,93344,186688,112.28995084762573,5.369638516264796e-06
11812,94144,94144,188288,113.20416188240051,5.361383657521053e-06
11912,94944,94944,189888,114.07621598243713,5.353992105512874e-06
12012,95744,95744,191488,114.94809079170227,5.347266919615798e-06
12112,96544,96544,193088,115.91251301765442,5.341064042036829e-06
12212,97344,97344,194688,116.83648586273193,5.335276896750111e-06
12312,98144,98144,196288,117.82964181900024,5.329825866342663e-06
12412,98944,98944,197888,118.68134498596191,5.324650900786245e-06
12513,99752,99752,199504,119.56882405281067,5.319657845143588e-06
12613,100552,100552,201104,120.44012999534607,5.31491010416988e-06
12713,101352,101352,202704,121.35282683372498,5.310329810370406e-06
12813,102152,102152,204304,122.31796383857727,5.30589542210023e-06
12913,102944,102944,205888,123.26762580871582,5.192621568150064e-06
13013,103744,103744,207488,124.133535861969,5.16479772963822e-06
13113,104544,104544,209088,124.99061870574951,5.142004920835586e-06
13213,105344,105344,210688,125.85401701927185,5.1231099305234735e-06
13313,106144,106144,212288,126.704833984375,5.107257847446768e-06
13413,106944,106944,213888,127.56999182701111,5.093801173906834e-06
13514,107752,107752,215504,128.430490732193,5.082139849072233e-06
13614,108552,108552,217104,129.28515577316284,5.072124986796357e-06
13714,109352,109352,218704,130.1589138507843,5.063342636365345e-06
13814,110152,110152,220304,131.01790380477905,5.055568101051718e-06
13914,110952,110952,221904,131.8923008441925,5.048625788082972e-06
14014,111752,111752,223504,132.75447988510132,5.04237737357884e-06
14114,112552,112552,225104,133.61401176452637,5.036712972719286e-06
14214,113352,113352,226704,134.48756885528564,5.031544529553057e-06
14314,114152,114152,228304,135.33707070350647,5.02680085013945e-06
14414,114952,114952,229904,136.2086319923401,5.022423855243657e-06
14515,115760,115760,231520,137.06181693077087,5.018326629130713e-06
14615,116560,116560,233120,137.8997449874878,5.014550312422205e-06
14715,117360,117360,234720,138.75052285194397,5.011019631983871e-06
14815,118160,118160,236320,139.58890986442566,5.0077065643186775e-06
14915,118960,118960,237920,140.42978978157043,5.004587261485966e-06
15015,119760,119760,239520,141.2569169998169,5.001641279663504e-06
15115,120560,120560,241120,142.07784700393677,4.998850972807352e-06
15215,121360,121360,242720,142.91890573501587,4.9962010146302325e-06
15315,122160,122160,244320,143.7598798274994,4.993678014896531e-06
15415,122960,122960,245920,144.8801829814911,4.991270213706705e-06
15516,123768,123768,247536,145.85919785499573,4.9889447000698655e-06
15616,124568,124568,249136,146.90839290618896,4.986738253236554e-06
15716,125368,125368,250736,147.82764101028442,4.984619163624402e-06
15816,126168,126168,252336,148.81653380393982,4.982580128397618e-06
15916,126968,126968,253936,149.85489296913147,4.980614604300355e-06
16016,127768,127768,255536,150.78765177726746,4.978716710934794e-06
16116,128568,128568,257136,151.72352981567383,4.97688115084674e-06
16216,129368,129368,258736,152.71759796142578,4.975103139092488e-06
16316,130168,130168,260336,153.5848367214203,4.9733783446441515e-06
16416,130968,130968,261936,154.42488169670105,4.971702839861684e-06
16517,131776,131776,263552,155.25937390327454,4.970056977581966e-06
16617,132576,132576,265152,156.12090182304382,4.96847007503903e-06
16717,133376,133376,266752,157.02502870559692,4.966922655717912e-06
16817,134176,134176,268352,157.87944173812866,4.965412018782064e-06
16917,134976,134976,269952,158.77211785316467,4.963935695571115e-06
17017,135776,135776,271552,159.64168286323547,4.962491425940999e-06
17117,136576,136576,273152,160.4925618171692,4.9610771391968174e-06
17217,137376,137376,274752,161.3494598865509,4.95969093471717e-06
17317,138176,138176,276352,162.27296996116638,4.958331067236122e-06
17417,138976,138976,277952,163.24627780914307,4.956995931715843e-06
17518,139784,139784,279568,164.17522287368774,4.955671044840833e-06
17618,140584,140584,281168,165.15838384628296,4.954381269944263e-06
17718,141384,141384,282768,166.15204977989197,4.953112120964265e-06
17818,142184,142184,284368,166.96804976463318,4.951862440025244e-06
17918,142984,142984,285968,167.77408289909363,4.950631157126128e-06
18018,143784,143784,287568,168.63221979141235,4.9494172823507566e-06
18118,144584,144584,289168,169.48170065879822,4.948219899866434e-06
18218,145384,145384,290768,170.4063549041748,4.947038160690222e-06
18318,146184,146184,292368,171.40724086761475,4.945871277590534e-06
18418,146984,146984,293968,172.41504979133606,4.944718520160994e-06
18519,147792,147792,295584,173.5036427974701,4.943567881934315e-06
18619,148592,148592,297184,174.54851388931274,4.9424415120070085e-06
18719,149392,149392,298784,175.63830399513245,4.941327364929787e-06
18819,150192,150192,300384,176.61627578735352,4.9402248938552925e-06
18919,150992,150992,301984,177.6413698196411,4.9391335893815905e-06
19019,151792,151792,303584,178.7753746509552,4.93805297615081e-06
19119,152592,152592,305184,179.894122838974,4.9369826100609116e-06
19219,153392,153392,306784,180.8796968460083,4.935922076426304e-06
19319,154192,154192,308384,181.86896467208862,4.93487098702412e-06
19419,154992,154992,309984,182.68357181549072,4.93382897844952e-06
19520,155800,155800,311600,183.52358388900757,4.932785420841633e-06
19620,156600,156600,313200,184.35950994491577,4.931760656522194e-06
19720,157400,157400,314800,185.56887292861938,4.930744011056225e-06
19820,158200,158200,316400,186.87751483917236,4.929735202655005e-06
19920,159000,159000,318000,188.01257181167603,4.928733967078879e-06
20020,159800,159800,319600,188.9733808040619,4.927740055307313e-06
20120,160600,160600,321200,189.8329257965088,4.926753232761681e-06
20220,161400,161400,322800,190.85738372802734,4.9257732787178775e-06
20320,162200,162200,324400,191.68229293823242,4.924799984467828e-06
20420,163000,163000,326000,192.81600689888,4.923833153096547e-06
20521,163808,163808,327616,193.80948185920715,4.922863024241698e-06
20621,164608,164608,329216,194.69390892982483,4.92190863091457e-06
20721,165408,165408,330816,195.55455470085144,4.920960170058639e-06
20821,166208,166208,332416,196.43030071258545,4.920017484250153e-06
20921,167008,167008,334016,197.29114484786987,4.919080423562327e-06
21021,167808,167808,335616,198.19066286087036,4.918148846148426e-06
21121,168608,168608,337216,199.06382083892822,4.917222617117805e-06
21221,169408,169408,338816,199.9280970096588,4.9163016082130124e-06
21321,170208,170208,340416,200.77890586853027,4.915385697379111e-06
21421,171008,171008,342016,201.60491490364075,4.914474768486693e-06
21522,171816,171816,343632,202.45354390144348,4.9135596743875945e-06
21622,172616,172616,345232,203.27708888053894,4.912658429265875e-06
21722,173416,173416,346832,204.10430002212524,4.91176184803219e-06
21822,174216,174216,348432,204.9461328983307,4.91086983405129e-06
21922,175016,175016,350032,205.7898817062378,4.909982295532316e-06
22022,175816,175816,351632,206.6513638496399,4.909099144396792e-06
22122,176616,176616,353232,207.5239598751068,4.90822029600857e-06
22222,177416,177416,354832,208.38232278823853,4.907345669585487e-06
22322,178216,178216,356432,209.26846885681152,4.906475187651591e-06
22422,179016,179016,358032,210.15039777755737,4.905608775775045e-06
22523,179824,179824,359648,211.0474009513855,4.904737758157217e-06
22623,180624,180624,361248,211.9204399585724,4.9038793132754394e-06
22723,181424,181424,362848,212.74619269371033,4.903024731245771e-06
22823,182224,182224,364448,213.59569191932678,4.90217394848497e-06
22923,183024,183024,366048,214.43516492843628,4.901326903363302e-06
23023,183824,183824,367648,215.28404784202576,4.900483537009076e-06
23123,184624,184624,369248,216.12264966964722,4.899643792292679e-06
23223,185424,185424,370848,216.98411178588867,4.898807613953216e-06
23323,186224,186224,372448,217.85246896743774,4.897974948929928e-06
23423,187024,187024,374048,218.69842386245728,4.8971457455601415e-06
23524,187832,187832,375664,219.5846288204193,4.896311713132123e-06
23624,188632,188632,377264,220.4475588798523,4.895489318677397e-06
23724,189432,189432,378864,221.30826377868652,4.894670240703785e-06
23824,190232,190232,380464,222.19872570037842,4.893854433838033e-06
23924,191032,191032,382064,223.0712399482727,4.893041854262482e-06
24024,191832,191832,383664,223.95579481124878,4.892232459248288e-06
24124,192632,192632,385264,224.77918887138367,4.891426207524228e-06
24224,193432,193432,386864,225.61920475959778,4.89062305875853e-06
24324,194232,194232,388464,226.46440482139587,4.889822973762024e-06
24424,195032,195032,390064,227.29020380973816,4.88902591476898e-06
24525,195840,195840,391680,228.15982484817505,4.8882239186026426e-06
24625,196640,196640,393280,229.01238870620728,4.887432830315789e-06
24725,197440,197440,394880,229.85817885398865,4.886644659212072e-06
24825,198240,198240,396480,230.72473978996277,4.8858593709398355e-06
24925,199040,199040,398080,231.57987189292908,4.885076932184582e-06
25025,199840,199840,399680,232.45204281806946,4.884297310261742e-06
25125,200640,200640,401280,233.4643907546997,4.883520473427146e-06
25225,201440,201440,402880,234.43414187431335,4.882746390446844e-06
25325,202240,202240,404480,235.5612998008728,4.8819750311302345e-06
25425,203040,203040,406080,236.3941798210144,4.881206365401439e-06
25526,203848,203848,407696,237.3497438430786,4.880432717790807e-06
25626,204648,204648,409296,238.19102096557617,4.879669379365874e-06
25726,205448,205448,410896,239.10012078285217,4.87890864907179e-06
25826,206248,206248,412496,239.95978474617004,4.878150499676639e-06
25926,207048,207048,414096,240.79580283164978,4.877394904184224e-06
26026,207848,207848,415696,241.65496683120728,4.87664183694365e-06
26126,208648,208648,417296,242.5050618648529,4.875891271896491e-06
26226,209448,209448,418896,243.37648487091064,4.875143183836067e-06
26326,210248,210248,420496,244.2464439868927,4.87439754818149e-06
26426,211048,211048,422096,245.1106469631195,4.873654340754695e-06
26527,211856,211856,423712,245.99679374694824,4.872906141619082e-06
26627,212656,212656,425312,246.96126985549927,4.8721677430374195e-06
26727,213456,213456,426912,247.80768465995789,4.871431702217687e-06
26827,214256,214256,428512,248.65327262878418,4.870697996449882e-06
26927,215056,215056,430112,249.50585079193115,4.869966603788587e-06
27027,215856,215856,431712,250.34847784042358,4.8692375022141085e-06
27127,216656,216656,433312,251.19623804092407,4.868510670209844e-06
27227,217456,217456,434912,252.06609892845154,4.867786086722743e-06
27327,218256,218256,436512,252.92696595191956,4.867063731033386e-06
27427,219056,219056,438112,253.79932594299316,4.86634358252248e-06
27528,219864,219864,439728,254.66587591171265,4.865618452514604e-06
27628,220664,220664,441328,255.52389979362488,4.8649026800900085e-06
27728,221464,221464,442928,256.39035391807556,4.864189055061051e-06
27828,222264,222264,444528,257.2500698566437,4.863477558393832e-06
27928,223064,223064,446128,258.12548780441284,4.8627681710635504e-06
28028,223864,223864,447728,258.98813104629517,4.86206087405649e-06
28128,224664,224664,449328,259.77605867385864,4.861355649380006e-06
28228,225464,225464,450928,260.52522373199463,4.86065247879821e-06
28328,226264,226264,452528,261.3929898738861,4.8599513439297705e-06
28428,227064,227064,454128,262.2297878265381,4.859252227516353e-06
28529,227872,227872,455744,263.0964767932892,4.858548150552324e-06
28629,228672,228672,457344,263.96510791778564,4.857853038265656e-06
28729,229472,229472,458944,264.83814883232117,4.85715989229644e-06
28829,230272,230272,460544,265.8015468120575,4.8564686957794885e-06
28929,231072,231072,462144,266.72592186927795,4.8557794322898615e-06
29029,231872,231872,463744,267.651154756546,4.855092085696993e-06
29129,232672,232672,465344,268.5532920360565,4.854406639361983e-06
29229,233472,233472,466944,269.5044207572937,4.8537230774488914e-06
29329,234272,234272,468544,270.5796809196472,4.853041384257598e-06
29429,235072,235072,470144,271.42698884010315,4.852361544207562e-06
29530,235880,235880,471760,272.24646973609924,4.851676770874589e-06
29630,236680,236680,473360,273.0845878124237,4.851000608963806e-06
29730,237480,237480,474960,273.9310188293457,4.850326254433214e-06
29830,238280,238280,476560,274.7721838951111,4.84965369204159e-06
29930,239080,239080,478160,275.64069867134094,4.848982907298591e-06
30030,239880,239880,479760,276.5107419490814,4.848313885627249e-06
30130,240680,240680,481360,277.39399695396423,4.847646612664651e-06
30230,241480,241480,482960,278.25378465652466,4.846981074000991e-06
30330,242280,242280,484560,279.1093487739563,4.846317255722349e-06
30430,243080,243080,486160,279.9962718486786,4.845655143855417e-06
30531,243888,243888,487776,280.86738872528076,4.84498812887101e-06
30631,244688,244688,489376,281.756728887558,4.844329405283994e-06
30731,245488,245488,490976,282.604291677475,4.843672347167358e-06
30831,246288,246288,492576,283.4243607521057,4.8430169409837094e-06
30931,247088,247088,494176,284.2591378688812,4.842363173538502e-06
31031,247888,247888,495776,285.07599091529846,4.841711031847414e-06
31131,248688,248688,497376,285.9197928905487,4.841060502887077e-06
31231,249488,249488,498976,286.7690348625183,4.840411573964157e-06
31331,250288,250288,500576,287.63460969924927,4.8397642321744656e-06
31431,251088,251088,502176,288.50277280807495,4.839118465207043e-06
31532,251896,251896,503792,289.3569269180298,4.838467826234232e-06
31632,252696,252696,505392,290.22660279273987,4.837825186795306e-06
31732,253496,253496,506992,291.07087087631226,4.837184085069309e-06
31832,254296,254296,508592,291.922376871109,4.8365445087957174e-06
31932,255096,255096,510192,292.7827777862549,4.835906446201516e-06
32032,255896,255896,511792,293.6375789642334,4.835269885319518e-06
32132,256696,256696,513392,294.52702379226685,4.834634814306966e-06
32232,257496,257496,514992,295.3943347930908,4.834001221924884e-06
32332,258296,258296,516592,296.2365906238556,4.8333690963550625e-06
32432,259096,259096,518192,297.09894585609436,4.832738426052974e-06
32533,259904,259904,519808,297.92349100112915,4.8321029151325255e-06
32633,260702,260702,521404,298.8180968761444,4.604629833097849e-06
32733,261502,261502,523004,299.67667508125305,4.600136419406604e-06
32833,262302,262302,524604,300.5567948818207,4.598995723804767e-06
32933,263102,263102,526204,301.49195075035095,4.59799024382155e-06
33033,263902,263902,527804,302.3635907173157,4.597029172412958e-06
33133,264702,264702,529404,303.28103399276733,4.596095111804067e-06
33233,265502,265502,531004,304.20198702812195,4.595182097446971e-06
33333,266302,266302,532604,305.0831227302551,4.594287307279866e-06
33433,267102,267102,534204,305.93928694725037,4.593409070575173e-06
33534,267910,267910,535820,306.75472378730774,4.592537672199313e-06
33634,268710,268710,537420,307.597305059433,4.59168945930272e-06
33734,269510,269510,539020,308.41223192214966,4.590854978280289e-06
33834,270310,270310,540620,309.2356929779053,4.590033572718997e-06
33934,271110,271110,542220,310.05858993530273,4.589224651523402e-06
34034,271910,271910,543820,310.88651275634766,4.588427672530782e-06
34134,272710,272710,545420,311.75761580467224,4.587642131591869e-06
34234,273510,273510,547020,312.6985809803009,4.586867556622695e-06
34334,274310,274310,548620,313.58072900772095,4.586103502595802e-06
34434,275110,275110,550220,314.4611887931824,4.585349548543548e-06
34535,275918,275918,551836,315.3573157787323,4.5845979001196075e-06
34635,276718,276718,553436,316.23239183425903,4.5838630585919506e-06
34735,277518,277518,555036,317.05743384361267,4.583137172192717e-06
34835,278318,278318,556636,317.8846950531006,4.582419896216173e-06
34935,279118,279118,558236,318.6962339878082,4.581710901786448e-06
35035,279918,279918,559836,319.5149998664856,4.581009874293144e-06
35135,280718,280718,561436,320.33840894699097,4.5803165133171275e-06
35235,281518,281518,563036,321.157292842865,4.579630531523523e-06
35335,282318,282318,564636,321.9951958656311,4.578951654450081e-06
35435,283118,283118,566236,322.8395128250122,4.5782796186758716e-06
35536,283926,283926,567852,323.6903610229492,4.577607550395796e-06
35636,284726,284726,569452,324.55676794052124,4.576948515006481e-06
35736,285526,285526,571052,325.43005895614624,4.576295594823995e-06
35836,286326,286326,572652,326.2960648536682,4.575648568793212e-06
35936,287126,287126,574252,327.15095591545105,4.5750072249533764e-06
36036,287926,287926,575852,328.0015528202057,4.574371360133256e-06
36136,288726,288726,577452,328.8373968601227,4.5737407795328165e-06
36236,289526,289526,579052,329.66507482528687,4.573115296510676e-06
36336,290326,290326,580652,330.4839859008789,4.5724947319996e-06
36436,291126,291126,582252,331.3189299106598,4.571878914236683e-06
36537,291934,291934,583868,332.14726185798645,4.5712615887379586e-06
36637,292734,292734,585468,332.98975467681885,4.57065482034825e-06
36737,293534,293534,587068,333.8265359401703,4.570052322558124e-06
36837,294334,294334,588668,334.661732673645,4.569453950245414e-06
36937,295134,295134,590268,335.51571774482727,4.568859563422218e-06
37037,295934,295934,591868,336.3485789299011,4.568269027976445e-06
37137,296734,296734,593468,337.2322108745575,4.56768221532667e-06
37237,297534,297534,595068,338.102303981781,4.567099001671959e-06
37337,298334,298334,596668,338.95053005218506,4.566519268536585e-06
37437,299134,299134,598268,339.79618096351624,4.565942901704047e-06
37538,299942,299942,599884,340.627445936203,4.565364076659206e-06
37638,300742,300742,601484,341.4716627597809,4.564794149082148e-06
37738,301542,301542,603084,342.3094928264618,4.564227270937175e-06
37838,302342,302342,604684,343.1310279369354,4.563663345093994e-06
37938,303142,303142,606284,343.97211170196533,4.563102278070568e-06
38038,303942,303942,607884,344.79497170448303,4.56254398018525e-06
38138,304742,304742,609484,345.64529395103455,4.561988365077883e-06
38238,305542,305542,611084,346.47989988327026,4.561435349716041e-06
38338,306342,306342,612684,347.31504583358765,4.560884854448118e-06
38438,307142,307142,614284,348.1879677772522,4.560336802368728e-06
38539,307950,307950,615900,349.05001974105835,4.559785674774761e-06
38639,308750,308750,617500,349.83297181129456,4.559242313078218e-06
38739,309550,309550,619100,350.66041898727417,4.558701181016537e-06
38839,310350,310350,620700,351.49822998046875,4.558162212476368e-06
38939,311150,311150,622300,352.38021874427795,4.557625344458531e-06
39039,311950,311950,623900,353.2207820415497,4.557090515972697e-06
39139,312750,312750,625500,354.0847599506378,4.556557668357964e-06
39239,313550,313550,627100,354.9390697479248,4.556026745130521e-06
39339,314350,314350,628700,355.8520188331604,4.555497692130276e-06
39439,315150,315150,630300,356.7360818386078,4.554970456821213e-06
39540,315958,315958,631916,357.642187833786,4.554439743033921e-06
39640,316758,316758,633516,358.53472995758057,4.553916011005039e-06
39740,317558,317558,635116,359.4381899833679,4.553393950338097e-06
39840,318358,318358,636716,360.4898109436035,4.552873516300069e-06
39940,319158,319158,638316,361.3630976676941,4.552354665307639e-06
40040,319958,319958,639916,362.2273428440094,4.5518373554659675e-06
40140,320758,320758,641516,363.0611128807068,4.5513215464001764e-06
40240,321558,321558,643116,363.873242855072,4.55080719921714e-06
40340,322358,322358,644716,364.7028238773346,4.550294276369271e-06
40440,323158,323158,646316,365.5385158061981,4.54978274179864e-06
40541,323966,323966,647932,366.36861276626587,4.549267465265683e-06
40641,324766,324766,649532,367.22014689445496,4.548758616499264e-06
40741,325566,325566,651132,368.0564568042755,4.5482510545093114e-06
40841,326366,326366,652732,368.9077949523926,4.547744747803345e-06
40941,327166,327166,654332,369.75778889656067,4.54723966626595e-06
41041,327966,327966,655932,370.6086540222168,4.5467357806738975e-06
41141,328766,328766,657532,371.4674518108368,4.546233062714463e-06
41241,329566,329566,659132,372.3226318359375,4.545731485207718e-06
41341,330366,330366,660732,373.1804118156433,4.545231021870882e-06
41441,331166,331166,662332,374.0215017795563,4.544731647151984e-06
41542,331974,331974,663948,374.84240889549255,4.5442283589715e-06
41642,332774,332774,665548,375.67625188827515,4.543731099118786e-06
41742,333574,333574,667148,376.49810671806335,4.5432348566189585e-06
41842,334374,334374,668748,377.31036901474,4.5427396090496e-06
41942,335174,335174,670348,378.1477608680725,4.542245335391556e-06
42042,335974,335974,671948,378.98577976226807,4.541752014398165e-06
42142,336774,336774,673548,379.85609579086304,4.541259626222222e-06
42242,337574,337574,675148,380.71719694137573,4.540768151683778e-06
42342,338374,338374,676748,381.5789318084717,4.540277571861651e-06
42442,339174,339174,678348,382.46274304389954,4.539787868449689e-06
42543,339982,339982,679964,383.33225178718567,4.539294139877735e-06
42643,340782,340782,681564,384.2068946361542,4.538806145685264e-06
42743,341582,341582,683164,385.025554895401,4.538318976774654e-06
42843,342382,342382,684764,385.84014987945557,4.537832617328752e-06
42943,343182,343182,686364,386.6870319843292,4.53734705160405e-06
43043,343982,343982,687964,387.53700590133667,4.536862264731915e-06
43143,344782,344782,689564,388.39708375930786,4.5363782423431245e-06
43243,345582,345582,691164,389.22591185569763,4.535894970212356e-06
43343,346382,346382,692764,390.07443499565125,4.535412434593025e-06
43443,347182,347182,694364,390.9308090209961,4.534930622547914e-06
43544,347990,347990,695980,391.7805030345917,4.534444713558768e-06
43644,348790,348790,697580,392.6474578380585,4.5339643170998035e-06
43744,349590,349590,699180,393.4966628551483,4.533484606584482e-06
43844,350390,350390,700780,394.3668968677521,4.533005570160431e-06
43944,351190,351190,702380,395.23564887046814,4.532527196600475e-06
44044,351990,351990,703980,396.0571939945221,4.5320494746626894e-06
44144,352790,352790,705580,396.90811800956726,4.5315723940323325e-06
44244,353590,353590,707180,397.7412328720093,4.531095943725527e-06
44344,354390,354390,708780,398.5853097438812,4.530620114090053e-06
44444,355190,355190,710380,399.4412217140198,4.5301448948582016e-06
44545,355998,355998,711996,400.2950849533081,4.529665533662585e-06
44645,356798,356798,713596,401.1493937969208,4.529191513137263e-06
44745,357598,357598,715196,401.9968638420105,4.528718075395577e-06
44845,358398,358398,716796,402.8418688774109,4.528245211329192e-06
44945,359198,359198,718396,403.72151279449463,4.527772912432723e-06
45045,359998,359998,719996,404.5745527744293,4.52730117057756e-06
45145,360798,360798,721596,405.44981598854065,4.52682997727656e-06
45245,361598,361598,723196,406.3095679283142,4.526359324958034e-06
45345,362398,362398,724796,407.16922998428345,4.52588920584027e-06
45445,363198,363198,726396,408.00772285461426,4.52541961235316e-06
45546,364006,364006,728012,408.83425283432007,4.524945849087261e-06
45646,364806,364806,729612,409.67748403549194,4.524477290261283e-06
45746,365606,365606,731212,410.52584171295166,4.5240092356034084e-06
45846,366406,366406,732812,411.35876870155334,4.5235416785357625e-06
45946,367206,367206,734412,412.20716166496277,4.523074612339908e-06
46046,368006,368006,736012,413.07431292533875,4.522608030567709e-06
46146,368806,368806,737612,413.9371078014374,4.5221419268933725e-06
46246,369606,369606,739212,414.7819848060608,4.521676295078724e-06
46346,370406,370406,740812,415.62191891670227,4.521211129534075e-06
46446,371206,371206,742412,416.4683289527893,4.52074642407511e-06
46547,372014,372014,744028,417.3904798030853,4.520277532753709e-06
46647,372814,372814,745628,418.19849276542664,4.519813735035613e-06
46747,373614,373614,747228,419.0173718929291,4.519350380793215e-06
46847,374414,374414,748828,419.9220037460327,4.518887464482064e-06
46947,375214,375214,750428,420.74579882621765,4.51842498115821e-06
47047,376014,376014,752028,421.6141617298126,4.517962925485357e-06
47147,376814,376814,753628,422.57165575027466,4.517501292560722e-06
47247,377614,377614,755228,423.3883128166199,4.517040077442627e-06
47347,378414,378414,756828,424.2993037700653,4.516579275538917e-06
47447,379214,379214,758428,425.1042637825012,4.516118882064248e-06
47548,380022,380022,760044,425.83719182014465,4.51565429453464e-06
47648,380822,380822,761644,426.69406270980835,4.515194708315209e-06
47748,381622,381622,763244,427.41465067863464,4.514735516961886e-06
47848,382422,382422,764844,428.09939670562744,4.514276716357121e-06
47948,383222,383222,766444,428.78592681884766,4.513818302267018e-06
48048,384022,384022,768044,429.4677770137787,4.513360270517133e-06
48148,384822,384822,769644,430.1439788341522,4.512902616914464e-06
48248,385622,385622,771244,430.82603788375854,4.512445337807345e-06
48348,386422,386422,772844,431.49393582344055,4.511988429012249e-06
48448,387222,387222,774444,432.17587876319885,4.5115318870023404e-06
48549,388030,388030,776060,432.86178183555603,4.511071147794614e-06
48649,388830,388830,777660,433.54260301589966,4.5106153314006604e-06
48749,389630,389630,779260,434.21233892440796,4.510159870537256e-06
48849,390430,390430,780860,434.88283681869507,4.509704761707304e-06
48949,391230,391230,782460,435.56576466560364,4.50925000149336e-06
49049,392030,392030,784060,436.2403109073639,4.5087955863804175e-06
49149,392830,392830,785660,436.91282391548157,4.5083415130721365e-06
49249,393628,393628,787256,437.60137271881104,4.2811613440091574e-06
49349,394428,394428,788856,438.26620388031006,4.279149905351285e-06
49449,395228,395228,790456,438.9322507381439,4.278267991906017e-06
49550,396036,396036,792072,439.62207794189453,4.277519405663049e-06
49650,396836,396836,793672,440.28833293914795,4.276827588954259e-06
49750,397636,397636,795272,440.9682049751282,4.276162249322784e-06
49850,398436,398436,796872,441.65726590156555,4.275514965707856e-06
49950,399236,399236,798472,442.3254859447479,4.274881706666361e-06
50050,400036,400036,800072,442.9983060359955,4.274260203280592e-06
50150,400836,400836,801672,443.70089173316956,4.273649020894579e-06
50250,401636,401636,803272,444.3693606853485,4.273047168815719e-06
50350,402436,402436,804872,445.0388159751892,4.272453911465919e-06
50450,403236,403236,806472,445.71952295303345,4.271868670512469e-06
50551,404044,404044,808088,446.39727878570557,4.271285229989237e-06
50651,404844,404844,809688,447.0629949569702,4.270714733140953e-06
50751,405644,405644,811288,447.7454209327698,4.270151009671269e-06
50851,406444,406444,812888,448.4210548400879,4.269593739421163e-06
50951,407244,407244,814488,449.09549379348755,4.269042629839699e-06
51051,408044,408044,816088,449.7794077396393,4.268497410972689e-06
51151,408840,408840,817680,450.44807171821594,3.8296867042511715e-06
51251,409638,409638,819276,451.12031292915344,3.594426338129996e-06
51351,410438,410438,820876,451.8029806613922,3.5400606683056335e-06
51451,411238,411238,822476,452.4754078388214,3.4962482928613617e-06
51552,412046,412046,824092,453.1487259864807,3.4593219659608056e-06
51652,412846,412846,825692,453.81065797805786,3.428055334031666e-06
51752,413646,413646,827292,454.4929008483887,3.4007800747659677e-06
51852,414446,414446,828892,455.15683674812317,3.3766250114890736e-06
51952,415246,415246,830492,455.82266902923584,3.3549720768525768e-06
52052,416046,416046,832092,456.50462889671326,3.335369500092996e-06
52152,416846,416846,833692,457.1861927509308,3.317478200766124e-06
52252,417646,417646,835292,457.8527789115906,3.3010376297035518e-06
52352,418446,418446,836892,458.5350978374481,3.285843392858299e-06
52452,419246,419246,838492,459.20307874679565,3.271732211555962e-06
52553,420054,420054,840108,459.87815380096436,3.2584443747405506e-06
52653,420854,420854,841708,460.572518825531,3.246133138568061e-06
52753,421654,421654,843308,461.2467758655548,3.234571703561925e-06
52853,422454,422454,844908,461.9201228618622,3.223683699355742e-06
52953,423254,423254,846508,462.6046619415283,3.2134041934287082e-06
53053,424054,424054,848108,463.2747230529785,3.203677498013672e-06
53153,424854,424854,849708,463.94705295562744,3.1944554787905707e-06
53253,425654,425654,851308,464.6268730163574,3.1856962281394353e-06
53353,426454,426454,852908,465.2961657047272,3.177363015772136e-06
53453,427254,427254,854508,465.969518661499,3.1694234475433375e-06
53554,428062,428062,856124,466.6589608192444,3.1617747942098056e-06
53654,428862,428862,857724,467.3267467021942,3.15454268305767e-06
53754,429662,429662,859324,468.010470867157,3.1476266510940117e-06
53854,430462,430462,860924,468.69107484817505,3.141006018186456e-06
53954,431262,431262,862524,469.35880279541016,3.1346620686029022e-06
54054,432062,432062,864124,470.02805495262146,3.128577792921577e-06
54154,432862,432862,865724,470.707722902298,3.1227376717756032e-06
54254,433662,433662,867324,471.37081599235535,3.1171274923839448e-06
54354,434462,434462,868924,472.04375171661377,3.1117341942388632e-06
54454,435262,435262,870524,472.7148768901825,3.106545738264017e-06
54555,436070,436070,872140,473.4052426815033,3.10150198951808e-06
54655,436870,436870,873740,474.07576179504395,3.096692423690446e-06
54755,437670,437670,875340,474.7402718067169,3.0920565710570304e-06
54855,438470,438470,876940,475.42448377609253,3.0875855075343113e-06
54955,439270,439270,878540,476.09077763557434,3.0832709038194283e-06
55055,440070,440070,880140,476.7721858024597,3.0791049711801535e-06
55155,440870,440870,881740,477.46339082717896,3.0750804141059163e-06
55255,441670,441670,883340,478.13604402542114,3.0711903879618465e-06
55355,442470,442470,884940,478.8070378303528,3.0674284619536607e-06
55455,443270,443270,886540,479.4933376312256,3.063788585996164e-06
55556,444078,444078,888156,480.1699357032776,3.060230395912923e-06
55656,444878,444878,889756,480.8388600349426,3.0568189344217648e-06
55756,445678,445678,891356,481.5193657875061,3.0535133313634625e-06
55856,446478,446478,892956,482.18526887893677,3.0503087978621714e-06
55956,447278,447278,894556,482.8539698123932,3.0472008067919614e-06
56056,448078,448078,896156,483.5408387184143,3.044185073557163e-06
56156,448878,448878,897756,484.21158480644226,3.0412575413533305e-06
56256,449678,449678,899356,484.87315678596497,3.0384143657726303e-06
56356,450478,450478,900956,485.5613868236542,3.0356519018993244e-06
56456,451278,451278,902556,486.22636103630066,3.0329666918226397e-06
56557,452086,452086,904172,486.91212797164917,3.0303297036470373e-06
56657,452886,452886,905772,487.60012102127075,3.0277900125222558e-06
56757,453686,453686,907372,488.28559279441833,3.025318185206183e-06
56857,454486,454486,908972,488.95743894577026,3.02291140759902e-06
56957,455286,455286,910572,489.6366708278656,3.0205670040805893e-06
57057,456086,456086,912172,490.3051257133484,3.0182824288827885e-06
57157,456886,456886,913772,490.9790768623352,3.0160552594641874e-06
57257,457686,457686,915372,491.6585199832916,3.013883189110839e-06
57357,458486,458486,916972,492.34930396080017,3.0117640211152345e-06
57457,459286,459286,918572,493.0219178199768,3.009695662729058e-06
57558,460094,460094,920188,493.7238540649414,3.0076561639078337e-06
57658,460894,460894,921788,494.40843892097473,3.005683993832743e-06
57758,461694,461694,923388,495.09333395957947,3.003756906387314e-06
57858,462494,462494,924988,495.76148676872253,3.0018731726158045e-06
57958,463294,463294,926588,496.4451148509979,3.00003114289077e-06
58058,464094,464094,928188,497.11572885513306,2.998229242748675e-06
58158,464894,464894,929788,497.7797968387604,2.996465968691238e-06
58258,465694,465694,931388,498.47498178482056,2.994739885189447e-06
58358,466494,466494,932988,499.1389207839966,2.993049620767382e-06
58458,467294,467294,934588,499.80557894706726,2.991393865316744e-06
58559,468102,468102,936204,500.5006399154663,2.9897553051065526e-06
58659,468902,468902,937804,501.1678977012634,2.988165179810929e-06
58759,469702,469702,939404,501.8319869041443,2.986605957584267e-06
58859,470502,470502,941004,502.5187876224518,2.985076543775712e-06
58959,471302,471302,942604,503.186648607254,2.9835758910367955e-06
59059,472102,472102,944204,503.85169887542725,2.9821029971465337e-06
59159,472902,472902,945804,504.54421281814575,2.980656902952329e-06
59259,473702,473702,947404,505.21136569976807,2.979236689973586e-06
59359,474502,474502,949004,505.8802638053894,2.9778414785071957e-06
59459,475302,475302,950604,506.56580877304077,2.9764704259930004e-06
59560,476110,476110,952220,507.31065583229065,2.9751093633191848e-06
59660,476910,476910,953820,507.99156403541565,2.9737844625574785e-06
59760,477710,477710,955420,508.67243480682373,2.9724813908355116e-06
59860,478510,478510,957020,509.339017868042,2.9711994373042187e-06
59960,479310,479310,958620,510.02536964416504,2.969937920523273e-06
60060,480110,480110,960220,510.7052619457245,2.9686961863873088e-06
60160,480910,480910,961820,511.3688817024231,2.9674736075422786e-06
60260,481710,481710,963420,512.0385589599609,2.9662695821089224e-06
60360,482510,482510,965020,512.7590148448944,2.965083531695628e-06
60460,483310,483310,966620,513.4714798927307,2.9639149017198834e-06
60561,484118,484118,968236,514.2134399414062,2.962751725059652e-06
60661,484918,484918,969836,514.9803018569946,2.9616165189122123e-06
60761,485718,485718,971436,515.7646749019623,2.96049719136962e-06
60861,486518,486518,973036,516.5173900127411,2.9593932700832103e-06
60961,487318,487318,974636,517.3245558738708,2.958304300782077e-06
61061,488118,488118,976236,518.0714728832245,2.957229846753192e-06
61161,488918,488918,977836,518.810311794281,2.956169487886017e-06
61261,489718,489718,979436,519.5679898262024,2.9551228206443893e-06
61361,490518,490518,981036,520.2526657581329,2.9540894559243118e-06
61461,491318,491318,982636,520.9511768817902,2.953069020197556e-06
61562,492126,492126,984252,521.6486468315125,2.952051136827488e-06
61662,492926,492926,985852,522.4032158851624,2.9510556125353734e-06
61762,493726,493726,987452,523.1403987407684,2.95007197362184e-06
61862,494526,494526,989052,523.8690679073334,2.9490998986244802e-06
61962,495326,495326,990652,524.6602597236633,2.9481390780948523e-06
62062,496126,496126,992252,525.516964673996,2.947189213597877e-06
62162,496926,496926,993852,526.2331328392029,2.946250017843603e-06
62262,497726,497726,995452,526.9244518280029,2.945321213603686e-06
62362,498526,498526,997052,527.6266407966614,2.944402533601126e-06
62462,499326,499326,998652,528.3122689723969,2.9434937200268073e-06
62563,500134,500134,1000268,529.0055060386658,2.942585580497354e-06
62663,500934,500934,1001868,529.697723865509,2.9416958555402648e-06
62763,501734,501734,1003468,530.3712570667267,2.9408152748852574e-06
62863,502534,502534,1005068,531.046238899231,2.9399436150952077e-06
62963,503334,503334,1006668,531.7250118255615,2.9390806602068955e-06
63063,504134,504134,1008268,532.4059519767761,2.938226202123167e-06
63163,504934,504934,1009868,533.0853607654572,2.9373800398117144e-06
63263,505734,505734,1011468,533.7651238441467,2.9365419784550657e-06
63363,506534,506534,1013068,534.4495129585266,2.9357118303654914e-06
63463,507334,507334,1014668,535.1362369060516,2.934889413792746e-06
63564,508142,508142,1016284,535.8077807426453,2.934066442312875e-06
63664,508942,508942,1017884,536.5007197856903,2.9332590410282095e-06
63764,509742,509742,1019484,537.1723036766052,2.9324588599722797e-06
63864,510542,510542,1021084,537.8418936729431,2.9316657405452123e-06
63964,511342,511342,1022684,538.5348908901215,2.9308795289117798e-06
64064,512142,512142,1024284,539.2033967971802,2.9301000762843337e-06
64164,512942,512942,1025884,539.8869078159332,2.929327238592095e-06
64264,513742,513742,1027484,540.6350839138031,2.928560876409481e-06
64364,514542,514542,1029084,541.3351306915283,2.927800854649138e-06
64464,515342,515342,1030684,542.0370597839355,2.9270470422338568e-06
64565,516150,516150,1032300,542.7601778507233,2.9262918656652888e-06
64665,516950,516950,1033900,543.4439578056335,2.92555015492639e-06
64765,517750,517750,1035500,544.1430988311768,2.9248142836554267e-06
64865,518550,518550,1037100,544.9131319522858,2.924084136143028e-06
64965,519350,519350,1038700,545.6813716888428,2.9233596006910872e-06
65065,520150,520150,1040300,546.3615937232971,2.9226405685864254e-06
65165,520950,520950,1041900,547.2141468524933,2.9219269343045795e-06
65265,521750,521750,1043500,548.0584697723389,2.9212185952195724e-06
65365,522550,522550,1045100,548.9060096740723,2.9205154524925916e-06
65465,523350,523350,1046700,549.6302709579468,2.919817409361015e-06
65566,524158,524158,1048316,550.4923257827759,2.9191174669293076e-06
65666,524958,524958,1049916,551.2982437610626,2.918429393469752e-06
65766,525758,525758,1051516,552.0069680213928,2.91774614568516e-06
65866,526558,526558,1053116,552.6878399848938,2.9170676378018503e-06
65966,527358,527358,1054716,553.4771230220795,2.9163937860604526e-06
66066,528158,528158,1056316,554.4352607727051,2.9157245093946404e-06
66166,528958,528958,1057916,555.1487908363342,2.9150597288120766e-06
66266,529758,529758,1059516,555.8469569683075,2.914399367587968e-06
66366,530558,530558,1061116,556.5233888626099,2.913743350928279e-06
66466,531358,531358,1062716,557.2139177322388,2.913091606074145e-06
66567,532166,532166,1064332,557.9248998165131,2.9124376076917646e-06
66667,532966,532966,1065932,558.6539378166199,2.9117942369550335e-06
66767,533766,533766,1067532,559.3536858558655,2.9111549304722505e-06
66867,534566,534566,1069132,560.1714890003204,2.9105196229565096e-06
66967,535366,535366,1070732,561.0698747634888,2.9098882507583323e-06
67067,536166,536166,1072332,561.7897357940674,2.9092607517101413e-06
67167,536966,536966,1073932,562.6272509098053,2.9086370653503617e-06
67267,537766,537766,1075532,563.5146877765656,2.908017132708817e-06
67367,538566,538566,1077132,564.199296951294,2.9074008964337946e-06
67467,539366,539366,1078732,564.9133598804474,2.9067883002566414e-06
67568,540174,540174,1080348,565.7529017925262,2.906173217266398e-06
67668,540974,540974,1081948,566.6313889026642,2.90556777355081e-06
67768,541774,541774,1083548,567.3412709236145,2.9049658093251557e-06
67868,542574,542574,1085148,568.1627378463745,2.9043672734759396e-06
67968,543374,543374,1086748,568.8508908748627,2.9037721166996506e-06
68068,544174,544174,1088348,569.7204208374023,2.9031802901989522e-06
68168,544974,544974,1089948,570.5598359107971,2.9025917468035987e-06
68268,545774,545774,1091548,571.478414773941,2.902006439960015e-06
68368,546574,546574,1093148,572.2174227237701,2.9014243247184597e-06
68468,547374,547374,1094748,572.9942028522491,2.900845356684095e-06
68569,548182,548182,1096364,573.7513718605042,2.9002637495677396e-06
68669,548982,548982,1097964,574.4517149925232,2.8996909776024024e-06
68769,549782,549782,1099564,575.2334866523743,2.8991212258834847e-06
68869,550582,550582,1101164,575.9715728759766,2.8985544534478898e-06
68969,551382,551382,1102764,576.7608449459076,2.897990621001346e-06
69069,552182,552182,1104364,577.4762270450592,2.8974296899253598e-06
69169,552982,552982,1105964,578.4549028873444,2.89687162215954e-06
69269,553782,553782,1107564,579.2529747486115,2.896316380457682e-06
69369,554582,554582,1109164,579.997181892395,2.895763928836362e-06
69469,555382,555382,1110764,580.7337188720703,2.89521423124002e-06
69570,556190,556190,1112380,581.5034277439117,2.8946617969840946e-06
69670,556990,556990,1113980,582.218181848526,2.8941175307301477e-06
69770,557790,557790,1115580,582.9819986820221,2.89357591587038e-06
69870,558590,558590,1117180,583.7158398628235,2.8930369194781428e-06
69970,559390,559390,1118780,584.490984916687,2.8925005095248943e-06
70070,560190,560190,1120380,585.2173597812653,2.8919666544727722e-06
70170,560990,560990,1121980,585.9113199710846,2.891435323148363e-06
70270,561790,561790,1123580,586.8215680122375,2.890906485282822e-06
70370,562590,562590,1125180,587.5543489456177,2.8903801111814377e-06
70470,563390,563390,1126780,588.2777190208435,2.889856171578342e-06
70571,564198,564198,1128396,588.9853386878967,2.889329434441934e-06
70671,564998,564998,1129996,589.6625978946686,2.8888103018158572e-06
70771,565798,565798,1131596,590.3398289680481,2.8882935188326295e-06
70871,566598,566598,1133196,591.0995230674744,2.887779058558327e-06
70971,567398,567398,1134796,591.8450269699097,2.8872668939943078e-06
71071,568198,568198,1136396,592.60537981987,2.8867569992831195e-06
71171,568998,568998,1137996,593.4254767894745,2.886249348357193e-06
71271,569798,569798,1139596,594.2983357906342,2.8857439159902005e-06
71371,570598,570598,1141196,595.2593579292297,2.8852406776476782e-06
71471,571398,571398,1142796,596.1781418323517,2.8847396085589496e-06
71572,572206,572206,1144412,596.9398949146271,2.884235706267738e-06
71672,573006,573006,1146012,597.6548488140106,2.883738925441429e-06
71772,573806,573806,1147612,598.3639197349548,2.8832442428053864e-06
71872,574606,574606,1149212,599.0947878360748,2.8827516355318564e-06
71972,575406,575406,1150812,599.853385925293,2.8822610811801873e-06
72072,576206,576206,1152412,600.6041898727417,2.88177255780339e-06
72172,577006,577006,1154012,601.3446877002716,2.881286043493232e-06
72272,577806,577806,1155612,602.2446010112762,2.8808015168742723e-06
72372,578606,578606,1157212,603.0779666900635,2.8803189568551275e-06
72472,579406,579406,1158812,603.881020784378,2.879838342624194e-06
72573,580214,580214,1160428,604.6405317783356,2.8793548766974055e-06
72673,581014,581014,1162028,605.3827557563782,2.8788781123840116e-06
72773,581814,581814,1163628,606.222339630127,2.8784032332004224e-06
72873,582614,582614,1165228,606.9742619991302,2.8779302200295254e-06
72973,583414,583414,1166828,607.7180557250977,2.877459053312639e-06
73073,584214,584214,1168428,608.4433326721191,2.876989714421222e-06
73173,585014,585014,1170028,609.1324830055237,2.8765221844264746e-06
73273,585814,585814,1171628,609.8438897132874,2.8760564452214853e-06
73373,586614,586614,1173228,610.6410918235779,2.8755924783199295e-06
73473,587414,587414,1174828,611.4380300045013,2.875130266299295e-06
73574,588222,588222,1176444,612.1531980037689,2.874665195384081e-06
73674,589022,589022,1178044,612.8449399471283,2.8742064571913053e-06
73774,589822,589822,1179644,613.557461977005,2.8737494215904376e-06
73874,590622,590622,1181244,614.2450108528137,2.8732940715233087e-06
73974,591422,591422,1182844,615.0319197177887,2.8728403903480505e-06
74074,592222,592222,1184444,615.7361488342285,2.8723883618085965e-06
74174,593022,593022,1186044,616.5306589603424,2.8719379694967657e-06
74274,593822,593822,1187644,617.5640408992767,2.8714891975613406e-06
74374,594622,594622,1189244,618.7295069694519,2.8710420303725093e-06
74474,595422,595422,1190844,619.6775989532471,2.8705964519866795e-06
74575,596230,596230,1192460,620.4913237094879,2.8701480154403196e-06
74675,597030,597030,1194060,621.2748956680298,2.8697055851213536e-06
74775,597830,597830,1195660,622.0670049190521,2.8692646981434317e-06
74875,598630,598630,1197260,622.8427209854126,2.868825340046429e-06
74975,599430,599430,1198860,623.6071479320526,2.8683874959933058e-06
75075,600230,600230,1200460,624.3430438041687,2.867951151838202e-06
75175,601030,601030,1202060,625.1543617248535,2.8675162932444827e-06
75275,601830,601830,1203660,625.9554669857025,2.867082906236852e-06
75375,602630,602630,1205260,626.6909687519073,2.866650977014385e-06
75475,603430,603430,1206860,627.4162917137146,2.8662204918888074e-06
75576,604238,604238,1208476,628.1211929321289,2.865787153793261e-06
75676,605038,605038,1210076,628.8096780776978,2.865359530628952e-06
75776,605838,605838,1211676,629.5241379737854,2.8649333112457506e-06
75876,606638,606638,1213276,630.2510018348694,2.8645084827177676e-06
75976,607438,607438,1214876,630.9990079402924,2.864085032424788e-06
76076,608238,608238,1216476,631.8362927436829,2.863662947290726e-06
76176,609038,609038,1218076,632.6128067970276,2.8632422149361798e-06
76276,609838,609838,1219676,633.4355597496033,2.862822823182281e-06
76376,610638,610638,1221276,634.2152497768402,2.86240475939841e-06
76476,611438,611438,1222876,634.9518840312958,2.861988011517387e-06
76577,612246,612246,1224492,635.7265667915344,2.8615684199980443e-06
76677,613046,613046,1226092,636.5504078865051,2.8611542812141984e-06
76777,613846,613846,1227692,637.5144996643066,2.8607414229509894e-06
76877,614646,614646,1229292,638.3691809177399,2.8603298333983283e-06
76977,615446,615446,1230892,639.1147499084473,2.859919501170031e-06
77077,616246,616246,1232492,639.8638348579407,2.859510414876835e-06
77177,617046,617046,1234092,640.5867550373077,2.859102563674912e-06
77277,617846,617846,1235692,641.3439748287201,2.8586959362073663e-06
77377,618646,618646,1237292,642.0746438503265,2.858290521499398e-06
77477,619446,619446,1238892,642.8280267715454,2.857886308848064e-06
77578,620254,620254,1240508,643.6258747577667,2.8574792633967367e-06
77678,621054,621054,1242108,644.3396427631378,2.857077434611679e-06
77778,621854,621854,1243708,645.0668389797211,2.8566767760787513e-06
77878,622654,622654,1245308,645.7955567836761,2.8562772774391283e-06
77978,623454,623454,1246908,646.5009078979492,2.855878928424108e-06
78078,624254,624254,1248508,647.267648935318,2.855481718828137e-06
78178,625054,625054,1250108,648.0180258750916,2.8550856388486374e-06
78278,625854,625854,1251708,648.9096350669861,2.854690678352222e-06
78378,626654,626654,1253308,649.6533010005951,2.854296827619749e-06
78478,627454,627454,1254908,650.4377799034119,2.853904076888813e-06
78579,628262,628262,1256524,651.1730690002441,2.8535085054752085e-06
78679,629062,629062,1258124,651.9188787937164,2.8531179369388997e-06
78779,629862,629862,1259724,652.6656997203827,2.8527284399116782e-06
78879,630662,630662,1261324,653.4400587081909,2.8523400050405004e-06
78979,631462,631462,1262924,654.165168762207,2.8519526230481265e-06
79079,632262,632262,1264524,654.9542577266693,2.851566284954542e-06
79179,633062,633062,1266124,655.6902267932892,2.8511809816865446e-06
79279,633862,633862,1267724,656.4171948432922,2.8507967042330423e-06
79379,634662,634662,1269324,657.1575307846069,2.850413443895712e-06
79479,635462,635462,1270924,657.9115138053894,2.850031191863992e-06
79580,636270,636270,1272540,658.7540168762207,2.849646131973673e-06
79680,637070,637070,1274140,659.4741020202637,2.8492658805666505e-06
79780,637870,637870,1275740,660.1773548126221,2.8488866117992126e-06
79880,638670,638670,1277340,660.9110310077667,2.84850831701559e-06
79980,639470,639470,1278940,661.6395697593689,2.8481309880313585e-06
80080,640270,640270,1280540,662.3733539581299,2.8477546167321712e-06
80180,641070,641070,1282140,663.1838278770447,2.84737919494369e-06
80280,641870,641870,1283740,663.9272239208221,2.8470047142951295e-06
80380,642670,642670,1285340,664.650224685669,2.8466311672393983e-06
80480,643470,643470,1286940,665.3621068000793,2.846258545607762e-06
80581,644278,644278,1288556,666.0661797523499,2.8458831291162136e-06
80681,645078,645078,1290156,666.8592779636383,2.845512344127753e-06
80781,645878,645878,1291756,667.5980107784271,2.8451424611563655e-06
80881,646678,646678,1293356,668.2852838039398,2.8447734727909193e-06
80981,647478,647478,1294956,669.0046818256378,2.844405371390117e-06
81081,648278,648278,1296556,669.6934509277344,2.84403814948359e-06
81181,649078,649078,1298156,670.4012138843536,2.8436717998762537e-06
81281,649878,649878,1299756,671.137776851654,2.843306314962009e-06
81381,650678,650678,1301356,671.8618927001953,2.842941687812606e-06
81481,651478,651478,1302956,672.5801410675049,2.842577911025031e-06
81582,652286,652286,1304572,673.3494489192963,2.8422113524603126e-06
81682,653086,653086,1306172,674.0840308666229,2.8418492636808655e-06
81782,653886,653886,1307772,674.7926859855652,2.8414880039348673e-06
81882,654686,654686,1309372,675.5370209217072,2.8411275667399744e-06
81982,655486,655486,1310972,676.2552587985992,2.840767945013052e-06
82082,656286,656286,1312572,676.9734647274017,2.8404091319954134e-06
82182,657086,657086,1314172,677.7308838367462,2.8400511209472664e-06
82282,657882,657882,1315764,678.4827938079834,2.6696365363294956e-06
82382,658682,658682,1317364,679.2169289588928,2.5053501642031878e-06
82482,659482,659482,1318964,679.9618747234344,2.502927881588802e-06
82583,660290,660290,1320580,680.6927769184113,2.501557135865115e-06
82683,661090,661090,1322180,681.4285619258881,2.500449358946527e-06
82783,661890,661890,1323780,682.1464729309082,2.4994471985923827e-06
82883,662690,662690,1325380,682.8791396617889,2.4985050556157355e-06
82983,663490,663490,1326980,683.5722508430481,2.4976037579784827e-06
83083,664290,664290,1328580,684.3574566841125,2.496733766361495e-06
83183,665090,665090,1330180,685.1130838394165,2.4958897111035144e-06
83283,665890,665890,1331780,685.8449966907501,2.4950682642161413e-06
83383,666690,666690,1333380,686.5869796276093,2.494267194377935e-06
83483,667490,667490,1334980,687.6244609355927,2.4934849004726865e-06
83584,668298,668298,1336596,688.4793207645416,2.4927126028031258e-06
83684,669098,669098,1338196,689.2053937911987,2.491964614230565e-06
83784,669898,669898,1339796,690.1056838035583,2.49123239189559e-06
83884,670698,670698,1341396,690.9097199440002,2.490515237158229e-06
83984,671498,671498,1342996,691.6665599346161,2.4898125308593876e-06
84084,672298,672298,1344596,692.6850717067719,2.4891237127763426e-06
84184,673098,673098,1346196,693.6342687606812,2.4884482682441877e-06
84284,673898,673898,1347796,694.3967819213867,2.487785719215878e-06
84384,674698,674698,1349396,695.2548108100891,2.487135616452342e-06
84484,675498,675498,1350996,696.0147678852081,2.486497536644431e-06
84585,676306,676306,1352612,696.7610607147217,2.4858648702828104e-06
84685,677106,677106,1354212,697.7124118804932,2.485249759460896e-06
84785,677906,677906,1355812,698.7723438739777,2.4846455168004023e-06
84885,678706,678706,1357412,699.8133509159088,2.484051792003605e-06
84985,679506,679506,1359012,700.824052810669,2.48346824883876e-06
85085,680306,680306,1360612,701.5957727432251,2.4828945645140907e-06
85185,681106,681106,1362212,702.402126789093,2.4823304282461234e-06
85285,681906,681906,1363812,703.1939718723297,2.4817755410413613e-06
85385,682706,682706,1365412,703.9404196739197,2.481229614628232e-06
85485,683506,683506,1367012,704.9779489040375,2.4806923713410694e-06
85586,684314,684314,1368628,706.0195198059082,2.4801582960285153e-06
85686,685114,685114,1370228,706.8577568531036,2.4796377037050406e-06
85786,685914,685914,1371828,707.6713428497314,2.4791250153054506e-06
85886,686714,686714,1373428,708.4431507587433,2.478619989729279e-06
85986,687514,687514,1375028,709.3725697994232,2.4781223934338455e-06
86086,688314,688314,1376628,710.4430248737335,2.477632001610339e-06
86186,689114,689114,1378228,711.4967248439789,2.477148596284174e-06
86286,689914,689914,1379828,712.4419617652893,2.476671967280305e-06
86386,690714,690714,1381428,713.4205968379974,2.476201910971237e-06
86486,691514,691514,1383028,714.2103910446167,2.4757382305087198e-06
86587,692322,692322,1384644,714.9909288883209,2.4752761911365823e-06
86687,693122,693122,1386244,715.748851776123,2.4748247564322964e-06
86787,693922,693922,1387844,716.5121939182281,2.4743791430714254e-06
86887,694722,694722,1389444,717.2908279895782,2.4739391787733442e-06
86987,695522,695522,1391044,718.074914932251,2.4735046964764097e-06
87087,696322,696322,1392644,718.7930917739868,2.47307553489816e-06
87187,697122,697122,1394244,719.5193059444427,2.472651537676676e-06
87287,697922,697922,1395844,720.3069477081299,2.4722325537229206e-06
87387,698722,698722,1397444,721.1342678070068,2.4718184361451795e-06
87487,699522,699522,1399044,721.8933317661285,2.471409043791398e-06
87588,700330,700330,1400660,722.611958026886,2.471000213556827e-06
87688,701130,701130,1402260,723.5188558101654,2.470599907176825e-06
87788,701930,701930,1403860,724.4162828922272,2.470203925344366e-06
87888,702730,702730,1405460,725.2061839103699,2.4698121435975124e-06
87988,703530,703530,1407060,725.8963928222656,2.469424441190212e-06
88088,704330,704330,1408660,726.6152029037476,2.4690407009374874e-06
88188,705130,705130,1410260,727.3274717330933,2.468660809705565e-06
88288,705930,705930,1411860,728.0054528713226,2.4682846579052773e-06
88388,706730,706730,1413460,728.8870198726654,2.4679121390404405e-06
88488,707530,707530,1415060,729.6742236614227,2.467543150124458e-06
88589,708338,708338,1416676,730.4026718139648,2.467173952767229e-06
88689,709138,709138,1418276,731.1116578578949,2.4668117604321792e-06
88789,709938,709938,1419876,731.8385148048401,2.466452806890863e-06
88889,710738,710738,1421476,732.6477317810059,2.466097001230313e-06
88989,711538,711538,1423076,733.3781669139862,2.4657442558258326e-06
89089,712338,712338,1424676,734.1011147499084,2.465394484886586e-06
89189,713138,713138,1426276,734.8975958824158,2.465047606149379e-06
89289,713938,713938,1427876,735.66539478302,2.4647035391703118e-06
89389,714738,714738,1429476,736.369295835495,2.4643622064436e-06
89489,715538,715538,1431076,737.1060059070587,2.4640235325302645e-06
89590,716346,716346,1432692,737.9119186401367,2.463684096484332e-06
89690,717146,717146,1434292,738.6838607788086,2.463350548206746e-06
89790,717946,717946,1435892,739.4467778205872,2.463019445653458e-06
89890,718746,718746,1437492,740.2506139278412,2.462690722080573e-06
89990,719546,719546,1439092,741.0319259166718,2.4623643130765014e-06
90090,720346,720346,1440692,741.809506893158,2.4620401561332373e-06
90190,721146,721146,1442292,742.6863470077515,2.4617181903205653e-06
90290,721946,721946,1443892,743.4035408496857,2.461398356740772e-06
90390,722746,722746,1445492,744.0939557552338,2.4610805981589044e-06
90490,723546,723546,1447092,745.0860779285431,2.4607648594095344e-06
90591,724354,724354,1448708,745.905957698822,2.4604479585540247e-06
90691,725154,725154,1450308,746.78364777565,2.460136118403859e-06
90791,725954,725954,1451908,747.6555099487305,2.4598261407808925e-06
90891,726754,726754,1453508,748.6399397850037,2.4595179766256964e-06
90991,727554,727554,1455108,749.4466338157654,2.4592115783775153e-06
91091,728354,728354,1456708,750.2854399681091,2.4589068996365686e-06
91191,729154,729154,1458308,751.0973470211029,2.4586038956606212e-06
91291,729954,729954,1459908,751.9377210140228,2.458302522705414e-06
91391,730754,730754,1461508,752.7262089252472,2.458002738703992e-06
91491,731554,731554,1463108,753.6606860160828,2.4577045024928565e-06
91592,732362,732362,1464724,754.6925098896027,2.4574048143427572e-06
91692,733162,733162,1466324,755.5247218608856,2.457109569741691e-06
91792,733962,733962,1467924,756.5274789333344,2.4568157564811167e-06
91892,734762,734762,1469524,757.3046677112579,2.456523338006819e-06
91992,735562,735562,1471124,758.1284987926483,2.4562322789324794e-06
92092,736362,736362,1472724,758.9097399711609,2.4559425449602976e-06
92192,737162,737162,1474324,759.6886878013611,2.4556541025568143e-06
92292,737962,737962,1475924,760.4833068847656,2.455366919545123e-06
92392,738762,738762,1477524,761.2223479747772,2.455080964270256e-06
92492,739562,739562,1479124,761.9700808525085,2.4547962058597536e-06
92593,740370,740370,1480740,762.7620317935944,2.4545097849848536e-06
92693,741170,741170,1482340,763.587201833725,2.4542273439816544e-06
92793,741970,741970,1483940,764.3615946769714,2.453946013169236e-06
92893,742770,742770,1485540,765.1277680397034,2.4536657653843456e-06
92993,743570,743570,1487140,765.8657939434052,2.453386573969768e-06
93093,744370,744370,1488740,766.7436809539795,2.453108413306136e-06
93193,745170,745170,1490340,767.7725818157196,2.452831258535445e-06
93293,745970,745970,1491940,768.5303149223328,2.452555085201648e-06
93393,746770,746770,1493540,769.2617106437683,2.4522798696370975e-06
93493,747570,747570,1495140,770.2267980575562,2.4520055889639992e-06
93594,748378,748378,1496756,771.0958209037781,2.45172949182061e-06
93694,749178,749178,1498356,771.9127616882324,2.451457023515838e-06
93794,749978,749978,1499956,772.7075986862183,2.4511854247672446e-06
93894,750778,750778,1501556,773.5196838378906,2.4509146751418336e-06
93994,751578,751578,1503156,774.4879946708679,2.4506447547974703e-06
94094,752378,752378,1504756,775.3301119804382,2.4503756441579967e-06
94194,753178,753178,1506356,776.2807078361511,2.450107324587916e-06
94294,753978,753978,1507956,777.1377589702606,2.449839777469841e-06
94394,754778,754778,1509556,777.9457619190216,2.4495729853290045e-06
94494,755578,755578,1511156,778.71013879776,2.4493069307876995e-06
94595,756386,756386,1512772,779.520260810852,2.449038946880224e-06
94695,757186,757186,1514372,780.4009499549866,2.4487743240427474e-06
94795,757986,757986,1515972,781.2757349014282,2.4485103892798324e-06
94895,758786,758786,1517572,782.1712996959686,2.448247127130375e-06
94995,759586,759586,1519172,782.9732048511505,2.4479845224712253e-06
95095,760386,760386,1520772,783.7086117267609,2.4477225605570355e-06
95195,761186,761186,1522372,784.4869067668915,2.4474612271806865e-06
95295,761986,761986,1523972,785.2645797729492,2.4472005084152543e-06
95395,762786,762786,1525572,786.0413780212402,2.446940390737576e-06
95495,763586,763586,1527172,786.7428269386292,2.4466808608699895e-06
95596,764394,764394,1528788,787.5186049938202,2.446419319462807e-06
95696,765194,765194,1530388,788.2580318450928,2.4461609327631493e-06
95796,765994,765994,1531988,788.9765598773956,2.4459030962686958e-06
95896,766794,766794,1533588,789.7217628955841,2.44564579827973e-06
95996,767594,767594,1535188,790.4604148864746,2.4453890271895707e-06
96096,768394,768394,1536788,791.2090878486633,2.445132771731149e-06
96196,769194,769194,1538388,792.0081059932709,2.44487702115304e-06
96296,769990,769990,1539980,792.769437789917,2.1807758698646533e-06
96396,770790,770790,1541580,793.5521547794342,2.172208876737374e-06
96496,771590,771590,1543180,794.3026437759399,2.1697395186380027e-06
96597,772398,772398,1544796,795.0778028964996,2.167904543934975e-06
96697,773198,773198,1546396,795.8579399585724,2.1663250974519596e-06
96797,773998,773998,1547996,796.5591788291931,2.1648670450341448e-06
96897,774798,774798,1549596,797.2388818264008,2.1634878708964602e-06
96997,775598,775598,1551196,797.9767308235168,2.1621682547995077e-06
97097,776398,776398,1552796,798.7308719158173,2.1608977925509792e-06
97197,777198,777198,1554396,799.5073268413544,2.1596700633130174e-06
97297,777998,777998,1555996,800.2979938983917,2.1584806801938324e-06
97397,778798,778798,1557596,801.0999050140381,2.1573264154086306e-06
97497,779598,779598,1559196,801.8526027202606,2.156204759271425e-06
97598,780406,780406,1560812,802.615327835083,2.1551029115697347e-06
97698,781206,781206,1562412,803.3625347614288,2.15404096664431e-06
97798,782006,782006,1564012,804.1248488426208,2.1530063894022536e-06
97898,782806,782806,1565612,804.848494052887,2.1519978771108077e-06
97998,783606,783606,1567212,805.5328989028931,2.1510142583410236e-06
98098,784406,784406,1568812,806.2726047039032,2.1500544656582067e-06
98198,785206,785206,1570412,807.048773765564,2.1491175150663405e-06
98298,786006,786006,1572012,807.765213727951,2.1482024916979503e-06
98398,786806,786806,1573612,808.5166010856628,2.147308538934553e-06
98498,787606,787606,1575212,809.2770717144012,2.146434850245368e-06
98599,788414,788414,1576828,810.0141470432281,2.1455722175132488e-06
98699,789214,789214,1578428,810.7475838661194,2.1447369935990473e-06
98799,790014,790014,1580028,811.4443566799164,2.143919853689865e-06
98899,790814,790814,1581628,812.185546875,2.1431201423103506e-06
98999,791614,791614,1583228,812.863452911377,2.1423372338419767e-06
99099,792414,792414,1584828,813.5719900131226,2.1415705299991436e-06
99199,793214,793214,1586428,814.3212189674377,2.1408194578780535e-06
99299,794014,794014,1588028,815.086639881134,2.1400834685005416e-06
99399,794814,794814,1589628,815.8800737857819,2.139362035979933e-06
99499,795614,795614,1591228,816.6726830005646,2.1386546551080843e-06
99600,796422,796422,1592844,817.3951368331909,2.1379539699894763e-06
99700,797222,797222,1594444,818.0839989185333,2.1372733860115384e-06
99800,798022,798022,1596044,818.846364736557,2.136605451859056e-06
99900,798822,798822,1597644,819.6157579421997,2.1359497372988015e-06
100000,799622,799622,1599244,820.2989549636841,2.1353058295195124e-06


==> extragradient/plot_data/bilinear_matrix_game_n500/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.004578828811645508,2.018959020339561
69,162,162,324,0.5456399917602539,0.059786073230173785
138,362,362,724,1.0914397239685059,0.01507175353552151
207,606,606,1212,1.6178748607635498,0.006802968350301351
276,854,854,1708,2.2067418098449707,0.003444646449262009
345,1124,1124,2248,2.8194258213043213,0.0028073235526150354
413,1390,1390,2780,3.3963279724121094,0.0021475962551178577
482,1656,1656,3312,4.299939870834351,0.0015811463673860975
551,1928,1928,3856,4.858036994934082,0.0013172553409269178
620,2198,2198,4396,5.475833892822266,0.0010024683676113034
689,2474,2474,4948,5.9514429569244385,0.0008031365805358339
758,2750,2750,5500,6.4927427768707275,0.0006681776194095929
827,3020,3020,6040,7.0113348960876465,0.0005085639104525426
896,3290,3290,6580,7.496543884277344,0.0004035657261022955
965,3566,3566,7132,7.974887847900391,0.0003585004704135169
1034,3842,3842,7684,8.452881813049316,0.0003329619936725249
1102,4114,4114,8228,8.92270278930664,0.0002713694035712921
1171,4390,4390,8780,9.42782974243164,0.00023184231104492845
1240,4666,4666,9332,9.914666891098022,0.00020626155997945992
1309,4942,4942,9884,10.395846843719482,0.00018590285321652873
1378,5218,5218,10436,10.879998922348022,0.00015901636808948527
1447,5486,5486,10972,11.363213777542114,0.00011797622395897509
1516,5762,5762,11524,11.851638793945312,0.00010116404468617912
1585,6038,6038,12076,12.335442781448364,8.929153885947352e-05
1654,6314,6314,12628,12.823810815811157,7.338889446726718e-05
1723,6590,6590,13180,13.300436019897461,6.50943815530093e-05
1792,6866,6866,13732,13.78229570388794,5.961726407905162e-05
1860,7138,7138,14276,14.247904777526855,5.676209587709056e-05
1929,7414,7414,14828,14.719422817230225,5.449163988795128e-05
1998,7690,7690,15380,15.192276000976562,5.170103272576408e-05
2067,7966,7966,15932,15.675442934036255,5.064870630975057e-05
2136,8242,8242,16484,16.14820885658264,4.988391862133933e-05
2205,8518,8518,17036,16.619136810302734,4.94680950431296e-05
2274,8794,8794,17588,17.19023060798645,4.907274356430394e-05
2343,9070,9070,18140,17.76914691925049,4.862028825735144e-05
2412,9346,9346,18692,18.38659381866455,4.836182259874062e-05
2481,9622,9622,19244,18.967670679092407,4.7838961380909206e-05
2549,9894,9894,19788,19.519465923309326,4.740810021484917e-05
2618,10170,10170,20340,20.10663676261902,4.708209595837559e-05
2687,10446,10446,20892,20.62573480606079,4.685625831742085e-05
2756,10722,10722,21444,21.330275774002075,4.643259057843834e-05
2825,10998,10998,21996,21.90008783340454,4.5912453744244845e-05
2894,11274,11274,22548,22.42951464653015,4.5151777475619436e-05
2963,11550,11550,23100,23.01525092124939,4.478454227214779e-05
3032,11826,11826,23652,23.63002872467041,4.448468329324223e-05
3101,12124,12124,24248,24.13505268096924,3.620353059135834e-05
3170,12400,12400,24800,24.663233757019043,3.251915887215331e-05
3238,12672,12672,25344,25.13606572151184,2.8239348201756584e-05
3307,12948,12948,25896,25.6695077419281,2.4409104790933668e-05
3376,13224,13224,26448,26.472150802612305,2.068078503720382e-05
3445,13500,13500,27000,27.128644704818726,1.7031458943989376e-05
3514,13776,13776,27552,28.02178692817688,1.4639992711182283e-05
3583,14052,14052,28104,28.580612897872925,1.3744720038568658e-05
3652,14328,14328,28656,29.467164754867554,1.2894622738995196e-05
3721,14604,14604,29208,30.031800746917725,1.1391260677440633e-05
3790,14880,14880,29760,30.71770668029785,1.0840637113303256e-05
3859,15156,15156,30312,31.465824604034424,9.567314571383638e-06
3928,15432,15432,30864,31.965258598327637,8.440378370343375e-06
3996,15704,15704,31408,32.45776581764221,8.00883928781533e-06
4065,15980,15980,31960,33.03022789955139,7.603169096266994e-06
4134,16256,16256,32512,33.67987680435181,7.249099309669078e-06
4203,16532,16532,33064,34.65804171562195,6.98605537064377e-06
4272,16808,16808,33616,35.156808853149414,6.813677447981931e-06
4341,17084,17084,34168,35.82108783721924,6.633958009424428e-06
4410,17360,17360,34720,36.315247774124146,6.511536951408726e-06
4479,17636,17636,35272,36.995630741119385,6.4024524244725075e-06
4548,17912,17912,35824,37.63811683654785,6.2423795468798714e-06
4617,18188,18188,36376,38.18744874000549,5.97454015020185e-06
4685,18460,18460,36920,38.662723779678345,5.776198361899567e-06
4754,18736,18736,37472,39.1594660282135,5.7066415871047025e-06
4823,19012,19012,38024,39.63657283782959,5.662363600606621e-06
4892,19288,19288,38576,40.118484020233154,5.608157874705812e-06
4961,19564,19564,39128,40.78804874420166,5.586862087440221e-06
5030,19840,19840,39680,41.674314737319946,5.555281483380804e-06
5099,20116,20116,40232,42.369223833084106,5.513130160111171e-06
5168,20392,20392,40784,42.86113882064819,5.492686441001222e-06
5237,20668,20668,41336,43.36520981788635,5.475088713179951e-06
5306,20944,20944,41888,44.03134799003601,5.46705334450441e-06
5375,21220,21220,42440,44.65252470970154,5.460848121567388e-06
5443,21492,21492,42984,45.22128367424011,5.453818894016797e-06
5512,21768,21768,43536,45.712486743927,5.447236580205579e-06
5581,22044,22044,44088,46.20673990249634,5.4387630950359455e-06
5650,22320,22320,44640,46.68996977806091,5.431394897585033e-06
5719,22596,22596,45192,47.194124698638916,5.427704849361499e-06
5788,22872,22872,45744,47.713292837142944,5.425989605747568e-06
5857,23148,23148,46296,48.2057158946991,5.424711908319121e-06
5926,23424,23424,46848,48.69077682495117,5.422924850565926e-06
5995,23700,23700,47400,49.167961835861206,5.4217238251780764e-06
6064,23976,23976,47952,49.65929865837097,5.420935028426244e-06
6132,24248,24248,48496,50.141685009002686,5.42040717169227e-06
6201,24524,24524,49048,50.62200880050659,5.4200651945350095e-06
6270,24800,24800,49600,51.12325978279114,5.419478662225166e-06
6339,25076,25076,50152,51.636194705963135,5.419085779662984e-06
6408,25352,25352,50704,52.12013483047485,5.41893747747273e-06
6477,25628,25628,51256,52.596930742263794,5.418821159457836e-06
6546,25904,25904,51808,53.07664895057678,5.418645145651468e-06
6615,26180,26180,52360,53.56790471076965,5.418487041407756e-06
6684,26456,26456,52912,54.056307792663574,5.418434387219458e-06
6753,26732,26732,53464,54.54692363739014,5.418414317821249e-06
6821,27004,27004,54008,55.019720792770386,5.418393387514571e-06
6890,27280,27280,54560,55.499666929244995,5.418368128302607e-06
6959,27556,27556,55112,55.991543769836426,5.4183457009122965e-06
7028,27832,27832,55664,56.46899080276489,5.418328923610278e-06
7097,28108,28108,56216,56.94961094856262,5.4183139780970555e-06
7166,28384,28384,56768,57.43232274055481,5.418305937423661e-06
7235,28660,28660,57320,57.92724680900574,5.418300152453088e-06
7304,28936,28936,57872,58.40895986557007,5.418288053802376e-06
7373,29212,29212,58424,58.88772201538086,5.4182801979015144e-06
7442,29488,29488,58976,59.36830472946167,5.4182743004584945e-06
7511,29764,29764,59528,59.84884190559387,5.418269572197874e-06
7579,30036,30036,60072,60.332435846328735,5.418263446889721e-06
7648,30312,30312,60624,60.85203981399536,5.418262281929102e-06
7717,30588,30588,61176,61.41766881942749,5.418261723282967e-06
7786,30864,30864,61728,61.9419846534729,5.418259716728734e-06
7855,31140,31140,62280,62.504610776901245,5.4182577139139575e-06
7924,31416,31416,62832,63.0895779132843,5.4182572722007674e-06
7993,31692,31692,63384,63.606979846954346,5.418256883295804e-06
8062,31976,31976,63952,64.13519167900085,5.418256216359825e-06
8131,32252,32252,64504,64.65218472480774,5.418255872450233e-06
8200,32538,32538,65076,65.1442518234253,5.418255674035442e-06
8268,32838,32838,65676,65.64438986778259,5.418255571075618e-06
8337,33152,33152,66304,66.22209072113037,5.418255502354908e-06
8406,33436,33436,66872,66.79581904411316,5.41825523066635e-06
8475,33714,33714,67428,67.38300490379333,5.418255126419933e-06
8544,34018,34018,68036,67.95306277275085,5.418255049628186e-06
8613,34422,34422,68844,68.5252468585968,5.418255021982535e-06
8682,34974,34974,69948,69.12334275245667,5.41825502005996e-06
8751,35526,35526,71052,69.70276474952698,5.418255018671845e-06
8820,36078,36078,72156,70.28041887283325,5.4182550174083004e-06
8889,36630,36630,73260,70.86144781112671,5.418255016345616e-06
8958,37182,37182,74364,71.43410086631775,5.41825501537391e-06
9026,37726,37726,75452,72.08378076553345,5.418255014386167e-06
9095,38278,38278,76556,72.75474786758423,5.418255013473212e-06
9164,38830,38830,77660,73.36643195152283,5.418255012718085e-06
9233,39382,39382,78764,73.92911171913147,5.418255011796792e-06
9302,39934,39934,79868,74.49487900733948,5.4182550111414e-06
9371,40486,40486,80972,75.08050680160522,5.418255010361636e-06
9440,41038,41038,82076,75.68770790100098,5.418255009653609e-06
9509,41590,41590,83180,76.3066029548645,5.418255009010715e-06
9578,42142,42142,84284,76.89820384979248,5.418255008396674e-06
9647,42694,42694,85388,77.5326600074768,5.4182550077918015e-06
9715,43238,43238,86476,78.10458970069885,5.418255007182623e-06
9784,43790,43790,87580,78.72326993942261,5.4182550065124455e-06
9853,44342,44342,88684,79.34092688560486,5.418255005972505e-06
9922,44894,44894,89788,79.90126085281372,5.41825500537467e-06
9991,45446,45446,90892,80.46528387069702,5.418255004875147e-06
10060,45998,45998,91996,81.02905988693237,5.418255004388995e-06
10129,46550,46550,93100,81.60380387306213,5.418255003793285e-06
10198,47102,47102,94204,82.17937588691711,5.418255003188061e-06
10267,47654,47654,95308,82.78198575973511,5.418255002686026e-06
10336,48206,48206,96412,83.50581479072571,5.418255002221748e-06
10404,48750,48750,97500,84.16928482055664,5.418255001808962e-06
10473,49302,49302,98604,84.79986095428467,5.4182550012904755e-06
10542,49854,49854,99708,85.47574090957642,5.418255000729741e-06
10611,50406,50406,100812,86.07367992401123,5.418255000343454e-06
10680,50958,50958,101916,86.68417882919312,5.41825499986559e-06
10749,51510,51510,103020,87.34366393089294,5.418254999425903e-06
10818,52062,52062,104124,88.02355480194092,5.418254999020172e-06
10887,52614,52614,105228,88.78230404853821,5.418254998486678e-06
10956,53166,53166,106332,89.38490080833435,5.418254998049228e-06
11025,53526,53526,107052,89.90795493125916,5.379547401755516e-06
11094,53802,53802,107604,90.40278887748718,5.3426670713357725e-06
11162,54074,54074,108148,90.88102459907532,5.309576309987809e-06
11231,54350,54350,108700,91.362637758255,5.228618145228647e-06
11300,54626,54626,109252,91.85619282722473,5.1381711934584415e-06
11369,54902,54902,109804,92.33656668663025,5.062428016607756e-06
11438,55178,55178,110356,92.8174238204956,4.969859668291807e-06
11507,55454,55454,110908,93.30003476142883,4.86847663901688e-06
11576,55730,55730,111460,93.79546594619751,4.755987280676342e-06
11645,56006,56006,112012,94.27767491340637,4.644532227667598e-06
11714,56282,56282,112564,94.758957862854,4.563349586281484e-06
11783,56558,56558,113116,95.23718786239624,4.533739135253155e-06
11851,56830,56830,113660,95.7141649723053,4.5210874601977395e-06
11920,57106,57106,114212,96.20344090461731,4.508520254346753e-06
11989,57382,57382,114764,96.6818368434906,4.484287019303792e-06
12058,57658,57658,115316,97.16001486778259,4.4630354275369e-06
12127,57934,57934,115868,97.64086771011353,4.443563763235381e-06
12196,58210,58210,116420,98.1308479309082,4.406499784912793e-06
12265,58486,58486,116972,98.60904383659363,4.332028206850215e-06
12334,58762,58762,117524,99.08745288848877,4.179523878315869e-06
12403,59038,59038,118076,99.57094669342041,4.101358422251185e-06
12472,59314,59314,118628,100.05453372001648,4.066338157524443e-06
12541,59590,59590,119180,100.54263663291931,4.042072198776329e-06
12609,59862,59862,119724,101.01864194869995,4.018938734216345e-06
12678,60138,60138,120276,101.49686789512634,4.000887569001475e-06
12747,60414,60414,120828,101.97273588180542,3.9733525362892284e-06
12816,60690,60690,121380,102.46234393119812,3.9342055477318715e-06
12885,60966,60966,121932,102.94093179702759,3.8650482095291755e-06
12954,61242,61242,122484,103.42078971862793,3.8109340206641276e-06
13023,61518,61518,123036,103.90232181549072,3.7649103833791135e-06
13092,61794,61794,123588,104.39420175552368,3.696113990085636e-06
13161,62070,62070,124140,104.87279891967773,3.6055238752519567e-06
13230,62346,62346,124692,105.35035276412964,3.5524983195185987e-06
13298,62618,62618,125236,105.82279872894287,3.5065767386028974e-06
13367,62894,62894,125788,106.30136680603027,3.446093724195037e-06
13436,63170,63170,126340,106.79411888122559,3.3855570258591333e-06
13505,63446,63446,126892,107.27620792388916,3.33406273000387e-06
13574,63722,63722,127444,107.7551896572113,3.309015222826138e-06
13643,63998,63998,127996,108.23607778549194,3.2908416674441734e-06
13712,64274,64274,128548,108.7286467552185,3.2785321132046944e-06
13781,64550,64550,129100,109.21156883239746,3.265927737613496e-06
13850,64826,64826,129652,109.68989372253418,3.2493750907092485e-06
13919,65102,65102,130204,110.16170597076416,3.227451908685225e-06
13987,65374,65374,130748,110.6427857875824,3.1953320519373076e-06
14056,65650,65650,131300,111.12254786491394,3.1590658898290943e-06
14125,65926,65926,131852,111.60080981254578,3.146278309381513e-06
14194,66202,66202,132404,112.07815980911255,3.122832000338217e-06
14263,66478,66478,132956,112.5546886920929,3.09471414007653e-06
14332,66754,66754,133508,113.04385995864868,3.0735605749670397e-06
14401,67030,67030,134060,113.52760767936707,3.0624759573872955e-06
14470,67306,67306,134612,114.00836086273193,3.054884208510233e-06
14539,67582,67582,135164,114.48928785324097,3.03930903352301e-06
14608,67858,67858,135716,114.97990465164185,3.0263525617670096e-06
14677,68134,68134,136268,115.46103501319885,2.9920327126437077e-06
14745,68406,68406,136812,115.93091773986816,2.9295877158557433e-06
14814,68682,68682,137364,116.4104425907135,2.874816925018769e-06
14883,68958,68958,137916,116.90064787864685,2.830029493067806e-06
14952,69234,69234,138468,117.38359093666077,2.779916292566648e-06
15021,69510,69510,139020,117.86635184288025,2.7339584903750026e-06
15090,69786,69786,139572,118.34165787696838,2.695673817906832e-06
15159,70062,70062,140124,118.81935286521912,2.6698145911623207e-06
15228,70338,70338,140676,119.31217885017395,2.654228314266887e-06
15297,70614,70614,141228,119.78511166572571,2.6391625276232674e-06
15366,70890,70890,141780,120.26530385017395,2.606295359743482e-06
15434,71162,71162,142324,120.73939776420593,2.583233934499561e-06
15503,71438,71438,142876,121.23155999183655,2.5664358154462755e-06
15572,71714,71714,143428,121.7150206565857,2.5519621579815e-06
15641,71990,71990,143980,122.1929087638855,2.531931294151587e-06
15710,72266,72266,144532,122.67445373535156,2.503489255404376e-06
15779,72542,72542,145084,123.1540858745575,2.466982805767326e-06
15848,72818,72818,145636,123.73884391784668,2.4314317719930634e-06
15917,73094,73094,146188,124.43646478652954,2.4091318040744467e-06
15986,73370,73370,146740,125.00150179862976,2.3904339999841636e-06
16055,73646,73646,147292,125.60482096672058,2.376863791655242e-06
16124,73922,73922,147844,126.32121086120605,2.359634565643593e-06
16192,74194,74194,148388,126.96366286277771,2.333418903938666e-06
16261,74470,74470,148940,127.65596270561218,2.3086168708927725e-06
16330,74746,74746,149492,128.18821573257446,2.2730733817043784e-06
16399,75022,75022,150044,128.76531791687012,2.2365216269952053e-06
16468,75298,75298,150596,129.3210108280182,2.2187470113601148e-06
16537,75574,75574,151148,129.95412182807922,2.199845508405292e-06
16606,75850,75850,151700,130.5681037902832,2.1814330684542478e-06
16675,76126,76126,152252,131.18356275558472,2.172503808892014e-06
16744,76402,76402,152804,131.7752640247345,2.16625852929633e-06
16813,76678,76678,153356,132.40534090995789,2.1516443758307487e-06
16881,76950,76950,153900,133.0773618221283,2.126511890966414e-06
16950,77226,77226,154452,133.66180086135864,2.116538043107509e-06
17019,77502,77502,155004,134.3171808719635,2.1077464725182797e-06
17088,77778,77778,155556,134.88161063194275,2.0923809873870935e-06
17157,78054,78054,156108,135.48418879508972,2.0465776339539337e-06
17226,78330,78330,156660,136.0952398777008,2.0064223858974566e-06
17295,78606,78606,157212,136.7511248588562,1.9882665420288513e-06
17364,78882,78882,157764,137.37223982810974,1.9726226475808127e-06
17433,79158,79158,158316,137.9405529499054,1.949843429886953e-06
17502,79434,79434,158868,138.48915886878967,1.898575797035018e-06
17570,79706,79706,159412,139.01702880859375,1.825812240710027e-06
17639,79982,79982,159964,139.77199387550354,1.7670667087923431e-06
17708,80258,80258,160516,140.36450672149658,1.695356879005043e-06
17777,80534,80534,161068,140.95298171043396,1.6624449907969114e-06
17846,80810,80810,161620,141.46453380584717,1.6519312959117966e-06
17915,81086,81086,162172,142.04820275306702,1.6441434431695751e-06
17984,81362,81362,162724,142.62411499023438,1.630399252387567e-06
18053,81638,81638,163276,143.12631583213806,1.6143139010391927e-06
18122,81914,81914,163828,143.62419366836548,1.6033632476360622e-06
18191,82190,82190,164380,144.12284183502197,1.5947452591192024e-06
18260,82466,82466,164932,144.6396119594574,1.5776860349530363e-06
18328,82738,82738,165476,145.13236260414124,1.5646476321530133e-06
18397,83014,83014,166028,145.62970781326294,1.5477648298014243e-06
18466,83290,83290,166580,146.13220977783203,1.5286419766736564e-06
18535,83566,83566,167132,146.71902799606323,1.5223604238744888e-06
18604,83842,83842,167684,147.26508378982544,1.5166957568915914e-06
18673,84118,84118,168236,147.79954886436462,1.513282337267129e-06
18742,84394,84394,168788,148.3522880077362,1.5086975197298485e-06
18811,84670,84670,169340,148.87463474273682,1.5011823137560756e-06
18880,84946,84946,169892,149.3893687725067,1.4924237302927829e-06
18949,85222,85222,170444,149.88780975341797,1.4784491511895857e-06
19017,85494,85494,170988,150.38222074508667,1.461681303758386e-06
19086,85770,85770,171540,150.89545679092407,1.4445150531194183e-06
19155,86046,86046,172092,151.4021918773651,1.4199759165226276e-06
19224,86322,86322,172644,151.90009093284607,1.4027188241343778e-06
19293,86598,86598,173196,152.3926568031311,1.3980436795145816e-06
19362,86874,86874,173748,152.90250706672668,1.3923136339774182e-06
19431,87150,87150,174300,153.40311574935913,1.3805372028031636e-06
19500,87426,87426,174852,153.90194368362427,1.3662198790610016e-06
19569,87702,87702,175404,154.40004467964172,1.3490319419563382e-06
19638,87978,87978,175956,154.89802479743958,1.3281318485553294e-06
19707,88254,88254,176508,155.40235376358032,1.3186388513945672e-06
19775,88526,88526,177052,155.8922939300537,1.3099714601188582e-06
19844,88802,88802,177604,156.39035868644714,1.303953012246928e-06
19913,89078,89078,178156,156.8865737915039,1.298735559702936e-06
19982,89354,89354,178708,157.3945438861847,1.2910084705819036e-06
20051,89630,89630,179260,157.89169883728027,1.2873215006626254e-06
20120,89906,89906,179812,158.5357849597931,1.2817563060710208e-06
20189,90182,90182,180364,159.2645399570465,1.2716255372986975e-06
20258,90458,90458,180916,159.81633687019348,1.2532575070518929e-06
20327,90734,90734,181468,160.30382585525513,1.1473436953976021e-06
20396,91010,91010,182020,160.79677963256836,1.0851608329482079e-06
20464,91282,91282,182564,161.28470396995544,1.0584566246509227e-06
20533,91558,91558,183116,161.8676779270172,1.0434514902594282e-06
20602,91834,91834,183668,162.48167085647583,1.0359026980603957e-06
20671,92110,92110,184220,163.00680661201477,1.0254069764230329e-06
20740,92386,92386,184772,163.58061289787292,1.0203345441734503e-06
20809,92662,92662,185324,164.0960488319397,1.0154704957168949e-06
20878,92938,92938,185876,164.59131979942322,1.00971258309033e-06
20947,93214,93214,186428,165.07269287109375,1.0021022460935357e-06
21016,93490,93490,186980,165.5636658668518,9.906048423369248e-07
21085,93766,93766,187532,166.05083394050598,9.699213117371869e-07
21153,94038,94038,188076,166.54242372512817,9.400182634328307e-07
21222,94314,94314,188628,167.0457637310028,9.151938773094182e-07
21291,94590,94590,189180,167.57129383087158,8.984040867255151e-07
21360,94866,94866,189732,168.1079728603363,8.840788182356527e-07
21429,95142,95142,190284,168.64778184890747,8.733381640492883e-07
21498,95418,95418,190836,169.17987275123596,8.658876642915251e-07
21567,95694,95694,191388,169.6691448688507,8.592701391158319e-07
21636,95970,95970,191940,170.198588848114,8.443412367382944e-07
21705,96246,96246,192492,170.72593784332275,8.25012109361403e-07
21774,96522,96522,193044,171.2292377948761,8.126607912454637e-07
21843,96798,96798,193596,171.79760575294495,8.073059474274276e-07
21911,97070,97070,194140,172.424222946167,8.01959418662202e-07
21980,97346,97346,194692,172.94713878631592,7.984426879752806e-07
22049,97622,97622,195244,173.43403482437134,7.939919817434364e-07
22118,97898,97898,195796,173.92277359962463,7.8087203001552e-07
22187,98174,98174,196348,174.44212889671326,7.603204120233894e-07
22256,98450,98450,196900,174.9587857723236,7.421182678033652e-07
22325,98726,98726,197452,175.44470977783203,7.318314211332239e-07
22394,99002,99002,198004,175.9348337650299,7.230773834374872e-07
22463,99278,99278,198556,176.45981287956238,7.093826863918587e-07
22532,99554,99554,199108,176.94859170913696,6.98171304938684e-07
22600,99826,99826,199652,177.42905187606812,6.945361157339042e-07
22669,100102,100102,200204,177.92191076278687,6.921058132271046e-07
22738,100378,100378,200756,178.41727685928345,6.885784789664433e-07
22807,100654,100654,201308,178.97648787498474,6.820300902537438e-07
22876,100930,100930,201860,179.53876090049744,6.769494496959827e-07
22945,101206,101206,202412,180.05971789360046,6.738213138870547e-07
23014,101482,101482,202964,180.5999937057495,6.71483172413822e-07
23083,101758,101758,203516,181.12906289100647,6.697619336209671e-07
23152,102034,102034,204068,181.62410187721252,6.656121919536343e-07
23221,102310,102310,204620,182.3446238040924,6.594194519797e-07
23290,102586,102586,205172,182.9580807685852,6.565239623791896e-07
23358,102858,102858,205716,183.59112882614136,6.522469162379786e-07
23427,103134,103134,206268,184.2047917842865,6.482124897592562e-07
23496,103410,103410,206820,184.76584577560425,6.449968407295649e-07
23565,103686,103686,207372,185.27368664741516,6.418520534121865e-07
23634,103962,103962,207924,185.788067817688,6.363629007049928e-07
23703,104238,104238,208476,186.28840279579163,6.287779424455271e-07
23772,104514,104514,209028,186.90825390815735,6.191427324205314e-07
23841,104790,104790,209580,187.48864483833313,6.065189961471137e-07
23910,105066,105066,210132,188.20597577095032,5.904301809218356e-07
23979,105342,105342,210684,188.88677978515625,5.694476783045236e-07
24047,105614,105614,211228,189.44515371322632,5.525427749368964e-07
24116,105890,105890,211780,190.0699667930603,5.357153146269196e-07
24185,106166,106166,212332,190.7250418663025,5.174091663324174e-07
24254,106442,106442,212884,191.26396870613098,4.969855731860432e-07
24323,106718,106718,213436,191.79122471809387,4.867648006982636e-07
24392,106994,106994,213988,192.37824487686157,4.7421732873092195e-07
24461,107270,107270,214540,193.0177538394928,4.691237399806547e-07
24530,107546,107546,215092,193.7070369720459,4.6385720330441294e-07
24599,107822,107822,215644,194.37032079696655,4.504870795197237e-07
24668,108098,108098,216196,195.01179766654968,4.3939604700883184e-07
24737,108374,108374,216748,195.65669679641724,4.2584430356560884e-07
24805,108646,108646,217292,196.28931093215942,4.226221376562356e-07
24874,108922,108922,217844,196.93034601211548,4.193931065169757e-07
24943,109198,109198,218396,197.57167792320251,4.158762988963848e-07
25012,109474,109474,218948,198.45741963386536,4.14186759828887e-07
25081,109750,109750,219500,199.14776873588562,4.1174728026577517e-07
25150,110026,110026,220052,199.8340549468994,4.0753415783939937e-07
25219,110302,110302,220604,200.4778037071228,4.0140628309749583e-07
25288,110578,110578,221156,201.12299704551697,3.904923196235539e-07
25357,110854,110854,221708,201.77380776405334,3.8222460850907154e-07
25426,111130,111130,222260,202.41849088668823,3.736825101400761e-07
25494,111402,111402,222804,203.05621099472046,3.6604533627855266e-07
25563,111678,111678,223356,203.72605276107788,3.6189190697284677e-07
25632,111954,111954,223908,204.51335096359253,3.604440624720314e-07
25701,112230,112230,224460,205.19433665275574,3.5906430110827535e-07
25770,112506,112506,225012,205.90044498443604,3.572780241508375e-07
25839,112782,112782,225564,206.5789430141449,3.5572242970569193e-07
25908,113058,113058,226116,207.31769680976868,3.5396727934222414e-07
25977,113334,113334,226668,208.00306677818298,3.5130967778377487e-07
26046,113610,113610,227220,208.66326189041138,3.491582075076855e-07
26115,113886,113886,227772,209.3343858718872,3.480960718397233e-07
26183,114158,114158,228316,209.9871768951416,3.467779826184963e-07
26252,114434,114434,228868,210.64050102233887,3.4554493264282956e-07
26321,114710,114710,229420,211.3166058063507,3.4395078401953363e-07
26390,114986,114986,229972,211.96480894088745,3.41296122736764e-07
26459,115262,115262,230524,212.62562775611877,3.3755422437841316e-07
26528,115538,115538,231076,213.35346484184265,3.3376826120619847e-07
26597,115814,115814,231628,214.04836893081665,3.2964236521976967e-07
26666,116090,116090,232180,214.79706597328186,3.2358601890400513e-07
26735,116366,116366,232732,215.4765908718109,3.161005719347034e-07
26804,116642,116642,233284,216.1779408454895,3.1133643243180285e-07
26873,116918,116918,233836,216.8323757648468,3.085086365463688e-07
26941,117190,117190,234380,217.4780149459839,3.0628621412350836e-07
27010,117466,117466,234932,218.14209985733032,3.028116180685083e-07
27079,117742,117742,235484,218.85747265815735,3.0021703904444676e-07
27148,118018,118018,236036,219.50494170188904,2.977368275002452e-07
27217,118294,118294,236588,220.15312004089355,2.941835517438351e-07
27286,118570,118570,237140,220.80410075187683,2.9071655681229157e-07
27355,118846,118846,237692,221.4570598602295,2.8979741943857235e-07
27424,119122,119122,238244,222.11467695236206,2.8911918115620434e-07
27493,119398,119398,238796,222.76910591125488,2.876853903431476e-07
27562,119674,119674,239348,223.42443776130676,2.8486909316030424e-07
27630,119946,119946,239892,224.06174898147583,2.8212475715809413e-07
27699,120222,120222,240444,224.70781898498535,2.790019380769651e-07
27768,120498,120498,240996,225.35825777053833,2.766207391723426e-07
27837,120774,120774,241548,225.99882984161377,2.7515489762164966e-07
27906,121050,121050,242100,226.67181873321533,2.7424820777028363e-07
27975,121326,121326,242652,227.35774683952332,2.7299159281630986e-07
28044,121602,121602,243204,228.05729484558105,2.7178798793784285e-07
28113,121878,121878,243756,228.73596858978271,2.697920312556463e-07
28182,122154,122154,244308,229.41913485527039,2.6477965818522863e-07
28251,122430,122430,244860,230.16819882392883,2.6024610813203045e-07
28320,122706,122706,245412,230.84040570259094,2.5617488911482987e-07
28388,122978,122978,245956,231.47265672683716,2.533229357772704e-07
28457,123254,123254,246508,232.1348967552185,2.496465631360814e-07
28526,123530,123530,247060,232.78393983840942,2.46789230091113e-07
28595,123806,123806,247612,233.4238748550415,2.4583526113063445e-07
28664,124082,124082,248164,234.0754566192627,2.44487981637092e-07
28733,124358,124358,248716,234.72709465026855,2.4272290450073585e-07
28802,124634,124634,249268,235.3767786026001,2.3956571896642965e-07
28871,124910,124910,249820,236.0384497642517,2.3315566270277283e-07
28940,125186,125186,250372,236.68685865402222,2.2883658732484045e-07
29009,125462,125462,250924,237.32569193840027,2.2567294809410412e-07
29077,125734,125734,251468,237.96625685691833,2.2392417651845067e-07
29146,126010,126010,252020,238.62996196746826,2.2273818222902288e-07
29215,126286,126286,252572,239.273521900177,2.2212666203007682e-07
29284,126562,126562,253124,239.91052293777466,2.2110603538175724e-07
29353,126838,126838,253676,240.55987977981567,2.1845132477990954e-07
29422,127114,127114,254228,241.203430891037,2.160027505960292e-07
29491,127390,127390,254780,241.84379172325134,2.1480538289272548e-07
29560,127666,127666,255332,242.4903507232666,2.1370895833494108e-07
29629,127942,127942,255884,243.13119888305664,2.1288053061217554e-07
29698,128218,128218,256436,243.7752227783203,2.1181875736117828e-07
29766,128490,128490,256980,244.4064269065857,2.1059939449617577e-07
29835,128766,128766,257532,245.05514478683472,2.0891634556288388e-07
29904,129042,129042,258084,245.69463562965393,2.0706120532770302e-07
29973,129318,129318,258636,246.3295476436615,2.0221842238583562e-07
30042,129594,129594,259188,246.97644066810608,1.9545145029553934e-07
30111,129870,129870,259740,247.61255884170532,1.8921106300299956e-07
30180,130146,130146,260292,248.2477309703827,1.8350255514487614e-07
30249,130422,130422,260844,248.89169001579285,1.7982156837081027e-07
30318,130698,130698,261396,249.52943897247314,1.7815860757490988e-07
30387,130974,130974,261948,250.16625380516052,1.7601310962337625e-07
30456,131250,131250,262500,250.80623579025269,1.715064809279877e-07
30524,131522,131522,263044,251.4348816871643,1.664861088791907e-07
30593,131798,131798,263596,252.06886887550354,1.6371368452323642e-07
30662,132074,132074,264148,252.71198081970215,1.5853168000553902e-07
30731,132350,132350,264700,253.37865591049194,1.5432128239490236e-07
30800,132626,132626,265252,254.04853987693787,1.5295707590396073e-07
30869,132902,132902,265804,254.72963571548462,1.5176413698610226e-07
30938,133178,133178,266356,255.4235348701477,1.5039967641636483e-07
31007,133454,133454,266908,256.10738372802734,1.495239342875822e-07
31076,133730,133730,267460,256.8021788597107,1.480012795564731e-07
31145,134006,134006,268012,257.5050427913666,1.4687677282874137e-07
31213,134278,134278,268556,258.1926968097687,1.4604284196718903e-07
31282,134554,134554,269108,258.85950899124146,1.4558705225831947e-07
31351,134830,134830,269660,259.53318667411804,1.4491048651426383e-07
31420,135106,135106,270212,260.1881170272827,1.4336938719654986e-07
31489,135382,135382,270764,260.8432557582855,1.4286191505661095e-07
31558,135658,135658,271316,261.4997498989105,1.4229411479175603e-07
31627,135934,135934,271868,262.1406726837158,1.407070653240422e-07
31696,136210,136210,272420,262.78220081329346,1.377832811094919e-07
31765,136486,136486,272972,263.4113817214966,1.353540122080494e-07
31834,136762,136762,273524,264.0613429546356,1.318679619038856e-07
31903,137038,137038,274076,264.7114658355713,1.2826107566339736e-07
31971,137308,137308,274616,265.34703278541565,1.171928960003993e-07
32040,137584,137584,275168,266.01116275787354,1.0132417749435293e-07
32109,137860,137860,275720,266.6687738895416,9.650243263749317e-08
32178,138136,138136,276272,267.33119082450867,9.43169996843555e-08
32247,138412,138412,276824,267.9954698085785,9.331792737875765e-08
32316,138688,138688,277376,268.6592288017273,9.264063588882561e-08
32385,138964,138964,277928,269.3211188316345,9.212432019597905e-08
32454,139240,139240,278480,269.9795117378235,9.176588640971987e-08
32523,139516,139516,279032,270.6572518348694,9.139952021059324e-08
32592,139792,139792,279584,271.3302128314972,9.087626009741395e-08
32660,140064,140064,280128,271.98853874206543,8.967201816813838e-08
32729,140340,140340,280680,272.6710617542267,8.836217372058603e-08
32798,140616,140616,281232,273.3497648239136,8.782883348378235e-08
32867,140892,140892,281784,274.00649070739746,8.756704903899811e-08
32936,141168,141168,282336,274.6531536579132,8.725012488511617e-08
33005,141444,141444,282888,275.29378271102905,8.66773924310983e-08
33074,141720,141720,283440,275.9339249134064,8.597079784935756e-08
33143,141996,141996,283992,276.58721470832825,8.563822453302807e-08
33212,142272,142272,284544,277.2322578430176,8.527511212740912e-08
33281,142548,142548,285096,277.8711757659912,8.4698734485662e-08
33349,142820,142820,285640,278.4963777065277,8.378761323805962e-08
33418,143096,143096,286192,279.13953280448914,8.362196681417924e-08
33487,143372,143372,286744,279.77154779434204,8.337397639506041e-08
33556,143648,143648,287296,280.4639256000519,8.283835279240032e-08
33625,143924,143924,287848,281.1617286205292,8.199480047054082e-08
33694,144200,144200,288400,281.84865164756775,8.093339114288381e-08
33763,144476,144476,288952,282.53495502471924,7.934371705683026e-08
33832,144752,144752,289504,283.2183287143707,7.808568637215932e-08
33901,145028,145028,290056,283.8971438407898,7.703089350830445e-08
33970,145304,145304,290608,284.65860199928284,7.651263278264364e-08
34039,145580,145580,291160,285.38020300865173,7.629183536683357e-08
34107,145852,145852,291704,286.0350296497345,7.59673693136612e-08
34176,146128,146128,292256,286.6893229484558,7.530684656913268e-08
34245,146404,146404,292808,287.35250878334045,7.480446304591012e-08
34314,146680,146680,293360,288.0057158470154,7.410970722169751e-08
34383,146956,146956,293912,288.75623297691345,7.326631062819864e-08
34452,147232,147232,294464,289.4334318637848,7.27193753063976e-08
34521,147508,147508,295016,290.15724873542786,7.245272023878989e-08
34590,147784,147784,295568,290.8470118045807,7.17252063146894e-08
34659,148060,148060,296120,291.5293457508087,7.10803535777876e-08
34728,148336,148336,296672,292.2022488117218,7.06294931258012e-08
34796,148608,148608,297216,292.85228180885315,7.03249274607657e-08
34865,148884,148884,297768,293.50874185562134,6.991528381434786e-08
34934,149160,149160,298320,294.1971278190613,6.938715860557984e-08
35003,149436,149436,298872,294.8630928993225,6.906329778356431e-08
35072,149712,149712,299424,295.50174283981323,6.877939140210791e-08
35141,149988,149988,299976,296.15096783638,6.836522673050149e-08
35210,150264,150264,300528,296.84655690193176,6.719074799508175e-08
35279,150540,150540,301080,297.48795080184937,6.611533697066439e-08
35348,150816,150816,301632,298.17958092689514,6.523090180646529e-08
35417,151092,151092,302184,298.8244049549103,6.479434965145409e-08
35486,151368,151368,302736,299.51485896110535,6.374411826001546e-08
35554,151640,151640,303280,300.1954996585846,6.296379456387648e-08
35623,151916,151916,303832,301.05082082748413,6.245135491003757e-08
35692,152192,152192,304384,301.7575888633728,6.213939287679705e-08
35761,152468,152468,304936,302.4301428794861,6.168659357225229e-08
35830,152744,152744,305488,303.0847339630127,6.137800717762748e-08
35899,153020,153020,306040,303.75619888305664,6.117526998383412e-08
35968,153296,153296,306592,304.42027282714844,6.098291219658838e-08
36037,153572,153572,307144,305.0764636993408,6.049508147852142e-08
36106,153848,153848,307696,305.74141693115234,6.000884080687201e-08
36175,154124,154124,308248,306.4669678211212,5.978675901893143e-08
36243,154396,154396,308792,307.1674346923828,5.956260456147538e-08
36312,154672,154672,309344,307.8939609527588,5.891665410713299e-08
36381,154948,154948,309896,308.5717329978943,5.846147565112455e-08
36450,155224,155224,310448,309.27128076553345,5.803098683807715e-08
36519,155500,155500,311000,309.92412185668945,5.760114291429521e-08
36588,155776,155776,311552,310.55934596061707,5.719733501432382e-08
36657,156052,156052,312104,311.24150562286377,5.6653620058837056e-08
36726,156328,156328,312656,312.080463886261,5.603753622351761e-08
36795,156604,156604,313208,312.7679109573364,5.566658600211047e-08
36864,156880,156880,313760,313.4206657409668,5.552303539918677e-08
36932,157152,157152,314304,314.0600326061249,5.541027937292887e-08
37001,157428,157428,314856,314.7267208099365,5.524794219093595e-08
37070,157704,157704,315408,315.4166567325592,5.504316639183883e-08
37139,157980,157980,315960,316.1104428768158,5.4818952409480265e-08
37208,158256,158256,316512,316.83944392204285,5.4543699654833795e-08
37277,158532,158532,317064,317.522176027298,5.393853292004666e-08
37346,158808,158808,317616,318.27353978157043,5.336001239452197e-08
37415,159084,159084,318168,318.98832988739014,5.2949140734512487e-08
37484,159360,159360,318720,319.66468572616577,5.199594474389038e-08
37553,159636,159636,319272,320.32919573783875,5.1053899173300757e-08
37622,159912,159912,319824,320.98120188713074,4.989683084712992e-08
37690,160184,160184,320368,321.62967562675476,4.865686035102206e-08
37759,160460,160460,320920,322.2804927825928,4.733327371898263e-08
37828,160736,160736,321472,322.95098781585693,4.5782538225368195e-08
37897,161012,161012,322024,323.6392488479614,4.323141394361311e-08
37966,161288,161288,322576,324.21842670440674,4.025843090267798e-08
38035,161564,161564,323128,324.78037190437317,3.887447883811857e-08
38104,161840,161840,323680,325.3633577823639,3.8211015974264216e-08
38173,162116,162116,324232,325.9757046699524,3.683301121112338e-08
38242,162392,162392,324784,326.5171809196472,3.646293309529641e-08
38311,162668,162668,325336,327.10060477256775,3.616874990233188e-08
38379,162940,162940,325880,327.7188799381256,3.574991690454122e-08
38448,163216,163216,326432,328.34158968925476,3.490118807184019e-08
38517,163492,163492,326984,329.02814388275146,3.418871709467111e-08
38586,163768,163768,327536,329.67919182777405,3.36042471374257e-08
38655,164044,164044,328088,330.38970398902893,3.3380988425129425e-08
38724,164320,164320,328640,331.00402784347534,3.324678469187364e-08
38793,164596,164596,329192,331.57908272743225,3.309484413960848e-08
38862,164872,164872,329744,332.10897278785706,3.274080966023562e-08
38931,165148,165148,330296,332.6475558280945,3.2426456447699345e-08
39000,165424,165424,330848,333.24768590927124,3.2273530783533174e-08
39069,165700,165700,331400,333.7359449863434,3.2103452369594196e-08
39137,165972,165972,331944,334.21406388282776,3.198741770676236e-08
39206,166248,166248,332496,334.72843170166016,3.189942510231858e-08
39275,166524,166524,333048,335.2157347202301,3.1669622378626716e-08
39344,166800,166800,333600,335.7026598453522,3.116418256158964e-08
39413,167076,167076,334152,336.17347264289856,2.9581404959419772e-08
39482,167352,167352,334704,336.67703080177307,2.8124716727284565e-08
39551,167628,167628,335256,337.161239862442,2.734010282874724e-08
39620,167904,167904,335808,337.6412229537964,2.718541223673838e-08
39689,168180,168180,336360,338.12448287010193,2.6977845908482417e-08
39758,168456,168456,336912,338.62051367759705,2.6742366551078775e-08
39826,168728,168728,337456,339.09021496772766,2.6284919573105782e-08
39895,169004,169004,338008,339.56635761260986,2.5617638033437815e-08
39964,169280,169280,338560,340.04421973228455,2.5394570686772807e-08
40033,169556,169556,339112,340.54634976387024,2.5295009783784887e-08
40102,169832,169832,339664,341.0632178783417,2.509741812885375e-08
40171,170108,170108,340216,341.54733872413635,2.4512805032040537e-08
40240,170384,170384,340768,342.02766966819763,2.429589312713311e-08
40309,170660,170660,341320,342.50435996055603,2.4177213255511873e-08
40378,170936,170936,341872,342.99747467041016,2.4091421697957917e-08
40447,171212,171212,342424,343.47495579719543,2.402329159802836e-08
40515,171484,171484,342968,343.94392681121826,2.3545493958117555e-08
40584,171760,171760,343520,344.41981172561646,2.303747183382659e-08
40653,172036,172036,344072,344.9082486629486,2.2561588041989718e-08
40722,172312,172312,344624,345.3904597759247,2.2078526278597626e-08
40791,172588,172588,345176,345.87769985198975,2.17913102265046e-08
40860,172864,172864,345728,346.35388684272766,2.161001804878353e-08
40929,173140,173140,346280,346.8334767818451,2.1293994530429697e-08
40998,173416,173416,346832,347.35002970695496,2.0943434008074683e-08
41067,173692,173692,347384,347.8476617336273,2.084000942874622e-08
41136,173968,173968,347936,348.34973788261414,2.077248749443322e-08
41205,174244,174244,348488,348.8436748981476,2.068724493080108e-08
41273,174516,174516,349032,349.3445818424225,2.0524849780940728e-08
41342,174792,174792,349584,349.85069489479065,2.0457112211350664e-08
41411,175068,175068,350136,350.34317803382874,2.0329897106409392e-08
41480,175344,175344,350688,350.8178708553314,2.022894959844226e-08
41549,175620,175620,351240,351.3001937866211,2.014214369051683e-08
41618,175896,175896,351792,351.77512979507446,1.99733745399545e-08
41687,176172,176172,352344,352.25613594055176,1.9794910349051174e-08
41756,176448,176448,352896,352.7922627925873,1.9577051213679814e-08
41825,176724,176724,353448,353.3258776664734,1.9439572929981147e-08
41894,177000,177000,354000,353.8826518058777,1.9301377690262157e-08
41962,177272,177272,354544,354.4010548591614,1.9234179562677915e-08
42031,177548,177548,355096,354.9055349826813,1.917107327187677e-08
42100,177824,177824,355648,355.3992006778717,1.9055565599172018e-08
42169,178100,178100,356200,355.8777937889099,1.8966599583791368e-08
42238,178376,178376,356752,356.35800075531006,1.889518515394689e-08
42307,178652,178652,357304,356.8611147403717,1.878286299157154e-08
42376,178928,178928,357856,357.3429298400879,1.8708034150103402e-08
42445,179204,179204,358408,357.9163568019867,1.8607228393260128e-08
42514,179480,179480,358960,358.4307358264923,1.8400460837927416e-08
42583,179756,179756,359512,358.950199842453,1.8159282963334205e-08
42652,180032,180032,360064,359.4471786022186,1.7955611969020902e-08
42720,180304,180304,360608,360.00181674957275,1.777905212863198e-08
42789,180580,180580,361160,360.52773880958557,1.7608190241520244e-08
42858,180856,180856,361712,361.1785228252411,1.73583200100653e-08
42927,181132,181132,362264,361.6801288127899,1.7053645442832836e-08
42996,181408,181408,362816,362.19471168518066,1.6925875988396743e-08
43065,181684,181684,363368,362.68168663978577,1.6872398358332787e-08
43134,181960,181960,363920,363.2916359901428,1.6770829680530976e-08
43203,182236,182236,364472,363.8091866970062,1.6601018281398506e-08
43272,182512,182512,365024,364.32421875,1.6414761119238676e-08
43341,182788,182788,365576,364.805392742157,1.6309574691491078e-08
43409,183060,183060,366120,365.2835838794708,1.6142398438558668e-08
43478,183336,183336,366672,365.7607398033142,1.6034279348782667e-08
43547,183612,183612,367224,366.2501440048218,1.5949146983948047e-08
43616,183888,183888,367776,366.7288398742676,1.586934298590346e-08
43685,184164,184164,368328,367.2061257362366,1.5807309838901874e-08
43754,184440,184440,368880,367.6799030303955,1.574366119908707e-08
43823,184716,184716,369432,368.18590688705444,1.5659979362749393e-08
43892,184992,184992,369984,368.6639087200165,1.5531526358519117e-08
43961,185268,185268,370536,369.1376929283142,1.5485223619875414e-08
44030,185544,185544,371088,369.6113398075104,1.5406139855185226e-08
44098,185816,185816,371632,370.07950472831726,1.5327015732567238e-08
44167,186092,186092,372184,370.56775283813477,1.526627322737932e-08
44236,186368,186368,372736,371.0422477722168,1.5164866127681813e-08
44305,186644,186644,373288,371.51371598243713,1.4895653297465927e-08
44374,186920,186920,373840,371.99114966392517,1.4783132638589661e-08
44443,187196,187196,374392,372.49057483673096,1.4700178261095942e-08
44512,187472,187472,374944,372.9672567844391,1.464081258703361e-08
44581,187748,187748,375496,373.4436078071594,1.457072184376416e-08
44650,188024,188024,376048,373.9204828739166,1.4448983035405149e-08
44719,188300,188300,376600,374.4041347503662,1.4400121024460208e-08
44788,188576,188576,377152,374.8864107131958,1.4365513859689097e-08
44856,188848,188848,377696,375.3533308506012,1.4296883362324932e-08
44925,189124,189124,378248,375.8280668258667,1.4195049916950638e-08
44994,189400,189400,378800,376.30389380455017,1.41222855480377e-08
45063,189676,189676,379352,376.7939918041229,1.4067449724420574e-08
45132,189952,189952,379904,377.2731018066406,1.3958838543700092e-08
45201,190228,190228,380456,377.7444038391113,1.3858254461930909e-08
45270,190504,190504,381008,378.2207918167114,1.3779557740568337e-08
45339,190780,190780,381560,378.7070438861847,1.3640193823380357e-08
45408,191056,191056,382112,379.1817977428436,1.3294849179345518e-08
45477,191332,191332,382664,379.6586208343506,1.3048054912118135e-08
45545,191604,191604,383208,380.19900703430176,1.296633419594049e-08
45614,191880,191880,383760,380.7521216869354,1.2920184461903211e-08
45683,192156,192156,384312,381.3169598579407,1.2835967816792208e-08
45752,192432,192432,384864,381.8391606807709,1.2635374063836347e-08
45821,192708,192708,385416,382.35349893569946,1.2268381107259145e-08
45890,192984,192984,385968,382.8474168777466,1.1251056291509347e-08
45959,193260,193260,386520,383.3540987968445,1.0655140987036657e-08
46028,193536,193536,387072,383.9781677722931,1.0282882476913885e-08
46097,193812,193812,387624,384.5168068408966,1.0137218135343047e-08
46166,194088,194088,388176,385.050550699234,1.0079348263221941e-08
46235,194364,194364,388728,385.58105087280273,1.0020515276001762e-08
46303,194636,194636,389272,386.1579577922821,9.990432463921724e-09
46372,194912,194912,389824,386.65403866767883,9.953134420979108e-09
46441,195188,195188,390376,387.14723896980286,9.916787171293523e-09
46510,195464,195464,390928,387.6568739414215,9.77220772434774e-09
46579,195740,195740,391480,388.1452338695526,9.685682371202764e-09
46648,196016,196016,392032,388.69078397750854,9.626878130161697e-09
46717,196292,196292,392584,389.2382278442383,9.521347256630837e-09
46786,196568,196568,393136,389.7477607727051,9.350486866134259e-09
46855,196844,196844,393688,390.25181579589844,9.058346851406907e-09
46924,197120,197120,394240,390.7405126094818,8.980620824167765e-09
46992,197392,197392,394784,391.2474477291107,8.913816126085181e-09
47061,197668,197668,395336,391.7372977733612,8.883720640832215e-09
47130,197944,197944,395888,392.2149178981781,8.834838241282082e-09
47199,198220,198220,396440,392.69472789764404,8.80717884057288e-09
47268,198496,198496,396992,393.1832377910614,8.76959077079573e-09
47337,198772,198772,397544,393.6761920452118,8.396559820535782e-09
47406,199048,199048,398096,394.1472358703613,7.697257444737086e-09
47475,199324,199324,398648,394.61879086494446,7.1879491194523704e-09
47544,199600,199600,399200,395.0909128189087,6.879690368770713e-09
47613,199876,199876,399752,395.57858085632324,6.651807322929095e-09
47682,200152,200152,400304,396.05532789230347,6.577756432901497e-09
47750,200424,200424,400848,396.5331027507782,6.4639847859304e-09
47819,200700,200700,401400,397.01554894447327,6.382253833026478e-09
47888,200976,200976,401952,397.4875919818878,6.3466599460061094e-09
47957,201252,201252,402504,398.05284571647644,6.321390368371481e-09
48026,201528,201528,403056,398.59196186065674,6.300697561686111e-09
48095,201804,201804,403608,399.12306690216064,6.27713806947328e-09
48164,202080,202080,404160,399.6855869293213,6.245453856939552e-09
48233,202356,202356,404712,400.2020049095154,6.194431107750746e-09
48302,202632,202632,405264,400.7430908679962,6.141611811039899e-09
48371,202908,202908,405816,401.30093693733215,6.0987899585010706e-09
48439,203180,203180,406360,401.83267092704773,6.061387114364413e-09
48508,203456,203456,406912,402.3458659648895,6.041132649005496e-09
48577,203732,203732,407464,402.8602776527405,6.012330061279831e-09
48646,204008,204008,408016,403.3982207775116,5.960149013165854e-09
48715,204284,204284,408568,404.1110887527466,5.943761754704202e-09
48784,204560,204560,409120,404.6865029335022,5.905116658312808e-09
48853,204836,204836,409672,405.33615899086,5.850398427986864e-09
48922,205112,205112,410224,405.8239486217499,5.824944870516106e-09
48991,205388,205388,410776,406.3220307826996,5.8052466304908995e-09
49060,205664,205664,411328,406.8220057487488,5.623871372257996e-09
49128,205936,205936,411872,407.30626678466797,5.1950209052941185e-09
49197,206212,206212,412424,407.7838237285614,4.5569015584789734e-09
49266,206488,206488,412976,408.31470584869385,4.4344995480608055e-09
49335,206764,206764,413528,408.8048529624939,4.35398838096287e-09
49404,207040,207040,414080,409.2810230255127,4.308420337132631e-09
49473,207316,207316,414632,409.75422167778015,4.269509467643095e-09
49542,207592,207592,415184,410.2357337474823,4.245218354680386e-09
49611,207868,207868,415736,410.7236957550049,4.211266519152842e-09
49680,208144,208144,416288,411.2348418235779,4.1762690440796006e-09
49749,208420,208420,416840,411.77395272254944,4.16050130949354e-09
49818,208696,208696,417392,412.3603856563568,4.145684578862457e-09
49886,208968,208968,417936,412.8803608417511,4.110247057512067e-09
49955,209244,209244,418488,413.39886474609375,4.049030241792203e-09
50024,209520,209520,419040,413.9005446434021,3.9357215603834355e-09
50093,209796,209796,419592,414.3935878276825,3.842768826812378e-09
50162,210072,210072,420144,414.8926947116852,3.819280656353185e-09
50231,210348,210348,420696,415.38057494163513,3.7879807092814795e-09
50300,210624,210624,421248,415.9393558502197,3.757417929079265e-09
50369,210900,210900,421800,416.45882987976074,3.735801774751609e-09
50438,211176,211176,422352,416.95729994773865,3.6950604747787495e-09
50507,211452,211452,422904,417.44596576690674,3.647564224736588e-09
50575,211724,211724,423448,417.9171736240387,3.5497098215738283e-09
50644,212000,212000,424000,418.3939347267151,3.4249449408725987e-09
50713,212276,212276,424552,418.87975096702576,3.3696260826169682e-09
50782,212552,212552,425104,419.35761880874634,3.3517040602094667e-09
50851,212828,212828,425656,419.8318510055542,3.3181082103516687e-09
50920,213104,213104,426208,420.30975890159607,3.290760446592035e-09
50989,213380,213380,426760,420.78755259513855,3.2350858639959197e-09
51058,213656,213656,427312,421.2766079902649,3.1901595921619057e-09
51127,213932,213932,427864,421.748982667923,3.1636094928587122e-09
51196,214208,214208,428416,422.2713689804077,3.1460277769951864e-09
51265,214484,214484,428968,422.78849482536316,3.1127703068175617e-09
51333,214756,214756,429512,423.306697845459,3.0871637877536724e-09
51402,215032,215032,430064,423.82774567604065,3.0584803187848747e-09
51471,215308,215308,430616,424.3418958187103,3.028341836284192e-09
51540,215584,215584,431168,424.85498881340027,2.9794455381733032e-09
51609,215860,215860,431720,425.3814957141876,2.9277597762108842e-09
51678,216136,216136,432272,425.8888318538666,2.9148358767368383e-09
51747,216412,216412,432824,426.4118158817291,2.8933239988879873e-09
51816,216688,216688,433376,426.9154257774353,2.878282921076666e-09
51885,216964,216964,433928,427.4749827384949,2.870102131058246e-09
51954,217240,217240,434480,428.0511507987976,2.8522446484670953e-09
52022,217512,217512,435024,428.5260407924652,2.8295998004661735e-09
52091,217788,217788,435576,429.00607681274414,2.822336564092519e-09
52160,218064,218064,436128,429.4997887611389,2.8078287180295076e-09
52229,218340,218340,436680,429.978551864624,2.7416271247039067e-09
52298,218616,218616,437232,430.45946073532104,2.6401724505977955e-09
52367,218892,218892,437784,430.93876361846924,2.457781308096212e-09
52436,219168,219168,438336,431.4251039028168,2.3751228470725177e-09
52505,219444,219444,438888,431.9069256782532,2.348258629901946e-09
52574,219720,219720,439440,432.387247800827,2.325631313868198e-09
52643,219996,219996,439992,432.8700969219208,2.3068077653752593e-09
52711,220268,220268,440536,433.36318373680115,2.2863140120358693e-09
52780,220544,220544,441088,433.85587191581726,2.2488127962117253e-09
52849,220820,220820,441640,434.4555928707123,2.2335890405516453e-09
52918,221096,221096,442192,434.96755194664,2.2245026199162873e-09
52987,221372,221372,442744,435.48082876205444,2.2094453615701704e-09
53056,221648,221648,443296,435.9915289878845,2.1956268249099064e-09
53125,221924,221924,443848,436.4737186431885,2.1808678856906877e-09
53194,222200,222200,444400,437.0761127471924,2.1569413107965688e-09
53263,222476,222476,444952,437.62628984451294,2.133473612466227e-09
53332,222752,222752,445504,438.147962808609,2.110115989871607e-09
53401,223028,223028,446056,438.6540858745575,2.0817059322994783e-09
53469,223300,223300,446600,439.19912481307983,2.0729633183188693e-09
53538,223576,223576,447152,439.72119092941284,2.062360247995324e-09
53607,223852,223852,447704,440.2203719615936,2.0543765905478996e-09
53676,224128,224128,448256,440.70250391960144,2.0333344550227096e-09
53745,224404,224404,448808,441.23166584968567,2.0162842299797854e-09
53814,224680,224680,449360,441.7659797668457,2.0064317737002327e-09
53883,224956,224956,449912,442.3088607788086,2.0002907984069454e-09
53952,225232,225232,450464,442.82453870773315,1.990982394717192e-09
54021,225508,225508,451016,443.31033086776733,1.9654918616000283e-09
54090,225784,225784,451568,443.89754581451416,1.953512502379722e-09
54158,226056,226056,452112,444.4168047904968,1.9410854989180417e-09
54227,226332,226332,452664,444.99092197418213,1.9347407238642083e-09
54296,226608,226608,453216,445.50373888015747,1.918317244611672e-09
54365,226884,226884,453768,446.0019438266754,1.8762375151407468e-09
54434,227160,227160,454320,446.5005588531494,1.838625519901394e-09
54503,227436,227436,454872,446.98861479759216,1.8223207056310332e-09
54572,227712,227712,455424,447.4724009037018,1.8081826706384006e-09
54641,227988,227988,455976,447.9542098045349,1.7974920990590113e-09
54710,228264,228264,456528,448.4942636489868,1.7861597172963949e-09
54779,228540,228540,457080,448.99636578559875,1.779741520393808e-09
54848,228816,228816,457632,449.5643746852875,1.76054284124284e-09
54916,229088,229088,458176,450.0652480125427,1.7272635773660054e-09
54985,229364,229364,458728,450.58923172950745,1.683448825600747e-09
55054,229640,229640,459280,451.0712068080902,1.6656943465194279e-09
55123,229916,229916,459832,451.5625648498535,1.6561825994001457e-09
55192,230192,230192,460384,452.04622888565063,1.650047141757345e-09
55261,230468,230468,460936,452.54358673095703,1.63603835046073e-09
55330,230744,230744,461488,453.02367186546326,1.6173012926335166e-09
55399,231020,231020,462040,453.501966714859,1.6056888805898053e-09
55468,231296,231296,462592,453.9765827655792,1.597752390433735e-09
55537,231572,231572,463144,454.453177690506,1.590453249433691e-09
55605,231844,231844,463688,454.9353096485138,1.5829850714672603e-09
55674,232120,232120,464240,455.4127869606018,1.5356057262021622e-09
55743,232396,232396,464792,455.8892867565155,1.4317017288187108e-09
55812,232672,232672,465344,456.3647298812866,1.304646609390832e-09
55881,232948,232948,465896,456.85492181777954,1.1780111838632805e-09
55950,233224,233224,466448,457.3392038345337,1.0682479452866582e-09
56019,233500,233500,467000,457.82509183883667,1.0270785063982181e-09
56088,233776,233776,467552,458.3135597705841,1.0066313637536928e-09
56157,234052,234052,468104,458.8647608757019,9.977432069366327e-10
56226,234328,234328,468656,459.35002398490906,9.865302017253653e-10
56294,234600,234600,469200,459.83343482017517,9.772548067613208e-10
56363,234876,234876,469752,460.31178879737854,9.651332492714114e-10
56432,235152,235152,470304,460.79155683517456,9.510833142698576e-10
56501,235428,235428,470856,461.2826247215271,9.435766775372483e-10
56570,235704,235704,471408,461.7572648525238,9.391447443295818e-10
56639,235980,235980,471960,462.23590874671936,9.216072473410704e-10
56708,236256,236256,472512,462.7122309207916,8.906911659557822e-10
56777,236532,236532,473064,463.20326566696167,8.750427785402999e-10
56846,236808,236808,473616,463.67874097824097,8.600868795331737e-10
56915,237084,237084,474168,464.1593017578125,8.546704874436489e-10
56984,237360,237360,474720,464.636088848114,8.503308026511166e-10
57052,237632,237632,475264,465.1159257888794,8.465086136507355e-10
57121,237908,237908,475816,465.59401679039,8.446288059075626e-10
57190,238184,238184,476368,466.07412981987,8.402862755447936e-10
57259,238460,238460,476920,466.5511407852173,8.317934401491716e-10
57328,238736,238736,477472,467.0298240184784,8.254957847335968e-10
57397,239012,239012,478024,467.5242030620575,7.998583663591589e-10
57466,239288,239288,478576,468.0046169757843,7.541586868695745e-10
57535,239564,239564,479128,468.48600482940674,7.19464717138544e-10
57604,239840,239840,479680,468.96535992622375,7.136943892550313e-10
57673,240116,240116,480232,469.44515895843506,7.108255148554479e-10
57741,240388,240388,480776,469.91805696487427,7.064388980588756e-10
57810,240664,240664,481328,470.3970558643341,7.031242718372024e-10
57879,240940,240940,481880,470.87483978271484,7.001973477719222e-10
57948,241216,241216,482432,471.3526887893677,6.933680251214118e-10
58017,241492,241492,482984,471.8382217884064,6.394342611504823e-10
58086,241768,241768,483536,472.31149077415466,5.786360493521619e-10
58155,242044,242044,484088,472.791298866272,5.611051189403305e-10
58224,242320,242320,484640,473.2658660411835,5.550181324237399e-10
58293,242596,242596,485192,473.7518699169159,5.513870567818612e-10
58362,242872,242872,485744,474.2298996448517,5.477361131055751e-10
58431,243148,243148,486296,474.7173328399658,5.462183482721908e-10
58499,243420,243420,486840,475.1957287788391,5.432613186015048e-10
58568,243696,243696,487392,475.69083070755005,5.411004199176294e-10
58637,243972,243972,487944,476.16540789604187,5.36241165996271e-10
58706,244248,244248,488496,476.6482229232788,5.337082201831936e-10
58775,244524,244524,489048,477.12703371047974,5.318409732037425e-10
58844,244800,244800,489600,477.60350489616394,5.286733399142967e-10
58913,245076,245076,490152,478.09300780296326,5.199007844736455e-10
58982,245352,245352,490704,478.5694646835327,5.091314996023779e-10
59051,245628,245628,491256,479.0492277145386,5.062824328560362e-10
59120,245904,245904,491808,479.52586483955383,5.027733232569621e-10
59188,246176,246176,492352,480.00602173805237,5.015349093610229e-10
59257,246452,246452,492904,480.4874486923218,4.969080652330707e-10
59326,246728,246728,493456,480.9647047519684,4.689934437936e-10
59395,247004,247004,494008,481.4386887550354,4.5996397546798535e-10
59464,247280,247280,494560,481.9193286895752,4.563181738760873e-10
59533,247556,247556,495112,482.39988470077515,4.491002402885118e-10
59602,247832,247832,495664,482.8776078224182,4.4496044561224936e-10
59671,248108,248108,496216,483.3548307418823,4.41403186913556e-10
59740,248384,248384,496768,483.8286609649658,4.3884455431015565e-10
59809,248660,248660,497320,484.3178927898407,4.3721778598119293e-10
59877,248932,248932,497864,484.7874298095703,4.3513891926179973e-10
59946,249208,249208,498416,485.260018825531,4.3215381082997955e-10
60015,249484,249484,498968,485.731675863266,4.2986428668878534e-10
60084,249760,249760,499520,486.226655960083,4.215795308951113e-10
60153,250036,250036,500072,486.7015266418457,4.147537646123436e-10
60222,250312,250312,500624,487.17402482032776,4.129593772402108e-10
60291,250588,250588,501176,487.65276288986206,4.1163538886123826e-10
60360,250864,250864,501728,488.1304018497467,4.100940710695433e-10
60429,251140,251140,502280,488.61781191825867,4.017170007790655e-10
60498,251416,251416,502832,489.0971736907959,3.715517204651431e-10
60567,251692,251692,503384,489.5862138271332,3.4567665577333703e-10
60635,251964,251964,503928,490.060950756073,3.404772362473657e-10
60704,252240,252240,504480,490.55983901023865,3.3772565158503376e-10
60773,252516,252516,505032,491.0431938171387,3.3543300249273077e-10
60842,252792,252792,505584,491.53103280067444,3.34080195492148e-10
60911,253068,253068,506136,492.0428276062012,3.3164114833137674e-10
60980,253344,253344,506688,492.54049587249756,3.2797581429597196e-10
61049,253620,253620,507240,493.0433306694031,3.245656845621023e-10
61118,253896,253896,507792,493.5284585952759,3.2281506217124017e-10
61187,254172,254172,508344,494.01967573165894,3.220310093254724e-10
61256,254448,254448,508896,494.5144658088684,3.1884197138576544e-10
61324,254720,254720,509440,495.0015916824341,3.042496595896231e-10
61393,254996,254996,509992,495.49003767967224,2.927004177103194e-10
61462,255272,255272,510544,495.96612191200256,2.8274654535614354e-10
61531,255548,255548,511096,496.44346594810486,2.804031382962144e-10
61600,255824,255824,511648,496.93802070617676,2.7844219216384224e-10
61669,256100,256100,512200,497.4132149219513,2.769490876510157e-10
61738,256376,256376,512752,497.89046478271484,2.747621104548797e-10
61807,256652,256652,513304,498.38600873947144,2.729666385995145e-10
61876,256928,256928,513856,498.9699957370758,2.7016002141516247e-10
61945,257204,257204,514408,499.51196789741516,2.69227656832365e-10
62014,257480,257480,514960,500.0541708469391,2.6744046264434876e-10
62082,257752,257752,515504,500.80252385139465,2.6523191133971087e-10
62151,258028,258028,516056,501.7229688167572,2.6393112484655907e-10
62220,258304,258304,516608,502.47943663597107,2.5856504310634584e-10
62289,258580,258580,517160,503.22122287750244,2.537248183091794e-10
62358,258856,258856,517712,503.9189577102661,2.522494676317861e-10
62427,259132,259132,518264,504.69376277923584,2.5060146744524133e-10
62496,259408,259408,518816,505.524778842926,2.498404678682855e-10
62565,259684,259684,519368,506.0643389225006,2.488462635754402e-10
62634,259960,259960,519920,506.58583974838257,2.482948550664054e-10
62703,260236,260236,520472,507.14372301101685,2.4709904688209097e-10
62771,260508,260508,521016,507.65938997268677,2.4444524403324717e-10
62840,260784,260784,521568,508.1775028705597,2.4326808496734935e-10
62909,261066,261066,522132,508.6686007976532,2.425466558035443e-10
62978,261342,261342,522684,509.18668961524963,2.419505876936139e-10
63047,261618,261618,523236,509.6890687942505,2.3575229578570296e-10
63116,261894,261894,523788,510.17324686050415,2.1461180573021576e-10
63185,262170,262170,524340,510.756306886673,1.9304151199180117e-10
63254,262446,262446,524892,511.2682387828827,1.8088437156679454e-10
63323,262722,262722,525444,511.82204389572144,1.766901030847456e-10
63392,262998,262998,525996,512.3725688457489,1.741684346087916e-10
63460,263270,263270,526540,513.0307159423828,1.7231710035008167e-10
63529,263546,263546,527092,513.9497380256653,1.7179520100026706e-10
63598,263822,263822,527644,514.6980049610138,1.7101877979551166e-10
63667,264098,264098,528196,515.7242388725281,1.698854197321954e-10
63736,264374,264374,528748,516.3172118663788,1.690932236114274e-10
63805,264650,264650,529300,517.022935628891,1.6764941772676888e-10
63874,264926,264926,529852,517.5816698074341,1.6648122795054715e-10
63943,265202,265202,530404,518.1180427074432,1.6586327169393982e-10
64012,265478,265478,530956,518.6717267036438,1.653875516155829e-10
64081,265754,265754,531508,519.2091069221497,1.649361154940856e-10
64150,266030,266030,532060,519.6864326000214,1.6388943812181412e-10
64218,266302,266302,532604,520.1945128440857,1.6218259622741124e-10
64287,266578,266578,533156,520.7325546741486,1.6066443294340131e-10
64356,266860,266860,533720,521.2358138561249,1.5973169087759508e-10
64425,267136,267136,534272,521.7176818847656,1.589954583034215e-10
64494,267412,267412,534824,522.1926369667053,1.5833787228047472e-10
64563,267688,267688,535376,522.671924829483,1.5795621412644305e-10
64632,267964,267964,535928,523.1444900035858,1.5719342798120898e-10
64701,268240,268240,536480,523.6125688552856,1.5633984281397136e-10
64770,268516,268516,537032,524.0828688144684,1.5522308553145977e-10
64839,268792,268792,537584,524.5660598278046,1.5469470707214966e-10
64907,269064,269064,538128,525.0229017734528,1.520161726644774e-10
64976,269340,269340,538680,525.486359834671,1.50005655663295e-10
65045,269616,269616,539232,525.9544577598572,1.4878544838797851e-10
65114,269892,269892,539784,526.4184367656708,1.481324805534563e-10
65183,270168,270168,540336,526.8961689472198,1.4755017464257888e-10
65252,270444,270444,540888,527.3645639419556,1.4405700325441007e-10
65321,270720,270720,541440,527.8314018249512,1.4275413649421134e-10
65390,270996,270996,541992,528.2984838485718,1.4164171865121527e-10
65459,271272,271272,542544,528.7766499519348,1.4105748384033124e-10
65528,271548,271548,543096,529.2443447113037,1.3988642888721074e-10
65597,271824,271824,543648,529.7288167476654,1.3824004372225948e-10
65665,272096,272096,544192,530.1909618377686,1.3731836850350162e-10
65734,272372,272372,544744,530.6639575958252,1.3673878494525755e-10
65803,272648,272648,545296,531.1515200138092,1.3606897763888546e-10
65872,272924,272924,545848,531.6213598251343,1.3513833417353897e-10
65941,273200,273200,546400,532.1270477771759,1.3322453019151397e-10
66010,273476,273476,546952,532.5967717170715,1.324318620142513e-10
66079,273752,273752,547504,533.1554276943207,1.3167491503280417e-10
66148,274028,274028,548056,533.619256734848,1.3035256045626918e-10
66217,274304,274304,548608,534.0892457962036,1.2933991242322576e-10
66286,274584,274584,549168,534.5723190307617,1.2799011261741937e-10
66354,274856,274856,549712,535.0435497760773,1.2728112888312506e-10
66423,275136,275136,550272,535.5105228424072,1.269776531755683e-10
66492,275412,275412,550824,535.9746487140656,1.26421145656976e-10
66561,275692,275692,551384,536.4405319690704,1.2597204988395968e-10
66630,275968,275968,551936,536.9031617641449,1.2477907905988092e-10
66699,276244,276244,552488,537.3748910427094,1.2399733989265328e-10
66768,276526,276526,553052,537.83846783638,1.2338983220697375e-10
66837,276802,276802,553604,538.2951807975769,1.2197201198055995e-10
66906,277078,277078,554156,538.7535009384155,1.2038260833667676e-10
66975,277354,277354,554708,539.2265067100525,1.195087325645255e-10
67043,277626,277626,555252,539.6795477867126,1.1915446856584062e-10
67112,277906,277906,555812,540.1367428302765,1.187741625905155e-10
67181,278182,278182,556364,540.596314907074,1.1723731729754077e-10
67250,278458,278458,556916,541.0698897838593,1.154999271588429e-10
67319,278734,278734,557468,541.5575108528137,1.1472042723373715e-10
67388,279016,279016,558032,542.0201337337494,1.1428445457592594e-10
67457,279292,279292,558584,542.4806237220764,1.1331242104288649e-10
67526,279568,279568,559136,542.9377846717834,1.1289743507052338e-10
67595,279844,279844,559688,543.4648127555847,1.1171704892953853e-10
67664,280120,280120,560240,544.0069987773895,1.111684592854643e-10
67733,280402,280402,560804,544.4764888286591,1.1096222191644483e-10
67801,280674,280674,561348,544.9431238174438,1.1039537777245288e-10
67870,280950,280950,561900,545.4117226600647,1.0924609982447427e-10
67939,281226,281226,562452,545.887631893158,1.0858180731402792e-10
68008,281502,281502,563004,546.3442566394806,1.0822547397224536e-10
68077,281778,281778,563556,546.8071618080139,1.079871319874029e-10
68146,282054,282054,564108,547.2682816982269,1.0730173332750318e-10
68215,282330,282330,564660,547.747410774231,1.0624507559378357e-10
68284,282606,282606,565212,548.2082996368408,1.055458783174553e-10
68353,282882,282882,565764,548.6656148433685,1.0470220597095206e-10
68422,283160,283160,566320,549.1204307079315,1.0442834161857392e-10
68490,283432,283432,566864,549.5773546695709,1.040471683544823e-10
68559,283708,283708,567416,550.050568819046,1.031774351678362e-10
68628,283984,283984,567968,550.5103828907013,1.0278969528089088e-10
68697,284260,284260,568520,550.9760746955872,1.022504065337219e-10
68766,284536,284536,569072,551.4327816963196,1.0146044244333267e-10
68835,284812,284812,569624,551.9037749767303,9.999176189053676e-11


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n10/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00010609626770019531,542.5060889379029
1,2,1,3,0.0001800060272216797,1666.8595157418215
2,3,2,5,0.0002791881561279297,212.04506609322962
3,4,3,7,0.0003669261932373047,208.02515743800268
4,5,4,9,0.0004439353942871094,207.7222062763633
5,6,5,11,0.0005209445953369141,207.34277179873342
6,7,6,13,0.0005981922149658203,206.84290521249017
7,8,7,15,0.0006742477416992188,206.1892319518037
8,9,8,17,0.0007488727569580078,205.33901138860733
9,10,9,19,0.0008420944213867188,204.23758412764963
10,11,10,21,0.0009171962738037109,202.81140143857675
11,12,11,23,0.0009911060333251953,200.95450579700974
12,13,12,25,0.0010790824890136719,190.5833072731874
13,14,13,27,0.0011670589447021484,173.72377418324155
14,15,14,29,0.001260995864868164,136.19078373965837
15,16,15,31,0.0013451576232910156,118.81474962300322
16,17,16,33,0.0014200210571289062,109.35756653363543
17,18,17,35,0.0014920234680175781,101.88990671760939
18,19,18,37,0.00156402587890625,83.77465309915809
19,20,19,39,0.001634836196899414,64.42534268294193
20,21,20,41,0.0017139911651611328,104.37222934765423
21,22,21,43,0.0017931461334228516,101.36976725742844
22,23,22,45,0.001867055892944336,99.99904759544981
23,24,23,47,0.0019421577453613281,96.28131709773105
24,25,24,49,0.0020182132720947266,87.22735280279764
25,26,25,51,0.002095937728881836,74.55422130888289
26,27,26,53,0.002179861068725586,67.86856403317122
27,28,27,55,0.002254962921142578,62.615958866200494
28,29,28,57,0.002334117889404297,57.66956515369755
29,30,29,59,0.0024149417877197266,32.90945641911591
30,31,30,61,0.0024971961975097656,23.454309436355246
31,32,31,63,0.0025739669799804688,20.437308297240886
32,33,32,65,0.0026519298553466797,57.448985024460804
33,34,33,67,0.0027370452880859375,54.613111909715435
34,35,34,69,0.003016948699951172,46.25721483909821
35,36,35,71,0.0031561851501464844,31.223228971632597
36,37,36,73,0.0032410621643066406,22.77614557805692
37,38,37,75,0.003332853317260742,21.114003593365613
38,39,38,77,0.003422975540161133,20.333008467508023
39,40,39,79,0.0035080909729003906,18.545482068492177
40,41,40,81,0.003583192825317383,19.205731691748937
41,42,41,83,0.0036780834197998047,21.800668450989452
42,43,42,85,0.003756999969482422,20.59523896400334
43,44,43,87,0.0038559436798095703,20.27162333362212
44,45,44,89,0.003936052322387695,19.87235261102326
45,46,45,91,0.0040090084075927734,19.36479376411522
46,47,46,93,0.0040819644927978516,18.726909025896465
47,48,47,95,0.0041501522064208984,17.9278866294255
48,49,48,97,0.004216909408569336,16.93171534501472
49,50,49,99,0.004287004470825195,15.701470612309878
50,51,50,101,0.004355907440185547,14.211645468360668
51,52,51,103,0.004431962966918945,12.465460593844128
52,53,52,105,0.00450587272644043,10.511389352088857
53,54,53,107,0.0045871734619140625,1.7211274189739494
54,55,54,109,0.004663228988647461,13.409862321788362
55,56,55,111,0.004744052886962891,13.261033243488574
56,57,56,113,0.004832029342651367,13.101052378815252
57,58,57,115,0.004915952682495117,12.893022357079781
58,59,58,117,0.004987001419067383,12.621522133724758
59,60,59,119,0.00506901741027832,12.26981008562788
60,61,60,121,0.005136966705322266,11.817341880620468
61,62,61,123,0.005208015441894531,11.240697323316205
62,63,62,125,0.005282163619995117,10.516038812929267
63,64,63,127,0.005349874496459961,3.7552435128580517
64,65,64,129,0.005421876907348633,5.57147963843948
65,66,65,131,0.0055179595947265625,10.96018639854843
66,67,66,133,0.005594015121459961,10.840636348115629
67,68,67,135,0.005667924880981445,10.695918238775139
68,69,68,137,0.005740165710449219,10.504936917837286
69,70,69,139,0.005813121795654297,7.199799799741188
70,71,70,141,0.005911111831665039,4.487726592521903
71,72,71,143,0.00598907470703125,3.688164992125455
72,73,72,145,0.006069183349609375,4.320356014092189
73,74,73,147,0.006140947341918945,4.360248496573518
74,75,74,149,0.006208181381225586,3.8968584235025916
75,76,75,151,0.006273031234741211,3.468219253691397
76,77,76,153,0.006340980529785156,2.990009095731937
77,78,77,155,0.006418943405151367,2.962873458996724
78,79,78,157,0.006487131118774414,2.3753487940119666
79,80,79,159,0.006557941436767578,2.865995402235806
80,81,80,161,0.006628990173339844,2.866574414279671
81,82,81,163,0.006696939468383789,2.619809814425414
82,83,82,165,0.006767988204956055,2.383789273815374
83,84,83,167,0.0068361759185791016,2.1230130384215866
84,85,84,169,0.0069119930267333984,1.8667149821866529
85,86,85,171,0.006989955902099609,1.751478605161731
86,87,86,173,0.007061004638671875,1.4579937912974015
87,88,87,175,0.007130861282348633,1.7616632136774035
88,89,88,177,0.0072021484375,1.837179899096737
89,90,89,179,0.007277011871337891,1.7291257191052187
90,91,90,181,0.007361173629760742,1.6280666626242182
91,92,91,183,0.0074310302734375,1.5112045357337265
92,93,92,185,0.007500886917114258,1.3883647028450417
93,94,93,187,0.007590055465698242,1.2599593870423642
94,95,94,189,0.007659196853637695,1.1274955695667603
95,96,95,191,0.007739067077636719,0.9880639853401243
96,97,96,193,0.007822990417480469,0.8413783323350533
97,98,97,195,0.007910966873168945,0.687962221332964
98,99,98,197,0.007999181747436523,0.5395601916345821
99,100,99,199,0.008083105087280273,0.4625369651120378
100,101,100,201,0.008170127868652344,0.7269251982224049
101,102,101,203,0.008257150650024414,0.664492000806044
102,103,102,205,0.008345842361450195,0.7577753109921761
103,104,103,207,0.008428096771240234,0.7415084039049615
104,105,104,209,0.008580923080444336,0.7277222846502204
105,106,105,211,0.008759021759033203,0.7093116539132149
106,107,106,213,0.008855104446411133,0.686179362531918
107,108,107,215,0.008945941925048828,0.6572566916786748
108,109,108,217,0.009020090103149414,0.6216007993481891
109,110,109,219,0.009109020233154297,0.5782186904318322
110,111,110,221,0.009183168411254883,0.526348092122027
111,112,111,223,0.00925302505493164,0.4658336157007213
112,113,112,225,0.009322166442871094,0.39778457548894974
113,114,113,227,0.009398221969604492,0.3250762814288778
114,115,114,229,0.009472131729125977,0.25253927821215855
115,116,115,231,0.009544134140014648,0.24041401841370916
116,117,116,233,0.009612798690795898,0.2863212880977248
117,118,117,235,0.00968313217163086,0.2165316446378098
118,119,118,237,0.009756088256835938,0.17979442894387035
119,120,119,239,0.00982522964477539,0.16351842298707808
120,121,120,241,0.009896039962768555,0.2479137578322988
121,122,121,243,0.009985923767089844,0.22470004887022174
122,123,122,245,0.010079145431518555,0.21040072385079667
123,124,123,247,0.010159015655517578,0.18838602562963638
124,125,124,249,0.010239124298095703,0.168426596033924
125,126,125,251,0.010316133499145508,0.17145306047624642
126,127,126,253,0.010389089584350586,0.20131516537925237
127,128,127,255,0.010464191436767578,0.19881260928861033
128,129,128,257,0.010538101196289062,0.19629156814808013
129,130,129,259,0.010629892349243164,0.19291485516129822
130,131,130,261,0.010701894760131836,0.18847694705905652
131,132,131,263,0.010773181915283203,0.18268460709196543
132,133,132,265,0.010843992233276367,0.17520883353197814
133,134,133,267,0.010917901992797852,0.16570092871565592
134,135,134,269,0.010992050170898438,0.15384454883457147
135,136,135,271,0.011063098907470703,0.13944263927869235
136,137,136,273,0.011135101318359375,0.12254826985949148
137,138,137,275,0.011205911636352539,0.10361831645411673
138,139,138,277,0.011277914047241211,0.0836296964069761
139,140,139,279,0.01135706901550293,0.06403008568008774
140,141,140,281,0.011451005935668945,0.07062433944522667
141,142,141,283,0.011530160903930664,0.06836576364699194
142,143,142,285,0.011600971221923828,0.05929383906538298
143,144,143,287,0.011673927307128906,0.0460330027563537
144,145,144,289,0.011766195297241211,0.05125827638724003
145,146,145,291,0.011867046356201172,0.07037767842949123
146,147,146,293,0.011938810348510742,0.06999007477387297
147,148,147,295,0.01201009750366211,0.06957186347885545
148,149,148,297,0.012076139450073242,0.06901552860894748
149,150,149,299,0.012153863906860352,0.06827464754107815
150,151,150,301,0.012225151062011719,0.06729228745111673
151,152,151,303,0.012300968170166016,0.06599665559635107
152,153,152,305,0.01237797737121582,0.06429985545818902
153,154,153,307,0.012454032897949219,0.062098195782455866
154,155,154,309,0.01252603530883789,0.05927615507416558
155,156,155,311,0.012600898742675781,0.05571680148863984
156,157,156,313,0.012673139572143555,0.051322490230029494
157,158,157,315,0.012750864028930664,0.04604963931845398
158,159,158,317,0.01282811164855957,0.039957876797503684
159,160,159,319,0.012903928756713867,0.03326288292512263
160,161,160,321,0.01298379898071289,0.026363155428263205
161,162,161,323,0.013064146041870117,0.021086785067088335
162,163,162,325,0.013138055801391602,0.024851665154871378
163,164,163,327,0.013224124908447266,0.02271142048029854
164,165,164,329,0.013309001922607422,0.0171468959459445
165,166,165,331,0.013392925262451172,0.014752841015747685
166,167,166,333,0.01347208023071289,0.019733236772055608
167,168,167,335,0.013555049896240234,0.01930569211686666
168,169,168,337,0.013635873794555664,0.022597443252298063
169,170,169,339,0.013717174530029297,0.022462986386180425
170,171,170,341,0.013788938522338867,0.022323373805563432
171,172,171,343,0.01386404037475586,0.022135892842769678
172,173,172,345,0.013936996459960938,0.021886121626525347
173,174,173,347,0.014019012451171875,0.021554587423748415
174,175,174,349,0.01409006118774414,0.021116844687140167
175,176,175,351,0.014158964157104492,0.020542964490837003
176,177,176,353,0.014230012893676758,0.019797797392129658
177,178,177,355,0.014301061630249023,0.018842669208736083
178,179,178,357,0.014371871948242188,0.01763958448477015
179,180,179,359,0.01444697380065918,0.01615922353689769
180,181,180,361,0.014519214630126953,0.01439368318303452
181,182,181,363,0.01459503173828125,0.012373229811791933
182,183,182,365,0.01466822624206543,0.010182366541901296
183,184,183,367,0.014741182327270508,0.007964192748299327
184,185,184,369,0.014814138412475586,0.007382265803966273
185,186,185,371,0.014887094497680664,0.007816810335025627
186,187,186,373,0.014956235885620117,0.006841316673029504
187,188,187,375,0.015043020248413086,0.005147661044628372
188,189,188,377,0.015127182006835938,0.005426660908576986
189,190,189,379,0.015214920043945312,0.007882892643287159
190,191,190,381,0.015304088592529297,0.0076619617344173396
191,192,191,383,0.015382051467895508,0.007473741322714033
192,193,192,385,0.015456199645996094,0.007222047148729345
193,194,193,387,0.015533924102783203,0.00689946497721021
194,195,194,389,0.015614986419677734,0.006490237746161834
195,196,195,391,0.01569390296936035,0.005983487638855283
196,197,196,393,0.01577305793762207,0.005372844074292427
197,198,197,395,0.0158538818359375,0.0046661423407632265
198,199,198,397,0.01593780517578125,0.0038859038494895863
199,200,199,399,0.016019105911254883,0.003085935477811096
200,201,200,401,0.016103029251098633,0.002591964705444328
201,202,201,403,0.016185998916625977,0.0031526820098663807
202,203,202,405,0.01625800132751465,0.003758116022331218
203,204,203,407,0.016332149505615234,0.0034987043294671346
204,205,204,409,0.016405105590820312,0.003185740193549921
205,206,205,411,0.016482830047607422,0.002919467514590297
206,207,206,413,0.016561031341552734,0.002966160174863141
207,208,207,415,0.016640186309814453,0.003337094630019871
208,209,208,417,0.016723155975341797,0.003282451287028511
209,210,209,419,0.016798973083496094,0.003225468601615311
210,211,210,421,0.016885042190551758,0.0031492863271203827
211,212,211,423,0.01696610450744629,0.003050104826039938
212,213,212,425,0.017045021057128906,0.0029220392828241165
213,214,213,427,0.017121076583862305,0.002759277765343828
214,215,214,429,0.01720404624938965,0.0025564950270562815
215,216,215,431,0.01727914810180664,0.0023106481638622677
216,217,216,433,0.01735520362854004,0.0020230727295785455
217,218,217,435,0.01743006706237793,0.0017023599483190484
218,219,218,437,0.017504215240478516,0.001365684601311561
219,220,219,439,0.017575979232788086,0.0010392881823125175
220,221,220,441,0.017650127410888672,0.0012283550337118029
221,222,221,443,0.017724037170410156,0.0012237679098390476
222,223,222,445,0.01779317855834961,0.0015988968799219663
223,224,223,447,0.017863988876342773,0.0015847346362420991
224,225,224,449,0.01793694496154785,0.0015701939522313703
225,226,225,451,0.01800990104675293,0.0015508160537717342
226,227,226,453,0.018085956573486328,0.0015251379772172286
227,228,227,455,0.018156051635742188,0.0014913127518086692
228,229,228,457,0.018234968185424805,0.0014471023890910845
229,230,229,459,0.018306970596313477,0.001389923341716876
230,231,230,461,0.018398046493530273,0.001317008090359222
231,232,231,463,0.018477916717529297,0.001225768972332609
232,233,232,465,0.018629074096679688,0.0011144548171447295
233,234,233,467,0.018732070922851562,0.000983152444820352
234,235,234,469,0.01881718635559082,0.0008350249759892974
235,236,235,471,0.018900156021118164,0.000677331301625878
236,237,236,473,0.01898193359375,0.0005212974684618184
237,238,237,475,0.019067049026489258,0.0005589212132141582
238,239,238,477,0.019150972366333008,0.0005459505598027518
239,240,239,479,0.019234180450439453,0.00044763544556626427
240,241,240,481,0.019318103790283203,0.0003547760984369796
241,242,241,483,0.019401073455810547,0.0003667649691736517
242,243,242,485,0.01947617530822754,0.000549058616030713
243,244,243,487,0.01955413818359375,0.0005444289216806876
244,245,244,489,0.019633054733276367,0.0005400340524011891
245,246,245,491,0.019717931747436523,0.0005341719868895568
246,247,246,493,0.01980304718017578,0.0005263900135027435
247,248,247,495,0.019877910614013672,0.0005161144207033198
248,249,248,497,0.019952058792114258,0.0005026396642898976
249,250,249,499,0.020032167434692383,0.0004851329476626917
250,251,250,501,0.020115137100219727,0.0004626681207309647
251,252,251,503,0.02018904685974121,0.00043431478963227134
252,253,252,505,0.02025890350341797,0.0003993131005613359
253,254,253,507,0.020334959030151367,0.0003573622686260982
254,255,254,509,0.020419836044311523,0.0003090186130530489
255,256,255,511,0.020503997802734375,0.00025610915276333423
256,257,256,513,0.020588159561157227,0.0002019132926007696
257,258,257,515,0.02068305015563965,0.00017450694568841186
258,259,258,517,0.020773887634277344,0.00019436813560974925
259,260,259,519,0.020860910415649414,0.00017604355145553246
260,261,260,521,0.020940065383911133,0.0001335294456189907
261,262,261,523,0.021021127700805664,0.00011398072412582067
262,263,262,525,0.021095991134643555,0.0001644532914452953
263,264,263,527,0.021168947219848633,0.0001489811224609695
264,265,264,529,0.021240949630737305,0.00015677161528193623
265,266,265,531,0.021320104598999023,0.00016405516917176557
266,267,266,533,0.021400928497314453,0.00015675169416871383
267,268,267,535,0.021494150161743164,0.00014952884451548338
268,269,268,537,0.021574020385742188,0.00013963200366948195
269,270,269,539,0.021663188934326172,0.000128095014206235
270,271,270,541,0.0217440128326416,0.00011362725173365497
271,272,271,543,0.021837949752807617,9.8410865403169e-05
272,273,272,545,0.0219271183013916,7.987083376213825e-05
273,274,273,547,0.02202296257019043,0.00010222847510153164
274,275,274,549,0.02211904525756836,0.00010700553941139655
275,276,275,551,0.022207021713256836,0.00010688143675687707
276,277,276,553,0.022296905517578125,0.00010493296313880637
277,278,277,555,0.02237701416015625,0.00010142895960917406
278,279,278,557,0.02245306968688965,9.681389132894115e-05
279,280,279,559,0.02252984046936035,9.106882193263568e-05
280,281,280,561,0.02260899543762207,8.389244888001287e-05
281,282,281,563,0.022684097290039062,7.533544311373369e-05
282,283,282,565,0.022754192352294922,6.532271703403199e-05
283,284,283,567,0.022821903228759766,5.4552639106991297e-05
284,285,284,569,0.022890090942382812,4.282568974293239e-05
285,286,285,571,0.02295994758605957,4.7055893780206465e-05
286,287,286,573,0.023029088973999023,6.39266005227027e-05
287,288,287,575,0.02309703826904297,6.370754650793207e-05
288,289,288,577,0.023164987564086914,6.345640450467803e-05
289,290,289,579,0.023234844207763672,6.31215172638044e-05
290,291,290,581,0.023308992385864258,6.267399039722037e-05
291,292,291,583,0.02338385581970215,6.207773816515656e-05
292,293,292,585,0.023463010787963867,6.128629183457477e-05
293,294,293,587,0.023543119430541992,6.024088991138827e-05
294,295,294,589,0.02362203598022461,5.8868857026007636e-05
295,296,295,591,0.0236968994140625,5.708308143613754e-05
296,297,296,593,0.02376413345336914,5.4783846627794496e-05
297,298,297,595,0.02383708953857422,5.1865074575106045e-05
298,299,298,597,0.023906230926513672,4.82280528850719e-05
299,300,299,599,0.02397608757019043,4.3806507880524136e-05
300,301,300,601,0.02404308319091797,3.8605772019052284e-05
301,302,301,603,0.024108171463012695,3.275218925397876e-05
302,303,302,605,0.024178028106689453,2.6533584141225033e-05
303,304,303,607,0.024253129959106445,2.039366703711251e-05
304,305,304,609,0.024321794509887695,2.2109622842606254e-05
305,306,305,611,0.024389028549194336,2.1096923104176122e-05
306,307,306,613,0.024466991424560547,2.0586026768461124e-05
307,308,307,615,0.024543046951293945,2.634409054155125e-05
308,309,308,617,0.024621963500976562,2.5026196672696643e-05
309,310,309,619,0.024738073348999023,2.3759712628610043e-05
310,311,310,621,0.02482008934020996,2.2176657077480136e-05
311,312,311,623,0.024903059005737305,2.0210057683450215e-05
312,313,312,625,0.024983882904052734,1.7921974835530702e-05
313,314,313,627,0.025070905685424805,1.5253337074545635e-05
314,315,314,629,0.025175809860229492,1.2606707196632908e-05
315,316,315,631,0.02526712417602539,1.2332092437718158e-05
316,317,316,633,0.025345802307128906,1.722337405938138e-05
317,318,317,635,0.02544999122619629,1.713165138502278e-05
318,319,318,637,0.02556300163269043,1.7049672927066865e-05
319,320,319,639,0.025668859481811523,1.693930211329276e-05
320,321,320,641,0.02577996253967285,1.6791832595320148e-05
321,322,321,643,0.025880813598632812,1.6595336238261327e-05
322,323,322,645,0.02596902847290039,1.6334548615953898e-05
323,324,323,647,0.026058197021484375,1.5990281433908304e-05
324,325,324,649,0.026135921478271484,1.5539101364583402e-05
325,326,325,651,0.026211977005004883,1.4953610446405971e-05
326,327,326,653,0.02628302574157715,1.4203937486792851e-05
327,328,327,655,0.0263519287109375,1.3261313344338953e-05
328,329,328,657,0.026441097259521484,1.2104733532399194e-05
329,330,329,659,0.026517152786254883,1.0731306455729167e-05
330,331,330,661,0.026588916778564453,9.169373058883452e-06
331,332,331,663,0.026660919189453125,7.490231938856399e-06
332,333,332,665,0.026731014251708984,5.8092393565527265e-06
333,334,333,667,0.026803970336914062,5.889851101478503e-06
334,335,334,669,0.02688288688659668,6.4361928364806016e-06
335,336,335,671,0.026955127716064453,4.785509397114417e-06
336,337,336,673,0.02702808380126953,3.961371894218908e-06
337,338,337,675,0.02709794044494629,5.096463217136462e-06
338,339,338,677,0.027174949645996094,5.578598244009184e-06
339,340,339,679,0.02724480628967285,5.852375065008761e-06
340,341,340,681,0.027313947677612305,5.687510238724106e-06
341,342,341,683,0.027383089065551758,5.468490344797307e-06
342,343,342,685,0.027476072311401367,5.200009309982704e-06
343,344,343,687,0.027565956115722656,4.855150496010245e-06
344,345,344,689,0.027659177780151367,4.438363823713637e-06
345,346,345,691,0.02774214744567871,3.935427149315263e-06
346,347,346,693,0.027816057205200195,3.3765662399994337e-06
347,348,347,695,0.027888059616088867,2.74344554252618e-06
348,349,348,697,0.027956008911132812,2.3207120960021382e-06
349,350,349,699,0.02803206443786621,3.45257823852768e-06
350,351,350,701,0.02810811996459961,3.229726353593783e-06
351,352,351,703,0.028181076049804688,2.974636945381511e-06
352,353,352,705,0.028250932693481445,2.7624786820855548e-06
353,354,353,707,0.028358936309814453,2.5055054551571225e-06
354,355,354,709,0.0284271240234375,2.844857549735781e-06
355,356,355,711,0.02849602699279785,2.621395517242284e-06
356,357,356,713,0.028649091720581055,2.463361431063036e-06
357,358,357,715,0.02873396873474121,2.2001654750612353e-06
358,359,358,717,0.028812885284423828,1.9992413594752266e-06
359,360,359,719,0.028936147689819336,2.195593647176598e-06
360,361,360,721,0.02903294563293457,2.2478609177920356e-06
361,362,361,723,0.0291290283203125,2.321982450097876e-06
362,363,362,725,0.029228925704956055,2.2844723528792943e-06
363,364,363,727,0.02931499481201172,2.2355914461851397e-06
364,365,364,729,0.029397010803222656,2.1721205557707293e-06
365,366,365,731,0.029475927352905273,2.089756162630882e-06
366,367,366,733,0.02955913543701172,1.9845790481919176e-06
367,368,367,735,0.02963113784790039,1.8525525007429005e-06
368,369,368,737,0.029695987701416016,1.6908557834962112e-06
369,370,369,739,0.029764890670776367,1.4990177877442895e-06
370,371,370,741,0.0298309326171875,1.2810491079634126e-06
371,372,371,743,0.029900074005126953,1.046572344601988e-06
372,373,372,745,0.029968976974487305,8.12461790515587e-07
373,374,373,747,0.030035018920898438,8.264169336341189e-07
374,375,374,749,0.030102014541625977,1.1847776694199893e-06
375,376,375,751,0.030167818069458008,1.0912427654542998e-06
376,377,376,753,0.030236005783081055,1.0193820679509448e-06
377,378,377,755,0.0303041934967041,9.245568683160205e-07
378,379,378,757,0.03037095069885254,8.170688706794758e-07
379,380,379,759,0.030440092086791992,6.893147063596336e-07
380,381,380,761,0.030508041381835938,5.776930418620683e-07
381,382,381,763,0.03057694435119629,7.316230671012965e-07
382,383,382,765,0.030668020248413086,7.544259296603818e-07
383,384,383,767,0.03075098991394043,8.005587310871629e-07
384,385,384,769,0.030828237533569336,7.930980269044938e-07
385,386,385,771,0.03097701072692871,7.832714799190624e-07
386,387,386,773,0.031095027923583984,7.70339032055037e-07
387,388,387,775,0.031211137771606445,7.532906677296758e-07
388,389,388,777,0.03131818771362305,7.310147496375663e-07
389,390,389,779,0.03142213821411133,7.022071462504639e-07
390,391,390,781,0.03153800964355469,6.654742080229828e-07
391,392,391,783,0.031655073165893555,6.195073144393044e-07
392,393,392,785,0.03175997734069824,5.634137052141592e-07
393,394,393,787,0.031854867935180664,4.972180192010728e-07
394,395,394,789,0.031941890716552734,4.224918815823644e-07
395,396,395,791,0.0320279598236084,3.4287166762537767e-07
396,397,396,793,0.03210711479187012,2.6402109947696565e-07
397,398,397,795,0.03217506408691406,2.8369072228559563e-07
398,399,398,797,0.032243967056274414,2.769966028396949e-07
399,400,399,799,0.032328128814697266,2.257160510630308e-07
400,401,400,801,0.03240203857421875,1.79390289502608e-07
401,402,401,803,0.03253507614135742,1.8701649900054167e-07
402,403,402,805,0.03260922431945801,2.7242205637549266e-07
403,404,403,807,0.032752037048339844,2.636201755363454e-07
404,405,404,809,0.03284788131713867,2.5556026232912507e-07
405,406,405,811,0.032930850982666016,2.451331086077341e-07
406,407,406,813,0.033010005950927734,2.3181185997220735e-07
407,408,407,815,0.03308916091918945,2.152311162426964e-07
408,409,408,817,0.03316903114318848,1.9503753365301479e-07
409,410,409,819,0.03324294090270996,1.7138156099914433e-07
410,411,410,821,0.033316850662231445,1.447541937792651e-07
411,412,411,823,0.03339195251464844,1.1692359740969683e-07
412,413,412,825,0.0334780216217041,8.86915409874495e-08
413,414,413,827,0.03355002403259277,1.0862881574639176e-07
414,415,414,829,0.03362107276916504,1.421035774799367e-07
415,416,415,831,0.033689022064208984,1.380360444917253e-07
416,417,416,833,0.03375816345214844,1.3339631238941687e-07
417,418,417,835,0.03382682800292969,1.2776216384478133e-07
418,419,418,837,0.03389406204223633,1.204427491933262e-07
419,420,419,839,0.03396320343017578,1.1148471667684191e-07
420,421,420,841,0.034034013748168945,1.0053750886971714e-07
421,422,421,843,0.0341038703918457,8.795079485227783e-08
422,423,422,845,0.03418087959289551,7.360962396267747e-08
423,424,423,847,0.034253835678100586,5.985606753354997e-08
424,425,424,849,0.03432798385620117,6.714087736621095e-08
425,426,425,851,0.03440594673156738,8.489666430933948e-08
426,427,426,853,0.034484148025512695,8.189915813514593e-08
427,428,427,855,0.03456282615661621,7.942319159233574e-08
428,429,428,857,0.03463315963745117,7.600180725535225e-08
429,430,429,859,0.03470182418823242,7.17478210456023e-08
430,431,430,861,0.034770965576171875,6.638737699617803e-08
431,432,431,863,0.03483986854553223,5.995706838785387e-08
432,433,432,865,0.034912109375,5.2355689216707066e-08
433,434,433,867,0.034986019134521484,4.409191473267053e-08
434,435,434,869,0.03506302833557129,3.4968821775496634e-08
435,436,435,871,0.0351409912109375,3.435488109330986e-08
436,437,436,873,0.03521585464477539,4.957058915868285e-08
437,438,437,875,0.03528904914855957,4.892424705507414e-08
438,439,438,877,0.03535914421081543,4.8213208102145275e-08
439,440,439,879,0.03542804718017578,4.729591487503236e-08
440,441,440,881,0.03550004959106445,4.6090550299828674e-08
441,442,441,883,0.0355830192565918,4.452799364823933e-08
442,443,442,885,0.035661935806274414,4.2524817605431294e-08
443,444,443,887,0.03574204444885254,3.999784216814137e-08
444,445,444,889,0.03582191467285156,3.6875438166605635e-08
445,446,445,891,0.03589892387390137,3.3123524173485615e-08
446,447,446,893,0.03597903251647949,2.8779528689903044e-08
447,448,447,895,0.036054134368896484,2.3992806852752408e-08
448,449,448,897,0.0361180305480957,1.9043206981874968e-08
449,450,449,899,0.036202192306518555,1.5365137676366465e-08
450,451,450,901,0.03627204895019531,1.8045725150593875e-08
451,452,451,903,0.03635096549987793,1.6783975465686262e-08
452,453,452,905,0.0364229679107666,1.4844414065158843e-08
453,454,453,907,0.036496877670288086,1.2113289553451002e-08
454,455,454,909,0.036570072174072266,1.656605077343612e-08
455,456,455,911,0.036643028259277344,1.626423773586727e-08
456,457,456,913,0.03671622276306152,1.7262547308387873e-08
457,458,457,915,0.036812782287597656,1.6927151416820445e-08
458,459,458,917,0.03688406944274902,1.647746000456257e-08
459,460,459,919,0.03695487976074219,1.5908847568206828e-08
460,461,460,921,0.037023067474365234,1.5173614541431305e-08
461,462,461,923,0.03709816932678223,1.424924188867324e-08
462,463,462,925,0.03720712661743164,1.3105873740899538e-08
463,464,463,927,0.03730607032775879,1.1737704577291375e-08
464,465,464,929,0.03738093376159668,1.0155798935548254e-08
465,466,465,931,0.03747892379760742,8.43158995282325e-09
466,467,466,933,0.03761601448059082,6.634532699740784e-09
467,468,467,935,0.03771805763244629,5.613964814693456e-09
468,469,468,937,0.03781318664550781,8.612929793321277e-09
469,470,469,939,0.037919044494628906,7.486632225590422e-09
470,471,470,941,0.0380251407623291,6.530364639418519e-09
471,472,471,943,0.038178205490112305,7.937071236417938e-09
472,473,472,945,0.0383760929107666,7.38646905831857e-09
473,474,473,947,0.03846406936645508,7.034562008968805e-09
474,475,474,949,0.03854084014892578,6.448150693565756e-09
475,476,475,951,0.03873491287231445,5.88911818397361e-09
476,477,476,953,0.03883719444274902,5.053678089990798e-09
477,478,477,955,0.03894209861755371,5.458840237413302e-09
478,479,478,957,0.03902101516723633,6.234186309794356e-09
479,480,479,959,0.039093017578125,6.183821799953213e-09
480,481,480,961,0.03917288780212402,6.118635078102181e-09
481,482,481,963,0.039244890213012695,6.032941275172608e-09
482,483,482,965,0.039314985275268555,5.919741553276812e-09
483,484,483,967,0.03939008712768555,5.771079600367884e-09
484,485,484,969,0.039457082748413086,5.57778589643932e-09
485,486,485,971,0.03952503204345703,5.3294811877229e-09
486,487,486,973,0.03959512710571289,5.015369293724071e-09
487,488,487,975,0.039662837982177734,4.6263599613798745e-09
488,489,488,977,0.039733171463012695,4.15804599637651e-09
489,490,489,979,0.03979992866516113,3.6149758464461275e-09
490,491,490,981,0.03986692428588867,3.015682847893983e-09
491,492,491,983,0.03993105888366699,2.3955204506006946e-09
492,493,492,985,0.03999590873718262,1.9294805038623023e-09
493,494,493,987,0.04006004333496094,2.2523969795889677e-09
494,495,494,989,0.040125131607055664,2.0494148728259296e-09
495,496,495,991,0.040193796157836914,1.5556632936622797e-09
496,497,496,993,0.04026198387145996,1.528356713059957e-09
497,498,497,995,0.04032588005065918,2.3128210870254084e-09
498,499,498,997,0.04041004180908203,2.3023176304331676e-09
499,500,499,999,0.04047703742980957,2.293298209049469e-09
500,501,500,1001,0.04054403305053711,2.280948736198089e-09
501,502,501,1003,0.04061102867126465,2.264571149235163e-09
502,503,502,1005,0.04067707061767578,2.242597126470766e-09
503,504,503,1007,0.040740013122558594,2.2135082092616518e-09
504,505,504,1009,0.04081106185913086,2.174832475906895e-09
505,506,505,1011,0.04087686538696289,2.1239257176940385e-09
506,507,506,1013,0.040946006774902344,2.0575197179438285e-09
507,508,507,1015,0.04102301597595215,1.9716793218240915e-09
508,509,508,1017,0.041097164154052734,1.8623987259289231e-09
509,510,509,1019,0.04117012023925781,1.7261217840117508e-09
510,511,510,1021,0.041236162185668945,1.5605590888249127e-09
511,512,511,1023,0.04130697250366211,1.366837803567545e-09
512,513,512,1025,0.04137396812438965,1.1504472480059875e-09
513,514,513,1027,0.041442155838012695,9.234773737215119e-10
514,515,514,1029,0.041506052017211914,7.017111196639038e-10
515,516,515,1031,0.04157614707946777,8.239718845634621e-10
516,517,516,1033,0.041654109954833984,7.656643308531208e-10
517,518,517,1035,0.04172992706298828,9.989066288617897e-10
518,519,518,1037,0.04180479049682617,9.155920296240036e-10
519,520,519,1039,0.04187512397766113,8.54103465877821e-10
520,521,520,1041,0.041970014572143555,7.648832740097262e-10
521,522,521,1043,0.04206490516662598,6.795719942436703e-10
522,523,522,1045,0.04213404655456543,6.139722293149492e-10
523,524,523,1047,0.04220294952392578,7.817061952699347e-10
524,525,524,1049,0.04227113723754883,7.486708726516493e-10
525,526,525,1051,0.04234004020690918,7.221798936971286e-10
526,527,526,1053,0.04241013526916504,6.850284036624972e-10
527,528,527,1055,0.04249405860900879,6.400468715448851e-10
528,529,528,1057,0.04257798194885254,5.834176030921633e-10
529,530,529,1059,0.04264998435974121,5.180526342009666e-10
530,531,530,1061,0.04273390769958496,4.40664577633904e-10
531,532,531,1063,0.04281306266784668,3.675633171781986e-10
532,533,532,1065,0.042945146560668945,4.203877259719344e-10
533,534,533,1067,0.043035030364990234,4.947163003891985e-10
534,535,534,1069,0.043109893798828125,4.733008917502649e-10
535,536,535,1071,0.04318094253540039,4.552046455132722e-10
536,537,536,1073,0.0432741641998291,4.2978978370695876e-10
537,538,537,1075,0.0433502197265625,3.9949435451408675e-10
538,539,538,1077,0.04342317581176758,3.611701283332229e-10
539,540,539,1079,0.043496131896972656,3.1830433647107326e-10
540,541,540,1081,0.04357504844665527,2.664770467686392e-10
541,542,541,1083,0.043660879135131836,2.294269537083464e-10
542,543,542,1085,0.043734073638916016,3.1220610842998927e-10
543,544,543,1087,0.04380512237548828,2.909540995603016e-10
544,545,544,1089,0.043879032135009766,2.641238861997499e-10
545,546,545,1091,0.04395914077758789,2.578145532115048e-10
546,547,546,1093,0.04404497146606445,2.8292842106717354e-10
547,548,547,1095,0.044129133224487305,2.749477395597132e-10
548,549,548,1097,0.04420113563537598,2.647713716412269e-10
549,550,549,1099,0.044445037841796875,2.522782038657e-10
550,551,550,1101,0.044548988342285156,2.3622875426061366e-10
551,552,551,1103,0.04463005065917969,2.167500697898633e-10
552,553,552,1105,0.044708967208862305,1.9311400696944083e-10
553,554,553,1107,0.044786930084228516,1.6661820849717503e-10
554,555,554,1109,0.044862985610961914,1.3662290704227962e-10
555,556,555,1111,0.044931888580322266,1.1255252923000918e-10
556,557,556,1113,0.045004844665527344,1.6111117245439242e-10
557,558,557,1115,0.04507613182067871,1.5149321385370566e-10
558,559,558,1117,0.04514789581298828,1.5219391262085882e-10
559,560,559,1119,0.04521894454956055,1.604437358230849e-10
560,561,560,1121,0.04528999328613281,1.565684615178189e-10
561,562,561,1123,0.04535794258117676,1.524624852662434e-10
562,563,562,1125,0.045456886291503906,1.4686183209281416e-10
563,564,563,1127,0.04553103446960449,1.3977480334307464e-10
564,565,564,1129,0.04561209678649902,1.308201379789687e-10
565,566,565,1131,0.0456850528717041,1.1982586473070732e-10
566,567,566,1133,0.04575181007385254,1.0673744502651324e-10
567,568,567,1135,0.04582095146179199,9.168593581113906e-11


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n10/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0001227855682373047,542.5060889379029
1,3,2,5,0.000308990478515625,409.6353395028631
2,5,4,9,0.0004279613494873047,294.6291701407307
3,7,6,13,0.0005319118499755859,197.24353095956113
4,9,8,17,0.0006310939788818359,131.75231590331154
5,11,10,21,0.0007450580596923828,85.91880628167098
6,13,12,25,0.0008530616760253906,65.03254300872524
7,15,14,29,0.0009658336639404297,41.285630953207175
8,17,16,33,0.001065969467163086,708.9286288511969
9,19,18,37,0.0016109943389892578,90.74981504690473
10,21,20,41,0.0017349720001220703,343.97713763941863
11,23,22,45,0.0018351078033447266,67.42351124787656
12,25,24,49,0.001920938491821289,2.926531869696776
13,27,26,53,0.002023935317993164,0.8458899526752867
14,29,28,57,0.002123117446899414,0.40033047553612555
15,31,30,61,0.0022368431091308594,0.23949100905408657
16,33,32,65,0.0023500919342041016,0.14267893333496387
17,35,34,69,0.0024640560150146484,0.08989523195733685
18,37,36,73,0.0025641918182373047,0.05019054962887102
19,39,38,77,0.0026607513427734375,0.033796314602463365
20,41,40,81,0.002763032913208008,0.012232801326463252
21,43,42,85,0.00286102294921875,0.00794360602484813
22,45,44,89,0.002958059310913086,0.004516048899076068
23,47,46,93,0.0030570030212402344,0.0028958014185372794
24,49,48,97,0.0031528472900390625,0.0038183401737358455
25,51,50,101,0.0032520294189453125,0.00368636533871323
26,53,52,105,0.0033311843872070312,0.0011457816367236226
27,55,54,109,0.003429889678955078,0.0006711793933413259
28,57,56,113,0.0035278797149658203,0.0004963280231576432
29,59,58,117,0.003760814666748047,0.00017160827918518928
30,61,60,121,0.0038788318634033203,0.00011406481495617977
31,63,62,125,0.004155874252319336,7.366308278459671e-05
32,65,64,129,0.004277944564819336,4.6293139937841126e-05
33,67,66,133,0.004394054412841797,3.0629956288868006e-05
34,69,68,137,0.0045299530029296875,1.92000904765276e-05
35,71,70,141,0.0046541690826416016,1.7787308873988487e-05
36,73,72,145,0.004758119583129883,4.0746577426772744e-05
37,75,74,149,0.004904985427856445,1.52698950794787e-05
38,77,76,153,0.005007028579711914,2.984659097657674e-05
39,79,78,157,0.005110025405883789,1.617973584199071e-05
40,81,80,161,0.0052258968353271484,1.2504439878285665e-05
41,83,82,165,0.0053730010986328125,2.8141597023106934e-05
42,85,84,169,0.005499839782714844,9.474317229480118e-06
43,87,86,173,0.005630970001220703,1.7468965446954278e-05
44,89,88,177,0.005836009979248047,1.0642520285212278e-05
45,91,90,181,0.00595402717590332,7.185910828408354e-06
46,93,92,185,0.006062030792236328,1.9668811091630222e-05
47,95,94,189,0.006180763244628906,6.668482856264436e-06
48,97,96,193,0.006283998489379883,7.54654828190053e-06
49,99,98,197,0.006384849548339844,9.826472179159455e-06
50,101,100,201,0.0064928531646728516,3.269104228819362e-06
51,103,102,205,0.0065920352935791016,1.4301033558340755e-05
52,105,104,209,0.006700992584228516,2.6335771760111477e-06
53,107,106,213,0.006829977035522461,1.4939626893556758e-06
54,109,108,217,0.007004976272583008,1.123455257947926e-06
55,111,110,221,0.007113933563232422,2.6469106951997896e-06
56,113,112,225,0.007215023040771484,8.904794723025736e-07
57,115,114,229,0.007312774658203125,1.4595479215346358e-06
58,117,116,233,0.007415056228637695,1.0828099531956602e-06
59,119,118,237,0.007523059844970703,5.510888223406352e-07
60,121,120,241,0.007631778717041016,2.2079135782737187e-06
61,123,122,245,0.007759809494018555,7.457191667324768e-07
62,125,124,249,0.007866144180297852,3.0037919219575125e-07
63,127,126,253,0.007967948913574219,1.2630523651797249e-06
64,129,128,257,0.008070945739746094,3.9423083706593603e-07
65,131,130,261,0.008178949356079102,1.324683964430944e-07
66,133,132,265,0.008276939392089844,2.2807799632852549e-07
67,135,134,269,0.008383989334106445,1.5634237135822493e-07
68,137,136,273,0.008485794067382812,8.848841478844611e-08
69,139,138,277,0.008599042892456055,3.1016277999440296e-07
70,141,140,281,0.008711814880371094,1.0583239011307027e-07
71,143,142,285,0.00880885124206543,6.058055551810527e-08
72,145,144,289,0.008932113647460938,2.091656142180143e-07
73,147,146,293,0.009054899215698242,7.140351966636998e-08
74,149,148,297,0.00917506217956543,4.2605894667862044e-08
75,151,150,301,0.009284019470214844,1.3905252300018056e-07
76,153,152,305,0.009387016296386719,4.7507209729943315e-08
77,155,154,309,0.009511947631835938,3.310365856786001e-08
78,157,156,313,0.009613990783691406,8.696510610582679e-08
79,159,158,317,0.009720087051391602,2.9504378381331194e-08
80,161,160,321,0.009817123413085938,3.662608199786493e-08
81,163,162,325,0.009914875030517578,4.171053964235848e-08
82,165,164,329,0.010015010833740234,1.4489362122527584e-08
83,167,166,333,0.010120868682861328,2.3089712122960386e-08
84,169,168,337,0.010452032089233398,5.00561583775111e-09
85,171,170,341,0.010764122009277344,6.855330156277213e-10
86,173,172,345,0.010889053344726562,2.454316844316619e-09
87,175,174,349,0.011236190795898438,7.434604907140231e-10
88,177,176,353,0.01137399673461914,2.514862597678451e-10
89,179,178,357,0.011487007141113281,2.5989020731145174e-10
90,181,180,361,0.01164698600769043,3.8729857812688484e-10
91,183,182,365,0.011807918548583984,1.2641235914026003e-10
92,185,184,369,0.01194906234741211,5.647297242013917e-10
93,187,186,373,0.012091875076293945,7.733581872838501e-11


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n10/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00012922286987304688,542.5060889379029
1,3,2,5,0.00023126602172851562,437.43651362206106
2,5,4,9,0.00031113624572753906,346.892909191993
3,7,6,13,0.00037932395935058594,272.4410508043172
4,9,8,17,0.00044536590576171875,212.0408052814726
5,11,10,21,0.0005252361297607422,166.69432451752004
6,13,12,25,0.0005900859832763672,133.3304668212217
7,15,14,29,0.0006620883941650391,107.35953271733689
8,17,16,33,0.0007352828979492188,88.87089053936654
9,19,18,37,0.000797271728515625,76.1398167426833
10,21,20,41,0.0008602142333984375,67.44790329122274
11,23,22,45,0.0009200572967529297,61.45455630670913
12,25,24,49,0.0009961128234863281,57.180289873746716
13,27,26,53,0.0010633468627929688,32.92216846413252
14,29,28,57,0.0011262893676757812,31.518443218527352
15,31,30,61,0.0012001991271972656,24.72720172827196
16,33,32,65,0.0012621879577636719,23.33459462064131
17,35,34,69,0.001329183578491211,22.151841447159534
18,37,36,73,0.0013911724090576172,21.11384989663433
19,39,38,77,0.0014531612396240234,20.177799263942465
20,41,40,81,0.0015223026275634766,19.315904047119957
21,43,42,85,0.0015861988067626953,18.51028419655607
22,45,44,89,0.0016529560089111328,17.749467052294484
23,47,46,93,0.0017333030700683594,17.02606537440799
24,49,48,97,0.001814126968383789,16.33526544552545
25,51,50,101,0.0018973350524902344,15.673856844393542
26,53,52,105,0.0019762516021728516,15.03961723765496
27,55,54,109,0.0020542144775390625,14.43092656652283
28,57,56,113,0.0021212100982666016,13.846527844572298
29,59,58,117,0.0021843910217285156,13.285380784392757
30,61,60,121,0.0022492408752441406,12.746573668322059
31,63,62,125,0.0023102760314941406,12.229271402786075
32,65,64,129,0.0023822784423828125,11.73268578584889
33,67,66,133,0.002452373504638672,11.256059205387718
34,69,68,137,0.0025212764739990234,10.798656292137993
35,71,70,141,0.002582073211669922,8.39592091400955
36,73,72,145,0.0026421546936035156,4.807180204852864
37,75,74,149,0.002704143524169922,4.023356988760287
38,77,76,153,0.0027642250061035156,3.393523621498062
39,79,78,157,0.0028252601623535156,2.8887254847740422
40,81,80,161,0.002887248992919922,2.4851131696304947
41,83,82,165,0.0029761791229248047,2.162965654776843
42,85,84,169,0.003045320510864258,1.9059427008094105
43,87,86,173,0.003117084503173828,1.7005272660684978
44,89,88,177,0.0031921863555908203,1.5356101471635766
45,91,90,181,0.0032732486724853516,1.4021649940177654
46,93,92,185,0.003337383270263672,1.29296885196626
47,95,94,189,0.0034041404724121094,1.2023402684526479
48,97,96,193,0.0034711360931396484,1.125886017566264
49,99,98,197,0.0035352706909179688,1.0602608170370167
50,101,100,201,0.003608226776123047,1.0029492168279008
51,103,102,205,0.0036783218383789062,0.952077184145346
52,105,104,209,0.0037581920623779297,0.9062565711432994
53,107,106,213,0.0038530826568603516,0.8644615135804111
54,109,108,217,0.00400996208190918,0.8259331238963948
55,111,110,221,0.004088163375854492,0.7901076806078755
56,113,112,225,0.0041620731353759766,0.7565634428527174
57,115,114,229,0.004229307174682617,0.724981742874848
58,117,116,233,0.0043010711669921875,0.6951187638521601
59,119,118,237,0.004373073577880859,0.6667851784912998
60,121,120,241,0.0044362545013427734,0.6398315013212134
61,123,122,245,0.00449824333190918,0.6141375602228843
62,125,124,249,0.004557132720947266,0.5896049221526096
63,127,126,253,0.004615306854248047,0.5661514312745007
64,129,128,257,0.004672050476074219,0.5437072558799938
65,131,130,261,0.004740238189697266,0.5222120133509649
66,133,132,265,0.004802227020263672,0.5016126666547746
67,135,134,269,0.00487518310546875,0.48186197451157853
68,137,136,273,0.004937410354614258,0.4629173403621552
69,139,138,277,0.0050013065338134766,0.4447399499004458
70,141,140,281,0.005068063735961914,0.4272941185270261
71,143,142,285,0.005132198333740234,0.4105467924451946
72,145,144,289,0.005208253860473633,0.3944671629681253
73,147,146,293,0.005277156829833984,0.37902636485747954
74,149,148,297,0.005341291427612305,0.36419723752005984
75,151,150,301,0.005403280258178711,0.3499541336139532
76,153,152,305,0.005469322204589844,0.3362727637166878
77,155,154,309,0.005563259124755859,0.3231300686668245
78,157,156,313,0.005631208419799805,0.31050411332950506
79,159,158,317,0.005700111389160156,0.29837399710317286
80,161,160,321,0.005767345428466797,0.2867197776221733
81,163,162,325,0.005837202072143555,0.2755224049618734
82,165,164,329,0.0058972835540771484,0.264763664273821
83,167,166,333,0.0059583187103271484,0.25442612525509783
84,169,168,337,0.006021261215209961,0.24449309720447854
85,171,170,341,0.006083250045776367,0.23494858868975627
86,173,172,345,0.006145000457763672,0.22577727105662584
87,175,174,349,0.0062122344970703125,0.2169644451648659
88,177,176,353,0.006274223327636719,0.2084960108641294
89,179,178,357,0.0063402652740478516,0.20035843881217194
90,181,180,361,0.006415128707885742,0.19253874431826218
91,183,182,365,0.00648808479309082,0.18502446295078648
92,185,184,369,0.006554126739501953,0.17780362769415875
93,187,186,373,0.006646156311035156,0.17086474748029595
94,189,188,377,0.00670623779296875,0.16419678694729425
95,191,190,381,0.00676727294921875,0.15778914730273347
96,193,192,385,0.006832122802734375,0.15163164818787586
97,195,194,389,0.006898164749145508,0.14571451045692685
98,197,196,393,0.006965160369873047,0.14002833979499105
99,199,198,397,0.007026195526123047,0.13456411111017286
100,201,200,401,0.0070841312408447266,0.1293131536454797
101,203,202,405,0.00714421272277832,0.1242671367610666
102,205,204,409,0.00720524787902832,0.119418056342969
103,207,206,413,0.0072650909423828125,0.11475822180171974
104,209,208,417,0.00732421875,0.11028024362626516
105,211,210,421,0.00738525390625,0.10597702146181512
106,213,212,425,0.007445096969604492,0.10184173268567166
107,215,214,429,0.007512092590332031,0.097867821453361
108,217,216,433,0.007573127746582031,0.0940489881945397
109,219,218,437,0.007643222808837891,0.09037917953473365
110,221,220,441,0.007708311080932617,0.08685257862487926
111,223,222,445,0.0077800750732421875,0.08346359585967973
112,225,224,449,0.00785207748413086,0.08020685996693115
113,227,226,453,0.007914066314697266,0.07707720945282427
114,229,228,457,0.00797724723815918,0.07406968438644278
115,231,230,461,0.008037090301513672,0.07117951851053991
116,233,232,465,0.008097171783447266,0.06840213166422236
117,235,234,469,0.008156299591064453,0.0657331225042708
118,237,236,473,0.008216142654418945,0.06316826151363833
119,239,238,477,0.008276224136352539,0.060703484285325494
120,241,240,481,0.008334159851074219,0.05833488506937798
121,243,242,485,0.008395195007324219,0.056058710573958004
122,245,244,489,0.008459091186523438,0.05387135400948592
123,247,246,493,0.008524179458618164,0.0517693493660266
124,249,248,497,0.008585214614868164,0.04974936591458566
125,251,250,501,0.008649349212646484,0.04780820292483645
126,253,252,505,0.008709192276000977,0.04594278458801918
127,255,254,509,0.008773088455200195,0.044150155139731764
128,257,256,513,0.008842229843139648,0.04242747417265084
129,259,258,517,0.008916378021240234,0.04077201213318525
130,261,260,521,0.009057044982910156,0.03918114599335533
131,263,262,525,0.009133100509643555,0.03765235509293629
132,265,264,529,0.009198188781738281,0.036183217142472676
133,267,266,533,0.009261131286621094,0.0347714043841882
134,269,268,537,0.009325027465820312,0.03341467990172313
135,271,270,541,0.009395360946655273,0.032110894074000244
136,273,272,545,0.009464263916015625,0.030857981168538454
137,275,274,549,0.00953817367553711,0.029653956066670706
138,277,276,553,0.009604215621948242,0.02849691111747005
139,279,278,557,0.009670257568359375,0.027385013113885876
140,281,280,561,0.009810209274291992,0.026316500387274358
141,283,282,565,0.009885311126708984,0.025289680015730745
142,285,284,569,0.009949207305908203,0.024302925140422784
143,287,286,573,0.010012149810791016,0.02335467238769415
144,289,288,577,0.010073184967041016,0.022443419391185677
145,291,290,581,0.01015019416809082,0.021567722411174058
146,293,292,585,0.010310173034667969,0.0207261940460586
147,295,294,589,0.010491132736206055,0.01991750103434357
148,297,296,593,0.010570287704467773,0.019140362140932815
149,299,298,597,0.010652303695678711,0.01839354612757884
150,301,300,601,0.01071929931640625,0.017675869801107177
151,303,302,605,0.010787248611450195,0.016986196138833374
152,305,304,609,0.010856389999389648,0.016323432486491395
153,307,306,613,0.010925054550170898,0.01568652882699357
154,309,308,617,0.010991096496582031,0.015074476116181014
155,311,310,621,0.011060237884521484,0.014486304684300722
156,313,312,625,0.01112818717956543,0.0139210826991567
157,315,314,629,0.011193275451660156,0.013377914689659789
158,317,316,633,0.011263370513916016,0.012855940126829165
159,319,318,637,0.01133418083190918,0.012354332060096231
160,321,320,641,0.01140141487121582,0.011872295807441974
161,323,322,645,0.011466264724731445,0.011409067695363307
162,325,324,649,0.011536121368408203,0.01096391384973048
163,327,326,653,0.011602163314819336,0.010536129032149278
164,329,328,657,0.011678218841552734,0.010125035523190344
165,331,330,661,0.011758089065551758,0.009729982047777334
166,333,332,665,0.011837244033813477,0.009350342743906918
167,335,334,669,0.011919260025024414,0.008985516170928926
168,337,336,673,0.012005090713500977,0.008634924355919307
169,339,338,677,0.012279033660888672,0.008298011878808914
170,341,340,681,0.01238703727722168,0.007974244991635111
171,343,342,685,0.012484073638916016,0.007663110773239533
172,345,344,689,0.012548208236694336,0.007364116316489199
173,347,346,693,0.012629985809326172,0.007076787947184648
174,349,348,697,0.012703418731689453,0.006800670473723784
175,351,350,701,0.012992143630981445,0.006535326465692955
176,353,352,705,0.013074159622192383,0.0062803355611051595
177,355,354,709,0.013147115707397461,0.006035293800050675
178,357,356,713,0.013219118118286133,0.005799812984792163
179,359,358,717,0.013290166854858398,0.0055735200649312385
180,361,360,721,0.01350712776184082,0.005356056546015208
181,363,362,725,0.013598203659057617,0.005147077921546557
182,365,364,729,0.013665199279785156,0.0049462531276114555
183,367,366,733,0.013733148574829102,0.0047532640178327154
184,369,368,737,0.013798236846923828,0.004567804859592573
185,371,370,741,0.013865232467651367,0.004389581849685407
186,373,372,745,0.013933181762695312,0.004218312648510509
187,375,374,749,0.014000177383422852,0.004053725933287791
188,377,376,753,0.014069080352783203,0.0038955609675745536
189,379,378,757,0.014136075973510742,0.0037435671886148487
190,381,380,761,0.014205217361450195,0.0035975038103751057
191,383,382,765,0.014281272888183594,0.003457139441701459
192,385,384,769,0.014349222183227539,0.0033222517201560242
193,387,386,773,0.014419317245483398,0.003192626959459821
194,389,388,777,0.014489173889160156,0.003068059810943388
195,391,390,781,0.014561176300048828,0.0029483529382753463
196,393,392,785,0.0146331787109375,0.002833316705001248
197,395,394,789,0.014721155166625977,0.002722768873867421
198,397,396,793,0.014796018600463867,0.0026165343181881627
199,399,398,797,0.01487112045288086,0.0025144447443065506
200,401,400,801,0.014945030212402344,0.0024163384253150194
201,403,402,805,0.015025138854980469,0.0023220599442951534
202,405,404,809,0.015099287033081055,0.0022314599485026955
203,407,406,813,0.015172243118286133,0.0021443949125897585
204,409,408,817,0.015248298645019531,0.0020607269114610726
205,411,410,821,0.01532125473022461,0.0019803234014133327
206,413,412,825,0.015394210815429688,0.0019030570103310742
207,415,414,829,0.015469074249267578,0.0018288053358947493
208,417,416,833,0.01554417610168457,0.001757450751668465
209,419,418,837,0.015610218048095703,0.0016888802207537842
210,421,420,841,0.01567220687866211,0.0016229851166448882
211,423,422,845,0.015735149383544922,0.0015596610514120451
212,425,424,849,0.015807390213012695,0.0014988077097954973
213,427,426,853,0.015882253646850586,0.0014403286907647504
214,429,428,857,0.015955209732055664,0.0013841313547355385
215,431,430,861,0.016028165817260742,0.0013301266764229728
216,433,432,865,0.016100168228149414,0.0012782291043898716
217,435,434,869,0.016172170639038086,0.0012283564250635051
218,437,436,873,0.01624441146850586,0.0011804296325674715
219,439,438,877,0.016318321228027344,0.0011343728039809155
220,441,440,881,0.016393184661865234,0.0010901129782634996
221,443,442,885,0.016468286514282227,0.001047580041340157
222,445,444,889,0.01656818389892578,0.001006706614968704
223,447,446,893,0.016646146774291992,0.0009674279495677968
224,449,448,897,0.01671910285949707,0.0009296818220983381
225,451,450,901,0.016793251037597656,0.0008934084372555575
226,453,452,905,0.016866207122802734,0.0008585503326549087
227,455,454,909,0.01694011688232422,0.0008250522881398469
228,457,456,913,0.017013072967529297,0.0007928612381221467
229,459,458,917,0.017089128494262695,0.0007619261873273383
230,461,460,921,0.01716303825378418,0.0007321981301929986
231,463,462,925,0.01723623275756836,0.0007036299733131437
232,465,464,929,0.017312049865722656,0.0006761764609298715
233,467,466,933,0.017400264739990234,0.0006497941025223991
234,469,468,937,0.017475128173828125,0.0006244411049403347
235,471,470,941,0.017550230026245117,0.0006000773054399955
236,473,472,945,0.017626285552978516,0.0005766641085249237
237,475,474,949,0.01770329475402832,0.0005541644241753831
238,477,476,953,0.01777815818786621,0.0005325426100877916
239,479,478,957,0.017853260040283203,0.0005117644141278338
240,481,480,961,0.017927169799804688,0.000491796920929384
241,483,482,965,0.01800227165222168,0.0004726084992122925
242,485,484,969,0.018077373504638672,0.0004541687519210449
243,487,486,973,0.01815319061279297,0.00043644846782421614
244,489,488,977,0.01822519302368164,0.00041941957578599904
245,491,490,981,0.018287181854248047,0.00040305509962813016
246,493,492,985,0.01834416389465332,0.0003873291159777035
247,495,494,989,0.018429279327392578,0.0003722167125160981
248,497,496,993,0.0185091495513916,0.0003576939493652657
249,499,498,997,0.01857924461364746,0.0003437378204199749
250,501,500,1001,0.018657207489013672,0.0003303262172771757
251,503,502,1005,0.01872730255126953,0.0003174378941979059
252,505,504,1009,0.01879119873046875,0.00030505243439892996
253,507,506,1013,0.018854141235351562,0.00029315021766018116
254,509,508,1017,0.018917083740234375,0.0002817123892437782
255,511,510,1021,0.018985271453857422,0.0002707208301286335
256,513,512,1025,0.019054174423217773,0.00026015812823353623
257,515,514,1029,0.019118070602416992,0.00025000755084199377
258,517,516,1033,0.019181251525878906,0.00024025301804221868
259,519,518,1037,0.019242048263549805,0.00023087907751694528
260,521,520,1041,0.01930522918701172,0.00022187087956473953
261,523,522,1045,0.019365310668945312,0.00021321415400175287
262,525,524,1049,0.019497394561767578,0.00020489518750305984
263,527,526,1053,0.01956915855407715,0.00019690080172976877
264,529,528,1057,0.01963329315185547,0.00018921833255674273
265,531,530,1061,0.019697189331054688,0.00018183560990394035
266,533,532,1065,0.019774198532104492,0.00017474093854457978
267,535,534,1069,0.019843101501464844,0.00016792307960275093
268,537,536,1073,0.01991724967956543,0.00016137123277423145
269,539,538,1077,0.01998734474182129,0.00015507501893295106
270,541,540,1081,0.020072221755981445,0.00014902446417375872
271,543,542,1085,0.02014017105102539,0.00014320998362964382
272,545,544,1089,0.020203113555908203,0.00013762236625912378
273,547,546,1093,0.020269155502319336,0.0001322527607170798
274,549,548,1097,0.02033519744873047,0.00012709266082525737
275,551,550,1101,0.020403385162353516,0.00012213389222079615
276,553,552,1105,0.020473241806030273,0.00011736859970032754
277,555,554,1109,0.02054119110107422,0.00011278923428642776
278,557,556,1113,0.020611047744750977,0.0001083885417104131
279,559,558,1117,0.020679235458374023,0.00010415955074536173
280,561,560,1121,0.020740270614624023,0.00010009556196515134
281,563,562,1125,0.0208132266998291,9.619013775718002e-05
282,565,564,1129,0.020876169204711914,9.24370912856949e-05
283,567,566,1133,0.02094101905822754,8.883047712913854e-05
284,569,568,1137,0.021007299423217773,8.536458207691356e-05
285,571,570,1141,0.021069049835205078,8.203391565899023e-05
286,573,572,1145,0.021128177642822266,7.88332016849376e-05
287,575,574,1149,0.021190166473388672,7.575736984077025e-05
288,577,576,1153,0.021254301071166992,7.280154756302927e-05
289,579,578,1157,0.021320343017578125,6.996105236090507e-05
290,581,580,1161,0.02138519287109375,6.723138462409784e-05
291,583,582,1165,0.0214540958404541,6.460822027175152e-05
292,585,584,1169,0.021555185317993164,6.208740369563189e-05
293,587,586,1173,0.02161717414855957,5.9664941725685195e-05
294,589,588,1177,0.021677255630493164,5.733699684196163e-05
295,591,590,1181,0.021737337112426758,5.509988125370876e-05
296,593,592,1185,0.021796226501464844,5.2950051109475524e-05
297,595,594,1189,0.021856069564819336,5.088410071673632e-05
298,597,596,1193,0.02191615104675293,4.889875750964775e-05
299,599,598,1197,0.021975040435791016,4.699087623684391e-05
300,601,600,1201,0.02203536033630371,4.5157434751187295e-05
301,603,602,1205,0.02209615707397461,4.339552855336934e-05
302,605,604,1209,0.02215719223022461,4.17023664608714e-05
303,607,606,1213,0.022220134735107422,4.0075266494943766e-05
304,609,608,1217,0.022286176681518555,3.8511651036839826e-05
305,611,610,1221,0.022345304489135742,3.700904304467993e-05
306,613,612,1225,0.022413253784179688,3.556506218770733e-05
307,615,614,1229,0.02247333526611328,3.417742112603628e-05
308,617,616,1233,0.022539138793945312,3.284392159346263e-05
309,619,618,1237,0.022607088088989258,3.156245114667204e-05
310,621,620,1241,0.022681236267089844,3.033097975973181e-05
311,623,622,1245,0.022736310958862305,2.9147556675579586e-05
312,625,624,1249,0.022792339324951172,2.8010307145211304e-05
313,627,626,1253,0.022863149642944336,2.691742963252594e-05
314,629,628,1257,0.022925138473510742,2.5867192861570113e-05
315,631,630,1261,0.02298903465270996,2.485793314001625e-05
316,633,632,1265,0.0230562686920166,2.3888051739747515e-05
317,635,634,1269,0.023122310638427734,2.295601205309767e-05
318,637,636,1273,0.02318739891052246,2.206033783225679e-05
319,639,638,1277,0.0232541561126709,2.1199610009351152e-05
320,641,640,1281,0.023324251174926758,2.037246517637046e-05
321,643,642,1285,0.023391246795654297,1.9577593039723553e-05
322,645,644,1289,0.023449182510375977,1.881373447127672e-05
323,647,646,1293,0.023513078689575195,1.807967922259979e-05
324,649,648,1297,0.023572206497192383,1.737426464706643e-05
325,651,650,1301,0.02363109588623047,1.6696373192604184e-05
326,653,652,1305,0.02369213104248047,1.6044931056640427e-05
327,655,654,1309,0.0237581729888916,1.5418906167735643e-05
328,657,656,1313,0.02382636070251465,1.4817306902354164e-05
329,659,658,1317,0.02390122413635254,1.423918016854675e-05
330,661,660,1321,0.023967266082763672,1.3683610235753103e-05
331,663,662,1325,0.024031400680541992,1.3149717032309135e-05
332,665,664,1329,0.024096012115478516,1.2636654581721193e-05
333,667,666,1333,0.024160146713256836,1.2143610401392343e-05
334,669,668,1337,0.024239301681518555,1.1669803155498594e-05
335,671,670,1341,0.024306297302246094,1.1214482524565392e-05
336,673,672,1345,0.02437615394592285,1.0776927185484824e-05
337,675,674,1349,0.02444911003112793,1.0356443885939597e-05
338,677,676,1353,0.024520158767700195,9.952366541121925e-06
339,679,678,1357,0.02459120750427246,9.564055112007646e-06
340,681,680,1361,0.02466726303100586,9.190894419656837e-06
341,683,682,1365,0.024735212326049805,8.832293240746775e-06
342,685,684,1369,0.02480316162109375,8.487683660061348e-06
343,687,686,1373,0.02487325668334961,8.15651979393122e-06
344,689,688,1377,0.024944305419921875,7.838276833193686e-06
345,691,690,1381,0.025008201599121094,7.5324507338155735e-06
346,693,692,1385,0.025069236755371094,7.238557185738857e-06
347,695,694,1389,0.025132179260253906,6.95613038904859e-06
348,697,696,1393,0.02519512176513672,6.684722993034641e-06
349,699,698,1397,0.025265216827392578,6.423905085704579e-06
350,701,700,1401,0.025336027145385742,6.173263596810279e-06
351,703,702,1405,0.025403261184692383,5.932401341219535e-06
352,705,704,1409,0.025471210479736328,5.700936845786831e-06
353,707,706,1413,0.025544166564941406,5.478503338642731e-06
354,709,708,1417,0.025606155395507812,5.264748568292871e-06
355,711,710,1421,0.02567911148071289,5.059333834531598e-06
356,713,712,1425,0.02574896812438965,4.861933754187416e-06
357,715,714,1429,0.025809288024902344,4.672235656337158e-06
358,717,716,1433,0.025870084762573242,4.489938928445738e-06
359,719,718,1437,0.02593207359313965,4.314755015406312e-06
360,721,720,1441,0.02599811553955078,4.1464061853515565e-06
361,723,722,1445,0.026064157485961914,3.984625725606023e-06
362,725,724,1449,0.026143312454223633,3.829157607719305e-06
363,727,726,1453,0.026240110397338867,3.679755344339546e-06
364,729,728,1457,0.02632617950439453,3.536182242741062e-06
365,731,730,1461,0.026407241821289062,3.3982109706382505e-06
366,733,732,1465,0.02649521827697754,3.2656229015866322e-06
367,735,734,1469,0.0265653133392334,3.1382080761556143e-06
368,737,736,1473,0.026642322540283203,3.0157645658837727e-06
369,739,738,1477,0.026731014251708984,2.8980984585155546e-06
370,741,740,1481,0.02681708335876465,2.785023277418465e-06
371,743,742,1485,0.0269010066986084,2.6763599658872474e-06
372,745,744,1489,0.027021169662475586,2.5719363879908382e-06
373,747,746,1493,0.02718520164489746,2.4715871344671204e-06
374,749,748,1497,0.027300119400024414,2.3751531427249943e-06
375,751,750,1501,0.02742624282836914,2.282481754367066e-06
376,753,752,1505,0.02753305435180664,2.1934260789694313e-06
377,755,754,1509,0.02770829200744629,2.1078451232280347e-06
378,757,756,1513,0.02783203125,2.02560329466403e-06
379,759,758,1517,0.027938127517700195,1.946570311442325e-06
380,761,760,1521,0.028028249740600586,1.870620925400814e-06
381,763,762,1525,0.02811717987060547,1.797634912380939e-06
382,765,764,1529,0.028180360794067383,1.727496533290736e-06
383,767,766,1533,0.028257131576538086,1.6600946971764276e-06
384,769,768,1537,0.028331995010375977,1.5953227233555441e-06
385,771,770,1541,0.028409242630004883,1.533078015006749e-06
386,773,772,1545,0.0284731388092041,1.4732618591773384e-06
387,775,774,1549,0.02854132652282715,1.4157796074242164e-06
388,777,776,1553,0.028614282608032227,1.3605400483330717e-06
389,779,778,1557,0.028695106506347656,1.3074558261597286e-06
390,781,780,1561,0.028783082962036133,1.2564428407111703e-06
391,783,782,1565,0.028872251510620117,1.2074201014662186e-06
392,785,784,1569,0.02899622917175293,1.1603102328314388e-06
393,787,786,1573,0.029078006744384766,1.1150383794015295e-06
394,789,788,1577,0.029146194458007812,1.071532881101824e-06
395,791,790,1581,0.029212236404418945,1.0297248175264282e-06
396,793,792,1585,0.029279232025146484,9.895480275183042e-07
397,795,794,1589,0.029348134994506836,9.509387963885513e-07
398,797,796,1593,0.0294952392578125,9.138359743289207e-07
399,799,798,1597,0.029577255249023438,8.781807706531322e-07
400,801,800,1601,0.029671192169189453,8.439167391227624e-07
401,803,802,1605,0.029770374298095703,8.109896565583979e-07
402,805,804,1609,0.029858112335205078,7.793472169709408e-07
403,807,806,1613,0.02994513511657715,7.489394277567106e-07
404,809,808,1617,0.03002333641052246,7.197180338116877e-07
405,811,810,1621,0.030091047286987305,6.916367787312482e-07
406,813,812,1625,0.03015613555908203,6.646511436101068e-07
407,815,814,1629,0.03021836280822754,6.387184082220201e-07
408,817,816,1633,0.030280351638793945,6.137975421983264e-07
409,819,818,1637,0.030344247817993164,5.898489574442705e-07
410,821,820,1641,0.03040623664855957,5.668347926299798e-07
411,823,822,1645,0.030476093292236328,5.447186626595682e-07
412,825,824,1649,0.030559301376342773,5.234652944780737e-07
413,827,826,1653,0.030643224716186523,5.030412389383088e-07
414,829,828,1657,0.03072834014892578,4.834140404312521e-07
415,831,830,1661,0.030810117721557617,4.645526457478158e-07
416,833,832,1665,0.030879974365234375,4.4642719628741204e-07
417,835,834,1669,0.030950307846069336,4.290089561459663e-07
418,837,836,1673,0.031022071838378906,4.1227022083558453e-07
419,839,838,1677,0.03110027313232422,3.9618474264776e-07
420,841,840,1681,0.03116631507873535,3.8072678864824034e-07
421,843,842,1685,0.031235218048095703,3.658719467096191e-07
422,845,844,1689,0.0312960147857666,3.515966448210108e-07
423,847,846,1693,0.0313572883605957,3.378784530737118e-07
424,849,848,1697,0.0314180850982666,3.2469539706482245e-07
425,851,850,1701,0.0314791202545166,3.1202676204288107e-07
426,853,852,1705,0.031539201736450195,2.998523557813865e-07
427,855,854,1709,0.031606197357177734,2.8815301742548464e-07
428,857,856,1713,0.03168010711669922,2.7691016790896364e-07
429,859,858,1717,0.03174138069152832,2.6610590895013917e-07
430,861,860,1721,0.03180432319641113,2.5572330378450633e-07
431,863,862,1725,0.031867265701293945,2.457457419435445e-07
432,865,864,1729,0.03193020820617676,2.3615740742846477e-07
433,867,866,1733,0.03199410438537598,2.269432864331384e-07
434,869,868,1737,0.0320591926574707,2.1808861280632527e-07
435,871,870,1741,0.032125234603881836,2.095794167965561e-07
436,873,872,1745,0.03218722343444824,2.0140227058579363e-07
437,875,874,1749,0.03225421905517578,1.9354415811040682e-07
438,877,876,1753,0.03232526779174805,1.859925975104904e-07
439,879,878,1757,0.0323944091796875,1.7873569060827695e-07
440,881,880,1761,0.032479286193847656,1.7176198205531542e-07
441,883,882,1765,0.032546043395996094,1.6506037396324237e-07
442,885,884,1769,0.032616376876831055,1.5862015106099078e-07
443,887,886,1773,0.03267717361450195,1.52431279859872e-07
444,889,888,1777,0.03273439407348633,1.4648391433177982e-07
445,891,890,1781,0.03279829025268555,1.4076855224087703e-07
446,893,892,1785,0.03286337852478027,1.352761332558194e-07
447,895,894,1789,0.032923221588134766,1.2999801368305085e-07
448,897,896,1793,0.03298306465148926,1.249259499642107e-07
449,899,898,1797,0.033042192459106445,1.20051683983753e-07
450,901,900,1801,0.033106327056884766,1.1536767629439138e-07
451,903,902,1805,0.0331723690032959,1.1086635251225883e-07
452,905,904,1809,0.03323221206665039,1.0654063159871462e-07
453,907,906,1813,0.03329610824584961,1.0238375788116406e-07
454,909,908,1817,0.03335714340209961,9.838900482199322e-08
455,911,910,1821,0.033419132232666016,9.455014605144168e-08
456,913,912,1825,0.033480167388916016,9.086109699860813e-08
457,915,914,1829,0.033550262451171875,8.731592264543317e-08
458,917,916,1833,0.033614158630371094,8.390911336722207e-08
459,919,918,1837,0.0336911678314209,8.063529745986107e-08
460,921,920,1841,0.03375840187072754,7.748910028430733e-08
461,923,922,1845,0.033820152282714844,7.446572314357436e-08
462,925,924,1849,0.03391122817993164,7.156025661712576e-08
463,927,926,1853,0.03398013114929199,6.87682370631272e-08
464,929,928,1857,0.03404426574707031,6.60851279979245e-08
465,931,930,1861,0.034110307693481445,6.350660951679668e-08
466,933,932,1865,0.0341792106628418,6.102883955984016e-08
467,935,934,1869,0.03424215316772461,5.864764971484541e-08
468,937,936,1873,0.03430604934692383,5.6359352343640924e-08
469,939,938,1877,0.03437209129333496,5.4160442384920695e-08
470,941,940,1881,0.03443717956542969,5.2047205948678984e-08
471,943,942,1885,0.03450131416320801,5.001645557045838e-08
472,945,944,1889,0.03456521034240723,4.806497947765475e-08
473,947,946,1893,0.03462815284729004,4.618968148958354e-08
474,949,948,1897,0.034690141677856445,4.438748774473138e-08
475,951,950,1901,0.034754037857055664,4.265562255584387e-08
476,953,952,1905,0.034815311431884766,4.0991250009575674e-08
477,955,954,1909,0.03493523597717285,3.939196542573217e-08
478,957,956,1913,0.03502917289733887,3.785497853193851e-08
479,959,958,1917,0.03510332107543945,3.6377972045425875e-08
480,961,960,1921,0.035178184509277344,3.495862479622804e-08
481,963,962,1925,0.0352482795715332,3.359464863394367e-08
482,965,964,1929,0.0353243350982666,3.2283868071071885e-08
483,967,966,1933,0.03541302680969238,3.1024295056238936e-08
484,969,968,1937,0.03548431396484375,2.9813797799304854e-08
485,971,970,1941,0.03555417060852051,2.8650599008075007e-08
486,973,972,1945,0.035627126693725586,2.7532696065330435e-08
487,975,974,1949,0.0357050895690918,2.6458401017310786e-08
488,977,976,1953,0.0357823371887207,2.542609487603269e-08
489,979,978,1957,0.03586411476135254,2.4434018805912255e-08
490,981,980,1961,0.03594017028808594,2.3480670342750388e-08
491,983,982,1965,0.03601717948913574,2.2564545106884706e-08
492,985,984,1969,0.036092281341552734,2.1684196980468794e-08
493,987,986,1973,0.03618025779724121,2.0838141955157397e-08
494,989,988,1977,0.03625130653381348,2.0025017444979148e-08
495,991,990,1981,0.03632211685180664,1.924366481044195e-08
496,993,992,1985,0.0363922119140625,1.8492938030535024e-08
497,995,994,1989,0.03646421432495117,1.777139293419102e-08
498,997,996,1993,0.036547183990478516,1.707794175976507e-08
499,999,998,1997,0.03662896156311035,1.6411624010131193e-08
500,1001,1000,2001,0.03670334815979004,1.577133930604825e-08
501,1003,1002,2005,0.03678321838378906,1.5155956190354236e-08
502,1005,1004,2009,0.03686404228210449,1.4564588938736502e-08
503,1007,1006,2013,0.03694319725036621,1.399636249613316e-08
504,1009,1008,2017,0.03703498840332031,1.3450291093053104e-08
505,1011,1010,2021,0.0371091365814209,1.2925485109457703e-08
506,1013,1012,2025,0.037194252014160156,1.24211316447961e-08
507,1015,1014,2029,0.0372772216796875,1.193648481882728e-08
508,1017,1016,2033,0.03735709190368652,1.1470786135546793e-08
509,1019,1018,2037,0.037450313568115234,1.1023235310339514e-08
510,1021,1020,2041,0.03753542900085449,1.0593117540697083e-08
511,1023,1022,2045,0.03762626647949219,1.0179785044135552e-08
512,1025,1024,2049,0.037722110748291016,9.782679373521822e-09
513,1027,1026,2053,0.037827253341674805,9.400991527337729e-09
514,1029,1028,2057,0.03790736198425293,9.034128081207756e-09
515,1031,1030,2061,0.03799033164978027,8.681634534648964e-09
516,1033,1032,2065,0.03807520866394043,8.342952440457601e-09
517,1035,1034,2069,0.038161277770996094,8.017363096199573e-09
518,1037,1036,2073,0.03825116157531738,7.704555743067209e-09
519,1039,1038,2077,0.03833818435668945,7.40398259711187e-09
520,1041,1040,2081,0.038433074951171875,7.115061933032515e-09
521,1043,1042,2085,0.03854632377624512,6.837487805341884e-09
522,1045,1044,2089,0.038616180419921875,6.570705666804301e-09
523,1047,1046,2093,0.03869009017944336,6.314413472409368e-09
524,1049,1048,2097,0.038767099380493164,6.06794011150924e-09
525,1051,1050,2101,0.03885841369628906,5.831212765055339e-09
526,1053,1052,2105,0.038938283920288086,5.603702112567803e-09
527,1055,1054,2109,0.0390012264251709,5.385093496176269e-09
528,1057,1056,2113,0.03906726837158203,5.174970256656906e-09
529,1059,1058,2117,0.03913712501525879,4.9730614270077926e-09
530,1061,1060,2121,0.0391993522644043,4.7789562028090585e-09
531,1063,1062,2125,0.039260149002075195,4.592546783755809e-09
532,1065,1064,2129,0.0393221378326416,4.413351442767816e-09
533,1067,1066,2133,0.03938722610473633,4.241180796371008e-09
534,1069,1068,2137,0.03944826126098633,4.0756696821957895e-09
535,1071,1070,2141,0.039527177810668945,3.9166248135357444e-09
536,1073,1072,2145,0.03959226608276367,3.763877226134218e-09
537,1075,1074,2149,0.0396573543548584,3.617010260529515e-09
538,1077,1076,2153,0.039716243743896484,3.4758442336779236e-09
539,1079,1078,2157,0.03977608680725098,3.340227655652756e-09
540,1081,1080,2161,0.039838314056396484,3.2099206387757545e-09
541,1083,1082,2165,0.0399012565612793,3.0846648264341577e-09
542,1085,1084,2169,0.039965152740478516,2.9643058204763465e-09
543,1087,1086,2173,0.040038108825683594,2.8486668459707524e-09
544,1089,1088,2177,0.04010319709777832,2.737509969956892e-09
545,1091,1090,2181,0.04016995429992676,2.630756516096193e-09
546,1093,1092,2185,0.040246009826660156,2.528085015405078e-09
547,1095,1094,2189,0.04032611846923828,2.429451777746748e-09
548,1097,1096,2193,0.04040336608886719,2.3346654662762753e-09
549,1099,1098,2197,0.04049515724182129,2.2435988562506917e-09
550,1101,1100,2201,0.04057908058166504,2.156026622328697e-09
551,1103,1102,2205,0.04066920280456543,2.0719196391533604e-09
552,1105,1104,2209,0.040763139724731445,1.991086568919414e-09
553,1107,1106,2213,0.04087018966674805,1.9134021406329454e-09
554,1109,1108,2217,0.040972232818603516,1.838670155185329e-09
555,1111,1110,2221,0.041056156158447266,1.7670100888673113e-09
556,1113,1112,2225,0.041129350662231445,1.6980004192799094e-09
557,1115,1114,2229,0.04120612144470215,1.6318227825473021e-09
558,1117,1116,2233,0.04127836227416992,1.5681226747702866e-09
559,1119,1118,2237,0.041355133056640625,1.5069000973037925e-09
560,1121,1120,2241,0.041419029235839844,1.448078324440392e-09
561,1123,1122,2245,0.0414881706237793,1.391659312925431e-09
562,1125,1124,2249,0.04155921936035156,1.3373196394658402e-09
563,1127,1126,2253,0.0416262149810791,1.285140886812653e-09
564,1129,1128,2257,0.04168820381164551,1.2350482843514632e-09
565,1131,1130,2261,0.041749000549316406,1.186860198545145e-09
566,1133,1132,2265,0.04181241989135742,1.140562065305281e-09
567,1135,1134,2269,0.041889190673828125,1.0960120978663005e-09
568,1137,1136,2273,0.04198813438415527,1.0532773156274416e-09
569,1139,1138,2277,0.04205012321472168,1.012159564631889e-09
570,1141,1140,2281,0.04211306571960449,9.726336316793775e-10
571,1143,1142,2285,0.042174339294433594,9.347626212499833e-10
572,1145,1144,2289,0.042240142822265625,8.982541932178419e-10
573,1147,1146,2293,0.04230237007141113,8.631918859737313e-10
574,1149,1148,2297,0.042368173599243164,8.295300533129466e-10
575,1151,1150,2301,0.04243206977844238,7.971560353247145e-10
576,1153,1152,2305,0.0424952507019043,7.660863494472152e-10
577,1155,1154,2309,0.04255819320678711,7.361752984059729e-10
578,1157,1156,2313,0.04262518882751465,7.074228817547586e-10
579,1159,1158,2317,0.04270315170288086,6.798019300741735e-10
580,1161,1160,2321,0.04277229309082031,6.533396127571754e-10
581,1163,1162,2325,0.04283618927001953,6.278795815104037e-10
582,1165,1164,2329,0.042899370193481445,6.033072171939017e-10
583,1167,1166,2333,0.042960166931152344,5.798187207352479e-10
584,1169,1168,2337,0.04302525520324707,5.571528271737344e-10
585,1171,1170,2341,0.04308724403381348,5.354124949142537e-10
586,1173,1172,2345,0.04324030876159668,5.145598302218189e-10
587,1175,1174,2349,0.04334115982055664,4.944384855414559e-10
588,1177,1176,2353,0.043410301208496094,4.751446025467098e-10
589,1179,1178,2357,0.043498992919921875,4.566131195353897e-10
590,1181,1180,2361,0.04355931282043457,4.387944811541427e-10
591,1183,1182,2365,0.043618202209472656,4.216634721420272e-10
592,1185,1184,2369,0.04367828369140625,4.0524726590565135e-10
593,1187,1186,2373,0.04375123977661133,3.894331971593097e-10
594,1189,1188,2377,0.043810129165649414,3.742067053234979e-10
595,1191,1190,2381,0.04387402534484863,3.5968045142699826e-10
596,1193,1192,2385,0.04393315315246582,3.45598031231814e-10
597,1195,1194,2389,0.0439910888671875,3.320886269620184e-10
598,1197,1196,2393,0.04405021667480469,3.1913571380833226e-10
599,1199,1198,2397,0.04411435127258301,3.067412557407374e-10
600,1201,1200,2401,0.04417610168457031,2.9470709670712815e-10
601,1203,1202,2405,0.04424905776977539,2.832003042321964e-10
602,1205,1204,2409,0.04431724548339844,2.722208797596574e-10
603,1207,1206,2413,0.04438614845275879,2.615871920555191e-10
604,1209,1208,2417,0.044448137283325195,2.51368215579273e-10
605,1211,1210,2421,0.04450821876525879,2.4157851173879045e-10
606,1213,1212,2425,0.04456806182861328,2.321054124285886e-10
607,1215,1214,2429,0.04462838172912598,2.2304702707899018e-10
608,1217,1216,2433,0.04468822479248047,2.144013935168305e-10
609,1219,1218,2437,0.04474902153015137,2.059597071422997e-10
610,1221,1220,2441,0.044830322265625,1.9801431036403613e-10
611,1223,1222,2445,0.044898033142089844,1.902437383534575e-10
612,1225,1224,2449,0.044970035552978516,1.8278781644674094e-10
613,1227,1226,2453,0.04503226280212402,1.757174850509383e-10
614,1229,1228,2457,0.0451052188873291,1.6883457724969176e-10
615,1231,1230,2461,0.04516720771789551,1.622372015955831e-10
616,1233,1232,2465,0.04523324966430664,1.5589622810134068e-10
617,1235,1234,2469,0.04529619216918945,1.4984274272880135e-10
618,1237,1236,2473,0.04536128044128418,1.4396016573236969e-10
619,1239,1238,2477,0.04543113708496094,1.3835051116178982e-10
620,1241,1240,2481,0.04550504684448242,1.330118267240005e-10
621,1243,1242,2485,0.04557228088378906,1.2774792185090235e-10
622,1245,1244,2489,0.045632123947143555,1.2280740999601188e-10
623,1247,1246,2493,0.04569435119628906,1.1805630151211657e-10
624,1249,1248,2497,0.04575514793395996,1.133488813466001e-10
625,1251,1250,2501,0.04582023620605469,1.0899792158560653e-10
626,1253,1252,2505,0.0458831787109375,1.0471976771979524e-10
627,1255,1254,2509,0.04594612121582031,1.0065237283999396e-10
628,1257,1256,2513,0.04600811004638672,9.66617062249053e-11


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n10/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0001709461212158203,542.5060889379029
1,2,1,3,0.0003020763397216797,207.98870940431505
2,3,2,5,0.00037407875061035156,274.0655574126137
3,4,3,7,0.0004291534423828125,175.81646225201428
4,5,4,9,0.0004961490631103516,164.98414436485226
6,7,6,13,0.0006132125854492188,120.69035731832143
7,8,7,15,0.0006670951843261719,110.05724136292307
8,9,8,17,0.0007190704345703125,100.9817631078583
9,10,9,19,0.0007741451263427734,93.9040070272565
10,11,10,21,0.0008270740509033203,89.6901587930119
11,12,11,23,0.0008780956268310547,86.48087704332885
12,13,12,25,0.0009322166442871094,83.90363237471003
13,14,13,27,0.00098419189453125,70.3354823560248
15,16,15,31,0.0010859966278076172,64.13835866777424
16,17,16,33,0.0011401176452636719,62.0248062633654
17,18,17,35,0.0012023448944091797,60.26569227733142
18,19,18,37,0.0012581348419189453,58.7275169303602
19,20,19,39,0.0013120174407958984,57.33681249756586
20,21,20,41,0.001373291015625,56.0428339377457
21,22,21,43,0.0014252662658691406,41.17109166754773
22,23,22,45,0.0014801025390625,35.56400995834689
24,25,24,49,0.0016040802001953125,32.90551431967733
25,26,25,51,0.0016751289367675781,31.80962744205267
26,27,26,53,0.0017271041870117188,23.98320898693349
27,28,27,55,0.0017800331115722656,23.14887668222036
28,29,28,57,0.0018301010131835938,22.570890908767296
29,30,29,59,0.0018811225891113281,22.021963668656266
30,31,30,61,0.0019309520721435547,21.496568136886992
31,32,31,63,0.001980304718017578,20.990871046760084
32,33,32,65,0.002031087875366211,20.501999198134996
34,35,34,69,0.002134084701538086,19.566765906681205
35,36,35,71,0.0021851062774658203,19.11764758580096
36,37,36,73,0.0022361278533935547,18.679588339189444
37,38,37,75,0.002286195755004883,18.251922413304875
38,39,38,77,0.002340078353881836,17.834139723805023
39,40,39,79,0.0023920536041259766,17.425841988121515
40,41,40,81,0.0024461746215820312,17.026710567443025
41,42,41,83,0.002504110336303711,16.63648302350121
43,44,43,87,0.0026140213012695312,15.881873716776415
44,45,44,89,0.0026760101318359375,15.517117886513235
45,46,45,91,0.002730131149291992,15.160502994707883
46,47,46,93,0.0027840137481689453,14.811871363214015
47,48,47,95,0.0028412342071533203,14.4710704082417
48,49,48,97,0.0029091835021972656,14.137950734300818
49,50,49,99,0.002973318099975586,13.812364922223416
50,51,50,101,0.0030410289764404297,13.494166805130115
51,52,51,103,0.0031092166900634766,13.183211082056683
53,54,53,107,0.0032472610473632812,12.582449148328152
54,55,54,109,0.003304004669189453,12.292355942812474
55,56,55,111,0.0033600330352783203,12.008931371424364
56,57,56,113,0.0034110546112060547,11.732034363102503
57,58,57,115,0.0034601688385009766,11.46152512782343
58,59,58,117,0.0035161972045898438,11.197265333420109
59,60,59,119,0.003576040267944336,10.939118271714221
60,61,60,121,0.0036270618438720703,10.686949009389792
62,63,62,125,0.003735065460205078,5.402158040438191
63,64,63,127,0.0038640499114990234,4.761358153405375
64,65,64,129,0.0039370059967041016,4.271520432759425
65,66,65,131,0.0040073394775390625,3.8370636416417843
66,67,66,133,0.004060268402099609,3.4587693629219842
67,68,67,135,0.004113197326660156,3.1287530232702094
68,69,68,137,0.004166126251220703,2.841345039817945
69,70,69,139,0.0042171478271484375,2.5912940307989034
71,72,71,143,0.004353046417236328,2.1851658209445826
72,73,72,145,0.0044422149658203125,2.02123160829976
73,74,73,147,0.00449824333190918,1.8788457522323445
74,75,74,149,0.00455021858215332,1.7550696464366484
75,76,75,151,0.0046041011810302734,1.6472985678540493
76,77,76,153,0.004658222198486328,1.5532350458182878
77,78,77,155,0.004719257354736328,1.4708646705912216
78,79,78,157,0.004770040512084961,1.3984330391989461
79,80,79,159,0.004820108413696289,1.3344230355887088
81,82,81,163,0.004918098449707031,1.2266497932218043
82,83,82,165,0.004965066909790039,1.1808352966214721
83,84,83,167,0.005029201507568359,1.1392964157497862
84,85,84,169,0.005095958709716797,1.101369362909225
85,86,85,171,0.005151987075805664,1.0665003323495321
86,87,86,173,0.0052149295806884766,1.0342288512086701
87,88,87,175,0.005275249481201172,1.0041730294632891
88,89,88,177,0.00533604621887207,0.9760166961785682
90,91,90,181,0.005448102951049805,0.9244016515855726
91,92,91,183,0.0054972171783447266,0.9005476780862695
92,93,92,185,0.005544900894165039,0.877788108339413
93,94,93,187,0.0055999755859375,0.8559998119210516
94,95,94,189,0.005647182464599609,0.8350802849518479
95,96,95,191,0.005693912506103516,0.814943911957379
96,97,96,193,0.005742073059082031,0.7955189020455389
97,98,97,195,0.005800008773803711,0.7767447841921623
98,99,98,197,0.005856037139892578,0.7585703634515314
100,101,100,201,0.005949974060058594,0.7238525299329535
101,102,101,203,0.005999088287353516,0.7072396070643435
102,103,102,205,0.006049156188964844,0.691085358165437
103,104,103,207,0.00609898567199707,0.6753653737326968
104,105,104,209,0.00614619255065918,0.6600581665352444
105,106,105,211,0.0061931610107421875,0.6451446845043806
106,107,106,213,0.006240129470825195,0.6306079126336457
107,108,107,215,0.006287097930908203,0.6164325470766233
109,110,109,219,0.0063931941986083984,0.5891118190180266
110,111,110,221,0.006442070007324219,0.5759422277900494
111,112,111,223,0.006500244140625,0.5630852547792591
112,113,112,225,0.0065572261810302734,0.5505309701534934
113,114,113,227,0.0066111087799072266,0.538270110635148
114,115,114,229,0.006667137145996094,0.5262939936488858
115,116,115,231,0.006724119186401367,0.5145944455065404
116,117,116,233,0.006781101226806641,0.5031637411246458
118,119,118,237,0.006887197494506836,0.48107990942512513
119,120,119,239,0.006942033767700195,0.4704131556739638
120,121,120,241,0.0069980621337890625,0.4599879252508989
121,122,121,243,0.007055044174194336,0.4497981121029822
122,123,122,245,0.007110118865966797,0.4398378479728607
123,124,123,247,0.0071659088134765625,0.4301014826454164
124,125,124,249,0.0072231292724609375,0.42058356681882325
125,126,125,251,0.0072782039642333984,0.41127883718828107
126,127,126,253,0.007333278656005859,0.4021822033978906
128,129,128,257,0.00745391845703125,0.38459365922365873
129,130,129,259,0.007521152496337891,0.3760923362355759
130,131,130,261,0.0075740814208984375,0.36778026692780263
131,132,131,263,0.007628202438354492,0.35965307789183115
132,133,132,265,0.007678031921386719,0.3517065165833811
133,134,133,267,0.007727146148681641,0.3439364455380017
134,135,134,269,0.007778167724609375,0.33633883713214574
135,136,135,271,0.007827043533325195,0.3289097688161205
137,138,137,275,0.007928133010864258,0.3145420618700312
138,139,138,277,0.007980108261108398,0.30759606609568313
139,140,139,279,0.008033037185668945,0.3008038890515508
140,141,140,281,0.008085012435913086,0.2941620748583548
141,142,141,283,0.008134126663208008,0.2876672512125353
142,143,142,285,0.008185148239135742,0.28131612664851496
143,144,143,287,0.008234024047851562,0.27510548797251766
144,145,144,289,0.008285284042358398,0.26903219785114363
145,146,145,291,0.008336067199707031,0.2630931925380429
147,148,147,295,0.008433103561401367,0.2516061365047946
148,149,148,297,0.008479118347167969,0.24605230743601103
149,150,149,299,0.008530139923095703,0.24062120269996232
150,151,150,301,0.008579015731811523,0.23531009634082653
151,152,151,303,0.008630990982055664,0.23011632458353506
152,153,152,305,0.008680105209350586,0.22503728422129732
153,154,153,307,0.008727073669433594,0.22007043106751703
154,155,154,309,0.008774280548095703,0.21521327846855828
156,157,156,313,0.008871316909790039,0.20581840743547744
157,158,157,315,0.008914947509765625,0.201275990713055
158,159,158,317,0.00896000862121582,0.19683387534527286
159,160,159,319,0.009008169174194336,0.19248984182186837
160,161,160,321,0.009057044982910156,0.18824172027180214
161,162,161,323,0.00910806655883789,0.1840873892908794
162,163,162,325,0.009163141250610352,0.1800247748063447
163,164,163,327,0.009213924407958984,0.17605184897228987
165,166,165,331,0.00931406021118164,0.16836717660636932
166,167,166,333,0.009371280670166016,0.16465159601749974
167,168,167,335,0.009427070617675781,0.16101803396446696
168,169,168,337,0.009484052658081055,0.15746467823137011
169,170,169,339,0.00953817367553711,0.15398975681713237
170,171,170,341,0.00959014892578125,0.15059153702358727
171,172,171,343,0.009639263153076172,0.14726832456674457
172,173,172,345,0.009767293930053711,0.14401846270960697
173,174,173,347,0.009890079498291016,0.14084033141634011
175,176,175,351,0.010036945343017578,0.1346929589560412
176,177,176,353,0.01010894775390625,0.131720653898841
177,178,177,355,0.010181188583374023,0.12881395007280683
178,179,178,357,0.010254144668579102,0.12597139896381346
179,180,179,359,0.01032400131225586,0.12319158409624681
180,181,180,361,0.010394096374511719,0.12047312031849117
181,182,181,363,0.010459184646606445,0.11781465310495985
182,183,182,365,0.010524272918701172,0.11521485787481088
184,185,184,369,0.010664939880371094,0.11018613078373568
185,186,185,371,0.010736227035522461,0.10775469356653737
186,187,186,373,0.010809183120727539,0.10537691636283472
187,188,187,375,0.01087808609008789,0.10305161462491585
188,189,188,377,0.010946035385131836,0.10077762997501194
189,190,189,379,0.011015892028808594,0.0985538296252799
190,191,190,381,0.011100292205810547,0.09637910581075006
191,192,191,383,0.011171102523803711,0.09425237523486613
192,193,192,385,0.011244058609008789,0.09217257852812377
194,195,194,389,0.01138615608215332,0.08814966570997212
195,196,195,391,0.011451244354248047,0.08620454578469486
196,197,196,393,0.011516332626342773,0.08430235109901553
197,198,197,395,0.011589288711547852,0.08244213420435499
198,199,198,397,0.011660099029541016,0.08062296857295405
199,200,199,399,0.011736154556274414,0.07884394813547066
200,201,200,401,0.011809110641479492,0.07710418682835267
201,202,201,403,0.011869192123413086,0.07540281815192632
203,204,203,407,0.011996269226074219,0.07211188792544311
204,205,204,409,0.012077093124389648,0.07052068735046704
205,206,205,411,0.012150049209594727,0.06896460053822821
206,207,206,413,0.012229204177856445,0.06744285251014266
207,208,207,415,0.012304067611694336,0.06595468539614385
208,209,208,417,0.01236104965209961,0.06449935805709435
209,210,209,419,0.012414932250976562,0.06307614571531585
210,211,210,421,0.012464284896850586,0.06168433959305711
212,213,212,425,0.012563943862915039,0.058992188781904396
213,214,213,427,0.012613058090209961,0.05769050339498308
214,215,214,429,0.012663125991821289,0.05641754216277564
215,216,215,431,0.012710094451904297,0.05517267115944222
216,217,216,433,0.012761116027832031,0.05395527045225669
217,218,217,435,0.012809991836547852,0.05276473379298964
218,219,218,437,0.012858152389526367,0.05160046831518218
219,220,219,439,0.012907028198242188,0.05046189423929462
220,221,220,441,0.012959957122802734,0.04934844458301679
222,223,222,445,0.013065099716186523,0.04719471289912895
223,224,223,447,0.013120174407958984,0.0461533583829401
224,225,224,449,0.013171911239624023,0.04513498277453306
225,226,225,451,0.013226032257080078,0.04413907896361874
226,227,226,453,0.013280153274536133,0.04316515103291216
227,228,227,455,0.013336181640625,0.04221271401114191
228,229,228,457,0.013392210006713867,0.04128129363107912
229,230,229,459,0.01345515251159668,0.040370426093512844
231,232,231,463,0.013586282730102539,0.03860854530644086
232,233,232,465,0.01377415657043457,0.03775665474323018
233,234,233,467,0.013926267623901367,0.036923561957991666
234,235,234,469,0.014014005661010742,0.036108852124683885
235,236,235,471,0.014101982116699219,0.035312119572801046
236,237,236,473,0.014246225357055664,0.034532967585366815
237,238,237,475,0.01439809799194336,0.033771008201202914
238,239,238,477,0.014467239379882812,0.033025862021703864
239,240,239,479,0.0145721435546875,0.032297158021608444
241,242,241,483,0.014898300170898438,0.03088763322196539
242,243,242,485,0.014952898025512695,0.030206110596187205
243,244,243,487,0.015007972717285156,0.029539626148107893
244,245,244,489,0.015061140060424805,0.028887848027625455
245,246,245,491,0.015115022659301758,0.02825045170848493
246,247,246,493,0.015166997909545898,0.027627119826772937
247,248,247,495,0.01521611213684082,0.027017542022629678
248,249,248,497,0.015267133712768555,0.02642141478560048
250,251,250,501,0.01536417007446289,0.02526833131510024
251,252,251,503,0.015410900115966797,0.024710800964211733
252,253,252,505,0.015461206436157227,0.024165572659698077
253,254,253,507,0.015510082244873047,0.023632374936395133
254,255,254,509,0.015559196472167969,0.02311094232001147
255,256,255,511,0.015614032745361328,0.022601015195210426
256,257,256,513,0.01566624641418457,0.022102339675920284
257,258,257,515,0.015716075897216797,0.0216146674790305
259,260,259,519,0.01581430435180664,0.020671367195368023
260,261,260,521,0.015864133834838867,0.020215269457740617
261,262,261,523,0.015916109085083008,0.019769235506674053
262,263,262,525,0.015965938568115234,0.01933304327246174
263,264,263,527,0.016016244888305664,0.018906475586043664
264,265,264,529,0.016068220138549805,0.018489320070924155
265,266,265,531,0.016117095947265625,0.01808136903730789
266,267,266,533,0.01616525650024414,0.01768241937871636
267,268,267,535,0.01621413230895996,0.01729227247087854
269,270,269,539,0.016316890716552734,0.016537614229555447
270,271,270,541,0.01636505126953125,0.016172727178671784
271,272,271,543,0.016413211822509766,0.01581589125677646
272,273,272,545,0.01646113395690918,0.015466928809089973
273,274,273,547,0.016510009765625,0.015125666101765278
274,275,274,549,0.016560077667236328,0.014791933234339825
275,276,275,551,0.01660919189453125,0.014465564056030411
276,277,276,553,0.01666092872619629,0.014146396082273438
278,279,278,557,0.016762256622314453,0.01352903165947384
279,280,279,559,0.016813039779663086,0.013230527854608152
280,281,280,561,0.01687312126159668,0.012938610389819786
281,282,281,563,0.016924142837524414,0.012653133934415074
282,283,282,565,0.016972064971923828,0.012373956364916703
283,284,283,567,0.01702404022216797,0.012100938693985177
284,285,284,569,0.01707601547241211,0.011833945001345908
285,286,285,571,0.01712512969970703,0.011572842365990538
286,287,286,573,0.01717519760131836,0.011317500800081029
288,289,288,577,0.017281055450439453,0.010823595204038973
289,290,289,579,0.017332077026367188,0.010584785288449066
290,291,290,581,0.017383337020874023,0.010351244548926114
291,292,291,583,0.017431020736694336,0.01012285672050335
292,293,292,585,0.017484188079833984,0.009899508103722574
293,294,293,587,0.01753711700439453,0.009681087508084397
294,295,294,589,0.017588138580322266,0.009467486196500128
295,296,295,591,0.01763916015625,0.009258597831661665
297,298,297,595,0.017742156982421875,0.008854546272220152
298,299,298,597,0.017797231674194336,0.008659181928993355
299,300,299,599,0.017856121063232422,0.008468128134932047
300,301,300,601,0.01790618896484375,0.008281289778366261
301,302,301,603,0.017956256866455078,0.008098573846115066
302,303,302,605,0.0180051326751709,0.007919889377944769
303,304,303,607,0.018053293228149414,0.007745147420329634
304,305,304,609,0.018100976943969727,0.007574260982682762
306,307,306,613,0.018198013305664062,0.007243716260558522
307,308,307,615,0.018246173858642578,0.0070838934240057124
308,309,308,617,0.0182950496673584,0.00692759692165988
309,310,309,619,0.01835799217224121,0.006774748945944709
310,311,310,621,0.018407106399536133,0.006625273406645923
311,312,311,623,0.018455028533935547,0.0064790958923083885
312,313,312,625,0.0185091495513916,0.006336143633428738
313,314,313,627,0.01856207847595215,0.006196345466146585
314,315,314,629,0.018620967864990234,0.0060596317969214735
316,317,316,633,0.01883411407470703,0.005795187222800078
317,318,317,635,0.01890110969543457,0.005667324674212056
318,319,318,637,0.01896500587463379,0.005542283270418612
319,320,319,639,0.019024133682250977,0.0054200007646637485
320,321,320,641,0.01908397674560547,0.005300416283589236
321,322,321,643,0.01914215087890625,0.005183470296844416
322,323,322,645,0.019204139709472656,0.00506910458764676
323,324,323,647,0.019260168075561523,0.004957262224031962
325,326,325,651,0.019360065460205078,0.004740926058266062
326,327,326,653,0.0194091796875,0.004636324562670909
327,328,327,655,0.019459009170532227,0.00453403097209422
328,329,328,657,0.01950693130493164,0.004433994364295724
329,330,329,659,0.019556045532226562,0.004336164940756072
330,331,330,661,0.01960611343383789,0.0042404940016833705
331,332,331,663,0.019654273986816406,0.004146933921796279
332,333,332,665,0.019704103469848633,0.004055438126812003
333,334,333,667,0.01975393295288086,0.003965961069901882
335,336,335,671,0.01986098289489746,0.0037928859863058315
336,337,336,673,0.01991415023803711,0.003709201802807134
337,338,337,675,0.019964218139648438,0.0036273640010897447
338,339,338,677,0.020017147064208984,0.003547331842487434
339,340,339,679,0.0200650691986084,0.003469065486941077
340,341,340,681,0.020113229751586914,0.0033925259738433505
341,342,341,683,0.020169973373413086,0.003317675202018212
342,343,342,685,0.020229101181030273,0.0032444759110702307
344,345,344,689,0.020355224609375,0.0031028868225573786
345,346,345,691,0.02040410041809082,0.0030344265425757007
346,347,346,693,0.020457983016967773,0.0029674767437474956
347,348,347,695,0.020509958267211914,0.0029020040988726337
348,349,348,697,0.020562171936035156,0.0028379760159543406
349,350,349,699,0.020617008209228516,0.0027753606224816493
350,351,350,701,0.020676136016845703,0.0027141267488115226
351,352,351,703,0.020731210708618164,0.0026542439133317355
353,354,353,707,0.02086019515991211,0.002538412777898195
354,355,354,709,0.020919084548950195,0.0024824068182858323
355,356,355,711,0.02108597755432129,0.0024276365488350377
356,357,356,713,0.021146059036254883,0.0023740747054084564
357,358,357,715,0.021206140518188477,0.0023216946254579246
358,359,358,717,0.02126312255859375,0.002270470234856464
359,360,359,719,0.02131819725036621,0.002220376034630402
360,361,360,721,0.02137303352355957,0.0021713870884986332
361,362,361,723,0.02142620086669922,0.0021234790104403267
363,364,363,727,0.021529197692871094,0.0020308105923713066
364,365,364,729,0.021602153778076172,0.0019860041232063115
365,366,365,731,0.0216519832611084,0.0019421862408806278
366,367,366,733,0.02171611785888672,0.0018993351335563834
367,368,367,735,0.021783113479614258,0.0018574294703631086
368,369,368,737,0.02184605598449707,0.0018164483915243427
369,370,369,739,0.021906137466430664,0.0017763714970246193
370,371,370,741,0.021959304809570312,0.001737178837425108
372,373,372,745,0.02207207679748535,0.0016613686151898824
373,374,373,747,0.022127151489257812,0.0016247133155114992
374,375,374,749,0.02218008041381836,0.0015888667577107253
375,376,375,751,0.022234201431274414,0.0015538110979405233
376,377,376,753,0.02228522300720215,0.0015195288861689546
377,378,377,755,0.022335052490234375,0.0014860030572434733
378,379,378,757,0.02238321304321289,0.0014532169226734687
379,380,379,759,0.02243208885192871,0.0014211541621291632
381,382,381,763,0.022533178329467773,0.001359135274173557
382,383,382,765,0.022584199905395508,0.0013291482749761734
383,384,383,767,0.022633075714111328,0.0012998228907309397
384,385,384,769,0.022683143615722656,0.0012711445239768399
385,386,385,771,0.022755146026611328,0.0012430988990539266
386,387,386,773,0.02281808853149414,0.0012156720554441448
387,388,387,775,0.022869110107421875,0.001188850340711998
388,389,388,777,0.022918224334716797,0.0011626204035876506
389,390,389,779,0.02297806739807129,0.0011369691871740788
391,392,391,783,0.02308821678161621,0.0010873521240182607
392,393,392,785,0.02313709259033203,0.0010633615790484763
393,394,393,787,0.023186206817626953,0.0010399003459303292
394,395,394,789,0.023234128952026367,0.0010169567463381558
395,396,395,791,0.023283958435058594,0.0009945193593081172
396,397,396,793,0.023333072662353516,0.0009725770161415304
397,398,397,795,0.023382186889648438,0.0009511187942865064
398,399,398,797,0.02343010902404785,0.0009301340125132091
400,401,400,801,0.023529052734375,0.0008895432165369584
401,402,401,803,0.023586034774780273,0.0008699169972282329
402,403,402,805,0.023637056350708008,0.0008507237975506286
403,404,403,807,0.023687124252319336,0.0008319540636327136
404,405,404,809,0.023736238479614258,0.0008135984524119996
405,406,405,811,0.023785114288330078,0.0007956478267911205
406,407,406,813,0.023835182189941406,0.0007780932514565319
407,408,407,815,0.023897171020507812,0.0007609259882423864
408,409,408,817,0.023946046829223633,0.0007441374915818346
410,411,410,821,0.02404308319091797,0.0007116635550997141
411,412,411,823,0.024091243743896484,0.0006959619504981624
412,413,412,825,0.024140119552612305,0.0006806067750341397
413,414,413,827,0.02418828010559082,0.00066559038542363
414,415,414,829,0.02423715591430664,0.0006509053066785315
415,416,415,831,0.024285316467285156,0.0006365442292159629
416,417,416,833,0.024334192276000977,0.0006225000043531535
417,418,417,835,0.02438211441040039,0.0006087656412060647
419,420,419,839,0.02448105812072754,0.0005821993045239375
420,421,420,841,0.02454400062561035,0.0005693541070361438
421,422,421,843,0.02459430694580078,0.000556792316733283
422,423,422,845,0.0246431827545166,0.000544507680675588
423,424,423,847,0.024693012237548828,0.0005324940838787319
424,425,424,849,0.02474212646484375,0.0005207455462751963
425,426,425,851,0.024796247482299805,0.0005092562198128969
426,427,426,853,0.024845123291015625,0.0004980203854446273
428,429,428,857,0.02495408058166504,0.0004762869448231322
429,430,429,859,0.025004148483276367,0.00046577852031052386
430,431,430,861,0.02505326271057129,0.00045550194583977
431,432,431,863,0.025103092193603516,0.00044545210604646397
432,433,432,865,0.025151968002319336,0.0004356239985420073
433,434,433,867,0.02520132064819336,0.00042601273098715083
434,435,434,869,0.02525019645690918,0.0004166135193066767
435,436,435,871,0.025303125381469727,0.0004074216846904455
436,437,436,873,0.025355100631713867,0.0003984326519324887
438,439,438,877,0.02546405792236328,0.00038104519235047235
439,440,439,879,0.025519132614135742,0.00037263811061508486
440,441,440,881,0.025577068328857422,0.0003644165163252031
441,442,441,883,0.025630950927734375,0.00035637631700843935
442,443,442,885,0.025686979293823242,0.0003485135106554684
443,444,443,887,0.02573704719543457,0.00034082418331530276
444,445,444,889,0.0257871150970459,0.00033330450730031225
445,446,445,891,0.02583599090576172,0.0003259507397382472
447,448,447,895,0.02592611312866211,0.0003117263686212227
448,449,448,897,0.0259702205657959,0.0003048486845830723
449,450,449,899,0.02602410316467285,0.0002981227444833437
450,451,450,901,0.026069164276123047,0.0002915452002944949
451,452,451,903,0.02611517906188965,0.0002851127780188185
452,453,452,905,0.026159048080444336,0.0002788222757495641
453,454,453,907,0.02620410919189453,0.00027267056219192786
454,455,454,909,0.026248931884765625,0.0002666545753837897
455,456,455,911,0.026293039321899414,0.0002607713206044924
457,458,457,915,0.02639007568359375,0.00024939135781170443
458,459,458,917,0.026435136795043945,0.0002438889851708443
459,460,459,919,0.026479244232177734,0.00023850801279715913
460,461,460,921,0.026523113250732422,0.00023324576178378092
461,462,461,923,0.02656722068786621,0.0002280996130182831
462,463,462,925,0.0266110897064209,0.00022306700489038345
463,464,463,927,0.026654958724975586,0.00021814543226725947
464,465,464,929,0.026699066162109375,0.00021333244544563738
466,467,466,933,0.02678704261779785,0.0002040226986784891
467,468,467,935,0.0268402099609375,0.00019952130472560386
468,469,468,937,0.02690410614013672,0.00019511922594162056
469,470,469,939,0.0269622802734375,0.00019081427110839326
470,471,470,941,0.02701711654663086,0.00018660429744396553
471,472,471,943,0.027081966400146484,0.00018248720943802313
472,473,472,945,0.02714705467224121,0.00017846095745648687
473,474,473,947,0.02721714973449707,0.00017452353756411317
475,476,475,951,0.027337074279785156,0.0001669073975079821
476,477,476,953,0.027390003204345703,0.00016322488627652334
477,478,477,955,0.02744007110595703,0.00015962362298147802
478,479,478,957,0.027492046356201172,0.0001561018151307343
479,480,479,959,0.027543067932128906,0.00015265770960735177
480,481,480,961,0.027595043182373047,0.00014928959219188886
481,482,481,963,0.027644872665405273,0.00014599578618782507
482,483,482,965,0.02769613265991211,0.00014277465197764383
483,484,483,967,0.02774500846862793,0.00013962458644032594
485,486,485,971,0.027848005294799805,0.00013353142362952175
486,487,486,973,0.027900218963623047,0.00013058529327932353
487,488,487,975,0.02794814109802246,0.0001277041640419485
488,489,488,977,0.027997970581054688,0.00012488660164821264
489,490,489,979,0.028050899505615234,0.00012213120382541706
490,491,490,981,0.028103113174438477,0.00011943659879708779
491,492,491,983,0.02815413475036621,0.00011680144544541835
492,493,492,985,0.02822089195251465,0.00011422443197714823
494,495,494,989,0.028335094451904297,0.00010923972211164034
495,496,495,991,0.028388261795043945,0.0001068295445142591
496,497,496,993,0.028437137603759766,0.00010447254305295783
497,498,497,995,0.028487205505371094,0.00010216754466810359
498,499,498,997,0.02853703498840332,9.991340187399322e-05
499,500,499,999,0.02858901023864746,9.770899270171721e-05
500,501,500,1001,0.028757095336914062,9.555321981155082e-05
501,502,501,1003,0.028810977935791016,9.344501013330934e-05
502,503,502,1005,0.02886509895324707,9.138331437774592e-05
504,505,504,1009,0.0290071964263916,8.73953820104558e-05
505,506,505,1011,0.029067039489746094,8.546716040661085e-05
506,507,506,1013,0.029125213623046875,8.35814814251813e-05
507,508,507,1015,0.029177188873291016,8.173740667065195e-05
508,509,508,1017,0.029226064682006836,7.993401804793474e-05
509,510,509,1019,0.029275178909301758,7.817041790931796e-05
510,511,510,1021,0.029325008392333984,7.64457284195039e-05
511,512,511,1023,0.029374122619628906,7.475909115153156e-05
513,514,513,1027,0.02948927879333496,7.149663337774589e-05
514,515,514,1029,0.0295412540435791,6.99191888711393e-05
515,516,515,1031,0.029588937759399414,6.837654789916817e-05
516,517,516,1033,0.02963709831237793,6.686794247241582e-05
517,518,517,1035,0.029688119888305664,6.53926217593597e-05
518,519,518,1037,0.029736042022705078,6.394985139440869e-05
519,520,519,1039,0.029801130294799805,6.253891304463458e-05
520,521,520,1041,0.029868125915527344,6.115910453853819e-05
522,523,522,1045,0.029986143112182617,5.849014476254239e-05
523,524,523,1047,0.03003716468811035,5.719966501464566e-05
524,525,524,1049,0.03009510040283203,5.593765734506459e-05
525,526,525,1051,0.03014516830444336,5.470349362255527e-05
526,527,526,1053,0.030222177505493164,5.3496559460289176e-05
527,528,527,1055,0.03032231330871582,5.231625413029969e-05
528,529,528,1057,0.03038620948791504,5.116199016487273e-05
529,530,529,1059,0.030440092086791992,5.00331928456284e-05
530,531,530,1061,0.030504941940307617,4.892930052189755e-05
532,533,532,1065,0.030620098114013672,4.6794044599315275e-05
533,534,533,1067,0.030678987503051758,4.576161808577329e-05
534,535,534,1069,0.03075408935546875,4.475197034333764e-05
535,536,535,1071,0.030820131301879883,4.376459861479928e-05
536,537,536,1073,0.03088212013244629,4.279901135879732e-05
537,538,537,1075,0.030935049057006836,4.1854728105493055e-05
538,539,538,1077,0.030994892120361328,4.09312788140013e-05
539,540,539,1079,0.031057119369506836,4.002820380574834e-05
541,542,541,1083,0.03125715255737305,3.8281388102905975e-05
542,543,542,1085,0.03132009506225586,3.743677814035546e-05
543,544,543,1087,0.03137516975402832,3.6610802887881596e-05
544,545,544,1089,0.03142714500427246,3.5803051288177883e-05
545,546,545,1091,0.03147602081298828,3.501312131179703e-05
546,547,546,1093,0.0315251350402832,3.424061961152563e-05
547,548,547,1095,0.03157925605773926,3.348516187301133e-05
548,549,548,1097,0.03163433074951172,3.2746371961816424e-05
549,550,549,1099,0.03168630599975586,3.202388201827929e-05
551,552,551,1103,0.03179121017456055,3.062637190340981e-05
552,553,552,1105,0.031852006912231445,2.995065596274533e-05
553,554,553,1107,0.03191113471984863,2.9289848460117702e-05
554,555,554,1109,0.0319669246673584,2.8643620547034954e-05
555,556,555,1111,0.03201723098754883,2.8011650476893378e-05
556,557,556,1113,0.03208303451538086,2.739362370577914e-05
557,558,557,1115,0.032241106033325195,2.6789232533047214e-05
558,559,558,1117,0.03232622146606445,2.619817618477594e-05
560,561,560,1121,0.03247809410095215,2.5054897491730444e-05
561,562,561,1123,0.03255200386047363,2.4502106111425138e-05
562,563,562,1125,0.032636165618896484,2.3961511063870686e-05
563,564,563,1127,0.03271293640136719,2.3432843326983816e-05
564,565,564,1129,0.03278803825378418,2.2915839643044647e-05
565,566,565,1131,0.032861948013305664,2.2410242742690288e-05
566,567,566,1133,0.032935142517089844,2.1915800878648077e-05
567,568,567,1135,0.03301715850830078,2.1432267966289655e-05
569,570,569,1139,0.03316926956176758,2.0496971741710957e-05
570,571,570,1141,0.03324317932128906,2.0044742782821493e-05
571,572,571,1143,0.03331303596496582,1.960249140877116e-05
572,573,572,1145,0.03337812423706055,1.9169997497325298e-05
573,574,573,1147,0.03344106674194336,1.8747045915038646e-05
574,575,574,1149,0.03350019454956055,1.8333425847695867e-05
575,576,575,1151,0.03355813026428223,1.7928931614885288e-05
576,577,576,1153,0.033618927001953125,1.7533361831711555e-05
577,578,577,1155,0.03369712829589844,1.714651961487854e-05
579,580,579,1159,0.0338139533996582,1.6398251726976647e-05
580,581,580,1161,0.033872127532958984,1.6036453657002352e-05
581,582,581,1163,0.03392624855041504,1.5682637960461056e-05
582,583,582,1165,0.03397512435913086,1.533662861764422e-05
583,584,583,1167,0.03402113914489746,1.4998253370522472e-05
584,585,584,1169,0.03406810760498047,1.466734371549774e-05
585,586,585,1171,0.03411412239074707,1.4343735006879948e-05
586,587,586,1173,0.03416013717651367,1.4027266095202094e-05
588,589,588,1177,0.03425097465515137,1.3415121257379603e-05
589,590,589,1179,0.03429722785949707,1.3119140561632764e-05
590,591,590,1181,0.03434324264526367,1.2829690172369761e-05
591,592,591,1183,0.034388065338134766,1.2546626056621504e-05
592,593,592,1185,0.03443312644958496,1.2269807099142835e-05
593,594,593,1187,0.03449821472167969,1.1999095756601988e-05
594,595,594,1189,0.034545183181762695,1.1734357125613668e-05
595,596,595,1191,0.034590959548950195,1.147545951841564e-05
596,597,596,1193,0.03463602066040039,1.1222273899534506e-05
598,599,598,1197,0.03473615646362305,1.073253790096571e-05
599,600,599,1199,0.03478193283081055,1.0495743556390904e-05
600,601,600,1201,0.03482818603515625,1.026417380226636e-05
601,602,601,1203,0.034873247146606445,1.0037713114797126e-05
602,603,602,1205,0.0349271297454834,9.816248798092387e-06
603,604,603,1207,0.03499007225036621,9.5996707806142e-06
604,605,604,1209,0.03504514694213867,9.387871140007273e-06
605,606,605,1211,0.03510403633117676,9.180744572332782e-06
607,608,607,1215,0.035218238830566406,8.780100079731466e-06
608,609,608,1217,0.03527712821960449,8.586382819728773e-06
609,610,609,1219,0.03533315658569336,8.396939553760424e-06
610,611,610,1221,0.0353851318359375,8.211676086458847e-06
611,612,611,1223,0.03544116020202637,8.03050010004875e-06
612,613,612,1225,0.03549814224243164,7.853321381183909e-06
613,614,613,1227,0.03555417060852051,7.680051879319413e-06
614,615,614,1229,0.03561115264892578,7.510605193323619e-06
616,617,616,1233,0.03573107719421387,7.1828450088324e-06
617,618,617,1235,0.03578329086303711,7.0243683255315075e-06
618,619,618,1237,0.03583526611328125,6.869388050636138e-06
619,620,619,1239,0.03590106964111328,6.717827241530595e-06
620,621,620,1241,0.035954952239990234,6.569610333463776e-06
621,622,621,1243,0.03600788116455078,6.424663659676869e-06
622,623,622,1245,0.03605914115905762,6.282914856783892e-06
623,624,623,1247,0.03611111640930176,6.144293487035874e-06
624,625,624,1249,0.03616619110107422,6.008730613422601e-06
626,627,626,1253,0.03627419471740723,5.746511639084111e-06
627,628,627,1255,0.03632712364196777,5.619725042337856e-06
628,629,628,1257,0.03638195991516113,5.4957358112185855e-06
629,630,629,1259,0.03643488883972168,5.3744821955023395e-06
630,631,630,1261,0.03648996353149414,5.2559037911301126e-06
631,632,631,1263,0.03654813766479492,5.139941609107002e-06
632,633,632,1265,0.03660702705383301,5.026537915327715e-06
633,634,633,1267,0.03666520118713379,4.915636345795654e-06
635,636,635,1271,0.036787986755371094,4.701119595481944e-06
636,637,636,1273,0.03684520721435547,4.597397743313911e-06
637,638,637,1275,0.03690505027770996,4.495964367146191e-06
638,639,638,1277,0.036962032318115234,4.39676883429937e-06
639,640,639,1279,0.03701925277709961,4.2997619852263335e-06
640,641,640,1281,0.037075042724609375,4.204895308450411e-06
641,642,641,1283,0.03714609146118164,4.112121776189699e-06
642,643,642,1285,0.03720211982727051,4.021395121394591e-06
643,644,643,1287,0.03726005554199219,3.9326701829827235e-06
645,646,645,1291,0.037371158599853516,3.7610497503306316e-06
646,647,646,1293,0.03742408752441406,3.678068793978288e-06
647,648,647,1295,0.03748202323913574,3.5969187349361283e-06
648,649,648,1297,0.03753399848937988,3.5175591468015492e-06
649,650,649,1299,0.037592172622680664,3.4399504725355412e-06
650,651,650,1301,0.037644147872924805,3.3640540630372703e-06
651,652,651,1303,0.03769397735595703,3.2898321764271736e-06
652,653,652,1305,0.03775620460510254,3.21724781858177e-06
654,655,654,1309,0.03786802291870117,3.076848169588334e-06
655,656,655,1311,0.0379180908203125,3.0089629848484995e-06
656,657,656,1313,0.03796815872192383,2.9425755814350398e-06
657,658,657,1315,0.038021087646484375,2.877652863714514e-06
658,659,658,1317,0.0380711555480957,2.814162513898904e-06
659,660,659,1319,0.03812098503112793,2.7520730329928966e-06
660,661,660,1321,0.03817009925842285,2.6913533677408062e-06
661,662,661,1323,0.03821897506713867,2.631973423397246e-06
663,664,663,1327,0.038329124450683594,2.5171150248078965e-06
664,665,664,1329,0.03838205337524414,2.4615792462423223e-06
665,666,665,1331,0.038436174392700195,2.407268895559149e-06
666,667,666,1333,0.03848600387573242,2.354156759653852e-06
667,668,667,1335,0.038535118103027344,2.302216447023986e-06
668,669,668,1337,0.03858828544616699,2.2514221810142497e-06
669,670,669,1339,0.03864288330078125,2.2017484510185646e-06
670,671,670,1341,0.038695335388183594,2.153170739027289e-06
671,672,671,1343,0.03875303268432617,2.105664858217672e-06
673,674,673,1347,0.03886008262634277,2.013774382500487e-06
674,675,674,1349,0.038908958435058594,1.969343968177682e-06
675,676,675,1351,0.038958072662353516,1.925893863786272e-06
676,677,676,1353,0.03900599479675293,1.8834024075715177e-06
677,678,677,1355,0.03905510902404785,1.841848446763889e-06
678,679,678,1357,0.039103031158447266,1.801211357843122e-06
679,680,679,1359,0.039153099060058594,1.7614707630764573e-06
680,681,680,1361,0.03920722007751465,1.7226070849480532e-06
682,683,682,1365,0.03931593894958496,1.6474330689307458e-06
683,684,683,1367,0.03937506675720215,1.6110853533109158e-06
684,685,684,1369,0.0394282341003418,1.5755395911326025e-06
685,686,685,1371,0.03948330879211426,1.5407780802643647e-06
686,687,686,1373,0.039541006088256836,1.506783562425623e-06
687,688,687,1375,0.03959918022155762,1.4735389978565335e-06
688,689,688,1377,0.0396580696105957,1.4410280063072856e-06
689,690,689,1379,0.03971409797668457,1.409234248255263e-06
690,691,690,1381,0.03977012634277344,1.378142026099197e-06
692,693,692,1385,0.03988504409790039,1.3180002755368412e-06
693,694,693,1387,0.03994107246398926,1.2889209379654233e-06
694,695,694,1389,0.039999961853027344,1.2604831577851149e-06
695,696,695,1391,0.04006505012512207,1.2326728215292235e-06
696,697,696,1393,0.04012918472290039,1.205476038054604e-06
697,698,697,1395,0.040183067321777344,1.178879350396357e-06
698,699,698,1397,0.040242910385131836,1.1528695055305866e-06
699,700,699,1399,0.040299177169799805,1.1274334165044736e-06
701,702,701,1403,0.04041910171508789,1.0782326142834613e-06
702,703,702,1405,0.04047513008117676,1.0544432433239328e-06
703,704,703,1407,0.04052925109863281,1.0311788650790242e-06
704,705,704,1409,0.040592193603515625,1.008427745528241e-06
705,706,705,1411,0.04064321517944336,9.861785216098412e-07
706,707,706,1413,0.04069209098815918,9.644202303777127e-07
707,708,707,1415,0.04074215888977051,9.431420652827042e-07
708,709,708,1417,0.04079413414001465,9.223332964752158e-07
710,711,710,1421,0.0408940315246582,8.820829368095245e-07
711,712,711,1423,0.04094409942626953,8.626212848196172e-07
712,713,712,1425,0.040995121002197266,8.43589082594216e-07
713,714,713,1427,0.041047096252441406,8.249767900084509e-07
714,715,714,1429,0.04109907150268555,8.067751408965151e-07
715,716,715,1431,0.04115724563598633,7.889750263116452e-07
716,717,716,1433,0.04120802879333496,7.715676966880661e-07
717,718,717,1435,0.041262149810791016,7.545444083162037e-07
718,719,718,1437,0.041322946548461914,7.378967214263209e-07
720,721,720,1441,0.041439056396484375,7.056951138074819e-07
721,722,721,1443,0.041494131088256836,6.901251915563995e-07
722,723,722,1445,0.04155111312866211,6.748988152946452e-07
723,724,723,1447,0.0416109561920166,6.600083922058918e-07
724,725,724,1449,0.041676998138427734,6.454464139400006e-07
725,726,725,1451,0.04173111915588379,6.312057537515734e-07
726,727,726,1453,0.04179501533508301,6.172793685234022e-07
727,728,727,1455,0.04184913635253906,6.036601335365658e-07
729,730,729,1459,0.04196619987487793,5.773165605838908e-07
730,731,730,1461,0.04202008247375488,5.645791424772669e-07
731,732,731,1463,0.04207205772399902,5.521226851784786e-07
732,733,732,1465,0.042124032974243164,5.399410730473839e-07
733,734,733,1467,0.04218006134033203,5.280281874634792e-07
734,735,734,1469,0.042236328125,5.163781983293458e-07
735,736,735,1471,0.042292118072509766,5.049852395870402e-07
736,737,736,1473,0.0423431396484375,4.938436345467465e-07
737,738,737,1475,0.042391061782836914,4.829478075865091e-07
739,740,739,1479,0.04250025749206543,4.6187206694494e-07
740,741,740,1481,0.04255104064941406,4.5168176141041903e-07
741,742,741,1483,0.04260396957397461,4.417161433208081e-07
742,743,742,1485,0.04267311096191406,4.319704450601988e-07
743,744,743,1487,0.04273724555969238,4.224397756114437e-07
744,745,744,1489,0.04278826713562012,4.131193965069388e-07
745,746,745,1491,0.04283905029296875,4.0400458577039963e-07
746,747,746,1493,0.042893171310424805,3.9509096325499146e-07
748,749,748,1497,0.043015241622924805,3.77849339046309e-07
749,750,749,1499,0.04306817054748535,3.6951276067188404e-07
750,751,750,1501,0.04312396049499512,3.61360088952392e-07
751,752,751,1503,0.043203115463256836,3.533873216133514e-07
752,753,752,1505,0.0432581901550293,3.455904553298304e-07
753,754,753,1507,0.04331207275390625,3.379655936787451e-07
754,755,754,1509,0.04336404800415039,3.30509051863949e-07
755,756,755,1511,0.04341411590576172,3.232169188894218e-07
757,758,757,1515,0.04351210594177246,3.091117659809256e-07
758,759,758,1517,0.043560028076171875,3.022918048535821e-07
759,760,759,1519,0.04360818862915039,2.956222157933265e-07
760,761,760,1521,0.043656110763549805,2.8909984433605273e-07
761,762,761,1523,0.04373311996459961,2.8272136216876104e-07
762,763,762,1525,0.04378318786621094,2.7648364397246845e-07
763,764,763,1527,0.043836116790771484,2.7038347409746545e-07
764,765,764,1529,0.0438840389251709,2.644180292598069e-07
765,766,765,1531,0.04393506050109863,2.5858406466584117e-07
767,768,767,1535,0.04403996467590332,2.472995094144579e-07
768,769,768,1537,0.04409909248352051,2.41843263453762e-07
769,770,769,1539,0.04415106773376465,2.3650740564686016e-07
770,771,770,1541,0.04419994354248047,2.3128932930127086e-07
771,772,771,1543,0.04425406455993652,2.261863480547186e-07
772,773,772,1545,0.04430413246154785,2.2119596595229156e-07
773,774,773,1547,0.04435300827026367,2.163156238664275e-07
774,775,774,1549,0.04440116882324219,2.115430190658377e-07
776,777,776,1553,0.04449892044067383,2.0231137149454668e-07
777,778,777,1555,0.044547080993652344,1.9784769026655788e-07
778,779,778,1557,0.04459500312805176,1.934825441925951e-07
779,780,779,1559,0.044646263122558594,1.8921365775728508e-07
780,781,780,1561,0.04469704627990723,1.8503896812809455e-07
781,782,781,1563,0.04474902153015137,1.8095642704366183e-07
782,783,782,1565,0.04479622840881348,1.7696396293197097e-07
783,784,783,1567,0.0448451042175293,1.730595294596731e-07
785,786,785,1571,0.04494619369506836,1.6550723638749725e-07
786,787,786,1573,0.044997215270996094,1.6185564251320335e-07
787,788,787,1575,0.045046091079711914,1.5828459230159952e-07
788,789,788,1577,0.04509711265563965,1.5479224143548598e-07
789,790,789,1579,0.04515719413757324,1.5137708358770283e-07
790,791,790,1581,0.04520606994628906,1.4803719284836342e-07
791,792,791,1583,0.045255184173583984,1.447710298904865e-07
792,793,792,1585,0.0453031063079834,1.4157695820163265e-07
793,794,793,1587,0.045352935791015625,1.3845325490815582e-07
795,796,795,1591,0.04545712471008301,1.3241117093449674e-07
796,797,796,1593,0.04551196098327637,1.294898018593051e-07
797,798,797,1595,0.04557204246520996,1.2663276417752112e-07
798,799,798,1597,0.04562997817993164,1.238388225291177e-07
799,800,799,1599,0.04568123817443848,1.2110659293946272e-07
800,801,800,1601,0.045736074447631836,1.184345982212447e-07
801,802,801,1603,0.045786142349243164,1.1582158163289262e-07
802,803,802,1605,0.04583406448364258,1.1326612619698239e-07
804,805,804,1609,0.045931100845336914,1.0832320398074545e-07
805,806,805,1611,0.04597926139831543,1.0593327423842855e-07
806,807,806,1613,0.046035051345825195,1.0359599622572091e-07
807,808,807,1615,0.04609107971191406,1.0131035502986396e-07
808,809,808,1617,0.0461421012878418,9.907515899904498e-08
809,810,809,1619,0.04620003700256348,9.68892116020239e-08
810,811,810,1621,0.046253204345703125,9.47515484461297e-08
811,812,811,1623,0.04631400108337402,9.26609564973877e-08
812,813,812,1625,0.046372175216674805,9.061661896596692e-08
814,815,814,1629,0.04647111892700195,8.666208717900616e-08
815,816,815,1631,0.046520233154296875,8.475008649181929e-08
816,817,816,1633,0.046569108963012695,8.28802330205764e-08
817,818,817,1635,0.04662013053894043,8.105157206387547e-08
818,819,818,1637,0.046671152114868164,7.926328102977443e-08
819,820,819,1639,0.046720027923583984,7.751451594486375e-08
820,821,820,1641,0.046772003173828125,7.580430753950502e-08
821,822,821,1643,0.04682612419128418,7.413180990485593e-08
823,824,823,1647,0.04692816734313965,7.089668563869345e-08
824,825,824,1649,0.04697704315185547,6.933248178719568e-08
825,826,825,1651,0.0470280647277832,6.780276916786294e-08
826,827,826,1653,0.047077178955078125,6.630687474330182e-08
827,828,827,1655,0.04712820053100586,6.484389626683674e-08
828,829,828,1657,0.047181129455566406,6.341330637283197e-08
829,830,829,1659,0.04723715782165527,6.201410084642774e-08
830,831,830,1661,0.047289133071899414,6.06458921759559e-08
832,833,832,1665,0.04739999771118164,5.79993119021972e-08
833,834,833,1667,0.04744911193847656,5.6719704939520123e-08
834,835,834,1669,0.047495126724243164,5.5468323017518135e-08
835,836,835,1671,0.047541141510009766,5.4244418319341976e-08
836,837,836,1673,0.04758715629577637,5.304766160685583e-08
837,838,837,1675,0.04763317108154297,5.187723804131085e-08
838,839,838,1677,0.04768514633178711,5.073260568866374e-08
839,840,839,1679,0.04775118827819824,4.961335859650853e-08
840,841,840,1681,0.0478060245513916,4.851871299936514e-08
842,843,842,1685,0.047942161560058594,4.640138391409565e-08
843,844,843,1687,0.04799914360046387,4.537756897807567e-08
844,845,844,1689,0.048052072525024414,4.4376407311604886e-08
845,846,845,1691,0.048104047775268555,4.3397286081131866e-08
846,847,846,1693,0.0481572151184082,4.2439859543538944e-08
847,848,847,1695,0.04820704460144043,4.1503458534923824e-08
848,849,848,1697,0.048258066177368164,4.058774994009136e-08
849,850,849,1699,0.04830813407897949,3.969229186058963e-08
851,852,851,1703,0.04840803146362305,3.7960141130944464e-08
852,853,852,1705,0.048461198806762695,3.712256274467641e-08
853,854,853,1707,0.048528194427490234,3.630359743787117e-08
854,855,854,1709,0.04858708381652832,3.5502554666803064e-08
855,856,855,1711,0.04864096641540527,3.471928488101185e-08
856,857,856,1713,0.0486910343170166,3.395320631848644e-08
857,858,857,1715,0.04874396324157715,3.320416942878849e-08
858,859,858,1717,0.048799991607666016,3.247156331590995e-08
859,860,859,1719,0.04885506629943848,3.1755154900523255e-08
861,862,861,1723,0.0491330623626709,3.0369327681157295e-08
862,863,862,1725,0.049202919006347656,2.9699277601940575e-08
863,864,863,1727,0.04925894737243652,2.9044039310921153e-08
864,865,864,1729,0.049329280853271484,2.8403183536860323e-08
865,866,865,1731,0.04938912391662598,2.7776568484012757e-08
866,867,866,1733,0.04944014549255371,2.7163733806255592e-08
867,868,867,1735,0.04949307441711426,2.6564423103106056e-08
868,869,868,1737,0.049543142318725586,2.597825274483951e-08
870,871,870,1741,0.049642086029052734,2.4844537673663018e-08
871,872,871,1743,0.04969334602355957,2.4296434518171103e-08
872,873,872,1745,0.04974532127380371,2.3760409219380607e-08
873,874,873,1747,0.04979419708251953,2.323616362093626e-08
874,875,874,1749,0.04985308647155762,2.2723497643857263e-08
875,876,875,1751,0.049900054931640625,2.2222119945107167e-08
876,877,876,1753,0.04994916915893555,2.173183627514593e-08
877,878,877,1755,0.049996137619018555,2.1252373723919184e-08
879,880,879,1759,0.05009317398071289,2.0324899999935675e-08
880,881,880,1761,0.05014300346374512,1.9876545030387486e-08
881,882,881,1763,0.05019211769104004,1.943795644356426e-08
882,883,882,1765,0.05023908615112305,1.9009082789223923e-08
883,884,883,1767,0.05028414726257324,1.8589696798087862e-08
884,885,884,1769,0.050330162048339844,1.817952750319496e-08
885,886,885,1771,0.050379037857055664,1.7778418544572487e-08
886,887,886,1773,0.050428152084350586,1.7386211618231685e-08
887,888,887,1775,0.05047607421875,1.700254833670357e-08
889,890,889,1779,0.0505681037902832,1.6260596359590516e-08
890,891,890,1781,0.0506131649017334,1.590185993762055e-08
891,892,891,1783,0.05065798759460449,1.555097081173522e-08
892,893,892,1785,0.0507051944732666,1.5207854209232705e-08
893,894,893,1787,0.0507509708404541,1.4872318803928916e-08
894,895,894,1789,0.05079817771911621,1.454423931323791e-08
895,896,895,1791,0.05084419250488281,1.4223275804343702e-08
896,897,896,1793,0.0509030818939209,1.3909549698451643e-08
898,899,898,1797,0.051004886627197266,1.330251211650884e-08
899,900,899,1799,0.05106210708618164,1.3009013205402411e-08
900,901,900,1801,0.051115989685058594,1.272203494847914e-08
901,902,901,1803,0.05116415023803711,1.2441328695625799e-08
902,903,902,1805,0.05121207237243652,1.216679054415826e-08
903,904,903,1807,0.051258087158203125,1.189840592894953e-08
904,905,904,1809,0.05130410194396973,1.1635849481458407e-08
905,906,905,1811,0.05135011672973633,1.137912801501069e-08
906,907,906,1813,0.05139613151550293,1.1128032716487084e-08
908,909,908,1817,0.051490068435668945,1.0642469088124688e-08
909,910,909,1819,0.051538944244384766,1.0407631694104922e-08
910,911,910,1821,0.05158519744873047,1.0177958172862686e-08
911,912,911,1823,0.05163121223449707,9.953437853389963e-09
912,913,912,1825,0.0516819953918457,9.733826951883057e-09
913,914,913,1827,0.051737070083618164,9.519096338482348e-09
914,915,914,1829,0.051792144775390625,9.30903330581499e-09
915,916,915,1831,0.051841020584106445,9.103648562193014e-09
917,918,917,1835,0.05194211006164551,8.706417612681972e-09
918,919,918,1837,0.051989078521728516,8.514283927011023e-09
919,920,919,1839,0.05203604698181152,8.326459466482152e-09
920,921,920,1841,0.05209016799926758,8.142685881233245e-09
921,922,921,1843,0.052146196365356445,7.9630467039615e-09
922,923,922,1845,0.052201032638549805,7.787429272598547e-09
923,924,923,1847,0.05225706100463867,7.615575236619038e-09
924,925,924,1849,0.05231213569641113,7.4475700775195894e-09
926,927,926,1853,0.05242013931274414,7.122555693849646e-09
927,928,927,1855,0.05246996879577637,6.965371652081703e-09
928,929,928,1857,0.052520036697387695,6.811667422647136e-09
929,930,929,1859,0.05257010459899902,6.661382798928771e-09
930,931,930,1861,0.05261516571044922,6.5144847545374474e-09
931,932,931,1863,0.05266404151916504,6.37071397085743e-09
932,933,932,1865,0.05271291732788086,6.23018797539801e-09
933,934,933,1867,0.05276012420654297,6.092696007706481e-09
934,935,934,1869,0.052805185317993164,5.958240016795014e-09
936,937,936,1873,0.052900075912475586,5.698242684981142e-09
937,938,937,1875,0.052947044372558594,5.572513910701756e-09
938,939,938,1877,0.05300402641296387,5.449579275351016e-09
939,940,939,1879,0.0530550479888916,5.329347494177657e-09
940,941,940,1881,0.05311012268066406,5.211818567311198e-09
941,942,941,1883,0.05315995216369629,5.096783683843895e-09
942,943,942,1885,0.0532071590423584,4.984324428417944e-09
943,944,943,1887,0.053255319595336914,4.874311624532917e-09
945,946,945,1891,0.053353071212768555,4.661627321287278e-09
946,947,946,1893,0.05340433120727539,4.558768388871017e-09
947,948,947,1895,0.0534520149230957,4.458228681887887e-09
948,949,948,1897,0.05350923538208008,4.359866409490801e-09
949,950,949,1899,0.0535731315612793,4.263665057883329e-09
950,951,950,1901,0.05363011360168457,4.169608112503921e-09
951,952,951,1903,0.05368924140930176,4.0775868118967275e-09
952,953,952,1905,0.05376005172729492,3.987666225528707e-09
953,954,953,1907,0.05382823944091797,3.8996482061967075e-09
955,956,955,1911,0.05392718315124512,3.729513205083479e-09
956,957,956,1913,0.053993940353393555,3.6471359191195203e-09
957,958,957,1915,0.054061174392700195,3.5667195081898446e-09
958,959,958,1917,0.054137229919433594,3.4880473594726533e-09
959,960,959,1919,0.0542299747467041,3.411108810674986e-09
960,961,960,1921,0.054305076599121094,3.3357746851690782e-09
961,962,961,1923,0.05437588691711426,3.262155693946089e-09
962,963,962,1925,0.05444502830505371,3.1902246601904834e-09
964,965,964,1929,0.05457305908203125,3.0510156069014238e-09
965,966,965,1931,0.05463123321533203,2.9837084595287415e-09
966,967,966,1933,0.054685354232788086,2.9178328672099618e-09
967,968,967,1935,0.05474209785461426,2.8535141047446713e-09
968,969,968,1937,0.0547940731048584,2.790528798118725e-09
969,970,969,1939,0.054842233657836914,2.7289896098874458e-09
970,971,970,1941,0.05488729476928711,2.6687547510363847e-09
971,972,971,1943,0.05493617057800293,2.609903853508794e-09
973,974,973,1947,0.05509305000305176,2.496013043956323e-09
974,975,974,1949,0.05514216423034668,2.44094205308474e-09
975,976,975,1951,0.055190086364746094,2.3870316509579367e-09
976,977,976,1953,0.05523824691772461,2.3343779835650525e-09
977,978,977,1955,0.05528402328491211,2.2828994682634745e-09
978,979,978,1957,0.055329084396362305,2.2325358992514584e-09
979,980,979,1959,0.055376291275024414,2.183249383256065e-09
980,981,980,1961,0.05542302131652832,2.1350612973345927e-09
981,982,981,1963,0.055477142333984375,2.0880027214375662e-09
983,984,983,1967,0.05557608604431152,1.9968545277996118e-09
984,985,984,1969,0.05562901496887207,1.9528154147945898e-09
985,986,985,1971,0.0556790828704834,1.9097115655982388e-09
986,987,986,1973,0.055730342864990234,1.8675624055989155e-09
987,988,987,1975,0.05578494071960449,1.8264174825199972e-09
988,989,988,1977,0.055834054946899414,1.7860310504165187e-09
989,990,989,1979,0.05589032173156738,1.7466158229990396e-09
990,991,990,1981,0.055938005447387695,1.708104781823992e-09
992,993,992,1985,0.056034088134765625,1.633583556513318e-09
993,994,993,1987,0.05608224868774414,1.5975209194049836e-09
994,995,994,1989,0.05612802505493164,1.5622692261776297e-09
995,996,995,1991,0.056176185607910156,1.527863466720342e-09
996,997,996,1993,0.05622291564941406,1.4940889731269788e-09
997,998,997,1995,0.056272268295288086,1.4611730227905125e-09
998,999,998,1997,0.056333065032958984,1.4289116668519644e-09
999,1000,999,1999,0.0563809871673584,1.39742727138252e-09
1000,1001,1000,2001,0.056429147720336914,1.3665139358918396e-09
1002,1003,1002,2005,0.05653190612792969,1.306962800229682e-09
1003,1004,1003,2007,0.0565800666809082,1.2780851138064408e-09
1004,1005,1004,2009,0.05662703514099121,1.2498891937498846e-09
1005,1006,1005,2011,0.05667400360107422,1.222282804159646e-09
1006,1007,1006,2013,0.05672311782836914,1.1953620897183009e-09
1007,1008,1007,2015,0.056767940521240234,1.1689288986667797e-09
1008,1009,1008,2017,0.05681419372558594,1.143166819589182e-09
1009,1010,1009,2019,0.05686497688293457,1.1179777540193763e-09
1011,1012,1011,2023,0.05698204040527344,1.0691205093271425e-09
1012,1013,1012,2025,0.057032108306884766,1.0455339133553966e-09
1013,1014,1013,2027,0.05708003044128418,1.0225222842478952e-09
1014,1015,1014,2029,0.05713200569152832,9.999379722375662e-10
1015,1016,1015,2031,0.05718517303466797,9.7791015743433e-10
1016,1017,1016,2033,0.05723428726196289,9.56342693225679e-10
1017,1018,1017,2035,0.0572810173034668,9.35204500487646e-10
1018,1019,1018,2037,0.057328224182128906,9.146393204366102e-10
1020,1021,1020,2041,0.05742311477661133,8.746530339066248e-10
1021,1022,1021,2043,0.05747103691101074,8.553902313279615e-10
1022,1023,1022,2045,0.05751919746398926,8.365256216531091e-10
1023,1024,1023,2047,0.057581186294555664,8.180232616760408e-10
1024,1025,1024,2049,0.057639122009277344,8.000026315114943e-10
1025,1026,1025,2051,0.05769801139831543,7.823442516717082e-10
1026,1027,1026,2053,0.05775904655456543,7.650840642271085e-10
1027,1028,1027,2055,0.05781722068786621,7.482385860736119e-10
1028,1029,1028,2057,0.05787491798400879,7.317242791843302e-10
1030,1031,1030,2061,0.05805706977844238,6.997795330236593e-10
1031,1032,1031,2063,0.05810999870300293,6.842820746519306e-10
1032,1033,1032,2065,0.05816221237182617,6.691828070489472e-10
1033,1034,1033,2067,0.05821514129638672,6.544836846885814e-10
1034,1035,1034,2069,0.05826616287231445,6.399865569653082e-10
1035,1036,1035,2071,0.05831503868103027,6.258750103902056e-10
1036,1037,1036,2073,0.058364152908325195,6.120800752748308e-10
1037,1038,1037,2075,0.058413028717041016,5.985395877898194e-10
1039,1040,1039,2079,0.058512210845947266,5.725065421427065e-10
1040,1041,1040,2081,0.05856204032897949,5.598556783223397e-10
1041,1042,1041,2083,0.05861020088195801,5.474903437361277e-10
1042,1043,1042,2085,0.05865907669067383,5.353959767434023e-10
1043,1044,1043,2087,0.05870699882507324,5.236036556816871e-10
1044,1045,1044,2089,0.058767080307006836,5.119842018621766e-10
1045,1046,1045,2091,0.058817148208618164,5.007483766505677e-10
1046,1047,1046,2093,0.05886697769165039,4.896854195281439e-10
1047,1048,1047,2095,0.05891609191894531,4.788953832972055e-10
1049,1050,1049,2099,0.05903005599975586,4.5801359683230384e-10
1050,1051,1050,2101,0.059087276458740234,4.478548242971066e-10
1051,1052,1051,2103,0.059144020080566406,4.3805055537893107e-10
1052,1053,1052,2105,0.059203147888183594,4.2828997376952316e-10
1053,1054,1053,2107,0.05927014350891113,4.1891497660075774e-10
1054,1055,1054,2109,0.059333086013793945,4.0960018715114647e-10
1055,1056,1055,2111,0.059388160705566406,4.0063794248832777e-10
1056,1057,1056,2113,0.059446096420288086,3.9175242124167735e-10
1058,1059,1058,2117,0.05959916114807129,3.746505393790235e-10
1059,1060,1059,2119,0.05967307090759277,3.664196137380893e-10
1060,1061,1060,2121,0.05975031852722168,3.583615565179284e-10
1061,1062,1061,2123,0.05982208251953125,3.5044724159302875e-10
1062,1063,1062,2125,0.0598909854888916,3.427057916794146e-10
1063,1064,1063,2127,0.059963226318359375,3.350770057795157e-10
1064,1065,1064,2129,0.060027122497558594,3.27750266125666e-10
1065,1066,1065,2131,0.06008601188659668,3.204380912833417e-10
1067,1068,1067,2135,0.060212135314941406,3.0645376899779945e-10
1068,1069,1068,2137,0.060272216796875,2.997146062684642e-10
1069,1070,1069,2139,0.06032729148864746,2.931026676484333e-10
1070,1071,1070,2141,0.06038403511047363,2.866179532803119e-10
1071,1072,1071,2143,0.060445308685302734,2.8030806205042515e-10
1072,1073,1072,2145,0.06050825119018555,2.741108315519524e-10
1073,1074,1073,2147,0.060572147369384766,2.680864708488592e-10
1074,1075,1074,2149,0.06063413619995117,2.621747682088018e-10
1075,1076,1075,2151,0.06069302558898926,2.5640681088465204e-10
1077,1078,1077,2155,0.060797929763793945,2.452311946412798e-10
1078,1079,1078,2157,0.06084609031677246,2.398614244647381e-10
1079,1080,1079,2159,0.06089615821838379,2.3453730077056327e-10
1080,1081,1080,2161,0.06094622611999512,2.293714793280497e-10
1081,1082,1081,2163,0.06099510192871094,2.243183257661177e-10
1082,1083,1082,2165,0.061044931411743164,2.19310806265918e-10
1083,1084,1083,2167,0.06109428405761719,2.144470383865247e-10
1084,1085,1084,2169,0.061144113540649414,2.098231484713792e-10
1086,1087,1086,2173,0.061244964599609375,2.0061906585764275e-10
1087,1088,1087,2175,0.06131720542907715,1.961699993914908e-10
1088,1089,1088,2177,0.06136822700500488,1.9184816221596238e-10
1089,1090,1089,2179,0.06144213676452637,1.8766810746188453e-10
1090,1091,1090,2181,0.06150102615356445,1.835045768196647e-10
1091,1092,1091,2183,0.06155800819396973,1.794682673554787e-10
1092,1093,1092,2185,0.061611175537109375,1.7546107804648654e-10
1093,1094,1093,2187,0.06166195869445801,1.715830741570755e-10
1094,1095,1094,2189,0.06171917915344238,1.6783229087103904e-10
1096,1097,1096,2193,0.06181812286376953,1.6049099156186033e-10
1097,1098,1097,2195,0.061866044998168945,1.5691307661382847e-10
1098,1099,1098,2197,0.06191515922546387,1.5346434350948917e-10
1099,1100,1099,2199,0.06196403503417969,1.5012827041115134e-10
1100,1101,1100,2201,0.06201291084289551,1.4679220930592685e-10
1101,1102,1101,2203,0.06209731101989746,1.435308945628077e-10
1102,1103,1102,2205,0.06215023994445801,1.4036964889450278e-10
1103,1104,1103,2207,0.062200069427490234,1.3731910488071225e-10
1105,1106,1105,2211,0.06230616569519043,1.3130930160015377e-10
1106,1107,1106,2213,0.06235694885253906,1.2843358458174707e-10
1107,1108,1107,2215,0.0624089241027832,1.2555590579833495e-10
1108,1109,1108,2217,0.06247305870056152,1.2280740999601188e-10
1109,1110,1109,2219,0.06252503395080566,1.2007347797270158e-10
1110,1111,1110,2221,0.0625762939453125,1.1746872890468555e-10
1111,1112,1111,2223,0.06262826919555664,1.1489309549807627e-10
1112,1113,1112,2225,0.06267595291137695,1.1231746528912807e-10
1114,1115,1114,2229,0.06277298927307129,1.0743717706238036e-10
1115,1116,1115,2231,0.0628211498260498,1.050888412949793e-10
1116,1117,1116,2233,0.06286811828613281,1.0270063080882094e-10
1117,1118,1117,2235,0.06291508674621582,1.0039596965017854e-10
1118,1119,1118,2237,0.06296300888061523,9.822048273450043e-11


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n10/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00016832351684570312,542.5060889379029
1,4,4,8,0.0003509521484375,437.43651362206106
2,6,6,12,0.0006814002990722656,500.9910455002406
3,8,8,16,0.0009562969207763672,283.995165641375
4,10,10,20,0.0011751651763916016,98.73967534940398
5,12,12,24,0.001379251480102539,48.64250305757986
6,14,14,28,0.0016331672668457031,45.98157682107862
7,16,16,32,0.0019252300262451172,30.634562708932165
8,18,18,36,0.0021822452545166016,25.34876679456932
9,24,24,48,0.0026361942291259766,20.946461685948265
10,28,28,56,0.002978086471557617,13.77872492523781
11,34,34,68,0.0033431053161621094,11.82937972302457
12,42,42,84,0.0038611888885498047,11.188307611800841
13,50,50,100,0.0043561458587646484,7.050555831482018
14,58,58,116,0.004944324493408203,5.800979760574122
15,66,66,132,0.005384922027587891,4.802213879133725
16,68,68,136,0.005591154098510742,7.601934771224064
17,70,70,140,0.005851268768310547,0.05058893989745001
18,72,72,144,0.006077289581298828,0.0479459468159699
19,74,74,148,0.006344318389892578,0.0022762552666861233
20,76,76,152,0.006565093994140625,0.0009311500991786255
21,78,78,156,0.006801128387451172,4.960706692318229e-12


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n10/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.081031799316406e-05,542.5060889379029
1,4,4,8,0.00020694732666015625,437.43651362206106
2,6,6,12,0.0004699230194091797,250.68522250518726
3,8,8,16,0.0007090568542480469,193.07695757789975
4,10,10,20,0.0009720325469970703,116.59292642060402
5,12,12,24,0.0011758804321289062,68.21186468102738
6,14,14,28,0.0014159679412841797,70.84898259738459
7,16,16,32,0.0016329288482666016,32.22718672548579
8,18,18,36,0.0019979476928710938,26.64452123526115
9,22,22,44,0.002329111099243164,24.606731282542263
10,26,26,52,0.002650022506713867,22.21388258074964
11,28,28,56,0.0029039382934570312,19.072857774546346
12,30,30,60,0.003159046173095703,12.412742376047396
13,36,36,72,0.003551959991455078,13.107095737336845
14,44,44,88,0.00400090217590332,5.7849392509685185
15,50,50,100,0.004400730133056641,4.9118785196109975
16,58,58,116,0.004823923110961914,3.5486959483862526
17,60,60,120,0.0050809383392333984,0.17347250016548185
18,62,62,124,0.005343914031982422,0.16450650845181203
19,64,64,128,0.0056018829345703125,0.02271219525515278
20,66,66,132,0.005810976028442383,5.1160245900507605e-12


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n100/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0001659393310546875,1624.447741208611
1,2,1,3,0.0003619194030761719,66480.312266118
2,3,2,5,0.0008180141448974609,14341.46814081151
3,4,3,7,0.0015728473663330078,14461.317840003707
4,5,4,9,0.0019469261169433594,14433.618717844925
5,6,5,11,0.0022039413452148438,14396.852887404397
6,7,6,13,0.0024399757385253906,14347.479192894445
7,8,7,15,0.002574920654296875,14281.255685788452
8,9,8,17,0.002716064453125,14192.575556676999
9,10,9,19,0.002907991409301758,14074.08233854318
10,11,10,21,0.003062009811401367,13916.218043252082
11,12,11,23,0.0032148361206054688,13706.733207527326
12,13,12,25,0.003401041030883789,13430.230862591334
13,14,13,27,0.0035867691040039062,13067.895133560034
14,15,14,29,0.0037698745727539062,12596.264706656275
15,16,15,31,0.004019021987915039,11955.95988615279
16,17,16,33,0.004194974899291992,11113.464924978862
17,18,17,35,0.004385948181152344,10048.982070197228
18,19,18,37,0.004560947418212891,8727.81879293032
19,20,19,39,0.004756927490234375,7180.805058867846
20,21,20,41,0.0049359798431396484,5584.378706764449
21,22,21,43,0.0052509307861328125,4202.480134190401
22,23,22,45,0.0055429935455322266,2999.138954000196
23,24,23,47,0.006330013275146484,3264.889341797864
24,25,24,49,0.006636857986450195,3412.343153645238
25,26,25,51,0.006834983825683594,2352.8850025209904
26,27,26,53,0.007047891616821289,1809.5747538939772
27,28,27,55,0.00724482536315918,1595.3048090201014
28,29,28,57,0.007501840591430664,1500.3146609901853
29,30,29,59,0.007652997970581055,1328.880560238683
30,31,30,61,0.007832765579223633,1207.6473496388983
31,32,31,63,0.008026838302612305,1001.1475342960471
32,33,32,65,0.008206844329833984,903.9535897388365
33,34,33,67,0.009765863418579102,694.6687185977336
34,35,34,69,0.01005697250366211,777.3117430420552
35,36,35,71,0.010441064834594727,810.3792926385242
36,37,36,73,0.010597944259643555,704.604802111637
37,38,37,75,0.010798931121826172,593.9726965086217
38,39,38,77,0.011052131652832031,488.45320765521217
39,40,39,79,0.011219024658203125,397.2831966338014
40,41,40,81,0.011361837387084961,288.44388149739746
41,42,41,83,0.011511087417602539,253.13674828935748
42,43,42,85,0.01164388656616211,211.99678386519972
43,44,43,87,0.012024879455566406,209.53369989489195
44,45,44,89,0.01227712631225586,179.04104446788813
45,46,45,91,0.012687921524047852,152.31559956315436
46,47,46,93,0.012848854064941406,171.15729466784816
47,48,47,95,0.01321101188659668,211.03276379821358
48,49,48,97,0.013535022735595703,208.37154346651172
49,50,49,99,0.013754844665527344,196.80024225903858
50,51,50,101,0.013961076736450195,177.82040656391362
51,52,51,103,0.014284133911132812,161.24486217707576
52,53,52,105,0.014627933502197266,153.38882020210585
53,54,53,107,0.016881942749023438,150.61097993265344
54,55,54,109,0.01787877082824707,135.76958053430312
55,56,55,111,0.018178939819335938,126.77788355928496
56,57,56,113,0.01838397979736328,141.84718278535036
57,58,57,115,0.019345998764038086,149.854735822487
58,59,58,117,0.01966381072998047,149.29759713698084
59,60,59,119,0.01989889144897461,148.61262535949174
60,61,60,121,0.020103931427001953,134.1097655197761
61,62,61,123,0.02034783363342285,129.61821999020552
62,63,62,125,0.02063584327697754,127.44058854786189
63,64,63,127,0.020817041397094727,125.28596557763727
64,65,64,129,0.021062850952148438,116.19280308703794
65,66,65,131,0.02126908302307129,113.38147538850397
66,67,66,133,0.021423816680908203,124.91022290460728
67,68,67,135,0.021804094314575195,117.12726507032242
68,69,68,137,0.022009849548339844,112.56254792581356
69,70,69,139,0.022497177124023438,102.83719623968022
70,71,70,141,0.022738933563232422,104.21770518435213
71,72,71,143,0.02295207977294922,118.63945735860626
72,73,72,145,0.02317190170288086,115.98516499429263
73,74,73,147,0.02336597442626953,115.65319338797408
74,75,74,149,0.02351999282836914,111.19439878400193
75,76,75,151,0.02371692657470703,104.39076960191902
76,77,76,153,0.02399587631225586,103.0696248671041
77,78,77,155,0.024293899536132812,101.60264780782458
78,79,78,157,0.024452924728393555,100.02040175527613
79,80,79,159,0.024662017822265625,98.37340684616927
80,81,80,161,0.024971961975097656,96.66423208494595
81,82,81,163,0.025355100631713867,94.80755318932252
82,83,82,165,0.02564692497253418,92.61929085812723
83,84,83,167,0.025935888290405273,82.20467883091727
84,85,84,169,0.026123046875,82.2276336179846
85,86,85,171,0.026276826858520508,93.41373837132049
86,87,86,173,0.026408910751342773,93.1517319305314
87,88,87,175,0.026525020599365234,92.85377700988873
88,89,88,177,0.02682805061340332,92.46553789833177
89,90,89,179,0.02739095687866211,91.96342646834663
90,91,90,181,0.027637004852294922,91.31221138337814
91,92,91,183,0.027830123901367188,87.36978006174586
92,93,92,185,0.027949810028076172,81.52768846267267
93,94,93,187,0.028123855590820312,79.97762508017738
94,95,94,189,0.028279781341552734,73.99020181783855
95,96,95,191,0.028472900390625,76.4313072728746
96,97,96,193,0.028609037399291992,85.59622610405714
97,98,97,195,0.030334949493408203,80.53924771322855
98,99,98,197,0.030627965927124023,80.139048829788
99,100,99,199,0.03119802474975586,79.6378129219736
100,101,100,201,0.031538963317871094,75.24638490190657
101,102,101,203,0.03183698654174805,74.22609156241481
102,103,102,205,0.03207993507385254,73.0635167267425
103,104,103,207,0.032257080078125,67.04428064270962
104,105,104,209,0.0324249267578125,65.31825182865164
105,106,105,211,0.032594919204711914,66.05070641356507
106,107,106,213,0.032788991928100586,72.53922026942206
107,108,107,215,0.03298783302307129,72.404081980174
108,109,108,217,0.03342080116271973,72.24099241556611
109,110,109,219,0.03365302085876465,72.02584820554755
110,111,110,221,0.033822059631347656,71.7441842010779
111,112,111,223,0.03401303291320801,66.68664534216039
112,113,112,225,0.034208059310913086,66.03907776918946
113,114,113,227,0.036170005798339844,65.27496863149007
114,115,114,229,0.03638195991516113,64.36291090607604
115,116,115,231,0.03656196594238281,63.26695724899916
116,117,116,233,0.036769866943359375,41.053399654700996
117,118,117,235,0.0369570255279541,39.75806275852081
118,119,118,237,0.03709602355957031,37.99046284633607
119,120,119,239,0.03723907470703125,36.091526421798235
120,121,120,241,0.037377119064331055,26.286419950819667
121,122,121,243,0.03751206398010254,38.203566208014486
122,123,122,245,0.03769874572753906,37.6464158733411
123,124,123,247,0.037867069244384766,37.30231938233656
124,125,124,249,0.03802299499511719,36.7792516252911
125,126,125,251,0.03816986083984375,36.1252312788008
126,127,126,253,0.03832507133483887,35.268352756834226
127,128,127,255,0.03855013847351074,27.64634537526409
128,129,128,257,0.038800954818725586,26.011098170455444
129,130,129,259,0.038977861404418945,28.14626413478884
130,131,130,261,0.03923988342285156,34.945132292472316
131,132,131,263,0.03950381278991699,34.8115637631556
132,133,132,265,0.039659976959228516,34.62359070489218
133,134,133,267,0.04034996032714844,34.37439158674657
134,135,134,269,0.04072403907775879,27.516130462820737
135,136,135,271,0.04139995574951172,26.89648792414325
136,137,136,273,0.04179096221923828,26.214114204686044
137,138,137,275,0.042085886001586914,25.424876388576987
138,139,138,277,0.04224801063537598,21.595524657869593
139,140,139,279,0.04251885414123535,20.763485350549875
140,141,140,281,0.04281187057495117,20.493499462689265
141,142,141,283,0.04311990737915039,21.238159792348153
142,143,142,285,0.0434267520904541,20.825768927194044
143,144,143,287,0.04367995262145996,20.339039472400103
144,145,144,289,0.04384589195251465,18.763839534692664
145,146,145,291,0.04401588439941406,17.982728372662297
146,147,146,293,0.04439997673034668,18.521217584717395
147,148,147,295,0.044754981994628906,20.045268367213325
148,149,148,297,0.04491901397705078,19.943585971892702
149,150,149,299,0.045194149017333984,19.813130208921198
150,151,150,301,0.04588913917541504,18.689135647777793
151,152,151,303,0.04620099067687988,18.425282899092124
152,153,152,305,0.04644489288330078,18.099639831993226
153,154,153,307,0.04657602310180664,17.689022860468814
154,155,154,309,0.0467379093170166,17.173316720234435
155,156,155,311,0.04688000679016113,16.522933105404036
156,157,156,313,0.047020912170410156,15.70311606888202
157,158,157,315,0.0471649169921875,7.269409531819816
158,159,158,317,0.04764080047607422,16.048535296917258
159,160,159,319,0.048219919204711914,15.61419732633783
160,161,160,321,0.0488588809967041,15.110883046675127
161,162,161,323,0.04908609390258789,6.86175600860245
162,163,162,325,0.04934096336364746,15.714283837481105
163,164,163,327,0.04964590072631836,15.678307557616668
164,165,164,329,0.049813032150268555,15.631355260104748
165,166,165,331,0.05016493797302246,15.568708547941736
166,167,166,333,0.05036807060241699,15.485211722410574
167,168,167,335,0.0514528751373291,15.37424259059334
168,169,168,337,0.05182194709777832,15.227228241040335
169,170,169,339,0.052014827728271484,15.033137715199583
170,171,170,341,0.05226707458496094,7.350017934603584
171,172,171,343,0.052461862564086914,15.061350801723588
172,173,172,345,0.052659034729003906,7.587286659508479
173,174,173,347,0.052906036376953125,7.320275997611698
174,175,174,349,0.05303192138671875,7.474882960645439
175,176,175,351,0.05484795570373535,7.546397717422357
176,177,176,353,0.05500602722167969,7.434545006098061
177,178,177,355,0.05516386032104492,7.302824442244538
178,179,178,357,0.05533909797668457,7.139599053889025
179,180,179,359,0.05551004409790039,6.943436996632568
180,181,180,361,0.05566287040710449,6.916189089907064
181,182,181,363,0.055809736251831055,6.698122211635634
182,183,182,365,0.05597281455993652,6.791050001269135
183,184,183,367,0.056169986724853516,6.89462583261384
184,185,184,369,0.05629897117614746,6.815839045334052
185,186,185,371,0.05641984939575195,6.723950038753889
186,187,186,373,0.056550025939941406,6.608597361855441
187,188,187,375,0.05668997764587402,5.081719251988298
188,189,188,377,0.056819915771484375,4.929845463484044
189,190,189,379,0.05697798728942871,4.822533982388492
190,191,190,381,0.057127952575683594,4.684962999078752
191,192,191,383,0.0572659969329834,4.508856446867718
192,193,192,385,0.05744194984436035,4.286011416172168
193,194,193,387,0.057598114013671875,4.007687467672218
194,195,194,389,0.05777096748352051,3.6670938598022187
195,196,195,391,0.05792117118835449,3.2621763397137156
196,197,196,393,0.05806398391723633,2.227088972392815
197,198,197,395,0.05822396278381348,3.7751892218765275
198,199,198,397,0.05840492248535156,3.746635164515441
199,200,199,399,0.058537960052490234,3.715697817111954
200,201,200,401,0.05865979194641113,3.6747394306870143
201,202,201,403,0.05878400802612305,3.6206080164915715
202,203,202,405,0.05894899368286133,3.549485752861317
203,204,203,407,0.05926799774169922,3.4566645370454605
204,205,204,409,0.059419870376586914,3.3365577515925615
205,206,205,411,0.059600830078125,3.1828734960920295
206,207,206,413,0.0597379207611084,2.4317659921488683
207,208,207,415,0.05989193916320801,3.1335629842218222
208,209,208,417,0.060025930404663086,3.2537054811488444
209,210,209,419,0.0601811408996582,3.2179695358006914
210,211,210,421,0.060324907302856445,3.173862240638381
211,212,211,423,0.06046700477600098,3.115485339250638
212,213,212,425,0.060647010803222656,2.4894356912774347
213,214,213,427,0.06082010269165039,2.376549439522118
214,215,214,429,0.06099200248718262,2.492022594955385
215,216,215,431,0.061192989349365234,3.068263882841167
216,217,216,433,0.061363935470581055,2.479923303639887
217,218,217,435,0.06149792671203613,2.4381509405375152
218,219,218,437,0.06164407730102539,2.3867723658766415
219,220,219,439,0.0617828369140625,2.3224421005865112
220,221,220,441,0.061921119689941406,2.2433067586912516
221,222,221,443,0.06368684768676758,2.2053444349065034
222,223,222,445,0.0640568733215332,2.105153573439436
223,224,223,447,0.06422901153564453,2.154027655358992
224,225,224,449,0.06441593170166016,2.220281745812093
225,226,225,451,0.06459975242614746,2.196200913203472
226,227,226,453,0.06477499008178711,2.1673253795168876
227,228,227,455,0.06492090225219727,2.1297730359195284
228,229,228,457,0.06508803367614746,2.0816213906801138
229,230,229,459,0.06525492668151855,2.020442755191433
230,231,230,461,0.06538891792297363,1.9434707565791276
231,232,231,463,0.06554508209228516,1.8475661810403092
232,233,232,465,0.06570100784301758,1.7293833048258431
233,234,233,467,0.06585192680358887,1.5859537293404178
234,235,234,469,0.06598687171936035,0.7252404474179305
235,236,235,471,0.06610584259033203,0.4185407753917853
236,237,236,473,0.0662529468536377,1.6861037474464389
237,238,237,475,0.06642484664916992,1.6851731962603582
238,239,238,477,0.06659698486328125,1.6838876296067853
239,240,239,479,0.0667579174041748,1.6821604390877678
240,241,240,481,0.06699395179748535,1.6798397517717565
241,242,241,483,0.06717801094055176,1.6767247051100043
242,243,242,485,0.06753396987915039,1.6725488238756219
243,244,243,487,0.06771373748779297,1.6669604060452743
244,245,244,489,0.06795907020568848,1.6594983303733066
245,246,245,491,0.0685579776763916,1.6495631116794278
246,247,246,493,0.06878018379211426,1.6363836015535016
247,248,247,495,0.0689401626586914,1.6189805567170612
248,249,248,497,0.06923079490661621,1.5961291977613332
249,250,249,499,0.06946492195129395,1.566323603870103
250,251,250,501,0.06972384452819824,1.5277466686869614
251,252,251,503,0.06987977027893066,1.4782532994147433
252,253,252,505,0.07003092765808105,0.6933876125098047
253,254,253,507,0.07031106948852539,0.5607530606607608
254,255,254,509,0.07051491737365723,1.5055914443206322
255,256,255,511,0.07135009765625,1.5033236175095301
256,257,256,513,0.07222294807434082,1.5002603057120256
257,258,257,515,0.07238507270812988,1.4961562912875006
258,259,258,517,0.0725870132446289,1.4906623869671758
259,260,259,519,0.07276487350463867,1.483323697708481
260,261,260,521,0.07294702529907227,1.4735477859328214
261,262,261,523,0.07320499420166016,1.4605709741864152
262,263,262,525,0.07335996627807617,1.4434210310118207
263,264,263,527,0.0736091136932373,0.6754406617502472
264,265,264,529,0.07378888130187988,0.6277636745228365
265,266,265,531,0.07434892654418945,1.4422581781464605
266,267,266,533,0.07482409477233887,1.4360715297418858
267,268,267,535,0.07499098777770996,1.42777315645342
268,269,268,537,0.0751340389251709,0.6574764542520731
269,270,269,539,0.07527899742126465,0.6355755144404837
270,271,270,541,0.075408935546875,0.6427907563601136
271,272,271,543,0.07572698593139648,0.6464244305576664
272,273,272,545,0.07615399360656738,0.633954580791477
273,274,273,547,0.07648587226867676,0.6184643195280267
274,275,274,549,0.07663393020629883,0.604570789429221
275,276,275,551,0.07676506042480469,0.6049178820156943
276,277,276,553,0.0768887996673584,0.5990756580792297
277,278,277,555,0.0770120620727539,0.5893732761327974
278,279,278,557,0.07716894149780273,0.579435510874912
279,280,279,559,0.07758593559265137,0.5741490630150198
280,281,280,561,0.07773399353027344,0.5677590605258795
281,282,281,563,0.07789182662963867,0.5607880363032088
282,283,282,565,0.07802295684814453,0.5531399782517495
283,284,283,567,0.07816672325134277,0.5464671624069432
284,285,284,569,0.07834196090698242,0.5401551739129268
285,286,285,571,0.07847309112548828,0.5336742686743067
286,287,286,573,0.07860302925109863,0.5270580758382414
287,288,287,575,0.07872891426086426,0.5206563987044027
288,289,288,577,0.07887697219848633,0.5144761230218802
289,290,289,579,0.07906699180603027,0.5083618961183305
290,291,290,581,0.07939314842224121,0.5022747317852584
291,292,291,583,0.07975602149963379,0.49627613459559883
292,293,292,585,0.08001899719238281,0.4903963920125888
293,294,293,587,0.0801858901977539,0.48461107049557867
294,295,294,589,0.08104205131530762,0.47889932601475277
295,296,295,591,0.08119988441467285,0.4732639079019063
296,297,296,593,0.08133101463317871,0.4677129689753158
297,298,297,595,0.08146214485168457,0.4622450798330764
298,299,298,597,0.08159995079040527,0.45685433315588975
299,300,299,599,0.08179378509521484,0.45153723640456706
300,301,300,601,0.0820009708404541,0.4462931658854212
301,302,301,603,0.08213472366333008,0.4411211375219804
302,303,302,605,0.08229899406433105,0.43601899583580056
303,304,303,607,0.08243680000305176,0.4309841543727129
304,305,304,609,0.08256101608276367,0.42601444486943063
305,306,305,611,0.08269691467285156,0.42110786808353495
306,307,306,613,0.0828409194946289,0.41626237449869935
307,308,307,615,0.0830228328704834,0.4114756715961943
308,309,308,617,0.08319902420043945,0.4067454266354768
309,310,309,619,0.08350896835327148,0.40206922367491715
310,311,310,621,0.08368897438049316,0.39744465601128653
311,312,311,623,0.08388781547546387,0.39286916771464037
312,313,312,625,0.08413290977478027,0.38834016150134976
313,314,313,627,0.08429694175720215,0.38385485356959975
314,315,314,629,0.0847010612487793,0.3794104340867314
315,316,315,631,0.08497095108032227,0.375003860656432
316,317,316,633,0.08514690399169922,0.3706320770779545
317,318,317,635,0.08536601066589355,0.366291700642812
318,319,318,637,0.08572506904602051,0.36197938260565715
319,320,319,639,0.08606910705566406,0.35769128856384447
320,321,320,641,0.0862119197845459,0.35342375386332686
321,322,321,643,0.0863649845123291,0.3491723100481855
322,323,322,645,0.08651089668273926,0.34493301434731355
323,324,323,647,0.0866551399230957,0.34070040645839084
324,325,324,649,0.0867919921875,0.33647052311427805
325,326,325,651,0.08691596984863281,0.3322360733724812
326,327,326,653,0.08705806732177734,0.327994089515171
327,328,327,655,0.08719396591186523,0.32373307623613956
328,329,328,657,0.08748793601989746,0.31945482946226317
329,330,329,659,0.08835315704345703,0.31513572265391865
330,331,330,661,0.0893259048461914,0.31079695412052627
331,332,331,663,0.08954286575317383,0.3063721583304791
332,333,332,665,0.08971500396728516,0.3019641309360552
333,334,333,667,0.08998298645019531,0.29732827977106996
334,335,334,669,0.09018301963806152,0.29294379045103136
335,336,335,671,0.09034395217895508,0.2876931398230988
336,337,336,673,0.09051203727722168,0.2839946668274124
337,338,337,675,0.09068083763122559,0.2751994427239268
338,339,338,677,0.09090209007263184,0.27581382947717054
339,340,339,679,0.0910789966583252,0.2874353214570422
340,341,340,681,0.09123110771179199,0.28675778167149324
341,342,341,683,0.09139680862426758,0.28591633058948807
342,343,342,685,0.09154701232910156,0.28479097085675087
343,344,343,687,0.09168481826782227,0.2832907448475324
344,345,344,689,0.09182095527648926,0.28129753475184355
345,346,345,691,0.09195184707641602,0.27866073860531393
346,347,346,693,0.09209394454956055,0.2751912519506226
347,348,347,695,0.0922708511352539,0.2706558395583119
348,349,348,697,0.09253311157226562,0.26477244649104614
349,350,349,699,0.09270691871643066,0.2572069387652933
350,351,350,701,0.09299898147583008,0.24757238411670957
351,352,351,703,0.09322094917297363,0.23940397849652206
352,353,352,705,0.09338998794555664,0.22708883533723045
353,354,353,707,0.0936899185180664,0.22997432777483937
354,355,354,709,0.09387707710266113,0.2435799041288883
355,356,355,711,0.0940408706665039,0.24166224705512868
356,357,356,713,0.09421086311340332,0.2393259815255683
357,358,357,715,0.09452390670776367,0.23622848485600617
358,359,358,717,0.09485697746276855,0.23214874598737864
359,360,359,719,0.09511899948120117,0.22680959355575184
360,361,360,721,0.0955960750579834,0.2198780957871772
361,362,361,723,0.09573101997375488,0.21096943677590774
362,363,362,725,0.09587216377258301,0.1996673207246075
363,364,363,727,0.09600496292114258,0.18557645348345495
364,365,364,729,0.09612298011779785,0.16842759533702387
365,366,365,731,0.09625887870788574,0.15586211684774778
366,367,366,733,0.09639310836791992,0.13371926250563898
367,368,367,735,0.09654402732849121,0.15868584916771908
368,369,368,737,0.09669780731201172,0.1639024141753832
369,370,369,739,0.09685492515563965,0.158137941973668
370,371,370,741,0.09699010848999023,0.15130547362875005
371,372,371,743,0.09714579582214355,0.1425918441238957
372,373,372,745,0.09829998016357422,0.13176974241445527
373,374,373,747,0.09887003898620605,0.11868406573582256
374,375,374,749,0.09904193878173828,0.10345677206635708
375,376,375,751,0.0991818904876709,0.08657182812786593
376,377,376,753,0.09936809539794922,0.08309196629068981
377,378,377,755,0.09951281547546387,0.06184898445277676
378,379,378,757,0.09965801239013672,0.09067995131694434
379,380,379,759,0.09981179237365723,0.09003785905406819
380,381,380,761,0.099945068359375,0.09657899138279351
381,382,381,763,0.10007405281066895,0.09636943979264737
382,383,382,765,0.1002039909362793,0.09611044293984768
383,384,383,767,0.10033893585205078,0.09576262143142342
384,385,384,769,0.10048389434814453,0.09529616762041856
385,386,385,771,0.10063600540161133,0.09467166282948808
386,387,386,773,0.10076403617858887,0.09383743256591973
387,388,387,775,0.10088205337524414,0.09272642005888754
388,389,388,777,0.10100698471069336,0.0912528331907601
389,390,389,779,0.10112905502319336,0.08930910057299095
390,391,390,781,0.10129380226135254,0.0867642396787898
391,392,391,783,0.10143184661865234,0.08346565705502312
392,393,392,785,0.10155701637268066,0.07924771252400852
393,394,393,787,0.1016850471496582,0.07395186902141064
394,395,394,789,0.10182881355285645,0.06746400700463402
395,396,395,791,0.10200095176696777,0.059772294680576016
396,397,396,793,0.10212898254394531,0.051040170755676954
397,398,397,795,0.1022958755493164,0.04166999937218997
398,399,398,797,0.10244297981262207,0.042642479311263484
399,400,399,799,0.10260796546936035,0.05247441558349193
400,401,400,801,0.10278582572937012,0.04737590623729484
401,402,401,803,0.10321593284606934,0.04309184718360677
402,403,402,805,0.10336112976074219,0.03779164810756731
403,404,403,807,0.10353589057922363,0.031891866022615054
404,405,404,809,0.10367298126220703,0.025734294791687134
405,406,405,811,0.10381197929382324,0.035365363556073615
406,407,406,813,0.10396695137023926,0.03388204234975861
407,408,407,815,0.10416388511657715,0.03546534490296981
408,409,408,817,0.10443902015686035,0.03396070816580271
409,410,409,819,0.1047508716583252,0.03222060901357562
410,411,410,821,0.10488390922546387,0.030033553725426675
411,412,411,823,0.1055459976196289,0.02735517223244065
412,413,412,825,0.10582590103149414,0.024194157154443174
413,414,413,827,0.10607600212097168,0.020606595763428496
414,415,414,829,0.10623908042907715,0.016792629769318324
415,416,415,831,0.10635805130004883,0.01993152484789297
416,417,416,833,0.10654807090759277,0.02136560926801935
417,418,417,835,0.10669898986816406,0.019405198242474483
418,419,418,837,0.10685396194458008,0.017526590322728495
419,420,419,839,0.10700201988220215,0.015356597832480404
420,421,420,841,0.10712003707885742,0.012917796411882456
421,422,421,843,0.10726785659790039,0.017305163791660937
422,423,422,845,0.1074368953704834,0.016306625647765548
423,424,423,847,0.10768795013427734,0.015411293115797422
424,425,424,849,0.10781192779541016,0.014281904532111658
425,426,425,851,0.10794711112976074,0.01290230312380845
426,427,426,853,0.10807991027832031,0.01130614845289011
427,428,427,855,0.1082310676574707,0.00949884564669223
428,429,428,857,0.10847997665405273,0.007682698721166698
429,430,429,859,0.1086721420288086,0.011626636502727453
430,431,430,861,0.10880112648010254,0.011115873558436233
431,432,431,863,0.10906195640563965,0.010679024274575847
432,433,432,865,0.10922408103942871,0.010114597756234984
433,434,433,867,0.10941195487976074,0.009407116455711045
434,435,434,869,0.10958194732666016,0.00854709918452284
435,436,435,871,0.10976195335388184,0.007531877604113676
436,437,436,873,0.10988497734069824,0.006392308240390558
437,438,437,875,0.11002874374389648,0.0051738658288600576
438,439,438,877,0.11016082763671875,0.004001686655688144
439,440,439,879,0.11034202575683594,0.0067299690865775565
440,441,440,881,0.11050987243652344,0.006284350466575288
441,442,441,883,0.11066985130310059,0.005945876602569633
442,443,442,885,0.11086297035217285,0.005511245461313119
443,444,443,887,0.11103010177612305,0.004981512321792579
444,445,444,889,0.11118602752685547,0.004367339484182401
445,446,445,891,0.11131715774536133,0.003672638763999776
446,447,446,893,0.11144495010375977,0.0029692991553993495
447,448,447,895,0.1115880012512207,0.004452364887128656
448,449,448,897,0.11171388626098633,0.004212897730160423
449,450,449,899,0.11182808876037598,0.004012159814168028
450,451,450,901,0.11197495460510254,0.003754970568891069
451,452,451,903,0.1125340461730957,0.003437453654834296
452,453,452,905,0.11292910575866699,0.003061182840691994
453,454,453,907,0.11357688903808594,0.0026281779614489497
454,455,454,909,0.11374807357788086,0.00216526238045758
455,456,455,911,0.11389708518981934,0.0027106960356530563
456,457,456,913,0.11405491828918457,0.0026995323283796582
457,458,457,915,0.11427783966064453,0.002996080494517269
458,459,458,917,0.1144568920135498,0.0029923538782303757
459,460,459,919,0.11461997032165527,0.0029879108248709943
460,461,460,921,0.11480498313903809,0.0029819347301472303
461,462,461,923,0.11496615409851074,0.002973903572404851
462,463,462,925,0.11509203910827637,0.00296312079918788
463,464,463,927,0.11525201797485352,0.002948661983885584
464,465,464,929,0.11541986465454102,0.0029293069441653306
465,466,465,931,0.11561083793640137,0.0029034571101197388
466,467,466,933,0.11575102806091309,0.0028690396929579335
467,468,467,935,0.11589574813842773,0.0028234054351714555
468,469,468,937,0.11603903770446777,0.002763236620510449
469,470,469,939,0.11617588996887207,0.0026844992054962068
470,471,470,941,0.1163017749786377,0.002582500334238168
471,472,471,943,0.1164398193359375,0.0024521512259875243
472,473,472,945,0.1165778636932373,0.0022885795608290154
473,474,473,947,0.11670684814453125,0.002088260322903461
474,475,474,949,0.1168220043182373,0.0018507771451557458
475,476,475,951,0.11695384979248047,0.0015810707771260633
476,477,476,953,0.1170969009399414,0.0012914424256939671
477,478,477,955,0.11722087860107422,0.0012005200329122038
478,479,478,957,0.11738204956054688,0.001258156964737714
479,480,479,959,0.11759185791015625,0.0011966516394558166
480,481,480,961,0.11778998374938965,0.0009981900187846858
481,482,481,963,0.11824584007263184,0.0008024446155144538
482,483,482,965,0.11840295791625977,0.0009752394641062047
483,484,483,967,0.11864709854125977,0.0010294865881905518
484,485,484,969,0.118804931640625,0.000936317461871704
485,486,485,971,0.11895084381103516,0.0008343803818475235
486,487,486,973,0.11926412582397461,0.00082971530163067
487,488,487,975,0.11957001686096191,0.000991840012350993
488,489,488,977,0.11978816986083984,0.0009912154757695901
489,490,489,979,0.11995983123779297,0.0009905262226936442
490,491,490,981,0.12009191513061523,0.000989598148559697
491,492,491,983,0.1204829216003418,0.000988349116820461
492,493,492,985,0.1215360164642334,0.0009866688631312223
493,494,493,987,0.12186813354492188,0.000984409839924737
494,495,494,989,0.12233495712280273,0.0009813750951310053
495,496,495,991,0.12246894836425781,0.000977302607535606
496,497,496,993,0.12261414527893066,0.0009718453762401469
497,498,497,995,0.12275099754333496,0.0009645467234961954
498,499,498,997,0.12290215492248535,0.000954810772917975
499,500,499,999,0.12313985824584961,0.0009418692515501208
500,501,500,1001,0.12341690063476562,0.0009247480896094653
501,502,501,1003,0.12366604804992676,0.0009022415782224391
502,503,502,1005,0.12391209602355957,0.0008729089983857786
503,504,503,1007,0.12452197074890137,0.0008351195589911302
504,505,504,1009,0.12479591369628906,0.0007871857288478566
505,506,505,1011,0.12520289421081543,0.0007276384148419363
506,507,506,1013,0.12554597854614258,0.0006556965536956321
507,508,507,1015,0.1258080005645752,0.0005719399046091268
508,509,508,1017,0.12605500221252441,0.00047906262924275327
509,510,509,1019,0.12621498107910156,0.0003823383261407503
510,511,510,1021,0.12634706497192383,0.00041556358051771835
511,512,511,1023,0.1264820098876953,0.0004169568902919952
512,513,512,1025,0.12663602828979492,0.00032995576403393887
513,514,513,1027,0.12679696083068848,0.00026959124522608213
514,515,514,1029,0.12722301483154297,0.00030959551862262116
515,516,515,1031,0.12747907638549805,0.00032720868477436265
516,517,516,1033,0.12766075134277344,0.00027663499729495955
517,518,517,1035,0.1278519630432129,0.00023632644302929416
518,519,518,1037,0.1280210018157959,0.0002871406614598096
519,520,519,1039,0.12816905975341797,0.0002811566762363627
520,521,520,1041,0.12832379341125488,0.0003046054221826435
521,522,521,1043,0.12853789329528809,0.0003001219973994963
522,523,522,1045,0.1288127899169922,0.00029480289516907134
523,524,523,1047,0.12897014617919922,0.0002877949446927499
524,525,524,1049,0.1292281150817871,0.0002786544810136465
525,526,525,1051,0.1307690143585205,0.00026686683042748095
526,527,526,1053,0.1317288875579834,0.00025189384711078695
527,528,527,1055,0.13201212882995605,0.00023325780523991986
528,529,528,1057,0.13222694396972656,0.00021068471707688167
529,530,529,1059,0.13316798210144043,0.0001843140682198331
530,531,530,1061,0.13340091705322266,0.00015493964377480792
531,532,531,1063,0.1335277557373047,0.0001241728762558038
532,533,532,1065,0.13367676734924316,0.0001294236591350424
533,534,533,1067,0.13391399383544922,0.00013188830848727214
534,535,534,1069,0.13421082496643066,0.0001078705274006648
535,536,535,1071,0.13439583778381348,8.71860011532785e-05
536,537,536,1073,0.13456106185913086,9.072923122134982e-05
537,538,537,1075,0.13469910621643066,7.329844959848635e-05
538,539,538,1077,0.13485383987426758,7.105034623301897e-05
539,540,539,1079,0.1350400447845459,0.00010348042431342327
540,541,540,1081,0.13527512550354004,0.00010247668319204456
541,542,541,1083,0.13556480407714844,0.000101535748941473
542,543,542,1085,0.1357588768005371,0.00010027899024394303
543,544,543,1087,0.1359550952911377,9.861378756462133e-05
544,545,544,1089,0.13613295555114746,9.642017635942056e-05
545,546,545,1091,0.13630390167236328,9.35530665034017e-05
546,547,546,1093,0.1366128921508789,8.98450138304448e-05
547,548,547,1095,0.13686585426330566,8.511686408534255e-05
548,549,548,1097,0.13701105117797852,7.920153336141747e-05
549,550,549,1099,0.13721203804016113,7.198683035416737e-05
550,551,550,1101,0.137376070022583,6.348051791586758e-05
551,552,551,1103,0.13753700256347656,5.389037033844798e-05
552,553,552,1105,0.1377098560333252,4.368940923620456e-05
553,554,553,1107,0.13786602020263672,4.129569447186343e-05
554,555,554,1109,0.13800787925720215,4.2728178823504556e-05
555,556,555,1111,0.13817501068115234,4.042699156976906e-05
556,557,556,1113,0.13834095001220703,3.29368437143913e-05
557,558,557,1115,0.13849878311157227,2.6299549837492763e-05
558,559,558,1117,0.13869094848632812,3.3353446700785706e-05
559,560,559,1119,0.13902902603149414,3.4244309568797964e-05
560,561,560,1121,0.13963985443115234,3.805335608129186e-05
561,562,561,1123,0.14063191413879395,3.721914669492418e-05
562,563,562,1125,0.1408400535583496,3.627245266597335e-05
563,564,563,1127,0.1412067413330078,3.5036313777584835e-05
564,565,564,1129,0.14150190353393555,3.344732722032278e-05
565,566,565,1131,0.1418769359588623,3.143794556600345e-05
566,567,566,1133,0.14215302467346191,2.8951606639151776e-05
567,568,567,1135,0.14231085777282715,2.5963709857897576e-05
568,569,568,1137,0.14261579513549805,2.2509305908073128e-05
569,570,569,1139,0.1428391933441162,1.87137962919938e-05
570,571,570,1141,0.14298605918884277,1.4806416105023654e-05
571,572,571,1143,0.1431901454925537,1.6363670817535298e-05
572,573,572,1145,0.14336705207824707,1.557734809205703e-05
573,574,573,1147,0.14356589317321777,1.2074101735323335e-05
574,575,574,1149,0.143812894821167,1.2900799864178555e-05
575,576,575,1151,0.14405298233032227,1.6568937007998404e-05
576,577,576,1153,0.14419007301330566,1.582709966371723e-05
577,578,577,1155,0.14434599876403809,1.5136227918251953e-05
578,579,578,1157,0.14449286460876465,1.4242372160316145e-05
579,580,579,1159,0.1446831226348877,1.3137353127513472e-05
580,581,580,1161,0.14485883712768555,1.180478718064724e-05
581,582,581,1163,0.1450350284576416,1.0261205667636852e-05
582,583,582,1165,0.1453239917755127,8.55536766520754e-06
583,584,583,1167,0.14572978019714355,6.799198994519411e-06
584,585,584,1169,0.14586997032165527,8.727218363257263e-06
585,586,585,1171,0.14601898193359375,8.983972744395711e-06
586,587,586,1173,0.14627313613891602,9.85753993508241e-06
587,588,587,1175,0.14642000198364258,9.674728657730781e-06
588,589,588,1177,0.1465599536895752,9.462655100954662e-06
589,590,589,1179,0.1466808319091797,9.184645474541015e-06
590,591,590,1181,0.1468219757080078,8.824861977735817e-06
591,592,591,1183,0.14698195457458496,8.36575872716566e-06
592,593,592,1185,0.14711785316467285,7.79078925939884e-06
593,594,593,1187,0.14752912521362305,7.0886147253272005e-06
594,595,594,1189,0.14779186248779297,6.259342106892222e-06
595,596,595,1191,0.14801692962646484,5.322428106872912e-06
596,597,596,1193,0.14815282821655273,4.323153158979861e-06
597,598,597,1195,0.14846086502075195,3.925549814518708e-06
598,599,598,1197,0.14878296852111816,4.17390228920901e-06
599,600,599,1199,0.14896106719970703,3.958603014378573e-06
600,601,600,1201,0.14909601211547852,3.3658050275692063e-06
601,602,601,1203,0.1492319107055664,2.6764191149119246e-06
602,603,602,1205,0.14936399459838867,3.2041886826868785e-06
603,604,603,1207,0.14950990676879883,3.5258200678099158e-06
604,605,604,1209,0.14967775344848633,3.173202477305132e-06
605,606,605,1211,0.14980411529541016,2.8528725962364416e-06
606,607,606,1213,0.15001392364501953,2.7422471801055516e-06
607,608,607,1215,0.1501908302307129,3.2313842859497985e-06
608,609,608,1217,0.15032410621643066,3.14446859271509e-06
609,610,609,1219,0.15044593811035156,3.053376179171684e-06
610,611,610,1221,0.15057682991027832,2.934367493264713e-06
611,612,611,1223,0.15082812309265137,2.7825635597345354e-06
612,613,612,1225,0.15120792388916016,2.5923145576574554e-06
613,614,613,1227,0.1514897346496582,2.3598550372601762e-06
614,615,614,1229,0.1517629623413086,2.0850731112294224e-06
615,616,615,1231,0.15192890167236328,1.7743573426002236e-06
616,617,616,1233,0.15211987495422363,1.442451504230832e-06
617,618,617,1235,0.15230798721313477,1.2634160125774093e-06
618,619,618,1237,0.15254592895507812,1.4791781399802375e-06
619,620,619,1239,0.15271306037902832,1.444043687203794e-06
620,621,620,1241,0.15285491943359375,1.6785716267665588e-06
621,622,621,1243,0.15303611755371094,1.6107031432957775e-06
622,623,622,1245,0.15314793586730957,1.5404354173955313e-06
623,624,623,1247,0.1532609462738037,1.4504114104220994e-06
624,625,624,1249,0.15337896347045898,1.338761647608497e-06
625,626,625,1251,0.15348482131958008,1.2041742637638083e-06
626,627,626,1253,0.1536860466003418,1.04780755161703e-06
627,628,627,1255,0.15386509895324707,8.751315733401114e-07
628,629,628,1257,0.15404295921325684,6.957450133353293e-07
629,630,629,1259,0.1541907787322998,6.455517865926803e-07
630,631,630,1261,0.15433406829833984,9.733680388533302e-07
631,632,631,1263,0.15448498725891113,9.27822875991075e-07
632,633,632,1265,0.15468287467956543,8.896409529192661e-07
633,634,633,1267,0.1548309326171875,8.399958991408978e-07
634,635,634,1269,0.15507197380065918,7.781960290358588e-07
635,636,635,1271,0.15529203414916992,7.033289640052263e-07
636,637,636,1273,0.15554094314575195,6.157051460064349e-07
637,638,637,1275,0.1557159423828125,5.180962905278567e-07
638,639,638,1277,0.1558690071105957,4.1540044415629854e-07
639,640,639,1279,0.15602684020996094,3.2808037924456743e-07
640,641,640,1281,0.15618109703063965,5.372344206121017e-07
641,642,641,1283,0.15630197525024414,4.790173925290075e-07
642,643,642,1285,0.15642881393432617,4.3927255125929794e-07
643,644,643,1287,0.15671515464782715,3.890152565995853e-07
644,645,644,1289,0.15701580047607422,4.086740437147313e-07
645,646,645,1291,0.1571640968322754,4.5894902563734044e-07
646,647,646,1293,0.1574258804321289,4.496969674851456e-07
647,648,647,1295,0.1576390266418457,4.39367046801127e-07
648,649,648,1297,0.15777802467346191,4.2580729667718877e-07
649,650,649,1299,0.15792012214660645,4.0830327408119805e-07
650,651,650,1301,0.1581110954284668,3.860260960060049e-07
651,652,651,1303,0.1582798957824707,3.5823257276292523e-07
652,653,652,1305,0.1584310531616211,3.244569566218033e-07
653,654,653,1307,0.15870904922485352,2.8483245238894333e-07
654,655,654,1309,0.15895414352416992,2.4045030643586215e-07
655,656,655,1311,0.15911507606506348,1.936467563690439e-07
656,657,656,1313,0.15926575660705566,1.836298701387651e-07
657,658,657,1315,0.15941405296325684,1.7810678671087662e-07
658,659,658,1317,0.15955901145935059,2.065531276053515e-07
659,660,659,1319,0.15978693962097168,1.7052684072467039e-07
660,661,660,1321,0.1600170135498047,1.4587275827296616e-07
661,662,661,1323,0.1602308750152588,1.156219899244643e-07
662,663,662,1325,0.16037988662719727,1.6384115706480607e-07
663,664,663,1327,0.16051101684570312,1.5414805324655072e-07
664,665,664,1329,0.16066598892211914,1.587383136188264e-07
665,666,665,1331,0.1608278751373291,1.5760678625243878e-07
666,667,666,1333,0.16095495223999023,1.5817756151800056e-07
667,668,667,1335,0.16111397743225098,1.5289671037279424e-07
668,669,668,1337,0.16130995750427246,1.4635406110626415e-07
669,670,669,1339,0.1615278720855713,1.380360353712995e-07
670,671,670,1341,0.16167306900024414,1.2769217013664072e-07
671,672,671,1343,0.16181087493896484,1.1518059257981035e-07
672,673,672,1345,0.1619420051574707,1.0058820099912389e-07
673,674,673,1347,0.1622300148010254,8.43757575462795e-08
674,675,674,1349,0.16237807273864746,6.743950143586681e-08
675,676,675,1351,0.1625349521636963,6.445704877605943e-08
676,677,676,1353,0.1626598834991455,8.667910629137427e-08
677,678,677,1355,0.16285490989685059,7.565575244041326e-08
678,679,678,1357,0.1630868911743164,6.776502457035718e-08
679,680,679,1359,0.16381502151489258,5.786273806846621e-08
680,681,680,1361,0.16492486000061035,5.298820145662533e-08
681,682,681,1363,0.1651301383972168,6.549837770462968e-08
682,683,682,1365,0.16529583930969238,5.9075367355829924e-08
683,684,683,1367,0.1655287742614746,5.38383504996078e-08
684,685,684,1369,0.16569781303405762,5.176148012542374e-08
685,686,685,1371,0.16583895683288574,5.9214036712708214e-08
686,687,686,1373,0.16612005233764648,5.730232121641318e-08
687,688,687,1375,0.1664741039276123,5.5268414674592546e-08
688,689,688,1377,0.16694879531860352,5.263262739424685e-08
689,690,689,1379,0.16710495948791504,4.931436020556364e-08
690,691,690,1381,0.1672511100769043,4.522423242556543e-08
691,692,691,1383,0.16748404502868652,4.0339066463981715e-08
692,693,692,1385,0.16767382621765137,3.473288579565445e-08
693,694,693,1387,0.16780805587768555,2.8640315161612707e-08
694,695,694,1389,0.16798710823059082,2.3140610397070877e-08
695,696,695,1391,0.16814494132995605,2.1612744973770494e-08
696,697,696,1393,0.16827392578125,3.325764520049203e-08
697,698,697,1395,0.16842198371887207,3.236832717466414e-08
698,699,698,1397,0.16861391067504883,3.1594055666870164e-08
699,700,699,1399,0.16882801055908203,3.0572589264540734e-08
700,701,700,1401,0.16903305053710938,2.9256224804849478e-08
701,702,701,1403,0.16917681694030762,2.7585951151947223e-08
702,703,702,1405,0.16936087608337402,2.550986819904457e-08
703,704,703,1407,0.16960692405700684,2.300011754247135e-08
704,705,704,1409,0.1698770523071289,2.0074656169758468e-08
705,706,705,1411,0.17002606391906738,1.682702494396246e-08
706,707,706,1413,0.1701669692993164,1.3438747951297046e-08
707,708,707,1415,0.17030096054077148,1.312305225806213e-08
708,709,708,1417,0.17044401168823242,1.5715007998173292e-08
709,710,709,1419,0.1705780029296875,1.2524741801304135e-08
710,711,710,1421,0.17072701454162598,1.0640553318087468e-08
711,712,711,1423,0.17087101936340332,8.18213798994825e-09
712,713,712,1425,0.17102384567260742,1.25511686798817e-08
713,714,713,1427,0.17122483253479004,1.1557778105689238e-08
714,715,714,1429,0.17136788368225098,1.103344446769077e-08
715,716,715,1431,0.17149710655212402,1.0884120066273268e-08
716,717,716,1433,0.17163705825805664,1.2015484026586467e-08
717,718,717,1435,0.17199087142944336,1.1887527498351184e-08
718,719,718,1437,0.17342901229858398,1.1737141353263696e-08
719,720,719,1439,0.17367887496948242,1.1538295314361068e-08
720,721,720,1441,0.17388391494750977,1.1275875118379231e-08
721,722,721,1443,0.17403292655944824,1.0933681120633532e-08
722,723,722,1445,0.1742081642150879,1.0491179205010649e-08
723,724,723,1447,0.17446589469909668,9.927531444514891e-09
724,725,724,1449,0.17479205131530762,9.223442932930333e-09
725,726,725,1451,0.1750028133392334,8.366369698367098e-09
726,727,726,1453,0.1751859188079834,7.358537549567513e-09
727,728,727,1455,0.17536187171936035,6.22662915428347e-09
728,729,728,1457,0.17550396919250488,5.028430126529233e-09
729,730,729,1459,0.17583489418029785,4.507598536168781e-09
730,731,730,1461,0.17602896690368652,4.7453449666157106e-09
731,732,731,1463,0.17622780799865723,4.067042104891707e-09
732,733,732,1465,0.17650318145751953,3.253093265665017e-09
733,734,733,1467,0.17671775817871094,4.114124465574654e-09
734,735,734,1469,0.1768798828125,4.256327519955027e-09
735,736,735,1471,0.17706704139709473,4.684631754573519e-09
736,737,736,1473,0.17721891403198242,4.579155051405645e-09
737,738,737,1475,0.17736411094665527,4.458574313807946e-09
738,739,738,1477,0.17749881744384766,4.301241546644073e-09
739,740,739,1479,0.17764592170715332,4.099667822718583e-09
740,741,740,1481,0.1778559684753418,3.8447966504252275e-09
741,742,741,1483,0.17800307273864746,3.530759061051434e-09
742,743,742,1485,0.17818093299865723,3.1546921189815532e-09
743,744,743,1487,0.17861294746398926,2.722215299387753e-09
744,745,744,1489,0.1787729263305664,2.250279169041266e-09
745,746,745,1491,0.17892098426818848,1.7685541252749223e-09
746,747,746,1493,0.1790931224822998,1.919832622534006e-09
747,748,747,1495,0.17927002906799316,1.769178714748502e-09
748,749,748,1497,0.179426908493042,1.3258814423051768e-09
749,750,749,1499,0.17956781387329102,1.7082243634066616e-09
750,751,750,1501,0.179732084274292,1.839970450554488e-09
751,752,751,1503,0.1799459457397461,1.8113510478932405e-09
752,753,752,1505,0.18019580841064453,1.924482873754195e-09
753,754,753,1507,0.18154597282409668,1.8876331318272975e-09
754,755,754,1509,0.18199992179870605,1.844237321645057e-09
755,756,755,1511,0.18214797973632812,1.7872049860726878e-09
756,757,756,1513,0.18232297897338867,1.713602398276652e-09
757,758,757,1515,0.18247199058532715,1.620170988501321e-09
758,759,758,1517,0.18262004852294922,1.5033261334328239e-09
759,760,759,1519,0.18275213241577148,1.3615021753688169e-09
760,761,760,1521,0.18290376663208008,1.195136039686332e-09
761,762,761,1523,0.18319177627563477,1.0087060452378568e-09
762,763,762,1525,0.18345999717712402,8.118445428176673e-10
763,764,763,1527,0.18359613418579102,7.434451202046483e-10
764,765,764,1529,0.18375396728515625,7.550875188815826e-10
765,766,765,1531,0.18391990661621094,6.814509636722767e-10
766,767,766,1533,0.18411707878112793,5.13818759064102e-10
767,768,767,1535,0.18426084518432617,7.022188787285602e-10
768,769,768,1537,0.18444299697875977,7.169792396109498e-10
769,770,769,1539,0.18456697463989258,7.918232727521341e-10
770,771,770,1541,0.18470096588134766,7.877596239072175e-10
771,772,771,1543,0.18481898307800293,7.830857872078105e-10
772,773,772,1545,0.18497586250305176,7.768041999989225e-10
773,774,773,1547,0.18508505821228027,7.688707070841052e-10
774,775,774,1549,0.1852130889892578,7.577809064616734e-10
775,776,775,1551,0.1853489875793457,7.43103107492323e-10
776,777,776,1553,0.18549489974975586,7.244520802403217e-10
777,778,777,1555,0.18579316139221191,6.996230502084038e-10
778,779,778,1557,0.18594598770141602,6.679030883966877e-10
779,780,779,1559,0.18615412712097168,6.27817061447573e-10
780,781,780,1561,0.18633604049682617,5.781603032693598e-10
781,782,781,1563,0.1868429183959961,5.18156873267592e-10
782,783,782,1565,0.18698596954345703,4.4904617376106024e-10
783,784,783,1567,0.18712496757507324,3.734164128521621e-10
784,785,784,1569,0.18728303909301758,2.9523997555338796e-10
785,786,785,1571,0.18742895126342773,3.092551179127568e-10
786,787,786,1573,0.1875600814819336,3.357862847333176e-10
787,788,787,1575,0.1877131462097168,2.6136149498077654e-10
788,789,788,1577,0.18793892860412598,2.1718001913278755e-10
789,790,789,1579,0.18865013122558594,2.8738689902785875e-10
790,791,790,1581,0.18940496444702148,2.776475218444594e-10
791,792,791,1583,0.18958401679992676,3.0841189727513084e-10
792,793,792,1585,0.1897568702697754,3.0212846689533487e-10
793,794,793,1587,0.18997693061828613,2.9537053160426424e-10
794,795,794,1589,0.190216064453125,2.8617082110354423e-10
795,796,795,1591,0.19038605690002441,2.7440999983140667e-10
796,797,796,1593,0.19058489799499512,2.5949561424335095e-10
797,798,797,1595,0.19076108932495117,2.408463508906231e-10
798,799,798,1597,0.19091105461120605,2.182383075653145e-10
799,800,799,1599,0.19106101989746094,1.9156359618803722e-10
800,801,800,1601,0.19120287895202637,1.6186552285535254e-10
801,802,801,1603,0.1914520263671875,1.302853533651303e-10
802,803,802,1605,0.19161081314086914,1.221625941182863e-10
803,804,803,1607,0.19189095497131348,1.0024650271294336e-10
804,805,804,1609,0.19203686714172363,1.4697070366712391e-10
805,806,805,1611,0.19234108924865723,1.2762084884901287e-10
806,807,806,1613,0.19251680374145508,1.1460837964211863e-10
807,808,807,1615,0.1926579475402832,1.0169017687819955e-10
808,809,808,1617,0.19300198554992676,1.2820954600271274e-10
809,810,809,1619,0.19329214096069336,1.237646494196996e-10
810,811,810,1621,0.19344687461853027,1.1899734297065564e-10
811,812,811,1623,0.1936049461364746,1.1294972281488796e-10
812,813,812,1625,0.19382572174072266,1.0525664521643934e-10
813,814,813,1627,0.19442486763000488,9.618530403259426e-11


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n100/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00016617774963378906,1624.447741208611
1,3,2,5,0.00046324729919433594,1272.8713625173957
2,5,4,9,0.0006520748138427734,961.6137427304949
3,7,6,13,0.0009510517120361328,698.4469064029521
4,9,8,17,0.0011839866638183594,497.92827037651625
5,11,10,21,0.0014050006866455078,385.1543340115312
6,13,12,25,0.0016498565673828125,334.70183338220033
7,15,14,29,0.0019240379333496094,316.76841860359195
8,17,16,33,0.0022020339965820312,327.92081477771296
9,19,18,37,0.003567218780517578,272.49749970969134
10,21,20,41,0.003902912139892578,580.6881017547407
11,23,22,45,0.004102230072021484,220.37726852264976
12,25,24,49,0.00448298454284668,224.8553449936177
13,27,26,53,0.004815101623535156,266.8895204854363
14,29,28,57,0.0050280094146728516,193.4461392124149
15,31,30,61,0.005266904830932617,834.3068414059894
16,33,32,65,0.0055811405181884766,239.0170517910166
17,35,34,69,0.005856990814208984,3407.7137433560315
18,37,36,73,0.00609898567199707,1248.784258972877
19,39,38,77,0.006293058395385742,139.41341914046623
20,41,40,81,0.0064928531646728516,21594.00614835975
21,43,42,85,0.006669044494628906,194.57039389801992
22,45,44,89,0.00693511962890625,350.2600749481253
23,47,46,93,0.007136106491088867,33.07326526419472
24,49,48,97,0.007324934005737305,2234.706125432987
25,51,50,101,0.007554054260253906,33.941357938318475
26,53,52,105,0.007800102233886719,14592.08385644159
27,55,54,109,0.008140087127685547,8.535298976600176
28,57,56,113,0.008419036865234375,1.9797757421528643
29,59,58,117,0.008686065673828125,708.1251614479401
30,61,60,121,0.008901119232177734,3.0406105836254578
31,63,62,125,0.009112119674682617,0.05033558955791663
32,65,64,129,0.009371280670166016,0.013555356108673694
33,67,66,133,0.009653091430664062,0.0016659262350161277
34,69,68,137,0.010061025619506836,0.0007543427002068241
35,71,70,141,0.010424137115478516,0.05669953626123291
36,73,72,145,0.010940074920654297,0.005812801321401162
37,75,74,149,0.011173248291015625,0.00027999462185209867
38,77,76,153,0.011576175689697266,5.531443138224024e-05
39,79,78,157,0.011789083480834961,1.8223553300803196e-05
40,81,80,161,0.011990070343017578,1.458594488182131e-05
41,83,82,165,0.012211084365844727,6.378948061889272e-05
42,85,84,169,0.016657114028930664,4.858754591547119e-07
43,87,86,173,0.017135143280029297,2.866684788390133e-07
44,89,88,177,0.01743793487548828,1.9825944825746362e-07
45,91,90,181,0.01818108558654785,6.766214604747112e-07
46,93,92,185,0.018453121185302734,1.972787088051743e-05
47,95,94,189,0.018705129623413086,1.0200175100283561e-07
48,97,96,193,0.018964052200317383,6.692561059923934e-08
49,99,98,197,0.019346952438354492,3.9603857126417814e-08
50,101,100,201,0.020010948181152344,5.604264415329674e-07
51,103,102,205,0.020631074905395508,2.7120724455841196e-08
52,105,104,209,0.021033048629760742,1.6431127223134333e-08
53,107,106,213,0.021338224411010742,1.8854614096691566e-08
54,109,108,217,0.02155590057373047,4.591250674012719e-06
55,111,110,221,0.021790027618408203,1.4128208926879017e-08
56,113,112,225,0.02392125129699707,5.224481012986719e-10
57,115,114,229,0.02492213249206543,8.689190939431684e-09
58,117,116,233,0.026108264923095703,7.738129801392896e-09
59,119,118,237,0.02697920799255371,3.588271974240823e-10
60,121,120,241,0.02750706672668457,3.7388744250579685e-10
61,123,122,245,0.027802228927612305,1.7566317819302195e-08
62,125,124,249,0.028042078018188477,5.05560233900088e-11


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n100/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.000225067138671875,1624.447741208611
2,5,4,9,0.003520965576171875,1074.9762595826073
4,9,8,17,0.004966020584106445,681.7815756458663
6,13,12,25,0.006433010101318359,463.5938329857111
8,17,16,33,0.007317066192626953,363.2997632560372
10,21,20,41,0.007950067520141602,310.1010433484549
12,25,24,49,0.009347915649414062,283.49492238268476
14,29,28,57,0.010691165924072266,265.63648716184593
16,33,32,65,0.011513233184814453,241.06426178394614
18,37,36,73,0.012611865997314453,234.03537577243546
20,41,40,81,0.013212919235229492,222.06145980842268
22,45,44,89,0.014168024063110352,209.41498544964557
24,49,48,97,0.017071008682250977,200.74033555129807
26,53,52,105,0.017852067947387695,188.64132703666422
28,57,56,113,0.018288850784301758,182.51331059309462
30,61,60,121,0.01868605613708496,168.09934603253112
32,65,64,129,0.01901698112487793,159.15802793415068
34,69,68,137,0.019357919692993164,155.30835317425192
36,73,72,145,0.020015954971313477,141.46198810810452
38,77,76,153,0.02047586441040039,137.66123385619966
40,81,80,161,0.02094292640686035,129.27776825774362
42,85,84,169,0.021355152130126953,124.0900664223253
44,89,88,177,0.022518157958984375,121.41934420331066
46,93,92,185,0.022849082946777344,119.39983820708568
48,97,96,193,0.02316904067993164,117.84080097273029
50,101,100,201,0.023467063903808594,110.73658910025752
52,105,104,209,0.02392411231994629,109.22864914657332
54,109,108,217,0.02424907684326172,108.0180346297841
56,113,112,225,0.024569034576416016,107.0175767838781
58,117,116,233,0.024879932403564453,106.1635655391015
60,121,120,241,0.025189876556396484,105.40999711959633
62,125,124,249,0.025495052337646484,104.72403047594116
64,129,128,257,0.02604389190673828,98.1301559079027
66,133,132,265,0.026340007781982422,97.31347085260819
68,137,136,273,0.026670217514038086,96.59119460505664
70,141,140,281,0.026973962783813477,92.55492770562087
72,145,144,289,0.027347087860107422,91.81415086375299
74,149,148,297,0.02764606475830078,91.15157004344363
76,153,152,305,0.028046846389770508,90.54478419572912
78,157,156,313,0.02846384048461914,89.97722019224601
80,161,160,321,0.028859853744506836,89.43673019546448
82,165,164,329,0.029223918914794922,88.9145019880561
84,169,168,337,0.029534101486206055,88.404220719104
86,173,172,345,0.03036022186279297,87.90142906828191
88,177,176,353,0.031110048294067383,87.40304197617908
90,181,180,361,0.031816959381103516,86.90698061718919
92,185,184,369,0.03248119354248047,86.41189768592928
94,189,188,377,0.03296303749084473,85.91697220576324
96,193,192,385,0.033358097076416016,85.42175701960993
98,197,196,393,0.033946990966796875,80.56034730897348
100,201,200,401,0.03435015678405762,77.06956513918219
102,205,204,409,0.034783124923706055,76.10163691707787
104,209,208,417,0.03700113296508789,71.18794986306793
106,213,212,425,0.037420034408569336,70.26576633337868
108,217,216,433,0.03819394111633301,69.59564888314954
110,221,220,441,0.03857111930847168,68.99149991945642
112,225,224,449,0.03893780708312988,68.44001081917901
114,229,228,457,0.03939104080200195,67.93040857110837
116,233,232,465,0.039888858795166016,67.4540121696671
118,237,236,473,0.04052090644836426,67.00385642644123
120,241,240,481,0.041259050369262695,66.57437630119239
122,245,244,489,0.04166007041931152,66.16114427000407
124,249,248,497,0.04217982292175293,65.76065333636919
126,253,252,505,0.04264187812805176,65.37013877664205
128,257,256,513,0.043107032775878906,64.98743240048361
130,261,260,521,0.04350590705871582,64.61084387208813
132,265,264,529,0.04388618469238281,64.2390643994702
134,269,268,537,0.04433584213256836,63.87108881159765
136,273,272,545,0.04477500915527344,63.506152684169386
138,277,276,553,0.04539012908935547,63.14368173617925
140,281,280,561,0.04583406448364258,43.05362782494803
142,285,284,569,0.04729509353637695,42.49177885828477
144,289,288,577,0.047883033752441406,41.97646035793068
146,293,292,585,0.0482790470123291,41.50087891390307
148,297,296,593,0.04870796203613281,41.05926500301267
150,301,300,601,0.04907083511352539,40.6467261325363
152,305,304,609,0.04962897300720215,40.25911810719962
154,309,308,617,0.05180001258850098,39.89293312135577
156,313,312,625,0.05258607864379883,39.54520315479662
158,317,316,633,0.05324292182922363,39.21341706390604
160,321,320,641,0.05377316474914551,38.8954497699031
162,325,324,649,0.05441117286682129,38.58950202001386
164,329,328,657,0.054901123046875,38.29404931010172
166,333,332,665,0.05537700653076172,38.00779868995192
168,337,336,673,0.05611395835876465,37.72965231183932
170,341,340,681,0.05653882026672363,37.458676720469455
172,345,344,689,0.057102203369140625,37.19407701239037
174,349,348,697,0.05766701698303223,36.93517511239121
176,353,352,705,0.05820918083190918,36.68139152184006
178,357,356,713,0.058873891830444336,36.432229989057426
180,361,360,721,0.059674978256225586,36.187264634941215
182,365,364,729,0.06016206741333008,30.02031504499176
184,369,368,737,0.06063389778137207,29.631314775608438
186,373,372,745,0.06339001655578613,29.273270353781925
188,377,376,753,0.06522202491760254,28.94200475222541
190,381,380,761,0.06553983688354492,28.633918140413318
192,385,384,769,0.06590795516967773,28.345912995016274
194,389,388,777,0.0663299560546875,28.07532725105172
196,393,392,785,0.06668710708618164,27.819875120361758
198,397,396,793,0.06727099418640137,27.57759506446527
200,401,400,801,0.06848001480102539,27.346804328604833
202,405,404,809,0.06883907318115234,25.56256956546132
204,409,408,817,0.06920003890991211,25.356983395907815
206,413,412,825,0.06952881813049316,25.20844320928263
208,417,416,833,0.06997203826904297,25.060801692928614
210,421,420,841,0.07030606269836426,24.914053652086505
212,425,424,849,0.07066082954406738,24.768193883119785
214,429,428,857,0.07106804847717285,24.62321717699849
216,433,432,865,0.07147598266601562,24.479118322480815
218,437,436,873,0.0719609260559082,24.335892109042256
220,441,440,881,0.07249116897583008,24.193533329555816
222,445,444,889,0.07291603088378906,24.052036782746818
224,449,448,897,0.07326698303222656,23.911397275437746
226,453,452,905,0.07367205619812012,23.771609624603638
228,457,456,913,0.07405400276184082,23.632668659248747
230,461,460,921,0.07441902160644531,23.494569222110368
232,465,464,929,0.07480502128601074,23.357306171222906
234,469,468,937,0.07525897026062012,23.220874381335484
236,473,472,945,0.07590603828430176,23.08526874519954
238,477,476,953,0.07644200325012207,21.631613847525454
240,481,480,961,0.07710504531860352,21.50167467099822
242,485,484,969,0.07744002342224121,21.37422272208519
244,489,488,977,0.0777890682220459,21.248963913561923
246,493,492,985,0.07815814018249512,21.12564544312637
248,497,496,993,0.07854223251342773,21.004050305339188
250,501,500,1001,0.07892990112304688,20.88399249652149
252,505,504,1009,0.0792999267578125,20.765312830886362
254,509,508,1017,0.07967591285705566,20.647875294596968
256,513,512,1025,0.08009719848632812,20.53156387221639
258,517,516,1033,0.08110594749450684,20.416279787334407
260,521,520,1041,0.0823509693145752,20.301939105709835
262,525,524,1049,0.08302903175354004,20.18847065529818
264,529,528,1057,0.08342885971069336,20.075814222946814
266,533,532,1065,0.0840461254119873,19.96391899234228
268,537,536,1073,0.08452105522155762,19.8527421921584
270,541,540,1081,0.08485102653503418,19.742247927161223
272,545,544,1089,0.08526897430419922,19.632406168419053
274,549,548,1097,0.08579111099243164,19.523191881788904
276,553,552,1105,0.08617496490478516,19.414584276466492
278,557,556,1113,0.08731389045715332,19.306566157729467
280,561,560,1121,0.08790302276611328,19.199123370011726
282,565,564,1129,0.08860015869140625,19.092244318280216
284,569,568,1137,0.08949518203735352,18.985919557189884
286,573,572,1145,0.09032821655273438,18.880141438918187
288,577,576,1153,0.09125399589538574,18.774903811719277
290,581,580,1161,0.09430885314941406,17.588038190234478
292,585,584,1169,0.09699797630310059,17.47575474085659
294,589,588,1177,0.09757494926452637,17.3662687083676
296,593,592,1185,0.09865593910217285,17.25930109930783
298,597,596,1193,0.10191106796264648,17.15460434053991
300,601,600,1201,0.10544490814208984,17.05195888954582
302,605,604,1209,0.10633993148803711,16.95117018621938
304,609,608,1217,0.1091458797454834,16.852065916132258
306,613,612,1225,0.11037397384643555,16.75449355701555
308,617,616,1233,0.1114649772644043,16.658318182024995
310,621,620,1241,0.11260390281677246,16.563420495222818
312,625,624,1249,0.11407995223999023,16.469695076611735
314,629,628,1257,0.11520099639892578,16.377048815898192
316,633,632,1265,0.11572504043579102,16.285399515922496
318,637,636,1273,0.1163029670715332,16.194674648392375
320,641,640,1281,0.1185150146484375,16.104810246137145
322,645,644,1289,0.1192011833190918,16.01574991759451
324,649,648,1297,0.11988997459411621,15.92744397061115
326,653,652,1305,0.12042903900146484,15.839848633897864
328,657,656,1313,0.12081694602966309,15.75292536566621
330,661,660,1321,0.12127208709716797,15.66664024000397
332,665,664,1329,0.12166309356689453,15.580963402558352
334,669,668,1337,0.12207221984863281,15.495868587925122
336,673,672,1345,0.12257099151611328,15.411332691986484
338,677,676,1353,0.12292313575744629,15.327335393100128
340,681,680,1361,0.12363600730895996,14.609550428198386
342,685,684,1369,0.12484502792358398,14.357452875413028
344,689,688,1377,0.12540078163146973,14.26640945131788
346,693,692,1385,0.12572693824768066,14.177386692201623
348,697,696,1393,0.12617921829223633,14.09020974241247
350,701,700,1401,0.126694917678833,14.004721077280868
352,705,704,1409,0.1271061897277832,13.920778867515148
354,709,708,1417,0.12757205963134766,13.838255485926483
356,713,712,1425,0.1280231475830078,5.810373159582504
358,717,716,1433,0.12838006019592285,5.693732568137597
360,721,720,1441,0.12874603271484375,5.583637709398936
362,725,724,1449,0.12906908988952637,5.479680806454381
364,729,728,1457,0.12972283363342285,5.381474035126806
366,733,732,1465,0.13018202781677246,5.288649113834686
368,737,736,1473,0.13060522079467773,5.200856863994831
370,741,740,1481,0.13098907470703125,5.11776673905473
372,745,744,1489,0.13144207000732422,5.039066321765213
374,749,748,1497,0.13300299644470215,4.9644607906049085
376,753,752,1505,0.13350296020507812,4.893672357422983
378,757,756,1513,0.1339409351348877,4.826439679279338
380,761,760,1521,0.13429617881774902,4.762517248160752
382,765,764,1529,0.1348729133605957,4.701674762769176
384,769,768,1537,0.13550996780395508,4.643696486854773
386,773,772,1545,0.13622403144836426,4.588380598705006
388,777,776,1553,0.13724589347839355,4.5355385363599865
390,781,780,1561,0.1379399299621582,4.484994342985319
392,785,784,1569,0.13839006423950195,4.436584016546761
394,789,788,1577,0.13882184028625488,4.390154867620876
396,793,792,1585,0.13926982879638672,4.345564888770336
398,797,796,1593,0.1413719654083252,4.302682138510012
400,801,800,1601,0.14204812049865723,4.261384142432892
402,805,804,1609,0.14263701438903809,4.221557313653099
404,809,808,1617,0.14322590827941895,4.183096394290559
406,813,812,1625,0.1437070369720459,4.145903919336139
408,817,816,1633,0.1442708969116211,4.109889703841717
410,821,820,1641,0.14476919174194336,4.074970354086526
412,825,824,1649,0.14556002616882324,4.041068803017976
414,829,828,1657,0.14605712890625,4.008113870045274
416,833,832,1665,0.14656400680541992,3.9760398450187053
418,837,836,1673,0.1469881534576416,3.944786096015071
420,841,840,1681,0.1474919319152832,3.914296700427439
422,845,844,1689,0.15047192573547363,3.8845200986917576
424,849,848,1697,0.15106201171875,3.855408769894528
426,853,852,1705,0.15198898315429688,3.826918928426905
428,857,856,1713,0.15272998809814453,3.7990102407845647
430,861,860,1721,0.1533060073852539,3.771645561588121
432,865,864,1729,0.15375113487243652,3.744790687857948
434,869,868,1737,0.15461111068725586,3.718414130584398
436,873,872,1745,0.15520596504211426,3.6924869026369658
438,877,876,1753,0.155897855758667,3.6669823220445776
440,881,880,1761,0.1563568115234375,3.6418758297451865
442,885,884,1769,0.158250093460083,3.617144820878758
444,889,888,1777,0.15868496894836426,3.5927684887617826
446,893,892,1785,0.1592390537261963,3.5687276807095496
448,897,896,1793,0.15981388092041016,3.5450047648984806
450,901,900,1801,0.16023802757263184,3.521583507508764
452,905,904,1809,0.1607990264892578,3.498448959430378
454,909,908,1817,0.16124200820922852,3.4755873518418574
456,913,912,1825,0.1616039276123047,3.4529860000209607
458,917,916,1833,0.16202092170715332,3.4306332147845793
460,921,920,1841,0.16236114501953125,3.4085182209834834
462,925,924,1849,0.16280293464660645,3.386631082528008
464,929,928,1857,0.16326498985290527,3.3649626334477682
466,933,932,1865,0.16362905502319336,3.3435044145136423
468,937,936,1873,0.16564202308654785,3.322248615001327
470,941,940,1881,0.16606998443603516,3.3011880191935914
472,945,944,1889,0.16650915145874023,3.280315957248566
474,949,948,1897,0.16696596145629883,3.2596262600836328
476,953,952,1905,0.16733002662658691,3.2391132179691486
478,957,956,1913,0.16773414611816406,3.218771542520649
480,961,960,1921,0.1681990623474121,3.1985963318289636
482,965,964,1929,0.1688530445098877,3.178583038468979
484,969,968,1937,0.16929411888122559,3.1587274401560896
486,973,972,1945,0.16958999633789062,3.1390256128309875
488,977,976,1953,0.17001104354858398,3.1194739059898047
490,981,980,1961,0.170928955078125,3.1000689200495843
492,985,984,1969,0.17136597633361816,3.080807485614032
494,989,988,1977,0.17186784744262695,3.0616866444551283
496,993,992,1985,0.17246007919311523,3.0427036320869765
498,997,996,1993,0.17282485961914062,3.023855861796521
501,1003,1002,2005,0.17332005500793457,2.9958325249577022
503,1007,1006,2013,0.1737380027770996,2.977312580827103
505,1011,1010,2021,0.17537212371826172,2.9589200246796143
507,1015,1014,2029,0.17584490776062012,2.940652905426399
509,1019,1018,2037,0.17623615264892578,2.9225093830032827
511,1023,1022,2045,0.17673206329345703,2.904487719328001
513,1027,1026,2053,0.1771390438079834,2.886586270013712
515,1031,1030,2061,0.17747783660888672,2.8688034767753545
517,1035,1034,2069,0.17783880233764648,2.54383724396991
519,1039,1038,2077,0.1782090663909912,2.2462688397207744
521,1043,1042,2085,0.17856907844543457,2.2244301293955133
523,1047,1046,2093,0.17898917198181152,2.2032664005568745
525,1051,1050,2101,0.17949390411376953,2.1827394327886718
527,1055,1054,2109,0.18024516105651855,2.1628132193131706
529,1059,1058,2117,0.18059301376342773,2.143453857558478
531,1063,1062,2125,0.18102407455444336,2.1246294428965906
533,1067,1066,2133,0.18282508850097656,2.1063099657194613
535,1071,1070,2141,0.18340682983398438,2.0884672119756655
537,1075,1074,2149,0.18398118019104004,2.07107466728716
539,1079,1078,2157,0.18441295623779297,2.054107424678921
541,1083,1082,2165,0.18480491638183594,2.037542095985451
543,1087,1086,2173,0.1853179931640625,2.021356726942106
545,1091,1090,2181,0.18572115898132324,2.005530715945752
547,1095,1094,2189,0.18644499778747559,1.9900447364546785
549,1099,1098,2197,0.18680906295776367,1.9748806629982953
551,1103,1102,2205,0.18727397918701172,1.9600215007004924
553,1107,1106,2213,0.18786311149597168,1.945451318281197
555,1111,1110,2221,0.18819522857666016,1.9311551844154973
557,1115,1114,2229,0.18851590156555176,1.91711910737687
559,1119,1118,2237,0.1888749599456787,1.903329977846354
561,1123,1122,2245,0.18938398361206055,1.8897755147991022
563,1127,1126,2253,0.1897890567779541,1.8764442143328828
565,1131,1130,2261,0.19082307815551758,1.8633253013399855
567,1135,1134,2269,0.19136595726013184,1.8504086839085918
569,1139,1138,2277,0.19173789024353027,1.8376849103109403
571,1143,1142,2285,0.192094087600708,1.8251451285062816
573,1147,1146,2293,0.19247698783874512,1.8127810479912534
575,1151,1150,2301,0.19282317161560059,1.8005849039269368
577,1155,1154,2309,0.19319510459899902,1.7885494234047583
579,1159,1158,2317,0.19353508949279785,1.7766677937563093
581,1163,1162,2325,0.1938610076904297,1.7649336327877898
583,1167,1166,2333,0.19417405128479004,1.7533409608563602
585,1171,1170,2341,0.1946859359741211,1.7418841746604061
587,1175,1174,2349,0.19506216049194336,1.73055802268021
589,1179,1178,2357,0.19541406631469727,1.7193575821515827
591,1183,1182,2365,0.19579386711120605,1.708278237501198
593,1187,1186,2373,0.1974179744720459,1.697315660145018
595,1191,1190,2381,0.19784998893737793,1.6864657895873274
597,1195,1194,2389,0.19838213920593262,1.67572481572394
599,1199,1198,2397,0.1988060474395752,1.665089162293896
601,1203,1202,2405,0.19912981986999512,1.654555471402307
603,1207,1206,2413,0.1996018886566162,1.644120589046107
605,1211,1210,2421,0.2000257968902588,1.633781551591254
607,1215,1214,2429,0.20039987564086914,1.6235355731298342
609,1219,1218,2437,0.20096111297607422,1.6133800336729485
611,1223,1222,2445,0.2016589641571045,1.6033124681188393
613,1227,1226,2453,0.20205283164978027,1.593330555952846
615,1231,1230,2461,0.2024080753326416,1.5834321116262295
617,1235,1234,2469,0.20295500755310059,1.573615075579938
619,1239,1238,2477,0.20334696769714355,1.5638775058630316
621,1243,1242,2485,0.20500397682189941,1.5542175703056431
623,1247,1246,2493,0.20614314079284668,1.5446335392247685
625,1251,1250,2501,0.20661616325378418,1.5351237786102467
627,1255,1254,2509,0.2071230411529541,1.5256867437720054
629,1259,1258,2517,0.2074439525604248,1.5163209734129157
631,1263,1262,2525,0.20783400535583496,1.5070250840987007
633,1267,1266,2533,0.2082200050354004,1.497797765103021
635,1271,1270,2541,0.2086038589477539,1.394753143914549
637,1275,1274,2549,0.20899319648742676,0.8261046481012412
639,1279,1278,2557,0.20940494537353516,0.811076510358488
641,1283,1282,2565,0.2097470760345459,0.7965868128058646
643,1287,1286,2573,0.2103288173675537,0.7826160111468873
645,1291,1290,2581,0.21070289611816406,0.769145092459996
647,1295,1294,2589,0.21111512184143066,0.7561555668413322
649,1299,1298,2597,0.21314477920532227,0.7436294594731283
651,1303,1302,2605,0.21365618705749512,0.7315493030501927
653,1307,1306,2613,0.21411585807800293,0.7198981304924273
655,1311,1310,2621,0.21456003189086914,0.7086594678848158
657,1315,1314,2629,0.21491694450378418,0.6978173275846542
659,1319,1318,2637,0.2154090404510498,0.6873562014328006
661,1323,1322,2645,0.215897798538208,0.6772610540244453
663,1327,1326,2653,0.2162470817565918,0.6675173159824528
665,1331,1330,2661,0.21663689613342285,0.6581108771967061
667,1335,1334,2669,0.21719813346862793,0.6490280799873468
669,1339,1338,2677,0.21766996383666992,0.640255712159642
671,1343,1342,2685,0.21838903427124023,0.6317809999224492
673,1347,1346,2693,0.21874094009399414,0.6235916006515233
675,1351,1350,2701,0.2190861701965332,0.6156755954740067
677,1355,1354,2709,0.21956896781921387,0.6080214816709898
679,1359,1358,2717,0.2202129364013672,0.600618164882785
681,1363,1362,2725,0.22163009643554688,0.5934549511217052
683,1367,1366,2733,0.2221660614013672,0.5865215385907163
685,1371,1370,2741,0.22257423400878906,0.5798080093155138
687,1375,1374,2749,0.22298192977905273,0.5733048205976252
689,1379,1378,2757,0.22335004806518555,0.5670027963054397
691,1383,1382,2765,0.22366905212402344,0.5608931180131841
693,1387,1386,2773,0.22406601905822754,0.5549673160087187
695,1391,1390,2781,0.22441601753234863,0.5492172601883055
697,1395,1394,2789,0.2247779369354248,0.5436351508594324
699,1399,1398,2797,0.22517800331115723,0.5382135094728443
701,1403,1402,2805,0.2256460189819336,0.532945169306036
703,1407,1406,2813,0.22601699829101562,0.5278232661190703
705,1411,1410,2821,0.22637391090393066,0.5228412288092734
707,1415,1414,2829,0.22689485549926758,0.5179927700819199
709,1419,1418,2837,0.2274320125579834,0.5132718771610238
711,1423,1422,2845,0.22780704498291016,0.5086728025598879
713,1427,1426,2853,0.228438138961792,0.5041900549313257
715,1431,1430,2861,0.2288651466369629,0.4998183900180182
717,1435,1434,2869,0.22919201850891113,0.49555280171556
719,1439,1438,2877,0.2295241355895996,0.49138851326877736
721,1443,1442,2885,0.22985291481018066,0.48732096861466
723,1447,1446,2893,0.23020124435424805,0.48334582388298336
725,1451,1450,2901,0.2304990291595459,0.47945893907032555
727,1455,1454,2909,0.2308349609375,0.4756563698954312
729,1459,1458,2917,0.23128604888916016,0.47193435984350507
731,1463,1462,2925,0.23172521591186523,0.46828933241174386
733,1467,1466,2933,0.23215007781982422,0.46471788355766813
735,1471,1470,2941,0.23322391510009766,0.46121677435935376
737,1475,1474,2949,0.2338418960571289,0.45778292388874303
739,1479,1478,2957,0.23582792282104492,0.4544134023010585
741,1483,1482,2965,0.23627090454101562,0.4511054241456127
743,1487,1486,2973,0.23666906356811523,0.4478563418939622
745,1491,1490,2981,0.23706293106079102,0.44466363968839523
747,1495,1494,2989,0.23747992515563965,0.4415249273106379
749,1499,1498,2997,0.2380070686340332,0.4384379343654403
751,1503,1502,3005,0.23839592933654785,0.43540050468129604
753,1507,1506,3013,0.23885393142700195,0.4324105909221864
755,1511,1510,3021,0.23932909965515137,0.42946624941056416
757,1515,1514,3029,0.23981809616088867,0.4265656351519966
759,1519,1518,3037,0.24057292938232422,0.423706997064041
761,1523,1522,3045,0.2410120964050293,0.42088867339995395
763,1527,1526,3053,0.24143385887145996,0.41810908736554214
765,1531,1530,3061,0.2421860694885254,0.4153667429209886
767,1535,1534,3069,0.24498510360717773,0.4126602207659163
769,1539,1538,3077,0.24567103385925293,0.4099881744994406
771,1543,1542,3085,0.2464299201965332,0.40734932695232345
773,1547,1546,3093,0.24733591079711914,0.4047424666835572
775,1551,1550,3101,0.2479538917541504,0.40216644463578316
777,1555,1554,3109,0.24845290184020996,0.399620170947167
779,1559,1558,3117,0.24941706657409668,0.39710261190953244
781,1563,1562,3125,0.24982190132141113,0.39461278707232467
783,1567,1566,3133,0.2501840591430664,0.39214976648003586
785,1571,1570,3141,0.250622034072876,0.3897126680470164
787,1575,1574,3149,0.2513909339904785,0.387300655055574
789,1579,1578,3157,0.25281786918640137,0.38491293377701913
791,1583,1582,3165,0.253216028213501,0.3825487512103434
793,1587,1586,3173,0.25365519523620605,0.38020739293082106
795,1591,1590,3181,0.25411105155944824,0.37788818104912153
797,1595,1594,3189,0.2545301914215088,0.3755904722669179
799,1599,1598,3197,0.25495290756225586,0.37331365603764066
801,1603,1602,3205,0.2552671432495117,0.3710571528144266
803,1607,1606,3213,0.2556149959564209,0.3688204123908952
805,1611,1610,3221,0.25609922409057617,0.36660291232434383
807,1615,1614,3229,0.25661301612854004,0.36440415644415847
809,1619,1618,3237,0.2569999694824219,0.36222367343101125
811,1623,1622,3245,0.2573409080505371,0.36006101547774194
813,1627,1626,3253,0.2588028907775879,0.3579157570125408
815,1631,1630,3261,0.25945186614990234,0.3557874934946165
817,1635,1634,3269,0.2599921226501465,0.3536758402698938
819,1639,1638,3277,0.2605729103088379,0.3515804314885204
821,1643,1642,3285,0.2610499858856201,0.34950091908011
823,1647,1646,3293,0.26163196563720703,0.34743697178113087
825,1651,1650,3301,0.26214599609375,0.3453882742173195
827,1655,1654,3309,0.26257801055908203,0.3433545260326307
829,1659,1658,3317,0.26303791999816895,0.3413354410674124
831,1663,1662,3325,0.26347804069519043,0.33933074657604406
833,1667,1666,3333,0.2638568878173828,0.3373401824933018
835,1671,1670,3341,0.26421093940734863,0.33536350073577964
837,1675,1674,3349,0.26456499099731445,0.3334004645421132
839,1679,1678,3357,0.2649059295654297,0.33145084784867457
841,1683,1682,3365,0.26542019844055176,0.32951443470219743
843,1687,1686,3373,0.2659170627593994,0.32759101870003426
845,1691,1690,3381,0.26625585556030273,0.3256804024644863
847,1695,1694,3389,0.266726016998291,0.32378239714383933
849,1699,1698,3397,0.26705479621887207,0.3218968219422105
851,1703,1702,3405,0.2673921585083008,0.3200235036745559
853,1707,1706,3413,0.26772212982177734,0.3181622763462518
855,1711,1710,3421,0.2680661678314209,0.316312980755314
857,1715,1714,3429,0.268420934677124,0.3144754641187991
859,1719,1718,3437,0.268751859664917,0.31264957971726204
861,1723,1722,3445,0.26912498474121094,0.3108351865599634
863,1727,1726,3453,0.26941394805908203,0.30903214906981935
865,1731,1730,3461,0.2697110176086426,0.30724033678353774
867,1735,1734,3469,0.2699930667877197,0.30545962407137006
869,1739,1738,3477,0.2704031467437744,0.30368988987017365
871,1743,1742,3485,0.2708089351654053,0.30193101743135875
873,1747,1746,3493,0.27118492126464844,0.30018289408568666
875,1751,1750,3501,0.27216482162475586,0.2984454110182448
877,1755,1754,3509,0.2724781036376953,0.2967184630575109
879,1759,1758,3517,0.2727780342102051,0.2950019484754627
881,1763,1762,3525,0.27309703826904297,0.2932957688011875
883,1767,1766,3533,0.2734510898590088,0.2915998286411093
885,1771,1770,3541,0.27376794815063477,0.2899140355133697
887,1775,1774,3549,0.2741100788116455,0.28823829968902215
889,1779,1778,3557,0.2744169235229492,0.2865725340426965
891,1783,1782,3565,0.27475595474243164,0.28491665391301724
893,1787,1786,3573,0.2751009464263916,0.283270576969813
895,1791,1790,3581,0.27538013458251953,0.2816342230873632
897,1795,1794,3589,0.27579283714294434,0.2800075142293881
899,1799,1798,3597,0.276080846786499,0.278390374336408
901,1803,1802,3605,0.2763631343841553,0.2767827292197999
903,1807,1806,3613,0.2766530513763428,0.2751845064648523
905,1811,1810,3621,0.27707600593566895,0.2735956353363521
907,1815,1814,3629,0.27750396728515625,0.27201604669185375
909,1819,1818,3637,0.2783019542694092,0.27044567289753263
911,1823,1822,3645,0.27879881858825684,0.2688844477521294
913,1827,1826,3653,0.2790868282318115,0.2673323064102096
915,1831,1830,3661,0.27942705154418945,0.2657891853165776
917,1835,1834,3669,0.2797820568084717,0.26425502213820357
919,1839,1838,3677,0.28011393547058105,0.2627297557042913
921,1843,1842,3685,0.28040289878845215,0.26121332594696356
923,1847,1846,3693,0.2808060646057129,0.25970567384872095
925,1851,1850,3701,0.28110218048095703,0.25820674138823535
927,1855,1854,3709,0.28145599365234375,0.2567164714947125
929,1859,1858,3717,0.28182291984558105,0.2552348079994717
931,1863,1862,3725,0.2821378707885742,0.25376169559588346
933,1867,1866,3733,0.28249406814575195,0.25229707979575916
935,1871,1870,3741,0.28286004066467285,0.2508409068942327
937,1875,1874,3749,0.2831850051879883,0.24939312393197405
939,1879,1878,3757,0.283627986907959,0.24795367866212886
941,1883,1882,3765,0.28423309326171875,0.24652251951728454
943,1887,1886,3773,0.2850508689880371,0.24509959558233635
945,1891,1890,3781,0.28560400009155273,0.24368485656261468
947,1895,1894,3789,0.28613710403442383,0.24227825276018136
949,1899,1898,3797,0.28647518157958984,0.2408797350479571
951,1903,1902,3805,0.2868940830230713,0.23948925484577652
953,1907,1906,3813,0.287229061126709,0.23810676409837825
955,1911,1910,3821,0.2875959873199463,0.236732215254979
957,1915,1914,3829,0.2881741523742676,0.23536556125015465
959,1919,1918,3837,0.2885429859161377,0.23400675548321362
961,1923,1922,3845,0.28890299797058105,0.23265575180395862
963,1927,1926,3853,0.28931212425231934,0.23131250449387575
965,1931,1930,3861,0.2896420955657959,0.22997696825154718
967,1935,1934,3869,0.29003024101257324,0.22864909817815962
969,1939,1938,3877,0.2903571128845215,0.22732884976535578
971,1943,1942,3885,0.29086804389953613,0.226016178879455
973,1947,1946,3893,0.29232096672058105,0.22471104175127232
975,1951,1950,3901,0.2928588390350342,0.2234133949656081
977,1955,1954,3909,0.29320812225341797,0.2221231954486789
979,1959,1958,3917,0.29364895820617676,0.2208404004591429
981,1963,1962,3925,0.2940511703491211,0.21956496757842248
983,1967,1966,3933,0.2943460941314697,0.21829685470156296
985,1971,1970,3941,0.29473304748535156,0.21703602002992062
987,1975,1974,3949,0.29506492614746094,0.2157824220613281
989,1979,1978,3957,0.29537487030029297,0.21453601958516336
991,1983,1982,3965,0.29579710960388184,0.21329677167323305
993,1987,1986,3973,0.2962069511413574,0.21206463767427286
995,1991,1990,3981,0.29685211181640625,0.210839577207624
997,1995,1994,3989,0.29717206954956055,0.20962155015696896
999,1999,1998,3997,0.29756903648376465,0.20841051666520555
1001,2003,2002,4005,0.29883813858032227,0.2072064371305031
1003,2007,2006,4013,0.29918909072875977,0.20600927219805187
1005,2011,2010,4021,0.29966115951538086,0.20481898275953545
1007,2015,2014,4029,0.30023813247680664,0.20363552994507003
1009,2019,2018,4037,0.30058813095092773,0.20245887512290592
1011,2023,2022,4045,0.30104494094848633,0.20128897989180133
1013,2027,2026,4053,0.3015260696411133,0.2001258060801959
1015,2031,2030,4061,0.30187296867370605,0.1989693157410637
1017,2035,2034,4069,0.30259108543395996,0.19781947114968026
1019,2039,2038,4077,0.30347704887390137,0.19667623480027116
1021,2043,2042,4085,0.30391407012939453,0.19553956940288594
1023,2047,2046,4093,0.3043079376220703,0.19440943788016746
1025,2051,2050,4101,0.3048369884490967,0.19328580336643822
1027,2055,2054,4109,0.3053300380706787,0.192168629203726
1029,2059,2058,4117,0.3077099323272705,0.19105787893934414
1031,2063,2062,4125,0.3084428310394287,0.18995351632475455
1033,2067,2066,4133,0.30883097648620605,0.18885550531233453
1035,2071,2070,4141,0.30928587913513184,0.18776381005453432
1037,2075,2074,4149,0.3097660541534424,0.18667839490102564
1039,2079,2078,4157,0.31009793281555176,0.18559922439632118
1041,2083,2082,4165,0.3105459213256836,0.18452626328044644
1043,2087,2086,4173,0.3109598159790039,0.18345947648487315
1045,2091,2090,4181,0.31132006645202637,0.18239882913155603
1047,2095,2094,4189,0.3118479251861572,0.18134428653260598
1049,2099,2098,4197,0.31255197525024414,0.1802958141865738
1051,2103,2102,4205,0.312974214553833,0.1792533777797251
1053,2107,2106,4213,0.31362199783325195,0.17821694318224007
1055,2111,2110,4221,0.3147909641265869,0.17718647644824287
1057,2115,2114,4229,0.31516003608703613,0.1761619438156307
1059,2119,2118,4237,0.31557297706604004,0.17514331170164965
1061,2123,2122,4245,0.31589603424072266,0.17413054670521633
1063,2127,2126,4253,0.316237211227417,0.17312361560335313
1065,2131,2130,4261,0.31657981872558594,0.17212248535204286
1067,2135,2134,4269,0.31693124771118164,0.17112712308316097
1069,2139,2138,4277,0.3172738552093506,0.17013749610517512
1071,2143,2142,4285,0.3176290988922119,0.169153571901508
1073,2147,2146,4293,0.3179929256439209,0.16817531812917286
1075,2151,2150,4301,0.3185911178588867,0.16720270261814404
1077,2155,2154,4309,0.3189680576324463,0.16623569337192265
1079,2159,2158,4317,0.3192861080169678,0.16527425856340308
1081,2163,2162,4325,0.31966280937194824,0.16431836653679366
1083,2167,2166,4333,0.32186293601989746,0.16336798580581846
1085,2171,2170,4341,0.3223130702972412,0.16242308505300404
1087,2175,2174,4349,0.32265806198120117,0.16148363312874686
1089,2179,2178,4357,0.3231821060180664,0.16054959904970817
1091,2183,2182,4365,0.3237619400024414,0.15962095200027188
1093,2187,2186,4373,0.32410597801208496,0.15869766132905516
1095,2191,2190,4381,0.3245048522949219,0.1577796965505485
1097,2195,2194,4389,0.3249499797821045,0.1568670273421225
1099,2199,2198,4397,0.32536911964416504,0.1559596235451076
1101,2203,2202,4405,0.3257730007171631,0.15505745516324587
1103,2207,2206,4413,0.3260691165924072,0.15416049236149987
1105,2211,2210,4421,0.32642602920532227,0.15326870546641563
1107,2215,2214,4429,0.3268868923187256,0.152382064964841
1109,2219,2218,4437,0.3272368907928467,0.15150054150285036
1111,2223,2222,4445,0.32764697074890137,0.15062410588561792
1113,2227,2226,4453,0.3280160427093506,0.14975272907661086
1115,2231,2230,4461,0.32833218574523926,0.14888638219640254
1117,2235,2234,4469,0.32871103286743164,0.14802503652277227
1119,2239,2238,4477,0.3293440341949463,0.14716866348897997
1121,2243,2242,4485,0.3297159671783447,0.14631723468435098
1123,2247,2246,4493,0.33044886589050293,0.14547072185196436
1125,2251,2250,4501,0.33083391189575195,0.14462909689021558
1127,2255,2254,4509,0.33115100860595703,0.14379233184980145
1129,2259,2258,4517,0.33144307136535645,0.14296039893405058
1131,2263,2262,4525,0.33177995681762695,0.1421332704992242
1133,2267,2266,4533,0.3320939540863037,0.14131091905172227
1135,2271,2270,4541,0.3323640823364258,0.14049331724917102
1137,2275,2274,4549,0.33266520500183105,0.13968043789926698
1139,2279,2278,4557,0.3330860137939453,0.13887225395803132
1141,2283,2282,4565,0.33343005180358887,0.13806873853161647
1143,2287,2286,4573,0.3338499069213867,0.13726986487223775
1145,2291,2290,4581,0.3342888355255127,0.13647560638128278
1147,2295,2294,4589,0.33515501022338867,0.13568593660525985
1149,2299,2298,4597,0.3355278968811035,0.13490082923701482
1151,2303,2302,4605,0.33605003356933594,0.13412025811529324
1153,2307,2306,4613,0.33941006660461426,0.13334419722181456
1155,2311,2310,4621,0.3398759365081787,0.13257262068396877
1157,2315,2314,4629,0.34040403366088867,0.13180550277187558
1159,2319,2318,4637,0.3408091068267822,0.1310428178974365
1161,2323,2322,4645,0.3411600589752197,0.1302845406153865
1163,2327,2326,4653,0.3415801525115967,0.12953064562104
1165,2331,2330,4661,0.3420240879058838,0.12878110775117962
1167,2335,2334,4669,0.3424389362335205,0.12803590198167103
1169,2339,2338,4677,0.34287381172180176,0.12729500342756062
1171,2343,2342,4685,0.3432741165161133,0.12655838734348454
1173,2347,2346,4693,0.3437530994415283,0.12582602912157204
1175,2351,2350,4701,0.34427714347839355,0.12509790429064002
1177,2355,2354,4709,0.3446929454803467,0.12437398851684903
1179,2359,2358,4717,0.345073938369751,0.12365425760175791
1181,2363,2362,4725,0.3454930782318115,0.12293868748325054
1183,2367,2366,4733,0.3462200164794922,0.12222725423262108
1185,2371,2370,4741,0.3476870059967041,0.12151993405593248
1187,2375,2374,4749,0.3480699062347412,0.12081670329247982
1189,2379,2378,4757,0.3484780788421631,0.12011753841435283
1191,2383,2382,4765,0.34893107414245605,0.1194224160254811
1193,2387,2386,4773,0.34929323196411133,0.11873131286065428
1195,2391,2390,4781,0.34963512420654297,0.1180442057868564
1197,2395,2394,4789,0.3500349521636963,0.1173610717997915
1199,2399,2398,4797,0.3503570556640625,0.11668188802554587
1201,2403,2402,4805,0.350783109664917,0.11600663171853123
1203,2407,2406,4813,0.35119104385375977,0.11533528026096407
1205,2411,2410,4821,0.35179710388183594,0.11466781116336343
1207,2415,2414,4829,0.35222411155700684,0.11400420206297161
1209,2419,2418,4837,0.35263705253601074,0.11334443072284187
1211,2423,2422,4845,0.35515713691711426,0.11268847503127606
1213,2427,2426,4853,0.35570788383483887,0.11203631300334642
1215,2431,2430,4861,0.3562331199645996,0.11138792277563259
1217,2435,2434,4869,0.35671401023864746,0.11074328261124088
1219,2439,2438,4877,0.35709500312805176,0.11010237089438656
1221,2443,2442,4885,0.3576059341430664,0.10946516613251696
1223,2447,2446,4893,0.35811519622802734,0.10883164695448108
1225,2451,2450,4901,0.35862088203430176,0.10820179211049885
1227,2455,2454,4909,0.35905909538269043,0.10757558047129247
1229,2459,2458,4917,0.3595468997955322,0.10695299102722423
1231,2463,2462,4925,0.3603529930114746,0.10633400288886548
1233,2467,2466,4933,0.36084794998168945,0.10571859528330428
1235,2471,2470,4941,0.36123013496398926,0.10510674755844646
1237,2475,2474,4949,0.36174607276916504,0.10449843917789986
1239,2479,2478,4957,0.36223602294921875,0.1038936497222941
1241,2483,2482,4965,0.3639349937438965,0.10329235888773945
1243,2487,2486,4973,0.364285945892334,0.10269454648784815
1245,2491,2490,4981,0.3646731376647949,0.10210019244911492
1247,2495,2494,4989,0.3650660514831543,0.10150927681376617
1249,2499,2498,4997,0.3653581142425537,0.10092177973722477
1251,2503,2502,5005,0.3656651973724365,0.10033768148744551
1253,2507,2506,5013,0.36595702171325684,0.09975696244616604
1255,2511,2510,5021,0.3663160800933838,0.09917960310615484
1257,2515,2514,5029,0.3667750358581543,0.0986055840715988
1259,2519,2518,5037,0.36708688735961914,0.0980348860579293
1261,2523,2522,5045,0.36742401123046875,0.09746748989012173
1263,2527,2526,5053,0.36782288551330566,0.09690337650244495
1265,2531,2530,5061,0.3681149482727051,0.0963425269391685
1267,2535,2534,5069,0.3684208393096924,0.0957849223518735
1269,2539,2538,5077,0.3687717914581299,0.09523054400033609
1271,2543,2542,5085,0.36944103240966797,0.09467937325112455
1273,2547,2546,5093,0.36997103691101074,0.09413139157839251
1275,2551,2550,5101,0.37035608291625977,0.09358658056155256
1277,2555,2554,5109,0.37071800231933594,0.0930449218850925
1279,2559,2558,5117,0.37119007110595703,0.09250639733903072
1281,2563,2562,5125,0.3715982437133789,0.09197098881799173
1283,2567,2566,5133,0.372006893157959,0.09143867831908412
1285,2571,2570,5141,0.37236499786376953,0.09090944794400567
1287,2575,2574,5149,0.3727607727050781,0.09038327989557608
1289,2579,2578,5157,0.37310004234313965,0.08986015648033822
1291,2583,2582,5165,0.37344908714294434,0.08934006010458785
1293,2587,2586,5173,0.37378478050231934,0.08882297327630624
1295,2591,2590,5181,0.37430500984191895,0.08830887860459023
1297,2595,2594,5189,0.3747270107269287,0.08779775879633653
1299,2599,2598,5197,0.3750569820404053,0.08728959666000823
1301,2603,2602,5205,0.37540197372436523,0.08678437510088664
1303,2607,2606,5213,0.37576985359191895,0.08628207712403117
1305,2611,2610,5221,0.37648892402648926,0.08578268583032754
1307,2615,2614,5229,0.37735414505004883,0.08528618441899323
1309,2619,2618,5237,0.3778839111328125,0.08479255618550097
1311,2623,2622,5245,0.37833404541015625,0.08430178452122435
1313,2627,2626,5253,0.3786790370941162,0.08381385291268142
1315,2631,2630,5261,0.3791959285736084,0.08332874494178778
1317,2635,2634,5269,0.37969112396240234,0.08284644428508274
1319,2639,2638,5277,0.3801591396331787,0.08236693471208818
1321,2643,2642,5285,0.3810131549835205,0.08189020008587228
1323,2647,2646,5293,0.3824341297149658,0.08141622436322762
1325,2651,2650,5301,0.3833470344543457,0.08094499159192053
1327,2655,2654,5309,0.38379502296447754,0.08047648591275991
1329,2659,2658,5317,0.38434696197509766,0.08001069155698881
1331,2663,2662,5325,0.3847789764404297,0.07954759284648201
1333,2667,2666,5333,0.3857741355895996,0.07908717419441844
1335,2671,2670,5341,0.3875248432159424,0.07862942010228534
1337,2675,2674,5349,0.38814282417297363,0.07817431516240578
1339,2679,2678,5357,0.3886301517486572,0.07772184405405337
1341,2683,2682,5365,0.38913488388061523,0.07727199154597991
1343,2687,2686,5373,0.38951611518859863,0.07682474249451232
1345,2691,2690,5381,0.38996005058288574,0.07638008184248717
1347,2695,2694,5389,0.3905320167541504,0.07593799462113024
1349,2699,2698,5397,0.39121007919311523,0.07549846594543538
1351,2703,2702,5405,0.39229607582092285,0.07506148101842487
1353,2707,2706,5413,0.3928380012512207,0.07462702512723628
1355,2711,2710,5421,0.39505791664123535,0.07419508364395708
1357,2715,2714,5429,0.39543890953063965,0.07376564202559302
1359,2719,2718,5437,0.39591407775878906,0.07333868581209743
1361,2723,2722,5445,0.3964049816131592,0.07291420062778305
1363,2727,2726,5453,0.39679908752441406,0.07249217217846272
1365,2731,2730,5461,0.39733099937438965,0.0720725862540304
1367,2735,2734,5469,0.3979761600494385,0.07165542872501013
1369,2739,2738,5477,0.3984670639038086,0.07124068554468159
1371,2743,2742,5485,0.3991730213165283,0.0708283427454418
1373,2747,2746,5493,0.39973902702331543,0.07041838644246795
1375,2751,2750,5501,0.40022778511047363,0.07001080282933801
1377,2755,2754,5509,0.40082406997680664,0.06960557818061765
1379,2759,2758,5517,0.4012291431427002,0.06920269884898034
1381,2763,2762,5525,0.40161991119384766,0.06880215126609682
1383,2767,2766,5533,0.4020400047302246,0.06840392194292835
1385,2771,2770,5541,0.40296101570129395,0.0680079974668031
1387,2775,2774,5549,0.4070260524749756,0.06761436450364208
1389,2779,2778,5557,0.40774106979370117,0.06722300979536261
1391,2783,2782,5565,0.4083709716796875,0.06683392016129094
1393,2787,2786,5573,0.4089200496673584,0.06644708249608859
1395,2791,2790,5581,0.4093310832977295,0.06606248377109873
1397,2795,2794,5589,0.40979695320129395,0.06568011103150727
1399,2799,2798,5597,0.4104771614074707,0.06529995139864096
1401,2803,2802,5605,0.41092419624328613,0.06492199206770745
1403,2807,2806,5613,0.41156888008117676,0.06454622030745694
1405,2811,2810,5621,0.41196703910827637,0.06417262346057899
1407,2815,2814,5629,0.4123690128326416,0.06380118894255843
1409,2819,2818,5637,0.4127938747406006,0.0634319042422694
1411,2823,2822,5645,0.41484498977661133,0.06306475692024537
1413,2827,2826,5653,0.4157130718231201,0.0626997346082699
1415,2831,2830,5661,0.41608309745788574,0.06233682501145439
1417,2835,2834,5669,0.4164140224456787,0.061976015904011666
1419,2839,2838,5677,0.416748046875,0.06161729513174757
1421,2843,2842,5685,0.4173450469970703,0.06126065061096072
1423,2847,2846,5693,0.4178040027618408,0.060906070326798754
1425,2851,2850,5701,0.4183471202850342,0.06055354233480747
1427,2855,2854,5709,0.4186840057373047,0.060203054758545246
1429,2859,2858,5717,0.4189920425415039,0.059854595790993684
1431,2863,2862,5725,0.41931915283203125,0.059508153693730914
1433,2867,2866,5733,0.4198009967803955,0.05916371679477375
1435,2871,2870,5741,0.4202849864959717,0.05882127349078263
1437,2875,2874,5749,0.42070603370666504,0.05848081224539339
1439,2879,2878,5757,0.42125391960144043,0.05814232158834848
1441,2883,2882,5765,0.4217848777770996,0.05780579011577348
1443,2887,2886,5773,0.42219018936157227,0.05747120649060815
1445,2891,2890,5781,0.42281198501586914,0.057138559439867634
1447,2895,2894,5789,0.42316603660583496,0.05680783775668174
1449,2899,2898,5797,0.42349910736083984,0.056479030299518146
1451,2903,2902,5805,0.4242110252380371,0.05615212598964411
1453,2907,2906,5813,0.4246399402618408,0.055827113813764324
1455,2911,2910,5821,0.4250361919403076,0.05550398282175064
1457,2915,2914,5829,0.4255349636077881,0.055182722126550746
1459,2919,2918,5837,0.42587900161743164,0.054863320904816645
1461,2923,2922,5845,0.42620086669921875,0.05454576839449595
1463,2927,2926,5853,0.4265620708465576,0.054230053897207725
1465,2931,2930,5861,0.42691898345947266,0.05391616677565851
1467,2935,2934,5869,0.427325963973999,0.05360409645416237
1469,2939,2938,5877,0.42776989936828613,0.053293832417923036
1471,2943,2942,5885,0.4282829761505127,0.05298536421337362
1473,2947,2946,5893,0.42872095108032227,0.05267868144772399
1475,2951,2950,5901,0.4290938377380371,0.052373773786827345
1477,2955,2954,5909,0.429426908493042,0.052070630958486075
1479,2959,2958,5917,0.4299349784851074,0.051769242748079355
1481,2963,2962,5925,0.4307420253753662,0.051469599000557587
1483,2967,2966,5933,0.4310920238494873,0.05117168962031887
1485,2971,2970,5941,0.4314389228820801,0.0508755045692796
1487,2975,2974,5949,0.4320390224456787,0.050581033867550626
1489,2979,2978,5957,0.43250584602355957,0.05028826759310672
1491,2983,2982,5965,0.432811975479126,0.04999719588197883
1493,2987,2986,5973,0.43343496322631836,0.04970780892604105
1495,2991,2990,5981,0.4337649345397949,0.04942009697490287
1497,2995,2994,5989,0.43409204483032227,0.049134050333649114
1499,2999,2998,5997,0.4344210624694824,0.0488496593643428
1502,3005,3004,6009,0.434967041015625,0.04842615634812345
1504,3009,3008,6017,0.4352760314941406,0.04814586275555157
1506,3013,3012,6025,0.4356701374053955,0.04786719153792814
1508,3017,3016,6033,0.436053991317749,0.047590133304834234
1510,3021,3020,6041,0.43648695945739746,0.047314678721154114
1512,3025,3024,6049,0.4369070529937744,0.047040818504639814
1514,3029,3028,6057,0.43740296363830566,0.04676854342757756
1516,3033,3032,6065,0.438230037689209,0.04649784431540898
1518,3037,3036,6073,0.43859195709228516,0.04622871204706478
1520,3041,3040,6081,0.43891215324401855,0.045961137553644206
1522,3045,3044,6089,0.4395751953125,0.04569511181871307
1524,3049,3048,6097,0.43993091583251953,0.045430625878718135
1526,3053,3052,6105,0.44043803215026855,0.04516767082055246
1528,3057,3056,6113,0.4409160614013672,0.04490623778445991
1530,3061,3060,6121,0.44129300117492676,0.04464631796093654
1532,3065,3064,6129,0.4416179656982422,0.0443879025912342
1534,3069,3068,6137,0.4420318603515625,0.04413098296798166
1536,3073,3072,6145,0.44240808486938477,0.04387555043347391
1538,3077,3076,6153,0.4427919387817383,0.04362159638117561
1540,3081,3080,6161,0.4431419372558594,0.04336911225318421
1542,3085,3084,6169,0.44357800483703613,0.04311808954132091
1544,3089,3088,6177,0.4439089298248291,0.04286851978723343
1546,3093,3092,6185,0.44419312477111816,0.04262039458138637
1548,3097,3096,6193,0.44455814361572266,0.04237370556234907
1550,3101,3100,6201,0.44488096237182617,0.042128444417599234
1552,3105,3104,6209,0.44531702995300293,0.04188460288230641
1554,3109,3108,6217,0.4456489086151123,0.041642172740123544
1556,3113,3112,6225,0.44601988792419434,0.0414011458214659
1558,3117,3116,6233,0.4467611312866211,0.04116151400480712
1560,3121,3120,6241,0.44714903831481934,0.04092326921447629
1562,3125,3124,6249,0.4475421905517578,0.04068640342327444
1564,3129,3128,6257,0.447890043258667,0.04045090864818179
1566,3133,3132,6265,0.4482738971710205,0.04021677695468506
1568,3137,3136,6273,0.44858598709106445,0.03998400045275991
1570,3141,3140,6281,0.4488980770111084,0.03975257129804201
1572,3145,3144,6289,0.44922399520874023,0.03952248169280242
1574,3149,3148,6297,0.4495508670806885,0.03929372388282557
1576,3153,3152,6305,0.44991326332092285,0.03906629015962443
1578,3157,3156,6313,0.4502449035644531,0.038840172859327164
1580,3161,3160,6321,0.4505600929260254,0.03861536436260856
1582,3165,3164,6329,0.45089006423950195,0.03839185709332355
1584,3169,3168,6337,0.45117807388305664,0.03816964352007991
1586,3173,3172,6345,0.45160508155822754,0.03794871615506781
1588,3177,3176,6353,0.4519460201263428,0.037729067553106566
1590,3181,3180,6361,0.4522559642791748,0.03751069031268962
1592,3185,3184,6369,0.4527151584625244,0.03729357707425086
1594,3189,3188,6377,0.4545018672943115,0.03707772052277053
1596,3193,3192,6385,0.45494794845581055,0.036863113383700054
1598,3197,3196,6393,0.45537590980529785,0.03664974842501734
1600,3201,3200,6401,0.45581603050231934,0.036437618457398256
1602,3205,3204,6409,0.4561269283294678,0.03622671633177147
1604,3209,3208,6417,0.4564940929412842,0.03601703494143174
1606,3213,3212,6425,0.4569549560546875,0.03580856722051206
1608,3217,3216,6433,0.45731306076049805,0.03560130614414468
1610,3221,3220,6441,0.45764684677124023,0.03539524472777244
1612,3225,3224,6449,0.45804286003112793,0.035190376027688396
1614,3229,3228,6457,0.4584920406341553,0.03498669314065735
1616,3233,3232,6465,0.45885705947875977,0.03478418920211227
1618,3237,3236,6473,0.4592020511627197,0.03458285738861258
1620,3241,3240,6481,0.45995402336120605,0.03438269091531742
1622,3245,3244,6489,0.4603121280670166,0.03418368303703128
1624,3249,3248,6497,0.46073102951049805,0.03398582704788138
1626,3253,3252,6505,0.4611079692840576,0.03378911628036608
1628,3257,3256,6513,0.46163201332092285,0.03359354410541188
1630,3261,3260,6521,0.4624168872833252,0.033399103932614145
1632,3265,3264,6529,0.4629518985748291,0.033205789209766724
1634,3269,3268,6537,0.4633190631866455,0.033013593422724294
1636,3273,3272,6545,0.4638090133666992,0.03282251009434652
1638,3277,3276,6553,0.4641869068145752,0.03263253278598907
1640,3281,3280,6561,0.464536190032959,0.032443655095290944
1642,3285,3284,6569,0.4649968147277832,0.03225587065782325
1644,3289,3288,6577,0.4653499126434326,0.03206917314530284
1646,3293,3292,6585,0.4656970500946045,0.03188355626641617
1648,3297,3296,6593,0.466001033782959,0.03169901376574045
1650,3301,3300,6601,0.46630406379699707,0.031515539425431754
1652,3305,3304,6609,0.4666318893432617,0.031333127061678866
1654,3309,3308,6617,0.4669661521911621,0.03115177052846618
1656,3313,3312,6625,0.46739697456359863,0.03097146371391286
1658,3317,3316,6633,0.4677901268005371,0.030792200541743975
1660,3321,3320,6641,0.46906089782714844,0.03061397497158509
1662,3325,3324,6649,0.46950793266296387,0.03043678099693437
1664,3329,3328,6657,0.47024106979370117,0.030260612647009185
1666,3333,3332,6665,0.47066593170166016,0.030085463985814725
1668,3337,3336,6673,0.4710547924041748,0.029911329109725132
1670,3341,3340,6681,0.47153496742248535,0.029738202152301725
1672,3345,3344,6689,0.4721710681915283,0.02956607727811981
1674,3349,3348,6697,0.47251105308532715,0.029394948687219792
1676,3353,3352,6705,0.4730062484741211,0.02922481061311198
1678,3357,3356,6713,0.47351598739624023,0.02905565732254712
1680,3361,3360,6721,0.4739370346069336,0.028887483114963003
1682,3365,3364,6729,0.47460412979125977,0.028720282323429207
1684,3369,3368,6737,0.4749939441680908,0.028554049313197924
1686,3373,3372,6745,0.4754040241241455,0.028388778483254707
1688,3377,3376,6753,0.4758448600769043,0.02822446426297787
1690,3381,3380,6761,0.4766349792480469,0.028061101116708002
1692,3385,3384,6769,0.47744202613830566,0.027898683537949425
1694,3389,3388,6777,0.47774386405944824,0.027737206054653112
1696,3393,3392,6785,0.4780712127685547,0.027576663224964798
1698,3397,3396,6793,0.47838497161865234,0.02741704963834547
1700,3401,3400,6801,0.47873497009277344,0.02725835991691794
1702,3405,3404,6809,0.47903895378112793,0.027100588712168687
1704,3409,3408,6817,0.4794430732727051,0.026943730708396615
1706,3413,3412,6825,0.4797670841217041,0.02678778061937461
1708,3417,3416,6833,0.48009300231933594,0.0266327331896507
1710,3421,3420,6841,0.4804549217224121,0.026478583194277837
1712,3425,3424,6849,0.4807710647583008,0.02632532543919655
1714,3429,3428,6857,0.48110389709472656,0.026172954759524157
1716,3433,3432,6865,0.481781005859375,0.02602146602081521
1718,3437,3436,6873,0.48213696479797363,0.025870854118237665
1720,3441,3440,6881,0.48248982429504395,0.02572111397608007
1722,3445,3444,6889,0.48286008834838867,0.02557224054850518
1724,3449,3448,6897,0.48398280143737793,0.02542422881864532
1726,3453,3452,6905,0.4843001365661621,0.025277073799086378
1728,3457,3456,6913,0.4846630096435547,0.025130770530521367
1730,3461,3460,6921,0.4851348400115967,0.024985314083256594
1732,3465,3464,6929,0.48557019233703613,0.024840699555052886
1734,3469,3468,6937,0.4859600067138672,0.024696922073477536
1736,3473,3472,6945,0.4863901138305664,0.02455397679288855
1738,3477,3476,6953,0.4867551326751709,0.02441185889626872
1740,3481,3480,6961,0.4871549606323242,0.02427056359460391
1742,3485,3484,6969,0.48755502700805664,0.02413008612687749
1744,3489,3488,6977,0.48797178268432617,0.023990421758583347
1746,3493,3492,6985,0.4886128902435303,0.023851565784002434
1748,3497,3496,6993,0.48899102210998535,0.02371351352313938
1750,3501,3500,7001,0.4893620014190674,0.023576260324435595
1752,3505,3504,7009,0.48979997634887695,0.023439801562596643
1754,3509,3508,7017,0.49021124839782715,0.023304132639300458
1756,3513,3512,7025,0.4907231330871582,0.023169248982723864
1758,3517,3516,7033,0.4922010898590088,0.023035146047022406
1760,3521,3520,7041,0.49269795417785645,0.022901819313583958
1762,3525,3524,7049,0.493074893951416,0.02276926429003511
1764,3529,3528,7057,0.49350500106811523,0.022637476508955815
1766,3533,3532,7065,0.4938671588897705,0.022506451529368865
1768,3537,3536,7073,0.49428892135620117,0.022376184936065142
1770,3541,3540,7081,0.49464988708496094,0.0222466723393408
1772,3545,3544,7089,0.49497294425964355,0.022117909374760793
1774,3549,3548,7097,0.4952688217163086,0.02198989170317996
1776,3553,3552,7105,0.49559879302978516,0.02186261501104412
1778,3557,3556,7113,0.4958930015563965,0.021736075009088984
1780,3561,3560,7121,0.49617910385131836,0.0216102674328408
1782,3565,3564,7129,0.49659085273742676,0.021485188043797714
1784,3569,3568,7137,0.4968750476837158,0.021360832626173925
1786,3573,3572,7145,0.49718785285949707,0.0212371969894221
1788,3577,3576,7153,0.4978492259979248,0.02111427696770715
1790,3581,3580,7161,0.4982438087463379,0.020992068418710222
1792,3585,3584,7169,0.49854016304016113,0.0208705672244321
1794,3589,3588,7177,0.49884796142578125,0.020749769290130414
1796,3593,3592,7185,0.49930286407470703,0.02062967054528968
1798,3597,3596,7193,0.49968910217285156,0.020510266942855022
1800,3601,3600,7201,0.49998998641967773,0.020391554459483454
1802,3605,3604,7209,0.5004820823669434,0.020273529094466565
1804,3609,3608,7217,0.5008959770202637,0.020156186870452474
1806,3613,3612,7225,0.5012218952178955,0.02003952383366418
1808,3617,3616,7233,0.5015602111816406,0.01992353605233685
1810,3621,3620,7241,0.5019810199737549,0.019808219618754685
1812,3625,3624,7249,0.5023150444030762,0.019693570645983996
1814,3629,3628,7257,0.5027370452880859,0.019579585271081223
1816,3633,3632,7265,0.503727912902832,0.019466259652932784
1818,3637,3636,7273,0.504356861114502,0.01935358997280368
1820,3641,3640,7281,0.5049550533294678,0.019241572433919166
1822,3645,3644,7289,0.5063638687133789,0.01913020326134575
1824,3649,3648,7297,0.5076239109039307,0.019019478702353973
1826,3653,3652,7305,0.5082900524139404,0.01890939502565997
1828,3657,3656,7313,0.5086860656738281,0.018799948521957856
1830,3661,3660,7321,0.5091469287872314,0.018691135503046023
1832,3665,3664,7329,0.5096211433410645,0.01858295230153458
1834,3669,3668,7337,0.5099380016326904,0.018475395272930406
1836,3673,3672,7345,0.5102968215942383,0.018368460792181285
1838,3677,3676,7353,0.5107159614562988,0.018262145255817572
1840,3681,3680,7361,0.5110621452331543,0.01815644508157272
1842,3685,3684,7369,0.511430025100708,0.018051356707192472
1844,3689,3688,7377,0.5118989944458008,0.01794687659194823
1846,3693,3692,7385,0.5122640132904053,0.0178430012147307
1848,3697,3696,7393,0.512969970703125,0.017739727074767665
1850,3701,3700,7401,0.513530969619751,0.017637050693046094
1852,3705,3704,7409,0.5138278007507324,0.017534968608734814
1854,3709,3708,7417,0.5142059326171875,0.017433477382258592
1856,3713,3712,7425,0.5147490501403809,0.017332573593405155
1858,3717,3716,7433,0.5151481628417969,0.017232253841932724
1860,3721,3720,7441,0.5155239105224609,0.01713251474755865
1862,3725,3724,7449,0.516024112701416,0.017033352949452123
1864,3729,3728,7457,0.5164120197296143,0.01693476510525302
1866,3733,3732,7465,0.5167779922485352,0.016836747893993743
1868,3737,3736,7473,0.5171310901641846,0.01673929801152137
1870,3741,3740,7481,0.5174589157104492,0.016642412174845682
1872,3745,3744,7489,0.5178382396697998,0.016546087119228756
1874,3749,3748,7497,0.5182070732116699,0.01645031959778739
1876,3753,3752,7505,0.5185389518737793,0.01635510638442757
1878,3757,3756,7513,0.5189390182495117,0.01626044427032508
1880,3761,3760,7521,0.519362211227417,0.01616633006529007
1882,3765,3764,7529,0.5199408531188965,0.01607276059873741
1884,3769,3768,7537,0.5203139781951904,0.015979732716584115
1886,3773,3772,7545,0.5206730365753174,0.015887243284449376
1888,3777,3776,7553,0.5210671424865723,0.01579528918598623
1890,3781,3780,7561,0.5217499732971191,0.01570386732214945
1892,3785,3784,7569,0.5223381519317627,0.015612974612391655
1894,3789,3788,7577,0.522935152053833,0.015522607993926671
1896,3793,3792,7585,0.5232930183410645,0.01543276442162451
1898,3797,3796,7593,0.5236349105834961,0.015343440868186828
1900,3801,3800,7601,0.5239920616149902,0.015254634323075042
1902,3805,3804,7609,0.5244560241699219,0.015166341794194137
1904,3809,3808,7617,0.5248169898986816,0.015078560305979143
1906,3813,3812,7625,0.5251321792602539,0.014991286900899044
1908,3817,3816,7633,0.5255041122436523,0.014904518637914175
1910,3821,3820,7641,0.5257940292358398,0.014818252592678731
1912,3825,3824,7649,0.5261421203613281,0.014732485858787545
1914,3829,3828,7657,0.5265090465545654,0.01464721554619025
1916,3833,3832,7665,0.5268759727478027,0.014562438781191274
1918,3837,3836,7673,0.5274450778961182,0.014478152706991352
1920,3841,3840,7681,0.5279140472412109,0.014394354483637446
1922,3845,3844,7689,0.5282120704650879,0.014311041287340264
1924,3849,3848,7697,0.5285651683807373,0.014228210310555767
1926,3853,3852,7705,0.5290069580078125,0.014145858762044992
1928,3857,3856,7713,0.5295271873474121,0.014063983867355755
1930,3861,3860,7721,0.5298471450805664,0.013982582866454632
1932,3865,3864,7729,0.5301520824432373,0.013901653017357655
1934,3869,3868,7737,0.5305039882659912,0.013821191592363172
1936,3873,3872,7745,0.5308430194854736,0.013741195880397065
1938,3877,3876,7753,0.531135082244873,0.013661663185317972
1940,3881,3880,7761,0.5315232276916504,0.01358259082801722
1942,3885,3884,7769,0.5318658351898193,0.013503976143536083
1944,3889,3888,7777,0.5321869850158691,0.013425816482631392
1946,3893,3892,7785,0.5325498580932617,0.013348109211756798
1948,3897,3896,7793,0.5328869819641113,0.013270851712119305
1950,3901,3900,7801,0.533257007598877,0.01319404138078172
1952,3905,3904,7809,0.5336101055145264,0.013117675629214303
1954,3909,3908,7817,0.5339651107788086,0.013041751884049857
1956,3913,3912,7825,0.5343930721282959,0.012966267586962356
1958,3917,3916,7833,0.5347089767456055,0.012891220194520806
1960,3921,3920,7841,0.5350751876831055,0.01281660717748162
1962,3925,3924,7849,0.535646915435791,0.012742426021643948
1964,3929,3928,7857,0.5359230041503906,0.012668674227700327
1966,3933,3932,7865,0.5362539291381836,0.012595349310356645
1968,3937,3936,7873,0.5367507934570312,0.012522448798371503
1970,3941,3940,7881,0.5373151302337646,0.012449970235626627
1972,3945,3944,7889,0.5377700328826904,0.012377911179409779
1974,3949,3948,7897,0.5381360054016113,0.012306269202318795
1976,3953,3952,7905,0.5387270450592041,0.012235041889176979
1978,3957,3956,7913,0.5391139984130859,0.012164226840963547
1980,3961,3960,7921,0.5396161079406738,0.012093821670162267
1982,3965,3964,7929,0.5399508476257324,0.012023824005736181
1984,3969,3968,7937,0.5403831005096436,0.011954231487735938
1986,3973,3972,7945,0.5408949851989746,0.011885041771729388
1988,3977,3976,7953,0.541262149810791,0.011816252526171082
1990,3981,3980,7961,0.5419621467590332,0.01174786143315135
1992,3985,3984,7969,0.5423581600189209,0.011679866188123849
1994,3989,3988,7977,0.5438499450683594,0.011612264499335306
1996,3993,3992,7985,0.5449340343475342,0.011545054089493963
1998,3997,3996,7993,0.5459010601043701,0.011478232693533517
2000,4001,4000,8001,0.5463180541992188,0.011411798059870162


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n100/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00020194053649902344,1624.447741208611
4,5,4,9,0.0008759498596191406,544.0363924486542
8,9,8,17,0.0013208389282226562,401.36173086288113
12,13,12,25,0.001981019973754883,357.6362406908207
16,17,16,33,0.002579927444458008,304.7035721234219
20,21,20,41,0.0031027793884277344,282.5429398756775
24,25,24,49,0.003531932830810547,263.545386602969
28,29,28,57,0.004087924957275391,237.93843605665717
32,33,32,65,0.004586935043334961,232.74209504525268
36,37,36,73,0.005198955535888672,220.62732228780956
40,41,40,81,0.005733013153076172,206.6600819236898
44,45,44,89,0.006302833557128906,195.8071309227584
48,49,48,97,0.006731986999511719,185.98499736100567
52,53,52,105,0.007124900817871094,176.4249801671244
56,57,56,113,0.0076639652252197266,160.99673438238366
60,61,60,121,0.008116960525512695,155.074669878236
64,65,64,129,0.008572101593017578,140.68248881187407
68,69,68,137,0.009264945983886719,136.7436112633426
72,73,72,145,0.010180950164794922,126.13555406669731
76,77,76,153,0.010729789733886719,122.6271767498189
80,81,80,161,0.01119089126586914,120.1033131263988
84,85,84,169,0.012272119522094727,118.24307803399842
88,89,88,177,0.013134002685546875,111.03160848755374
92,93,92,185,0.013734102249145508,109.3209356466436
96,97,96,193,0.014208793640136719,107.9916479742846
100,101,100,201,0.014654874801635742,106.91733970853818
104,105,104,209,0.015380859375,106.01145651130207
108,109,108,217,0.016025066375732422,105.21442637828665
112,113,112,225,0.016675949096679688,104.48584861162735
116,117,116,233,0.01816701889038086,97.67474138373207
120,121,120,241,0.019238948822021484,96.84624281394237
124,125,124,249,0.01974010467529297,92.74771647581538
128,129,128,257,0.02053380012512207,91.91509966615192
132,133,132,265,0.021397829055786133,91.18224271567236
136,137,136,273,0.022439956665039062,90.51735649943699
140,141,140,281,0.023251056671142578,89.89785040541214
144,145,144,289,0.024168014526367188,89.30787727274557
148,149,148,297,0.02477097511291504,88.73647502499213
152,153,152,305,0.025660991668701172,88.17619040764093
156,157,156,313,0.026256084442138672,87.62206905106336
160,161,160,321,0.028964996337890625,87.07091988800155
164,165,164,329,0.02959609031677246,86.52078289621288
168,169,168,337,0.030236005783081055,85.97054634171977
172,173,172,345,0.031232833862304688,85.41967326824538
176,177,176,353,0.031828880310058594,80.48713944352677
180,181,180,361,0.03242897987365723,76.51439549094081
184,185,184,369,0.03319692611694336,75.89004502747424
188,189,188,377,0.034355878829956055,70.61728750362394
192,193,192,385,0.035459041595458984,69.83631139639554
196,197,196,393,0.03595900535583496,69.14499527167709
200,201,200,401,0.037843942642211914,68.52331642120069
204,205,204,409,0.0386967658996582,67.95546289645084
208,209,208,417,0.0392909049987793,67.42903078438667
212,213,212,425,0.03988909721374512,66.93434279160262
216,217,216,433,0.04048895835876465,66.46388913799011
220,221,220,441,0.04096078872680664,66.01187365771331
224,225,224,449,0.041525840759277344,65.57384841501334
228,229,228,457,0.042059898376464844,65.14642156904569
232,233,232,465,0.04266095161437988,64.72702509833591
236,237,236,473,0.04343390464782715,64.31373097304711
240,241,240,481,0.045243024826049805,63.90510624540377
244,245,244,489,0.04606890678405762,63.50009921859921
248,249,248,497,0.04659914970397949,63.097950316462374
252,253,252,505,0.04706978797912598,42.928681601131835
256,257,256,513,0.04754805564880371,42.31386496047765
260,261,260,521,0.048104047775268555,41.75511564194155
264,265,264,529,0.04870104789733887,41.243319637147486
268,269,268,537,0.04923582077026367,40.77090063718943
272,273,272,545,0.04976201057434082,40.33156954690536
276,277,276,553,0.050779104232788086,39.920111580527845
280,281,280,561,0.05128788948059082,39.53220534107694
284,285,284,569,0.051841020584106445,39.1642702706694
288,289,288,577,0.05273103713989258,38.813338833140236
292,293,292,585,0.053900957107543945,38.47694996361897
296,297,296,593,0.054566144943237305,38.15306060715899
300,301,300,601,0.055130958557128906,37.83997251045455
304,305,304,609,0.05572700500488281,37.53627178625901
308,309,308,617,0.05624890327453613,37.24077911442421
312,313,312,625,0.056715965270996094,36.952508761712366
316,317,316,633,0.05713391304016113,36.67063488781365
320,321,320,641,0.05757880210876465,36.394463854972344
324,325,324,649,0.05818295478820801,36.12341147412815
328,329,328,657,0.05860280990600586,29.865925543727368
332,333,332,665,0.05952882766723633,29.44784519348868
336,337,336,673,0.06109309196472168,29.06593245041313
340,341,340,681,0.06172800064086914,28.714757557990858
344,345,344,689,0.06225299835205078,28.389732415638928
348,349,348,697,0.06268787384033203,28.08698598009602
352,353,352,705,0.0631258487701416,27.803256108071604
356,357,356,713,0.06362485885620117,27.535795888509604
360,361,360,721,0.06407690048217773,27.282293138009276
364,365,364,729,0.06450915336608887,25.450190182078607
368,369,368,737,0.06510496139526367,25.28488829886332
372,373,372,745,0.06610798835754395,25.1206770110684
376,377,376,753,0.07094383239746094,24.957548230065413
380,381,380,761,0.07262706756591797,24.795496788854646
384,385,384,769,0.07330608367919922,24.634517344435352
388,389,388,777,0.07378077507019043,24.474604396685685
392,393,392,785,0.0743410587310791,24.3157523058087
396,397,396,793,0.07500886917114258,24.157955308388512
400,401,400,801,0.07596611976623535,24.001207532169683
404,405,404,809,0.07655477523803711,23.845503009641643
408,409,408,817,0.07723498344421387,23.690835690487255
412,413,412,825,0.0785069465637207,23.53719945301423
416,417,416,833,0.08077406883239746,23.384588114610608
420,421,420,841,0.08258199691772461,23.23299544130487
424,425,424,849,0.08413410186767578,23.082415156513356
428,429,428,857,0.08503103256225586,21.615457079608014
432,433,432,865,0.08555102348327637,21.47159438434253
436,437,436,873,0.08709096908569336,21.330744227379853
440,441,440,881,0.08784890174865723,21.192511919558825
444,445,444,889,0.09101605415344238,21.056564123663524
448,449,448,897,0.09402108192443848,20.922620145173763
452,453,452,905,0.09514999389648438,20.79044406821151
456,457,456,913,0.09605908393859863,20.659838011098987
460,461,460,921,0.09940505027770996,20.530636350795973
464,465,464,929,0.10022377967834473,20.40270078376111
468,469,468,937,0.10082793235778809,20.275916107488808
472,473,472,945,0.10131692886352539,20.150186621901526
476,477,476,953,0.10183215141296387,20.025433063048073
480,481,480,961,0.10286092758178711,19.901589993317494
484,485,484,969,0.10356283187866211,19.778603582684593
488,489,488,977,0.10423898696899414,19.65642972452914
492,493,492,985,0.10490989685058594,19.535032437437053
496,497,496,993,0.10547804832458496,19.41438251120289
501,502,501,1003,0.1060950756072998,19.264585605582983
505,506,505,1011,0.10655879974365234,19.145538025655593
509,510,509,1019,0.10696578025817871,19.027176953741304
513,514,513,1027,0.10769295692443848,18.909491149954025
517,518,517,1035,0.1083838939666748,18.792471818905863
521,522,521,1043,0.10926103591918945,17.593531374547773
525,526,525,1051,0.10973095893859863,17.468789168505587
529,530,529,1059,0.11039090156555176,17.34754628684548
533,534,533,1067,0.11083197593688965,17.229370822407297
537,538,537,1075,0.11137509346008301,17.113928110593758
541,542,541,1083,0.1118917465209961,17.000925663288168
545,546,545,1091,0.11245393753051758,16.89010805708794
549,550,549,1099,0.11291313171386719,16.78125240562571
553,554,553,1107,0.11348795890808105,16.674164356111977
557,558,557,1115,0.11393499374389648,16.568674554878626
561,562,561,1123,0.11435794830322266,16.46463553119361
565,566,565,1131,0.11484003067016602,16.361918953300126
569,570,569,1139,0.11815786361694336,16.260413214866336
573,574,573,1147,0.12055587768554688,16.160021314213047
577,578,577,1155,0.12176203727722168,16.06065899252718
581,582,581,1163,0.12252187728881836,15.962253100820071
585,586,585,1171,0.12323689460754395,15.86474016864462
589,590,589,1179,0.12375998497009277,15.768065150595534
593,594,593,1187,0.1243281364440918,15.672180329231544
597,598,597,1195,0.12486004829406738,15.577044355596275
601,602,601,1203,0.12532591819763184,15.482621410560496
605,606,605,1211,0.12752389907836914,15.388880472279665
609,610,609,1219,0.12835383415222168,15.29579467672093
613,614,613,1227,0.1288619041442871,14.40395859398114
617,618,617,1235,0.12962603569030762,14.301780376941366
621,622,621,1243,0.13014793395996094,14.202197274772644
625,626,625,1251,0.13071298599243164,14.104958629311172
629,630,629,1259,0.1313319206237793,14.009840930872933
633,634,633,1267,0.1318509578704834,13.916645399881343
637,638,637,1275,0.13251709938049316,12.598575013848881
641,642,641,1283,0.13425302505493164,5.782445343921283
645,646,645,1291,0.1347799301147461,5.6544576030634826
649,650,649,1299,0.1354978084564209,5.534454775684021
653,654,653,1307,0.1360948085784912,5.421880387553471
657,658,657,1315,0.13713979721069336,5.316208659390859
661,662,661,1323,0.13832306861877441,5.216943774893515
665,666,665,1331,0.1397998332977295,5.123619087963474
669,670,669,1339,0.14033913612365723,5.035796268137652
673,674,673,1347,0.14081406593322754,4.953064385470764
677,678,677,1355,0.14142298698425293,4.875038938973531
681,682,681,1363,0.14196014404296875,4.801360834987081
685,686,685,1371,0.1424710750579834,4.7316953235630494
689,690,689,1379,0.1449570655822754,4.665730902071809
693,694,693,1387,0.14560294151306152,4.603178195854054
697,698,697,1395,0.14802193641662598,4.543768825909008
701,702,701,1403,0.14864492416381836,4.487254273366698
705,706,705,1411,0.1495358943939209,4.4334047499642635
709,710,709,1419,0.15008091926574707,4.382008082988144
713,714,713,1427,0.15060901641845703,4.332868622215
717,718,717,1435,0.1511549949645996,4.285806175373983
721,722,721,1443,0.15267491340637207,4.240654977616675
725,726,725,1451,0.1533200740814209,4.197262699420698
729,730,729,1459,0.15424489974975586,4.155489496357391
733,734,733,1467,0.15486598014831543,4.115207103236635
737,738,737,1475,0.15552878379821777,4.076297974259821
741,742,741,1483,0.15630602836608887,4.038654470088903
745,746,745,1491,0.15685105323791504,4.002178092046624
749,750,749,1499,0.15749192237854004,3.9667787631347764
753,754,753,1507,0.15839815139770508,3.9323741550506397
757,758,757,1515,0.15887999534606934,3.898889060034813
761,762,761,1523,0.1593928337097168,3.866254806059838
765,766,765,1531,0.16135597229003906,3.8344087136450655
769,770,769,1539,0.1619129180908203,3.8032935924216917
773,774,773,1547,0.16254711151123047,3.772857275457154
777,778,777,1555,0.16299891471862793,3.7430521892680515
781,782,781,1563,0.16350412368774414,3.713834957461397
785,786,785,1571,0.163970947265625,3.6851660359000893
789,790,789,1579,0.16450190544128418,3.6570093773595915
793,794,793,1587,0.16498303413391113,3.62933212368159
797,798,797,1595,0.1656968593597412,3.6021043234762016
801,802,801,1603,0.16650891304016113,3.575298673552952
805,806,805,1611,0.1672511100769043,3.5488902822780957
809,810,809,1619,0.16994190216064453,3.522856453218773
813,814,813,1627,0.17064905166625977,3.497176487474093
817,818,817,1635,0.17223286628723145,3.471831503218151
821,822,821,1643,0.1737661361694336,3.4468042710618434
825,826,825,1651,0.17563581466674805,3.4220790639448944
829,830,829,1659,0.17716288566589355,3.3976415203426207
833,834,833,1667,0.1780109405517578,3.3734785196759947
837,838,837,1675,0.17870616912841797,3.3495780688869683
841,842,841,1683,0.17930006980895996,3.3259291992179185
845,846,845,1691,0.1799020767211914,3.3025218723214715
849,850,849,1699,0.18188095092773438,3.2793468948794304
853,854,853,1707,0.1824181079864502,3.25639584098783
857,858,857,1715,0.18320989608764648,3.2336609816215685
861,862,861,1723,0.18374991416931152,3.2111352205496346
865,866,865,1731,0.18462085723876953,3.188812036126301
869,870,869,1739,0.1852269172668457,3.1666854284284787
873,874,873,1747,0.1858210563659668,3.1447498712589637
877,878,877,1755,0.18886995315551758,3.1230002685783123
881,882,881,1763,0.18964385986328125,3.1014319149566507
885,886,885,1771,0.19016003608703613,3.080040459688916
889,890,889,1779,0.1907508373260498,3.0588218742266586
893,894,893,1787,0.1913299560546875,3.037772422635141
897,898,897,1795,0.19181203842163086,3.01688863479086
901,902,901,1803,0.192518949508667,2.9961672820696954
905,906,905,1811,0.19302892684936523,2.975605355297039
909,910,909,1819,0.19400691986083984,2.95520004474309
913,914,913,1827,0.1946089267730713,2.934948721992712
917,918,917,1835,0.19525909423828125,2.91484892349093
921,922,921,1843,0.19584083557128906,2.8948983356372175
925,926,925,1851,0.19702696800231934,2.8750947812544174
929,930,929,1859,0.19822406768798828,2.8554362073293813
933,934,933,1867,0.19966983795166016,2.2495048218023213
937,938,937,1875,0.2002239227294922,2.225129297906036
941,942,941,1883,0.20083403587341309,2.2015948125247875
945,946,945,1891,0.20135998725891113,2.178848380795309
949,950,949,1899,0.2018437385559082,2.156840433128436
953,954,953,1907,0.2022838592529297,2.1355246252098774
957,958,957,1915,0.2027120590209961,2.114857656039003
961,962,961,1923,0.20311284065246582,2.094799092454854
965,966,965,1931,0.20416879653930664,2.0753112004131657
969,970,969,1939,0.20534992218017578,2.0563587831844834
973,974,973,1947,0.2059187889099121,2.0379090265876023
977,978,977,1955,0.20720195770263672,2.019931351299467
981,982,981,1963,0.20774388313293457,2.0023972722312
985,986,985,1971,0.20836997032165527,1.9852802649181345
989,990,989,1979,0.20887374877929688,1.9685556388145433
993,994,993,1987,0.20931291580200195,1.9522004173528398
997,998,997,1995,0.20994281768798828,1.9361932246110767
1001,1002,1001,2003,0.2105109691619873,1.9205141783802298
1005,1006,1005,2011,0.21105694770812988,1.9051447894289122
1009,1010,1009,2019,0.21177315711975098,1.890067866735804
1013,1014,1013,2027,0.21224212646484375,1.8752674284560393
1017,1018,1017,2035,0.21291685104370117,1.860728618358714
1021,1022,1021,2043,0.21352314949035645,1.8464376275109253
1025,1026,1025,2051,0.21421408653259277,1.8323816209387997
1029,1030,1029,2059,0.2146449089050293,1.8185486690234594
1033,1034,1033,2067,0.21507906913757324,1.8049276833790497
1037,1038,1037,2075,0.2157909870147705,1.7915083569840533
1041,1042,1041,2083,0.21660780906677246,1.7782811083031167
1045,1046,1045,2091,0.21730709075927734,1.7652370292013286
1049,1050,1049,2099,0.21810388565063477,1.7523678364039468
1053,1054,1053,2107,0.21915698051452637,1.739665826298046
1057,1058,1057,2115,0.22142696380615234,1.7271238328720435
1061,1062,1061,2123,0.22205781936645508,1.71473518859239
1065,1066,1065,2131,0.22285676002502441,1.702493688032251
1069,1070,1069,2139,0.22336101531982422,1.6903935540809036
1073,1074,1073,2147,0.22399306297302246,1.6784294065473315
1077,1078,1077,2155,0.22443675994873047,1.666596233026288
1081,1082,1081,2163,0.22499489784240723,1.6548893618455922
1085,1086,1085,2171,0.22585201263427734,1.6433044369784833
1089,1090,1089,2179,0.22690391540527344,1.6318373947725497
1093,1094,1093,2187,0.22748780250549316,1.6204844423694857
1097,1098,1097,2195,0.22818589210510254,1.609242037710629
1101,1102,1101,2203,0.22864389419555664,1.5981068710020723
1105,1106,1105,2211,0.230604887008667,1.5870758475453062
1109,1110,1109,2219,0.23119592666625977,1.5761460718322375
1113,1114,1113,2227,0.231964111328125,1.5653148328206459
1117,1118,1117,2235,0.2325611114501953,1.554579590294459
1121,1122,1121,2243,0.23334217071533203,1.543937962241531
1125,1126,1125,2251,0.2338268756866455,1.5333877131672007
1129,1130,1129,2259,0.23444080352783203,1.5229267432862112
1133,1134,1133,2267,0.23502779006958008,1.5125530785087418
1137,1138,1137,2275,0.2355518341064453,1.502264861186468
1141,1142,1141,2283,0.2360069751739502,1.4920603415456681
1145,1146,1145,2291,0.2377159595489502,0.8304834359113775
1149,1150,1149,2299,0.2384810447692871,0.8136089404653333
1153,1154,1153,2307,0.23935198783874512,0.7974069942858905
1157,1158,1157,2315,0.24022793769836426,0.7818505446205847
1161,1162,1161,2323,0.2411518096923828,0.7669132957504431
1165,1166,1165,2331,0.2418510913848877,0.7525697565568208
1169,1170,1169,2339,0.24290704727172852,0.7387952270322665
1173,1174,1173,2347,0.24358487129211426,0.7255657854466626
1177,1178,1177,2355,0.2443699836730957,0.712858276035837
1181,1182,1181,2363,0.24484491348266602,0.7006502970733024
1185,1186,1185,2371,0.24547505378723145,0.688920189201595
1189,1190,1189,2379,0.24604105949401855,0.6776470239038594
1193,1194,1193,2387,0.24688196182250977,0.666810592009419
1197,1198,1197,2395,0.24859881401062012,0.6563913921415775
1201,1202,1201,2403,0.24909305572509766,0.6463706190179203
1205,1206,1205,2411,0.24954795837402344,0.6367301515399042
1209,1210,1209,2419,0.25005412101745605,0.6274525406099924
1213,1214,1213,2427,0.2505369186401367,0.6185209966326219
1217,1218,1217,2435,0.2510371208190918,0.6099193766700071
1221,1222,1221,2443,0.2514641284942627,0.601632171226784
1225,1226,1225,2451,0.25199103355407715,0.5936444906630177
1229,1230,1229,2459,0.25345396995544434,0.5859420512305273
1233,1234,1233,2467,0.2539801597595215,0.578511160746579
1237,1238,1237,2475,0.2544889450073242,0.5713387039290884
1241,1242,1241,2483,0.2551441192626953,0.5644121274113506
1245,1246,1245,2491,0.25568604469299316,0.5577194244799988
1249,1250,1249,2499,0.25643205642700195,0.5512491195682615
1253,1254,1253,2507,0.25689196586608887,0.5449902525475029
1257,1258,1257,2515,0.2575390338897705,0.5389323628643411
1261,1262,1261,2523,0.2585489749908447,0.5330654735699204
1265,1266,1265,2531,0.25936198234558105,0.5273800752869996
1269,1270,1269,2539,0.2600250244140625,0.5218671101657764
1273,1274,1273,2547,0.2606649398803711,0.5165179558709114
1277,1278,1277,2555,0.261077880859375,0.5113244096518587
1281,1282,1281,2563,0.26153993606567383,0.5062786725342693
1285,1286,1285,2571,0.2619490623474121,0.501373333676657
1289,1290,1289,2579,0.2626228332519531,0.49660135492982216
1293,1294,1293,2587,0.2641267776489258,0.49195605563738903
1297,1298,1297,2595,0.2646949291229248,0.4874310977036176
1301,1302,1301,2603,0.2651839256286621,0.4830204709664045
1305,1306,1305,2611,0.2659449577331543,0.47871847889089947
1309,1310,1309,2619,0.2664909362792969,0.4745197246177038
1313,1314,1313,2627,0.26935696601867676,0.47041909737103255
1317,1318,1317,2635,0.26995182037353516,0.4664117592579236
1321,1322,1321,2643,0.2713019847869873,0.46249313245751145
1325,1326,1325,2651,0.27193474769592285,0.45865888681976386
1329,1330,1329,2659,0.2733888626098633,0.4549049278760385
1333,1334,1333,2667,0.277385950088501,0.4512273852688535
1337,1338,1337,2675,0.27861595153808594,0.4476226015994192
1341,1342,1341,2683,0.2792038917541504,0.4440871216992089
1345,1346,1345,2691,0.28005003929138184,0.44061768231650983
1349,1350,1349,2699,0.2808659076690674,0.43721120222103776
1353,1354,1353,2707,0.282088041305542,0.4338647727176026
1357,1358,1357,2715,0.28339505195617676,0.43057564856281866
1361,1362,1361,2723,0.28517889976501465,0.42734123927899603
1365,1366,1365,2731,0.2861759662628174,0.4241591008568908
1369,1370,1369,2739,0.2869999408721924,0.4210269278338884
1373,1374,1373,2747,0.2888941764831543,0.41794254574341877
1377,1378,1377,2755,0.2893648147583008,0.41490390391999965
1381,1382,1381,2763,0.28999805450439453,0.41190906865149624
1385,1386,1385,2771,0.29054999351501465,0.40895621666663623
1389,1390,1389,2779,0.29110288619995117,0.4060436289448085
1393,1394,1393,2787,0.2921891212463379,0.40316968484050336
1397,1398,1397,2795,0.29273104667663574,0.4003328565015572
1401,1402,1401,2803,0.2937638759613037,0.3975317035835102
1405,1406,1405,2811,0.294266939163208,0.3947648682317937
1409,1410,1409,2819,0.29475998878479004,0.39203107033511375
1413,1414,1413,2827,0.29544901847839355,0.38932910302686624
1417,1418,1417,2835,0.2959861755371094,0.3866578284320578
1421,1422,1421,2843,0.2965400218963623,0.38401617364291923
1425,1426,1425,2851,0.2971959114074707,0.3814031269161988
1429,1430,1429,2859,0.2979397773742676,0.37881773407694336
1433,1434,1433,2867,0.29848313331604004,0.3762590951256464
1437,1438,1437,2875,0.29894399642944336,0.3737263610341928
1441,1442,1441,2883,0.29936814308166504,0.37121873071927014
1445,1446,1445,2891,0.2998690605163574,0.36873544819078463
1449,1450,1449,2899,0.30036187171936035,0.3662757998611856
1453,1454,1453,2907,0.3013029098510742,0.36383911200709895
1457,1458,1457,2915,0.30173206329345703,0.36142474838092686
1461,1462,1461,2923,0.302152156829834,0.3590321079557587
1465,1466,1465,2931,0.3025698661804199,0.3566606228054295
1469,1470,1469,2939,0.3029599189758301,0.3543097561062665
1473,1474,1473,2947,0.3033158779144287,0.3519790002560917
1477,1478,1477,2955,0.30370497703552246,0.3496678751036569
1481,1482,1481,2963,0.3041250705718994,0.3473759262820464
1485,1486,1485,2971,0.3045229911804199,0.3451027236440108
1489,1490,1489,2979,0.3049740791320801,0.3428478597858858
1493,1494,1493,2987,0.3053920269012451,0.3406109486613887
1497,1498,1497,2995,0.30608391761779785,0.3383916242811402
1502,1503,1502,3005,0.30660390853881836,0.3356416729852381
1506,1507,1506,3013,0.30703306198120117,0.3334606763003361
1510,1511,1510,3021,0.30744099617004395,0.3312962010827291
1514,1515,1514,3029,0.30785703659057617,0.32914795377159106
1518,1519,1518,3037,0.3083679676055908,0.32701565520190395
1522,1523,1522,3045,0.30887794494628906,0.3248990397221639
1526,1527,1526,3053,0.30942201614379883,0.32279785436459285
1530,1531,1530,3061,0.30994701385498047,0.32071185806818014
1534,1535,1534,3069,0.31067514419555664,0.31864082094651247
1538,1539,1538,3077,0.31122803688049316,0.3165845236024685
1542,1543,1542,3085,0.3118579387664795,0.31454275648494334
1546,1547,1546,3093,0.31232595443725586,0.312515319283273
1550,1551,1550,3101,0.31282901763916016,0.31050202036258084
1554,1555,1554,3109,0.31327390670776367,0.3085026762299642
1558,1559,1558,3117,0.31375885009765625,0.30651711103640483
1562,1563,1562,3125,0.3142850399017334,0.3045451561091146
1566,1567,1566,3133,0.3167269229888916,0.3025866495118356
1570,1571,1570,3141,0.31722211837768555,0.3006414356346439
1574,1575,1574,3149,0.3176109790802002,0.2987093648062779
1578,1579,1578,3157,0.31804800033569336,0.2967902929332278
1582,1583,1582,3165,0.31848907470703125,0.29488408116180076
1586,1587,1586,3173,0.3190019130706787,0.2929905955573933
1590,1591,1590,3181,0.31946802139282227,0.2911097068087943
1594,1595,1594,3189,0.31993579864501953,0.28924128994786535
1598,1599,1598,3197,0.3204519748687744,0.2873852240889178
1602,1603,1602,3205,0.3214409351348877,0.28554139218104574
1606,1607,1606,3213,0.3220489025115967,0.2837096807819017
1610,1611,1610,3221,0.3227040767669678,0.28188997983937847
1614,1615,1614,3229,0.32337284088134766,0.2800821824917321
1618,1619,1618,3237,0.3239269256591797,0.2782861848781429
1622,1623,1622,3245,0.3244037628173828,0.2765018859619645
1626,1627,1626,3253,0.32503485679626465,0.2747291873651564
1630,1631,1630,3261,0.32566118240356445,0.2729679932134051
1634,1635,1634,3269,0.3262648582458496,0.2712182099914898
1638,1639,1638,3277,0.32666993141174316,0.2694797464051123
1642,1643,1642,3285,0.32719874382019043,0.2677525132563789
1646,1647,1646,3293,0.3278040885925293,0.26603642332341587
1650,1651,1650,3301,0.32843685150146484,0.26433139124966226
1654,1655,1654,3309,0.3302009105682373,0.26263733343782447
1658,1659,1658,3317,0.3306751251220703,0.26095416795543935
1662,1663,1662,3325,0.33110594749450684,0.25928181443968146
1666,1667,1666,3333,0.33150410652160645,0.25762019401499325
1670,1671,1670,3341,0.3319358825683594,0.2559692292127202
1674,1675,1674,3349,0.33245086669921875,0.254328843895258
1678,1679,1678,3357,0.3329341411590576,0.25269896318624735
1682,1683,1682,3365,0.3333399295806885,0.2510795134063772
1686,1687,1686,3373,0.3338310718536377,0.2494704220110485
1690,1691,1690,3381,0.3347928524017334,0.24787161753513767
1694,1695,1694,3389,0.3354480266571045,0.2462830295356894
1698,1699,1698,3397,0.3360569477081299,0.24470458854734342
1702,1703,1702,3405,0.3367750644683838,0.24313622603089824
1706,1707,1706,3413,0.33844709396362305,0.24157787433152117
1710,1711,1710,3421,0.33950185775756836,0.24002946663852884
1714,1715,1714,3429,0.34039998054504395,0.23849093694663498
1718,1719,1718,3437,0.34132909774780273,0.23696222001989195
1722,1723,1722,3445,0.3430299758911133,0.23544325135971833
1726,1727,1726,3453,0.34398603439331055,0.23393396717204468
1730,1731,1730,3461,0.3447299003601074,0.2324343043389616
1734,1735,1734,3469,0.3453538417816162,0.23094420039277883
1738,1739,1738,3477,0.3490898609161377,0.22946359348913323
1742,1743,1742,3485,0.3514058589935303,0.22799242238228737
1746,1747,1746,3493,0.35190296173095703,0.22653062640654165
1750,1751,1750,3501,0.3523728847503662,0.22507814545187088
1754,1755,1754,3509,0.3528721332550049,0.22363491994645804
1758,1759,1758,3517,0.35390305519104004,0.22220089083895964
1762,1763,1762,3525,0.3545799255371094,0.22077599957955477
1766,1767,1766,3533,0.3554558753967285,0.21936018810666394
1770,1771,1770,3541,0.3562040328979492,0.21795339883037854
1774,1775,1774,3549,0.3568379878997803,0.2165555746197254
1778,1779,1778,3557,0.35745906829833984,0.21516665878888755
1782,1783,1782,3565,0.3581089973449707,0.2137865950866935
1786,1787,1786,3573,0.3588130474090576,0.21241532768308144
1790,1791,1790,3581,0.35973286628723145,0.21105280116068337
1794,1795,1794,3589,0.3605830669403076,0.20969896050392267
1798,1799,1798,3597,0.3614010810852051,0.20835375109008858
1802,1803,1802,3605,0.3619821071624756,0.20701711868079578
1806,1807,1806,3613,0.36399292945861816,0.20568900941287416
1810,1811,1810,3621,0.36446189880371094,0.204369369792877
1814,1815,1814,3629,0.3649630546569824,0.20305814668829522
1818,1819,1818,3637,0.3657100200653076,0.20175528732134657
1822,1823,1822,3645,0.36736202239990234,0.2004607392627841
1826,1827,1826,3653,0.36904096603393555,0.19917445042697848
1830,1831,1830,3661,0.3713860511779785,0.19789636906444638
1834,1835,1834,3669,0.37293195724487305,0.19662644375806182
1838,1839,1838,3677,0.37378978729248047,0.1953646234194421
1842,1843,1842,3685,0.37432003021240234,0.19411085728101227
1846,1847,1846,3693,0.37482786178588867,0.19286509489494866
1850,1851,1850,3701,0.3759629726409912,0.1916272861272068
1854,1855,1854,3709,0.3771491050720215,0.19039738115495025
1858,1859,1858,3717,0.3780341148376465,0.18917533046189783
1862,1863,1862,3725,0.37868309020996094,0.187961084835882
1866,1867,1866,3733,0.37943482398986816,0.1867545953650554
1870,1871,1870,3741,0.3802018165588379,0.18555581343442398
1874,1875,1874,3749,0.3821909427642822,0.18436469072484013
1878,1879,1878,3757,0.3830399513244629,0.18318117920739976
1882,1883,1882,3765,0.3835740089416504,0.18200523114327088
1886,1887,1886,3773,0.38660693168640137,0.1808367990805792
1890,1891,1890,3781,0.3893918991088867,0.1796758358506431
1894,1895,1894,3789,0.3903629779815674,0.17852229456838398
1898,1899,1898,3797,0.39112210273742676,0.17737612862696442
1902,1903,1902,3805,0.3922419548034668,0.1762372916990448
1906,1907,1906,3813,0.3932168483734131,0.1751057377316911
1910,1911,1910,3821,0.394212007522583,0.17398142094710808
1914,1915,1914,3829,0.395035982131958,0.17286429583876922
1918,1919,1918,3837,0.39570093154907227,0.17175431717130882
1922,1923,1922,3845,0.39647889137268066,0.17065143997650695
1926,1927,1926,3853,0.3972609043121338,0.16955561955469067
1930,1931,1930,3861,0.39795899391174316,0.1684668114707269
1934,1935,1934,3869,0.3985929489135742,0.16738497155335463
1938,1939,1938,3877,0.40048885345458984,0.1663100558935925
1942,1943,1942,3885,0.40108203887939453,0.16524202084291245
1946,1947,1946,3893,0.40157508850097656,0.1641808230125297
1950,1951,1950,3901,0.4042348861694336,0.1631264192711898
1954,1955,1954,3909,0.4049408435821533,0.1620787667444469
1958,1959,1958,3917,0.405925989151001,0.16103782281293652
1962,1963,1962,3925,0.40648698806762695,0.16000354511118164
1966,1967,1966,3933,0.40700793266296387,0.15897589152512326
1970,1971,1970,3941,0.40753984451293945,0.1579548201936105
1974,1975,1974,3949,0.4081587791442871,0.1569402895038741
1978,1979,1978,3957,0.40901899337768555,0.15593225809320505
1982,1983,1982,3965,0.40958404541015625,0.15493068484442515
1986,1987,1986,3973,0.41016101837158203,0.15393552888869297
1990,1991,1990,3981,0.4108140468597412,0.15294674960008933
1994,1995,1994,3989,0.4114859104156494,0.15196430659765484
1998,1999,1998,3997,0.4120359420776367,0.15098815974326202
2002,2003,2002,4005,0.4126420021057129,0.15001826913856944
2006,2007,2006,4013,0.4130830764770508,0.14905459512680289
2010,2011,2010,4021,0.4144108295440674,0.1480970982893223
2014,2015,2014,4029,0.41656494140625,0.14714573944569345
2018,2019,2018,4037,0.41716694831848145,0.14620047965255906
2022,2023,2022,4045,0.41860294342041016,0.14526128020061538
2026,2027,2026,4053,0.41951513290405273,0.14432810261700776
2030,2031,2030,4061,0.42206287384033203,0.1434009086595875
2034,2035,2034,4069,0.42290592193603516,0.14247966032026865
2038,2039,2038,4077,0.4237940311431885,0.14156431982110032
2042,2043,2042,4085,0.4242820739746094,0.1406548496134976
2046,2047,2046,4093,0.4250028133392334,0.1397512123777541
2050,2051,2050,4101,0.42560815811157227,0.13885337102196652
2054,2055,2054,4109,0.42656707763671875,0.13796128868035998
2058,2059,2058,4117,0.42772698402404785,0.1370749287118399
2062,2063,2062,4125,0.4285099506378174,0.13619425470037239
2066,2067,2066,4133,0.4292418956756592,0.13531923045168096
2070,2071,2070,4141,0.4298851490020752,0.134449819994342
2074,2075,2074,4149,0.43170976638793945,0.13358598757720713
2078,2079,2078,4157,0.432811975479126,0.13272769766822884
2082,2083,2082,4165,0.433596134185791,0.13187491495486833
2086,2087,2086,4173,0.4342508316040039,0.13102760434073518
2090,2091,2090,4181,0.43488597869873047,0.1301857309465068
2094,2095,2094,4189,0.43559694290161133,0.1293492601066908
2098,2099,2098,4197,0.4366590976715088,0.12851815737178057
2102,2103,2102,4205,0.4378509521484375,0.12769238850348363
2106,2107,2106,4213,0.43848586082458496,0.12687191947524565
2110,2111,2110,4221,0.43999290466308594,0.1260567164719452
2114,2115,2114,4229,0.4406120777130127,0.12524674588741183
2118,2119,2118,4237,0.4412698745727539,0.12444197432355229
2122,2123,2122,4245,0.4417870044708252,0.12364236859037966
2126,2127,2126,4253,0.4422750473022461,0.12284789570337942
2130,2131,2130,4261,0.44275403022766113,0.12205852288325895
2134,2135,2134,4269,0.4432528018951416,0.12127421755430087
2138,2139,2138,4277,0.44379591941833496,0.12049494734428673
2142,2143,2142,4285,0.4443490505218506,0.11972068008244575
2146,2147,2146,4293,0.44525694847106934,0.11895138379829265
2150,2151,2150,4301,0.44576597213745117,0.11818702672126884
2154,2155,2154,4309,0.44632577896118164,0.11742757727877677
2158,2159,2158,4317,0.44845104217529297,0.11667300409556132
2162,2163,2162,4325,0.4490480422973633,0.11592327599358612
2166,2167,2166,4333,0.4495887756347656,0.11517836198828098
2170,2171,2170,4341,0.45004892349243164,0.11443823129064833
2174,2175,2174,4349,0.45049595832824707,0.11370285330382658
2178,2179,2178,4357,0.45094990730285645,0.11297219762254944
2182,2183,2182,4365,0.45137977600097656,0.11224623403337082
2186,2187,2186,4373,0.4518239498138428,0.1115249325111409
2190,2191,2190,4381,0.45235395431518555,0.11080826322059237
2194,2195,2194,4389,0.453110933303833,0.11009619651384053
2198,2199,2198,4397,0.4536721706390381,0.10938870292798213
2202,2203,2202,4405,0.45505404472351074,0.10868575318786862
2206,2207,2206,4413,0.4578239917755127,0.1079873182003694
2210,2211,2210,4421,0.45859289169311523,0.10729336905736525
2214,2215,2214,4429,0.45915985107421875,0.10660387703263383
2218,2219,2218,4437,0.4597890377044678,0.10591881358030551
2222,2223,2222,4445,0.4602987766265869,0.10523815033492712
2226,2227,2226,4453,0.4607689380645752,0.10456185911055337
2230,2231,2230,4461,0.46143198013305664,0.10388991189909129
2234,2235,2234,4469,0.46188998222351074,0.10322228086945487
2238,2239,2238,4477,0.46269893646240234,0.10255893836534329
2242,2243,2242,4485,0.46321988105773926,0.10189985690736096
2246,2247,2246,4493,0.46367597579956055,0.1012450091884132
2250,2251,2250,4501,0.46422791481018066,0.10059436807493395
2254,2255,2254,4509,0.4676520824432373,0.09994790660542789
2258,2259,2258,4517,0.470761775970459,0.09930559798760026
2262,2263,2262,4525,0.4753129482269287,0.09866741560121706
2266,2267,2266,4533,0.47766685485839844,0.09803333299300138
2270,2271,2270,4541,0.4788808822631836,0.09740332387822757
2274,2275,2274,4549,0.4804048538208008,0.09677736213876373
2278,2279,2278,4557,0.4823038578033447,0.0961554218225594
2282,2283,2282,4565,0.4842410087585449,0.09553747714170734
2286,2287,2286,4573,0.48531389236450195,0.09492350247202247
2290,2291,2290,4581,0.491225004196167,0.0943134723533625
2294,2295,2294,4589,0.49323415756225586,0.09370736148537931
2298,2299,2298,4597,0.4948880672454834,0.09310514473045498
2302,2303,2302,4605,0.4956240653991699,0.09250679710920602
2306,2307,2306,4613,0.4962730407714844,0.09191229380214622
2310,2311,2310,4621,0.4969758987426758,0.09132161014754012
2314,2315,2314,4629,0.49794507026672363,0.09073472164020316
2318,2319,2318,4637,0.49857592582702637,0.09015160393159118
2322,2323,2322,4645,0.4993860721588135,0.08957223282709839
2326,2327,2326,4653,0.4999070167541504,0.08899658428754491
2330,2331,2330,4661,0.5003819465637207,0.08842463442547563
2334,2335,2334,4669,0.500856876373291,0.08785635950726849
2338,2339,2338,4677,0.5013899803161621,0.08729173594888498
2342,2343,2342,4685,0.5032470226287842,0.08673074031776826
2346,2347,2346,4693,0.5039777755737305,0.08617334933073968
2350,2351,2350,4701,0.5044231414794922,0.08561953985232738
2354,2355,2354,4709,0.5049350261688232,0.08506928889522258
2358,2359,2358,4717,0.5054299831390381,0.08452257361835604
2362,2363,2362,4725,0.5059170722961426,0.08397937132705799
2366,2367,2366,4733,0.5063860416412354,0.08343965947144688
2370,2371,2370,4741,0.5068888664245605,0.08290341564523672
2374,2375,2374,4749,0.5073609352111816,0.08237061758460362
2378,2379,2378,4757,0.5079059600830078,0.08184124316903285
2382,2383,2382,4765,0.509958028793335,0.0813152704191796
2386,2387,2386,4773,0.5105850696563721,0.08079267749561077
2390,2391,2390,4781,0.5111219882965088,0.08027344269847105
2394,2395,2394,4789,0.5116598606109619,0.07975754446682569
2398,2399,2398,4797,0.5121550559997559,0.07924496137745278
2402,2403,2402,4805,0.5127608776092529,0.07873567214441106
2406,2407,2406,4813,0.5132420063018799,0.07822965561691857
2410,2411,2410,4821,0.5137529373168945,0.07772689078044429
2414,2415,2414,4829,0.5143280029296875,0.07722735675460618
2418,2419,2418,4837,0.514826774597168,0.0767310327916241
2422,2423,2422,4845,0.5153241157531738,0.07623789827820189
2426,2427,2426,4853,0.5158817768096924,0.0757479327319588
2430,2431,2430,4861,0.5164980888366699,0.07526111580066158
2434,2435,2434,4869,0.5170688629150391,0.07477742726414573
2438,2439,2438,4877,0.5191121101379395,0.07429684703057766
2442,2443,2442,4885,0.5198090076446533,0.07381935513682207
2446,2447,2446,4893,0.5210490226745605,0.07334493174752646
2450,2451,2450,4901,0.5228121280670166,0.07287355715427982
2454,2455,2454,4909,0.5234649181365967,0.07240521177531445
2458,2459,2458,4917,0.5243649482727051,0.07193987615422008
2462,2463,2462,4925,0.5250759124755859,0.07147753095881654
2466,2467,2466,4933,0.5257000923156738,0.07101815698061509
2470,2471,2470,4941,0.5264737606048584,0.0705617351345886
2474,2475,2474,4949,0.529433012008667,0.070108246458183
2478,2479,2478,4957,0.5306239128112793,0.06965767210914796
2482,2483,2482,4965,0.5312018394470215,0.06920999336746454
2486,2487,2486,4973,0.5320439338684082,0.0687651916323492
2490,2491,2490,4981,0.5326859951019287,0.068323248422401
2494,2495,2494,4989,0.5335378646850586,0.06788414537415684
2498,2499,2498,4997,0.5340840816497803,0.06744786424224093
2503,2504,2503,5007,0.5350749492645264,0.06690645354116886
2507,2508,2507,5015,0.5355818271636963,0.06647645561647983
2511,2512,2511,5023,0.5377969741821289,0.06604922111438438
2515,2516,2515,5031,0.5384328365325928,0.06562473228212844
2519,2520,2519,5039,0.5395071506500244,0.06520297147997187
2523,2524,2523,5047,0.5400490760803223,0.06478392118093909
2527,2528,2527,5055,0.5408380031585693,0.06436756397147202
2531,2532,2531,5063,0.5414609909057617,0.06395388254896409
2535,2536,2535,5071,0.5425469875335693,0.06354285972207524
2539,2540,2539,5079,0.5431079864501953,0.06313447841008506
2543,2544,2543,5087,0.5437428951263428,0.06272872164060224
2547,2548,2547,5095,0.5446319580078125,0.062325572551096234
2551,2552,2551,5103,0.5453190803527832,0.06192501438757186
2555,2556,2555,5111,0.5458409786224365,0.06152703050253078
2559,2560,2559,5119,0.546950101852417,0.06113160435587208
2563,2564,2563,5127,0.5480349063873291,0.06073871951328228
2567,2568,2567,5135,0.5485098361968994,0.06034835964644191
2571,2572,2571,5143,0.5491559505462646,0.05996050853105337
2575,2576,2575,5151,0.549656867980957,0.059575150047559575
2579,2580,2579,5159,0.5502228736877441,0.05919226817995475
2583,2584,2583,5167,0.5506429672241211,0.05881184701379559
2587,2588,2587,5175,0.5511348247528076,0.05843387073850857
2591,2592,2591,5183,0.5515601634979248,0.05805832364400515
2595,2596,2595,5191,0.552191972732544,0.05768519012085101
2599,2600,2599,5199,0.5527300834655762,0.05731445466023477
2603,2604,2603,5207,0.5532469749450684,0.05694610185299025
2607,2608,2607,5215,0.554002046585083,0.056580116388344814
2611,2612,2611,5223,0.554542064666748,0.056216483054771595
2615,2616,2615,5231,0.5552408695220947,0.055855186736827045
2619,2620,2619,5239,0.5557301044464111,0.055496212418130804
2623,2624,2623,5247,0.5561890602111816,0.055139545176424394
2627,2628,2627,5255,0.5566449165344238,0.054785170187407854
2631,2632,2631,5263,0.5571281909942627,0.05443307272035289
2635,2636,2635,5271,0.5575978755950928,0.05408323814067652
2639,2640,2639,5279,0.5579988956451416,0.05373565190564457
2643,2644,2643,5287,0.5584690570831299,0.05339029956762315
2647,2648,2647,5295,0.5589230060577393,0.053047166771540616
2651,2652,2651,5303,0.5594568252563477,0.05270623925353253
2655,2656,2655,5311,0.560621976852417,0.052367502842893494
2659,2660,2659,5319,0.5617749691009521,0.05203094345832344
2663,2664,2663,5327,0.56227707862854,0.05169654710978734
2667,2668,2667,5335,0.562856912612915,0.05136429989680391
2671,2672,2671,5343,0.5632610321044922,0.051034188008792045
2675,2676,2675,5351,0.563784122467041,0.05070619772285227
2679,2680,2679,5359,0.5641829967498779,0.050380315404790876
2683,2684,2683,5367,0.5645890235900879,0.0500565275085795
2687,2688,2687,5375,0.5650510787963867,0.04973482057392071
2691,2692,2691,5383,0.5657439231872559,0.049415181227776286
2695,2696,2695,5391,0.5664448738098145,0.04909759618287368
2699,2700,2699,5399,0.5674099922180176,0.048782052237201314
2703,2704,2703,5407,0.568317174911499,0.0484685362735265
2707,2708,2707,5415,0.5691177845001221,0.04815703525910831
2711,2712,2711,5423,0.5696721076965332,0.04784753624435417
2715,2716,2715,5431,0.5700960159301758,0.047540026364038215
2719,2720,2719,5439,0.5708639621734619,0.04723449283394639
2723,2724,2723,5447,0.5714578628540039,0.04693092295354268
2727,2728,2727,5455,0.5721209049224854,0.046629304102730265
2731,2732,2731,5463,0.5731790065765381,0.04632962374290723
2735,2736,2735,5471,0.5737528800964355,0.0460318694164518
2739,2740,2739,5479,0.574321985244751,0.04573602874445909
2743,2744,2743,5487,0.5749459266662598,0.045442089429233466
2747,2748,2747,5495,0.5755171775817871,0.0451500392513484
2751,2752,2751,5503,0.5778720378875732,0.04485986606959038
2755,2756,2755,5511,0.5783870220184326,0.044571557820671494
2759,2760,2759,5519,0.5789580345153809,0.04428510251991772
2763,2764,2763,5527,0.5796248912811279,0.04400048825823924
2767,2768,2767,5535,0.5802018642425537,0.043717703203816884
2771,2772,2771,5543,0.5807111263275146,0.04343673560046185
2775,2776,2775,5551,0.581183910369873,0.04315757376807334
2779,2780,2779,5559,0.5819261074066162,0.04288020610165274
2783,2784,2783,5567,0.5839929580688477,0.042604621069695904
2787,2788,2787,5575,0.5846388339996338,0.04233080721607541
2791,2792,2791,5583,0.5850729942321777,0.042058753157068314
2795,2796,2795,5591,0.5856280326843262,0.041788447583054174
2799,2800,2799,5599,0.586061954498291,0.04151987925711527
2803,2804,2803,5607,0.5869410037994385,0.04125303701321092
2807,2808,2807,5615,0.5875470638275146,0.0409879097591279
2811,2812,2811,5623,0.588148832321167,0.040724486472290725
2815,2816,2815,5631,0.5893499851226807,0.040462756201448416
2819,2820,2819,5639,0.5899240970611572,0.040202708065401126
2823,2824,2823,5647,0.5908818244934082,0.03994433125380305
2827,2828,2827,5655,0.5919249057769775,0.039687615024603023
2831,2832,2831,5663,0.5939130783081055,0.03943254870611054
2835,2836,2835,5671,0.5952529907226562,0.0391791216934485
2839,2840,2839,5679,0.5962221622467041,0.038927323451618645
2843,2844,2843,5687,0.5979049205780029,0.03867714351231007
2847,2848,2847,5695,0.5986490249633789,0.03842857147498952
2851,2852,2851,5703,0.5992469787597656,0.038181597005524474
2855,2856,2855,5711,0.5998177528381348,0.037936209836125105
2859,2860,2859,5719,0.6002829074859619,0.03769239976539099
2863,2864,2863,5727,0.6007001399993896,0.03745015665797693
2867,2868,2867,5735,0.6020798683166504,0.03720947044174804
2871,2872,2871,5743,0.6027910709381104,0.03697033111189857
2875,2876,2875,5751,0.6032359600067139,0.0367327287255243
2879,2880,2879,5759,0.6037158966064453,0.0364966534053401
2883,2884,2883,5767,0.6041970252990723,0.036262095336248995
2887,2888,2887,5775,0.604701042175293,0.036029044767878195
2891,2892,2891,5783,0.6051549911499023,0.035797492010091546
2895,2896,2895,5791,0.6056721210479736,0.03556742743790119
2899,2900,2899,5799,0.6062109470367432,0.035338841485442876
2903,2904,2903,5807,0.6071667671203613,0.035111724650290825
2907,2908,2907,5815,0.6076469421386719,0.03488606748993428
2911,2912,2911,5823,0.6091780662536621,0.03466186062364821
2915,2916,2915,5831,0.610090970993042,0.034439094729508506
2919,2920,2919,5839,0.6107089519500732,0.03421776054660845
2923,2924,2923,5847,0.6113471984863281,0.03399784887382974
2927,2928,2927,5855,0.6119449138641357,0.033779350567914
2931,2932,2931,5863,0.6125190258026123,0.03356225654492072
2935,2936,2935,5871,0.6129469871520996,0.03334655778029662
2939,2940,2939,5879,0.6134328842163086,0.03313224530599332
2943,2944,2943,5887,0.6139109134674072,0.032919310212305
2947,2948,2947,5895,0.614569902420044,0.032707743646961426
2951,2952,2951,5903,0.6149909496307373,0.032497536814036894
2955,2956,2955,5911,0.6171848773956299,0.03228868097444443
2959,2960,2959,5919,0.6176609992980957,0.03208116744516638
2963,2964,2963,5927,0.6183860301971436,0.03187498759939177
2967,2968,2967,5935,0.618959903717041,0.03167013286556535
2971,2972,2971,5943,0.6194729804992676,0.031466594726454876
2975,2976,2975,5951,0.6199541091918945,0.03126436472076119
2979,2980,2979,5959,0.6207478046417236,0.03106343444088875
2983,2984,2983,5967,0.6217589378356934,0.03086379553292434
2987,2988,2987,5975,0.6225178241729736,0.030665439697670282
2991,2992,2991,5983,0.6231169700622559,0.030468358688576485
2995,2996,2995,5991,0.6236450672149658,0.030272544312178396
2999,3000,2999,5999,0.6244378089904785,0.03007798842722398
3003,3004,3003,6007,0.6255037784576416,0.029884682946028605
3007,3008,3007,6015,0.6260771751403809,0.029692619831879753
3011,3012,3011,6023,0.6266500949859619,0.029501791099887636
3015,3016,3015,6031,0.6271500587463379,0.029312188816285008
3019,3020,3019,6039,0.6277270317077637,0.029123805099251457
3023,3024,3023,6047,0.6282138824462891,0.028936632116472374
3027,3028,3027,6055,0.6287598609924316,0.028750662086294475
3031,3032,3031,6063,0.6291928291320801,0.028565887277522555
3035,3036,3035,6071,0.6299710273742676,0.028382300008508353
3039,3040,3039,6079,0.632314920425415,0.028199892646168383
3043,3044,3043,6087,0.632796049118042,0.028018657607587105
3047,3048,3047,6095,0.6333439350128174,0.02783858735817077
3051,3052,3051,6103,0.6338951587677002,0.027659674411922065
3055,3056,3055,6111,0.6344280242919922,0.02748191132973143
3059,3060,3059,6119,0.6350040435791016,0.02730529072280552
3063,3064,3063,6127,0.6356220245361328,0.027129805246703914
3067,3068,3067,6135,0.6361339092254639,0.026955447607347235
3071,3072,3071,6143,0.636652946472168,0.02678221055480195
3075,3076,3075,6151,0.6375110149383545,0.0266100868877643
3079,3080,3079,6159,0.6382489204406738,0.02643906944987764
3083,3084,3083,6167,0.6390807628631592,0.026269151131499406
3087,3088,3087,6175,0.6397778987884521,0.026100324868645282
3091,3092,3091,6183,0.6409168243408203,0.02593258364212947
3095,3096,3095,6191,0.642064094543457,0.025765920478698832
3099,3100,3099,6199,0.6425659656524658,0.025600328449551554
3103,3104,3103,6207,0.6433048248291016,0.025435800669815826
3107,3108,3107,6215,0.6439309120178223,0.025272330300364944
3111,3112,3111,6223,0.6447179317474365,0.025109910544599243
3115,3116,3115,6231,0.645845890045166,0.024948534649947333
3119,3120,3119,6239,0.6464889049530029,0.024788195907532652
3123,3124,3123,6247,0.6473848819732666,0.024628887651658157
3127,3128,3127,6255,0.6479299068450928,0.024470603259128584
3131,3132,3131,6263,0.6492359638214111,0.024313336149639847
3135,3136,3135,6271,0.6497268676757812,0.02415707978491894
3139,3140,3139,6279,0.6500940322875977,0.024001827668771864
3143,3144,3143,6287,0.6505889892578125,0.023847573346884497
3147,3148,3147,6295,0.6510100364685059,0.02369431040602178
3151,3152,3151,6303,0.6514301300048828,0.02354203247513928
3155,3156,3155,6311,0.6518309116363525,0.023390733222700667
3159,3160,3159,6319,0.6522419452667236,0.023240406359360158
3163,3164,3163,6327,0.6526648998260498,0.023091045634739456
3167,3168,3167,6335,0.6531538963317871,0.02294264484004006
3171,3172,3171,6343,0.6535539627075195,0.02279519780537801
3175,3176,3175,6351,0.6539490222930908,0.022648698400634305
3179,3180,3179,6359,0.6544759273529053,0.02250314053609398
3183,3184,3183,6367,0.6555459499359131,0.022358518159583944
3187,3188,3187,6375,0.6567349433898926,0.022214825259149886
3191,3192,3191,6383,0.6572320461273193,0.022072055860160873
3195,3196,3195,6391,0.6576318740844727,0.021930204028582687
3199,3200,3199,6399,0.658052921295166,0.02178926386583703
3203,3204,3203,6407,0.6585168838500977,0.021649229513020403
3207,3208,3207,6415,0.6589829921722412,0.021510095148855393
3211,3212,3211,6423,0.6594557762145996,0.021371854988457683
3215,3216,3215,6431,0.6599390506744385,0.021234503284420787
3219,3220,3219,6439,0.660689115524292,0.021098034327645905
3223,3224,3223,6447,0.6611208915710449,0.020962442443445594
3227,3228,3227,6455,0.6616799831390381,0.020827721995698892
3231,3232,3231,6463,0.6622538566589355,0.020693867383322066
3235,3236,3235,6471,0.6628341674804688,0.020560873041642194
3239,3240,3239,6479,0.6633551120758057,0.020428733441023465
3243,3244,3243,6487,0.6638062000274658,0.020297443088674205
3247,3248,3247,6495,0.6642000675201416,0.020166996525961767
3251,3252,3251,6503,0.6646559238433838,0.02003738833017532
3255,3256,3255,6511,0.6651418209075928,0.01990861311299273
3259,3260,3259,6519,0.6657488346099854,0.019780665520809638
3263,3264,3263,6527,0.6662890911102295,0.01965354023373255
3267,3268,3267,6535,0.6667947769165039,0.019527231967778225
3271,3272,3271,6543,0.6675307750701904,0.01940173547141502
3275,3276,3275,6551,0.6679999828338623,0.019277045527069575
3279,3280,3279,6559,0.6700019836425781,0.019153156951382637
3283,3284,3283,6567,0.671022891998291,0.019030064594086828
3287,3288,3287,6575,0.671666145324707,0.018907763337028795
3291,3292,3291,6583,0.6721539497375488,0.01878624809637969
3295,3296,3295,6591,0.6727759838104248,0.018665513820695794
3299,3300,3299,6599,0.6732268333435059,0.018545555489905323
3303,3304,3303,6607,0.6738300323486328,0.018426368117514143
3307,3308,3307,6615,0.674278974533081,0.018307946748278278
3311,3312,3311,6623,0.6750590801239014,0.01819028645870106
3315,3316,3315,6631,0.6755490303039551,0.018073382357973247
3319,3320,3319,6639,0.6761131286621094,0.017957229585572793
3323,3324,3323,6647,0.6767899990081787,0.017841823312740205
3327,3328,3327,6655,0.6784417629241943,0.017727158742102584
3331,3332,3331,6663,0.6788730621337891,0.017613231105934168
3335,3336,3335,6671,0.6796159744262695,0.017500035668522602
3339,3340,3339,6679,0.6802568435668945,0.017387567723924
3343,3344,3343,6687,0.6808819770812988,0.017275822596037358
3347,3348,3347,6695,0.6812949180603027,0.017164795639956276
3351,3352,3351,6703,0.6817519664764404,0.017054482239288155
3355,3356,3355,6711,0.6825368404388428,0.016944877808715095
3359,3360,3359,6719,0.6831448078155518,0.01683597779092987
3363,3364,3363,6727,0.6836230754852295,0.016727777659048728
3367,3368,3367,6735,0.686161994934082,0.016620272915029936
3371,3372,3371,6743,0.6869080066680908,0.016513459088974846
3375,3376,3375,6751,0.6900119781494141,0.01640733174103471
3379,3380,3379,6759,0.6909878253936768,0.016301886458880754
3383,3384,3383,6767,0.6915419101715088,0.016197118858445644
3387,3388,3387,6775,0.6921019554138184,0.016093024584877207
3391,3392,3391,6783,0.6926708221435547,0.015989599310551623
3395,3396,3395,6791,0.6931791305541992,0.015886838735642533
3399,3400,3399,6799,0.6936941146850586,0.015784738587995718
3403,3404,3403,6807,0.6942451000213623,0.015683294623472784
3407,3408,3407,6815,0.694861888885498,0.015582502624403907
3411,3412,3411,6823,0.6963968276977539,0.0154823584003159
3415,3416,3415,6831,0.6969079971313477,0.01538285778860801
3419,3420,3419,6839,0.697627067565918,0.015283996652110384
3423,3424,3423,6847,0.6981539726257324,0.015185770881564293
3427,3428,3427,6855,0.6987481117248535,0.01508817639285073
3431,3432,3431,6863,0.6992087364196777,0.014991209129188348
3435,3436,3435,6871,0.7012038230895996,0.014894865059181247
3439,3440,3439,6879,0.7017130851745605,0.014799140177223905
3443,3444,3443,6887,0.7021548748016357,0.014704030504834618
3447,3448,3447,6895,0.7026100158691406,0.01460953208666446
3451,3452,3451,6903,0.7032380104064941,0.014515640995193785
3455,3456,3455,6911,0.703711986541748,0.014422353326456416
3459,3460,3459,6919,0.7049829959869385,0.014329665202740897
3463,3464,3463,6927,0.7055509090423584,0.014237572770654025
3467,3468,3467,6935,0.7060787677764893,0.014146072201400796
3471,3472,3471,6943,0.7066619396209717,0.014055159691614427
3475,3476,3475,6951,0.7070958614349365,0.01396483146126848
3479,3480,3479,6959,0.7075691223144531,0.013875083755168636
3483,3484,3483,6967,0.7080228328704834,0.013785912842843825
3487,3488,3487,6975,0.7085118293762207,0.013697315017190072
3491,3492,3491,6983,0.7089860439300537,0.013609286594541185
3495,3496,3495,6991,0.7105848789215088,0.013521823915505946
3499,3500,3499,6999,0.7111551761627197,0.01343492334396674
3504,3505,3504,7009,0.7119128704071045,0.013327082592135234
3508,3509,3508,7017,0.7124509811401367,0.013241433589411999
3512,3513,3512,7025,0.7129108905792236,0.013156335037610585
3516,3517,3516,7033,0.7133510112762451,0.013071783399396493
3520,3521,3520,7041,0.7138779163360596,0.01298777515962672
3524,3525,3524,7049,0.7144670486450195,0.01290430682575357
3528,3529,3528,7057,0.7161300182342529,0.0128213749276769
3532,3533,3532,7065,0.7165710926055908,0.01273897601784292
3536,3537,3536,7073,0.717033863067627,0.012657106671222187
3540,3541,3540,7081,0.7177808284759521,0.012575763483597843
3544,3545,3544,7089,0.7184679508209229,0.012494943073796463
3548,3549,3548,7097,0.7197248935699463,0.012414642081698414
3552,3553,3552,7105,0.7206919193267822,0.012334857169007405
3556,3557,3556,7113,0.7213249206542969,0.012255585019213122
3560,3561,3560,7121,0.7221038341522217,0.01217682233677683
3564,3565,3564,7129,0.7229108810424805,0.012098565846944256
3568,3569,3568,7137,0.7235438823699951,0.012020812296659312
3572,3573,3572,7145,0.7242698669433594,0.011943558453519588
3576,3577,3576,7153,0.7248349189758301,0.011866801106023356
3580,3581,3580,7161,0.7253289222717285,0.011790537063112802
3584,3585,3584,7169,0.727341890335083,0.011714763154446169
3588,3589,3588,7177,0.7281241416931152,0.011639476229813404
3592,3593,3592,7185,0.7287662029266357,0.011564673159178586
3596,3597,3596,7193,0.7292490005493164,0.011490350832977933
3600,3601,3600,7201,0.7299680709838867,0.011416506161994855
3604,3605,3604,7209,0.7322380542755127,0.011343136075926945
3608,3609,3608,7217,0.7327959537506104,0.011270237524470053
3612,3613,3612,7225,0.7335889339447021,0.011197807477196165
3616,3617,3616,7233,0.734529972076416,0.01112584292325243
3620,3621,3620,7241,0.7351100444793701,0.011054340870728657
3624,3625,3624,7249,0.7356340885162354,0.010983298347454522
3628,3629,3628,7257,0.7365238666534424,0.010912712399348086
3632,3633,3632,7265,0.7371959686279297,0.010842580093029066
3636,3637,3636,7273,0.7381389141082764,0.010772898511971427
3640,3641,3640,7281,0.738853931427002,0.010703664759797275
3644,3645,3644,7289,0.7395150661468506,0.010634875958824189
3648,3649,3648,7297,0.7401609420776367,0.010566529248524964
3652,3653,3652,7305,0.7406740188598633,0.010498621788208139
3656,3657,3656,7313,0.7426700592041016,0.010431150754632367
3660,3661,3660,7321,0.7433550357818604,0.010364113342698203
3664,3665,3664,7329,0.7442779541015625,0.010297506765842844
3668,3669,3668,7337,0.7449090480804443,0.010231328255089716
3672,3673,3672,7345,0.7455258369445801,0.010165575059197879
3676,3677,3676,7353,0.7461569309234619,0.010100244444623999
3680,3681,3680,7361,0.7485458850860596,0.010035333695489162
3684,3685,3684,7369,0.7492649555206299,0.009970840113560458
3688,3689,3688,7377,0.7499759197235107,0.009906761017566419
3692,3693,3692,7385,0.7505021095275879,0.009843093743498057
3696,3697,3696,7393,0.7511188983917236,0.00977983564474486
3700,3701,3700,7401,0.7515549659729004,0.009716984091728876
3704,3705,3704,7409,0.7520408630371094,0.009654536471385065
3708,3709,3708,7417,0.7525439262390137,0.009592490187593434
3712,3713,3712,7425,0.7531759738922119,0.00953084266107071
3716,3717,3716,7433,0.7536699771881104,0.00946959132943168
3720,3721,3720,7441,0.7542591094970703,0.009408733645494273
3724,3725,3724,7449,0.7548210620880127,0.009348267080141803
3728,3729,3728,7457,0.7555711269378662,0.009288189119172412
3732,3733,3732,7465,0.7561159133911133,0.009228497265499293
3736,3737,3736,7473,0.7569839954376221,0.009169189037729343
3740,3741,3740,7481,0.7580358982086182,0.009110261969207587
3744,3745,3744,7489,0.7585630416870117,0.009051713611686194
3748,3749,3748,7497,0.7590789794921875,0.008993541529732267
3752,3753,3752,7505,0.7595088481903076,0.008935743306803795
3756,3757,3756,7513,0.7600197792053223,0.008878316538772638
3760,3761,3760,7521,0.7605648040771484,0.008821258838932663
3764,3765,3764,7529,0.761091947555542,0.008764567835068604
3768,3769,3768,7537,0.761512041091919,0.00870824117081753
3772,3773,3772,7545,0.7628319263458252,0.008652276504112584
3776,3777,3776,7553,0.7641189098358154,0.00859667150863377
3780,3781,3780,7561,0.7647089958190918,0.008541423872763793
3784,3785,3784,7569,0.7652449607849121,0.008486531299953788
3788,3789,3788,7577,0.765841007232666,0.008431991508293112
3792,3793,3792,7585,0.7663819789886475,0.008377802230095667
3796,3797,3796,7593,0.7681918144226074,0.008323961213127798
3800,3801,3800,7601,0.7694239616394043,0.008270466218584413
3804,3805,3804,7609,0.7716331481933594,0.008217315023094543
3808,3809,3808,7617,0.7724928855895996,0.008164505417070103
3812,3813,3812,7625,0.7732677459716797,0.008112035205259873
3816,3817,3816,7633,0.7738111019134521,0.008059902205682654
3820,3821,3820,7641,0.7744290828704834,0.008008104251572721
3824,3825,3824,7649,0.7753100395202637,0.007956639189853003
3828,3829,3828,7657,0.7769310474395752,0.007905504880851818
3832,3833,3832,7665,0.7784779071807861,0.007854699199204828
3836,3837,3836,7673,0.7800118923187256,0.007804220031991777
3840,3841,3840,7681,0.7807090282440186,0.00775406528145514
3844,3845,3844,7689,0.7812650203704834,0.007704232862523071
3848,3849,3848,7697,0.7839980125427246,0.007654720703623676
3852,3853,3852,7705,0.7845289707183838,0.007605526745976502
3856,3857,3856,7713,0.7852001190185547,0.007556648945126575
3860,3861,3860,7721,0.7859060764312744,0.007508085269063343
3864,3865,3864,7729,0.7882997989654541,0.007459833698578979
3868,3869,3868,7737,0.7891759872436523,0.007411892228319841
3872,3873,3872,7745,0.7898459434509277,0.007364258864886764
3876,3877,3876,7753,0.7903027534484863,0.007316931628308851
3880,3881,3880,7761,0.7910709381103516,0.007269908551165236
3884,3885,3884,7769,0.7918910980224609,0.007223187678916693
3888,3889,3888,7777,0.7950990200042725,0.007176767068469503
3892,3893,3892,7785,0.7962448596954346,0.007130644791356951
3896,3897,3896,7793,0.7968831062316895,0.007084818929144193
3900,3901,3900,7801,0.7989940643310547,0.007039287577013009
3904,3905,3904,7809,0.7994248867034912,0.006994048842453964
3908,3909,3908,7817,0.7999138832092285,0.00694910084471216
3912,3913,3912,7825,0.8003509044647217,0.006904441715593747
3916,3917,3916,7833,0.8008780479431152,0.006860069598086546
3920,3921,3920,7841,0.801367998123169,0.006815982647528443
3924,3925,3924,7849,0.8018548488616943,0.006772179031765711
3928,3929,3928,7857,0.8024020195007324,0.006728656929584978
3932,3933,3932,7865,0.8028628826141357,0.006685414531643812
3936,3937,3936,7873,0.8034100532531738,0.006642450040260595
3940,3941,3940,7881,0.8039331436157227,0.006599761669990163
3944,3945,3944,7889,0.804405927658081,0.006557347645148018
3948,3949,3948,7897,0.8049619197845459,0.006515206203413191
3952,3953,3952,7905,0.8055860996246338,0.006473335592256027
3956,3957,3956,7913,0.8061738014221191,0.006431734071895598
3960,3961,3960,7921,0.8068158626556396,0.006390399912153385
3964,3965,3964,7929,0.8073649406433105,0.006349331395672245
3968,3969,3968,7937,0.8079419136047363,0.006308526814406099
3972,3973,3972,7945,0.8085780143737793,0.006267984472169173
3976,3977,3976,7953,0.8091728687286377,0.0062277026837764616
3980,3981,3980,7961,0.8097398281097412,0.0061876797745790335
3984,3985,3984,7969,0.8102009296417236,0.006147914081388676
3988,3989,3988,7977,0.8107030391693115,0.006108403950004827
3992,3993,3992,7985,0.8123149871826172,0.0060691477384105475
3996,3997,3996,7993,0.8130199909210205,0.006030143815382422
4000,4001,4000,8001,0.8135027885437012,0.005991390558725566


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n100/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00021386146545410156,1624.447741208611
1,4,4,8,0.0006029605865478516,1332.3408024303455
2,8,8,16,0.0016217231750488281,946.088855039766
3,12,12,24,0.0023679733276367188,1048.4445827706136
4,14,14,28,0.0027930736541748047,700.8173612812878
5,18,18,36,0.0035610198974609375,374.0520303968597
6,20,20,40,0.0040547847747802734,363.80259197800035
7,26,26,52,0.005124807357788086,268.3075638288215
8,30,30,60,0.005939006805419922,254.22324001709478
9,36,36,72,0.006865978240966797,238.01529429042202
10,42,42,84,0.007664918899536133,209.92580578584443
11,50,50,100,0.008615970611572266,185.20198181997657
12,58,58,116,0.011673927307128906,184.68000690015896
13,66,66,132,0.01262974739074707,180.15955022740363
14,74,74,148,0.013566970825195312,175.92814377228046
15,82,82,164,0.014426946640014648,161.5227899951169
16,90,90,180,0.015360116958618164,159.6240688022446
17,96,96,192,0.01619577407836914,172.05406464160546
18,102,102,204,0.016971826553344727,156.9859077757749
19,110,110,220,0.018186092376708984,136.68764642330362
20,118,118,236,0.019320964813232422,135.42950475530338
21,126,126,252,0.02074289321899414,134.3453868940889
22,134,134,268,0.0220949649810791,125.23053712345713
23,142,142,284,0.02314591407775879,123.6218509878528
24,150,150,300,0.026421785354614258,122.3053119060085
25,158,158,316,0.027647972106933594,121.16241464860279
26,166,166,332,0.028783798217773438,120.16601216249201
27,174,174,348,0.030184030532836914,119.29269567003288
28,182,182,364,0.031610965728759766,118.52238313899163
29,190,190,380,0.03269696235656738,117.83792649180641
30,198,198,396,0.034149885177612305,117.22474500544486
31,206,206,412,0.03567910194396973,110.74853334384088
32,214,214,428,0.03830289840698242,109.97759630554185
33,222,222,444,0.039758920669555664,109.28987583764722
34,230,230,460,0.04269289970397949,108.67238186157404
35,238,238,476,0.04396867752075195,108.11395150423476
36,246,246,492,0.044943809509277344,107.60502473099753
37,254,254,508,0.045886993408203125,107.1374402288755
38,262,262,524,0.04764080047607422,106.70425172116786
39,270,270,540,0.04916787147521973,106.29956416908547
40,278,278,556,0.05014204978942871,105.91838882463065
41,286,286,572,0.05122494697570801,105.5565157951386
42,294,294,588,0.05233287811279297,105.21040261936378
43,302,302,604,0.05371689796447754,104.87707729971883
44,310,310,620,0.054892778396606445,104.55405425373888
45,318,318,636,0.056114912033081055,102.23428262310215
46,326,326,652,0.05926680564880371,97.85112401895425
47,334,334,668,0.060440778732299805,97.45519979669801
48,342,342,684,0.061548709869384766,97.08290543723847
49,350,350,700,0.062486886978149414,96.73050757860472
50,358,358,716,0.06377100944519043,93.21567618825011
51,366,366,732,0.06463384628295898,92.70678973892663
52,374,374,748,0.06580996513366699,92.32081952456242
53,382,382,764,0.06677103042602539,91.95833157814324
54,390,390,780,0.06774783134460449,91.61578097635804
55,398,398,796,0.06878399848937988,91.29010483392668
56,406,406,812,0.06981301307678223,90.97866254017157
57,414,414,828,0.07374787330627441,90.67918256321833
58,422,422,844,0.07482099533081055,90.38971528145184
59,430,430,860,0.07585787773132324,90.10859129899255
60,438,438,876,0.07684683799743652,89.83438471528343
61,446,446,892,0.07786774635314941,89.56588084316704
62,454,454,908,0.07880496978759766,89.30204790120438
63,462,462,924,0.08016586303710938,89.04201224119419
64,470,470,940,0.08130478858947754,88.78503670876194
65,478,478,956,0.0824117660522461,88.53050177187912
66,486,486,972,0.08352375030517578,88.27788908804094
67,494,494,988,0.08450698852539062,88.0267672149437
68,502,502,1004,0.0889427661895752,87.77677920136175
69,510,510,1020,0.08992290496826172,87.52763182429098
70,518,518,1036,0.0908968448638916,87.27908626526333
71,526,526,1052,0.09190201759338379,87.03095004297649
72,534,534,1068,0.09295082092285156,86.7830700412778
73,542,542,1084,0.09395289421081543,86.53532649103141
74,550,550,1100,0.09501194953918457,86.28762778178728
75,558,558,1116,0.09595775604248047,86.03990599464616
76,566,566,1132,0.09701299667358398,85.79211306128495
77,574,574,1148,0.09802079200744629,85.54421746620257
78,582,582,1164,0.09932804107666016,81.61868393807545
79,590,590,1180,0.10084271430969238,80.67673255421042
80,598,598,1196,0.10206079483032227,80.42974323347462
81,606,606,1212,0.10344195365905762,80.18723339704606
82,614,614,1228,0.10445380210876465,76.51970647608681
83,622,622,1244,0.10542488098144531,76.23100554867823
84,630,630,1260,0.10632205009460449,75.95398453689943
85,638,638,1276,0.10727787017822266,75.687155082936
86,646,646,1292,0.1082918643951416,70.80381930479876
87,654,654,1308,0.10928583145141602,70.42952135489813
88,662,662,1324,0.11028003692626953,70.07673564499059
89,668,668,1336,0.11113572120666504,63.470895566119786
90,676,676,1352,0.11206889152526855,56.15538941258864
91,684,684,1368,0.11428189277648926,40.663914927846946
92,692,692,1384,0.11569786071777344,40.538488590865356
93,700,700,1400,0.11683988571166992,40.4134105483917
94,706,706,1412,0.11791491508483887,36.671129081323635
95,714,714,1428,0.11887288093566895,36.560038629947364
96,722,722,1444,0.11977577209472656,36.44919563530819
97,730,730,1460,0.12091302871704102,36.33860206176196
98,738,738,1476,0.12218189239501953,36.22825996199132
99,746,746,1492,0.12328100204467773,36.11817145069235
100,754,754,1508,0.12441611289978027,36.00833868161398
101,762,762,1524,0.12558293342590332,35.898763827561915
102,770,770,1540,0.12816286087036133,31.904821760967362
103,778,778,1556,0.12942290306091309,29.407113843660866
104,786,786,1572,0.1304337978363037,29.247468350489108
105,794,794,1588,0.13149094581604004,29.09331527544887
106,802,802,1604,0.13263583183288574,28.944275274016324
107,810,810,1620,0.13396000862121582,28.799996675279427
108,818,818,1636,0.13477492332458496,28.660153541506467
109,826,826,1652,0.136185884475708,28.524443845986042
110,834,834,1668,0.13741803169250488,28.392587764777122
111,842,842,1684,0.13862204551696777,28.264326077731372
112,850,850,1700,0.1398627758026123,28.139418673911596
113,858,858,1716,0.14254093170166016,28.017643156417325
114,866,866,1732,0.1444697380065918,27.898793541570505
115,874,874,1748,0.14556598663330078,27.782679047391927
116,882,882,1764,0.14654183387756348,27.669122966404338
117,890,890,1780,0.1476140022277832,27.55796161785389
118,898,898,1796,0.14864683151245117,27.449043374553664
119,906,906,1812,0.14955496788024902,27.342227759759172
120,914,914,1828,0.15057587623596191,27.23738460961745
121,922,922,1844,0.1515820026397705,27.134393296910126
122,930,930,1860,0.1524968147277832,26.543020684393106
123,938,938,1876,0.1535639762878418,25.397633339919985
124,946,946,1892,0.15552806854248047,25.324827743720622
125,954,954,1908,0.15741491317749023,25.252188383582858
126,960,960,1920,0.15827679634094238,22.533039587678186
127,968,968,1936,0.15924286842346191,21.60176690056621
128,976,976,1952,0.16016483306884766,21.53333302406177
129,984,984,1968,0.1618208885192871,21.46582382585808
130,990,990,1980,0.1624767780303955,19.474369846681316
131,998,998,1996,0.16360688209533691,19.41451990043444
132,1006,1006,2012,0.16463279724121094,19.355361743953548
133,1014,1014,2028,0.16561174392700195,19.29685151762185
134,1022,1022,2044,0.1666257381439209,19.238948494712307
135,1030,1030,2060,0.16760683059692383,19.18161487018163
136,1038,1038,2076,0.17075276374816895,19.12481556287217
137,1046,1046,2092,0.17194199562072754,19.06851803023941
138,1054,1054,2108,0.17287468910217285,19.01269209499636
139,1062,1062,2124,0.17378902435302734,18.957309782882465
140,1070,1070,2140,0.17468690872192383,18.902345170983924
141,1078,1078,2156,0.1759018898010254,18.847774245906496
142,1086,1086,2172,0.17685198783874512,18.79357477125626
143,1094,1094,2188,0.17791295051574707,18.739726163832096
144,1102,1102,2204,0.17894983291625977,17.766839325614892
145,1110,1110,2220,0.17995786666870117,17.700204933700064
146,1118,1118,2236,0.18105387687683105,17.634913329941103
147,1124,1124,2248,0.181898832321167,15.989688636010285
148,1132,1132,2264,0.1848609447479248,15.932528680624022
149,1140,1140,2280,0.18578577041625977,15.876404825945297
150,1148,1148,2296,0.18705081939697266,15.82126159580744
151,1156,1156,2312,0.1882917881011963,15.767046618202734
152,1164,1164,2328,0.18975186347961426,15.713710463477582
153,1172,1172,2344,0.19078993797302246,15.66120648981694
154,1180,1180,2360,0.19178295135498047,15.609490695852445
155,1188,1188,2376,0.19282889366149902,15.558521580154824
156,1196,1196,2392,0.1942129135131836,15.244753744132487
157,1204,1204,2408,0.19568586349487305,14.858313134310988
158,1212,1212,2424,0.19683384895324707,14.794897180790398
159,1220,1220,2440,0.19951391220092773,14.732901497917437
160,1228,1228,2456,0.20061492919921875,14.6722595674365
161,1236,1236,2472,0.20145702362060547,14.612907930399308
162,1244,1244,2488,0.2023320198059082,14.554786064888798
163,1252,1252,2504,0.20360994338989258,14.49783626704941
164,1260,1260,2520,0.20463895797729492,14.442003535516818
165,1268,1268,2536,0.2056899070739746,14.387235459241605
166,1276,1276,2552,0.20665884017944336,14.333482108759128
167,1284,1284,2568,0.20777201652526855,14.2806959308985
168,1292,1292,2584,0.2087419033050537,14.228831646925356
169,1300,1300,2600,0.2096998691558838,14.17784615410652
170,1308,1308,2616,0.21294689178466797,14.127698430647307
171,1316,1316,2632,0.21385407447814941,14.078349444014824
172,1324,1324,2648,0.21467876434326172,14.02976206253219
173,1332,1332,2664,0.21554279327392578,13.981900970249065
174,1340,1340,2680,0.21689605712890625,13.934732585002626
175,1348,1348,2696,0.21789073944091797,13.888224979616997
176,1356,1356,2712,0.218919038772583,5.437464608419467
177,1364,1364,2728,0.22005295753479004,5.392753021209952
178,1372,1372,2744,0.22152090072631836,5.349253479943514
179,1376,1376,2752,0.2223367691040039,3.714983969073515
180,1382,1382,2764,0.22327303886413574,3.3543789734725236
181,1390,1390,2780,0.226456880569458,3.3288197083214026
182,1398,1398,2796,0.22766685485839844,3.3039336718739065
183,1406,1406,2812,0.2286369800567627,3.2796976570921528
184,1414,1414,2828,0.22968673706054688,3.256089147544076
185,1422,1422,2844,0.23085498809814453,3.2330863050680736
186,1430,1430,2860,0.2316598892211914,3.210667957221446
187,1438,1438,2876,0.23255085945129395,3.1888135845131336
188,1446,1446,2892,0.23352670669555664,3.1675033074614922
189,1454,1454,2908,0.23459100723266602,3.146717873488265
190,1462,1462,2924,0.23572897911071777,3.126438643674987
191,1470,1470,2940,0.23702573776245117,3.106647579413797
192,1478,1478,2956,0.24006390571594238,3.087327228963184
193,1486,1486,2972,0.24122285842895508,3.068460713941889
194,1494,1494,2988,0.24216890335083008,3.0500317157858996
195,1502,1502,3004,0.24313783645629883,3.032024462182306
196,1510,1510,3020,0.2445969581604004,3.014423713511689
197,1518,1518,3036,0.24541592597961426,2.9972147493187213
198,1526,1526,3052,0.24643182754516602,2.9803833548283967
199,1534,1534,3068,0.24734187126159668,2.963915807532271
200,1542,1542,3084,0.24834585189819336,2.9477988638615127
201,1550,1550,3100,0.24938082695007324,2.9320197459657855
202,1558,1558,3116,0.2503387928009033,2.847828029209055
203,1566,1566,3132,0.2535848617553711,2.0434278844766616
204,1574,1574,3148,0.25474095344543457,2.0372702912400027
205,1580,1580,3160,0.25556492805480957,2.152216264074068
206,1586,1586,3172,0.25632786750793457,1.6770096355540969
207,1592,1592,3184,0.2570807933807373,1.5215889967271905
208,1600,1600,3200,0.2581768035888672,1.5170080756141235
209,1608,1608,3216,0.25912976264953613,1.5124411481929645
210,1616,1616,3232,0.26004791259765625,1.507888166609641
211,1624,1624,3248,0.26097989082336426,1.5033490833540804
212,1632,1632,3264,0.26186084747314453,1.4988238512573613
213,1640,1640,3280,0.2627279758453369,1.4943124234796301
214,1648,1648,3296,0.26528072357177734,0.8990544807698934
215,1656,1656,3312,0.26650404930114746,0.8898702227110277
216,1664,1664,3328,0.26733875274658203,0.8808510195718355
217,1666,1666,3332,0.26769590377807617,0.0033170330226337088
218,1668,1668,3336,0.2680659294128418,3.1422033963378556e-05
219,1670,1670,3340,0.2684199810028076,3.1422033963378556e-12


==> extragradient/plot_data/cournot-nash_equilibrium_problem_n100/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00014495849609375,1624.447741208611
1,4,4,8,0.0005040168762207031,1332.3408024303455
2,6,6,12,0.0011529922485351562,713.8531607135735
3,8,8,16,0.0016009807586669922,580.7956376294903
4,10,10,20,0.0020999908447265625,472.9563599805472
5,12,12,24,0.0025238990783691406,345.1253851566417
6,14,14,28,0.0029449462890625,296.18461714048766
7,16,16,32,0.003381967544555664,286.75853000995244
8,18,18,36,0.003888845443725586,271.0587803845099
9,20,20,40,0.0043277740478515625,272.01279104591094
10,22,22,44,0.004740715026855469,261.96009757850805
11,26,26,52,0.0070667266845703125,267.08261112874806
12,30,30,60,0.007916927337646484,239.37750354060705
13,32,32,64,0.008332014083862305,227.78929663502146
14,36,36,72,0.008916854858398438,223.43164777229262
15,38,38,76,0.00931692123413086,211.12579165307358
16,42,42,84,0.009906768798828125,204.72315180456658
17,44,44,88,0.010340690612792969,203.83061653575888
18,48,48,96,0.01089787483215332,207.06792554388173
19,52,52,104,0.011629104614257812,193.5604859578759
20,56,56,112,0.012386798858642578,182.3675935801982
21,60,60,120,0.01297307014465332,181.22747019150304
22,62,62,124,0.01354074478149414,178.4466408944507
23,64,64,128,0.014073848724365234,169.08748702938055
24,68,68,136,0.015002727508544922,141.23441710762054
25,74,74,148,0.016119956970214844,139.72880791237182
26,78,78,156,0.016873836517333984,135.68485137827224
27,84,84,168,0.017760038375854492,137.2493434272932
28,90,90,180,0.018580913543701172,132.2932287474023
29,96,96,192,0.02175593376159668,121.78411857856216
30,100,100,200,0.022783994674682617,117.08921062562699
31,108,108,216,0.023813724517822266,116.64547294961959
32,116,116,232,0.024866104125976562,109.68431251541442
33,124,124,248,0.02578878402709961,109.10149458161898
34,132,132,264,0.026677846908569336,108.5718387388363
35,140,140,280,0.02766275405883789,108.08663828298728
36,148,148,296,0.028599023818969727,107.63847485916313
37,156,156,312,0.029561758041381836,107.221046328338
38,164,164,328,0.030426740646362305,106.82901404553975
39,172,172,344,0.03135991096496582,106.4578682913725
40,180,180,360,0.032472848892211914,106.10381038979901
41,188,188,376,0.0334169864654541,105.76364995521601
42,196,196,392,0.0366368293762207,105.43471570688006
43,204,204,408,0.03758096694946289,105.11477834144542
44,212,212,424,0.03854179382324219,104.80198404367745
45,220,220,440,0.039502859115600586,104.49479732562725
46,228,228,456,0.04122805595397949,99.41303150256806
47,236,236,472,0.04205894470214844,97.61152377086131
48,244,244,488,0.04306483268737793,97.24826593326785
49,252,252,504,0.043962717056274414,96.90331476916404
50,260,260,520,0.044882774353027344,96.57370224287219
51,268,268,536,0.04585981369018555,92.88463722710284
52,276,276,552,0.04675889015197754,92.4998202727144
53,284,284,568,0.04999971389770508,92.13823293375128
54,292,292,584,0.051030874252319336,91.79636353775416
55,300,300,600,0.05201101303100586,91.47117846770927
56,308,308,616,0.05297589302062988,91.16006281198537
57,316,316,632,0.0538177490234375,90.86076755390683
58,324,324,648,0.054718971252441406,90.57136275834229
59,332,332,664,0.0555877685546875,90.29019621141042
60,340,340,680,0.05664777755737305,90.01585698377365
61,348,348,696,0.05767488479614258,89.74714341307543
62,356,356,712,0.05870485305786133,89.48303503291612
63,364,364,728,0.0598149299621582,89.22266801124472
64,372,372,744,0.06085991859436035,88.96531369815962
65,380,380,760,0.06462287902832031,88.71035992004633
66,388,388,776,0.06578469276428223,88.45729469288023
67,396,396,792,0.06694769859313965,88.20569206151536
68,404,404,808,0.06808590888977051,87.95519980352847
69,412,412,824,0.0694427490234375,87.7055287653946
70,420,420,840,0.07068181037902832,87.45644362548921
71,428,428,856,0.07199478149414062,87.20775490250672
72,436,436,872,0.07329583168029785,86.95931204960348
73,444,444,888,0.07441878318786621,86.71099749396791
74,452,452,904,0.07546496391296387,86.46272149877137
75,460,460,920,0.07814288139343262,86.21441773979113
76,468,468,936,0.07940101623535156,85.96603950251263
77,476,476,952,0.08030104637145996,85.71755641745646
78,484,484,968,0.08118772506713867,85.46895166197719
79,492,492,984,0.08209681510925293,80.8368079825627
80,500,500,1000,0.08301496505737305,80.5875082096376
81,508,508,1016,0.0839238166809082,80.34301931997655
82,516,516,1032,0.0851137638092041,77.6499160931704
83,524,524,1048,0.08618807792663574,76.40787490213843
84,532,532,1064,0.08715295791625977,76.12476490288904
85,540,540,1080,0.08823609352111816,75.85261587916605
86,548,548,1096,0.08927273750305176,71.73352556344149
87,556,556,1112,0.0931546688079834,70.65490064540349
88,564,564,1128,0.09436488151550293,70.29007432445832
89,572,572,1144,0.0953378677368164,69.94577275450258
90,578,578,1156,0.09614896774291992,63.438762653579275
91,586,586,1172,0.09713482856750488,59.46024281122072
92,594,594,1188,0.09794998168945312,40.708254753766724
93,602,602,1204,0.09905385971069336,40.58110258355566
94,608,608,1216,0.09996175765991211,39.91816310167587
95,616,616,1232,0.10110187530517578,36.7459896035863
96,624,624,1248,0.10206794738769531,36.63211734074269
97,632,632,1264,0.10304784774780273,36.51860170012257
98,640,640,1280,0.10594677925109863,36.40544186988257
99,648,648,1296,0.10727882385253906,36.29263702362454
100,656,656,1312,0.10834407806396484,36.180186321245856
101,664,664,1328,0.10940694808959961,36.068088909759254
102,672,672,1344,0.11026573181152344,35.9563439240612
103,680,680,1360,0.11111187934875488,30.978291652014498
104,688,688,1376,0.11194705963134766,29.542917657600896
105,696,696,1392,0.11286282539367676,29.3748577477875
106,704,704,1408,0.11386275291442871,29.212903153186158
107,712,712,1424,0.1150357723236084,29.0566297942741
108,720,720,1440,0.11631178855895996,28.905644359247834
109,728,728,1456,0.11735773086547852,28.75958218267534
110,736,736,1472,0.11834979057312012,28.618105247774853
111,744,744,1488,0.12122964859008789,28.48090030869356
112,752,752,1504,0.12230086326599121,28.347677128658788
113,760,760,1520,0.12338590621948242,28.218166829512505
114,768,768,1536,0.12426495552062988,28.092120347885235
115,776,776,1552,0.12512469291687012,27.96930699306927
116,784,784,1568,0.12594985961914062,27.849513101616424
117,792,792,1584,0.12677502632141113,27.732540783591404
118,800,800,1600,0.12761378288269043,27.618206755474603
119,808,808,1616,0.12854504585266113,27.506341254793153
120,816,816,1632,0.1295018196105957,27.396787031621002
121,824,824,1648,0.1304187774658203,27.28939841230653
122,832,832,1664,0.13130807876586914,27.18404043084
123,840,840,1680,0.13421392440795898,25.51872476467503
124,848,848,1696,0.13526201248168945,25.4358332541519
125,856,856,1712,0.136124849319458,25.36243784545523
126,862,862,1724,0.1367969512939453,26.66623928642606
127,870,870,1740,0.13768386840820312,21.70555709986321
128,878,878,1756,0.13864970207214355,21.63877079167312
129,886,886,1772,0.13949179649353027,21.572754026080112
130,892,892,1784,0.14021086692810059,19.593935732281786
131,900,900,1800,0.14110898971557617,19.53520235606641
132,908,908,1816,0.14206290245056152,19.4770423335768
133,916,916,1832,0.14301085472106934,19.41942039450476
134,924,924,1848,0.1439647674560547,19.362303822287352
135,932,932,1864,0.14478111267089844,19.30566227959125
136,940,940,1880,0.1478438377380371,19.249467645052697
137,948,948,1896,0.14878582954406738,19.19369386061461
138,956,956,1912,0.14974594116210938,19.138316788813214
139,964,964,1928,0.1506187915802002,19.083314079410176
140,972,972,1944,0.15192699432373047,19.028665044811667
141,980,980,1960,0.15284490585327148,18.97435054373976
142,988,988,1976,0.15368986129760742,18.920352872604397
143,996,996,1992,0.15462994575500488,18.866655664153818
144,1004,1004,2008,0.15548181533813477,18.813243792896202
145,1012,1012,2024,0.15636682510375977,18.13613492823198
146,1020,1020,2040,0.15721869468688965,17.754992347750786
147,1028,1028,2056,0.16012072563171387,17.69112587124343
148,1036,1036,2072,0.16113877296447754,17.62843332503099
149,1042,1042,2084,0.16187691688537598,15.989494600257544
150,1050,1050,2100,0.16269373893737793,15.934424566054227
151,1058,1058,2116,0.16384387016296387,15.880260296466659
152,1066,1066,2132,0.16460394859313965,15.82695365488675
153,1074,1074,2148,0.1656198501586914,15.77445922595541
154,1082,1082,2164,0.1666579246520996,15.722734171093464
155,1090,1090,2180,0.1676008701324463,15.671738090856987
156,1098,1098,2196,0.1685628890991211,15.621432893847173
157,1106,1106,2212,0.16958093643188477,15.571782671967021
158,1114,1114,2228,0.17239093780517578,15.522753581783501
159,1122,1122,2244,0.17357277870178223,15.47431373174751
160,1130,1130,2260,0.1744828224182129,14.803440647435467
161,1138,1138,2276,0.1753687858581543,14.742600306767724
162,1146,1146,2292,0.17625093460083008,14.683051696305899
163,1154,1154,2308,0.17728281021118164,14.624734223092688
164,1162,1162,2324,0.17814874649047852,14.567590116949127
165,1170,1170,2340,0.1790318489074707,14.511564314598488
166,1178,1178,2356,0.17998003959655762,14.456604347190034
167,1186,1186,2372,0.18105483055114746,14.402660231307172
168,1194,1194,2388,0.18198680877685547,14.349684363411825
169,1202,1202,2404,0.1829240322113037,14.297631417748935
170,1210,1210,2420,0.18568181991577148,14.246458247691615
171,1218,1218,2436,0.18658876419067383,14.1961237904757
172,1226,1226,2452,0.18739986419677734,14.146588975316254
173,1234,1234,2468,0.18819308280944824,14.097816634831128
174,1242,1242,2484,0.18909382820129395,14.049771419732998
175,1250,1250,2500,0.1900317668914795,14.002419716746106
176,1258,1258,2516,0.1908280849456787,13.955729569636015
177,1266,1266,2532,0.1916790008544922,13.90967060334317
178,1274,1274,2548,0.1925487518310547,13.757841323475837
179,1282,1282,2564,0.19343996047973633,5.473275180549204
180,1290,1290,2580,0.19427990913391113,5.426734523640236
181,1298,1298,2596,0.19516897201538086,5.3814695541161175
182,1302,1302,2604,0.19806170463562012,3.7370558806611074
183,1308,1308,2616,0.19887375831604004,3.373421906000708
184,1316,1316,2632,0.1997509002685547,3.3468576003285033
185,1324,1324,2648,0.2005786895751953,3.3210025692849774
186,1332,1332,2664,0.20135784149169922,3.2958325774071136
187,1340,1340,2680,0.20276093482971191,3.271324094985925
188,1348,1348,2696,0.20365595817565918,3.2474542862688374
189,1356,1356,2712,0.20460176467895508,3.2242009973996955
190,1364,1364,2728,0.20545578002929688,3.2015427441223867
191,1372,1372,2744,0.20645594596862793,3.17945869926108
192,1380,1380,2760,0.207413911819458,3.1579286800051034
193,1388,1388,2776,0.20830988883972168,3.1369331350164176
194,1396,1396,2792,0.2114109992980957,3.116453131389013
195,1404,1404,2808,0.21222400665283203,3.096470341473579
196,1412,1412,2824,0.21297693252563477,3.076967029601341
197,1420,1420,2840,0.21384596824645996,3.0579260387288283
198,1428,1428,2856,0.21483492851257324,3.039330777020514
199,1436,1436,2872,0.21562480926513672,3.02116520440053
200,1444,1444,2888,0.21650481224060059,3.0034138190949027
201,1452,1452,2904,0.21746397018432617,2.9860616441816035
202,1460,1460,2920,0.21856379508972168,2.9690942141764527
203,1468,1468,2936,0.21956396102905273,2.952497561669348
204,1476,1476,2952,0.22048473358154297,2.9362582040381207
205,1484,1484,2968,0.22143101692199707,2.0517737196816634
206,1492,1492,2984,0.2245008945465088,2.0392196306491015
207,1500,1500,3000,0.22542285919189453,2.033063273813949
208,1508,1508,3016,0.22626471519470215,2.02692611541341
209,1514,1514,3028,0.22694993019104004,1.8393627654299343
210,1520,1520,3040,0.2282397747039795,1.6687717838988827
211,1526,1526,3052,0.2291889190673828,1.5140026391506165
212,1534,1534,3068,0.23032808303833008,1.5094361032287131
213,1542,1542,3084,0.2312939167022705,1.5048837522719285
214,1550,1550,3100,0.23224186897277832,1.5003455294015655
215,1558,1558,3116,0.23310089111328125,1.4958213784182588
216,1566,1566,3132,0.2339777946472168,1.0263082211184575
217,1574,1574,3148,0.2371828556060791,0.8986612295500099
218,1582,1582,3164,0.23815488815307617,0.8893968483222792
219,1590,1590,3180,0.2391507625579834,0.8802987156344021
220,1592,1592,3184,0.23961091041564941,0.003972305643875937
221,1594,1594,3188,0.24010896682739258,2.679901527966293e-05
222,1596,1596,3192,0.24056792259216309,3.1422033963378556e-12


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.006479978561401367,7526.915480382486
1001,2004,1002,3006,3.5441129207611084,16.607310482411776
2002,4006,2003,6009,6.740976810455322,8.44604186183642
3003,6008,3004,9012,10.131140947341919,5.384187945803205
4004,8010,4005,12015,13.564121961593628,3.953212580012405
5005,10012,5006,15018,16.912140130996704,3.1670385358302156
6006,12014,6007,18021,20.323441982269287,2.6660191487208067
7007,14016,7008,21024,24.03473997116089,2.322857366572862
8008,16018,8009,24027,27.344194173812866,2.0735852000416344
9009,18020,9010,27030,30.581588983535767,1.8774693972100067
10010,20022,10011,30033,33.7753050327301,1.7188494503752736
11011,22024,11012,33036,37.083268880844116,1.582673018288915
12012,24026,12013,36039,40.37950587272644,1.471707319997222
13013,26028,13014,39042,43.583324909210205,1.3744369879677834
14014,28030,14015,42045,46.76132893562317,1.2886299983183562
15015,30032,15016,45048,49.984355211257935,1.2140860543386225
16016,32034,16017,48051,53.22905397415161,1.1476694552820845
17017,34036,17018,51054,56.370681047439575,1.088071876201866
18018,36038,18019,54057,59.64098405838013,1.0332849611713755
19019,38040,19020,57060,62.88238787651062,0.9833981326173671
20020,40042,20021,60063,66.11721611022949,0.939032640593723
21021,42044,21022,63066,69.34110999107361,0.8974108840684494
22022,44046,22023,66069,72.53726387023926,0.8600530857729609
23023,46048,23024,69072,75.76485824584961,0.8258471587159875
24024,48050,24025,72075,79.35508894920349,0.7934561818037764
25025,50052,25026,75078,82.54595994949341,0.7642925602212927
26026,52054,26027,78081,85.69618797302246,0.7367598122000345
27027,54056,27028,81084,88.8949499130249,0.7111625554553029
28028,56058,28029,84087,92.06171607971191,0.6871552191914816
29029,58060,29030,87090,95.23148393630981,0.6645381343878398
30030,60062,30031,90093,98.5493950843811,0.6432413014699705
31031,62064,31032,93096,101.71502685546875,0.6238021842946182
32032,64066,32033,96099,104.91014289855957,0.605301730125575
33033,66068,33034,99102,108.10603904724121,0.5878315822774312
34034,68070,34035,102105,111.3280041217804,0.571435268062487
35035,70072,35036,105108,114.57196593284607,0.5557054523924307
36036,72074,36037,108111,117.90704202651978,0.5408851722713734
37037,74076,37038,111114,121.14691686630249,0.5269430078697042
38038,76078,38039,114117,124.3833589553833,0.5132465510723705
39039,78080,39040,117120,127.63018488883972,0.5003511031427479
40040,80082,40041,120123,130.8636269569397,0.48800866575220425
41041,82084,41042,123126,134.1103868484497,0.4766423442415544
42042,84086,42043,126129,137.3918080329895,0.4654066780785797
43043,86088,43044,129132,140.55379104614258,0.4548106745551195
44044,88090,44045,132135,144.5558421611786,0.4446414657140849
45045,90092,45046,135138,148.3430380821228,0.4348921094715479
46046,92094,46047,138141,151.7042691707611,0.425505028826592
47047,94096,47048,141144,155.1401391029358,0.4165199768503953
48048,96098,48049,144147,158.46228504180908,0.4079241794333939
49049,98100,49050,147150,161.7031590938568,0.39948473689764796
50050,100102,50051,150153,165.0432939529419,0.39134187462150294
51051,102104,51052,153156,168.34076809883118,0.3836366670020652
52052,104106,52053,156159,171.66346406936646,0.3764342811409733
53053,106108,53054,159162,175.01661014556885,0.36919396650773706
54054,108110,54055,162165,178.28645205497742,0.36230758592137136
55055,110112,55056,165168,181.50732588768005,0.3556901604988525
56056,112114,56057,168171,184.76968097686768,0.3492317360396555
57057,114116,57058,171174,188.0262668132782,0.34296508188526786
58058,116118,58059,174177,191.27908205986023,0.33697372967253614
59059,118120,59060,177180,194.50817584991455,0.3313018955868756
60060,120122,60061,180183,197.73727703094482,0.3256641824846156
61061,122124,61062,183186,200.96349906921387,0.32019864118410624
62062,124126,62063,186189,204.2221441268921,0.3148136218151194
63063,126128,63064,189192,207.53573894500732,0.30967236786091235
64064,128130,64065,192195,210.956472158432,0.3046702432202437
65065,130132,65066,195198,214.305321931839,0.2998149078212009
66066,132134,66067,198201,217.58343291282654,0.29516451411655
67067,134136,67068,201204,220.82792711257935,0.29064668407045247
68068,136138,68069,204207,224.07446718215942,0.28621519477565016
69069,138140,69070,207210,227.49353289604187,0.2819115918082389
70070,140142,70071,210213,230.83379006385803,0.27779908519005403
71071,142144,71072,213216,234.12945580482483,0.27384245153007214
72072,144146,72073,216219,237.40497207641602,0.26989217328082304
73073,146148,73074,219222,240.65365505218506,0.2660547712475818
74074,148150,74075,222225,245.24590301513672,0.262335357894699
75075,150152,75076,225228,249.40277409553528,0.25864909180018003
76076,152154,76077,228231,252.74715280532837,0.2550970652282558
77077,154156,77078,231234,257.4114010334015,0.2516935070234467
78078,156158,78079,234237,263.5583050251007,0.24833497777217417
79079,158160,79080,237240,268.9645400047302,0.2451368044330593
80080,160162,80081,240243,273.8991701602936,0.24199128226064204
81081,162164,81082,243246,279.00500416755676,0.23894381176251045
82082,164166,82083,246249,283.99812293052673,0.23594794828204613
83083,166168,83084,249252,288.9537580013275,0.23296090906842437
84084,168170,84085,252255,294.17182993888855,0.23004385963031382
85085,170172,85086,255258,299.3436770439148,0.2272559894117876
86086,172174,86087,258261,304.46783423423767,0.22452971490747586
87087,174176,87088,261264,309.3200240135193,0.22186004084687738
88088,176178,88089,264267,313.90145993232727,0.21924445435251982
89089,178180,89090,267270,318.95341396331787,0.21668076603782538
90090,180182,90091,270273,324.4294159412384,0.21416691177546454
91091,182184,91092,273276,329.07114696502686,0.21166160795291944
92092,184186,92093,276279,334.1726059913635,0.20914881158751086
93093,186188,93094,279282,339.33644914627075,0.20667534263156995
94094,188190,94095,282285,345.2051479816437,0.20424204975097382
95095,190192,95096,285288,350.3596920967102,0.20184840537331183
96096,192194,96097,288291,355.2950921058655,0.19949390214969753
97097,194196,97098,291294,361.2078421115875,0.19717854433110915
98098,196198,98099,294297,366.43927001953125,0.19494487212250533
99099,198200,99100,297300,371.0514039993286,0.1927948216034565
100100,200202,100101,300303,375.6520059108734,0.19065856019915373
101101,202204,101102,303306,380.68790197372437,0.18859509082176373
102102,204206,102103,306309,385.72709703445435,0.18659051755639666
103103,206208,103104,309312,391.30790305137634,0.18460732131643454
104104,208210,104105,312315,395.605299949646,0.18260361287866544
105105,210212,105106,315318,400.6962938308716,0.18068051412956265
106106,212214,106107,318321,405.32034516334534,0.17880895168309507
107107,214216,107108,321324,409.469938993454,0.17694370840217744
108108,216218,108109,324327,414.1092028617859,0.17512045776493324
109109,218220,109110,327330,418.7154178619385,0.17335131644176727
110110,220222,110111,330333,423.14688205718994,0.17159818137224647
111111,222224,111112,333336,427.8711919784546,0.16987975322990678
112112,224226,112113,336339,433.5740427970886,0.16822902301464637
113113,226228,113114,339342,438.4849100112915,0.16659121578049962
114114,228230,114115,342345,442.56773495674133,0.1650106808192504
115115,230232,115116,345348,446.56058287620544,0.16341408167863847
116116,232234,116117,348351,451.53994703292847,0.16187666171208548
117117,234236,117118,351354,456.75928497314453,0.1603578229460254
118118,236238,118119,354357,461.74205589294434,0.15886139585563797
119119,238240,119120,357360,466.11524415016174,0.15735733398105367
120120,240242,120121,360363,470.6618571281433,0.15587040044556488
121121,242244,121122,363366,475.3424069881439,0.1544428653724026
122122,244246,122123,366369,479.8399109840393,0.15301780183472147
123123,246248,123124,369372,484.2531490325928,0.1516400990931288
124124,248250,124125,372375,487.92694306373596,0.15025963716652768
125125,250252,125126,375378,491.560574054718,0.1489112307990581
126126,252254,126127,378381,495.66027188301086,0.14761421217917814
127127,254256,127128,381384,499.3764638900757,0.14631680492857413
128128,256258,128129,384387,503.1838059425354,0.1450752294385893
129129,258260,129130,387390,506.76850986480713,0.14381988993591222
130130,260262,130131,390393,510.5091321468353,0.14257792303396855
131131,262264,131132,393396,514.2886819839478,0.14136632160807494
132132,264266,132133,396399,517.8366301059723,0.14019431189080933
133133,266268,133134,399402,522.9184319972992,0.13901773133693496
134134,268270,134135,402405,527.3423249721527,0.13785333586383786
135135,270272,135136,405408,531.458701133728,0.13669293777275016
136136,272274,136137,408411,535.7159569263458,0.13559269618235703
137137,274276,137138,411414,540.0425250530243,0.13449485313685727
138138,276278,138139,414417,544.9074518680573,0.13338498170378443
139139,278280,139140,417420,550.2467231750488,0.13231213131803088
140140,280282,140141,420423,555.8437299728394,0.13124558982963208
141141,282284,141142,423426,561.0479009151459,0.13023391386195726
142142,284286,142143,426429,565.546816110611,0.1292165988470515
143143,286288,143144,429432,569.4098098278046,0.12819196858436044
144144,288290,144145,432435,573.4714970588684,0.12716854414975387
145145,290292,145146,435438,578.2710769176483,0.12620230870015803
146146,292294,146147,438441,582.5513129234314,0.12526358662398707
147147,294296,147148,441444,586.7244758605957,0.12434501083589566
148148,296298,148149,444447,590.9844501018524,0.123400823391421
149149,298300,149150,447450,595.2063500881195,0.12249096163759532
150150,300302,150151,450453,599.4106910228729,0.12158502898273582
151151,302304,151152,453456,603.5037441253662,0.12070627397224598
152152,304306,152153,456459,607.5897841453552,0.11984584042693314
153153,306308,153154,459462,611.9162650108337,0.11897642279836873
154154,308310,154155,462465,616.8101971149445,0.11810693065308442
155155,310312,155156,465468,621.1397597789764,0.11726718153477123
156156,312314,156157,468471,625.7284700870514,0.11642346645749058
157157,314316,157158,471474,630.0109748840332,0.11561519744282123
158158,316318,158159,474477,634.327791929245,0.11479682040771877
159159,318320,159160,477480,638.878338098526,0.11399117269502312
160160,320322,160161,480483,643.7178289890289,0.11320039781276137
161161,322324,161162,483486,648.250862121582,0.11240221921434568
162162,324326,162163,486489,652.5657229423523,0.11164483547690907
163163,326328,163164,489492,656.7928121089935,0.1108815559600771
164164,328330,164165,492495,661.0727119445801,0.11011743099516025
165165,330332,165166,495498,665.2357289791107,0.10937031366302108
166166,332334,166167,498501,669.4791309833527,0.10862555021776643
167167,334336,167168,501504,673.8401222229004,0.10790561618887295
168168,336338,168169,504507,678.2316060066223,0.10718855160666863
169169,338340,169170,507510,682.6850008964539,0.10646122358775756
170170,340342,170171,510513,687.0982069969177,0.10577157904663181
171171,342344,171172,513516,691.341481924057,0.10505977850880299
172172,344346,172173,516519,695.6489100456238,0.10437878124685085
173173,346348,173174,519522,699.729532957077,0.10370472200884251
174174,348350,174175,522525,704.4017758369446,0.10302122304165096
175175,350352,175176,525528,709.2964150905609,0.10237048447015695
176176,352354,176177,528531,713.5630369186401,0.10173174938063312
177177,354356,177178,531534,717.8149580955505,0.10108055990531284
178178,356358,178179,534537,722.3299300670624,0.10044570981153811
179179,358360,179180,537540,726.4267590045929,0.09981958184835094
180180,360362,180181,540543,731.2850840091705,0.09919241784336918
181181,362364,181182,543546,736.0189590454102,0.09858298464496329
182182,364366,182183,546549,740.6452720165253,0.09796748981716519
183183,366368,183184,549552,745.1168930530548,0.09736162174885976
184184,368370,184185,552555,749.3616809844971,0.09675337709813903
185185,370372,185186,555558,753.6861639022827,0.09616819443908753
186186,372374,186187,558561,758.9634029865265,0.09559156182695006
187187,374376,187188,561564,763.4359469413757,0.09501270678447327
188188,376378,188189,564567,767.8466548919678,0.09443522115543601
189189,378380,189190,567570,772.1993019580841,0.09386824761713797
190190,380382,190191,570573,776.6636869907379,0.09331787455812446
191191,382384,191192,573576,781.1524701118469,0.09276613868132699
192192,384386,192193,576579,785.6537630558014,0.09221484820773185
193193,386388,193194,579582,790.0265390872955,0.091677767199144
194194,388390,194195,582585,794.383159160614,0.0911399445758434
195195,390392,195196,585588,798.7441279888153,0.09062665188139363
196196,392394,196197,588591,803.1104259490967,0.09010046880030131
197197,394396,197198,591594,807.3738648891449,0.08958799116408045
198198,396398,198199,594597,811.627259016037,0.08907978457500576
199199,398400,199200,597600,815.9751529693604,0.08856669398119266
200200,400402,200201,600603,820.2421870231628,0.0880655324071995
201201,402404,201202,603606,824.5262529850006,0.08756885958973726
202202,404406,202203,606609,828.955323934555,0.08707849906750198
203203,406408,203204,609612,833.4505050182343,0.08660245967075753
204204,408410,204205,612615,837.8961520195007,0.086111599144715
205205,410412,205206,615618,842.23770403862,0.08565389002433221
206206,412414,206207,618621,846.6163311004639,0.08518198994170234
207207,414416,207208,621624,850.9905190467834,0.08473386992227461
208208,416418,208209,624627,855.407151222229,0.08427084970026044
209209,418420,209210,627630,859.7565879821777,0.0838338905468845
210210,420422,210211,630633,863.9814341068268,0.08338153458862507
211211,422424,211212,633636,868.3440451622009,0.08293659274204401
212212,424426,212213,636639,872.7082340717316,0.082500408132546
213213,426428,213214,639642,877.0785768032074,0.08207298989509582
214214,428430,214215,642645,881.4167170524597,0.08165115026713465
215215,430432,215216,645648,885.8426110744476,0.08122702955188288
216216,432434,216217,648651,890.1791560649872,0.08082239213581488
217217,434436,217218,651654,894.5441091060638,0.08042151403606113
218218,436438,218219,654657,898.82963514328,0.08000549956886971
219219,438440,219220,657660,903.0747220516205,0.07959238119838119
220220,440442,220221,660663,907.5196630954742,0.07919900827982929
221221,442444,221222,663666,911.8981690406799,0.07880747086710471
222222,444446,222223,666669,916.0751240253448,0.07841909605122055
223223,446448,223224,669672,920.2910521030426,0.07802783463739615
224224,448450,224225,672675,924.6232478618622,0.07763058551790891
225225,450452,225226,675678,928.7265322208405,0.07724427419452695
226226,452454,226227,678681,932.9298710823059,0.07685819561447715
227227,454456,227228,681684,937.143541097641,0.07648496453293774
228228,456458,228229,684687,941.3715209960938,0.07611063340118562
229229,458460,229230,687690,945.8224101066589,0.0757255789667397
230230,460462,230231,690693,950.2664940357208,0.07536120260192547
231231,462464,231232,693696,954.7544620037079,0.07499600686605845
232232,464466,232233,696699,959.2349970340729,0.07464385523053352
233233,466468,233234,699702,963.5875442028046,0.07427229031418392
234234,468470,234235,702705,967.9414489269257,0.07391028472557082
235235,470472,235236,705708,972.2568209171295,0.07355090622331772
236236,472474,236237,708711,976.6209149360657,0.07320209811950917
237237,474476,237238,711714,980.9468328952789,0.07286511062193313
238238,476478,238239,714717,985.2770659923553,0.07250273810677754
239239,478480,239240,717720,989.7086260318756,0.07216610703108017
240240,480482,240241,720723,994.1199131011963,0.07183349221122626
241241,482484,241242,723726,998.4430961608887,0.0714962379552162
242242,484486,242243,726729,1002.5176770687103,0.0711534223810304
243243,486488,243244,729732,1006.76953291893,0.07082581918075448
244244,488490,244245,732735,1011.0284831523895,0.0704867765725794
245245,490492,245246,735738,1015.3633949756622,0.0701750759526476
246246,492494,246247,738741,1019.6918761730194,0.06985486609846703
247247,494496,247248,741744,1023.9797840118408,0.0695395885304606
248248,496498,248249,744747,1028.3045120239258,0.06921285118005471
249249,498500,249250,747750,1032.649866104126,0.06889476538162853
250250,500502,250251,750753,1036.933357000351,0.06857697793930129
251251,502504,251252,753756,1041.4226381778717,0.06827420561967301
252252,504506,252253,756759,1045.8927989006042,0.06796137230776367
253253,506508,253254,759762,1050.2440881729126,0.06765711242769612
254254,508510,254255,762765,1054.5330739021301,0.06734790730115492
255255,510512,255256,765768,1058.8238849639893,0.06704151672602165
256256,512514,256257,768771,1062.9980511665344,0.06675027380879328
257257,514516,257258,771774,1067.4260959625244,0.06644428369327215
258258,516518,258259,774777,1071.8809430599213,0.06615332470391877
259259,518520,259260,777780,1076.140769958496,0.0658577934573259
260260,520522,260261,780783,1080.3904540538788,0.06556909136452305
261261,522524,261262,783786,1084.9063308238983,0.06528670097213762
262262,524526,262263,786789,1089.3435850143433,0.06500484663047246
263263,526528,263264,789792,1093.660549879074,0.06472449207285536
264264,528530,264265,792795,1098.012680053711,0.06444293089407438
265265,530532,265266,795798,1102.285768032074,0.0641603163585387
266266,532534,266267,798801,1106.7277569770813,0.0638921062436566
267267,534536,267268,801804,1110.9907488822937,0.06361693733924767
268268,536538,268269,804807,1115.130713224411,0.06334646259711008
269269,538540,269270,807810,1119.2814090251923,0.06307743637808017
270270,540542,270271,810813,1123.36580991745,0.06281655627208238
271271,542544,271272,813816,1127.607300043106,0.06255138261076354
272272,544546,272273,816819,1131.8722620010376,0.06229056183474313
273273,546548,273274,819822,1136.1376781463623,0.06202264130115509
274274,548550,274275,822825,1140.481891155243,0.06176848407085345
275275,550552,275276,825828,1144.830134153366,0.06151886341467616
276276,552554,276277,828831,1149.1673369407654,0.06125758933558245
277277,554556,277278,831834,1153.5398840904236,0.06100141256865754
278278,556558,278279,834837,1157.6964468955994,0.06074882749999233
279279,558560,279280,837840,1161.817885875702,0.06050732125368086
280280,560562,280281,840843,1166.0080881118774,0.06025894721642544
281281,562564,281282,843846,1170.5618550777435,0.060008233436747105
282282,564566,282283,846849,1174.7093970775604,0.05976371100769029
283283,566568,283284,849852,1178.960186958313,0.05951964972882706
284284,568570,284285,852855,1183.2018010616302,0.059283695760314004
285285,570572,285286,855858,1187.9271161556244,0.059045855810836656
286286,572574,286287,858861,1192.4553060531616,0.058808509493246675
287287,574576,287288,861864,1196.8752131462097,0.05857745984576468
288288,576578,288289,864867,1201.3813440799713,0.05834453810894047
289289,578580,289290,867870,1205.8487710952759,0.05812028709624428
290290,580582,290291,870873,1210.2644119262695,0.057891811560693895
291291,582584,291292,873876,1214.7429950237274,0.05766478814257425
292292,584586,292293,876879,1218.6215710639954,0.05743860463735473
293293,586588,293294,879882,1222.8418271541595,0.057215856439142954
294294,588590,294295,882885,1227.3284060955048,0.056989711987625924
295295,590592,295296,885888,1231.665533065796,0.05676464362477418
296296,592594,296297,888891,1235.9234869480133,0.05654486270759662
297297,594596,297298,891894,1240.2741661071777,0.05632711717044003
298298,596598,298299,894897,1244.8976891040802,0.056105868134181947
299299,598600,299300,897900,1249.5075788497925,0.055890497900691116
300300,600602,300301,900903,1253.9100008010864,0.05567845566656615
301301,602604,301302,903906,1258.1922810077667,0.05546463220161968
302302,604606,302303,906909,1262.680517911911,0.05525064425455639
303303,606608,303304,909912,1267.1205041408539,0.055037134274243726
304304,608610,304305,912915,1271.5624310970306,0.05482591118561686
305305,610612,305306,915918,1275.9306800365448,0.05461271436797688
306306,612614,306307,918921,1280.308053970337,0.05440817330236314
307307,614616,307308,921924,1284.4897820949554,0.05420153496561397
308308,616618,308309,924927,1288.6366121768951,0.05399002982812817
309309,618620,309310,927930,1292.8736708164215,0.053787573904628516
310310,620622,310311,930933,1297.2203562259674,0.05359131342447654
311311,622624,311312,933936,1301.411076784134,0.05339077615644783
312312,624626,312313,936939,1305.6430988311768,0.05319426237110747
313313,626628,313314,939942,1310.0357229709625,0.05299681124415656
314314,628630,314315,942945,1314.4505400657654,0.052803079031946254
315315,630632,315316,945948,1318.7736330032349,0.05260463263766724
316316,632634,316317,948951,1322.9787549972534,0.05241148790628358
317317,634636,317318,951954,1327.245577096939,0.05222041825072665
318318,636638,318319,954957,1331.582582950592,0.05203339199943002
319319,638640,319320,957960,1335.8252229690552,0.05184671259485185
320320,640642,320321,960963,1340.0114409923553,0.051660822366102366
321321,642644,321322,963966,1344.2498669624329,0.05147211063376744
322322,644646,322323,966969,1347.9698469638824,0.05128980839799624
323323,646648,323324,969972,1352.112231016159,0.051108065294101834
324324,648650,324325,972975,1356.4153809547424,0.05092636479639623
325325,650652,325326,975978,1360.7814168930054,0.050745644883136265
326326,652654,326327,978981,1364.9910998344421,0.05056677149332245
327327,654656,327328,981984,1369.3719749450684,0.05038340997998603
328328,656658,328329,984987,1373.7319340705872,0.050206687843456166
329329,658660,329330,987990,1377.9727518558502,0.05002541392968851
330330,660662,330331,990993,1382.1831080913544,0.04984921791947272
331331,662664,331332,993996,1386.4450287818909,0.04967083075644041
332332,664666,332333,996999,1390.7986319065094,0.049497911293656216
333333,666668,333334,1000002,1395.1584980487823,0.049327015674862196
334334,668670,334335,1003005,1399.4754140377045,0.04915543411880208
335335,670672,335336,1006008,1404.033303976059,0.04898564734503452
336336,672674,336337,1009011,1408.647933959961,0.04881498788927274
337337,674676,337338,1012014,1413.6827139854431,0.0486425261151453
338338,676678,338339,1015017,1419.5801320075989,0.04847606619659928
339339,678680,339340,1018020,1424.4225630760193,0.048311585873307195
340340,680682,340341,1021023,1429.6636228561401,0.04814044620979985
341341,682684,341342,1024026,1434.6547808647156,0.047974894967410364
342342,684686,342343,1027029,1439.2440190315247,0.04781206494226353
343343,686688,343344,1030032,1443.739443063736,0.04765117110400752
344344,688690,344345,1033035,1448.2138860225677,0.04748884103537421
345345,690692,345346,1036038,1452.9589009284973,0.04733080626647279
346346,692694,346347,1039041,1457.5750479698181,0.04716929404094117
347347,694696,347348,1042044,1462.175528049469,0.047010728774694144
348348,696698,348349,1045047,1467.595967054367,0.04685283571052423
349349,698700,349350,1048050,1472.6678819656372,0.04669271315469814
350350,700702,350351,1051053,1477.1064541339874,0.04653653740933805
351351,702704,351352,1054056,1482.8788208961487,0.04637488254775235
352352,704706,352353,1057059,1488.2148990631104,0.04621758290704747
353353,706708,353354,1060062,1493.0646238327026,0.046063350071563036
354354,708710,354355,1063065,1497.5827479362488,0.04590932781502488
355355,710712,355356,1066068,1503.019248008728,0.045757941572446725
356356,712714,356357,1069071,1508.1637098789215,0.04560716612286342
357357,714716,357358,1072074,1513.3378601074219,0.04545624764068634
358358,716718,358359,1075077,1518.3599691390991,0.045307938460609876
359359,718720,359360,1078080,1523.388510942459,0.04515975670074113
360360,720722,360361,1081083,1528.4442739486694,0.04500741261472285
361361,722724,361362,1084086,1533.6441929340363,0.04485749819468765
362362,724726,362363,1087089,1538.6611142158508,0.04470969021167548
363363,726728,363364,1090092,1543.6120541095734,0.044566010330527206
364364,728730,364365,1093095,1548.6640660762787,0.044421509010135196
365365,730732,365366,1096098,1553.7200231552124,0.04427856866095681
366366,732734,366367,1099101,1558.8231790065765,0.04413917690362723
367367,734736,367368,1102104,1564.0453791618347,0.0439972136682627
368368,736738,368369,1105107,1569.2186679840088,0.04386076282753493
369369,738740,369370,1108110,1574.2954471111298,0.04372426187546807
370370,740742,370371,1111113,1579.3713128566742,0.043581809653915116
371371,742744,371372,1114116,1584.421725988388,0.043440588047815254
372372,744746,372373,1117119,1589.4576110839844,0.043301920415615314
373373,746748,373374,1120122,1594.4903259277344,0.04316419739370758
374374,748750,374375,1123125,1599.5889239311218,0.04302864734927425
375375,750752,375376,1126128,1604.7002379894257,0.04289396665808454
376376,752754,376377,1129131,1609.775190114975,0.04275948312533728
377377,754756,377378,1132134,1614.912794828415,0.042624812078429386
378378,756758,378379,1135137,1619.955677986145,0.042494374234593124
379379,758760,379380,1138140,1624.9883551597595,0.04236323380609974
380380,760762,380381,1141143,1629.9996769428253,0.04223205002381292
381381,762764,381382,1144146,1635.0428202152252,0.04210188959041261
382382,764766,382383,1147149,1640.0478339195251,0.04197493167157518
383383,766768,383384,1150152,1645.1299998760223,0.04184750352578703
384384,768770,384385,1153155,1650.4425179958344,0.041718936337929335
385385,770772,385386,1156158,1655.550038099289,0.041590581809941796
386386,772774,386387,1159161,1660.6501140594482,0.0414609066065168
387387,774776,387388,1162164,1665.6917481422424,0.04133366572023078
388388,776778,388389,1165167,1670.7405169010162,0.0412082675320562
389389,778780,389390,1168170,1675.7800810337067,0.04108608501155686
390390,780782,390391,1171173,1680.8514912128448,0.040962984356156085
391391,782784,391392,1174176,1685.9319622516632,0.0408419935429265
392392,784786,392393,1177179,1691.0303711891174,0.04072047852241667
393393,786788,393394,1180182,1696.1497480869293,0.04060268424655078
394394,788790,394395,1183185,1701.199126958847,0.040482558721123496
395395,790792,395396,1186188,1706.2635111808777,0.04036137088951364
396396,792794,396397,1189191,1711.332388162613,0.04024480269072228
397397,794796,397398,1192194,1716.4188060760498,0.040124972350895405
398398,796798,398399,1195197,1721.5751948356628,0.04000431529857451
399399,798800,399400,1198200,1726.7196140289307,0.03988512080468354
400400,800802,400401,1201203,1731.8441879749298,0.03977020697311673
401401,802804,401402,1204206,1736.960275888443,0.039653535810430185
402402,804806,402403,1207209,1742.0737080574036,0.039533675750135444
403403,806808,403404,1210212,1747.3468008041382,0.03941970781306736
404404,808810,404405,1213215,1753.1247239112854,0.03930946279797354
405405,810812,405406,1216218,1758.4514350891113,0.039194468101413804
406406,812814,406407,1219221,1763.8978259563446,0.03907710058228986
407407,814816,407408,1222224,1769.455883026123,0.03895875290436379
408408,816818,408409,1225227,1774.5593359470367,0.038845803232106846
409409,818820,409410,1228230,1779.6928341388702,0.03873352640584926
410410,820822,410411,1231233,1784.812143087387,0.03861791294548311
411411,822824,411412,1234236,1789.866250038147,0.03850806591253786
412412,824826,412413,1237239,1794.9593431949615,0.03839558967774792
413413,826828,413414,1240242,1800.0855360031128,0.038285840882963385
414414,828830,414415,1243245,1805.1076610088348,0.0381766406026145
415415,830832,415416,1246248,1810.1808540821075,0.03806774684562697
416416,832834,416417,1249251,1815.2640759944916,0.037960061728881556
417417,834836,417418,1252254,1820.3160152435303,0.03784918571182061
418418,836838,418419,1255257,1825.3528640270233,0.037742511714895954
419419,838840,419420,1258260,1830.3271119594574,0.03764060911271372
420420,840842,420421,1261263,1835.3754858970642,0.03753883842546202
421421,842844,421422,1264266,1840.3289148807526,0.037430369080539094
422422,844846,422423,1267269,1845.4228811264038,0.037325085804695846
423423,846848,423424,1270272,1850.51233792305,0.037221603575744666
424424,848850,424425,1273275,1855.59960603714,0.0371157511635829
425425,850852,425426,1276278,1860.67298579216,0.03701080606151663
426426,852854,426427,1279281,1865.7338471412659,0.03690726146669476
427427,854856,427428,1282284,1870.832051038742,0.03680133240050054
428428,856858,428429,1285287,1875.8745758533478,0.03669564176198037
429429,858860,429430,1288290,1880.892982006073,0.03659407235318213
430430,860862,430431,1291293,1885.9538187980652,0.03649444243819744
431431,862864,431432,1294296,1890.960589170456,0.036395170383912046
432432,864866,432433,1297299,1895.9707589149475,0.036292699243858806
433433,866868,433434,1300302,1901.2210619449615,0.036195224476614385
434434,868870,434435,1303305,1906.2994420528412,0.036095320912863826
435435,870872,435436,1306308,1911.3527340888977,0.03599710618073004
436436,872874,436437,1309311,1916.4280078411102,0.03590107568925305
437437,874876,437438,1312314,1921.4643788337708,0.035805823525151936
438438,876878,438439,1315317,1926.554846048355,0.035710251389900804
439439,878880,439440,1318320,1931.6845791339874,0.03561364046254312
440440,880882,440441,1321323,1936.8185939788818,0.035516636535248836
441441,882884,441442,1324326,1941.8904840946198,0.035420189658907475
442442,884886,442443,1327329,1946.9556930065155,0.03532763242947112
443443,886888,443444,1330332,1951.9991879463196,0.035229221984991455
444444,888890,444445,1333335,1957.057079076767,0.03513332899274246
445445,890892,445446,1336338,1962.063714981079,0.03503836212075839
446446,892894,446447,1339341,1967.073143005371,0.034945950899782474
447447,894896,447448,1342344,1972.1218750476837,0.034850748228564044
448448,896898,448449,1345347,1977.1782190799713,0.03475903026628657
449449,898900,449450,1348350,1982.2367029190063,0.03466451563872397
450450,900902,450451,1351353,1987.317284822464,0.03457361690016114
451451,902904,451452,1354356,1992.398607969284,0.034480550268199295
452452,904906,452453,1357359,1997.500526189804,0.03439088423692738
453453,906908,453454,1360362,2002.5449750423431,0.03429976174265903
454454,908910,454455,1363365,2007.6049630641937,0.03421080378211627
455455,910912,455456,1366368,2012.6559071540833,0.03412189520531683
456456,912914,456457,1369371,2017.726636171341,0.03403361251184833
457457,914916,457458,1372374,2022.8495681285858,0.03394727558224986
458458,916918,458459,1375377,2027.9665248394012,0.03386092021173681
459459,918920,459460,1378380,2033.0360901355743,0.033769838339139824
460460,920922,460461,1381383,2038.0941388607025,0.0336824520072696
461461,922924,461462,1384386,2043.1228449344635,0.03359842493409815
462462,924926,462463,1387389,2048.197168827057,0.03351182504775352
463463,926928,463464,1390392,2053.213039159775,0.033427153755837935
464464,928930,464465,1393395,2058.280753850937,0.03334321582769917
465465,930932,465466,1396398,2063.3822588920593,0.03326007237046724
466466,932934,466467,1399401,2068.4607050418854,0.03317654531565495
467467,934936,467468,1402404,2073.6470079421997,0.0330939364630467
468468,936938,468469,1405407,2078.6938619613647,0.033008914102538256
469469,938940,469470,1408410,2083.7873060703278,0.03292496244648646
470470,940942,470471,1411413,2088.861361026764,0.03284465470824216
471471,942944,471472,1414416,2093.86109995842,0.03276387186269858
472472,944946,472473,1417419,2098.8908009529114,0.03268489466063329
473473,946948,473474,1420422,2103.967283964157,0.03260604661227262
474474,948950,474475,1423425,2109.0084660053253,0.03252705502927711
475475,950952,475476,1426428,2114.0708129405975,0.0324487421894446
476476,952954,476477,1429431,2119.0964539051056,0.03237007860298036
477477,954956,477478,1432434,2124.1280069351196,0.03229219048262166
478478,956958,478479,1435437,2129.2044439315796,0.03221421306989214
479479,958960,479480,1438440,2134.2465369701385,0.03213578978102305
480480,960962,480481,1441443,2139.197616815567,0.032057712794994586
481481,962964,481482,1444446,2144.2372028827667,0.031977578402802465
482482,964966,482483,1447449,2149.329483985901,0.03189944287078106
483483,966968,483484,1450452,2154.3982331752777,0.03182352978910785
484484,968970,484485,1453455,2159.439774990082,0.03174579840924707
485485,970972,485486,1456458,2164.4984951019287,0.03166827814675344
486486,972974,486487,1459461,2169.5500481128693,0.03159003734253929
487487,974976,487488,1462464,2174.566032886505,0.03151240916486131
488488,976978,488489,1465467,2179.597470998764,0.031433211455805576
489489,978980,489490,1468470,2184.6584680080414,0.0313572668346751
490490,980982,490491,1471473,2189.682249069214,0.031281660729291616
491491,982984,491492,1474476,2194.667774915695,0.031205871053316514
492492,984986,492493,1477479,2199.6951019763947,0.03113351223510108
493493,986988,493494,1480482,2204.6832609176636,0.03106100780860288
494494,988990,494495,1483485,2209.700492143631,0.030986623220087495
495495,990992,495496,1486488,2214.737590074539,0.030912169513612753
496496,992994,496497,1489491,2219.7545421123505,0.03084027588556637
497497,994996,497498,1492494,2224.8419280052185,0.030768238348173327
498498,996998,498499,1495497,2229.946949005127,0.030697683891048655
499499,999000,499500,1498500,2234.9482839107513,0.030624584960605716
500501,1001004,500502,1501506,2239.9798018932343,0.03055277090606978
501502,1003006,501503,1504509,2245.163866996765,0.03048247186234221
502503,1005008,502504,1507512,2250.233274936676,0.030411687535888632
503504,1007010,503505,1510515,2255.3130609989166,0.03033823973419203
504505,1009012,504506,1513518,2260.363610982895,0.030267203534094733
505506,1011014,505507,1516521,2265.4386179447174,0.030196914483894943
506507,1013016,506508,1519524,2270.495674133301,0.030128009064355865
507508,1015018,507509,1522527,2275.55410695076,0.03005784659399069
508509,1017020,508510,1525530,2280.5331478118896,0.02998779078370717
509510,1019022,509511,1528533,2285.5011830329895,0.029918425954747363
510511,1021024,510512,1531536,2290.5240609645844,0.029849488400941482
511512,1023026,511513,1534539,2295.576826095581,0.02978057131622336
512513,1025028,512514,1537542,2300.602767944336,0.029711302599025657
513514,1027030,513515,1540545,2305.6484150886536,0.02964230059842521
514515,1029032,514516,1543548,2310.714085817337,0.02957351433178701
515516,1031034,515517,1546551,2315.762857913971,0.02950624296499882
516517,1033036,516518,1549554,2320.8116569519043,0.02943904551830201
517518,1035038,517519,1552557,2325.8354501724243,0.02937337247749383
518519,1037040,518520,1555560,2330.9279968738556,0.029306242666280014
519520,1039042,519521,1558563,2335.984943151474,0.02923958359315293
520521,1041044,520522,1561566,2340.8349299430847,0.029172906364692608
521522,1043046,521523,1564569,2345.8395688533783,0.029104296892910497
522523,1045048,522524,1567572,2350.854734182358,0.029038154541922268
523524,1047050,523525,1570575,2355.8821001052856,0.02897107864919235
524525,1049052,524526,1573578,2360.903522014618,0.02890371649482404
525526,1051054,525527,1576581,2365.946841955185,0.028837573052442167
526527,1053056,526528,1579584,2370.9811499118805,0.0287711929759098
527528,1055058,527529,1582587,2376.0850670337677,0.028706750792480307
528529,1057060,528530,1585590,2381.0882980823517,0.028642730379942805
529530,1059062,529531,1588593,2386.1125819683075,0.02857901329298329
530531,1061064,530532,1591596,2391.1785390377045,0.028514807316241786
531532,1063066,531533,1594599,2396.204950094223,0.028451865193346748
532533,1065068,532534,1597602,2401.247498989105,0.028387068887241185
533534,1067070,533535,1600605,2406.231716156006,0.028325738056082628
534535,1069072,534536,1603608,2411.23481798172,0.028264613980354625
535536,1071074,535537,1606611,2416.2891829013824,0.028202130588397267
536537,1073076,536538,1609614,2421.388920068741,0.02813884437091474
537538,1075078,537539,1612617,2426.4556879997253,0.02807657562152599
538539,1077080,538540,1615620,2431.556135892868,0.02801499728411727
539540,1079082,539541,1618623,2436.5519070625305,0.027954871995461872
540541,1081084,540542,1621626,2441.569060087204,0.02789443900473998
541542,1083086,541543,1624629,2446.587517976761,0.02783186986016517
542543,1085088,542544,1627632,2451.6421377658844,0.0277695474360371
543544,1087090,543545,1630635,2456.650676012039,0.027709299580237712
544545,1089092,544546,1633638,2461.6013209819794,0.027648888462863397
545546,1091094,545547,1636641,2466.649796962738,0.02758881116460543
546547,1093096,546548,1639644,2471.627110004425,0.02752798253277433
547548,1095098,547549,1642647,2476.6414120197296,0.027469175487567554
548549,1097100,548550,1645650,2481.637104988098,0.027410530761699192
549550,1099102,549551,1648653,2486.64240694046,0.027352244413123117
550551,1101104,550552,1651656,2491.68963098526,0.027293446133626276
551552,1103106,551553,1654659,2496.764561891556,0.027232852082306636
552553,1105108,552554,1657662,2501.7842450141907,0.027171640444066725
553554,1107110,553555,1660665,2506.818787097931,0.027109872333312524
554555,1109112,554556,1663668,2511.812516927719,0.027051153267166228
555556,1111114,555557,1666671,2516.8079030513763,0.02699237147317035
556557,1113116,556558,1669674,2521.8355457782745,0.026935664305710816
557558,1115118,557559,1672677,2526.8377289772034,0.026878572098212317
558559,1117120,558560,1675680,2531.9522619247437,0.026820778200999484
559560,1119122,559561,1678683,2537.0170118808746,0.02676137042544724
560561,1121124,560562,1681686,2542.074553012848,0.02670246244088048
561562,1123126,561563,1684689,2547.1770281791687,0.02664556944000651
562563,1125128,562564,1687692,2552.230341911316,0.026588856600938016
563564,1127130,563565,1690695,2557.339318037033,0.02653266406196053
564565,1129132,564566,1693698,2562.418394804001,0.026476221422853996
565566,1131134,565567,1696701,2567.475772857666,0.026419150137371616
566567,1133136,566568,1699704,2572.5508019924164,0.026362920694737113
567568,1135138,567569,1702707,2577.6086831092834,0.02630786900044768
568569,1137140,568570,1705710,2582.661028146744,0.026251921484799823
569570,1139142,569571,1708713,2587.792274951935,0.026195985517915688
570571,1141144,570572,1711716,2592.8876581192017,0.026140345240492024
571572,1143146,571573,1714719,2597.9339468479156,0.026085906491061905
572573,1145148,572574,1717722,2602.9822750091553,0.02603073666068667
573574,1147150,573575,1720725,2607.9923429489136,0.025975415454013273
574575,1149152,574576,1723728,2613.0521750450134,0.025920983131072717
575576,1151154,575577,1726731,2618.09507894516,0.02586824206082383
576577,1153156,576578,1729734,2623.1826298236847,0.02581461422232678
577578,1155158,577579,1732737,2628.279876947403,0.025759624508282286
578579,1157160,578580,1735740,2633.4228279590607,0.025706399266709923
579580,1159162,579581,1738743,2638.390406847,0.0256536794713611
580581,1161164,580582,1741746,2643.3621780872345,0.02560013013862772
581582,1163166,581583,1744749,2648.4252989292145,0.025546816304995446
582583,1165168,582584,1747752,2653.4313740730286,0.02549512975201651
583584,1167170,583585,1750755,2658.4795949459076,0.02544167430824018
584585,1169172,584586,1753758,2663.5191061496735,0.025389089101736317
585586,1171174,585587,1756761,2668.70921087265,0.02533710865827743
586587,1173176,586588,1759764,2675.5508880615234,0.025284614821430296
587588,1175178,587589,1762767,2681.4723358154297,0.025233764932636404
588589,1177180,588590,1765770,2687.0584042072296,0.025182962212056736
589590,1179182,589591,1768773,2692.1324710845947,0.025132862510872656
590591,1181184,590592,1771776,2697.2480289936066,0.025082192338231835
591592,1183186,591593,1774779,2702.2971761226654,0.025030706687175552
592593,1185188,592594,1777782,2707.4709718227386,0.02497998540820845
593594,1187190,593595,1780785,2712.6002650260925,0.02492929537402233
594595,1189192,594596,1783788,2717.7122070789337,0.02487930429924745
595596,1191194,595597,1786791,2722.8287942409515,0.024828896755934693
596597,1193196,596598,1789794,2727.9777789115906,0.02477845186331251
597598,1195198,597599,1792797,2733.086852788925,0.02472811682309839
598599,1197200,598600,1795800,2738.217730998993,0.024678895049873972
599600,1199202,599601,1798803,2743.3140890598297,0.024628056862638914
600601,1201204,600602,1801806,2748.397339820862,0.024577403821240296
601602,1203206,601603,1804809,2753.4855811595917,0.024526854256691877
602603,1205208,602604,1807812,2758.589607000351,0.024476873430103296
603604,1207210,603605,1810815,2763.680558204651,0.02442747150780633
604605,1209212,604606,1813818,2768.7533388137817,0.024378649513892015
605606,1211214,605607,1816821,2773.8556730747223,0.024329544270585757
606607,1213216,606608,1819824,2778.9536340236664,0.024280602068756707
607608,1215218,607609,1822827,2784.007075071335,0.02423231538887194
608609,1217220,608610,1825830,2789.1208119392395,0.024183603027267964
609610,1219222,609611,1828833,2794.222640991211,0.024136176105457707
610611,1221224,610612,1831836,2799.280015230179,0.024088882139039924
611612,1223226,611613,1834839,2804.3602209091187,0.0240423479135643
612613,1225228,612614,1837842,2809.4332160949707,0.023995380655833287
613614,1227230,613615,1840845,2814.499589920044,0.023947172387124738
614615,1229232,614616,1843848,2819.5928819179535,0.02389893206236593
615616,1231234,615617,1846851,2824.6283588409424,0.023852137028370635
616617,1233236,616618,1849854,2829.708373069763,0.023804748278053012
617618,1235238,617619,1852857,2834.75927901268,0.023758095618177322
618619,1237240,618620,1855860,2839.7856290340424,0.023711841395197553
619620,1239242,619621,1858863,2844.801190853119,0.023666363253141753
620621,1241244,620622,1861866,2849.936150074005,0.023620231742825126
621622,1243246,621623,1864869,2855.0306289196014,0.023573961601869087
622623,1245248,622624,1867872,2860.1009290218353,0.023526917439085082
623624,1247250,623625,1870875,2865.1959869861603,0.023479902285544085
624625,1249252,624626,1873878,2870.32169508934,0.023434427934262203
625626,1251254,625627,1876881,2875.420555114746,0.02338964815317013
626627,1253256,626628,1879884,2880.481360912323,0.02334406360932917
627628,1255258,627629,1882887,2885.5173370838165,0.023298564163269475
628629,1257260,628630,1885890,2890.6042170524597,0.023253674065927044
629630,1259262,629631,1888893,2895.6669471263885,0.023208806214825017
630631,1261264,630632,1891896,2900.7354822158813,0.02316362495366775
631632,1263266,631633,1894899,2905.767075061798,0.02311850535807025
632633,1265268,632634,1897902,2910.810198068619,0.02307336948979355
633634,1267270,633635,1900905,2915.9093911647797,0.023028804749628762
634635,1269272,634636,1903908,2920.997645139694,0.022985105206316803
635636,1271274,635637,1906911,2926.0861167907715,0.02293994057981763
636637,1273276,636638,1909914,2931.141484975815,0.022895582536875736
637638,1275278,637639,1912917,2936.189961910248,0.022851990534036304
638639,1277280,638640,1915920,2941.241902112961,0.022808519051977783
639640,1279282,639641,1918923,2946.2738728523254,0.022763765651689027
640641,1281284,640642,1921926,2951.3692610263824,0.022720093986208667
641642,1283286,641643,1924929,2956.427929162979,0.022676230079014204
642643,1285288,642644,1927932,2961.4770748615265,0.02263369298998441
643644,1287290,643645,1930935,2966.5330288410187,0.022590768201553146
644645,1289292,644646,1933938,2971.802234172821,0.022547086562553886
645646,1291294,645647,1936941,2976.863373041153,0.022504133492475376
646647,1293296,646648,1939944,2981.819939136505,0.02246051405563776
647648,1295298,647649,1942947,2986.946756839752,0.022417340695028543
648649,1297300,648650,1945950,2992.017895936966,0.022375768239726312
649650,1299302,649651,1948953,2997.104129076004,0.022332702112180414
650651,1301304,650652,1951956,3002.156389951706,0.022291132758255117
651652,1303306,651653,1954959,3007.3000252246857,0.022248990935622714
652653,1305308,652654,1957962,3012.362287044525,0.022207021342182998
653654,1307310,653655,1960965,3017.4444348812103,0.022165781339936075
654655,1309312,654656,1963968,3022.505744934082,0.02212286667781882
655656,1311314,655657,1966971,3027.5205240249634,0.022080154456489254
656657,1313316,656658,1969974,3032.631113052368,0.022038802797396784
657658,1315318,657659,1972977,3037.725741147995,0.02199714380731166
658659,1317320,658660,1975980,3042.754639863968,0.021956053935355158
659660,1319322,659661,1978983,3048.391279220581,0.021914605940764886
660661,1321324,660662,1981986,3053.491203069687,0.02187375237008382
661662,1323326,661663,1984989,3058.938863992691,0.021832442242157413
662663,1325328,662664,1987992,3064.021273136139,0.021791986742755398
663664,1327330,663665,1990995,3069.0647439956665,0.021752671427748282
664665,1329332,664666,1993998,3074.084265947342,0.021711908808356384
665666,1331334,665667,1997001,3079.0882618427277,0.02167105288026505
666667,1333336,666668,2000004,3084.102189064026,0.02163062789441028
667668,1335338,667669,2003007,3089.149281024933,0.02159244432732521
668669,1337340,668670,2006010,3094.2049539089203,0.021553048745772685
669670,1339342,669671,2009013,3099.2505819797516,0.02151257345940394
670671,1341344,670672,2012016,3104.3393399715424,0.021472844668096513
671672,1343346,671673,2015019,3109.4389219284058,0.021434119233163074
672673,1345348,672674,2018022,3114.4794340133667,0.02139573952263163
673674,1347350,673675,2021025,3119.5785150527954,0.021357074843763257
674675,1349352,674676,2024028,3124.5783910751343,0.021317314120096853
675676,1351354,675677,2027031,3129.597018957138,0.021277616257066256
676677,1353356,676678,2030034,3134.599982023239,0.021239871959551238
677678,1355358,677679,2033037,3139.506089925766,0.021201863508395036
678679,1357360,678680,2036040,3144.551132917404,0.021164025307371048
679680,1359362,679681,2039043,3149.6110990047455,0.021127415328010102
680681,1361364,680682,2042046,3154.6832780838013,0.02108831848454429
681682,1363366,681683,2045049,3159.827050924301,0.021049933471658733
682683,1365368,682684,2048052,3164.8989861011505,0.021011512671975652
683684,1367370,683685,2051055,3169.987279176712,0.02097443275852129
684685,1369372,684686,2054058,3175.0385389328003,0.020936598170010257
685686,1371374,685687,2057061,3180.113821029663,0.020898914484860143
686687,1373376,686688,2060064,3185.1560440063477,0.02086181468439463
687688,1375378,687689,2063067,3190.166235923767,0.020824324656132376
688689,1377380,688690,2066070,3195.224860906601,0.020785998451174237
689690,1379382,689691,2069073,3200.2928099632263,0.02074845155220828
690691,1381384,690692,2072076,3205.3089740276337,0.02071170715316839
691692,1383386,691693,2075079,3210.3009548187256,0.020675080457294825
692693,1385388,692694,2078082,3215.355717897415,0.020637165900552645
693694,1387390,693695,2081085,3220.399067878723,0.02060045347570849
694695,1389392,694696,2084088,3225.510549068451,0.02056390410689346
695696,1391394,695697,2087091,3230.5540289878845,0.02052722582811839
696697,1393396,696698,2090094,3235.6033878326416,0.02049065571372921
697698,1395398,697699,2093097,3240.6557791233063,0.02045390738203423
698699,1397400,698700,2096100,3245.700420856476,0.02041757850565773
699700,1399402,699701,2099103,3250.8384029865265,0.02038132037341711
700701,1401404,700702,2102106,3255.923697948456,0.020346176646853564
701702,1403406,701703,2105109,3260.979302883148,0.020310221229010494
702703,1405408,702704,2108112,3266.093628883362,0.02027410071059421
703704,1407410,703705,2111115,3271.2174830436707,0.02023745402584609
704705,1409412,704706,2114118,3276.320612192154,0.020202626157697523
705706,1411414,705707,2117121,3281.4372680187225,0.020166510896160617
706707,1413416,706708,2120124,3286.5603201389313,0.02013018356410612
707708,1415418,707709,2123127,3291.6646699905396,0.020094705318115302
708709,1417420,708710,2126130,3296.7947731018066,0.020058495736520854
709710,1419422,709711,2129133,3301.86936712265,0.020023780978590366
710711,1421424,710712,2132136,3306.9589791297913,0.01998935609299224
711712,1423426,711713,2135139,3312.028855085373,0.019954092143962043
712713,1425428,712714,2138142,3317.139322042465,0.019919357924663927
713714,1427430,713715,2141145,3322.1897950172424,0.01988521732891968
714715,1429432,714716,2144148,3327.284959077835,0.019850751321428106
715716,1431434,715717,2147151,3332.393529176712,0.01981542357316357
716717,1433436,716718,2150154,3337.4942779541016,0.019780362094024895
717718,1435438,717719,2153157,3342.591475009918,0.019745738261917722
718719,1437440,718720,2156160,3347.6817829608917,0.01971149326345767
719720,1439442,719721,2159163,3352.7471430301666,0.019677375947139808
720721,1441444,720722,2162166,3357.8745028972626,0.019642150362415123
721722,1443446,721723,2165169,3362.9416630268097,0.0196084205454099
722723,1445448,722724,2168172,3368.0154390335083,0.01957379544910509
723724,1447450,723725,2171175,3373.0658071041107,0.019538946380635025
724725,1449452,724726,2174178,3378.190851211548,0.019505525522617972
725726,1451454,725727,2177181,3383.3185460567474,0.019472166168270633
726727,1453456,726728,2180184,3388.347388982773,0.019438200783042703
727728,1455458,727729,2183187,3393.39053106308,0.01940469520377519
728729,1457460,728730,2186190,3398.4673862457275,0.019371583288375405
729730,1459462,729731,2189193,3403.5831089019775,0.01933799470134545
730731,1461464,730732,2192196,3408.683351993561,0.019305455340145272
731732,1463466,731733,2195199,3413.73095703125,0.019272699566499796
732733,1465468,732734,2198202,3418.8322370052338,0.019238240927734296
733734,1467470,733735,2201205,3423.9878220558167,0.019205243179385434
734735,1469472,734736,2204208,3429.0612239837646,0.019172515587342787
735736,1471474,735737,2207211,3434.7410459518433,0.01913939547011978
736737,1473476,736738,2210214,3440.001937866211,0.019106712210486876
737738,1475478,737739,2213217,3445.147306919098,0.019073901195952203
738739,1477480,738740,2216220,3450.345160007477,0.019040668405068573
739740,1479482,739741,2219223,3455.4186811447144,0.01900848418517853
740741,1481484,740742,2222226,3460.535646915436,0.018975230002979515
741742,1483486,741743,2225229,3465.6222410202026,0.018943326509543112
742743,1485488,742744,2228232,3470.7019789218903,0.018911324443251942
743744,1487490,743745,2231235,3475.797894001007,0.018878664248404675
744745,1489492,744746,2234238,3480.6814579963684,0.018846175004000543
745746,1491494,745747,2237241,3485.774365901947,0.018813040987879504
746747,1493496,746748,2240244,3490.9132208824158,0.018780595461066696
747748,1495498,747749,2243247,3495.9678630828857,0.018748884978776914
748749,1497500,748750,2246250,3501.079297065735,0.018717261518759187
749750,1499502,749751,2249253,3506.16854596138,0.018686197789065773
750751,1501504,750752,2252256,3511.22429895401,0.018655106501682894
751752,1503506,751753,2255259,3516.30717587471,0.018622587511345046
752753,1505508,752754,2258262,3521.36355304718,0.018591095251395018
753754,1507510,753755,2261265,3526.491029024124,0.01855975334547111
754755,1509512,754756,2264268,3531.5351190567017,0.01852727485129435
755756,1511514,755757,2267271,3536.6377930641174,0.018496565926398034
756757,1513516,756758,2270274,3541.7792451381683,0.018465420153006562
757758,1515518,757759,2273277,3546.8566529750824,0.018433846857078606
758759,1517520,758760,2276280,3551.9935359954834,0.018401963210635586
759760,1519522,759761,2279283,3557.18279504776,0.01837119712763524
760761,1521524,760762,2282286,3562.246603012085,0.018339682808800717
761762,1523526,761763,2285289,3567.3695390224457,0.01830861701637332
762763,1525528,762764,2288292,3572.4393570423126,0.018277748855325626
763764,1527530,763765,2291295,3577.5254011154175,0.01824668247718364
764765,1529532,764766,2294298,3582.583316087723,0.018216928099718643
765766,1531534,765767,2297301,3587.7051849365234,0.018186513740147348
766767,1533536,766768,2300304,3592.7822189331055,0.01815564065145736
767768,1535538,767769,2303307,3597.9041001796722,0.01812537418481952
768769,1537540,768770,2306310,3603.0079958438873,0.018095942035870394
769770,1539542,769771,2309313,3608.104528903961,0.018065209638734814
770771,1541544,770772,2312316,3613.191265106201,0.018034809503660654
771772,1543546,771773,2315319,3618.2624049186707,0.01800459305741242
772773,1545548,772774,2318322,3623.363918066025,0.017974527947444585
773774,1547550,773775,2321325,3628.4337599277496,0.01794458064796345
774775,1549552,774776,2324328,3633.520315885544,0.017914650359671214
775776,1551554,775777,2327331,3638.5606348514557,0.017884473281810642
776777,1553556,776778,2330334,3643.596621990204,0.0178548501462501
777778,1555558,777779,2333337,3648.6340239048004,0.017825533062932664
778779,1557560,778780,2336340,3653.765609025955,0.017796169040593668
779780,1559562,779781,2339343,3658.8834948539734,0.017767054956493666
780781,1561564,780782,2342346,3663.952523946762,0.017738355145411333
781782,1563566,781783,2345349,3669.0253808498383,0.01770831338581047
782783,1565568,782784,2348352,3674.1155869960785,0.017679680888250005
783784,1567570,783785,2351355,3679.2047171592712,0.01764980896587076
784785,1569572,784786,2354358,3684.2631299495697,0.017620852144318633
785786,1571574,785787,2357361,3689.3140370845795,0.017592166224858374
786787,1573576,786788,2360364,3694.360384941101,0.017563413515745196
787788,1575578,787789,2363367,3699.406674861908,0.017534088094180333
788789,1577580,788790,2366370,3704.4990870952606,0.01750681214798533
789790,1579582,789791,2369373,3709.587635040283,0.017479266027294216
790791,1581584,790792,2372376,3714.636505126953,0.0174508406289533
791792,1583586,791793,2375379,3719.7214138507843,0.01742308816028526
792793,1585588,792794,2378382,3724.7597692012787,0.0173952777768136
793794,1587590,793795,2381385,3729.827425956726,0.017367892411130015
794795,1589592,794796,2384388,3734.9145851135254,0.017340188556772773
795796,1591594,795797,2387391,3739.9804100990295,0.017312131290964317
796797,1593596,796798,2390394,3745.042585849762,0.017284340407059062
797798,1595598,797799,2393397,3750.117518186569,0.017256205890589627
798799,1597600,798800,2396400,3755.198007106781,0.01722920649444859
799800,1599602,799801,2399403,3760.3092589378357,0.017201798775204225
800801,1601604,800802,2402406,3765.4493792057037,0.017175068922369974
801802,1603606,801803,2405409,3770.49005484581,0.01714843032641511
802803,1605608,802804,2408412,3775.5708980560303,0.01712084924110968
803804,1607610,803805,2411415,3780.6436910629272,0.0170937045422761
804805,1609612,804806,2414418,3785.693081140518,0.017067357743144385
805806,1611614,805807,2417421,3790.7975721359253,0.017040923188687884
806807,1613616,806808,2420424,3795.849420070648,0.017014018949339516
807808,1615618,807809,2423427,3800.9105780124664,0.016986821832688292
808809,1617620,808810,2426430,3805.964513063431,0.016959119817329338
809810,1619622,809811,2429433,3810.9970569610596,0.016932852977333823
810811,1621624,810812,2432436,3816.068302154541,0.016906371565710288
811812,1623626,811813,2435439,3821.10653591156,0.016879748725841637
812813,1625628,812814,2438442,3826.3623371124268,0.01685351315245498
813814,1627630,813815,2441445,3831.425033092499,0.016827408548124367
814815,1629632,814816,2444448,3836.477447986603,0.016801436628156807
815816,1631634,815817,2447451,3841.6295969486237,0.016775100824816036
816817,1633636,816818,2450454,3846.739065170288,0.01674938899486733
817818,1635638,817819,2453457,3851.830878973007,0.01672272205723857
818819,1637640,818820,2456460,3856.9327590465546,0.01669733927883499
819820,1639642,819821,2459463,3862.0156140327454,0.016672141007802566
820821,1641644,820822,2462466,3867.1237041950226,0.016645970363242668
821822,1643646,821823,2465469,3872.419163942337,0.016620562360913027
822823,1645648,822824,2468472,3877.530163049698,0.01659451690102287
823824,1647650,823825,2471475,3882.648535013199,0.016568963161262218
824825,1649652,824826,2474478,3887.733654975891,0.01654359622443735
825826,1651654,825827,2477481,3892.784110069275,0.016518663434908376
826827,1653656,826828,2480484,3897.9392352104187,0.01649397358414717
827828,1655658,827829,2483487,3903.06041097641,0.016468055291625205
828829,1657660,828830,2486490,3908.104063987732,0.016442739652120508
829830,1659662,829831,2489493,3913.1634271144867,0.016417400824138895
830831,1661664,830832,2492496,3918.2480981349945,0.016391861032388988
831832,1663666,831833,2495499,3923.341726064682,0.01636632837653451
832833,1665668,832834,2498502,3928.46239900589,0.016341779717549798
833834,1667670,833835,2501505,3933.5214989185333,0.016316090632244595
834835,1669672,834836,2504508,3938.6032581329346,0.01629134506219998
835836,1671674,835837,2507511,3943.7309861183167,0.016266791275484138
836837,1673676,836838,2510514,3948.8425850868225,0.0162426154493005
837838,1675678,837839,2513517,3954.0122740268707,0.016217877935559954
838839,1677680,838840,2516520,3959.1584310531616,0.016192726132430835
839840,1679682,839841,2519523,3964.2685110569,0.016168718435437768
840841,1681684,840842,2522526,3969.3612768650055,0.01614502326810907
841842,1683686,841843,2525529,3974.467148065567,0.016120098100145697
842843,1685688,842844,2528532,3979.602703809738,0.016095582373964135
843844,1687690,843845,2531535,3984.6663269996643,0.016071317619207548
844845,1689692,844846,2534538,3989.7571761608124,0.016046715065385797
845846,1691694,845847,2537541,3994.86066699028,0.01602274656033842
846847,1693696,846848,2540544,3999.9304950237274,0.015998575816411176
847848,1695698,847849,2543547,4005.0533640384674,0.015974887257470982
848849,1697700,848850,2546550,4010.1683089733124,0.015950065080687637
849850,1699702,849851,2549553,4015.245239019394,0.01592538413387956
850851,1701704,850852,2552556,4020.376783847809,0.015900744871032657
851852,1703706,851853,2555559,4025.5274341106415,0.015876584457146237
852853,1705708,852854,2558562,4030.646073102951,0.01585215645172866
853854,1707710,853855,2561565,4035.7305238246918,0.015827993765924475
854855,1709712,854856,2564568,4040.81675696373,0.015804769147507614
855856,1711714,855857,2567571,4045.9190599918365,0.0157816136143083
856857,1713716,856858,2570574,4051.8485050201416,0.015758167099193088
857858,1715718,857859,2573577,4057.1110379695892,0.015734627462734352
858859,1717720,858860,2576580,4062.3244631290436,0.015710691821368528
859860,1719722,859861,2579583,4067.3830420970917,0.015686904214817332
860861,1721724,860862,2582586,4072.4930980205536,0.015663748206861783
861862,1723726,861863,2585589,4077.5593349933624,0.015640081761375768
862863,1725728,862864,2588592,4082.6404659748077,0.015616759101249045
863864,1727730,863865,2591595,4087.712558031082,0.015593018693834892
864865,1729732,864866,2594598,4092.809909105301,0.015569747456538607
865866,1731734,865867,2597601,4097.87025308609,0.0155470107729343
866867,1733736,866868,2600604,4102.967668056488,0.015524093701969832
867868,1735738,867869,2603607,4108.047170162201,0.015500818724831333
868869,1737740,868870,2606610,4113.198755025864,0.015477497699976084
869870,1739742,869871,2609613,4118.336612224579,0.015455133194336668
870871,1741744,870872,2612616,4123.39834189415,0.01543115102685988
871872,1743746,871873,2615619,4128.554255962372,0.015408698438477586
872873,1745748,872874,2618622,4133.630530118942,0.015384998519948567
873874,1747750,873875,2621625,4138.766978025436,0.01536263652087655
874875,1749752,874876,2624628,4143.885117053986,0.015340115813160082
875876,1751754,875877,2627631,4149.019075155258,0.015317424542445224
876877,1753756,876878,2630634,4154.102138996124,0.01529539241528255
877878,1755758,877879,2633637,4159.14902305603,0.015272579477823456
878879,1757760,878880,2636640,4164.243474006653,0.015250306414600345
879880,1759762,879881,2639643,4169.373923063278,0.015227724621581729
880881,1761764,880882,2642646,4174.4378299713135,0.0152056121150963
881882,1763766,881883,2645649,4179.542949914932,0.015183518418780295
882883,1765768,882884,2648652,4184.604154825211,0.015160993341851281
883884,1767770,883885,2651655,4189.648718118668,0.015138812648729072
884885,1769772,884886,2654658,4194.745015144348,0.0151165903389483
885886,1771774,885887,2657661,4199.979943037033,0.015093827760210843
886887,1773776,886888,2660664,4205.039128065109,0.015071400597662432
887888,1775778,887889,2663667,4210.142323970795,0.01504968779590854
888889,1777780,888890,2666670,4215.247072935104,0.015027497320261318
889890,1779782,889891,2669673,4220.356239080429,0.0150053524885152
890891,1781784,890892,2672676,4225.431928157806,0.014983353137722588
891892,1783786,891893,2675679,4230.581293106079,0.0149615927166451
892893,1785788,892894,2678682,4235.657039880753,0.014939856439013965
893894,1787790,893895,2681685,4240.723741054535,0.014917786007572431
894895,1789792,894896,2684688,4245.828486919403,0.014895786367560504
895896,1791794,895897,2687691,4250.903079986572,0.014873959384203772
896897,1793796,896898,2690694,4255.965214014053,0.014852244648864144
897898,1795798,897899,2693697,4261.032084941864,0.014830353493380244
898899,1797800,898900,2696700,4266.08957695961,0.0148088260248187
899900,1799802,899901,2699703,4271.171262025833,0.014787133470235858
900901,1801804,900902,2702706,4276.225015163422,0.014766357569897082
901902,1803806,901903,2705709,4281.274971961975,0.014744889065696043
902903,1805808,902904,2708712,4286.358780860901,0.01472325760187232
903904,1807810,903905,2711715,4291.455300807953,0.014702588703585207
904905,1809812,904906,2714718,4296.587146997452,0.014680973634312977
905906,1811814,905907,2717721,4301.702888011932,0.01466020716179628
906907,1813816,906908,2720724,4306.84165096283,0.014638854523582268
907908,1815818,907909,2723727,4311.969553947449,0.014618471917856368
908909,1817820,908910,2726730,4317.004378795624,0.014596956822060747
909910,1819822,909911,2729733,4322.08340716362,0.014576108049368486
910911,1821824,910912,2732736,4327.1218910217285,0.014555144482073956
911912,1823826,911913,2735739,4332.20153093338,0.014534422494762111
912913,1825828,912914,2738742,4337.231876134872,0.01451347226065991
913914,1827830,913915,2741745,4342.263226985931,0.014493131051494856
914915,1829832,914916,2744748,4347.34670996666,0.014472658282102202
915916,1831834,915917,2747751,4352.427247047424,0.014451878218096681
916917,1833836,916918,2750754,4357.52149605751,0.014431131934543373
917918,1835838,917919,2753757,4362.566132068634,0.014410289248189656
918919,1837840,918920,2756760,4367.644317865372,0.014389462487088167
919920,1839842,919921,2759763,4372.737969875336,0.014369398088092566
920921,1841844,920922,2762766,4377.693478822708,0.014349069979289197
921922,1843846,921923,2765769,4382.669604063034,0.014328979401398101
922923,1845848,922924,2768772,4387.799116134644,0.014309152860732866
923924,1847850,923925,2771775,4392.912702083588,0.0142889055859996
924925,1849852,924926,2774778,4397.85480594635,0.01426850606003427
925926,1851854,925927,2777781,4402.904017925262,0.014247683300709468
926927,1853856,926928,2780784,4407.955713033676,0.014226935265469365
927928,1855858,927929,2783787,4413.071985006332,0.014206585601641564
928929,1857860,928930,2786790,4418.1576471328735,0.014186792506734491
929930,1859862,929931,2789793,4423.2482759952545,0.014166029110128875
930931,1861864,930932,2792796,4428.26637005806,0.014145797760647838
931932,1863866,931933,2795799,4433.270223140717,0.014125997411611024
932933,1865868,932934,2798802,4438.30912899971,0.014105643009315827
933934,1867870,933935,2801805,4443.451858997345,0.014085241107750335
934935,1869872,934936,2804808,4448.546061038971,0.014065102272070362
935936,1871874,935937,2807811,4453.634725809097,0.014045045150851365
936937,1873876,936938,2810814,4458.65873003006,0.01402482492630952
937938,1875878,937939,2813817,4463.728119134903,0.014004706328705652
938939,1877880,938940,2816820,4468.779617071152,0.013984996505314484
939940,1879882,939941,2819823,4473.868222951889,0.013964926631160779
940941,1881884,940942,2822826,4478.926600933075,0.013945865739515284
941942,1883886,941943,2825829,4483.981558084488,0.013925866007411969
942943,1885888,942944,2828832,4489.05570101738,0.01390708944745711
943944,1887890,943945,2831835,4494.111169099808,0.013886947286664508
944945,1889892,944946,2834838,4499.232390880585,0.013867587411368731
945946,1891894,945947,2837841,4504.339838027954,0.013848298052835162
946947,1893896,946948,2840844,4509.452238082886,0.013829078243361437
947948,1895898,947949,2843847,4514.528733968735,0.013809987551212544
948949,1897900,948950,2846850,4520.523329973221,0.013790714954666328
949950,1899902,949951,2849853,4525.791663169861,0.013771430833003251
950951,1901904,950952,2852856,4530.928453922272,0.013752439288509777
951952,1903906,951953,2855859,4536.030052185059,0.013732727642491227
952953,1905908,952954,2858862,4541.160413980484,0.013712737549212761
953954,1907910,953955,2861865,4546.317992925644,0.013693695500478498
954955,1909912,954956,2864868,4551.398238897324,0.013674060754055972
955956,1911914,955957,2867871,4556.570384979248,0.013654651314936928
956957,1913916,956958,2870874,4561.642952919006,0.013635697403515223
957958,1915918,957959,2873877,4566.692248106003,0.013616412947158096
958959,1917920,958960,2876880,4571.783644914627,0.013597691042377846
959960,1919922,959961,2879883,4576.915172100067,0.01357834760165133
960961,1921924,960962,2882886,4582.020961046219,0.013559566465119133
961962,1923926,961963,2885889,4587.100341081619,0.013540189203922637
962963,1925928,962964,2888892,4592.1946840286255,0.013521358330763178
963964,1927930,963965,2891895,4597.277769088745,0.013503047406629776
964965,1929932,964966,2894898,4602.369556903839,0.013484580373187782
965966,1931934,965967,2897901,4607.4918830394745,0.01346570071655151
966967,1933936,966968,2900904,4612.5626718997955,0.013447053257550579
967968,1935938,967969,2903907,4617.533753156662,0.013427770480120671
968969,1937940,968970,2906910,4622.566130876541,0.013409364015387837
969970,1939942,969971,2909913,4627.662883043289,0.013391120599408168
970971,1941944,970972,2912916,4632.751710891724,0.01337333478841174
971972,1943946,971973,2915919,4637.705342054367,0.013354957865885808
972973,1945948,972974,2918922,4642.73305606842,0.01333652027642529
973974,1947950,973975,2921925,4647.766247034073,0.013318349809196661
974975,1949952,974976,2924928,4652.946713924408,0.013300056149091688
975976,1951954,975977,2927931,4658.085014104843,0.013281990361065255
976977,1953956,976978,2930934,4663.202142953873,0.0132636335438292
977978,1955958,977979,2933937,4668.257688999176,0.013245369496871717
978979,1957960,978980,2936940,4673.34935593605,0.013227413361164508
979980,1959962,979981,2939943,4678.409354925156,0.01320918763121881
980981,1961964,980982,2942946,4683.492333173752,0.013191154957894469
981982,1963966,981983,2945949,4688.6017780303955,0.013172833843782428
982983,1965968,982984,2948952,4693.656134843826,0.013154374362784438
983984,1967970,983985,2951955,4698.720791101456,0.013136908972228412
984985,1969972,984986,2954958,4703.769487142563,0.013118996857883758
985986,1971974,985987,2957961,4709.264213085175,0.013101335749524878
986987,1973976,986988,2960964,4714.362923145294,0.013083759789878968
987988,1975978,987989,2963967,4719.4905071258545,0.013066122961390647
988989,1977980,988990,2966970,4724.595649957657,0.013048490749497432
989990,1979982,989991,2969973,4729.699789047241,0.013030834859819151
990991,1981984,990992,2972976,4734.866631031036,0.013012743198487442
991992,1983986,991993,2975979,4739.99410200119,0.012995333854632918
992993,1985988,992994,2978982,4745.122359991074,0.01297767075629963
993994,1987990,993995,2981985,4750.418992996216,0.012960078045580303
994995,1989992,994996,2984988,4755.540995121002,0.01294264793250477
995996,1991994,995997,2987991,4760.665301084518,0.01292502881551627
996997,1993996,996998,2990994,4765.802766084671,0.012907340180390747
997998,1995998,997999,2993997,4771.116171121597,0.012890412088381709
998999,1998000,999000,2997000,4776.185784101486,0.012873223600763595
1000000,2000002,1000001,3000003,4781.300567150116,0.012855969429438119


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0041158199310302734,12064.44795143716
1001,2003,2002,4005,3.324941635131836,17.92880950331164
2002,4005,4004,8009,6.630133867263794,16.401999899311704
3003,6007,6006,12013,10.223201990127563,15.070671778463293
4004,8009,8008,16017,13.486610889434814,13.902342173496436
5005,10011,10010,20021,16.71485686302185,12.871259313851624
6006,12013,12012,24025,20.087517976760864,11.956797952941997
7007,14015,14014,28029,23.67992377281189,11.142266176926569
8008,16017,16016,32033,27.441759824752808,10.413826686319226
9009,18019,18018,36037,30.956442832946777,9.760046656858322
10010,20021,20020,40041,34.775346755981445,9.171386866471948
11011,22023,22022,44045,38.70197296142578,8.639782031601499
12012,24025,24024,48049,42.04182505607605,8.158381768433173
13013,26027,26026,52053,46.04702591896057,7.721333615045296
14014,28029,28028,56057,50.85399079322815,7.323603309418104
15015,30031,30030,60061,54.865328788757324,6.960836875367022
16016,32033,32032,64065,59.13472366333008,6.629250251957274
17017,34035,34034,68069,63.31971788406372,6.3255402110498835
18018,36037,36036,72073,67.14822196960449,6.046811860220259
19019,38039,38038,76077,70.96784996986389,5.790519169438994
20020,40041,40040,80081,76.05370378494263,5.55441580515253
21021,42043,42042,84085,80.11780667304993,5.336514185966735
22022,44045,44044,88089,84.58468580245972,5.135051147446575
23023,46047,46046,92093,88.50550174713135,4.948458960898279
24024,48049,48048,96097,92.02466893196106,4.77534072236449
25025,50051,50050,100101,95.72560000419617,4.614449335365862
26026,52053,52052,104105,99.34877276420593,4.464669470045919
27027,54055,54054,108109,102.66942572593689,4.325002004370617
28028,56057,56056,112113,106.3328697681427,4.194550548676489
29029,58059,58058,116117,109.63951373100281,4.072509729601734
30030,60061,60060,120121,113.11764788627625,3.9581549682989134
31031,62063,62062,124125,116.5249457359314,3.850833534499543
32032,64065,64064,128129,119.72111582756042,3.7499566952210444
33033,66067,66066,132133,123.18446278572083,3.6549960559823376
34034,68069,68068,136137,127.53291082382202,3.5654789983273076
35035,70071,70070,140141,131.82025861740112,3.48095852951883
36036,72073,72072,144145,136.16951179504395,3.401040469940199
37037,74075,74074,148149,140.3315508365631,3.3253672696118883
38038,76077,76076,152153,144.3822226524353,3.2536142538538115
39039,78079,78078,156157,148.35342693328857,3.1854862845193566
40040,80081,80080,160161,152.07024002075195,3.12071478695907
41041,82083,82082,164165,156.2957158088684,3.0590550995293597
42042,84085,84084,168169,160.0401737689972,3.0002841079913196
43043,86087,86086,172173,163.79556584358215,2.944198131977828
44044,88089,88088,176177,167.36362481117249,2.8906110348489165
45045,90091,90090,180181,171.55208587646484,2.839352531671466
46046,92093,92092,184185,175.83548998832703,2.790266673255246
47047,94095,94094,188189,180.2948169708252,2.7432104867111775
48048,96097,96096,192193,184.3102147579193,2.6980527553678257
49049,98099,98098,196197,188.35195064544678,2.6546729228812183
50050,100101,100100,200201,191.87412190437317,2.6129601080592693
51051,102103,102102,204205,195.75852489471436,2.5728122185937536
52052,104105,104104,208209,199.43206882476807,2.5341351530551037
53053,106107,106106,212213,203.36970806121826,2.4968420819113817
54054,108109,108108,216217,206.70710277557373,2.4608527991731535
55055,110111,110110,220221,210.3947787284851,2.426094178099447
56056,112113,112112,224225,214.15370178222656,2.3924973407592915
57057,114115,114114,228229,218.60742092132568,2.3599977922349353
58058,116117,116116,232233,222.77012491226196,2.3285365085448575
59059,118119,118118,236237,226.79618096351624,2.2980586779831356
60060,120121,120120,240241,230.12700176239014,2.2685133439390484
61061,122123,122122,244245,233.8624119758606,2.2398530838327133
62062,124125,124124,248249,237.82881379127502,2.2120337177875626
63063,126127,126126,252253,241.49989295005798,2.18501404412018
64064,128129,128128,256257,245.23371386528015,2.1587555990008696
65065,130131,130130,260261,248.8006546497345,2.1332224378129467
66066,132133,132132,264265,252.577565908432,2.108380936218964
67067,134135,134134,268269,256.91417384147644,2.084199608894778
68068,136137,136136,272273,260.4874439239502,2.060648944305285
69069,138139,138138,276277,264.47605085372925,2.0377012539447605
70070,140141,140140,280281,268.16710591316223,2.0153305346648267
71071,142143,142142,284285,271.82746291160583,1.993512342860413
72072,144145,144144,288289,275.6107017993927,1.9722236793841148
73073,146147,146146,292293,279.2464928627014,1.951442884208518
74074,148149,148148,296297,282.7101628780365,1.9311495398887928
75075,150151,150150,300301,286.18091797828674,1.911324383065221
76076,152153,152152,304305,289.49778985977173,1.8919492232271296
77077,154155,154154,308309,292.97616481781006,1.8730068681143166
78078,156157,156156,312313,296.9077696800232,1.8544810551120463
79079,158159,158158,316317,300.66420578956604,1.8363563881612208
80080,160161,160160,320321,303.91416788101196,1.8186182796343928
81081,162163,162162,324325,307.1186807155609,1.8012528967847174
82082,164165,164164,328329,310.3492269515991,1.7842471123440191
83083,166167,166166,332333,313.6125648021698,1.7675884589152702
84084,168169,168168,336337,317.30382895469666,1.7512650868393393
85085,170171,170170,340341,320.7290508747101,1.7352680557069107
86086,172173,172172,344345,324.80642676353455,1.7195843450936081
87087,174175,174174,348349,328.9288697242737,1.7042035396716528
88088,176177,176176,352353,332.7513380050659,1.689115905761355
89089,178179,178178,356357,336.619993686676,1.6743121591498493
90090,180181,180180,360361,341.02839970588684,1.6597834384137968
91091,182183,182182,364365,344.8284306526184,1.645521280112007
92092,184185,184184,368369,348.0961380004883,1.631517595727928
93093,186187,186186,372373,351.4033269882202,1.6177646502110292
94094,188189,188188,376377,354.8166558742523,1.6042550419915642
95095,190191,190190,380381,358.0861837863922,1.5909816843413864
96096,192193,192192,384385,361.6288409233093,1.5779377880044194
97097,194195,194194,388389,365.25761580467224,1.5651168449712713
98098,196197,196196,392393,368.90152978897095,1.5525126133215963
99099,198199,198198,396397,372.5045759677887,1.5401191030505288
100100,200201,200200,400401,375.78626465797424,1.527930562824622
101101,202203,202202,404405,379.2514708042145,1.5159414675545122
102102,204205,204204,408409,382.9693019390106,1.5041465067697573
103103,206207,206206,412413,386.5322186946869,1.4925405737230903
104104,208209,208208,416417,390.09463381767273,1.4811187551531475
105105,210211,210210,420421,393.40246391296387,1.4698763216802035
106106,212213,212212,424425,396.6301517486572,1.4588087187821657
107107,214215,214214,428429,400.2193078994751,1.4479115583144448
108108,216217,216216,432433,403.4312677383423,1.4371806105209544
109109,218219,218218,436437,406.6360728740692,1.4266117965325975
110110,220221,220220,440441,409.825532913208,1.4162011812804849
111111,222223,222222,444445,413.05437898635864,1.4059449668202433
112112,224225,224224,448449,416.2739977836609,1.3958394860655972
113113,226227,226226,452453,419.4558298587799,1.3858811968220834
114114,228229,228228,456457,422.6840350627899,1.376066676202754
115115,230231,230230,460461,425.90293192863464,1.3663926153112698
116116,232233,232232,464465,429.1213538646698,1.3568558142560505
117117,234235,234234,468469,432.3138370513916,1.3474531773990748
118118,236237,236236,472473,435.5760450363159,1.3381817088811658
119119,238239,238238,476477,438.81749081611633,1.3290385083746514
120120,240241,240240,480481,442.1486117839813,1.3200207670543023
121121,242243,242242,484485,445.3962998390198,1.3111257637920062
122122,244245,244244,488489,448.5914077758789,1.3023508615460742
123123,246247,246246,492493,451.800345659256,1.2936935039178934
124124,248249,248248,496497,454.9857647418976,1.2058881962057058
125125,250251,250250,500501,458.18637681007385,1.1984658891433355
126126,252253,252252,504505,461.6445598602295,1.191133968279246
127127,254255,254254,508509,464.91990971565247,1.1838907270266645
128128,256257,256256,512513,468.2354938983917,1.1767345040207147
129129,258259,258258,516517,472.9939639568329,1.1696636815649981
130130,260261,260260,520521,477.83856678009033,1.1626766841054632
131131,262263,262262,524525,482.7037079334259,1.1557719767952221
132132,264265,264264,528529,486.6636378765106,1.1489480640902912
133133,266267,266266,532533,490.45665669441223,1.142203488458108
134134,268269,268268,536537,494.02960205078125,1.1355368290678598
135135,270271,270270,540541,497.6901879310608,1.1289467006063205
136136,272273,272272,544545,500.9822647571564,1.1224317520864133
137137,274275,274274,548549,504.4122910499573,1.1159906657485408
138138,276277,276276,552553,507.9495987892151,1.1096221559782862
139139,278279,278278,556557,511.2153947353363,1.1033249682732276
140140,280281,280280,560561,514.5224659442902,1.0970978782679595
141141,282283,282282,564565,517.7735288143158,1.0909396907627524
142142,284285,284284,568569,520.9895269870758,1.0848492388395243
143143,286287,286286,572573,524.1599490642548,1.0788253829614405
144144,288289,288288,576577,527.635321855545,1.0728670101452735
145145,290291,290290,580581,531.0791099071503,1.0669730331446772
146146,292293,292292,584585,534.7461287975311,1.0611423896771157
147147,294295,294294,588589,539.8920576572418,1.0553740416671644
148148,296297,296296,592593,543.435183763504,1.0496669745298277
149149,298299,298298,596597,546.7762968540192,1.0440201964811422
150150,300301,300300,600601,550.2225368022919,1.0384327378560556
151151,302303,302302,604605,553.8503308296204,1.0329036504735996
152152,304305,304304,608609,557.2358620166779,1.02743200702389
153153,306307,306306,612613,560.4129078388214,1.022016900449671
154154,308309,308308,616617,563.6492767333984,1.016657443382428
155155,310311,310310,620621,567.7310807704926,1.0113527675894147
156156,312313,312312,624625,572.3401217460632,1.0061020234279567
157157,314315,314314,628629,577.3512289524078,1.0009043793288583
158158,316317,316316,632633,581.032461643219,0.9957590213089134
159159,318319,318318,636637,584.3221907615662,0.9906651524652261
160160,320321,320320,640641,587.8244769573212,0.985621992533197
161161,322323,322322,644645,591.7850968837738,0.9806287774190423
162162,324325,324324,648649,595.5266859531403,0.9756847587741504
163163,326327,326326,652653,599.6498627662659,0.9707892035712575
164164,328329,328328,656657,604.208646774292,0.965941393706089
165165,330331,330330,660661,608.923811674118,0.9611406255789916
166166,332333,332332,664665,612.881454706192,0.9563862097511446
167167,334335,334334,668669,616.5729279518127,0.9516774705534772
168168,336337,336336,672673,620.6299998760223,0.9470137457337842
169169,338339,338338,676677,625.1332867145538,0.9423943861129374
170170,340341,340340,680681,628.8158609867096,0.9378187552629242
171171,342343,342342,684685,632.2945778369904,0.933286229166697
172172,344345,344344,688689,635.7035520076752,0.9287961959198583
173173,346347,346346,692693,639.0017538070679,0.924348055414157
174174,348349,348348,696697,642.5461559295654,0.9199412190591829
175175,350351,350350,700701,646.2068059444427,0.9155751094895095
176176,352353,352352,704705,650.5352230072021,0.9112491602882073
177177,354355,354354,708709,653.9783086776733,0.9069628157230909
178178,356357,356356,712713,658.8707618713379,0.9027155304866028
179179,358359,358358,716717,663.6995067596436,0.8985067694466125
180180,360361,360360,720721,668.5300738811493,0.8943360073972144
181181,362363,362362,724725,672.9234209060669,0.8902027288295358
182182,364365,364364,728729,676.8934090137482,0.8861064276970865
183183,366367,366366,732733,681.7767198085785,0.8820466071865667
184184,368369,368368,736737,686.706536769867,0.8780227795232349
185185,370371,370370,740741,690.308671951294,0.8740344657362584
186186,372373,372372,744745,693.8199667930603,0.8700811954713572
187187,374375,374374,748749,698.2579047679901,0.8661625067816203
188188,376377,376376,752753,702.2339887619019,0.8622779459437879
189189,378379,378378,756757,705.7588078975677,0.8584270672672574
190190,380381,380380,760761,709.497368812561,0.8546094329121843
191191,382383,382382,764765,713.5711879730225,0.8508246127112216
192192,384385,384384,768769,718.0500726699829,0.8470721840039914
193193,386387,386386,772773,721.9442648887634,0.8433517314606434
194194,388389,388388,776777,726.0648078918457,0.83966284692724
195195,390391,390390,780781,731.680253982544,0.8360051292675053
196196,392393,392392,784785,735.4549238681793,0.8323781842045719
197197,394395,394394,788789,738.8122527599335,0.8287816241700057
198198,396397,396396,792793,742.8294429779053,0.8006585201146663
199199,398399,398398,796797,747.5361127853394,0.7973228817372728
200200,400401,400400,800801,751.9038078784943,0.7940140466398589
201201,402403,402402,804805,755.4648959636688,0.790731693017733
202202,404405,404404,808809,758.8297426700592,0.7874755042375909
203203,406407,406406,812813,762.526930809021,0.7842451687556604
204204,408409,408408,816817,766.5029847621918,0.7810403799903725
205205,410411,410410,820821,770.5114579200745,0.7778608362368686
206206,412413,412412,824825,774.3705847263336,0.7747062405578617
207207,414415,414414,828829,778.3196406364441,0.7715763007017813
208208,416417,416416,832833,782.0509879589081,0.7684707289954531
209209,418419,418418,836837,785.807089805603,0.7653892422640638
210210,420421,420420,840841,789.129576921463,0.7623315617347544
211211,422423,422422,844845,792.8498718738556,0.7592974129565846
212212,424425,424424,848849,796.6503069400787,0.7562865257023077
213213,426427,426426,852853,800.4470720291138,0.7532986339065246
214214,428429,428428,856857,804.5177438259125,0.7503334755710966
215215,430431,430430,860861,808.843475818634,0.7473907926887478
216216,432433,432432,864865,813.6537280082703,0.7444703311630292
217217,434435,434434,868869,817.6274697780609,0.7415718407410168
218218,436437,436436,872873,821.996090888977,0.7386950749405514
219219,438439,438438,876877,826.4506378173828,0.7358397909683845
220220,440441,440440,880881,830.9624879360199,0.7330057496583322
221221,442443,442442,884885,835.2373778820038,0.7301927153985162
222222,444445,444444,888889,839.5415060520172,0.7274004560713365
223223,446447,446446,892893,843.3176918029785,0.7246287429843505
224224,448449,448448,896897,847.1073698997498,0.7218773507993319
225225,450451,450450,900901,852.0985679626465,0.7191460574849771
226226,452453,452452,904905,857.6403877735138,0.7164346442441456
227227,454455,454454,908909,862.0304179191589,0.7137428954592906
228228,456457,456456,912913,866.2176048755646,0.7110706113708147
229229,458459,458458,916917,870.1368708610535,0.7084176078114979
230230,460461,460460,920921,874.3818647861481,0.7057836423027766
231231,462463,462462,924925,878.2574646472931,0.7031685113088315
232232,464465,464464,928929,883.5893890857697,0.7005720141951315
233233,466467,466466,932933,887.5309250354767,0.6979939531720447
234234,468469,468468,936937,891.0923347473145,0.69543413325664
235235,470471,470470,940941,894.8885507583618,0.6928923622126604
236236,472473,472472,944945,898.7092039585114,0.6903684505032288
237237,474475,474474,948949,902.453795671463,0.687862211249012
238238,476477,476476,952953,906.0678288936615,0.6853734601718315
239239,478479,478478,956957,910.1148347854614,0.6829020155528269
240240,480481,480480,960961,913.9672248363495,0.6804476981978951
241241,482483,482482,964965,917.9687879085541,0.6780103313740256
242242,484485,484484,968969,921.9592278003693,0.6755897407892917
243243,486487,486486,972973,925.6251268386841,0.673185754523729
244244,488489,488488,976977,929.1665637493134,0.6707982030166022
245245,490491,490490,980981,933.034717798233,0.6684269190118357
246246,492493,492492,984985,936.5925559997559,0.6660717375089007
247247,494495,494494,988989,940.1783969402313,0.6637324957537203
248248,496497,496496,992993,944.2013058662415,0.661409033162272
249249,498499,498498,996997,948.4024839401245,0.6591011913187685
250250,500501,500500,1001001,952.173889875412,0.6568088139156316
251251,502503,502502,1005005,956.2669937610626,0.6545317467353016
252252,504505,504504,1009009,959.8834018707275,0.6522698375993059
253253,506507,506506,1013013,963.2590379714966,0.6500229363446124
254254,508509,508508,1017017,967.0817520618439,0.6477908947890683
255255,510511,510510,1021021,970.8757948875427,0.6455735666968394
256256,512513,512512,1025025,974.6752030849457,0.6433708077438496
257257,514515,514514,1029029,978.2858469486237,0.6411824754923146
258258,516517,516516,1033033,981.8917548656464,0.6390084293543623
259259,518519,518518,1037037,985.7488157749176,0.6368485305683862
260260,520521,520520,1041041,989.1861748695374,0.6347026421608462
261261,522523,522522,1045045,992.4754590988159,0.6325706289244408
262262,524525,524524,1049049,995.7813267707825,0.6304523573817278
263263,526527,526526,1053053,999.3207778930664,0.6283476957742096
264264,528529,528528,1057057,1002.9319317340851,0.62625651401504
265265,530531,530530,1061061,1006.2803666591644,0.6241786836671963
266266,532533,532532,1065065,1009.9811868667603,0.6221140779271082
267267,534535,534534,1069069,1013.9625227451324,0.6200664479729312
268268,536537,536536,1073073,1018.9425799846649,0.6180325114873995
269269,538539,538538,1077077,1023.6329107284546,0.6160115079728712
270270,540541,540540,1081081,1027.6393427848816,0.6140032741277537
271271,542543,542542,1085085,1032.5578680038452,0.612007665235069
272272,544545,544544,1089089,1036.5431008338928,0.6100245481538877
273273,546547,546546,1093093,1040.628928899765,0.6080537972666207
274274,548549,548548,1097097,1044.3775389194489,0.6060952920797718
275275,550551,550550,1101101,1047.738163948059,0.6041489158014883
276276,552553,552552,1105105,1052.357260942459,0.6022145544284285
277277,554555,554554,1109109,1056.2178449630737,0.6002920962146163
278278,556557,556556,1113113,1059.5908846855164,0.5983814313203766
279279,558559,558558,1117117,1064.7304317951202,0.5964824515740474
280280,560561,560560,1121121,1068.1757838726044,0.5945989224783261
281281,562563,562562,1125125,1071.9927887916565,0.592727324412408
282282,564565,564564,1129129,1075.5849568843842,0.5908671640045213
283283,566567,566566,1133133,1079.1380050182343,0.589018285030761
284284,568569,568568,1137137,1084.83500790596,0.587180562901267
285285,570571,570570,1141141,1089.4366698265076,0.5853538873197976
286286,572573,572572,1145145,1094.51238489151,0.5835381549222802
287287,574575,574574,1149149,1098.6729667186737,0.5817332660644752
288288,576577,576576,1153153,1102.105204820633,0.5799391234213545
289289,578579,578578,1157157,1106.4149029254913,0.5781556313340843
290290,580581,580580,1161161,1110.857988834381,0.57638269553172
291291,582583,582582,1165165,1114.5154139995575,0.5746202229674964
292292,584585,584584,1169169,1118.6037440299988,0.5728681217588019
293293,586587,586586,1173173,1122.8781349658966,0.5711263011271512
294294,588589,588588,1177177,1127.0753998756409,0.569394671379996
295295,590591,590590,1181181,1130.9752397537231,0.5676731438688876
296296,592593,592592,1185185,1135.4399280548096,0.5659616309876583
297297,594595,594594,1189189,1139.8837478160858,0.5642600461487746
298298,596597,596596,1193193,1143.6044127941132,0.562568303756052
299299,598599,598598,1197197,1148.0008687973022,0.5608863192082936
300300,600601,600600,1201201,1152.5375957489014,0.5592140088720043
301301,602603,602602,1205205,1156.7624158859253,0.557551290061383
302302,604605,604604,1209209,1160.770537853241,0.5558980810383218
303303,606607,606606,1213213,1165.1745216846466,0.5542543009887595
304304,608609,608608,1217217,1169.6184928417206,0.5526198700154055
305305,610611,610610,1221221,1174.0004658699036,0.550994709114093
306306,612613,612612,1225225,1178.324185848236,0.5493787401737791
307307,614615,614614,1229229,1182.2744088172913,0.5477718859565357
308308,616617,616616,1233233,1185.8036358356476,0.5461740700829978
309309,618619,618618,1237237,1189.2868168354034,0.5445852170305443
310310,620621,620620,1241241,1193.5482187271118,0.5430052521096513
311311,622623,622622,1245245,1198.021714925766,0.5414341014566162
312312,624625,624624,1249249,1202.3812339305878,0.5398716920262814
313313,626627,626626,1253253,1206.624452829361,0.5383179515720258
314314,628629,628628,1257257,1210.6311378479004,0.5367728086475836
315315,630631,630630,1261261,1214.682848930359,0.5352361925797595
316316,632633,632632,1265265,1219.0255496501923,0.5337080334684288
317317,634635,634634,1269269,1223.4383099079132,0.5321882621774421
318318,636637,636636,1273273,1227.872309923172,0.5306768103182549
319319,638639,638638,1277277,1231.9106287956238,0.5291736102390132
320320,640641,640640,1281281,1235.9528419971466,0.5276785950245539
321321,642643,642642,1285285,1239.651175737381,0.5261916984727577
322322,644645,644644,1289289,1243.2435009479523,0.524712855098187
323323,646647,646646,1293293,1246.887461900711,0.5232420001102582
324324,648649,648648,1297297,1250.5796809196472,0.5217790694132418
325325,650651,650650,1301301,1254.0643157958984,0.5203239995935292
326326,652653,652652,1305305,1257.6226449012756,0.5188767279105377
327327,654655,654654,1309309,1261.3220298290253,0.5174371922857972
328328,656657,656656,1313313,1264.8095967769623,0.5160053312956734
329329,658659,658658,1317317,1268.262764930725,0.5145810841713683
330330,660661,660660,1321321,1271.8544147014618,0.5131643907734542
331331,662663,662662,1325325,1276.769453048706,0.5117551915955119
332332,664665,664664,1329329,1281.7848727703094,0.5103534277532162
333333,666667,666666,1333333,1287.2740919589996,0.5089590409752418
334334,668669,668668,1337337,1292.098040819168,0.5075719735978055
335335,670671,670670,1341341,1296.275075674057,0.5061921685537527
336336,672673,672672,1345345,1300.1250019073486,0.5048195693598245
337337,674675,674674,1349349,1303.580547094345,0.5034541201312095
338338,676677,676676,1353353,1307.7742857933044,0.5020957655415259
339339,678679,678678,1357357,1315.721935749054,0.5007444508391927
340340,680681,680680,1361361,1320.444816827774,0.49940012183287763
341341,682683,682682,1365365,1325.2421298027039,0.4980627248842211
342342,684685,684684,1369369,1329.656350851059,0.4967322068987414
343343,686687,686686,1373373,1335.575157880783,0.4954085153294727
344344,688689,688688,1377377,1339.6985578536987,0.4940915981460421
345345,690691,690690,1381381,1343.9325637817383,0.49278140386195446
346346,692693,692692,1385385,1347.9146358966827,0.4914778814982128
347347,694695,694694,1389389,1352.0370228290558,0.4901809805905941
348348,696697,696696,1393393,1357.4650647640228,0.4888906511805544
349349,698699,698698,1397397,1362.3820507526398,0.4876068438115908
350350,700701,700700,1401401,1367.7355320453644,0.48632950951832754
351351,702703,702702,1405405,1372.339558839798,0.485058599830154
352352,704705,704704,1409409,1376.4531137943268,0.48379406674393977
353353,706707,706706,1413413,1382.4526557922363,0.4825358627440437
354354,708709,708708,1417417,1387.7686078548431,0.4812839407786669
355355,710711,710710,1421421,1392.1185657978058,0.4800382542616717
356356,712713,712712,1425425,1396.5254809856415,0.4787987570671248
357357,714715,714714,1429429,1400.9866807460785,0.4775654035147454
358358,716717,716716,1433433,1406.0982458591461,0.4763381483753619
359359,718719,718718,1437437,1411.6822409629822,0.47511694686545525
360360,720721,720720,1441441,1416.2734189033508,0.47390175463078776
361361,722723,722722,1445445,1420.8931000232697,0.4726925277518603
362362,724725,724724,1449449,1425.4123587608337,0.4714892227311793
363363,726727,726726,1453453,1431.0877847671509,0.47029179649871367
364364,728729,728728,1457457,1436.5228867530823,0.4691002063882479
365365,730731,730730,1461461,1442.044564962387,0.4679144101555721
366366,732733,732732,1465465,1447.8734579086304,0.46673436595847306
367367,734735,734734,1469469,1452.9658377170563,0.4655600323494582
368368,736737,736736,1473473,1458.1136498451233,0.4643913682866696
369369,738739,738738,1477477,1463.0914158821106,0.46322833311023714
370370,740741,740740,1481481,1468.2335050106049,0.4620708865550114
371371,742743,742742,1485485,1475.2202229499817,0.46091898872509773
372372,744745,744744,1489489,1481.5091440677643,0.4597726001211413
373373,746747,746746,1493493,1487.6842679977417,0.4586316815984901
374374,748749,748748,1497497,1494.4154307842255,0.457496194392661
375375,750751,750750,1501501,1500.6838960647583,0.45636610009751166
376376,752753,752752,1505505,1507.2555058002472,0.45524136066887877
377377,754755,754754,1509509,1514.7166168689728,0.45412193841912085
378378,756757,756756,1513513,1521.6667687892914,0.4530077960098424
379379,758759,758758,1517517,1527.1572227478027,0.45189889645371295
380380,760761,760760,1521521,1533.4854528903961,0.45079520310173393
381381,762763,762762,1525525,1540.0162868499756,0.4496966796468769
382382,764765,764764,1529529,1544.4858798980713,0.4486032901240833
383383,766767,766766,1533533,1549.5390558242798,0.44751499888661783
384384,768769,768768,1537537,1554.6188459396362,0.44643177063153416
385385,770771,770770,1541541,1559.3165807724,0.44535357036329515
386386,772773,772772,1545545,1563.2846639156342,0.4442803634210577
387387,774775,774774,1549549,1566.9910509586334,0.4432121154568449
388388,776777,776776,1553553,1570.8058428764343,0.4421487924282701
389389,778779,778778,1557557,1574.4296338558197,0.4410903606094507
390390,780781,780780,1561561,1578.0822179317474,0.4400367865800945
391391,782783,782782,1565565,1582.1022758483887,0.4389880372254993
392392,784785,784784,1569569,1586.2350850105286,0.43794407972200133
393393,786787,786786,1573573,1590.2301638126373,0.4369048815497081
394394,788789,788788,1577577,1594.7154307365417,0.4358704104779463
395395,790791,790790,1581581,1598.8912320137024,0.43484063455980504
396396,792793,792792,1585585,1603.030954837799,0.4338155221485067
397397,794795,794794,1589589,1606.7308809757233,0.4327950418664841
398398,796797,796796,1593593,1610.7494938373566,0.4317791626217513
399399,798799,798798,1597597,1614.650382757187,0.43076785359880887
400400,800801,800800,1601601,1619.0070457458496,0.4297610842531867
401401,802803,802802,1605605,1623.0202569961548,0.42875882431690115
402402,804805,804804,1609609,1627.102255821228,0.427761043780265
403403,806807,806806,1613613,1632.5093927383423,0.42676771289370663
404404,808809,808808,1617617,1636.949308872223,0.4257788021641318
405405,810811,810810,1621621,1640.6492178440094,0.42479428235674277
406406,812813,812812,1625625,1644.2109627723694,0.4238141244950384
407407,814815,814814,1629629,1647.768905878067,0.422838299857176
408408,816817,816816,1633633,1651.7398090362549,0.4218667799686955
409409,818819,818818,1637637,1656.2286348342896,0.42089953661161417
410410,820821,820820,1641641,1660.5043478012085,0.4199365418062371
411411,822823,822822,1645645,1664.8841667175293,0.41897776781843277
412412,824825,824824,1649649,1668.6724858283997,0.4180231871559954
413413,826827,826826,1653653,1672.7822136878967,0.41707277256500674
414414,828829,828828,1657657,1677.6370527744293,0.4161264970243792
415415,830831,830830,1661661,1682.5661268234253,0.41518433374585584
416416,832833,832832,1665665,1687.511513710022,0.41424625617401034
417417,834835,834834,1669669,1691.517413854599,0.4133122379771521
418418,836837,836836,1673673,1695.366348028183,0.4123822530509642
419419,838839,838838,1677677,1699.3428909778595,0.4114562755148654
420420,840841,840840,1681681,1703.0434937477112,0.4105342797065532
421421,842843,842842,1685685,1706.8292388916016,0.4096162401856418
422422,844845,844844,1689689,1710.4723420143127,0.40870213172456715
423423,846847,846846,1693693,1714.2975406646729,0.40779192930313
424424,848849,848848,1697697,1717.88631772995,0.40688560812486685
425425,850851,850850,1701701,1721.6449069976807,0.4059831435952219
426426,852853,852852,1705705,1725.2954549789429,0.4050845113233663
427427,854855,854854,1709709,1729.452096939087,0.4041896871276549
428428,856857,856856,1713713,1733.0219948291779,0.40329864703198837
429429,858859,858858,1717717,1736.5907068252563,0.4024113672476233
430430,860861,860860,1721721,1740.1389858722687,0.40152782420227595
431431,862863,862862,1725725,1743.5231947898865,0.4006479945019237
432432,864865,864864,1729729,1747.0380239486694,0.3997718549599085
433433,866867,866866,1733733,1750.5632908344269,0.3988993825732905
434434,868869,868868,1737737,1754.2332339286804,0.39803055453194247
435435,870871,870870,1741741,1757.8466589450836,0.3971653482167312
436436,872873,872872,1745745,1761.7935569286346,0.39630374118860345
437437,874875,874874,1749749,1765.9667358398438,0.3954457111976808
438438,876877,876876,1753753,1770.7700617313385,0.3945912361759838
439439,878879,878878,1757757,1775.1647357940674,0.393740294231975
440440,880881,880880,1761761,1778.788004875183,0.3928928636596538
441441,882883,882882,1765765,1782.7751557826996,0.39204892292036675
442442,884885,884884,1769769,1786.7211277484894,0.3912084506573592
443443,886887,886886,1773773,1790.5766878128052,0.3903714256848616
444444,888889,888888,1777777,1794.8417909145355,0.3895378269953653
445445,890891,890890,1781781,1799.8997039794922,0.38870763373415684
446446,892893,892892,1785785,1804.2881426811218,0.3878808252320596
447447,894895,894894,1789789,1807.9331016540527,0.387057380978149
448448,896897,896896,1793793,1812.4253330230713,0.38623728062702867
449449,898899,898898,1797797,1816.705058813095,0.3854205039970111
450450,900901,900900,1801801,1821.607677936554,0.384607031064661
451451,902903,902902,1805805,1826.7935559749603,0.38379684197388997
452452,904905,904904,1809809,1832.050853729248,0.38298991701594787
453453,906907,906906,1813813,1836.97913980484,0.38218623664761253
454454,908909,908908,1817817,1841.4663848876953,0.3742215231377486
455455,910911,910910,1821821,1846.0782489776611,0.36149026241037063
456456,912913,912912,1825825,1850.652662038803,0.3607718103121442
457457,914915,914914,1829829,1855.9738428592682,0.36005609045787423
458458,916917,916916,1833833,1861.9441299438477,0.3593430873934267
459459,918919,918918,1837837,1867.5956008434296,0.35863278577926394
460460,920921,920920,1841841,1873.147864818573,0.3579251703922637
461461,922923,922922,1845845,1878.210881948471,0.3572202261275379
462462,924925,924924,1849849,1883.3109438419342,0.356517937978424
463463,926927,926926,1853853,1887.5685648918152,0.3558182910637697
464464,928929,928928,1857857,1891.9712717533112,0.3551212706024671
465465,930931,930930,1861861,1896.3279390335083,0.3544268619389186
466466,932933,932932,1865865,1901.5897808074951,0.353735050508476
467467,934935,934934,1869869,1906.2153708934784,0.35304582185926847
468468,936937,936936,1873873,1910.3317527770996,0.3523591616540216
469469,938939,938938,1877877,1914.1164968013763,0.3516750556482293
470470,940941,940940,1881881,1918.8843219280243,0.35099348971198197
471471,942943,942942,1885885,1923.4185328483582,0.3503144498135953
472472,944945,944944,1889889,1927.5844378471375,0.3496379220250674
473473,946947,946946,1893893,1931.6891477108002,0.3489638925238978
474474,948949,948948,1897897,1935.4539608955383,0.34829234758035454
475475,950951,950950,1901901,1939.6212847232819,0.34762327357202594
476476,952953,952952,1905905,1943.6794559955597,0.3469566569710878
477477,954955,954954,1909909,1947.241882801056,0.3462924843533983
478478,956957,956956,1913913,1950.7584340572357,0.3456307423821272
479479,958959,958958,1917917,1954.743379831314,0.34497141782594554
480480,960961,960960,1921921,1958.3609399795532,0.34431449754447385
481481,962963,962962,1925925,1962.4050376415253,0.34365996849373914
482482,964965,964964,1929929,1966.1609318256378,0.34300781772253686
483483,966967,966966,1933933,1970.242925643921,0.3423580323706119
484484,968969,968968,1937937,1974.7275698184967,0.34171059967593465
485485,970971,970970,1941941,1978.7310078144073,0.34106550695651094
486486,972973,972972,1945945,1982.926727771759,0.34042274163584807
487487,974975,974974,1949949,1987.2708768844604,0.33978229121203185
488488,976977,976976,1953953,1991.5768308639526,0.33914414328319253
489489,978979,978978,1957957,1995.6968667507172,0.3385082855311339
490490,980981,980980,1961961,2000.8932490348816,0.33787470572315215
491491,982983,982982,1965965,2005.84791970253,0.3372433917138551
492492,984985,984984,1969969,2010.0364758968353,0.33661433144516195
493493,986987,986986,1973973,2013.882917881012,0.3359875129444845
494494,988989,988988,1977977,2018.040312051773,0.33536292432290793
495495,990991,990990,1981981,2022.0556569099426,0.3347405537751911
496496,992993,992992,1985985,2026.8820238113403,0.33412038957249024
497497,994995,994994,1989989,2031.6968128681183,0.3335024200787302
498498,996997,996996,1993993,2036.2201647758484,0.33288663372877636
499499,998999,998998,1997997,2040.556412935257,0.33227301904662454
500501,1001003,1001002,2002005,2044.8325397968292,0.3316609548674023
501502,1003005,1003004,2006009,2049.225912809372,0.33105165154302085
502503,1005007,1005006,2010013,2052.8892107009888,0.3304444859131763
503504,1007009,1007008,2014017,2056.5206730365753,0.3298394468129118
504505,1009011,1009010,2018021,2060.2105028629303,0.3292365231554868
505506,1011013,1011012,2022025,2063.9766159057617,0.3286357039323775
506507,1013015,1013014,2026029,2067.5822677612305,0.32803697820600064
507508,1015017,1015016,2030033,2071.2226388454437,0.3274403351206274
508509,1017019,1017018,2034037,2075.085922718048,0.3268457638896507
509510,1019021,1019020,2038041,2078.6903989315033,0.32625325380104186
510511,1021023,1021022,2042045,2082.3156168460846,0.32566279422098887
511512,1023025,1023024,2046049,2085.9722168445587,0.3250743745811633
512513,1025027,1025026,2050053,2089.667641878128,0.32448798438781523
513514,1027029,1027028,2054057,2093.295697927475,0.3239036132235924
514515,1029031,1029030,2058061,2096.918212890625,0.3233212507348071
515516,1031033,1031032,2062065,2100.5289237499237,0.3227408866441692
516517,1033035,1033034,2066069,2104.1426360607147,0.32216251073623425
517518,1035037,1035036,2070073,2108.056923866272,0.32158611287377425
518519,1037039,1037038,2074077,2111.725907802582,0.32101168297958793
519520,1039041,1039040,2078081,2115.315244913101,0.32043921105105255
520521,1041043,1041042,2082085,2118.936168909073,0.319868687151029
521522,1043045,1043044,2086089,2122.875895023346,0.3193001014042238
522523,1045047,1045046,2090093,2127.429765701294,0.3187334440062841
523524,1047049,1047048,2094097,2131.5107576847076,0.3181687052219786
524525,1049051,1049050,2098101,2135.4526147842407,0.31760587537246465
525526,1051053,1051052,2102105,2139.231696844101,0.31704494484984025
526527,1053055,1053054,2106109,2143.6121039390564,0.316485904108049
527528,1055057,1055056,2110113,2147.1682460308075,0.31592874366651813
528529,1057059,1057058,2114117,2151.1298859119415,0.31537345410106354
529530,1059061,1059060,2118121,2154.9449458122253,0.3148200260584417
530531,1061063,1061062,2122125,2158.5591280460358,0.3142684502454358
531532,1063065,1063064,2126129,2162.2488429546356,0.31371871742157964
532533,1065067,1065066,2130133,2165.830778837204,0.3131708184209856
533534,1067069,1067068,2134137,2169.2973098754883,0.3126247441286978
534535,1069071,1069070,2138141,2172.7287118434906,0.31208048548796796
535536,1071073,1071072,2142145,2176.1484248638153,0.3115380335129885
536537,1073075,1073074,2146149,2179.58766579628,0.3109973792688834
537538,1075077,1075076,2150153,2183.6703717708588,0.3104585138771654
538539,1077079,1077078,2154157,2187.6244139671326,0.3099214285193739
539540,1079081,1079080,2158161,2191.064523935318,0.30938611443707487
540541,1081083,1081082,2162165,2195.3819057941437,0.30885256293004204
541542,1083085,1083084,2166169,2200.0529747009277,0.3083207653453428
542543,1085087,1085086,2170173,2205.1945729255676,0.30779071309916617
543544,1087089,1087088,2174177,2211.9050998687744,0.30726239765317587
544545,1089091,1089090,2178181,2218.477370738983,0.3067358105272433
545546,1091093,1091092,2182185,2225.1350107192993,0.30621094329944754
546547,1093095,1093094,2186189,2231.7545840740204,0.30568778759879933
547548,1095097,1095096,2190193,2236.9117319583893,0.30516633510524116
548549,1097099,1097098,2194197,2242.1501858234406,0.3046465775605611
549550,1099101,1099100,2198201,2248.6768786907196,0.30412850675566006
550551,1101103,1101102,2202205,2254.927337884903,0.3036121145287325
551552,1103105,1103104,2206209,2260.9818527698517,0.30309739277436165
552553,1105107,1105106,2210213,2266.31010389328,0.30258433344170044
553554,1107109,1107108,2214217,2270.8581218719482,0.30207292852901446
554555,1109111,1109110,2218221,2275.908758878708,0.30156317008368205
555556,1111113,1111112,2222225,2281.361030817032,0.3010550502076512
556557,1113115,1113114,2226229,2287.394870996475,0.3005485610483447
557558,1115117,1115116,2230233,2293.6209008693695,0.30004369480593596
558559,1117119,1117118,2234237,2299.455641746521,0.2995404437278921
559560,1119121,1119120,2238241,2305.75741481781,0.29903880011625006
560561,1121123,1121122,2242245,2311.863963842392,0.29853875631306437
561562,1123125,1123124,2246249,2318.4077808856964,0.29804030471495935
562563,1125127,1125126,2250253,2324.054884672165,0.29754343776221504
563564,1127129,1127128,2254257,2328.984248638153,0.29704814794968115
564565,1129131,1129130,2258261,2334.9620718955994,0.2965544278067682
565566,1131133,1131132,2262265,2339.81800699234,0.2960622699265514
566567,1133135,1133134,2266269,2344.827488899231,0.2955716669330286
567568,1135137,1135136,2270273,2349.520320892334,0.2950826115011296
568569,1137139,1137138,2274277,2354.11368393898,0.29459509635671566
569570,1139141,1139140,2278281,2358.6788268089294,0.294109114265666
570571,1141143,1141142,2282285,2363.3485958576202,0.2936246580375155
571572,1143145,1143144,2286289,2368.2870347499847,0.2931417205345497
572573,1145147,1145146,2290293,2373.081207036972,0.292660294649977
573574,1147149,1147148,2294297,2377.8714706897736,0.2921803733333945
574575,1149151,1149150,2298301,2381.834977865219,0.2917019495725981
575576,1151153,1151152,2302305,2385.60213971138,0.2912250163990393
576577,1153155,1153154,2306309,2389.3901488780975,0.2907495668860065
577578,1155157,1155156,2310313,2393.4639286994934,0.2902755941522628
578579,1157159,1157158,2314317,2397.699189901352,0.289803091356589
579580,1159161,1159160,2318321,2401.606738805771,0.28933205169960274
580581,1161163,1161162,2322325,2406.1934456825256,0.2888624684237584
581582,1163165,1163164,2326329,2410.4613387584686,0.28839433481698507
582583,1165167,1165166,2330333,2414.4073729515076,0.28792764419631567
583584,1167169,1167168,2334337,2418.23957490921,0.2874623899351718
584585,1169171,1169170,2338341,2423.2556779384613,0.28699856543607893
585586,1171173,1171172,2342345,2428.3553149700165,0.2865361641452182
586587,1173175,1173174,2346349,2434.433511734009,0.28607517955242656
587588,1175177,1175176,2350353,2438.482707977295,0.28561560518028273
588589,1177179,1177178,2354357,2444.335681915283,0.2851574345913832
589590,1179181,1179180,2358361,2448.8951008319855,0.28470066139016126
590591,1181183,1181182,2362365,2453.2339067459106,0.2842452792210679
591592,1183185,1183184,2366369,2459.01474404335,0.283791281761296
592593,1185187,1185186,2370373,2464.3572018146515,0.28333866273351305
593594,1187189,1187188,2374377,2469.67120885849,0.2828874158876715
594595,1189191,1189190,2378381,2474.6067218780518,0.2824375350246555
595596,1191193,1191192,2382385,2479.2544288635254,0.281989013967177
596597,1193195,1193194,2386389,2484.949017763138,0.2815418465870607
597598,1195197,1195196,2390393,2490.0826058387756,0.2810960267906921
598599,1197199,1197198,2394397,2494.5398037433624,0.28065154851174157
599600,1199201,1199200,2398401,2498.9406328201294,0.2802084057311731
600601,1201203,1201202,2402405,2503.236294746399,0.27976659245905466
601602,1203205,1203204,2406409,2507.4265546798706,0.27932610274729086
602603,1205207,1205206,2410413,2511.6113216876984,0.2788869306787092
603604,1207209,1207208,2414417,2515.46680188179,0.2784490703652409
604605,1209211,1209210,2418421,2519.8469178676605,0.2780125159606541
605606,1211213,1211212,2422425,2524.2970638275146,0.27757726165873464
606607,1213215,1213214,2426429,2528.5062787532806,0.27714330167691514
607608,1215217,1215216,2430433,2532.394630908966,0.2767106302708271
608609,1217219,1217218,2434437,2536.925117969513,0.27627924173066276
609610,1219221,1219220,2438441,2540.9458050727844,0.2758491303775372
610611,1221223,1221222,2442445,2545.6947009563446,0.27542029057076434
611612,1223225,1223224,2446449,2551.0204207897186,0.27499271669330483
612613,1225227,1225226,2450453,2555.305030822754,0.27456640317359415
613614,1227229,1227228,2454457,2558.986738920212,0.27414134446371463
614615,1229231,1229230,2458461,2563.4682297706604,0.2737175350484904
615616,1231233,1231232,2462465,2567.841829776764,0.27329496944912535
616617,1233235,1233234,2466469,2571.87472987175,0.27287364221592725
617618,1235237,1235236,2470473,2576.47994184494,0.27245354793012666
618619,1237239,1237238,2474477,2579.9365317821503,0.27203468120387697
619620,1239241,1239240,2478481,2583.5812406539917,0.27161703668571135
620621,1241243,1241242,2482485,2588.212193965912,0.27120060904599086
621622,1243245,1243244,2486489,2592.3405208587646,0.27078539300055127
622623,1245247,1245246,2490493,2596.4530107975006,0.2703713832761423
623624,1247249,1247248,2494497,2600.660953760147,0.2699585746431694
624625,1249251,1249250,2498501,2605.4251997470856,0.2695469618993229
625626,1251253,1251252,2502505,2609.360321044922,0.26913653987321595
626627,1253255,1253254,2506509,2613.347054719925,0.2687273034171085
627628,1255257,1255256,2510513,2617.631491661072,0.2683192474250973
628629,1257259,1257258,2514517,2621.991857767105,0.267912366802193
629630,1259261,1259260,2518521,2626.6542768478394,0.26750665650070005
630631,1261263,1261262,2522525,2631.5695848464966,0.26710211148929375
631632,1263265,1263264,2526529,2635.8527569770813,0.2666987267730292
632633,1265267,1265266,2530533,2640.195891857147,0.26629649737697036
633634,1267269,1267268,2534537,2644.6621749401093,0.26589541836256103
634635,1269271,1269270,2538541,2649.32909488678,0.2654954848185298
635636,1271273,1271272,2542545,2653.3045399188995,0.2650966918536142
636637,1273275,1273274,2546549,2657.8391489982605,0.2646990346147504
637638,1275277,1275276,2550553,2662.339572906494,0.2643025082670647
638639,1277279,1277278,2554557,2666.318499803543,0.263907108006606
639640,1279281,1279280,2558561,2670.3150520324707,0.26351282905852713
640641,1281283,1281282,2562565,2674.519570827484,0.2631196666716278
641642,1283285,1283284,2566569,2679.373345851898,0.26272761612563045
642643,1285287,1285286,2570573,2683.7674050331116,0.2623366727184475
643644,1287289,1287288,2574577,2687.3731520175934,0.2619468317825522
644645,1289291,1289290,2578581,2690.8295068740845,0.2615580886758835
645646,1291293,1291292,2582585,2694.315222978592,0.26117043877820834
646647,1293295,1293294,2586589,2697.8112308979034,0.2607838774947595
647648,1295297,1295296,2590593,2701.2965466976166,0.2603984002580546
648649,1297299,1297298,2594597,2704.8080339431763,0.2600140025278961
649650,1299301,1299300,2598601,2708.3597197532654,0.25963067978955223
650651,1301303,1301302,2602605,2711.812643766403,0.25924842755011923
651652,1303305,1303304,2606609,2715.229898929596,0.2588672413385211
652653,1305307,1305306,2610613,2718.7503039836884,0.25848711672006175
653654,1307309,1307308,2614617,2722.230530977249,0.2581080492709589
654655,1309311,1309310,2618621,2725.7167208194733,0.25773003460199106
655656,1311313,1311312,2622625,2729.1529989242554,0.2573530683421268
656657,1313315,1313314,2626629,2733.7946009635925,0.25697714614761935
657658,1315317,1315316,2630633,2738.132884979248,0.2566022636983689
658659,1317319,1317318,2634637,2742.6304240226746,0.25622841669246554
659660,1319321,1319320,2638641,2747.132806777954,0.2558556008589221
660661,1321323,1321322,2642645,2751.7760198116302,0.2554838119485794
661662,1323325,1323324,2646649,2755.928713798523,0.255113045732287
662663,1325327,1325326,2650653,2759.662071943283,0.2547432980063604
663664,1327329,1327328,2654657,2763.5456037521362,0.25437456458894303
664665,1329331,1329330,2658661,2767.691009044647,0.25400684132182505
665666,1331333,1331332,2662665,2772.0890057086945,0.2536401240686246
666667,1333335,1333334,2666669,2776.101720094681,0.25327440871660656
667668,1335337,1335336,2670673,2781.4926319122314,0.25290969117304485
668669,1337339,1337338,2674677,2785.8912518024445,0.2525459673724981
669670,1339341,1339340,2678681,2790.4071097373962,0.252183233264077
670671,1341343,1341342,2682685,2795.192625761032,0.2518214848205389
671672,1343345,1343344,2686689,2800.0170817375183,0.25146071804374515
672673,1345347,1345346,2690693,2804.3834507465363,0.25110092894828995
673674,1347349,1347348,2694697,2808.90957903862,0.25074211357423337
674675,1349351,1349350,2698701,2813.4600989818573,0.25038426798346336
675676,1351353,1351352,2702705,2817.871077775955,0.25002738825423876
676677,1353355,1353354,2706709,2822.299571990967,0.24967147049574123
677678,1355357,1355356,2710713,2826.633657693863,0.24931651082260942
678679,1357359,1357358,2714717,2831.127420902252,0.24896250538586173
679680,1359361,1359360,2718721,2835.7032418251038,0.24860945035106852
680681,1361363,1361362,2722725,2840.303611755371,0.24825734189653303
681682,1363365,1363364,2726729,2844.742038011551,0.24790617623330036
682683,1365367,1365366,2730733,2849.268275976181,0.24755594958696747
683684,1367369,1367368,2734737,2853.9601278305054,0.24720665820314025
684685,1369371,1369370,2738741,2858.230297803879,0.24685829834197648
685686,1371373,1371372,2742745,2864.331550836563,0.24651086629637575
686687,1373375,1373374,2746749,2870.6694378852844,0.24616435836833261
687688,1375377,1375376,2750753,2875.652879714966,0.24581877088166948
688689,1377379,1377378,2754757,2879.955429792404,0.24547410018385563
689690,1379381,1379380,2758761,2884.789486646652,0.24513034263145528
690691,1381383,1381382,2762765,2889.410856962204,0.24478749461377447
691692,1383385,1383384,2766769,2894.4624519348145,0.2444455525273952
692693,1385387,1385386,2770773,2899.281720638275,0.2441045127943653
693694,1387389,1387388,2774777,2903.9548358917236,0.2437643718549225
694695,1389391,1389390,2778781,2908.999627828598,0.24342512616567547
695696,1391393,1391392,2782785,2914.267712831497,0.24308677219960373
696697,1393395,1393394,2786789,2919.1123287677765,0.2427493064551527
697698,1395397,1395396,2790793,2923.7481977939606,0.24241272544531967
698699,1397399,1397398,2794797,2927.710518836975,0.24207702569947287
699700,1399401,1399400,2798801,2932.2261476516724,0.24174220376517042
700701,1401403,1401402,2802805,2937.036244869232,0.2414082562117983
701702,1403405,1403404,2806809,2941.3627650737762,0.24107517962511338
702703,1405407,1405406,2810813,2945.1754927635193,0.2407429706017865
703704,1407409,1407408,2814817,2949.163949728012,0.24041162576759234
704705,1409411,1409410,2818821,2952.8469808101654,0.24008114175921946
705706,1411413,1411412,2822825,2956.5351328849792,0.23975151522972737
706707,1413415,1413414,2826829,2960.2062578201294,0.23942274285218446
707708,1415417,1415416,2830833,2963.922313928604,0.239094821314211
708709,1417419,1417418,2834837,2967.589695930481,0.2387677473252552
709710,1419421,1419420,2838841,2971.2685129642487,0.23844151760386012
710711,1421423,1421422,2842845,2974.8970329761505,0.23811612889221578
711712,1423425,1423424,2846849,2978.5189859867096,0.23779157795070205
712713,1425427,1425426,2850853,2982.1703679561615,0.23746786154515576
713714,1427429,1427428,2854857,2985.8433096408844,0.23714497647051758
714715,1429431,1429430,2858861,2989.5031938552856,0.23682291953264212
715716,1431433,1431432,2862865,2993.138036966324,0.2365016875519359
716717,1433435,1433434,2866869,2996.7645778656006,0.23618127736881434
717718,1435437,1435436,2870873,3000.349557876587,0.23586168583642575
718719,1437439,1437438,2874877,3004.1474339962006,0.23554290982610837
719720,1439441,1439440,2878881,3007.903217792511,0.23522494622193335
720721,1441443,1441442,2882885,3011.5561068058014,0.2349077919316187
721722,1443445,1443444,2886889,3015.1535007953644,0.23410214331306634
722723,1445447,1445446,2890893,3018.884165763855,0.23378788202171563
723724,1447449,1447448,2894897,3022.6068489551544,0.23347441631813126
724725,1449451,1449450,2898901,3026.205041885376,0.23316174314823002
725726,1451453,1451452,2902905,3029.828929901123,0.23284985949794645
726727,1453455,1453454,2906909,3033.418187856674,0.23253876236958604
727728,1455457,1455456,2910913,3037.0964727401733,0.23222844879273907
728729,1457459,1457458,2914917,3040.728461742401,0.2319189158079098
729730,1459461,1459460,2918921,3044.3316328525543,0.2316101604810683
730731,1461463,1461462,2922925,3047.99046087265,0.23130217988182267
731732,1463465,1463464,2926929,3051.671684741974,0.23099497109797085
732733,1465467,1465466,2930933,3055.2713158130646,0.23068853124277666
733734,1467469,1467468,2934937,3058.8492007255554,0.2303828574331419
734735,1469471,1469470,2938941,3062.447569847107,0.23007794680415827
735736,1471473,1471472,2942945,3066.049865961075,0.2297737964981934
736737,1473475,1473474,2946949,3069.6924958229065,0.22947040368853777
737738,1475477,1475476,2950953,3073.2678887844086,0.22916776554666285
738739,1477479,1477478,2954957,3076.8580737113953,0.228865879265868
739740,1479481,1479480,2958961,3080.578707933426,0.2285647420485475
740741,1481483,1481482,2962965,3084.25533080101,0.22826435111528554
741742,1483485,1483484,2966969,3087.8153426647186,0.22796470369576127
742743,1485487,1485486,2970973,3091.466614961624,0.2276657970414817
743744,1487489,1487488,2974977,3095.0807087421417,0.22736762840941083
744745,1489491,1489490,2978981,3098.6595997810364,0.2270701950728835
745746,1491493,1491492,2982985,3102.2575738430023,0.22677349431978655
746747,1493495,1493494,2986989,3105.873510837555,0.2264775234489207
747748,1495497,1495496,2990993,3109.4987750053406,0.22618227977363858
748749,1497499,1497498,2994997,3113.1273028850555,0.2258877606218448
749750,1499501,1499500,2999001,3116.7391879558563,0.22559396333053883
750751,1501503,1501502,3003005,3120.3792717456818,0.22530088525127212
751752,1503505,1503504,3007009,3123.995851993561,0.225008523753786
752753,1505507,1505506,3011013,3127.5515038967133,0.22471687621327874
753754,1507509,1507508,3015017,3131.152140855789,0.22442594002131955
754755,1509511,1509510,3019021,3134.73290681839,0.22413571257857257
755756,1511513,1511512,3023025,3138.3300478458405,0.22384619130571082
756757,1513515,1513514,3027029,3141.973912000656,0.2235573736288643
757758,1515517,1515516,3031033,3145.579670906067,0.22326925698871491
758759,1517519,1517518,3035037,3149.199034690857,0.2229818388386775
759760,1519521,1519520,3039041,3152.776062965393,0.22269511664671882
760761,1521523,1521522,3043045,3156.386976957321,0.22240908788990055
761762,1523525,1523524,3047049,3159.97908782959,0.22212375005619833
762763,1525527,1525526,3051053,3163.581766843796,0.2218391006499587
763764,1527529,1527528,3055057,3167.2012169361115,0.22155513718644215
764765,1529531,1529530,3059061,3170.822250843048,0.2212718571881851
765766,1531533,1531532,3063065,3174.4879398345947,0.22098925819409487
766767,1533535,1533534,3067069,3178.0719270706177,0.22070733775581175
767768,1535537,1535536,3071073,3181.726245880127,0.22042609343407094
768769,1537539,1537538,3075077,3185.3984158039093,0.22014552280234057
769770,1539541,1539540,3079081,3189.052486896515,0.21986562344318372
770771,1541543,1541542,3083085,3192.6217699050903,0.2195863929537154
771772,1543545,1543544,3087089,3196.225849866867,0.21930782894378353
772773,1545547,1545546,3091093,3199.8191406726837,0.219029929030512
773774,1547549,1547548,3095097,3203.4723057746887,0.2187526908437576
774775,1549551,1549550,3099101,3207.047405719757,0.21847611202429107
775776,1551553,1551552,3103105,3210.7616577148438,0.21820019022925408
776777,1553555,1553554,3107109,3214.406893014908,0.21792492311760725
777778,1555557,1555556,3111113,3218.001667022705,0.21765030836468213
778779,1557559,1557558,3115117,3221.5872247219086,0.2173763436585432
779780,1559561,1559560,3119121,3225.207083940506,0.21710302669634984
780781,1561563,1561562,3123125,3228.8774857521057,0.21683035518253746
781782,1563565,1563564,3127129,3232.5179419517517,0.21655832683791232
782783,1565567,1565566,3131133,3236.0817399024963,0.21628693939237564
783784,1567569,1567568,3135137,3239.668076992035,0.21601619058128563
784785,1569571,1569570,3139141,3243.260766983032,0.21574607816000935
785786,1571573,1571572,3143145,3247.0055170059204,0.21547659988755186
786787,1573575,1573574,3147149,3250.642616033554,0.21520775353383215
787788,1575577,1575576,3151153,3254.2246708869934,0.21493953688514011
788789,1577579,1577578,3155157,3257.8281667232513,0.21467194772776566
789790,1579581,1579580,3159161,3261.613182783127,0.21440498386800755
790791,1581583,1581582,3163165,3265.3281819820404,0.21413864311762154
791792,1583585,1583584,3167169,3268.952100753784,0.21387292329927732
792793,1585587,1585586,3171173,3272.57976603508,0.2136078222447395
793794,1587589,1587588,3175177,3276.1618428230286,0.21334333780032466
794795,1589591,1589590,3179181,3279.750385761261,0.2130794678159873
795796,1591593,1591592,3183185,3283.4695217609406,0.20885690041541238
796797,1593595,1593594,3187189,3287.251095056534,0.2020343063340988
797798,1595597,1595596,3191193,3290.933069705963,0.19568280861676612
798799,1597599,1597598,3195197,3294.724268913269,0.19029158085504605
799800,1599601,1599600,3199201,3298.4257867336273,0.1847958872658637
800801,1601603,1601602,3203205,3302.193165063858,0.17965895112138242
801802,1603605,1603604,3207209,3305.9695858955383,0.17487518094094412
802803,1605607,1605606,3211213,3309.7116837501526,0.1704392269894015
803804,1607609,1607608,3215217,3313.4262409210205,0.16640104659200006
804805,1609611,1609610,3219221,3317.1055936813354,0.16238411661652208
805806,1611613,1611612,3223225,3320.8052599430084,0.1586518068688747
806807,1613615,1613614,3227229,3324.5275609493256,0.15526963089723722
807808,1615617,1615616,3231233,3328.131694793701,0.1519450352752756
808809,1617619,1617618,3235237,3331.7380516529083,0.14897826765445643
809810,1619621,1619620,3239241,3335.3310327529907,0.1459649997195811
810811,1621623,1621622,3243245,3338.9058890342712,0.144699126462001
811812,1623625,1623624,3247249,3342.50847196579,0.1445712373006245
812813,1625627,1625626,3251253,3346.1098868846893,0.1444435557386896
813814,1627629,1627628,3255257,3349.748548746109,0.1443160812723363
814815,1629631,1629630,3259261,3353.4126749038696,0.1441888133995235
815816,1631633,1631632,3263265,3357.0011699199677,0.1440617516200291
816817,1633635,1633634,3267269,3360.6238758563995,0.14393489544090698
817818,1635637,1635636,3271273,3364.216481924057,0.14380824436193507
818819,1637639,1637638,3275277,3367.8062887191772,0.14368179789016722
819820,1639641,1639640,3279281,3371.401440858841,0.1435555555344763
820821,1641643,1641642,3283285,3374.997018814087,0.14342951680555416
821822,1643645,1643644,3287289,3378.5854988098145,0.1433036812068167
822823,1645647,1645646,3291293,3382.252492904663,0.14317804825986968
823824,1647649,1647648,3295297,3385.8855378627777,0.143052617471767
824825,1649651,1649650,3299301,3389.4992558956146,0.14292738836047647
825826,1651653,1651652,3303305,3393.127963781357,0.14280236044578487
826827,1653655,1653654,3307309,3396.772750854492,0.14267753323838406
827828,1655657,1655656,3311313,3400.497256755829,0.1425529062653368
828829,1657659,1657658,3315317,3404.141907930374,0.14242847904642986
829830,1659661,1659660,3319321,3407.7591989040375,0.14230425110508804
830831,1661663,1661662,3323325,3411.406584739685,0.14218022196291713
831832,1663665,1663664,3327329,3415.076231956482,0.14205639115061786
832833,1665667,1665666,3331333,3418.693960905075,0.141932758189796
833834,1667669,1667668,3335337,3422.3535227775574,0.14180932261660928
834835,1669671,1669670,3339341,3425.9507958889008,0.14168608395630145
835836,1671673,1671672,3343345,3429.5650696754456,0.14156304174321122
836837,1673675,1673674,3347349,3433.1536309719086,0.1414401955134963
837838,1675677,1675676,3351353,3436.7503967285156,0.14131754479421943
838839,1677679,1677678,3355357,3440.4416887760162,0.1411950891288143
839840,1679681,1679680,3359361,3444.0830488204956,0.14107282805707655
840841,1681683,1681682,3363365,3447.6803319454193,0.14095076111152594
841842,1683685,1683684,3367369,3451.2785589694977,0.14082888783923408
842843,1685687,1685686,3371373,3454.878748893738,0.14070720777999668
843844,1687689,1687688,3375377,3458.448063850403,0.1405857204754284
844845,1689691,1689690,3379381,3462.018306016922,0.14046442547441984
845846,1691693,1691692,3383385,3465.642936706543,0.14034332232222368
846847,1693695,1693694,3387389,3469.327234983444,0.14022241056591156
847848,1695697,1695696,3391393,3472.9340119361877,0.14010168975619308
848849,1697699,1697698,3395397,3476.563300848007,0.13998115944559686
849850,1699701,1699700,3399401,3480.159147977829,0.1398608191848325
850851,1701703,1701702,3403405,3483.7811279296875,0.13974066852824762
851852,1703705,1703704,3407409,3487.4079928398132,0.13962070702837082
852853,1705707,1705706,3411413,3491.007845878601,0.13950093424500665
853854,1707709,1707708,3415417,3494.635505914688,0.13938134973795968
854855,1709711,1709710,3419421,3498.270605802536,0.13926195306157751
855856,1711713,1711712,3423425,3501.919126033783,0.1391427437793027
856857,1713715,1713714,3427429,3505.5143270492554,0.13902372145275876
857858,1715717,1715716,3431433,3509.1144268512726,0.1389048856435693
858859,1717719,1717718,3435437,3512.7101340293884,0.13878623592063377
859860,1719721,1719720,3439441,3516.2975590229034,0.13866777184739476
860861,1721723,1721722,3443445,3519.8821120262146,0.13854949299275177
861862,1723725,1723724,3447449,3523.4605448246,0.1384313989256043
862863,1725727,1725726,3451453,3527.1027069091797,0.13831348921303288
863864,1727729,1727728,3455457,3530.698008775711,0.13819576343121298
864865,1729731,1729730,3459461,3534.3392267227173,0.13807822114722512
865866,1731733,1731732,3463465,3538.0009326934814,0.13796086194452073
866867,1733735,1733734,3467469,3541.6069350242615,0.13784368539018033
867868,1735737,1735736,3471473,3545.211637020111,0.13772669106219837
868869,1737739,1737738,3475477,3548.7985389232635,0.1376098785403883
869870,1739741,1739740,3479481,3552.408362865448,0.13749324741002056
870871,1741743,1741742,3483485,3556.003350019455,0.13737679724181362
871872,1743745,1743744,3487489,3559.580186843872,0.13726052761921892
872873,1745747,1745746,3491493,3563.208492040634,0.13714443813296384
873874,1747749,1747748,3495497,3566.7719280719757,0.13702852836104285
874875,1749751,1749750,3499501,3570.384217739105,0.1369127978941833
875876,1751753,1751752,3503505,3574.006630897522,0.13679724631401768
876877,1753755,1753754,3507509,3577.573017835617,0.13668187321491132
877878,1755757,1755756,3511513,3581.298736810684,0.13656667818031565
878879,1757759,1757758,3515517,3584.897894859314,0.13645166080641502
879880,1759761,1759760,3519521,3588.582797050476,0.13633682068393682
880881,1761763,1761762,3523525,3592.1988627910614,0.1362221574072464
881882,1763765,1763764,3527529,3595.8108468055725,0.13610767056889017
882883,1765767,1765766,3531533,3599.4466817379,0.13599335976687144
883884,1767769,1767768,3535537,3603.0808687210083,0.1358792245919176
884885,1769771,1769770,3539541,3606.6961369514465,0.1357652646547649
885886,1771773,1771772,3543545,3610.3384687900543,0.13565147954250278
886887,1773775,1773774,3547549,3613.9637529850006,0.1355378688658675
887888,1775777,1775776,3551553,3617.5885560512543,0.1354244322210434
888889,1777779,1777778,3555557,3621.234988927841,0.13531116921330977
889890,1779781,1779780,3559561,3624.927244901657,0.13519807944794593
890891,1781783,1781782,3563565,3628.7190656661987,0.13508516252841218
891892,1783785,1783784,3567569,3632.345482826233,0.1349724180636258
892893,1785787,1785786,3571573,3636.0097818374634,0.13485984566250409
893894,1787789,1787788,3575577,3639.6281888484955,0.1347474449321453
894895,1789791,1789790,3579581,3643.224168777466,0.13463521548146673
895896,1791793,1791792,3583585,3646.8232119083405,0.1345231569284806
896897,1793795,1793794,3587589,3650.4349949359894,0.13441126887846622
897898,1795797,1795796,3591593,3654.105963945389,0.1342995509494358
898899,1797799,1797798,3595597,3657.710335969925,0.13418800275758258
899900,1799801,1799800,3599601,3661.3174679279327,0.1340766239172808
900901,1801803,1801802,3603605,3664.967038869858,0.13396541404654272
901902,1803805,1803804,3607609,3668.565277814865,0.13385437276519951
902903,1805807,1805806,3611613,3672.175880908966,0.13374349968944443
903904,1807809,1807808,3615617,3675.73659491539,0.13363279444456566
904905,1809811,1809810,3619621,3679.3892827033997,0.1335222566522134
905906,1811813,1811812,3623625,3683.034810781479,0.13341188593403785
906907,1813815,1813814,3627629,3686.7658207416534,0.13330168190987024
907908,1815817,1815816,3631633,3690.3774857521057,0.13319164421409369
908909,1817819,1817818,3635637,3694.0404238700867,0.1330817724665394
909910,1819821,1819820,3639641,3697.6284358501434,0.13297206629977154
910911,1821823,1821822,3643645,3701.44717168808,0.13286252534089726
911912,1823825,1823824,3647649,3705.149317741394,0.13275314921884274
912913,1825827,1825826,3651653,3708.8040878772736,0.1326439375643531
913914,1827829,1827828,3655657,3712.4334387779236,0.13253489000999252
914915,1829831,1829830,3659661,3716.019847869873,0.1324260061901441
915916,1831833,1831832,3663665,3719.630683898926,0.132317285739191
916917,1833835,1833834,3667669,3723.283770799637,0.13220872828969732
917918,1835837,1835836,3671673,3726.901026725769,0.13210033348332217
918919,1837839,1837838,3675677,3730.4797019958496,0.1319921009544487
919920,1839841,1839840,3679681,3734.1462666988373,0.13188403034109797
920921,1841843,1841842,3683685,3737.7254610061646,0.13177612128311011
921922,1843845,1843844,3687689,3741.343384027481,0.1316683734221442
922923,1845847,1845846,3691693,3744.9897940158844,0.13156078640167834
923924,1847849,1847848,3695697,3748.5683748722076,0.13145335986519058
924925,1849851,1849850,3699701,3752.191475868225,0.13134609345252102
925926,1851853,1851852,3703705,3755.7461297512054,0.13123898680896673
926927,1853855,1853854,3707709,3759.38619184494,0.13113203958528175
927928,1855857,1855856,3711713,3763.0257267951965,0.13102525142312516
928929,1857859,1857858,3715717,3766.6464257240295,0.13091862197688897
929930,1859861,1859860,3719721,3770.3396258354187,0.13081215089187026
930931,1861863,1861862,3723725,3773.947581768036,0.13070583781700407
931932,1863865,1863864,3727729,3777.551880836487,0.1305996824066824
932933,1865867,1865866,3731733,3781.166429758072,0.1304936843134783
933934,1867869,1867868,3735737,3784.731048822403,0.13038784318814578
934935,1869871,1869870,3739741,3788.3327407836914,0.13028215868689585
935936,1871873,1871872,3743745,3791.922129869461,0.13017663046230155
936937,1873875,1873874,3747749,3795.5117678642273,0.13007125817603082
937938,1875877,1875876,3751753,3799.0858857631683,0.1299660414824757
938939,1877879,1877878,3755757,3802.754678964615,0.1298609800360282
939940,1879881,1879880,3759761,3806.354826927185,0.12975607350563223
940941,1881883,1881882,3763765,3809.974511861801,0.12965132154386083
941942,1883885,1883884,3767769,3813.5975069999695,0.12954672381420096
942943,1885887,1885886,3771773,3817.250095844269,0.12944227998013957
943944,1887889,1887888,3775777,3820.853320837021,0.12933798970516364
944945,1889891,1889890,3779781,3824.485050678253,0.12923385265094112
945946,1891893,1891892,3783785,3828.122454881668,0.12912986848641594
946947,1893895,1893894,3787789,3831.7527170181274,0.1290260368732561
947948,1895897,1895896,3791793,3835.3385016918182,0.12892235748404346
948949,1897899,1897898,3795797,3838.92968082428,0.128818829985903
949950,1899901,1899900,3799801,3842.566512823105,0.12871545404595963
950951,1901903,1901902,3803805,3846.2441399097443,0.1286122293349763
951952,1903905,1903904,3807809,3850.0734508037567,0.1285091555237159
952953,1905907,1905906,3811813,3853.6472907066345,0.12840623228476034
953954,1907909,1907908,3815817,3857.2542808055878,0.12830345929251052
954955,1909911,1909910,3819821,3860.8393547534943,0.12820083621954836
955956,1911913,1911912,3823825,3864.4552929401398,0.12809836274209374
956957,1913915,1913914,3827829,3868.062983751297,0.12799603853272856
957958,1915917,1915916,3831833,3871.6920108795166,0.12789386327494867
958959,1917919,1917918,3835837,3875.3489048480988,0.127791836637698
959960,1919921,1919920,3839841,3878.9932746887207,0.12768995830629137
960961,1921923,1921922,3843845,3882.631864786148,0.12758822795694869
961962,1923925,1923924,3847849,3886.2068848609924,0.12748664527316578
962963,1925927,1925926,3851853,3889.8488509655,0.1273852099366195
963964,1927929,1927928,3855857,3893.468845844269,0.12728392162352975
964965,1929931,1929930,3859861,3897.0943479537964,0.12718278002284933
965966,1931933,1931932,3863865,3900.7011518478394,0.12708178481807408
966967,1933935,1933934,3867869,3904.286017894745,0.12698093569451885
967968,1935937,1935936,3871873,3907.9062128067017,0.12688023233567947
968969,1937939,1937938,3875877,3911.494158744812,0.12677967443232774
969970,1939941,1939940,3879881,3915.0775077342987,0.12667926166614052
970971,1941943,1941942,3883885,3918.6577668190002,0.1265789937315276
971972,1943945,1943944,3887889,3922.2792177200317,0.12647887031562277
972973,1945947,1945946,3891893,3925.901725769043,0.12637889111101686
973974,1947949,1947948,3895897,3929.532614707947,0.12627905580666265
974975,1949951,1949950,3899901,3933.119994878769,0.12617936409696995
975976,1951953,1951952,3903905,3936.765904903412,0.12607981567089155
976977,1953955,1953954,3907909,3940.3606638908386,0.1259804102282942
977978,1955957,1955956,3911913,3943.9799506664276,0.12588114745813073
978979,1957959,1957958,3915917,3947.637640953064,0.12578202706026786
979980,1959961,1959960,3919921,3951.283096075058,0.1256830487309344
980981,1961963,1961962,3923925,3954.9614968299866,0.12558421216635907
981982,1963965,1963964,3927929,3958.566120862961,0.12548551706822764
982983,1965967,1965966,3931933,3962.2098937034607,0.1253869631254929
983984,1967969,1967968,3935937,3965.880481004715,0.12528855005075457
984985,1969971,1969970,3939941,3969.5183777809143,0.12519027754024137
985986,1971973,1971972,3943945,3973.076618909836,0.12509214529200108
986987,1973975,1973974,3947949,3976.6769938468933,0.1249941530131764
987988,1975977,1975976,3951953,3980.3022577762604,0.12489630040545308
988989,1977979,1977978,3955957,3983.9372918605804,0.12479858717233583
989990,1979981,1979980,3959961,3987.570255756378,0.12470101302096737
990991,1981983,1981982,3963965,3991.2121448516846,0.12460357765485242
991992,1983985,1983984,3967969,3994.841962814331,0.12450628078477166
992993,1985987,1985986,3971973,3998.4472119808197,0.12440912211241084
993994,1987989,1987988,3975977,4002.0632367134094,0.12431210134855064
994995,1989991,1989990,3979981,4005.71049785614,0.12421521820397174
995996,1991993,1991992,3983985,4009.3665368556976,0.12411847239127383
996997,1993995,1993994,3987989,4013.0476636886597,0.1240218636157806
997998,1995997,1995996,3991993,4017.1067719459534,0.12392539159009175
998999,1997999,1997998,3995997,4020.8275089263916,0.12382905602862593
1000000,2000001,2000000,4000001,4024.4522228240967,0.12373285664216382


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0035982131958007812,12064.44795143716
1001,2003,2002,4005,3.8882622718811035,65.38449138327269
2002,4005,4004,8009,7.948341369628906,42.2154127642043
3003,6007,6006,12013,12.002243041992188,33.90174222643145
4004,8009,8008,16017,16.12182116508484,28.84319011385014
5005,10011,10010,20021,19.728594303131104,25.22268890097439
6006,12013,12012,24025,23.365817070007324,22.42065265709971
7007,14015,14014,28029,26.99235725402832,20.15004075854631
8008,16017,16016,32033,30.618634939193726,18.255867237425264
9009,18019,18018,36037,34.21288323402405,16.644924627120417
10010,20021,20020,40041,37.8082001209259,15.256259435958782
11011,22023,22022,44045,41.40822124481201,14.04716756882226
12012,24025,24024,48049,45.06582021713257,12.986141411429344
13013,26027,26026,52053,48.61799430847168,12.049111192072814
14014,28029,28028,56057,52.23655128479004,11.217231971750152
15015,30031,30030,60061,55.7975013256073,10.475259290258691
16016,32033,32032,64065,59.39685821533203,9.810784742190663
17017,34035,34034,68069,62.946776151657104,9.213588128843185
18018,36037,36036,72073,66.51810503005981,8.67509578481804
19019,38039,38038,76077,70.11822938919067,8.188094868561166
20020,40041,40040,80081,73.85724115371704,7.746456546892659
21021,42043,42042,84085,77.44075417518616,7.344936499697724
22022,44045,44044,88089,80.98412322998047,6.979019482529111
23023,46047,46046,92093,84.5825400352478,6.644796545697318
24024,48049,48048,96097,88.25771307945251,6.338866989019152
25025,50051,50050,100101,91.83079814910889,6.058259293347874
26026,52053,52052,104105,95.38628125190735,5.8003667720786325
27027,54055,54054,108109,99.05189323425293,5.562894754204535
28028,56057,56056,112113,102.7015471458435,5.34381688436406
29029,58059,58058,116117,106.29325723648071,5.14133869384932
30030,60061,60060,120121,109.9285101890564,4.953867018881283
31031,62063,62062,124125,113.50830936431885,4.779984159364176
32032,64065,64064,128129,117.11837005615234,4.618425910906808
33033,66067,66066,132133,120.65442419052124,4.46806278542681
34034,68069,68068,136137,124.24468922615051,4.327883875652333
35035,70071,70070,140141,128.4076452255249,4.196982926987403
36036,72073,72072,144145,131.98642301559448,4.0745462642044
37037,74075,74074,148149,135.53232407569885,3.9598422862709413
38038,76077,76076,152153,139.14230918884277,3.8522122943613795
39039,78079,78078,156157,142.6928472518921,3.7510624592814565
40040,80081,80080,160161,146.2425491809845,3.6558613114921172
41041,82083,82082,164165,149.8064842224121,3.566129789558545
42042,84085,84084,168169,153.39581322669983,3.4814190444340056
43043,86087,86086,172173,156.94034814834595,3.401332075274695
44044,88089,88088,176177,160.565269947052,3.32550887767502
45045,90091,90090,180181,164.15765023231506,3.2536226351949153
46046,92093,92092,184185,167.77509117126465,3.185376335550245
47047,94095,94094,188189,171.3869071006775,3.120499759867016
48048,96097,96096,192193,174.9719033241272,3.058746800541485
49049,98099,98098,196197,178.60749101638794,2.9998930688743712
50050,100101,100100,200201,182.15090036392212,2.9437337589097297
51051,102103,102102,204205,185.72179913520813,2.8900817379417276
52052,104105,104104,208209,189.3591160774231,2.8387658380506764
53053,106107,106106,212213,192.92078304290771,2.7896293259727827
54054,108109,108108,216217,196.56375908851624,2.742528531491189
55055,110111,110110,220221,200.1053171157837,2.697331616869633
56056,112113,112112,224225,203.74623608589172,2.653917471836394
57057,114115,114114,228229,207.32011723518372,2.6121747205324937
58058,116117,116116,232233,211.02904415130615,2.572000828349701
59059,118119,118118,236237,214.59930419921875,2.533301297957223
60060,120121,120120,240241,218.25865817070007,2.4959889450437913
61061,122123,122122,244245,221.86557531356812,2.4599832453677664
62062,124125,124124,248249,225.45019721984863,2.425211069314173
63063,126127,126126,252253,229.03374409675598,2.391602714491455
64064,128129,128128,256257,232.73784804344177,2.3590937382832635
65065,130131,130130,260261,236.27825117111206,2.3276249103255395
66066,132133,132132,264265,239.8943111896515,2.2971412315273483
67067,134135,134134,268269,243.4142882823944,2.267591576312043
68068,136137,136136,272273,247.03720426559448,2.238928369633868
69069,138139,138138,276277,250.5957863330841,2.2111072939496808
70070,140141,140140,280281,254.28893518447876,2.1840870231935696
71071,142143,142142,284285,258.7126340866089,2.1578289810713613
72072,144145,144144,288289,262.7164611816406,2.1322971212430275
73073,146147,146146,292293,266.8357570171356,2.107457727290239
74074,148149,148148,296297,270.51077818870544,2.0832792305045587
75075,150151,150150,300301,274.27176213264465,2.0597320438027964
76076,152153,152152,304305,278.496089220047,2.0367884101960954
77077,154155,154154,308309,282.7754900455475,2.0144222644375986
78078,156157,156156,312313,287.1283640861511,1.9926091065881337
79079,158159,158158,316317,291.7021441459656,1.971325886379418
80080,160161,160160,320321,295.12670516967773,1.9505508973688848
81081,162163,162162,324325,298.4981760978699,1.9302636799784523
82082,164165,164164,328329,301.89953112602234,1.9104449325750466
83083,166167,166166,332333,305.31486415863037,1.8910764298871072
84084,168169,168168,336337,308.7006850242615,1.8721409480604052
85085,170171,170170,340341,313.13223910331726,1.853622195785647
86086,172173,172172,344345,318.19966101646423,1.8355047509230644
87087,174175,174174,348349,322.58982014656067,1.8177740021492355
88088,176177,176176,352353,326.4793472290039,1.8004160951877566
89089,178179,178178,356357,330.31257700920105,1.7834178832090402
90090,180181,180180,360361,334.1131420135498,1.766766881044532
91091,182183,182182,364365,338.2126262187958,1.7504515684831858
92092,184185,184184,368369,342.0464291572571,1.7344624748329807
93093,186187,186186,372373,346.4044840335846,1.7187865341365978
94094,188189,188188,376377,350.41197896003723,1.7034135223966587
95095,190191,190190,380381,354.18487334251404,1.6883336949704244
96096,192193,192192,384385,357.82920598983765,1.6735377577206236
97097,194195,194194,388389,361.4940941333771,1.6590168402235577
98098,196197,196196,392393,365.4502053260803,1.6447624709071533
99099,198199,198198,396397,369.2518062591553,1.6307665539043228
100100,200201,200200,400401,372.6926131248474,1.617021347536138
101101,202203,202202,404405,376.72474122047424,1.603519444252015
102102,204205,204204,408409,380.42090916633606,1.5902537519468751
103103,206207,206206,412413,384.3952491283417,1.5772174765352247
104104,208209,208208,416417,387.94224095344543,1.5644041056784772
105105,210211,210210,420421,392.1014862060547,1.5518073935854773
106106,212213,212212,424425,395.59817695617676,1.5394213468080125
107107,214215,214214,428429,399.2603623867035,1.527240210938544
108108,216217,216216,432433,403.6152853965759,1.5152584581774136
109109,218219,218218,436437,408.7325973510742,1.5034707756622083
110110,220221,220220,440441,413.17922925949097,1.4918720545556425
111111,222223,222222,444445,418.6150851249695,1.480457379759173
112112,224225,224224,448449,424.1068410873413,1.4692220203178294
113113,226227,226226,452453,428.9699430465698,1.4581614203507343
114114,228229,228228,456457,433.19059205055237,1.447271190569154
115115,230231,230230,460461,436.7775421142578,1.4365471002583945
116116,232233,232232,464465,440.15698623657227,1.4259850697617367
117117,234235,234234,468469,443.54811120033264,1.4155811633736448
118118,236237,236236,472473,446.9386281967163,1.4053315826786275
119119,238239,238238,476477,450.45614528656006,1.3952326602247922
120120,240241,240240,480481,454.1458752155304,1.3852808535921213
121121,242243,242242,484485,457.8456561565399,1.3754727397590614
122122,244245,244244,488489,461.29187512397766,1.3658050098201784
123123,246247,246246,492493,464.685583114624,1.3562744639420998
124124,248249,248248,496497,468.1335690021515,1.3468780066377803
125125,250251,250250,500501,471.57833218574524,1.337612642271779
126126,252253,252252,504505,475.0053360462189,1.3284754708038236
127127,254255,254254,508509,478.57123708724976,1.319463683765207
128128,256257,256256,512513,481.98952317237854,1.3105745604425465
129129,258259,258258,516517,485.33553409576416,1.3018054642470815
130130,260261,260260,520521,488.7066111564636,1.2931538392822404
131131,262263,262262,524525,492.2223711013794,1.2846189332267386
132132,264265,264264,528529,495.75946021080017,1.2761968457252806
133133,266267,266266,532533,499.3893401622772,1.2678849911717407
134134,268269,268268,536537,502.7874963283539,1.2596811055791477
135135,270271,270270,540541,506.1599111557007,1.2515829910626053
136136,272273,272272,544545,509.56912207603455,1.2435885131653777
137137,274275,274274,548549,512.9699552059174,1.2356955984068918
138138,276277,276276,552553,516.3512990474701,1.227902231970802
139139,278279,278278,556557,519.8855800628662,1.2202064555076504
140140,280281,280280,560561,523.4368870258331,1.2126063650557626
141141,282283,282282,564565,527.0931262969971,1.205100109022169
142142,284285,284284,568569,530.7019560337067,1.1976858863072266
143143,286287,286286,572573,536.0508699417114,1.1903619444656215
144144,288289,288288,576577,539.7955021858215,1.183126577978328
145145,290291,290290,580581,543.1456291675568,1.1759781266009668
146146,292293,292292,584585,546.480535030365,1.1689149737703701
147147,294295,294294,588589,549.8182771205902,1.1619355450930016
148148,296297,296296,592593,553.198361158371,1.1550383068934025
149149,298299,298298,596597,556.5192470550537,1.148221764828122
150150,300301,300300,600601,559.9051420688629,1.1414844625542173
151151,302303,302302,604605,563.2308993339539,1.134824980465055
152152,304305,304304,608609,566.7772052288055,1.1282419344570371
153153,306307,306306,612613,570.2426452636719,1.1217339747709048
154154,308309,308308,616617,573.6279730796814,1.1152997848730593
155155,310311,310310,620621,577.0635502338409,1.1089380803732638
156156,312313,312312,624625,580.3887951374054,1.1026476080023713
157157,314315,314314,628629,583.8351261615753,1.096427144604604
158158,316317,316316,632633,587.1637032032013,1.0902754962116887
159159,318319,318318,636637,590.9735562801361,1.08419149711699
160160,320321,320320,640641,595.032909154892,1.078174008986025
161161,322323,322322,644645,598.5550403594971,1.0722219200451946
162162,324325,324324,648649,602.4061682224274,1.0663341442304954
163163,326327,326326,652653,606.7079672813416,1.060509620456287
164164,328329,328328,656657,611.4131321907043,1.0547473118112975
165165,330331,330330,660661,615.1866359710693,1.0490462048801419
166166,332333,332332,664665,619.1476762294769,1.0434053090284579
167167,334335,334334,668669,623.6023690700531,1.0378236557371565
168168,336337,336336,672673,627.4817492961884,1.0323002979566809
169169,338339,338338,676677,631.1769051551819,1.0268343094867305
170170,340341,340340,680681,635.0655381679535,1.021424784377814
171171,342343,342342,684685,640.0242962837219,1.0160708363564481
172172,344345,344344,688689,644.9028842449188,1.0107715982721857
173173,346347,346346,692693,649.1954381465912,1.005526221542823
174174,348349,348348,696697,652.9757113456726,1.000333875655997
175175,350351,350350,700701,656.5776813030243,0.9951937476635067
176176,352353,352352,704705,660.2646253108978,0.9901050416865473
177177,354355,354354,708709,663.8679192066193,0.9850669784755155
178178,356357,356356,712713,668.0356051921844,0.9800787949352525
179179,358359,358358,716717,671.919319152832,0.9751397436939442
180180,360361,360360,720721,675.9488081932068,0.970249092699305
181181,362363,362362,724725,679.559582233429,0.9654061247983918
182182,364365,364364,728729,682.8860001564026,0.9606101373392448
183183,366367,366366,732733,686.8987760543823,0.955860441805271
184184,368369,368368,736737,690.3873200416565,0.951156363440532
185185,370371,370370,740741,693.8249850273132,0.9464972408986796
186186,372373,372372,744745,697.9178631305695,0.9418824258827954
187187,374375,374374,748749,701.2998189926147,0.9373112828379817
188188,376377,376376,752753,704.6782472133636,0.9327831886112108
189189,378379,378378,756757,708.2353031635284,0.9282975321366393
190190,380381,380380,760761,712.0029621124268,0.9238537141445704
191191,382383,382382,764765,715.782338142395,0.91945114686132
192192,384385,384384,768769,719.7723503112793,0.9150892537309119
193193,386387,386386,772773,723.2217342853546,0.910767469129496
194194,388389,388388,776777,726.5924451351166,0.9064852381070523
195195,390391,390390,780781,729.9082312583923,0.9022420161218179
196196,392393,392392,784785,734.1089992523193,0.8980372688001808
197197,394395,394394,788789,737.932046175003,0.8938704716838402
198198,396397,396396,792793,741.7402150630951,0.8897411099860619
199199,398399,398398,796797,746.1522212028503,0.8856486783879518
200200,400401,400400,800801,749.815181016922,0.8815926807874348
201201,402403,402402,804805,753.6073632240295,0.8775726300973474
202202,404405,404404,808809,758.0359883308411,0.8735880480435299
203203,406407,406406,812813,762.6959691047668,0.8696384649338142
204204,408409,408408,816817,766.1974220275879,0.8657234194943157
205205,410411,410410,820821,770.0588102340698,0.8618424586456968
206206,412413,412412,824825,773.8684332370758,0.8579951373467338
207207,414415,414414,828829,778.128396987915,0.854181018377858
208208,416417,416416,832833,782.325679063797,0.8503996722065494
209209,418419,418418,836837,786.1213111877441,0.8466506767672399
210210,420421,420420,840841,789.8103301525116,0.8429336173394404
211211,422423,422422,844845,793.9313831329346,0.8392480863567471
212212,424425,424424,848849,797.7769801616669,0.8355936832595035
213213,426427,426426,852853,801.7052111625671,0.831970014345643
214214,428429,428428,856857,805.401641368866,0.8283766926051612
215215,430431,430430,860861,809.1752700805664,0.8248135627745796
216216,432433,432432,864865,813.0948390960693,0.8212803906553745
217217,434435,434434,868869,817.9788892269135,0.8177764469292015
218218,436437,436436,872873,822.8108930587769,0.8143013615190284
219219,438439,438438,876877,827.7778301239014,0.8108547787942371
220220,440441,440440,880881,832.3343253135681,0.8074363490995893
221221,442443,442442,884885,836.6380832195282,0.8040457285442244
222222,444445,444444,888889,840.0414340496063,0.8006825788870628
223223,446447,446446,892893,843.734904050827,0.7973465674112958
224224,448449,448448,896897,847.261194229126,0.7940373668116081
225225,450451,450450,900901,851.175971031189,0.7907546550759434
226226,452453,452452,904905,855.2420210838318,0.7874981153800036
227227,454455,454454,908909,858.750764131546,0.7842674359853845
228228,456457,456456,912913,862.1784932613373,0.7810623101322562
229229,458459,458458,916917,866.0286903381348,0.7778824359320424
230230,460461,460460,920921,870.2608001232147,0.7747275162801088
231231,462463,462462,924925,875.1588530540466,0.7715972587575379
232232,464465,464464,928929,879.619104385376,0.7684913755329035
233233,466467,466466,932933,883.7147121429443,0.765409583269502
234234,468469,468468,936937,888.9980461597443,0.7623516030453175
235235,470471,470470,940941,893.8469052314758,0.7593171602602524
236236,472473,472472,944945,898.5353002548218,0.7563059845524549
237237,474475,474474,948949,903.1606271266937,0.7533178097128257
238238,476477,476476,952953,907.6903049945831,0.7503523736104398
239239,478479,478478,956957,912.0796432495117,0.7474094181088731
240240,480481,480480,960961,916.4654712677002,0.7444886889898044
241241,482483,482482,964965,921.3947072029114,0.7415899358729803
242242,484485,484484,968969,926.1949019432068,0.7387129121598264
243243,486487,486486,972973,930.7813920974731,0.7358573749443167
244244,488489,488488,976977,935.5699870586395,0.7330230849456711
245245,490491,490490,980981,941.1516101360321,0.7302098064465099
246246,492493,492492,984985,946.1918830871582,0.7274173072255508
247247,494495,494494,988989,950.4976282119751,0.7246453584848496
248248,496497,496496,992993,955.6843943595886,0.7218937347915926
249249,498499,498498,996997,959.8007261753082,0.7191622140180698
250250,500501,500500,1001001,964.1884820461273,0.7164505772707344
251251,502503,502502,1005005,968.6207082271576,0.7137586088410899
252252,504505,504504,1009009,973.6453042030334,0.7110861044602643
253253,506507,506506,1013013,978.6540422439575,0.7084328886212461
254254,508509,508508,1017017,982.9233803749084,0.7057987144507933
255255,510511,510510,1021021,986.8508930206299,0.7031833783294132
256256,512513,512512,1025025,991.4910881519318,0.7005866795407201
257257,514515,514514,1029029,995.2930431365967,0.6980084202241414
258258,516517,516516,1033033,999.7409472465515,0.6954484053239867
259259,518519,518518,1037037,1004.2620091438293,0.6929064425221441
260260,520521,520520,1041041,1008.8224623203278,0.6903823422162532
261261,522523,522522,1045045,1012.7507922649384,0.687875917461497
262262,524525,524524,1049049,1016.9264371395111,0.6853869839069375
263263,526527,526526,1053053,1020.7484021186829,0.6829153597773256
264264,528529,528528,1057057,1024.876347064972,0.6804608658057987
265265,530531,530530,1061061,1029.2141313552856,0.6780233252047765
266266,532533,532532,1065065,1033.5218570232391,0.6756025636168488
267267,534535,534534,1069069,1037.2364153862,0.6731984090711194
268268,536537,536536,1073073,1040.7161831855774,0.6708106919468264
269269,538539,538538,1077077,1044.14586019516,0.6684392449278675
270270,540541,540540,1081081,1047.6245560646057,0.6660839029682393
271271,542543,542542,1085085,1052.2278912067413,0.663744503253838
272272,544545,544544,1089089,1056.7511463165283,0.6614208851533476
273273,546547,546546,1093093,1061.4749891757965,0.6591128902036871
274274,548549,548548,1097097,1065.5449793338776,0.6568203620463464
275275,550551,550550,1101101,1069.6838593482971,0.6545431464146532
276276,552553,552552,1105105,1074.3656511306763,0.6522810910882981
277277,554555,554554,1109109,1078.5629041194916,0.6500340458551364
278278,556557,556556,1113113,1082.4044601917267,0.6478018624911783
279279,558559,558558,1117117,1086.1876270771027,0.6455843947205722
280280,560561,560560,1121121,1089.8606872558594,0.6433814981719479
281281,562563,562562,1125125,1093.5893912315369,0.6411930303711415
282282,564565,564564,1129129,1097.8954610824585,0.6390188506920822
283283,566567,566566,1133133,1102.2103481292725,0.6368588203295076
284284,568569,568568,1137137,1106.5552382469177,0.6347128022753168
285285,570571,570570,1141141,1110.6858241558075,0.6325806612840097
286286,572573,572572,1145145,1115.17293715477,0.630462263847221
287287,574575,574574,1149149,1119.0555832386017,0.6283574781664356
288288,576577,576576,1153153,1123.0218741893768,0.6262661741184274
289289,578579,578578,1157157,1126.8736600875854,0.6241882232425269
290290,580581,580580,1161161,1131.5062642097473,0.6221234986933268
291291,582583,582582,1165165,1136.3736109733582,0.620075567620006
292292,584585,584584,1169169,1141.506997346878,0.6180415113940398
293293,586587,586586,1173173,1145.6248261928558,0.6160203920262575
294294,588589,588588,1177177,1149.7534823417664,0.6140120452710107
295295,590591,590590,1181181,1154.401908159256,0.6120163258565299
296296,592593,592592,1185185,1159.0058062076569,0.6100331002871826
297297,594595,594594,1189189,1163.2603282928467,0.608062242723463
298298,596597,596596,1193193,1167.385400056839,0.6061036325336318
299299,598599,598598,1197197,1171.1011183261871,0.6041571528203349
300300,600601,600600,1201201,1174.6044752597809,0.6022226895129279
301301,602603,602602,1205205,1178.0783081054688,0.6003001308090461
302302,604605,604604,1209209,1181.543424129486,0.5983893668289966
303303,606607,606606,1213213,1185.1531882286072,0.5964902893610997
304304,608609,608608,1217217,1188.6234080791473,0.5946064948675485
305305,610611,610610,1221221,1192.1017031669617,0.5927347973192809
306306,612613,612612,1225225,1195.5969820022583,0.5908745419401384
307307,614615,614614,1229229,1199.034418106079,0.589025570643571
308308,616617,616616,1233233,1202.4582509994507,0.587187758032087
309309,618619,618618,1237237,1205.9368391036987,0.5853609934511042
310310,620621,620620,1241241,1209.4567711353302,0.5835451733692025
311311,622623,622622,1245245,1212.9010820388794,0.5817401980475552
312312,624625,624624,1249249,1216.3419570922852,0.5799459701065643
313313,626627,626626,1253253,1219.7905042171478,0.5781623938655684
314314,628629,628628,1257257,1223.1667261123657,0.5763893750154239
315315,630631,630630,1261261,1226.7409892082214,0.5746268204984517
316316,632633,632632,1265265,1230.3473782539368,0.5728746384047554
317317,634635,634634,1269269,1233.9139420986176,0.5711327379449358
318318,636637,636636,1273273,1239.0840742588043,0.5694010293955216
319319,638639,638638,1277277,1243.9810991287231,0.5676794241007883
320320,640641,640640,1281281,1247.4920091629028,0.5659678344381973
321321,642643,642642,1285285,1251.2219722270966,0.5642661737947492
322322,644645,644644,1289289,1255.0074911117554,0.5625743565706216
323323,646647,646646,1293293,1259.3197371959686,0.5608922981409705
324324,648649,648648,1297297,1263.515601158142,0.5592199148577492
325325,650651,650650,1301301,1267.8572373390198,0.5575571240224235
326326,652653,652652,1305305,1272.4200892448425,0.5559038438805146
327327,654655,654654,1309309,1277.1754531860352,0.5542599936070474
328328,656657,656656,1313313,1281.3545053005219,0.5526254932847223
329329,658659,658658,1317317,1286.2246491909027,0.5510002639020968
330330,660661,660660,1321321,1290.7185173034668,0.5493842273299379
331331,662663,662662,1325325,1295.1890811920166,0.5477773063194036
332332,664665,664664,1329329,1299.783907175064,0.546179424480215
333333,666667,666666,1333333,1304.6851303577423,0.544590506271561
334334,668669,668668,1337337,1309.4837012290955,0.543010476998461
335335,670671,670670,1341341,1313.4726431369781,0.5414392627772031
336336,672673,672672,1345345,1317.733546257019,0.5398767905589921
337337,674675,674674,1349349,1322.330244064331,0.5383229880826548
338338,676677,676676,1353353,1325.865757226944,0.5367777838837355
339339,678679,678678,1357357,1329.3155381679535,0.5352411072890391
340340,680681,680680,1361361,1332.8576292991638,0.5337128883784317
341341,682683,682682,1365365,1336.4902420043945,0.5321930580103071
342342,684685,684684,1369369,1339.993324995041,0.53068154777975
343343,686687,686686,1373373,1344.6457033157349,0.5291782900349062
344344,688689,688688,1377377,1350.2570459842682,0.5276832178387849
345345,690691,690690,1381381,1356.005315065384,0.5261962649892666
346346,692693,692692,1385385,1360.6808743476868,0.524717365982724
347347,694695,694694,1389389,1364.989179134369,0.5232464560231165
348348,696697,696696,1393393,1368.9566712379456,0.5217834710038005
349349,698699,698698,1397397,1372.7180552482605,0.5203283475020726
350350,700701,700700,1401401,1376.601849079132,0.5188810227682552
351351,702703,702702,1405405,1381.4420561790466,0.5174414347147831
352352,704705,704704,1409409,1386.0807271003723,0.5160095219143841
353353,706707,706706,1413413,1390.0318830013275,0.5145852235818893
354354,708709,708708,1417417,1394.1821072101593,0.5131684795705951
355355,710711,710710,1421421,1398.2742471694946,0.5117592303686251
356356,712713,712712,1425425,1402.4046802520752,0.5103574170825596
357357,714715,714714,1429429,1406.4652881622314,0.5089629814319778
358358,716717,716716,1433433,1412.4596982002258,0.5075758657476399
359359,718719,718718,1437437,1417.2204620838165,0.5061960129478393
360360,720721,720720,1441441,1421.8511400222778,0.5048233665547741
361361,722723,722722,1445445,1426.4552931785583,0.5034578706618049
362362,724725,724724,1449449,1431.2153673171997,0.5020994699407311
363363,726727,726726,1453453,1436.4769971370697,0.5007481096363335
364364,728729,728728,1457457,1441.5361881256104,0.4994037355463661
365365,730731,730730,1461461,1446.2551171779633,0.4980662940251932
366366,732733,732732,1465465,1450.9590542316437,0.49673573197287624
367367,734735,734734,1469469,1456.796420097351,0.49541199683335435
368368,736737,736736,1473473,1462.2334172725677,0.49409503657807363
369369,738739,738738,1477477,1468.5720052719116,0.49278479969871114
370370,740741,740740,1481481,1473.936504125595,0.49148123521990783
371371,742743,742742,1485485,1478.8655881881714,0.49018429266834573
372372,744745,744744,1489489,1483.782291173935,0.4888939220854809
373373,746747,746746,1493493,1488.8481931686401,0.48761007400025846
374374,748749,748748,1497497,1494.4667613506317,0.48633269944548374
375375,750751,750750,1501501,1500.1719789505005,0.48506174993963214
376376,752753,752752,1505505,1505.535562992096,0.48379717748321127
377377,754755,754754,1509509,1510.2867341041565,0.48253893454420904
378378,756757,756756,1513513,1515.2033281326294,0.48128697407264553
379379,758759,758758,1517517,1519.9594333171844,0.4800412494751072
380380,760761,760760,1521521,1524.7632203102112,0.47880171461656573
381381,762763,762762,1525525,1529.5435631275177,0.4775683238131023
382382,764765,764764,1529529,1534.5856742858887,0.47634103183554544
383383,766767,766766,1533533,1539.4419281482697,0.475119793887643
384384,768769,768768,1537537,1544.2431001663208,0.4739045656151575
385385,770771,770770,1541541,1549.1065862178802,0.4726953030876757
386386,772773,772772,1545545,1553.9089422225952,0.4714919628095231
387387,774775,774774,1549549,1558.737622976303,0.4702945016997546
388388,776777,776776,1553553,1563.4843802452087,0.4691028770957928
389389,778779,778778,1557557,1568.6419591903687,0.4679170467388758
390390,780781,780780,1561561,1573.4107670783997,0.4667369687849714
391391,782783,782782,1565565,1578.3499341011047,0.46556260178658704
392392,784785,784784,1569569,1583.1400320529938,0.46439390469458885
393393,786787,786786,1573573,1588.0486941337585,0.46323083683819277
394394,788789,788788,1577577,1592.781967163086,0.46207335795588733
395395,790791,790790,1581581,1597.619972229004,0.46092142815177795
396396,792793,792792,1585585,1602.3776743412018,0.4597750079083198
397397,794795,794794,1589589,1607.1510062217712,0.45863405808631796
398398,796797,796796,1593593,1612.0480470657349,0.45749853991401324
399399,798799,798798,1597597,1616.7545430660248,0.4563684149816254
400400,800801,800800,1601601,1622.0734519958496,0.4552436452413531
401401,802803,802802,1605605,1627.0845229625702,0.4541241930000979
402402,804805,804804,1609609,1631.9854190349579,0.4530100209176453
403403,806807,806806,1613613,1637.0663783550262,0.45190109200302686
404404,808809,808808,1617617,1641.2258653640747,0.4507973695999681
405405,810811,810810,1621621,1645.8773260116577,0.44969881740325945
406406,812813,812812,1625625,1650.1589500904083,0.44860539943692856
407407,814815,814814,1629629,1653.856714963913,0.447517080061516
408408,816817,816816,1633633,1658.0349543094635,0.4464338239540666
409409,818819,818818,1637637,1661.9289720058441,0.4453555961335951
410410,820821,820820,1641641,1666.130210161209,0.4442823619247065
411411,822823,822822,1645645,1669.6481840610504,0.4432140869739669
412412,824825,824824,1649649,1673.4715340137482,0.44215073724080867
413413,826827,826826,1653653,1677.1264083385468,0.4410922789993492
414414,828829,828828,1657657,1680.6413581371307,0.4400386788202013
415415,830831,830830,1661661,1684.4364511966705,0.43898990358684387
416416,832833,832832,1665665,1688.616670370102,0.4379459204737941
417417,834835,834834,1669669,1692.2700412273407,0.4369066969575215
418418,836837,836836,1673673,1696.1736302375793,0.4358722008000768
419419,838839,838838,1677677,1700.5045311450958,0.4348424000581872
420420,840841,840840,1681681,1704.9272429943085,0.43381726307598
421421,842843,842842,1685685,1708.7812809944153,0.43279675847770704
422422,844845,844844,1689689,1712.5898931026459,0.43178085516592546
423423,846847,846846,1693693,1716.4002873897552,0.4307695223233168
424424,848849,848848,1697697,1721.0046591758728,0.42976272940177296
425425,850851,850850,1701701,1725.0590620040894,0.42876044612967235
426426,852853,852852,1705705,1729.6357321739197,0.4277626424936898
427427,854855,854854,1709709,1733.244648218155,0.42676928874789155
428428,856857,856856,1713713,1737.080070257187,0.42578035538645054
429429,858859,858858,1717717,1740.6764752864838,0.424795813180026
430430,860861,860860,1721721,1744.0223271846771,0.4238156331466598
431431,862863,862862,1725725,1747.410441160202,0.4228397865608713
432432,864865,864864,1729729,1750.8246581554413,0.4218682449482003
433433,866867,866866,1733733,1754.2602121829987,0.4209009800833883
434434,868869,868868,1737737,1757.6699981689453,0.4199379639903782
435435,870871,870870,1741741,1761.033910036087,0.41897916892958165
436436,872873,872872,1745745,1764.4561681747437,0.4180245674069738
437437,874875,874874,1749749,1767.9414582252502,0.41707413216317946
438438,876877,876876,1753753,1771.2986731529236,0.41612783617893
439439,878879,878878,1757757,1774.6986773014069,0.41518565266051155
440440,880881,880880,1761761,1778.0653681755066,0.4142475550506788
441441,882883,882882,1765765,1781.472073316574,0.4133135170177411
442442,884885,884884,1769769,1784.9698233604431,0.4123835124555626
443443,886887,886886,1773773,1788.2921640872955,0.41145751547810505
444444,888889,888888,1777777,1791.7067413330078,0.41053550042306597
445445,890891,890890,1781781,1796.610784292221,0.4096174418446026
446446,892893,892892,1785785,1801.6142671108246,0.40870331451515085
447447,894895,894894,1789789,1805.6892442703247,0.4077930934181495
448448,896897,896896,1793793,1809.9175691604614,0.4068867537462211
449449,898899,898898,1797797,1813.8758211135864,0.4059842709048098
450450,900901,900900,1801801,1818.9941339492798,0.4050856205049058
451451,902903,902902,1805805,1823.1029653549194,0.40419077836122597
452452,904905,904904,1809809,1827.0884501934052,0.403299720490395
453453,906907,906906,1813813,1831.6608412265778,0.40241242311458336
454454,908909,908908,1817817,1835.7834141254425,0.40152886264331755
455455,910911,910910,1821821,1839.8921611309052,0.40064901569348876
456456,912913,912912,1825825,1844.373458147049,0.39977285906752513
457457,914915,914914,1829829,1847.9315283298492,0.39890036976612464
458458,916917,916916,1833833,1851.3296251296997,0.39803152498097916
459459,918919,918918,1837837,1854.7605612277985,0.3971663020820415
460460,920921,920920,1841841,1858.1779391765594,0.3963046786320774
461461,922923,922922,1845845,1861.7013471126556,0.39544663238302746
462462,924925,924924,1849849,1865.1827402114868,0.3945921412578173
463463,926927,926926,1853853,1868.885555267334,0.39374118337036634
464464,928929,928928,1857857,1872.2696101665497,0.39289373700739816
465465,930931,930930,1861861,1875.8367280960083,0.39204978063389717
466466,932933,932932,1865865,1879.2131371498108,0.3912092928912898
467467,934935,934934,1869869,1882.6602239608765,0.3903722525883495
468468,936937,936936,1873873,1886.0829710960388,0.3895386387139297
469469,938939,938938,1877877,1889.628573179245,0.3887084304169548
470470,940941,940940,1881881,1892.9925680160522,0.38788160702642926
471471,942943,942942,1885885,1896.4744791984558,0.3870581480296096
472472,944945,944944,1889889,1899.8893361091614,0.3862380330756423
473473,946947,946946,1893893,1903.4184532165527,0.385421241984659
474474,948949,948948,1897897,1906.8314232826233,0.3846077547332243
475475,950951,950950,1901901,1910.2604310512543,0.3837975514561549
476476,952953,952952,1905905,1913.6364710330963,0.3829906124537956
477477,954955,954954,1909909,1917.1315541267395,0.3821869181738293
478478,956957,956956,1913913,1920.5220773220062,0.3813866466007312
479479,958959,958958,1917917,1923.9538233280182,0.38059045380578027
480480,960961,960960,1921921,1927.5849850177765,0.37979747100507666
481481,962963,962962,1925925,1931.3182101249695,0.3790076554978441
482482,964965,964964,1929929,1935.6588401794434,0.3782209870478255
483483,966967,966966,1933933,1940.141041278839,0.3774374464137509
484484,968969,968968,1937937,1944.5798723697662,0.37665701482728764
485485,970971,970970,1941941,1948.4910531044006,0.3758796738293313
486486,972973,972972,1945945,1952.9113702774048,0.37510540515722823
487487,974975,974974,1949949,1956.485532283783,0.3743341907284048
488488,976977,976976,1953953,1959.788553237915,0.37356601630199293
489489,978979,978978,1957957,1963.1790392398834,0.3728008618181775
490490,980981,980980,1961961,1966.78635430336,0.37203870870143874
491491,982983,982982,1965965,1970.1354880332947,0.37127953921299195
492492,984985,984984,1969969,1973.5113971233368,0.370523335866892
493493,986987,986986,1973973,1976.9553091526031,0.3697700813681877
494494,988989,988988,1977977,1980.3737442493439,0.3690197585765418
495495,990991,990990,1981981,1983.9994843006134,0.3682723505080503
496496,992993,992992,1985985,1988.610433101654,0.36752784030977637
497497,994995,994994,1989989,1993.0840141773224,0.3667862112615694
498498,996997,996996,1993993,1997.769424200058,0.366047446781522
499499,998999,998998,1997997,2002.0296003818512,0.36531153041141806
500501,1001003,1001002,2002005,2006.0177471637726,0.3645777148758498
501502,1003005,1003004,2006009,2010.097617149353,0.3638474486560881
502503,1005007,1005006,2010013,2014.3587582111359,0.3631199819064932
503504,1007009,1007008,2014017,2018.309172153473,0.3623952986636141
504505,1009011,1009010,2018021,2022.11687707901,0.36167338308951
505506,1011013,1011012,2022025,2026.289174079895,0.3609542194590176
506507,1013015,1013014,2026029,2030.2054562568665,0.36023779217430274
507508,1015017,1015016,2030033,2034.0663380622864,0.3595240857448516
508509,1017019,1017018,2034037,2037.88183426857,0.3588130848020228
509510,1019021,1019020,2038041,2041.7393951416016,0.3581047740917711
510511,1021023,1021022,2042045,2045.560776233673,0.35739913847646676
511512,1023025,1023024,2046049,2049.4223160743713,0.35669616292216233
512513,1025027,1025026,2050053,2053.353338241577,0.3559958325186017
513514,1027029,1027028,2054057,2058.6507182121277,0.35529813245739206
514515,1029031,1029030,2058061,2064.006545305252,0.3546030480410991
515516,1031033,1031032,2062065,2068.5824749469757,0.35391056469052273
516517,1033035,1033034,2066069,2073.737066268921,0.35322066792105034
517518,1035037,1035036,2070073,2080.0226442813873,0.35253334336084663
518519,1037039,1037038,2074077,2085.249703168869,0.35184857674175873
519520,1039041,1039040,2078081,2090.1787481307983,0.3511663539065921
520521,1041043,1041042,2082085,2095.0051572322845,0.3504866607945587
521522,1043045,1043044,2086089,2099.3284101486206,0.34980948345582874
522523,1045047,1045046,2090093,2103.5663232803345,0.349134808029703
523524,1047049,1047048,2094097,2107.8050141334534,0.3484626207700785
524525,1049051,1049050,2098101,2112.1243031024933,0.34779290801998286
525526,1051053,1051052,2102105,2116.386913061142,0.34712565623522096
526527,1053055,1053054,2106109,2120.741932153702,0.34646085194981424
527528,1055057,1055056,2110113,2125.278600215912,0.34579848181783746
528529,1057059,1057058,2114117,2129.532879114151,0.3451385325697629
529530,1059061,1059060,2118121,2133.945965051651,0.3444809910488402
530531,1061063,1061062,2122125,2138.333424091339,0.3438258441783546
531532,1063065,1063064,2126129,2142.5362071990967,0.3431730789852736
532533,1065067,1065066,2130133,2147.9036540985107,0.3425226825875143
533534,1067069,1067068,2134137,2152.117287158966,0.34187464219030517
534535,1069071,1069070,2138141,2156.0139582157135,0.3412289451007382
535536,1071073,1071072,2142145,2159.9061481952667,0.34058557870412187
536537,1073075,1073074,2146149,2163.906302213669,0.3399445304839901
537538,1075077,1075076,2150153,2167.7261941432953,0.33930578801300726
538539,1077079,1077078,2154157,2171.6819932460785,0.3386693389438733
539540,1079081,1079080,2158161,2175.5847132205963,0.33803517102751357
540541,1081083,1081082,2162165,2179.4896721839905,0.33740327209488896
541542,1083085,1083084,2166169,2183.43017911911,0.33677363006245287
542543,1085087,1085086,2170173,2187.4664533138275,0.33614623293760815
543544,1087089,1087088,2174177,2191.489891052246,0.3355210688041552
544545,1089091,1089090,2178181,2195.374687194824,0.334898125836844
545546,1091093,1091092,2182185,2199.280172109604,0.33427739228864084
546547,1093095,1093094,2186189,2203.2208292484283,0.33365885649618576
547548,1095097,1095096,2190193,2207.152501344681,0.3330425068779732
548549,1097099,1097098,2194197,2211.382154941559,0.33242833193617116
549550,1099101,1099100,2198201,2215.4820053577423,0.3318163202438882
550551,1101103,1101102,2202205,2219.4628479480743,0.3312064604670013
551552,1103105,1103104,2206209,2223.4993681907654,0.3305987413350522
552553,1105107,1105106,2210213,2227.656678199768,0.32999315166671295
553554,1107109,1107108,2214217,2231.4911301136017,0.3293896803570533
554555,1109111,1109110,2218221,2235.7479553222656,0.3287883163757215
555556,1111113,1111112,2222225,2239.6273012161255,0.32818904875966837
556557,1113115,1113114,2226229,2243.7461450099945,0.32759186664043227
557558,1115117,1115116,2230233,2247.6856219768524,0.3269967592059402
558559,1117119,1117118,2234237,2251.7518503665924,0.3264037157277926
559560,1119121,1119120,2238241,2255.7585892677307,0.32581272555034957
560561,1121123,1121122,2242245,2259.882063150406,0.3252237780889118
561562,1123125,1123124,2246249,2263.9423060417175,0.3246368628297205
562563,1125127,1125126,2250253,2268.0437881946564,0.3240519693317765
563564,1127129,1127128,2254257,2271.9162571430206,0.3234690872304782
564565,1129131,1129130,2258261,2275.9665870666504,0.3228882062212506
565566,1131133,1131132,2262265,2279.932613134384,0.3223093160777353
566567,1133135,1133134,2266269,2284.8305191993713,0.32173240663905744
567568,1135137,1135136,2270273,2289.645221233368,0.32115746781528287
568569,1137139,1137138,2274277,2294.2820081710815,0.320584489578323
569570,1139141,1139140,2278281,2298.329277276993,0.3200134619783057
570571,1141143,1141142,2282285,2302.459857225418,0.3194443751217477
571572,1143145,1143144,2286289,2306.1786201000214,0.3188772191879252
572573,1145147,1145146,2290293,2309.7698612213135,0.31831198441977904
573574,1147149,1147148,2294297,2313.1011922359467,0.31774866112391464
574575,1149151,1149150,2298301,2316.5494000911713,0.3171872396742401
575576,1151153,1151152,2302305,2320.0270183086395,0.31662771050832816
576577,1153155,1153154,2306309,2323.513035058975,0.3160700641292351
577578,1155157,1155156,2310313,2327.233255147934,0.31551429109458695
578579,1157159,1157158,2314317,2330.7878980636597,0.31496038203658827
579580,1159161,1159160,2318321,2334.642966032028,0.3144083276420133
580581,1161163,1161162,2322325,2339.2455921173096,0.313858118657663
581582,1163165,1163164,2326329,2343.2196111679077,0.3133097459012788
582583,1165167,1165166,2330333,2347.2988801002502,0.31276320023971493
583584,1167169,1167168,2334337,2351.2134730815887,0.3122184726053092
584585,1169171,1169170,2338341,2355.0969161987305,0.3116755539922451
585586,1171173,1171172,2342345,2358.8451471328735,0.3111344354456378
586587,1173175,1173174,2346349,2363.0910251140594,0.310595108077905
587588,1175177,1175176,2350353,2367.8284211158752,0.31005756305785326
588589,1177179,1177178,2354357,2372.640011072159,0.30952179160158266
589590,1179181,1179180,2358361,2377.980401277542,0.30898778500340995
590591,1181183,1181182,2362365,2382.0924232006073,0.30845553459039365
591592,1183185,1183184,2366369,2386.3172092437744,0.30792503176598984
592593,1185187,1185186,2370373,2390.540163040161,0.30739626797549136
593594,1187189,1187188,2374377,2395.822480201721,0.3068692347242177
594595,1189191,1189190,2378381,2400.6161913871765,0.30634392357751494
595596,1191193,1191192,2382385,2406.2859382629395,0.30582032614438504
596597,1193195,1193194,2386389,2411.311756134033,0.30529843410113244
597598,1195197,1195196,2390393,2415.6853642463684,0.3047782391658984
598599,1197199,1197198,2394397,2420.255615234375,0.30425973311685084
599600,1199201,1199200,2398401,2425.0329761505127,0.30374290778127033
600601,1201203,1201202,2402405,2430.7922642230988,0.3032277550428262
601602,1203205,1203204,2406409,2435.797045946121,0.3027142668288434
602603,1205207,1205206,2410413,2440.4683990478516,0.30220243512849265
603604,1207209,1207208,2414417,2444.99489402771,0.30169225197823835
604605,1209211,1209210,2418421,2449.1912171840668,0.3011837094600196
605606,1211213,1211212,2422425,2453.6202170848846,0.3006767997103452
606607,1213215,1213214,2426429,2457.7583191394806,0.3001715149202937
607608,1215217,1215216,2430433,2462.241960287094,0.2996678473227803
608609,1217219,1217218,2434437,2466.2153992652893,0.29916578920165193
609610,1219221,1219220,2438441,2470.095078229904,0.2986653328916873
610611,1221223,1221222,2442445,2474.1374802589417,0.2981664707749587
611612,1223225,1223224,2446449,2478.094075202942,0.2976691952771944
612613,1225227,1225226,2450453,2482.6767992973328,0.297173498884149
613614,1227229,1227228,2454457,2487.823217153549,0.2966793741143192
614615,1229231,1229230,2458461,2492.723930120468,0.29618681353895226
615616,1231233,1231232,2462465,2497.2767663002014,0.29569580977658916
616617,1233235,1233234,2466469,2501.11354804039,0.2952063554948836
617618,1235237,1235236,2470473,2505.6589481830597,0.2947184433978691
618619,1237239,1237238,2474477,2510.700328350067,0.2942320662441489
619620,1239241,1239240,2478481,2515.5438010692596,0.29374721683052485
620621,1241243,1241242,2482485,2520.4555842876434,0.29326388800836867
621622,1243245,1243244,2486489,2524.7237679958344,0.2927820726599748
622623,1245247,1245246,2490493,2528.6877710819244,0.2923017637240264
623624,1247249,1247248,2494497,2533.1125180721283,0.29182295417194837
624625,1249251,1249250,2498501,2536.9188022613525,0.2913456370260974
625626,1251253,1251252,2502505,2540.84997010231,0.29086980535248586
626627,1253255,1253254,2506509,2544.691376209259,0.29039545224986796
627628,1255257,1255256,2510513,2548.484896183014,0.2899225708733866
628629,1257259,1257258,2514517,2552.3949921131134,0.2894511544109264
629630,1259261,1259260,2518521,2556.3258333206177,0.28898119609402784
630631,1261263,1261262,2522525,2560.107931137085,0.2885126891960681
631632,1263265,1263264,2526529,2563.9389741420746,0.2880456270304421
632633,1265267,1265266,2530533,2567.7882602214813,0.2875800029542006
633634,1267269,1267268,2534537,2571.6607241630554,0.28711581036077405
634635,1269271,1269270,2538541,2575.7631862163544,0.2866530426854297
635636,1271273,1271272,2542545,2580.1092541217804,0.2861916934052715
636637,1273275,1273274,2546549,2584.019475221634,0.2857317560374213
637638,1275277,1275276,2550553,2587.9754853248596,0.2852732241299236
638639,1277279,1277278,2554557,2591.904461145401,0.2848160912817548
639640,1279281,1279280,2558561,2595.849263191223,0.2843603511191759
640641,1281283,1281282,2562565,2599.668538093567,0.2839059973193798
641642,1283285,1283284,2566569,2603.565357208252,0.2834530235868442
642643,1285287,1285286,2570573,2607.4621522426605,0.2830014236642455
643644,1287289,1287288,2574577,2611.6844589710236,0.28255119134155393
644645,1289291,1289290,2578581,2615.736438035965,0.28210232043420547
645646,1291293,1291292,2582585,2620.3500893115997,0.28165480480674887
646647,1293295,1293294,2586589,2624.816430091858,0.28120863834556076
647648,1295297,1295296,2590593,2629.486376285553,0.28076381498431147
648649,1297299,1297298,2594597,2634.4627912044525,0.2803203286930511
649650,1299301,1299300,2598601,2638.6784512996674,0.2798781734727527
650651,1301303,1301302,2602605,2642.7129940986633,0.2794373433589499
651652,1303305,1303304,2606609,2647.37988615036,0.2789978324290132
652653,1305307,1305306,2610613,2652.0488970279694,0.278559634791236
653654,1307309,1307308,2614617,2656.4028720855713,0.2781227445884724
654655,1309311,1309310,2618621,2660.9182393550873,0.2776871559963183
655656,1311313,1311312,2622625,2665.8875682353973,0.27725286323220644
656657,1313315,1313314,2626629,2670.738715171814,0.2768198605408543
657658,1315317,1315316,2630633,2675.213366985321,0.2763881422015402
658659,1317319,1317318,2634637,2679.9327280521393,0.27595770253174123
659660,1319321,1319320,2638641,2684.6244921684265,0.2755285358725814
660661,1321323,1321322,2642645,2688.6398482322693,0.27510063660884043
661662,1323325,1323324,2646649,2692.4339802265167,0.27467399915258284
662663,1325327,1325326,2650653,2696.3190472126007,0.27424861795225297
663664,1327329,1327328,2654657,2700.2591800689697,0.273824487481761
664665,1329331,1329330,2658661,2704.3001792430878,0.27340160225321597
665666,1331333,1331332,2662665,2708.256058216095,0.2729799568114686
666667,1333335,1333334,2666669,2712.452346086502,0.2725595457250165
667668,1335337,1335336,2670673,2716.377921104431,0.27214036360237515
668669,1337339,1337338,2674677,2720.2181470394135,0.27172240507934475
669670,1339341,1339340,2678681,2724.2023112773895,0.2713056648262864
670671,1341343,1341342,2682685,2728.238890171051,0.2708901375372079
671672,1343345,1343344,2686689,2732.1759662628174,0.2704758179424971
672673,1345347,1345346,2690693,2736.212969303131,0.2700627007998264
673674,1347349,1347348,2694697,2740.6351573467255,0.26965078090324823
674675,1349351,1349350,2698701,2745.145215988159,0.26924005306864274
675676,1351353,1351352,2702705,2749.8501551151276,0.26883051214463194
676677,1353355,1353354,2706709,2754.412851333618,0.2684221530089417
677678,1355357,1355356,2710713,2759.1700100898743,0.2680149705702206
678679,1357359,1357358,2714717,2763.8282899856567,0.26760895976622123
679680,1359361,1359360,2718721,2768.4428951740265,0.26720411556198087
680681,1361363,1361362,2722725,2773.308799266815,0.2668004329480027
681682,1363365,1363364,2726729,2778.3421223163605,0.2663979069511697
682683,1365367,1365366,2730733,2783.4723110198975,0.2659965326220117
683684,1367369,1367368,2734737,2788.474067211151,0.2655963050365244
684685,1369371,1369370,2738741,2793.131668329239,0.2651972193052643
685686,1371373,1371372,2742745,2798.152595281601,0.2647992705587967
686687,1373375,1373374,2746749,2803.0262660980225,0.26440245395860984
687688,1375377,1375376,2750753,2807.7096843719482,0.2640067646989337
688689,1377379,1377378,2754757,2812.440008163452,0.26361219799036917
689690,1379381,1379380,2758761,2817.4404122829437,0.26321874908171594
690691,1381383,1381382,2762765,2822.302119255066,0.2628264132363256
691692,1383385,1383384,2766769,2827.1937172412872,0.26243518575574853
692693,1385387,1385386,2770773,2832.816375017166,0.262045061959725
693694,1387389,1387388,2774777,2838.0903301239014,0.2616560371952801
694695,1389391,1389390,2778781,2842.8503732681274,0.2612681068403617
695696,1391393,1391392,2782785,2848.632763147354,0.26088126629474573
696697,1393395,1393394,2786789,2853.7768721580505,0.26049551098549273
697698,1395397,1395396,2790793,2858.6637670993805,0.2601108363633102
698699,1397399,1397398,2794797,2863.4022283554077,0.2597272379007336
699700,1399401,1399400,2798801,2868.3988831043243,0.259344711106678
700701,1401403,1401402,2802805,2873.8751032352448,0.25896325150279154
701702,1403405,1403404,2806809,2880.345852136612,0.2585828546416451
702703,1405407,1405406,2810813,2886.342609167099,0.25820351610127545
703704,1407409,1407408,2814817,2891.6619622707367,0.25782523147972825
704705,1409411,1409410,2818821,2896.974911212921,0.25744799640051497
705706,1411413,1411412,2822825,2901.8947381973267,0.25707180651625094
706707,1413415,1413414,2826829,2906.718607187271,0.2566966574995604
707708,1415417,1415416,2830833,2911.559735059738,0.2563225450430764
708709,1417419,1417418,2834837,2916.515273332596,0.25594946486853587
709710,1419421,1419420,2838841,2921.601709127426,0.2555774127213226
710711,1421423,1421422,2842845,2926.680436372757,0.25520638436137233
711712,1423425,1423424,2846849,2931.905862092972,0.2548363755850005
712713,1425427,1425426,2850853,2938.114709377289,0.2544673822048935
713714,1427429,1427428,2854857,2944.3923723697662,0.25409940005374665
714715,1429431,1429430,2858861,2949.3946681022644,0.25373242498790205
715716,1431433,1431432,2862865,2954.424651145935,0.25336645289462467
716717,1433435,1433434,2866869,2959.3020589351654,0.25300147966845543
717718,1435437,1435436,2870873,2963.3436920642853,0.25263750124031503
718719,1437439,1437438,2874877,2967.8830151557922,0.2522745135556761
719720,1439441,1439440,2878881,2971.655750274658,0.2519125125836581
720721,1441443,1441442,2882885,2975.401031255722,0.2515514943133894
721722,1443445,1443444,2886889,2978.7874920368195,0.25119145475946425
722723,1445447,1445446,2890893,2982.1913599967957,0.2508323899546667
723724,1447449,1447448,2894897,2985.6497342586517,0.2504742959536088
724725,1449451,1449450,2898901,2989.4414851665497,0.2501171688309114
725726,1451453,1451452,2902905,2992.9159893989563,0.24976100468848017
726727,1453455,1453454,2906909,2996.559947013855,0.24940579963913478
727728,1455457,1455456,2910913,3001.002346277237,0.2490515498247987
728729,1457459,1457458,2914917,3005.6408910751343,0.24869825140376633
729730,1459461,1459460,2918921,3010.6413333415985,0.2483459005579789
730731,1461463,1461462,2922925,3015.144773244858,0.24799449348574854
731732,1463465,1463464,2926929,3018.5315062999725,0.24764402640721528
732733,1465467,1465466,2930933,3022.0127601623535,0.24729449556434702
733734,1467469,1467468,2934937,3025.8483831882477,0.24694589721730154
734735,1469471,1469470,2938941,3029.3338911533356,0.24659822764442652
735736,1471473,1471472,2942945,3032.80007314682,0.2462514831495355
736737,1473475,1473474,2946949,3036.2491402626038,0.24590566004735592
737738,1475477,1475476,2950953,3039.5801362991333,0.24556075467808114
738739,1477479,1477478,2954957,3043.0785291194916,0.24521676340191334
739740,1479481,1479480,2958961,3046.484062194824,0.24487368259360665
740741,1481483,1481482,2962965,3049.875679254532,0.24453150865156204
741742,1483485,1483484,2966969,3053.265248298645,0.24419023799237038
742743,1485487,1485486,2970973,3057.1912240982056,0.24384986705081246
743744,1487489,1487488,2974977,3061.1397643089294,0.24351039227258298
744745,1489491,1489490,2978981,3064.5405061244965,0.24317181013429945
745746,1491493,1491492,2982985,3067.9453961849213,0.24283411712531233
746747,1493495,1493494,2986989,3071.5221722126007,0.24249730975316197
747748,1495497,1495496,2990993,3075.844973087311,0.24216138454175962
748749,1497499,1497498,2994997,3079.9878561496735,0.24182633804048237
749750,1499501,1499500,2999001,3084.420312166214,0.2414921668059833
750751,1501503,1501502,3003005,3088.7487790584564,0.24115886742220027
751752,1503505,1503504,3007009,3093.312391281128,0.24082643648398516
752753,1505507,1505506,3011013,3097.003988265991,0.24049487061165564
753754,1507509,1507508,3015017,3100.8956921100616,0.24016416643280536
754755,1509511,1509510,3019021,3105.2026612758636,0.2398343206004938
755756,1511513,1511512,3023025,3109.9316132068634,0.23950532978051342
756757,1513515,1513514,3027029,3114.186671257019,0.2391771906586655
757758,1515517,1515516,3031033,3118.471620082855,0.23884989993894123
758759,1517519,1517518,3035037,3121.98721408844,0.2385234543344268
759760,1519521,1519520,3039041,3126.3245401382446,0.23819785058549314
760761,1521523,1521522,3043045,3131.1259241104126,0.23787308544524421
761762,1523525,1523524,3047049,3135.306313276291,0.23754915567769785
762763,1525527,1525526,3051053,3140.3014571666718,0.23722605806869979
763764,1527529,1527528,3055057,3145.992125272751,0.2369037894259236
764765,1529531,1529530,3059061,3151.3027822971344,0.2365823465606809
765766,1531533,1531532,3063065,3156.391442298889,0.23626172631156805
766767,1533535,1533534,3067069,3160.949261188507,0.23594192552809545
767768,1535537,1535536,3071073,3165.844600200653,0.23562294107614434
768769,1537539,1537538,3075077,3173.175401210785,0.23530476983978588
769770,1539541,1539540,3079081,3181.5291740894318,0.23498740871582413
770771,1541543,1541542,3083085,3187.409699201584,0.2346708546156151
771772,1543545,1543544,3087089,3193.2137322425842,0.23435510447052366
772773,1545547,1545546,3091093,3198.5261261463165,0.23404015522828558
773774,1547549,1547548,3095097,3203.9737191200256,0.23372602167728473
774775,1549551,1549550,3099101,3210.027833223343,0.23341270703349437
775776,1551553,1551552,3103105,3215.4425930976868,0.233100185289004
776777,1553555,1553554,3107109,3220.2418780326843,0.2327884526566777
777778,1555557,1555556,3111113,3225.1430792808533,0.2324775060515094
778779,1557559,1557558,3115117,3229.9782462120056,0.23216734247580462
779780,1559561,1559560,3119121,3234.6858479976654,0.23185795895915362
780781,1561563,1561562,3123125,3239.458393096924,0.23154935255843156
781782,1563565,1563564,3127129,3245.164924144745,0.23124152034324652
782783,1565567,1565566,3131133,3253.1613070964813,0.23093445940503443
783784,1567569,1567568,3135137,3260.6484310626984,0.23062816684978316
784785,1569571,1569570,3139141,3268.2834134101868,0.23032263980530843
785786,1571573,1571572,3143145,3275.715228319168,0.23001787539760699
786787,1573575,1573574,3147149,3283.326473236084,0.22971387078723637
787788,1575577,1575576,3151153,3290.8169481754303,0.22941062313111615
788789,1577579,1577578,3155157,3298.6061103343964,0.2291081296170887
789790,1579581,1579580,3159161,3306.7663872241974,0.22880638743299642
790791,1581583,1581582,3163165,3315.0606923103333,0.22850539378850954
791792,1583585,1583584,3167169,3323.192142009735,0.22820514590603125
792793,1585587,1585586,3171173,3330.971155166626,0.22790564101887867
793794,1587589,1587588,3175177,3338.572552204132,0.22760687637492083
794795,1589591,1589590,3179181,3346.577210187912,0.22730884923839767
795796,1591593,1591592,3183185,3354.6717162132263,0.22701155688446306
796797,1593595,1593594,3187189,3362.530310153961,0.2267149966010038
797798,1595597,1595596,3191193,3370.58385515213,0.2264191656922776
798799,1597599,1597598,3195197,3378.985915184021,0.22612406147527508
799800,1599601,1599600,3199201,3387.114328145981,0.22582968127426284
800801,1601603,1601602,3203205,3395.2907671928406,0.22553602243533533
801802,1603605,1603604,3207209,3403.3951210975647,0.22524308231186296
802803,1605607,1605606,3211213,3412.8424570560455,0.2249508582699491
803804,1607609,1607608,3215217,3421.914238214493,0.22465934769206797
804805,1609611,1609610,3219221,3431.744725227356,0.22436854797160777
805806,1611613,1611612,3223225,3441.067983150482,0.22407845650923264
806807,1613615,1613614,3227229,3449.6597340106964,0.22378907073289156
807808,1615617,1615616,3231233,3458.3735830783844,0.22350038806507655
808809,1617619,1617618,3235237,3467.110871076584,0.22321240595374547
809810,1619621,1619620,3239241,3475.7241451740265,0.22292512185413216
810811,1621623,1621622,3243245,3484.437296152115,0.22263853323056537
811812,1623625,1623624,3247249,3493.1625320911407,0.22235263757102075
812813,1625627,1625626,3251253,3501.786389350891,0.22206743235983595
813814,1627629,1627628,3255257,3511.1194140911102,0.2217829151031765
814815,1629631,1629630,3259261,3519.8272802829742,0.22149908332175983
815816,1631633,1631632,3263265,3529.253045320511,0.22121593453994137
816817,1633635,1633634,3267269,3538.170619249344,0.22093346629844746
817818,1635637,1635636,3271273,3546.709141969681,0.22065167614891834
818819,1637639,1637638,3275277,3555.255844116211,0.2203705616575462
819820,1639641,1639640,3279281,3564.0813863277435,0.2200901203941612
820821,1641643,1641642,3283285,3573.626139163971,0.21981034995405935
821822,1643645,1643644,3287289,3582.618198156357,0.21953124792707968
822823,1645647,1645646,3291293,3591.990026950836,0.2192528119267081
823824,1647649,1647648,3295297,3600.7386631965637,0.21897503957552544
824825,1649651,1649650,3299301,3611.086451292038,0.21869792850156955
825826,1651653,1651652,3303305,3621.493383169174,0.2184214763565251
826827,1653655,1653654,3307309,3632.2160172462463,0.2181456807829818
827828,1655657,1655656,3311313,3643.796555995941,0.2178705394580902
828829,1657659,1657658,3315317,3652.3333423137665,0.21759605005354388
829830,1659661,1659660,3319321,3661.0143580436707,0.21732221025740728
830831,1661663,1661662,3323325,3669.7670860290527,0.2170490177704778
831832,1663665,1663664,3327329,3679.4889709949493,0.21677647029900982
832833,1665667,1665666,3331333,3688.910982131958,0.21650456556562858
833834,1667669,1667668,3335337,3697.777684211731,0.21623330130205431
834835,1669671,1669670,3339341,3706.673821210861,0.21596267524910218
835836,1671673,1671672,3343345,3715.5988132953644,0.21569268516032025
836837,1673675,1673674,3347349,3724.51518201828,0.2154233287947136
837838,1675677,1675676,3351353,3734.454131126404,0.21515460393129615
838839,1677679,1677678,3355357,3744.1093401908875,0.21488650834908185
839840,1679681,1679680,3359361,3753.1913273334503,0.21461903984345554
840841,1681683,1681682,3363365,3761.715914964676,0.21435219622253499
841842,1683685,1683684,3367369,3771.4179232120514,0.21408597529443796
842843,1685687,1685686,3371373,3781.7828600406647,0.2138203748872911
843844,1687689,1687688,3375377,3791.0950503349304,0.21355539283649705
844845,1689691,1689690,3379381,3800.0930433273315,0.21329102698655333
845846,1691693,1691692,3383385,3808.9316811561584,0.2130272769718431
846847,1693695,1693694,3387389,3817.876328229904,0.21276418453999213
847848,1695697,1695696,3391393,3826.821038007736,0.21250172047621163
848849,1697699,1697698,3395397,3835.865839242935,0.21223986901895842
849850,1699701,1699700,3399401,3847.2713062763214,0.21197862445842475
850851,1701703,1701702,3403405,3856.249873161316,0.21171798366958683
851852,1703705,1703704,3407409,3868.3184020519257,0.2114579442604736
852853,1705707,1705706,3411413,3879.034994125366,0.2111985040592117
853854,1707709,1707708,3415417,3888.714592218399,0.21093966098123929
854855,1709711,1709710,3419421,3897.3154151439667,0.21068141295472742
855856,1711713,1711712,3423425,3907.1747171878815,0.21042375792967505
856857,1713715,1713714,3427429,3916.089472055435,0.21016669386517606
857858,1715717,1715716,3431433,3925.0854601860046,0.20991021873305726
858859,1717719,1717718,3435437,3934.195997238159,0.2096543305178784
859860,1719721,1719720,3439441,3943.012731075287,0.20939902720056125
860861,1721723,1721722,3443445,3951.8431169986725,0.20914430678567442
861862,1723725,1723724,3447449,3960.7453951835632,0.20889016727960552
862863,1725727,1725726,3451453,3970.5131661891937,0.2086366066996561
863864,1727729,1727728,3455457,3982.2728292942047,0.2083836230685847
864865,1729731,1729730,3459461,3993.298065185547,0.20813121442552074
865866,1731733,1731732,3463465,4007.0637571811676,0.2078793788114126
866867,1733735,1733734,3467469,4018.218947172165,0.20762811427994166
867868,1735737,1735736,3471473,4030.386236190796,0.2073774188902462
868869,1737739,1737738,3475477,4040.7734031677246,0.20712729071783542
869870,1739741,1739740,3479481,4050.4507870674133,0.20687772783458058
870871,1741743,1741742,3483485,4060.231951236725,0.20662872833418078
871872,1743745,1743744,3487489,4069.759891271591,0.20638029030669713
872873,1745747,1745746,3491493,4078.793795108795,0.20613241186219966
873874,1747749,1747748,3495497,4087.775068283081,0.20588509111257736
874875,1749751,1749750,3499501,4096.989281177521,0.20563832617881417
875876,1751753,1751752,3503505,4107.576776266098,0.205392115190989
876877,1753755,1753754,3507509,4117.1283440589905,0.20514645628463768
877878,1755757,1755756,3511513,4126.010889291763,0.204901347613486
878879,1757759,1757758,3515517,4134.800635099411,0.20465678732580272
879880,1759761,1759760,3519521,4143.671045064926,0.20441277358986554
880881,1761763,1761762,3523525,4154.312458276749,0.2041693045739521
881882,1763765,1763764,3527529,4165.739144325256,0.203926378460892
882883,1765767,1765766,3531533,4174.545470237732,0.20368399343533383
883884,1767769,1767768,3535537,4184.747846126556,0.20344214769465907
884885,1769771,1769770,3539541,4193.78284907341,0.20320083944352518
885886,1771773,1771772,3543545,4202.544151067734,0.2029600668902276
886887,1773775,1773774,3547549,4211.24317407608,0.2027198282594327
887888,1775777,1775776,3551553,4221.23131108284,0.20248012177398778
888889,1777779,1777778,3555557,4230.983318090439,0.20224094567129214
889890,1779781,1779780,3559561,4240.972854137421,0.20200229819784
890891,1781783,1781782,3563565,4251.770377159119,0.20176417760012555
891892,1783785,1783784,3567569,4262.78558921814,0.20152658213737595
892893,1785787,1785786,3571573,4273.086463928223,0.2012895100779133
893894,1787789,1787788,3575577,4283.075603246689,0.20105295969369763
894895,1789791,1789790,3579581,4293.474320173264,0.20081692926942196
895896,1791793,1791792,3583585,4304.189484119415,0.20058141709159827
896897,1793795,1793794,3587589,4315.0615911483765,0.20034642145583348
897898,1795797,1795796,3591593,4325.998502254486,0.20011194066682947
898899,1797799,1797798,3595597,4336.343725204468,0.19987797303838306
899900,1799801,1799800,3599601,4347.153606176376,0.19964451688611007
900901,1801803,1801802,3603605,4356.663206100464,0.19941157053835923
901902,1803805,1803804,3607609,4367.09770321846,0.19917913233075524
902903,1805807,1805806,3611613,4376.971967935562,0.19894720060074178
903904,1807809,1807808,3615617,4387.987623214722,0.1987157736930385
904905,1809811,1809810,3619621,4398.496542215347,0.19848484997237392
905906,1811813,1811812,3623625,4408.608777284622,0.19825442779256264
906907,1813815,1813814,3627629,4419.4725041389465,0.19802450552379014
907908,1815817,1815816,3631633,4429.519345283508,0.19779508154715586
908909,1817819,1817818,3635637,4440.020916223526,0.19756615424194024
909910,1819821,1819820,3639641,4449.6171362400055,0.19733772200015665
910911,1821823,1821822,3643645,4459.046957015991,0.19710978321927541
911912,1823825,1823824,3647649,4467.704124212265,0.19688233630768082
912913,1825827,1825826,3651653,4476.222738265991,0.19665537966648117
913914,1827829,1827828,3655657,4484.727791070938,0.19642891172406962
914915,1829831,1829830,3659661,4493.278173208237,0.1962029308961064
915916,1831833,1831832,3663665,4501.421577215195,0.19597743562189862
916917,1833835,1833834,3667669,4510.451247215271,0.19575242433529638
917918,1835837,1835836,3671673,4520.291295289993,0.19552789548470173
918919,1837839,1837838,3675677,4528.923567056656,0.1953038475185167
919920,1839841,1839840,3679681,4537.500285148621,0.19508027889787627
920921,1841843,1841842,3683685,4546.021283149719,0.1948571880839154
921922,1843845,1843844,3687689,4554.5576202869415,0.19463457355050195
922923,1845847,1845846,3691693,4563.071155309677,0.19441243377696082
923924,1847849,1847848,3695697,4571.571081161499,0.19419076724625484
924925,1849851,1849850,3699701,4580.107153177261,0.1939695724468038
925926,1851853,1851852,3703705,4588.690680027008,0.19374884788157942
926927,1853855,1853854,3707709,4597.1876101493835,0.19352859204627748
927928,1855857,1855856,3711713,4605.695560216904,0.1933088034620596
928929,1857859,1857858,3715717,4614.6655061244965,0.19308948063735443
929930,1859861,1859860,3719721,4624.978462219238,0.19287062209150463
930931,1861863,1861862,3723725,4635.393958091736,0.1926522263620427
931932,1863865,1863864,3727729,4646.32662820816,0.19243429198104423
932933,1865867,1865866,3731733,4656.876565217972,0.19221681748786068
933934,1867869,1867868,3735737,4666.822055101395,0.19199980142911954
934935,1869871,1869870,3739741,4676.5471522808075,0.19178324236236222
935936,1871873,1871872,3743745,4685.7976541519165,0.1915671388433111
936937,1873875,1873874,3747749,4694.472738027573,0.19135148944042157
937938,1875877,1875876,3751753,4703.2395231723785,0.19113629272578692
938939,1877879,1877878,3755757,4712.114273071289,0.19092154727331945
939940,1879881,1879880,3759761,4721.51641535759,0.1907072516678454
940941,1881883,1881882,3763765,4731.005597114563,0.190493404503286
941942,1883885,1883884,3767769,4739.924067020416,0.19028001099650282
942943,1885887,1885886,3771773,4749.016988277435,0.19006707363769237
943944,1887889,1887888,3775777,4758.048006296158,0.18985458207498596
944945,1889891,1889890,3779781,4767.1040761470795,0.18964253366539197
945946,1891893,1891892,3783785,4775.739253282547,0.18943092683912255
946947,1893895,1893894,3787789,4784.359100103378,0.18921976019191789
947948,1895897,1895896,3791793,4792.984539270401,0.18900903235225996
948949,1897899,1897898,3795797,4801.630628108978,0.18879874195044977
949950,1899901,1899900,3799801,4810.209264278412,0.18858888763134019
950951,1901903,1901902,3803805,4818.197125196457,0.18837946803432715
951952,1903905,1903904,3807809,4827.01046705246,0.18817048182063445
952953,1905907,1905906,3811813,4836.147899150848,0.18796192764239095
953954,1907909,1907908,3815817,4847.292273283005,0.18775380416445842
954955,1909911,1909910,3819821,4860.074617147446,0.1875461100553366
955956,1911913,1911912,3823825,4870.719047307968,0.18733884399443923
956957,1913915,1913914,3827829,4880.5382261276245,0.18713200465754198
957958,1915917,1915916,3831833,4890.9580950737,0.18692559072951553
958959,1917919,1917918,3835837,4902.074375152588,0.1867196009043255
959960,1919921,1919920,3839841,4912.292825222015,0.18651403387593746
960961,1921923,1921922,3843845,4921.8882212638855,0.186308888347412
961962,1923925,1923924,3847849,4932.224029302597,0.18610416302362864
962963,1925927,1925926,3851853,4942.5497941970825,0.1858998566185619
963964,1927929,1927928,3855857,4952.748279094696,0.18569596785164322
964965,1929931,1929930,3859861,4961.617380142212,0.18549249544230406
965966,1931933,1931932,3863865,4971.307018995285,0.18528943811907084
966967,1933935,1933934,3867869,4980.264045000076,0.1850867946195649
967968,1935937,1935936,3871873,4990.033259153366,0.18488456367413164
968969,1937939,1937938,3875877,4999.563332080841,0.18468274403312535
969970,1939941,1939940,3879881,5008.93634724617,0.18448133444144332
970971,1941943,1941942,3883885,5017.949813365936,0.18428033365489682
971972,1943945,1943944,3887889,5027.139635324478,0.18407974043111608
972973,1945947,1945946,3891893,5036.580265283585,0.1838795535350073
973974,1947949,1947948,3895897,5047.704317331314,0.18367977173147665
974975,1949951,1949950,3899901,5058.097496032715,0.18348039379816328
975976,1951953,1951952,3903905,5067.44180226326,0.18328141851452528
976977,1953955,1953954,3907909,5076.29954123497,0.18308284466365876
977978,1955957,1955956,3911913,5085.118828058243,0.18288467103047878
978979,1957959,1957958,3915917,5094.376396179199,0.18268689640899538
979980,1959961,1959960,3919921,5104.26030421257,0.1824895196041325
980981,1961963,1961962,3923925,5114.71527504921,0.1822925394099002
981982,1963965,1963964,3927929,5124.97597527504,0.18209595464031736
982983,1965967,1965966,3931933,5135.3084881305695,0.18189976410576492
983984,1967969,1967968,3935937,5144.642578125,0.18170396662389976
984985,1969971,1969970,3939941,5153.781028032303,0.18150856101601676
985986,1971973,1971972,3943945,5162.335116147995,0.18131354611068673
986987,1973975,1973974,3947949,5170.809029102325,0.18111892074011848
987988,1975977,1975976,3951953,5180.338858366013,0.1809246837401588
988989,1977979,1977978,3955957,5189.785209178925,0.18073083394665446
989990,1979981,1979980,3959961,5199.039835214615,0.18053737021182314
990991,1981983,1981982,3963965,5208.225892066956,0.18034429138424457
991992,1983985,1983984,3967969,5217.232542276382,0.18015159631431743
992993,1985987,1985986,3971973,5227.1373081207275,0.17995928386699234
993994,1987989,1987988,3975977,5235.683979988098,0.17976735290358192
994995,1989991,1989990,3979981,5244.524653196335,0.17957580229267478
995996,1991993,1991992,3983985,5253.694795131683,0.1793846309028595
996997,1993995,1993994,3987989,5262.784217119217,0.17919383761727659
997998,1995997,1995996,3991993,5271.923894166946,0.17900342131360958
998999,1997999,1997998,3995997,5281.427743196487,0.17881338088227494
1000000,2000001,2000000,4000001,5290.428626298904,0.17862371521187015


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.003580331802368164,12064.44795143716
1001,2003,1001,3004,3.297255277633667,1.0208544809865998
2002,4005,2002,6007,6.5950400829315186,0.1963330649305135
3003,6007,3003,9010,10.403073072433472,0.07454063132900046
4004,8009,4004,12013,14.045221328735352,0.036095311308599776
5005,10011,5005,15016,17.96530818939209,0.0203003074911976
6006,12013,6006,18019,21.80432415008545,0.01303998796720407
7007,14015,7007,21022,25.312960147857666,0.008390385557504487
8008,16017,8008,24025,28.575016975402832,0.005935084329394158
9009,18019,9009,27028,32.209025144577026,0.004151742561589344
10010,20021,10010,30031,35.89528703689575,0.002722964271015371
11011,22023,11011,33034,39.16694140434265,0.001570305317727616
12012,24025,12012,36037,44.19223618507385,0.0011662387132673757
13013,26027,13013,39040,48.38088822364807,0.0009639094387239311
14014,28029,14014,42043,52.51697635650635,0.0008122627114062198
15015,30031,15015,45046,56.256795167922974,0.0008630201446067076
16016,32033,16016,48049,60.85531711578369,0.0008201777545764344
17017,34035,17017,51052,64.16259717941284,0.0007163337904785294
18018,36037,18018,54055,68.25585412979126,0.0006060321884433506
19019,38039,19019,57058,71.88515424728394,0.0005556192627409473
20020,40041,20020,60061,75.46630024909973,0.0003564142516552238
21021,42043,21021,63064,78.91943407058716,0.00029010928483330645
22022,44045,22022,66067,82.78361916542053,0.0003425906706979731
23023,46047,23023,69070,86.4918761253357,0.00017186377226607874
24024,48049,24024,72073,89.95764923095703,0.000212398945222958
25025,50051,25025,75076,93.41383123397827,0.00018215225281892344
26026,52053,26026,78079,97.03635931015015,0.00017645176194491796
27027,54055,27027,81082,100.83073735237122,0.00017036563622241374
28028,56057,28028,84085,105.0214033126831,0.00010074830788653344
29029,58059,29029,87088,108.204763174057,0.0001371430462313583
30030,60061,30030,90091,111.40122604370117,0.00014272142107074615
31031,62063,31031,93094,114.60598921775818,0.00011921375335077755
32032,64065,32032,96097,117.8048882484436,0.00012144873471697792
33033,66067,33033,99100,120.94433617591858,0.00015765292846481316
34034,68069,34034,102103,124.10033321380615,9.251608207705431e-05
35035,70071,35035,105106,127.30742025375366,9.336265065940097e-05
36036,72073,36036,108109,130.45642113685608,6.60748773952946e-05
37037,74075,37037,111112,133.7576870918274,7.306640145543497e-05
38038,76077,38038,114115,136.9587631225586,7.999372792255599e-05
39039,78079,39039,117118,140.1417043209076,3.6568211726262234e-05
40040,80081,40040,120121,143.3206582069397,6.276683052419685e-05
41041,82083,41041,123124,146.49146914482117,5.126327778270934e-05
42042,84085,42042,126127,149.62916111946106,4.9657883209874853e-05
43043,86087,43043,129130,152.79939723014832,5.61745237064315e-05
44044,88089,44044,132133,155.93991231918335,4.753062785312068e-05
45045,90091,45045,135136,159.14311623573303,5.61164542887127e-05
46046,92093,46046,138139,162.32872414588928,4.3460244341986254e-05
47047,94095,47047,141142,165.60465717315674,4.160032403888181e-05
48048,96097,48048,144145,168.97816014289856,4.0584447560831904e-05
49049,98099,49049,147148,172.19834923744202,3.739330713870004e-05
50050,100101,50050,150151,175.40866613388062,2.1718948119087145e-05
51051,102103,51051,153154,178.58151721954346,2.4137611035257578e-05
52052,104105,52052,156157,181.86277723312378,2.3374417651211843e-05
53053,106107,53053,159160,185.03511714935303,2.8929569452884607e-05
54054,108109,54054,162163,188.17504739761353,2.57865776802646e-05
55055,110111,55055,165166,191.3879861831665,2.516750646464061e-05
56056,112113,56056,168169,194.57408022880554,1.990168857446406e-05
57057,114115,57057,171172,197.73601007461548,1.9727178369066678e-05
58058,116117,58058,174175,200.9184992313385,1.7300282706855796e-05
59059,118119,59059,177178,204.0706250667572,1.5901217921054922e-05
60060,120121,60060,180181,207.30166220664978,1.4990311683504842e-05
61061,122123,61061,183184,210.49787020683289,1.7393573216395453e-05
62062,124125,62062,186187,213.66258215904236,1.2470214642235078e-05
63063,126127,63063,189190,216.85601615905762,1.3740555004915223e-05
64064,128129,64064,192193,220.01064229011536,1.1518548490130343e-05
65065,130131,65065,195196,223.1496262550354,1.0775558621389791e-05
66066,132133,66066,198199,226.34386920928955,1.0985613698721863e-05
67067,134135,67067,201202,229.5062391757965,6.312797268037684e-06
68068,136137,68068,204205,232.69480228424072,8.129776688292623e-06
69069,138139,69069,207208,235.8570532798767,8.23834488983266e-06
70070,140141,70070,210211,239.08361506462097,7.72059865994379e-06
71071,142143,71071,213214,242.2823622226715,6.724583727191202e-06
72072,144145,72072,216217,245.42807817459106,6.124108040239662e-06
73073,146147,73073,219220,248.5796720981598,4.367906512925401e-06
74074,148149,74074,222223,251.74220418930054,3.304276106064208e-06
75075,150151,75075,225226,254.87605142593384,3.2687148632248864e-06
76076,152153,76076,228229,258.0489022731781,2.1690939320251346e-06
77077,154155,77077,231232,261.1933083534241,1.6267495084321126e-06
78078,156157,78078,234235,264.29287815093994,2.0032184693263844e-06
79079,158159,79079,237238,267.44551706314087,2.462809788994491e-06
80080,160161,80080,240241,270.559451341629,2.8357189876260236e-06
81081,162163,81081,243244,273.76848125457764,3.2661500881658867e-06
82082,164165,82082,246247,276.85422801971436,3.326456862851046e-06
83083,166167,83083,249250,279.99240016937256,3.2561856642132625e-06
84084,168169,84084,252253,283.1654920578003,3.1800173019291833e-06
85085,170171,85085,255256,286.2973051071167,2.623892214614898e-06
86086,172173,86086,258259,289.4583013057709,2.0789993868675083e-06
87087,174175,87087,261262,292.642804145813,1.5854766388656572e-06
88088,176177,88088,264265,295.8160722255707,9.143132047029212e-07
89089,178179,89089,267268,299.010498046875,8.343868103111163e-07
90090,180181,90090,270271,302.1786892414093,8.144979801727459e-07
91091,182183,91091,273274,306.8746192455292,8.688512025400996e-07
92092,184185,92092,276277,310.2984571456909,1.3256794773042202e-06
93093,186187,93093,279280,313.5646622180939,1.5226760297082365e-06
94094,188189,94094,282283,316.79523730278015,1.8473419913789257e-06
95095,190191,95095,285286,320.26638627052307,2.193231921410188e-06
96096,192193,96096,288289,323.7895612716675,2.11359110835474e-06
97097,194195,97097,291292,327.32075214385986,1.9830913515761495e-06
98098,196197,98098,294295,330.8375811576843,1.7146630852948874e-06
99099,198199,99099,297298,335.1216871738434,1.246815372724086e-06
100100,200201,100100,300301,338.8825333118439,9.155774023383856e-07
101101,202203,101101,303304,342.3950500488281,6.462068995460868e-07
102102,204205,102102,306307,345.76324915885925,3.758286766242236e-07
103103,206207,103103,309310,349.089768409729,3.674704203149304e-07
104104,208209,104104,312313,352.5329473018646,4.931334842694923e-07
105105,210211,105105,315316,355.8682162761688,6.672198651358485e-07
106106,212213,106106,318319,359.23396730422974,9.961604519048706e-07
107107,214215,107107,321322,363.0134162902832,1.22525125334505e-06
108108,216217,108108,324325,366.3960962295532,1.3425215001916513e-06
109109,218219,109109,327328,370.4585871696472,1.433800207450986e-06
110110,220221,110110,330331,374.30129623413086,1.32111381390132e-06
111111,222223,111111,333334,377.81336522102356,1.1299871403025463e-06
112112,224225,112112,336337,380.9395761489868,9.039413271239027e-07
113113,226227,113113,339340,384.14056396484375,5.773890734417364e-07
114114,228229,114114,342343,387.321622133255,3.665591066237539e-07
115115,230231,115115,345346,390.44110012054443,2.54722181125544e-07
116116,232233,116116,348349,393.5697112083435,1.8745959096122533e-07
117117,234235,117117,351352,396.7194871902466,3.028253559023142e-07
118118,236237,118118,354355,399.91465520858765,4.525572876445949e-07
119119,238239,119119,357358,403.0905044078827,6.094778655096889e-07
120120,240241,120120,360361,406.212354183197,8.387705747736618e-07
121121,242243,121121,363364,409.3611693382263,9.45403371588327e-07
122122,244245,122122,366367,412.5560541152954,9.721879905555397e-07
123123,246247,123123,369370,415.87339425086975,9.503000910626724e-07
124124,248249,124124,372373,419.0607831478119,7.860271580284461e-07
125125,250251,125125,375376,422.20889234542847,6.07578840572387e-07
126126,252253,126126,378379,425.35492730140686,4.390694812173024e-07
127127,254255,127127,381382,428.4773733615875,2.5410918169654906e-07
128128,256257,128128,384385,431.6292722225189,1.5341538528446108e-07
129129,258259,129129,387388,434.7275803089142,1.406751835020259e-07
130130,260261,130130,390391,438.0094599723816,1.7588536138646305e-07
131131,262263,131131,393394,441.2619512081146,2.9684633773285896e-07
132132,264265,132132,396397,444.4083571434021,4.5144042815081775e-07
133133,266267,133133,399400,447.53328824043274,5.589354259427637e-07
134134,268269,134134,402403,450.66063022613525,6.648970156675205e-07
135135,270271,135135,405406,453.8954863548279,7.018825272098184e-07
136136,272273,136136,408409,457.01966619491577,6.507216312456876e-07
137137,274275,137137,411412,460.14765906333923,5.851870810147375e-07
138138,276277,138138,414415,463.3576192855835,4.4223452277947217e-07
139139,278279,139139,417418,466.5001952648163,2.9618058761116117e-07
140140,280281,140140,420421,469.66695618629456,1.982516550924629e-07
141141,282283,141141,423424,472.90657210350037,1.0734220268204808e-07
142142,284285,142142,426427,477.9913651943207,1.0315125109627843e-07
143143,286287,143143,429430,482.01249837875366,1.4760189515072852e-07
144144,288289,144144,432433,485.731121301651,2.109773049596697e-07
145145,290291,145145,435436,489.2296311855316,3.2230855140369385e-07
146146,292293,146146,438439,492.86696910858154,4.164212441537529e-07
147147,294295,147147,441442,496.3175003528595,4.791345418198034e-07
148148,296297,148148,444445,499.48525738716125,5.109413905302063e-07
149149,298299,149149,447448,503.25299525260925,4.840130714001134e-07
150150,300301,150150,450451,507.1379282474518,4.1035673348233104e-07
151151,302303,151151,453454,511.13674330711365,3.258573997300118e-07
152152,304305,152152,456457,515.7137973308563,2.2945096134208143e-07
153153,306307,153153,459460,519.9109551906586,1.3869248505216092e-07
154154,308309,154154,462463,524.0524742603302,9.924042387865484e-08
155155,310311,155155,465466,527.869707107544,8.159440767485648e-08
156156,312313,156156,468469,532.6489143371582,1.0572694009169936e-07
157157,314315,157157,471472,536.6530072689056,1.7883576219901443e-07
158158,316317,158158,474475,540.5184662342072,2.393790055066347e-07
159159,318319,159159,477478,544.3114802837372,3.11465555569157e-07
160160,320321,160160,480481,548.1780722141266,3.6365418054629117e-07
161161,322323,161161,483484,552.2479212284088,3.666864358820021e-07
162162,324325,162162,486487,556.0151982307434,3.572367859305814e-07
163163,326327,163163,489490,559.9871129989624,3.061777533730492e-07
164164,328329,164164,492493,563.5196161270142,2.345077518839389e-07
165165,330331,165165,495496,567.2732653617859,1.7125967133324593e-07
166166,332333,166166,498499,571.1982622146606,1.0875010048039258e-07
167167,334335,167167,501502,575.0881590843201,7.592461770400405e-08
168168,336337,168168,504505,578.6301991939545,7.547896530013531e-08
169169,338339,169169,507508,582.1504702568054,9.775067155715078e-08
170170,340341,170170,510511,585.7338240146637,1.4158104022499174e-07
171171,342343,171171,513514,589.3606162071228,1.9676554074976593e-07
172172,344345,172172,516517,593.0365533828735,2.427295839879662e-07
173173,346347,173173,519520,596.691504240036,2.725155354710296e-07
174174,348349,174174,522523,600.5350782871246,2.849719749065116e-07
175175,350351,175175,525526,604.7113630771637,2.6173620426561683e-07
176176,352353,176176,528529,609.6812691688538,2.244760253233835e-07
177177,354355,177177,531532,613.5665583610535,1.78561094799079e-07
178178,356357,178178,534535,617.5913071632385,1.2122109183110297e-07
179179,358359,179179,537538,621.1076142787933,8.796450856607407e-08
180180,360361,180180,540541,624.6756701469421,6.60929799778387e-08
181181,362363,181181,543544,628.3491752147675,6.247501005418599e-08
182182,364365,182182,546547,631.9639141559601,9.06111381482333e-08
183183,366367,183183,549550,635.5171382427216,1.2089003575965762e-07
184184,368369,184184,552553,639.7546441555023,1.6050580597948283e-07
185185,370371,185185,555556,643.2861351966858,1.9730214262381196e-07
186186,372373,186186,558559,646.813449382782,2.1265259420033544e-07
187187,374375,187187,561562,650.8220753669739,2.1603773348033428e-07
188188,376377,188188,564565,655.1491982936859,1.9921390048693866e-07
189189,378379,189189,567568,659.2043421268463,1.6637204680591822e-07
190190,380381,190190,570571,662.9885582923889,1.2870077625848353e-07
191191,382383,191191,573574,666.5117242336273,9.279392543248832e-08
192192,384385,192192,576577,670.1399192810059,6.525806384161115e-08
193193,386387,193193,579580,673.8844721317291,5.4047632147558033e-08
194194,388389,194194,582583,677.4621760845184,6.157824827823788e-08
195195,390391,195195,585586,681.0028622150421,7.847484084777534e-08
196196,392393,196196,588589,684.7254571914673,1.0863732313737273e-07
197197,394395,197197,591592,688.2639622688293,1.3879616744816303e-07
198198,396397,198198,594595,692.0071370601654,1.588941813679412e-07
199199,398399,199199,597598,695.6107652187347,1.743010216159746e-07
200200,400401,200200,600601,699.1460702419281,1.6844023775774986e-07
201201,402403,201201,603604,702.8883442878723,1.5061050362419337e-07
202202,404405,202202,606607,707.4539241790771,1.2697091733571142e-07
203203,406407,203203,609610,712.1870472431183,9.291761671192944e-08
204204,408409,204204,612613,717.1675882339478,6.851223588455468e-08
205205,410411,205205,615616,722.4786350727081,5.135007086209953e-08
206206,412413,206206,618619,726.368860244751,4.424691724125296e-08
207207,414415,207207,621622,729.8849720954895,5.4898919188417494e-08
208208,416417,208208,624625,733.5643000602722,7.226663001347333e-08
209209,418419,209209,627628,737.3000960350037,9.596988093107939e-08
210210,420421,210210,630631,741.2170603275299,1.1974225344602019e-07
211211,422423,211211,633634,744.9905710220337,1.3559838407672942e-07
212212,424425,212212,636637,748.9725542068481,1.407825038768351e-07
213213,426427,213213,639640,753.2986931800842,1.3443059287965298e-07
214214,428429,214214,642643,757.046795129776,1.1800511856563389e-07
215215,430431,215215,645646,760.5621271133423,9.310133464168757e-08
216216,432433,216216,648649,764.4663150310516,7.01074895914644e-08
217217,434435,217217,651652,768.9625542163849,4.9569280236028135e-08
218218,436437,218218,654655,773.3335492610931,3.713466867338866e-08
219219,438439,219219,657658,776.8104393482208,3.936474968213588e-08
220220,440441,220220,660661,780.4282743930817,4.7475623432546854e-08
221221,442443,221221,663664,784.8535051345825,6.603477231692523e-08
222222,444445,222222,666667,789.1819462776184,8.768984116613865e-08
223223,446447,223223,669670,792.7778642177582,1.0352050594519824e-07
224224,448449,224224,672673,796.3341481685638,1.1696829460561275e-07
225225,450451,225225,675676,800.0525844097137,1.1766314855776727e-07
226226,452453,226226,678679,803.5481052398682,1.0859912435989827e-07
227227,454455,227227,681682,807.0784330368042,9.343602869194001e-08
228228,456457,228228,684685,811.7108631134033,7.106973498594016e-08
229229,458459,229229,687688,815.8964853286743,5.135007086209953e-08
230230,460461,230230,690691,819.5051522254944,3.608874976634979e-08
231231,462463,231231,693694,822.8244171142578,2.8774593374691904e-08
232232,464465,232232,696697,826.1715121269226,3.16504156216979e-08
233233,466467,233233,699700,829.5032742023468,4.2755345930345356e-08
234234,468469,234234,702703,832.8586812019348,5.973015504423529e-08
235235,470471,235235,705706,836.1645362377167,7.714697858318686e-08
236236,472473,236236,708709,839.4943952560425,9.287577995564789e-08
237237,474475,237237,711712,842.814935207367,1.0018811735790223e-07
238238,476477,238238,714715,846.1391360759735,9.908217180054635e-08
239239,478479,239239,717718,849.4112660884857,9.066206985153258e-08
240240,480481,240240,720721,852.6966421604156,7.308335625566542e-08
241241,482483,241241,723724,856.0682492256165,5.544461600948125e-08
242242,484485,242242,726727,859.3855392932892,3.8155121728777885e-08
243243,486487,243243,729730,862.6605021953583,2.515480446163565e-08
244244,488489,244244,732733,866.2431411743164,2.2688254830427468e-08
245245,490491,245245,735736,870.4019992351532,2.5956978788599372e-08
246246,492493,246246,738739,874.4645733833313,3.786772140301764e-08
247247,494495,247247,741742,878.178572177887,5.419860826805234e-08
248248,496497,248248,744745,881.7521800994873,6.90961314830929e-08
249249,498499,249249,747748,885.7161211967468,8.217102731578052e-08
250250,500501,250250,750751,889.654158115387,8.733513823244721e-08
251251,502503,251251,753754,892.9297332763672,8.488495950587094e-08
252252,504505,252252,756757,896.2202570438385,7.519702194258571e-08
253253,506507,253253,759760,899.5308690071106,5.988840712234378e-08
254254,508509,254254,762763,902.8108253479004,4.331013769842684e-08
255255,510511,255255,765766,906.0389711856842,2.8172507882118225e-08
256256,512513,256256,768769,909.3159942626953,1.9248545868322253e-08
257257,514515,257257,771772,912.8224601745605,1.663283910602331e-08
258258,516517,258258,774775,916.1385793685913,2.209890226367861e-08
259259,518519,259259,777778,919.7754471302032,3.3927790354937315e-08
260260,520521,260260,780781,923.6313152313232,4.7522917157039046e-08
261261,522523,261261,783784,928.0428280830383,6.253139872569591e-08
262262,524525,262262,786787,931.6499762535095,7.229209586512297e-08
263263,526527,263263,789790,935.1990432739258,7.593916961923242e-08
264264,528529,264264,792793,938.7020783424377,7.35071807866916e-08
265265,530531,265265,795796,942.2780282497406,6.269874575082213e-08
266266,532533,266266,798799,945.6212034225464,4.934736352879554e-08
267267,534535,267267,801802,949.2798571586609,3.432978701312095e-08
268268,536537,268268,804805,952.8654112815857,2.1165760699659586e-08
269269,538539,269269,807808,956.434953212738,1.4380930224433541e-08
270270,540541,270270,810811,959.6467282772064,1.3009412214159966e-08
271271,542543,271271,813814,962.870658159256,1.907937985379249e-08
272272,544545,272272,816817,966.2136001586914,3.000604920089245e-08
273273,546547,273273,819820,969.7196662425995,4.305184120312333e-08
274274,548549,274274,822823,973.2172532081604,5.5631971918046474e-08
275275,550551,275275,825826,976.7209930419922,6.385926099028438e-08
276276,552553,276276,828829,980.035961151123,6.689879228360951e-08
277277,554555,277277,831832,983.6406753063202,6.278605724219233e-08
278278,556557,278278,834835,987.0575802326202,5.361471266951412e-08
279279,558559,279279,837838,990.6119680404663,4.099638317711651e-08
280280,560561,280280,840841,994.2274522781372,2.7224814402870834e-08
281281,562563,281281,843844,997.7959711551666,1.707303454168141e-08
282282,564565,282282,846847,1001.2741451263428,1.057560439221561e-08
283283,566567,283283,849850,1004.8791811466217,1.0722942533902824e-08
284284,568569,284284,852853,1008.3681161403656,1.696207618806511e-08
285285,570571,285285,855856,1011.8631024360657,2.6408088160678744e-08
286286,572573,286286,858859,1015.3900873661041,3.892091626767069e-08
287287,574575,287287,861862,1018.6910762786865,4.937282938044518e-08
288288,576577,288288,864865,1022.239128112793,5.634501576423645e-08
289289,578579,289289,867868,1026.1240870952606,5.853144102729857e-08
290290,580581,290290,870871,1030.0159192085266,5.404945113696158e-08
291291,582583,291291,873874,1034.0195672512054,4.5656634029001e-08
292292,584585,292292,876877,1037.8162910938263,3.399509296286851e-08
293293,586587,293293,879880,1041.4148013591766,2.229717210866511e-08
294294,588589,294294,882883,1044.6740591526031,1.3335011317394674e-08
295295,590591,295295,885886,1048.1651301383972,8.414644980803132e-09
296296,592593,296296,888889,1052.0424420833588,9.40781319513917e-09
297297,594595,297297,891892,1055.4161961078644,1.4902980183251202e-08
298298,596597,298298,894895,1058.777096271515,2.4383552954532206e-08
299299,598599,299299,897898,1062.1974611282349,3.4933691495098174e-08
300300,600601,300300,900901,1065.562902212143,4.394860297907144e-08
301301,602603,301301,903904,1069.1020963191986,5.016045179218054e-08
302302,604605,302302,906907,1072.54741024971,5.0702510634437203e-08
303303,606607,303303,909910,1076.1711213588715,4.691173671744764e-08
304304,608609,304304,912913,1080.3752629756927,3.890818334184587e-08
305305,610611,305305,915916,1084.2200713157654,2.8272552299313247e-08
306306,612613,306306,918919,1087.8659942150116,1.866646925918758e-08
307307,614615,307307,921922,1091.3681662082672,1.0611984180286527e-08
308308,616617,308308,924925,1095.198043346405,7.137714419513941e-09
309309,618619,309309,927928,1099.008723974228,8.481947588734329e-09
310310,620621,310310,930931,1103.2485401630402,1.3640601537190378e-08
311311,622623,311311,933934,1107.651560306549,2.2417225409299135e-08
312312,624625,312312,936937,1111.584478378296,3.143577487207949e-08
313313,626627,313313,939940,1115.6237502098083,3.9384758565574884e-08
314314,628629,314314,942943,1120.2629492282867,4.411595000419766e-08
315315,630631,315315,945946,1124.4143471717834,4.426510713528842e-08
316316,632633,316316,948949,1127.7497782707214,4.0477971197105944e-08
317317,634635,317317,951952,1131.761773109436,3.282912075519562e-08
318318,636637,318318,954955,1135.3627922534943,2.391607267782092e-08
319319,638639,319319,957958,1138.7875893115997,1.51885615196079e-08
320320,640641,320320,960961,1142.6090512275696,8.769347914494574e-09
321321,642643,321321,963964,1146.1748201847076,6.422851583920419e-09
322322,644645,322322,966967,1150.0042932033539,7.674316293559968e-09
323323,646647,323323,969970,1153.4393231868744,1.3191311154514551e-08
324324,648649,324324,972973,1157.019893169403,2.0700099412351847e-08
325325,650651,325325,975976,1160.8284742832184,2.8598151402547956e-08
326326,652653,326326,978979,1165.0779721736908,3.5521225072443485e-08
327327,654655,327327,981982,1168.9638051986694,3.8773578125983477e-08
328328,656657,328328,984985,1173.3059933185577,3.876448317896575e-08
329329,658659,329329,987988,1177.7016232013702,3.4784534364007413e-08
330330,660661,330330,990991,1182.1085031032562,2.7837813831865788e-08
331331,662663,331331,993994,1186.5642082691193,2.013257471844554e-08
332332,664665,332332,996997,1190.6040351390839,1.2496457202360034e-08
333333,666667,333333,1000000,1194.776700258255,7.517883204855025e-09
334334,668669,334334,1003003,1199.148383140564,5.73345459997654e-09
335335,670671,335335,1006006,1203.5001153945923,7.499693310819566e-09
336336,672673,336336,1009009,1207.8804681301117,1.2643795344047248e-08
337337,674675,337337,1012012,1212.2740232944489,1.923217496369034e-08
338338,676677,338338,1015015,1216.6082119941711,2.6364432414993644e-08
339339,678679,339339,1018018,1221.0556952953339,3.173408913426101e-08
340340,680681,340340,1021021,1225.3189933300018,3.4387994674034417e-08
341341,682683,341341,1024024,1228.9710652828217,3.38241079589352e-08
342342,684685,342342,1027027,1233.194803237915,2.9682269087061286e-08
343343,686687,343343,1030030,1236.9912242889404,2.373599272686988e-08
344344,688689,344344,1033033,1240.3909041881561,1.659827830735594e-08
345345,690691,345345,1036036,1244.2511103153229,1.0355506674386561e-08
346346,692693,346346,1039039,1248.5125651359558,6.484697223640978e-09
347347,694695,347347,1042042,1252.6473290920258,5.211404641158879e-09
348348,696697,348348,1045045,1257.0008990764618,7.583366823382676e-09
349349,698699,349349,1048048,1261.2100772857666,1.2187229003757238e-08
350350,700701,350350,1051051,1265.289705991745,1.8217178876511753e-08
351351,702703,351351,1054054,1269.5393691062927,2.43635440710932e-08
352352,704705,352352,1057057,1273.9944331645966,2.858359948731959e-08
353353,706707,353353,1060060,1278.3605921268463,3.0622686608694494e-08
354354,708709,354354,1063063,1282.6865541934967,2.9409420676529408e-08
355355,710711,355355,1066066,1287.2398731708527,2.5542249204590917e-08
356356,712713,356356,1069069,1291.4561762809753,2.0019797375425696e-08
357357,714715,357357,1072072,1295.7476541996002,1.3737007975578308e-08
358358,716717,358358,1075075,1300.2396001815796,8.692950359545648e-09
359359,718719,359359,1078078,1304.2871811389923,5.4551492212340236e-09
360360,720721,360360,1081081,1308.1786141395569,5.0895323511213064e-09
361361,722723,361361,1084084,1311.5802462100983,7.503331289626658e-09
362362,724725,362362,1087087,1315.6508994102478,1.1799784260801971e-08
363363,726727,363363,1090090,1319.2439692020416,1.742409949656576e-08
364364,728729,364364,1093093,1323.2681481838226,2.238448360003531e-08
365365,730731,365365,1096096,1326.9301261901855,2.5986082619056106e-08
366366,732733,366366,1099099,1330.9406452178955,2.722663339227438e-08
367367,734735,367367,1102102,1335.7637422084808,2.5573172024451196e-08
368368,736737,368368,1105105,1339.6438663005829,2.2000676835887134e-08
369369,738739,369369,1108108,1343.886057138443,1.6696503735147417e-08
370370,740741,370370,1111111,1348.0380942821503,1.1381416697986424e-08
371371,742743,371371,1114114,1352.6129071712494,7.148628355935216e-09
372372,744745,372372,1117117,1356.1618392467499,4.676621756516397e-09
373373,746747,373373,1120120,1360.148954153061,4.998582880944014e-09
374374,748749,374374,1123123,1364.8761851787567,7.397829904220998e-09
375375,750751,375375,1126126,1368.9015443325043,1.165062712971121e-08
376376,752753,376376,1129129,1372.3676953315735,1.657645043451339e-08
377377,754755,377377,1132132,1375.9112582206726,2.0809238776564598e-08
378378,756757,378378,1135135,1379.4242544174194,2.3728716769255698e-08
379379,758759,379379,1138138,1383.0964653491974,2.417982614133507e-08
380380,760761,380380,1141141,1386.583280324936,2.247179509140551e-08
381381,762763,381381,1144144,1390.3724942207336,1.8810169422067702e-08
382382,764765,382382,1147147,1394.4236001968384,1.3991666492074728e-08
383383,766767,383383,1150150,1397.83779835701,9.455106919631362e-09
384384,768769,384384,1153153,1401.2077140808105,5.764377419836819e-09
385385,770771,385385,1156156,1404.7439172267914,4.200046532787383e-09
386386,772773,386386,1159159,1408.0531301498413,4.793037078343332e-09
387387,774775,387387,1162162,1411.4393632411957,7.325070328079164e-09
388388,776777,388388,1165165,1414.8145911693573,1.145781425293535e-08
389389,778779,389389,1168168,1418.1441671848297,1.5688783605583012e-08
390390,780781,390390,1171171,1421.5825374126434,1.9457729649730027e-08
391391,782783,391391,1174174,1424.8746492862701,2.1604137145914137e-08
392392,784785,392392,1177177,1428.191665172577,2.1593223209492862e-08
393393,786787,393393,1180180,1431.6645550727844,1.973239704966545e-08
394394,788789,394394,1183183,1435.1935131549835,1.602711563464254e-08
395395,790791,395395,1186186,1438.544798374176,1.1761585483327508e-08
396396,792793,396396,1189189,1442.9886972904205,7.683411240577698e-09
397397,794795,397397,1192192,1447.761105298996,4.718458512797952e-09
398398,796797,398398,1195195,1452.7962112426758,3.752575139515102e-09
399399,798799,399399,1198198,1456.9255402088165,4.5947672333568335e-09
400400,800801,400400,1201201,1461.188047170639,7.374183041974902e-09
401401,802803,401401,1204204,1465.408194065094,1.1123120202682912e-08
402402,804805,402402,1207207,1469.449018239975,1.499574864283204e-08
403403,806807,403403,1210210,1473.1918063163757,1.8208083929494023e-08
404404,808809,404404,1213213,1476.8824772834778,1.9677827367559075e-08
405405,810811,405405,1216216,1480.560042142868,1.944681571330875e-08
406406,812813,406406,1219219,1484.227233171463,1.7264028429053724e-08
407407,814815,407407,1222222,1488.1228852272034,1.376247382722795e-08
408408,816817,408408,1225225,1491.344093322754,9.884388418868184e-09
409409,818819,409409,1228228,1494.5997960567474,6.2045728554949164e-09
410410,820821,410410,1231231,1497.8381161689758,3.954482963308692e-09
411411,822823,411411,1234234,1501.1086132526398,3.308741725049913e-09
412412,824825,412412,1237237,1504.4736561775208,4.49108483735472e-09
413413,826827,413413,1240240,1507.8459112644196,7.303242455236614e-09
414414,828829,414414,1243243,1511.126587152481,1.0741132427938282e-08
415415,830831,415415,1246246,1514.414588212967,1.4335455489344895e-08
416416,832833,416416,1249249,1517.6720242500305,1.6929334378801286e-08
417417,834835,417417,1252252,1520.8678493499756,1.802982296794653e-08
418418,836837,418418,1255255,1524.171203136444,1.7462298274040222e-08
419419,838839,419419,1258258,1528.089774131775,1.5115801943466067e-08
420420,840841,420420,1261261,1531.9908633232117,1.1867086868733168e-08
421421,842843,421421,1264264,1535.3770833015442,8.185452315956354e-09
422422,844845,422422,1267267,1538.7243301868439,5.078618414700031e-09
423423,846847,423423,1270270,1541.970857143402,3.27054294757545e-09
424424,848849,424424,1273273,1545.6634449958801,2.9576767701655626e-09
425425,850851,425425,1276276,1548.969876050949,4.474713932722807e-09
426426,852853,426426,1279279,1552.2052292823792,7.132257451303303e-09
427427,854855,427427,1282282,1555.4774241447449,1.0459189070388675e-08
428428,856857,428428,1285285,1559.1084952354431,1.3642420526593924e-08
429429,858859,429429,1288288,1562.54035115242,1.5752448234707117e-08
430430,860861,430430,1291291,1565.8432312011719,1.6581907402724028e-08
431431,862863,431431,1294294,1569.476490020752,1.5637851902283728e-08
432432,864865,432432,1297297,1572.7444741725922,1.3338649296201766e-08
433433,866867,433433,1300300,1575.9444181919098,1.0208168532699347e-08
434434,868869,434434,1303303,1579.3908281326294,6.8121153162792325e-09
435435,870871,435435,1306306,1583.0966620445251,4.2018655221909285e-09
436436,872873,436436,1309309,1586.871336221695,2.68664734903723e-09
437437,874875,437437,1312312,1590.387410402298,2.775777829810977e-09
438438,876877,438438,1315315,1594.0656032562256,4.380126483738422e-09
439439,878879,439439,1318318,1597.6384000778198,6.96672941558063e-09
440440,880881,440440,1321321,1601.0260531902313,1.014086592476815e-08
441441,882883,441441,1324324,1604.6435792446136,1.2872988008894026e-08
442442,884885,442442,1327327,1608.138776063919,1.4713805285282433e-08
443443,886887,443443,1330330,1611.6681292057037,1.5159457689151168e-08
444444,888889,444444,1333333,1615.3485991954803,1.40262272907421e-08
445445,890891,445445,1336336,1620.0544531345367,1.1785232345573604e-08
446446,892893,446446,1339339,1624.2304420471191,8.712959242984653e-09
447447,894895,447447,1342342,1627.8702092170715,5.727997631765902e-09
448448,896897,448448,1345345,1631.470540046692,3.4251570468768477e-09
449449,898899,449449,1348348,1635.3794882297516,2.2610038286074996e-09
450450,900901,450450,1351351,1639.57488322258,2.6684574550017715e-09
451451,902903,451451,1354354,1643.5655171871185,4.270987119525671e-09
452452,904905,452452,1357357,1647.3497982025146,6.883055903017521e-09
453453,906907,453453,1360360,1650.9587502479553,9.760697139427066e-09
454454,908909,454454,1363363,1655.4612562656403,1.2174496077932417e-08
455455,910911,455455,1366366,1659.6716012954712,1.3727913028560579e-08
456456,912913,456456,1369369,1664.0435950756073,1.3818862498737872e-08
457457,914915,457457,1372372,1668.694999217987,1.263833837583661e-08
458458,916917,458458,1375375,1673.0838272571564,1.0362782632000744e-08
459459,918919,459459,1378378,1676.959604024887,7.490598363801837e-09
460460,920921,460460,1381381,1680.7406902313232,4.833054845221341e-09
461461,922923,461461,1384384,1685.8441591262817,2.7921487344428897e-09
462462,924925,462462,1387387,1690.822219133377,2.013621269725263e-09
463463,926927,463463,1390390,1695.8724312782288,2.5429471861571074e-09
464464,928929,464464,1393393,1700.5608041286469,4.220055416226387e-09
465465,930931,465465,1396396,1705.2654333114624,6.750269676558673e-09
466466,932933,466466,1399399,1709.8331441879272,9.325958671979606e-09
467467,934935,467467,1402402,1713.1751990318298,1.153239281848073e-08
468468,936937,468468,1405405,1717.0151071548462,1.2714735930785537e-08
469469,938939,469469,1408408,1721.026349067688,1.261651050299406e-08
470470,940941,470470,1411411,1725.3068282604218,1.1359588825143874e-08
471471,942943,471471,1414414,1729.1611211299896,9.067662176676095e-09
472472,944945,472472,1417417,1733.548433303833,6.468326319009066e-09
473473,946947,473473,1420420,1737.9936780929565,4.02542355004698e-09
474474,948949,474474,1423423,1742.3084502220154,2.3228494683280587e-09
475475,950951,475475,1426426,1746.3931493759155,1.82626536116004e-09
476476,952953,476476,1429429,1750.2061502933502,2.4629116524010897e-09
477477,954955,477477,1432432,1753.748300075531,4.238245310261846e-09
478478,956957,478478,1435435,1757.2830522060394,6.579284672625363e-09
479479,958959,479479,1438438,1761.1673271656036,8.96397978067398e-09
480480,960961,480480,1441441,1764.7549221515656,1.0888470569625497e-08
481481,962963,481481,1444444,1768.8421580791473,1.175612851511687e-08
482482,964965,482482,1447447,1772.261283159256,1.1537849786691368e-08
483483,966967,483483,1450450,1775.7402131557465,1.0149960871785879e-08
484484,968969,484484,1453453,1779.0564811229706,7.978087523952127e-09
485485,970971,485485,1456456,1782.360374212265,5.571564543060958e-09
486486,972973,486486,1459459,1785.9987852573395,3.356035449542105e-09
487487,974975,487487,1462462,1789.6570081710815,2.002707333303988e-09
488488,976977,488488,1465465,1793.5226323604584,1.6625563148409128e-09
489489,978979,489489,1468468,1797.7382462024689,2.4629116524010897e-09
490490,980981,490490,1471471,1801.29843211174,4.225512384437025e-09
491491,982983,491491,1474474,1805.0262310504913,6.397385732270777e-09
492492,984985,492492,1477477,1808.897881269455,8.614733815193176e-09
493493,986987,493493,1480480,1812.3549933433533,1.0209987522102892e-08
494494,988989,494494,1483483,1815.814614057541,1.0886651580221951e-08
495495,990991,495495,1486486,1819.3383402824402,1.0499206837266684e-08
496496,992993,496496,1489489,1822.7878391742706,9.045834303833544e-09
497497,994995,497497,1492492,1826.2569663524628,7.0158421294763684e-09
498498,996997,498498,1495495,1830.240157365799,4.742105375044048e-09
499499,998999,499499,1498498,1833.91251206398,2.8339854907244444e-09
500501,1001003,500501,1501504,1837.9024012088776,1.7207639757543802e-09
501502,1003005,501502,1504507,1841.8051960468292,1.5679688658565283e-09
502503,1005007,502503,1507510,1845.569467306137,2.5174813345074654e-09
503504,1007009,503504,1510513,1849.1389961242676,4.192770575173199e-09
504505,1009011,504505,1513516,1852.639876127243,6.275513442233205e-09
505506,1011013,505506,1516519,1856.169622182846,8.249116945080459e-09
506507,1013015,506507,1519522,1859.671166419983,9.582436177879572e-09
507508,1015017,507508,1522525,1863.7899851799011,1.0082658263854682e-08
508509,1017019,508509,1525528,1867.0675110816956,9.507857612334192e-09
509510,1019021,509510,1528531,1870.3279030323029,8.087226888164878e-09
510511,1021023,510511,1531534,1874.0298812389374,6.129994289949536e-09
511512,1023025,511512,1534537,1877.7560122013092,4.043613444082439e-09
512513,1025027,512513,1537540,1881.2735192775726,2.4137989385053515e-09
513514,1027029,513514,1540543,1884.794504404068,1.482476363889873e-09
514515,1029031,514515,1543546,1888.7608833312988,1.5497789718210697e-09
515516,1031033,515516,1546549,1892.068627357483,2.546585164964199e-09
516517,1033035,516517,1549552,1895.9819951057434,4.174580681137741e-09
517518,1035037,517518,1552555,1899.5497300624847,6.146365194581449e-09
518519,1037039,518519,1555558,1903.2177772521973,7.8580342233181e-09
519520,1039041,519520,1558561,1906.6960361003876,9.009454515762627e-09
520521,1041043,520521,1561564,1910.2201390266418,9.289578883908689e-09
521522,1043045,521522,1564567,1913.8591930866241,8.602000889368355e-09
522523,1045047,522523,1567570,1917.815264225006,7.206836016848683e-09
523524,1047049,523524,1570573,1921.0469992160797,5.313268047757447e-09
524525,1049051,524525,1573576,1924.7149341106415,3.459717845544219e-09
525526,1051053,525526,1576579,1928.5968520641327,2.02817318495363e-09
526527,1053055,526527,1579582,1931.8853392601013,1.318767317570746e-09
527528,1055057,527528,1582585,1935.3473641872406,1.5643308870494366e-09
528529,1057059,528529,1585588,1938.9294731616974,2.5756889954209328e-09
529530,1059061,529530,1588591,1942.8052201271057,4.200046532787383e-09
530531,1061063,530531,1591594,1946.5932371616364,5.9881131164729595e-09
531532,1063065,531532,1594597,1950.4266769886017,7.508788257837296e-09
532533,1065067,532533,1597600,1954.6548643112183,8.465576684102416e-09
533534,1067069,533534,1600603,1958.6647872924805,8.534698281437159e-09
534535,1069071,534535,1603606,1962.755511045456,7.803464541211724e-09
535536,1071073,535536,1606609,1967.303278207779,6.384652806445956e-09
536537,1073075,536537,1609612,1970.9511172771454,4.611138137988746e-09
537538,1075077,537538,1612615,1975.0986533164978,2.9576767701655626e-09
538539,1077079,538539,1615618,1979.152723312378,1.7025740817189217e-09
539540,1079081,539540,1618621,1983.1255731582642,1.2278178473934531e-09
540541,1081083,540541,1621624,1986.8060421943665,1.5661498764529824e-09
541542,1083085,541542,1624627,1990.4876492023468,2.6266206987202168e-09
542543,1085087,542543,1627630,1994.7731420993805,4.200046532787383e-09
543544,1087089,543544,1630633,1998.1107211112976,5.817128112539649e-09
544545,1089091,544545,1633636,2001.3938512802124,7.185008144006133e-09
545546,1091093,545546,1636639,2004.5964679718018,7.914422894828022e-09
546547,1093095,546547,1639642,2008.3726241588593,7.84893927630037e-09
547548,1095097,547548,1642645,2012.22403216362,7.05040292814374e-09
548549,1097099,548549,1645648,2016.2050611972809,5.626134225167334e-09
549550,1099101,549550,1648651,2019.7617211341858,4.00359567720443e-09
550551,1101103,550551,1651654,2023.2295081615448,2.4883775040507317e-09
551552,1103105,551552,1654657,2026.6996462345123,1.4497345546260476e-09
552553,1105107,552553,1657660,2030.1920402050018,1.1550582712516189e-09
553554,1107109,553554,1660663,2033.649587392807,1.5788828022778034e-09
554555,1109111,554555,1663666,2037.1850962638855,2.7030182536691427e-09
555556,1111113,555556,1666669,2041.1870641708374,4.174580681137741e-09
556557,1113115,556557,1669672,2044.8916773796082,5.6716089602559805e-09
557558,1115117,557558,1672675,2049.009145259857,6.859409040771425e-09
558559,1117119,558559,1675678,2052.5379803180695,7.390553946606815e-09
559560,1119121,559560,1678681,2056.1092932224274,7.228663889691234e-09
560561,1121123,560561,1681684,2059.6444861888885,6.3428160501644015e-09
561562,1123125,561562,1684687,2063.1020271778107,4.973117029294372e-09
562563,1125127,562563,1687690,2066.5742332935333,3.457898856140673e-09
563564,1127129,563564,1690693,2070.0343692302704,2.0863808458670974e-09
564565,1129131,564565,1693696,2074.033324241638,1.2605596566572785e-09
565566,1131133,565566,1696699,2077.3018333911896,1.0841176845133305e-09
566567,1133135,566567,1699702,2080.592852115631,1.622538547962904e-09
567568,1135137,567568,1702705,2084.3288362026215,2.7539499569684267e-09
568569,1137139,568569,1705708,2088.0034470558167,4.140019882470369e-09
569570,1139141,569570,1708711,2091.5371532440186,5.529727786779404e-09
570571,1141143,570571,1711714,2095.4029953479767,6.517439032904804e-09
571572,1143145,571572,1714717,2099.8325192928314,6.912159733474255e-09
572573,1145147,572573,1717720,2103.913843393326,6.630216375924647e-09
573574,1147149,573574,1720723,2107.841821193695,5.689798854291439e-09
574575,1149151,574575,1723726,2112.1729390621185,4.38558345194906e-09
575576,1151153,575576,1726729,2115.47185921669,2.950400812551379e-09
576577,1153155,576577,1729732,2119.0502462387085,1.762600732035935e-09
577578,1155157,577578,1732735,2122.780804157257,1.0913936421275139e-09
578579,1157159,578579,1735738,2126.2674412727356,1.0422809282317758e-09
579580,1159161,579580,1738741,2130.1511821746826,1.684384187683463e-09
580581,1161163,580581,1741744,2133.4775512218475,2.7812347980216146e-09
581582,1163165,581582,1744747,2136.810883283615,4.118192009627819e-09
582583,1165167,582583,1747750,2140.090053319931,5.366018740460277e-09
583584,1167169,583584,1750753,2143.390540122986,6.193658919073641e-09
584585,1169171,584585,1753756,2146.678922176361,6.4701453084126115e-09
585586,1171173,585586,1756759,2150.396532058716,6.06269168201834e-09
586587,1173175,586587,1759762,2154.40625,5.120455170981586e-09
587588,1175177,587588,1762765,2158.3732900619507,3.848981577903032e-09
588589,1177179,588589,1765768,2161.887267112732,2.5193003239110112e-09
589590,1179181,589590,1768771,2165.4509811401367,1.4970282791182399e-09
590591,1181183,590591,1771774,2168.9442150592804,9.440555004402995e-10
591592,1183185,591592,1774777,2172.416310071945,1.038642949424684e-09
592593,1185187,592593,1777780,2176.462948322296,1.722582965157926e-09
593594,1187189,593594,1780783,2179.8404512405396,2.8103386284783483e-09
594595,1189191,594595,1783786,2183.238263130188,4.083631210960448e-09
595596,1191193,595596,1786789,2186.5199213027954,5.180481821298599e-09
596597,1193195,596597,1789792,2189.782261133194,5.891706678085029e-09
597598,1195197,597598,1792795,2193.047008037567,6.0263118939474225e-09
598599,1197199,598599,1795798,2196.344351053238,5.542460712604225e-09
599600,1199201,599600,1798801,2199.6192440986633,4.596586222760379e-09
600601,1201203,600601,1801804,2202.9141511917114,3.3542164601385593e-09
601602,1203205,601602,1804807,2206.176778078079,2.1591404220089316e-09
602603,1205207,602603,1807810,2209.5101273059845,1.255102688446641e-09
603604,1207209,603604,1810813,2212.783844232559,8.440110832452774e-10
604605,1209211,604605,1813816,2216.1447591781616,1.0495568858459592e-09
605606,1211213,605606,1816819,2219.5993463993073,1.7571437638252974e-09
606607,1213215,606607,1819822,2224.034769296646,2.8485374059528112e-09
607608,1215217,607608,1822825,2228.3071942329407,4.0236045606434345e-09
608609,1217219,608609,1825828,2232.6150941848755,5.007677827961743e-09
609610,1219221,609610,1828831,2236.6122632026672,5.593392415903509e-09
610611,1221223,610611,1831834,2240.274564266205,5.5970303947106e-09
611612,1223225,611612,1834837,2243.7558352947235,5.071342457085848e-09
612613,1225227,612613,1837840,2247.7989661693573,4.105459083802998e-09
613614,1227229,613614,1840843,2251.4872193336487,2.928572939708829e-09
614615,1229231,614615,1843846,2255.315894126892,1.8408172763884068e-09
615616,1231233,615616,1846849,2259.0968194007874,1.0495568858459592e-09
616617,1233235,616617,1849852,2263.432407140732,7.821654435247183e-10
617618,1235237,617618,1852855,2267.262869119644,1.053194864653051e-09
618619,1237239,618619,1855858,2270.874014377594,1.8026184989139438e-09
619620,1239241,619620,1858861,2275.1698141098022,2.86672729998827e-09
620621,1241243,620621,1861864,2279.178287267685,3.9472070056945086e-09
621622,1243245,621622,1864867,2283.3358912467957,4.836692824028432e-09
622623,1245247,622623,1867870,2286.8618171215057,5.284164217300713e-09
623624,1247249,623624,1870873,2290.30233502388,5.2023096941411495e-09
624625,1249251,624625,1873876,2293.6476941108704,4.625690053217113e-09
625626,1251253,625626,1876879,2297.2872200012207,3.648892743512988e-09
626627,1253255,626627,1879882,2300.937591075897,2.5556801119819283e-09
627628,1255257,627628,1882885,2304.224819421768,1.5552359400317073e-09
628629,1257259,628629,1885888,2307.531107187271,8.949427865445614e-10
629630,1259261,629630,1888891,2310.791617155075,7.34871719032526e-10
630631,1261263,630631,1891894,2314.1805140972137,1.0677467798814178e-09
631632,1263265,631632,1894897,2317.4895050525665,1.8553691916167736e-09
632633,1265267,632633,1897900,2320.736481189728,2.86672729998827e-09
633634,1267269,633634,1900903,2324.0958280563354,3.87626641895622e-09
634635,1269271,634635,1903906,2327.4058492183685,4.654793883673847e-09
635636,1271273,635636,1906909,2330.5996313095093,4.984030965715647e-09
636637,1273275,636637,1909912,2333.8403000831604,4.833054845221341e-09
637638,1275277,637638,1912915,2337.061793088913,4.198227543383837e-09
638639,1277279,638639,1915918,2340.330974340439,3.2541720429435372e-09
639640,1279281,639640,1918921,2343.5193321704865,2.2209860617294908e-09
640641,1281283,640641,1921924,2346.711131334305,1.3114913599565625e-09
641642,1283285,641642,1924927,2349.868310213089,7.767084753140807e-10
642643,1285287,642643,1927930,2353.1361973285675,6.930349627509713e-10
643644,1287289,643644,1930933,2356.266009092331,1.102307578548789e-09
644645,1289291,644645,1933936,2359.5486583709717,1.8953869584947824e-09
645646,1291293,645646,1936939,2362.850431203842,2.8594513423740864e-09
646647,1293295,646647,1939942,2366.066677093506,3.799868864007294e-09
647648,1295297,647648,1942945,2369.2692873477936,4.456524038687348e-09
648649,1297299,648649,1945948,2372.5291261672974,4.698449629358947e-09
649650,1299301,649650,1948951,2375.802319288254,4.472894943319261e-09
650651,1301303,650651,1951954,2378.918338060379,3.803506842814386e-09
651652,1303305,651652,1954957,2382.072918176651,2.892193151637912e-09
652653,1305307,652653,1957960,2385.2435472011566,1.911757863126695e-09
653654,1307309,653654,1960963,2388.5028071403503,1.1132215149700642e-09
654655,1309311,654655,1963966,2391.659942150116,6.766640581190586e-10
655656,1311313,655656,1966969,2394.791353225708,6.784830475226045e-10
656657,1313315,656657,1969972,2397.978793144226,1.1477823136374354e-09
657658,1315317,657658,1972975,2401.1379630565643,1.924490788951516e-09
658659,1317319,658659,1975978,2404.2990663051605,2.8558133635669947e-09
659660,1319321,659660,1978981,2407.5262594223022,3.7052814150229096e-09
660661,1321323,660661,1981984,2412.460277080536,4.261892172507942e-09
661662,1323325,661662,1984987,2416.9079802036285,4.425601218827069e-09
662663,1325327,662663,1987990,2420.7513811588287,4.120010999031365e-09
663664,1327329,663664,1990993,2424.426408290863,3.448803909122944e-09
664665,1329331,664665,1993996,2427.997693300247,2.557499101385474e-09
665666,1331333,665666,1996999,2432.06596827507,1.648004399612546e-09
666667,1333335,666667,2000002,2435.9330933094025,9.51331458054483e-10
667668,1335337,667668,2003005,2440.02756524086,5.948095349594951e-10
668669,1337339,668669,2006008,2444.512073278427,6.857590051367879e-10
669670,1339341,669670,2009011,2448.5094830989838,1.1823431123048067e-09
670671,1341343,670671,2012014,2452.0840542316437,1.9554136088117957e-09
671672,1343345,671672,2015017,2455.267348051071,2.8430804377421737e-09
672673,1345347,672673,2018020,2458.559526205063,3.59978002961725e-09
673674,1347349,673674,2021023,2461.7706441879272,4.076355253346264e-09
674675,1349351,674675,2024026,2464.972827196121,4.145476850681007e-09
675676,1351353,675676,2027029,2468.173994064331,3.790773916989565e-09
676677,1353355,676677,2030032,2471.3498752117157,3.115928848274052e-09
677678,1355357,677678,2033035,2474.5874240398407,2.2464519133791327e-09
678679,1357359,678679,2036038,2477.8902671337128,1.418811734765768e-09
679680,1359361,679680,2039041,2481.1050040721893,8.039933163672686e-10
680681,1361363,680681,2042044,2484.3446152210236,5.402398528531194e-10
681682,1363365,681682,2045047,2487.520992040634,7.021299097687006e-10
682683,1365367,682683,2048050,2490.694133043289,1.2205418897792697e-09
683684,1367369,683684,2051053,2493.866065263748,1.991793396882713e-09
684685,1369371,684685,2054056,2497.221679210663,2.812157617881894e-09
685686,1371373,685686,2057059,2502.7470202445984,3.496097633615136e-09
686687,1373375,686687,2060062,2508.615662097931,3.887180355377495e-09
687688,1375377,687688,2063065,2513.567031145096,3.874447429552674e-09
688689,1377379,688689,2066068,2518.446862220764,3.4888216760009527e-09
689690,1379381,689690,2069071,2523.111448287964,2.799424692057073e-09
690691,1381383,690691,2072074,2527.5141501426697,1.9754224922508e-09
691692,1383385,691692,2075077,2532.5236213207245,1.2187229003757238e-09
692693,1385387,692693,2078080,2537.231582403183,6.821210263296962e-10
693694,1387389,693694,2081083,2541.927297115326,5.111360223963857e-10
694695,1389391,694695,2084086,2546.4231700897217,7.22138793207705e-10
695696,1391393,695696,2087089,2550.692679166794,1.2623786460608244e-09
696697,1393395,696697,2090092,2555.359990119934,2.015440259128809e-09
697698,1395397,697698,2093095,2559.4040372371674,2.773958840407431e-09
698699,1397399,698699,2096098,2563.2002432346344,3.3869582694023848e-09
699700,1399401,699700,2099101,2567.1812691688538,3.6907294997945428e-09
700701,1401403,700701,2102104,2571.1982831954956,3.6179699236527085e-09
701702,1403405,701702,2105107,2575.078835248947,3.19596438203007e-09
702703,1405407,702703,2108110,2579.232953310013,2.5047484086826444e-09
703704,1407409,703704,2111113,2582.875641107559,1.7316779121756554e-09
704705,1409411,704705,2114116,2586.6285331249237,1.0368239600211382e-09
705706,1411413,705706,2117119,2590.3936882019043,5.875335773453116e-10
706707,1413415,706707,2120122,2593.729389190674,4.893081495538354e-10
707708,1415417,707708,2123125,2597.382571220398,7.457856554538012e-10
708709,1417419,708709,2126128,2601.268566131592,1.3114913599565625e-09
709710,1419421,709710,2129131,2604.604564189911,2.02817318495363e-09
710711,1421423,710711,2132134,2608.1259472370148,2.7412170311436057e-09
711712,1423425,711712,2135137,2611.4229102134705,3.2778189051896334e-09
712713,1425427,712713,2138140,2615.128274202347,3.496097633615136e-09
713714,1427429,713714,2141143,2619.268974304199,3.3742253435775638e-09
714715,1429431,714715,2144146,2623.339537382126,2.915840013884008e-09
715716,1431433,715716,2147149,2626.762392282486,2.2391759557649493e-09
716717,1433435,716717,2150152,2630.4689421653748,1.5115801943466067e-09
717718,1435437,717718,2153155,2634.4279811382294,8.785718819126487e-10
718719,1437439,718719,2156158,2638.256607055664,5.147740012034774e-10
719720,1439441,719720,2159161,2642.331586122513,4.747562343254685e-10
720721,1441443,720721,2162164,2646.23282623291,7.803464541211724e-10
721722,1443445,721722,2165167,2650.396065235138,1.3515091268345714e-09
722723,1445447,722723,2168170,2654.251409292221,2.039087121374905e-09
723724,1447449,723724,2171173,2657.8031141757965,2.697561285458505e-09
724725,1449451,724725,2174176,2661.7179741859436,3.1523086363449693e-09
725726,1451453,725726,2177179,2665.337967157364,3.3105607144534588e-09
726727,1453455,726727,2180182,2668.849778175354,3.1341187423095107e-09
727728,1455457,727728,2183185,2672.3663680553436,2.6520865503698587e-09
728729,1457459,728729,2186188,2675.88538813591,1.9972503650933504e-09
729730,1459461,729730,2189191,2679.417528152466,1.304215402342379e-09
730731,1461463,730731,2192194,2683.6929881572723,7.494236342608929e-10
731732,1463465,731732,2195197,2687.3584911823273,4.5292836148291826e-10
732733,1465467,732733,2198200,2691.463066339493,4.747562343254685e-10
733734,1467469,733734,2201203,2695.4947032928467,8.221832104027271e-10
734735,1469471,734735,2204206,2699.3586270809174,1.3842509360983968e-09
735736,1471473,735736,2207209,2703.3454842567444,2.0500010577961802e-09
736737,1473475,736737,2210212,2706.7353100776672,2.646629582159221e-09
737738,1475477,737738,2213215,2710.0335800647736,3.0322553357109427e-09
738739,1477479,738739,2216218,2713.3239171504974,3.130480763502419e-09
739740,1479481,739740,2219221,2716.5936381816864,2.8994691092520952e-09
740741,1481483,740741,2222224,2719.9031682014465,2.4119799491018057e-09
741742,1483485,741742,2225227,2723.204814195633,1.7716956790536642e-09
742743,1485487,742743,2228230,2726.4522371292114,1.1259544407948852e-09
743744,1487489,743744,2231233,2729.69784116745,6.402842700481415e-10
744745,1489491,744745,2234236,2732.922909259796,4.0381564758718014e-10
745746,1491493,745746,2237239,2736.476382255554,4.874891601502895e-10
746747,1493495,746747,2240242,2740.046219110489,8.549250196665525e-10
747748,1495497,747748,2243245,2745.448000192642,1.418811734765768e-09
748749,1497499,748749,2246248,2751.395127058029,2.051820047199726e-09
749750,1499501,749750,2249251,2755.9028232097626,2.586602931842208e-09
750751,1501503,750751,2252254,2759.8565921783447,2.9122020350769162e-09
751752,1503505,751752,2255257,2763.9447071552277,2.9467628337442875e-09
752753,1505507,752753,2258260,2768.188818216324,2.6793713914230466e-09
753754,1507509,753754,2261263,2771.972650051117,2.1827872842550278e-09
754755,1509511,754755,2264266,2775.160377264023,1.558873918838799e-09
755756,1511513,755756,2267269,2778.3834130764008,9.713403414934874e-10
756757,1513515,756757,2270272,2781.599817276001,5.420588422566652e-10
757758,1515517,757758,2273275,2784.920111179352,3.710738383233547e-10
758759,1517519,758759,2276278,2788.1362001895905,5.056790541857481e-10
759760,1519521,759760,2279281,2791.5473721027374,8.931237971410155e-10
760761,1521523,760761,2282284,2794.73854637146,1.4533725334331393e-09
761762,1523525,761762,2285287,2798.033088207245,2.042725100181997e-09
762763,1525527,762763,2288290,2801.425119161606,2.5247572921216488e-09
763764,1527529,763764,2291293,2804.6460983753204,2.790329745039344e-09
764765,1529531,764765,2294296,2807.94069814682,2.7666828827932477e-09
765766,1531533,765766,2297299,2811.5006172657013,2.472006599418819e-09
766767,1533535,766767,2300302,2815.070963382721,1.9681465346366167e-09
767768,1535537,767768,2303305,2818.294783115387,1.3733369996771216e-09
768769,1537539,768769,2306308,2821.4617381095886,8.330971468240023e-10
769770,1539541,769770,2309311,2824.713522195816,4.5838532969355583e-10
770771,1541543,770771,2312314,2827.9184432029724,3.5288394428789616e-10
771772,1543545,771772,2315317,2831.0510931015015,5.220499588176608e-10
772773,1545547,772773,2318320,2834.734838247299,9.276845958083868e-10
773774,1547549,773774,2321323,2837.9560811519623,1.4806573744863272e-09
774775,1549551,774775,2324326,2841.1554062366486,2.026354195550084e-09
775776,1551553,775776,2327329,2844.3567481040955,2.461092662997544e-09
776777,1553555,776777,2330332,2847.888763189316,2.663000486791134e-09
777778,1555557,777778,2333335,2852.8667330741882,2.5938788894563913e-09
778779,1557559,778779,2336338,2857.3033742904663,2.2737367544323206e-09
779780,1559561,779780,2339341,2861.037922143936,1.7644197214394808e-09
780781,1561563,780781,2342344,2864.464655160904,1.204170985147357e-09
781782,1563565,781782,2345347,2867.912141084671,7.057678885757923e-10
782783,1565567,782783,2348350,2871.336527109146,3.9472070056945086e-10
783784,1567569,783784,2351353,2874.7458782196045,3.41970007866621e-10
784785,1569571,784785,2354356,2878.203850030899,5.438778316602111e-10
785786,1571573,785786,2357359,2882.1107251644135,9.695213520899415e-10
786787,1573575,786787,2360362,2885.5899741649628,1.4970282791182399e-09
787788,1575577,787788,2363365,2889.013243198395,2.0118022803217173e-09
788789,1577579,788789,2366368,2892.306687116623,2.3919710656628013e-09
789790,1579581,789790,2369371,2896.7727570533752,2.535671228542924e-09
790791,1581583,790791,2372374,2901.8932774066925,2.4301698431372643e-09
791792,1583585,791792,2375377,2907.0032012462616,2.0827428670600057e-09
792793,1585587,792793,2378380,2912.1032230854034,1.584339770488441e-09
793794,1587589,793794,2381383,3043.178678035736,1.0495568858459592e-09
794795,1589591,794795,2384386,3048.5091631412506,5.984475137665868e-10
795796,1591593,795796,2387389,3060.5326499938965,3.4560798667371273e-10
796797,1593595,796797,2390392,3077.6459782123566,3.346940502524376e-10
797798,1595597,797798,2393395,3094.0000302791595,5.766196409240365e-10
798799,1597599,798799,2396398,3316.1863560676575,1.002263161353767e-09
799800,1599601,799800,2399401,3321.483691215515,1.5097612049430609e-09
800801,1601603,800801,2402404,3337.2648293972015,1.988155418075621e-09
801802,1603605,801802,2405407,3581.2890853881836,2.3119355319067836e-09
802803,1605607,802803,2408410,3586.9609100818634,2.4119799491018057e-09
803804,1607609,803804,2411413,3601.7909801006317,2.2646418074145913e-09
804805,1609611,804805,2414416,3972.7191112041473,1.90084392670542e-09
805806,1611613,805806,2417419,3978.3842282295227,1.4151737559586763e-09
806807,1613615,806807,2420422,3993.465014219284,9.094947017729282e-10
807808,1615617,807808,2423425,4004.3358783721924,5.093170329928398e-10
808809,1617619,808809,2426428,4009.426323413849,3.0740920919924974e-10
809810,1619621,809810,2429431,4520.010407209396,3.383320290595293e-10
810811,1621623,810811,2432434,4551.249640226364,6.075424607843161e-10
811812,1623625,811812,2435437,4556.752989292145,1.0331859812140465e-09
812813,1625627,812813,2438440,4564.881210327148,1.5243131201714277e-09
813814,1627629,813814,2441443,4906.97042632103,1.9572325982153416e-09
814815,1629631,814815,2444446,4919.416699171066,2.2337189875543118e-09
815816,1631633,815816,2447449,4924.866777181625,2.2901076590642333e-09
816817,1633635,816817,2450452,4931.835343122482,2.104570739902556e-09
817818,1635637,817818,2453455,4950.770079135895,1.7316779121756554e-09
818819,1637639,818819,2456458,4983.057963132858,1.2569216778501868e-09
819820,1639641,819820,2459461,4988.196266174316,7.839844329282641e-10
820821,1641643,820821,2462464,4999.778615236282,4.347384674474597e-10
821822,1643645,821822,2465467,5016.007645368576,2.7466739993542433e-10
822823,1645647,822823,2468470,6735.698296070099,3.510649548843503e-10
823824,1647649,823824,2471473,6742.3715903759,6.348273018375039e-10
824825,1649651,824825,2474476,6747.2542362213135,1.0604708222672343e-09
825826,1651653,825826,2477479,6751.537607192993,1.5297700883820653e-09
826827,1653655,826827,2480482,6755.901738166809,1.9208528101444244e-09
827828,1655657,827828,2483485,6759.965269088745,2.153683453798294e-09
828829,1657659,828829,2486488,6764.275462150574,2.164597390219569e-09
829830,1659661,829830,2489491,6768.620796203613,1.951775630004704e-09
830831,1661663,830831,2492494,6772.492253303528,1.5752448234707117e-09
831832,1663665,831832,2495497,6776.140933275223,1.1077645467594266e-09
832833,1665667,832833,2498500,6779.407901287079,6.766640581190586e-10
833834,1667669,833834,2501503,6782.907155990601,3.6561687011271715e-10
834835,1669671,834835,2504506,6786.668029308319,2.5283952709287405e-10
835836,1671673,835836,2507509,6790.101169347763,3.6561687011271715e-10
836837,1673675,836837,2510512,6793.7152371406555,6.675691111013293e-10
837838,1675677,837838,2513515,6797.51366519928,1.089574652723968e-09
838839,1677679,838839,2516518,6801.667042255402,1.5279510989785194e-09
839840,1679681,839840,2519521,6805.492425441742,1.8826540326699615e-09
840841,1681683,840841,2522524,6809.691873073578,2.0700099412351847e-09
841842,1683685,841842,2525527,6813.410325050354,2.039087121374905e-09
842843,1685687,842843,2528530,6816.913640975952,1.8062564777210355e-09
843844,1687689,843844,2531533,6820.383045196533,1.4224497135728598e-09
844845,1689691,844845,2534536,6823.862487077713,9.786162991076708e-10
845846,1691693,845846,2537539,6828.046031236649,5.802576197311282e-10
846847,1693695,846847,2540542,6832.7320392131805,3.128661774098873e-10
847848,1695697,847848,2543545,6837.4867742061615,2.4374458007514477e-10
848849,1697699,848849,2546548,6841.78751206398,3.838067641481757e-10
849850,1699701,849850,2549551,6846.938661336899,6.984919309616089e-10
850851,1701703,850851,2552554,6851.415395259857,1.1114025255665183e-09
851852,1703705,851852,2555557,6855.737832307816,1.520675141364336e-09
852853,1705707,852853,2558560,6859.781392335892,1.838998286984861e-09
853854,1707709,853854,2561563,6863.166802406311,1.9826984498649836e-09
854855,1709711,854855,2564566,6866.815851211548,1.9172148313373327e-09
855856,1711713,855856,2567569,6870.090624094009,1.6661942936480045e-09
856857,1713715,856857,2570572,6873.423003196716,1.278749550692737e-09
857858,1715717,857858,2573575,6876.76368522644,8.585629984736443e-10
858859,1717719,858859,2576578,6880.035274028778,4.911271389573812e-10
859860,1719721,859860,2579581,6883.949195146561,2.6921043172478676e-10
860861,1721723,860861,2582584,6888.359049320221,2.382876118645072e-10
861862,1723725,861862,2585587,6892.1287753582,4.0381564758718014e-10
862863,1725727,862863,2588590,6897.872997283936,7.294147508218884e-10
863864,1727729,863864,2591593,6902.682107210159,1.1314114090055227e-09
864865,1729731,864865,2594596,6907.34006023407,1.5152181731536984e-09
865866,1731733,865866,2597599,6910.851347208023,1.7917045624926686e-09
866867,1733735,866867,2600602,6914.40172123909,1.8917489796876907e-09
867868,1735737,867868,2603605,6917.918593168259,1.800799509510398e-09
868869,1737739,868869,2606608,6921.51734828949,1.5297700883820653e-09
869870,1739741,869870,2609611,6924.992821216583,1.1496013030409813e-09
870871,1741743,870871,2612614,6929.397313117981,7.494236342608929e-10
871872,1743745,871872,2615617,6933.215014219284,4.1654857341200113e-10
872873,1745747,872873,2618620,6937.069431066513,2.346496330574155e-10
873874,1747749,873874,2621623,6940.337334156036,2.382876118645072e-10
874875,1749751,874875,2624626,6943.652614355087,4.2928149923682213e-10
875876,1751753,875876,2627629,6947.167523145676,7.585185812786222e-10
876877,1753755,876877,2630632,6950.668491125107,1.1441443348303437e-09
877878,1755757,877878,2633635,6954.827015399933,1.5024852473288774e-09
878879,1757759,878879,2636638,6959.060093402863,1.737134880386293e-09
879880,1759761,879880,2639641,6962.633086204529,1.8044374883174896e-09
880881,1761763,880881,2642644,6966.303299188614,1.6807462088763714e-09
881882,1763765,881882,2645647,6970.0769102573395,1.3988028513267636e-09
882883,1765767,882883,2648650,6974.428118228912,1.027729013003409e-09
883884,1767769,883884,2651653,6979.0549330711365,6.475602276623249e-10
884885,1769771,884885,2654656,6984.340147256851,3.5288394428789616e-10
885886,1771773,885886,2657659,6989.2647223472595,2.091837814077735e-10
886887,1773775,886887,2660662,6992.76113319397,2.4374458007514477e-10
887888,1775777,887888,2663665,6996.285879135132,4.5656634029001e-10
888889,1777779,888889,2666668,6999.562583208084,7.839844329282641e-10
889890,1779781,889890,2669671,7002.86917924881,1.1568772606551647e-09
890891,1781783,890891,2672674,7006.640300035477,1.4842953532934189e-09
891892,1783785,891892,2675677,7010.080147981644,1.6825651982799172e-09
892893,1785787,892893,2678680,7015.166558265686,1.7153070075437427e-09
893894,1787789,893894,2681683,7020.91349196434,1.5661498764529824e-09
894895,1789791,894895,2684686,7025.922127246857,1.278749550692737e-09
895896,1791793,895896,2687689,7029.24610209465,9.149516699835658e-10
896897,1793795,896897,2690692,7032.483439207077,5.584297468885779e-10
897898,1795797,897898,2693695,7035.705412149429,3.001332515850663e-10
898899,1797799,898899,2696698,7038.958849191666,1.8917489796876907e-10
899900,1799801,899900,2699701,7042.189169168472,2.5647750589996576e-10
900901,1801803,900901,2702704,7045.476186275482,4.82032191939652e-10
901902,1803805,901902,2705707,7048.815662145615,8.094502845779061e-10
902903,1805807,902903,2708710,7052.049074172974,1.165972207672894e-09
903904,1807809,903904,2711713,7055.320916175842,1.4588295016437769e-09
904905,1809811,904905,2714716,7058.541572093964,1.6261765267699957e-09
905906,1811813,905906,2717719,7061.842265129089,1.6243575373664498e-09
906907,1813815,906907,2720722,7065.036437034607,1.4551915228366852e-09
907908,1815817,907908,2723725,7068.209545373917,1.1623342288658023e-09
908909,1817819,908909,2726728,7071.375659227371,8.076312951743603e-10
909910,1819821,909910,2729731,7074.59802031517,4.802132025361061e-10
910911,1821823,910911,2732734,7077.761850118637,2.5283952709287405e-10
911912,1823825,911912,2735737,7080.9590582847595,1.7826096154749393e-10
912913,1825827,912913,2738740,7084.162415266037,2.710294211283326e-10
913914,1827829,913914,2741743,7087.311136007309,5.07498043589294e-10
914915,1829831,914915,2744746,7090.52698135376,8.349161362275481e-10
915916,1831833,915916,2747749,7093.699334144592,1.1696101864799857e-09
916917,1833835,916917,2750752,7096.888296365738,1.433363649994135e-09
917918,1835837,917918,2753755,7100.0612070560455,1.5661498764529824e-09
918919,1837839,918919,2756758,7103.253433227539,1.5352270565927029e-09
919920,1839841,919920,2759761,7106.496868133545,1.3515091268345714e-09
920921,1841843,920921,2762764,7109.658318281174,1.051375875249505e-09
921922,1843845,921922,2765767,7112.785790205002,7.112248567864299e-10
922923,1845847,922923,2768770,7116.008377313614,4.1109160520136356e-10
923924,1847849,923924,2771773,7119.135715246201,2.1464074961841106e-10
924925,1849851,924925,2774776,7122.292296409607,1.7280399333685637e-10
925926,1851853,925926,2777779,7125.463452339172,2.874003257602453e-10
926927,1853855,926927,2780782,7128.630537986755,5.347828846424818e-10
927928,1855857,927928,2783785,7131.777525186539,8.549250196665525e-10
928929,1857859,928929,2786788,7134.991672277451,1.1677911970764399e-09
929930,1859861,929930,2789791,7138.1582572460175,1.4042598195374012e-09
930931,1861863,930931,2792794,7141.381271123886,1.5043042367324233e-09
931932,1863865,931932,2795797,7144.550966024399,1.446096575818956e-09
932933,1865867,932933,2798800,7147.694025278091,1.2478267308324575e-09
933934,1867869,933934,2801803,7150.881658315659,9.476934792473912e-10
934935,1869871,934935,2804806,7154.056929111481,6.257323548197746e-10
935936,1871873,935936,2807809,7157.265622138977,3.474269760772586e-10
936937,1873875,936937,2810812,7160.406618118286,1.8553691916167736e-10
937938,1875877,937938,2813815,7163.592141151428,1.709850039333105e-10
938939,1877879,938939,2816818,7166.8051471710205,3.055902197957039e-10
939940,1879881,939940,2819821,7169.995300292969,5.620677256956697e-10
940941,1881883,940941,2822824,7173.135371208191,8.731149137020111e-10
941942,1883885,941942,2825827,7176.327881336212,1.165972207672894e-09
942943,1885887,942943,2828830,7179.4462831020355,1.36969902087003e-09
943944,1887889,943944,2831833,7182.6290991306305,1.4406396076083183e-09
944945,1889891,944945,2834836,7185.810330152512,1.3587850844487548e-09
945946,1891893,945946,2837839,7189.015078306198,1.1477823136374354e-09
946947,1893895,946947,2840842,7192.165714263916,8.49468051455915e-10
947948,1895897,947948,2843845,7195.343794345856,5.438778316602111e-10
948949,1897899,948949,2846848,7198.517322063446,2.9103830456733704e-10
949950,1899901,949950,2849851,7201.708632230759,1.6189005691558123e-10
950951,1901903,950951,2852854,7204.921075344086,1.7280399333685637e-10
951952,1903905,951952,2855857,7208.099728345871,3.2741809263825417e-10
952953,1905907,952953,2858860,7211.461229085922,5.857145879417658e-10
953954,1907909,953954,2861863,7214.749589204788,8.858478395268321e-10
954955,1909911,954955,2864866,7217.9327030181885,1.1568772606551647e-09
955956,1911913,955956,2867869,7221.068781137466,1.331500243395567e-09
956957,1913915,956957,2870872,7224.269334077835,1.3751559890806675e-09
957958,1915917,957958,2873875,7227.524897098541,1.2732925824820995e-09
958959,1917919,958959,2876878,7230.71652507782,1.0495568858459592e-09
959960,1919921,959960,2879881,7233.924180030823,7.60337570682168e-10
960961,1921923,960961,2882884,7237.128484249115,4.69299266114831e-10
961962,1923925,961962,2885887,7240.3002161979675,2.473825588822365e-10
962963,1925927,962963,2888890,7243.448436021805,1.418811734765768e-10
963964,1927929,963964,2891893,7246.632872343063,1.800799509510398e-10
964965,1929931,964965,2894896,7249.772546052933,3.510649548843503e-10
965966,1931933,965966,2897899,7252.9374232292175,6.093614501878619e-10
966967,1933935,966967,2900902,7256.135243177414,8.967617759481072e-10
967968,1935937,967968,2903905,7259.3071372509,1.1459633242338896e-09
968969,1937939,968969,2906908,7262.475455999374,1.293301465921104e-09
969970,1939941,969970,2909911,7265.636107206345,1.3096723705530167e-09
970971,1941943,970971,2912914,7268.760858297348,1.1896190699189901e-09
971972,1943945,971972,2915917,7272.094693183899,9.604264050722122e-10
972973,1945947,972973,2918920,7275.408621072769,6.748450687155128e-10
973974,1947949,973974,2921923,7278.606066226959,4.0381564758718014e-10
974975,1949951,974975,2924926,7281.759749174118,2.0736479200422764e-10
975976,1951953,975976,2927929,7285.0685613155365,1.291482476517558e-10
976977,1953955,976977,2930932,7288.266876220703,1.9099388737231493e-10
977978,1955957,977978,2933935,7291.418568372726,3.728928277269006e-10
978979,1957959,978979,2936938,7294.595208406448,6.293703336268663e-10
979980,1959961,979980,2939941,7297.788108110428,9.040377335622907e-10
980981,1961963,980981,2942944,7301.004690408707,1.1295924196019769e-09
981982,1963965,981982,2945947,7304.180283308029,1.2532836990430951e-09
982983,1965967,982983,2948950,7307.383549213409,1.2441887520253658e-09
983984,1967969,983984,2951953,7310.529706001282,1.1059455573558807e-09
984985,1969971,984985,2954956,7313.7852873802185,8.712959242984653e-10
985986,1971973,985986,2957959,7316.961370229721,5.966285243630409e-10
986987,1973975,986987,2960962,7320.201455116272,3.4560798667371273e-10
987988,1975977,987988,2963965,7323.36323428154,1.7462298274040222e-10
988989,1977979,988989,2966968,7326.555935144424,1.2369127944111824e-10
989990,1979981,989990,2969971,7329.906496047974,2.0372681319713593e-10
990991,1981983,990991,2972974,7333.1927921772,3.92901711165905e-10
991992,1983985,991992,2975977,7336.542483329773,6.511982064694166e-10
992993,1985987,992993,2978980,7339.712801218033,9.113136911764741e-10
993994,1987989,993994,2981983,7342.91934633255,1.1132215149700642e-09
994995,1989991,994995,2984986,7346.115130186081,1.2096279533579946e-09
995996,1991993,995996,2987989,7349.297986268997,1.1768861440941691e-09
996997,1993995,996997,2990992,7352.441415309906,1.027729013003409e-09
997998,1995997,997998,2993995,7355.626323223114,7.894414011389017e-10
998999,1997999,998999,2996998,7359.094793319702,5.238689482212067e-10
1000000,2000001,1000000,3000001,7362.588329076767,2.9103830456733704e-10


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0057239532470703125,12064.44795143716
2002,2003,2002,4005,12.436393976211548,60.51993723720079
4004,4005,4004,8009,25.71987295150757,39.88241343054506
6006,6007,6006,12013,38.19901394844055,32.00320195854874
8008,8009,8008,16017,50.22892189025879,27.11878342527234
10010,10011,10010,20021,62.043492794036865,23.600809461513563
12012,12013,12012,24025,74.60394597053528,20.87201122395527
14014,14015,14014,28029,86.38209104537964,18.662265440172632
16016,16017,16016,32033,98.00693202018738,16.824269278082284
18018,18019,18018,36037,110.01513075828552,15.26812653666093
20020,20021,20020,40041,122.02707886695862,13.933915243173033
22022,22023,22022,44045,134.24667978286743,12.7789585000246
24024,24025,24024,48049,146.3578817844391,11.771532716749789
26026,26027,26026,52053,158.34342575073242,10.887304434972975
28028,28029,28028,56057,170.08169078826904,10.106940923971706
30030,30031,30030,60061,181.90570878982544,9.415009303915213
32032,32033,32032,64065,193.57988691329956,8.798924690163403
34034,34035,34034,68069,205.30493688583374,8.248303509202742
36036,36037,36036,72073,218.9467749595642,7.754504986927714
38038,38039,38038,76077,231.09176397323608,7.310268688397628
40040,40041,40040,80081,243.01428389549255,6.909446919986294
42042,42043,42042,84085,254.84966778755188,6.546798895624306
44044,44045,44044,88089,266.65815782546997,6.217830272196807
46046,46047,46046,92093,278.47862792015076,5.9186665376364544
48048,48049,48048,96097,290.37919998168945,5.64595199842006
50050,50051,50050,100101,302.99673771858215,5.396768357961264
52052,52053,52052,104105,315.020770072937,5.168568454482738
54054,54055,54054,108109,327.00134086608887,4.959121853180477
56056,56057,56056,112113,338.9367609024048,4.7664698020507785
58058,58059,58058,116117,350.7897849082947,4.58888765613483
60060,60061,60060,120121,364.6209900379181,4.424853314429129
62062,62063,62062,124125,376.65045189857483,4.2730205407206086
64064,64065,64064,128129,388.3451919555664,4.132196285041573
66066,66067,66066,132133,400.19295167922974,4.001321308174738
68068,68069,68068,136137,412.1706256866455,3.879453553347048
70070,70071,70070,140141,424.5643730163574,3.7657538182211283
72072,72073,72072,144145,436.7355830669403,3.6594773410542984
74074,74075,74074,148149,448.8546619415283,3.5599631590121135
76076,76077,76076,152153,461.0212297439575,3.466599750589012
78078,78079,78078,156157,473.01087188720703,3.378850675193462
80080,80081,80080,160161,484.99418091773987,3.296234586088758
82082,82083,82082,164165,496.9757888317108,3.2183189854094962
84084,84085,84084,168169,508.9748728275299,3.144714744823432
86086,86087,86086,172173,521.1559927463531,3.075071289913467
88088,88089,88088,176177,534.1229887008667,3.009072361419385
90090,90091,90090,180181,547.4847009181976,2.946432278959037
92092,92093,92092,184185,560.69677901268,2.886892643324245
94094,94095,94094,188189,574.0359108448029,2.830219422305163
96096,96097,96096,192193,587.1588208675385,2.776200372385574
98098,98099,98098,196197,599.5922870635986,2.7246427550617227
100100,100101,100100,200201,612.2796759605408,2.6753713119760505
102102,102103,102102,204205,624.2887878417969,2.6282264676283376
104104,104105,104104,208209,636.6425428390503,2.5830627325176465
106106,106107,106106,212213,649.4141659736633,2.539747282902681
108108,108109,108108,216217,661.291729927063,2.4981586964659073
110110,110111,110110,220221,674.5944588184357,2.458185825658802
112112,112113,112112,224225,687.0721189975739,2.419728418746672
114114,114115,114114,228229,700.1456429958344,2.3826917704482184
116116,116117,116116,232233,712.5705690383911,2.3469894577210653
118118,118119,118118,236237,726.6118957996368,2.3125424037352786
120120,120121,120120,240241,739.7932078838348,2.2792777431986906
122122,122123,122122,244245,753.282194852829,2.2471282462211093
124124,124125,124124,248249,766.1182217597961,2.2160318020432896
126126,126127,126126,252253,779.7206218242645,2.185930955405638
128128,128129,128128,256257,792.6831839084625,2.156772489848663
130130,130131,130130,260261,805.3283257484436,2.1285070527756034
132132,132133,132132,264265,818.0841867923737,2.101088817762502
134134,134135,134134,268269,832.237548828125,2.074475180121226
136136,136137,136136,272273,845.7020077705383,2.0486264821665827
138138,138139,138138,276277,858.3537449836731,2.0235057650261297
140140,140141,140140,280281,871.7645168304443,1.999078544205986
142142,142143,142142,284285,884.2345380783081,1.9753126064442768
144144,144145,144144,288289,896.6575119495392,1.9521778256057587
146146,146147,146146,292293,911.8370177745819,1.9296459957095067
148148,148149,148148,296297,928.2627310752869,1.907690679301595
150150,150151,150150,300301,942.5262930393219,1.8862870696302707
152152,152153,152152,304305,956.9589538574219,1.8654118652539182
154154,154155,154154,308309,969.4725189208984,1.8450431557976117
156156,156157,156156,312313,981.6946058273315,1.8251603178177902
158158,158159,158158,316317,994.0580518245697,1.8057439197345957
160160,160161,160160,320321,1005.7127039432526,1.786775634966034
162162,162163,162162,324325,1019.3803677558899,1.7682381624836125
164164,164165,164164,328329,1032.294604063034,1.750115555969387
166166,166167,166166,332333,1047.8579938411713,1.7323943171086285
168168,168169,168168,336337,1061.5030510425568,1.7150572421560355
170170,170171,170170,340341,1074.345566034317,1.6980904722713603
172172,172173,172172,344345,1088.7563667297363,1.6814808655835805
174174,174175,174174,348349,1101.6455948352814,1.6652159496188688
176176,176177,176176,352353,1113.6186158657074,1.6492838775011478
178178,178179,178178,356357,1128.7404947280884,1.633673387554154
180180,180181,180180,360361,1141.9701509475708,1.618373766043078
182182,182183,182182,364365,1155.8671288490295,1.6033748127374565
184184,184185,184184,368369,1168.6076848506927,1.588666809066126
186186,186187,186186,372373,1180.1918830871582,1.5742404886641452
188188,188189,188188,376377,1193.8216331005096,1.5600870100624888
190190,190191,190190,380381,1207.136992931366,1.5461979313786287
192192,192193,192192,384385,1219.127534866333,1.5325651868151908
194194,194195,194194,388389,1231.8551909923553,1.5191810648429964
196196,196197,196196,392393,1243.8286719322205,1.5060381879084161
198198,198199,198198,396397,1256.722396850586,1.4931294935413462
200200,200201,200200,400401,1268.4278347492218,1.4804482167728565
202202,202203,202202,404405,1280.7494778633118,1.4679878737460967
204204,204205,204204,408409,1293.9298660755157,1.4557422464022238
206206,206207,206206,412413,1307.349361896515,1.4437053682177066
208208,208209,208208,416417,1319.3975067138672,1.4318715108456672
210210,210211,210210,420421,1331.3609087467194,1.4202351716412522
212212,212213,212212,424425,1343.1036500930786,1.4087910619764443
214214,214215,214214,428429,1354.8843069076538,1.3975340963006602
216216,216217,216216,432433,1367.5499289035797,1.3864593818798312
218218,218219,218218,436437,1384.2030079364777,1.3755622091830446
220220,220221,220220,440441,1397.7674989700317,1.364838042845804
222222,222223,222222,444445,1411.605272769928,1.3542825131826248
224224,224225,224224,448449,1424.8626708984375,1.3438914082180418
226226,226227,226226,452453,1438.3287608623505,1.3336606661760015
228228,228229,228228,456457,1451.3452298641205,1.323586368424003
230230,230231,230230,460461,1464.2619998455048,1.313664732810139
232232,232233,232232,464465,1476.928631067276,1.3038921074039536
234234,234235,234234,468469,1489.2473368644714,1.294264964564718
236236,236237,236236,472473,1502.4832429885864,1.284781583435688
238238,238239,238238,476477,1515.8099808692932,1.2754374627220386
240240,240241,240240,480481,1528.5791397094727,1.2662289049112587
242242,242243,242242,484485,1541.096617937088,1.257152827014579
244244,244245,244244,488489,1553.6392469406128,1.2482062455619598
246246,246247,246246,492493,1566.2238228321075,1.239386272194679
248248,248249,248248,496497,1578.7233929634094,1.2306901096308138
250250,250251,250250,500501,1591.0744078159332,1.2221150478617346
252252,252253,252252,504505,1603.4611568450928,1.213658460557781
254254,254255,254254,508509,1616.454274892807,1.2053178016558377
256256,256257,256256,512513,1629.264592885971,1.1970906021233532
258258,258259,258258,516517,1643.3768830299377,1.1889744668806088
260260,260261,260260,520521,1657.1598699092865,1.1809670718939742
262262,262263,262262,524525,1670.782167673111,1.1730661613728444
264264,264265,264264,528529,1683.5909428596497,1.165269545157571
266266,266267,266266,532533,1697.804841041565,1.1575750961819722
268268,268269,268268,536537,1711.2884407043457,1.1499807480904565
270270,270271,270270,540541,1724.6725058555603,1.142484492962467
272272,272273,272272,544545,1737.6296887397766,1.1350843791242369
274274,274275,274274,548549,1750.2737798690796,1.1277785090842372
276276,276277,276276,552553,1762.9676077365875,1.1205650375632104
278278,278279,278278,556557,1775.440813779831,1.113442169589689
280280,280281,280280,560561,1788.0645167827606,1.106408158715567
282282,282283,282282,564565,1800.469456911087,1.0994613052844215
284284,284285,284284,568569,1815.9201438426971,1.092599954790785
286286,286287,286286,572573,1830.4021179676056,1.0858224963048997
288288,288289,288288,576577,1843.8353190422058,1.079127360972052
290290,290291,290290,580581,1857.1701409816742,1.0725130205682945
292292,292293,292292,584585,1872.0150468349457,1.065977986128928
294294,294295,294294,588589,1884.6017858982086,1.0595208066242776
296296,296297,296296,592593,1897.4450199604034,1.0531400676991325
298298,298299,298298,596597,1910.5697510242462,1.0468343904612993
300300,300301,300300,600601,1922.6424479484558,1.04060243031563
302302,302303,302302,604605,1936.4769790172577,1.0344428758617141
304304,304305,304304,608609,1949.7964890003204,1.028354447806123
306306,306307,306306,612613,1962.519910812378,1.022335897965604
308308,308309,308308,616617,1975.4930489063263,1.0163860082484462
310310,310311,310310,620621,1988.8836948871613,1.0105035897377093
312312,312313,312312,624625,2002.3053770065308,1.0046874817689968
314314,314315,314314,628629,2016.0459520816803,0.9989365510573407
316316,316317,316316,632633,2030.028657913208,0.9932496908622852
318318,318319,318318,636637,2043.6190469264984,0.9876258201802557
320320,320321,320320,640641,2056.511157989502,0.9820638829642121
322322,322323,322322,644645,2069.0415139198303,0.9765628473796824
324324,324325,324324,648649,2082.677750110626,0.9711217050808045
326326,326327,326326,652653,2095.9720509052277,0.9657394705227489
328328,328329,328328,656657,2107.9979219436646,0.9604151802941487
330330,330331,330330,660661,2121.4130918979645,0.9551478924713592
332332,332333,332332,664665,2135.2459127902985,0.9499366860000009
334334,334335,334334,668669,2148.730887889862,0.9447806600946933
336336,336337,336336,672673,2162.387978076935,0.9396789336697111
338338,338339,338338,676677,2175.961683034897,0.9346306447750976
340340,340341,340340,680681,2190.5152208805084,0.9296349500655197
342342,342343,342342,684685,2202.984610080719,0.9246910242891317
344344,344345,344344,688689,2215.7431168556213,0.919798059765526
346346,346347,346346,692693,2228.665988922119,0.9149552659291658
348348,348349,348348,696697,2241.1729769706726,0.9101618688546296
350350,350351,350350,700701,2253.857395887375,0.9054171107909497
352352,352353,352352,704705,2266.3755128383636,0.9007202497523394
354354,354355,354354,708709,2278.7559299468994,0.896070559079817
356356,356357,356356,712713,2291.195673942566,0.8914673270392086
358358,358359,358358,716717,2304.1715857982635,0.8869098564282467
360360,360361,360360,720721,2317.039179086685,0.8823974641964014
362362,362363,362362,724725,2329.9535529613495,0.8779294810738065
364364,364365,364364,728729,2342.473002910614,0.8735052512238326
366366,366367,366366,732733,2355.018185853958,0.869124131886565
368368,368369,368368,736737,2366.9916837215424,0.8647854930513859
370370,370371,370370,740741,2378.997701883316,0.8604887171313749
372372,372373,372372,744745,2392.327955007553,0.8562331986540812
374374,374375,374374,748749,2405.3300170898438,0.8520183439468383
376376,376377,376376,752753,2418.4522778987885,0.8478435708675534
378378,378379,378378,756757,2431.81685090065,0.8437083084827464
380380,380381,380380,760761,2444.863914012909,0.8396119968274434
382382,382383,382382,764765,2456.9826679229736,0.8355540866105002
384384,384385,384384,768769,2468.972272872925,0.8315340389726771
386386,386387,386386,772773,2480.946861743927,0.8275513252247038
388388,388389,388388,776777,2494.5223019123077,0.823605849289379
390390,390391,390390,780781,2508.3469598293304,0.8196969175605773
392392,392393,392392,784785,2521.7119858264923,0.8158237875995837
394394,394395,394394,788789,2535.266530752182,0.811985967480723
396396,396397,396396,792793,2548.3147678375244,0.808182975899399
398398,398399,398398,796797,2561.3257191181183,0.804414340396761
400400,400401,400400,800801,2574.0794739723206,0.800679597121416
402402,402403,402402,804805,2586.815207004547,0.7969782906257024
404404,404405,404404,808809,2598.9453258514404,0.7933099736819713
406406,406407,406406,812813,2611.8092958927155,0.7896742070752225
408408,408409,408408,816817,2625.302619934082,0.7860705594393949
410410,410411,410410,820821,2637.18074798584,0.7824986070663726
412412,412413,412412,824825,2650.405716896057,0.7789579337368195
414414,414415,414414,828829,2662.7680048942566,0.7754481305619265
416416,416417,416416,832833,2675.2952420711517,0.7719687957978749
418418,418419,418418,836837,2686.934940814972,0.7685195347148692
420420,420421,420420,840841,2699.8706629276276,0.7650999594152381
422422,422423,422422,844845,2713.025932788849,0.7617096887133812
424424,424425,424424,848849,2727.2112929821014,0.7583483479575079
426426,426427,426426,852853,2740.7151119709015,0.7550155689077656
428428,428429,428428,856857,2754.4733397960663,0.7517109895998146
430430,430431,430430,860861,2767.3416709899902,0.7484342541920341
432432,432433,432432,864865,2778.824870824814,0.745185012856382
434434,434435,434434,868869,2790.198425769806,0.7419629216274188
436436,436437,436436,872873,2802.393215894699,0.738767642298626
438438,438439,438438,876877,2816.1583228111267,0.7355988422896189
440440,440441,440440,880881,2829.272639989853,0.7324561945260939
442442,442443,442442,884885,2843.0711948871613,0.7293393773379648
444444,444445,444444,888889,2855.3805010318756,0.7262480743265769
446446,446447,446446,892893,2868.363438844681,0.723181974281033
448448,448449,448448,896897,2881.4017260074615,0.7201407710435888
450450,450451,450450,900901,2893.8148880004883,0.7171241634277976
452452,452453,452452,904905,2906.279236793518,0.7141318551039149
454454,454455,454454,908909,2919.3031549453735,0.7111635613619001
456456,456457,456456,912913,2932.065527677536,0.7082190378696396
458458,458459,458458,916917,2944.88738489151,0.705297955288188
460460,460461,460460,920921,2959.066305875778,0.7024000356959732
462462,462463,462462,924925,2972.166332960129,0.6995250055406359
464464,464465,464464,928929,2987.2646107673645,0.6966725955990114
466466,466467,466466,932933,3004.01775097847,0.6938425408516196
468468,468469,468468,936937,3016.986512899399,0.6910345804280951
470470,470471,470470,940941,3030.527004957199,0.688248457514419
472472,472473,472472,944945,3042.49551486969,0.6854839192710642
474474,474475,474474,948949,3054.28698182106,0.682740716758417
476476,476477,476476,952953,3065.7613368034363,0.6800186048676551
478478,478479,478478,956957,3077.402570962906,0.6773173422279797
480480,480481,480480,960961,3089.2032039165497,0.6746366911593213
482482,482483,482482,964965,3100.793107032776,0.6719764175868477
484484,484485,484484,968969,3112.444744825363,0.6693362909718417
486486,486487,486486,972973,3123.9330229759216,0.6667160842498561
488488,488489,488488,976977,3135.5045788288116,0.6641155737615918
490490,490491,490490,980981,3147.569133758545,0.6615345391965093
492492,492493,492492,984985,3160.3730659484863,0.6589727635109739
494494,494495,494494,988989,3172.4351818561554,0.6564300328955142
496496,496497,496496,992993,3184.71506690979,0.6539061366820533
498498,498499,498498,996997,3197.372960090637,0.6514008673239005
500501,500502,500501,1001003,3209.6635839939117,0.6489127826826007
502503,502504,502503,1005007,3221.5128247737885,0.6464441655152768
504505,504506,504505,1009011,3233.2372949123383,0.6439935704584059
506507,506508,506507,1013015,3244.9402298927307,0.641560801794185
508509,508510,508509,1017019,3256.222494840622,0.6391456666369777
510511,510512,510511,1021023,3267.246356010437,0.6367479748732876
512513,512514,512513,1025027,3278.258519887924,0.6343675391108263
514515,514516,514515,1029031,3289.5222997665405,0.6320041746421339
516517,516518,516517,1033035,3300.7477419376373,0.629657699380914
518519,518520,518519,1037039,3311.7653279304504,0.6273279338274733
520521,520522,520521,1041043,3322.668732881546,0.6250147010177898
522523,522524,522523,1045047,3333.583937883377,0.6227178264725808
524525,524526,524525,1049051,3344.539895772934,0.6204400265232834
526527,526528,526527,1053055,3355.457500934601,0.6181804328025464
528529,528530,528529,1057059,3366.358989715576,0.6159367944001133
530531,530532,530531,1061063,3377.19726896286,0.6137088857522031
532533,532534,532533,1065067,3388.1366369724274,0.6114965098204266
534535,534536,534535,1069071,3398.940510034561,0.6092994864266075
536537,536538,536537,1073075,3410.1583087444305,0.6071176459354319
538539,538540,538539,1077079,3421.1507778167725,0.6049508256819536
540541,540542,540541,1081083,3431.9294810295105,0.602798867968886
542543,542544,542543,1085087,3442.9948921203613,0.6006616188460612
544545,544546,544545,1089091,3454.2583696842194,0.598538927415575
546547,546548,546547,1093095,3465.4883248806,0.5964306453988684
548549,548550,548549,1097099,3476.714877843857,0.594340935585933
550551,550552,550551,1101103,3488.4569249153137,0.5922658603249147
552553,552554,552553,1105107,3499.696594953537,0.5902048294192355
554555,554556,554555,1109111,3510.7623360157013,0.5881576432420843
556557,556558,556557,1113115,3521.9187738895416,0.586124140132597
558559,558560,558559,1117119,3532.941642999649,0.5841041745170514
560561,560562,560561,1121123,3544.064374923706,0.5820976083541609
562563,562564,562563,1125127,3554.8622949123383,0.5801043077408394
564565,564566,564565,1129131,3564.4470448493958,0.5781241414933902
566567,566568,566567,1133135,3572.042683839798,0.5761569805854379
568569,568570,568569,1137139,3582.5840079784393,0.5742026978496142
570571,570572,570571,1141143,3593.5576848983765,0.5722611678866087
572573,572574,572573,1145147,3604.4027438163757,0.5703322669596673
574575,574576,574575,1149151,3615.5273637771606,0.5684158729618503
576577,576578,576577,1153155,3626.2027378082275,0.5665118653705576
578579,578580,578579,1157159,3634.974147796631,0.5646201252202445
580581,580582,580581,1161163,3641.5354340076447,0.562740535076955
582583,582584,582583,1165167,3648.0535349845886,0.5608729790055804
584585,584586,584585,1169171,3657.0430369377136,0.5590173425407556
586587,586588,586587,1173175,3666.3478269577026,0.557173512670488
588589,588590,588589,1177179,3674.1167368888855,0.5553413778106915
590591,590592,590591,1181183,3681.3372209072113,0.553520827774264
592593,592594,592593,1185187,3688.7228679656982,0.5517117537656304
594595,594596,594595,1189191,3695.3708579540253,0.5499140483298106
596597,596598,596597,1193195,3701.553076982498,0.5481276053633337
598599,598600,598599,1197199,3707.55463886261,0.5463523200705822
600601,600602,600601,1201203,3713.6492817401886,0.544588088952878
602603,602604,602603,1205207,3720.201534986496,0.5428348097848357
604605,604606,604605,1209211,3726.053242921829,0.5410923815961723
606607,606608,606607,1213215,3731.1867849826813,0.539360704655337
608609,608610,608609,1217219,3736.9457080364227,0.5376396804404067
610611,610612,610611,1221223,3743.1484208106995,0.5359292116336292
612613,612614,612613,1225227,3748.3595221042633,0.5342292020923196
614615,614616,614615,1229231,3754.0804460048676,0.5325395568379463
616617,616618,616617,1233235,3760.2432539463043,0.5308601820361218
618619,618620,618619,1237239,3767.4221358299255,0.5291909849784133
620621,620622,620621,1241243,3774.479855775833,0.5275318740659714
622623,622624,622623,1245247,3779.7799627780914,0.5258827587967971
624625,624626,624625,1249251,3785.6613528728485,0.5242435497402766
626627,626628,626627,1253255,3792.0845420360565,0.5226141585335426
628629,628630,628629,1257259,3798.340866804123,0.5209944978523708
630631,630632,630631,1261263,3804.2628648281097,0.5193844814075419
632633,632634,632633,1265267,3810.685384988785,0.5177840239211946
634635,634636,634635,1269271,3816.843044757843,0.5161930411195499
636637,636638,636637,1273275,3822.501832008362,0.514611449705626
638639,638640,638639,1277279,3827.8420050144196,0.5130391673665144
640641,640642,640641,1281283,3832.6859877109528,0.5114761127351812
642643,642644,642643,1285287,3837.6897218227386,0.5099222053922858
644645,644646,644645,1289291,3843.2958719730377,0.5083773658443533
646647,646648,646647,1293295,3848.598186969757,0.5068415155219554
648649,648650,648649,1297299,3853.8505368232727,0.5053145767469687
650651,650652,650651,1301303,3858.698084831238,0.5037964727362123
652653,652654,652653,1305307,3863.7135388851166,0.5022871275923535
654655,654656,654655,1309311,3869.2474088668823,0.5007864662638895
656657,656658,656657,1313315,3875.1999328136444,0.4992944145706133
658659,658660,658659,1317319,3881.073315858841,0.49781089916177734
660661,660662,660661,1321323,3887.456116914749,0.49633584751973103
662663,662664,662663,1325327,3893.6296210289,0.4948691879380931
664665,664666,664665,1329331,3899.438309907913,0.4934108495217515
666667,666668,666667,1333335,3906.207049846649,0.4919607621650357
668669,668670,668669,1337339,3913.0087287425995,0.49051885655353544
670671,670672,670671,1341343,3919.13432097435,0.4890850641295401
672673,672674,672673,1345347,3925.240109682083,0.48765931711386656
674675,674676,674675,1349351,3931.8753249645233,0.4862415484676603
676677,676678,676677,1353355,3937.8133749961853,0.4848316918942146
678679,678680,678679,1357359,3943.2455937862396,0.48342968182805635
680681,680682,680681,1361363,3948.995223760605,0.4820354534258513
682683,682684,682683,1365367,3954.1421320438385,0.4806489425518521
684685,684686,684685,1369371,3959.1747648715973,0.47927008577062225
686687,686688,686687,1373375,3963.844841003418,0.4778988203379413
688689,688690,688689,1377379,3968.5268239974976,0.4765350841989857
690691,690692,690691,1381383,3973.3278846740723,0.4751788159574062
692693,692694,692693,1385387,3978.614935874939,0.4738299548935174
694695,694696,694695,1389391,3983.558469772339,0.4724884409315564
696697,696698,696697,1393395,3988.5291221141815,0.47115421464877727
698699,698700,698699,1397399,3993.8383429050446,0.4698272172608995
700701,700702,700701,1401403,3998.907707929611,0.4685073906020989
702703,702704,702703,1405407,4003.955164909363,0.46719467713592167
704705,704706,704705,1409411,4009.4379110336304,0.46588901993527543
706707,706708,706707,1413415,4015.5749378204346,0.4645903626769723
708709,708710,708709,1417419,4021.614762067795,0.4632986496308149
710711,710712,710711,1421423,4028.330680847168,0.4620138256595965
712713,712714,712713,1425427,4034.325530767441,0.46073583620272984
714715,714716,714715,1429431,4040.505446910858,0.4594646272762475
716717,716718,716717,1433435,4046.3376269340515,0.45820014545461163
718719,718720,718719,1437439,4052.4025559425354,0.4569423378779902
720721,720722,720721,1441443,4058.796544075012,0.45569115222861
722723,722724,722723,1445447,4066.0419347286224,0.45444653674167057
724725,724726,724725,1449451,4072.074672937393,0.4532084401780594
726727,726728,726727,1453455,4078.134169816971,0.4519768118407228
728729,728730,728729,1457459,4084.5070950984955,0.4507516015419242
730731,730732,730731,1461463,4090.039997816086,0.4495327596214338
732733,732734,732733,1465467,4097.180171966553,0.44832023692106304
734735,734736,734735,1469471,4104.195430994034,0.44711398478648334
736737,736738,736737,1473475,4110.199882030487,0.44591395506176923
738739,738740,738739,1477479,4116.189069747925,0.4447201000784844
740741,740742,740741,1481483,4121.483787059784,0.4435323726538627
742743,742744,742743,1485487,4127.149904966354,0.4423507260835322
744745,744746,744745,1489491,4134.121069908142,0.44117511413787724
746747,746748,746747,1493495,4140.203313827515,0.44000549104202946
748749,748750,748749,1497499,4146.345674037933,0.4388418114904198
750751,750752,750751,1501503,4152.68705201149,0.4376840306358645
752753,752754,752753,1505507,4158.5335948467255,0.43653210406409926
754755,754756,754755,1509511,4164.172788858414,0.43538598781378823
756757,756758,756757,1513515,4169.73092675209,0.4342456383692479
758759,758760,758759,1517519,4175.036051988602,0.43311101262588636
760761,760762,760761,1521523,4180.482174873352,0.4319820679247641
762763,762764,762763,1525527,4185.853889703751,0.4308587620180333
764765,764766,764765,1529531,4191.072395086288,0.42974105308167054
766767,766768,766767,1533535,4196.578696012497,0.42862889969183016
768769,768770,768769,1537539,4202.032540798187,0.42752226083757705
770771,770772,770771,1541543,4207.483628034592,0.4264210958936019
772773,772774,772773,1545547,4213.024808883667,0.4253253646184021
774775,774776,774775,1549551,4219.182490825653,0.4242350271797477
776777,776778,776777,1553555,4226.657056093216,0.4231500441183016
778779,778780,778779,1557559,4232.362294912338,0.42207037636399036
780781,780782,780781,1561563,4237.35993885994,0.4209959852287284
782783,782784,782783,1565567,4242.128581762314,0.4199268323936849
784785,784786,784785,1569571,4247.405993938446,0.4188628799129219
786787,786788,786787,1573575,4253.0028438568115,0.41780409020248044
788789,788790,788789,1577579,4258.875963926315,0.41675042604219925
790791,790792,790791,1581583,4264.308646917343,0.4157018505666201
792793,792794,792793,1585587,4270.012740850449,0.4146583272595308
794795,794796,794795,1589591,4275.094332933426,0.41361981996124086
796797,796798,796797,1593595,4280.355321884155,0.4125862928431161
798799,798800,798799,1597599,4284.934052944183,0.41155771042758715
800801,800802,800801,1601603,4289.486024856567,0.4105340375663218
802803,802804,802803,1605607,4294.145545959473,0.40951523944022483
804805,804806,804805,1609611,4298.64532995224,0.4085012815630762
806807,806808,806807,1613615,4303.5122628211975,0.4074921297724359
808809,808810,808809,1617619,4308.115703821182,0.40648775021873007
810811,810812,810811,1621623,4312.738679885864,0.4054881093743461
812813,812814,812813,1625627,4318.657091856003,0.4044931740281754
814815,814816,814815,1629631,4323.645150899887,0.4035029112656048
816817,816818,816817,1633635,4328.781987905502,0.4025172884885251
818819,818820,818819,1637639,4333.698354005814,0.4015362733935035
820821,820822,820821,1641643,4338.880596876144,0.4005598339736025
822823,822824,822823,1645647,4344.440878868103,0.39958793852929375
824825,824826,824825,1649651,4349.821624755859,0.3986205556357163
826827,826828,826827,1653655,4354.698379993439,0.39765765416814247
828829,828830,828829,1657659,4359.818124771118,0.39669920328014996
830831,830832,830831,1661663,4364.365699768066,0.3957451724072598
832833,832834,832833,1665667,4369.40478181839,0.39479553126329847
834835,834836,834835,1669671,4374.282012939453,0.3938502498422167
836837,836838,836837,1673675,4379.809066057205,0.39290929839989985
838839,838840,838839,1677679,4384.809836864471,0.3919726474705385
840841,840842,840841,1681683,4390.680941820145,0.3910402678484388
842843,842844,842843,1685687,4395.737122774124,0.3901121305916604
844845,844846,844845,1689691,4400.957841873169,0.3891882070201973
846847,846848,846847,1693695,4406.166111946106,0.38826846870506415
848849,848850,848849,1697699,4410.715786933899,0.38735288748102903
850851,850852,850851,1701703,4415.242920875549,0.3864414354266046
852853,852854,852853,1705707,4419.828320980072,0.38553408486768603
854855,854856,854855,1709711,4424.637412786484,0.38463080837937014
856857,856858,856857,1713715,4429.2001140117645,0.38373157878231723
858859,858860,858859,1717719,4433.846656084061,0.3828363691300183
860861,860862,860861,1721723,4439.972784757614,0.3819451527160709
862863,862864,862863,1725727,4445.461322069168,0.38105852941771445
864865,864866,864865,1729731,4450.412357807159,0.3801764308936981
866867,866868,866867,1733735,4455.410667896271,0.3792982493778254
868869,868870,868869,1737739,4461.505923748016,0.37842395435836806
870871,870872,870871,1741743,4466.759452819824,0.3775535191907693
872873,872874,872873,1745747,4472.1079750061035,0.37668691810176824
874875,874876,874875,1749751,4477.80911898613,0.37582412579831725
876877,876878,876877,1753755,4482.8341319561005,0.37496511731842475
878879,878880,878879,1757759,4487.430838108063,0.37410986874419905
880881,880882,880881,1761763,4492.139890909195,0.3732583589753631
882883,882884,882883,1765767,4496.743131875992,0.37241056059792754
884885,884886,884885,1769771,4501.257176876068,0.3715664489845949
886887,886888,886887,1773775,4505.858793020248,0.3707260000792303
888889,888890,888889,1777779,4510.331367969513,0.36988919015493593
890891,890892,890891,1781783,4514.860918998718,0.36905599572855863
892893,892894,892893,1785787,4519.398862838745,0.36822639354431885
894895,894896,894895,1789791,4523.979068994522,0.3674003605628968
896897,896898,896897,1793795,4528.520212888718,0.36657787393414765
898899,898900,898899,1797799,4533.085356712341,0.3657589110225672
900901,900902,900901,1801803,4537.613943099976,0.36494344937455026
902903,902904,902903,1805807,4542.344341993332,0.36413146672566654
904905,904906,904905,1809811,4546.985957860947,0.3633229410115746
906907,906908,906907,1813815,4551.672353982925,0.3625178503425559
908909,908910,908909,1817819,4556.694780826569,0.3617161730180669
910911,910912,910911,1821823,4563.372940778732,0.36091788752310094
912913,912914,912913,1825827,4569.038534879684,0.3601229725063604
914915,914916,914915,1829831,4574.6852197647095,0.3593314068202744
916917,916918,916917,1833835,4580.95414185524,0.3585431694646104
918919,918920,918919,1837839,4586.19809794426,0.3577582396410435
920921,920922,920921,1841843,4591.294232845306,0.35697659669676796
922923,922924,922923,1845847,4596.954165935516,0.35619822017179104
924925,924926,924925,1849851,4602.492560863495,0.355423089764372
926927,926928,926927,1853855,4607.61025595665,0.3546511853401171
928929,928930,928929,1857859,4612.381989955902,0.35388248693197966
930931,930932,930931,1861863,4617.600532054901,0.3531169747348031
932933,932934,932933,1865867,4622.490839719772,0.35235462911077775
934935,934936,934935,1869871,4627.107048988342,0.3515954305712512
936937,936938,936937,1873875,4631.616614818573,0.35083935980037495
938939,938940,938939,1877879,4636.0397799015045,0.3500863976260007
940941,940942,940941,1881883,4640.693208694458,0.34933652504332713
942943,942944,942943,1885887,4645.204140663147,0.34858972319307213
944945,944946,944945,1889891,4649.620880842209,0.3478459733687487
946947,946948,946947,1893895,4654.76638007164,0.3471052570221218
948949,948950,948949,1897899,4659.889716863632,0.34636755574501876
950951,950952,950951,1901903,4664.326145648956,0.3456328512838809
952953,952954,952953,1905907,4669.112834692001,0.34490112552884966
954955,954956,954955,1909911,4675.287544727325,0.34417236051558575
956957,956958,956957,1913915,4681.316027879715,0.343446538419812
958959,958960,958959,1917919,4686.2646498680115,0.34272364156277035
960961,960962,960961,1921923,4691.537542819977,0.342003652405765
962963,962964,962963,1925927,4696.296371936798,0.34128655355016235
964965,964966,964965,1929931,4700.895061969757,0.3405723277337529
966967,966968,966967,1933935,4705.689305782318,0.33986095783075143
968969,968970,968969,1937939,4710.825269937515,0.33915242684997793
970971,970972,970971,1941943,4715.3773357868195,0.33844671793849557
972973,972974,972973,1945947,4719.931447029114,0.3377438143652398
974975,974976,974975,1949951,4724.482553720474,0.3370436995428463
976977,976978,976977,1953955,4729.054510831833,0.3363463570094609
978979,978980,978979,1957959,4733.677906990051,0.33565177042328287
980981,980982,980981,1961963,4738.34775185585,0.3349599235862115
982983,982984,982983,1965967,4742.955549001694,0.3342708004111046
984985,984986,984985,1969971,4747.568529844284,0.33358438494542497
986987,986988,986987,1973975,4752.112090826035,0.33290066135305096
988989,988990,988989,1977979,4756.658801794052,0.33221961393064703
990991,990992,990991,1981983,4761.270407915115,0.331541227084017
992993,992994,992993,1985987,4765.886277914047,0.330865485346294
994995,994996,994995,1989991,4770.433772087097,0.3301923733706644
996997,996998,996997,1993995,4774.9511387348175,0.329521875921273
998999,999000,998999,1997999,4779.627534866333,0.3288539778877748
1001001,1001002,1001001,2002003,4784.221988916397,0.3281886642653262
1003003,1003004,1003003,2006007,4788.768249750137,0.3275259201764129
1005005,1005006,1005005,2010011,4793.354526042938,0.32686573084720294
1007007,1007008,1007007,2014015,4797.92226099968,0.3262080816184607
1009009,1009010,1009009,2018019,4802.52365899086,0.32555295794009
1011011,1011012,1011011,2022023,4807.055500745773,0.3249003453802288
1013013,1013014,1013013,2026027,4811.63431596756,0.32425022960524075
1015015,1015016,1015015,2030031,4816.191326856613,0.32360259640336153
1017017,1017018,1017017,2034035,4820.73074388504,0.32295743165195745
1019019,1019020,1019019,2038039,4825.303936004639,0.32231472135026706
1021021,1021022,1021021,2042043,4829.807498931885,0.32167445159757335
1023023,1023024,1023023,2046047,4834.363724708557,0.3210366085950227
1025025,1025026,1025025,2050051,4838.909561872482,0.3204011786474439
1027027,1027028,1027027,2054055,4843.4537088871,0.3197681481633481
1029029,1029030,1029029,2058059,4847.97435092926,0.3191375036549289
1031031,1031032,1031031,2062063,4852.530962944031,0.3185092317289673
1033033,1033034,1033033,2066067,4857.181500911713,0.3178833190959267
1035035,1035036,1035035,2070071,4862.260901927948,0.317259752564496
1037037,1037038,1037037,2074075,4867.09419798851,0.31663851903977047
1039039,1039040,1039039,2078079,4871.778208971024,0.3160196055214328
1041041,1041042,1041041,2082083,4876.48356795311,0.3154029991110292
1043043,1043044,1043043,2086087,4881.64897108078,0.31478868699741724
1045045,1045046,1045045,2090091,4886.412800073624,0.314176656471318
1047047,1047048,1047047,2094095,4891.264453887939,0.31356689491076395
1049049,1049050,1049049,2098099,4896.417747974396,0.31295938978655613
1051051,1051052,1051051,2102103,4901.729318857193,0.31235412866772094
1053053,1053054,1053053,2106107,4906.6482989788055,0.31175109920150135
1055055,1055056,1055055,2110111,4912.025633096695,0.3111502891388227
1057057,1057058,1057057,2114115,4917.264209985733,0.3105516863124649
1059059,1059060,1059059,2118119,4922.56670498848,0.3099552786370623
1061061,1061062,1061061,2122123,4927.632023096085,0.3093610541327507
1063063,1063064,1063063,2126127,4932.736760854721,0.30876900088878756
1065065,1065066,1065065,2130131,4937.935338020325,0.30817910708537966
1067067,1067068,1067067,2134135,4943.164881944656,0.30759136099186435
1069069,1069070,1069069,2138139,4947.923549890518,0.3070057509594335
1071071,1071072,1071071,2142143,4952.480514764786,0.3064222654229525
1073073,1073074,1073073,2146147,4957.173677682877,0.30584089290096017
1075075,1075076,1075075,2150151,4961.701231956482,0.305261621988393
1077077,1077078,1077077,2154155,4966.293132066727,0.30468444136931794
1079079,1079080,1079079,2158159,4971.234192848206,0.3041093398078374
1081081,1081082,1081081,2162163,4975.964017868042,0.3035363061426324
1083083,1083084,1083083,2166167,4980.6173787117,0.3029653292942385
1085085,1085086,1085085,2170171,4985.141084909439,0.30239639826322673
1087087,1087088,1087087,2174175,4989.659781932831,0.3018295021265658
1089089,1089090,1089089,2178179,4994.3680419921875,0.3012646300394408
1091091,1091092,1091091,2182183,4998.955102920532,0.3007017712297966
1093093,1093094,1093093,2186187,5003.597646713257,0.30014091500743234
1095095,1095096,1095095,2190191,5008.241469860077,0.299582050751269
1097097,1097098,1097097,2194195,5013.090375900269,0.2990251679184439
1099099,1099100,1099099,2198199,5017.966705799103,0.2984702560406731
1101101,1101102,1101101,2202203,5022.799950838089,0.2979173047206132
1103103,1103104,1103103,2206207,5027.627104997635,0.29736630363186123
1105105,1105106,1105105,2210211,5033.2843408584595,0.296817242524412
1107107,1107108,1107107,2214215,5039.418381690979,0.2962701112155628
1109109,1109110,1109109,2218219,5045.356537818909,0.2957248995971895
1111111,1111112,1111111,2222223,5051.8577709198,0.2951815976284706
1113113,1113114,1113113,2226227,5058.337679862976,0.29464019533952523
1115115,1115116,1115115,2230231,5064.143140792847,0.29410068282231805
1117117,1117118,1117117,2234235,5068.66331076622,0.2935630502488493
1119119,1119120,1119119,2238239,5073.323064804077,0.29302728785296495
1121121,1121122,1121121,2242243,5078.792990922928,0.2924933859358134
1123123,1123124,1123123,2246247,5083.628935813904,0.29196133486402687
1125125,1125126,1125125,2250251,5088.68439078331,0.291431125073359
1127127,1127128,1127127,2254255,5093.7575969696045,0.2909027470595902
1129129,1129130,1129129,2258259,5098.669502019882,0.2903761913894414
1131131,1131132,1131131,2262263,5103.360232830048,0.2898514486896602
1133133,1133134,1133133,2266267,5108.4453728199005,0.2893285096524778
1135135,1135136,1135135,2270271,5113.471379995346,0.2888073650337901
1137137,1137138,1137137,2274275,5118.075543880463,0.2882880056531576
1139139,1139140,1139139,2278279,5122.614551782608,0.2877704223883484
1141141,1141142,1141141,2282283,5127.2440440654755,0.28725460618079524
1143143,1143144,1143143,2286287,5131.789764881134,0.28674054803559557
1145145,1145146,1145145,2290291,5136.343441963196,0.28622823901605443
1147147,1147148,1147147,2294295,5140.921498775482,0.28571767024550354
1149149,1149150,1149149,2298299,5146.244611740112,0.28520883290548227
1151151,1151152,1151151,2302303,5152.02401471138,0.2847017182393756
1153153,1153154,1153153,2306307,5156.928164720535,0.2841963175469573
1155155,1155156,1155155,2310311,5162.495882034302,0.28369262219348457
1157157,1157158,1157157,2314315,5166.982992887497,0.2831906235842325
1159159,1159160,1159159,2318319,5171.416391849518,0.28269031320633076
1161161,1161162,1161161,2322323,5175.825987815857,0.28219168257965066
1163163,1163164,1163163,2326327,5180.395891904831,0.2816947232968232
1165165,1165166,1165165,2330331,5184.838183879852,0.2811994269959541
1167167,1167168,1167167,2334335,5189.243308067322,0.28070578537881374
1169169,1169170,1169169,2338339,5193.788635969162,0.2802137901999231
1171171,1171172,1171171,2342343,5198.275225877762,0.27972343326291593
1173173,1173174,1173173,2346347,5202.702685832977,0.2792347064259957
1175175,1175176,1175175,2350351,5207.331475973129,0.2787476016092114
1177177,1177178,1177177,2354355,5211.832864046097,0.27826211077808694
1179179,1179180,1179179,2358359,5216.293675899506,0.27777822595089674
1181181,1181182,1181181,2362363,5220.781254768372,0.277295939204123
1183183,1183184,1183183,2366367,5225.370840787888,0.27681524265972257
1185185,1185186,1185185,2370371,5229.8007118701935,0.2763361284924031
1187187,1187188,1187187,2374375,5234.2492599487305,0.27585858893326076
1189189,1189190,1189189,2378379,5238.7202298641205,0.27538261625522864
1191191,1191192,1191191,2382383,5243.0998730659485,0.27490820278217143
1193193,1193194,1193193,2386387,5247.610431909561,0.2744353408997995
1195195,1195196,1195195,2390391,5252.03733587265,0.27396402303020295
1197197,1197198,1197197,2394395,5256.432172775269,0.2734942416464037
1199199,1199200,1199199,2398399,5260.873626947403,0.2730259892759932
1201201,1201202,1201201,2402403,5265.2876517772675,0.2725592584883998
1203203,1203204,1203203,2406407,5269.67730307579,0.27209404190580244
1205205,1205206,1205205,2410411,5274.176853895187,0.2716303321922169
1207207,1207208,1207207,2414415,5278.613901853561,0.27116812206440954
1209209,1209210,1209209,2418419,5283.018865823746,0.2707074042809836
1211211,1211212,1211211,2422423,5287.394817113876,0.270248171649655
1213213,1213214,1213213,2426427,5292.341337919235,0.2697904170236143
1215215,1215216,1215215,2430431,5297.856072902679,0.2693341333015269
1217217,1217218,1217217,2434435,5303.989568948746,0.2688793134275329
1219219,1219220,1219219,2438439,5308.90336894989,0.2684259503876092
1221221,1221222,1221221,2442443,5314.444131851196,0.2679740372168453
1223223,1223224,1223223,2446447,5320.235439777374,0.2675235669921676
1225225,1225226,1225225,2450451,5325.988439083099,0.2670745328323392
1227227,1227228,1227227,2454455,5331.5082218647,0.2666269279034168
1229229,1229230,1229229,2458459,5336.723392963409,0.2661807454114751
1231231,1231232,1231231,2462463,5342.065901756287,0.2657359786098823
1233233,1233234,1233233,2466467,5348.554561853409,0.2652926207847486
1235235,1235236,1235235,2470471,5354.512899875641,0.2648506652767537
1237237,1237238,1237237,2474475,5359.764008998871,0.2644101054593193
1239239,1239240,1239239,2478479,5364.842181921005,0.26397093474588473
1241241,1241242,1241241,2482483,5370.059077978134,0.26353314660264004
1243243,1243244,1243243,2486487,5375.3752319812775,0.26309673452669813
1245245,1245246,1245245,2490491,5380.8680629730225,0.2626616920588276
1247247,1247248,1247247,2494495,5385.982218027115,0.26222801277253893
1249249,1249250,1249249,2498499,5390.602140903473,0.2617956902977312
1251251,1251252,1251251,2502503,5395.1891458034515,0.2613647182861314
1253253,1253254,1253253,2506507,5399.901926994324,0.2609350904440362
1255255,1255256,1255255,2510511,5405.548369884491,0.2605068004995701
1257257,1257258,1257257,2514515,5411.069795846939,0.26007984223906533
1259259,1259260,1259259,2518519,5416.668910741806,0.25965420947250095
1261261,1261262,1261261,2522523,5421.210109949112,0.2592298960498738
1263263,1263264,1263263,2526527,5426.370733737946,0.2588068958666554
1265265,1265266,1265265,2530531,5432.042713880539,0.2583852028456022
1267267,1267268,1267267,2534535,5437.793962955475,0.25796481095858326
1269269,1269270,1269269,2538539,5443.2271847724915,0.2575457142029336
1271271,1271272,1271271,2542543,5448.116353034973,0.2571279066178249
1273273,1273274,1273273,2546547,5452.830889940262,0.25671138228062773
1275275,1275276,1275275,2550551,5458.39186000824,0.25629613530145434
1277277,1277278,1277277,2554555,5464.297344923019,0.25588215982497786
1279279,1279280,1279279,2558559,5469.749102830887,0.25546945003588917
1281281,1281282,1281281,2562563,5475.112411975861,0.25505800015343993
1283283,1283284,1283283,2566567,5480.1780071258545,0.2546478044241667
1285285,1285286,1285285,2570571,5485.53879404068,0.25423885714371863
1287287,1287288,1287287,2574575,5490.779470920563,0.2538311526295729
1289289,1289290,1289289,2578579,5496.53626704216,0.25342468523922435
1291291,1291292,1291291,2582583,5501.119783878326,0.2530194493592717
1293293,1293294,1293293,2586587,5505.680660009384,0.25261543941451237
1295295,1295296,1295295,2590591,5510.27424788475,0.2522126498679427
1297297,1297298,1297297,2594595,5514.92941904068,0.2518110752043867
1299299,1299300,1299299,2598599,5519.602097988129,0.2514107099486864
1301301,1301302,1301301,2602603,5525.052471876144,0.25101154865660646
1303303,1303304,1303303,2606607,5530.554458856583,0.25061358592029137
1305305,1305306,1305305,2610611,5535.964621782303,0.2502168163518945
1307307,1307308,1307307,2614615,5542.371006011963,0.24982123461268202
1309309,1309310,1309309,2618619,5548.2586669921875,0.24942683538574784
1311311,1311312,1311311,2622623,5554.1238489151,0.24903361338692775
1313313,1313314,1313313,2626627,5559.052188873291,0.2486415633593424
1315315,1315316,1315315,2630631,5564.188989877701,0.24825068008431117
1317317,1317318,1317317,2634635,5569.606400966644,0.2478609583740763
1319319,1319320,1319319,2638639,5575.4299829006195,0.24747239306452684
1321321,1321322,1321321,2642643,5580.566390037537,0.2470849790279317
1323323,1323324,1323323,2646647,5586.241718053818,0.24669871116384456
1325325,1325326,1325325,2650651,5590.833034038544,0.24631358440274198
1327327,1327328,1327327,2654655,5595.787615060806,0.2459295937060233
1329329,1329330,1329329,2658659,5600.623514890671,0.2455467340623727
1331331,1331332,1331331,2662663,5605.950741052628,0.24516500048775924
1333333,1333334,1333333,2666667,5610.827143907547,0.2447843880381697
1335335,1335336,1335335,2670671,5615.685125827789,0.24440489178232383
1337337,1337338,1337337,2674675,5620.3902468681335,0.2440265068271401
1339339,1339340,1339339,2678679,5624.967035770416,0.24364922831045988
1341341,1341342,1341341,2682683,5629.560567855835,0.2432730513937713
1343343,1343344,1343343,2686687,5634.488076686859,0.24289797126402846
1345345,1345346,1345345,2690691,5639.639261960983,0.24252398314274615
1347347,1347348,1347347,2694695,5644.757818937302,0.2421510822732671
1349349,1349350,1349349,2698699,5649.486265897751,0.24177926392803784
1351351,1351352,1351351,2702703,5654.058301925659,0.24140852341224672
1353353,1353354,1353353,2706707,5659.435300827026,0.241038856049272
1355355,1355356,1355355,2710711,5664.890222787857,0.24067025719523372
1357357,1357358,1357357,2714715,5670.067280769348,0.2403027222280798
1359359,1359360,1359359,2718719,5674.716387748718,0.23993624656031898
1361361,1361362,1361361,2722723,5679.299602985382,0.23957082562264986
1363363,1363364,1363363,2726727,5683.9174427986145,0.2392064548748749
1365365,1365366,1365365,2730731,5688.498087882996,0.2388431298059004
1367367,1367368,1367367,2734735,5693.517944812775,0.23848084592464147
1369369,1369370,1369369,2738739,5698.4071209430695,0.23811959876729816
1371371,1371372,1371371,2742743,5703.138248920441,0.23775938389917428
1373373,1373374,1373373,2746747,5707.770149946213,0.23740019690376357
1375375,1375376,1375375,2750751,5712.396089792252,0.23704203339912056
1377377,1377378,1377377,2754755,5716.949668884277,0.23668488902148965
1379379,1379380,1379379,2758759,5721.529042959213,0.23632875942894316
1381381,1381382,1381381,2762763,5726.103996992111,0.23597364031411416
1383383,1383384,1383383,2766767,5730.792006969452,0.23561952738418768
1385385,1385386,1385385,2770771,5735.483191013336,0.23526641637363355
1387387,1387388,1387387,2774775,5740.106241703033,0.23491430304602545
1389389,1389390,1389389,2778779,5745.107842683792,0.23456318318130798
1391391,1391392,1391391,2782783,5750.598644018173,0.23421305258489156
1393393,1393394,1393393,2786787,5756.120817899704,0.23386390940868296
1395395,1395396,1395395,2790791,5762.277685880661,0.23351578891742975
1397397,1397398,1397397,2794795,5768.080096960068,0.2331686487668776
1399399,1399400,1399399,2798799,5774.113744974136,0.23282248175928544
1401401,1401402,1401401,2802803,5779.2142589092255,0.23247728362730413
1403403,1403404,1403403,2806807,5785.013068675995,0.2321330502636556
1405405,1405406,1405405,2810811,5790.609031915665,0.2317897776101745
1407407,1407408,1407407,2814815,5796.261479854584,0.23144746163779928
1409409,1409410,1409409,2818819,5802.047855854034,0.2311060983556672
1411411,1411412,1411411,2822823,5808.544107913971,0.2307656837929244
1413413,1413414,1413413,2826827,5814.755990028381,0.23042621400054486
1415415,1415416,1415415,2830831,5820.644172668457,0.23008768505860644
1417417,1417418,1417417,2834835,5826.975443840027,0.22975009306173888
1419419,1419420,1419419,2838839,5833.2618889808655,0.2294134341282188
1421421,1421422,1421421,2842843,5839.591372013092,0.22907770440360764
1423423,1423424,1423423,2846847,5846.025762796402,0.2287429000461998
1425425,1425426,1425425,2850851,5852.751660823822,0.22840901724521245
1427427,1427428,1427427,2854855,5858.934088945389,0.22807605220077676
1429429,1429430,1429429,2858859,5864.3177399635315,0.22774400114030868
1431431,1431432,1431431,2862863,5868.975678920746,0.2274128603094141
1433433,1433434,1433433,2866867,5874.006974935532,0.22708262597734574
1435435,1435436,1435435,2870871,5879.046786785126,0.22675329442790826
1437437,1437438,1437437,2874875,5885.342272043228,0.22642486197037215
1439439,1439440,1439439,2878879,5891.342223882675,0.2260973249340168
1441441,1441442,1441441,2882883,5897.284862041473,0.2257706796608545
1443443,1443444,1443443,2886887,5903.725106954575,0.22544492252200143
1445445,1445446,1445445,2890891,5908.689918041229,0.2251200499049446
1447447,1447448,1447447,2894895,5913.858527898788,0.22479605821354198
1449449,1449450,1449449,2898899,5918.988556861877,0.22447294387529837
1451451,1451452,1451451,2902903,5923.750787734985,0.22415070333408948
1453453,1453454,1453453,2906907,5928.554456710815,0.22382933305561892
1455455,1455456,1455455,2910911,5933.597282886505,0.22350882952014217
1457457,1457458,1457457,2914915,5938.735731840134,0.2231891892333806
1459459,1459460,1459459,2918919,5943.839911937714,0.2228704087137885
1461461,1461462,1461461,2922923,5949.7272210121155,0.222552484501648
1463463,1463464,1463463,2926927,5955.243183851242,0.22223541315361217
1465465,1465466,1465465,2930931,5961.148135900497,0.22191919124634296
1467467,1467468,1467467,2934935,5965.766874790192,0.22160381537833018
1469469,1469470,1469469,2938939,5970.735469818115,0.2212892821571586
1471471,1471472,1471471,2942943,5975.203907728195,0.22097558821405983
1473473,1473474,1473473,2946947,5979.687976837158,0.22066273020391236
1475475,1475476,1475475,2950951,5984.198615074158,0.22035070478523267
1477477,1477478,1477477,2954955,5989.016486883163,0.22003950864200306
1479479,1479480,1479479,2958959,5993.7781410217285,0.2197291384836717
1481481,1481482,1481481,2962963,5998.8136649131775,0.21941959102150577
1483483,1483484,1483483,2966967,6003.347090005875,0.21911086299769522
1485485,1485486,1485485,2970971,6007.939852714539,0.218802951161706
1487487,1487488,1487487,2974975,6013.395589828491,0.21849585228483193
1489489,1489490,1489489,2978979,6018.788200855255,0.21818956316019467
1491491,1491492,1491491,2982983,6023.925347805023,0.21788408058455389
1493493,1493494,1493493,2986987,6028.496406078339,0.21757940138195409
1495495,1495496,1495495,2990991,6033.377789974213,0.21727552239099168
1497497,1497498,1497497,2994995,6038.375821828842,0.216972440466634
1499499,1499500,1499499,2998999,6043.004897117615,0.21667015247840027
1501502,1501503,1501502,3003005,6047.592898845673,0.21636850491449877
1503504,1503505,1503504,3007009,6052.111756801605,0.21606779587091296
1505506,1505507,1505506,3011013,6057.069021940231,0.21576787147387222
1507508,1507509,1507508,3015017,6061.772212028503,0.2154687286601984
1509510,1509511,1509510,3019021,6066.331017971039,0.21517036437580828
1511512,1511513,1511512,3023025,6070.972116947174,0.2148727755939035
1513514,1513515,1513514,3027029,6076.17863202095,0.21457595929678064
1515516,1515517,1515516,3031033,6081.014851808548,0.21427991247765021
1517518,1517519,1517518,3035037,6085.804709911346,0.21398463215700758
1519520,1519521,1519520,3039041,6091.129111766815,0.21369011536444305
1521522,1521523,1521522,3043045,6096.239576816559,0.21339635913864186
1523524,1523525,1523524,3047049,6100.849698066711,0.21310336054375512
1525526,1525527,1525526,3051053,6105.727855920792,0.21281115536476136
1527528,1527529,1527528,3055057,6110.339494943619,0.21251973512516997
1529530,1529531,1529530,3059061,6114.8319680690765,0.21222907061383012
1531532,1531533,1531532,3063065,6119.85812997818,0.21193915371441108
1533534,1533535,1533534,3067069,6124.245937824249,0.21164998025415116
1535536,1535537,1535536,3071073,6128.7326118946075,0.21136154704072396
1537538,1537539,1537538,3075077,6133.24310874939,0.21107385115828947
1539540,1539541,1539540,3079081,6137.69180393219,0.2107868897546723
1541542,1541543,1541542,3083085,6142.107456922531,0.21050066002135281
1543544,1543545,1543544,3087089,6146.592581748962,0.21021515916436329
1545546,1545547,1545546,3091093,6151.070791959763,0.20993038440064993
1547548,1547549,1547548,3095097,6155.4467878341675,0.20964633297080582
1549550,1549551,1549550,3099101,6159.822592020035,0.209363002119062
1551552,1551553,1551552,3103105,6164.205864906311,0.20908038911693438
1553554,1553555,1553554,3107109,6168.862958908081,0.20879849123593885
1555556,1555557,1555556,3111113,6173.361418008804,0.20851730576941918
1557558,1557559,1557558,3115117,6177.808700799942,0.20823683002163307
1559560,1559561,1559560,3119121,6182.455990076065,0.20795706131139013
1561562,1561563,1561562,3123125,6186.936721801758,0.2076779969738709
1563564,1563565,1563564,3127129,6191.332417726517,0.20739963435335085
1565566,1565567,1565566,3131133,6195.7386469841,0.20712197080501937
1567568,1567569,1567568,3135137,6200.1335299015045,0.20684500370771275
1569570,1569571,1569570,3139141,6204.512003898621,0.20656873044026725
1571572,1571573,1571572,3143145,6208.9010617733,0.206293148405166
1573574,1573575,1573574,3147149,6213.3188490867615,0.20601825501216808
1575576,1575577,1575576,3151153,6217.705935955048,0.20574404768558452
1577578,1577579,1577578,3155157,6222.331023931503,0.20547052386245923
1579580,1579581,1579580,3159161,6226.708256959915,0.20519768099620705
1581582,1581583,1581582,3163165,6231.146019697189,0.2049255165438808
1583584,1583585,1583584,3167169,6235.574204921722,0.20465402798254217
1585586,1585587,1585586,3171173,6239.933876991272,0.2043832128001668
1587588,1587589,1587588,3175177,6244.352187871933,0.20411306849928224
1589590,1589591,1589590,3179181,6248.733810901642,0.203843592587873
1591592,1591593,1591592,3183185,6253.133549690247,0.20357478259211348
1593594,1593595,1593594,3187189,6257.593024015427,0.20330663605273003
1595596,1595597,1595596,3191193,6262.067286968231,0.20303915051226795
1597598,1597599,1597598,3195197,6266.4606828689575,0.20277232353691943
1599600,1599601,1599600,3199201,6270.8758227825165,0.2025061526983336
1601602,1601603,1601602,3203205,6275.241010904312,0.20224063557907357
1603604,1603605,1603604,3207209,6279.663468837738,0.20197576978171128
1605606,1605607,1605606,3211213,6284.081244945526,0.2017115529069997
1607608,1607609,1607608,3215217,6288.57399892807,0.2014479825811577
1609610,1609611,1609610,3219221,6292.966054916382,0.20118505643404205
1611612,1611613,1611612,3223225,6297.413215875626,0.2009227721100615
1613614,1613615,1613614,3227229,6301.828366756439,0.20066112726271967
1615616,1615617,1615616,3231233,6306.264003753662,0.2004001195582532
1617618,1617619,1617618,3235237,6310.661834001541,0.2001397466756316
1619620,1619621,1619620,3239241,6315.059362888336,0.19988000630473834
1621622,1621623,1621622,3243245,6319.500789880753,0.1996208961445518
1623624,1623625,1623624,3247249,6324.011469841003,0.19936241390314535
1625626,1625627,1625626,3251253,6328.446273088455,0.19910455730678223
1627628,1627629,1627628,3255257,6332.841107845306,0.19884732408718264
1629630,1629631,1629630,3259261,6337.235272884369,0.19859071199061873
1631632,1631633,1631632,3263265,6341.6473977565765,0.19833471877245756
1633634,1633635,1633634,3267269,6346.0207459926605,0.19807934219534218
1635636,1635637,1635636,3271273,6350.467463970184,0.19782458003646752
1637638,1637639,1637638,3275277,6354.8812890052795,0.19757043008758046
1639640,1639641,1639640,3279281,6359.302092075348,0.19731689014042786
1641642,1641643,1641642,3283285,6363.774348020554,0.19706395801222243
1643644,1643645,1643644,3287289,6368.186816930771,0.19681163151290093
1645646,1645647,1645646,3291293,6372.549284934998,0.19655990847786597
1647648,1647649,1647648,3295297,6376.951040029526,0.19630878674070118
1649650,1649651,1649650,3299301,6381.328193664551,0.19605826415863703
1651652,1651653,1651652,3303305,6385.712616920471,0.195808338590723
1653654,1653655,1653654,3307309,6390.135596036911,0.1955590079032845
1655656,1655657,1655656,3311313,6394.503906011581,0.19531026998265588
1657658,1657659,1657658,3315317,6398.900309085846,0.19506212271517143
1659660,1659661,1659660,3319321,6403.319543838501,0.19481456400171737
1661662,1661663,1661662,3323325,6407.85279583931,0.19456759175591287
1663664,1663665,1663664,3327329,6412.520545005798,0.19432120389683405
1665666,1665667,1665666,3331333,6417.124979019165,0.19407539835447096
1667668,1667669,1667668,3335337,6421.532407045364,0.1938301730715466
1669670,1669671,1669670,3339341,6425.928443908691,0.19358552599260292
1671672,1671673,1671672,3343345,6431.476413011551,0.1933414550821908
1673674,1673675,1673674,3347349,6436.547544717789,0.19309795830849907
1675676,1675677,1675676,3351353,6442.4235298633575,0.1928550336506305
1677678,1677679,1677678,3355357,6447.5134489536285,0.19261267909314483
1679680,1679681,1679680,3359361,6452.6167278289795,0.1923708926369727
1681682,1681683,1681682,3363365,6457.50807094574,0.19212967228850175
1683684,1683685,1683684,3367369,6462.4428169727325,0.1918890160632145
1685686,1685687,1685686,3371373,6467.304271936417,0.1916489219856885
1687688,1687689,1687688,3375377,6472.15213394165,0.19140938809505315
1689690,1689691,1689690,3379381,6478.3225219249725,0.19117041243043786
1691692,1691693,1691692,3383385,6484.694344997406,0.19093199304916197
1693694,1693695,1693694,3387389,6490.671014785767,0.1906941280085448
1695696,1695697,1695696,3391393,6496.091022729874,0.19045681538591452
1697698,1697699,1697698,3395397,6502.0760707855225,0.19022006432714988
1699700,1699701,1699700,3399401,6507.209232807159,0.18998387071223988
1701702,1701703,1701702,3403405,6512.601669788361,0.1897482247932203
1703704,1703705,1703704,3407409,6517.470152854919,0.18951312386889185
1705706,1705707,1705706,3411413,6522.207150936127,0.1892785659583751
1707708,1707709,1707708,3415417,6528.179767131805,0.18904454916992108
1709710,1709711,1709710,3419421,6533.5065269470215,0.18881107163724664
1711712,1711713,1711712,3423425,6538.619865894318,0.18857813149406866
1713714,1713715,1713714,3427429,6543.604341030121,0.18834572689411289
1715716,1715717,1715716,3431433,6548.598554849625,0.18811385599292407
1717718,1717719,1717718,3435437,6553.379396915436,0.18788251696059888
1719720,1719721,1719720,3439441,6558.547029018402,0.18765170796541497
1721722,1721723,1721722,3443445,6563.175659894943,0.1874214271974779
1723724,1723725,1723724,3447449,6567.8244659900665,0.18719167284325522
1725726,1725727,1725726,3451453,6572.363568782806,0.18696244310376642
1727728,1727729,1727728,3455457,6577.03283572197,0.18673373618912592
1729730,1729731,1729730,3459461,6581.619139909744,0.18650555031490512
1731732,1731733,1731732,3463465,6586.059822797775,0.18627788370395137
1733734,1733735,1733734,3467469,6591.695126056671,0.186050734586388
1735736,1735737,1735736,3471473,6597.147672891617,0.18582410120870918
1737738,1737739,1737738,3475477,6601.540307998657,0.1855979818119522
1739740,1739741,1739740,3479481,6605.95348572731,0.18537237466080114
1741742,1741743,1741742,3483485,6610.377541780472,0.18514727801266417
1743744,1743745,1743744,3487489,6615.01743888855,0.18492269014132034
1745746,1745747,1745746,3491493,6619.6053059101105,0.18469860932964366
1747748,1747749,1747748,3495497,6624.072289943695,0.18447503385868913
1749750,1749751,1749750,3499501,6628.444972038269,0.18425196203133964
1751752,1751753,1751752,3503505,6632.907791852951,0.1840293921468401
1753754,1753755,1753754,3507509,6637.503868818283,0.18380732251534937
1755756,1755757,1755756,3511513,6642.10107088089,0.18358575145612122
1757758,1757759,1757758,3515517,6646.578812837601,0.1833646772938664
1759760,1759761,1759760,3519521,6651.060322761536,0.18314409836239065
1761762,1761763,1761762,3523525,6655.505933761597,0.1829240130027756
1763764,1763765,1763764,3527529,6659.980808019638,0.1827044195633789
1765766,1765767,1765766,3531533,6664.448819875717,0.18248531639983412
1767768,1767769,1767768,3535537,6668.859917879105,0.1822667018732318
1769770,1769771,1769770,3539541,6673.23977971077,0.18204857435557642
1771772,1771773,1771772,3543545,6677.635067939758,0.18183093222432944
1773774,1773775,1773774,3547549,6682.004834890366,0.1816137738624093
1775776,1775777,1775776,3551553,6686.4007749557495,0.18139709766182932
1777778,1777779,1777778,3555557,6690.792168855667,0.18118090202369785
1779780,1779781,1779780,3559561,6695.18464589119,0.1809651853509422
1781782,1781783,1781782,3563565,6699.752811908722,0.18074994605922257
1783784,1783785,1783784,3567569,6704.285532951355,0.18053518256783718
1785786,1785787,1785786,3571573,6708.711842060089,0.1803208933051792
1787788,1787789,1787788,3575577,6713.136353969574,0.18010707669964177
1789790,1789791,1789790,3579581,6717.7407858371735,0.17989373120144592
1791792,1791793,1791792,3583585,6722.137866020203,0.17968085524989874
1793794,1793795,1793794,3587589,6726.572706699371,0.17946844730431621
1795796,1795797,1795796,3591593,6730.949846982956,0.17925650582219532
1797798,1797799,1797798,3595597,6735.328789949417,0.17904502927376598
1799800,1799801,1799800,3599601,6739.759479045868,0.17883401613835304
1801802,1801803,1801802,3603605,6744.1750910282135,0.1786234648898244
1803804,1803805,1803804,3607609,6748.515212059021,0.17841337402205681
1805806,1805807,1805806,3611613,6752.941475868225,0.1782037420252891
1807808,1807809,1807808,3615617,6757.328505754471,0.17799456740794994
1809810,1809811,1809810,3619621,6761.726157903671,0.1777858486675541
1811812,1811813,1811812,3623625,6766.087419986725,0.17757758432890114
1813814,1813815,1813814,3627629,6770.455399990082,0.17736977290405775
1815816,1815817,1815816,3631633,6774.878770828247,0.17716241292691848
1817818,1817819,1817818,3635637,6779.295504808426,0.17695550292773987
1819820,1819821,1819820,3639641,6783.671586751938,0.17674904144587344
1821822,1821823,1821822,3643645,6788.083201885223,0.17654302703158464
1823824,1823825,1823824,3647649,6792.514917850494,0.1763374582351389
1825826,1825827,1825826,3651653,6796.891375780106,0.17613233361225866
1827828,1827829,1827828,3655657,6801.241739988327,0.17592765173503722
1829830,1829831,1829830,3659661,6805.62225985527,0.17572341117011092
1831832,1831833,1831832,3663665,6809.991852045059,0.17551961049321108
1833834,1833835,1833834,3667669,6814.360536813736,0.1753162482909829
1835836,1835837,1835836,3671673,6818.762189865112,0.17511332315552863
1837838,1837839,1837838,3675677,6823.232143878937,0.17491083367713145
1839840,1839841,1839840,3679681,6827.644805908203,0.17470877846244548
1841842,1841843,1841842,3683685,6832.124967813492,0.17450715611448686
1843844,1843845,1843844,3687689,6837.024589776993,0.17430596525082365
1845846,1845847,1845846,3691693,6841.598299980164,0.1741052044890239
1847848,1847849,1847848,3695697,6846.078585863113,0.1739048724539316
1849850,1849851,1849850,3699701,6851.3495218753815,0.17370496777948574
1851852,1851853,1851852,3703705,6855.984461784363,0.17350548910144425
1853854,1853855,1853854,3707709,6860.851053714752,0.17330643506466004
1855856,1855857,1855856,3711713,6866.131582021713,0.17310780431580497
1857858,1857859,1857858,3715717,6871.142914772034,0.1729095955070079
1859860,1859861,1859860,3719721,6875.792916059494,0.17271180730494962
1861862,1861863,1861862,3723725,6880.874497652054,0.1725144383708539
1863864,1863865,1863864,3727729,6886.673879861832,0.17231748737685848
1865866,1865867,1865866,3731733,6891.133558034897,0.17212095300055807
1867868,1867869,1867868,3735737,6895.530143022537,0.17192483392682334
1869870,1869871,1869870,3739741,6900.00271987915,0.17172912884052494
1871872,1871873,1871872,3743745,6904.40402674675,0.17153383643926645
1873874,1873875,1873874,3747749,6908.8742089271545,0.17133895541883248
1875876,1875877,1875876,3751753,6913.285845041275,0.17114448448592157
1877878,1877879,1877878,3755757,6919.633762121201,0.1709504223526892
1879880,1879881,1879880,3759761,6928.348181009293,0.1707567677312909
1881882,1881883,1881882,3763765,6934.842335939407,0.17056351934479608
1883884,1883885,1883884,3767769,6939.889405012131,0.17037067591991217
1885886,1885887,1885886,3771773,6944.701292037964,0.1701782361851656
1887888,1887889,1887888,3775777,6950.125039815903,0.16998619888363464
1889890,1889891,1889890,3779781,6955.367079973221,0.1697945627529407
1891892,1891893,1891892,3783785,6960.580970048904,0.169603326545257
1893894,1893895,1893894,3787789,6965.927808046341,0.1694124890054809
1895896,1895897,1895896,3791793,6972.040957927704,0.16922204890215653
1897898,1897899,1897898,3795797,6977.9625589847565,0.16903200499109516
1899900,1899901,1899900,3799801,6982.59140586853,0.16884235604084097
1901902,1901903,1901902,3803805,6987.440189838409,0.16865310082903306
1903904,1903905,1903904,3807809,6992.618392705917,0.16846423813149158
1905906,1905907,1905906,3811813,6997.519407749176,0.16827576673131261
1907908,1907909,1907908,3815817,7002.885993003845,0.1680879560408357
1909910,1909911,1909910,3819821,7008.125239133835,0.16790073889569612
1911912,1911913,1911912,3823825,7014.502367973328,0.16771393165618065
1913914,1913915,1913914,3827829,7019.827627897263,0.16752751768217422
1915916,1915917,1915916,3831833,7024.659764051437,0.16734149122385134
1917918,1917919,1917918,3835837,7029.373505115509,0.16715584919620596
1919920,1919921,1919920,3839841,7034.784754991531,0.16697058960198774
1921922,1921923,1921922,3843845,7040.972080945969,0.16678571091324557
1923924,1923925,1923924,3847849,7047.324033737183,0.1666012118148501
1925926,1925927,1925926,3851853,7052.560672044754,0.16641709106625058
1927928,1927929,1927928,3855857,7058.868510961533,0.1662333474814659
1929930,1929931,1929930,3859861,7064.408024787903,0.16604997989634285
1931932,1931933,1931932,3863865,7069.954263687134,0.16586698714127124
1933934,1933935,1933934,3867869,7075.766191959381,0.16568436807574471
1935936,1935937,1935936,3871873,7081.740336894989,0.16550212155379995
1937938,1937939,1937938,3875877,7089.591381072998,0.16532024643674958
1939940,1939941,1939940,3879881,7096.938350915909,0.1651387415931822
1941942,1941943,1941942,3883885,7102.7548089027405,0.1649576058916864
1943944,1943945,1943944,3887889,7109.46373295784,0.1647768382099457
1945946,1945947,1945946,3891893,7115.765955924988,0.16459643743110064
1947948,1947949,1947948,3895897,7122.296474933624,0.1644164024401107
1949950,1949951,1949950,3899901,7129.6875948905945,0.16423673212739232
1951952,1951953,1951952,3903905,7136.325741767883,0.164057425383362
1953954,1953955,1953954,3907909,7141.586328744888,0.16387848111298808
1955956,1955957,1955956,3911913,7146.68771481514,0.16369989821942
1957958,1957959,1957958,3915917,7151.741986751556,0.16352167560944508
1959960,1959961,1959960,3919921,7156.924081802368,0.1633438121953077
1961962,1961963,1961962,3923925,7162.092285871506,0.16316630689470912
1963964,1963965,1963964,3927929,7167.352110862732,0.16298915863262664
1965966,1965967,1965966,3931933,7172.583300828934,0.16281236633221852
1967968,1967969,1967968,3935937,7178.253123760223,0.16263592892391898
1969970,1969971,1969970,3939941,7184.047181844711,0.16245984534361924
1971972,1971973,1971972,3943945,7190.673936843872,0.16228411452721048
1973974,1973975,1973974,3947949,7197.509047031403,0.16210873542331683
1975976,1975977,1975976,3951953,7203.211173772812,0.16193370697692444
1977978,1977979,1977978,3955957,7208.897807836533,0.1617590281402954
1979980,1979981,1979980,3959961,7214.114971876144,0.16158469786932983
1981982,1981983,1981982,3963965,7218.608076810837,0.16141071512356575
1983984,1983985,1983984,3967969,7223.11546087265,0.1612370788698172
1985986,1985987,1985986,3971973,7227.622876882553,0.1610637880730792
1987988,1987989,1987988,3975977,7232.08314704895,0.1608908417110797
1989990,1989991,1989990,3979981,7236.588862895966,0.1607182387560897
1991992,1991993,1991992,3983985,7241.0296268463135,0.16054597819129413
1993994,1993995,1993994,3987989,7245.438562870026,0.16037405900351587
1995996,1995997,1995996,3991993,7249.903501749039,0.16020248017775884
1997998,1997999,1997998,3995997,7254.350649833679,0.1600312407081219
2000000,2000001,2000000,4000001,7258.835234880447,0.15986033959961787


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002052783966064453,12064.44795143716
360,2490,2490,4980,3.3353936672210693,0.4583388177998131
721,5280,5280,10560,6.8332908153533936,0.31035213555878727
1081,8008,8008,16016,10.319485902786255,0.084708208543816
1441,10812,10812,21624,14.013197660446167,0.075534563688052
1802,13592,13592,27184,17.588513612747192,0.07000530239565705
2162,16390,16390,32780,21.251136541366577,0.06674257136910455
2522,19216,19216,38432,25.123957872390747,0.06501342345109151
2883,21988,21988,43976,28.911458730697632,0.042276417383618536
3243,24824,24824,49648,33.084638833999634,0.04189340341872594
3603,27640,27640,55280,36.932971715927124,0.03895886525060632
3964,30498,30498,60996,40.92040395736694,0.03852479658598895
4324,33332,33332,66664,44.85427665710449,0.036593014219761244
4684,36176,36176,72352,48.99788284301758,0.03639800104974711
5045,39004,39004,78008,53.31104588508606,0.03505098634377646
5405,41846,41846,83692,57.235915660858154,0.03422757205044036
5765,44694,44694,89388,61.188965797424316,0.033605409085794236
6125,47462,47462,94924,65.0127899646759,0.02106791718506429
6486,50328,50328,100656,68.98988962173462,0.02096373889435199
6846,53182,53182,106364,73.06409859657288,0.02072342238170677
7206,56010,56010,112020,76.96991276741028,0.016745869048463646
7567,58852,58852,117704,80.86206483840942,0.015371178300483734
7927,61708,61708,123416,84.80714964866638,0.015061802192576579
8287,64588,64588,129176,88.77300882339478,0.01506090143993788
8648,67460,67460,134920,92.78398895263672,0.015026678371214075
9008,70320,70320,140640,96.66565775871277,0.01495941970642889
9368,73184,73184,146368,100.69606971740723,0.014889309371937998
9729,76068,76068,152136,104.76848483085632,0.014882211386066047
10089,78932,78932,157864,108.74544477462769,0.01487767334401724
10449,81740,81740,163480,112.62320375442505,0.012236906235557399
10810,84608,84608,169216,116.68013882637024,0.01209875820131856
11170,87480,87480,174960,120.74181461334229,0.012095590962417191
11530,90346,90346,180692,124.70021986961365,0.012090483271094854
11891,93220,93220,186440,128.6783139705658,0.01206702594026865
12251,96082,96082,192164,132.74566173553467,0.011993510708634858
12611,98940,98940,197880,136.80996179580688,0.011832022402813891
12972,101782,101782,203564,140.87783670425415,0.009120136966885184
13332,104628,104628,209256,144.9932506084442,0.009104670496526523
13692,107496,107496,214992,149.18883085250854,0.009087816193641629
14053,110374,110374,220748,153.33507990837097,0.009061853392267949
14413,113240,113240,226480,157.36819195747375,0.009013164191856049
14773,116116,116116,232232,161.61079573631287,0.009005905843878281
15134,118998,118998,237996,165.74559879302979,0.008988955909444485
15494,121868,121868,243736,169.76634287834167,0.00897036396418116
15854,124740,124740,249480,173.85708856582642,0.00896236650805804
16215,127622,127622,255244,178.03062558174133,0.008816968862447538
16575,130498,130498,260996,182.09035682678223,0.008809027935058111
16935,133366,133366,266732,186.15984463691711,0.008682629058966995
17296,136238,136238,272476,190.36952757835388,0.008609743659690139
17656,139116,139116,278232,194.37928676605225,0.008608470227045473
18016,141988,141988,283976,198.51495671272278,0.008584949066062109
18376,144854,144854,289708,202.67348670959473,0.008553359422876383
18737,147734,147734,295468,206.71412682533264,0.008527686753950547
19097,150608,150608,301216,210.76261973381042,0.008524251115886727
19457,153486,153486,306972,214.86557960510254,0.008507006514264503
19818,156374,156374,312748,219.004953622818,0.008506609439791646
20178,159230,159230,318460,223.16551876068115,0.008488776265949127
20538,162092,162092,324184,227.187668800354,0.008461368299322203
20899,164934,164934,329868,231.21090078353882,0.006427179288948537
21259,167792,167792,335584,235.4808168411255,0.006412034876120742
21619,170656,170656,341312,239.5808026790619,0.006399188607247197
21980,173542,173542,347084,243.9259488582611,0.006394464737240924
22340,176418,176418,352836,248.09308886528015,0.006387159050063929
22700,179290,179290,358580,252.12749791145325,0.006381962242812733
23061,182174,182174,364348,256.106187582016,0.0063699157362862024
23421,185046,185046,370092,260.2386736869812,0.006355530191285652
23781,187916,187916,375832,264.2830798625946,0.006208932549270685
24142,190792,190792,381584,268.222553730011,0.006097746154409833
24502,193652,193652,387304,272.289963722229,0.006023392013958073
24862,196528,196528,393056,276.2908058166504,0.006016313802319928
25223,199410,199410,398820,280.23147678375244,0.006008175267197657
25583,202288,202288,404576,284.27365279197693,0.0060071994939789874
25943,205160,205160,410320,288.2586245536804,0.0059793454074679175
26304,208044,208044,416088,292.3207778930664,0.005972126915366971
26664,210922,210922,421844,296.28816175460815,0.005969061607174808
27024,213800,213800,427600,300.35339856147766,0.005967906687146751
27385,216684,216684,433368,304.5117027759552,0.005956985676675686
27745,219548,219548,439096,308.47636580467224,0.005869015360076446
28105,222420,222420,444840,312.477041721344,0.0058457958220969886
28466,225306,225306,450612,316.56445956230164,0.005844947505465825
28826,228176,228176,456352,320.5863926410675,0.005832664604895399
29186,231052,231052,462104,324.69407892227173,0.005813408077301574
29547,233938,233938,467876,328.8415606021881,0.0058091604896617355
29907,236816,236816,473632,332.8843057155609,0.005807076180644799
30267,239690,239690,479380,336.9142436981201,0.005798968237286317
30627,242570,242570,485140,341.02860283851624,0.005798699405204388
30988,245454,245454,490908,345.1152517795563,0.005793268486740999
31348,248328,248328,496656,349.2731728553772,0.005775922127213562
31708,251204,251204,502408,353.36934185028076,0.005772443004389061
32069,254090,254090,508180,357.38579177856445,0.005766655089246342
32429,256964,256964,513928,361.40272879600525,0.005758415076343226
32789,259830,259830,519660,365.55172300338745,0.0053337458721216535
33150,262716,262716,525432,369.6553888320923,0.005330852565748501
33510,265592,265592,531184,373.763623714447,0.005324668083630968
33870,268470,268470,536940,377.9181807041168,0.005322854412952438
34231,271348,271348,542696,381.8716707229614,0.005285292701955768
34591,274224,274224,548448,385.91061186790466,0.005281117644699407
34951,277084,277084,554168,389.9327266216278,0.004602130144121475
35312,279968,279968,559936,393.9751806259155,0.0045990878588781925
35672,282846,282846,565692,398.1381776332855,0.004597971070325002
36032,285722,285722,571444,402.15420269966125,0.0045806038160662865
36393,288608,288608,577216,406.1867399215698,0.004578413176204776
36753,291486,291486,582972,410.2378816604614,0.004575917868351098
37113,294360,294360,588720,414.34069561958313,0.004531525901256828
37474,297248,297248,594496,418.4928078651428,0.004531292368483264
37834,300124,300124,600248,422.62343764305115,0.00452272832262679
38194,302998,302998,605996,426.5814719200134,0.004499914288317086
38555,305886,305886,611772,430.6800436973572,0.004499681523157051
38915,308758,308758,617516,434.850882768631,0.004487060690735234
39275,311636,311636,623272,438.8841679096222,0.004480711017095018
39636,314522,314522,629044,443.10919189453125,0.00447958900622325
39996,317400,317400,634800,447.3195598125458,0.004474376251891954
40356,320280,320280,640560,451.3234717845917,0.004474144705454819
40717,323146,323146,646292,455.36489272117615,0.004464152705622837
41077,326022,326022,652044,459.4878237247467,0.0044607604595512385
41437,328898,328898,657796,463.54856181144714,0.004457288476260146
41798,331776,331776,663552,467.6924488544464,0.004441116701855208
42158,334644,334644,669288,471.8770658969879,0.004402272257721052
42518,337520,337520,675040,475.91535472869873,0.004397147202325868
42878,340398,340398,680796,480.0683755874634,0.004395147932882537
43239,343284,343284,686568,484.1691966056824,0.004384983665659092
43599,346160,346160,692320,488.1107656955719,0.004381034268590156
43959,349040,349040,698080,492.12537384033203,0.004380821161248605
44320,351924,351924,703848,496.2549297809601,0.004376170481918962
44680,354794,354794,709588,500.3214998245239,0.004132255719014211
45040,357672,357672,715344,504.2895197868347,0.004131050740397768
45401,360554,360554,721108,508.3818476200104,0.004113830007554498
45761,363426,363426,726852,512.4446818828583,0.004075867875144468
46121,366300,366300,732600,516.4898936748505,0.004010892816950218
46482,369186,369186,738372,520.7574617862701,0.004006257884611841
46842,372062,372062,744124,524.750706911087,0.004003319874755107
47202,374936,374936,749872,528.7624537944794,0.003982096906838706
47563,377824,377824,755648,532.8949267864227,0.003981893609307008
47923,380700,380700,761400,536.9890098571777,0.003976790578235523
48283,383576,383576,767152,540.9299228191376,0.003965028043239727
48644,386464,386464,772928,545.0166988372803,0.00396482520045538
49004,389338,389338,778676,549.0717198848724,0.00395472758282267
49364,392214,392214,784428,553.2202968597412,0.0039448465322493576
49725,395102,395102,790204,557.4690697193146,0.003944644195144065
50085,397980,397980,795960,561.5275738239288,0.0039409578166669235
50445,400856,400856,801712,565.5206699371338,0.003926970222892123
50806,403742,403742,807484,569.5925557613373,0.003926134380890289
51166,406620,406620,813240,573.685144662857,0.003922709342077724
51526,409498,409498,818996,577.6863358020782,0.003916148658390739
51887,412386,412386,824772,581.6201527118683,0.003915947027053335
52247,415262,415262,830524,585.6673467159271,0.0039041849104251014
52607,418140,418140,836280,589.7348258495331,0.0038991129586065654
52968,421026,421026,842052,593.8865888118744,0.003897436732586357
53328,423904,423904,847808,598.0542478561401,0.003894548686730559
53688,426782,426782,853564,602.1762449741364,0.0038927511468500597
54048,429662,429662,859324,606.1676378250122,0.0038925506505620433
54409,432534,432534,865068,610.2281057834625,0.003414816874283133
54769,435412,435412,870824,614.2493648529053,0.0034128114821214695
55129,438288,438288,876576,618.302916765213,0.003410123666981235
55490,441174,441174,882348,622.3793489933014,0.0034085990064340876
55850,444052,444052,888104,626.4387776851654,0.003405427987672738
56210,446932,446932,893864,630.4185826778412,0.0034052387709380127
56571,449820,449820,899640,634.4527056217194,0.003405049032153329
56931,452700,452700,905400,638.5189027786255,0.0034048598263325403
57291,455580,455580,911160,642.4950368404388,0.0034046706205117516
57652,458468,458468,916936,646.5817227363586,0.0034044809617626015
58012,461324,461324,922648,650.6146628856659,0.0034009343908110168
58372,464202,464202,928404,654.6489567756653,0.00339376753072429
58733,467088,467088,934176,658.7596297264099,0.003392539905689773
59093,469966,469966,939932,662.7940275669098,0.003389185709238518
59453,472838,472838,945676,666.8695726394653,0.003357433315613889
59814,475724,475724,951448,671.028874874115,0.0033570766827324405
60174,478602,478602,957204,674.9857678413391,0.00335170047947031
60534,481482,481482,962964,679.0052528381348,0.0033515407722006785
60895,484368,484368,968736,683.0636117458344,0.003349256474393769
61255,487248,487248,974496,687.0662908554077,0.003349096839883714
61615,490126,490126,980252,691.0877659320831,0.0033449243874201784
61976,493010,493010,986020,695.1397969722748,0.003342034598972532
62336,495890,495890,991780,699.2062315940857,0.0033418751427234383
62696,498768,498768,997536,703.2705538272858,0.0033385187034582486
63057,501656,501656,1003312,707.2679796218872,0.003338358887049253
63417,504532,504532,1009064,711.4207878112793,0.0033369388547725976
63777,507388,507388,1014776,715.4386458396912,0.0026911954664683435
64138,510274,510274,1020548,719.455308675766,0.0026893833546637325
64498,513150,513150,1026300,723.5859487056732,0.002686730842469842
64858,516028,516028,1032056,727.6045339107513,0.0026819470385817112
65219,518916,518916,1037832,731.6121258735657,0.0026818020924110897
65579,521796,521796,1043592,735.7511277198792,0.002681657555513084
65939,524672,524672,1049344,739.904632806778,0.002675767007531249
66299,527550,527550,1055100,743.9543647766113,0.0026742113986983895
66660,530438,530438,1060876,748.0455837249756,0.002674066650797613
67020,533316,533316,1066632,752.2100417613983,0.002670618996489793
67380,536196,536196,1072392,756.3145868778229,0.002670474723345251
67741,539080,539080,1078160,760.3623096942902,0.0026660581643227488
68101,541958,541958,1083916,764.4918527603149,0.0026606294286466436
68461,544836,544836,1089672,768.5904886722565,0.002658502135091112
68822,547724,547724,1095448,772.6416757106781,0.0026583577073324705
69182,550602,550602,1101204,776.746396780014,0.0026565437110548373
69542,553480,553480,1106960,780.9229388237,0.002655607224369305
69903,556362,556362,1112724,784.9986958503723,0.0026019391589215957
70263,559240,559240,1118480,789.030131816864,0.002598473241960164
70623,562120,562120,1124240,793.1079947948456,0.002598330380351399
70984,565004,565004,1130008,797.2102167606354,0.0025949201026378432
71344,567882,567882,1135764,801.3298716545105,0.0025836730455921497
71704,570758,570758,1141516,805.2889997959137,0.002582971357696806
72065,573642,573642,1147284,809.3860218524933,0.002570169826867641
72425,576518,576518,1153036,813.4822568893433,0.002566636232586461
72785,579398,579398,1158796,817.6243007183075,0.0025664939894340932
73146,582280,582280,1164560,821.800274848938,0.002526628524719854
73506,585158,585158,1170316,825.9656608104706,0.0025258072037104284
73866,588038,588038,1176076,830.1046888828278,0.002525665719076642
74227,590922,590922,1181844,834.3835499286652,0.0025197915856551845
74587,593800,593800,1187600,838.4888668060303,0.00251829375338275
74947,596678,596678,1193356,842.6165859699249,0.0025139975787169533
75308,599562,599562,1199124,846.6492428779602,0.0025063898665393936
75668,602440,602440,1204880,850.5570785999298,0.002504969959773007
76028,605318,605318,1210636,854.5579497814178,0.0025043783007276943
76389,608204,608204,1216408,858.5424077510834,0.0025017317802848993
76749,611084,611084,1222168,862.6046998500824,0.002501590739484527
77109,613960,613960,1227920,866.8267426490784,0.0024980243269965285
77470,616846,616846,1233692,870.8194527626038,0.002494614185707178
77830,619724,619724,1239448,874.7776277065277,0.0024934723078331444
78190,622602,622602,1245204,878.8084359169006,0.0024921989133872557
78550,625480,625480,1250960,882.8658995628357,0.0024883495534595568
78911,628366,628366,1256732,886.8664667606354,0.0024859102613845607
79271,631242,631242,1262484,890.8581387996674,0.002482669673554483
79631,634116,634116,1268232,895.1170587539673,0.0024612405177322216
79992,637002,637002,1274004,899.178201675415,0.0024592006138846045
80352,639882,639882,1279764,903.239284992218,0.0024590603443357395
80712,642758,642758,1285516,907.262987613678,0.002453694058203837
81073,645646,645646,1291292,911.2256577014923,0.0024535534848837415
81433,648522,648522,1297044,915.2235708236694,0.002447731034408207
81793,651402,651402,1302804,919.2176089286804,0.0024475909704051446
82154,654284,654284,1308568,923.1146328449249,0.002442342289214139
82514,657162,657162,1314324,927.0625128746033,0.002441210353936185
82874,660038,660038,1320076,931.054381608963,0.0024355015866603935
83235,662924,662924,1325848,935.0053586959839,0.002433891964756185
83595,665804,665804,1331608,938.9870536327362,0.0024337521572306287
83955,668682,668682,1337364,943.004264831543,0.0024305080260091927
84316,671568,671568,1343136,946.9801347255707,0.002429659596600686
84676,674446,674446,1348892,950.9459898471832,0.0024274485167552484
85036,677324,677324,1354648,955.0038678646088,0.0024231885272456566
85397,680210,680210,1360420,959.0314376354218,0.002422560781269567
85757,683088,683088,1366176,962.9594886302948,0.0024108089892251883
86117,685968,685968,1371936,966.9540228843689,0.002410669580058311
86478,688854,688854,1377708,971.0747518539429,0.0024088814188871766
86838,691732,691732,1383464,975.0277309417725,0.002407491807389306
87198,694612,694612,1389224,979.019428730011,0.0024073524728009943
87559,697496,697496,1394992,983.049195766449,0.002387289598118514
87919,700374,700374,1400748,986.9622666835785,0.0023860242108639795
88279,703252,703252,1406504,990.9804468154907,0.002384664705459727
88640,706138,706138,1412276,995.0871276855469,0.0023801713086868403
89000,709018,709018,1418036,999.1443247795105,0.002380032452492742
89360,711896,711896,1423792,1003.2563388347626,0.0023753740952088265
89721,714782,714782,1429564,1007.2537887096405,0.002372833580011502
90081,717660,717660,1435320,1011.2365758419037,0.0023712936435913434
90441,720538,720538,1441076,1015.354095697403,0.0023707389354967745
90801,723416,723416,1446832,1019.2862956523895,0.0023694472529314226
91162,726296,726296,1452592,1023.3313097953796,0.0022110275822342373
91522,729176,729176,1458352,1027.348112821579,0.002210891643699142
91882,732054,732054,1464108,1031.3568568229675,0.0022045213991077617
92243,734942,734942,1469884,1035.2881295681,0.0022043851640773937
92603,737820,737820,1475640,1039.3002407550812,0.002203261477916385
92963,740700,740700,1481400,1043.315388917923,0.0022031256739865057
93324,743586,743586,1487172,1047.2348380088806,0.0022021557688276516
93684,746462,746462,1492924,1051.2478725910187,0.002188822154494119
94044,749342,749342,1498684,1055.2732226848602,0.002188686577937915
94405,752228,752228,1504456,1059.5195965766907,0.0021874364701943705
94765,755106,755106,1510212,1063.4574909210205,0.0021812454651808366
95125,757986,757986,1515972,1067.4221827983856,0.0021811099904880393
95486,760872,760872,1521744,1071.4980607032776,0.0021783564043289516
95846,763750,763750,1527500,1075.530134677887,0.002177891321480274
96206,766628,766628,1533256,1079.5382537841797,0.002173863904317841
96567,769516,769516,1539032,1083.6357429027557,0.002173728205889347
96927,772394,772394,1544788,1087.7629268169403,0.002168460794564453
97287,775272,775272,1550544,1091.8990626335144,0.002167176751754596
97648,778148,778148,1556296,1095.8861849308014,0.0018803617094818037
98008,781018,781018,1562036,1099.878318786621,0.0018798621549649397
98368,783896,783896,1567792,1103.908813714981,0.0018790987323882291
98729,786782,786782,1573564,1107.9643766880035,0.0018767761248454917
99089,789662,789662,1579324,1112.0939917564392,0.0018766454904834973
99449,792538,792538,1585076,1116.2387146949768,0.0018751689785858616
99810,795422,795422,1590844,1120.3134138584137,0.0018699975898925913
100170,798298,798298,1596596,1124.3440928459167,0.001860456741269445
100530,801178,801178,1602356,1128.4043507575989,0.0018603263542900095
100891,804062,804062,1608124,1132.5588088035583,0.001855630967838806
101251,806940,806940,1613880,1136.5131478309631,0.0018538937238190556
101611,809818,809818,1619636,1140.56995677948,0.0018524292863730807
101972,812704,812704,1625408,1144.7227597236633,0.001848921894634259
102332,815582,815582,1631164,1148.7310168743134,0.0018487552370061167
102692,818462,818462,1636924,1152.735800743103,0.0018486250264686532
103052,821340,821340,1642680,1156.7565257549286,0.001845391536335228
103413,824228,824228,1648456,1160.7257068157196,0.0018452610111125978
103773,827108,827108,1654216,1164.6551659107208,0.001845130853325827
104133,829988,829988,1659976,1168.6856718063354,0.0018450006973580457
104494,832876,832876,1665752,1172.662666797638,0.0018448701812303625
104854,835756,835756,1671512,1176.591736793518,0.0018447400270815706
105214,838636,838636,1677272,1180.6508688926697,0.0018446098783897469
105575,841524,841524,1683048,1184.7020127773285,0.0018444793677190319
105935,844404,844404,1688808,1188.6280629634857,0.0018443492208461976
106295,847284,847284,1694568,1192.5813319683075,0.001844219077611342
106656,850172,850172,1700344,1196.8208618164062,0.0018440885705786059
107016,852990,852990,1705980,1200.8661468029022,0.0018336224602535367
107376,855860,855860,1711720,1204.798770904541,0.001831862862673006
107737,858740,858740,1717480,1208.8066718578339,0.0018247201078338549
108097,861610,861610,1723220,1212.9002668857574,0.0018188319209002657
108457,864488,864488,1728976,1216.8332617282867,0.0018173775533796288
108818,867346,867346,1734692,1220.8389329910278,0.0016767214438004885
109178,870222,870222,1740444,1224.8504047393799,0.0016751186158217024
109538,873098,873098,1746196,1228.8806986808777,0.0016749873975641094
109899,875972,875972,1751944,1232.9422497749329,0.0016737355563236633
110259,878844,878844,1757688,1237.1623549461365,0.0016698318031558301
110619,881718,881718,1763436,1241.2732815742493,0.0016671604207658675
110980,884606,884606,1769212,1245.3118867874146,0.0016670816658006515
111340,887484,887484,1774968,1249.3188407421112,0.0016663639580656309
111700,890360,890360,1780720,1253.4353857040405,0.0016641367055854062
112061,893244,893244,1786488,1257.4265348911285,0.0016634208241157467
112421,896108,896108,1792216,1261.3941869735718,0.0016137878574227216
112781,898984,898984,1797968,1265.4555327892303,0.001609892720807693
113142,901870,901870,1803740,1269.5256378650665,0.0016089994041976752
113502,904744,904744,1809488,1273.6419398784637,0.0016052439586928813
113862,907620,907620,1815240,1277.6200377941132,0.001603634995262837
114222,910494,910494,1820988,1281.6604647636414,0.0016025372060539667
114583,913376,913376,1826752,1285.7491688728333,0.0016002713200578
114943,916250,916250,1832500,1289.8556337356567,0.00159216038264276
115303,919124,919124,1838248,1293.7953147888184,0.0015859757368161809
115664,922010,922010,1844020,1297.8203446865082,0.0015854956272960408
116024,924886,924886,1849772,1301.8403508663177,0.0015813266836630646
116384,927764,927764,1855528,1305.8795099258423,0.0015811016037332593
116745,930650,930650,1861300,1309.809782743454,0.001577561124577187
117105,933524,933524,1867048,1313.7968208789825,0.001575492715346627
117465,936400,936400,1872800,1317.8110988140106,0.0015726842375443084
117826,939282,939282,1878564,1321.756740808487,0.00156996477926441
118186,942158,942158,1884316,1325.8068268299103,0.0015689387400925625
118546,945032,945032,1890064,1329.7917618751526,0.0015649931356165325
118907,947916,947916,1895832,1333.7985427379608,0.0015636085572623415
119267,950796,950796,1901592,1337.8338649272919,0.0015635329018550692
119627,953672,953672,1907344,1341.8773567676544,0.0015616484452039003
119988,956558,956558,1913116,1345.8775129318237,0.001560672197228996
120348,959438,959438,1918876,1349.9666516780853,0.0015605966254952364
120708,962318,962318,1924636,1354.2104687690735,0.001560521055580466
121069,965206,965206,1930412,1358.2521197795868,0.0015604452764819143
121429,968086,968086,1936172,1362.2928187847137,0.0015603697102051228
121789,970966,970966,1941932,1366.3357276916504,0.0015602941475663101
122150,973854,973854,1947708,1370.3754317760468,0.0015602183739247266
122510,976734,976734,1953468,1374.5100858211517,0.0015601428149238927
122870,979614,979614,1959228,1378.613811969757,0.0015600672559230588
123231,982502,982502,1965004,1382.8619756698608,0.0015599914913764223
123591,985382,985382,1970764,1386.9857556819916,0.0015599159378325567
123951,988262,988262,1976524,1391.014791727066,0.001559840384288691
124312,991150,991150,1982300,1395.0258848667145,0.0015597646251990227
124672,994030,994030,1988060,1399.0665159225464,0.0015596890771121252
125032,996910,996910,1993820,1403.0466239452362,0.0015596135308442172
125393,999798,999798,1999596,1407.0829648971558,0.0015595377753925277
125753,1002678,1002678,2005356,1411.1723308563232,0.0015594622345815878
126113,1005554,1005554,2011108,1415.1755237579346,0.0015571375479339622
126473,1008416,1008416,2016832,1419.0643298625946,0.001550882088849903
126834,1011300,1011300,2022600,1423.0176796913147,0.0015496883097512182
127194,1014170,1014170,2028340,1426.9891138076782,0.0015384055695903953
127554,1017048,1017048,2034096,1430.897118806839,0.0015377621093648486
127915,1019934,1019934,2039868,1434.8423907756805,0.0015362127578555373
128275,1022804,1022804,2045608,1438.8513488769531,0.0015321468345064204
128635,1025682,1025682,2051364,1442.9894227981567,0.0015318603873311076
128996,1028562,1028562,2057124,1447.009332895279,0.0015283634147635894
129356,1031430,1031430,2062860,1450.9699356555939,0.0015203038419713266
129716,1034306,1034306,2068612,1454.974514722824,0.001519528897915734
130077,1037190,1037190,2074380,1459.0992939472198,0.001518280460004462
130437,1040066,1040066,2080132,1463.0643198490143,0.0015156247427512426
130797,1042944,1042944,2085888,1467.0698266029358,0.0015150246981647797
131158,1045828,1045828,2091656,1471.1828668117523,0.0015130550109461183
131518,1048706,1048706,2097412,1475.2054116725922,0.0015120673524506856
131878,1051584,1051584,2103168,1479.1512308120728,0.001511092166765593
132239,1054446,1054446,2108892,1483.3795137405396,0.0002813263163261581
132599,1057322,1057322,2114644,1487.4343066215515,0.0002810723690345185
132959,1060202,1060202,2120404,1491.49653673172,0.0002810307614709018
133320,1063090,1063090,2126180,1495.6846487522125,0.00028098903749196324
133680,1065970,1065970,2131940,1499.8129577636719,0.00028094743174733594
134040,1068850,1068850,2137700,1503.9717757701874,0.00028090582964068744
134401,1071738,1071738,2143476,1508.0281698703766,0.0002808641111187171
134761,1074618,1074618,2149236,1512.1066718101501,0.000280822510831058
135121,1077386,1077386,2154772,1516.2314977645874,0.0002785170800052583
135482,1080268,1080268,2160536,1520.2348017692566,0.00027830168801301625
135842,1083140,1083140,2166280,1524.2069098949432,0.00027807996957562864
136202,1086018,1086018,2172036,1528.2301478385925,0.00027784229860117193
136563,1088896,1088896,2177792,1532.212671995163,0.0002770501778286416
136923,1091746,1091746,2183492,1536.2887697219849,0.0002668294710019836
137283,1094620,1094620,2189240,1540.337884902954,0.0002666221062099794
137644,1097500,1097500,2195000,1544.255474805832,0.0002663766990735894
138004,1100374,1100374,2200748,1548.3228137493134,0.0002660690042830538
138364,1103246,1103246,2206492,1552.554027557373,0.00026419975256430916
138724,1106116,1106116,2212232,1556.7284607887268,0.00026327379055146594
139085,1108964,1108964,2217928,1560.7137558460236,0.00010899851804424543
139445,1111782,1111782,2223564,1564.7729978561401,0.00010844979260582477
139805,1114640,1114640,2229280,1568.7258577346802,0.00010793309593282174
140166,1117514,1117514,2235028,1572.6891419887543,0.00010715404278016649
140526,1120390,1120390,2240780,1576.901516675949,0.00010702284998842515
140886,1123268,1123268,2246536,1580.9353559017181,0.00010694200864236336
141247,1126152,1126152,2252304,1584.9160528182983,0.00010688125075830612
141607,1129026,1129026,2258052,1588.8693985939026,0.0001065200394805288
141967,1131904,1131904,2263808,1592.8669328689575,0.00010629459393385332
142328,1134786,1134786,2269572,1596.76508975029,0.00010619000386213884
142688,1137656,1137656,2275312,1600.6639957427979,0.00010497380208107643
143048,1140534,1140534,2281068,1604.5668306350708,0.00010493063746253029
143409,1143418,1143418,2286836,1608.4658596515656,0.00010475033923285082
143769,1146292,1146292,2292584,1612.3682239055634,0.00010461359124747105
144129,1149172,1149172,2298344,1616.3403327465057,0.0001046069974108832
144490,1152060,1152060,2304120,1620.4391658306122,0.0001046003817464225
144850,1154940,1154940,2309880,1624.589323759079,0.00010459378427185584
145210,1157820,1157820,2315640,1628.5630836486816,0.00010458718861627858
145571,1160616,1160616,2321232,1632.4521605968475,0.00010397378537163604
145931,1163428,1163428,2326856,1636.4229328632355,0.00010239637776976451
146291,1166276,1166276,2332552,1640.3980107307434,0.00010175865645578597
146652,1169114,1169114,2338228,1644.2932579517365,0.00010034730985353235
147012,1171978,1171978,2343956,1648.3045797348022,0.00010020252739195712
147372,1174700,1174700,2349400,1652.166919708252,3.189343260601163e-07
147733,1177496,1177496,2354992,1656.0235269069672,3.164386725984514e-07
148093,1180358,1180358,2360716,1660.0092039108276,3.158020263072103e-07
148453,1183222,1183222,2366444,1664.0204167366028,3.1491435947827995e-07
148814,1186090,1186090,2372180,1667.9807176589966,3.1226772989612073e-07
149174,1188962,1188962,2377924,1671.8995189666748,3.1204217521008104e-07
149534,1191838,1191838,2383676,1675.918999671936,3.113109414698556e-07
149895,1194720,1194720,2389440,1679.953192949295,3.1120907806325704e-07
150255,1197592,1197592,2395184,1683.9032068252563,3.1020681490190327e-07
150615,1200470,1200470,2400940,1687.906789779663,3.0999945010989904e-07
150975,1203346,1203346,2406692,1692.1361169815063,3.0992850952316076e-07
151336,1206226,1206226,2412452,1696.2200796604156,3.0919909477233887e-07
151696,1209100,1209100,2418200,1700.137199640274,3.081659087911248e-07
152056,1211968,1211968,2423936,1704.2561717033386,3.080094757024199e-07
152417,1214848,1214848,2429696,1708.2578887939453,3.0774572223890573e-07
152777,1217726,1217726,2435452,1712.2245078086853,3.077129804296419e-07
153137,1220592,1220592,2441184,1716.2640867233276,3.051736712222919e-07
153498,1223478,1223478,2446956,1720.3045806884766,3.0513183446601033e-07
153858,1226346,1226346,2452692,1724.2160766124725,2.9805232770740986e-07
154218,1229214,1229214,2458428,1728.1309587955475,2.977558324346319e-07
154579,1232100,1232100,2464200,1732.2622096538544,2.9771399567835033e-07
154939,1234972,1234972,2469944,1736.249434709549,2.956694515887648e-07
155299,1237838,1237838,2475676,1740.1697657108307,2.9542934498749673e-07
155660,1240722,1240722,2481444,1744.251339673996,2.9533111955970526e-07
156020,1243596,1243596,2487192,1748.2612385749817,2.9524017008952796e-07
156380,1246466,1246466,2492932,1752.2772998809814,2.929773472715169e-07
156741,1249354,1249354,2498708,1756.2538278102875,2.929646143456921e-07
157101,1252232,1252232,2504464,1760.2129187583923,2.929136826423928e-07
157461,1255104,1255104,2510208,1764.2505469322205,2.9182047001086175e-07
157822,1257984,1257984,2515968,1768.2101256847382,2.917022356996313e-07
158182,1260860,1260860,2521720,1772.2117757797241,2.916403900599107e-07
158542,1263724,1263724,2527448,1776.1649918556213,2.914021024480462e-07
158903,1266604,1266604,2533208,1780.0744347572327,2.911601768573746e-07
159263,1269472,1269472,2538944,1784.0681076049805,2.2676613298244774e-07
159623,1272292,1272292,2544584,1788.0840456485748,2.6697307475842535e-08
159984,1275148,1275148,2550296,1792.1952848434448,2.6358975446783006e-08
160344,1277962,1277962,2555924,1796.324461698532,2.4507244233973324e-08
160704,1280836,1280836,2561672,1800.5232865810394,2.448723535053432e-08
161065,1283722,1283722,2567444,1804.7920336723328,2.4489054339937866e-08
161425,1286600,1286600,2573200,1808.8175837993622,2.4476321414113045e-08
161785,1289478,1289478,2578956,1812.8380358219147,2.4472683435305953e-08
162145,1292356,1292356,2584712,1816.9946947097778,2.4470864445902407e-08
162506,1295242,1295242,2590484,1821.0498926639557,2.4461769498884678e-08
162866,1298120,1298120,2596240,1825.256918668747,2.4445398594252765e-08
163226,1301000,1301000,2602000,1829.4251098632812,2.4445398594252765e-08
163587,1303884,1303884,2607768,1833.4539709091187,2.4407199816778302e-08
163947,1306762,1306762,2613524,1837.486498594284,2.436900103930384e-08
164307,1309642,1309642,2619284,1841.5835168361664,2.4367182049900293e-08
164668,1312528,1312528,2625056,1845.6258778572083,2.43635440710932e-08
165028,1315408,1315408,2630816,1849.6446409225464,2.4361725081689656e-08
165388,1318286,1318286,2636572,1853.6510179042816,2.4348992155864835e-08
165749,1321174,1321174,2642348,1857.7902138233185,2.435081114526838e-08
166109,1324052,1324052,2648104,1861.833863735199,2.4327164283022285e-08
166469,1326930,1326930,2653860,1865.8398067951202,2.4318069336004555e-08
166830,1329818,1329818,2659636,1869.7734367847443,2.43198883254081e-08
167190,1332692,1332692,2665384,1873.7514407634735,2.4261680664494634e-08
167550,1335570,1335570,2671140,1877.752713918686,2.4228938855230808e-08
167911,1338458,1338458,2676916,1881.6627316474915,2.4227119865827262e-08
168271,1341336,1341336,2682672,1885.5600218772888,2.4225300876423717e-08
168631,1344216,1344216,2688432,1889.502837896347,2.4227119865827262e-08
168992,1347102,1347102,2694204,1893.502460718155,2.421984390821308e-08
169352,1349980,1349980,2699960,1897.5147547721863,2.4172550183720887e-08
169712,1352858,1352858,2705716,1901.4538958072662,2.417073119431734e-08
170073,1355744,1355744,2711488,1905.5030808448792,2.412707544863224e-08
170433,1358624,1358624,2717248,1909.482509613037,2.4125256459228694e-08
170793,1361502,1361502,2723004,1913.510729789734,2.4125256459228694e-08
171154,1364388,1364388,2728776,1917.6320927143097,2.4112523533403873e-08
171514,1367268,1367268,2734536,1921.7291786670685,2.4110704544000328e-08
171874,1370146,1370146,2740292,1925.7774348258972,2.4108885554596782e-08
172235,1373034,1373034,2746068,1929.9569137096405,2.4107066565193236e-08
172595,1375910,1375910,2751820,1934.0855119228363,2.4057953851297498e-08
172955,1378790,1378790,2757580,1938.042457818985,2.4057953851297498e-08
173316,1381678,1381678,2763356,1942.0446107387543,2.4056134861893952e-08
173676,1384556,1384556,2769112,1946.1991558074951,2.4045220925472677e-08
174036,1387434,1387434,2774868,1950.5252096652985,2.4003384169191122e-08
174396,1390314,1390314,2780628,1954.558861732483,2.399974619038403e-08
174757,1393200,1393200,2786400,1958.6791307926178,2.4001565179787576e-08
175117,1396078,1396078,2792156,1963.1097688674927,2.399610821157694e-08
175477,1398956,1398956,2797912,1967.302963733673,2.395609044469893e-08
175838,1401844,1401844,2803688,1971.274250984192,2.3954271455295384e-08
176198,1404722,1404722,2809444,1975.332308769226,2.3952452465891838e-08
176558,1407602,1407602,2815204,1979.3879368305206,2.3952452465891838e-08
176919,1410488,1410488,2820976,1983.3255228996277,2.3948814487084746e-08
177279,1413366,1413366,2826732,1987.4013347625732,2.3910615709610283e-08
177639,1416244,1416244,2832488,1991.452553987503,2.3910615709610283e-08
178000,1419130,1419130,2838260,1995.5059819221497,2.3901520762592554e-08
178360,1422010,1422010,2844020,1999.5430719852448,2.3901520762592554e-08
178720,1424888,1424888,2849776,2003.465684890747,2.3897882783785462e-08
179081,1427772,1427772,2855544,2007.5809297561646,2.383239916525781e-08
179441,1430652,1430652,2861304,2011.8018028736115,2.3830580175854266e-08
179801,1433530,1433530,2867060,2016.1680927276611,2.381057129241526e-08
180162,1436416,1436416,2872832,2021.313954591751,2.3808752303011715e-08
180522,1439292,1439292,2878584,2025.9573638439178,2.3786924430169165e-08
180882,1442172,1442172,2884344,2030.106009721756,2.3786924430169165e-08
181243,1445052,1445052,2890104,2034.3417489528656,2.3717802832834423e-08
181603,1447930,1447930,2895860,2038.679040670395,2.371416485402733e-08
181963,1450806,1450806,2901612,2043.462554693222,2.3641405277885497e-08
182324,1453694,1453694,2907388,2048.266612768173,2.3643224267289042e-08
182684,1456570,1456570,2913140,2053.024683713913,2.362685336265713e-08
183044,1459450,1459450,2918900,2057.7197246551514,2.3625034373253584e-08
183405,1462336,1462336,2924672,2062.297724723816,2.3621396394446492e-08
183765,1465214,1465214,2930428,2066.4484128952026,2.3615939426235855e-08
184125,1468094,1468094,2936188,2070.6229887008667,2.36177584156394e-08
184486,1470976,1470976,2941952,2074.737708568573,2.3506800062023103e-08
184846,1473856,1473856,2947712,2078.9663639068604,2.3504981072619557e-08
185206,1476734,1476734,2953468,2083.2641699314117,2.349952410440892e-08
185567,1479622,1479622,2959244,2088.068870782852,2.3497705115005374e-08
185927,1482500,1482500,2965000,2093.247412919998,2.3443135432898998e-08
186287,1485380,1485380,2970760,2098.8033599853516,2.3441316443495452e-08
186647,1488256,1488256,2976512,2103.371319770813,2.3395841708406806e-08
187008,1491140,1491140,2982280,2107.4937467575073,2.3395841708406806e-08
187368,1494018,1494018,2988036,2111.6036248207092,2.339038474019617e-08
187728,1496894,1496894,2993788,2115.8155739307404,2.3330358089879155e-08
188089,1499780,1499780,2999560,2119.920970916748,2.3330358089879155e-08
188449,1502660,1502660,3005320,2123.924115896225,2.332853910047561e-08
188809,1505538,1505538,3011076,2128.0475997924805,2.3324901121668518e-08
189170,1508424,1508424,3016848,2132.147962808609,2.3317625164054334e-08
189530,1511304,1511304,3022608,2136.1799318790436,2.3315806174650788e-08
189890,1514182,1514182,3028364,2140.303640604019,2.331034920644015e-08
190251,1517070,1517070,3034140,2144.4814257621765,2.331034920644015e-08
190611,1519948,1519948,3039896,2148.611836910248,2.3308530217036605e-08
190971,1522820,1522820,3045640,2152.704917907715,2.3215761757455766e-08
191332,1525708,1525708,3051416,2156.897519826889,2.321394276805222e-08
191692,1528586,1528586,3057172,2160.958869934082,2.320484782103449e-08
192052,1531466,1531466,3062932,2165.4247579574585,2.320484782103449e-08
192413,1534352,1534352,3068704,2170.8978576660156,2.318301994819194e-08
192773,1537230,1537230,3074460,2175.639812707901,2.3181200958788395e-08
193133,1540110,1540110,3080220,2180.260452747345,2.3181200958788395e-08
193494,1542996,1542996,3085992,2185.048796892166,2.317028702236712e-08
193854,1545876,1545876,3091752,2190.216796875,2.317028702236712e-08
194214,1548752,1548752,3097504,2194.5490548610687,2.3141183191910386e-08
194575,1551636,1551636,3103272,2198.864629983902,2.313936420250684e-08
194935,1554512,1554512,3109024,2203.749034881592,2.3122993297874928e-08
195295,1557392,1557392,3114784,2208.857181787491,2.3122993297874928e-08
195656,1560274,1560274,3120548,2213.2994287014008,2.3068423615768552e-08
196016,1563154,1563154,3126308,2217.5695888996124,2.3068423615768552e-08
196376,1566034,1566034,3132068,2221.8852999210358,2.3068423615768552e-08
196737,1568918,1568918,3137836,2226.2040917873383,2.3044776753522456e-08
197097,1571796,1571796,3143592,2231.0893869400024,2.3017491912469268e-08
197457,1574676,1574676,3149352,2236.217805624008,2.3015672923065722e-08
197818,1577562,1577562,3155124,2240.6794838905334,2.3006577976047993e-08
198178,1580440,1580440,3160880,2244.7335228919983,2.299930201843381e-08
198538,1583320,1583320,3166640,2248.8476238250732,2.299930201843381e-08
198898,1586198,1586198,3172396,2252.9809918403625,2.2993845050223172e-08
199259,1589086,1589086,3178172,2257.0403838157654,2.2993845050223172e-08
199619,1591964,1591964,3183928,2261.310980796814,2.2993845050223172e-08
199979,1594838,1594838,3189676,2265.4424448013306,2.2848325897939503e-08
200340,1597722,1597722,3195444,2269.5377867221832,2.284104994032532e-08
200700,1600602,1600602,3201204,2273.610765695572,2.284104994032532e-08
201060,1603480,1603480,3206960,2277.7958776950836,2.2833773982711136e-08
201421,1606368,1606368,3212736,2283.300372838974,2.2833773982711136e-08
201781,1609244,1609244,3218488,2288.353967666626,2.2830136003904045e-08
202141,1612122,1612122,3224244,2292.5549437999725,2.2764652385376394e-08
202502,1615010,1615010,3230020,2297.263193845749,2.2761014406569302e-08
202862,1617888,1617888,3235776,2302.2028658390045,2.274828148074448e-08
203222,1620768,1620768,3241536,2306.56685590744,2.2746462491340935e-08
203583,1623654,1623654,3247308,2310.9537427425385,2.2742824512533844e-08
203943,1626532,1626532,3253064,2315.478418827057,2.2741005523130298e-08
204303,1629412,1629412,3258824,2320.265790939331,2.2739186533726752e-08
204664,1632294,1632294,3264588,2326.9239938259125,2.2680978872813284e-08
205024,1635172,1635172,3270344,2332.1129677295685,2.264278009533882e-08
205384,1638052,1638052,3276104,2336.559072971344,2.2640961105935276e-08
205745,1640938,1640938,3281876,2342.122130870819,2.263914211653173e-08
206105,1643818,1643818,3287636,2348.4120547771454,2.2637323127128184e-08
206465,1646686,1646686,3293372,2354.3551087379456,2.229171514045447e-08
206826,1649572,1649572,3299144,2359.9639108181,2.2289896151050925e-08
207186,1652452,1652452,3304904,2364.4694147109985,2.228807716164738e-08
207546,1655328,1655328,3310656,2368.890483856201,2.2249878384172916e-08
207907,1658214,1658214,3316428,2373.1154465675354,2.224805939476937e-08
208267,1661092,1661092,3322184,2377.2142946720123,2.224442141596228e-08
208627,1663970,1663970,3327940,2381.852790594101,2.219167072325945e-08
208988,1666858,1666858,3333716,2386.0732197761536,2.219167072325945e-08
209348,1669736,1669736,3339472,2390.1900238990784,2.218621375504881e-08
209708,1672616,1672616,3345232,2394.360668897629,2.218621375504881e-08
210068,1675494,1675494,3350988,2398.453575849533,2.2171661839820445e-08
210429,1678382,1678382,3356764,2402.891300678253,2.2171661839820445e-08
210789,1681260,1681260,3362520,2407.611290693283,2.2166204871609807e-08
211149,1684138,1684138,3368276,2412.3206646442413,2.216438588220626e-08
211510,1687020,1687020,3374040,2416.4606835842133,2.207707439083606e-08
211870,1689900,1689900,3379800,2420.4870688915253,2.207707439083606e-08
212230,1692776,1692776,3385552,2424.6774389743805,2.2053427528589964e-08
212591,1695662,1695662,3391324,2428.9927899837494,2.2047970560379326e-08
212951,1698542,1698542,3397084,2433.6568179130554,2.2047970560379326e-08
213311,1701416,1701416,3402832,2438.083863735199,2.1966116037219763e-08
213672,1704304,1704304,3408608,2442.48193359375,2.1966116037219763e-08
214032,1707182,1707182,3414364,2446.9904177188873,2.1953383111394942e-08
214392,1710060,1710060,3420120,2451.235229730606,2.1944288164377213e-08
214753,1712948,1712948,3425896,2455.729246854782,2.1944288164377213e-08
215113,1715826,1715826,3431652,2461.0990509986877,2.1871528588235378e-08
215473,1718706,1718706,3437412,2466.68740773201,2.1871528588235378e-08
215834,1721592,1721592,3443184,2471.648412704468,2.1869709598831832e-08
216194,1724472,1724472,3448944,2476.6809096336365,2.1869709598831832e-08
216554,1727350,1727350,3454700,2481.969719648361,2.1864252630621195e-08
216915,1730234,1730234,3460468,2486.676855802536,2.1833329810760915e-08
217275,1733114,1733114,3466228,2491.545940876007,2.1833329810760915e-08
217635,1735992,1735992,3471984,2496.0289556980133,2.1827872842550278e-08
217996,1738880,1738880,3477760,2500.408362865448,2.1827872842550278e-08
218356,1741756,1741756,3483512,2505.97709774971,2.1753294277004898e-08
218716,1744634,1744634,3489268,2510.862913608551,2.1751475287601352e-08
219077,1747522,1747522,3495044,2515.293940782547,2.1749656298197806e-08
219437,1750400,1750400,3500800,2520.069007873535,2.1744199329987168e-08
219797,1753278,1753278,3506556,2524.4785068035126,2.1740561351180077e-08
220158,1756166,1756166,3512332,2528.7703437805176,2.1740561351180077e-08
220518,1759042,1759042,3518084,2533.1912717819214,2.1706000552512705e-08
220878,1761920,1761920,3523840,2537.8513889312744,2.170418156310916e-08
221239,1764808,1764808,3529616,2543.0637958049774,2.1702362573705614e-08
221599,1767684,1767684,3535368,2548.340161561966,2.166416379623115e-08
221959,1770564,1770564,3541128,2552.7882030010223,2.1662344806827605e-08
222319,1773444,1773444,3546888,2557.75470161438,2.1662344806827605e-08
222680,1776328,1776328,3552656,2563.614450931549,2.163869794458151e-08
223040,1779208,1779208,3558416,2567.9142467975616,2.1635059965774417e-08
223400,1782086,1782086,3564172,2572.3021278381348,2.1596861188299954e-08
223761,1784972,1784972,3569944,2576.879426717758,2.1595042198896408e-08
224121,1787852,1787852,3575704,2581.4799869060516,2.1595042198896408e-08
224481,1790730,1790730,3581460,2586.47833275795,2.1591404220089316e-08
224842,1793616,1793616,3587232,2590.6730806827545,2.158594725187868e-08
225202,1796496,1796496,3592992,2595.455641746521,2.1582309273071587e-08
225562,1799374,1799374,3598748,2601.133986711502,2.1542291506193578e-08
225923,1802262,1802262,3604524,2606.3435287475586,2.1542291506193578e-08
226283,1805140,1805140,3610280,2611.8690598011017,2.1538653527386487e-08
226643,1808016,1808016,3616032,2616.7952115535736,2.148044586647302e-08
227004,1810902,1810902,3621804,2622.289661884308,2.1478626877069473e-08
227364,1813778,1813778,3627556,2627.068473815918,2.1456799004226923e-08
227724,1816658,1816658,3633316,2631.6286277770996,2.1456799004226923e-08
228085,1819544,1819544,3639088,2637.064178943634,2.145316102541983e-08
228445,1822424,1822424,3644848,2641.7602138519287,2.145316102541983e-08
228805,1825302,1825302,3650604,2646.2236108779907,2.144952304661274e-08
229166,1828188,1828188,3656376,2650.68145775795,2.140950527973473e-08
229526,1831066,1831066,3662132,2655.093069791794,2.1360392565838993e-08
229886,1833942,1833942,3667884,2660.033100605011,2.1360392565838993e-08
230247,1836830,1836830,3673660,2665.303678750992,2.1358573576435447e-08
230607,1839708,1839708,3679416,2669.86367893219,2.13567545870319e-08
230967,1842586,1842586,3685172,2674.581178665161,2.135311660822481e-08
231328,1845472,1845472,3690944,2679.049566745758,2.1345840650610626e-08
231688,1848352,1848352,3696704,2684.0000348091125,2.1345840650610626e-08
232048,1851228,1851228,3702456,2689.0279817581177,2.1338564692996442e-08
232409,1854112,1854112,3708224,2693.809685945511,2.1305822883732617e-08
232769,1856984,1856984,3713968,2698.499107837677,2.1302184904925525e-08
233129,1859862,1859862,3719724,2702.8261897563934,2.130036591552198e-08
233490,1862748,1862748,3725496,2707.0256838798523,2.1227606339380145e-08
233850,1865628,1865628,3731256,2711.1973328590393,2.12257873499766e-08
234210,1868506,1868506,3737012,2715.3244726657867,2.1227606339380145e-08
234570,1871380,1871380,3742760,2719.903144836426,2.1187588572502136e-08
234931,1874268,1874268,3748536,2724.3246598243713,2.1187588572502136e-08
235291,1877146,1877146,3754292,2728.476920604706,2.117667463608086e-08
235651,1880026,1880026,3760052,2732.7066287994385,2.117667463608086e-08
236012,1882912,1882912,3765824,2737.7043278217316,2.1169398678466678e-08
236372,1885788,1885788,3771576,2742.819718837738,2.116394171025604e-08
236732,1888668,1888668,3777336,2747.4873967170715,2.116394171025604e-08
237093,1891550,1891550,3783100,2752.0676698684692,2.112392394337803e-08
237453,1894430,1894430,3788860,2756.7633757591248,2.112392394337803e-08
237813,1897308,1897308,3794616,2762.3142836093903,2.1113010006956756e-08
238174,1900196,1900196,3800392,2766.736150741577,2.111119101755321e-08
238534,1903070,1903070,3806140,2771.011683702469,2.0629158825613558e-08
238894,1905944,1905944,3811888,2775.1312777996063,2.0627339836210012e-08
239255,1908832,1908832,3817664,2779.268969774246,2.0627339836210012e-08
239615,1911710,1911710,3823420,2783.4041736125946,2.0625520846806467e-08
239975,1914588,1914588,3829176,2787.4783487319946,2.0621882867999375e-08
240336,1917472,1917472,3834944,2791.619095802307,2.0618244889192283e-08
240696,1920348,1920348,3840696,2795.6825788021088,2.0605511963367462e-08
241056,1923228,1923228,3846456,2799.8525156974792,2.0605511963367462e-08
241417,1926114,1926114,3852228,2804.0252459049225,2.059277903754264e-08
241777,1928988,1928988,3857976,2808.0756447315216,2.0498191588558257e-08
242137,1931868,1931868,3863736,2812.1814708709717,2.0498191588558257e-08
242498,1934754,1934754,3869508,2816.354877948761,2.049637259915471e-08
242858,1937630,1937630,3875260,2820.40700173378,2.048363967332989e-08
243218,1940510,1940510,3881020,2824.4451987743378,2.0481820683926344e-08
243579,1943392,1943392,3886784,2828.5860679149628,2.0379957277327776e-08
243939,1946272,1946272,3892544,2832.7738676071167,2.037813828792423e-08
244299,1949150,1949150,3898300,2837.2280967235565,2.0372681319713593e-08
244660,1952036,1952036,3904072,2841.326315641403,2.03690433409065e-08
245020,1954912,1954912,3909824,2845.4456708431244,2.034721546806395e-08
245380,1957792,1957792,3915584,2849.719714641571,2.0345396478660405e-08
245741,1960676,1960676,3921352,2853.942790746689,2.0305378711782396e-08
246101,1963554,1963554,3927108,2858.3656067848206,2.0305378711782396e-08
246461,1966432,1966432,3932864,2862.464081764221,2.0301740732975304e-08
246821,1969312,1969312,3938624,2866.536012649536,2.0299921743571758e-08
247182,1972198,1972198,3944396,2870.7614719867706,2.0298102754168212e-08
247542,1975074,1975074,3950148,2875.0381219387054,2.0267179934307933e-08
247902,1977954,1977954,3955908,2879.107084751129,2.0265360944904387e-08
248263,1980840,1980840,3961680,2883.195101737976,2.026354195550084e-08
248623,1983716,1983716,3967432,2887.2978036403656,2.021624823100865e-08
248983,1986596,1986596,3973192,2891.4525775909424,2.0214429241605103e-08
249344,1989482,1989482,3978964,2895.5132637023926,2.016713551711291e-08
249704,1992362,1992362,3984724,2899.5552546977997,2.0168954506516457e-08
250064,1995240,1995240,3990480,2903.6367769241333,2.016713551711291e-08
250425,1998128,1998128,3996256,2907.696657896042,2.016349753830582e-08
250785,2001006,2001006,4002012,2911.759621858597,2.0159859559498727e-08
251145,2003884,2003884,4007768,2915.75483584404,2.015804057009518e-08
251506,2006768,2006768,4013536,2920.012847661972,2.0152583601884544e-08
251866,2009646,2009646,4019292,2924.4197697639465,2.0112565835006535e-08
252226,2012526,2012526,4025052,2928.4708528518677,2.0112565835006535e-08
252587,2015410,2015410,4030820,2932.6193528175354,2.009255695156753e-08
252947,2018290,2018290,4036580,2938.058931827545,2.009255695156753e-08
253307,2021168,2021168,4042336,2942.862607717514,2.008891897276044e-08
253668,2024054,2024054,4048108,2947.2652275562286,2.0085280993953347e-08
254028,2026932,2026932,4053864,2951.7573566436768,2.0056177163496614e-08
254388,2029812,2029812,4059624,2956.3736917972565,2.0052539184689522e-08
254749,2032698,2032698,4065396,2961.164933681488,2.003616828005761e-08
255109,2035578,2035578,4071156,2965.8532989025116,2.003616828005761e-08
255469,2038456,2038456,4076912,2970.2804396152496,2.0034349290654063e-08
255830,2041344,2041344,4082688,2975.041823863983,2.0032530301250517e-08
256190,2044222,2044222,4088444,2979.917187690735,2.0028892322443426e-08
256550,2047102,2047102,4094204,2984.7749347686768,2.002707333303988e-08
256911,2049986,2049986,4099972,2989.776422739029,1.9985236576758325e-08
257271,2052862,2052862,4105724,2994.891504764557,1.9981598597951233e-08
257631,2055740,2055740,4111480,2999.0613617897034,1.9914295990020037e-08
257991,2058618,2058618,4117236,3003.1104588508606,1.991247700061649e-08
258352,2061506,2061506,4123012,3007.1929848194122,1.9914295990020037e-08
258712,2064384,2064384,4128768,3011.238262653351,1.9905201043002307e-08
259072,2067264,2067264,4134528,3015.4531667232513,1.9905201043002307e-08
259433,2070150,2070150,4140300,3019.391910791397,1.989974407479167e-08
259793,2073028,2073028,4146056,3023.4262647628784,1.9897925085388124e-08
260153,2075906,2075906,4151812,3027.578373670578,1.9892468117177486e-08
260514,2078792,2078792,4157584,3031.6407396793365,1.984699338208884e-08
260874,2081670,2081670,4163340,3035.784863948822,1.984699338208884e-08
261234,2084550,2084550,4169100,3039.9111337661743,1.984699338208884e-08
261595,2087436,2087436,4174872,3044.02410697937,1.9841536413878202e-08
261955,2090316,2090316,4180632,3049.0097477436066,1.9841536413878202e-08
262315,2093194,2093194,4186388,3054.0870547294617,1.983789843507111e-08
262676,2096078,2096078,4192156,3058.3909339904785,1.9832441466860473e-08
263036,2098956,2098956,4197912,3062.3622148036957,1.9826984498649836e-08
263396,2101836,2101836,4203672,3066.5867426395416,1.9826984498649836e-08
263757,2104722,2104722,4209444,3072.0732595920563,1.9821527530439198e-08
264117,2107600,2107600,4215200,3076.414261817932,1.9821527530439198e-08
264477,2110478,2110478,4220956,3080.638945579529,1.9801518647000194e-08
264838,2113366,2113366,4226732,3084.9513866901398,1.9799699657596648e-08
265198,2116240,2116240,4232480,3089.3342068195343,1.9765138858929276e-08
265558,2119118,2119118,4238236,3093.4947838783264,1.9739673007279634e-08
265919,2122004,2122004,4244008,3097.753609895706,1.9736035028472543e-08
266279,2124884,2124884,4249768,3102.2094116210938,1.973785401787609e-08
266639,2127762,2127762,4255524,3106.627217769623,1.972875907085836e-08
267000,2130648,2130648,4261296,3110.943238735199,1.9725121092051268e-08
267360,2133526,2133526,4267052,3115.2750086784363,1.9723302102647722e-08
267720,2136404,2136404,4272808,3120.1649737358093,1.971966412384063e-08
268081,2139290,2139290,4278580,3124.761791944504,1.9621438696049154e-08
268441,2142168,2142168,4284336,3129.2165718078613,1.9615981727838516e-08
268801,2145046,2145046,4290092,3133.2980756759644,1.9615981727838516e-08
269162,2147930,2147930,4295860,3137.2056319713593,1.9528670236468315e-08
269522,2150810,2150810,4301620,3141.234712600708,1.952685124706477e-08
269882,2153684,2153684,4307368,3145.8658187389374,1.9521394278854132e-08
270242,2156562,2156562,4313124,3151.571588754654,1.9510480342432857e-08
270603,2159450,2159450,4318900,3155.976133823395,1.950866135302931e-08
270963,2162328,2162328,4324656,3160.2594878673553,1.950866135302931e-08
271323,2165206,2165206,4330412,3166.0816926956177,1.950502337422222e-08
271684,2168092,2168092,4336184,3170.1874418258667,1.9501385395415127e-08
272044,2170970,2170970,4341940,3174.17928981781,1.9497747416608036e-08
272404,2173848,2173848,4347696,3178.235188961029,1.9497747416608036e-08
272765,2176730,2176730,4353460,3182.3765897750854,1.9432263798080385e-08
273125,2179608,2179608,4359216,3186.5558807849884,1.943044480867684e-08
273485,2182484,2182484,4364968,3190.6468527317047,1.9379513105377555e-08
273846,2185372,2185372,4370744,3194.720607995987,1.9379513105377555e-08
274206,2188250,2188250,4376500,3198.8069398403168,1.9332219380885363e-08
274566,2191128,2191128,4382256,3202.9597675800323,1.933403837028891e-08
274927,2194016,2194016,4388032,3206.9994246959686,1.9330400391481817e-08
275287,2196894,2196894,4393788,3211.056858778,1.9330400391481817e-08
275647,2199774,2199774,4399548,3215.213100671768,1.9330400391481817e-08
276008,2202658,2202658,4405316,3219.1433238983154,1.9299477571621537e-08
276368,2205536,2205536,4411072,3223.8735597133636,1.92940206034109e-08
276728,2208416,2208416,4416832,3228.6669178009033,1.9295839592814445e-08
277089,2211302,2211302,4422604,3233.787077665329,1.9292201614007354e-08
277449,2214178,2214178,4428356,3238.328024625778,1.9252183847129345e-08
277809,2217058,2217058,4434116,3243.068797826767,1.9255821825936437e-08
278170,2219944,2219944,4439888,3248.0422966480255,1.924126991070807e-08
278530,2222824,2222824,4445648,3252.8463218212128,1.9239450921304524e-08
278890,2225700,2225700,4451400,3257.3401288986206,1.9199433154426515e-08
279251,2228584,2228584,4457168,3262.2555928230286,1.919761416502297e-08
279611,2231462,2231462,4462924,3266.982183933258,1.9192157196812332e-08
279971,2234342,2234342,4468684,3271.769203901291,1.9192157196812332e-08
280332,2237228,2237228,4474456,3276.23978972435,1.9173967302776873e-08
280692,2240106,2240106,4480212,3280.680942773819,1.9173967302776873e-08
281052,2242984,2242984,4485968,3285.4399275779724,1.9121216610074043e-08
281413,2245870,2245870,4491740,3290.324005842209,1.911757863126695e-08
281773,2248748,2248748,4497496,3294.725512742996,1.9115759641863406e-08
282133,2251624,2251624,4503248,3298.85630774498,1.9110302673652768e-08
282493,2254502,2254502,4509004,3302.9831957817078,1.9084836822003126e-08
282854,2257390,2257390,4514780,3307.3509197235107,1.9084836822003126e-08
283214,2260268,2260268,4520536,3312.30885887146,1.907937985379249e-08
283574,2263148,2263148,4526296,3317.2351248264313,1.907937985379249e-08
283935,2266034,2266034,4532068,3321.899136543274,1.9066646927967668e-08
284295,2268914,2268914,4537828,3326.600266933441,1.9063008949160576e-08
284655,2271792,2271792,4543584,3331.0730097293854,1.9064827938564122e-08
285016,2274680,2274680,4549360,3335.4580779075623,1.9063008949160576e-08
285376,2277556,2277556,4555112,3340.0905599594116,1.9022991182282567e-08
285736,2280436,2280436,4560872,3345.0428416728973,1.902117219287902e-08
286097,2283320,2283320,4566640,3349.2581696510315,1.9019353203475475e-08
286457,2286198,2286198,4572396,3354.256385564804,1.9015715224668384e-08
286817,2289074,2289074,4578148,3358.634217977524,1.8975697457790375e-08
287178,2291960,2291960,4583920,3363.296413898468,1.896842150017619e-08
287538,2294840,2294840,4589680,3367.900018930435,1.896842150017619e-08
287898,2297716,2297716,4595432,3372.886338710785,1.8932041712105274e-08
288259,2300604,2300604,4601208,3377.4380297660828,1.8932041712105274e-08
288619,2303482,2303482,4606964,3382.0024058818817,1.8919308786280453e-08
288979,2306362,2306362,4612724,3386.969740629196,1.891567080747336e-08
289340,2309248,2309248,4618496,3391.377111673355,1.8897480913437903e-08
289700,2312128,2312128,4624256,3395.6923298835754,1.8897480913437903e-08
290060,2315006,2315006,4630012,3400.575266599655,1.8895661924034357e-08
290421,2317892,2317892,4635784,3405.168040752411,1.8842911231331527e-08
290781,2320770,2320770,4641540,3409.357596874237,1.884109224192798e-08
291141,2323646,2323646,4647292,3414.6436347961426,1.8839273252524436e-08
291502,2326534,2326534,4653068,3419.372496843338,1.883745426312089e-08
291862,2329412,2329412,4658824,3423.5342106819153,1.8835635273717344e-08
292222,2332290,2332290,4664580,3427.5460076332092,1.878834154922515e-08
292583,2335176,2335176,4670352,3431.931500673294,1.8773789633996785e-08
292943,2338056,2338056,4676112,3436.052515745163,1.8773789633996785e-08
293303,2340932,2340932,4681864,3440.247738838196,1.8770151655189693e-08
293664,2343820,2343820,4687640,3444.477398633957,1.8768332665786147e-08
294024,2346696,2346696,4693392,3448.5233767032623,1.8724676920101047e-08
294384,2349574,2349574,4699148,3452.6412127017975,1.87228579306975e-08
294744,2352450,2352450,4704900,3456.751980781555,1.871921995189041e-08
295105,2355336,2355336,4710672,3460.9375648498535,1.870103005785495e-08
295465,2358216,2358216,4716432,3465.181047677994,1.8699211068451405e-08
295825,2361096,2361096,4722192,3469.2751359939575,1.8699211068451405e-08
296186,2363974,2363974,4727948,3473.5925776958466,1.8579157767817378e-08
296546,2366850,2366850,4733700,3477.7482466697693,1.8575519789010286e-08
296906,2369728,2369728,4739456,3481.9955537319183,1.8562786863185465e-08
297267,2372616,2372616,4745232,3486.272297859192,1.856460585258901e-08
297627,2375494,2375494,4750988,3490.3093235492706,1.8522769096307456e-08
297987,2378372,2378372,4756744,3494.3860898017883,1.852095010690391e-08
298348,2381260,2381260,4762520,3498.73673081398,1.852095010690391e-08
298708,2384136,2384136,4768272,3502.7638766765594,1.851731212809682e-08
299068,2387016,2387016,4774032,3506.740118741989,1.8515493138693273e-08
299429,2389902,2389902,4779804,3510.8946266174316,1.8513674149289727e-08
299789,2392778,2392778,4785556,3515.0073778629303,1.8470018403604627e-08
300149,2395658,2395658,4791316,3519.270738840103,1.8470018403604627e-08
300510,2398542,2398542,4797084,3523.4805738925934,1.8448190530762076e-08
300870,2401420,2401420,4802840,3527.722856760025,1.84372765943408e-08
301230,2404298,2404298,4808596,3532.0905187129974,1.8435457604937255e-08
301591,2407184,2407184,4814368,3536.7333278656006,1.843363861553371e-08
301951,2410064,2410064,4820128,3541.49293589592,1.843363861553371e-08
302311,2412940,2412940,4825880,3546.1592009067535,1.83499651029706e-08
302672,2415828,2415828,4831656,3551.1289489269257,1.8348146113567054e-08
303032,2418706,2418706,4837412,3556.475759744644,1.8348146113567054e-08
303392,2421584,2421584,4843168,3561.447790622711,1.834632712416351e-08
303753,2424470,2424470,4848940,3565.850157737732,1.8342689145356417e-08
304113,2427348,2427348,4854696,3570.3535108566284,1.8320861272513866e-08
304473,2430228,2430228,4860456,3575.126728773117,1.8320861272513866e-08
304834,2433112,2433112,4866224,3579.6575837135315,1.829357643146068e-08
305194,2435988,2435988,4871976,3584.217933654785,1.8291757442057133e-08
305554,2438868,2438868,4877736,3588.794379711151,1.8291757442057133e-08
305915,2441754,2441754,4883508,3594.2619268894196,1.8286300473846495e-08
306275,2444632,2444632,4889264,3598.596974849701,1.8282662495039403e-08
306635,2447510,2447510,4895020,3602.7017498016357,1.8246282706968486e-08
306995,2450388,2450388,4900776,3607.1153178215027,1.824446371756494e-08
307356,2453274,2453274,4906548,3611.5247616767883,1.823536877054721e-08
307716,2456152,2456152,4912304,3615.703008890152,1.822263584472239e-08
308076,2459032,2459032,4918064,3619.9882748126984,1.822263584472239e-08
308437,2461918,2461918,4923836,3624.359893798828,1.8198988982476294e-08
308797,2464798,2464798,4929596,3628.3992528915405,1.8198988982476294e-08
309157,2467676,2467676,4935352,3632.577778816223,1.8197169993072748e-08
309518,2470564,2470564,4941128,3636.8206589221954,1.8195351003669202e-08
309878,2473442,2473442,4946884,3641.6193726062775,1.819171302486211e-08
310238,2476320,2476320,4952640,3645.9803977012634,1.8186256056651473e-08
310599,2479206,2479206,4958412,3650.444263935089,1.8186256056651473e-08
310959,2482080,2482080,4964160,3655.418373823166,1.8153514247387648e-08
311319,2484958,2484958,4969916,3660.3740496635437,1.8146238289773464e-08
311680,2487846,2487846,4975692,3665.5468537807465,1.8146238289773464e-08
312040,2490724,2490724,4981448,3670.17453789711,1.8137143342755735e-08
312400,2493602,2493602,4987204,3674.6657857894897,1.812986738514155e-08
312761,2496490,2496490,4992980,3679.5925629138947,1.8128048395738006e-08
313121,2499368,2499368,4998736,3684.108011007309,1.811349648050964e-08
313481,2502248,2502248,5004496,3689.0499198436737,1.8111677491106093e-08
313842,2505136,2505136,5010272,3693.5738768577576,1.8111677491106093e-08
314202,2508012,2508012,5016024,3698.1604957580566,1.8106220522895455e-08
314562,2510888,2510888,5021776,3703.04611992836,1.8058926798403263e-08
314923,2513774,2513774,5027548,3707.606219768524,1.8058926798403263e-08
315283,2516650,2516650,5033300,3712.2971057891846,1.803346094675362e-08
315643,2519528,2519528,5039056,3716.574967622757,1.8031641957350075e-08
316004,2522414,2522414,5044828,3721.1160538196564,1.802982296794653e-08
316364,2525292,2525292,5050584,3725.5213136672974,1.8028003978542984e-08
316724,2528172,2528172,5056344,3730.9291257858276,1.8028003978542984e-08
317085,2531056,2531056,5062112,3736.2468717098236,1.7982529243454337e-08
317445,2533936,2533936,5067872,3743.5951647758484,1.798071025405079e-08
317805,2536814,2536814,5073628,3750.859871864319,1.7973434296436608e-08
318165,2539690,2539690,5079380,3758.54842877388,1.7953425412997603e-08
318526,2542576,2542576,5085152,3766.261151790619,1.7947968444786966e-08
318886,2545456,2545456,5090912,3773.9783828258514,1.794614945538342e-08
319246,2548336,2548336,5096672,3780.5006217956543,1.794614945538342e-08
319607,2551216,2551216,5102432,3785.658171892166,1.7898855730891228e-08
319967,2554096,2554096,5108192,3789.950305700302,1.7897036741487682e-08
320327,2556974,2556974,5113948,3793.9891607761383,1.789339876268059e-08
320688,2559862,2559862,5119724,3798.379609823227,1.789339876268059e-08
321048,2562736,2562736,5125472,3802.9503498077393,1.7771526472643018e-08
321408,2565616,2565616,5131232,3807.1512398719788,1.7771526472643018e-08
321769,2568500,2568500,5137000,3811.8356528282166,1.7760612536221743e-08
322129,2571380,2571380,5142760,3815.9933297634125,1.7760612536221743e-08
322489,2574256,2574256,5148512,3820.079509973526,1.775333657860756e-08
322850,2577144,2577144,5154288,3824.151716709137,1.7755155568011105e-08
323210,2580022,2580022,5160044,3828.2790546417236,1.7729689716361463e-08
323570,2582902,2582902,5165804,3832.4848897457123,1.7727870726957917e-08
323931,2585788,2585788,5171576,3836.705338716507,1.7727870726957917e-08
324291,2588664,2588664,5177328,3841.277996778488,1.7662387108430266e-08
324651,2591542,2591542,5183084,3845.7111258506775,1.7662387108430266e-08
325012,2594430,2594430,5188860,3850.457128763199,1.7662387108430266e-08
325372,2597310,2597310,5194620,3854.645491838455,1.766056811902672e-08
325732,2600188,2600188,5200376,3858.9981648921967,1.766056811902672e-08
326093,2603074,2603074,5206148,3863.1955115795135,1.761691237334162e-08
326453,2605954,2605954,5211908,3867.59570980072,1.7615093383938074e-08
326813,2608832,2608832,5217664,3872.273717880249,1.7613274394534528e-08
327174,2611718,2611718,5223436,3876.4550788402557,1.7609636415727437e-08
327534,2614596,2614596,5229192,3880.4774730205536,1.759872247930616e-08
327894,2617476,2617476,5234952,3884.6082158088684,1.759872247930616e-08
328255,2620358,2620358,5240716,3888.782961845398,1.7562342691235244e-08
328615,2623236,2623236,5246472,3893.546134710312,1.7535057850182056e-08
328975,2626114,2626114,5252228,3898.7606909275055,1.753323886077851e-08
329336,2629002,2629002,5258004,3903.0195248126984,1.7535057850182056e-08
329696,2631880,2631880,5263760,3907.443579673767,1.7516867956146598e-08
330056,2634760,2634760,5269520,3911.935358762741,1.7515048966743052e-08
330416,2637638,2637638,5275276,3916.1014268398285,1.7515048966743052e-08
330777,2640524,2640524,5281048,3920.447411775589,1.751141098793596e-08
331137,2643402,2643402,5286804,3925.2015948295593,1.7495040083304048e-08
331497,2646282,2646282,5292564,3930.2849338054657,1.7493221093900502e-08
331858,2649170,2649170,5298340,3934.706168651581,1.7495040083304048e-08
332218,2652040,2652040,5304080,3939.57084274292,1.734042598400265e-08
332578,2654920,2654920,5309840,3946.768500804901,1.7338606994599104e-08
332939,2657806,2657806,5315612,3954.1734778881073,1.7334969015792012e-08
333299,2660682,2660682,5321364,3961.8591496944427,1.7293132259510458e-08
333659,2663560,2663560,5327120,3969.6397025585175,1.7293132259510458e-08
334020,2666448,2666448,5332896,3977.0535638332367,1.7293132259510458e-08
334380,2669326,2669326,5338652,3983.643107652664,1.7291313270106912e-08
334740,2672204,2672204,5344408,3988.5992488861084,1.728767529129982e-08
335101,2675088,2675088,5350176,3992.927635908127,1.7245838535018265e-08
335461,2677968,2677968,5355936,3997.2320036888123,1.7245838535018265e-08
335821,2680846,2680846,5361692,4001.7359249591827,1.7242200556211174e-08
336182,2683732,2683732,5367464,4009.723568677902,1.7224010662175715e-08
336542,2686606,2686606,5373212,4017.6623265743256,1.7218553693965077e-08
336902,2689484,2689484,5378968,4025.155924797058,1.7209458746947348e-08
337263,2692370,2692370,5384740,4032.3579766750336,1.7207639757543802e-08
337623,2695250,2695250,5390500,4039.329527616501,1.720400177873671e-08
337983,2698128,2698128,5396256,4046.0127696990967,1.7176716937683523e-08
338344,2701012,2701012,5402024,4051.2434797286987,1.7176716937683523e-08
338704,2703892,2703892,5407784,4055.542356967926,1.7174897948279977e-08
339064,2706770,2706770,5413540,4059.720435857773,1.717307895887643e-08
339425,2709658,2709658,5419316,4064.258918762207,1.7171259969472885e-08
339785,2712536,2712536,5425072,4068.5967679023743,1.7165803001262248e-08
340145,2715414,2715414,5430828,4073.2399458885193,1.7162165022455156e-08
340506,2718302,2718302,5436604,4077.847771883011,1.7162165022455156e-08
340866,2721176,2721176,5442352,4082.2464456558228,1.7149432096630335e-08
341226,2724052,2724052,5448104,4086.407493829727,1.7143975128419697e-08
341587,2726940,2726940,5453880,4090.774323940277,1.714215613901615e-08
341947,2729816,2729816,5459632,4095.4947578907013,1.7140337149612606e-08
342307,2732694,2732694,5465388,4099.888446807861,1.7109414329752326e-08
342667,2735574,2735574,5471148,4104.626206874847,1.7109414329752326e-08
343028,2738460,2738460,5476920,4109.466094732285,1.710395736154169e-08
343388,2741338,2741338,5482676,4114.525926828384,1.709850039333105e-08
343748,2744218,2744218,5488436,4118.863149642944,1.7100319382734597e-08
344109,2747104,2747104,5494208,4123.375774860382,1.7096681403927505e-08
344469,2749982,2749982,5499964,4127.74947476387,1.7091224435716867e-08
344829,2752860,2752860,5505720,4131.945068597794,1.7080310499295592e-08
345190,2755748,2755748,5511496,4136.15613079071,1.7080310499295592e-08
345550,2758628,2758628,5517256,4140.388199806213,1.7078491509892046e-08
345910,2761500,2761500,5523000,4144.846319675446,1.7025740817189217e-08
346271,2764386,2764386,5528772,4149.2713396549225,1.7022102838382125e-08
346631,2767266,2767266,5534532,4153.528617858887,1.7022102838382125e-08
346991,2770144,2770144,5540288,4157.756012678146,1.701482688076794e-08
347352,2773028,2773028,5546056,4162.098173856735,1.6991180018521845e-08
347712,2775908,2775908,5551816,4166.232213973999,1.69893610291183e-08
348072,2778788,2778788,5557576,4170.484130620956,1.6987542039714754e-08
348433,2781674,2781674,5563348,4175.102346897125,1.696207618806511e-08
348793,2784554,2784554,5569108,4179.621218681335,1.6960257198661566e-08
349153,2787430,2787430,5574860,4183.953980922699,1.69457052834332e-08
349514,2790318,2790318,5580636,4188.4249086380005,1.69457052834332e-08
349874,2793196,2793196,5586392,4192.8143038749695,1.6942067304626107e-08
350234,2796076,2796076,5592152,4197.282493829727,1.6942067304626107e-08
350595,2798962,2798962,5597924,4202.664827823639,1.6938429325819016e-08
350955,2801840,2801840,5603680,4208.2084147930145,1.6907506505958736e-08
351315,2804718,2804718,5609436,4213.191251754761,1.6907506505958736e-08
351676,2807604,2807604,5615208,4218.341681718826,1.69020495377481e-08
352036,2810484,2810484,5620968,4222.809587955475,1.69020495377481e-08
352396,2813360,2813360,5626720,4226.903668880463,1.6898411558941007e-08
352757,2816248,2816248,5632496,4231.006661653519,1.689659256953746e-08
353117,2819124,2819124,5638248,4235.130917787552,1.687476469669491e-08
353477,2822002,2822002,5644004,4239.256595849991,1.6872945707291365e-08
353838,2824890,2824890,5649780,4243.414589881897,1.6872945707291365e-08
354198,2827768,2827768,5655536,4247.613415718079,1.6869307728484273e-08
354558,2830646,2830646,5661292,4252.0276618003845,1.6863850760273635e-08
354918,2833526,2833526,5667052,4256.143405675888,1.686203177087009e-08
355279,2836412,2836412,5672824,4260.329142570496,1.6858393792062998e-08
355639,2839292,2839292,5678584,4264.788489818573,1.6858393792062998e-08
355999,2842170,2842170,5684340,4268.898906707764,1.6856574802659452e-08
356360,2845056,2845056,5690112,4272.9347977638245,1.6854755813255906e-08
356720,2847934,2847934,5695868,4277.192501783371,1.6842022887431085e-08
357080,2850814,2850814,5701628,4281.491809606552,1.684384187683463e-08
357441,2853702,2853702,5707404,4285.751234769821,1.6842022887431085e-08
357801,2856580,2856580,5713160,4289.86142373085,1.684020389802754e-08
358161,2859456,2859456,5718912,4294.033836603165,1.6811100067570806e-08
358522,2862344,2862344,5724688,4299.153206586838,1.6811100067570806e-08
358882,2865220,2865220,5730440,4304.221641778946,1.680928107816726e-08
359242,2868098,2868098,5736196,4309.173952579498,1.680018613114953e-08
359603,2870986,2870986,5741972,4313.764647722244,1.6798367141745985e-08
359963,2873828,2873828,5747656,4318.172541856766,5.820766091346741e-11


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.008523941040039062,12064.44795143716
18,78,78,156,0.545835018157959,186.6780789084769
35,130,130,260,0.9698019027709961,52.03996526174706
53,182,182,364,1.3502981662750244,31.390393178175145
70,234,234,468,1.7225189208984375,23.792855511128437
88,288,288,576,2.128303050994873,13.383975569950053
105,344,344,688,2.6043498516082764,11.226262697015045
123,400,400,800,2.9871420860290527,6.399659026390509
141,456,456,912,3.351170063018799,4.988719561508333
158,510,510,1020,3.7232398986816406,3.448211087104937
176,566,566,1132,4.081860065460205,2.9030140740560455
193,628,628,1256,4.498257875442505,2.798770119148685
211,692,692,1384,5.043619155883789,2.447700696713582
229,756,756,1512,5.475239038467407,2.1403247818852833
246,814,814,1628,5.874090909957886,1.8867371270152944
264,876,876,1752,6.229607105255127,1.6031077646130143
281,934,934,1868,6.609287977218628,1.5252701746157982
299,1000,1000,2000,7.113217115402222,1.3431818714198016
316,1058,1058,2116,7.482725143432617,1.2664874232741568
334,1128,1128,2256,7.883991003036499,1.1101710653056216
352,1188,1188,2376,8.327441215515137,0.9636950304975471
369,1258,1258,2516,8.774407148361206,0.87101092652847
387,1318,1318,2636,9.237066984176636,0.7009521903055429
404,1374,1374,2748,9.576102018356323,0.5714227668559033
422,1446,1446,2892,10.009589910507202,0.5391367563479434
439,1518,1518,3036,10.587734937667847,0.47245098192433943
457,1584,1584,3168,11.00003719329834,0.45551057767988823
475,1650,1650,3300,11.449191093444824,0.4078379964339547
492,1716,1716,3432,11.848550081253052,0.3929713399429602
510,1780,1780,3560,12.199944972991943,0.35762860208524216
527,1838,1838,3676,12.570460796356201,0.33090880640156684
545,1902,1902,3804,12.98271894454956,0.3070690127369744
563,1968,1968,3936,13.494712114334106,0.29074154691443255
580,2040,2040,4080,13.982043027877808,0.2719217648555059
598,2110,2110,4220,14.452256917953491,0.26564294296076696
615,2170,2170,4340,14.848871946334839,0.24919297657106654
633,2244,2244,4488,15.262983083724976,0.2373433865050174
650,2310,2310,4620,15.633616209030151,0.227475689847779
668,2378,2378,4756,16.02666401863098,0.21458056677511195
686,2450,2450,4900,16.459550857543945,0.20297222315821273
703,2516,2516,5032,16.847686052322388,0.1979835620004451
721,2588,2588,5176,17.24881100654602,0.19269977658768767
738,2656,2656,5312,17.57779097557068,0.18583770886652928
756,2728,2728,5456,17.951308012008667,0.1760501370044949
773,2794,2794,5588,18.31699800491333,0.1698913127547712
791,2872,2872,5744,18.728942155838013,0.16329731778023415
809,2942,2942,5884,19.14528512954712,0.15506569339049747
826,3010,3010,6020,19.531729221343994,0.14898546385848022
844,3082,3082,6164,19.889671087265015,0.13840658656954474
861,3146,3146,6292,20.261607885360718,0.12795234242730658
879,3218,3218,6436,20.660335063934326,0.11906224482117977
897,3286,3286,6572,21.036291122436523,0.11721991901322326
914,3364,3364,6728,21.48008394241333,0.11069107493494812
932,3436,3436,6872,21.910665035247803,0.10888695742505661
949,3510,3510,7020,22.311100244522095,0.10763013629366469
967,3586,3586,7172,22.743237018585205,0.1057322159231262
984,3654,3654,7308,23.146135091781616,0.10523171477325377
1002,3726,3726,7452,23.550729990005493,0.10403917851181177
1020,3800,3800,7600,24.059110164642334,0.1015293894433853
1037,3868,3868,7736,24.550487995147705,0.09966841277127969
1055,3940,3940,7880,24.96114706993103,0.09832279377405939
1072,4010,4010,8020,25.338443994522095,0.09670935535541503
1090,4088,4088,8176,25.846252918243408,0.09348689385478792
1107,4156,4156,8312,26.267674207687378,0.09110278210755496
1125,4234,4234,8468,26.725542068481445,0.08788807355813333
1143,4314,4314,8628,27.310423135757446,0.08554775925040303
1160,4394,4394,8788,27.83256506919861,0.07909236179693835
1178,4508,4508,9016,28.53194308280945,0.07895669340723543
1195,4576,4576,9152,29.0047709941864,0.0787548444022832
1213,4648,4648,9296,29.46639895439148,0.07832095040976128
1231,4720,4720,9440,29.844398975372314,0.07805732872657245
1248,4788,4788,9576,30.268410205841064,0.07770945152697095
1266,4860,4860,9720,30.695609092712402,0.07725835209930665
1283,4928,4928,9856,31.110475063323975,0.07671861768358212
1301,5000,5000,10000,31.521543979644775,0.07576696926844306
1318,5068,5068,10136,31.97202706336975,0.07539443228415621
1336,5146,5146,10292,32.454379081726074,0.07475594474817626
1354,5258,5258,10516,33.07144021987915,0.07454996628621302
1371,5376,5376,10752,33.621039152145386,0.07446180805527547
1389,5504,5504,11008,34.22784996032715,0.07428604468441335
1406,5628,5628,11256,34.798628091812134,0.0742105614826869
1424,5766,5766,11532,35.58963394165039,0.07421123716630973
1441,5902,5902,11804,36.31736493110657,0.07421057616556936
1459,6046,6046,12092,37.02195191383362,0.07420987640580279
1477,6190,6190,12380,37.76164102554321,0.07420917678427941
1494,6326,6326,12652,38.40672516822815,0.07420851629285607
1512,6422,6422,12844,38.925060987472534,0.07399582759535406
1529,6498,6498,12996,39.3047080039978,0.07334019194058783
1547,6636,6636,13272,39.949265241622925,0.07333339225624513
1564,6768,6768,13536,40.563623905181885,0.07333035421106615
1582,6910,6910,13820,41.2497341632843,0.07332960193343752
1600,7050,7050,14100,41.901556968688965,0.07332841976676718
1617,7186,7186,14372,42.53762602806091,0.07332778036652599
1635,7330,7330,14660,43.214483976364136,0.07332710345144733
1652,7440,7440,14880,43.74110794067383,0.07316289164373302
1670,7512,7512,15024,44.116791009902954,0.07259251369214326
1688,7584,7584,15168,44.500104904174805,0.0703509640898119
1705,7652,7652,15304,44.852880001068115,0.06760904184739047
1723,7744,7744,15488,45.318695068359375,0.0645243733724783
1740,7840,7840,15680,45.791651010513306,0.06266497388423886
1758,7934,7934,15868,46.261778831481934,0.05991226545484096
1775,8006,8006,16012,46.62340712547302,0.05797107000944379
1793,8086,8086,16172,47.0198130607605,0.055519242716400186
1811,8200,8200,16400,47.58934020996094,0.051366101750318194
1828,8270,8270,16540,47.947964906692505,0.04931000967917498
1846,8368,8368,16736,48.43897008895874,0.04513350788147363
1863,8432,8432,16864,48.77931308746338,0.04441637552372413
1881,8508,8508,17016,49.16467308998108,0.04235202087147627
1898,8628,8628,17256,49.76086497306824,0.042337817652878584
1916,8766,8766,17532,50.47520995140076,0.04233678526543372
1934,8864,8864,17728,51.10572695732117,0.04225873280847736
1951,8932,8932,17864,51.487711906433105,0.04216218196961563
1969,9040,9040,18080,52.19878816604614,0.042090108938282356
1986,9174,9174,18348,52.87075400352478,0.042090412385732634
2004,9270,9270,18540,53.353610038757324,0.04203328695803066
2022,9366,9366,18732,53.85330820083618,0.04194276494126825
2039,9500,9500,19000,54.525131940841675,0.04194024002754304
2057,9644,9644,19288,55.25265192985535,0.041939938557334244
2074,9758,9758,19516,55.88354802131653,0.04188858088673442
2092,9888,9888,19776,56.60247015953064,0.04184613780853397
2109,10022,10022,20044,57.33397698402405,0.04184594533398922
2127,10160,10160,20320,57.99653601646423,0.041837825052425615
2145,10238,10238,20476,58.417054891586304,0.04160594208224211
2162,10306,10306,20612,58.79260492324829,0.040858187598132645
2180,10378,10378,20756,59.40687417984009,0.04052009352017194
2197,10466,10466,20932,59.95050382614136,0.04033674614765914
2215,10602,10602,21204,60.70676398277283,0.040333216051294585
2232,10720,10720,21440,61.33024501800537,0.04029477586846042
2250,10792,10792,21584,61.74459218978882,0.0401673544129153
2268,10864,10864,21728,62.22864007949829,0.040055680021396256
2285,10968,10968,21936,62.91841983795166,0.04000629514666798
2303,11108,11108,22216,63.75286293029785,0.04000604071006819
2320,11234,11234,22468,64.48812890052795,0.039968471335669165
2338,11320,11320,22640,65.02715396881104,0.03981168126301782
2356,11392,11392,22784,65.47428512573242,0.039610215866559884
2373,11460,11460,22920,65.95159387588501,0.03940086136572063
2391,11532,11532,23064,66.50221991539001,0.03892961228666536
2408,11610,11610,23220,67.03638005256653,0.03810218225589779
2426,11684,11684,23368,67.58377003669739,0.03738585050996335
2443,11752,11752,23504,68.0487310886383,0.036817678479565075
2461,11832,11832,23664,68.6975769996643,0.03523130999565183
2479,11942,11942,23884,69.4107928276062,0.034954862254380714
2496,12068,12068,24136,70.20440602302551,0.03480777388722345
2514,12206,12206,24412,71.0616660118103,0.03480180729275162
2531,12330,12330,24660,71.81856799125671,0.03478460891165014
2549,12402,12402,24804,72.25790619850159,0.03472452671849169
2566,12470,12470,24940,72.65760612487793,0.03463161746367405
2584,12542,12542,25084,73.09338688850403,0.03448598078284704
2602,12618,12618,25236,73.52142596244812,0.03432832358703308
2619,12686,12686,25372,73.94265222549438,0.03415210035745986
2637,12758,12758,25516,74.41770696640015,0.034042763960314915
2654,12888,12888,25776,75.17619919776917,0.03403196551153087
2672,13030,13030,26060,75.9875099658966,0.0340317599093396
2690,13148,13148,26296,76.73203301429749,0.034006799942289945
2707,13222,13222,26444,77.1757161617279,0.03390038332872791
2725,13294,13294,26588,77.63348293304443,0.03381265519601584
2742,13362,13362,26724,78.12707614898682,0.03364946367764787
2760,13438,13438,26876,78.58268117904663,0.0333410408529744
2777,13506,13506,27012,79.04088497161865,0.03299004089058144
2795,13578,13578,27156,79.52771925926208,0.03264416602360143
2813,13680,13680,27360,80.22253108024597,0.03251358694797091
2830,13806,13806,27612,80.91199612617493,0.03250740065050195
2848,13946,13946,27892,81.71867108345032,0.03250666927669954
2865,14022,14022,28044,82.18233609199524,0.032483992692505126
2883,14094,14094,28188,82.63901114463806,0.03241519443872676
2900,14162,14162,28324,83.02828311920166,0.03229077217838494
2918,14238,14238,28476,83.60348105430603,0.032159971098735696
2936,14310,14310,28620,84.07139301300049,0.03195683087869838
2953,14378,14378,28756,84.54113101959229,0.03186416369317158
2971,14450,14450,28900,85.01906609535217,0.03168441400157462
2988,14518,14518,29036,85.42106604576111,0.03141069114280981
3006,14590,14590,29180,85.8934919834137,0.030948915589760873
3024,14662,14662,29324,86.36121606826782,0.03046025154799281
3041,14730,14730,29460,86.78989005088806,0.030022271690540947
3059,14810,14810,29620,87.26087021827698,0.028814357763621956
3076,14886,14886,29772,87.71902203559875,0.027176566612979514
3094,14976,14976,29952,88.26751112937927,0.02638744842624874
3111,15110,15110,30220,89.14347100257874,0.026387212310510222
3129,15240,15240,30480,89.9553849697113,0.026380495490229805
3147,15338,15338,30676,90.5274109840393,0.02634680687697255
3164,15406,15406,30812,90.92484712600708,0.02630407502692833
3182,15478,15478,30956,91.35534310340881,0.026262699379003607
3199,15606,15606,31212,92.03050398826599,0.026258748741383897
3217,15750,15750,31500,92.75168800354004,0.026258635811245767
3234,15886,15886,31772,93.4345440864563,0.026258529176629963
3252,16030,16030,32060,94.15711903572083,0.02625841628287162
3270,16168,16168,32336,94.86783504486084,0.026258599133143434
3287,16300,16300,32600,95.55170392990112,0.02625850265212648
3305,16444,16444,32888,96.25719809532166,0.026258389831127715
3322,16580,16580,33160,96.93067598342896,0.02625828329655633
3340,16714,16714,33428,97.61455011367798,0.026242778096275288
3358,16824,16824,33648,98.19057822227478,0.026215071919068578
3375,16892,16892,33784,98.57954406738281,0.02616503918397939
3393,16990,16990,33980,99.10375714302063,0.026121965667698532
3410,17058,17058,34116,99.49130487442017,0.026065244577694102
3428,17130,17130,34260,99.89805316925049,0.02594316118666029
3445,17198,17198,34396,100.27371215820312,0.02587820162261778
3463,17270,17270,34540,100.66981506347656,0.02579127331773634
3481,17342,17342,34684,101.07755303382874,0.02570823692076374
3498,17410,17410,34820,101.45288181304932,0.025491299802524736
3516,17482,17482,34964,101.84963512420654,0.02531920409637678
3533,17550,17550,35100,102.240895986557,0.024990319669086603
3551,17626,17626,35252,102.68439197540283,0.024568217379055568
3568,17740,17740,35480,103.37634897232056,0.024526684332158766
3586,17878,17878,35756,104.1561689376831,0.024526814317141543
3604,18016,18016,36032,105.08208298683167,0.02452649185215705
3621,18148,18148,36296,105.93827700614929,0.024526383853299194
3639,18292,18292,36584,106.75659418106079,0.02452628310129512
3656,18378,18378,36756,107.41911125183105,0.02449397659074748
3674,18450,18450,36900,107.90521812438965,0.024429582117591053
3692,18522,18522,37044,108.33397817611694,0.02435453991893155
3709,18590,18590,37180,108.81491613388062,0.02429720657892176
3727,18662,18662,37324,109.35216999053955,0.024216623274696758
3744,18730,18730,37460,109.84938311576843,0.02417620209416782
3762,18802,18802,37604,110.3812038898468,0.024098694570056978
3779,18870,18870,37740,111.0084159374237,0.02402477322721097
3797,18942,18942,37884,111.5519630908966,0.023863075675762957
3815,19018,19018,38036,112.09682297706604,0.023612840530404355
3832,19086,19086,38172,112.53091716766357,0.023234433096149587
3850,19158,19158,38316,112.95603394508362,0.022780598141252995
3867,19236,19236,38472,113.51561903953552,0.021723235497120186
3885,19312,19312,38624,114.00390815734863,0.01972160160948988
3902,19380,19380,38760,114.45456790924072,0.018998856054167845
3920,19490,19490,38980,115.1525309085846,0.018647401846465073
3938,19596,19596,39192,115.7950451374054,0.018659541890883702
3955,19716,19716,39432,116.48945307731628,0.01859928679004952
3973,19836,19836,39672,117.18318009376526,0.018593362761748722
3990,19960,19960,39920,117.89746403694153,0.018589678236821783
4008,20098,20098,40196,118.68223094940186,0.018587480031783343
4025,20198,20198,40396,119.27022194862366,0.018525234150729375
4043,20270,20270,40540,119.72670412063599,0.018490253656636924
4061,20342,20342,40684,120.17842197418213,0.018468559319444466
4078,20410,20410,40820,120.6351969242096,0.018446740295985364
4096,20482,20482,40964,121.15259099006653,0.01844126507967303
4113,20550,20550,41100,121.66359186172485,0.01839108361127728
4131,20622,20622,41244,122.15210008621216,0.01833499560234486
4149,20694,20694,41388,122.61934518814087,0.018205746358944452
4166,20762,20762,41524,123.03242206573486,0.0180268891799642
4184,20834,20834,41668,123.46773600578308,0.01784447077443474
4201,20902,20902,41804,123.89955186843872,0.017636931217566598
4219,20974,20974,41948,124.34090495109558,0.01752824459981639
4236,21050,21050,42100,124.83719897270203,0.01718426701700082
4254,21122,21122,42244,125.30485510826111,0.01692548412938777
4272,21196,21196,42392,125.7641179561615,0.016321574667017558
4289,21264,21264,42528,126.260409116745,0.016121167534947745
4307,21342,21342,42684,126.7505431175232,0.015584370376018342
4324,21412,21412,42824,127.17525911331177,0.014690482741571032
4342,21502,21502,43004,127.79208302497864,0.01386903189268196
4359,21624,21624,43248,128.52743697166443,0.013870380071239197
4377,21744,21744,43488,129.2276029586792,0.013859320633855532
4395,21844,21844,43688,129.80545711517334,0.01385223228862742
4412,21974,21974,43948,130.55839204788208,0.013851939969754312
4430,22118,22118,44236,131.36100697517395,0.013851896257619956
4447,22216,22216,44432,131.9265170097351,0.013844327213519136
4465,22288,22288,44576,132.361093044281,0.013810319203912513
4483,22360,22360,44720,132.81728100776672,0.013786508974590106
4500,22428,22428,44856,133.23837304115295,0.013774424291113974
4518,22564,22564,45128,134.00305891036987,0.01377365419648413
4535,22642,22642,45284,134.4741690158844,0.013753324554272695
4553,22748,22748,45496,135.09693217277527,0.013737421086261747
4570,22880,22880,45760,135.8334288597107,0.013736609200350358
4588,22956,22956,45912,136.29758095741272,0.01372609926147561
4606,23028,23028,46056,136.7424190044403,0.013701612100703642
4623,23096,23096,46192,137.1652889251709,0.013652567549797823
4641,23172,23172,46344,137.6272828578949,0.013571686131399474
4658,23240,23240,46480,138.04583501815796,0.01343190068291733
4676,23312,23312,46624,138.49663090705872,0.013336078271095175
4693,23380,23380,46760,138.91206407546997,0.01331087830112665
4711,23452,23452,46904,139.3679769039154,0.013279866296215914
4729,23524,23524,47048,139.80642890930176,0.013149649170372868
4746,23592,23592,47184,140.22260189056396,0.013055095485469792
4764,23664,23664,47328,140.66240620613098,0.012818376282666577
4781,23732,23732,47464,141.08987307548523,0.012620019901078194
4799,23842,23842,47684,141.73637914657593,0.01260578407709545
4817,23974,23974,47948,142.48466086387634,0.012606457041329122
4834,24102,24102,48204,143.21557903289795,0.012606558089828468
4852,24234,24234,48468,143.97088098526,0.012602390517713502
4869,24308,24308,48616,144.41491508483887,0.012581143313582288
4887,24384,24384,48768,144.89505004882812,0.012567660298373085
4904,24458,24458,48916,145.3417489528656,0.012537724756839452
4922,24598,24598,49196,146.13024997711182,0.012537695958599215
4940,24710,24710,49420,146.76891016960144,0.012532046537671704
4957,24778,24778,49556,147.19289207458496,0.012515169129983406
4975,24850,24850,49700,147.64376711845398,0.012493170939706033
4992,24918,24918,49836,148.07389116287231,0.012472348344090278
5010,24990,24990,49980,148.52246713638306,0.012416091147315456
5027,25058,25058,50116,148.9388620853424,0.012361425451672403
5045,25178,25178,50356,149.63174080848694,0.012342407635514974
5063,25288,25288,50576,150.27484107017517,0.012338688147792709
5080,25396,25396,50792,150.896959066391,0.012335609548244975
5098,25476,25476,50952,151.38562512397766,0.012322412028879626
5115,25544,25544,51088,151.79587507247925,0.01229985743702855
5133,25632,25632,51264,152.33212304115295,0.012282744242838817
5151,25772,25772,51544,153.1202630996704,0.012281194403840345
5168,25906,25906,51812,153.86199188232422,0.012280903931241482
5186,26018,26018,52036,154.51976490020752,0.012268638836758328
5203,26088,26088,52176,154.94658708572388,0.012250086954736616
5221,26160,26160,52320,155.39313101768494,0.012222971927258186
5238,26228,26228,52456,155.80633997917175,0.012180584702946362
5256,26326,26326,52652,156.3978888988495,0.012121727590056253
5274,26422,26422,52844,156.97381711006165,0.01196530547895236
5291,26496,26496,52992,157.4249279499054,0.011478279273433145
5309,26568,26568,53136,157.88466620445251,0.01089015879733779
5326,26636,26636,53272,158.30004000663757,0.009480361213718425
5344,26712,26712,53424,158.78026914596558,0.008859945262884139
5361,26780,26780,53560,159.20347118377686,0.008370275021661655
5379,26896,26896,53792,159.86822390556335,0.008171864137693774
5397,27010,27010,54020,160.51787495613098,0.008180136581358965
5414,27120,27120,54240,161.16302800178528,0.00817768545493891
5432,27248,27248,54496,161.88889908790588,0.008173308722689399
5449,27366,27366,54732,162.57725310325623,0.008171301298716571
5467,27498,27498,54996,163.3320550918579,0.008170939971023472
5485,27638,27638,55276,164.11354994773865,0.008170922150384285
5502,27762,27762,55524,164.81671810150146,0.008170397404683172
5520,27840,27840,55680,165.29429292678833,0.008162858459400013
5537,27908,27908,55816,165.72025203704834,0.008146494461470866
5555,27994,27994,55988,166.23602890968323,0.008135874093568418
5572,28126,28126,56252,166.98286700248718,0.008135730580761447
5590,28270,28270,56540,167.78539109230042,0.008135711001159507
5608,28414,28414,56828,168.59288215637207,0.008135691427014535
5625,28504,28504,57008,169.12176704406738,0.008129452146022231
5643,28576,28576,57152,169.57958602905273,0.008119266480207443
5660,28644,28644,57288,170.0054430961609,0.008113528370813583
5678,28716,28716,57432,170.4404001235962,0.00809843152637768
5695,28830,28830,57660,171.0909869670868,0.00809202471646131
5713,28972,28972,57944,171.886461019516,0.008091957608485245
5731,29116,29116,58232,172.68498396873474,0.008091938982033753
5748,29230,29230,58460,173.3424859046936,0.008089511711659725
5766,29302,29302,58604,173.78017783164978,0.008079374634689884
5783,29370,29370,58740,174.20945620536804,0.008074845376540907
5801,29442,29442,58884,174.65987610816956,0.008056907281570602
5819,29514,29514,59028,175.0967080593109,0.008007414977328153
5836,29582,29582,59164,175.51601004600525,0.00795119142094336
5854,29654,29654,59308,175.96108412742615,0.007932945951324655
5871,29722,29722,59444,176.38174414634705,0.007923986624518875
5889,29794,29794,59588,176.82802891731262,0.007913189259852516
5906,29862,29862,59724,177.25171494483948,0.00788600959640462
5924,29934,29934,59868,177.7088439464569,0.007842152186640305
5942,30012,30012,60024,178.19022011756897,0.007811032402969431
5959,30080,30080,60160,178.6309711933136,0.0077713203099847306
5977,30152,30152,60304,179.07430815696716,0.007735495979432017
5994,30220,30220,60440,179.48997902870178,0.007652421752936789
6012,30296,30296,60592,179.950679063797,0.007554743910077377
6029,30364,30364,60728,180.37750005722046,0.007499740384446341
6047,30436,30436,60872,180.8351800441742,0.007438555378030287
6065,30508,30508,61016,181.28532910346985,0.007355783289312967
6082,30576,30576,61152,181.71383023262024,0.007242336734634591
6100,30648,30648,61296,182.18061518669128,0.007210789815871976
6117,30716,30716,61432,182.61383390426636,0.007160437411585008
6135,30792,30792,61584,183.08780002593994,0.006943693364519277
6153,30868,30868,61736,183.5629198551178,0.006717043439493864
6170,30940,30940,61880,184.01540207862854,0.006535545577207813
6188,31012,31012,62024,184.46927785873413,0.006334904303002986
6205,31084,31084,62168,184.9262478351593,0.006195413048772025
6223,31158,31158,62316,185.38512301445007,0.006154844615593902
6240,31226,31226,62452,185.8141520023346,0.00604445305725676
6258,31298,31298,62596,186.2640061378479,0.005842124599439558
6276,31370,31370,62740,186.7110080718994,0.005649297345371451
6293,31442,31442,62884,187.17379093170166,0.005510435368705657
6311,31514,31514,63028,187.64945006370544,0.005373657748350524
6328,31586,31586,63172,188.1236321926117,0.005275599572996725
6346,31658,31658,63316,188.60972118377686,0.0051757395413005725
6363,31726,31726,63452,189.05004501342773,0.00503670180842164
6381,31798,31798,63596,189.52609705924988,0.004909123383185943
6399,31870,31870,63740,190.02074098587036,0.004620091784090619
6416,31938,31938,63876,190.47470784187317,0.004186211936030304
6434,32034,32034,64068,191.09317708015442,0.004099266712728422
6451,32154,32154,64308,191.82345008850098,0.004042110869704629
6469,32258,32258,64516,192.44185209274292,0.004039587853185367
6486,32374,32374,64748,193.14999103546143,0.0040383432951784926
6504,32518,32518,65036,194.07416915893555,0.004038331302581355
6522,32600,32600,65200,194.64214611053467,0.004035298074086313
6539,32670,32670,65340,195.0757281780243,0.004029777706819004
6557,32766,32766,65532,195.6422519683838,0.004026773860459798
6574,32834,32834,65668,196.07771801948547,0.004021072660179925
6592,32906,32906,65812,196.52176094055176,0.003990070053987438
6610,32978,32978,65956,196.96317887306213,0.003964629300753586
6627,33046,33046,66092,197.38338994979858,0.00394159770985425
6645,33118,33118,66236,197.8403241634369,0.0039279970314964885
6662,33186,33186,66372,198.26970314979553,0.003907657994204783
6680,33258,33258,66516,198.71776795387268,0.0038851795143273193
6697,33326,33326,66652,199.1416370868683,0.0038764416312915273
6715,33398,33398,66796,199.59131503105164,0.0038664105431962525
6733,33470,33470,66940,200.04475378990173,0.003853693833661964
6750,33538,33538,67076,200.47167420387268,0.00384491323166003
6768,33610,33610,67220,200.9136519432068,0.0038315946239890764
6785,33678,33678,67356,201.34684205055237,0.0038242170703597367
6803,33750,33750,67500,201.79806995391846,0.0038155211150296964
6820,33818,33818,67636,202.21934509277344,0.0038113771752250614
6838,33890,33890,67780,202.67801809310913,0.0037995540551492013
6856,33962,33962,67924,203.11886310577393,0.003781776094911038
6873,34030,34030,68060,203.5418210029602,0.0037552217254415154
6891,34102,34102,68204,203.98447799682617,0.003737160002856399
6908,34170,34170,68340,204.40234899520874,0.0037210530226730043
6926,34242,34242,68484,204.85165214538574,0.0037025295769126387
6944,34314,34314,68628,205.29064297676086,0.003687470116346958
6961,34382,34382,68764,205.79144406318665,0.0036603408116206992
6979,34454,34454,68908,206.23673486709595,0.00364053996054281
6996,34522,34522,69044,206.67499899864197,0.0036237539916328387
7014,34594,34594,69188,207.1325650215149,0.0035862187814927893
7031,34662,34662,69324,207.56559109687805,0.0035538304637157125
7049,34734,34734,69468,208.0306429862976,0.003481805484625511
7067,34806,34806,69612,208.48696899414062,0.0034582694843265926
7084,34874,34874,69748,208.91766905784607,0.00342713249483495
7102,34946,34946,69892,209.39818596839905,0.003360558217536891
7119,35014,35014,70028,209.8230540752411,0.003275851282523945
7137,35086,35086,70172,210.28209400177002,0.003178304777975427
7154,35154,35154,70308,210.702810049057,0.0030798253064858727
7172,35226,35226,70452,211.15587496757507,0.0030357458508660784
7190,35352,35352,70704,211.87515592575073,0.0030222718778532
7207,35474,35474,70948,212.56598901748657,0.003022025795871741
7225,35614,35614,71228,213.37332391738892,0.003021984330189298
7242,35708,35708,71416,213.92241883277893,0.0030213120953703765
7260,35782,35782,71564,214.38041591644287,0.0030204085778677836
7278,35854,35854,71708,214.83151197433472,0.0030191782425390556
7295,35922,35922,71844,215.24862003326416,0.0030154550968291005
7313,35994,35994,71988,215.70488214492798,0.003008557207067497
7330,36062,36062,72124,216.1262969970703,0.0030046626889088657
7348,36134,36134,72268,216.55832695960999,0.0030010210484761046
7365,36202,36202,72404,216.97973203659058,0.002996529256051872
7383,36274,36274,72548,217.4153871536255,0.0029892684196966
7401,36346,36346,72692,217.8757610321045,0.0029776458777632797
7418,36414,36414,72828,218.30001401901245,0.002965821484394837
7436,36486,36486,72972,218.74509596824646,0.0029605413328681607
7453,36554,36554,73108,219.16454195976257,0.0029565419936261605
7471,36626,36626,73252,219.6051061153412,0.0029518049814214464
7488,36694,36694,73388,220.04410696029663,0.0029450468719005585
7506,36766,36766,73532,220.47873306274414,0.002926752718849457
7524,36838,36838,73676,220.91318082809448,0.0029176470397942467
7541,36906,36906,73812,221.33536314964294,0.0029020361689617857
7559,36978,36978,73956,221.7783968448639,0.0028838900434493553
7576,37046,37046,74092,222.20946192741394,0.002861809267415083
7594,37118,37118,74236,222.65412187576294,0.002817647155097802
7612,37190,37190,74380,223.10288000106812,0.002784195490676211
7629,37258,37258,74516,223.52048802375793,0.0027581742506299634
7647,37330,37330,74660,223.95103788375854,0.002725969583480037
7664,37400,37400,74800,224.39624691009521,0.002677054344530916
7682,37472,37472,74944,224.83997702598572,0.0026507882812438766
7699,37540,37540,75080,225.26056504249573,0.002614579763758229
7717,37612,37612,75224,225.70110297203064,0.0025389223392267013
7735,37684,37684,75368,226.15409088134766,0.0023649565173400333
7752,37754,37754,75508,226.5911250114441,0.0022144558733998565
7770,37826,37826,75652,227.03689002990723,0.002087119990392239
7787,37900,37900,75800,227.49165511131287,0.0018970614910358563
7805,37988,37988,75976,228.01623916625977,0.0016976477418211289
7822,38110,38110,76220,228.70877695083618,0.001695095614195452
7840,38248,38248,76496,229.4879879951477,0.0016950179706327617
7858,38392,38392,76784,230.28879618644714,0.0016950116969383089
7875,38454,38454,76908,230.69243597984314,0.0016905606662476202
7893,38526,38526,77052,231.15338706970215,0.0016900438731681788
7910,38594,38594,77188,231.57673001289368,0.0016893879437702708
7928,38666,38666,77332,232.02274203300476,0.0016883714888535906
7946,38738,38738,77476,232.458172082901,0.0016870250274223508
7963,38806,38806,77612,232.88303518295288,0.0016861135372892022
7981,38878,38878,77756,233.3412630558014,0.0016848885679792147
7998,38946,38946,77892,233.75241208076477,0.0016829090636747424
8016,39018,39018,78036,234.2042829990387,0.001680854549704236
8033,39086,39086,78172,234.617928981781,0.0016776471238699742
8051,39158,39158,78316,235.07199692726135,0.0016722034615668235
8069,39230,39230,78460,235.5247721672058,0.0016686677627149038
8086,39298,39298,78596,235.94563508033752,0.0016669047381583368
8104,39370,39370,78740,236.38514494895935,0.0016573666034673806
8121,39438,39438,78876,236.79933404922485,0.001647879771553562
8139,39510,39510,79020,237.2606270313263,0.0016294463694066508
8156,39578,39578,79156,237.6875069141388,0.0016166757668543141
8174,39650,39650,79300,238.13563108444214,0.001601913025297108
8192,39722,39722,79444,238.59161901474,0.0015865312016103417
8209,39790,39790,79580,239.01021313667297,0.001580852089318796
8227,39862,39862,79724,239.4533019065857,0.0015664552011003252
8244,39930,39930,79860,239.88110208511353,0.0015535499405814335
8262,40002,40002,80004,240.3205590248108,0.0015541652755928226
8280,40074,40074,80148,240.76506304740906,0.0015343930244853254
8297,40142,40142,80284,241.18977308273315,0.0015190195063041756
8315,40214,40214,80428,241.64485907554626,0.00150893130012264
8332,40286,40286,80572,242.08255004882812,0.001490674976594164
8350,40382,40382,80764,242.6490020751953,0.0014778006661799736
8367,40500,40500,81000,243.3128640651703,0.0014789859360462287
8385,40628,40628,81256,244.06019616127014,0.0014785840085096424
8403,40768,40768,81536,244.85751509666443,0.001478671700169798
8420,40900,40900,81800,245.60486388206482,0.0014777528631384484
8438,41040,41040,82080,246.40218806266785,0.0014776787284063175
8455,41174,41174,82348,247.17049288749695,0.0014776770094613312
8473,41318,41318,82636,248.00115084648132,0.0014776734242332168
8490,41444,41444,82888,248.7249038219452,0.0014775723921047756
8508,41528,41528,83056,249.24086022377014,0.0014766865915589733
8526,41600,41600,83200,249.6926920413971,0.0014746030210517347
8543,41668,41668,83336,250.1240701675415,0.0014705532321386272
8561,41740,41740,83480,250.59250807762146,0.0014613480689149583
8578,41808,41808,83616,251.0169689655304,0.001456582695027464
8596,41880,41880,83760,251.46322894096375,0.0014520109707518714
8614,41976,41976,83952,252.03485298156738,0.001447796526917955
8631,42094,42094,84188,252.70384001731873,0.001447954740797286
8649,42212,42212,84424,253.4076120853424,0.0014478724042419344
8666,42346,42346,84692,254.17509293556213,0.0014477140794042498
8684,42488,42488,84976,255.26796007156372,0.0014476913656835677
8701,42624,42624,85248,256.03619289398193,0.0014476880824076943
8719,42766,42766,85532,256.82829904556274,0.0014476831256615696
8737,42910,42910,85820,257.6367690563202,0.0014476796495728195
8754,43038,43038,86076,258.3566892147064,0.0014467047221842222
8772,43122,43122,86244,258.8681719303131,0.0014433751130127348
8789,43190,43190,86380,259.30317401885986,0.0014412937525776215
8807,43262,43262,86524,259.74973320961,0.0014408285151148448
8824,43330,43330,86660,260.16955494880676,0.0014396651276911143
8842,43402,43402,86804,260.6181402206421,0.00143824301812856
8860,43474,43474,86948,261.06806802749634,0.001437261898900033
8877,43542,43542,87084,261.5037889480591,0.0014355462535604602
8895,43614,43614,87228,261.9468448162079,0.0014314974832814187
8912,43682,43682,87364,262.3651828765869,0.0014208963420969667
8930,43754,43754,87508,262.8012809753418,0.0014110976408119313
8947,43822,43822,87644,263.2201430797577,0.0013869471677026013
8965,43894,43894,87788,263.68461298942566,0.0013237965376902139
8983,43966,43966,87932,264.1311049461365,0.0012812032418878516
9000,44034,44034,88068,264.5462441444397,0.0012626292791537708
9018,44106,44106,88212,265.0093159675598,0.0012593337032740237
9035,44174,44174,88348,265.41939997673035,0.0012465621184674092
9053,44246,44246,88492,265.8746769428253,0.0012320387013460277
9071,44318,44318,88636,266.3075420856476,0.001217236917000264
9088,44386,44386,88772,266.7331099510193,0.0012121684976591496
9106,44458,44458,88916,267.1724269390106,0.0012015514657832682
9123,44530,44530,89060,267.61313104629517,0.0011883013721671887
9141,44602,44602,89204,268.065447807312,0.001157748100013123
9158,44670,44670,89340,268.4849531650543,0.0011250974330323515
9176,44742,44742,89484,268.9287760257721,0.0010532398719078628
9194,44814,44814,89628,269.3716778755188,0.0009688213795016054
9211,44882,44882,89764,269.78682017326355,0.000904743783394224
9229,44954,44954,89908,270.2385039329529,0.0008737725311220856
9246,45026,45026,90052,270.6846570968628,0.0008357916831300827
9264,45102,45102,90204,271.1519470214844,0.0007303331767616328
9281,45170,45170,90340,271.58580708503723,0.0007268191584444139
9299,45242,45242,90484,272.03606510162354,0.0006561591617355589
9317,45318,45318,90636,272.5163850784302,0.0005036812381149502
9334,45392,45392,90784,272.9617249965668,0.0004523912193690194
9352,45468,45468,90936,273.419771194458,0.00036558655119733885
9369,45536,45536,91072,273.84405493736267,0.0002830583780450979
9387,45638,45638,91276,274.4509561061859,0.00024119429326674435
9405,45744,45744,91488,275.0829141139984,0.00024864643819455523
9422,45840,45840,91680,275.6311228275299,0.0002454401364957448
9440,45972,45972,91944,276.37260603904724,0.0002520927409932483
9457,46090,46090,92180,277.0539610385895,0.00024066955847956706
9475,46200,46200,92400,277.6826000213623,0.00024274415227409918
9492,46314,46314,92628,278.33503794670105,0.0002410593442618847
9510,46438,46438,92876,279.0493860244751,0.0002403953294560779
9528,46574,46574,93148,279.8015179634094,0.00024039613708737306
9545,46702,46702,93404,280.5305540561676,0.00024039545496634673
9563,46844,46844,93688,281.3238480091095,0.0002403938415227458
9580,46972,46972,93944,282.0533890724182,0.000240077437410946
9598,47032,47032,94064,282.44266390800476,0.00023962733030202799
9615,47098,47098,94196,282.8607852458954,0.00023943864653119817
9633,47170,47170,94340,283.3153541088104,0.0002391540056123631
9651,47240,47240,94480,283.77162504196167,0.00023865421098889783
9668,47310,47310,94620,284.21414399147034,0.00023833375234971754
9686,47382,47382,94764,284.66203904151917,0.0002380777496000519
9703,47450,47450,94900,285.09081387519836,0.000237802119954722
9721,47522,47522,95044,285.55673694610596,0.0002370625861658482
9739,47594,47594,95188,286.00532603263855,0.00023574416627525352
9756,47702,47702,95404,286.6274869441986,0.0002349266505916603
9774,47794,47794,95588,287.17506885528564,0.000234790355534642
9791,47928,47928,95856,287.9313440322876,0.00023478883122152183
9809,48052,48052,96104,288.648638010025,0.0002347317185922293
9826,48154,48154,96308,289.23221707344055,0.0002344589156564325
9844,48298,48298,96596,290.05710792541504,0.00023445827719115186
9862,48428,48428,96856,290.78179597854614,0.00023442374003934674
9879,48496,48496,96992,291.20616006851196,0.00023430288820236456
9897,48568,48568,97136,291.65761613845825,0.00023271836653293576
9914,48636,48636,97272,292.0907380580902,0.00023137012613005936
9932,48708,48708,97416,292.53445291519165,0.00023072879230312537
9949,48776,48776,97552,292.9446110725403,0.0002285295158799272
9967,48848,48848,97696,293.39341592788696,0.00022634949345956556
9985,48920,48920,97840,293.83472895622253,0.0002238841298094485
10002,48988,48988,97976,294.2660129070282,0.00022367535348166712
10020,49060,49060,98120,294.7095820903778,0.000223223551074625
10037,49128,49128,98256,295.1369888782501,0.0002226449578301981
10055,49200,49200,98400,295.5899691581726,0.00022224232270673383
10073,49272,49272,98544,296.0454828739166,0.0002218363206338836
10090,49340,49340,98680,296.47853684425354,0.00022142099624034017
10108,49416,49416,98832,296.94588899612427,0.00022127771080704406
10125,49484,49484,98968,297.3762800693512,0.00022109189194452483
10143,49560,49560,99120,297.8484752178192,0.00022061208437662572
10160,49628,49628,99256,298.26730394363403,0.00022029256797395647
10178,49700,49700,99400,298.71511006355286,0.00021981890859024134
10196,49772,49772,99544,299.15923404693604,0.00021889450727030635
10213,49840,49840,99680,299.5847120285034,0.0002175496756535722
10231,49912,49912,99824,300.0163309574127,0.00021617931997752748
10248,49980,49980,99960,300.43440890312195,0.00021273571292113047
10266,50052,50052,100104,300.882737159729,0.000205797994567547
10283,50120,50120,100240,301.29133200645447,0.00020037022295582574
10301,50192,50192,100384,301.73591899871826,0.00019491208331601229
10319,50264,50264,100528,302.1772999763489,0.00018904679745901376
10336,50332,50332,100664,302.60194087028503,0.00018238758275401779
10354,50404,50404,100808,303.0472528934479,0.0001709638090687804
10371,50472,50472,100944,303.4609489440918,0.0001599399056431139
10389,50544,50544,101088,303.8988130092621,0.00014700911196996458
10407,50618,50618,101236,304.3497290611267,0.00014114294026512653
10424,50686,50686,101372,304.77114391326904,0.00014007023128215224
10442,50762,50762,101524,305.2404520511627,0.00012189529479655903
10459,50830,50830,101660,305.6557459831238,0.0001148887076851679
10477,50902,50902,101804,306.10032510757446,0.00010475193084857892
10494,51008,51008,102016,306.71082401275635,0.000103642374597257
10512,51138,51138,102276,307.45897221565247,0.00010342069435864687
10530,51242,51242,102484,308.0726499557495,0.00010336796185583808
10547,51378,51378,102756,308.81920623779297,0.00010336759078199975
10565,51454,51454,102908,309.2947430610657,0.00010324814684281591
10582,51522,51522,103044,309.7150650024414,0.00010321127047063783
10600,51594,51594,103188,310.1639349460602,0.00010316825137124397
10617,51662,51662,103324,310.5826590061188,0.00010312612539564725
10635,51734,51734,103468,311.0243079662323,0.00010299366840627044
10653,51806,51806,103612,311.4759521484375,0.00010250188097415958
10670,51874,51874,103748,311.90017199516296,0.00010184966413362417
10688,51946,51946,103892,312.3523051738739,0.00010166763422603253
10705,52014,52014,104028,312.76515102386475,0.00010141648999706376
10723,52086,52086,104172,313.2082450389862,0.00010090160867548548
10741,52158,52158,104316,313.66693091392517,0.00010045789349533152
10758,52226,52226,104452,314.0883700847626,0.00010023588220064994
10776,52298,52298,104596,314.54194712638855,0.00010003837996919174
10793,52366,52366,104732,314.9696629047394,9.971853251045104e-05
10811,52438,52438,104876,315.40252900123596,9.915515511238482e-05
10828,52506,52506,105012,315.83110904693604,9.884091377898585e-05
10846,52578,52578,105156,316.288724899292,9.877719276119024e-05
10864,52650,52650,105300,316.7293059825897,9.859442798187956e-05
10881,52720,52720,105440,317.1635630130768,9.824397966440301e-05
10899,52792,52792,105584,317.6043050289154,9.76749124674825e-05
10916,52860,52860,105720,318.0371539592743,9.754752863955218e-05
10934,52932,52932,105864,318.4813129901886,9.730656347528566e-05
10951,53000,53000,106000,318.9026801586151,9.71981389739085e-05
10969,53072,53072,106144,319.3499331474304,9.691367449704558e-05
10987,53144,53144,106288,319.7840430736542,9.659554234531242e-05
11004,53212,53212,106424,320.2171981334686,9.638520896260161e-05
11022,53284,53284,106568,320.66186594963074,9.581505582900718e-05
11039,53356,53356,106712,321.10296297073364,9.559195132169407e-05
11057,53428,53428,106856,321.5461881160736,9.505678463028744e-05
11075,53500,53500,107000,321.99758100509644,9.463752030569594e-05
11092,53568,53568,107136,322.4241452217102,9.378116010339e-05
11110,53640,53640,107280,322.85344099998474,9.355902511742897e-05
11127,53708,53708,107416,323.26676082611084,9.26680750126252e-05
11145,53780,53780,107560,323.7129981517792,9.13631356525002e-05
11162,53848,53848,107696,324.14174699783325,9.088255501410458e-05
11180,53920,53920,107840,324.59850811958313,9.00181275937939e-05
11198,53992,53992,107984,325.04811120033264,8.936119593272451e-05
11215,54060,54060,108120,325.4686179161072,8.837439054332208e-05
11233,54132,54132,108264,325.905305147171,8.801575313555077e-05
11250,54200,54200,108400,326.31748604774475,8.69482355483342e-05
11268,54272,54272,108544,326.7752799987793,8.477127266814932e-05
11285,54340,54340,108680,327.2001910209656,8.12177240732126e-05
11303,54416,54416,108832,327.6695590019226,7.731395817245357e-05
11321,54488,54488,108976,328.11119318008423,7.294298666238319e-05
11338,54556,54556,109112,328.52862524986267,7.007899512245785e-05
11356,54628,54628,109256,328.98190903663635,6.30374106549425e-05
11373,54696,54696,109392,329.4003219604492,5.7625964473118074e-05
11391,54766,54766,109532,329.83529806137085,4.69499354949221e-05
11408,54834,54834,109668,330.25649189949036,4.091543814865872e-05
11426,54906,54906,109812,330.6993169784546,3.989858851127792e-05
11444,54974,54974,109948,331.14095091819763,3.645724427769892e-05
11461,55040,55040,110080,331.5488979816437,2.8676089641521685e-05
11479,55106,55106,110212,331.96558594703674,2.3979244360816665e-05
11496,55168,55168,110336,332.36027002334595,1.8356442524236627e-05
11514,55240,55240,110480,332.80074310302734,1.677115142229013e-05
11532,55310,55310,110620,333.24342918395996,1.6061732821981423e-05
11549,55378,55378,110756,333.6677510738373,1.6867881640791893e-05
11567,55442,55442,110884,334.0772850513458,1.363454430247657e-05
11584,55506,55506,111012,334.47969102859497,1.1780237400671467e-05
11602,55576,55576,111152,334.90942001342773,1.1317115422571078e-05
11619,55640,55640,111280,335.30877113342285,9.78926800598856e-06
11637,55708,55708,111416,335.7449531555176,7.999313311302103e-06
11655,55778,55778,111556,336.1932919025421,6.615675374632701e-06
11672,55846,55846,111692,336.61773014068604,5.493222488439642e-06
11690,55916,55916,111832,337.0620369911194,5.012418114347383e-06
11707,55984,55984,111968,337.47475004196167,4.788058504345827e-06
11725,56056,56056,112112,337.96133303642273,3.994640792370774e-06
11742,56122,56122,112244,338.376051902771,3.524299245327711e-06
11760,56190,56190,112380,338.80019998550415,2.6945363060804084e-06
11778,56254,56254,112508,339.21297311782837,2.080601916532032e-06
11795,56312,56312,112624,339.5832939147949,1.6603898984612897e-06
11813,56374,56374,112748,339.99017000198364,1.2346663424978033e-06
11830,56428,56428,112856,340.32919812202454,5.49189280718565e-07
11848,56488,56488,112976,340.7160098552704,2.2394669940695167e-07
11866,56550,56550,113100,341.11321210861206,1.7676211427897215e-07
11883,56602,56602,113204,341.4483959674835,7.389462552964687e-08
11901,56662,56662,113324,341.8332860469818,7.536800694651902e-08
11918,56718,56718,113436,342.20435094833374,5.477704689837992e-08
11936,56782,56782,113564,342.61551785469055,3.713830665219575e-08
11953,56840,56840,113680,342.98881793022156,2.74376361630857e-08
11971,56898,56898,113796,343.3552739620209,1.5519617591053247e-08
11989,56960,56960,113920,343.7490129470825,1.3489625416696072e-08
12006,57024,57024,114048,344.1659698486328,1.1497832019813359e-08
12024,57088,57088,114176,344.57024097442627,1.0459189070388675e-08
12041,57146,57146,114292,344.93530011177063,9.897121344693005e-09
12059,57214,57214,114428,345.3643569946289,1.0144503903575242e-08
12076,57276,57276,114552,345.7522349357605,1.0601070243865252e-08
12094,57336,57336,114672,346.1397738456726,1.1033989721909165e-08
12112,57400,57400,114800,346.56052803993225,1.2096279533579946e-08
12129,57468,57468,114936,346.9719910621643,1.2239979696460068e-08
12147,57534,57534,115068,347.38385701179504,1.1772499419748783e-08
12164,57604,57604,115208,347.81546998023987,1.1394149623811245e-08
12182,57674,57674,115348,348.24487709999084,1.1063093552365899e-08
12200,57750,57750,115500,348.7126362323761,1.0990333976224065e-08
12217,57816,57816,115632,349.12638306617737,1.0952135198749602e-08
12235,57882,57882,115764,349.5457270145416,1.0804797057062387e-08
12252,57942,57942,115884,349.91609501838684,1.0479197953827679e-08
12270,58002,58002,116004,350.2870240211487,1.0275471140630543e-08
12287,58070,58070,116140,350.78876304626465,1.0111762094311416e-08
12305,58140,58140,116280,351.2380449771881,1.0029907571151853e-08
12323,58206,58206,116412,351.67058086395264,9.78070602286607e-09
12340,58270,58270,116540,352.08577609062195,9.516952559351921e-09
12358,58342,58342,116684,352.5355272293091,9.43873601499945e-09
12375,58410,58410,116820,352.9610469341278,9.391442290507257e-09
12393,58480,58480,116960,353.3968198299408,9.265932021662593e-09
12410,58548,58548,117096,353.8126268386841,9.07857611309737e-09
12428,58620,58620,117240,354.25100207328796,8.947608876042068e-09
12446,58692,58692,117384,354.69634199142456,8.87666828930378e-09
12463,58764,58764,117528,355.15522503852844,8.813003660179675e-09
12481,58840,58840,117680,355.62704706192017,8.8020897237584e-09
12498,58910,58910,117820,356.06824493408203,8.77116690389812e-09
12516,58986,58986,117972,356.53270387649536,8.747520041652024e-09
12534,59066,59066,118132,357.02104806900024,8.70932126417756e-09
12551,59138,59138,118276,357.47382712364197,8.700226317159832e-09
12569,59214,59214,118428,357.9383909702301,8.702045306563377e-09
12586,59296,59296,118592,358.42308616638184,8.698407327756286e-09
12604,59374,59374,118748,358.89332818984985,8.694769348949194e-09
12621,59446,59446,118892,359.3347849845886,8.689312380738556e-09
12639,59538,59538,119076,359.889906167984,8.682036423124373e-09
12657,59614,59614,119228,360.34460496902466,8.656570571474731e-09
12674,59702,59702,119404,360.8629810810089,8.647475624457002e-09
12692,59810,59810,119620,361.5025670528412,8.642018656246364e-09
12709,59894,59894,119788,362.00697803497314,8.623828762210906e-09
12727,59984,59984,119968,362.54458379745483,8.620190783403814e-09
12744,60066,60066,120132,363.0304071903229,8.611095836386085e-09
12762,60158,60158,120316,363.5738790035248,8.605638868175447e-09
12780,60266,60266,120532,364.2073760032654,8.60018189996481e-09
12797,60352,60352,120704,364.71674704551697,8.594724931754172e-09
12815,60442,60442,120884,365.2546350955963,8.585629984736443e-09
12832,60526,60526,121052,365.7570490837097,8.580173016525805e-09
12850,60602,60602,121204,366.2291069030762,8.571078069508076e-09
12868,60686,60686,121372,366.72724199295044,8.5601641330868e-09
12885,60764,60764,121528,367.1903910636902,8.541974239051342e-09
12903,60862,60862,121724,367.77194380760193,8.521965355612338e-09
12920,60948,60948,121896,368.29545283317566,8.50741344038397e-09
12938,61032,61032,122064,368.79594588279724,8.500137482769787e-09
12955,61118,61118,122236,369.2950110435486,8.480128599330783e-09
12973,61212,61212,122424,369.8552601337433,8.456481737084687e-09
12991,61300,61300,122600,370.3909249305725,8.434653864242136e-09
13008,61400,61400,122800,370.98450994491577,8.425558917224407e-09
13026,61490,61490,122980,371.53358793258667,8.363713277503848e-09
13043,61572,61572,123144,372.03139996528625,8.303686627186835e-09
13061,61658,61658,123316,372.55646204948425,8.247297955676913e-09
13078,61742,61742,123484,373.0532238483429,8.176357368938625e-09
13096,61826,61826,123652,373.5559780597687,8.096321835182607e-09
13114,61910,61910,123820,374.0685098171234,8.078131941147149e-09
13131,61986,61986,123972,374.5836081504822,7.979906513355672e-09
13149,62074,62074,124148,375.1235771179199,7.856215233914554e-09
13166,62158,62158,124316,375.6333291530609,7.719791028648615e-09
13184,62250,62250,124500,376.183562040329,7.654307410120964e-09
13202,62348,62348,124696,376.78191685676575,7.585185812786222e-09
13219,62442,62442,124884,377.34219694137573,7.45421857573092e-09
13237,62524,62524,125048,377.8477449417114,7.374183041974902e-09
13254,62596,62596,125192,378.28739619255066,7.201379048638046e-09
13272,62672,62672,125344,378.771653175354,7.17773218639195e-09
13289,62754,62754,125508,379.2717502117157,7.117705536074936e-09
13307,62830,62830,125660,379.7417299747467,7.037670002318919e-09
13325,62912,62912,125824,380.2275900840759,7.0140231400728226e-09
13342,62988,62988,125976,380.6891050338745,7.008566171862185e-09
13360,63070,63070,126140,381.1955900192261,6.884874892421067e-09
13377,63146,63146,126292,381.6649498939514,6.76482159178704e-09
13395,63222,63222,126444,382.1294798851013,6.515620043501258e-09
13412,63290,63290,126580,382.5504870414734,6.280970410443842e-09
13430,63372,63372,126744,383.0476861000061,6.088157533667982e-09
13448,63450,63450,126900,383.52926683425903,5.888068699277937e-09
13465,63526,63526,127052,383.97959899902344,5.7098077377304435e-09
13483,63604,63604,127208,384.44085907936096,5.2787072490900755e-09
13500,63672,63672,127344,384.8569190502167,5.034962669014931e-09
13518,63752,63752,127504,385.34279108047485,4.86397766508162e-09
13536,63828,63828,127656,385.80226707458496,4.585672286339104e-09
13553,63896,63896,127792,386.2326190471649,4.380126483738422e-09
13571,63972,63972,127944,386.6943008899689,3.965396899729967e-09
13588,64040,64040,128080,387.1222689151764,3.941750037483871e-09
13606,64112,64112,128224,387.55932807922363,3.6598066799342632e-09
13623,64184,64184,128368,388.01223492622375,3.445165930315852e-09
13641,64256,64256,128512,388.4551019668579,3.246896085329354e-09
13659,64328,64328,128656,388.8964750766754,2.6393536245450377e-09
13676,64400,64400,128800,389.32992005348206,2.3410393623635173e-09
13694,64470,64470,128940,389.76746106147766,2.042725100181997e-09
13711,64540,64540,129080,390.21354389190674,1.6061676433309913e-09
13729,64612,64612,129224,390.652636051178,1.5661498764529824e-09
13746,64680,64680,129360,391.0710279941559,1.4424585970118642e-09
13764,64758,64758,129516,391.54775190353394,1.2205418897792697e-09
13782,64828,64828,129656,391.97892808914185,9.49512468650937e-10
13799,64900,64900,129800,392.4260129928589,8.549250196665525e-10
13817,64968,64968,129936,392.8543019294739,7.548806024715304e-10
13834,65032,65032,130064,393.2503969669342,6.912159733474255e-10
13852,65104,65104,130208,393.698566198349,6.784830475226045e-10
13869,65174,65174,130348,394.13183403015137,6.657501216977835e-10
13887,65256,65256,130512,394.6343080997467,6.639311322942376e-10
13905,65326,65326,130652,395.0708920955658,6.657501216977835e-10
13922,65386,65386,130772,395.4371500015259,6.821210263296962e-10
13940,65458,65458,130916,395.881227016449,6.96672941558063e-10
13957,65534,65534,131068,396.34519386291504,7.112248567864299e-10
13975,65608,65608,131216,396.8054687976837,7.22138793207705e-10
13993,65680,65680,131360,397.24649691581726,7.275957614183426e-10
14010,65762,65762,131524,397.7366211414337,7.257767720147967e-10
14028,65838,65838,131676,398.2167510986328,7.275957614183426e-10
14045,65910,65910,131820,398.66164207458496,7.166818249970675e-10
14063,65988,65988,131976,399.1421160697937,7.166818249970675e-10
14080,66064,66064,132128,399.59959506988525,7.185008144006133e-10
14098,66144,66144,132288,400.08025217056274,7.112248567864299e-10
14116,66226,66226,132452,400.5742530822754,7.148628355935216e-10
14133,66312,66312,132624,401.09697103500366,7.130438461899757e-10
14151,66398,66398,132796,401.60869097709656,7.057678885757923e-10
14168,66474,66474,132948,402.0704929828644,7.057678885757923e-10
14186,66560,66560,133120,402.58385825157166,7.075868779793382e-10
14203,66636,66636,133272,403.05891704559326,7.075868779793382e-10
14221,66710,66710,133420,403.5173370838165,6.96672941558063e-10
14239,66786,66786,133572,403.9763288497925,6.893969839438796e-10
14256,66862,66862,133724,404.4338631629944,6.857590051367879e-10
14274,66956,66956,133912,404.9949131011963,6.803020369261503e-10
14291,67032,67032,134064,405.46851921081543,6.784830475226045e-10
14309,67140,67140,134280,406.09042406082153,6.766640581190586e-10
14327,67226,67226,134452,406.60156416893005,6.730260793119669e-10
14344,67308,67308,134616,407.0906710624695,6.675691111013293e-10
14362,67394,67394,134788,407.61927700042725,6.621121428906918e-10
14379,67482,67482,134964,408.131224155426,6.621121428906918e-10
14397,67566,67566,135132,408.63950419425964,6.566551746800542e-10
14414,67650,67650,135300,409.1297469139099,6.566551746800542e-10
14432,67748,67748,135496,409.7136290073395,6.548361852765083e-10
14450,67836,67836,135672,410.24290704727173,6.530171958729625e-10
14467,67932,67932,135864,410.80012583732605,6.511982064694166e-10
14485,68008,68008,136016,411.27218103408813,6.493792170658708e-10
14502,68088,68088,136176,411.76123809814453,6.45741238258779e-10
14520,68190,68190,136380,412.358717918396,6.421032594516873e-10
14537,68266,68266,136532,412.81666898727417,6.348273018375039e-10
14555,68370,68370,136740,413.43403601646423,6.330083124339581e-10
14573,68472,68472,136944,414.03968715667725,6.330083124339581e-10
14590,68558,68558,137116,414.5464520454407,6.293703336268663e-10
14608,68656,68656,137312,415.12228083610535,6.257323548197746e-10
14625,68732,68732,137464,415.5786349773407,6.220943760126829e-10
14643,68824,68824,137648,416.13301396369934,6.184563972055912e-10
14661,68916,68916,137832,416.6749920845032,6.166374078020453e-10
14678,68998,68998,137996,417.1590600013733,6.129994289949536e-10
14696,69088,69088,138176,417.6977798938751,6.057234713807702e-10
14713,69188,69188,138376,418.2852919101715,6.057234713807702e-10
14731,69292,69292,138584,418.9085569381714,6.020854925736785e-10
14748,69376,69376,138752,419.32754611968994,6.002665031701326e-10
14766,69468,69468,138936,419.70752000808716,6.002665031701326e-10
14784,69568,69568,139136,420.2383668422699,5.948095349594951e-10
14801,69678,69678,139356,420.93699979782104,5.966285243630409e-10
14819,69778,69778,139556,421.61164116859436,5.966285243630409e-10
14836,69864,69864,139728,422.1672029495239,5.929905455559492e-10
14854,69958,69958,139916,422.74544882774353,5.911715561524034e-10
14871,70030,70030,140060,423.2034192085266,5.893525667488575e-10
14889,70116,70116,140232,423.73933696746826,5.838955985382199e-10
14907,70202,70202,140404,424.27164697647095,5.802576197311282e-10
14924,70296,70296,140592,424.8629779815674,5.784386303275824e-10
14942,70394,70394,140788,425.4918301105499,5.711626727133989e-10
14959,70468,70468,140936,425.96573209762573,5.566107574850321e-10
14977,70554,70554,141108,426.5047228336334,5.420588422566652e-10
14995,70636,70636,141272,427.0237410068512,5.275069270282984e-10
15012,70748,70748,141496,427.68577098846436,5.238689482212067e-10
15030,70832,70832,141664,428.2180678844452,5.165929906070232e-10
15047,70918,70918,141836,428.76767897605896,5.07498043589294e-10
15065,71000,71000,142000,429.3991050720215,5.056790541857481e-10
15082,71084,71084,142168,429.84851598739624,4.94765117764473e-10
15100,71170,71170,142340,430.32856917381287,4.929461283609271e-10
15118,71260,71260,142520,430.96519589424133,4.984030965715647e-10
15135,71332,71332,142664,431.5500102043152,4.965841071680188e-10
15153,71416,71416,142832,432.19306325912476,4.856701707467437e-10
15170,71504,71504,143008,432.7588551044464,4.765752237290144e-10
15188,71588,71588,143176,433.30138397216797,4.5838532969355583e-10
15205,71664,71664,143328,433.8081030845642,4.5292836148291826e-10
15223,71746,71746,143492,434.37489891052246,4.43833414465189e-10
15241,71830,71830,143660,434.91682505607605,4.3655745685100555e-10
15258,71922,71922,143844,435.5434250831604,4.2382453102618456e-10
15276,72002,72002,144004,436.0765309333801,4.147295840084553e-10
15293,72104,72104,144208,436.70938205718994,4.092726157978177e-10
15311,72196,72196,144392,437.2989430427551,4.0745362639427185e-10
15329,72276,72276,144552,437.8275079727173,3.9472070056945086e-10
15346,72356,72356,144712,438.35712003707886,3.892637323588133e-10
15364,72456,72456,144912,438.99555921554565,3.8562575355172157e-10
15381,72536,72536,145072,439.50918102264404,3.8198777474462986e-10
15399,72628,72628,145256,440.0900819301605,3.7834979593753815e-10
15416,72712,72712,145424,440.6483860015869,3.728928277269006e-10
15434,72804,72804,145608,441.23346495628357,3.6925484891980886e-10
15452,72898,72898,145796,441.82425594329834,3.728928277269006e-10
15469,72986,72986,145972,442.3923919200897,3.710738383233547e-10
15487,73092,73092,146184,443.0391962528229,3.6561687011271715e-10
15504,73176,73176,146352,443.59133410453796,3.67435859516263e-10
15522,73260,73260,146520,444.12137484550476,3.67435859516263e-10
15539,73346,73346,146692,444.68535017967224,3.6561687011271715e-10
15557,73430,73430,146860,445.22390818595886,3.6561687011271715e-10
15575,73516,73516,147032,445.77087688446045,3.6561687011271715e-10
15592,73600,73600,147200,446.3084089756012,3.6197889130562544e-10
15610,73688,73688,147376,446.8800208568573,3.6197889130562544e-10
15627,73778,73778,147556,447.44548201560974,3.6197889130562544e-10
15645,73860,73860,147720,447.97000002861023,3.601599019020796e-10
15663,73940,73940,147880,448.49221086502075,3.583409124985337e-10
15680,74024,74024,148048,449.03001403808594,3.5652192309498787e-10
15698,74112,74112,148224,449.5948979854584,3.583409124985337e-10
15715,74190,74190,148380,450.0838530063629,3.583409124985337e-10
15733,74292,74292,148584,450.7187809944153,3.5652192309498787e-10
15750,74396,74396,148792,451.3751950263977,3.5652192309498787e-10
15768,74496,74496,148992,452.01466393470764,3.5652192309498787e-10
15786,74604,74604,149208,452.70705103874207,3.5652192309498787e-10
15803,74708,74708,149416,453.35921001434326,3.5652192309498787e-10
15821,74810,74810,149620,454.00413703918457,3.54702933691442e-10
15838,74894,74894,149788,454.52926802635193,3.54702933691442e-10
15856,74984,74984,149968,455.0930528640747,3.54702933691442e-10
15873,75102,75102,150204,455.7884290218353,3.54702933691442e-10
15891,75208,75208,150416,456.43153619766235,3.54702933691442e-10
15909,75326,75326,150652,457.1358001232147,3.54702933691442e-10
15926,75446,75446,150892,457.8502209186554,3.54702933691442e-10
15944,75566,75566,151132,458.592787027359,3.5652192309498787e-10
15961,75650,75650,151300,459.1157760620117,3.54702933691442e-10
15979,75746,75746,151492,459.6998920440674,3.54702933691442e-10
15997,75856,75856,151712,460.3777780532837,3.54702933691442e-10
16014,75962,75962,151924,461.02243304252625,3.54702933691442e-10
16032,76070,76070,152140,461.6770570278168,3.5288394428789616e-10
16049,76160,76160,152320,462.2340478897095,3.54702933691442e-10
16067,76282,76282,152564,462.9714369773865,3.510649548843503e-10
16084,76366,76366,152732,463.52081990242004,3.510649548843503e-10
16102,76474,76474,152948,464.1717429161072,3.510649548843503e-10
16120,76586,76586,153172,464.83589005470276,3.510649548843503e-10
16137,76690,76690,153380,465.4724621772766,3.510649548843503e-10
16155,76782,76782,153564,466.05231404304504,3.510649548843503e-10
16172,76892,76892,153784,466.7129011154175,3.4924596548080444e-10
16190,76998,76998,153996,467.33819794654846,3.4924596548080444e-10
16207,77082,77082,154164,467.8602201938629,3.474269760772586e-10
16225,77184,77184,154368,468.49118208885193,3.41970007866621e-10
16243,77276,77276,154552,469.0895240306854,3.3651303965598345e-10
16260,77364,77364,154728,469.6559250354767,3.310560714453459e-10
16278,77450,77450,154900,470.20124316215515,3.2741809263825417e-10
16295,77548,77548,155096,470.8158960342407,3.255991032347083e-10
16313,77636,77636,155272,471.3794209957123,3.255991032347083e-10
16330,77728,77728,155456,471.9452919960022,3.219611244276166e-10
16348,77814,77814,155628,472.49620294570923,3.1468516681343317e-10
16366,77928,77928,155856,473.1958260536194,3.0377123039215803e-10
16383,78008,78008,156016,473.69225692749023,3.019522409886122e-10
16401,78100,78100,156200,474.2686960697174,2.9831426218152046e-10
16418,78178,78178,156356,474.7724220752716,2.9831426218152046e-10
16436,78268,78268,156536,475.3477749824524,2.9467628337442875e-10
16454,78350,78350,156700,475.8767569065094,2.9103830456733704e-10
16471,78426,78426,156852,476.36575198173523,2.892193151637912e-10
16489,78516,78516,157032,476.938236951828,2.874003257602453e-10
16506,78602,78602,157204,477.49523305892944,2.837623469531536e-10
16524,78684,78684,157368,478.0161249637604,2.8194335754960775e-10
16541,78778,78778,157556,478.6189639568329,2.7830537874251604e-10
16559,78884,78884,157768,479.2693519592285,2.801243681460619e-10
16577,78970,78970,157940,479.83618998527527,2.7466739993542433e-10
16594,79072,79072,158144,480.4481899738312,2.7466739993542433e-10
16612,79172,79172,158344,481.06986808776855,2.7284841053187847e-10
16629,79270,79270,158540,481.6625180244446,2.7284841053187847e-10
16647,79358,79358,158716,482.2307481765747,2.7284841053187847e-10
16664,79450,79450,158900,482.8076651096344,2.710294211283326e-10
16682,79546,79546,159092,483.4167709350586,2.6921043172478676e-10
16700,79632,79632,159264,483.9752640724182,2.710294211283326e-10
16717,79726,79726,159452,484.56347703933716,2.710294211283326e-10
16735,79820,79820,159640,485.14606404304504,2.6921043172478676e-10
16752,79910,79910,159820,485.71405506134033,2.673914423212409e-10
16770,80008,80008,160016,486.3300609588623,2.673914423212409e-10
16788,80094,80094,160188,486.88350009918213,2.6921043172478676e-10
16805,80182,80182,160364,487.4285922050476,2.6557245291769505e-10
16823,80292,80292,160584,488.1125519275665,2.673914423212409e-10
16840,80382,80382,160764,488.6902229785919,2.673914423212409e-10
16858,80500,80500,161000,489.4087920188904,2.673914423212409e-10
16875,80602,80602,161204,490.0428788661957,2.673914423212409e-10
16893,80710,80710,161420,490.7089898586273,2.6557245291769505e-10
16911,80822,80822,161644,491.3992519378662,2.6557245291769505e-10
16928,80916,80916,161832,491.9764018058777,2.673914423212409e-10
16946,81024,81024,162048,492.63805890083313,2.673914423212409e-10
16963,81136,81136,162272,493.3031370639801,2.6557245291769505e-10
16981,81246,81246,162492,493.98095512390137,2.6557245291769505e-10
16998,81352,81352,162704,494.66614389419556,2.673914423212409e-10
17016,81484,81484,162968,495.44978880882263,2.6557245291769505e-10
17034,81602,81602,163204,496.1712911128998,2.6557245291769505e-10
17051,81704,81704,163408,496.7886610031128,2.6557245291769505e-10
17069,81812,81812,163624,497.46503806114197,2.637534635141492e-10
17086,81896,81896,163792,497.9870309829712,2.6557245291769505e-10
17104,82004,82004,164008,498.6457772254944,2.637534635141492e-10
17122,82106,82106,164212,499.27056193351746,2.637534635141492e-10
17139,82214,82214,164428,499.94007301330566,2.637534635141492e-10
17157,82328,82328,164656,500.6296570301056,2.637534635141492e-10
17174,82446,82446,164892,501.3366279602051,2.637534635141492e-10
17192,82554,82554,165108,502.005038022995,2.6193447411060333e-10
17209,82652,82652,165304,502.60765409469604,2.6193447411060333e-10
17227,82744,82744,165488,503.17577505111694,2.601154847070575e-10
17245,82820,82820,165640,503.6708002090454,2.582964953035116e-10
17262,82910,82910,165820,504.22543501853943,2.510205376893282e-10
17280,83002,83002,166004,504.7994108200073,2.4920154828578234e-10
17297,83098,83098,166196,505.38690209388733,2.455635694786906e-10
17315,83186,83186,166372,505.9483959674835,2.419255906715989e-10
17332,83278,83278,166556,506.5407910346985,2.3283064365386963e-10
17350,83362,83362,166724,507.0845649242401,2.3101165425032377e-10
17368,83450,83450,166900,507.6479160785675,2.1100277081131935e-10
17385,83518,83518,167036,508.1091070175171,1.8917489796876907e-10
17403,83602,83602,167204,508.6669280529022,1.7644197214394808e-10
17420,83676,83676,167352,509.1769971847534,1.7462298274040222e-10
17438,83766,83766,167532,509.8193678855896,1.709850039333105e-10
17456,83866,83866,167732,510.51147413253784,1.6552803572267294e-10
17473,83934,83934,167868,511.0028851032257,1.5279510989785194e-10
17491,84016,84016,168032,511.5217831134796,1.4370016288012266e-10
17508,84084,84084,168168,511.95978903770447,1.291482476517558e-10
17526,84170,84170,168340,512.518630027771,1.2732925824820995e-10
17543,84256,84256,168512,513.0579509735107,1.1459633242338896e-10
17561,84344,84344,168688,513.6188111305237,9.822542779147625e-11


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.0016930103302001953,846.9037197860796
29,60,30,90,0.039572954177856445,60.951221914780945
58,118,59,177,0.07233691215515137,53.228602328563966
87,176,88,264,0.10537409782409668,49.275385401012954
116,234,117,351,0.13831686973571777,46.25781249962188
146,294,147,441,0.17371201515197754,43.918484493305186
175,352,176,528,0.20476508140563965,41.83134364314242
204,410,205,615,0.23752188682556152,39.92161091974481
233,468,234,702,0.27086591720581055,38.198276928415225
262,526,263,789,0.30205202102661133,36.58449389617044
291,584,292,876,0.3333439826965332,35.14654932934695
320,642,321,963,0.3637509346008301,33.67963510577556
349,700,350,1050,0.39542508125305176,32.53935789042907
379,760,380,1140,0.4283139705657959,31.191326678237147
408,818,409,1227,0.4605698585510254,30.152408010080308
437,876,438,1314,0.49192190170288086,29.06048061384331
466,934,467,1401,0.5230629444122314,28.10302663556422
495,992,496,1488,0.5544657707214355,27.255525696333734
524,1050,525,1575,0.5861020088195801,26.455033537691634
553,1108,554,1662,0.6179070472717285,25.414717880271155
582,1166,583,1749,0.649616003036499,24.60193441237061
611,1224,612,1836,0.682790994644165,23.930370450290184
641,1284,642,1926,0.7174570560455322,23.163079723194187
670,1342,671,2013,0.7518038749694824,22.459298269544433
699,1400,700,2100,0.7862107753753662,21.82455376283201
728,1458,729,2187,0.8212869167327881,21.243206171056045
757,1516,758,2274,0.8529648780822754,20.603258079325542
786,1574,787,2361,0.8880488872528076,19.91399805876722
815,1632,816,2448,0.9206008911132812,19.354075068272323
844,1690,845,2535,0.9523780345916748,18.917193060691034
874,1750,875,2625,0.9891128540039062,18.34961304335411
903,1808,904,2712,1.0222117900848389,17.899635458278453
932,1866,933,2799,1.054142951965332,17.43428428506695
961,1924,962,2886,1.088385820388794,16.975013422579423
990,1982,991,2973,1.1202208995819092,16.498502633626686
1019,2040,1020,3060,1.1516618728637695,16.03499723517507
1048,2098,1049,3147,1.1833600997924805,15.618203430524318
1077,2156,1078,3234,1.2144410610198975,15.252971766646397
1106,2214,1107,3321,1.2463188171386719,14.771383511103522
1136,2274,1137,3411,1.2791588306427002,14.232319153182289
1165,2332,1166,3498,1.3104310035705566,13.894681214127786
1194,2390,1195,3585,1.342052936553955,13.529045718075395
1223,2448,1224,3672,1.374709129333496,13.202526950457013
1252,2506,1253,3759,1.406402826309204,12.85889646039368
1281,2564,1282,3846,1.4387521743774414,12.45263506059132
1310,2622,1311,3933,1.470823049545288,12.23029731707038
1339,2680,1340,4020,1.502579927444458,11.847923136651048
1369,2740,1370,4110,1.535027027130127,11.542563283272102
1398,2798,1399,4197,1.5672509670257568,11.189579971601802
1427,2856,1428,4284,1.5988719463348389,10.917991457380367
1456,2914,1457,4371,1.6308271884918213,10.622263968651964
1485,2972,1486,4458,1.6625409126281738,10.387834290546834
1514,3030,1515,4545,1.6953349113464355,10.13172567487618
1543,3088,1544,4632,1.7265748977661133,9.881284007480417
1572,3146,1573,4719,1.758241891860962,9.645403989764077
1601,3204,1602,4806,1.7896971702575684,9.39275562897285
1631,3264,1632,4896,1.822234869003296,9.150557959200569
1660,3322,1661,4983,1.8532838821411133,8.919474765848122
1689,3380,1690,5070,1.8840699195861816,8.660853633872534
1718,3438,1719,5157,1.9159698486328125,8.447753447746209
1747,3496,1748,5244,1.9476749897003174,8.250129587882498
1776,3554,1777,5331,1.9797170162200928,8.050550228831753
1805,3612,1806,5418,2.011215925216675,7.854436751350704
1834,3670,1835,5505,2.0433759689331055,7.677896798261031
1863,3728,1864,5592,2.0776150226593018,7.498090308653332
1893,3788,1894,5682,2.1102778911590576,7.325775498949611
1922,3846,1923,5769,2.1423168182373047,7.130687095118674
1951,3904,1952,5856,2.174175977706909,6.954575164519838
1980,3962,1981,5943,2.205399990081787,6.789757109955076
2009,4020,2010,6030,2.23836612701416,6.632740179676148
2038,4078,2039,6117,2.2700459957122803,6.474404224974251
2067,4136,2068,6204,2.3011317253112793,6.307933758705417
2096,4194,2097,6291,2.3328909873962402,6.15268277504731
2126,4254,2127,6381,2.3642029762268066,5.994241092332231
2155,4312,2156,6468,2.395737886428833,5.830024772650177
2184,4370,2185,6555,2.427137851715088,5.676245522320073
2213,4428,2214,6642,2.4573569297790527,5.5598247995751535
2242,4486,2243,6729,2.489691972732544,5.4315186543615255
2271,4544,2272,6816,2.526550769805908,5.310211170384264
2300,4602,2301,6903,2.557508945465088,5.176127152685581
2329,4660,2330,6990,2.5884108543395996,5.051405803971079
2358,4718,2359,7077,2.617927074432373,4.935355849076586
2388,4778,2389,7167,2.649061918258667,4.819528935714402
2417,4836,2418,7254,2.680598735809326,4.71596452314418
2446,4894,2447,7341,2.7099108695983887,4.617080319237743
2475,4952,2476,7428,2.741237163543701,4.512429562220063
2504,5010,2505,7515,2.773329019546509,4.397105606100467
2533,5068,2534,7602,2.803753137588501,4.315307898798437
2562,5126,2563,7689,2.835939884185791,4.18466676952653
2591,5184,2592,7776,2.8681480884552,4.089463573012836
2621,5244,2622,7866,2.901458978652954,3.998652784037631
2650,5302,2651,7953,2.9350128173828125,3.905425323696022
2679,5360,2680,8040,2.970883846282959,3.8089198927424377
2708,5418,2709,8127,3.0028328895568848,3.7212423425719408
2737,5476,2738,8214,3.0356388092041016,3.6310773960460665
2766,5534,2767,8301,3.0675108432769775,3.543207383011577
2795,5592,2796,8388,3.098602056503296,3.466161284867553
2824,5650,2825,8475,3.1299338340759277,3.3836124373485745
2853,5708,2854,8562,3.160325050354004,3.313289292518334
2883,5768,2884,8652,3.1923270225524902,3.22664018309365
2912,5826,2913,8739,3.223345994949341,3.158045593478505
2941,5884,2942,8826,3.254225969314575,3.0686442192785535
2970,5942,2971,8913,3.2859909534454346,3.003744298642232
2999,6000,3000,9000,3.317633867263794,2.9323665394699674
3028,6058,3029,9087,3.3510711193084717,2.863301116070147
3057,6116,3058,9174,3.386721134185791,2.801095254321126
3086,6174,3087,9261,3.417452812194824,2.73484812053357
3116,6234,3117,9351,3.450334072113037,2.660501050153357
3145,6292,3146,9438,3.482532024383545,2.6082797022216937
3174,6350,3175,9525,3.513150930404663,2.547743920578
3203,6408,3204,9612,3.5455498695373535,2.4927409477489846
3232,6466,3233,9699,3.5763227939605713,2.4348603042082004
3261,6524,3262,9786,3.606624126434326,2.3819470878109996
3290,6582,3291,9873,3.637624979019165,2.3264743533139836
3319,6640,3320,9960,3.6685938835144043,2.276706777553727
3348,6698,3349,10047,3.6991817951202393,2.2344986860829295
3378,6758,3379,10137,3.731281042098999,2.178202127424811
3407,6816,3408,10224,3.761666774749756,2.1258783925002263
3436,6874,3437,10311,3.792301893234253,2.0862036443031684
3465,6932,3466,10398,3.824105978012085,2.0320216268862623
3494,6990,3495,10485,3.8546979427337646,1.9875914201483056
3523,7048,3524,10572,3.885382890701294,1.9434519061711626
3552,7106,3553,10659,3.916184902191162,1.8948053698981084
3581,7164,3582,10746,3.9466159343719482,1.8460580897603904
3611,7224,3612,10836,3.9793617725372314,1.80611971459075
3640,7282,3641,10923,4.0102219581604,1.768951809888108
3669,7340,3670,11010,4.041441202163696,1.7300598009387613
3698,7398,3699,11097,4.074518918991089,1.6903075722818812
3727,7456,3728,11184,4.10517692565918,1.6514278754756333
3756,7514,3757,11271,4.136922836303711,1.61171944017417
3785,7572,3786,11358,4.168210029602051,1.5777931214203136
3814,7630,3815,11445,4.199465990066528,1.5442127271118125
3843,7688,3844,11532,4.230730056762695,1.5112407042005316
3873,7748,3874,11622,4.262557029724121,1.4664823571225725
3902,7806,3903,11709,4.293398141860962,1.434422203608051
3931,7864,3932,11796,4.325336933135986,1.4050488647088741
3960,7922,3961,11883,4.3560631275177,1.3793675958723952
3989,7980,3990,11970,4.388200044631958,1.3451372946462925
4018,8038,4019,12057,4.419524908065796,1.3186524726515927
4047,8096,4048,12144,4.450844049453735,1.2917370951885232
4076,8154,4077,12231,4.48339319229126,1.2651580976557852
4106,8214,4107,12321,4.516021013259888,1.2375177784992957
4135,8272,4136,12408,4.548692941665649,1.2104617874526866
4164,8330,4165,12495,4.5808117389678955,1.1800067770142277
4193,8388,4194,12582,4.611126184463501,1.156634294208402
4222,8446,4223,12669,4.642241954803467,1.1308184059843143
4251,8504,4252,12756,4.673821926116943,1.1068154901275875
4280,8562,4281,12843,4.704502105712891,1.085513387746687
4309,8620,4310,12930,4.735284090042114,1.0586986739530175
4338,8678,4339,13017,4.76633095741272,1.0356971710839389
4368,8738,4369,13107,4.797612190246582,1.0143041563455881
4397,8796,4398,13194,4.828818082809448,0.9935661950909207
4426,8854,4427,13281,4.8595311641693115,0.9713619451797513
4455,8912,4456,13368,4.890197038650513,0.9501976300565502
4484,8970,4485,13455,4.921787977218628,0.9315564651490149
4513,9028,4514,13542,4.9526097774505615,0.9129445177630942
4542,9086,4543,13629,4.985087156295776,0.894284711491423
4571,9144,4572,13716,5.017228841781616,0.8720143617262011
4601,9204,4602,13806,5.052308082580566,0.8540746060050424
4630,9262,4631,13893,5.084568977355957,0.8343483698336058
4659,9320,4660,13980,5.117369890213013,0.8182596662786636
4688,9378,4689,14067,5.149121046066284,0.8003067976788998
4717,9436,4718,14154,5.180513143539429,0.7823803154426514
4746,9494,4747,14241,5.210700750350952,0.7642233674662293
4775,9552,4776,14328,5.241745948791504,0.7482667492616883
4804,9610,4805,14415,5.272559881210327,0.7329584684711108
4833,9668,4834,14502,5.302897930145264,0.7171808864000013
4863,9728,4864,14592,5.334881782531738,0.702129367978273
4892,9786,4893,14679,5.364887952804565,0.6876833976565422
4921,9844,4922,14766,5.396244049072266,0.6738568646106842
4950,9902,4951,14853,5.427511930465698,0.6573097095285902
4979,9960,4980,14940,5.458127021789551,0.6444668237600126
5008,10018,5009,15027,5.48919415473938,0.6288499107412235
5037,10076,5038,15114,5.519880056381226,0.6169541525623572
5066,10134,5067,15201,5.550632953643799,0.6024051319574255
5095,10192,5096,15288,5.58176589012146,0.589703682042682
5125,10252,5126,15378,5.614714860916138,0.5757010456799208
5154,10310,5155,15465,5.645753860473633,0.5653805056331294
5183,10368,5184,15552,5.676687955856323,0.5524794183560289
5212,10426,5213,15639,5.7071051597595215,0.5420401781201463
5241,10484,5242,15726,5.738207101821899,0.5313745140515493
5270,10542,5271,15813,5.769248008728027,0.5185334140790019
5299,10600,5300,15900,5.799830913543701,0.5080535371452015
5328,10658,5329,15987,5.831647157669067,0.4974109724653317
5358,10718,5359,16077,5.86326003074646,0.4874389058529687
5387,10776,5388,16164,5.89489483833313,0.47727617315149473
5416,10834,5417,16251,5.926530838012695,0.46832990156622145
5445,10892,5446,16338,5.956541061401367,0.45909970667878497
5474,10950,5475,16425,5.987181901931763,0.44887137429395807
5503,11008,5504,16512,6.0181121826171875,0.43902943262321514
5532,11066,5533,16599,6.049593925476074,0.4301195441217942
5561,11124,5562,16686,6.0821919441223145,0.42171527337518455
5590,11182,5591,16773,6.112838983535767,0.41253010082368746
5620,11242,5621,16863,6.145243883132935,0.4025907782651075
5649,11300,5650,16950,6.177121877670288,0.39473960348891524
5678,11358,5679,17037,6.20865797996521,0.3865221029651593
5707,11416,5708,17124,6.240890979766846,0.3790474057252595
5736,11474,5737,17211,6.273207902908325,0.37055440953804464
5765,11532,5766,17298,6.304973840713501,0.36340829730204405
5794,11590,5795,17385,6.3378119468688965,0.3559195359523528
5823,11648,5824,17472,6.370161056518555,0.34888247867343125
5853,11708,5854,17562,6.4029541015625,0.3417026331701436
5882,11766,5883,17649,6.435777902603149,0.3333816996959058
5911,11824,5912,17736,6.468667984008789,0.32835750796652974
5940,11882,5941,17823,6.500825881958008,0.31991201460971297
5969,11940,5970,17910,6.532867908477783,0.3140749010528907
5998,11998,5999,17997,6.565505027770996,0.30774299773349867
6027,12056,6028,18084,6.598207950592041,0.3015486240580003
6056,12114,6057,18171,6.630064964294434,0.29474056910135005
6085,12172,6086,18258,6.661743879318237,0.289585509084759
6115,12232,6116,18348,6.694607973098755,0.2838041139150391
6144,12290,6145,18435,6.727094888687134,0.2774220372655236
6173,12348,6174,18522,6.758849859237671,0.2725147962173651
6202,12406,6203,18609,6.790631055831909,0.26729226273869244
6231,12464,6232,18696,6.823275089263916,0.2620876888630619
6260,12522,6261,18783,6.855681896209717,0.2564890560789763
6289,12580,6290,18870,6.8871588706970215,0.2514814360223454
6318,12638,6319,18957,6.918459892272949,0.24671333433707332
6348,12698,6349,19047,6.951575994491577,0.24163939113839206
6377,12756,6378,19134,6.983794927597046,0.2367817596310715
6406,12814,6407,19221,7.0154571533203125,0.22940041304957504
6435,12872,6436,19308,7.047777891159058,0.22522457782645233
6464,12930,6465,19395,7.080045938491821,0.2208107165840829
6493,12988,6494,19482,7.112185001373291,0.21648997169540962
6522,13046,6523,19569,7.145473957061768,0.21211885850379986
6551,13104,6552,19656,7.179941892623901,0.2076170916401452
6580,13162,6581,19743,7.213392972946167,0.20296928092784583
6610,13222,6611,19833,7.249237060546875,0.19880007804772504
6639,13280,6640,19920,7.284289836883545,0.19527162752297045
6668,13338,6669,20007,7.316338062286377,0.19097310158770142
6697,13396,6698,20094,7.348922967910767,0.18747884222193534
6726,13454,6727,20181,7.381350040435791,0.18294216952733677
6755,13512,6756,20268,7.412744045257568,0.17939313180738736
6784,13570,6785,20355,7.445637941360474,0.17583308599409975
6813,13628,6814,20442,7.477927923202515,0.17216165367835856
6843,13688,6844,20532,7.511029005050659,0.1685689380030908
6872,13746,6873,20619,7.544081926345825,0.16532197315927988
6901,13804,6902,20706,7.576236963272095,0.16231887987851223
6930,13862,6931,20793,7.608198881149292,0.15802129524456632
6959,13920,6960,20880,7.643280029296875,0.15502768236274278
6988,13978,6989,20967,7.675903081893921,0.1520496433763583
7017,14036,7018,21054,7.706954002380371,0.1485699421315303
7046,14094,7047,21141,7.738860845565796,0.14569961617939953
7075,14152,7076,21228,7.771007061004639,0.1426705738072087
7105,14212,7106,21318,7.803532838821411,0.13987352919832574
7134,14270,7135,21405,7.835726976394653,0.13720931978150475
7163,14328,7164,21492,7.867788791656494,0.1345769493638045
7192,14386,7193,21579,7.899536848068237,0.13194543659767533
7221,14444,7222,21666,7.931519985198975,0.12889272057316248
7250,14502,7251,21753,7.963287830352783,0.12649929196504672
7279,14560,7280,21840,7.995000839233398,0.12416689282292737
7308,14618,7309,21927,8.026902914047241,0.12166306891697332
7338,14678,7339,22017,8.059254884719849,0.11925453036099043
7367,14736,7368,22104,8.091273069381714,0.11678076250814229
7396,14794,7397,22191,8.123235940933228,0.11428962398281328
7425,14852,7426,22278,8.15447211265564,0.11195618863155232
7454,14910,7455,22365,8.185526847839355,0.10984442175094955
7483,14968,7484,22452,8.216684103012085,0.10765981280871983
7512,15026,7513,22539,8.247800827026367,0.10542855784569838
7541,15084,7542,22626,8.27950382232666,0.10321481563482848
7570,15142,7571,22713,8.311347007751465,0.10117566687404178
7600,15202,7601,22803,8.34654712677002,0.09888128879890701
7629,15260,7630,22890,8.37751293182373,0.09699103132788878
7658,15318,7659,22977,8.408145904541016,0.09512163807130491
7687,15376,7688,23064,8.440208911895752,0.09340798263747274
7716,15434,7717,23151,8.472330093383789,0.09122767871679116
7745,15492,7746,23238,8.503190755844116,0.08926532634859541
7774,15550,7775,23325,8.535510063171387,0.08767078931839478
7803,15608,7804,23412,8.5696861743927,0.08572644913965632
7833,15668,7834,23502,8.603244066238403,0.0839397593637159
7862,15726,7863,23589,8.635893106460571,0.08210917598989909
7891,15784,7892,23676,8.670467853546143,0.0807106057859528
7920,15842,7921,23763,8.70349907875061,0.07894205043112379
7949,15900,7950,23850,8.736982107162476,0.07743172451318969
7978,15958,7979,23937,8.773235082626343,0.07592929110001023
8007,16016,8008,24024,8.807416915893555,0.07435606534079398
8036,16074,8037,24111,8.84226393699646,0.0729381069234023
8065,16132,8066,24198,8.876715183258057,0.07138375287479448
8095,16192,8096,24288,8.909446001052856,0.0699216771713509
8124,16250,8125,24375,8.94206690788269,0.06868792836507964
8153,16308,8154,24462,8.98051905632019,0.06717125438319727
8182,16366,8183,24549,9.011476993560791,0.0657506236991594
8211,16424,8212,24636,9.043601989746094,0.0644714782677056
8240,16482,8241,24723,9.078067064285278,0.06303540590681678
8269,16540,8270,24810,9.111089944839478,0.06191786381907605
8298,16598,8299,24897,9.143879890441895,0.06050318309519298
8327,16656,8328,24984,9.17539381980896,0.05927667362709599
8357,16716,8358,25074,9.207780838012695,0.0580998416176044
8386,16774,8387,25161,9.239696025848389,0.05700011927649484
8415,16832,8416,25248,9.273388147354126,0.05578596596183161
8444,16890,8445,25335,9.305535078048706,0.054742738961522264
8473,16948,8474,25422,9.339708089828491,0.053382350122546995
8502,17006,8503,25509,9.372128009796143,0.05242216916258258
8531,17064,8532,25596,9.403770923614502,0.05142260473235183
8560,17122,8561,25683,9.437663078308105,0.050569342566745945
8590,17182,8591,25773,9.471410036087036,0.049534206706312034
8619,17240,8620,25860,9.504122972488403,0.04847687162418879
8648,17298,8649,25947,9.53747010231018,0.047516398397419835
8677,17356,8678,26034,9.57016897201538,0.04660236926633843
8706,17414,8707,26121,9.601435899734497,0.04573560227731832
8735,17472,8736,26208,9.633634805679321,0.044677959096475206
8764,17530,8765,26295,9.66714096069336,0.04387944902896379
8793,17588,8794,26382,9.699862003326416,0.042896895824924286
8822,17646,8823,26469,9.734046936035156,0.042179280616892356
8852,17706,8853,26559,9.772485971450806,0.0413134367265684
8881,17764,8882,26646,9.809260845184326,0.04047712294493522
8910,17822,8911,26733,9.852044820785522,0.039696430603044064
8939,17880,8940,26820,9.88949203491211,0.03891861693421106
8968,17938,8969,26907,9.921656847000122,0.03823840841926085
8997,17996,8998,26994,9.95350694656372,0.03747799083703285
9026,18054,9027,27081,9.98790192604065,0.036805622854785724
9055,18112,9056,27168,10.020561933517456,0.03612392496177108
9085,18172,9086,27258,10.056823968887329,0.03540308177593943
9114,18230,9115,27345,10.094748973846436,0.03468051087884305
9143,18288,9144,27432,10.128682136535645,0.03393495673799407
9172,18346,9173,27519,10.162568092346191,0.033348775377248785
9201,18404,9202,27606,10.198042869567871,0.03266560644169658
9230,18462,9231,27693,10.231553077697754,0.03208484094648156
9259,18520,9260,27780,10.263713121414185,0.031507217790135655
9288,18578,9289,27867,10.296050071716309,0.03075835704396468
9317,18636,9318,27954,10.328837871551514,0.03016285945625441
9347,18696,9348,28044,10.360673904418945,0.029608473912389854
9376,18754,9377,28131,10.392300844192505,0.0289135948397643
9405,18812,9406,28218,10.42335295677185,0.028323685928853592
9434,18870,9435,28305,10.454155921936035,0.027759340438365143
9463,18928,9464,28392,10.487997055053711,0.0271198705183906
9492,18986,9493,28479,10.525300979614258,0.026689979954539922
9521,19044,9522,28566,10.55988097190857,0.02614016588108825
9550,19102,9551,28653,10.596662759780884,0.025630748120534008
9580,19162,9581,28743,10.637542963027954,0.025106049065357183
9609,19220,9610,28830,10.677089929580688,0.02463892584455607
9638,19278,9639,28917,10.720012903213501,0.024133006984243366
9667,19336,9668,29004,10.757045984268188,0.02349037152555411
9696,19394,9697,29091,10.792165040969849,0.023095694954236023
9725,19452,9726,29178,10.830573797225952,0.02259599267915746
9754,19510,9755,29265,10.866929054260254,0.022193790001438174
9783,19568,9784,29352,10.906100034713745,0.021740111008625718
9812,19626,9813,29439,10.950599908828735,0.021283344994571962
9842,19686,9843,29529,10.992140769958496,0.020860828510421925
9871,19744,9872,29616,11.031058073043823,0.020458655789298064
9900,19802,9901,29703,11.067085981369019,0.020085897173999
9929,19860,9930,29790,11.103982925415039,0.019640079298369528
9958,19918,9959,29877,11.138510942459106,0.019261896764191988
9987,19976,9988,29964,11.17615294456482,0.01889321330554594
10016,20034,10017,30051,11.212494850158691,0.018464012303525124
10045,20092,10046,30138,11.25209093093872,0.018155800764816377
10075,20152,10076,30228,11.28978705406189,0.01777600457785411
10104,20210,10105,30315,11.32607913017273,0.017425127384854022
10133,20268,10134,30402,11.360295057296753,0.017092864647111128
10162,20326,10163,30489,11.398244857788086,0.01677353288823724
10191,20384,10192,30576,11.440684795379639,0.016414455802873817
10220,20442,10221,30663,11.490529775619507,0.01620419723201394
10249,20500,10250,30750,11.531763076782227,0.015754060776657752
10278,20558,10279,30837,11.58162808418274,0.015477299433769076
10307,20616,10308,30924,11.618864059448242,0.015161483628503447
10337,20676,10338,31014,11.66131591796875,0.014861609904301076
10366,20734,10367,31101,11.715622901916504,0.014586538744538302
10395,20792,10396,31188,11.749862909317017,0.014257890731869338
10424,20850,10425,31275,11.788789987564087,0.014004832416048885
10453,20908,10454,31362,11.824993133544922,0.013683826489796047
10482,20966,10483,31449,11.864131927490234,0.013415066681545795
10511,21024,10512,31536,11.902066946029663,0.013269456266584712
10540,21082,10541,31623,11.941003799438477,0.012894481273974634
10570,21142,10571,31713,11.97578501701355,0.012632382177912405
10599,21200,10600,31800,12.012027025222778,0.012405170182660186
10628,21258,10629,31887,12.05566692352295,0.012176589839441476
10657,21316,10658,31974,12.098566055297852,0.011926653904993145
10686,21374,10687,32061,12.134987831115723,0.011646920430166574
10715,21432,10716,32148,12.173557043075562,0.011446218893752302
10744,21490,10745,32235,12.211055994033813,0.011226079500715969
10773,21548,10774,32322,12.25102710723877,0.011009751445158145
10802,21606,10803,32409,12.292464017868042,0.010761774400407376
10832,21666,10833,32499,12.33395791053772,0.010554556684610361
10861,21724,10862,32586,12.369045972824097,0.010350667094940036
10890,21782,10891,32673,12.403892040252686,0.010200458664257894
10919,21840,10920,32760,12.44006896018982,0.009953710973036323
10948,21898,10949,32847,12.478790044784546,0.00976606834501581
10977,21956,10978,32934,12.51141095161438,0.009544857339619739
11006,22014,11007,33021,12.550462007522583,0.009368611558670636
11035,22072,11036,33108,12.586288928985596,0.009169786250708967
11065,22132,11066,33198,12.626658916473389,0.008982299190506637
11094,22190,11095,33285,12.662121057510376,0.00881314335447314
11123,22248,11124,33372,12.697684049606323,0.008640835678875192
11152,22306,11153,33459,12.733206748962402,0.008474465615108784
11181,22364,11182,33546,12.7672860622406,0.008315187064454221
11210,22422,11211,33633,12.80234980583191,0.008121814970195373
11239,22480,11240,33720,12.850359916687012,0.007977447662256054
11268,22538,11269,33807,12.885967016220093,0.007835050074277206
11297,22596,11298,33894,12.921030044555664,0.0076498794693407035
11327,22656,11328,33984,12.953319072723389,0.007488845576745007
11356,22714,11357,34071,12.984071016311646,0.00736406434100445
11385,22772,11386,34158,13.01477599143982,0.00718293154022831
11414,22830,11415,34245,13.045942783355713,0.0070522350209785145
11443,22888,11444,34332,13.077129125595093,0.006910796121132989
11472,22946,11473,34419,13.107703924179077,0.006752544284154283
11501,23004,11502,34506,13.138571739196777,0.00662803027978498
11530,23062,11531,34593,13.169251918792725,0.0065018655900530575
11559,23120,11560,34680,13.199732065200806,0.00637221995600612
11589,23180,11590,34770,13.232017993927002,0.006244417251878076
11618,23238,11619,34857,13.26266098022461,0.006135546149607762
11647,23296,11648,34944,13.29380202293396,0.005993968793404747
11676,23354,11677,35031,13.324934959411621,0.005881609537595978
11705,23412,11706,35118,13.355571985244751,0.005749322527208278
11734,23470,11735,35205,13.388023853302002,0.005632539635939793
11763,23528,11764,35292,13.41978406906128,0.005525608093876144
11792,23586,11793,35379,13.452595949172974,0.005431863625858568
11822,23646,11823,35469,13.49531102180481,0.005305183096879773
11851,23704,11852,35556,13.533642053604126,0.005200911509973594
11880,23762,11881,35643,13.56827712059021,0.005095285126003546
11909,23820,11910,35730,13.599952936172485,0.00497671615892159
11938,23878,11939,35817,13.633462905883789,0.004888063726411929
11967,23936,11968,35904,13.670928001403809,0.00479798091032535
11996,23994,11997,35991,13.703648090362549,0.004711990677606082
12025,24052,12026,36078,13.737281084060669,0.004618253003059181
12054,24110,12055,36165,13.769069910049438,0.004521186076885897
12084,24170,12085,36255,13.801131010055542,0.0044210089383796
12113,24228,12114,36342,13.832444906234741,0.004342341737697097
12142,24286,12143,36429,13.86284613609314,0.0042529098695922585
12171,24344,12172,36516,13.895238876342773,0.004174577923208744
12200,24402,12201,36603,13.926599979400635,0.00416642033530934
12229,24460,12230,36690,13.956979036331177,0.0039813839948692475
12258,24518,12259,36777,13.988667964935303,0.003904232460399726
12287,24576,12288,36864,14.019259929656982,0.003837919507532206
12317,24636,12318,36954,14.051721096038818,0.003764454693168773
12346,24694,12347,37041,14.083359956741333,0.003691869232056888
12375,24752,12376,37128,14.113852977752686,0.00361647018792155
12404,24810,12405,37215,14.145378828048706,0.0035449284954438554
12433,24868,12434,37302,14.177927017211914,0.003484058416916014
12462,24926,12463,37389,14.208120822906494,0.0034081847185234437
12491,24984,12492,37476,14.239758968353271,0.0033407391573518908
12520,25042,12521,37563,14.271785020828247,0.0032763040730969806
12549,25100,12550,37650,14.303668022155762,0.003215975399712079
12579,25160,12580,37740,14.336013793945312,0.0031542400172384077
12608,25218,12609,37827,14.366461038589478,0.003097820114021488
12637,25276,12638,37914,14.39707612991333,0.0030328074180943076
12666,25334,12667,38001,14.42812705039978,0.0029755122704955284
12695,25392,12696,38088,14.458499908447266,0.002914194639629386
12724,25450,12725,38175,14.489812135696411,0.0028593097442808357
12753,25508,12754,38262,14.520061016082764,0.0028008659651277412
12782,25566,12783,38349,14.551020860671997,0.002747838300138028
12812,25626,12813,38439,14.583074808120728,0.0026942699798837566
12841,25684,12842,38526,14.61365294456482,0.002642318771108876
12870,25742,12871,38613,14.644659042358398,0.0025917020064980534
12899,25800,12900,38700,14.676844120025635,0.0025418230208060777
12928,25858,12929,38787,14.708530902862549,0.002475328436162272
12957,25916,12958,38874,14.739276885986328,0.00242247597759615
12986,25974,12987,38961,14.769859790802002,0.0023769582188606364
13015,26032,13016,39048,14.800136089324951,0.002335318877726422
13044,26090,13045,39135,14.83086085319519,0.0022828991818641953
13074,26150,13075,39225,14.863914012908936,0.002230963634701766
13103,26208,13104,39312,14.895987033843994,0.0021872128844506733
13132,26266,13133,39399,14.925755977630615,0.002140972423489984
13161,26324,13162,39486,14.955007076263428,0.0021033281989275565
13190,26382,13191,39573,14.98500680923462,0.002068062843250118
13219,26440,13220,39660,15.014111995697021,0.002029677284326681
13248,26498,13249,39747,15.044431924819946,0.001988614474953465
13277,26556,13278,39834,15.07497787475586,0.0019511744902729333
13307,26616,13308,39924,15.10522985458374,0.001924333455121996
13336,26674,13337,40011,15.135035037994385,0.0018779796986336805
13365,26732,13366,40098,15.164186954498291,0.001842091946173241
13394,26790,13395,40185,15.194923162460327,0.0018057395037658353
13423,26848,13424,40272,15.224922895431519,0.0017681957344848342
13452,26906,13453,40359,15.254562854766846,0.0017442445716824295
13481,26964,13482,40446,15.285380840301514,0.0017034216416504933
13510,27022,13511,40533,15.314950942993164,0.0016708416648043567
13539,27080,13540,40620,15.345386981964111,0.0016410550417731429
13569,27140,13570,40710,15.375917911529541,0.0016048302018134564
13598,27198,13599,40797,15.404989004135132,0.001570428315631034
13627,27256,13628,40884,15.434823036193848,0.0015400237562062102
13656,27314,13657,40971,15.464834928512573,0.0015119285919809045
13685,27372,13686,41058,15.494795799255371,0.0014817587085644846
13714,27430,13715,41145,15.527734756469727,0.0014395110089253649
13743,27488,13744,41232,15.55699896812439,0.0014173436350120028
13772,27546,13773,41319,15.588976860046387,0.001387604144042598
13802,27606,13803,41409,15.619745969772339,0.0013601856969671644
13831,27664,13832,41496,15.649409770965576,0.001334190085458431
13860,27722,13861,41583,15.680194854736328,0.0013071752988480512
13889,27780,13890,41670,15.709681034088135,0.0012830383990376504
13918,27838,13919,41757,15.739753007888794,0.0012552079435863561
13947,27896,13948,41844,15.770594835281372,0.0012326663062367516
13976,27954,13977,41931,15.802250146865845,0.0012110360078168014
14005,28012,14006,42018,15.835054874420166,0.0011883411154940404
14034,28070,14035,42105,15.866114854812622,0.0011665135353950973
14064,28130,14065,42195,15.902318954467773,0.001144460508157863
14093,28188,14094,42282,15.9322509765625,0.0011228299977119605
14122,28246,14123,42369,15.96189284324646,0.0011013851491270543
14151,28304,14152,42456,15.992034912109375,0.001079671517004499
14180,28362,14181,42543,16.022155046463013,0.0010604266252585148
14209,28420,14210,42630,16.05188298225403,0.0010392201046443006
14238,28478,14239,42717,16.08375883102417,0.0010187432297925625
14267,28536,14268,42804,16.11275815963745,0.0009975916530038376
14297,28596,14298,42894,16.143792867660522,0.000977173022874922
14326,28654,14327,42981,16.17385697364807,0.0009589664833811185
14355,28712,14356,43068,16.203269004821777,0.0009401520708252065
14384,28770,14385,43155,16.233014822006226,0.0009238423201622936
14413,28828,14414,43242,16.262216091156006,0.0009053976683617293
14442,28886,14443,43329,16.291831970214844,0.0008872526871073205
14471,28944,14472,43416,16.321359872817993,0.0008697774503616529
14500,29002,14501,43503,16.35172986984253,0.0008551508155960619
14529,29060,14530,43590,16.38328504562378,0.0008381891345834447
14559,29120,14560,43680,16.413676023483276,0.0008220329558525918
14588,29178,14589,43767,16.449821949005127,0.0008005191996289795
14617,29236,14618,43854,16.480228900909424,0.0007847961695688355
14646,29294,14647,43941,16.509418964385986,0.000769388628782508
14675,29352,14676,44028,16.539873838424683,0.0007543602135910987
14704,29410,14705,44115,16.569676876068115,0.0007374676322342566
14733,29468,14734,44202,16.599446773529053,0.0007231674724152981
14762,29526,14763,44289,16.62946891784668,0.0007097382213032688
14791,29584,14792,44376,16.65936017036438,0.0006973699217951435
14821,29644,14822,44466,16.69030213356018,0.0006849001948694422
14850,29702,14851,44553,16.72021484375,0.0006714505294667106
14879,29760,14880,44640,16.749879837036133,0.0006587284575516605
14908,29818,14909,44727,16.779457092285156,0.0006455275147345674
14937,29876,14938,44814,16.808660984039307,0.0006358413507996374
14966,29934,14967,44901,16.83819818496704,0.0006215565838374459
14995,29992,14996,44988,16.86756420135498,0.0006099295161448026
15024,30050,15025,45075,16.896867990493774,0.0005967783453115771
15054,30110,15055,45165,16.928165912628174,0.0005846520248269371
15083,30168,15084,45252,16.95869493484497,0.0005740098446267439
15112,30226,15113,45339,16.989969968795776,0.0005639550570322172
15141,30284,15142,45426,17.020540952682495,0.0005541514105971146
15170,30342,15171,45513,17.05134606361389,0.000543837296959282
15199,30400,15200,45600,17.086882829666138,0.0005327806139803215
15228,30458,15229,45687,17.117491960525513,0.0005219209679125925
15257,30516,15258,45774,17.14653491973877,0.0005121356659856247
15286,30574,15287,45861,17.176331758499146,0.0005022362267936842
15316,30634,15317,45951,17.2064688205719,0.0004931996280674866
15345,30692,15346,46038,17.236403942108154,0.00048398472426924855
15374,30750,15375,46125,17.268635034561157,0.0004744023254943386
15403,30808,15404,46212,17.298789024353027,0.000465862296891828
15432,30866,15433,46299,17.32812809944153,0.0004558879362548396
15461,30924,15462,46386,17.35725712776184,0.00044658327146862575
15490,30982,15491,46473,17.387269020080566,0.00043879084694253834
15519,31040,15520,46560,17.416883945465088,0.000429251957143606
15549,31100,15550,46650,17.447686910629272,0.0004210210491919497
15578,31158,15579,46737,17.477521896362305,0.0004129353997086582
15607,31216,15608,46824,17.506664991378784,0.0004046590064490374
15636,31274,15637,46911,17.53656506538391,0.00039726674106077553
15665,31332,15666,46998,17.566111087799072,0.0003897854386423205
15694,31390,15695,47085,17.596536874771118,0.00038165413013757643
15723,31448,15724,47172,17.626276969909668,0.0003730794753664668
15752,31506,15753,47259,17.655583143234253,0.0003655054712226047
15781,31564,15782,47346,17.685658931732178,0.0003589112537838446
15811,31624,15812,47436,17.715837001800537,0.00035108908809888817
15840,31682,15841,47523,17.745502948760986,0.0003441465249807152
15869,31740,15870,47610,17.774930000305176,0.0003361099965104586
15898,31798,15899,47697,17.804126024246216,0.0003308043187644216
15927,31856,15928,47784,17.833834171295166,0.0003244334952796635
15956,31914,15957,47871,17.8639178276062,0.0003172714555148559
15985,31972,15986,47958,17.89406180381775,0.00031061284357747354
16014,32030,16015,48045,17.925405979156494,0.00030471887453131785
16044,32090,16045,48135,17.98616099357605,0.0002993699865783128
16073,32148,16074,48222,18.0226149559021,0.0002933372763891384
16102,32206,16103,48309,18.056176900863647,0.0002877423031577564
16131,32264,16132,48396,18.089503049850464,0.0002819435898118172
16160,32322,16161,48483,18.119753122329712,0.000276166888284024
16189,32380,16190,48570,18.150357007980347,0.00027137316544667556
16218,32438,16219,48657,18.180511951446533,0.0002664800003913115
16247,32496,16248,48744,18.21019697189331,0.00026013523768142477
16276,32554,16277,48831,18.240808963775635,0.0002547403439621121
16306,32614,16307,48921,18.272382974624634,0.0002498473968444159
16335,32672,16336,49008,18.30630087852478,0.00024529286667984707
16364,32730,16365,49095,18.336984872817993,0.00024092873525205505
16393,32788,16394,49182,18.366662979125977,0.00023640855340545386
16422,32846,16423,49269,18.396320104599,0.00023203543844374508
16451,32904,16452,49356,18.42597198486328,0.0002272502781579533
16480,32962,16481,49443,18.458826065063477,0.0002227107336238987
16509,33020,16510,49530,18.49289298057556,0.00021864167342755536
16539,33080,16540,49620,18.523783922195435,0.00021419861161575682
16568,33138,16569,49707,18.55443000793457,0.0002099276647413717
16597,33196,16598,49794,18.584264039993286,0.00020564065471262438
16626,33254,16627,49881,18.613837957382202,0.00020080608669559297
16655,33312,16656,49968,18.643388986587524,0.0001970703150391273
16684,33370,16685,50055,18.672863006591797,0.00019327262430124392
16713,33428,16714,50142,18.70227599143982,0.00018880276991239953
16742,33486,16743,50229,18.732560873031616,0.0001848512512196976
16771,33544,16772,50316,18.762197971343994,0.00018121737775800284
16801,33604,16802,50406,18.793179035186768,0.00017775865899238852
16830,33662,16831,50493,18.822661876678467,0.00017447702566641965
16859,33720,16860,50580,18.85321879386902,0.0001711652338372005
16888,33778,16889,50667,18.883493900299072,0.0001680188059935972
16917,33836,16918,50754,18.91436195373535,0.0001641816601249957
16946,33894,16947,50841,18.945794820785522,0.00016072818448265025
16975,33952,16976,50928,18.97816514968872,0.00015788131042882014
17004,34010,17005,51015,19.009400844573975,0.00015506000966070133
17034,34070,17035,51105,19.046530961990356,0.00015210933599973941
17063,34128,17064,51192,19.0843448638916,0.00014900745395607373
17092,34186,17093,51279,19.115803956985474,0.00014594654021493625
17121,34244,17122,51366,19.147568941116333,0.00014309945345303277
17150,34302,17151,51453,19.17928695678711,0.00014019818388533167
17179,34360,17180,51540,19.210449934005737,0.00013784831207885873
17208,34418,17209,51627,19.243553161621094,0.00013476104948040302
17237,34476,17238,51714,19.278038024902344,0.0001322303016877413
17266,34534,17267,51801,19.310703992843628,0.00012973693674211972
17296,34594,17297,51891,19.345052003860474,0.00012728744786727475
17325,34652,17326,51978,19.37859797477722,0.00012494669749685272
17354,34710,17355,52065,19.408023834228516,0.00012245095683738327
17383,34768,17384,52152,19.440746068954468,0.00011994345049970434
17412,34826,17413,52239,19.47328281402588,0.00011783855563862744
17441,34884,17442,52326,19.505764961242676,0.00011531568043210427
17470,34942,17471,52413,19.536356925964355,0.00011334290059039631
17499,35000,17500,52500,19.56590700149536,0.00011107137231647357
17529,35060,17530,52590,19.59785795211792,0.00010898318441832089
17558,35118,17559,52677,19.629857778549194,0.00010681985190785781
17587,35176,17588,52764,19.662891149520874,0.00010478573733507801
17616,35234,17617,52851,19.695466995239258,0.0001027540552058781
17645,35292,17646,52938,19.7260320186615,0.00010085456688102568
17674,35350,17675,53025,19.755393028259277,9.883089046525129e-05
17703,35408,17704,53112,19.786623001098633,9.684311373803212e-05
17732,35466,17733,53199,19.824150800704956,9.48483574347847e-05
17761,35524,17762,53286,19.85405397415161,9.318763761712034e-05
17791,35584,17792,53376,19.88606595993042,9.137589438523719e-05
17820,35642,17821,53463,19.915777921676636,8.973868057182699e-05
17849,35700,17850,53550,19.95297598838806,8.78112983855317e-05
17878,35758,17879,53637,19.984994888305664,8.612624105808209e-05
17907,35816,17908,53724,20.01465606689453,8.510960219609842e-05
17936,35874,17937,53811,20.04548215866089,8.264940902336093e-05
17965,35932,17966,53898,20.076705932617188,8.121155701701355e-05
17994,35990,17995,53985,20.107932090759277,7.962187635257578e-05
18023,36048,18024,54072,20.14154601097107,7.819569145794958e-05
18053,36108,18054,54162,20.181108951568604,7.666314229481941e-05
18082,36166,18083,54249,20.212162971496582,7.509532895255688e-05
18111,36224,18112,54336,20.252924919128418,7.376329222097411e-05
18140,36282,18141,54423,20.286422967910767,7.233853330035345e-05
18169,36340,18170,54510,20.31767988204956,7.092831833688251e-05
18198,36398,18199,54597,20.348809003829956,6.96206079737749e-05
18227,36456,18228,54684,20.37957787513733,6.828535526892665e-05
18256,36514,18257,54771,20.408516883850098,6.702839107219916e-05
18286,36574,18287,54861,20.440542936325073,6.577928400020028e-05
18315,36632,18316,54948,20.477442979812622,6.447649127494515e-05
18344,36690,18345,55035,20.50822901725769,6.313326662166219e-05
18373,36748,18374,55122,20.542707920074463,6.19561149051151e-05
18402,36806,18403,55209,20.57528781890869,6.0775292581638496e-05
18431,36864,18432,55296,20.605217933654785,5.947610907242051e-05
18460,36922,18461,55383,20.638251066207886,5.848444698131061e-05
18489,36980,18490,55470,20.669686794281006,5.735671652473684e-05
18518,37038,18519,55557,20.703542947769165,5.630666714750987e-05
18548,37098,18549,55647,20.735332012176514,5.5115913596637256e-05
18577,37156,18578,55734,20.764750003814697,5.37931381359158e-05
18606,37214,18607,55821,20.79511308670044,5.2820386827079346e-05
18635,37272,18636,55908,20.83195400238037,5.177615639695432e-05
18664,37330,18665,55995,20.87677812576294,5.076279023796815e-05
18693,37388,18694,56082,20.906325101852417,4.981339452569955e-05
18722,37446,18723,56169,20.941472053527832,4.8946258630166994e-05
18751,37504,18752,56256,20.971987009048462,4.805469257007644e-05
18781,37564,18782,56346,21.00275206565857,4.716682383332227e-05
18810,37622,18811,56433,21.03352689743042,4.6261314196271996e-05
18839,37680,18840,56520,21.062886953353882,4.536748349437403e-05
18868,37738,18869,56607,21.093580961227417,4.4502433752313664e-05
18897,37796,18898,56694,21.123565912246704,4.35711235695635e-05
18926,37854,18927,56781,21.152922868728638,4.2704047359620745e-05
18955,37912,18956,56868,21.183068990707397,4.192728272300883e-05
18984,37970,18985,56955,21.212941884994507,4.112957310553611e-05
19013,38028,19014,57042,21.243948936462402,4.018701224595134e-05
19043,38088,19044,57132,21.283692836761475,3.942875991924666e-05
19072,38146,19073,57219,21.31360101699829,3.874568733408523e-05
19101,38204,19102,57306,21.35516905784607,3.801819673299178e-05
19130,38262,19131,57393,21.394623041152954,3.7250388459142414e-05
19159,38320,19160,57480,21.43054699897766,3.648555946256238e-05
19188,38378,19189,57567,21.460375785827637,3.573774222331849e-05
19217,38436,19218,57654,21.492353200912476,3.506534051211929e-05
19246,38494,19247,57741,21.5225670337677,3.4335045029365574e-05
19276,38554,19277,57831,21.553004026412964,3.3672337508505734e-05
19305,38612,19306,57918,21.583671808242798,3.306147129933379e-05
19334,38670,19335,58005,21.612925052642822,3.244634456223139e-05
19363,38728,19364,58092,21.644093990325928,3.182237594501203e-05
19392,38786,19393,58179,21.675534963607788,3.122276041267469e-05
19421,38844,19422,58266,21.706350803375244,3.0692748282490356e-05
19450,38902,19451,58353,21.745950937271118,3.008125338510581e-05
19479,38960,19480,58440,21.78766393661499,2.951434453279944e-05
19508,39018,19509,58527,21.829267024993896,2.895277543757402e-05
19538,39078,19539,58617,21.860449075698853,2.8370082418405218e-05
19567,39136,19568,58704,21.90279984474182,2.78121007113441e-05
19596,39194,19597,58791,21.942392826080322,2.7265746666671475e-05
19625,39252,19626,58878,21.974507093429565,2.6640817509360204e-05
19654,39310,19655,58965,22.005282878875732,2.613908418425126e-05
19683,39368,19684,59052,22.037766933441162,2.5601386255402758e-05
19712,39426,19713,59139,22.07314705848694,2.5076416022784542e-05
19741,39484,19742,59226,22.10479497909546,2.465571753873519e-05
19771,39544,19772,59316,22.140310764312744,2.410591764601122e-05
19800,39602,19801,59403,22.177778005599976,2.3630749183212174e-05
19829,39660,19830,59490,22.20933485031128,2.3191809418676712e-05
19858,39718,19859,59577,22.245776891708374,2.2735788661520928e-05
19887,39776,19888,59664,22.280375957489014,2.2305633365249378e-05
19916,39834,19917,59751,22.313249826431274,2.1910631176069728e-05
19945,39892,19946,59838,22.34829092025757,2.152937236132857e-05
19974,39950,19975,59925,22.382774829864502,2.1088711719130515e-05
20003,40008,20004,60012,22.414297819137573,2.0700633854175976e-05
20033,40068,20034,60102,22.452419996261597,2.030835798905173e-05
20062,40126,20063,60189,22.49514603614807,1.9833402461699734e-05
20091,40184,20092,60276,22.536343812942505,1.9558119106477534e-05
20120,40242,20121,60363,22.573680877685547,1.907601858874841e-05
20149,40300,20150,60450,22.606915950775146,1.868735603238747e-05
20178,40358,20179,60537,22.642218112945557,1.82904716439225e-05
20207,40416,20208,60624,22.67529797554016,1.7934603874891764e-05
20236,40474,20237,60711,22.70619797706604,1.759421184033272e-05
20266,40534,20267,60801,22.73852801322937,1.7191384472425852e-05
20295,40592,20296,60888,22.76930594444275,1.690625242645183e-05
20324,40650,20325,60975,22.802342891693115,1.6598249771959672e-05
20353,40708,20354,61062,22.834693908691406,1.625990296361124e-05
20382,40766,20383,61149,22.866328954696655,1.5954458376654657e-05
20411,40824,20412,61236,22.899653911590576,1.5644599898223532e-05
20440,40882,20441,61323,22.938273191452026,1.535365970539715e-05
20469,40940,20470,61410,22.977433919906616,1.5069399296407937e-05
20498,40998,20499,61497,23.014028787612915,1.4789507076784503e-05
20528,41058,20529,61587,23.050002098083496,1.4488472288576304e-05
20557,41116,20558,61674,23.088406085968018,1.4204780995896726e-05
20586,41174,20587,61761,23.121590852737427,1.3911230553276255e-05
20615,41232,20616,61848,23.1598699092865,1.3614998579214443e-05
20644,41290,20645,61935,23.200129747390747,1.3364599453780102e-05
20673,41348,20674,62022,23.245875120162964,1.3062807738606352e-05
20702,41406,20703,62109,23.28574800491333,1.2763154359163309e-05
20731,41464,20732,62196,23.319477081298828,1.2479265819820284e-05
20761,41524,20762,62286,23.353603839874268,1.2236447560098895e-05
20790,41582,20791,62373,23.388503789901733,1.1974751032539643e-05
20819,41640,20820,62460,23.43289303779602,1.173110968011315e-05
20848,41698,20849,62547,23.476903915405273,1.1493490546854446e-05
20877,41756,20878,62634,23.507819175720215,1.1278663464509009e-05
20906,41814,20907,62721,23.55040693283081,1.104304544696788e-05
20935,41872,20936,62808,23.592947006225586,1.0831389658960688e-05
20964,41930,20965,62895,23.63287091255188,1.062838850884873e-05
20993,41988,20994,62982,23.663340091705322,1.0379462651144422e-05
21023,42048,21024,63072,23.705272912979126,1.021042328375188e-05
21052,42106,21053,63159,23.73805809020996,9.980577942769742e-06
21081,42164,21082,63246,23.76912498474121,9.817405612011498e-06
21110,42222,21111,63333,23.800182104110718,9.618820058676647e-06
21139,42280,21140,63420,23.832481145858765,9.42721806040936e-06
21168,42338,21169,63507,23.866971969604492,9.229399779542291e-06
21197,42396,21198,63594,23.89829993247986,9.07222056412138e-06
21226,42454,21227,63681,23.931344032287598,8.892205642041517e-06
21255,42512,21256,63768,23.962602138519287,8.693876452525728e-06
21285,42572,21286,63858,23.99613904953003,8.527647310074826e-06
21314,42630,21315,63945,24.028895139694214,8.366676979676413e-06
21343,42688,21344,64032,24.059355974197388,8.195719146897318e-06
21372,42746,21373,64119,24.091284036636353,8.026730142773886e-06
21401,42804,21402,64206,24.123180866241455,7.888511845521862e-06
21430,42862,21431,64293,24.15436601638794,7.714118282819982e-06
21459,42920,21460,64380,24.194358110427856,7.557411549896642e-06
21488,42978,21489,64467,24.23822593688965,7.410775651806034e-06
21518,43038,21519,64557,24.28326416015625,7.262208669089887e-06
21547,43096,21548,64644,24.330167770385742,7.1489664605906e-06
21576,43154,21577,64731,24.361403942108154,6.987305823713541e-06
21605,43212,21606,64818,24.407012939453125,6.855091783108946e-06
21634,43270,21635,64905,24.452502965927124,6.713075663355994e-06
21663,43328,21664,64992,24.499172925949097,6.5791700762929395e-06
21692,43386,21693,65079,24.536648988723755,6.4507091792620486e-06
21721,43444,21722,65166,24.570065021514893,6.326773018372478e-06
21750,43502,21751,65253,24.6025390625,6.207595220075746e-06
21780,43562,21781,65343,24.638493061065674,6.0906531871296465e-06
21809,43620,21810,65430,24.670977115631104,5.979501338515547e-06
21838,43678,21839,65517,24.70610785484314,5.872201882084482e-06
21867,43736,21868,65604,24.739288806915283,5.759349505751743e-06
21896,43794,21897,65691,24.783151865005493,5.652035383718612e-06
21925,43852,21926,65778,24.827385902404785,5.543867132473679e-06
21954,43910,21955,65865,24.8591890335083,5.449808895718888e-06
21983,43968,21984,65952,24.901614904403687,5.352998869057046e-06
22013,44028,22014,66042,24.94395089149475,5.235814796833438e-06
22042,44086,22043,66129,24.9862539768219,5.130145950715814e-06
22071,44144,22072,66216,25.027027130126953,5.032015337746998e-06
22100,44202,22101,66303,25.05866813659668,4.935396418659366e-06
22129,44260,22130,66390,25.095183849334717,4.840527367377945e-06
22158,44318,22159,66477,25.12839412689209,4.736679215966433e-06
22187,44376,22188,66564,25.160424947738647,4.644697241928952e-06
22216,44434,22217,66651,25.192800998687744,4.552254949885537e-06
22245,44492,22246,66738,25.224284887313843,4.473418812267482e-06
22275,44552,22276,66828,25.25570797920227,4.384485237096669e-06
22304,44610,22305,66915,25.287340879440308,4.301510443838197e-06
22333,44668,22334,67002,25.328798055648804,4.203207140562881e-06
22362,44726,22363,67089,25.360389947891235,4.123722419535625e-06
22391,44784,22392,67176,25.402112007141113,4.047439006171771e-06
22420,44842,22421,67263,25.442019939422607,3.9781831446816796e-06
22449,44900,22450,67350,25.481218814849854,3.878343477481394e-06
22478,44958,22479,67437,25.51162099838257,3.797294539253926e-06
22508,45018,22509,67527,25.553609132766724,3.712137186084874e-06
22537,45076,22538,67614,25.59365200996399,3.6423734854906797e-06
22566,45134,22567,67701,25.633466958999634,3.5709867916011717e-06
22595,45192,22596,67788,25.66436791419983,3.5016727224501665e-06
22624,45250,22625,67875,25.70063805580139,3.4319828046136536e-06
22653,45308,22654,67962,25.733274936676025,3.365607540217752e-06
22682,45366,22683,68049,25.762502908706665,3.3036176319001243e-06
22711,45424,22712,68136,25.793381929397583,3.2400794225395657e-06
22740,45482,22741,68223,25.824362993240356,3.167693762406998e-06
22770,45542,22771,68313,25.854636907577515,3.102795403719938e-06
22799,45600,22800,68400,25.885719776153564,3.0379388817891595e-06
22828,45658,22829,68487,25.915699005126953,2.985852916026488e-06
22857,45716,22858,68574,25.946638822555542,2.92795914447197e-06
22886,45774,22887,68661,25.977808952331543,2.872112531804305e-06
22915,45832,22916,68748,26.006969928741455,2.818334110088472e-06
22944,45890,22945,68835,26.037222862243652,2.770089395198738e-06
22973,45948,22974,68922,26.06690788269043,2.7141353484694264e-06
23003,46008,23004,69012,26.09786605834961,2.65864957782469e-06
23032,46066,23033,69099,26.128354787826538,2.6060733944177628e-06
23061,46124,23062,69186,26.157864093780518,2.5424329805900925e-06
23090,46182,23091,69273,26.188756942749023,2.4866410512913717e-06
23119,46240,23120,69360,26.218204021453857,2.4410338710367796e-06
23148,46298,23149,69447,26.248334884643555,2.3918761371533037e-06
23177,46356,23178,69534,26.278897047042847,2.3436455194314476e-06
23206,46414,23207,69621,26.308865070343018,2.3095640244719107e-06
23235,46472,23236,69708,26.338721752166748,2.2525094891534536e-06
23265,46532,23266,69798,26.369295835494995,2.2092170866017113e-06
23294,46590,23295,69885,26.399361848831177,2.1491412098839646e-06
23323,46648,23324,69972,26.42909288406372,2.106631427523098e-06
23352,46706,23353,70059,26.458359956741333,2.0712044488391257e-06
23381,46764,23382,70146,26.488550901412964,2.0264966451577493e-06
23410,46822,23411,70233,26.517996788024902,1.9900335246347822e-06
23439,46880,23440,70320,26.548972845077515,1.9521360172802815e-06
23468,46938,23469,70407,26.58166003227234,1.915450980050082e-06
23498,46998,23499,70497,26.61321997642517,1.8799953522830037e-06
23527,47056,23528,70584,26.645572900772095,1.8369211147728493e-06
23556,47114,23557,70671,26.67868709564209,1.8058202613246976e-06
23585,47172,23586,70758,26.709557056427002,1.7655343071965035e-06
23614,47230,23615,70845,26.739692211151123,1.7345262222079327e-06
23643,47288,23644,70932,26.769665956497192,1.6988084325930686e-06
23672,47346,23673,71019,26.79877781867981,1.6617154869891237e-06
23701,47404,23702,71106,26.828396797180176,1.631522536627017e-06
23730,47462,23731,71193,26.85826277732849,1.598087123966252e-06
23760,47522,23761,71283,26.891674041748047,1.5661784118492506e-06
23789,47580,23790,71370,26.921120166778564,1.5364274759122054e-06
23818,47638,23819,71457,26.950618982315063,1.5050018191686831e-06
23847,47696,23848,71544,26.980735063552856,1.4750248737982474e-06
23876,47754,23877,71631,27.010493993759155,1.4450043863689643e-06
23905,47812,23906,71718,27.04121494293213,1.416068698745221e-06
23934,47870,23935,71805,27.070791959762573,1.3906009144193376e-06
23963,47928,23964,71892,27.100564002990723,1.3539429346565157e-06
23993,47988,23994,71982,27.131290912628174,1.3247148444861523e-06
24022,48046,24023,72069,27.160823822021484,1.3012098634135327e-06
24051,48104,24052,72156,27.19133496284485,1.2753389455610886e-06
24080,48162,24081,72243,27.220911979675293,1.2509660791693022e-06
24109,48220,24110,72330,27.250513076782227,1.2251645102878683e-06
24138,48278,24139,72417,27.28067374229431,1.1976114819844952e-06
24167,48336,24168,72504,27.309969902038574,1.1710160379152512e-06
24196,48394,24197,72591,27.339958906173706,1.1492973044369137e-06
24225,48452,24226,72678,27.37005090713501,1.1274885309831006e-06
24255,48512,24256,72768,27.40063500404358,1.101699467653816e-06
24284,48570,24285,72855,27.430917978286743,1.07924915937474e-06
24313,48628,24314,72942,27.463001012802124,1.0585373502181028e-06
24342,48686,24343,73029,27.50547218322754,1.0368388529968797e-06
24371,48744,24372,73116,27.540467023849487,1.0159571957046865e-06
24400,48802,24401,73203,27.57779312133789,9.926717439157073e-07
24429,48860,24430,73290,27.608389854431152,9.71353983914014e-07
24458,48918,24459,73377,27.65056300163269,9.509897154202918e-07
24487,48976,24488,73464,27.691514015197754,9.328671239927644e-07
24517,49036,24518,73554,27.73319411277771,9.134959100265405e-07
24546,49094,24547,73641,27.762924909591675,8.950451046985108e-07
24575,49152,24576,73728,27.80402112007141,8.774027264735196e-07
24604,49210,24605,73815,27.844559907913208,8.624934935141937e-07
24633,49268,24634,73902,27.88814091682434,8.43995735522185e-07
24662,49326,24663,73989,27.931001901626587,8.264474899988272e-07
24691,49384,24692,74076,27.962317943572998,8.0810184499569e-07
24720,49442,24721,74163,27.994548082351685,7.917614084362867e-07
24750,49502,24751,74253,28.02641201019287,7.746600658720126e-07
24779,49560,24780,74340,28.055835008621216,7.594119324494386e-07
24808,49618,24809,74427,28.086731910705566,7.440995659635519e-07
24837,49676,24838,74514,28.11637306213379,7.299755679923692e-07
24866,49734,24867,74601,28.14729595184326,7.15702299203258e-07
24895,49792,24896,74688,28.178112983703613,6.999329116297304e-07
24924,49850,24925,74775,28.2079119682312,6.85950908518862e-07
24953,49908,24954,74862,28.238287925720215,6.715306426485768e-07
24982,49966,24983,74949,28.268322944641113,6.589875738427509e-07
25012,50026,25013,75039,28.302134037017822,6.450601404139888e-07
25041,50084,25042,75126,28.34648895263672,6.314425036180182e-07
25070,50142,25071,75213,28.38944387435913,6.183501000123215e-07
25099,50200,25100,75300,28.421813011169434,6.055383892089594e-07
25128,50258,25129,75387,28.453507900238037,5.930979796175961e-07
25157,50316,25158,75474,28.486783027648926,5.818534418722265e-07
25186,50374,25187,75561,28.529435873031616,5.705486501028645e-07
25215,50432,25216,75648,28.574640035629272,5.57159637537552e-07
25245,50492,25246,75738,28.60849118232727,5.455402742882143e-07
25274,50550,25275,75825,28.65116596221924,5.331240799932857e-07
25303,50608,25304,75912,28.690838098526,5.22460709362349e-07
25332,50666,25333,75999,28.732687950134277,5.129901410327875e-07
25361,50724,25362,76086,28.763415813446045,5.0165817810921e-07
25390,50782,25391,76173,28.80258798599243,4.9041216243495e-07
25419,50840,25420,76260,28.842772006988525,4.790347247762838e-07
25448,50898,25449,76347,28.88181781768799,4.685695103034959e-07
25477,50956,25478,76434,28.910754919052124,4.5874685383751057e-07
25507,51016,25508,76524,28.948171138763428,4.4887542571814265e-07
25536,51074,25537,76611,28.991771936416626,4.3978820940537844e-07
25565,51132,25566,76698,29.084707975387573,4.3027409901696956e-07
25594,51190,25595,76785,29.130148887634277,4.2053568449773593e-07
25623,51248,25624,76872,29.159934997558594,4.1368764414073667e-07
25652,51306,25653,76959,29.195854902267456,4.03403646487277e-07
25681,51364,25682,77046,29.231196880340576,3.947152436012402e-07
25710,51422,25711,77133,29.260915994644165,3.848294909403194e-07
25740,51482,25741,77223,29.29952907562256,3.7568918287433917e-07
25769,51540,25770,77310,29.341737031936646,3.678238726934069e-07
25798,51598,25799,77397,29.384535789489746,3.600932814151747e-07
25827,51656,25828,77484,29.41614603996277,3.5215077787142945e-07
25856,51714,25857,77571,29.45371699333191,3.4540232718427433e-07
25885,51772,25886,77658,29.492758750915527,3.3748699479474453e-07
25914,51830,25915,77745,29.54266595840454,3.3040112157323165e-07
25943,51888,25944,77832,29.589242935180664,3.226959961466491e-07
25972,51946,25973,77919,29.63338804244995,3.1490583296545083e-07
26002,52006,26003,78009,29.67902183532715,3.0786998195253545e-07
26031,52064,26032,78096,29.712574005126953,3.011430180777097e-07
26060,52122,26061,78183,29.750337839126587,2.9392674605333013e-07
26089,52180,26090,78270,29.78938889503479,2.876489588743425e-07
26118,52238,26119,78357,29.83120894432068,2.8149258923804155e-07
26147,52296,26148,78444,29.861371994018555,2.7501471322466386e-07
26176,52354,26177,78531,29.904866933822632,2.6949078346660826e-07
26205,52412,26206,78618,29.945921897888184,2.631722963997163e-07
26235,52472,26236,78708,29.986008882522583,2.553231297497405e-07
26264,52530,26265,78795,30.033087968826294,2.505794327589683e-07
26293,52588,26294,78882,30.077862977981567,2.4451674107695e-07
26322,52646,26323,78969,30.107218980789185,2.385205561949988e-07
26351,52704,26352,79056,30.151428937911987,2.3283553218789166e-07
26380,52762,26381,79143,30.192997932434082,2.2639210328634363e-07
26409,52820,26410,79230,30.227200031280518,2.221166823801468e-07
26438,52878,26439,79317,30.256489038467407,2.171739197365241e-07
26467,52936,26468,79404,30.289308071136475,2.1215760170889553e-07
26497,52996,26498,79494,30.323330879211426,2.074198164336849e-07
26526,53054,26527,79581,30.353869915008545,2.0237280295987148e-07
26555,53112,26556,79668,30.39570689201355,1.978377213163185e-07
26584,53170,26585,79755,30.435851097106934,1.936687112902291e-07
26613,53228,26614,79842,30.466317892074585,1.8860100681195036e-07
26642,53286,26643,79929,30.500854969024658,1.8442119653627742e-07
26671,53344,26672,80016,30.53305983543396,1.8000355339609087e-07
26700,53402,26701,80103,30.562665939331055,1.7528088847029721e-07
26730,53462,26731,80193,30.596932888031006,1.7067759472411126e-07
26759,53520,26760,80280,30.638383865356445,1.657513166719582e-07
26788,53578,26789,80367,30.679797172546387,1.6173589756363072e-07
26817,53636,26818,80454,30.714584827423096,1.575089072503033e-07
26846,53694,26847,80541,30.807987928390503,1.5382795481855283e-07
26875,53752,26876,80628,30.850913047790527,1.500999360359856e-07
26904,53810,26905,80715,30.892449855804443,1.4665204162156442e-07
26933,53868,26934,80802,30.94045400619507,1.432011913493625e-07
26962,53926,26963,80889,30.982383012771606,1.396248308083159e-07
26992,53986,26993,80979,31.01396894454956,1.3608860172098503e-07
27021,54044,27022,81066,31.05334210395813,1.3274484444991685e-07
27050,54102,27051,81153,31.097004890441895,1.2907639757031575e-07
27079,54160,27080,81240,31.134080171585083,1.2594875897775637e-07
27108,54218,27109,81327,31.1663761138916,1.2272664662305033e-07
27137,54276,27138,81414,31.197402000427246,1.1903989616257604e-07
27166,54334,27167,81501,31.233131170272827,1.1658607945719268e-07
27195,54392,27196,81588,31.262609004974365,1.1298072877252707e-07
27225,54452,27226,81678,31.307544946670532,1.0986570941895479e-07
27254,54510,27255,81765,31.34969997406006,1.0714222753449576e-07
27283,54568,27284,81852,31.389124870300293,1.0426424523757305e-07
27312,54626,27313,81939,31.42640709877014,1.0131418548553484e-07
27341,54684,27342,82026,31.455985069274902,9.802499789657304e-08
27370,54742,27371,82113,31.486698150634766,9.559562386129983e-08
27399,54800,27400,82200,31.51749587059021,9.313851023762254e-08
27428,54858,27429,82287,31.54803991317749,9.029974989971379e-08
27457,54916,27458,82374,31.578490018844604,8.766744485910749e-08
27487,54976,27488,82464,31.608755111694336,8.501262982463231e-08
27516,55034,27517,82551,31.639319896697998,8.260144568339456e-08
27545,55092,27546,82638,31.669832944869995,8.033657650230452e-08
27574,55150,27575,82725,31.70025897026062,7.790799827489536e-08
27603,55208,27604,82812,31.730498790740967,7.546509550593328e-08
27632,55266,27633,82899,31.759648084640503,7.303901838895399e-08
27661,55324,27662,82986,31.791148900985718,7.08148490957683e-08
27690,55382,27691,83073,31.822057962417603,6.857715106889373e-08
27719,55440,27720,83160,31.852150917053223,6.657137419097126e-08
27749,55500,27750,83250,31.885108947753906,6.422123988159001e-08
27778,55558,27779,83337,31.915423154830933,6.226457571756328e-08
27807,55616,27808,83424,31.951364994049072,6.024913545843447e-08
27836,55674,27837,83511,31.988078832626343,5.815570602862863e-08
27865,55732,27866,83598,32.02492594718933,5.614731435343856e-08
27894,55790,27895,83685,32.05873107910156,5.433173555502435e-08
27923,55848,27924,83772,32.10167098045349,5.246238288236782e-08
27952,55906,27953,83859,32.14052104949951,5.013168902223697e-08
27982,55966,27983,83949,32.17709493637085,4.815706233785022e-08
28011,56024,28012,84036,32.208839893341064,4.667356279242085e-08
28040,56082,28041,84123,32.241211891174316,4.4549096855917014e-08
28069,56140,28070,84210,32.27468705177307,4.299738520785468e-08
28098,56198,28099,84297,32.30714988708496,4.108699158678064e-08
28127,56256,28128,84384,32.33984017372131,3.9242081584234256e-08
28156,56314,28157,84471,32.37233209609985,3.784009550145129e-08
28185,56372,28186,84558,32.40425205230713,3.634340828284621e-08
28214,56430,28215,84645,32.43646001815796,3.479772203718312e-08
28244,56490,28245,84735,32.46820402145386,3.324203134980053e-08
28273,56548,28274,84822,32.499255895614624,3.182969976478489e-08
28302,56606,28303,84909,32.529435873031616,3.0435558073804714e-08
28331,56664,28332,84996,32.55926299095154,2.9063130568829365e-08
28360,56722,28361,85083,32.58969187736511,2.7617602427199017e-08
28389,56780,28390,85170,32.61989092826843,2.6356133275839966e-08
28418,56838,28419,85257,32.650554895401,2.5006215764733497e-08
28447,56896,28448,85344,32.680809020996094,2.3195411813503597e-08
28477,56956,28478,85434,32.7118079662323,2.1954292606096715e-08
28506,57014,28507,85521,32.74192500114441,2.071521976176882e-08
28535,57072,28536,85608,32.77291798591614,1.966486706805881e-08
28564,57130,28565,85695,32.80322790145874,1.8336208995606285e-08
28593,57188,28594,85782,32.8334379196167,1.7252659745281562e-08
28622,57246,28623,85869,32.862919092178345,1.616001554793911e-08
28651,57304,28652,85956,32.89459490776062,1.5117848306545056e-08
28680,57362,28681,86043,32.925647020339966,1.3975181900605094e-08
28709,57420,28710,86130,32.9557089805603,1.2800001059076749e-08
28739,57480,28740,86220,32.98841094970703,1.1771817298722453e-08
28768,57538,28769,86307,33.02295899391174,1.06649622466648e-08
28797,57596,28798,86394,33.05431604385376,9.702944225864485e-09
28826,57654,28827,86481,33.086246967315674,8.636334314360283e-09
28855,57712,28856,86568,33.11931896209717,7.549488145741634e-09
28884,57770,28885,86655,33.15017509460449,6.58121734886663e-09
28913,57828,28914,86742,33.1803719997406,5.662514013238251e-09
28942,57886,28943,86829,33.211215019226074,4.320781954447739e-09
28972,57946,28973,86919,33.24301195144653,3.3888909456436522e-09
29001,58004,29002,87006,33.273301124572754,2.482920535840094e-09
29030,58062,29031,87093,33.303414821624756,1.6307240002788603e-09
29059,58120,29060,87180,33.33357906341553,9.115410648519173e-10
29088,58178,29089,87267,33.36736297607422,6.673417374258861e-11


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007259845733642578,2180.042156630883
1001,2003,2002,4005,1.1795940399169922,26.14702239094254
2002,4005,4004,8009,2.3262481689453125,25.525668687436337
3003,6007,6006,12013,3.71964693069458,24.927473239068604
4004,8009,8008,16017,4.8932459354400635,24.350708440477774
5005,10011,10010,20021,5.921699047088623,23.793850993024307
6006,12013,12012,24025,7.118941307067871,23.255550456593937
7007,14015,14014,28029,8.222760200500488,22.73460611589303
8008,16017,16016,32033,9.309657096862793,22.229947315816844
9009,18019,18018,36037,10.399500131607056,21.74061641815024
10010,20021,20020,40041,11.526769161224365,21.265754038815658
11011,22023,22022,44045,12.682967185974121,20.804586294355204
12012,24025,24024,48049,13.776388168334961,20.35641380682364
13013,26027,26026,52053,14.854856967926025,19.920602236250488
14014,28029,28028,56057,15.909304141998291,19.49657413254613
15015,30031,30030,60061,17.004013061523438,19.0838019223811
16016,32033,32032,64065,18.055104970932007,18.68180186959694
17017,34035,34034,68069,19.10994815826416,18.29012886914711
18018,36037,36036,72073,20.18428897857666,11.918281582526106
19019,38039,38038,76077,21.4948410987854,11.684517022200112
20020,40041,40040,80081,22.78827428817749,11.455797829887729
21021,42043,42042,84085,24.064653158187866,11.231997822684548
22022,44045,44044,88089,25.176217079162598,11.012995041667182
23023,46047,46046,92093,26.286429166793823,10.798671525875193
24024,48049,48048,96097,27.385496139526367,10.588913105067604
25025,50051,50050,100101,28.64294409751892,10.38360920928801
26026,52053,52052,104105,30.02674412727356,10.182652693471141
27027,54055,54054,108109,31.32183814048767,9.985939675502777
28028,56057,56056,112113,32.619301080703735,9.793369386336622
29029,58059,58058,116117,33.885931968688965,9.60484403092164
30030,60061,60060,120121,35.14361810684204,9.420268658853502
31031,62063,62062,124125,36.387397050857544,9.239551043784331
32032,64065,64064,128129,37.625450134277344,9.062601570740298
33033,66067,66066,132133,38.86813807487488,8.889333130602267
34034,68069,68068,136137,40.11537504196167,8.719661021083539
35035,70071,70070,140141,41.366605043411255,8.553502853622945
36036,72073,72072,144145,42.61755013465881,8.390778465685457
37037,74075,74074,148149,43.875221967697144,8.231409838005902
38038,76077,76076,152153,45.13353109359741,8.075321016384578
39039,78079,78078,156157,46.41010308265686,7.922438037678944
40040,80081,80080,160161,47.71730709075928,7.772688859676464
41041,82083,82082,164165,48.958730936050415,7.626003294577117
42042,84085,84084,168169,50.21700310707092,7.482312945832632
43043,86087,86086,172173,51.50854825973511,7.341551148130634
44044,88089,88088,176177,53.02587604522705,7.20365291031851
45045,90091,90090,180181,54.42783308029175,7.068554861092025
46046,92093,92092,184185,55.861876010894775,6.936195197286793
47047,94095,94094,188189,57.218971252441406,6.806513634615385
48048,96097,96096,192193,58.51663112640381,6.679451360717508
49049,98099,98098,196197,59.82755208015442,6.554950990383759
50050,100101,100100,200201,61.13320016860962,6.432956522836093
51051,102103,102102,204205,62.415101289749146,6.313413300938578
52052,104105,104104,208209,63.69599199295044,6.196267972230999
53053,106107,106106,212213,65.00720405578613,6.081468451671753
54054,108109,108108,216217,66.28872799873352,5.96896388599032
55055,110111,110110,220221,67.61755704879761,5.858704619544483
56056,112113,112112,224225,68.98797702789307,5.750642161593305
57057,114115,114114,228229,70.32323408126831,5.644729154886704
58058,116117,116116,232233,71.65373015403748,5.540919345498196
59059,118119,118118,236237,72.95379400253296,5.439167553805987
60060,120121,120120,240241,74.2729001045227,5.339429646559211
61061,122123,122122,244245,75.62810802459717,5.241662509952107
62062,124125,124124,248249,76.95198893547058,5.145824023643854
63063,126127,126126,252253,78.27419114112854,5.051873035662538
64064,128129,128128,256257,79.57120513916016,4.959769338139267
65065,130131,130130,260261,80.86096000671387,4.869473643823085
66066,132133,132132,264265,82.17218518257141,4.780947563328482
67067,134135,134134,268269,83.42770624160767,4.694153583074467
68068,136137,136136,272273,84.8796181678772,4.609055043879607
69069,138139,138138,276277,86.36798119544983,4.525616120176437
70070,140141,140140,280281,88.19514918327332,4.443801799813059
71071,142143,142142,284285,89.67325520515442,4.363577864417721
72072,144145,144144,288289,91.43114018440247,4.284910870297722
73073,146147,146146,292293,93.28204607963562,4.207768129848205
74074,148149,148148,296297,94.98753619194031,4.132117693455598
75075,150151,150150,300301,96.4235692024231,4.057928331867629
76076,152153,152152,304305,97.81100606918335,3.9851695190202463
77077,154155,154154,308309,99.26710915565491,3.9138114153007564
78078,156157,156156,312313,101.05611228942871,3.8438248512326254
79079,158159,158158,316317,103.13152527809143,3.7751813115697814
80080,160161,160160,320321,104.61657333374023,3.707852919785182
81081,162163,162162,324325,106.32327008247375,3.6418124229431896
82082,164165,164164,328329,107.70073819160461,3.5770331769455197
83083,166167,166166,332333,109.41236090660095,3.5134891321358737
84084,168169,168168,336337,111.78809118270874,3.451154819258136
85085,170171,170170,340341,114.22790908813477,3.390005335756655
86086,172173,172172,344345,116.28816723823547,3.3300163324073537
87087,174175,174174,348349,118.05696201324463,3.2711640002773947
88088,176177,176176,352353,119.66448402404785,3.2134250579944137
89089,178179,178178,356357,121.26038026809692,3.1567767393310078
90090,180181,180180,360361,122.7654070854187,3.1011967810850365
91091,182183,182182,364365,124.23370313644409,3.0466634112548263
92092,184185,184184,368369,125.74173307418823,2.993155337499502
93093,186187,186186,372373,127.24480628967285,2.9406517358798965
94094,188189,188188,376377,128.7165629863739,2.8891322398704915
95095,190191,190190,380381,130.22077703475952,2.8385769296378385
96096,192193,192192,384385,131.7515721321106,2.7889663215786413
97097,194195,194194,388389,133.32785606384277,2.7402813581106784
98098,196197,196196,392393,134.9156632423401,2.69250339771213
99099,198199,198198,396397,136.42434811592102,2.6456142052011273
100100,200201,200200,400401,137.92635917663574,2.5995959422509713
101101,202203,202202,404405,139.39918303489685,2.554431158137618
102102,204205,204204,408409,140.9534990787506,2.510102780708962
103103,206207,206206,412413,142.4923939704895,2.466594107574224
104104,208209,208208,416417,143.99782824516296,2.4238887975091075
105105,210211,210210,420421,145.55578422546387,2.3819708620668507
106106,212213,212212,424425,147.12378025054932,2.340824657395501
107107,214215,214214,428429,148.6491482257843,2.3004348762527798
108108,216217,216216,432433,150.1728072166443,2.2607865402159177
109109,218219,218218,436437,151.65597224235535,2.221864992079304
110110,220221,220220,440441,153.1646511554718,2.183655888439489
111111,222223,222222,444445,154.65175414085388,2.1461451924579933
112112,224225,224224,448449,156.13468527793884,2.1093191668012423
113113,226227,226226,452453,157.67368602752686,2.0731643667526214
114114,228229,228228,456457,159.19512391090393,2.0376676334899457
115115,230231,230230,460461,160.73475098609924,2.0028160875287995
116116,232233,232232,464465,162.28593730926514,1.9685971223231036
117117,234235,234234,468469,163.80637407302856,1.934998398021321
118118,236237,236236,472473,165.30495715141296,1.9020078353759118
119119,238239,238238,476477,166.82346320152283,1.8696136097973977
120120,240241,240240,480481,168.34947419166565,1.8378041455559924
121121,242243,242242,484485,169.85480308532715,1.8065681101206792
122122,244245,244244,488489,171.41497325897217,1.775894408637214
123123,246247,246246,492493,172.95771431922913,1.7457721785399372
124124,248249,248248,496497,174.47086691856384,1.7161907842914843
125125,250251,250250,500501,175.98939108848572,1.6871398122522123
126126,252253,252252,504505,177.51455211639404,1.6586090656724082
127127,254255,254254,508509,179.02296018600464,1.6305885598046643
128128,256257,256256,512513,180.5037522315979,1.6030685171351706
129129,258259,258258,516517,182.00149416923523,1.576039362728693
130130,260261,260260,520521,183.54354214668274,1.5494917196859888
131131,262263,262262,524525,185.07923197746277,1.5234164047108152
132132,264265,264264,528529,186.8024880886078,1.4978044237818722
133133,266267,266266,532533,188.54477429389954,1.4726469679309275
134134,268269,268268,536537,190.18777513504028,1.4479354091182586
135135,270271,270270,540541,191.8640420436859,1.4236612962107529
136136,272273,272272,544545,193.5749990940094,1.3998163510535733
137137,274275,274274,548549,195.17804217338562,1.3763924646360692
138138,276277,276276,552553,196.70530200004578,1.3533816933494336
139139,278279,278278,556557,198.17506313323975,1.3307762553329212
140140,280281,280280,560561,199.67023730278015,1.3085685269072656
141141,282283,282282,564565,201.17241024971008,1.2867510390917687
142142,284285,284284,568569,202.6632161140442,1.2653164742059744
143143,286287,286286,572573,204.3516390323639,1.2442576625493302
144144,288289,288288,576577,206.0634422302246,1.2235675791613403
145145,290291,290290,580581,207.77424716949463,1.203239340656296
146146,292293,292292,584585,209.47972512245178,1.183266202135087
147147,294295,294294,588589,211.74727296829224,1.1636415541661336
148148,296297,296296,592593,213.6308789253235,1.1443589198412383
149149,298299,298298,596597,215.14835619926453,1.1254119518971493
150150,300301,300300,600601,216.61712098121643,1.106794429906813
151151,302303,302302,604605,218.10503125190735,1.0885002575352019
152152,304305,304304,608609,219.5931911468506,1.0705234598590323
153153,306307,306306,612613,221.05269193649292,1.0528581807502633
154154,308309,308308,616617,222.5551791191101,1.0354986803187103
155155,310311,310310,620621,224.02160716056824,1.018439332416051
156156,312313,312312,624625,225.48346710205078,1.001674622195992
157157,314315,314314,628629,226.99916219711304,0.9851991437313927
158158,316317,316316,632633,228.47133612632751,0.96900759768846
159159,318319,318318,636637,230.00146508216858,0.9530947890505104
160160,320321,320320,640641,231.47496509552002,0.9374556248991439
161161,322323,322322,644645,232.9546821117401,0.9220851122425984
162162,324325,324324,648649,234.43201518058777,0.9069783558959443
163163,326327,326326,652653,235.96005010604858,0.8921305564089153
164164,328329,328328,656657,237.44164109230042,0.8775370080428502
165165,330331,330330,660661,238.93870520591736,0.8631930967909511
166166,332333,332332,664665,240.43890404701233,0.8490942984474259
167167,334335,334334,668669,241.96577095985413,0.8352361767173306
168168,336337,336336,672673,243.5674171447754,0.8216143813713188
169169,338339,338338,676677,245.31973314285278,0.8082246464417722
170170,340341,340340,680681,247.0700011253357,0.7950627884599726
171171,342343,342342,684685,248.71241331100464,0.7821247047317001
172172,344345,344344,688689,250.42980027198792,0.7694063716559185
173173,346347,346346,692693,252.18307828903198,0.7569038430748378
174174,348349,348348,696697,253.75297832489014,0.7446132486683155
175175,350351,350350,700701,255.6963551044464,0.7325307923786113
176176,352353,352352,704705,257.34341621398926,0.7206527508733416
177177,354355,354354,708709,258.93831515312195,0.7089754720423116
178178,356357,356356,712713,260.61542201042175,0.6974953735289091
179179,358359,358358,716717,262.21469616889954,0.6862089412910564
180180,360361,360360,720721,263.72581028938293,0.6751127281978597
181181,362363,362362,724725,265.35804533958435,0.6642033526565001
182182,364365,364364,728729,267.2003011703491,0.6534774972679998
183183,366367,366366,732733,268.9291250705719,0.6429319075140256
184184,368369,368368,736737,270.50851106643677,0.6325633904739334
185185,370371,370370,740741,272.124587059021,0.62236881356705
186186,372373,372372,744745,273.784019947052,0.6123451033257652
187187,374375,374374,748749,275.3061990737915,0.6024892441938619
188188,376377,376376,752753,276.9939179420471,0.5927982773522444
189189,378379,378378,756757,278.5402190685272,0.5832692995684283
190190,380381,380380,760761,280.0576729774475,0.5738994620750191
191191,382383,382382,764765,281.5452160835266,0.5646859694684281
192192,384385,384384,768769,283.0817000865936,0.555626078634532
193193,386387,386386,772773,284.7252290248871,0.5467170976962734
194194,388389,388388,776777,286.61313819885254,0.5379563849847955
195195,390391,390390,780781,288.6849820613861,0.5293413480334266
196196,392393,392392,784785,290.27971625328064,0.5208694425912199
197197,394395,394394,788789,292.6612300872803,0.5125381716610491
198198,396397,396396,792793,295.1947331428528,0.50434508455578
199199,398399,398398,796797,297.2018790245056,0.49628777597592943
200200,400401,400400,800801,298.97299909591675,0.48836388510744655
201201,402403,402402,804805,300.86432218551636,0.48057109473791115
202202,404405,404404,808809,302.99670028686523,0.47290713039274124
203203,406407,406406,812813,304.6389181613922,0.46536975948879444
204204,408409,408408,816817,306.21801018714905,0.45795679050741
205205,410411,410410,820821,307.866464138031,0.4506660721835942
206206,412413,412412,824825,309.80682706832886,0.4434954927135095
207207,414415,414414,828829,312.64795112609863,0.4364429789782207
208208,416417,416416,832833,315.58292603492737,0.4295064957842669
209209,418419,418418,836837,318.0308301448822,0.4226840451209455
210210,420421,420420,840841,320.91439723968506,0.41597366543123826
211211,422423,422422,844845,323.2616980075836,0.40937343090058675
212212,424425,424424,848849,324.79346990585327,0.4028814507586276
213213,426427,426426,852853,326.28093218803406,0.3964958685972988
214214,428429,428428,856857,327.7789659500122,0.390214861702475
215215,430431,430430,860861,329.25873708724976,0.3840366403982216
216216,432433,432432,864865,330.79500102996826,0.37795944740821596
217217,434435,434434,868869,332.28206515312195,0.37198155722717274
218218,436437,436436,872873,333.7859010696411,0.3661012755071624
219219,438439,438438,876877,335.4068121910095,0.3603169384555258
220220,440441,440440,880881,336.9550371170044,0.3546269122469994
221221,442443,442442,884885,338.49807119369507,0.34902959244629983
222222,444445,444444,888889,339.995548248291,0.3435234034437826
223223,446447,446446,892893,341.51244711875916,0.33810679790212816
224224,448449,448448,896897,343.00766611099243,0.33277825621496504
225225,450451,450450,900901,344.53441619873047,0.3275362859760662
226226,452453,452452,904905,345.9988579750061,0.3223794214602549
227227,454455,454454,908909,347.47288393974304,0.3173062231142012
228228,456457,456456,912913,349.00755500793457,0.31231527705836015
229229,458459,458458,916917,350.7804663181305,0.3074051945980045
230230,460461,460460,920921,352.28906321525574,0.30257461174608125
231231,462463,462462,924925,353.981290102005,0.297822188753571
232232,464465,464464,928929,355.5675640106201,0.29314660965121675
233233,466467,466466,932933,357.0582709312439,0.2885465818001194
234234,468469,468468,936937,359.20693826675415,0.284020835450292
235235,470471,470470,940941,361.2550621032715,0.2795681233103551
236236,472473,472472,944945,363.4934060573578,0.2751872201243941
237237,474475,474474,948949,365.15199732780457,0.2708769222565479
238238,476477,476476,952953,366.75338912010193,0.26663604728685186
239239,478479,478478,956957,368.3124601840973,0.2624634336125382
240240,480481,480480,960961,369.87755012512207,0.2583579400582039
241241,482483,482482,964965,371.43376302719116,0.2543184454945049
242242,484485,484484,968969,373.0047879219055,0.2503438484634444
243243,486487,486486,972973,374.592493057251,0.2464330668119601
244244,488489,488488,976977,376.17693519592285,0.24258503733233283
245245,490491,490490,980981,377.6888921260834,0.23879871541021203
246246,492493,492492,984985,379.30817317962646,0.23507307467878036
247247,494495,494494,988989,380.9773449897766,0.23140710668064912
248248,496497,496496,992993,382.53432607650757,0.2277998205372569
249249,498499,498498,996997,384.05974292755127,0.22425024262213356
250250,500501,500500,1001001,385.63947224617004,0.22075741624360035
251251,502503,502502,1005005,387.20777130126953,0.21732040133122155
252252,504505,504504,1009009,388.7677011489868,0.21393827413135114
253253,506507,506506,1013013,390.25963592529297,0.21061012690518055
254254,508509,508508,1017017,391.84009313583374,0.20733506763610876
255255,510511,510510,1021021,393.3335340023041,0.20411221973995453
256256,512513,512512,1025025,394.8935899734497,0.20094072178369515
257257,514515,514514,1029029,396.52060532569885,0.19781972720636531
258258,516517,516516,1033033,398.2976040840149,0.19474840404859606
259259,518519,518518,1037037,399.87741708755493,0.19172593468647392
260260,520521,520520,1041041,401.3858461380005,0.1887515155683559
261261,522523,522522,1045045,402.9370491504669,0.18582435696089306
262262,524525,524524,1049049,404.66888213157654,0.1829436826960773
263263,526527,526526,1053053,406.20707726478577,0.18010872992624627
264264,528529,528528,1057057,407.94826912879944,0.17731874888102084
265265,530531,530530,1061061,409.95349192619324,0.1745730026318597
266266,532533,532532,1065065,411.50649213790894,0.1718707668588877
267267,534535,534534,1069069,413.2206621170044,0.16921132962306729
268268,536537,536536,1073073,414.7425501346588,0.1665939911431451
269269,538539,538538,1077077,416.93540930747986,0.16401806357669102
270270,540541,540540,1081081,418.53764605522156,0.16148287080409318
271271,542543,542542,1085085,420.11750507354736,0.15898774821891948
272272,544545,544544,1089089,421.64338421821594,0.15653204252055275
273273,546547,546546,1093093,423.6504690647125,0.15411511151160084
274274,548549,548548,1097097,425.66623306274414,0.15173632389883096
275275,550551,550550,1101101,427.2003390789032,0.14939505909808304
276276,552553,552552,1105105,428.721204996109,0.14709070704270744
277277,554555,554554,1109109,430.7197461128235,0.1448226679964364
278278,556557,556556,1113113,432.34219908714294,0.14259035236784712
279279,558559,558558,1117117,433.8383810520172,0.14039318053107763
280280,560561,560560,1121121,435.33324122428894,0.13823058264813426
281281,562563,562562,1125125,436.8505551815033,0.13610199849381388
282282,564565,564564,1129129,438.31437706947327,0.1340068772867653
283283,566567,566566,1133133,439.83183097839355,0.13194467752134642
284284,568569,568568,1137137,441.3703889846802,0.12991486680266462
285285,570571,570570,1141141,442.86720609664917,0.1279169216866194
286286,572573,572572,1145145,444.34007716178894,0.12595032752051338
287287,574575,574574,1149149,445.8329322338104,0.12401457828934781
288288,576577,576576,1153153,447.3150372505188,0.12210917646223152
289289,578579,578578,1157157,449.32796597480774,0.12023363284311017
290290,580581,580580,1161161,451.41433119773865,0.11838746642513343
291291,582583,582582,1165165,453.0999901294708,0.11657020424570419
292292,584585,584584,1169169,455.19635009765625,0.11478138124550696
293293,586587,586586,1173173,457.5887451171875,0.11302054013026464
294294,588589,588588,1177177,459.6534252166748,0.11128723123465534
295295,590591,590590,1181181,461.363379240036,0.10958101238850304
296296,592593,592592,1185185,463.14642810821533,0.10790144878603769
297297,594595,594594,1189189,464.7587630748749,0.10624811285708802
298298,596597,596596,1193193,466.25017499923706,0.10462058414123021
299299,598599,598598,1197197,467.73979806900024,0.10301844916364189
300300,600601,600600,1201201,469.26269793510437,0.10144130131379825
301301,602603,602602,1205205,471.1866521835327,0.09988874072575982
302302,604605,604604,1209209,473.1780331134796,0.09836037416130239
303303,606607,606606,1213213,474.9058561325073,0.09685581489463857
304304,608609,608608,1217217,476.59424209594727,0.09537468259952675
305305,610611,610610,1221221,478.1454691886902,0.09391660323979067
306306,612613,612612,1225225,479.7596561908722,0.09248120895779266
307307,614615,614614,1229229,481.3715012073517,0.09106813797041013
308308,616617,616616,1233233,482.89807510375977,0.0896770344622837
309309,618619,618618,1237237,484.39459705352783,0.08830754848452216
310310,620621,620620,1241241,485.875675201416,0.08695933585170224
311311,622623,622622,1245245,487.516371011734,0.08563205804443896
312312,624625,624624,1249249,489.1335492134094,0.08432538211093288
313313,626627,626626,1253253,490.69351720809937,0.08303898057181414
314314,628629,628628,1257257,492.29329204559326,0.08177253132555506
315315,630631,630630,1261261,493.8545620441437,0.080525717557407
316316,632633,632632,1265265,495.39056730270386,0.07929822764765504
317317,634635,634634,1269269,497.0248181819916,0.07808975508351068
318318,636637,636636,1273273,498.61791610717773,0.07689999837145933
319319,638639,638638,1277277,500.20578622817993,0.07572866095199515
320320,640641,640640,1281281,501.78021907806396,0.07457545111446962
321321,642643,642642,1285285,503.315443277359,0.07344008191546436
322322,644645,644644,1289289,504.8793489933014,0.07232227109648193
323323,646647,646646,1293293,506.4813241958618,0.07122174100584289
324324,648649,648648,1297297,508.06101512908936,0.07013821851865032
325325,650651,650650,1301301,509.5917110443115,0.06907143496118806
326326,652653,652652,1305305,511.08121705055237,0.06802112603475052
327327,654655,654654,1309309,512.6914203166962,0.06698703174106413
328328,656657,656656,1313313,514.3622419834137,0.0659688963106646
329329,658659,658658,1317317,516.1433589458466,0.06496646813047846
330330,660661,660660,1321321,517.7964069843292,0.06397949967333716
331331,662663,662662,1325325,520.2968990802765,0.06300774742953763
332332,664665,664664,1329329,523.2275912761688,0.06205097183919861
333333,666667,666666,1333333,525.8577771186829,0.06110893722450328
334334,668669,668668,1337337,528.0438961982727,0.060181411725466205
335335,670671,670670,1341341,529.8068730831146,0.05926816723558659
336336,672673,672672,1345345,531.390064239502,0.05836897933738783
337337,674675,674674,1349349,532.9355289936066,0.05748362724239087
338338,676677,676676,1353353,534.5206830501556,0.056611893728700124
339339,678679,678678,1357357,536.0964012145996,0.055753565081545275
340340,680681,680680,1361361,537.663003206253,0.05490843103518728
341341,682683,682682,1365365,539.7003610134125,0.0540762847139149
342342,684685,684684,1369369,542.3308391571045,0.05325692257611081
343343,686687,686686,1373373,545.1068360805511,0.052450144358545
344344,688689,688688,1377377,548.5826501846313,0.05165575302146408
345345,690691,690690,1381381,551.3040211200714,0.05087355469413524
346346,692693,692692,1385385,552.901643037796,0.05010335862334614
347347,694695,694694,1389389,554.8709750175476,0.04934497712008579
348348,696697,696696,1393393,557.1469252109528,0.04859822550952231
349349,698699,698698,1397397,559.3552892208099,0.0478629220797302
350350,700701,700700,1401401,561.3339900970459,0.04713888803394184
351351,702703,702702,1405405,562.9791371822357,0.04642594744063899
352352,704705,704704,1409409,564.5845000743866,0.04572392718739593
353353,706707,706706,1413413,567.077445268631,0.04503265693222147
354354,708709,708708,1417417,568.6232941150665,0.04435196905956218
355355,710711,710710,1421421,570.1065752506256,0.043681698634486565
356356,712713,712712,1425425,571.6650969982147,0.04302168335755141
357357,714715,714714,1429429,573.1418361663818,0.042371763522510264
358358,716717,716716,1433433,574.6664183139801,0.04173178197220295
359359,718719,718718,1437437,576.1841042041779,0.041101584057628315
360360,720721,720720,1441441,577.6829092502594,0.04048101759542533
361361,722723,722722,1445445,579.2352561950684,0.0398699328281964
362362,724725,724724,1449449,581.0741429328918,0.039268182384375905
363363,726727,726726,1453453,582.7797319889069,0.038675621238098756
364364,728729,728728,1457457,585.1400640010834,0.038092106671570036
365365,730731,730730,1461461,586.7927751541138,0.037517498236752544
366366,732733,732732,1465465,588.3198721408844,0.03695165771830489
367367,734735,734734,1469469,590.1658930778503,0.03639444909640588
368368,736737,736736,1473473,591.7107923030853,0.035845738510829506
369369,738739,738738,1477477,593.2155442237854,0.035305394226725184
370370,740741,740740,1481481,594.7619199752808,0.0347732865980106
371371,742743,742742,1485485,596.4641170501709,0.0342492880346299
372372,744745,744744,1489489,598.000785112381,0.033733272967765515
373373,746747,746746,1493493,599.5298130512238,0.03322511781789217
374374,748749,748748,1497497,601.0883829593658,0.03272470096123925
375375,750751,750750,1501501,602.7636561393738,0.03223190269909537
376376,752753,752752,1505505,604.3578491210938,0.0317466052247255
377377,754755,754754,1509509,605.8951869010925,0.031268692594494496
378378,756757,756756,1513513,607.6248090267181,0.030798050695807433
379379,758759,758758,1517517,609.2632071971893,0.03033456721868788
380380,760761,760760,1521521,610.8217370510101,0.029878131624627713
381381,762763,762762,1525525,612.3644690513611,0.02942863512043914
382382,764765,764764,1529529,614.0532360076904,0.02898597062733188
383383,766767,766766,1533533,615.7891619205475,0.028550032754424137
384384,768769,768768,1537537,617.6531262397766,0.028120717771230375
385385,770771,770770,1541541,619.1610281467438,0.027697923580603856
386386,772773,772772,1545545,620.6630730628967,0.027281549691679174
387387,774775,774774,1549549,622.171067237854,0.026871497195429583
388388,776777,776776,1553553,623.644562959671,0.026467668737041095
389389,778779,778778,1557557,625.1332352161407,0.02606996849283405
390390,780781,780780,1561561,626.8594212532043,0.025678302143319343
391391,782783,782782,1565565,628.3972952365875,0.025292576851256854
392392,784785,784784,1569569,629.907014131546,0.024912701235507484
393393,786787,786786,1573573,631.4175832271576,0.02453858534909159
394394,788789,788788,1577577,633.0173420906067,0.024170140655883188
395395,790791,790790,1581581,634.5330770015717,0.02380728000639465
396396,792793,792792,1585585,636.0590801239014,0.023449917617767824
397397,794795,794794,1589589,637.8171992301941,0.023097969050127176
398398,796797,796796,1593593,639.4200539588928,0.02275135118520666
399399,798799,798798,1597597,640.9992492198944,0.022409982205658707
400400,800801,800800,1601601,642.5034720897675,0.022073781574022178
401401,802803,802802,1605605,644.0190951824188,0.02174267001134922
402402,804805,804804,1609609,645.7599742412567,0.021416569478105885
403403,806807,806806,1613613,647.3812081813812,0.02109540315382219
404404,808809,808808,1617617,649.3574032783508,0.020779095417424287
405405,810811,810810,1621621,651.4843780994415,0.020467571828589826
406406,812813,812812,1625625,653.5293941497803,0.020160759107398007
407407,814815,814814,1629629,655.5177159309387,0.01985858511807237
408408,816817,816816,1633633,657.5923199653625,0.019560978848062405
409409,818819,818818,1637637,660.1882429122925,0.019267870392809527
410410,820821,820820,1641641,662.0819020271301,0.018979190935851875
411411,822823,822822,1645645,665.397066116333,0.018694872732112344
412412,824825,824824,1649649,667.6630783081055,0.01841484909130031
413413,826827,826826,1653653,669.7466340065002,0.018139054360631235
414414,828829,828828,1657657,672.384458065033,0.01786742390845575
415415,830831,830830,1661661,674.3378810882568,0.01759989410788876
416416,832833,832832,1665665,677.810711145401,0.01733640232112066
417417,834835,834834,1669669,681.4378671646118,0.01707688688259168
418418,836837,836836,1673673,684.5225789546967,0.016821287085349468
419419,838839,838838,1677677,686.9299609661102,0.016569543164109746
420420,840841,840840,1681681,688.788064956665,0.016321596281272832
421421,842843,842842,1685685,692.3182451725006,0.016077388512030666
422422,844845,844844,1689689,695.3223762512207,0.015836862829360143
423423,846847,846846,1693693,697.3879821300507,0.015599963090835445
424424,848849,848848,1697697,698.9617540836334,0.015366634023052939
425425,850851,850850,1701701,700.4826261997223,0.015136821209580376
426426,852853,852852,1705705,702.8047559261322,0.01491047107583654
427427,854855,854854,1709709,705.8013679981232,0.014687530877381505
428428,856857,856856,1713713,708.7302520275116,0.01446794868456891
429429,858859,858858,1717717,711.6042001247406,0.014251673372427831
430430,860861,860860,1721721,714.3998332023621,0.014038654605542433
431431,862863,862862,1725725,717.0025761127472,0.013828842826569598
432432,864865,864864,1729729,718.6707310676575,0.013622189244188121
433433,866867,866866,1733733,720.3875179290771,0.013418645820479469
434434,868869,868868,1737737,722.1322441101074,0.013218165259786474
435435,870871,870870,1741741,723.5288870334625,0.013020700995639345
436436,872873,872872,1745745,725.3416330814362,0.012826207180864913
437437,874875,874874,1749749,727.169379234314,0.012634638674967391
438438,876877,876876,1753753,728.9817941188812,0.012445951033782876
439439,878879,878878,1757757,730.949716091156,0.01226010049845172
440440,880881,880880,1761761,732.792720079422,0.012077043983822477
441441,882883,882882,1765765,734.568883895874,0.011896739069470641
442442,884885,884884,1769769,736.3967680931091,0.011719143987193092
443443,886887,886886,1773773,738.2464921474457,0.011544217612595276
444444,888889,888888,1777777,740.0928580760956,0.011371919453836199
445445,890891,890890,1781781,741.8705153465271,0.011202209642306116
446446,892893,892892,1785785,743.6093370914459,0.011035048922394708
447447,894895,894894,1789789,745.5456829071045,0.01087039864239614
448448,896897,896896,1793793,747.0367112159729,0.010708220744277241
449449,898899,898898,1797797,748.555260181427,0.010548477755264685
450450,900901,900900,1801801,750.401407957077,0.01039113277784054
451451,902903,902902,1805805,752.6495380401611,0.010236149481784196
452452,904905,904904,1809809,754.1847331523895,0.010083492093713176
453453,906907,906906,1813813,755.7092111110687,0.009933125390489295
454454,908909,908908,1817817,757.2073981761932,0.009785014688418414
455455,910911,910910,1821821,758.7280261516571,0.009639125836315543
456456,912913,912912,1825825,760.2682130336761,0.009495425206523578
457457,914915,914914,1829829,761.7895221710205,0.009353879687068911
458458,916917,916916,1833833,763.3428790569305,0.009214456673134919
459459,918919,918918,1837837,764.8480451107025,0.009077124060354436
460460,920921,920920,1841841,766.5401821136475,0.008941850234805315
461461,922923,922922,1845845,768.1959221363068,0.00880860406755346
462462,924925,924924,1849849,769.8621640205383,0.008677354906353685
463463,926927,926926,1853853,771.8039722442627,0.0085480725671232
464464,928929,928928,1857857,773.4362001419067,0.008420727328484645
465465,930931,930930,1861861,775.0396552085876,0.00829528992358064
466466,932933,932932,1865865,776.6521451473236,0.008171731532911508
467467,934935,934934,1869869,778.1301419734955,0.008050023777400384
468468,936937,936936,1873873,779.7703700065613,0.00793013871191306
469469,938939,938938,1877877,781.3749771118164,0.007812048818664152
470470,940941,940940,1881881,783.583419084549,0.007695726999486396
471471,942943,942942,1885885,785.4646000862122,0.007581146570259989
472472,944945,944944,1889889,787.9025871753693,0.007468281254887188
473473,946947,946946,1893893,790.5282521247864,0.007357105178016354
474474,948949,948948,1897897,792.4607989788055,0.007247592858561802
475475,950951,950950,1901901,794.0889840126038,0.007139719205156325
476476,952953,952952,1905905,795.7511191368103,0.007033459507965745
477477,954955,954954,1909909,797.3106770515442,0.006928789434937244
478478,956957,956956,1913913,798.8483581542969,0.0068256850249781564
479479,958959,958958,1917917,800.5611410140991,0.006724122681362132
480480,960961,960960,1921921,802.0570139884949,0.00662407916763641
481481,962963,962962,1925925,803.5787560939789,0.006525531600573231
482482,964965,964964,1929929,805.2137882709503,0.006428457446645552
483483,966967,966966,1933933,806.7932181358337,0.0063328345140689635
484484,968969,968968,1937937,808.3869462013245,0.006238640949845831
485485,970971,970970,1941941,809.9829759597778,0.0061458552328303995
486486,972973,972972,1945945,811.5577092170715,0.006054456170204503
487487,974975,974974,1949949,813.1222379207611,0.005964422890542664
488488,976977,976976,1953953,814.5959300994873,0.0058757348407425525
489489,978979,978978,1957957,816.1297950744629,0.0057883717792037714
490490,980981,980980,1961961,817.8149790763855,0.005702313772872003
491491,982983,982982,1965965,819.3522491455078,0.005617541191440978
492492,984985,984984,1969969,820.8476331233978,0.005534034702691315
493493,986987,986986,1973973,822.3351612091064,0.005451775267829362
494494,988989,988988,1977977,823.8725380897522,0.005370744137849215
495495,990991,990990,1981981,825.6499111652374,0.005290922847962065
496496,992993,992992,1985985,827.3890151977539,0.005212293213844532
497497,994995,994994,1989989,829.4466390609741,0.005134837326977504
498498,996997,996996,1993993,831.0240662097931,0.005058537551008158
499499,998999,998998,1997997,833.0552780628204,0.0049833765167477395
500501,1001003,1001002,2002005,836.1048760414124,0.004909263707872924
501502,1003005,1003004,2006009,838.6466691493988,0.004836330194734728
502503,1005007,1005006,2010013,841.2880780696869,0.004764484864153928
503504,1007009,1007008,2014017,843.5925559997559,0.004693711376830834
504505,1009011,1009010,2018021,845.8557350635529,0.004623993641530433
505506,1011013,1011012,2022025,847.6878709793091,0.004555315810421234
506507,1013015,1013014,2026029,849.3420243263245,0.004487662275892035
507508,1015017,1015016,2030033,850.9028761386871,0.004421017666686566
508509,1017019,1017018,2034037,852.5422389507294,0.004355366844492892
509510,1019021,1019020,2038041,854.0552771091461,0.004290694900191738
510511,1021023,1021022,2042045,855.5235331058502,0.0042269871496500855
511512,1023025,1023024,2046049,857.0147771835327,0.004164229132015862
512513,1025027,1025026,2050053,858.5559821128845,0.0041024066042609775
513514,1027029,1027028,2054057,860.50776720047,0.0040415055392486465
514515,1029031,1029030,2058061,862.3261382579803,0.00398151212209541
515516,1031033,1031032,2062065,864.1315839290619,0.003922412746874215
516517,1033035,1033034,2066069,866.2438342571259,0.0038641940129764407
517518,1035037,1035036,2070073,868.0963389873505,0.0038068427224970947
518519,1037039,1037038,2074077,869.6889662742615,0.00375034587727896
519520,1039041,1039040,2078081,871.1749949455261,0.0036946906751609276
520521,1041043,1041042,2082085,872.776819229126,0.00363986450770426
521522,1043045,1043044,2086089,874.3531792163849,0.003585854956440926
522523,1045047,1045046,2090093,875.880743265152,0.003532649791281983
523524,1047049,1047048,2094097,877.4042181968689,0.003480236966083794
524525,1049051,1049050,2098101,878.8895652294159,0.0034286046166016604
525526,1051053,1051052,2102105,880.3550572395325,0.0033777410579887146
526527,1053055,1053054,2106109,881.9977781772614,0.0033276347814990004
527528,1055057,1055056,2110113,883.6058731079102,0.003278274452327423
528529,1057059,1057058,2114117,885.1387960910797,0.0032296489058580846
529530,1059061,1059060,2118121,886.6425981521606,0.003181747147209535
530531,1061063,1061062,2122125,888.1362800598145,0.0031345583460051785
531532,1063065,1063064,2126129,889.636155128479,0.00308807183580484
532533,1065067,1065066,2130133,891.1420862674713,0.003042277110694158
533534,1067069,1067068,2134137,892.7921981811523,0.002997163823692972
534535,1069071,1069070,2138141,894.3886179924011,0.002952721783231027
535536,1071073,1071072,2142145,896.070867061615,0.002908940950874239
536537,1073075,1073074,2146149,897.6103191375732,0.002865811440642574
537538,1075077,1075076,2150153,899.7677550315857,0.0028233235142351987
538539,1077079,1077078,2154157,901.8834321498871,0.0027814675809167966
539540,1079081,1079080,2158161,903.6667912006378,0.0027402341936522134
540541,1081083,1081082,2162165,905.810506105423,0.0026996140481969633
541542,1083085,1083084,2166169,907.4173691272736,0.00265959797980031
542543,1085087,1085086,2170173,909.201238155365,0.0026201769624094595
543544,1087089,1087088,2174177,910.911865234375,0.002581342105031581
544545,1089091,1089090,2178181,912.5965192317963,0.002543084651051686
545546,1091093,1091092,2182185,914.1418323516846,0.002505395974935709
546547,1093095,1093094,2186189,915.7088830471039,0.002468267581662076
547548,1095097,1095096,2190193,917.4667460918427,0.002431691102970035
548549,1097099,1097098,2194197,919.2477612495422,0.0023956582973596596
549550,1099101,1099100,2198201,921.2025473117828,0.002360161047135989
550551,1101103,1101102,2202205,923.8152089118958,0.002325191355680545
551552,1103105,1103104,2206209,925.7929100990295,0.002290741347792391
552553,1105107,1105106,2210213,927.7145531177521,0.002256803265936469
553554,1107109,1107108,2214217,929.5067710876465,0.0022233694692204153
554555,1109111,1109110,2218221,931.4372930526733,0.002190432431575573
555556,1111113,1111112,2222225,933.7844779491425,0.0021579847399380014
556557,1113115,1113114,2226229,936.6204779148102,0.002126019092884235
557558,1115117,1115116,2230233,938.9176681041718,0.0020945282980164848
558559,1117119,1117118,2234237,940.7468600273132,0.0020635052715078928
559560,1119121,1119120,2238241,942.8552482128143,0.002032943035487733
560561,1121123,1121122,2242245,944.837485074997,0.002002834717245605
561562,1123125,1123124,2246249,947.1041362285614,0.0019731735466166356
562563,1125127,1125126,2250253,949.239520072937,0.001943952855867792
563564,1127129,1127128,2254257,951.1296372413635,0.0019151660764009648
564565,1129131,1129130,2258261,953.1783459186554,0.0018868067386392795
565566,1131133,1131132,2262265,955.0523393154144,0.0018588684698670477
566567,1133135,1133134,2266269,956.9866979122162,0.001831344993206585
567568,1135137,1135136,2270273,959.0573220252991,0.001804230125912909
568569,1137139,1137138,2274277,961.0046830177307,0.001777517777554749
569570,1139141,1139140,2278281,962.9685859680176,0.0017512019492187392
570571,1141143,1141142,2282285,964.7051980495453,0.0017252767320314888
571572,1143145,1143144,2286289,967.0113160610199,0.001699736305681654
572573,1145147,1145146,2290293,968.9869351387024,0.0016745749368283214
573574,1147149,1147148,2294297,971.2727501392365,0.001649786978305201
574575,1149151,1149150,2298301,972.9682869911194,0.0016253668671879495
575576,1151153,1151152,2302305,974.5549621582031,0.0016013091244531097
576577,1153155,1153154,2306309,976.6750421524048,0.0015776083524770002
577578,1155157,1155156,2310313,978.4744801521301,0.001554259235263089
578579,1157159,1157158,2314317,980.1851179599762,0.00153125653571351
579580,1159161,1159160,2318321,982.3390951156616,0.0015085950956290617
580581,1161163,1161162,2322325,984.3168849945068,0.0014862698335491586
581582,1163165,1163164,2326329,986.2876541614532,0.0014642757444107701
582583,1165167,1165166,2330333,988.1852931976318,0.0014426078982978652
583584,1167169,1167168,2334337,990.7245411872864,0.0014212614386224232
584585,1169171,1169170,2338341,992.9262919425964,0.001400231581214939
585586,1171173,1171172,2342345,995.0768890380859,0.001379513614665484
586587,1173175,1173174,2346349,997.1208891868591,0.0013591028966857266
587588,1175177,1175176,2350353,999.3885953426361,0.0013389948552458009
588589,1177179,1177178,2354357,1001.8025572299957,0.0013191849866416305
589590,1179181,1179180,2358361,1004.1730370521545,0.0012996688541306867
590591,1181183,1181182,2362365,1006.6939721107483,0.001280442087818301
591592,1183185,1183184,2366369,1008.4283781051636,0.0012615003824976156
592593,1185187,1185186,2370373,1010.0879952907562,0.0012428394981043311
593594,1187189,1187188,2374377,1012.2809252738953,0.0012244552572155953
594595,1189191,1189190,2378381,1014.340765953064,0.001206343545618438
595596,1191193,1191192,2382385,1016.4234330654144,0.0011885003099223468
596597,1193195,1193194,2386389,1018.1745882034302,0.0011709215574455811
597598,1195197,1195196,2390393,1020.2896840572357,0.0011536033555330505
598599,1197199,1197198,2394397,1022.3095669746399,0.0011365418298510122
599600,1199201,1199200,2398401,1024.4930229187012,0.0011197331642733843
600601,1201203,1201202,2402405,1026.4428851604462,0.0011031735991764435
601602,1203205,1203204,2406409,1028.563856124878,0.0010868594321209457
602603,1205207,1205206,2410413,1030.449823141098,0.0010707870146688947
603604,1207209,1207208,2414417,1032.1830151081085,0.0010549527538614711
604605,1209211,1209210,2418421,1033.8438053131104,0.0010393531098316089
605606,1211213,1211212,2422425,1035.5546402931213,0.001023984595803995
606607,1213215,1213214,2426429,1037.469918012619,0.0010088437769582015
607608,1215217,1215216,2430433,1039.2710070610046,0.0009939272695191903
608609,1217219,1217218,2434437,1041.124252319336,0.0009792317409846873
609610,1219221,1219220,2438441,1042.7576892375946,0.0009647539076240719
610611,1221223,1221222,2442445,1045.0053009986877,0.0009504905353878712
611612,1223225,1223224,2446449,1047.0057060718536,0.0009364384382024582
612613,1225227,1225226,2450453,1049.0252270698547,0.0009225944777426776
613614,1227229,1227228,2454457,1050.8084700107574,0.0009089555619539169
614615,1229231,1229230,2458461,1052.5128309726715,0.0008955186457342279
615616,1231233,1231232,2462465,1054.4367260932922,0.0008822807286605894
616617,1233235,1233234,2466469,1056.3818521499634,0.0008692388554436548
617618,1235237,1235236,2470473,1058.1422581672668,0.0008563901147908837
618619,1237239,1237238,2474477,1060.458722114563,0.0008437316386107341
619620,1239241,1239240,2478481,1062.5679411888123,0.0008312606021263491
620621,1241243,1241242,2482485,1064.3781960010529,0.0008189742220565677
621622,1243245,1243244,2486489,1066.6340773105621,0.0008068697568432981
622623,1245247,1245246,2490493,1068.7439920902252,0.0007949445059693971
623624,1247249,1247248,2494497,1070.7350809574127,0.0007831958089354885
624625,1249251,1249250,2498501,1072.57355594635,0.0007716210452599626
625626,1251253,1251252,2502505,1074.807636976242,0.0007602176326599874
626627,1253255,1253254,2506509,1076.6504321098328,0.0007489830281883769
627628,1255257,1255256,2510513,1078.6804699897766,0.0007379147267556618
628629,1257259,1257258,2514517,1080.8538491725922,0.0007270102598795347
629630,1259261,1259260,2518521,1083.2362382411957,0.0007162671965943446
630631,1261263,1261262,2522525,1084.943349123001,0.0007056831418594811
631632,1263265,1263264,2526529,1086.8966190814972,0.0006952557362183143
632633,1265267,1265266,2530533,1088.6470441818237,0.0006849826553434468
633634,1267269,1267268,2534537,1090.7213671207428,0.0006748616095819671
634635,1269271,1269270,2538541,1092.9485449790955,0.0006648903436143883
635636,1271273,1271272,2542545,1095.1926550865173,0.0006550666354314671
636637,1273275,1273274,2546549,1097.6387820243835,0.0006453882961068302
637638,1275277,1275276,2550553,1099.8760421276093,0.0006358531694559133
638639,1277279,1277278,2554557,1101.7378532886505,0.0006264591310127798
639640,1279281,1279280,2558561,1103.745126247406,0.0006172040885985552
640641,1281283,1281282,2562565,1105.421198129654,0.000608085980843498
641642,1283285,1283284,2566569,1107.0709722042084,0.0005991027763911916
642643,1285287,1285286,2570573,1109.1360230445862,0.0005902524752627869
643644,1287289,1287288,2574577,1110.9205050468445,0.0005815331065832652
644645,1289291,1289290,2578581,1112.705765247345,0.0005729427291498723
645646,1291293,1291292,2582585,1114.3673241138458,0.0005644794296131295
646647,1293295,1293294,2586589,1115.9042291641235,0.0005561413249779434
647648,1295297,1295296,2590593,1117.8419771194458,0.0005479265581698201
648649,1297299,1297298,2594597,1120.411992073059,0.0005398333013317824
649650,1299301,1299300,2598601,1122.5229182243347,0.0005318597532095737
650651,1301303,1301302,2602605,1124.1293733119965,0.0005240041390379702
651652,1303305,1303304,2606609,1125.9328451156616,0.0005162647107681551
652653,1305307,1305306,2610613,1127.6989431381226,0.0005086397466129711
653654,1307309,1307308,2614617,1129.26234126091,0.0005011275496826784
654655,1309311,1309310,2618621,1131.1913652420044,0.0004937264488944493
655656,1311313,1311312,2622625,1134.038523197174,0.0004864347980628736
656657,1313315,1313314,2626629,1135.550742149353,0.0004792509747630902
657658,1315317,1315316,2630633,1137.053551197052,0.0004721733814676554
658659,1317319,1317318,2634637,1138.558718919754,0.0004652004439549273
659660,1319321,1319320,2638641,1140.029333114624,0.00045833061165012623
660661,1321323,1321322,2642645,1141.633619070053,0.00045156235694321367
661662,1323325,1323324,2646649,1143.218913078308,0.00044489417473414505
662663,1325327,1325326,2650653,1144.7095112800598,0.000438324582887617
663664,1327329,1327328,2654657,1146.2268772125244,0.00043185212007301743
664665,1329331,1329330,2658661,1147.706570148468,0.0004254753481518492
665666,1331333,1331332,2662665,1149.2136871814728,0.00041919284944924584
666667,1333335,1333334,2666669,1150.6863832473755,0.00041300322709503234
667668,1335337,1335336,2670673,1152.1645390987396,0.00040690510604690644
668669,1337339,1337338,2674677,1153.6583542823792,0.0004008971309303888
669670,1339341,1339340,2678681,1155.1403529644012,0.0003949779663798836
670671,1341343,1341342,2682685,1156.6232681274414,0.0003891462973797388
671672,1343345,1343344,2686689,1158.100084066391,0.00038340082801369135
672673,1345347,1345346,2690693,1159.5596780776978,0.00037774028191961406
673674,1347349,1347348,2694697,1161.0412640571594,0.0003721634014937081
674675,1349351,1349350,2698701,1162.5260531902313,0.00036666894789050275
675676,1351353,1351352,2702705,1163.9969742298126,0.00036125570045442146
676677,1353355,1353354,2706709,1165.489140033722,0.00035592245706084213
677678,1355357,1355356,2710713,1166.9646751880646,0.0003506680330929157
678679,1357359,1357358,2714717,1168.4246530532837,0.00034549126166893984
679680,1359361,1359360,2718721,1169.9142792224884,0.0003403909929602378
680681,1361363,1361362,2722725,1171.4346911907196,0.0003353660948732795
681682,1363365,1363364,2726729,1172.9302740097046,0.00033041545123069227
682683,1365367,1365366,2730733,1174.4462399482727,0.0003255379632491895
683684,1367369,1367368,2734737,1175.917473077774,0.000320732547947955
684685,1369371,1369370,2738741,1177.3984150886536,0.0003159981381486432
685686,1371373,1371372,2742745,1178.8831129074097,0.00031133368338487344
686687,1373375,1373374,2746749,1180.1753251552582,0.0003067381481969278
687688,1375377,1375376,2750753,1181.4831261634827,0.00030221051235912455
688689,1377379,1377378,2754757,1182.7399821281433,0.0002977497713345656
689690,1379381,1379380,2758761,1184.3211450576782,0.00029335493456983386
690691,1381383,1381382,2762765,1186.0672602653503,0.0002890250275413564
691692,1383385,1383384,2766769,1187.6541812419891,0.00028475908902692026
692693,1385387,1385386,2770773,1189.273950099945,0.00028055617235622776
693694,1387389,1387388,2774777,1190.9278650283813,0.00027641534529720957
694695,1389391,1389390,2778781,1192.5045340061188,0.00027233568914653006
695696,1391393,1391392,2782785,1194.6502752304077,0.0002683162987295873
696697,1393395,1393394,2786789,1196.8003051280975,0.00026435628228682617
697698,1395397,1395396,2790793,1198.4386641979218,0.00026045476136005163
698699,1397399,1397398,2794797,1200.1201589107513,0.0002566108710198023
699700,1399401,1399400,2798801,1201.8520221710205,0.00025282375838742155
700701,1401403,1401402,2802805,1203.379240989685,0.0002490925835445523
701702,1403405,1403404,2806809,1204.8545279502869,0.000245416518851016
702703,1405407,1405406,2810813,1206.3943011760712,0.00024179474951324664
703704,1407409,1407408,2814817,1207.859764099121,0.0002382264722200489
704705,1409411,1409410,2818821,1209.394294977188,0.0002347108957110322
705706,1411413,1411412,2822825,1210.9610311985016,0.0002312472403218635
706707,1413415,1413414,2826829,1212.5359771251678,0.00022783473843901447
707708,1415417,1415416,2830833,1214.005359172821,0.00022447263347658009
708709,1417419,1417418,2834837,1215.5132751464844,0.00022116018010365224
709710,1419421,1419420,2838841,1216.9898490905762,0.0002178966437895724
710711,1421423,1421422,2842845,1218.4537200927734,0.00021468130159973953
711712,1423425,1423424,2846849,1219.9899730682373,0.00021151344037662057
712713,1425427,1425426,2850853,1221.4534380435944,0.00020839235821767943
713714,1427429,1427428,2854857,1222.9378671646118,0.00020531736345219542
714715,1429431,1429430,2858861,1224.4180312156677,0.00020228777430020273
715716,1431433,1431432,2862865,1225.9127271175385,0.00019930292000935879
716717,1433435,1433434,2866869,1227.3811662197113,0.00019636213835383387
717718,1435437,1435436,2870873,1228.8646421432495,0.0001934647783627952
718719,1437439,1437438,2874877,1230.3324520587921,0.00019061019793298328
719720,1439441,1439440,2878881,1231.8465023040771,0.00018779776416977256
720721,1441443,1441442,2882885,1233.3193731307983,0.00018502685452403966
721722,1443445,1443444,2886889,1234.8403189182281,0.0001822968548594872
722723,1445447,1445446,2890893,1236.311795949936,0.00017960716036213853
723724,1447449,1447448,2894897,1237.805507183075,0.00017695717531296395
724725,1449451,1449450,2898901,1239.2577311992645,0.00017434631274682033
725726,1451453,1451452,2902905,1240.726408958435,0.00017177399433876417
726727,1453455,1453454,2906909,1242.241277217865,0.0001692396502903648
727728,1455457,1455456,2910913,1243.695701122284,0.00016674271967076493
728729,1457459,1457458,2914917,1245.1624381542206,0.00016428264882506483
729730,1459461,1459460,2918921,1246.6203610897064,0.00016185889307962498
730731,1461463,1461462,2922925,1248.0880651474,0.00015947091651469236
731732,1463465,1463464,2926929,1249.5760011672974,0.00015711818946329004
732733,1465467,1465466,2930933,1251.0676860809326,0.00015480019135338807
733734,1467469,1467468,2934937,1252.5247139930725,0.00015251640877522732
734735,1469471,1469470,2938941,1253.9946522712708,0.00015026633627712727
735736,1471473,1471472,2942945,1255.5083701610565,0.00014804947556967818
736737,1473475,1473474,2946949,1256.9979321956635,0.00014586533586680162
737738,1475477,1475476,2950953,1258.4680042266846,0.00014371343377206358
738739,1477479,1477478,2954957,1259.9480981826782,0.00014159329271024035
739740,1479481,1479480,2958961,1261.399138212204,0.00013950444372312631
740741,1481483,1481482,2962965,1262.962158203125,0.00013744642410529195
741742,1483485,1483484,2966969,1264.4427120685577,0.00013541877819989168
742743,1485487,1485486,2970973,1265.9812381267548,0.0001334210576260375
743744,1487489,1487488,2974977,1267.4172711372375,0.00013145282025561755
744745,1489491,1489490,2978981,1268.8862390518188,0.00012951363032698282
745746,1491493,1491492,2982985,1270.3767092227936,0.0001276030586723209
746747,1493495,1493494,2986989,1271.8566052913666,0.00012572068249028234
747748,1495497,1495496,2990993,1273.326651096344,0.00012386608511860686
748749,1497499,1497498,2994997,1274.804897069931,0.00012203885660255764
749750,1499501,1499500,2999001,1276.250473022461,0.00012023859233067924
750751,1501503,1501502,3003005,1277.7197711467743,0.00011846489394429227
751752,1503505,1503504,3007009,1279.1945521831512,0.00011671736911011976
752753,1505507,1505506,3011013,1280.6656460762024,0.00011499563117922662
753754,1507509,1507508,3015017,1282.1467792987823,0.00011329929930070648
754755,1509511,1509510,3019021,1283.6323840618134,0.00011162799808062118
755756,1511513,1511512,3023025,1285.119388103485,0.00010998135780937446
756757,1513515,1513514,3027029,1286.5922842025757,0.00010835901423433825
757758,1515517,1515516,3031033,1288.0661182403564,0.00010676060878722637
758759,1517519,1517518,3035037,1289.523192167282,0.00010518578767459985
759760,1519521,1519520,3039041,1290.998630285263,0.0001036342025599879
760761,1521523,1521522,3043045,1292.4833362102509,0.0001021055101091406
761762,1523525,1523524,3047049,1294.126531124115,0.00010059937255846307
762763,1525527,1525526,3051053,1295.924741268158,9.911545669183397e-05
763764,1527529,1527528,3055057,1298.0007631778717,9.76534340679791e-05
764765,1529531,1529530,3059061,1299.8159942626953,9.621298181627935e-05
765766,1531533,1531532,3063065,1301.5041000843048,9.479378127252858e-05
766767,1533535,1533534,3067069,1303.3658742904663,9.339551854736783e-05
767768,1535537,1535536,3071073,1305.2397429943085,9.20178844125985e-05
768769,1537539,1537538,3075077,1307.1685922145844,9.066057407380868e-05
769770,1539541,1539540,3079081,1308.780030965805,8.93232878524941e-05
770771,1541543,1541542,3083085,1310.8228311538696,8.80057298218162e-05
771772,1543545,1543544,3087089,1312.683410167694,8.670760882978357e-05
772773,1545547,1545546,3091093,1314.6852040290833,8.542863770344411e-05
773774,1547549,1547548,3095097,1316.7753820419312,8.416853358994558e-05
774775,1549551,1549550,3099101,1319.0006589889526,8.292701841128292e-05
775776,1551553,1551552,3103105,1321.785082101822,8.17038172726825e-05
776777,1553555,1553554,3107109,1324.0883209705353,8.049865994053107e-05
777778,1555557,1555556,3111113,1326.1459131240845,7.931127993288101e-05
778779,1557559,1557558,3115117,1327.9328520298004,7.814141474682401e-05
779780,1559561,1559560,3119121,1330.1700451374054,7.698880608586478e-05
780781,1561563,1561562,3123125,1332.0521640777588,7.585319906411314e-05
781782,1563565,1563564,3127129,1334.400348186493,7.47343426610314e-05
782783,1565567,1565566,3131133,1336.1840062141418,7.363198949406069e-05
783784,1567569,1567568,3135137,1338.1559779644012,7.25458960459946e-05
784785,1569571,1569570,3139141,1339.7689571380615,7.147582221023185e-05
785786,1571573,1571572,3143145,1341.5361862182617,7.042153163183684e-05
786787,1573575,1573574,3147149,1343.5233480930328,6.93827914801659e-05
787788,1575577,1575576,3151153,1345.4359459877014,6.83593716530595e-05
788789,1577579,1577578,3155157,1347.1237812042236,6.735104648214474e-05
789790,1579581,1579580,3159161,1348.9574053287506,6.635759302753286e-05
790791,1581583,1581582,3163165,1350.6482701301575,6.537879175994021e-05
791792,1583585,1583584,3167169,1352.4088501930237,6.441442667437514e-05
792793,1585587,1585586,3171173,1354.1909341812134,6.346428426695638e-05
793794,1587589,1587588,3175177,1355.863750219345,6.25281548991552e-05
794795,1589591,1589590,3179181,1357.6513741016388,6.160583143355325e-05
795796,1591593,1591592,3183185,1359.4865732192993,6.069711059808469e-05
796797,1593595,1593594,3187189,1361.142441034317,5.9801791280733596e-05
797798,1595597,1595596,3191193,1363.3625841140747,5.891967566640233e-05
798799,1597599,1597598,3195197,1364.9259362220764,5.805056900953787e-05
799800,1599601,1599600,3199201,1366.4412951469421,5.719427940675814e-05
800801,1601603,1601602,3203205,1367.9900102615356,5.635061768316518e-05
801802,1603605,1603604,3207209,1369.4622631072998,5.551939727865829e-05
802803,1605607,1605606,3211213,1371.0080161094666,5.470043493005505e-05
803804,1607609,1607608,3215217,1372.5911331176758,5.389354930684931e-05
804805,1609611,1609610,3219221,1374.127594947815,5.30985627165137e-05
805806,1611613,1611612,3223225,1375.6303012371063,5.231529894444975e-05
806807,1613615,1613614,3227229,1377.1238770484924,5.154358541403781e-05
807808,1615617,1615616,3231233,1378.6791121959686,5.078325182239496e-05
808809,1617619,1617618,3235237,1380.3344750404358,5.003412979931454e-05
809810,1619621,1619620,3239241,1381.8631191253662,4.9296054157821345e-05
810811,1621623,1621622,3243245,1383.3513872623444,4.8568861984676914e-05
811812,1623625,1623624,3247249,1384.8357191085815,4.785239264037955e-05
812813,1625627,1625626,3251253,1386.3304121494293,4.7146487645477464e-05
813814,1627629,1627628,3255257,1388.056279182434,4.6450991590063495e-05
814815,1629631,1629630,3259261,1389.6160991191864,4.576575054215937e-05
815816,1631633,1631632,3263265,1391.1879510879517,4.509061318458407e-05
816817,1633635,1633634,3267269,1392.6760601997375,4.442543070126703e-05
817818,1635637,1635636,3271273,1394.1461582183838,4.37700558677534e-05
818819,1637639,1637638,3275277,1395.7135632038116,4.31243444154461e-05
819820,1639641,1639640,3279281,1397.4430561065674,4.248815343999013e-05
820821,1641643,1641642,3283285,1399.4645512104034,4.1861342651827727e-05
821822,1643645,1643644,3287289,1401.0643162727356,4.124377358039055e-05
822823,1645647,1645646,3291293,1402.6035220623016,4.063530991516018e-05
823824,1647649,1647648,3295297,1404.2919840812683,4.0035817278294417e-05
824825,1649651,1649650,3299301,1405.8808162212372,3.944516322462732e-05
825826,1651653,1651652,3303305,1407.643802165985,3.88632175827297e-05
826827,1653655,1653654,3307309,1409.4559891223907,3.82898517727881e-05
827828,1655657,1655656,3311313,1411.0166709423065,3.772493937503896e-05
828829,1657659,1657658,3315317,1412.7797529697418,3.7168355561334465e-05
829830,1659661,1659660,3319321,1414.477902173996,3.661997709514253e-05
830831,1661663,1661662,3323325,1416.138798236847,3.6079683695788844e-05
831832,1663665,1663664,3327329,1417.6176362037659,3.554735553734645e-05
832833,1665667,1665666,3331333,1419.1013071537018,3.502287529499881e-05
833834,1667669,1667668,3335337,1420.676244020462,3.45061271218583e-05
834835,1669671,1669670,3339341,1422.128454208374,3.399699721740035e-05
835836,1671673,1671672,3343345,1423.6029570102692,3.3495373145342455e-05
836837,1673675,1673674,3347349,1425.1045832633972,3.3001143833644164e-05
837838,1675677,1675676,3351353,1427.175921201706,3.2514200597688614e-05
838839,1677679,1677678,3355357,1428.7404990196228,3.2034435662353644e-05
839840,1679681,1679680,3359361,1430.24556016922,3.156174341256701e-05
840841,1681683,1681682,3363365,1431.7221250534058,3.109601948381169e-05
841842,1683685,1683684,3367369,1433.2802681922913,3.06371608758127e-05
842843,1685687,1685686,3371373,1434.84446310997,3.0185066862031817e-05
843844,1687689,1687688,3375377,1436.4043781757355,2.9739636829617666e-05
844845,1689691,1689690,3379381,1438.104483127594,2.9300773235263478e-05
845846,1691693,1691692,3383385,1439.827542066574,2.8868378876723e-05
846847,1693695,1693694,3387389,1441.7396709918976,2.844235859811306e-05
847848,1695697,1695696,3391393,1443.407114982605,2.8022618153045187e-05
848849,1697699,1697698,3395397,1444.9305431842804,2.76090647730598e-05
849850,1699701,1699700,3399401,1446.4595119953156,2.720160750868672e-05
850851,1701703,1701702,3403405,1447.9628551006317,2.6800156661010988e-05
851852,1703705,1703704,3407409,1449.5107691287994,2.6404623099551827e-05
852853,1705707,1705706,3411413,1451.065895318985,2.6014919853878382e-05
853854,1707709,1707708,3415417,1452.5575292110443,2.5630960976741335e-05
854855,1709711,1709710,3419421,1454.0501880645752,2.5252661544072907e-05
855856,1711713,1711712,3423425,1455.515715122223,2.4879938337107887e-05
856857,1713715,1713714,3427429,1457.0000083446503,2.4512709160262602e-05
857858,1715717,1715716,3431433,1458.4716160297394,2.415089272744808e-05
858859,1717719,1717718,3435437,1459.9624071121216,2.379440934419108e-05
859860,1719721,1719720,3439441,1461.4653732776642,2.3443180339199898e-05
860861,1721723,1721722,3443445,1462.945475101471,2.3097128291738045e-05
861862,1723725,1723724,3447449,1464.415817975998,2.275617691793741e-05
862863,1725727,1725726,3451453,1465.941281080246,2.2420250843424583e-05
863864,1727729,1727728,3455457,1467.4283571243286,2.2089276171755046e-05
864865,1729731,1729730,3459461,1468.9277131557465,2.176317946123163e-05
865866,1731733,1731732,3463465,1470.4211602210999,2.144188954389392e-05
866867,1733735,1733734,3467469,1471.8837912082672,2.112533456966048e-05
867868,1735737,1735736,3471473,1473.3883829116821,2.0813445416933973e-05
868869,1737739,1737738,3475477,1474.8875000476837,2.050615319149074e-05
869870,1739741,1739740,3479481,1476.41956615448,2.020338990860182e-05
870871,1741743,1741742,3483485,1477.901884317398,1.9905088947780314e-05
871872,1743745,1743744,3487489,1479.3943552970886,1.9611184598034015e-05
872873,1745747,1745746,3491493,1480.9001562595367,1.9321611603118072e-05
873874,1747749,1747748,3495497,1482.3828420639038,1.903630675315071e-05
874875,1749751,1749750,3499501,1483.8908700942993,1.8755206724563322e-05
875876,1751753,1751752,3503505,1485.3725371360779,1.8478249103281996e-05
876877,1753755,1753754,3507509,1486.8388900756836,1.8205373521595902e-05
877878,1755757,1755756,3511513,1488.3212931156158,1.7936519952854724e-05
878879,1757759,1757758,3515517,1489.8125250339508,1.767162802934763e-05
879880,1759761,1759760,3519521,1491.2867913246155,1.7410640339221573e-05
880881,1761763,1761762,3523525,1492.675504207611,1.7153498902189313e-05
881882,1763765,1763764,3527529,1493.9964752197266,1.6900147215892503e-05
882883,1765767,1765766,3531533,1495.3226659297943,1.6650529119033308e-05
883884,1767769,1767768,3535537,1496.615854024887,1.6404589814555948e-05
884885,1769771,1769770,3539541,1497.8712639808655,1.616227496015199e-05
885886,1771773,1771772,3543545,1499.1373591423035,1.5923531009320868e-05
886887,1773775,1773774,3547549,1500.4207501411438,1.5688305779804068e-05
887888,1775777,1775776,3551553,1502.086906194687,1.5456546748282562e-05
888889,1777779,1777778,3555557,1503.6469650268555,1.5228203210426727e-05
889890,1779781,1779780,3559561,1505.1670620441437,1.5003224802967452e-05
890891,1781783,1781782,3563565,1506.6773209571838,1.4781561617382977e-05
891892,1783785,1783784,3567569,1508.1809830665588,1.4563165223080432e-05
892893,1785787,1785786,3571573,1509.8570611476898,1.4347987416840624e-05
893894,1787789,1787788,3575577,1511.4946439266205,1.4135980222818034e-05
894895,1789791,1789790,3579581,1513.0153031349182,1.392709737046971e-05
895896,1791793,1791792,3583585,1514.6558442115784,1.3721292816626374e-05
896897,1793795,1793794,3587589,1516.376960992813,1.3518520745492424e-05
897898,1795797,1795796,3591593,1518.0871522426605,1.3318737160261662e-05
898899,1797799,1797798,3595597,1519.7219140529633,1.3121897382006864e-05
899900,1799801,1799800,3599601,1521.879565000534,1.2927958323416533e-05
900901,1801803,1801802,3603605,1525.0349071025848,1.273687701086601e-05
901902,1803805,1803804,3607609,1527.555426120758,1.2548611607599014e-05
902903,1805807,1805806,3611613,1530.9658181667328,1.23631203905461e-05
903904,1807809,1807808,3615617,1534.5319900512695,1.218036243244569e-05
904905,1809811,1809810,3619621,1537.246267080307,1.2000297715530905e-05
905906,1811813,1811812,3623625,1539.442698955536,1.1822886222034867e-05
906907,1813815,1813814,3627629,1541.5444490909576,1.1648088957372238e-05
907908,1815817,1815816,3631633,1543.1435840129852,1.1475867495391867e-05
908909,1817819,1817818,3635637,1545.0557811260223,1.1306183751003118e-05
909910,1819821,1819820,3639641,1547.2851729393005,1.113900032123638e-05
910911,1821823,1821822,3643645,1549.5982332229614,1.0974280485243071e-05
911912,1823825,1823824,3647649,1551.8800649642944,1.081198774954828e-05
912913,1825827,1825826,3651653,1553.8020231723785,1.0652086302798125e-05
913914,1827829,1827828,3655657,1555.7871642112732,1.0494541243133426e-05
914915,1829831,1829830,3659661,1557.5675330162048,1.0339317441321327e-05
915916,1831833,1831832,3663665,1559.4563109874725,1.018638090499735e-05
916917,1833835,1833834,3667669,1561.0996589660645,1.0035697755483852e-05
917918,1835837,1835836,3671673,1562.6293921470642,9.887234909911058e-06
918919,1837839,1837838,3675677,1564.1890811920166,9.740959853843378e-06
919920,1839841,1839840,3679681,1566.07808303833,9.596839959158388e-06
920921,1841843,1841842,3683685,1568.123250246048,9.454843507228361e-06
921922,1843845,1843844,3687689,1569.9234881401062,9.314939234172925e-06
922923,1845847,1845846,3691693,1572.045599937439,9.177096558232734e-06
923924,1847849,1847848,3695697,1573.5674800872803,9.041285011335276e-06
924925,1849851,1849850,3699701,1575.9708452224731,8.907474352781719e-06
925926,1851853,1851852,3703705,1578.1308600902557,8.77563525136793e-06
926927,1853855,1853854,3707709,1580.2869811058044,8.64573871695029e-06
927928,1855857,1855856,3711713,1582.503086090088,8.51775632781937e-06
928929,1857859,1857858,3715717,1584.4652032852173,8.391659434892063e-06
929930,1859861,1859860,3719721,1586.3545231819153,8.26742052595364e-06
930931,1861863,1861862,3723725,1588.3904871940613,8.145011975102534e-06
931932,1863865,1863864,3727729,1590.2164311408997,8.02440717961872e-06
932933,1865867,1865866,3731733,1592.08789396286,7.905579195721657e-06
933934,1867869,1867868,3735737,1593.873463153839,7.788502102812345e-06
934935,1869871,1869870,3739741,1595.5922832489014,7.67315009397862e-06
935936,1871873,1871872,3743745,1597.3785772323608,7.559497589681996e-06
936937,1873875,1873874,3747749,1599.0709221363068,7.447519465131336e-06
937938,1875877,1875876,3751753,1600.862879037857,7.337191163969692e-06
938939,1877879,1877878,3755757,1602.6017379760742,7.228488470900629e-06
939940,1879881,1879880,3759761,1604.2669780254364,7.121387284314551e-06
940941,1881883,1881882,3763765,1605.966586112976,7.015864071036049e-06
941942,1883885,1883884,3767769,1607.9571330547333,6.9118955252633896e-06
942943,1885887,1885886,3771773,1610.1803262233734,6.809458909629029e-06
943944,1887889,1887888,3775777,1612.228375196457,6.708531486765423e-06
944945,1889891,1889890,3779781,1614.2180371284485,6.609090860365541e-06
945946,1891893,1891892,3783785,1616.1885521411896,6.511115429930214e-06
946947,1893895,1893894,3787789,1618.4973471164703,6.414583594960277e-06
947948,1895897,1895896,3791793,1620.4924139976501,6.319473754956562e-06
948949,1897899,1897898,3795797,1622.5704741477966,6.225765218914603e-06
949950,1899901,1899900,3799801,1624.5796620845795,6.133437182143098e-06
950951,1901903,1901902,3803805,1626.5768933296204,6.042469749445445e-06
951952,1903905,1903904,3807809,1628.5990390777588,5.952842229817179e-06
952953,1905907,1905906,3811813,1630.9603073596954,5.8645352964958875e-06
953954,1907909,1907908,3815817,1633.098001241684,5.777529167971807e-06
954955,1909911,1909910,3819821,1634.7033472061157,5.691804972229875e-06
955956,1911913,1911912,3823825,1636.2653131484985,5.607343723568192e-06
956957,1913915,1913914,3827829,1637.8252251148224,5.524126777345373e-06
957958,1915917,1915916,3831833,1639.4252090454102,5.442135829980543e-06
958959,1917919,1917918,3835837,1640.962368965149,5.361352918953344e-06
959960,1919921,1919920,3839841,1642.4751360416412,5.281759854369739e-06
960961,1921923,1921922,3843845,1643.9751522541046,5.203339696890907e-06
961962,1923925,1923924,3847849,1645.4951710700989,5.126074825057003e-06
962963,1925927,1925926,3851853,1647.0081470012665,5.04994807215553e-06
963964,1927929,1927928,3855857,1648.6602230072021,4.9749429535950185e-06
964965,1929931,1929930,3859861,1651.172401189804,4.901042530036648e-06
965966,1931933,1931932,3863865,1652.6815810203552,4.82823122638365e-06
966967,1933935,1933934,3867869,1654.4367191791534,4.756492330670881e-06
967968,1935937,1935936,3871873,1655.993567943573,4.685810267801571e-06
968969,1937939,1937938,3875877,1657.6239531040192,4.616169576365792e-06
969970,1939941,1939940,3879881,1659.2502851486206,4.547554794953612e-06
970971,1941943,1941942,3883885,1660.780151128769,4.479950916902453e-06
971972,1943945,1943944,3887889,1662.2691791057587,4.413342821862898e-06
972973,1945947,1945946,3891893,1663.751177072525,4.347716185293393e-06
973974,1947949,1947948,3895897,1665.5003461837769,4.2830562279050355e-06
974975,1949951,1949950,3899901,1667.4020512104034,4.2193487388431095e-06
975976,1951953,1951952,3903905,1669.2245502471924,4.156579962000251e-06
976977,1953955,1953954,3907909,1670.7720410823822,4.094735572834907e-06
977978,1955957,1955956,3911913,1672.8186581134796,4.033802611047577e-06
978979,1957959,1957958,3915917,1674.5404651165009,3.973767093157221e-06
979980,1959961,1959960,3919921,1676.154095172882,3.914615831490664e-06
980981,1961963,1961962,3923925,1677.67529129982,3.856336093122081e-06
981982,1963965,1963964,3927929,1679.5216071605682,3.798914917751972e-06
982983,1965967,1965966,3931933,1681.209328174591,3.7423396861413494e-06
983984,1967969,1967968,3935937,1683.5186879634857,3.686597892738064e-06
984985,1969971,1969970,3939941,1685.0886399745941,3.631677031989966e-06
985986,1971973,1971972,3943945,1686.544186115265,3.5775653941527708e-06
986987,1973975,1973974,3947949,1688.0586659908295,3.5242508147348417e-06
987988,1975977,1975976,3951953,1689.5228962898254,3.471721811365569e-06
988989,1977979,1977978,3955957,1691.1935470104218,3.419966446926992e-06
989990,1979981,1979980,3959961,1692.9723241329193,3.368973466422176e-06
990991,1981983,1981982,3963965,1694.5143291950226,3.3187317285410245e-06
991992,1983985,1983984,3967969,1696.0308611392975,3.2692300919734407e-06
992993,1985987,1985986,3971973,1697.4996333122253,3.2204576427830034e-06
993994,1987989,1987988,3975977,1699.1104292869568,3.1724036944069667e-06
994995,1989991,1989990,3979981,1700.560563325882,3.125057446595747e-06
995996,1991993,1991992,3983985,1702.0206820964813,3.078408894907625e-06
996997,1993995,1993994,3987989,1703.5521399974823,3.0324473527798546e-06
997998,1995997,1995996,3991993,1705.0981981754303,2.987162929457554e-06
998999,1997999,1997998,3995997,1707.171144247055,2.942545620499004e-06
1000000,2000001,2000000,4000001,1708.7047271728516,2.898585535149323e-06


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.013862848281860352,2180.042156630883
1001,2003,2002,4005,2.1144208908081055,59.50785960800022
2002,4005,4004,8009,3.806501865386963,53.069953055727865
3003,6007,6006,12013,6.497259855270386,50.23287214458628
4004,8009,8008,16017,8.870810747146606,48.011470954668084
5005,10011,10010,20021,10.446680068969727,46.034239271139995
6006,12013,12012,24025,12.066550970077515,44.22397270747979
7007,14015,14014,28029,13.955816984176636,42.551356224505525
8008,16017,16016,32033,15.77367091178894,40.99882237549582
9009,18019,18018,36037,17.638158798217773,39.55358199049692
10010,20021,20020,40041,20.43228006362915,38.205379619941596
11011,22023,22022,44045,22.122371673583984,36.94544630893597
12012,24025,24024,48049,24.016366720199585,35.76595715561052
13013,26027,26026,52053,25.488724946975708,34.65975853578084
14014,28029,28028,56057,27.060860872268677,33.620244488709886
15015,30031,30030,60061,28.558502912521362,32.64131021783305
16016,32033,32032,64065,30.07087469100952,31.717339273637435
17017,34035,34034,68069,31.671834707260132,30.843199816600873
18018,36037,36036,72073,33.103928089141846,30.01423768535301
19019,38039,38038,76077,34.613853931427,29.226261611111795
20020,40041,40040,80081,36.03676700592041,28.475520193335797
21021,42043,42042,84085,37.560017824172974,27.758672299758928
22022,44045,44044,88089,38.97228288650513,27.072753240235443
23023,46047,46046,92093,40.39877200126648,26.41513900422433
24024,48049,48048,96097,41.83213782310486,25.78351044992087
25025,50051,50050,100101,43.2357497215271,25.17581882966465
26026,52053,52052,104105,44.79340887069702,24.59025355898507
27027,54055,54054,108109,46.3217978477478,24.02521274135711
28028,56057,56056,112113,47.88962388038635,23.47927666178134
29029,58059,58058,116117,49.3883159160614,22.951184252855683
30030,60061,60060,120121,51.22951889038086,22.439812401351446
31031,62063,62062,124125,52.718047857284546,21.94415788401261
32032,64065,64064,128129,54.11799693107605,21.46332168241679
33033,66067,66066,132133,55.730883836746216,20.99649541523695
34034,68069,68068,136137,57.19547700881958,20.54294963220218
35035,70071,70070,140141,58.66676092147827,20.102023730283918
36036,72073,72072,144145,60.72150492668152,19.673117274136075
37037,74075,74074,148149,62.98289084434509,19.255682526329565
38038,76077,76076,152153,64.49984574317932,18.84921801638393
39039,78079,78078,156157,65.93615484237671,18.453262999794106
40040,80081,80080,160161,67.36772608757019,18.06772520472282
41041,82083,82082,164165,68.78239679336548,17.692301676856687
42042,84085,84084,168169,70.73880887031555,17.326216665661605
43043,86087,86086,172173,72.55309677124023,16.969117112451613
44044,88089,88088,176177,74.83304691314697,16.620678670884445
45045,90091,90090,180181,76.55391097068787,16.280599832997723
46046,92093,92092,184185,78.25416088104248,15.948598824924602
47047,94095,94094,188189,80.33215093612671,15.624411281018638
48048,96097,96096,192193,82.36047887802124,15.307788331851498
49049,98099,98098,196197,83.88169479370117,14.99849499324273
50050,100101,100100,200201,85.4631290435791,14.696308793875687
51051,102103,102102,204205,86.95214796066284,14.401018596686981
52052,104105,104104,208209,88.83047485351562,14.112423579519941
53053,106107,106106,212213,90.40578293800354,13.830332347910826
54054,108109,108108,216217,92.17846179008484,13.5545621584223
55055,110111,110110,220221,94.6769118309021,13.284938235176355
56056,112113,112112,224225,96.60566091537476,13.021293165528618
57057,114115,114114,228229,98.09316182136536,12.763466363368366
58058,116117,116116,232233,99.94396996498108,12.511303590553098
59059,118119,118118,236237,101.54084992408752,12.264656528564501
60060,120121,120120,240241,103.19280195236206,12.023382393771726
61061,122123,122122,244245,104.75357389450073,11.787343590700743
62062,124125,124124,248249,106.28275489807129,11.556407398568922
63063,126127,126126,252253,107.82523488998413,11.330445687023143
64064,128129,128128,256257,109.50667476654053,11.109334657604222
65065,130131,130130,260261,111.03550577163696,10.892954607934712
66066,132133,132132,264265,112.57132387161255,10.681189716030985
67067,134135,134134,268269,114.22957682609558,10.473927842483363
68068,136137,136136,272273,115.78842806816101,10.27106034853523
69069,138139,138138,276277,117.35763883590698,10.072481928344473
70070,140141,140140,280281,118.9733099937439,9.878090453921118
71071,142143,142142,284285,120.48506903648376,9.687786831418066
72072,144145,144144,288289,121.90334892272949,9.501474867617162
73073,146147,146146,292293,123.27881193161011,9.319061145587284
74074,148149,148148,296297,124.56561470031738,9.140454908614515
75075,150151,150150,300301,125.854012966156,8.965567951612229
76076,152153,152152,304305,127.1259138584137,8.79431451931191
77077,154155,154154,308309,128.44260501861572,8.626611210618535
78078,156157,156156,312313,129.7790448665619,8.462376888585254
79079,158159,158158,316317,131.07860589027405,8.301532595530489
80080,160161,160160,320321,132.6848497390747,8.144001472874265
81081,162163,162162,324325,134.39307069778442,7.989708685318078
82082,164165,164164,328329,136.06289982795715,7.838581349042329
83083,166167,166166,332333,137.8710117340088,7.69054846362792
84084,168169,168168,336337,139.69441390037537,7.545540847441998
85085,170171,170170,340341,141.51062488555908,7.403491076259002
86086,172173,172172,344345,143.27926182746887,7.264333424909296
87087,174175,174174,348349,145.0389039516449,7.128003811768053
88088,176177,176176,352353,146.74304580688477,6.994439745915088
89089,178179,178178,356357,148.44142985343933,6.863580276808648
90090,180181,180180,360361,150.46890497207642,6.73536594633174
91091,182183,182182,364365,152.07852697372437,6.609738743068647
92092,184185,184184,368369,153.7125220298767,6.486642058692496
93093,186187,186186,372373,155.28264808654785,6.366020646336096
94094,188189,188188,376377,156.89172077178955,6.247820580833263
95095,190191,190190,380381,158.63695573806763,6.131989220719106
96096,192193,192192,384385,160.30103278160095,6.018475171882187
97097,194195,194194,388389,161.92124104499817,5.907228252769983
98098,196197,196196,392393,163.50998401641846,5.798199461044533
99099,198199,198198,396397,165.05253291130066,5.691340941603016
100100,200201,200200,400401,166.59953999519348,5.58660595586889
101101,202203,202202,404405,168.1648907661438,5.483948852274807
102102,204205,204204,408409,169.76540803909302,5.383325037858299
103103,206207,206206,412413,171.46410584449768,5.284690950897925
104104,208209,208208,416417,173.1182918548584,5.188004034522692
105105,210211,210210,420421,174.75783395767212,5.093222711230851
106106,212213,212212,424425,176.43683981895447,5.0003063582644245
107107,214215,214214,428429,177.95281982421875,4.909215283783851
108108,216217,216216,432433,179.51908087730408,4.819910703796268
109109,218219,218218,436437,181.06799793243408,4.732354719794671
110110,220221,220220,440441,182.84424686431885,4.646510297065902
111111,222223,222222,444445,184.9273316860199,4.562341243635501
112112,224225,224224,448449,186.68183279037476,4.479812189812833
113113,226227,226226,452453,188.54801297187805,4.398888568310213
114114,228229,228228,456457,190.3177080154419,4.319536594907959
115115,230231,230230,460461,191.78791880607605,4.241723249640472
116116,232233,232232,464465,193.25264382362366,4.16541625848356
117117,234235,234234,468469,194.681786775589,4.090584075518791
118118,236237,236236,472473,196.159117937088,4.017195865562712
119119,238239,238238,476477,197.60028290748596,3.945221487236495
120120,240241,240240,480481,199.03476667404175,3.874631476467698
121121,242243,242242,484485,200.4725697040558,3.805397030403583
122122,244245,244244,488489,201.96619391441345,3.7374899917276707
123123,246247,246246,492493,203.45116090774536,3.67088283336318
124124,248249,248248,496497,204.9722580909729,3.6055486435553803
125125,250251,250250,500501,206.58128476142883,3.541461111318199
126126,252253,252252,504505,208.25682997703552,3.4785945122380326
127127,254255,254254,508509,209.84695887565613,3.4169236946225965
128128,256257,256256,512513,211.3993489742279,3.3564240659883353
129129,258259,258258,516517,213.18768310546875,3.297071579873432
130130,260261,260260,520521,214.90505480766296,3.2388427229732315
131131,262263,262262,524525,216.42531204223633,3.181714502584896
132132,264265,264264,528529,218.01518201828003,3.125664434358441
133133,266267,266266,532533,219.61183190345764,3.0706705303413173
134134,268269,268268,536537,221.2239270210266,3.0167112873145925
135135,270271,270270,540541,222.74138188362122,2.963765675409718
136136,272273,272272,544545,224.32001996040344,2.911813127001892
137137,274275,274274,548549,226.0165376663208,2.8608335258705893
138138,276277,276276,552553,227.74670696258545,2.8108071966245234
139139,278279,278278,556557,229.22333598136902,2.761714894380134
140140,280281,280280,560561,230.7668800354004,2.713537794693366
141141,282283,282282,564565,232.52838492393494,2.6662574837314423
142142,284285,284284,568569,234.1241888999939,2.619855948687132
143143,286287,286286,572573,235.74911093711853,2.5743155684215253
144144,288289,288288,576577,237.50642466545105,2.5296191043375984
145145,290291,290290,580581,239.28449392318726,2.485749691472506
146146,292293,292292,584585,240.93807005882263,2.442690829806793
147147,294295,294294,588589,242.71904468536377,2.4004263757867648
148148,296297,296296,592593,244.5451009273529,2.3589405340496796
149149,298299,298298,596597,246.29083895683289,2.3182178493519814
150150,300301,300300,600601,247.73667979240417,2.278243198693872
151151,302303,302302,604605,249.25366282463074,2.2390017836347624
152152,304305,304304,608609,251.035484790802,2.2004791227944906
153153,306307,306306,612613,252.57309007644653,2.162661044539391
154154,308309,308308,616617,254.1163878440857,2.1255336798438975
155155,310311,310310,620621,255.50708985328674,2.0890834553263176
156156,312313,312312,624625,256.94729685783386,2.053297086455359
157157,314315,314314,628629,258.28710889816284,2.0181615709182097
158158,316317,316316,632633,259.6331169605255,1.9836641821536887
159159,318319,318318,636637,260.9882388114929,1.9497924630398984
160160,320321,320320,640641,262.32428073883057,1.9165342197352402
161161,322323,322322,644645,263.88084077835083,1.8838775156701786
162162,324325,324324,648649,265.4737777709961,1.8518106656836153
163163,326327,326326,652653,266.9676887989044,1.820322230300917
164164,328329,328328,656657,268.9258608818054,1.7894010101522326
165165,330331,330330,660661,270.59731793403625,1.7590360405238243
166166,332333,332332,664665,272.17492389678955,1.7292165860430941
167167,334335,334334,668669,273.7603099346161,1.6999321354899166
168168,336337,336336,672673,275.39829182624817,1.6711723967355283
169169,338339,338338,676677,277.32773876190186,1.6429272918018114
170170,340341,340340,680681,279.258798122406,1.615186952040517
171171,342343,342342,684685,280.96760177612305,1.5879417134279947
172172,344345,344344,688689,283.4140169620514,1.5611821119737215
173173,346347,346346,692693,285.1190218925476,1.5348988792381988
174174,348349,348348,696697,286.89527702331543,1.509082937959647
175175,350351,350350,700701,288.55931782722473,1.4837253977859746
176176,352353,352352,704705,290.2405219078064,1.4588175511053123
177177,354355,354354,708709,291.92757773399353,1.4343508689813689
178178,356357,356356,712713,293.4851429462433,1.4103169971824627
179179,358359,358358,716717,295.1461989879608,1.3867077523075295
180180,360361,360360,720721,296.72603487968445,1.3635151180009188
181181,362363,362362,724725,298.3772737979889,1.340731241262688
182182,364365,364364,728729,299.9497368335724,1.318348428841091
183183,366367,366366,732733,301.76080679893494,1.2963591437148807
184184,368369,368368,736737,303.61338806152344,1.2747560016571242
185185,370371,370370,740741,305.10129404067993,1.2535317678797355
186186,372373,372372,744745,306.5703959465027,1.2326793537594085
187187,374375,374374,748749,308.00961089134216,1.2121918136394925
188188,376377,376376,752753,309.4510688781738,1.1920623417067873
189189,378379,378378,756757,310.9323778152466,1.1722842689435993
190190,380381,380380,760761,312.38937187194824,1.152851060149942
191191,382383,382382,764765,313.8443830013275,1.1337563110359952
192192,384385,384384,768769,315.3201138973236,1.1149937453830034
193193,386387,386386,772773,316.8454267978668,1.096557212270909
194194,388389,388388,776777,318.26972484588623,1.078440683369763
195195,390391,390390,780781,319.7279508113861,1.0606382502953693
196196,392393,392392,784785,321.17313289642334,1.04314412202541
197197,394395,394394,788789,322.74239206314087,1.02595262237719
198198,396397,396396,792793,324.24584794044495,1.0090581875423368
199199,398399,398398,796797,325.89395689964294,0.9924553636801647
200200,400401,400400,800801,327.6289620399475,0.9761388045651529
201201,402403,402402,804805,329.2377369403839,0.9601032692900162
202202,404405,404404,808809,330.9758358001709,0.9443436200218684
203203,406407,406406,812813,332.6294677257538,0.9288548198084072
204204,408409,408408,816817,334.14356780052185,0.9136319304367362
205205,410411,410410,820821,335.64502787590027,0.8986701103399355
206206,412413,412412,824825,337.1516718864441,0.883964612552063
207207,414415,414414,828829,338.7228238582611,0.8695107827094262
208208,416417,416416,832833,340.16077995300293,0.8553040570986923
209209,418419,418418,836837,341.6165277957916,0.8413399607485417
210210,420421,420420,840841,343.06130290031433,0.8276141055644075
211211,422423,422422,844845,344.46720790863037,0.8141221885068717
212212,424425,424424,848849,345.89508080482483,0.800859989810192
213213,426427,426426,852853,347.3481788635254,0.7878233712420979
214214,428429,428428,856857,348.84115505218506,0.775008274402694
215215,430431,430430,860861,350.2943048477173,0.76241071906054
216216,432433,432432,864865,351.74511981010437,0.7500268015282927
217217,434435,434434,868869,353.1664879322052,0.7378526930735916
218218,436437,436436,872873,354.64158272743225,0.7258846383653008
219219,438439,438438,876877,356.10124492645264,0.714118953956131
220220,440441,440440,880881,357.5421268939972,0.702552026797207
221221,442443,442442,884885,358.9781439304352,0.6911803127879921
222222,444445,444444,888889,360.4863998889923,0.680000335355885
223223,446447,446446,892893,361.9301817417145,0.6690086840701497
224224,448449,448448,896897,363.46474599838257,0.6582020132855178
225225,450451,450450,900901,365.0041389465332,0.6475770408145536
226226,452453,452452,904905,366.50223207473755,0.6371305466320791
227227,454455,454454,908909,368.01187777519226,0.6268593716055193
228228,456457,456456,912913,369.58196783065796,0.616760416255488
229229,458459,458458,916917,371.03687286376953,0.6068306395427499
230230,460461,460460,920921,372.4777977466583,0.5970670576806469
231231,462463,462462,924925,373.93252301216125,0.5874667429762894
232232,464465,464464,928929,375.4169428348541,0.5780268226947101
233233,466467,466466,932933,376.94908905029297,0.568744477948826
234234,468469,468468,936937,378.4169490337372,0.5596169426141842
235235,470471,470470,940941,380.089567899704,0.5506415022658757
236236,472473,472472,944945,381.69663095474243,0.5418154931398931
237237,474475,474474,948949,383.14546298980713,0.533136301116997
238238,476477,476476,952953,384.5869507789612,0.524601360727388
239239,478479,478478,956957,386.0482397079468,0.5162081541783436
240240,480481,480480,960961,387.4985408782959,0.5079542104023176
241241,482483,482482,964965,388.9465899467468,0.4998371041252767
242242,484485,484484,968969,390.41764879226685,0.4918544549549324
243243,486487,486486,972973,391.93841791152954,0.48400392649000423
244244,488489,488488,976977,393.4370517730713,0.4762832254469913
245245,490491,490490,980981,395.2219429016113,0.4686901008062705
246246,492493,492492,984985,396.97860407829285,0.46122234297547493
247247,494495,494494,988989,398.59185576438904,0.453877782973791
248248,496497,496496,992993,400.190043926239,0.446654291629784
249249,498499,498498,996997,401.8790919780731,0.43954977879798207
250250,500501,500500,1001001,403.3226737976074,0.43256219259376394
251251,502503,502502,1005005,404.7409658432007,0.4256895186404108
252252,504505,504504,1009009,406.19427394866943,0.4189297793367359
253253,506507,506506,1013013,407.6685209274292,0.41228103313619613
254254,508509,508508,1017017,409.13446283340454,0.40574137384419373
255255,510511,510510,1021021,410.5524799823761,0.39930892992822464
256256,512513,512512,1025025,412.00243306159973,0.3929818638436018
257257,514515,514514,1029029,413.5419189929962,0.3867583713725935
258258,516517,516516,1033033,415.0876479148865,0.3806366809780002
259259,518519,518518,1037037,416.68630290031433,0.37461505317037336
260260,520521,520520,1041041,418.3098340034485,0.3686917798868308
261261,522523,522522,1045045,419.83580899238586,0.362865183885674
262262,524525,524524,1049049,421.3105237483978,0.35713361815089684
263263,526527,526526,1053053,422.73610281944275,0.3514954653098812
264264,528529,528528,1057057,424.18474793434143,0.34594913706519037
265265,530531,530530,1061061,425.6454520225525,0.3404930736339793
266266,532533,532532,1065065,427.13373279571533,0.3351257432033208
267267,534535,534534,1069069,428.59644174575806,0.3298456413938311
268268,536537,536536,1073073,430.09413981437683,0.3246512907352326
269269,538539,538538,1077077,431.5842549800873,0.31954124015373964
270270,540541,540540,1081081,433.02210688591003,0.31451406446808505
271271,542543,542542,1085085,434.5503017902374,0.3095683638969149
272272,544545,544544,1089089,436.0314438343048,0.3047027635767563
273273,546547,546546,1093093,437.57390999794006,0.29991591308839816
274274,548549,548548,1097097,439.0514888763428,0.29520648599498145
275275,550551,550550,1101101,440.50590109825134,0.29057317938679716
276276,552553,552552,1105105,441.9276957511902,0.28601471343768026
277277,554555,554554,1109109,443.3998279571533,0.28152983096958906
278278,556557,556556,1113113,444.8656487464905,0.2771172970257112
279279,558559,558558,1117117,446.322705745697,0.2727758984525508
280280,560561,560560,1121121,447.8077178001404,0.26850444349031477
281281,562563,562562,1125125,449.25231099128723,0.2643017613710299
282282,564565,564564,1129129,450.69699573516846,0.2601667019270053
283283,566567,566566,1133133,452.145201921463,0.25609813520327407
284284,568569,568568,1137137,453.61426997184753,0.2520949510819719
285285,570571,570570,1141141,455.05595088005066,0.2481560589108085
286286,572573,572572,1145145,456.4677209854126,0.24428038714142986
287287,574575,574574,1149149,457.94344186782837,0.24046688297335095
288288,576577,576576,1153153,459.41764783859253,0.23671451200618776
289289,578579,578578,1157157,460.93534207344055,0.23302225789780096
290290,580581,580580,1161161,462.37557077407837,0.22938912203017026
291291,582583,582582,1165165,463.8108289241791,0.22581412318106686
292292,584585,584584,1169169,465.23941588401794,0.2222962972030018
293293,586587,586586,1173173,466.6848089694977,0.21883469670763134
294294,588589,588588,1177177,468.16278195381165,0.21542839075743814
295295,590591,590590,1181181,470.2547698020935,0.2120764645625286
296296,592593,592592,1185185,472.47871685028076,0.20877801918402383
297297,594595,594594,1189189,474.1548008918762,0.20553217124302137
298298,596597,596596,1193193,475.88162779808044,0.20233805263546856
299299,598599,598598,1197197,477.69382977485657,0.1991948102521519
300300,600601,600600,1201201,479.26684284210205,0.19610160570516655
301301,602603,602602,1205205,480.7535889148712,0.19305761505813734
302302,604605,604604,1209209,482.2598829269409,0.19006202856394339
303303,606607,606606,1213213,483.7219789028168,0.1871140504044888
304304,608609,608608,1217217,485.19603991508484,0.1842128984392275
305305,610611,610610,1221221,486.6816029548645,0.18135780395505208
306306,612613,612612,1225225,488.1754937171936,0.17854801142345877
307307,614615,614614,1229229,489.7905237674713,0.17578277826157773
308308,616617,616616,1233233,491.3449308872223,0.17306137459763704
309309,618619,618618,1237237,493.0115840435028,0.1703830830407469
310310,620621,620620,1241241,494.6836779117584,0.16774719845705022
311311,622623,622622,1245245,496.2642538547516,0.165153027746328
312312,624625,624624,1249249,497.741436958313,0.16259988962713123
313313,626627,626626,1253253,499.2059369087219,0.16008711442384538
314314,628629,628628,1257257,500.6600968837738,0.1576140438570519
315315,630631,630630,1261261,502.11505579948425,0.1551800308403699
316316,632633,632632,1265265,503.60949993133545,0.15278443927900298
317317,634635,634634,1269269,505.07317090034485,0.15042664387306104
318318,636637,636636,1273273,506.5312440395355,0.14810602992429267
319319,638639,638638,1277277,508.03394389152527,0.14582199314793343
320320,640641,640640,1281281,509.52919602394104,0.14357393948489516
321321,642643,642642,1285285,511.00053882598877,0.14136128492134503
322322,644645,644644,1289289,512.5424177646637,0.13918345530839815
323323,646647,646646,1293293,513.9914228916168,0.13703988618829044
324324,648649,648648,1297297,515.4520750045776,0.1349300226208925
325325,650651,650650,1301301,516.9132189750671,0.1328533190157941
326326,652653,652652,1305305,518.3990199565887,0.1308092389659805
327327,654655,654654,1309309,519.8533089160919,0.12879725508560114
328328,656657,656656,1313313,521.3227188587189,0.12681684885069444
329329,658659,658658,1317317,522.8085277080536,0.12486751044252742
330330,660661,660660,1321321,524.2952938079834,0.12294873859354993
331331,662663,662662,1325325,525.7818238735199,0.12106004043744178
332332,664665,664664,1329329,527.2843339443207,0.11920093136109244
333333,666667,666666,1333333,528.7735307216644,0.11737093485919559
334334,668669,668668,1337337,530.2075479030609,0.11556958239191317
335335,670671,670670,1341341,531.6931538581848,0.11379641324549539
336336,672673,672672,1345345,533.1990888118744,0.11205097439460587
337337,674675,674674,1349349,534.6645770072937,0.11033282036839864
338338,676677,676676,1353353,536.1470749378204,0.10864151311773185
339339,678679,678678,1357357,537.6130278110504,0.10697662188601953
340340,680681,680680,1361361,539.0774779319763,0.10533772308178868
341341,682683,682682,1365365,540.6029939651489,0.10372440015339635
342342,684685,684684,1369369,542.100823879242,0.10213624346783945
343343,686687,686686,1373373,543.5675110816956,0.10057285018797302
344344,688689,688688,1377377,545.0319449901581,0.09903382415723172
345345,690691,690690,1381381,546.5108940601349,0.09751877578150925
346346,692693,692692,1385385,548.0106148719788,0.09602732191603991
347347,694695,694694,1389389,549.5390157699585,0.09455908575455396
348348,696697,696696,1393393,550.9920530319214,0.09311369671809189
349349,698699,698698,1397397,552.4517188072205,0.09169079034825245
350350,700701,700700,1401401,554.1354448795319,0.09029000820146393
351351,702703,702702,1405405,555.7805287837982,0.0889109977449607
352352,704705,704704,1409409,557.4148168563843,0.08755341225491975
353353,706707,706706,1413413,559.1161720752716,0.08621691071653004
354354,708709,708708,1417417,560.7918589115143,0.084901157725767
355355,710711,710710,1421421,562.3000960350037,0.08360582339287248
356356,712713,712712,1425425,563.7890758514404,0.0823305832478809
357357,714715,714714,1429429,565.3675248622894,0.08107511814773716
358358,716717,716716,1433433,566.8146297931671,0.07983911418443768
359359,718719,718718,1437437,568.3247747421265,0.0786222625957862
360360,720721,720720,1441441,569.819121837616,0.07742425967774125
361361,722723,722722,1445445,571.2688598632812,0.0762448066975594
362362,724725,724724,1449449,572.891371011734,0.07508360980887119
363363,726727,726726,1453453,574.425656080246,0.0739403799681213
364364,728729,728728,1457457,575.980771780014,0.0728148328540783
365365,730731,730730,1461461,577.4601888656616,0.07170668878552533
366366,732733,732732,1465465,578.9620578289032,0.07061567264418045
367367,734735,734734,1469469,580.417074918747,0.06954151379511586
368368,736737,736736,1473473,581.9401950836182,0.06848394601297514
369369,738739,738738,1477477,583.5206298828125,0.06744270740512093
370370,740741,740740,1481481,585.0879848003387,0.06641754033978486
371371,742743,742742,1485485,586.5905058383942,0.06540819137273957
372372,744745,744744,1489489,588.0915768146515,0.06441441117715385
373373,746747,746746,1493493,589.5670309066772,0.06343595447424377
374374,748749,748748,1497497,591.0401318073273,0.06247257996380995
375375,750751,750750,1501501,592.4848399162292,0.061524050258185525
376376,752753,752752,1505505,593.9677350521088,0.06059013181584305
377377,754755,754754,1509509,595.4768860340118,0.05967059487670667
378378,756757,756756,1513513,596.9986937046051,0.05876521339860119
379379,758759,758758,1517517,598.4643619060516,0.05787376499495167
380380,760761,760760,1521521,599.9389278888702,0.05699603087191463
381381,762763,762762,1525525,601.4980900287628,0.05613179577051142
382382,764765,764764,1529529,602.9750277996063,0.05528084790591947
383383,766767,766766,1533533,604.4621288776398,0.054442978908355144
384384,768769,768768,1537537,605.921984910965,0.05361798376816296
385385,770771,770770,1541541,607.3771789073944,0.05280566077817639
386386,772773,772772,1545545,608.8913488388062,0.052005811478238684
387387,774775,774774,1549549,610.3508427143097,0.051218240601883736
388388,776777,776776,1553553,611.8300940990448,0.050442756022675894
389389,778779,778778,1557557,613.338131904602,0.049679168701800336
390390,780781,780780,1561561,614.8007071018219,0.048927292636562925
391391,782783,782782,1565565,617.0965230464935,0.048186944810026944
392392,784785,784784,1569569,619.1884858608246,0.047457945141445634
393393,786787,786786,1573573,621.2590398788452,0.04674011643680842
394394,788789,788788,1577577,623.1846327781677,0.04603328434188825
395395,790791,790790,1581581,624.8901040554047,0.045337277294493106
396396,792793,792792,1585585,626.4074969291687,0.04465192647796812
397397,794795,794794,1589589,627.8726327419281,0.04397706577651661
398398,796797,796796,1593593,629.3652107715607,0.04331253172972538
399399,798799,798798,1597597,630.8402438163757,0.04265816348902263
400400,800801,800800,1601601,632.3015208244324,0.04201380277447697
401401,802803,802802,1605605,633.8002827167511,0.04137929383171013
402402,804805,804804,1609609,635.2883048057556,0.04075448339176546
403403,806807,806806,1613613,636.8738067150116,0.040139220628475414
404404,808809,808808,1617617,638.4286887645721,0.03953335711889849
405405,810811,810810,1621621,640.0165717601776,0.038936746803983624
406406,812813,812812,1625625,641.4329447746277,0.03834924594957556
407407,814815,814814,1629629,642.8371729850769,0.037770713107079246
408408,816817,816816,1633633,644.3126137256622,0.03720100907798951
409409,818819,818818,1637637,645.7816927433014,0.03663999687512387
410410,820821,820820,1641641,647.2602250576019,0.036087541687152225
411411,822823,822822,1645645,648.7618386745453,0.03554351084278551
412412,824825,824824,1649649,650.2440869808197,0.03500777377576014
413413,826827,826826,1653653,651.7075629234314,0.034480201990049864
414414,828829,828828,1657657,653.1610207557678,0.03396066902689654
415415,830831,830830,1661661,654.6450927257538,0.03344905042990831
416416,832833,832832,1665665,656.1270608901978,0.03294522371413677
417417,834835,834834,1669669,657.5983588695526,0.03244906833231198
418418,836837,836836,1673673,659.0698528289795,0.031960465644601754
419419,838839,838838,1677677,660.5707807540894,0.03147929888655199
420420,840841,840840,1681681,662.0455558300018,0.03100545313884595
421421,842843,842842,1685685,663.5074319839478,0.03053881529717728
422422,844845,844844,1689689,664.9679307937622,0.030079274043032456
423423,846847,846846,1693693,666.4468958377838,0.029626719814245916
424424,848849,848848,1697697,667.9403839111328,0.029181044776237286
425425,850851,850850,1701701,669.4628400802612,0.028742142795067593
426426,852853,852852,1705705,671.0493988990784,0.028309909408562817
427427,854855,854854,1709709,672.5961577892303,0.027884241799938536
428428,856857,856856,1713713,674.1630227565765,0.027465038770742467
429429,858859,858858,1717717,675.7380349636078,0.02705220071527492
430430,860861,860860,1721721,677.3197839260101,0.026645629593645026
431431,862863,862862,1725725,678.8544597625732,0.02624522890789649
432432,864865,864864,1729729,680.3575568199158,0.025850903675518566
433433,866867,866866,1733733,681.8274238109589,0.02546256040636763
434434,868869,868868,1737737,683.4795618057251,0.02508010707788344
435435,870871,870870,1741741,685.1207499504089,0.024703453111442286
436436,872873,872872,1745745,686.7814719676971,0.02433250934905118
437437,874875,874874,1749749,688.4105439186096,0.023967188030269426
438438,876877,876876,1753753,690.1855227947235,0.023607402770267072
439439,878879,878878,1757757,691.7262740135193,0.02325306853776965
440440,880881,880880,1761761,693.3034517765045,0.022904101631752383
441441,882883,882882,1765765,694.8006629943848,0.022560419662113418
442442,884885,884884,1769769,696.2891447544098,0.022221941527163835
443443,886887,886886,1773773,697.7535979747772,0.021888587393505077
444444,888889,888888,1777777,699.2088639736176,0.021560278675906375
445445,890891,890890,1781781,700.6941130161285,0.021236938016841123
446446,892893,892892,1785785,702.2820868492126,0.020918489266250617
447447,894895,894894,1789789,703.8661508560181,0.020604857463808912
448448,896897,896896,1793793,705.4181339740753,0.020295968818459187
449449,898899,898898,1797797,706.9168167114258,0.019991750690564913
450450,900901,900900,1801801,708.4181728363037,0.019692131572583094
451451,902903,902902,1805805,709.8972778320312,0.019397041071556487
452452,904905,904904,1809809,711.4498560428619,0.01910640989149215
453453,906907,906906,1813813,713.0435299873352,0.018820169815626286
454454,908909,908908,1817817,714.591050863266,0.018538253688916484
455455,910911,910910,1821821,716.163792848587,0.018260595401329738
456456,912913,912912,1825825,717.6968996524811,0.017987129871471552
457457,914915,914914,1829829,719.1900658607483,0.017717793029760287
458458,916917,916916,1833833,720.6543328762054,0.017452521802283627
459459,918919,918918,1837837,722.1359570026398,0.017191254095223485
460460,920921,920920,1841841,723.6618340015411,0.01693392877984934
461461,922923,922922,1845845,725.1717579364777,0.016680485675124146
462462,924925,924924,1849849,726.6834506988525,0.01643086553519879
463463,926927,926926,1853853,728.1932709217072,0.016185010033154867
464464,928929,928928,1857857,729.6734027862549,0.015942861746452763
465465,930931,930930,1861861,731.1744089126587,0.015704364142379745
466466,932933,932932,1865865,732.6980168819427,0.015469461564975973
467467,934935,934934,1869869,734.2121467590332,0.015238099220482582
468468,936937,936936,1873873,735.6489708423615,0.015010223162903458
469469,938939,938938,1877877,737.1606419086456,0.014785780282409178
470470,940941,940940,1881881,738.6222116947174,0.014564718290330347
471471,942943,942942,1885885,740.0508117675781,0.014346985706879423
472472,944945,944944,1889889,741.564740896225,0.014132531848986218
473473,946947,946946,1893893,743.1438939571381,0.013921306816428114
474474,948949,948948,1897897,744.665549993515,0.01371326148046137
475475,950951,950950,1901901,746.1525597572327,0.013508347471201887
476476,952953,952952,1905905,747.6910438537598,0.013306517165688092
477477,954955,954954,1909909,749.2769448757172,0.013107723676398564
478478,956957,956956,1913913,750.826751947403,0.012911920839087543
479479,958959,958958,1917917,752.3405539989471,0.012719063201984682
480480,960961,960960,1921921,753.8371829986572,0.0125291060140853
481481,962963,962962,1925925,755.3108158111572,0.012342005214691198
482482,964965,964964,1929929,756.7515330314636,0.012157717421700909
483483,966967,966966,1933933,758.2367808818817,0.011976199921832631
484484,968969,968968,1937937,759.7676129341125,0.011797410659255547
485485,970971,970970,1941941,761.3050050735474,0.011621308226381188
486486,972973,972972,1945945,762.8467798233032,0.01144785185249475
487487,974975,974974,1949949,764.3547329902649,0.011277001393750652
488488,976977,976976,1953953,765.870414018631,0.01110871732544183
489489,978979,978978,1957957,767.3464179039001,0.010942960729153128
490490,980981,980980,1961961,768.8093156814575,0.010779693285257963
491491,982983,982982,1965965,770.3039517402649,0.010618877263368631
492492,984985,984984,1969969,771.7829697132111,0.010460475512445555
493493,986987,986986,1973973,773.2459666728973,0.010304451452157082
494494,988989,988988,1977977,774.7573759555817,0.010150769063784537
495495,990991,990990,1981981,776.2972726821899,0.009999392882036773
496496,992993,992992,1985985,777.8357338905334,0.009850287985159412
497497,994995,994994,1989989,779.3317837715149,0.00970341998731783
498498,996997,996996,1993993,780.9711217880249,0.009558755030411703
499499,998999,998998,1997997,782.6284689903259,0.009416259775207436
500501,1001003,1001002,2002005,784.3374209403992,0.009275762232732632
501502,1003005,1003004,2006009,786.2453119754791,0.009137510485743405
502503,1005007,1005006,2010013,787.9230668544769,0.009001331425565695
503504,1007009,1007008,2014017,789.5997266769409,0.008867193710329957
504505,1009011,1009010,2018021,791.2721848487854,0.008735066477811415
505506,1011013,1011012,2022025,792.9900639057159,0.008604919338381478
506507,1013015,1013014,2026029,794.561399936676,0.008476722367277034
507508,1015017,1015016,2030033,796.0658197402954,0.008350446097665554
508509,1017019,1017018,2034037,798.1062128543854,0.008226061513255445
509510,1019021,1019020,2038041,799.9522259235382,0.00810354004158853
510511,1021023,1021022,2042045,801.9086079597473,0.007982853546650404
511512,1023025,1023024,2046049,803.6116049289703,0.007863974322731337
512513,1025027,1025026,2050053,805.3055658340454,0.007746875087264016
513514,1027029,1027028,2054057,807.0136587619781,0.0076315289742296955
514515,1029031,1029030,2058061,808.7631969451904,0.0075179095281328046
515516,1031033,1031032,2062065,810.3768517971039,0.007405990696952358
516517,1033035,1033034,2066069,811.9506690502167,0.007295746826798677
517518,1035037,1035036,2070073,813.6604070663452,0.00718715265463743
518519,1037039,1037038,2074077,815.2666518688202,0.007080183302946352
519520,1039041,1039040,2078081,817.1360387802124,0.006974814274258279
520521,1041043,1041042,2082085,818.8677768707275,0.006871021443316749
521522,1043045,1043044,2086089,820.6930229663849,0.006768781053665407
522523,1045047,1045046,2090093,822.5621449947357,0.006668069710599411
523524,1047049,1047048,2094097,824.418338060379,0.006568864375481098
524525,1049051,1049050,2098101,826.108720779419,0.006471142361078819
525526,1051053,1051052,2102105,827.9768397808075,0.006374881325200477
526527,1053055,1053054,2106109,829.8522288799286,0.006280059266032367
527528,1055057,1055056,2110113,831.6175827980042,0.0061866545167958975
528529,1057059,1057058,2114117,833.4183087348938,0.006094645739608495
529530,1059061,1059060,2118121,835.081426858902,0.006004011922527752
530531,1061063,1061062,2122125,836.8658077716827,0.005914732371934406
531532,1063065,1063064,2126129,838.646194934845,0.0058267867094627945
532533,1065067,1065066,2130133,840.5334599018097,0.005740154866657576
533534,1067069,1067068,2134137,842.299544095993,0.005654817079744134
534535,1069071,1069070,2138141,843.9808497428894,0.005570753885535851
535536,1071073,1071072,2142145,845.7714958190918,0.005487946116318199
536537,1073075,1073074,2146149,847.5491418838501,0.0054063748957560165
537538,1075077,1075076,2150153,849.1058449745178,0.005326021633663913
538539,1077079,1077078,2154157,850.6846950054169,0.005246868022936724
539540,1079081,1079080,2158161,852.240975856781,0.005168896033637793
540541,1081083,1081082,2162165,853.9465839862823,0.005092087909815746
541542,1083085,1083084,2166169,855.5093150138855,0.005016426164502263
542543,1085087,1085086,2170173,857.1428830623627,0.004941893576187795
543544,1087089,1087088,2174177,858.8009119033813,0.004868473184956201
544545,1089091,1089090,2178181,860.3578178882599,0.004796148287368851
545546,1091093,1091092,2182185,861.8506097793579,0.004724902433736133
546547,1093095,1093094,2186189,863.5056269168854,0.004654719423228926
547548,1095097,1095096,2190193,865.1371088027954,0.0045855833008090485
548549,1097099,1097098,2194197,866.8665618896484,0.004517478353363913
549550,1099101,1099100,2198201,868.7048008441925,0.00445038910504536
550551,1101103,1101102,2202205,870.3324747085571,0.004384300315109613
551552,1103105,1103104,2206209,871.9666728973389,0.004319196973142425
552553,1105107,1105106,2210213,873.474488735199,0.004255064296216915
553554,1107109,1107108,2214217,874.9701118469238,0.004191887724687149
554555,1109111,1109110,2218221,876.4769809246063,0.004129652919914406
555556,1111113,1111112,2222225,878.0148589611053,0.004068345759492331
556557,1113115,1113114,2226229,879.5124769210815,0.0040079523354279445
557558,1115117,1115116,2230233,881.0310180187225,0.003948458948912048
558559,1117119,1117118,2234237,882.5198037624359,0.003889852109182357
559560,1119121,1119120,2238241,884.0113620758057,0.0038321185293170856
560561,1121123,1121122,2242245,885.5191769599915,0.0037752451228243444
561562,1123125,1123124,2246249,887.0841557979584,0.0037192190012547144
562563,1125127,1125126,2250253,889.0279810428619,0.003664027470790643
563564,1127129,1127128,2254257,890.4949197769165,0.0036096580294042724
564565,1129131,1129130,2258261,891.9591391086578,0.0035560983637878962
565566,1131133,1131132,2262265,893.4582278728485,0.003503336346625474
566567,1133135,1133134,2266269,894.9415059089661,0.0034513600337504613
567568,1135137,1135136,2270273,896.4265668392181,0.0034001576613036377
568569,1137139,1137138,2274277,897.9348719120026,0.003349717642890937
569570,1139141,1139140,2278281,899.6875467300415,0.0033000285668549623
570571,1141143,1141142,2282285,901.3366787433624,0.003251079193660189
571572,1143145,1143144,2286289,903.2111239433289,0.003202858453846602
572573,1145147,1145146,2290293,904.8023657798767,0.0031553554441643428
573574,1147149,1147148,2294297,906.2858397960663,0.003108559426323154
574575,1149151,1149150,2298301,908.3917880058289,0.0030624598235817757
575576,1151153,1151152,2302305,909.9233129024506,0.00301704621870158
576577,1153155,1153154,2306309,911.4107618331909,0.0029723083517865234
577578,1155157,1155156,2310313,912.9318978786469,0.00292823611687254
578579,1157159,1157158,2314317,914.3902928829193,0.0028848195609043614
579580,1159161,1159160,2318321,915.8708107471466,0.00284204888032491
580581,1161163,1161162,2322325,917.3713629245758,0.0027999144194836845
581582,1163165,1163164,2326329,918.8861298561096,0.002758406668021962
582583,1165167,1165166,2330333,920.3260757923126,0.002717516258599062
583584,1167169,1167168,2334337,921.8298759460449,0.002677233965414416
584585,1169171,1169170,2338341,923.3148028850555,0.0026375507007969645
585586,1171173,1171172,2342345,924.887218952179,0.0025984575146367206
586587,1173175,1173174,2346349,926.3870520591736,0.0025599455908604796
587588,1175177,1175176,2350353,927.867547750473,0.002522006246181263
588589,1177179,1177178,2354357,929.4365267753601,0.0024846309279382695
589590,1179181,1179180,2358361,931.1442427635193,0.0024478112125052576
590591,1181183,1181182,2362365,932.865504026413,0.002411538801993629
591592,1183185,1183184,2366369,935.3355538845062,0.0023758055245934884
592593,1185187,1185186,2370373,937.2412989139557,0.002340603329912483
593594,1187189,1187188,2374377,938.79984998703,0.002305924289316863
594595,1189191,1189190,2378381,940.4784798622131,0.0022717605937714325
595596,1191193,1191192,2382385,942.1493167877197,0.002238104550428943
596597,1193195,1193194,2386389,943.7630929946899,0.002204948583312216
597598,1195197,1195196,2390393,945.299103975296,0.002172285229107729
598599,1197199,1197198,2394397,946.9106900691986,0.0021401071369382407
599600,1199201,1199200,2398401,948.3856558799744,0.0021084070667711785
600601,1201203,1201202,2402405,949.8504378795624,0.0020771778871448987
601602,1203205,1203204,2406409,951.3147037029266,0.002046412572894951
602603,1205207,1205206,2410413,952.9986097812653,0.002016104205267766
603604,1207209,1207208,2414417,954.559898853302,0.0019862459690784817
604605,1209211,1209210,2418421,956.4462478160858,0.0019568311510056446
605606,1211213,1211212,2422425,958.0999810695648,0.0019278531391364595
606607,1213215,1213214,2426429,960.055330991745,0.0018993054202383064
607608,1215217,1215216,2430433,962.0162208080292,0.0018711815788492459
608609,1217219,1217218,2434437,963.3304979801178,0.00184347529580009
609610,1219221,1219220,2438441,964.7453429698944,0.001816180347077534
610611,1221223,1221222,2442445,966.1545579433441,0.0017892906010956722
611612,1223225,1223224,2446449,968.0262126922607,0.0017628000190370585
612613,1225227,1225226,2450453,969.7936828136444,0.0017367026521242224
613614,1227229,1227228,2454457,971.3377730846405,0.0017109926411649212
614615,1229231,1229230,2458461,973.0177547931671,0.0016856642143920908
615616,1231233,1231232,2462465,974.6280038356781,0.001660711686781724
616617,1233235,1233234,2466469,976.3413798809052,0.0016361294580065078
617618,1235237,1235236,2470473,978.1947147846222,0.001611912012663197
618619,1237239,1237238,2474477,980.0930869579315,0.0015880539166346352
619620,1239241,1239240,2478481,981.9073848724365,0.0015645498182266238
620621,1241243,1241242,2482485,983.7527589797974,0.0015413944454394368
621622,1243245,1243244,2486489,985.5337338447571,0.0015185826051720142
622623,1245247,1245246,2490493,987.5273268222809,0.0014961091827672135
623624,1247249,1247248,2494497,990.1847269535065,0.0014739691390559528
624625,1249251,1249250,2498501,991.922632932663,0.001452157510698271
625626,1251253,1251252,2502505,993.7002489566803,0.0014306694093875194
626627,1253255,1253254,2506509,995.6486699581146,0.001409500018894505
627628,1255257,1255256,2510513,997.1132049560547,0.0013886445952948634
628629,1257259,1257258,2514517,998.716470003128,0.0013680984664006246
629630,1259261,1259260,2518521,1000.5155987739563,0.0013478570290317293
630631,1261263,1261262,2522525,1002.0257089138031,0.0013279157491297156
631632,1263265,1263264,2526529,1003.6967198848724,0.001308270160848224
632633,1265267,1265266,2530533,1005.5444939136505,0.0012889158643929477
633634,1267269,1267268,2534537,1008.0369987487793,0.0012698485264763804
634635,1269271,1269270,2538541,1009.8587439060211,0.0012510638781577654
635636,1271273,1271272,2542545,1011.5214788913727,0.0012325577143883493
636637,1273275,1273274,2546549,1013.1815187931061,0.0012143258931018863
637638,1275277,1275276,2550553,1014.7015590667725,0.001196364333850397
638639,1277279,1277278,2554557,1016.314778804779,0.0011786690175767944
639640,1279281,1279280,2558561,1017.8613178730011,0.0011612359851369547
640641,1281283,1281282,2562565,1019.6178276538849,0.001144061336390223
641642,1283285,1283284,2566569,1021.3212299346924,0.001127141229744666
642643,1285287,1285286,2570573,1023.0592617988586,0.0011104718802243951
643644,1287289,1287288,2574577,1024.7128639221191,0.0010940495604927492
644645,1289291,1289290,2578581,1026.4174058437347,0.0010778705983511827
645646,1291293,1291292,2582585,1028.0658690929413,0.0010619313763982063
646647,1293295,1293294,2586589,1029.574266910553,0.0010462283312335785
647648,1295297,1295296,2590593,1031.2828669548035,0.0010307579526624977
648649,1297299,1297298,2594597,1032.917011976242,0.0010155167830134815
649650,1299301,1299300,2598601,1034.5513410568237,0.0010005014161151848
650651,1301303,1301302,2602605,1036.2795209884644,0.0009857084969553398
651652,1303305,1303304,2606609,1038.1882178783417,0.0009711347198617659
652653,1305307,1305306,2610613,1039.88906788826,0.0009567768295255519
653654,1307309,1307308,2614617,1042.0243587493896,0.0009426316183862582
654655,1309311,1309310,2618621,1043.6962230205536,0.0009286959267456041
655656,1311313,1311312,2622625,1045.2048139572144,0.0009149666428811543
656657,1313315,1313314,2626629,1046.7168130874634,0.0009014407004315217
657658,1315317,1315316,2630633,1048.4215638637543,0.0008881150793058623
658659,1317319,1317318,2634637,1050.1648769378662,0.0008749868046606935
659660,1319321,1319320,2638641,1052.0008897781372,0.0008620529456493387
660661,1321323,1321322,2642645,1053.6579377651215,0.0008493106150808671
661662,1323325,1323324,2646649,1055.2346138954163,0.0008367569690790333
662663,1325327,1325326,2650653,1056.7534918785095,0.000824389206172782
663664,1327329,1327328,2654657,1058.3178670406342,0.0008122045665004407
664665,1329331,1329330,2658661,1059.852826833725,0.0008002003312412853
665666,1331333,1331332,2662665,1061.4032278060913,0.0007883738225018533
666667,1333335,1333334,2666669,1063.0067319869995,0.0007767224017243279
667668,1335337,1335336,2670673,1064.566969871521,0.0007652434702549726
668669,1337339,1337338,2674677,1066.3552329540253,0.0007539344676388282
669670,1339341,1339340,2678681,1068.1277260780334,0.0007427928719607735
670671,1341343,1341342,2682685,1069.9071049690247,0.0007318161990497174
671672,1343345,1343344,2686689,1071.4136147499084,0.0007210020007732965
672673,1345347,1345346,2690693,1073.02002286911,0.0007103478667431773
673674,1347349,1347348,2694697,1074.611249923706,0.0006998514215865725
674675,1349351,1349350,2698701,1076.5512907505035,0.0006895103256283619
675676,1351353,1351352,2702705,1078.0598809719086,0.0006793222739815974
676677,1353355,1353354,2706709,1079.5843057632446,0.0006692849959790692
677678,1355357,1355356,2710713,1081.2196538448334,0.0006593962550596189
678679,1357359,1357358,2714717,1083.0285558700562,0.0006496538478586444
679680,1359361,1359360,2718721,1084.986722946167,0.000640055603298606
680681,1361363,1361362,2722725,1087.1133108139038,0.0006305993833848333
681682,1363365,1363364,2726729,1089.0682470798492,0.000621283081841284
682683,1365367,1365366,2730733,1090.6421728134155,0.0006121046229736749
683684,1367369,1367368,2734737,1092.236268043518,0.0006030619629200373
684685,1369371,1369370,2738741,1094.529109954834,0.0005941530876043544
685686,1371373,1371372,2742745,1096.462809085846,0.0005853760134186814
686687,1373375,1373374,2746749,1098.9542348384857,0.0005767287858589043
687688,1375377,1375376,2750753,1100.7411577701569,0.0005682094795247394
688689,1377379,1377378,2754757,1102.302486896515,0.0005598161980060468
689690,1379381,1379380,2758761,1104.039636850357,0.0005515470725185878
690691,1381383,1381382,2762765,1105.6042909622192,0.0005434002629272072
691692,1383385,1383384,2766769,1107.053288936615,0.0005353739556994697
692693,1385387,1385386,2770773,1108.5011599063873,0.0005274663647014677
693694,1387389,1387388,2774777,1109.9653198719025,0.0005196757300609534
694695,1389391,1389390,2778781,1111.3911418914795,0.0005120003180536514
695696,1391393,1391392,2782785,1112.8586807250977,0.000504438421330633
696697,1393395,1393394,2786789,1114.57342004776,0.0004969883574403866
697698,1395397,1395396,2790793,1116.529593706131,0.0004896484687151315
698699,1397399,1397398,2794797,1118.0498039722443,0.00048241712261187786
699700,1399401,1399400,2798801,1119.7612237930298,0.00047529271080293256
700701,1401403,1401402,2802805,1121.3404097557068,0.00046827364849377773
701702,1403405,1403404,2806809,1122.8122699260712,0.00046135837476413144
702703,1405407,1405406,2810813,1124.273675918579,0.00045454535177213984
703704,1407409,1407408,2814817,1125.8390378952026,0.0004478330647543771
704705,1409411,1409410,2818821,1127.7681069374084,0.000441220021002664
705706,1411413,1411412,2822825,1129.3797817230225,0.00043470475054618873
706707,1413415,1413414,2826829,1131.0800459384918,0.00042828580501463875
707708,1415417,1415416,2830833,1133.1014127731323,0.00042196175706976646
708709,1417419,1417418,2834837,1134.9192688465118,0.0004157312014285708
709710,1419421,1419420,2838841,1136.3909187316895,0.0004095927529306209
710711,1421423,1421422,2842845,1137.8250188827515,0.00040354504778861156
711712,1423425,1423424,2846849,1139.2743117809296,0.0003975867417693735
712713,1425427,1425426,2850853,1140.87677693367,0.0003917165109896814
713714,1427429,1427428,2854857,1142.755136013031,0.00038593305066569883
714715,1429431,1429430,2858861,1144.392017841339,0.00038023507636353315
715716,1431433,1431432,2862865,1145.8596317768097,0.00037462132183918584
716717,1433435,1433434,2866869,1147.2946078777313,0.00036909054017542076
717718,1435437,1435436,2870873,1148.7329490184784,0.00036364150275858265
718719,1437439,1437438,2874877,1150.177176952362,0.00035827299905122345
719720,1439441,1439440,2878881,1151.6239559650421,0.0003529838369331628
720721,1441443,1441442,2882885,1153.0523970127106,0.00034777284156461974
721722,1443445,1443444,2886889,1154.5005249977112,0.0003426388558409599
722723,1445447,1445446,2890893,1156.0989367961884,0.00033758073971057456
723724,1447449,1447448,2894897,1157.9578158855438,0.00033259736983382027
724725,1449451,1449450,2898901,1160.0334861278534,0.0003276876398103923
725726,1451453,1451452,2902905,1162.0306448936462,0.0003228504598382642
726727,1453455,1453454,2906909,1164.193202972412,0.0003180847555768196
727728,1455457,1455456,2910913,1166.2699048519135,0.00031338946962478076
728729,1457459,1457458,2914917,1168.1133818626404,0.00030876355924647214
729730,1459461,1459460,2918921,1169.754893064499,0.00030420599830449646
730731,1461463,1461462,2922925,1171.8540868759155,0.0002997157744175638
731732,1463465,1463464,2926929,1173.910395860672,0.0002952918915752889
732733,1465467,1465466,2930933,1176.0536530017853,0.00029093336820551485
733734,1467469,1467468,2934937,1178.9122788906097,0.0002866392363785053
734735,1469471,1469470,2938941,1181.045578956604,0.000282408544194368
735736,1471473,1471472,2942945,1183.4132108688354,0.0002782403523724497
736737,1473475,1473474,2946949,1185.4758548736572,0.00027413373607032554
737738,1475477,1475476,2950953,1187.5784549713135,0.0002700877844290517
738739,1477479,1477478,2954957,1189.5931210517883,0.00026610160000473115
739740,1479481,1479480,2958961,1191.4309628009796,0.0002621742983137665
740741,1481483,1481482,2962965,1193.0886788368225,0.0002583050084012939
741742,1483485,1483484,2966969,1194.5604877471924,0.00025449287193168857
742743,1485487,1485486,2970973,1196.3736109733582,0.0002507370434159384
743744,1487489,1487488,2974977,1197.9523267745972,0.0002470366899842702
744745,1489491,1489490,2978981,1199.6173958778381,0.00024339099093140248
745746,1491493,1491492,2982985,1202.0499110221863,0.00023979913794391905
746747,1493495,1493494,2986989,1204.1816980838776,0.00023626033430446114
747748,1495497,1495496,2990993,1206.120440006256,0.0002327737956875353
748749,1497499,1497498,2994997,1208.5531919002533,0.00022933874879527139
749750,1499501,1499500,2999001,1210.1815967559814,0.00022595443238060398
750751,1501503,1501502,3003005,1212.6180090904236,0.00022262009588303044
751752,1503505,1503504,3007009,1214.6489398479462,0.00021933500022441876
752753,1505507,1505506,3011013,1216.5740087032318,0.00021609841724057333
753754,1507509,1507508,3015017,1218.0564279556274,0.00021290962968123495
754755,1509511,1509510,3019021,1219.505816936493,0.000209767930414273
755756,1511513,1511512,3023025,1220.9283289909363,0.00020667262322149327
756757,1513515,1513514,3027029,1222.405014038086,0.00020362302245757746
757758,1515517,1515516,3031033,1223.8707818984985,0.0002006184521405885
758759,1517519,1517518,3035037,1225.6113839149475,0.00019765824617934413
759760,1519521,1519520,3039041,1227.586539030075,0.00019474174871447758
760761,1521523,1521522,3043045,1229.1482989788055,0.00019186831400475057
761762,1523525,1523524,3047049,1230.6639318466187,0.00018903730472175084
762763,1525527,1525526,3051053,1232.2137548923492,0.00018624809388256836
763764,1527529,1527528,3055057,1233.7239327430725,0.00018350006382661377
764765,1529531,1529530,3059061,1235.2535219192505,0.00018079260541981057
765766,1531533,1531532,3063065,1237.1498680114746,0.0001781251193051503
766767,1533535,1533534,3067069,1238.6546988487244,0.0001754970140837031
767768,1535537,1535536,3071073,1240.1641159057617,0.00017290770790623355
768769,1537539,1537538,3075077,1241.5507400035858,0.000170356627450019
769770,1539541,1539540,3079081,1243.0010077953339,0.00016784320723672863
770771,1541543,1541542,3083085,1244.5229077339172,0.00016536689099666546
771772,1543545,1543544,3087089,1246.0037078857422,0.0001629271301908375
772773,1545547,1545546,3091093,1247.4939618110657,0.00016052338446570502
773774,1547549,1547548,3095097,1248.9029669761658,0.00015815512165318069
774775,1549551,1549550,3099101,1250.4508028030396,0.00015582181731588207
775776,1551553,1551552,3103105,1252.111828804016,0.00015352295486081857
776777,1553555,1553554,3107109,1253.9536929130554,0.00015125802508464403
777778,1555557,1555556,3111113,1255.6091659069061,0.00014902652685577777
778779,1557559,1557558,3115117,1257.0617978572845,0.00014682796575016255
779780,1559561,1559560,3119121,1258.5001509189606,0.00014466185552919342
780781,1561563,1561562,3123125,1259.919843673706,0.00014252771632072836
781782,1563565,1563564,3127129,1261.387990951538,0.00014042507575595664
782783,1565567,1565566,3131133,1262.8153839111328,0.00013835346851465147
783784,1567569,1567568,3135137,1264.2728538513184,0.00013631243587042263
784785,1569571,1569570,3139141,1265.701635837555,0.00013430152637283754
785786,1571573,1571572,3143145,1267.1188097000122,0.00013232029482423968
786787,1573575,1573574,3147149,1268.527718782425,0.00013036830250712228
787788,1575577,1575576,3151153,1269.9681730270386,0.00012844511786624935
788789,1577579,1577578,3155157,1271.403558731079,0.00012655031503072678
789790,1579581,1579580,3159161,1272.857558965683,0.00012468347460981022
790791,1581583,1581582,3163165,1274.3189239501953,0.00012284418357921822
791792,1583585,1583584,3167169,1275.778638124466,0.00012103203505375859
792793,1585587,1585586,3171173,1278.3077340126038,0.00011924662828732835
793794,1587589,1587588,3175177,1280.5714848041534,0.0001174875678771059
794795,1589591,1589590,3179181,1282.6968340873718,0.0001157544645593589
795796,1591593,1591592,3183185,1284.4341859817505,0.00011404693555050471
796797,1593595,1593594,3187189,1286.092236995697,0.00011236460227337375
797798,1595597,1595596,3191193,1288.4804940223694,0.00011070709319938032
798799,1597599,1597598,3195197,1290.088917016983,0.00010907404123372544
799800,1599601,1599600,3199201,1291.5291998386383,0.00010746508542069932
800801,1601603,1601602,3203205,1292.9642658233643,0.00010587986992049991
801802,1603605,1603604,3207209,1294.4031238555908,0.00010431804366817232
802803,1605607,1605606,3211213,1295.8450129032135,0.00010277926162416406
803804,1607609,1607608,3215217,1297.3644659519196,0.000101263183410083
804805,1609611,1609610,3219221,1299.258094072342,9.97694737634447e-05
805806,1611613,1611612,3223225,1301.1244139671326,9.829780196923821e-05
806807,1613615,1613614,3227229,1302.9172847270966,9.68478429967945e-05
807808,1615617,1615616,3231233,1305.1363897323608,9.541927590817068e-05
808809,1617619,1617618,3235237,1307.8950567245483,9.401178510870523e-05
809810,1619621,1619620,3239241,1311.0492379665375,9.262505909646279e-05
810811,1621623,1621622,3243245,1313.132670879364,9.125879159910255e-05
811812,1623625,1623624,3247249,1314.9935097694397,8.991267998226249e-05
812813,1625627,1625626,3251253,1316.698980808258,8.858642695486196e-05
813814,1627629,1627628,3255257,1318.4191617965698,8.727973931854649e-05
814815,1629631,1629630,3259261,1319.8999009132385,8.599232819506142e-05
815816,1631633,1631632,3263265,1321.5038557052612,8.472390879887826e-05
816817,1633635,1633634,3267269,1323.3447318077087,8.347420066456834e-05
817818,1635637,1635636,3271273,1325.0557188987732,8.224292787417653e-05
818819,1637639,1637638,3275277,1326.6761629581451,8.102981803403964e-05
819820,1639641,1639640,3279281,1328.35196185112,7.983460284322064e-05
820821,1641643,1641642,3283285,1329.9181249141693,7.865701843456918e-05
821822,1643645,1643644,3287289,1331.3665280342102,7.749680423785321e-05
822823,1645647,1645646,3291293,1332.816508769989,7.63537040029405e-05
823824,1647649,1647648,3295297,1334.2447159290314,7.522746489030396e-05
824825,1649651,1649650,3299301,1335.9561228752136,7.411783803945582e-05
825826,1651653,1651652,3303305,1338.8577799797058,7.302457845526078e-05
826827,1653655,1653654,3307309,1341.1140730381012,7.194744409844134e-05
827828,1655657,1655656,3311313,1342.9546637535095,7.088619736350665e-05
828829,1657659,1657658,3315317,1344.4688758850098,6.984060348713683e-05
829830,1659661,1659660,3319321,1345.9433958530426,6.881043145767762e-05
830831,1661663,1661662,3323325,1347.4171090126038,6.779545356039307e-05
831832,1663665,1663664,3327329,1350.0611789226532,6.679544560483919e-05
832833,1665667,1665666,3331333,1351.7679789066315,6.581018669749028e-05
833834,1667669,1667668,3335337,1353.732712984085,6.483945890067844e-05
834835,1669671,1669670,3339341,1355.2237360477448,6.388304791471455e-05
835836,1671673,1671672,3343345,1356.7223489284515,6.294074262314098e-05
836837,1673675,1673674,3347349,1358.209017753601,6.201233441061049e-05
837838,1675677,1675676,3351353,1359.7032570838928,6.109761829975469e-05
838839,1677679,1677678,3355357,1361.3262519836426,6.01963924964366e-05
839840,1679681,1679680,3359361,1363.4774677753448,5.930845748025604e-05
840841,1681683,1681682,3363365,1364.9409310817719,5.84336173687916e-05
841842,1683685,1683684,3367369,1366.4258427619934,5.757167878073233e-05
842843,1685687,1685686,3371373,1367.9436929225922,5.6722451517998707e-05
843844,1687689,1687688,3375377,1369.3912630081177,5.5885747769934824e-05
844845,1689691,1689690,3379381,1370.8511517047882,5.506138290911622e-05
845846,1691693,1691692,3383385,1372.3312108516693,5.4249174695542024e-05
846847,1693695,1693694,3387389,1373.779364824295,5.344894361769548e-05
847848,1695697,1695696,3391393,1375.2336146831512,5.2660513119917596e-05
848849,1697699,1697698,3395397,1376.7238988876343,5.188370903397299e-05
849850,1699701,1699700,3399401,1378.2641298770905,5.111835992011038e-05
850851,1701703,1701702,3403405,1380.177484035492,5.0364296384941554e-05
851852,1703705,1703704,3407409,1382.102077960968,4.9621352331996604e-05
852853,1705707,1705706,3411413,1385.086744070053,4.888936348379502e-05
853854,1707709,1707708,3415417,1387.2790310382843,4.816816817765357e-05
854855,1709711,1709710,3419421,1389.317463874817,4.745760702462576e-05
855856,1711713,1711712,3423425,1391.4199569225311,4.675752347793605e-05
856857,1713715,1713714,3427429,1393.670891046524,4.606776246873778e-05
857858,1715717,1715716,3431433,1395.2207489013672,4.538817222510261e-05
858859,1717719,1717718,3435437,1396.906798839569,4.471860211197054e-05
859860,1719721,1719720,3439441,1398.423178911209,4.4058904677513056e-05
860861,1721723,1721722,3443445,1399.9123487472534,4.340893440257787e-05
861862,1723725,1723724,3447449,1401.4438619613647,4.276854735962843e-05
862863,1725727,1725726,3451453,1403.263070821762,4.213760223592544e-05
863864,1727729,1727728,3455457,1404.9326887130737,4.1515960106153216e-05
864865,1729731,1729730,3459461,1406.9414117336273,4.090348318186443e-05
865866,1731733,1731732,3463465,1408.466784954071,4.030003674415639e-05
866867,1733735,1733734,3467469,1410.4937028884888,3.970548721099476e-05
867868,1735737,1735736,3471473,1412.3728818893433,3.911970350145566e-05
868869,1737739,1737738,3475477,1414.488226890564,3.854255623991776e-05
869870,1739741,1739740,3479481,1416.2526128292084,3.7973918097122805e-05
870871,1741743,1741742,3483485,1418.0151557922363,3.741366356280196e-05
871872,1743745,1743744,3487489,1419.6593868732452,3.686166860461526e-05
872873,1745747,1745746,3491493,1421.1739447116852,3.631781180502003e-05
873874,1747749,1747748,3495497,1422.7853429317474,3.5781973224402464e-05
874875,1749751,1749750,3499501,1424.381609916687,3.525403394633031e-05
875876,1751753,1751752,3503505,1425.857302904129,3.473387812391593e-05
876877,1753755,1753754,3507509,1427.660033941269,3.422139047870587e-05
877878,1755757,1755756,3511513,1429.4007768630981,3.3716458347043954e-05
878879,1757759,1757758,3515517,1431.0491378307343,3.321896986108186e-05
879880,1759761,1759760,3519521,1432.3759417533875,3.272881519933435e-05
880881,1761763,1761762,3523525,1433.6993207931519,3.22458867003661e-05
881882,1763765,1763764,3527529,1434.9607639312744,3.177007715748914e-05
882883,1765767,1765766,3531533,1436.228453874588,3.1301282092499605e-05
883884,1767769,1767768,3535537,1437.5865757465363,3.083939770931465e-05
884885,1769771,1769770,3539541,1438.847068786621,3.0384322258214524e-05
885886,1771773,1771772,3543545,1440.2869129180908,2.9935955012660997e-05
886887,1773775,1773774,3547549,1441.8507568836212,2.9494197406165767e-05
887888,1775777,1775776,3551553,1443.4000618457794,2.905895189542207e-05
888889,1777779,1777778,3555557,1445.0059688091278,2.8630122187678353e-05
889890,1779781,1779780,3559561,1446.5039298534393,2.8207614036546147e-05
890891,1781783,1781782,3563565,1448.3179769515991,2.779133376407117e-05
891892,1783785,1783784,3567569,1450.258292913437,2.738118996603589e-05
892893,1785787,1785786,3571573,1451.9864220619202,2.6977091692970134e-05
893894,1787789,1787788,3575577,1453.6352219581604,2.657895015545364e-05
894895,1789791,1789790,3579581,1455.890956878662,2.6186677246187173e-05
895896,1791793,1791792,3583585,1458.2495198249817,2.5800186563174066e-05
896897,1793795,1793794,3587589,1460.1230220794678,2.5419392841286026e-05
897898,1795797,1795796,3591593,1461.7365407943726,2.5044212065949978e-05
898899,1797799,1797798,3595597,1463.39612698555,2.4674561359461222e-05
899900,1799801,1799800,3599601,1465.4730479717255,2.431035932204395e-05
900901,1801803,1801802,3603605,1467.0349488258362,2.3951525463417056e-05
901902,1803805,1803804,3607609,1468.566555738449,2.3597980657541484e-05
902903,1805807,1805806,3611613,1470.0191888809204,2.3249647028933396e-05
903904,1807809,1807808,3615617,1471.4652190208435,2.2906447611603653e-05
904905,1809811,1809810,3619621,1472.9162647724152,2.2568306576431496e-05
905906,1811813,1811812,3623625,1474.4281969070435,2.2235149572225055e-05
906907,1813815,1813814,3627629,1475.8588087558746,2.190690315728716e-05
907908,1815817,1815816,3631633,1477.3321678638458,2.1583494458354835e-05
908909,1817819,1817818,3635637,1478.8353006839752,2.1264852762215014e-05
909910,1819821,1819820,3639641,1480.2928688526154,2.095090712828096e-05
910911,1821823,1821822,3643645,1481.7269339561462,2.064158888970269e-05
911912,1823825,1823824,3647649,1483.1803557872772,2.0336829493317055e-05
912913,1825827,1825826,3651653,1484.6174457073212,2.003656197757664e-05
913914,1827829,1827828,3655657,1486.0719459056854,1.9740719721994537e-05
914915,1829831,1829830,3659661,1487.5402429103851,1.944923781138641e-05
915916,1831833,1831832,3663665,1489.1120519638062,1.9162051671628433e-05
916917,1833835,1833834,3667669,1490.647341966629,1.8879098320212506e-05
917918,1835837,1835836,3671673,1493.045637845993,1.8600315115691046e-05
918919,1837839,1837838,3675677,1494.4724879264832,1.8325640667171683e-05
919920,1839841,1839840,3679681,1495.8947451114655,1.8055014265883074e-05
920921,1841843,1841842,3683685,1497.3440277576447,1.778837633992225e-05
921922,1843845,1843844,3687689,1498.8062818050385,1.752566788582044e-05
922923,1845847,1845846,3691693,1500.2637376785278,1.7266831150664075e-05
923924,1847849,1847848,3695697,1501.6871438026428,1.701180917734746e-05
924925,1849851,1849850,3699701,1503.1335060596466,1.676054569088592e-05
925926,1851853,1851852,3703705,1504.5898077487946,1.6512984984728973e-05
926927,1853855,1853854,3707709,1506.0187330245972,1.626907260288135e-05
927928,1855857,1855856,3711713,1507.4618458747864,1.602875488515565e-05
928929,1857859,1857858,3715717,1508.8911318778992,1.579197873979865e-05
929930,1859861,1859860,3719721,1510.4490458965302,1.555869209823868e-05
930931,1861863,1861862,3723725,1512.5386259555817,1.5328843119277735e-05
931932,1863865,1863864,3727729,1514.1214110851288,1.5102381780707219e-05
932933,1865867,1865866,3731733,1515.8948678970337,1.4879257378197508e-05
933934,1867869,1867868,3735737,1517.4125518798828,1.4659421140095219e-05
934935,1869871,1869870,3739741,1518.8952770233154,1.444282474949432e-05
935936,1871873,1871872,3743745,1520.3681910037994,1.4229420003175619e-05
936937,1873875,1873874,3747749,1521.781301021576,1.4019160289535648e-05
937938,1875877,1875876,3751753,1523.17201089859,1.3811998883284105e-05
938939,1877879,1877878,3755757,1524.61110496521,1.36078903096859e-05
939940,1879881,1879880,3759761,1526.021934747696,1.340678977612697e-05
940941,1881883,1881882,3763765,1527.3919439315796,1.3208652376306418e-05
941942,1883885,1883884,3767769,1528.8269398212433,1.3013434909225907e-05
942943,1885887,1885886,3771773,1530.2505469322205,1.2821094173887104e-05
943944,1887889,1887888,3775777,1531.6416997909546,1.2631587765099539e-05
944945,1889891,1889890,3779781,1533.027864933014,1.2444873505046417e-05
945946,1891893,1891892,3783785,1534.4300708770752,1.2260911034900346e-05
946947,1893895,1893894,3787789,1535.843554019928,1.2079659200026072e-05
947948,1895897,1895896,3791793,1537.2858917713165,1.1901078551090905e-05
948949,1897899,1897898,3795797,1538.6855590343475,1.1725129070327966e-05
949950,1899901,1899900,3799801,1540.5908510684967,1.1551772331586108e-05
950951,1901903,1901902,3803805,1542.376450061798,1.1380970022401016e-05
951952,1903905,1903904,3807809,1544.0899667739868,1.121268473980308e-05
952953,1905907,1905906,3811813,1546.2242999076843,1.1046878967135854e-05
953954,1907909,1907908,3815817,1547.7297358512878,1.088351655198494e-05
954955,1909911,1909910,3819821,1549.282557964325,1.0722561114562268e-05
955956,1911913,1911912,3823825,1550.88272190094,1.0563977411948144e-05
956957,1913915,1913914,3827829,1552.4594287872314,1.0407730542283389e-05
957958,1915917,1915916,3831833,1553.9791049957275,1.0253786058456171e-05
958959,1917919,1917918,3835837,1555.5028448104858,1.0102109854415176e-05
959960,1919921,1919920,3839841,1557.049036026001,9.952668392543274e-06
960961,1921923,1921922,3843845,1558.5137889385223,9.80542904471804e-06
961962,1923925,1923924,3847849,1560.110701084137,9.660359296503884e-06
962963,1925927,1925926,3851853,1561.59525680542,9.517426974525733e-06
963964,1927929,1927928,3855857,1563.4327018260956,9.376600587529538e-06
964965,1929931,1929930,3859861,1565.744600057602,9.237849326382275e-06
965966,1931933,1931932,3863865,1567.6659047603607,9.101142381950922e-06
966967,1933935,1933934,3867869,1569.1091630458832,8.966449968283996e-06
967968,1935937,1935936,3871873,1570.6018407344818,8.833741958369501e-06
968969,1937939,1937938,3875877,1572.0389947891235,8.702989362063818e-06
969970,1939941,1939940,3879881,1573.613891839981,8.574163189223327e-06
970971,1941943,1941942,3883885,1575.1189138889313,8.447235245512275e-06
971972,1943945,1943944,3887889,1576.643573999405,8.322177677655418e-06
972973,1945947,1945946,3891893,1578.1158657073975,8.198962291317002e-06
973974,1947949,1947948,3895897,1579.5258748531342,8.077562597463839e-06
974975,1949951,1949950,3899901,1581.0197818279266,7.95795153862855e-06
975976,1951953,1951952,3903905,1582.53679895401,7.840102625777945e-06
976977,1953955,1953954,3907909,1584.088654756546,7.723990279373538e-06
977978,1955957,1955956,3911913,1585.6160428524017,7.609588692503166e-06
978979,1957959,1957958,3915917,1587.015862941742,7.4968725130020175e-06
979980,1959961,1959960,3919921,1588.4822657108307,7.3858172981999815e-06
980981,1961963,1961962,3923925,1589.9382038116455,7.276398150679597e-06
981982,1963965,1963964,3927929,1591.368080854416,7.168591082518105e-06
982983,1965967,1965966,3931933,1592.812540769577,7.06237244685326e-06
983984,1967969,1967968,3935937,1594.2706108093262,6.957718596822815e-06
984985,1969971,1969970,3939941,1595.7517681121826,6.854606795059226e-06
985986,1971973,1971972,3943945,1597.1654210090637,6.753014190508111e-06
986987,1973975,1973974,3947949,1598.6018559932709,6.652918386862439e-06
987988,1975977,1975976,3951953,1600.0442008972168,6.5542972151888534e-06
988989,1977979,1977978,3955957,1601.429100036621,6.4571289613013505e-06
989990,1979981,1979980,3959961,1602.8317487239838,6.361392365761276e-06
990991,1981983,1981982,3963965,1604.2393300533295,6.267066396503651e-06
991992,1983985,1983984,3967969,1605.6557450294495,6.17412990777666e-06
992993,1985987,1985986,3971973,1607.0788757801056,6.082562663323188e-06
993994,1987989,1987988,3975977,1608.4785888195038,5.992344654259796e-06
994995,1989991,1989990,3979981,1609.889886856079,5.9034556443293695e-06
995996,1991993,1991992,3983985,1611.3209290504456,5.8158761930826586e-06
996997,1993995,1993994,3987989,1612.7654919624329,5.729587087444088e-06
997998,1995997,1995996,3991993,1614.1833610534668,5.6445692280249204e-06
998999,1997999,1997998,3995997,1615.6372537612915,5.560803856496932e-06
1000000,2000001,2000000,4000001,1617.1285779476166,5.478272555592412e-06


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007669925689697266,2180.042156630883
7,15,7,22,0.008723974227905273,414.4111683940796
13,27,13,40,0.014967918395996094,225.76746587107368
20,41,20,61,0.02197098731994629,145.8255695275161
27,55,27,82,0.029317855834960938,109.4558204131788
34,69,34,103,0.03636884689331055,89.98215269380376
40,81,40,121,0.0422520637512207,80.0340112122251
47,95,47,142,0.048967838287353516,72.7699283998536
54,109,54,163,0.0559999942779541,67.80266873069786
61,123,61,184,0.06306791305541992,64.10175602888171
67,135,67,202,0.07184195518493652,61.530190712698186
74,149,74,223,0.07957601547241211,58.976714359307834
81,163,81,244,0.08729290962219238,56.940181479457124
87,175,87,262,0.0940859317779541,55.611295282713854
94,189,94,283,0.10444188117980957,54.452590750704076
101,203,101,304,0.1129310131072998,53.61782095360809
108,217,108,325,0.12169909477233887,52.99222110110145
114,229,114,343,0.13109779357910156,52.53022394126674
121,243,121,364,0.13997387886047363,51.98460723043809
128,257,128,385,0.14846372604370117,51.38980050307123
135,271,135,406,0.15711474418640137,50.74694300645342
141,283,141,424,0.1645660400390625,50.16612764397519
148,297,148,445,0.17325115203857422,49.45580092378714
155,311,155,466,0.1821918487548828,48.7095318171946
161,323,161,484,0.18962574005126953,48.04562499645499
168,337,168,505,0.19829201698303223,47.253653677788634
175,351,175,526,0.20679879188537598,46.45569110584097
182,365,182,547,0.21551799774169922,45.66533931462459
188,377,188,565,0.22286391258239746,45.001134976618005
195,391,195,586,0.2322707176208496,44.2425491882625
202,405,202,607,0.2408139705657959,43.49633609495163
208,417,208,625,0.2482891082763672,42.86208948378135
215,431,215,646,0.25704097747802734,42.12520450817465
222,445,222,667,0.2655768394470215,41.38954354363432
229,459,229,688,0.27443885803222656,40.65323818727302
235,471,235,706,0.28116297721862793,40.02031819670037
242,485,242,727,0.2887568473815918,39.2786870518255
249,499,249,748,0.2966759204864502,38.53332037409382
256,513,256,769,0.30486488342285156,37.78563492192961
262,525,262,787,0.3119380474090576,37.14539769593989
269,539,269,808,0.3208029270172119,36.40299364617749
276,553,276,829,0.33077502250671387,35.66911733455731
282,565,282,847,0.33883070945739746,35.04861649648842
289,579,289,868,0.3465709686279297,34.33517557985215
296,593,296,889,0.3541378974914551,33.63250644917821
303,607,303,910,0.36156702041625977,32.939811044314865
309,619,309,928,0.36805200576782227,32.35371008696575
316,633,316,949,0.3757157325744629,31.678948806985318
323,647,323,970,0.3832120895385742,31.014084959764887
330,661,330,991,0.39032602310180664,30.358875431820024
336,673,336,1009,0.39616990089416504,29.8044238340442
343,687,343,1030,0.4029860496520996,29.165267235209512
350,701,350,1051,0.4098937511444092,28.534103425470676
356,713,356,1069,0.41562986373901367,27.99963246411062
363,727,363,1090,0.4224729537963867,27.384228608230615
370,741,370,1111,0.4296739101409912,26.77819890737328
377,755,377,1132,0.4367978572845459,26.181895294742844
383,767,383,1150,0.44255685806274414,25.678499301055353
390,781,390,1171,0.4494028091430664,25.099967548544782
397,795,397,1192,0.45648884773254395,24.530564136124667
404,809,404,1213,0.46324777603149414,23.970014281525437
410,821,410,1231,0.4689500331878662,23.49639410504551
417,835,417,1252,0.4759397506713867,22.951552706779694
424,849,424,1273,0.48305487632751465,22.414652347854826
430,861,430,1291,0.4890298843383789,21.96046758489115
437,875,437,1312,0.49574708938598633,21.437310512274507
444,889,444,1333,0.5026679039001465,20.92120623908386
451,903,451,1354,0.5095758438110352,20.412083209952243
457,915,457,1372,0.5153779983520508,19.981251411032872
464,929,464,1393,0.5222017765045166,19.48512240123273
471,943,471,1414,0.5291588306427002,18.996327111850178
478,957,478,1435,0.536125898361206,18.51486899101519
484,969,484,1453,0.5419950485229492,18.107860215944584
491,983,491,1474,0.5486741065979004,17.639705741797115
498,997,498,1495,0.5554580688476562,17.178797089765794
504,1009,504,1513,0.5613298416137695,16.789474965864656
511,1023,511,1534,0.5680367946624756,16.341862533067797
518,1037,518,1555,0.5749790668487549,15.901201822247913
525,1051,525,1576,0.5836780071258545,15.467348692518499
531,1063,531,1594,0.5897858142852783,15.100825477237777
538,1077,538,1615,0.5967748165130615,14.679427221110814
545,1091,545,1636,0.6040699481964111,14.264706183517205
552,1105,552,1657,0.6110978126525879,13.856636789370441
558,1117,558,1675,0.6171388626098633,13.512124176411703
565,1131,565,1696,0.624600887298584,13.116298502528252
572,1145,572,1717,0.6318938732147217,12.727053828106023
578,1157,578,1735,0.6381168365478516,12.398700963227498
585,1171,585,1756,0.6451678276062012,12.021882830427671
592,1185,592,1777,0.6524348258972168,11.65191153299395
599,1199,599,1798,0.6598179340362549,11.28886233424032
605,1211,605,1816,0.6659750938415527,10.983202551963359
612,1225,612,1837,0.6730499267578125,10.63301846025854
619,1239,619,1858,0.6803650856018066,10.289684190610615
625,1251,625,1876,0.6866309642791748,10.00078570080916
632,1265,632,1897,0.6937949657440186,9.669942977327764
639,1279,639,1918,0.7007298469543457,9.34569966113429
646,1293,646,1939,0.7078249454498291,9.027983471360585
652,1305,652,1957,0.7138957977294922,8.760816718877663
659,1319,659,1978,0.720923900604248,8.455136229150867
666,1333,666,1999,0.7283380031585693,8.155955260663859
673,1347,673,2020,0.7355568408966064,7.863316018115825
679,1359,679,2038,0.7417027950286865,7.617721170625032
686,1373,686,2059,0.748701810836792,7.337330548253249
693,1387,693,2080,0.7558679580688477,7.063556065419107
699,1399,699,2098,0.7620139122009277,6.83414962201789
706,1413,706,2119,0.7690958976745605,6.572616662409814
713,1427,713,2140,0.776425838470459,6.317616476460671
720,1441,720,2161,0.7838699817657471,6.069082552529039
726,1453,726,2179,0.7900009155273438,5.861136310380061
733,1467,733,2200,0.7969248294830322,5.624378830025307
740,1481,740,2221,0.8039870262145996,5.393828971483572
747,1495,747,2242,0.8110380172729492,5.169406383814021
753,1507,753,2260,0.8171539306640625,4.981874160683674
760,1521,760,2281,0.8243019580841064,4.76868269622787
767,1535,767,2302,0.831881046295166,4.561486880269854
773,1547,773,2320,0.8381249904632568,4.3886399735954456
780,1561,780,2341,0.8452448844909668,4.192495035150841
787,1575,787,2362,0.8524050712585449,4.002237597218823
794,1589,794,2383,0.8595988750457764,3.817801270280256
800,1601,800,2401,0.8657159805297852,3.664281085762127
807,1615,807,2422,0.8731729984283447,3.4904132930605556
814,1629,814,2443,0.8807859420776367,3.3220818650618185
821,1643,821,2464,0.8883929252624512,3.1591768633614947
827,1655,827,2482,0.8944289684295654,3.023786992698547
834,1669,834,2503,0.901663064956665,2.8707062638105754
841,1683,841,2524,0.9089059829711914,2.7228053824909466
847,1695,847,2542,0.9149179458618164,2.6001068027339898
854,1709,854,2563,0.9220719337463379,2.461654882073958
861,1723,861,2584,0.9297358989715576,2.328195759421533
868,1737,868,2605,0.9370548725128174,2.199653147041886
874,1749,874,2623,0.9430508613586426,2.0933224203929512
881,1763,881,2644,0.9500858783721924,1.9736785233990304
888,1777,888,2665,0.9572470188140869,1.8586910133519723
895,1791,895,2686,0.964378833770752,1.7482638740259517
901,1803,901,2704,0.9704709053039551,1.6571709646921136
908,1817,908,2725,0.9779930114746094,1.5549686120125443
915,1831,915,2746,0.9855659008026123,1.4570688506368015
921,1843,921,2764,0.991786003112793,1.3765122807221815
928,1857,928,2785,0.9990668296813965,1.286364800185197
935,1871,935,2806,1.0062029361724854,1.2002529046000063
942,1885,942,2827,1.013481855392456,1.1180699083614627
948,1897,948,2845,1.0195777416229248,1.0506689451440252
955,1911,955,2866,1.0271077156066895,0.9754804432019455
962,1925,962,2887,1.0346460342407227,0.9038931211264298
969,1939,969,2908,1.0418260097503662,0.8357965957684428
975,1951,975,2926,1.047834873199463,0.780129479672155
982,1965,982,2947,1.0552020072937012,0.7182560416480328
989,1979,989,2968,1.062134027481079,0.6596148376531801
995,1991,995,2986,1.0681829452514648,0.611869597013424
1002,2005,1002,3007,1.0756618976593018,0.5590457038110799
1009,2019,1009,3028,1.0851011276245117,0.5092565690873698
1016,2033,1016,3049,1.0934100151062012,0.4624274808484188
1022,2045,1022,3067,1.0996589660644531,0.42458159468003487
1029,2059,1029,3088,1.1068379878997803,0.3830238808086506
1036,2073,1036,3109,1.1138911247253418,0.3441708306613691
1042,2085,1042,3127,1.1200687885284424,0.3129471096389125
1049,2099,1049,3148,1.1274988651275635,0.27885953081920434
1056,2113,1056,3169,1.1346559524536133,0.2472029825167965
1063,2127,1063,3190,1.1420018672943115,0.21788721670998257
1069,2139,1069,3208,1.148155927658081,0.19455576980601563
1076,2153,1076,3229,1.1553409099578857,0.16935405576009543
1083,2167,1083,3250,1.1625280380249023,0.1462417102040945
1090,2181,1090,3271,1.1696269512176514,0.12512977737208075
1096,2193,1096,3289,1.1761200428009033,0.10855976274660861
1103,2207,1103,3310,1.1835057735443115,0.09093549237059051
1110,2221,1110,3331,1.1906428337097168,0.07507941753738123
1116,2233,1116,3349,1.1967859268188477,0.06284676637653774
1123,2247,1123,3370,1.203887939453125,0.050110279903378796
1130,2261,1130,3391,1.2109549045562744,0.0389778551514155
1137,2275,1137,3412,1.217998743057251,0.029397919748475942
1143,2287,1143,3430,1.224323034286499,0.022379646674380638
1150,2301,1150,3451,1.2319560050964355,0.015527599217648458
1157,2315,1157,3472,1.2393360137939453,0.01004705638536052
1164,2329,1164,3493,1.2464048862457275,0.0058625435859767094
1170,2341,1170,3511,1.2526118755340576,0.0032490617454641324
1177,2355,1177,3532,1.2600409984588623,0.0012693949472577515
1184,2369,1184,3553,1.2673008441925049,0.00037476265515579144
1190,2381,1190,3571,1.2751009464263916,0.0004225870362688511
1197,2395,1197,3592,1.283538818359375,0.0013760386623289378
1204,2409,1204,3613,1.2908217906951904,0.003242479096570605
1211,2423,1211,3634,1.2978079319000244,0.005967132288333232
1217,2435,1217,3652,1.3041260242462158,0.008944692467480309
1224,2449,1224,3673,1.311302900314331,0.013120831767423624
1231,2463,1231,3694,1.3182578086853027,0.018004869596097706
1238,2477,1238,3715,1.3256456851959229,0.023549315761329126
1244,2489,1244,3733,1.332258939743042,0.02879440748210982
1251,2503,1251,3754,1.3395969867706299,0.03545338799506226
1258,2517,1258,3775,1.3466298580169678,0.04265797144421413
1264,2529,1264,3793,1.35274076461792,0.04923951710952679
1271,2543,1271,3814,1.3598778247833252,0.05735789105767708
1278,2557,1278,3835,1.366905927658081,0.0659110867252366
1285,2571,1285,3856,1.3743958473205566,0.07485591620024934
1291,2583,1291,3874,1.3813297748565674,0.08280096652356406
1298,2597,1298,3895,1.3888518810272217,0.09235573423552523
1305,2611,1305,3916,1.3960049152374268,0.1021780827186376
1312,2625,1312,3937,1.4032268524169922,0.11222896030074025
1318,2637,1318,3955,1.4092659950256348,0.12099845669240494
1325,2651,1325,3976,1.4163079261779785,0.13137967665977612
1332,2665,1332,3997,1.4235658645629883,0.14189151912341913
1338,2677,1338,4015,1.4302940368652344,0.15098158465900724
1345,2691,1345,4036,1.438391923904419,0.16165282907525125
1352,2705,1352,4057,1.445694923400879,0.1723679604518793
1359,2719,1359,4078,1.4530251026153564,0.18310094540447608
1365,2731,1365,4096,1.4592549800872803,0.19229746327323483
1372,2745,1372,4117,1.4664487838745117,0.20300511693710632
1379,2759,1379,4138,1.4737648963928223,0.2136717202275804
1385,2771,1385,4156,1.4804737567901611,0.22276786578720476
1392,2785,1392,4177,1.4879648685455322,0.23330849933267928
1399,2799,1399,4198,1.495116949081421,0.24375239028108808
1406,2813,1406,4219,1.5022118091583252,0.25407784051287763
1412,2825,1412,4237,1.5083320140838623,0.26281740329102377
1419,2839,1419,4258,1.5154109001159668,0.2728657483397683
1426,2853,1426,4279,1.5225458145141602,0.2827365650825868
1433,2867,1433,4300,1.5304248332977295,0.2924125358672427
1439,2879,1439,4318,1.536942720413208,0.3005393299010848
1446,2893,1446,4339,1.5439369678497314,0.30981317412613407
1453,2907,1453,4360,1.5510878562927246,0.31885062993364954
1459,2919,1459,4378,1.5572559833526611,0.32639881892964695
1466,2933,1466,4399,1.5643420219421387,0.3349624899410628
1473,2947,1473,4420,1.5713598728179932,0.34325354068857905
1480,2961,1480,4441,1.579150915145874,0.35126123528164044
1486,2973,1486,4459,1.5855648517608643,0.3578924883051968
1493,2987,1493,4480,1.592736005783081,0.36535102450454815
1500,3001,1500,4501,1.5998280048370361,0.3725043453996477
1507,3015,1507,4522,1.607011079788208,0.37934716618701714
1513,3027,1513,4540,1.6132228374481201,0.3849616623855354
1520,3041,1520,4561,1.620668888092041,0.3912152098550905
1527,3055,1527,4582,1.6284308433532715,0.39714482691874764
1533,3067,1533,4600,1.6350829601287842,0.40196609382269344
1540,3081,1540,4621,1.6425888538360596,0.4072822996145078
1547,3095,1547,4642,1.6501109600067139,0.412262419442186
1554,3109,1554,4663,1.6576550006866455,0.4169029333116896
1560,3121,1560,4681,1.664160966873169,0.42060783455644923
1567,3135,1567,4702,1.6714911460876465,0.42460960867617814
1574,3149,1574,4723,1.6798100471496582,0.428263801011326
1581,3163,1581,4744,1.6879990100860596,0.4315685353677736
1587,3175,1587,4762,1.694502830505371,0.4341222023812179
1594,3189,1594,4783,1.7019739151000977,0.4367759741805912
1601,3203,1601,4804,1.7094647884368896,0.4390802291294449
1607,3215,1607,4822,1.715775966644287,0.4407787074156886
1614,3229,1614,4843,1.723397970199585,0.4424401353116991
1621,3243,1621,4864,1.7312419414520264,0.4437600139621054
1628,3257,1628,4885,1.739001750946045,0.44474187051741865
1634,3269,1634,4903,1.745412826538086,0.4453170919034619
1641,3283,1641,4924,1.7531960010528564,0.44568051210546855
1648,3297,1648,4945,1.761136770248413,0.4457160086137719
1655,3311,1655,4966,1.768779993057251,0.44542740836720895
1661,3323,1661,4984,1.775115966796875,0.4449252588337913
1668,3337,1668,5005,1.7829010486602783,0.4440462578526194
1675,3351,1675,5026,1.7900879383087158,0.44285634085724723
1681,3363,1681,5044,1.796072006225586,0.44159304425420487
1688,3377,1688,5065,1.8031589984893799,0.43984035478172245
1695,3391,1695,5086,1.810241937637329,0.43779315797655727
1702,3405,1702,5107,1.8174619674682617,0.4354578358652361
1708,3417,1708,5125,1.8238310813903809,0.4332318523822778
1715,3431,1715,5146,1.8315799236297607,0.43037928139210635
1722,3445,1722,5167,1.8392009735107422,0.4272580977343523
1729,3459,1729,5188,1.8464488983154297,0.4238752859426995
1735,3471,1735,5206,1.852691888809204,0.4207727688359455
1742,3485,1742,5227,1.8602428436279297,0.4169225243639403
1749,3499,1749,5248,1.8674230575561523,0.41283063439004763
1755,3511,1755,5266,1.8739609718322754,0.4091365380534171
1762,3525,1762,5287,1.8817028999328613,0.404615750131029
1769,3539,1769,5308,1.8893508911132812,0.3998756286380285
1776,3553,1776,5329,1.8965251445770264,0.39492497775734137
1782,3565,1782,5347,1.902590036392212,0.39052096256102686
1789,3579,1789,5368,1.909881830215454,0.3852038765646739
1796,3593,1796,5389,1.9169847965240479,0.37970288928704576
1802,3605,1802,5407,1.9232048988342285,0.37484840587592316
1809,3619,1809,5428,1.930804967880249,0.36903028051847286
1816,3633,1816,5449,1.9381167888641357,0.36305416007098756
1823,3647,1823,5470,1.945328950881958,0.35692879485156936
1829,3659,1829,5488,1.9514269828796387,0.35156627667140583
1836,3673,1836,5509,1.958622932434082,0.3451867516080256
1843,3687,1843,5530,1.9659268856048584,0.33868271089568225
1850,3701,1850,5551,1.9731528759002686,0.3320627558882734
1856,3713,1856,5569,1.9796478748321533,0.3263027535213041
1863,3727,1863,5590,1.9870216846466064,0.319490303770408
1870,3741,1870,5611,1.994196891784668,0.3125865594188326
1876,3753,1876,5629,2.0001578330993652,0.30660308823075866
1883,3767,1883,5650,2.007290840148926,0.2995533689623926
1890,3781,1890,5671,2.0143489837646484,0.2924380872899519
1897,3795,1897,5692,2.0215160846710205,0.2852665288735352
1903,3807,1903,5710,2.027956962585449,0.27908171971773754
1910,3821,1910,5731,2.0355329513549805,0.2718301566911805
1917,3835,1917,5752,2.0427017211914062,0.26454841558506814
1924,3849,1924,5773,2.049889087677002,0.25724525137172805
1930,3861,1930,5791,2.0559589862823486,0.25097483965430456
1937,3875,1937,5812,2.0629889965057373,0.2436544911375904
1944,3889,1944,5833,2.0699949264526367,0.23633680552723035
1950,3901,1950,5851,2.0764400959014893,0.23007281691843673
1957,3915,1957,5872,2.084192991256714,0.22278159158622657
1964,3929,1964,5893,2.0914299488067627,0.21551578259573034
1971,3943,1971,5914,2.0984699726104736,0.20828282446734647
1977,3955,1977,5932,2.1045339107513428,0.20211470202082182
1984,3969,1984,5953,2.111680030822754,0.194961473750368
1991,3983,1991,5974,2.1187970638275146,0.1878609000328879
1998,3997,1998,5995,2.1279358863830566,0.1808197176063686
2004,4009,2004,6013,2.1347768306732178,0.17483683835155261
2011,4023,2011,6034,2.141869068145752,0.16792405095804952
2018,4037,2018,6055,2.1489977836608887,0.16109027085849448
2024,4049,2024,6073,2.1551380157470703,0.15530085905356827
2031,4063,2031,6094,2.1622750759124756,0.14863200816284916
2038,4077,2038,6115,2.1694228649139404,0.14206145680884674
2045,4091,2045,6136,2.1771469116210938,0.1355955152818069
2051,4103,2051,6154,2.1837990283966064,0.13014109519849626
2058,4117,2058,6175,2.1910629272460938,0.12388508023809663
2065,4131,2065,6196,2.1982977390289307,0.11774987899161715
2072,4145,2072,6217,2.2055540084838867,0.11174042690231545
2078,4157,2078,6235,2.211664915084839,0.106692977630928
2085,4171,2085,6256,2.218660831451416,0.10092866290199254
2092,4185,2092,6277,2.2261340618133545,0.09530180231945451
2098,4197,2098,6295,2.2325758934020996,0.0905907324013242
2105,4211,2105,6316,2.239896059036255,0.08522786689252371
2112,4225,2112,6337,2.2470388412475586,0.08001151256667072
2119,4239,2119,6358,2.25426983833313,0.07494465146191942
2125,4251,2125,6376,2.2604379653930664,0.07072288591155029
2132,4265,2132,6397,2.2675719261169434,0.06594162752674038
2139,4279,2139,6418,2.2750298976898193,0.06131843517709967
2146,4293,2146,6439,2.283108949661255,0.05685619789630891
2152,4305,2152,6457,2.291167974472046,0.05316159600135961
2159,4319,2159,6478,2.2986271381378174,0.04900531180453527
2166,4333,2166,6499,2.305753707885742,0.045017105085776166
2172,4345,2172,6517,2.312203884124756,0.04173390990547432
2179,4359,2179,6538,2.3196370601654053,0.038062782508973214
2186,4373,2186,6559,2.3276407718658447,0.03456439239619158
2193,4387,2193,6580,2.3355777263641357,0.03123961006645004
2199,4399,2199,6598,2.342072010040283,0.02852829921346256
2206,4413,2206,6619,2.3495659828186035,0.02552667333361569
2213,4427,2213,6640,2.3571767807006836,0.02269863667845584
2219,4439,2219,6658,2.3635828495025635,0.020412195246422016
2226,4453,2226,6679,2.371532917022705,0.01790432149755361
2233,4467,2233,6700,2.379661798477173,0.015567293354820322
2240,4481,2240,6721,2.3881449699401855,0.013399933601021985
2246,4493,2246,6739,2.394460916519165,0.011676348048695218
2253,4507,2253,6760,2.4018988609313965,0.009820980896165565
2260,4521,2260,6781,2.409398078918457,0.008131941531132725
2267,4535,2267,6802,2.416727066040039,0.006608005714269893
2273,4547,2273,6820,2.423342704772949,0.005432176660178811
2280,4561,2280,6841,2.4316248893737793,0.004211196576534348
2287,4575,2287,6862,2.439290761947632,0.0031510242092736007
2293,4587,2293,6880,2.445773124694824,0.0023688243903734474
2300,4601,2300,6901,2.4535129070281982,0.0016018869647496103
2307,4615,2307,6922,2.4613020420074463,0.0009893391028299447
2314,4629,2314,6943,2.4687459468841553,0.0005282736865410698
2320,4641,2320,6961,2.4763619899749756,0.00025118601774920535
2327,4655,2327,6982,2.4844439029693604,6.258705775508133e-05
2334,4669,2334,7003,2.4917848110198975,1.5430387520609656e-05
2341,4683,2341,7024,2.4988298416137695,0.00010579604941085563
2347,4695,2347,7042,2.5050408840179443,0.00028967623131848086
2354,4709,2354,7063,2.5123329162597656,0.0006248066156331333
2361,4723,2361,7084,2.519489049911499,0.0010859965024110352
2367,4735,2367,7102,2.5257949829101562,0.0015786064852818527
2374,4749,2374,7123,2.5334529876708984,0.0022633103794760245
2381,4763,2381,7144,2.5407228469848633,0.003062648032141624
2388,4777,2388,7165,2.5478599071502686,0.003972563986849309
2394,4789,2394,7183,2.554028034210205,0.004837378629304112
2401,4803,2401,7204,2.561173915863037,0.00594164365963934
2408,4817,2408,7225,2.5688140392303467,0.007144455546722384
2415,4831,2415,7246,2.5766139030456543,0.008441399083494616
2421,4843,2421,7264,2.5835649967193604,0.009624548161241364
2428,4857,2428,7285,2.590902090072632,0.0110841641441084
2435,4871,2435,7306,2.5980679988861084,0.012624598939964926
2441,4883,2441,7324,2.6041719913482666,0.014005592632202024
2448,4897,2448,7345,2.6112377643585205,0.01568307966078919
2455,4911,2455,7366,2.6183128356933594,0.017427209280981515
2462,4925,2462,7387,2.625688076019287,0.019232931609053594
2468,4937,2468,7405,2.632481098175049,0.02082589169685889
2475,4951,2475,7426,2.6399760246276855,0.02273263781114565
2482,4965,2482,7447,2.6470448970794678,0.02468665277638138
2489,4979,2489,7468,2.6542088985443115,0.026683016179390506
2495,4991,2495,7486,2.6603620052337646,0.028424209341437745
2502,5005,2502,7507,2.667393922805786,0.030486397029903856
2509,5019,2509,7528,2.674860954284668,0.03257725970001957
2515,5031,2515,7546,2.6814358234405518,0.03438872798687953
2522,5045,2522,7567,2.6888508796691895,0.03652056828093464
2529,5059,2529,7588,2.6960740089416504,0.03866796467355016
2536,5073,2536,7609,2.7032909393310547,0.0408264062912167
2542,5085,2542,7627,2.7092747688293457,0.042681883914383434
2549,5099,2549,7648,2.7163939476013184,0.044848926134704925
2556,5113,2556,7669,2.7238378524780273,0.04701421101606229
2563,5127,2563,7690,2.7313599586486816,0.049173301639143574
2569,5139,2569,7708,2.737764835357666,0.051015695598607635
2576,5153,2576,7729,2.7448489665985107,0.05315171131860552
2583,5167,2583,7750,2.7519538402557373,0.05526923685215479
2589,5179,2589,7768,2.7580769062042236,0.05706643503719988
2596,5193,2596,7789,2.76515793800354,0.05913886423286385
2603,5207,2603,7810,2.772359848022461,0.061181478860362404
2610,5221,2610,7831,2.7797298431396484,0.0631905971309834
2616,5233,2616,7849,2.78597092628479,0.06488335381516208
2623,5247,2623,7870,2.7931110858917236,0.06682098699911876
2630,5261,2630,7891,2.800520896911621,0.06871537588597221
2636,5273,2636,7909,2.806705951690674,0.07030231004091547
2643,5287,2643,7930,2.8136887550354004,0.07210804971862217
2650,5301,2650,7951,2.820828914642334,0.07386176246552623
2657,5315,2657,7972,2.8280839920043945,0.07556058515763198
2663,5327,2663,7990,2.8343539237976074,0.07697095110256669
2670,5341,2670,8011,2.84161376953125,0.07856067610396167
2677,5355,2677,8032,2.8487799167633057,0.08008807664043616
2684,5369,2684,8053,2.85591197013855,0.08155086445447068
2690,5381,2690,8071,2.8620479106903076,0.08275165233669668
2697,5395,2697,8092,2.869036912918091,0.08408898245579621
2704,5409,2704,8113,2.876585006713867,0.08535613190258573
2710,5421,2710,8131,2.8829569816589355,0.08638515499808364
2717,5435,2717,8152,2.890084743499756,0.08751771892946181
2724,5449,2724,8173,2.8973379135131836,0.08857575698198161
2731,5463,2731,8194,2.904461145401001,0.08955797140549748
2737,5475,2737,8212,2.910651922225952,0.09033861247905861
2744,5489,2744,8233,2.9176671504974365,0.09117692704251112
2751,5503,2751,8254,2.9248907566070557,0.091936304234423
2758,5517,2758,8275,2.9323649406433105,0.09261589532206926
2764,5529,2764,8293,2.938720941543579,0.09313436751017434
2771,5543,2771,8314,2.9458019733428955,0.0936640719675097
2778,5557,2778,8335,2.953075885772705,0.09411247666855616
2784,5569,2784,8353,2.959152936935425,0.09443198583892354
2791,5583,2791,8374,2.9662578105926514,0.09472911989689692
2798,5597,2798,8395,2.9735779762268066,0.09494500346261248
2805,5611,2805,8416,2.9813120365142822,0.0950800084834782
2811,5623,2811,8434,2.9878180027008057,0.09513174905532651
2818,5637,2818,8455,2.994929790496826,0.09511804348926489
2825,5651,2825,8476,3.0021581649780273,0.09502528385110054
2832,5665,2832,8497,3.0091938972473145,0.09485430222071045
2838,5677,2838,8515,3.0154669284820557,0.09464617198614178
2845,5691,2845,8536,3.0226707458496094,0.09433237001996986
2852,5705,2852,8557,3.0305731296539307,0.09394310438642606
2858,5717,2858,8575,3.037202835083008,0.09355021644898898
2865,5731,2865,8596,3.044234037399292,0.09302378513905296
2872,5745,2872,8617,3.051265001296997,0.09242526815535257
2879,5759,2879,8638,3.0591509342193604,0.09175604620781996
2885,5771,2885,8656,3.0655128955841064,0.09112728893148869
2892,5785,2892,8677,3.0728588104248047,0.09033084900636368
2899,5799,2899,8698,3.0805158615112305,0.08946835402491615
2906,5813,2906,8719,3.0882108211517334,0.08854168714742627
2912,5825,2912,8737,3.0944318771362305,0.08769784426351634
2919,5839,2919,8758,3.101464033126831,0.08665741224160683
2926,5853,2926,8779,3.1086997985839844,0.0855588282406643
2932,5865,2932,8797,3.115341901779175,0.08457262765034557
2939,5879,2939,8818,3.123198986053467,0.08337214200605558
2946,5893,2946,8839,3.130788803100586,0.08212015759579572
2953,5907,2953,8860,3.1383578777313232,0.08081906672634886
2959,5919,2959,8878,3.144526720046997,0.07966658001123506
2966,5933,2966,8899,3.151798963546753,0.07828065651483485
2973,5947,2973,8920,3.158947706222534,0.07685247877748225
2979,5959,2979,8938,3.1650469303131104,0.07559651422718616
2986,5973,2986,8959,3.1720540523529053,0.07409624037916274
2993,5987,2993,8980,3.1799910068511963,0.07256061317082185
3000,6001,3000,9001,3.1874399185180664,0.07099210486705942
3006,6013,3006,9019,3.1934568881988525,0.06962340836412295
3013,6027,3013,9040,3.200511932373047,0.0680005674506674
3020,6041,3020,9061,3.2077560424804688,0.06635219974145912
3027,6055,3027,9082,3.214991807937622,0.06468098447817283
3033,6067,3033,9100,3.221176862716675,0.06323239043376816
3040,6081,3040,9121,3.229592800140381,0.06152597810375937
3047,6095,3047,9142,3.237541913986206,0.05980453441077316
3053,6107,3053,9160,3.2440378665924072,0.05831911625762132
3060,6121,3060,9181,3.251640796661377,0.05657696514992949
3067,6135,3067,9202,3.2591748237609863,0.054827458948693675
3074,6149,3074,9223,3.267021894454956,0.05307317187157423
3080,6161,3080,9241,3.2741029262542725,0.051567591317052575
3087,6175,3087,9262,3.283331871032715,0.04981101417615719
3094,6189,3094,9283,3.2921218872070312,0.048056632524662746
3101,6203,3101,9304,3.2998249530792236,0.046306779284577715
3107,6215,3107,9322,3.3072240352630615,0.044812250704694634
3114,6229,3114,9343,3.3150908946990967,0.04307688053677339
3121,6243,3121,9364,3.3230090141296387,0.041352540251409664
3127,6255,3127,9382,3.330656051635742,0.039885014653577855
3134,6269,3134,9403,3.3384499549865723,0.03818710229768385
3141,6283,3141,9424,3.3459620475769043,0.036506591668171495
3148,6297,3148,9445,3.353379726409912,0.0348456693712933
3154,6309,3154,9463,3.3600358963012695,0.0334392398503951
3161,6323,3161,9484,3.367777109146118,0.03182034397013922
3168,6337,3168,9505,3.3828659057617188,0.030227001312027824
3175,6351,3175,9526,3.391004800796509,0.028661152375548227
3181,6363,3181,9544,3.3974478244781494,0.027342279078538922
3188,6377,3188,9565,3.40516996383667,0.025832302126900686
3195,6391,3195,9586,3.413655996322632,0.024354809167448366
3201,6403,3201,9604,3.4207699298858643,0.023115416213158824
3208,6417,3208,9625,3.429743766784668,0.021702281215652874
3215,6431,3215,9646,3.4387898445129395,0.020325803289551914
3222,6445,3222,9667,3.446729898452759,0.01898728365745228
3228,6457,3228,9685,3.4535417556762695,0.017871131111064642
3235,6471,3235,9706,3.4616289138793945,0.016606340395810548
3242,6485,3242,9727,3.4691238403320312,0.01538289056497888
3249,6499,3249,9748,3.4774861335754395,0.014201863291418704
3255,6511,3255,9766,3.4842917919158936,0.013224098903833692
3262,6525,3262,9787,3.4916679859161377,0.012124533007181526
3269,6539,3269,9808,3.498973846435547,0.01107014975571019
3275,6551,3275,9826,3.505326747894287,0.010202978959569009
3282,6565,3282,9847,3.5127298831939697,0.009234613747366893
3289,6579,3289,9868,3.5202088356018066,0.008313523825904667
3296,6593,3296,9889,3.527817964553833,0.007440246127089267
3302,6605,3302,9907,3.5345840454101562,0.006730106861141394
3309,6619,3309,9928,3.542232036590576,0.005946690821815537
3316,6633,3316,9949,3.5496199131011963,0.0052120558503929715
3323,6647,3323,9970,3.5572218894958496,0.0045263645648674355
3329,6659,3329,9988,3.5635321140289307,0.003977651900527235
3336,6673,3336,10009,3.570823907852173,0.0033830351204642284
3343,6687,3343,10030,3.578681707382202,0.0028374379148772277
3349,6699,3349,10048,3.585000991821289,0.002408733825973286
3356,6713,3356,10069,3.5924458503723145,0.0019538992030447844
3363,6727,3363,10090,3.6001389026641846,0.001547687697893707
3370,6741,3370,10111,3.6075119972229004,0.001189849109437091
3376,6753,3376,10129,3.613830804824829,0.000921393845487728
3383,6767,3383,10150,3.6212427616119385,0.000652499165653353
3390,6781,3390,10171,3.6292059421539307,0.00043088166398774774
3396,6793,3396,10189,3.635877847671509,0.00027815089606519905
3403,6807,3403,10210,3.643286943435669,0.00014285866609498044
3410,6821,3410,10231,3.650819778442383,5.310701794769557e-05
3417,6835,3417,10252,3.658521890640259,8.137844247357862e-06
3423,6847,3423,10270,3.664918899536133,4.6106458739814116e-06
3430,6861,3430,10291,3.672466993331909,4.0567501173427445e-05
3437,6875,3437,10312,3.6808598041534424,0.00011878734528636414
3444,6889,3444,10333,3.688978910446167,0.000238290352626791
3450,6901,3450,10351,3.695481777191162,0.00037280842116160784
3457,6915,3457,10372,3.7030510902404785,0.0005662527520371441
3464,6929,3464,10393,3.7104477882385254,0.0007979848948025392
3470,6941,3470,10411,3.7168357372283936,0.001026249237384036
3477,6955,3477,10432,3.724514961242676,0.0013261332446745655
3484,6969,3484,10453,3.732408046722412,0.0016610708609050562
3491,6983,3491,10474,3.740032911300659,0.002029871126183025
3497,6995,3497,10492,3.74635910987854,0.0023720090077858913
3504,7009,3504,10513,3.753955125808716,0.002800414410671692
3511,7023,3511,10534,3.7614259719848633,0.0032590745288416656
3518,7037,3518,10555,3.768795967102051,0.0037466476608187804
3524,7049,3524,10573,3.7756128311157227,0.004186532912058283
3531,7063,3531,10594,3.7833521366119385,0.004724104842921406
3538,7077,3538,10615,3.791207790374756,0.005286543522743159
3544,7089,3544,10633,3.797576904296875,0.00578730839902164
3551,7103,3551,10654,3.8054420948028564,0.0063920016413021585
3558,7117,3558,10675,3.8134069442749023,0.00701730641173981
3565,7131,3565,10696,3.821230888366699,0.007661718424174069
3571,7143,3571,10714,3.828760862350464,0.008228142202142408
3578,7157,3578,10735,3.837127923965454,0.008904066913601127
3585,7171,3585,10756,3.8449690341949463,0.009594840894010304
3592,7185,3592,10777,3.8526289463043213,0.010298996905817148
3598,7197,3598,10795,3.8604719638824463,0.010912106092177964
3605,7211,3605,10816,3.869119882583618,0.011637256649123628
3612,7225,3612,10837,3.8782129287719727,0.012371645048460778
3618,7237,3618,10855,3.8856430053710938,0.013007377214989901
3625,7251,3625,10876,3.8934919834136963,0.013755082108332317
3632,7265,3632,10897,3.901279926300049,0.014507882665725447
3639,7279,3639,10918,3.909233808517456,0.015264321820723126
3645,7291,3645,10936,3.9164528846740723,0.015914489902570494
3652,7305,3652,10957,3.924445867538452,0.01667382625339542
3659,7319,3659,10978,3.931968927383423,0.017432661697739604
3666,7333,3666,10999,3.939687967300415,0.018189578247870486
3672,7345,3672,11017,3.945917844772339,0.018835782546261726
3679,7359,3679,11038,3.9530739784240723,0.01958547601736882
3686,7373,3686,11059,3.960441827774048,0.020329377690700312
3692,7385,3692,11077,3.966791868209839,0.020961427080578687
3699,7399,3699,11098,3.97428297996521,0.021691209830237312
3706,7413,3706,11119,3.9818010330200195,0.022411653107042184
3713,7427,3713,11140,3.989137887954712,0.023121587823766276
3719,7439,3719,11158,3.9952640533447266,0.023720876096945176
3726,7453,3726,11179,4.0025410652160645,0.02440829687668611
3733,7467,3733,11200,4.009848117828369,0.02508202781075397
3740,7481,3740,11221,4.017202854156494,0.025741001788560425
3746,7493,3746,11239,4.023971796035767,0.02629329935837177
3753,7507,3753,11260,4.0319437980651855,0.02692211757471341
3760,7521,3760,11281,4.039638042449951,0.027533267969829467
3766,7533,3766,11299,4.045874834060669,0.028042321811426518
3773,7547,3773,11320,4.053358793258667,0.028618149618750977
3780,7561,3780,11341,4.060913801193237,0.02917368458099645
3787,7575,3787,11362,4.068557024002075,0.02970809914563688
3793,7587,3793,11380,4.075085878372192,0.030148770868663632
3800,7601,3800,11401,4.08306097984314,0.030641952329119704
3807,7615,3807,11422,4.090616703033447,0.031111952379887953
3813,7627,3813,11440,4.096826791763306,0.0314958919215087
3820,7641,3820,11461,4.104413986206055,0.03192125029408999
3827,7655,3827,11482,4.112018823623657,0.032321806783215834
3834,7669,3834,11503,4.119624853134155,0.032697084705091584
3840,7681,3840,11521,4.126416921615601,0.032998299837800005
3847,7695,3847,11542,4.134432077407837,0.033325501176364014
3854,7709,3854,11563,4.1420509815216064,0.033626271455545975
3861,7723,3861,11584,4.149708986282349,0.03390027329226086
3867,7735,3867,11602,4.156481027603149,0.0341135955760592
3874,7749,3874,11623,4.164358854293823,0.03433710697584047
3881,7763,3881,11644,4.172309875488281,0.0345330815143825
3887,7775,3887,11662,4.183315992355347,0.03467899686575038
3894,7789,3894,11683,4.191461801528931,0.034823361593566915
3901,7803,3901,11704,4.198925733566284,0.03493977334301235
3908,7817,3908,11725,4.20662784576416,0.03502818623837811
3914,7829,3914,11743,4.213223934173584,0.03508168969722192
3921,7843,3921,11764,4.220920085906982,0.03511817237483683
3928,7857,3928,11785,4.230967998504639,0.035126829785667724
3935,7871,3935,11806,4.238724946975708,0.035107824455621994
3941,7883,3941,11824,4.245000839233398,0.035069674262786066
3948,7897,3948,11845,4.2524309158325195,0.034999881623775764
3955,7911,3955,11866,4.260438919067383,0.034903129443819125
3961,7923,3961,11884,4.266932964324951,0.034798978247295054
3968,7937,3968,11905,4.274990081787109,0.03465301119376818
3975,7951,3975,11926,4.283168077468872,0.034481052295177506
3982,7965,3982,11947,4.29079794883728,0.034283489552876745
3988,7977,3988,11965,4.297098875045776,0.03409408418690418
3995,7991,3995,11986,4.304595947265625,0.033850089311954434
4002,8005,4002,12007,4.312211990356445,0.03358174764048272
4009,8019,4009,12028,4.3197550773620605,0.03328956016503071
4015,8031,4015,12046,4.326766729354858,0.03302054118353226
4022,8045,4022,12067,4.334517002105713,0.03268552577526407
4029,8059,4029,12088,4.341956853866577,0.032328307134889656
4035,8071,4035,12106,4.348197937011719,0.0320049412298431
4042,8085,4042,12127,4.355751991271973,0.031608247906660836
4049,8099,4049,12148,4.3633599281311035,0.03119131412177012
4056,8113,4056,12169,4.371043920516968,0.030754891122455774
4062,8125,4062,12187,4.3780837059021,0.03036589037469639
4069,8139,4069,12208,4.386244773864746,0.029895347676870188
4076,8153,4076,12229,4.39353084564209,0.02940758125339471
4083,8167,4083,12250,4.400959014892578,0.0289034093303826
4089,8179,4089,12268,4.407927989959717,0.028458829838427846
4096,8193,4096,12289,4.415513753890991,0.02792638355163035
4103,8207,4103,12310,4.423215866088867,0.027379902683946966
4109,8219,4109,12328,4.429859161376953,0.026900956909912566
4116,8233,4116,12349,4.437583923339844,0.026330647188729017
4123,8247,4123,12370,4.445044994354248,0.025748726858864757
4130,8261,4130,12391,4.453892946243286,0.025156065980468156
4136,8273,4136,12409,4.460469961166382,0.024640192928359284
4143,8287,4143,12430,4.467988967895508,0.02402994645012768
4150,8301,4150,12451,4.47583270072937,0.02341153266411311
4156,8313,4156,12469,4.482648134231567,0.022875668966094054
4163,8327,4163,12490,4.490492820739746,0.022244568639507634
4170,8341,4170,12511,4.497675895690918,0.0216079936768665
4177,8355,4177,12532,4.505144119262695,0.020966901098177004
4183,8367,4183,12550,4.5118248462677,0.02041452268304056
4190,8381,4190,12571,4.519531011581421,0.019767573644003278
4197,8395,4197,12592,4.527200937271118,0.01911882097556372
4204,8409,4204,12613,4.535107135772705,0.018469193065243417
4210,8421,4210,12631,4.541385889053345,0.017912364418407378
4217,8435,4217,12652,4.548768043518066,0.0172635178469136
4224,8449,4224,12673,4.556510925292969,0.01661635601544731
4230,8461,4230,12691,4.562947750091553,0.01606364178314834
4237,8475,4237,12712,4.570734024047852,0.015421888822174878
4244,8489,4244,12733,4.5786659717559814,0.014784251275955285
4251,8503,4251,12754,4.586443901062012,0.014151557155400951
4257,8515,4257,12772,4.592957973480225,0.013613803561725035
4264,8529,4264,12793,4.600560903549194,0.01299245683674144
4271,8543,4271,12814,4.608257055282593,0.012378371439467628
4278,8557,4278,12835,4.615714073181152,0.011772340792958857
4284,8569,4284,12853,4.622365951538086,0.011259889359962472
4291,8583,4291,12874,4.630843877792358,0.010670878231962888
4298,8597,4298,12895,4.6385416984558105,0.010092109960851303
4304,8609,4304,12913,4.644848823547363,0.009604727613805153
4311,8623,4311,12934,4.652305841445923,0.009046893368577003
4318,8637,4318,12955,4.659800052642822,0.008501312215912549
4325,8651,4325,12976,4.667369842529297,0.007968633429186411
4331,8663,4331,12994,4.674030065536499,0.00752279062692196
4338,8677,4338,13015,4.682055950164795,0.0070156912238417135
4345,8691,4345,13036,4.69166374206543,0.006523179909777355
4352,8705,4352,13057,4.699400901794434,0.006045788243568495
4358,8717,4358,13075,4.705910921096802,0.00564901123573236
4365,8731,4365,13096,4.7134788036346436,0.00520101168160636
4372,8745,4372,13117,4.721077919006348,0.00476949534868254
4378,8757,4378,13135,4.727713108062744,0.004413066923007136
4385,8771,4385,13156,4.735652923583984,0.004013272019278702
4392,8785,4392,13177,4.743063926696777,0.003631107345086093
4399,8799,4399,13198,4.750426769256592,0.003266923097385188
4405,8811,4405,13216,4.756980895996094,0.002969321205569031
4412,8825,4412,13237,4.764631032943726,0.0026393622002842676
4419,8839,4419,13258,4.7723541259765625,0.002328226223880847
4426,8853,4426,13279,4.780243873596191,0.0020361490190907716
4432,8865,4432,13297,4.78670597076416,0.001801121335802236
4439,8879,4439,13318,4.793977737426758,0.0015449531490503432
4446,8893,4446,13339,4.801394939422607,0.0013083362191537162
4452,8905,4452,13357,4.808043003082275,0.0011211655912575225
4459,8919,4459,13378,4.8156468868255615,0.0009211192575548921
4466,8933,4466,13399,4.823314905166626,0.0007408451299397711
4473,8947,4473,13420,4.831121921539307,0.0005803585272587952
4479,8959,4479,13438,4.837614059448242,0.0004585370179484016
4486,8973,4486,13459,4.844963073730469,0.0003347354332845498
4493,8987,4493,13480,4.852466821670532,0.00023059934630964563
4500,9001,4500,13501,4.860450029373169,0.00014603052534312155
4506,9013,4506,13519,4.867125988006592,8.902198158011743e-05
4513,9027,4513,13540,4.877519845962524,4.043635954076308e-05
4520,9041,4520,13561,4.885625839233398,1.0983416018461867e-05
4526,9053,4526,13579,4.892096996307373,8.10708570497809e-07
4533,9067,4533,13600,4.899610757827759,6.322122317214962e-06
4540,9081,4540,13621,4.907290935516357,3.03032641113532e-05
4547,9095,4547,13642,4.9150710105896,7.246830205076549e-05
4553,9107,4553,13660,4.92178201675415,0.00012284609886137332
4560,9121,4560,13681,4.929797887802124,0.00019793076592122816
4567,9135,4567,13702,4.937502861022949,0.00029023598960975505
4573,9147,4573,13720,4.9439170360565186,0.0003827696497182842
4580,9161,4580,13741,4.9514079093933105,0.0005060171013155923
4587,9175,4587,13762,4.9590840339660645,0.0006453258322380862
4594,9189,4594,13783,4.966640949249268,0.0008002494747643141
4600,9201,4600,13801,4.9731810092926025,0.0009451168770056029
4607,9215,4607,13822,4.981168985366821,0.0011277900557615794
4614,9229,4614,13843,4.98882794380188,0.0013246986680996997
4621,9243,4621,13864,4.996222019195557,0.0015353250515772743
4627,9255,4627,13882,5.00262975692749,0.001726374939607922
4634,9269,4634,13903,5.010770797729492,0.0019610441569284376
4641,9283,4641,13924,5.019052982330322,0.002207856720019663
4647,9295,4647,13942,5.027544736862183,0.002428634198849977
4654,9309,4654,13963,5.037016868591309,0.002696441614034484
4661,9323,4661,13984,5.0449090003967285,0.0029746895310154287
4668,9337,4668,14005,5.053153991699219,0.003262757172478814
4674,9349,4674,14023,5.059660911560059,0.00351701010083616
4681,9363,4681,14044,5.067551851272583,0.0038216347529669292
4688,9377,4688,14065,5.07635498046875,0.004134256799602554
4695,9391,4695,14086,5.085377931594849,0.004454226761026803
4701,9403,4701,14104,5.092685699462891,0.004733839905497916
4708,9417,4708,14125,5.101020812988281,0.005065720315087674
4715,9431,4715,14146,5.109606981277466,0.00540307430037501
4721,9443,4721,14164,5.116788864135742,0.005696090519222707
4728,9457,4728,14185,5.125226974487305,0.0060418548938514505
4735,9471,4735,14206,5.133877992630005,0.006391199265863179
4742,9485,4742,14227,5.142008066177368,0.006743457302832212
4748,9497,4748,14245,5.149194002151489,0.007047205855883476
4755,9511,4755,14266,5.157716989517212,0.00740310389824117
4762,9525,4762,14287,5.165708065032959,0.007760008797276896
4769,9539,4769,14308,5.174242973327637,0.008117255958495662
4775,9551,4775,14326,5.181692838668823,0.008423239476201161
4782,9565,4782,14347,5.19023585319519,0.008779374824257502
4789,9579,4789,14368,5.198807954788208,0.009133983507013
4795,9591,4795,14386,5.206166982650757,0.009436235154453243
4802,9605,4802,14407,5.214404821395874,0.009786325873278656
4809,9619,4809,14428,5.22358775138855,0.010133099850463623
4816,9633,4816,14449,5.233016014099121,0.01047595549482594
4822,9645,4822,14467,5.2402801513671875,0.010766267420081022
4829,9659,4829,14488,5.2481958866119385,0.011100298584892698
4836,9673,4836,14509,5.256390810012817,0.0114287711758152
4843,9687,4843,14530,5.264430046081543,0.011751138589715993
4849,9699,4849,14548,5.271408796310425,0.012022190138623046
4856,9713,4856,14569,5.279232978820801,0.012331816585060551
4863,9727,4863,14590,5.286958932876587,0.012633852561521053
4869,9739,4869,14608,5.293407917022705,0.012886325195040627
4876,9753,4876,14629,5.3007659912109375,0.01317296840511517
4883,9767,4883,14650,5.3085808753967285,0.013450653398194845
4890,9781,4890,14671,5.31621789932251,0.013718932822371244
4896,9793,4896,14689,5.323117017745972,0.013941074905346795
4903,9807,4903,14710,5.331213712692261,0.014190764046020377
4910,9821,4910,14731,5.338842868804932,0.014429876269559827
4917,9835,4917,14752,5.3460328578948975,0.014658043406598154
4923,9847,4923,14770,5.352419137954712,0.014844641900140232
4930,9861,4930,14791,5.360214948654175,0.015051586151344054
4937,9875,4937,14812,5.367771863937378,0.015246664440837776
4943,9887,4943,14830,5.374696969985962,0.015404220431605609
4950,9901,4950,14851,5.38249397277832,0.01557654846112655
4957,9915,4957,14872,5.390044927597046,0.01573628523226489
4964,9929,4964,14893,5.397380828857422,0.015883221060107644
4970,9941,4970,14911,5.40380072593689,0.015998834569359133
4977,9955,4977,14932,5.411401987075806,0.016121514989094976
4984,9969,4984,14953,5.419137954711914,0.016230914105562988
4990,9981,4990,14971,5.425992012023926,0.01631401680901945
4997,9995,4997,14992,5.43407678604126,0.016398428866978065
5004,10009,5004,15013,5.441673040390015,0.01646925270574684
5011,10023,5011,15034,5.449096918106079,0.016526423417303704
5017,10035,5017,15052,5.455862998962402,0.016564527785931205
5024,10049,5024,15073,5.463854789733887,0.016596249770373106
5031,10063,5031,15094,5.471556901931763,0.01661426250268505
5038,10077,5038,15115,5.479726076126099,0.016618592950976563
5044,10089,5044,15133,5.486276865005493,0.016611452944744087
5051,10103,5051,15154,5.49360203742981,0.016590527332709826
5058,10117,5058,15175,5.501131057739258,0.016556128322918084
5064,10129,5064,15193,5.5078558921813965,0.0165160079202451
5071,10143,5071,15214,5.515448093414307,0.01645691368298685
5078,10157,5078,15235,5.523101806640625,0.01638473608068125
5085,10171,5085,15256,5.53068995475769,0.016299649980510367
5091,10183,5091,15274,5.537229061126709,0.016216590916428686
5098,10197,5098,15295,5.544685125350952,0.016108057973042378
5105,10211,5105,15316,5.552199840545654,0.015987215248628672
5112,10225,5112,15337,5.559973955154419,0.01585430558702683
5118,10237,5118,15355,5.566509008407593,0.015730975251926793
5125,10251,5125,15376,5.574086904525757,0.015576357974282473
5132,10265,5132,15397,5.582107782363892,0.01541046160116366
5138,10277,5138,15415,5.588810920715332,0.015259521019856948
5145,10291,5145,15436,5.596375942230225,0.015073509590820322
5152,10305,5152,15457,5.603844881057739,0.014877145565833416
5159,10319,5159,15478,5.611501932144165,0.014670784540498971
5165,10331,5165,15496,5.61802077293396,0.014486227363818216
5172,10345,5172,15517,5.625798940658569,0.014262294066270442
5179,10359,5179,15538,5.633635759353638,0.01402945814402301
5186,10373,5186,15559,5.641092777252197,0.013788126144959278
5192,10385,5192,15577,5.6474738121032715,0.013574823499084232
5199,10399,5199,15598,5.654998064041138,0.013318825024157377
5206,10413,5206,15619,5.662576913833618,0.01305554331975145
5212,10425,5212,15637,5.669209718704224,0.012824409134282178
5219,10439,5219,15658,5.677306890487671,0.012548771339311315
5226,10453,5226,15679,5.6851959228515625,0.012267121503441558
5233,10467,5233,15700,5.693231821060181,0.011979915744859682
5239,10479,5239,15718,5.699649095535278,0.011729666914675363
5246,10493,5246,15739,5.707259893417358,0.011433370829877276
5253,10507,5253,15760,5.7147767543792725,0.011132849852060644
5260,10521,5260,15781,5.722651958465576,0.010828578306472991
5266,10533,5266,15799,5.72970175743103,0.010565151024479746
5273,10547,5273,15820,5.737421751022339,0.010255183502181353
5280,10561,5280,15841,5.7447309494018555,0.009942836266645827
5286,10573,5286,15859,5.751016855239868,0.009673581507172457
5293,10587,5293,15880,5.7585649490356445,0.009358093594642014
5300,10601,5300,15901,5.76618504524231,0.009041601116791753
5307,10615,5307,15922,5.7739458084106445,0.008724581538672282
5313,10627,5313,15940,5.780781984329224,0.008452790234628083
5320,10641,5320,15961,5.788561820983887,0.0081360455186541
5327,10655,5327,15982,5.795869827270508,0.007820115208005518
5334,10669,5334,16003,5.803260803222656,0.007505458753257699
5340,10681,5340,16021,5.8096699714660645,0.007237110967253102
5347,10695,5347,16042,5.81715989112854,0.00692601827472572
5354,10709,5354,16063,5.824792146682739,0.00661747744902641
5360,10721,5360,16081,5.831480026245117,0.006355374033660155
5367,10735,5367,16102,5.839183807373047,0.0060527175523930055
5374,10749,5374,16123,5.846617937088013,0.005753831467359305
5381,10763,5381,16144,5.854182958602905,0.005459125792981467
5387,10775,5387,16162,5.860733985900879,0.005210151920550743
5394,10789,5394,16183,5.868438005447388,0.004924264004785073
5401,10803,5401,16204,5.876728057861328,0.00464367184895309
5407,10815,5407,16222,5.883858919143677,0.00440765880091476
5414,10829,5414,16243,5.893471002578735,0.004137869252872406
5421,10843,5421,16264,5.90116286277771,0.00387439396672562
5428,10857,5428,16285,5.908920049667358,0.0036175639068005694
5434,10869,5434,16303,5.91543984413147,0.0034029536673187977
5441,10883,5441,16324,5.923827886581421,0.0031592953916970146
5448,10897,5448,16345,5.932147026062012,0.0029231509491864927
5455,10911,5455,16366,5.939949035644531,0.0026947969646471392
5461,10923,5461,16384,5.946694850921631,0.0025054647716160616
5468,10937,5468,16405,5.954463005065918,0.002292263796903171
5475,10951,5475,16426,5.9625608921051025,0.0020875644433999696
5481,10963,5481,16444,5.969781875610352,0.0019190421926396084
5488,10977,5488,16465,5.978307723999023,0.0017307058868709646
5495,10991,5495,16486,5.986311912536621,0.00155146186955335
5502,11005,5502,16507,5.994428873062134,0.0013814870329724727
5508,11017,5508,16525,6.001097917556763,0.0012432941118731833
5515,11031,5515,16546,6.00892186164856,0.0010909473451192753
5522,11045,5522,16567,6.016709804534912,0.0009482847401613981
5529,11059,5529,16588,6.024786949157715,0.0008154188034268373
5535,11071,5535,16606,6.032014846801758,0.0007094037115393803
5542,11085,5542,16627,6.039911985397339,0.0005949711279527037
5549,11099,5549,16648,6.047769784927368,0.0004905615950292486
5555,11111,5555,16666,6.054543733596802,0.00040908088544711063
5562,11125,5562,16687,6.062877893447876,0.00032339627443889185
5569,11139,5569,16708,6.073307991027832,0.00024782397179023974
5576,11153,5576,16729,6.083317041397095,0.00018236443418118142
5582,11165,5582,16747,6.090009927749634,0.00013429432931388874
5589,11179,5589,16768,6.097346067428589,8.756477745919256e-05
5596,11193,5596,16789,6.104888916015625,5.086573628432234e-05
5603,11207,5603,16810,6.112441778182983,2.4139760853358894e-05
5609,11219,5609,16828,6.118973970413208,9.115170541917905e-06
5616,11233,5616,16849,6.126997947692871,7.076876045175595e-07
5623,11247,5623,16870,6.134954929351807,2.0274059124858468e-06
5629,11259,5629,16888,6.141397953033447,1.0814012284754426e-05
5636,11273,5636,16909,6.148861885070801,2.9882596322750032e-05
5643,11287,5643,16930,6.156548738479614,5.8310949384576816e-05
5650,11301,5650,16951,6.1646599769592285,9.594234370524646e-05
5656,11313,5656,16969,6.171478986740112,0.00013539370445414534
5663,11327,5663,16990,6.1796958446502686,0.00018965362107792316
5670,11341,5670,17011,6.187473773956299,0.0002525942749116439
5677,11355,5677,17032,6.194950819015503,0.00032400897566731146
5683,11367,5683,17050,6.201145887374878,0.0003918013869679271
5690,11381,5690,17071,6.2087507247924805,0.00047836773921972053
5697,11395,5697,17092,6.216355800628662,0.0005727585336217089
5703,11407,5703,17110,6.2229039669036865,0.0006597062368882689
5710,11421,5710,17131,6.230916738510132,0.0007679683538981408
5717,11435,5717,17152,6.238749980926514,0.000883328023633112
5724,11449,5724,17173,6.246145009994507,0.0010055139916858025
5730,11461,5730,17191,6.252639055252075,0.0011154661804084753
5737,11475,5737,17212,6.260453939437866,0.001249581074944217
5744,11489,5744,17233,6.2680089473724365,0.0013897010323944414
5750,11501,5750,17251,6.274677991867065,0.0015143539376367698
5757,11515,5757,17272,6.28286600112915,0.0016648166607637904
5764,11529,5764,17293,6.2904887199401855,0.0018203994003442858
5771,11543,5771,17314,6.29786491394043,0.0019807794568578174
5777,11555,5777,17332,6.304313898086548,0.0021218177236050906
5784,11569,5784,17353,6.312010049819946,0.002290232970494799
5791,11583,5791,17374,6.3197197914123535,0.0024624965855082337
5798,11597,5798,17395,6.327779054641724,0.002638269940689497
5804,11609,5804,17413,6.334810733795166,0.0027914681916172412
5811,11623,5811,17434,6.342423915863037,0.00297285532224123
5818,11637,5818,17455,6.349870920181274,0.0031567767522346912
5824,11649,5824,17473,6.356487989425659,0.0033161814048980887
5831,11663,5831,17494,6.3640828132629395,0.0035039017828921715
5838,11677,5838,17515,6.372114896774292,0.0036931797529859978
5845,11691,5845,17536,6.380082845687866,0.0038836745197841083
5851,11703,5851,17554,6.386989116668701,0.004047666455221588
5858,11717,5858,17575,6.39431095123291,0.004239519580778506
5865,11731,5865,17596,6.4016969203948975,0.004431620582067808
5872,11745,5872,17617,6.409430027008057,0.004623632643415476
5878,11757,5878,17635,6.415970087051392,0.004787889596286732
5885,11771,5885,17656,6.423872947692871,0.004978849349981829
5892,11785,5892,17677,6.431984901428223,0.005168769603642431
5898,11797,5898,17695,6.438628911972046,0.005330483435500355
5905,11811,5905,17716,6.446051836013794,0.0055176104084466715
5912,11825,5912,17737,6.453662872314453,0.0057027777243092714
5919,11839,5919,17758,6.461305856704712,0.005885674081014258
5925,11851,5925,17776,6.467844724655151,0.006040403902147773
5932,11865,5932,17797,6.475743055343628,0.006218280653683905
5939,11879,5939,17818,6.483844757080078,0.006393036735175883
5946,11893,5946,17839,6.491513729095459,0.006564390179846669
5952,11905,5952,17857,6.49786901473999,0.0067083487713262
5959,11919,5959,17878,6.50548791885376,0.006872663815101987
5966,11933,5966,17899,6.513147830963135,0.007032817350591358
5972,11945,5972,17917,6.5197179317474365,0.007166590485326196
5979,11959,5979,17938,6.527523756027222,0.007318360893577847
5986,11973,5986,17959,6.535402059555054,0.0074652804714787635
5993,11987,5993,17980,6.542909860610962,0.0076071245126740905
5999,11999,5999,17998,6.549147844314575,0.0077245015436346876
6006,12013,6006,18019,6.556736946105957,0.00785635387626371
6013,12027,6013,18040,6.564407110214233,0.007982538626606583
6020,12041,6020,18061,6.571923017501831,0.008102867322918428
6026,12053,6026,18079,6.578746795654297,0.008201210072343201
6033,12067,6033,18100,6.586606740951538,0.008310199437119081
6040,12081,6040,18121,6.594040870666504,0.008412853857976188
6046,12093,6046,18139,6.600387096405029,0.008495690759218633
6053,12107,6053,18160,6.608125925064087,0.008586203798358838
6060,12121,6060,18181,6.615808963775635,0.008669998729487816
6067,12135,6067,18202,6.623591899871826,0.008746964978740834
6073,12147,6073,18220,6.630378007888794,0.008807426065231994
6080,12161,6080,18241,6.638054847717285,0.008871458553926459
6087,12175,6087,18262,6.645417928695679,0.008928412984232637
6094,12189,6094,18283,6.653079986572266,0.008978224750308073
6100,12201,6100,18301,6.659860849380493,0.00901519493959313
6107,12215,6107,18322,6.66776704788208,0.009051609125435789
6114,12229,6114,18343,6.675740957260132,0.009080758346044604
6120,12241,6120,18361,6.682755708694458,0.009099944581407726
6127,12255,6127,18382,6.690496921539307,0.009115553467836435
6134,12269,6134,18403,6.697800874710083,0.009123865873220893
6141,12283,6141,18424,6.705626964569092,0.009124892396130235
6147,12295,6147,18442,6.712384939193726,0.009119989671148687
6154,12309,6154,18463,6.72041392326355,0.009107552356454107
6161,12323,6161,18484,6.729145765304565,0.009087922583375985
6167,12335,6167,18502,6.736119985580444,0.009065413806297329
6174,12349,6174,18523,6.743557929992676,0.009032581125211436
6181,12363,6181,18544,6.751003980636597,0.008992743301860173
6188,12377,6188,18565,6.758652925491333,0.008945987510287523
6194,12389,6194,18583,6.765125751495361,0.008900478914142695
6201,12403,6201,18604,6.77305793762207,0.008841143089512116
6208,12417,6208,18625,6.78161883354187,0.008775196200645041
6215,12431,6215,18646,6.7896177768707275,0.008702764642976035
6221,12443,6221,18664,6.795969009399414,0.008635621708208419
6228,12457,6228,18685,6.803489923477173,0.008551513545512535
6235,12471,6235,18706,6.8109519481658936,0.008461331128046368
6241,12483,6241,18724,6.817274808883667,0.008379318233551203
6248,12497,6248,18745,6.825101137161255,0.008278285090341342
6255,12511,6255,18766,6.833302021026611,0.008171655180376547
6262,12525,6262,18787,6.840908050537109,0.008059610366103698
6268,12537,6268,18805,6.847333908081055,0.007959405320775659
6275,12551,6275,18826,6.854783058166504,0.007837811454578514
6282,12565,6282,18847,6.862137794494629,0.00771136168771136
6289,12579,6289,18868,6.869761943817139,0.007580264693388017
6295,12591,6295,18886,6.876446962356567,0.007464359803861953
6302,12605,6302,18907,6.884436845779419,0.007325207043095361
6309,12619,6309,18928,6.89191198348999,0.0071820366758856835
6315,12631,6315,18946,6.898244857788086,0.007056296415385077
6322,12645,6322,18967,6.905930995941162,0.006906280965381484
6329,12659,6329,18988,6.913335084915161,0.006752919907398791
6336,12673,6336,19009,6.920710802078247,0.006596456560828301
6342,12685,6342,19027,6.927374839782715,0.0064600629319784275
6349,12699,6349,19048,6.935281991958618,0.006298495196119802
6356,12713,6356,19069,6.942878007888794,0.006134537848765831
6363,12727,6363,19090,6.950225830078125,0.005968445005464673
6369,12739,6369,19108,6.956517934799194,0.005824573905329089
6376,12753,6376,19129,6.963868856430054,0.005655194802216101
6383,12767,6383,19150,6.9712278842926025,0.005484414140596527
6389,12779,6389,19168,6.978632926940918,0.005337111001381345
6396,12793,6396,19189,6.986158132553101,0.005164412888689185
6403,12807,6403,19210,6.993457794189453,0.004991051269371383
6410,12821,6410,19231,7.00081992149353,0.004817283751208379
6416,12833,6416,19249,7.007277011871338,0.004668211677198997
6423,12847,6423,19270,7.0146801471710205,0.004494370261681979
6430,12861,6430,19291,7.02209997177124,0.004320852489968274
6437,12875,6437,19312,7.0298779010772705,0.004147910369056262
6443,12887,6443,19330,7.036532878875732,0.004000321811190588
6450,12901,6450,19351,7.043910980224609,0.0038291093683255895
6457,12915,6457,19372,7.051417827606201,0.003659178968746346
6463,12927,6463,19390,7.05794095993042,0.0035147278374552116
6470,12941,6470,19411,7.06532096862793,0.0033478161742550583
6477,12955,6477,19432,7.072927951812744,0.0031828665551074664
6484,12969,6484,19453,7.080909013748169,0.0030201091984736195
6490,12981,6490,19471,7.089643955230713,0.0028825188732071183
6497,12995,6497,19492,7.097584962844849,0.0027244274933764245
6504,13009,6504,19513,7.1052727699279785,0.0025691591755503396
6511,13023,6511,19534,7.113173007965088,0.002416924040289814
6517,13035,6517,19552,7.120345830917358,0.0022890057443873957
6524,13049,6524,19573,7.1289379596710205,0.0021429399416774686
6531,13063,6531,19594,7.137464761734009,0.0020004727051627924
6537,13075,6537,19612,7.144270896911621,0.0018813622809830122
6544,13089,6544,19633,7.152318000793457,0.0017460625664398322
6551,13103,6551,19654,7.160745859146118,0.0016148696804521023
6558,13117,6558,19675,7.168566942214966,0.001487947100713427
6564,13129,6564,19693,7.174996852874756,0.0013826734251551898
6571,13143,6571,19714,7.182801961898804,0.0012640887827046754
6578,13157,6578,19735,7.190244913101196,0.0011501987315796214
6584,13169,6584,19753,7.196609020233154,0.0010564163873141297
6591,13183,6591,19774,7.204093933105469,0.0009515921096863167
6598,13197,6598,19795,7.211451768875122,0.0008518213746810943
6605,13211,6605,19816,7.219003915786743,0.0007572138255227401
6611,13223,6611,19834,7.225514888763428,0.0006803079710380189
6618,13237,6618,19855,7.233237981796265,0.0005955507349426625
6625,13251,6625,19876,7.241055965423584,0.0005162221063983452
6632,13265,6632,19897,7.248887062072754,0.00044239764031317463
6638,13277,6638,19915,7.2554240226745605,0.00038355088634034473
6645,13291,6645,19936,7.263079881668091,0.0003201171628006705
6652,13305,6652,19957,7.271542072296143,0.0002623519825419862
6658,13317,6658,19975,7.279984951019287,0.0002173806867631356
6665,13331,6665,19996,7.2876060009002686,0.0001702397767076036
6672,13345,6672,20017,7.295017957687378,0.0001288544849558093
6679,13359,6679,20038,7.302637100219727,9.323719962139876e-05
6685,13371,6685,20056,7.308974027633667,6.730163181600801e-05
6692,13385,6692,20077,7.316393852233887,4.239799170591141e-05
6699,13399,6699,20098,7.32398796081543,2.32476229484746e-05
6706,13413,6706,20119,7.3321027755737305,9.828263046074426e-06
6712,13425,6712,20137,7.338464021682739,2.8641520657401998e-06
6719,13439,6719,20158,7.345659971237183,4.955609256285243e-10


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012731552124023438,2180.042156630883
2002,2003,2002,4005,2.599030017852783,58.25374124224231
4004,4005,4004,8009,5.550410032272339,52.3325146079394
6006,6007,6006,12013,8.399940252304077,49.460442359107674
8008,8009,8008,16017,12.707967042922974,47.11599220764424
10010,10011,10010,20021,16.910256147384644,45.01839520660428
12012,12013,12012,24025,20.07123613357544,43.1041342096305
14014,14015,14014,28029,22.234843254089355,41.34442017011406
16016,16017,16016,32033,24.46739625930786,39.72023725225745
18018,18019,18018,36037,27.24409008026123,38.217042626841476
20020,20021,20020,40041,29.938059091567993,36.82271904943559
22022,22023,22022,44045,32.28457713127136,35.52660307526935
24024,24025,24024,48049,34.81133532524109,34.319031355813195
26026,26027,26026,52053,37.3308470249176,33.1911537993999
28028,28029,28028,56057,40.411330223083496,32.13487290836338
30030,30031,30030,60061,42.95606303215027,31.14282994231644
32032,32033,32032,64065,45.43171811103821,30.208397006197856
34034,34035,34034,68069,47.86099028587341,29.32565773483998
36036,36037,36036,72073,49.98659038543701,28.48937249582923
38038,38039,38038,76077,52.266645193099976,27.69493045643776
40040,40041,40040,80081,54.5657160282135,26.938293162014816
42042,42043,42042,84085,56.80834937095642,26.215934371844924
44044,44045,44044,88089,59.21900796890259,25.52478002400767
46046,46047,46046,92093,61.93172025680542,24.86215105790029
48048,48049,48048,96097,64.49579119682312,24.225710762503468
50050,50051,50050,100101,66.95311307907104,23.613417476868108
52052,52053,52052,104105,69.22466826438904,23.023482868537712
54054,54055,54054,108109,71.5374813079834,22.454335625142676
56056,56057,56056,112113,73.92988634109497,21.9045901665354
58058,58059,58058,116117,76.20664024353027,21.37301987265505
60060,60061,60060,120121,78.53979539871216,20.858534286747044
62062,62063,62062,124125,80.68638110160828,20.36015976509907
64064,64065,64064,128129,83.02073121070862,19.877023082339747
66066,66067,66066,132133,85.22011518478394,19.40833755175686
68068,68069,68068,136137,87.52609205245972,18.953391274319983
70070,70071,70070,140141,89.66470503807068,18.51153718304704
72072,72073,72072,144145,91.83437633514404,18.08248844999025
74074,74075,74074,148149,93.9465901851654,17.665934156932735
76076,76077,76076,152153,96.128573179245,17.26085446709567
78078,78079,78078,156157,98.71073007583618,16.866771724344744
80080,80081,80080,160161,101.05764722824097,16.483250035031688
82082,82083,82082,164165,103.2496120929718,16.109886687983817
84084,84085,84084,168169,105.5673291683197,15.746307450084714
86086,86087,86086,172173,107.6981360912323,15.392162986714538
88088,88089,88088,176177,109.82220315933228,15.047125936799148
90090,90091,90090,180181,111.91037797927856,14.710888475447632
92092,92093,92092,184185,114.02033829689026,14.383160260547015
94094,94095,94094,188189,116.21445226669312,14.0636666872972
96096,96097,96096,192193,118.42794418334961,13.752147392701886
98098,98099,98098,196197,120.60367894172668,13.448354965090061
100100,100101,100100,200201,122.67649936676025,13.152053823399683
102102,102103,102102,204205,124.52444219589233,12.863019238252946
104104,104105,104104,208209,126.45313310623169,12.581036472378742
106106,106107,106106,212213,128.38393807411194,12.305900022172523
108108,108109,108108,216217,130.4476113319397,12.037412945500591
110110,110111,110110,220221,133.10494828224182,11.775386263436417
112112,112113,112112,224225,135.7337942123413,11.519638425694438
114114,114115,114114,228229,138.11872625350952,11.269994831166741
116116,116117,116116,232233,140.4447832107544,11.026287396320754
118118,118119,118118,236237,142.82550406455994,10.788354165312285
120120,120121,120120,240241,145.2939100265503,10.556038956571342
122122,122123,122122,244245,147.74786925315857,10.329191041376816
124124,124125,124124,248249,150.317889213562,10.107664850561719
126126,126127,126126,252253,153.08126616477966,9.89131970602864
128128,128129,128128,256257,155.2761800289154,9.68001957420347
130130,130131,130130,260261,157.9019901752472,9.473632838940262
132132,132133,132132,264265,160.09006214141846,9.272032091716596
134134,134135,134134,268269,162.20411229133606,9.075093937253314
136136,136137,136136,272273,164.451913356781,8.88269881292183
138138,138139,138138,276277,166.6570851802826,8.694730820531163
140140,140141,140140,280281,168.84525227546692,8.511077569257509
142142,142143,142142,284285,171.0157151222229,8.331630028648988
144144,144145,144144,288289,173.1730432510376,8.156282390773413
146146,146147,146146,292293,175.36536598205566,7.984931940698175
148148,148149,148148,296297,177.62288522720337,7.8174789345964655
150150,150151,150150,300301,179.8526041507721,7.65382648486343
152152,152153,152152,304305,182.09009408950806,7.4938804517049675
154154,154155,154154,308309,184.30994415283203,7.337549340718169
156156,156157,156156,312313,186.50056910514832,7.184744206047526
158158,158159,158158,316317,188.61428308486938,7.03537855873833
160160,160161,160160,320321,190.8081452846527,6.889368279945643
162162,162163,162162,324325,193.01863503456116,6.746631538689144
164164,164165,164164,328329,195.25345826148987,6.607088713862709
166166,166167,166166,332333,197.5209641456604,6.470662320235874
168168,168169,168168,336337,199.76155018806458,6.337276938185369
170170,170171,170170,340341,201.88551926612854,6.20685914692308
172172,172173,172172,344345,204.01611638069153,6.079337460986267
174174,174175,174174,348349,206.16153216362,5.954642269773672
176176,176177,176176,352353,208.32231497764587,5.832705779917887
178178,178179,178178,356357,210.52235221862793,5.7134619602970815
180180,180181,180180,360361,212.75186109542847,5.596846489497466
182182,182183,182182,364365,214.98792338371277,5.4827967055521185
184184,184185,184184,368369,217.12072014808655,5.371251557790401
186186,186187,186186,372373,219.28395819664001,5.262151560649954
188188,188189,188188,376377,221.43391823768616,5.155438749303357
190190,190191,190190,380381,223.58544325828552,5.051056636979297
192192,192193,192192,384385,225.82999396324158,4.948950173855906
194194,194195,194194,388389,228.03504729270935,4.849065707421914
196196,196197,196196,392393,230.2543122768402,4.751350944211708
198198,198199,198198,396397,232.40882110595703,4.655754912823113
200200,200201,200200,400401,234.5628433227539,4.562227928148445
202202,202203,202202,404405,236.74334716796875,4.470721556741864
204204,204205,204204,408409,238.9401831626892,4.3811885832645885
206206,206207,206206,412413,241.2309021949768,4.293582977952951
208208,208209,208208,416417,243.68491220474243,4.207859865057912
210210,210211,210210,420421,246.08915209770203,4.123975492207933
212212,212213,212212,424425,248.49859023094177,4.041887200662131
214214,214215,214214,428429,250.66003036499023,3.9615533964076803
216216,216217,216216,432433,252.85056018829346,3.882933522074609
218218,218219,218218,436437,255.0303349494934,3.8059880296335677
220220,220221,220220,440441,257.40616607666016,3.7306783538494983
222222,222223,222222,444445,259.73456716537476,3.656966886465284
224224,224225,224224,448449,262.22797322273254,3.5848169510911703
226226,226227,226226,452453,264.7601342201233,3.5141927787757368
228228,228229,228228,456457,266.960488319397,3.445059484240346
230230,230231,230230,460461,269.2586522102356,3.3773830427541043
232232,232233,232232,464465,272.3837833404541,3.3111302676321657
234234,234235,234234,468469,274.5964252948761,3.2462687883398758
236236,236237,236236,472473,277.85747027397156,3.1827670291839922
238238,238239,238238,476477,280.7028751373291,3.1205941885766606
240240,240241,240240,480481,283.1667683124542,3.059720218854409
242242,242243,242242,484485,285.8840560913086,3.000115806639883
244244,244245,244244,488489,288.357084274292,2.9417523537283614
246246,246247,246246,492493,291.1954972743988,2.8846019584888154
248248,248249,248248,496497,293.7174391746521,2.8286373977613266
250250,250251,250250,500501,296.25027418136597,2.773832109243699
252252,252253,252252,504505,298.5271670818329,2.720160174347029
254254,254255,254254,508509,300.8274083137512,2.6675963015154593
256256,256257,256256,512513,303.5860722064972,2.6161158099912427
258258,258259,258258,516517,306.53852701187134,2.5656946140189802
260260,260261,260260,520521,308.8104512691498,2.5163092074714086
262262,262263,262262,524525,311.05359625816345,2.4679366488925325
264264,264265,264264,528529,313.37713408470154,2.420554546941048
266266,266267,266266,532533,315.7950382232666,2.374141046226555
268268,268269,268268,536537,318.08701515197754,2.328674813526277
270270,270271,270270,540541,320.52282524108887,2.284135024375587
272272,272273,272272,544545,323.5352282524109,2.2405013500176665
274274,274275,274274,548549,325.83986616134644,2.1977539447048002
276276,276277,276276,552553,328.11139726638794,2.1558734333435723
278278,278279,278278,556557,330.36385011672974,2.1148408994716874
280280,280281,280280,560561,333.96388721466064,2.0746378735589133
282282,282283,282282,564565,336.5761661529541,2.0352463216235037
284284,284285,284284,568569,340.1240303516388,1.9966486341548944
286286,286287,286286,572573,342.2639582157135,1.9588276153351671
288288,288289,288288,576577,344.51355600357056,1.9217664725491659
290290,290291,290290,580581,346.8835949897766,1.8854488061788288
292292,292293,292292,584585,349.0089011192322,1.8498585996693464
294294,294295,294294,588589,351.20543217658997,1.8149802098645296
296296,296297,296296,592593,353.4293041229248,1.7807983576008155
298298,298299,298298,596597,356.65806102752686,1.747298118552294
300300,300301,300300,600601,359.5782582759857,1.7144649143231163
302302,302303,302302,604605,362.0418653488159,1.6822845037768275
304304,304305,304304,608609,364.5471670627594,1.650742974599325
306306,306307,306306,612613,366.89907026290894,1.6198267350854394
308308,308309,308308,616617,369.2629702091217,1.5895225061460678
310310,310311,310310,620621,371.55578231811523,1.559817313528697
312312,312313,312312,624625,373.7832372188568,1.530698480244041
314314,314315,314314,628629,376.01899313926697,1.5021536191948144
316316,316317,316316,632633,378.2740032672882,1.4741706260010687
318318,318319,318318,636637,380.48268699645996,1.4467376720150469
320320,320321,320320,640641,382.72800731658936,1.4198431975216863
322322,322323,322322,644645,385.1314561367035,1.3934759051186347
324324,324325,324324,648649,387.3582401275635,1.3676247532722527
326326,326327,326326,652653,389.8724431991577,1.3422789500427825
328328,328329,328328,656657,392.2821843624115,1.317427946975954
330330,330331,330330,660661,394.56707406044006,1.2930614331538663
332332,332333,332332,664665,396.8106451034546,1.2691693294044626
334334,334335,334334,668669,398.98766016960144,1.245741782660275
336336,336337,336336,672673,401.20540618896484,1.2227691604679194
338338,338339,338338,676677,403.3750972747803,1.2002420456394702
340340,340341,340340,680681,405.6083400249481,1.1781512310425342
342342,342343,342342,684685,407.8965313434601,1.1564877145299306
344344,344345,344344,688689,410.07972621917725,1.1352426939970428
346346,346347,346346,692693,412.33556509017944,1.1144075625707046
348348,348349,348348,696697,414.6582541465759,1.0939739039216647
350350,350351,350350,700701,416.8442301750183,1.0739334876989233
352352,352353,352352,704705,419.0006101131439,1.0542782650812796
354354,354355,354354,708709,421.34193110466003,1.0350003644455228
356356,356357,356356,712713,423.76086926460266,1.0160920871442158
358358,358359,358358,716717,425.94870829582214,0.9975459033931884
360360,360361,360360,720721,428.20590901374817,0.979354448264985
362362,362363,362362,724725,430.4506323337555,0.961510517784177
364364,364365,364364,728729,432.63280510902405,0.9440070651229462
366366,366367,366366,732733,434.8005881309509,0.9268371968939846
368368,368369,368368,736737,436.9976010322571,0.9099941695378675
370370,370371,370370,740741,439.1478431224823,0.8934713858016039
372372,372373,372372,744745,441.3499262332916,0.8772623913085908
374374,374375,374374,748749,445.72120237350464,0.8613608712126961
376376,376377,376376,752753,449.2512662410736,0.845760646939766
378378,378379,378378,756757,452.43699312210083,0.8304556730099648
380380,380381,380380,760761,455.36054706573486,0.8154400339399217
382382,382383,382382,764765,458.5096733570099,0.8007079412240046
384384,384385,384384,768769,461.30771040916443,0.7862537303907402
386386,386387,386386,772773,463.81040930747986,0.7720718581329038
388388,388389,388388,776777,466.55113220214844,0.7581568995099133
390390,390391,390390,780781,469.1878089904785,0.7445035452194588
392392,392393,392392,784785,471.7414960861206,0.7311065989376857
394394,394395,394394,788789,474.4277970790863,0.7179609747248605
396396,396397,396396,792793,476.75355315208435,0.7050616944972035
398398,398399,398398,796797,479.04983615875244,0.6924038855587469
400400,400401,400400,800801,481.4195091724396,0.6799827781953809
402402,402403,402402,804805,483.7926080226898,0.667793703330176
404404,404405,404404,808809,486.13891410827637,0.6558320902331616
406406,406407,406406,812813,488.68701219558716,0.6440934642897673
408408,408409,408408,816817,491.01044821739197,0.6325734448231515
410410,410411,410410,820821,494.49910712242126,0.6212677429699625
412412,412413,412412,824825,497.4975152015686,0.6101721596085099
414414,414415,414414,828829,500.7863039970398,0.5992825833362758
416416,416417,416416,832833,503.6718981266022,0.5885949884981301
418418,418419,418418,836837,506.2159721851349,0.5781054332612712
420420,420421,420420,840841,508.6760470867157,0.5678100577383702
422422,422423,422422,844845,511.0462472438812,0.5577050821538023
424424,424425,424424,848849,513.425252199173,0.5477868050571715
426426,426427,426426,852853,515.6754050254822,0.5380516015763988
428428,428429,428428,856857,517.8295040130615,0.5284959217166261
430430,430431,430430,860861,520.0653700828552,0.5191162886969778
432432,432433,432432,864865,522.1543872356415,0.509909297328818
434434,434435,434434,868869,524.2443311214447,0.5008716124320927
436436,436437,436436,872873,526.3054902553558,0.4919999672902122
438438,438439,438438,876877,528.5027191638947,0.48329116214063106
440440,440441,440440,880881,531.5053412914276,0.4747420627026031
442442,442443,442442,884885,533.7638993263245,0.46634959873904336
444444,444445,444444,888889,536.3153171539307,0.4581107626526091
446446,446447,446446,892893,538.8093671798706,0.45002260811577344
448448,448449,448448,896897,541.2881033420563,0.4420822487315945
450450,450451,450450,900901,543.6329700946808,0.4342868567281357
452452,452453,452452,904905,545.9292690753937,0.4266336616809667
454454,454455,454454,908909,548.0692563056946,0.41911994926931584
456456,456457,456456,912913,550.252509355545,0.4117430600571197
458458,458459,458458,916917,552.3679301738739,0.404500388306019
460460,460461,460460,920921,554.4270961284637,0.39738938081438846
462462,462463,462462,924925,556.507618188858,0.3904075357833108
464464,464465,464464,928929,558.6371812820435,0.38355240171006244
466466,466467,466466,932933,561.6757130622864,0.3768215763062699
468468,468469,468468,936937,564.0395519733429,0.37021270544096296
470470,470471,470470,940941,566.7845942974091,0.36372348210966265
472472,472473,472472,944945,569.3374311923981,0.3573516454249557
474474,474475,474474,948949,571.6887652873993,0.3510949796324212
476476,476477,476476,952953,573.8977053165436,0.34495131314770333
478478,478479,478478,956957,576.1339371204376,0.3389185176159799
480480,480481,480480,960961,578.2656321525574,0.3329945069937139
482482,482483,482482,964965,580.822005033493,0.32717723665132326
484484,484485,484484,968969,583.5637440681458,0.32146470249517733
486486,486487,486486,972973,586.2939803600311,0.315854940110853
488488,488489,488488,976977,588.4221892356873,0.3103460239249216
490490,490491,490490,980981,590.8156261444092,0.304936066386972
492492,492493,492492,984985,593.1153881549835,0.29962321716811857
494494,494495,494494,988989,595.5117952823639,0.29440566238008614
496496,496497,496496,992993,597.7695543766022,0.2892816238107798
498498,498499,498498,996997,599.9802792072296,0.28424935817611185
500501,500502,500501,1001003,602.2109751701355,0.2793047099822843
502503,502504,502503,1005007,604.3505582809448,0.2744509401803725
504505,504506,504505,1009011,606.430902004242,0.26968391499815425
506507,506508,506507,1013015,609.0252101421356,0.26500202373938464
508509,508510,508509,1017019,611.665854215622,0.26040368714450324
510511,510512,510511,1021023,613.967395067215,0.2558873567380715
512513,512514,512513,1025027,616.0622432231903,0.2514515141907623
514515,514516,514515,1029031,618.117269039154,0.2470946706959012
516517,516518,516517,1033035,621.1099503040314,0.24281536635987777
518519,518520,518519,1037039,623.9097692966461,0.238612169605517
520521,520522,520521,1041043,626.0393011569977,0.23448367658920688
522523,522524,522523,1045047,628.4394171237946,0.23042851063109993
524525,524526,524525,1049051,630.8983891010284,0.22644532165656983
526527,526528,526527,1053055,633.0539042949677,0.22253278565165147
528529,528530,528529,1057059,635.9442501068115,0.21868960412882643
530531,530532,530531,1061063,638.4704382419586,0.21491450360610997
532533,532534,532533,1065067,641.0513052940369,0.21120623509602865
534535,534536,534535,1069071,643.7782850265503,0.20756357360676247
536537,536538,536537,1073075,646.2452630996704,0.20398531765420103
538539,538540,538539,1077079,648.8715472221375,0.2004702887829808
540541,540542,540541,1081083,651.6030471324921,0.19701733110105124
542543,542544,542543,1085087,654.3699731826782,0.1936253108206074
544545,544546,544545,1089091,657.3312261104584,0.19029311581266484
546547,546548,546547,1093095,659.9528503417969,0.1870196551672052
548549,548550,548549,1097099,662.3882741928101,0.18380385876776018
550551,550552,550551,1101103,664.7957491874695,0.18064467687031538
552553,552554,552553,1105107,667.2796142101288,0.17754107969403776
554555,554556,554555,1109111,670.3776512145996,0.17449205702030213
556557,556558,556557,1113115,672.6773381233215,0.17149661780069891
558559,558560,558559,1117119,674.9081931114197,0.16855378977140845
560561,560562,560561,1121123,677.4043221473694,0.16566261907883018
562563,562564,562563,1125127,679.9212071895599,0.16282216991112364
564565,564566,564565,1129131,682.183806180954,0.16003152413782118
566567,566568,566567,1133135,684.7545731067657,0.15728978095762614
568569,568570,568569,1137139,686.9668023586273,0.15459605655416908
570571,570572,570571,1141143,689.442066192627,0.1519494837577895
572573,572574,572573,1145147,691.7772531509399,0.149349211714366
574575,574576,574575,1149151,694.0166771411896,0.1467944055635826
576577,576578,576577,1153155,696.264909029007,0.1442842461208329
578579,578580,578579,1157159,698.5034801959991,0.1418179295678783
580581,580582,580581,1161163,700.7320640087128,0.1393946671496451
582583,582584,582583,1165167,702.959614276886,0.13701368487613763
584585,584586,584585,1169171,705.2019572257996,0.13467422323265055
586587,586588,586587,1173175,707.8620893955231,0.1323755368947559
588589,588590,588589,1177179,710.1241700649261,0.13011689444908825
590591,590592,590591,1181183,712.5426201820374,0.12789757812095104
592593,592594,592593,1185187,715.4310550689697,0.12571688350647037
594595,594596,594595,1189191,717.9289281368256,0.12357411931077422
596597,596598,596597,1193195,720.3487732410431,0.12146860709287921
598599,598600,598599,1197199,722.8753771781921,0.1193996810131921
600601,600602,600601,1201203,725.7763941287994,0.1173666875889694
602603,602604,602603,1205207,728.1169202327728,0.11536898545250551
604605,604606,604605,1209211,730.3668072223663,0.1134059451169378
606607,606608,606607,1213215,732.5367321968079,0.11147694874330227
608609,608610,608609,1217219,734.622896194458,0.10958138991679789
610611,610612,610611,1221223,736.7861721515656,0.10771867342305086
612613,612614,612613,1225227,738.9510593414307,0.1058882150334739
614615,614616,614615,1229231,741.0494582653046,0.10408944129096653
616617,616618,616617,1233235,743.1341121196747,0.102321789302664
618619,618620,618619,1237239,745.304749250412,0.10058470653609675
620621,620622,620621,1241243,747.383415222168,0.09887765061932896
622623,622624,622623,1245247,749.8839392662048,0.09720008914575828
624625,624626,624625,1249251,752.4292573928833,0.09555149948130293
626627,626628,626627,1253255,755.3200581073761,0.09393136857863738
628629,628630,628629,1257259,757.8690192699432,0.09233919279165548
630631,630632,630631,1261263,760.5983150005341,0.09077447769550417
632633,632634,632633,1265267,763.318311214447,0.08923673791139208
634635,634636,634635,1269271,765.9258680343628,0.08772549693162546
636637,636638,636637,1273275,768.6855113506317,0.08624028695169272
638639,638640,638639,1277279,771.1283621788025,0.08478064870314483
640641,640642,640641,1281283,773.3942201137543,0.08334613129238733
642643,642644,642643,1285287,776.521222114563,0.08193629203924502
644645,644646,644645,1289291,778.8189971446991,0.08055069632268896
646647,646648,646647,1293295,781.5466501712799,0.07918891742610867
648649,648650,648649,1297299,783.8294951915741,0.07785053638826867
650651,650652,650651,1301303,786.2195162773132,0.07653514185653876
652653,652654,652653,1305307,788.6756691932678,0.07524232994126123
654655,654656,654655,1309311,791.3919901847839,0.07397170407648446
656657,656658,656657,1313315,793.981448173523,0.07272287488058282
658659,658660,658659,1317319,796.5742721557617,0.07149546002040097
660661,660662,660661,1321323,799.1474380493164,0.07028908407869494
662663,662664,662663,1325327,801.8214793205261,0.06910337842396075
664665,664666,664665,1329331,804.3427422046661,0.067937981082423
666667,666668,666667,1333335,806.8578443527222,0.06679253661275197
668669,668670,668669,1337339,809.4228341579437,0.06566669598430508
670671,670672,670671,1341343,812.0417683124542,0.0645601164552545
672673,672674,672673,1345347,814.5414440631866,0.06347246145548979
674675,674676,674675,1349351,817.1821472644806,0.062403400471907844
676677,676678,676677,1353355,820.3440570831299,0.06135260893336181
678679,678680,678679,1357359,823.3435320854187,0.06031976810118067
680681,680682,680681,1361363,826.2980041503906,0.05930456495877934
682683,682684,682683,1365367,828.6375453472137,0.05830669210627093
684685,684686,684685,1369371,830.7203822135925,0.05732584765507909
686687,686688,686687,1373375,833.3922669887543,0.056361735124937695
688689,688690,688689,1377379,835.4090461730957,0.0554140633444149
690691,690692,690691,1381383,837.4944021701813,0.05448254635109606
692693,692694,692693,1385387,839.5661292076111,0.05356690329529101
694695,694696,694695,1389391,841.6200520992279,0.05266685834578766
696697,696698,696697,1393395,843.7994561195374,0.05178214059549191
698699,698700,698699,1397399,846.2595620155334,0.05091248397150139
700701,700702,700701,1401403,848.6687111854553,0.05005762714506545
702703,702704,702703,1405407,851.0102090835571,0.04921731344404634
704705,704706,704705,1409411,853.9002282619476,0.048391290766630846
706707,706708,706707,1413415,856.34543633461,0.047579311497429444
708709,708710,708709,1417419,858.4698503017426,0.04678113242493964
710711,710712,710711,1421423,860.6417682170868,0.04599651465946408
712713,712714,712713,1425427,862.8127369880676,0.04522522355409819
714715,714716,714715,1429431,865.1115162372589,0.04446702862765051
716717,716718,716717,1433435,867.3141303062439,0.043721703485971375
718719,718720,718719,1437439,869.6073253154755,0.04298902574953445
720721,720722,720721,1441443,871.776397228241,0.042268776977380185
722723,722724,722723,1445447,873.9626302719116,0.04156074259697107
724725,724726,724725,1449451,876.3805413246155,0.04086471183154572
726727,726728,726727,1453455,878.7173912525177,0.04018047763224786
728729,728730,728729,1457459,880.9949362277985,0.039507836608777325
730731,730732,730731,1461463,883.4875221252441,0.03884658896311066
732733,732734,732733,1465467,885.65052318573,0.038196538424585924
734735,734736,734735,1469471,887.8222773075104,0.03755749218419169
736737,736738,736737,1473475,890.2340512275696,0.03692926083215298
738739,738740,738739,1477479,892.4953742027283,0.03631165829699512
740741,740742,740741,1481483,894.7116811275482,0.03570450178256124
742743,742744,742743,1485487,896.9493532180786,0.03510761171105514
744745,744746,744745,1489491,899.181948184967,0.034520811662559936
746747,746748,746747,1493495,901.3989591598511,0.03394392831876303
748749,748750,748749,1497499,903.6443240642548,0.033376791406908524
750751,750752,750751,1501503,905.8149690628052,0.032819233643635926
752753,752754,752753,1505507,908.0367460250854,0.032271090681433634
754755,754756,754755,1509511,910.2208092212677,0.03173220105577457
756757,756758,756757,1513515,912.3933770656586,0.031202406132479155
758759,758760,758759,1517519,914.6077451705933,0.03068155005666995
760761,760762,760761,1521523,916.810967206955,0.030169479702976787
762763,762764,762763,1525527,919.0261042118073,0.029666044626424082
764765,764766,764765,1529531,921.2735261917114,0.029171097012522296
766767,766768,766767,1533535,923.4243183135986,0.028684491632589015
768769,768770,768769,1537539,925.6588962078094,0.028206085794408864
770771,770772,770771,1541543,927.8599412441254,0.02773573929880513
772773,772774,772773,1545547,930.0389680862427,0.02727331439371028
774775,774776,774775,1549551,932.312016248703,0.026818675730282848
776777,776778,776777,1553555,934.5373811721802,0.02637169032004749
778779,778780,778779,1557559,936.9308431148529,0.025932227492262427
780781,780782,780781,1561563,939.4397151470184,0.02550015885310586
782783,782784,782783,1565567,941.9095861911774,0.025075358243611845
784785,784786,784785,1569571,944.181624174118,0.024657701700789403
786787,786788,786787,1573575,946.4922091960907,0.024247067418173174
788789,788790,788789,1577579,948.7797422409058,0.023843335706487778
790791,790792,790791,1581583,951.0021071434021,0.02344638895715434
792793,792794,792793,1585587,953.3278300762177,0.023056111603864338
794795,794796,794795,1589591,955.7221081256866,0.022672390086540872
796797,796798,796797,1593595,958.0103240013123,0.022295112816095752
798799,798800,798799,1597599,960.3419110774994,0.021924170138959198
800801,800802,800801,1601603,962.6621050834656,0.021559454302177983
802803,802804,802803,1605607,964.7439570426941,0.02120085942044625
804805,804806,804805,1609611,966.9230542182922,0.020848281442567895
806807,806808,806807,1613615,969.0820751190186,0.02050161811803264
808809,808810,808809,1617619,971.2629392147064,0.02016076896643426
810811,810812,810811,1621623,973.5199680328369,0.01982563524506986
812813,812814,812813,1625627,975.8457911014557,0.019496119918812838
814815,814816,814815,1629631,978.0582630634308,0.019172127628735325
816817,816818,816817,1633635,980.1374151706696,0.01885356466414123
818819,818820,818819,1637639,982.2050533294678,0.01854033893164342
820821,820822,820821,1641643,984.4058282375336,0.0182323599275378
822823,822824,822823,1645647,986.9726850986481,0.01792953870949532
824825,824826,824825,1649651,989.2169153690338,0.01763178786904973
826827,826828,826827,1653655,991.307920217514,0.01733902150385802
828829,828830,828829,1657659,993.3736340999603,0.017051155192234546
830831,830832,830831,1661663,995.4372711181641,0.016768105966320945
832833,832834,832833,1665667,997.5036661624908,0.0164897922865066
834835,834836,834835,1669671,999.7129981517792,0.016216134016190153
836837,836838,836837,1673675,1001.7721991539001,0.015947052397336847
838839,838840,838839,1677679,1003.8407971858978,0.01568247002649059
840841,840842,840841,1681683,1005.9057061672211,0.015422310829649177
842843,842844,842843,1685687,1007.9787933826447,0.015166500040663777
844845,844846,844845,1689691,1010.0902872085571,0.014914964177023649
846847,846848,846847,1693695,1012.1309843063354,0.014667631017573513
848849,848850,848849,1697699,1014.1973650455475,0.01442442958079937
850851,850852,850851,1701703,1016.2897479534149,0.014185290102773251
852853,852854,852853,1705707,1018.349362373352,0.013950144015211663
854855,854856,854855,1709711,1020.8120741844177,0.013718923925921445
856857,856858,856857,1713715,1023.3971762657166,0.013491563596744527
858859,858860,858859,1717719,1025.875479221344,0.013267997924685915
860861,860862,860861,1721723,1028.5172500610352,0.013048162920426876
862863,862864,862863,1725727,1030.7523062229156,0.012831995690930853
864865,864866,864865,1729731,1032.9841811656952,0.012619434418297715
866867,866868,866867,1733735,1035.5241332054138,0.01241041834225598
868869,868870,868869,1737739,1037.9363882541656,0.01220488774106343
870871,870872,870871,1741743,1040.1812751293182,0.012002783914113024
872873,872874,872873,1745747,1043.2113621234894,0.01180404916271982
874875,874876,874875,1749751,1045.4340121746063,0.011608626774545883
876877,876878,876877,1753755,1047.4888801574707,0.011416461004614575
878879,878880,878879,1757759,1049.5528151988983,0.011227497059962843
880881,880882,880881,1761763,1052.1607780456543,0.011041681081906063
882883,882884,882883,1765767,1054.5190091133118,0.01085896013034926
884885,884886,884885,1769771,1057.3569102287292,0.010679282167870952
886887,886888,886887,1773775,1060.3795990943909,0.010502596043693302
888889,888890,888889,1777779,1062.6061980724335,0.010328851478902834
890891,890892,890891,1781783,1064.8008980751038,0.010157999050420585
892893,892894,892893,1785787,1066.9623851776123,0.009989990176791252
894895,894896,894895,1789791,1069.194337129593,0.009824777103290216
896897,896898,896897,1793795,1071.320400238037,0.009662312887940061
898899,898900,898899,1797799,1074.5202431678772,0.009502551386958658
900901,900902,900901,1801803,1076.8162531852722,0.009345447241116744
902903,902904,902903,1805807,1078.9454782009125,0.009190955862891315
904905,904906,904905,1809811,1081.0598289966583,0.009039033421345266
906907,906908,906907,1813815,1083.205830335617,0.008889636830645031
908909,908910,908909,1817819,1085.3578102588654,0.008742723736872904
910911,910912,910911,1821823,1087.425302028656,0.008598252504498305
912913,912914,912913,1825827,1089.709635257721,0.00845618220535016
914915,914916,914915,1829831,1091.8833441734314,0.008316472604974479
916917,916918,916917,1833835,1093.985100030899,0.00817908415194779
918919,918920,918919,1837839,1096.156655073166,0.008043977965030535
920921,920922,920921,1841843,1098.3118541240692,0.007911115822253123
922923,922924,922923,1845847,1100.4050223827362,0.007780460149319879
924925,924926,924925,1849851,1102.5804522037506,0.007651974008467732
926927,926928,926927,1853855,1104.7086441516876,0.007525621087552281
928929,928930,928929,1857859,1106.8215301036835,0.007401365689361228
930931,930932,930931,1861863,1108.8905100822449,0.007279172720586757
932933,932934,932933,1865867,1111.0044343471527,0.007159007682048468
934935,934936,934935,1869871,1113.104165315628,0.007040836658120497
936937,936938,936937,1873875,1115.2054042816162,0.006924626306840764
938939,938940,938939,1877879,1117.3523173332214,0.006810343849451783
940941,940942,940941,1881883,1119.4862871170044,0.006697957062328896
942943,942944,942943,1885887,1122.300695180893,0.006587434265043157
944945,944946,944945,1889891,1124.9055652618408,0.006478744313653806
946947,946948,946947,1893895,1127.6622033119202,0.006371856588998526
948949,948950,948949,1897899,1130.0714161396027,0.006266740989872233
950951,950952,950951,1901903,1132.9171230793,0.006163367922908947
952953,952954,952953,1905907,1135.6849291324615,0.0060617082938279054
954955,954956,954955,1909911,1138.36883020401,0.005961733499361799
956957,956958,956957,1913915,1140.9703443050385,0.00586341541929869
958959,958960,958959,1917919,1143.2789902687073,0.0057667264065912605
960961,960962,960961,1921923,1145.3919820785522,0.005671639280990348
962963,962964,962963,1925927,1147.5318593978882,0.0055781273197226255
964965,964966,964965,1929931,1150.1412091255188,0.005486164251465198
966967,966968,966967,1933935,1152.7992181777954,0.005395724245886413
968969,968970,968969,1937939,1155.3255171775818,0.005306781908871017
970971,970972,970971,1941943,1158.0445861816406,0.0052193122736525766
972973,972974,972973,1945947,1160.6136093139648,0.0051332907931964655
974975,974976,974975,1949951,1163.0657563209534,0.005048693334288146
976977,976978,976977,1953955,1165.7702062129974,0.004965496169006656
978979,978980,978979,1957959,1168.531524181366,0.004883675969267642
980981,980982,980981,1961963,1170.8666710853577,0.004803209798978969
982983,982984,982983,1965967,1173.1699299812317,0.004724075107674253
984985,984986,984985,1969971,1175.5082013607025,0.004646249723919027
986987,986988,986987,1973975,1177.7851531505585,0.004569711849285341
988989,988990,988989,1977979,1180.2882571220398,0.004494440050734738
990991,990992,990991,1981983,1182.9855341911316,0.004420413256411848
992993,992994,992993,1985987,1185.261782169342,0.0043476107470041825
994995,994996,994995,1989991,1187.6047410964966,0.004276012152445219
996997,996998,996997,1993995,1189.9512152671814,0.004205597443615261
998999,999000,998999,1997999,1192.3411672115326,0.004136346928135026
1001001,1001002,1001001,2002003,1194.8167781829834,0.004068241243658122
1003003,1003004,1003003,2006007,1197.1719810962677,0.0040012613528688235
1005005,1005006,1005005,2010011,1199.3794782161713,0.003935388537684048
1007007,1007008,1007007,2014015,1201.614478111267,0.0038706043940237578
1009009,1009010,1009009,2018019,1204.2271931171417,0.0038068908263539925
1011011,1011012,1011011,2022023,1206.2877871990204,0.003744230041888841
1013013,1013014,1013013,2026027,1208.5749261379242,0.003682604546725088
1015015,1015016,1015015,2030031,1210.9348783493042,0.0036219971400441864
1017017,1017018,1017017,2034035,1213.1880640983582,0.0035623909087689754
1019019,1019020,1019019,2038039,1215.3308563232422,0.0035037692230162065
1021021,1021022,1021021,2042043,1218.1480913162231,0.0034461157320038183
1023023,1023024,1023023,2046047,1220.1748132705688,0.0033894143579118463
1025025,1025026,1025025,2050051,1222.2618401050568,0.0033336492924718186
1027027,1027028,1027027,2054055,1224.407692193985,0.003278804991623474
1029029,1029030,1029029,2058059,1226.4741320610046,0.003224866172331531
1031031,1031032,1031031,2062063,1228.535471200943,0.00317181780599185
1033033,1033034,1033033,2066067,1230.6524722576141,0.0031196451154755778
1035035,1035036,1035035,2070071,1232.9386551380157,0.0030683335721732874
1037037,1037038,1037037,2074075,1235.1354501247406,0.0030178688883779614
1039039,1039040,1039039,2078079,1237.4506721496582,0.0029682370167165573
1041041,1041042,1041041,2082083,1239.6317381858826,0.0029194241435561707
1043043,1043044,1043043,2086087,1241.9600751399994,0.0028714166871850466
1045045,1045046,1045045,2090091,1244.5244841575623,0.0028242012916734893
1047047,1047048,1047047,2094095,1246.732135295868,0.0027777648246001263
1049049,1049050,1049049,2098099,1249.560039281845,0.002732094373413929
1051051,1051052,1051051,2102103,1251.9772911071777,0.0026871772399772453
1053053,1053054,1053053,2106107,1254.0928401947021,0.00264300093942893
1055055,1055056,1055055,2110111,1257.0956852436066,0.002599553194386317
1057057,1057058,1057057,2114115,1259.423079252243,0.0025568219325577957
1059059,1059060,1059059,2118119,1261.4677441120148,0.002514795283445892
1061061,1061062,1061061,2122123,1263.5260400772095,0.0024734615739134824
1063063,1063064,1063063,2126127,1265.5768942832947,0.002432809326478491
1065065,1065066,1065065,2130131,1267.6188271045685,0.0023928272539706086
1067067,1067068,1067067,2134135,1269.6467893123627,0.0023535042582807364
1069069,1069070,1069069,2138139,1271.7201263904572,0.0023148294260408875
1071071,1071072,1071071,2142143,1273.7711281776428,0.0022767920256683283
1073073,1073074,1073073,2146147,1275.9714543819427,0.002239381504409721
1075075,1075076,1075075,2150151,1278.037364244461,0.002202587485726326
1077077,1077078,1077077,2154155,1280.0908341407776,0.0021663997652012768
1079079,1079080,1079079,2158159,1283.5019991397858,0.002130808309289023
1081081,1081082,1081081,2162163,1285.7625510692596,0.0020958032511089186
1083083,1083084,1083083,2166167,1287.9974081516266,0.002061374887716738
1085085,1085086,1085085,2170171,1290.2491693496704,0.0020275136788541204
1087087,1087088,1087087,2174175,1292.4980311393738,0.001994210241946348
1089089,1089090,1089089,2178179,1294.7663700580597,0.0019614553509654797
1091091,1091092,1091091,2182183,1296.9687941074371,0.0019292399335881782
1093093,1093094,1093093,2186187,1299.1187472343445,0.0018975550681261666
1095095,1095096,1095095,2190191,1301.319542169571,0.001866391981934612
1097097,1097098,1097097,2194195,1303.7209441661835,0.0018357420473193997
1099099,1099100,1099099,2198199,1305.9268951416016,0.001805596780968699
1101101,1101102,1101101,2202203,1308.1688861846924,0.0017759478403149842
1103103,1103104,1103103,2206207,1310.4853880405426,0.0017467870217160453
1105105,1105106,1105105,2210211,1312.546067237854,0.0017181062573854433
1107107,1107108,1107107,2214215,1314.457887172699,0.001689897613687208
1109109,1109110,1109109,2218219,1316.3134751319885,0.001662153289885282
1111111,1111112,1111111,2222223,1318.1481909751892,0.0016348656134823614
1113113,1113114,1113113,2226227,1320.0358493328094,0.0016080270404472685
1115115,1115116,1115115,2230231,1322.2218461036682,0.0015816301516906606
1117117,1117118,1117117,2234235,1324.1415350437164,0.00155566765124604
1119119,1119120,1119119,2238239,1326.231944322586,0.0015301323646781384
1121121,1121122,1121121,2242243,1328.4589731693268,0.0015050172361270597
1123123,1123124,1123123,2246247,1330.8714501857758,0.0014803153276261583
1125125,1125126,1125125,2250251,1333.3365733623505,0.0014560198160324944
1127127,1127128,1127127,2254255,1335.7756612300873,0.0014321239910941586
1129129,1129130,1129129,2258259,1338.1173272132874,0.0014086212547681498
1131131,1131132,1131131,2262263,1340.5541491508484,0.0013855051174687105
1133133,1133134,1133133,2266267,1343.1789700984955,0.0013627691982946999
1135135,1135136,1135135,2270271,1345.793743133545,0.0013404072216189888
1137137,1137138,1137137,2274275,1348.1536660194397,0.0013184130160652785
1139139,1139140,1139139,2278279,1350.5362989902496,0.0012967805128027976
1141141,1141142,1141141,2282283,1353.0203230381012,0.001275503743045192
1143143,1143144,1143143,2286287,1355.7530512809753,0.0012545768379368383
1145145,1145146,1145145,2290291,1358.4144022464752,0.0012339940251422377
1147147,1147148,1147147,2294295,1361.3713910579681,0.0012137496283912697
1149149,1149150,1149149,2298299,1364.0423061847687,0.0011938380654328284
1151151,1151152,1151151,2302303,1366.824567079544,0.0011742538463295205
1153153,1153154,1153153,2306307,1369.5287051200867,0.0011549915724344828
1155155,1155156,1155155,2310311,1372.0178802013397,0.0011360459343450202
1157157,1157158,1157157,2314315,1374.3111772537231,0.0011174117111067972
1159159,1159160,1159159,2318319,1376.4112980365753,0.001099083767371667
1161161,1161162,1161161,2322323,1378.56765127182,0.001081057053738732
1163163,1163164,1163163,2326327,1380.7185153961182,0.0010633266039121736
1165165,1165166,1165165,2330331,1383.2383670806885,0.0010458875341328167
1167167,1167168,1167167,2334335,1385.8589360713959,0.0010287350413591412
1169169,1169170,1169169,2338339,1389.0954780578613,0.001011864401789353
1171171,1171172,1171171,2342343,1391.472924232483,0.0009952709705203233
1173173,1173174,1173173,2346347,1393.9734163284302,0.0009789501791601651
1175175,1175176,1175175,2350351,1396.4904992580414,0.000962897534577678
1177177,1177178,1177177,2354355,1398.9983921051025,0.0009471086187886613
1179179,1179180,1179179,2358359,1401.0524551868439,0.0009315790860000561
1181181,1181182,1181181,2362363,1402.9503972530365,0.0009163046635194405
1183183,1183184,1183183,2366367,1404.8616650104523,0.0009012811478896765
1185185,1185186,1185185,2370371,1406.7294611930847,0.0008865044065942129
1187187,1187188,1187187,2374375,1408.5671360492706,0.0008719703744191065
1189189,1189190,1189189,2378379,1410.370450258255,0.0008576750537940825
1191191,1191192,1191191,2382383,1412.1848492622375,0.0008436145135419792
1193193,1193194,1193193,2386387,1414.0001673698425,0.0008297848870597591
1195195,1195196,1195195,2390391,1415.8314633369446,0.0008161823717500738
1197197,1197198,1197197,2394395,1417.7210323810577,0.0008028032279980835
1199199,1199200,1199199,2398399,1419.5677301883698,0.0007896437782619614
1201201,1201202,1201201,2402403,1421.4268610477448,0.000776700405253905
1203203,1203204,1203203,2406407,1423.182498216629,0.0007639695514853884
1205205,1205206,1205205,2410411,1424.988319158554,0.0007514477191534752
1207207,1207208,1207207,2414415,1426.8349282741547,0.0007391314670712745
1209209,1209210,1209209,2418419,1428.7253832817078,0.0007270174114637484
1211211,1211212,1211211,2422423,1431.5391612052917,0.0007151022247171568
1213213,1213214,1213213,2426427,1433.33420920372,0.0007033826340148153
1215215,1215216,1215215,2430431,1435.0761482715607,0.0006918554200865401
1217217,1217218,1217217,2434435,1437.0924081802368,0.0006805174175497086
1219219,1219220,1219219,2438439,1438.9062063694,0.0006693655128628961
1221221,1221222,1221221,2442443,1441.0520651340485,0.0006583966442121891
1223223,1223224,1223223,2446447,1443.9855360984802,0.00064760780026063
1225225,1225226,1225225,2450451,1446.757259130478,0.000636996018897662
1227227,1227228,1227227,2454455,1448.8933081626892,0.0006265583876938763
1229229,1229230,1229229,2458459,1450.9510452747345,0.000616292041968336
1231231,1231232,1231231,2462463,1453.0181312561035,0.0006061941639927682
1233233,1233234,1233233,2466467,1455.055857181549,0.0005962619831052507
1235235,1235236,1235235,2470471,1457.0987341403961,0.0005864927740049097
1237237,1237238,1237237,2474475,1459.1687133312225,0.000576883856524546
1239239,1239240,1239239,2478479,1461.2784292697906,0.00056743259472114
1241241,1241242,1241241,2482483,1463.709720134735,0.0005581363960800445
1243243,1243244,1243243,2486487,1466.3196983337402,0.0005489927107191761
1245245,1245246,1245245,2490491,1469.0143122673035,0.000539999031161642
1247247,1247248,1247247,2494495,1471.172743320465,0.0005311528911988717
1249249,1249250,1249249,2498499,1473.6917560100555,0.0005224518650948085
1251251,1251252,1251251,2502503,1476.0801901817322,0.0005138935671311629
1253253,1253254,1253253,2506507,1478.391636133194,0.0005054756514937253
1255255,1255256,1255255,2510511,1480.4885032176971,0.0004971958099986296
1257257,1257258,1257257,2514515,1482.5204751491547,0.0004890517735702815
1259259,1259260,1259259,2518519,1484.550014257431,0.00048104130974024883
1261261,1261262,1261261,2522523,1486.5887641906738,0.00047316222389781615
1263263,1263264,1263263,2526527,1488.6121771335602,0.0004654123562204404
1265265,1265266,1265265,2530531,1490.602679014206,0.0004577895833790535
1267267,1267268,1267267,2534535,1492.5633862018585,0.00045029181717382016
1269269,1269270,1269269,2538539,1494.4360961914062,0.00044291700305620907
1271271,1271272,1271271,2542543,1496.579166173935,0.0004356631211521744
1273273,1273274,1273273,2546547,1499.0668642520905,0.0004285281843294797
1275275,1275276,1275275,2550551,1501.3359291553497,0.0004215102384250713
1277277,1277278,1277277,2554555,1503.6643161773682,0.0004146073614492707
1279279,1279280,1279279,2558559,1505.98495221138,0.0004078176632447139
1281281,1281282,1281281,2562563,1508.0931651592255,0.00040113928412210953
1283283,1283284,1283283,2566567,1510.6822972297668,0.00039457039599710697
1285285,1285286,1285285,2570571,1512.6912531852722,0.0003881092003439335
1287287,1287288,1287287,2574575,1514.6833033561707,0.00038175392830908095
1289289,1289290,1289289,2578579,1516.77956032753,0.0003755028400291849
1291291,1291292,1291291,2582583,1518.998693227768,0.00036935422451733757
1293293,1293294,1293293,2586587,1521.344279050827,0.0003633063988672802
1295295,1295296,1295295,2590591,1523.7385931015015,0.0003573577083670898
1297297,1297298,1297297,2594595,1525.587776184082,0.0003515065246801896
1299299,1299300,1299299,2598599,1527.5868201255798,0.0003457512466411572
1301301,1301302,1301301,2602603,1529.7176892757416,0.0003400902999146638
1303303,1303304,1303303,2606607,1531.7785782814026,0.0003345221351764849
1305305,1305306,1305305,2610611,1533.7900080680847,0.0003290452298188029
1307307,1307308,1307307,2614615,1535.7973229885101,0.00032365808499434934
1309309,1309310,1309309,2618619,1537.941004037857,0.00031835922720802046
1311311,1311312,1311311,2622623,1540.691546201706,0.00031314720729369583
1313313,1313314,1313313,2626627,1543.1299781799316,0.0003080205996184304
1315315,1315316,1315315,2630631,1545.335966348648,0.00030297800242351514
1317317,1317318,1317317,2634635,1547.9879002571106,0.0002980180364602347
1319319,1319320,1319319,2638639,1550.8601961135864,0.000293139345558302
1321321,1321322,1321321,2642643,1553.1318871974945,0.00028834059583005
1323323,1323324,1323323,2646647,1555.2193472385406,0.0002836204753293714
1325325,1325326,1325325,2650651,1557.2101881504059,0.0002789776935969712
1327327,1327328,1327327,2654655,1559.1453292369843,0.00027441098143299314
1329329,1329330,1329329,2658659,1561.9806201457977,0.000269919090555959
1331331,1331332,1331331,2662663,1564.384889125824,0.00026550079292064765
1333333,1333334,1333333,2666667,1566.757558107376,0.0002611548812865294
1335335,1335336,1335335,2670671,1568.8532102108002,0.00025688016785352374
1337337,1337338,1337337,2674675,1570.9877932071686,0.00025267548414831253
1339339,1339340,1339339,2678679,1573.35000705719,0.00024853968147908745
1341341,1341342,1341341,2682683,1576.0137991905212,0.0002444716300260552
1343343,1343344,1343343,2686687,1578.1671812534332,0.00024047021770456922
1345345,1345346,1345345,2690691,1580.3447680473328,0.00023653435152937163
1347347,1347348,1347347,2694695,1582.5681700706482,0.00023266295647772495
1349349,1349350,1349349,2698699,1585.2064383029938,0.0002288549744662305
1351351,1351352,1351351,2702703,1587.750158071518,0.00022510936571507045
1353353,1353354,1353353,2706707,1591.2707200050354,0.0002214251069290185
1355355,1355356,1355355,2710711,1594.3498821258545,0.00021780119197956083
1357357,1357358,1357357,2714715,1596.867522239685,0.00021423663099540136
1359359,1359360,1359359,2718719,1599.4958522319794,0.0002107304504761487
1361361,1361362,1361361,2722723,1601.9854242801666,0.00020728169329231605
1363363,1363364,1363363,2726727,1604.5351402759552,0.0002038894172073924
1365365,1365366,1365365,2730731,1607.1892552375793,0.00020055269612839766
1367367,1367368,1367367,2734735,1609.920359134674,0.00019727061942376167
1369369,1369370,1369369,2738739,1612.6001372337341,0.0001940422903317085
1371371,1371372,1371371,2742743,1615.296625137329,0.0001908668281203063
1373373,1373374,1373373,2746747,1619.2620830535889,0.00018774336547267012
1375375,1375376,1375375,2750751,1622.8189301490784,0.00018467105007857754
1377377,1377378,1377377,2754755,1626.7747201919556,0.00018164904315653985
1379379,1379380,1379379,2758759,1630.5735251903534,0.0001786765196811757
1381381,1381382,1381381,2762763,1634.1573061943054,0.00017575266895164532
1383383,1383384,1383383,2766767,1637.7038731575012,0.0001728766923179137
1385385,1385386,1385385,2770771,1641.2598819732666,0.0001700478054544874
1387387,1387388,1387387,2774775,1644.0515441894531,0.00016726523608667776
1389389,1389390,1389389,2778779,1645.939462184906,0.00016452822512746934
1391391,1391392,1391391,2782783,1647.8761520385742,0.00016183602542696462
1393393,1393394,1393393,2786787,1650.0838191509247,0.00015918790256819193
1395395,1395396,1395395,2790791,1652.4033341407776,0.00015658313418498437
1397397,1397398,1397397,2794795,1654.5120272636414,0.00015402100996197987
1399399,1399400,1399399,2798799,1656.922348022461,0.00015150083015669225
1401401,1401402,1401401,2802803,1659.7955520153046,0.00014902190787324798
1403403,1403404,1403403,2806807,1662.2319161891937,0.00014658356667496264
1405405,1405406,1405405,2810811,1664.49463224411,0.00014418514149383554
1407407,1407408,1407407,2814815,1666.3423421382904,0.00014182597840317612
1409409,1409410,1409409,2818819,1668.240555047989,0.00013950543359442236
1411411,1411412,1411411,2822823,1670.2248282432556,0.0001372228742866355
1413413,1413414,1413413,2826827,1672.1851062774658,0.00013497767815806583
1415415,1415416,1415415,2830831,1674.3281302452087,0.00013276923266403173
1417417,1417418,1417417,2834835,1676.1695411205292,0.00013059693617378798
1419419,1419420,1419419,2838839,1678.172904253006,0.00012846019558310218
1421421,1421422,1421421,2842843,1680.1632702350616,0.00012635842892905202
1423423,1423424,1423423,2846847,1682.0626561641693,0.00012429106266154122
1425425,1425426,1425425,2850851,1684.0048162937164,0.000122257533348602
1427427,1427428,1427427,2854855,1686.0637822151184,0.00012025728665321367
1429429,1429430,1429429,2858859,1687.9987063407898,0.00011828977721961564
1431431,1431432,1431431,2862863,1689.8602900505066,0.0001163544687869944
1433433,1433434,1433433,2866867,1691.7059090137482,0.00011445083373473608
1435435,1435436,1435435,2870871,1693.5749843120575,0.00011257835296873964
1437437,1437438,1437437,2874875,1695.4759922027588,0.00011073651637616422
1439439,1439440,1439439,2878879,1697.3360812664032,0.0001089248218022476
1441441,1441442,1441441,2882883,1699.214765071869,0.00010714277573242725
1443443,1443444,1443443,2886887,1701.1033961772919,0.0001053898921554719
1445445,1445446,1445445,2890891,1702.9999392032623,0.00010366569358666311
1447447,1447448,1447447,2894895,1704.9969279766083,0.00010196970993092691
1449449,1449450,1449449,2898899,1706.9692060947418,0.00010030147939232847
1451451,1451452,1451451,2902903,1708.9324610233307,9.866054710983008e-05
1453453,1453454,1453453,2906907,1710.7838802337646,9.70464660667858e-05
1455455,1455456,1455455,2910911,1712.6189119815826,9.545879640882049e-05
1457457,1457458,1457457,2914915,1714.462384223938,9.389710567120346e-05
1459459,1459460,1459459,2918919,1716.3520221710205,9.236096832410112e-05
1461461,1461462,1461461,2922923,1718.307018995285,9.084996577257698e-05
1463463,1463464,1463463,2926927,1720.2584981918335,8.936368647027848e-05
1465465,1465466,1465465,2930931,1722.2293412685394,8.79017255783765e-05
1467467,1467468,1467467,2934935,1724.1674642562866,8.64636848518785e-05
1469469,1469470,1469469,2938939,1726.068528175354,8.504917229856801e-05
1471471,1471472,1471471,2942943,1727.9444222450256,8.365780286112567e-05
1473473,1473474,1473473,2946947,1729.7966830730438,8.22891977350082e-05
1475475,1475476,1475475,2950951,1731.6467621326447,8.094298380001419e-05
1477477,1477478,1477477,2954955,1733.5285003185272,7.961879441609199e-05
1479479,1479480,1479479,2958959,1735.416570186615,7.831626942333969e-05
1481481,1481482,1481481,2962963,1737.3814573287964,7.70350537777631e-05
1483483,1483484,1483483,2966967,1739.332602262497,7.577479823339672e-05
1485485,1485486,1485485,2970971,1741.2400772571564,7.453516013811168e-05
1487487,1487488,1487487,2974975,1743.1468060016632,7.331580172831309e-05
1489489,1489490,1489489,2978979,1745.074909210205,7.211639081106114e-05
1491491,1491492,1491491,2982983,1746.9580841064453,7.093660099144472e-05
1493493,1493494,1493493,2986987,1748.774500131607,6.977611099046044e-05
1495495,1495496,1495495,2990991,1750.6107711791992,6.863460487238626e-05
1497497,1497498,1497497,2994995,1752.4298181533813,6.751177181740786e-05
1499499,1499500,1499499,2998999,1754.36927318573,6.640730589424493e-05
1501502,1501503,1501502,3003005,1756.2052080631256,6.53203687761561e-05
1503504,1503505,1503504,3007009,1758.025547027588,6.42517492224215e-05
1505506,1505507,1505506,3011013,1759.8068630695343,6.320060958842078e-05
1507508,1507509,1507508,3015017,1761.6572012901306,6.216666383807024e-05
1509510,1509511,1509510,3019021,1763.49964427948,6.1149630255386e-05
1511512,1511513,1511512,3023025,1765.3991022109985,6.014923212660506e-05
1513514,1513515,1513514,3027029,1767.2704641819,5.916519705806422e-05
1515516,1515517,1515516,3031033,1769.1513800621033,5.8197257317260664e-05
1517518,1517519,1517518,3035037,1771.0321111679077,5.724514937810454e-05
1519520,1519521,1519520,3039041,1772.9127123355865,5.630861403460585e-05
1521522,1521523,1521522,3043045,1774.7639203071594,5.5387396741934936e-05
1523524,1523525,1523524,3047049,1776.6182851791382,5.44812464795541e-05
1525526,1525527,1525526,3051053,1778.4508574008942,5.3589916547025496e-05
1527528,1527529,1527528,3055057,1780.5595331192017,5.2713164564011095e-05
1529530,1529531,1529530,3059061,1783.0683462619781,5.1850752129212196e-05
1531532,1531533,1531532,3063065,1785.6638813018799,5.100244391087472e-05
1533534,1533535,1533534,3067069,1787.9977202415466,5.016800992052595e-05
1535536,1535537,1535536,3071073,1790.135362148285,4.934722244342993e-05
1537538,1537539,1537538,3075077,1792.306223154068,4.853985842601105e-05
1539540,1539541,1539540,3079081,1794.458999156952,4.7745698338985676e-05
1541542,1541543,1541542,3083085,1796.509369134903,4.696452583630162e-05
1543544,1543545,1543544,3087089,1798.5196900367737,4.619612832357234e-05
1545546,1545547,1545546,3091093,1800.432097196579,4.544029707176378e-05
1547548,1547549,1547548,3095097,1802.333036184311,4.469682619401283e-05
1549550,1549551,1549550,3099101,1804.1762759685516,4.396551344143518e-05
1551552,1551553,1551552,3103105,1806.250158071518,4.3246159862064815e-05
1553554,1553555,1553554,3107109,1808.2610869407654,4.2538570028227696e-05
1555556,1555557,1555556,3111113,1810.1434559822083,4.1842551127047045e-05
1557558,1557559,1557558,3115117,1812.0528650283813,4.1157913983624894e-05
1559560,1559561,1559560,3119121,1813.8898780345917,4.048447203786054e-05
1561562,1561563,1561562,3123125,1815.7001264095306,3.982204259500577e-05
1563564,1563565,1563564,3127129,1817.8334941864014,3.917044546142279e-05
1565566,1565567,1565566,3131133,1820.2495889663696,3.852950294458424e-05
1567568,1567569,1567568,3135137,1822.6455261707306,3.789904098994157e-05
1569570,1569571,1569570,3139141,1824.8130853176117,3.7278888157743495e-05
1571572,1571573,1571572,3143145,1826.9305651187897,3.666887573672284e-05
1573574,1573575,1573574,3147149,1829.1158912181854,3.60688379714702e-05
1575576,1575577,1575576,3151153,1831.3170051574707,3.54786112666261e-05
1577578,1577579,1577578,3155157,1833.4672372341156,3.489803555112303e-05
1579580,1579581,1579580,3159161,1835.5658881664276,3.432695268656971e-05
1581582,1581583,1581582,3163165,1837.8032031059265,3.376520726305898e-05
1583584,1583585,1583584,3167169,1839.5869660377502,3.321264682654146e-05
1585586,1585587,1585586,3171173,1841.5174372196198,3.2669120855643996e-05
1587588,1587589,1587588,3175177,1843.5516772270203,3.213448178485123e-05
1589590,1589591,1589590,3179181,1845.6037240028381,3.1608583981324045e-05
1591592,1591593,1591592,3183185,1847.5273311138153,3.109128465439426e-05
1593594,1593595,1593594,3187189,1849.4603261947632,3.058244317344361e-05
1595596,1595597,1595596,3191193,1851.3735632896423,3.0081920954216912e-05
1597598,1597599,1597598,3195197,1853.3133962154388,2.9589581913569418e-05
1599600,1599601,1599600,3199201,1855.1879251003265,2.910529258315364e-05
1601602,1601603,1601602,3203205,1857.0550022125244,2.8628921086237824e-05
1603604,1603605,1603604,3207209,1858.899146080017,2.816033747876645e-05
1605606,1605607,1605606,3211213,1860.7347021102905,2.769941499991546e-05
1607608,1607609,1607608,3215217,1862.614827156067,2.7246027912042337e-05
1609610,1609611,1609610,3219221,1864.4746260643005,2.6800053092301823e-05
1611612,1611613,1611612,3223225,1866.3795471191406,2.6361369464211748e-05
1613614,1613615,1613614,3227229,1868.2723541259766,2.5929857656592503e-05
1615616,1615617,1615616,3231233,1870.2301633358002,2.5505400117253885e-05
1617618,1617619,1617618,3235237,1872.1608309745789,2.5087881795116118e-05
1619620,1619621,1619620,3239241,1874.017753124237,2.467718911702832e-05
1621622,1621623,1621622,3243245,1875.8831181526184,2.427321032882901e-05
1623624,1623625,1623624,3247249,1877.8915841579437,2.3875835836406623e-05
1625626,1625627,1625626,3251253,1879.7247092723846,2.348495729620481e-05
1627628,1627629,1627628,3255257,1881.5668280124664,2.3100468865777657e-05
1629630,1629631,1629630,3259261,1883.3421161174774,2.2722265612173942e-05
1631632,1631633,1631632,3263265,1885.1131629943848,2.235024498986604e-05
1633634,1633635,1633634,3267269,1886.908818244934,2.198430593125522e-05
1635636,1635637,1635636,3271273,1888.739580154419,2.1624348846671637e-05
1637638,1637639,1637638,3275277,1890.5690932273865,2.127027596543485e-05
1639640,1639641,1639640,3279281,1892.350063085556,2.0921991108480142e-05
1641642,1641643,1641642,3283285,1894.0895681381226,2.057939946098486e-05
1643644,1643645,1643644,3287289,1895.8543133735657,2.0242408027115744e-05
1645646,1645647,1645646,3291293,1897.6069633960724,1.991092517528159e-05
1647648,1647649,1647648,3295297,1899.3004369735718,1.9584860865506926e-05
1649650,1649651,1649650,3299301,1901.0030462741852,1.9264126649432e-05
1651652,1651653,1651652,3303305,1902.6930561065674,1.8948634874504933e-05
1653654,1653655,1653654,3307309,1904.4507982730865,1.8638300389284268e-05
1655656,1655657,1655656,3311313,1906.217740058899,1.8333038497075904e-05
1657658,1657659,1657658,3315317,1907.9893600940704,1.8032766206488304e-05
1659660,1659661,1659660,3319321,1909.7177662849426,1.7737402231432498e-05
1661662,1661663,1661662,3323325,1911.4169600009918,1.7446866195314215e-05
1663664,1663665,1663664,3327329,1913.1136441230774,1.716107908578124e-05
1665666,1665667,1665666,3331333,1914.9025242328644,1.687996314103657e-05
1667668,1667669,1667668,3335337,1916.7459602355957,1.660344219089893e-05
1669670,1669671,1669670,3339341,1918.6857752799988,1.6331440974681755e-05
1671672,1671673,1671672,3343345,1920.6089379787445,1.606388559594052e-05
1673674,1673675,1673674,3347349,1922.4648711681366,1.580070340878592e-05
1675676,1675677,1675676,3351353,1924.1271350383759,1.5541822790510196e-05
1677678,1677679,1677678,3355357,1925.8556821346283,1.5287173710021307e-05
1679680,1679681,1679680,3359361,1927.6517992019653,1.503668647728773e-05
1681682,1681683,1681682,3363365,1929.4878482818604,1.4790293789701536e-05
1683684,1683685,1683684,3367369,1931.3209471702576,1.4547927889907442e-05
1685686,1685687,1685686,3371373,1933.0615952014923,1.4309523294286919e-05
1687688,1687689,1687688,3375377,1934.8375651836395,1.4075015315029304e-05
1689690,1689691,1689690,3379381,1936.5531771183014,1.3844340173818637e-05
1691692,1691693,1691692,3383385,1938.2405281066895,1.3617435115520493e-05
1693694,1693695,1693694,3387389,1939.9355680942535,1.3394238635555666e-05
1695696,1695697,1695696,3391393,1941.6477313041687,1.3174690025152813e-05
1697698,1697699,1697698,3395397,1943.3906590938568,1.2958729939782643e-05
1699700,1699701,1699700,3399401,1945.1509461402893,1.2746298921229027e-05
1701702,1701703,1701702,3403405,1946.9084331989288,1.2537340239759942e-05
1703704,1703705,1703704,3407409,1948.678705215454,1.2331796597209177e-05
1705706,1705707,1705706,3411413,1950.357327222824,1.2129611832278897e-05
1707708,1707709,1707708,3415417,1952.074386358261,1.1930731943721185e-05
1709710,1709711,1709710,3419421,1953.7672402858734,1.1735101907106582e-05
1711712,1711713,1711712,3423425,1955.4566230773926,1.1542669426489738e-05
1713714,1713715,1713714,3427429,1957.1816849708557,1.1353381751177949e-05
1715716,1715717,1715716,3431433,1958.9523792266846,1.1167187608407403e-05
1717718,1717719,1717718,3435437,1960.7257351875305,1.0984036293848476e-05
1719720,1719721,1719720,3439441,1962.4351150989532,1.0803878353726759e-05
1721722,1721723,1721722,3443445,1964.1247701644897,1.0626664561641519e-05
1723724,1723725,1723724,3447449,1965.8320870399475,1.0452346941747237e-05
1725726,1725727,1725726,3451453,1967.5248801708221,1.0280878200319421e-05
1727728,1727729,1727728,3455457,1969.2094180583954,1.0112211384694092e-05
1729730,1729731,1729730,3459461,1970.9297263622284,9.946301247509837e-06
1731732,1731733,1731732,3463465,1972.6417860984802,9.783102314031566e-06
1733734,1733735,1733734,3467469,1974.3674981594086,9.622570360079408e-06
1735736,1735737,1735736,3471473,1976.1149580478668,9.464662070968188e-06
1737738,1737739,1737738,3475477,1977.8747293949127,9.309334018325899e-06
1739740,1739741,1739740,3479481,1979.5564501285553,9.156544592769933e-06
1741742,1741743,1741742,3483485,1981.2537262439728,9.00625195754401e-06
1743744,1743745,1743744,3487489,1982.8966131210327,8.858415299073386e-06
1745746,1745747,1745746,3491493,1984.588875055313,8.712994713278022e-06
1747748,1747749,1747748,3495497,1986.3765749931335,8.569950296077877e-06
1749750,1749751,1749750,3499501,1988.1390793323517,8.429243621321802e-06
1751752,1751753,1751752,3503505,1989.8781971931458,8.29083614917181e-06
1753754,1753755,1753754,3507509,1991.5771782398224,8.154690704031964e-06
1755756,1755757,1755756,3511513,1993.2520191669464,8.020769655558979e-06
1757758,1757759,1757758,3515517,1994.9563591480255,7.889037306085811e-06
1759760,1759761,1759760,3519521,1996.6587970256805,7.75945773057174e-06
1761762,1761763,1761762,3523525,1998.3666303157806,7.631995345036557e-06
1763764,1763765,1763764,3527529,2000.0707120895386,7.506616043428949e-06
1765766,1765767,1765766,3531533,2001.8123903274536,7.383285378637083e-06
1767768,1767769,1767768,3535537,2003.5480182170868,7.261970154104347e-06
1769770,1769771,1769770,3539541,2005.2449700832367,7.142637286960962e-06
1771772,1771773,1771772,3543545,2006.9343872070312,7.0252544901450165e-06
1773774,1773775,1773774,3547549,2008.6554334163666,6.9097899313419475e-06
1775776,1775777,1775776,3551553,2010.3440272808075,6.796211891924031e-06
1777778,1777779,1777778,3555557,2012.0510301589966,6.684489903818758e-06
1779780,1779781,1779780,3559561,2013.733852148056,6.574593271579943e-06
1781782,1781783,1781782,3563565,2015.4374871253967,6.466492664003454e-06
1783784,1783785,1783784,3567569,2017.0964033603668,6.360158295137808e-06
1785786,1785787,1785786,3571573,2018.8401362895966,6.255561629586737e-06
1787788,1787789,1787788,3575577,2020.6043021678925,6.152673904580297e-06
1789790,1789791,1789790,3579581,2022.3167653083801,6.051467494216922e-06
1791792,1791793,1791792,3583585,2024.005564212799,5.9519149999687215e-06
1793794,1793795,1793794,3587589,2025.6777453422546,5.853988909620966e-06
1795796,1795797,1795796,3591593,2027.379316329956,5.757662847827305e-06
1797798,1797799,1797798,3595597,2029.0701141357422,5.662911121362413e-06
1799800,1799801,1799800,3599601,2030.7804281711578,5.569707354879938e-06
1801802,1801803,1801802,3603605,2032.467357158661,5.478026537275582e-06
1803804,1803805,1803804,3607609,2034.1883692741394,5.3878438848187216e-06
1805806,1805807,1805806,3611613,2035.8775432109833,5.2991345000918955e-06
1807808,1807809,1807808,3615617,2037.5836012363434,5.211874736232858e-06
1809810,1809811,1809810,3619621,2039.2626371383667,5.126040946379362e-06
1811812,1811813,1811812,3623625,2041.0208671092987,5.041609483669163e-06
1813814,1813815,1813814,3627629,2043.0460443496704,4.958557497047877e-06
1815816,1815817,1815816,3631633,2044.9190912246704,4.876862703895313e-06
1817818,1817819,1817818,3635637,2046.7628381252289,4.7965027079044376e-06
1819820,1819821,1819820,3639641,2048.6271212100983,4.717455567515572e-06
1821822,1821823,1821822,3643645,2050.3191170692444,4.639700250663736e-06
1823824,1823825,1823824,3647649,2052.0325062274933,4.563215156849765e-06
1825826,1825827,1825826,3651653,2053.757273197174,4.487979936129705e-06
1827828,1827829,1827828,3655657,2055.326004266739,4.4139738974990905e-06
1829830,1829831,1829830,3659661,2056.92356133461,4.341177145761321e-06
1831832,1831833,1831832,3663665,2058.4569931030273,4.2695694446592825e-06
1833834,1833835,1833834,3667669,2060.033944129944,4.199132263238425e-06
1835836,1835837,1835836,3671673,2061.603980064392,4.129845592615311e-06
1837838,1837839,1837838,3675677,2063.157674074173,4.061691129209066e-06
1839840,1839841,1839840,3679681,2064.7104861736298,3.994650228378305e-06
1841842,1841843,1841842,3683685,2066.2768971920013,3.9287044728553155e-06
1843844,1843845,1843844,3687689,2067.8148663043976,3.8638363548670895e-06
1845846,1845847,1845846,3691693,2069.433662176132,3.800028139266942e-06
1847848,1847849,1847848,3695697,2070.992333173752,3.737262431968702e-06
1849850,1849851,1849850,3699701,2072.8066811561584,3.675522066259873e-06
1851852,1851853,1851852,3703705,2074.4963121414185,3.614790557548986e-06
1853854,1853855,1853854,3707709,2076.174430370331,3.555051193870895e-06
1855856,1855857,1855856,3711713,2077.8967730998993,3.49628805906832e-06
1857858,1857859,1857858,3715717,2079.6941282749176,3.4384847822366282e-06
1859860,1859861,1859860,3719721,2081.5870542526245,3.3816261293395655e-06
1861862,1861863,1861862,3723725,2083.654437303543,3.325696411593526e-06
1863864,1863865,1863864,3727729,2085.3642790317535,3.2706803949622554e-06
1865866,1865867,1865866,3731733,2087.057013988495,3.2165631864700117e-06
1867868,1867869,1867868,3735737,2088.740165233612,3.1633302342015668e-06
1869870,1869871,1869870,3739741,2090.428026199341,3.110966986241692e-06
1871872,1871873,1871872,3743745,2092.1682782173157,3.0594593454225105e-06
1873874,1873875,1873874,3747749,2093.9147300720215,3.0087931008893065e-06
1875876,1875877,1875876,3751753,2095.755023241043,2.9589546102215536e-06
1877878,1877879,1877878,3755757,2097.5728492736816,2.9099305720592383e-06
1879880,1879881,1879880,3759761,2099.3340632915497,2.8617071166081587e-06
1881882,1881883,1881882,3763765,2101.0775270462036,2.8142717383161653e-06
1883884,1883885,1883884,3767769,2102.79260802269,2.76761136319692e-06
1885886,1885887,1885886,3771773,2104.545634031296,2.721713372011436e-06
1887888,1887889,1887888,3775777,2106.4365150928497,2.6765650318338885e-06
1889890,1889891,1889890,3779781,2108.3222472667694,2.632154519233154e-06
1891892,1891893,1891892,3783785,2110.0844752788544,2.5884694423439214e-06
1893894,1893895,1893894,3787789,2111.7030081748962,2.5454979777350673e-06
1895896,1895897,1895896,3791793,2113.345516204834,2.5032287567228195e-06
1897898,1897899,1897898,3795797,2114.952176094055,2.4616498421892175e-06
1899900,1899901,1899900,3799801,2116.7417652606964,2.420750547571515e-06
1901902,1901903,1901902,3803805,2118.4592230319977,2.380519276812265e-06
1903904,1903905,1903904,3807809,2120.311215162277,2.3409452296618838e-06
1905906,1905907,1905906,3811813,2122.2345151901245,2.302017833244463e-06
1907908,1907909,1907908,3815817,2124.23056101799,2.263726400997257e-06
1909910,1909911,1909910,3819821,2126.0451531410217,2.226060473731195e-06
1911912,1911913,1911912,3823825,2127.8901782035828,2.1890099333177204e-06
1913914,1913915,1913914,3827829,2129.553138256073,2.1525644342546e-06
1915916,1915917,1915916,3831833,2131.2351911067963,2.1167146542211412e-06
1917918,1917919,1917918,3835837,2132.8204061985016,2.081450588775624e-06
1919920,1919921,1919920,3839841,2134.3503890037537,2.046762347163167e-06
1921922,1921923,1921922,3843845,2135.8582372665405,2.0126410618104273e-06
1923924,1923925,1923924,3847849,2137.3647632598877,1.9790769556493615e-06
1925926,1925927,1925926,3851853,2138.9628789424896,1.94606150216714e-06
1927928,1927929,1927928,3855857,2140.562608242035,1.9135851516693947e-06
1929930,1929931,1929930,3859861,2142.1781351566315,1.8816392639564583e-06
1931932,1931933,1931932,3863865,2143.7648010253906,1.850215653576015e-06
1933934,1933935,1933934,3867869,2145.390197992325,1.8193049982073717e-06
1935936,1935937,1935936,3871873,2146.9631791114807,1.788899680832401e-06
1937938,1937939,1937938,3875877,2148.5607800483704,1.7589908338777605e-06
1939940,1939941,1939940,3879881,2150.1272552013397,1.7295707266384852e-06
1941942,1941943,1941942,3883885,2151.7117261886597,1.7006310599754215e-06
1943944,1943945,1943944,3887889,2153.282216310501,1.6721645579309552e-06
1945946,1945947,1945946,3891893,2154.8831470012665,1.6441626939922571e-06
1947948,1947949,1947948,3895897,2156.5548782348633,1.6166184195753885e-06
1949950,1949951,1949950,3899901,2158.3143060207367,1.5895241176622221e-06
1951952,1951953,1951952,3903905,2159.89119720459,1.5628725122951437e-06
1953954,1953955,1953954,3907909,2161.4306581020355,1.5366561001428636e-06
1955956,1955957,1955956,3911913,2162.9929621219635,1.5108681736819563e-06
1957958,1957959,1957958,3915917,2164.572580099106,1.4855015706416452e-06
1959960,1959961,1959960,3919921,2166.1308732032776,1.460549128751154e-06
1961962,1961963,1961962,3923925,2167.70582818985,1.4360043678607326e-06
1963964,1963965,1963964,3927929,2169.3290281295776,1.4118608078206307e-06
1965966,1965967,1965966,3931933,2171.0279171466827,1.388111286360072e-06
1967968,1967969,1967968,3935937,2172.6648111343384,1.3647501191371703e-06
1969970,1969971,1969970,3939941,2174.233220100403,1.3417703712548246e-06
1971972,1971973,1971972,3943945,2175.8138790130615,1.3191661309974734e-06
1973974,1973975,1973974,3947949,2177.364848136902,1.2969310319022043e-06
1975976,1975977,1975976,3951953,2178.9230461120605,1.275059048566618e-06
1977978,1977979,1977978,3955957,2180.4912571907043,1.2535446103356662e-06
1979980,1979981,1979980,3959961,2182.073307275772,1.232381578120112e-06
1981982,1981983,1981982,3963965,2183.5830001831055,1.2115642675780691e-06
1983984,1983985,1983984,3967969,2185.098221063614,1.191086880680814e-06
1985986,1985987,1985986,3971973,2186.674784183502,1.1709441878338112e-06
1987988,1987989,1987988,3975977,2188.214732170105,1.1511305046951747e-06
1989990,1989991,1989990,3979981,2189.763837337494,1.131640374296694e-06
1991992,1991993,1991992,3983985,2191.301254272461,1.1124686807306716e-06
1993994,1993995,1993994,3987989,2192.8354251384735,1.09361030808941e-06
1995996,1995997,1995996,3991993,2194.319990158081,1.0750600267783739e-06
1997998,1997999,1997998,3995997,2195.7925910949707,1.0568124935161904e-06
2000000,2000001,2000000,4000001,2197.329564332962,1.0388632745161885e-06


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007841587066650391,2180.042156630883
1,4,4,8,0.0024390220642089844,1649.7561110534912
2,6,6,12,0.004012107849121094,785.7772573014074
3,8,8,16,0.005352973937988281,442.5565902014723
4,12,12,24,0.008124351501464844,299.58060016479703
5,20,20,40,0.012027263641357422,288.42098736223693
6,24,24,48,0.014342308044433594,222.79071163786648
7,32,32,64,0.019233226776123047,219.8174211852122
8,36,36,72,0.02129220962524414,182.82409958985522
9,44,44,88,0.025138139724731445,181.1625523972575
10,50,50,100,0.027877330780029297,180.18797708248076
11,56,56,112,0.03189730644226074,169.06558190080818
12,60,60,120,0.034420013427734375,147.797171410916
13,64,64,128,0.036414146423339844,132.88970567018487
14,70,70,140,0.03920412063598633,108.42904570778978
15,72,72,144,0.04049110412597656,81.2908408201049
16,76,76,152,0.04236316680908203,80.04216520899013
17,80,80,160,0.04428601264953613,78.11845813338005
18,88,88,176,0.047805070877075195,77.93138891778767
19,92,92,184,0.050045013427734375,74.64651519897939
20,96,96,192,0.05231809616088867,72.99211134776715
21,102,102,204,0.055663108825683594,72.548014062849
22,106,106,212,0.05771231651306152,69.85426173878295
23,110,110,220,0.059754133224487305,68.37483358601662
24,116,116,232,0.06266307830810547,67.62893753122967
25,124,124,248,0.06622123718261719,67.57982315185723
26,128,128,256,0.06877708435058594,64.59191084797544
27,134,134,268,0.07203221321105957,64.16374442350593
28,142,142,284,0.07604312896728516,64.13078866404521
29,146,146,292,0.07806706428527832,61.046931533643374
30,154,154,308,0.08182096481323242,61.02128696393902
31,158,158,316,0.08409500122070312,58.3318786823213
32,164,164,328,0.08736324310302734,57.88102457756281
33,168,168,336,0.08945727348327637,56.45686616600369
34,176,176,352,0.09334611892700195,56.444005438999966
35,180,180,360,0.09557318687438965,55.35707983153543
36,186,186,372,0.09884405136108398,55.172040298464026
37,192,192,384,0.10162210464477539,54.9249142956553
38,196,196,392,0.10362029075622559,54.285632034928994
39,200,200,400,0.10554814338684082,53.732067931315896
40,208,208,416,0.10900712013244629,53.72591086589023
41,212,212,424,0.11101436614990234,53.3163392683191
42,220,220,440,0.11576414108276367,53.31155104441427
43,224,224,448,0.11848020553588867,52.78026172633736
44,232,232,464,0.12180924415588379,52.77557731512297
45,238,238,476,0.12455606460571289,52.50272793667182
46,246,246,492,0.12804937362670898,52.49865468513076
47,252,252,504,0.13146400451660156,52.041562629835425
48,260,260,520,0.13524103164672852,52.03782986296483
49,266,266,532,0.13827013969421387,51.42412881481482
50,274,274,548,0.14178729057312012,51.420766245845016
51,280,280,560,0.14463520050048828,50.53798739544527
52,288,288,576,0.14831805229187012,50.534690665627295
53,296,296,592,0.15175914764404297,50.5314216142915
54,304,304,608,0.15506219863891602,50.52817776216534
55,310,310,620,0.15800023078918457,48.768255750700746
56,318,318,636,0.16224908828735352,48.76513156940473
57,326,326,652,0.16925716400146484,48.76205195984153
58,334,334,668,0.17270612716674805,48.759012511759465
59,340,340,680,0.17565703392028809,46.493711236571926
60,348,348,696,0.17908835411071777,46.49079841566868
61,354,354,708,0.18199825286865234,44.28085656875692
62,362,362,724,0.1853621006011963,44.27808342213916
63,370,370,740,0.18880796432495117,44.275346539714064
64,378,378,756,0.1921381950378418,44.272643166865464
65,386,386,772,0.19530010223388672,44.26997081023569
66,392,392,784,0.19812512397766113,41.563666509011455
67,400,400,800,0.20127320289611816,41.56128295640565
68,406,406,812,0.20400619506835938,39.05573219380585
69,414,414,828,0.2075052261352539,39.053450650393415
70,422,422,844,0.21389317512512207,39.051195564681166
71,428,428,856,0.21702027320861816,36.51277561082293
72,436,436,872,0.22063803672790527,36.510567505275276
73,442,442,884,0.22327613830566406,34.13993009750584
74,450,450,900,0.22646617889404297,34.13790166912759
75,456,456,912,0.22916007041931152,31.931261949557666
76,464,464,928,0.23267912864685059,31.92938752364421
77,470,470,940,0.23538517951965332,30.306012844679117
78,478,478,956,0.2388460636138916,30.30426986992211
79,484,484,968,0.24169707298278809,28.182758258589956
80,492,492,984,0.2452101707458496,28.181097247017306
81,498,498,996,0.24870610237121582,25.522167302695834
82,506,506,1012,0.25225305557250977,25.520546468070734
83,514,514,1028,0.255587100982666,25.518947020199448
84,520,520,1040,0.25855517387390137,23.254165606992956
85,528,528,1056,0.26393604278564453,23.25263986511095
86,534,534,1068,0.26691627502441406,20.852545308053777
87,542,542,1084,0.27046918869018555,20.851125056655746
88,550,550,1100,0.2738959789276123,20.849722731964675
89,558,558,1116,0.27712321281433105,20.848336805146573
90,564,564,1128,0.28014707565307617,18.352308650206623
91,572,572,1144,0.2835042476654053,18.351000233229115
92,580,580,1160,0.28681516647338867,18.34971246567261
93,586,586,1172,0.2896382808685303,16.208337035662453
94,594,594,1188,0.29318928718566895,16.207123809763743
95,600,600,1200,0.29630327224731445,13.80701082686403
96,608,608,1216,0.3005530834197998,13.80584871953181
97,614,614,1228,0.3031632900238037,11.856431004155183
98,622,622,1244,0.30671024322509766,11.85538920123895
99,628,628,1256,0.31057000160217285,10.12969781700474
100,636,636,1272,0.31565332412719727,10.12878681886707
101,642,642,1284,0.3190481662750244,8.636728036849263
102,650,650,1300,0.32240915298461914,8.635899590610165
103,656,656,1312,0.3254561424255371,7.459277379821401
104,664,664,1328,0.32889604568481445,7.458483184772717
105,670,670,1340,0.3318212032318115,6.5104547030983895
106,678,678,1356,0.335252046585083,6.509683370376251
107,686,686,1372,0.33898401260375977,6.508920661625325
108,692,692,1384,0.34189414978027344,5.6405075057772365
109,700,700,1400,0.3464682102203369,5.639760691997367
110,706,706,1412,0.34963321685791016,4.888544973648095
111,714,714,1428,0.3533132076263428,4.887893159784539
112,720,720,1440,0.35596799850463867,4.228695557667152
113,728,728,1456,0.3596763610839844,4.2280992488199445
114,734,734,1468,0.36237025260925293,3.63903782606792
115,740,740,1480,0.36522722244262695,3.150173823882483
116,748,748,1496,0.3688161373138428,3.1496625634127895
117,754,754,1508,0.37139415740966797,2.723046011101701
118,762,762,1524,0.3747901916503906,2.7225985839427267
119,768,768,1536,0.3774101734161377,2.324210980625594
120,774,774,1548,0.3799631595611572,2.0883573010875125
121,780,780,1560,0.38266706466674805,1.8042181646878817
122,788,788,1576,0.38603806495666504,1.803854243113392
123,794,794,1588,0.38901424407958984,1.5313382841387693
124,802,802,1604,0.39280223846435547,1.5310244127934993
125,806,806,1612,0.39477109909057617,0.8648810872601871
126,814,814,1628,0.39884018898010254,0.8646318182625237
127,818,818,1636,0.4010181427001953,0.49279549503728504
128,826,826,1652,0.40471506118774414,0.492587056028583
129,830,830,1660,0.40718817710876465,0.28753988447908796
130,838,838,1676,0.41142916679382324,0.2873468273943445
131,842,842,1684,0.41407108306884766,0.16876278010215628
132,850,850,1700,0.4177131652832031,0.16861658004881974
133,854,854,1708,0.4197711944580078,0.10366949346314414
134,862,862,1724,0.42305898666381836,0.10355420270093418
135,866,866,1732,0.42500925064086914,0.06542716339311028
136,874,874,1748,0.4286370277404785,0.06534397942346004
137,878,878,1756,0.430861234664917,0.04173566734539236
138,884,884,1768,0.4336540699005127,0.037750232559233154
139,888,888,1776,0.4355630874633789,0.02531091120442852
140,896,896,1792,0.43894004821777344,0.025265331456921558
141,900,900,1800,0.44122910499572754,0.01835837639350757
142,908,908,1816,0.44520115852355957,0.018327249257936273
143,912,912,1824,0.4474959373474121,0.013442600109442537
144,920,920,1840,0.4508821964263916,0.013420242567804053
145,924,924,1848,0.45279812812805176,0.009901279769678695
146,932,932,1864,0.45609307289123535,0.00988539804473021
147,936,936,1872,0.45862627029418945,0.007169918314843926
148,942,942,1884,0.4617140293121338,0.006708295288603949
149,946,946,1892,0.4639103412628174,0.005018852230818993
150,954,954,1908,0.4673800468444824,0.005009791490124371
151,958,958,1916,0.4694821834564209,0.003725994024648571
152,966,966,1932,0.4730050563812256,0.003719653896609998
153,970,970,1940,0.4750852584838867,0.002750046719143029
154,978,978,1956,0.4782412052154541,0.002745281307170444
155,982,982,1964,0.4802722930908203,0.0019438868719134916
156,990,990,1980,0.48340725898742676,0.001940203338676838
157,994,994,1988,0.4853072166442871,0.0013434714095410527
158,1000,1000,2000,0.487990140914917,0.0012409508383370849
159,1004,1004,2008,0.48995423316955566,0.0009532533691753997
160,1010,1010,2020,0.4925382137298584,0.0009032211474959695
161,1014,1014,2028,0.4943962097167969,0.0007083621352421687
162,1022,1022,2044,0.49772119522094727,0.00070698905858535
163,1026,1026,2052,0.49965429306030273,0.0005443137937390929
164,1032,1032,2064,0.502249002456665,0.0005158767912689655
165,1036,1036,2072,0.5043511390686035,0.0004098085497616921
166,1040,1040,2080,0.5062181949615479,0.0003567171451095419
167,1044,1044,2088,0.508418083190918,0.00031385052409405034
168,1050,1050,2100,0.5113821029663086,0.00030651137751647184
169,1056,1056,2112,0.5143871307373047,0.0002965251048863138
170,1062,1062,2124,0.5171811580657959,0.0002864219236471399
171,1066,1066,2132,0.5194733142852783,0.00025147978590212006
172,1074,1074,2148,0.5226421356201172,0.00025110603439770784
173,1078,1078,2156,0.5245051383972168,0.0002185415484063924
174,1086,1086,2172,0.5277619361877441,0.00021826697832239006
175,1090,1090,2180,0.5296740531921387,0.00018676089803193463
176,1098,1098,2196,0.5330450534820557,0.00018653284132597037
177,1102,1102,2204,0.5350039005279541,0.00015424448849898909
178,1108,1108,2216,0.5374631881713867,0.00014648222997948324
179,1114,1114,2228,0.5399312973022461,0.0001398359077029454
180,1118,1118,2236,0.5417571067810059,0.00011138416050471278
181,1126,1126,2252,0.5449061393737793,0.00011124470995582669
182,1130,1130,2260,0.5468113422393799,8.552440908715653e-05
183,1134,1134,2268,0.5486752986907959,6.597270396468957e-05
184,1142,1142,2284,0.5518221855163574,6.586321387658245e-05
185,1146,1146,2292,0.5538132190704346,5.109316180096357e-05
186,1154,1154,2308,0.5570733547210693,5.09960029830836e-05
187,1158,1158,2316,0.559333324432373,3.8775264783907915e-05
188,1162,1162,2324,0.5615301132202148,2.9847154223716643e-05
189,1170,1170,2340,0.5651531219482422,2.979014641368849e-05
190,1174,1174,2348,0.5672702789306641,2.240809180875658e-05
191,1178,1178,2356,0.5693283081054688,1.736970762067358e-05
192,1186,1186,2372,0.5723490715026855,1.7337641793346847e-05
193,1190,1190,2380,0.5741770267486572,1.3667561461261357e-05
194,1198,1198,2396,0.577390193939209,1.3643996680912096e-05
195,1202,1202,2404,0.5792660713195801,1.0814019674398878e-05
196,1210,1210,2420,0.5823521614074707,1.0795597859214467e-05
197,1214,1214,2428,0.5842199325561523,8.412962642978528e-06
198,1222,1222,2444,0.5873312950134277,8.399445505347103e-06
199,1226,1226,2452,0.5891931056976318,6.5001939901776495e-06
200,1230,1230,2460,0.5910420417785645,5.561638431572646e-06
201,1234,1234,2468,0.5929989814758301,4.869880740443477e-06
202,1240,1240,2480,0.5960409641265869,4.749642016577127e-06
203,1244,1244,2488,0.5984351634979248,4.304332378524123e-06
204,1250,1250,2500,0.6018099784851074,4.226418923281017e-06
205,1254,1254,2508,0.6037702560424805,3.942716375604505e-06
206,1260,1260,2520,0.6065301895141602,3.893126404364011e-06
207,1264,1264,2528,0.6088352203369141,3.7092759157530963e-06
208,1272,1272,2544,0.6127970218658447,3.707522068907565e-06
209,1276,1276,2552,0.615103006362915,3.523658051562961e-06
210,1284,1284,2568,0.6189150810241699,3.5223910117565538e-06
211,1288,1288,2576,0.6209652423858643,3.3652529509708984e-06
212,1296,1296,2592,0.6244051456451416,3.3643282222328708e-06
213,1300,1300,2600,0.6265602111816406,3.2171925568036386e-06
214,1306,1306,2612,0.6296069622039795,3.180710109518259e-06
215,1312,1312,2624,0.6324820518493652,3.1488646072830306e-06
216,1316,1316,2632,0.6344962120056152,3.035656618521898e-06
217,1322,1322,2644,0.6373310089111328,3.0092055567365605e-06
218,1328,1328,2656,0.6400871276855469,2.9861159873689758e-06
219,1332,1332,2664,0.6422910690307617,2.898373054449621e-06
220,1340,1340,2680,0.6459043025970459,2.8978878390262253e-06
221,1344,1344,2688,0.6484081745147705,2.8328261123533593e-06
222,1352,1352,2704,0.6519513130187988,2.832468567248725e-06
223,1356,1356,2712,0.6537952423095703,2.782742399176641e-06
224,1364,1364,2728,0.6573293209075928,2.7824645485452493e-06
225,1368,1368,2736,0.659644365310669,2.7427803388491157e-06
226,1376,1376,2752,0.6665170192718506,2.742547849265975e-06
227,1380,1380,2760,0.6684660911560059,2.7094326924270717e-06
228,1388,1388,2776,0.6717431545257568,2.709268414946564e-06
229,1392,1392,2784,0.6737570762634277,2.685227855181438e-06
230,1400,1400,2800,0.6770751476287842,2.6851030270336196e-06
231,1404,1404,2808,0.6789712905883789,2.6660883349904907e-06
232,1412,1412,2824,0.683305025100708,2.6659960212782607e-06
233,1416,1416,2832,0.6852080821990967,2.6497465341890347e-06
234,1424,1424,2848,0.6884710788726807,2.6496575173950987e-06
235,1430,1430,2860,0.6911540031433105,2.6444879495102214e-06
236,1436,1436,2872,0.6937973499298096,2.6400516617286485e-06
237,1442,1442,2884,0.6975600719451904,2.635880719026318e-06
238,1450,1450,2900,0.7009432315826416,2.6358086415712023e-06
239,1456,1456,2912,0.7035410404205322,2.6303558797735604e-06
240,1462,1462,2924,0.7060642242431641,2.6256459477735916e-06
241,1470,1470,2940,0.7095413208007812,2.6255842158207088e-06
242,1476,1476,2952,0.712285041809082,2.6191878532699775e-06
243,1484,1484,2968,0.717156171798706,2.6191328288405202e-06
244,1490,1490,2980,0.7198452949523926,2.611418153719569e-06
245,1498,1498,2996,0.7230911254882812,2.61136722201627e-06
246,1504,1504,3008,0.7256600856781006,2.600344600978133e-06
247,1512,1512,3024,0.729013204574585,2.6002940103353467e-06
248,1520,1520,3040,0.7334961891174316,2.6002437607530737e-06
249,1528,1528,3056,0.7367260456085205,2.6001937385444762e-06
250,1536,1536,3072,0.7399890422821045,2.600144057396392e-06
251,1540,1540,3080,0.7420182228088379,2.6039683689305093e-06
252,1544,1544,3088,0.7439560890197754,2.6030143089883495e-06
253,1548,1548,3096,0.7458431720733643,2.5930518177119666e-06
254,1556,1556,3112,0.7497711181640625,2.593007934592606e-06
255,1564,1564,3128,0.7529022693634033,2.5929643925337587e-06
256,1572,1572,3144,0.7561023235321045,2.5929210778485867e-06
257,1580,1580,3160,0.7596821784973145,2.5928777631634148e-06
258,1588,1588,3176,0.7632641792297363,2.5928345621650806e-06
259,1590,1590,3180,0.764721155166626,2.5592227075321716e-06
260,1594,1594,3188,0.7666971683502197,2.5606835833968944e-06
261,1596,1596,3192,0.7679293155670166,2.5650533643784e-06
262,1604,1604,3208,0.7711241245269775,2.565013005551009e-06
263,1612,1612,3224,0.7742111682891846,2.5649727604104555e-06
264,1620,1620,3240,0.7773680686950684,2.5649328563304152e-06
265,1628,1628,3256,0.7807350158691406,2.5648927248766995e-06
266,1632,1632,3264,0.7826640605926514,2.5580579858797137e-06
267,1640,1640,3280,0.7858850955963135,2.558018195486511e-06
268,1644,1644,3288,0.7880163192749023,2.552072260186833e-06
269,1652,1652,3304,0.7915310859680176,2.5520326971673057e-06
270,1660,1660,3320,0.7950930595397949,2.551993361521454e-06
271,1668,1668,3336,0.7988259792327881,2.5519539121887647e-06
272,1676,1676,3352,0.8027482032775879,2.5519143491692375e-06
273,1680,1680,3360,0.8050000667572021,2.5317555127912783e-06
274,1688,1688,3376,0.8086233139038086,2.5317166318927775e-06
275,1694,1694,3388,0.8114612102508545,2.523895091144368e-06
276,1702,1702,3404,0.8150100708007812,2.523856664993218e-06
277,1710,1710,3420,0.8184692859649658,2.523818011468393e-06
278,1718,1718,3436,0.8216531276702881,2.523779471630405e-06
279,1726,1726,3452,0.8249039649963379,2.5237409317924175e-06
280,1730,1730,3460,0.8268401622772217,2.5077413283725036e-06
281,1738,1738,3476,0.830125093460083,2.507703129595029e-06
282,1742,1742,3484,0.8319523334503174,2.4914122604968725e-06
283,1750,1750,3500,0.8350663185119629,2.491374402779911e-06
284,1758,1758,3516,0.8385522365570068,2.4913366587497876e-06
285,1766,1766,3532,0.8419163227081299,2.4912990284065017e-06
286,1774,1774,3548,0.8451461791992188,2.4912610570027027e-06
287,1778,1778,3556,0.8470311164855957,2.47308435064042e-06
288,1782,1782,3564,0.8489401340484619,2.455523031130724e-06
289,1790,1790,3580,0.8522109985351562,2.455485969221627e-06
290,1798,1798,3596,0.8554461002349854,2.4554485662520165e-06
291,1806,1806,3612,0.8586733341217041,2.4554112769692438e-06
292,1814,1814,3628,0.8621652126312256,2.4553743287469842e-06
293,1822,1822,3644,0.8655083179473877,2.455336925777374e-06
294,1828,1828,3656,0.8680531978607178,2.4558941049690475e-06
295,1836,1836,3672,0.871211051940918,2.4558569293731125e-06
296,1838,1838,3676,0.8724522590637207,2.382662955824344e-06
297,1846,1846,3692,0.875535249710083,2.382626576036273e-06
298,1852,1852,3704,0.8780550956726074,1.9949585521317204e-06
299,1860,1860,3720,0.881195068359375,1.9949229681515135e-06
300,1868,1868,3736,0.8843791484832764,1.994887270484469e-06
301,1876,1876,3752,0.8874802589416504,1.994852141251613e-06
302,1884,1884,3768,0.8905651569366455,1.9948168983319192e-06
303,1888,1888,3776,0.892484188079834,2.082751734633348e-06
304,1896,1896,3792,0.8957099914550781,2.0827179696425446e-06
305,1900,1900,3800,0.8974931240081787,2.1329913124645827e-06
306,1906,1906,3812,0.8999922275543213,1.8283180907019414e-06
307,1914,1914,3828,0.9030232429504395,1.828286826821568e-06
308,1918,1918,3836,0.9049670696258545,8.897465022528195e-07
309,1926,1926,3852,0.9081361293792725,8.897181942302268e-07
310,1932,1932,3864,0.9106771945953369,7.334622296184534e-07
311,1938,1938,3876,0.9132659435272217,6.038090987203759e-07
312,1946,1946,3892,0.9166059494018555,6.037855655449675e-07
313,1950,1950,3900,0.9185910224914551,2.8368685889290646e-07
314,1958,1958,3916,0.9218611717224121,2.83666622635792e-07
315,1962,1962,3924,0.9239561557769775,1.2550196970551042e-07
316,1970,1970,3940,0.9272041320800781,1.254844619325013e-07
317,1974,1974,3948,0.9291541576385498,4.663206709665246e-08
318,1982,1982,3964,0.9324991703033447,4.6618083615612704e-08
319,1986,1986,3972,0.9344289302825928,7.239236765599344e-09
320,1994,1994,3988,0.9375860691070557,7.225935405585915e-09
321,2000,2000,4000,0.9403483867645264,1.6336798580596223e-10
322,2006,2006,4012,0.943134069442749,5.699234861822333e-09


==> extragradient/plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0013186931610107422,2180.042156630883
1,4,4,8,0.003532886505126953,1649.7561110534912
2,6,6,12,0.007798910140991211,810.127181747561
3,8,8,16,0.009359121322631836,539.389226626289
4,10,10,20,0.01087188720703125,339.4804780114555
5,12,12,24,0.013466835021972656,245.09872895812805
6,14,14,28,0.015086889266967773,178.2528852958667
7,18,18,36,0.01758408546447754,175.18675618515363
8,22,22,44,0.01940178871154785,178.59077517268156
9,24,24,48,0.020538806915283203,131.40293201501822
10,26,26,52,0.02160191535949707,126.53791140683165
11,28,28,56,0.022656917572021484,130.47739703622142
12,32,32,64,0.024371862411499023,126.01903467464103
13,34,34,68,0.02581191062927246,105.51311594862955
14,36,36,72,0.027257919311523438,101.96868056198309
15,40,40,80,0.030156850814819336,101.54805401814247
16,44,44,88,0.03237485885620117,100.9655802753091
17,48,48,96,0.03420376777648926,99.58113103139681
18,52,52,104,0.03631401062011719,90.95868771932965
19,54,54,108,0.038034915924072266,80.31014610159127
20,56,56,112,0.0395197868347168,80.71895976171572
21,58,58,116,0.040708065032958984,80.87330253928258
22,60,60,120,0.0425410270690918,80.42850369535881
23,62,62,124,0.04463791847229004,73.90294020393867
24,64,64,128,0.046437740325927734,74.2253497634697
25,66,66,132,0.04755091667175293,74.3708571145471
26,68,68,136,0.04864692687988281,74.21600448695972
27,70,70,140,0.049652814865112305,73.40675221629385
28,72,72,144,0.05070304870605469,73.25289053626398
29,74,74,148,0.051744937896728516,72.85164622381672
30,76,76,152,0.052845001220703125,70.73692845466871
31,78,78,156,0.05391407012939453,69.67930347464267
32,82,82,164,0.05567002296447754,69.59616793905843
33,84,84,168,0.05680084228515625,64.92930595163102
34,88,88,176,0.05921673774719238,64.91260165008316
35,90,90,180,0.060482025146484375,62.48231174591956
36,94,94,188,0.06221199035644531,62.50260711551414
37,96,96,192,0.06337404251098633,58.61465481275104
38,98,98,196,0.06461095809936523,58.598060825168204
39,102,102,204,0.06638097763061523,58.60825778646404
40,104,104,208,0.06771087646484375,56.59043284198333
41,106,106,212,0.06897783279418945,56.421337882904936
42,108,108,216,0.06999492645263672,56.17435295854989
43,110,110,220,0.0711359977722168,56.304039257365275
44,112,112,224,0.07230401039123535,55.66437197096457
45,114,114,228,0.07390475273132324,55.13469968746267
46,116,116,232,0.07520580291748047,54.95147441701647
47,118,118,236,0.07644200325012207,54.455596329665696
48,120,120,240,0.07774782180786133,54.07602739028562
49,124,124,248,0.07950592041015625,54.06672606934217
50,126,126,252,0.08053398132324219,53.840704873565755
51,128,128,256,0.0815730094909668,53.80459284000426
52,132,132,264,0.08314895629882812,53.79590168958816
53,134,134,268,0.08420395851135254,53.55199583474746
54,138,138,276,0.08584070205688477,53.544652597298864
55,140,140,280,0.08685088157653809,53.21127701114278
56,144,144,288,0.08854913711547852,53.20525298914322
57,146,146,292,0.08960986137390137,53.00005255428255
58,150,150,300,0.0914449691772461,52.99420109543894
59,152,152,304,0.09251976013183594,52.74678968815624
60,156,156,312,0.09411191940307617,52.735961984027654
61,160,160,320,0.09569883346557617,52.68804455249915
62,162,162,324,0.09674906730651855,52.22270398069827
63,166,166,332,0.09841680526733398,52.21525744506698
64,168,168,336,0.09946990013122559,51.697137968833886
65,172,172,344,0.10111093521118164,51.685990548468226
66,174,174,348,0.10216069221496582,51.29791100351781
67,178,178,356,0.10390901565551758,51.30086282069419
68,180,180,360,0.10503911972045898,50.907050916286835
69,184,184,368,0.10671401023864746,50.90838733254736
70,188,188,376,0.10854291915893555,50.90532450908904
71,192,192,384,0.11018896102905273,50.90365345442228
72,196,196,392,0.11181378364562988,50.90293554349137
73,200,200,400,0.11333489418029785,50.77757613508629
74,204,204,408,0.11493396759033203,50.67539995580887
75,206,206,412,0.11598992347717285,49.206591602504204
76,210,210,420,0.11753010749816895,49.18755919207001
77,212,212,424,0.11851787567138672,47.21836362704471
78,216,216,432,0.12007284164428711,47.22496645595015
79,218,218,436,0.12107992172241211,46.62540974549938
80,222,222,444,0.12266373634338379,46.59387425591967
81,226,226,452,0.12416410446166992,46.53719063911558
82,230,230,460,0.1257638931274414,46.43658969645003
83,234,234,468,0.12737083435058594,46.40927873939745
84,238,238,476,0.12898683547973633,46.37727093386252
85,240,240,480,0.12994885444641113,45.5816881468279
86,244,244,488,0.13149309158325195,45.52935455187003
87,248,248,496,0.13310575485229492,45.370244210982264
88,252,252,504,0.13468194007873535,45.23139474612526
89,254,254,508,0.13562679290771484,44.130109950136784
90,258,258,516,0.13711309432983398,44.070427866784485
91,262,262,524,0.13868284225463867,43.93074148847586
92,264,264,528,0.13970184326171875,43.01087875912981
93,268,268,536,0.14123988151550293,42.996726740230315
94,270,270,540,0.1422419548034668,41.05119781951407
95,276,276,552,0.1443018913269043,41.06158289924656
96,278,278,556,0.14529776573181152,40.623973252071664
97,282,282,564,0.14698004722595215,40.44528875859169
98,286,286,572,0.14858698844909668,40.14329880877608
99,288,288,576,0.14965295791625977,38.907943403519766
100,290,290,580,0.15068387985229492,38.27097375350445
101,294,294,588,0.15226483345031738,38.27019847418774
102,296,296,592,0.15328574180603027,37.60792659895651
103,300,300,600,0.15486884117126465,37.608139277216424
104,302,302,604,0.15590810775756836,36.73954260003461
105,306,306,612,0.15752792358398438,36.71389417079399
106,308,308,616,0.1585099697113037,34.06674003733201
107,312,312,624,0.1600348949432373,34.08144727329932
108,314,314,628,0.16106796264648438,32.34218926609833
109,316,316,632,0.16204595565795898,31.12709178457567
110,320,320,640,0.1635739803314209,30.998493740731874
111,322,322,644,0.16457271575927734,28.258091421225117
112,326,326,652,0.16610980033874512,28.43056041812656
113,330,330,660,0.16771292686462402,28.487179572653986
114,332,332,664,0.16869497299194336,25.467477824180833
115,336,336,672,0.17020893096923828,25.704290915149386
116,338,338,676,0.17118000984191895,27.393485636474225
117,342,342,684,0.17272591590881348,27.420517288618612
118,344,344,688,0.17370390892028809,26.679502734768676
119,348,348,696,0.17525076866149902,26.58051642041346
120,350,350,700,0.1762857437133789,24.7357096189603
121,354,354,708,0.17787575721740723,24.791918718938177
122,356,356,712,0.17888879776000977,21.12267827242158
123,360,360,720,0.180405855178833,21.275291131650874
124,362,362,724,0.1813957691192627,21.876982218154808
125,366,366,732,0.18322396278381348,21.939664254494346
126,368,368,736,0.18430209159851074,20.22887744074592
127,372,372,744,0.18588995933532715,20.2338929083694
128,374,374,748,0.18691086769104004,17.264112494586243
129,380,380,760,0.18935275077819824,17.241561096853957
130,384,384,768,0.19109082221984863,17.089968096257508
131,390,390,780,0.1933608055114746,17.044268590477714
132,392,392,784,0.19449687004089355,18.241337685322378
133,396,396,792,0.19622182846069336,18.33339393361075
134,398,398,796,0.19725298881530762,18.73062557532512
135,402,402,804,0.19901585578918457,18.625547142386267
136,406,406,812,0.20083093643188477,18.46299037701783
137,408,408,816,0.20195388793945312,16.94615155030965
138,412,412,824,0.20357990264892578,16.810062584168236
139,414,414,828,0.20457172393798828,16.277167015027317
140,418,418,836,0.20614910125732422,16.32882435472311
141,422,422,844,0.2077498435974121,16.367978166200373
142,424,424,848,0.20880579948425293,14.746524154090253
143,428,428,856,0.210493803024292,14.79719310734231
144,430,430,860,0.21159076690673828,13.640758649972895
145,434,434,868,0.21373200416564941,13.616246857723013
146,436,436,872,0.21488404273986816,12.282277414570899
147,440,440,880,0.21657395362854004,12.33994389655561
148,442,442,884,0.21761775016784668,10.668878569404797
149,446,446,892,0.21922683715820312,10.711602572986976
150,448,448,896,0.22025275230407715,8.419640325777436
151,456,456,912,0.22295904159545898,8.4193319631662
152,458,458,916,0.22404813766479492,7.552935557968453
153,466,466,932,0.2269117832183838,7.552637765085478
154,468,468,936,0.2279958724975586,8.268244553474233
155,472,472,944,0.22961187362670898,8.043434360266929
156,476,476,952,0.23130106925964355,8.066232489426056
157,478,478,956,0.23239803314208984,8.11201988075402
158,482,482,964,0.23398494720458984,8.105209442577689
159,484,484,968,0.23498272895812988,8.192359670403903
160,488,488,976,0.2366929054260254,8.172458336300565
161,490,490,980,0.23780488967895508,7.400200974148902
162,498,498,996,0.24060678482055664,7.399980551538647
163,502,502,1004,0.24234986305236816,7.229833180424862
164,510,510,1020,0.24547696113586426,7.2296168685358
165,512,512,1024,0.24652385711669922,6.58420562666322
166,520,520,1040,0.24923110008239746,6.58399589415626
167,522,522,1044,0.25029492378234863,6.687033232133217
168,524,524,1048,0.2513010501861572,6.395290940338441
169,532,532,1064,0.2539660930633545,6.39510304721864
170,534,534,1068,0.2550678253173828,6.212330300789631
171,538,538,1076,0.25678300857543945,6.218693251021705
172,540,540,1080,0.25789880752563477,6.092412965329572
173,542,542,1084,0.25897789001464844,5.840301059969761
174,546,546,1092,0.26059389114379883,5.82288934895098
175,550,550,1100,0.2622859477996826,5.823721596453197
176,554,554,1108,0.26396679878234863,5.794661799384585
177,556,556,1112,0.26510095596313477,5.64405635121534
178,558,558,1116,0.2661728858947754,5.380430347898027
179,562,562,1124,0.26786088943481445,5.3683366334483935
180,566,566,1132,0.2697887420654297,5.331311180194916
181,568,568,1136,0.27123403549194336,5.103626390068939
182,572,572,1144,0.27329182624816895,5.085362519662226
183,574,574,1148,0.2746407985687256,4.726565232063081
184,578,578,1156,0.27635979652404785,4.7252917540514545
185,580,580,1160,0.2778959274291992,4.714985581540759
186,584,584,1168,0.2798130512237549,4.717567464452372
187,586,586,1172,0.2809758186340332,4.341502687084812
188,590,590,1180,0.28262805938720703,4.351770285227417
189,592,592,1184,0.28375911712646484,3.94998843370297
190,596,596,1192,0.28543591499328613,3.953567705747787
191,598,598,1196,0.2865128517150879,3.765440667114376
192,602,602,1204,0.28813695907592773,3.764254273565598
193,604,604,1208,0.289154052734375,3.5146064881253096
194,608,608,1216,0.2908968925476074,3.516611877357832
195,610,610,1220,0.2921440601348877,3.3482877471685697
196,614,614,1228,0.29401087760925293,3.350150465877846
197,616,616,1232,0.29514288902282715,3.2735319530848983
198,620,620,1240,0.29768896102905273,3.2781486370812445
199,624,624,1248,0.2998230457305908,3.2772080619769213
200,628,628,1256,0.3015599250793457,3.2822605928686244
201,632,632,1264,0.3034207820892334,3.284312206804202
202,634,634,1268,0.3047058582305908,2.979699227729384
203,638,638,1276,0.3064858913421631,2.951037925447281
204,642,642,1284,0.30823683738708496,2.896052663499404
205,648,648,1296,0.3104979991912842,2.8807422356466077
206,656,656,1312,0.3134148120880127,2.880673167148757
207,658,658,1316,0.31450700759887695,2.6048240677197327
208,664,664,1328,0.3167107105255127,2.594979590284993
209,668,668,1336,0.3183767795562744,2.6241139725131006
210,676,676,1352,0.321213960647583,2.6240471525828752
211,680,680,1360,0.3229207992553711,2.564523215790473
212,682,682,1364,0.32404398918151855,2.6859655608931234
213,686,686,1372,0.32568907737731934,2.6868812205934773
214,688,688,1376,0.3268008232116699,2.7426717965544185
215,694,694,1388,0.3292107582092285,2.727157823440507
216,700,700,1400,0.3316018581390381,2.713321907436921
217,706,706,1412,0.33391475677490234,2.7072006462332183
218,710,710,1420,0.335676908493042,2.7034230664633014
219,714,714,1428,0.3373439311981201,2.6890978420200327
220,716,716,1432,0.3384208679199219,2.5909021363929696
221,720,720,1440,0.3400449752807617,2.589979328390882
222,722,722,1444,0.34116387367248535,2.4339638904541516
223,726,726,1452,0.34270572662353516,2.430775248374175
224,728,728,1456,0.3437349796295166,2.193415695046724
225,732,732,1464,0.34526991844177246,2.1920391501555514
226,734,734,1468,0.3463437557220459,2.019873415245229
227,738,738,1476,0.34809374809265137,2.020489930255735
228,740,740,1480,0.3491189479827881,1.985143344129483
229,744,744,1488,0.35075879096984863,1.9862878240725195
230,746,746,1492,0.35182785987854004,2.0124519220231605
231,750,750,1500,0.353543758392334,2.015269102101115
232,752,752,1504,0.3546149730682373,1.9256560156587739
233,756,756,1512,0.35630297660827637,1.9232920227367458
234,758,758,1516,0.3573570251464844,1.870394913832115
235,762,762,1524,0.3590860366821289,1.8691503857098724
236,766,766,1532,0.3606698513031006,1.8619088539551285
237,768,768,1536,0.36170291900634766,1.7503096479271107
238,772,772,1544,0.36356496810913086,1.7514546555714787
239,774,774,1548,0.3646578788757324,1.7190404887351178
240,778,778,1556,0.3663308620452881,1.7172456230649686
241,780,780,1560,0.3674659729003906,1.671705234441788
242,782,782,1564,0.3685569763183594,1.5919965089075276
243,786,786,1572,0.37022995948791504,1.5773718743495238
244,790,790,1580,0.371931791305542,1.5637772834567158
245,792,792,1584,0.37305498123168945,1.539804422827956
246,796,796,1592,0.3748018741607666,1.5399324976606295
247,798,798,1596,0.3759748935699463,1.4595216815865797
248,802,802,1604,0.3776588439941406,1.457492779633526
249,806,806,1612,0.3793158531188965,1.451351983615723
250,810,810,1620,0.38126587867736816,1.4441461736146266
251,812,812,1624,0.3824307918548584,1.3962984076256362
252,816,816,1632,0.3843538761138916,1.3943894129631644
253,818,818,1636,0.38561081886291504,1.3277647048759036
254,822,822,1644,0.38762903213500977,1.3238124109149112
255,824,824,1648,0.3889288902282715,1.1894627307544852
256,828,828,1656,0.3907890319824219,1.1889302402944395
257,830,830,1660,0.3918938636779785,1.0921027037509248
258,834,834,1668,0.39353179931640625,1.0945440605648855
259,836,836,1672,0.394608736038208,0.9863003129419212
260,840,840,1680,0.3961479663848877,0.9973781345938733
261,842,842,1684,0.39714670181274414,0.9948753715854082
262,844,844,1688,0.39816999435424805,0.9772026523509112
263,846,846,1692,0.3993048667907715,0.8573236492251226
264,848,848,1696,0.40035390853881836,0.8743930175274954
265,850,850,1700,0.401439905166626,0.754503721637434
266,854,854,1708,0.40308403968811035,0.7558048810915352
267,858,858,1716,0.4047539234161377,0.7587031211469366
268,860,860,1720,0.4058527946472168,0.7716867454963676
269,864,864,1728,0.40758395195007324,0.771385399726114
270,866,866,1732,0.40866684913635254,0.7242090134044474
271,870,870,1740,0.4103820323944092,0.7203558221382309
272,872,872,1744,0.41150403022766113,0.6308759675746387
273,876,876,1752,0.41318583488464355,0.6319081397109585
274,878,878,1756,0.41420578956604004,0.5667572657995379
275,882,882,1764,0.4158189296722412,0.5671467623543549
276,884,884,1768,0.4168848991394043,0.5086225884303985
277,888,888,1776,0.4185788631439209,0.5084680447280334
278,890,890,1780,0.41959595680236816,0.4486280803811269
279,894,894,1788,0.42117810249328613,0.45133379304809296
280,896,896,1792,0.4222707748413086,0.41860255537051216
281,900,900,1800,0.4239368438720703,0.4174434871081303
282,902,902,1804,0.4250187873840332,0.38735124546474253
283,906,906,1812,0.4266810417175293,0.39004057791385094
284,908,908,1816,0.4278247356414795,0.40530233886363476
285,910,910,1820,0.42917704582214355,0.4057127836173322
286,914,914,1828,0.4308500289916992,0.4031189305451335
287,916,916,1832,0.43187594413757324,0.33426900414190186
288,920,920,1840,0.433499813079834,0.33448825810171456
289,922,922,1844,0.43454408645629883,0.2848654882205892
290,926,926,1852,0.4361138343811035,0.2846243862148867
291,928,928,1856,0.4371068477630615,0.2384620617310702
292,932,932,1864,0.4387798309326172,0.23849762407769504
293,934,934,1868,0.4398839473724365,0.2100547479050192
294,938,938,1876,0.4415128231048584,0.21062888181336348
295,940,940,1880,0.4425027370452881,0.18409018853446923
296,944,944,1888,0.44402599334716797,0.18434489713990843
297,946,946,1892,0.4450507164001465,0.15992406703901452
298,950,950,1900,0.44677090644836426,0.16079331080436532
299,952,952,1904,0.4478340148925781,0.16029505669303035
300,954,954,1908,0.44883084297180176,0.1604635138901358
301,956,956,1912,0.44983911514282227,0.13108065334381536
302,960,960,1920,0.45154285430908203,0.13235792240323008
303,962,962,1924,0.4525768756866455,0.14060514807022173
304,966,966,1932,0.4541597366333008,0.1408280324212683
305,968,968,1936,0.45519471168518066,0.12263215844359365
306,970,970,1940,0.45627903938293457,0.11920363278613877
307,972,972,1944,0.457348108291626,0.10345324050013005
308,974,974,1948,0.4584319591522217,0.1053063422376681
309,978,978,1956,0.46015000343322754,0.09532300421017226
310,980,980,1960,0.46129679679870605,0.08712464280245058
311,984,984,1968,0.46297788619995117,0.08743290136499127
312,986,986,1972,0.46411895751953125,0.059991802363811075
313,990,990,1980,0.46582984924316406,0.06048623336118908
314,992,992,1984,0.4669978618621826,0.037213052649008205
315,994,994,1988,0.4681127071380615,0.03880695651287169
316,996,996,1992,0.4691479206085205,0.030890633285366675
317,1000,1000,2000,0.47072887420654297,0.03051995976852595
318,1002,1002,2004,0.4719359874725342,0.01824624274445341
319,1006,1006,2012,0.47362494468688965,0.018497229099125434
320,1008,1008,2016,0.47467899322509766,0.015044478316553977
321,1012,1012,2024,0.4763786792755127,0.015281504212566688
322,1014,1014,2028,0.4774138927459717,0.013159970866354342
323,1018,1018,2036,0.4790778160095215,0.013125264242717094
324,1020,1020,2040,0.48012471199035645,0.007427691634347866
325,1024,1024,2048,0.48179197311401367,0.007492982382018454
326,1026,1026,2052,0.4829699993133545,0.004969460768620593
327,1030,1030,2060,0.4846348762512207,0.0049983834584281794
328,1032,1032,2064,0.4857158660888672,0.004117810798220489
329,1036,1036,2072,0.48745083808898926,0.004145348536894744
330,1038,1038,2076,0.48874688148498535,0.004543947947468041
331,1042,1042,2084,0.4904508590698242,0.004590832591588878
332,1044,1044,2088,0.4915499687194824,0.005094218050658128
333,1048,1048,2096,0.4932279586791992,0.00504700694341409
334,1050,1050,2100,0.4943568706512451,0.004062382156007516
335,1054,1054,2108,0.4960057735443115,0.004052525135762153
336,1056,1056,2112,0.49709486961364746,0.0022521288677808116
337,1060,1060,2120,0.4987189769744873,0.002231443461255367
338,1062,1062,2124,0.4997899532318115,0.001953661173047294
339,1066,1066,2132,0.501413106918335,0.0019599522879616416
340,1068,1068,2136,0.5024549961090088,0.0017890079175231222
341,1072,1072,2144,0.5040907859802246,0.0017885119320908416
342,1074,1074,2148,0.5051476955413818,0.0016220983193306893
343,1078,1078,2156,0.5067758560180664,0.0015988236041266646
344,1080,1080,2160,0.5078277587890625,0.001309760402136817
345,1084,1084,2168,0.509443998336792,0.0013175341464375379
346,1086,1086,2172,0.5105068683624268,0.0013842497971836565
347,1088,1088,2176,0.5115368366241455,0.0013302389994578334
348,1092,1092,2184,0.5131468772888184,0.0013302050630272788
349,1094,1094,2188,0.514178991317749,0.0012356490050251523
350,1096,1096,2192,0.5151958465576172,0.0010869600306477878
351,1100,1100,2200,0.5167839527130127,0.0010834728612962863
352,1102,1102,2204,0.5178968906402588,0.0010692574192034954
353,1106,1106,2212,0.5195648670196533,0.0010763324435174582
354,1108,1108,2216,0.5206079483032227,0.0010432292019686429
355,1112,1112,2224,0.5222969055175781,0.0010413427842195233
356,1114,1114,2228,0.5234568119049072,0.0009379308415873311
357,1116,1116,2232,0.5244317054748535,0.0009690133158528624
358,1120,1120,2240,0.5260210037231445,0.0009698730060563321
359,1122,1122,2244,0.5270998477935791,0.0007656827336859351
360,1126,1126,2252,0.528846025466919,0.0007627885324836825
361,1128,1128,2256,0.5299897193908691,0.0006824496250601442
362,1132,1132,2264,0.5316469669342041,0.0006827453945561501
363,1134,1134,2268,0.5328118801116943,0.000710093037923798
364,1136,1136,2272,0.5339057445526123,0.0007159102344758139
365,1140,1140,2280,0.5355219841003418,0.0007156880801630905
366,1142,1142,2284,0.5365757942199707,0.0007186215414094477
367,1146,1146,2292,0.5383169651031494,0.0007242524734465405
368,1148,1148,2296,0.539438009262085,0.0007132210423606011
369,1152,1152,2304,0.5411298274993896,0.0007129911109586828
370,1154,1154,2308,0.5421369075775146,0.0007145973704609787
371,1156,1156,2312,0.5431699752807617,0.0006916273342767454
372,1160,1160,2320,0.5448460578918457,0.000691410778131285
373,1162,1162,2324,0.5459837913513184,0.0006693202099086193
374,1166,1166,2332,0.5476510524749756,0.0006689297832735974
375,1168,1168,2336,0.5488450527191162,0.0006408379225604222
376,1172,1172,2344,0.5505459308624268,0.0006399883427548048
377,1174,1174,2348,0.5516228675842285,0.0006064188684149485
378,1178,1178,2356,0.5534529685974121,0.0006062104910142807
379,1180,1180,2360,0.5545799732208252,0.0005725041925188634
380,1184,1184,2368,0.5562517642974854,0.0005695498996374226
381,1188,1188,2376,0.5579738616943359,0.0005664805835294828
382,1190,1190,2380,0.5591049194335938,0.0005412692418076404
383,1194,1194,2388,0.5607731342315674,0.0005407048988672614
384,1196,1196,2392,0.5618698596954346,0.0005206251781828541
385,1200,1200,2400,0.5635890960693359,0.0005203316314918993
386,1202,1202,2404,0.5647079944610596,0.0004865196059427035
387,1206,1206,2412,0.5663449764251709,0.00048635211021519353
388,1208,1208,2416,0.5674459934234619,0.0004703863062331948
389,1212,1212,2424,0.5690689086914062,0.00047006845238684036
390,1214,1214,2428,0.5701498985290527,0.0004538879855999767
391,1218,1218,2436,0.5717818737030029,0.0004524458557852995
392,1220,1220,2440,0.5728259086608887,0.0004461830535547051
393,1224,1224,2448,0.5744328498840332,0.0004460470754565904
394,1226,1226,2452,0.5754878520965576,0.00043044906340128364
395,1228,1228,2456,0.5766057968139648,0.0004198590888790932
396,1232,1232,2464,0.5782630443572998,0.0004196349591438775
397,1234,1234,2468,0.5793099403381348,0.00040597236727535346
398,1238,1238,2476,0.5809609889984131,0.00040617061392822507
399,1242,1242,2484,0.58266282081604,0.00040591005426904303
400,1246,1246,2492,0.5843949317932129,0.0004050892520126581
401,1250,1250,2500,0.5862069129943848,0.00040262266747959075
402,1254,1254,2508,0.5879578590393066,0.0004012647622175791
403,1258,1258,2516,0.5895757675170898,0.000400154734620628
404,1260,1260,2520,0.5906150341033936,0.00036911935876560165
405,1264,1264,2528,0.5924818515777588,0.00036903863281168015
406,1266,1266,2532,0.5937788486480713,0.00035618920105662255
407,1270,1270,2540,0.595465898513794,0.00035601043703081814
408,1272,1272,2544,0.5966000556945801,0.00034578333816170925
409,1276,1276,2552,0.598505973815918,0.0003458306305219594
410,1278,1278,2556,0.5998189449310303,0.0003234764535591239
411,1282,1282,2564,0.601524829864502,0.00032364377557314583
412,1284,1284,2568,0.6026170253753662,0.0003238208300899714
413,1288,1288,2576,0.6042778491973877,0.0003189317455962737
414,1292,1292,2584,0.6058709621429443,0.00031283232158330065
415,1294,1294,2588,0.6068918704986572,0.00028843903737652
416,1298,1298,2596,0.6084928512573242,0.00028803691714074375
417,1300,1300,2600,0.6095919609069824,0.00025929847811312356
418,1304,1304,2608,0.6114108562469482,0.000258920481428504
419,1306,1306,2612,0.6124420166015625,0.00024275955649954994
420,1310,1310,2620,0.6141397953033447,0.0002424792031661127
421,1312,1312,2624,0.6152598857879639,0.00021720905795064027
422,1316,1316,2632,0.6170098781585693,0.00021634213044308126
423,1318,1318,2636,0.618034839630127,0.00019605517945819884
424,1322,1322,2644,0.6195659637451172,0.00019418428917106212
425,1326,1326,2652,0.6211638450622559,0.00019109083177681896
426,1328,1328,2656,0.6222450733184814,0.00016028905122311699
427,1332,1332,2664,0.6238148212432861,0.00016006585735794943
428,1334,1334,2668,0.6248791217803955,0.00013955919973795972
429,1338,1338,2676,0.6264939308166504,0.00014020771266132215
430,1340,1340,2680,0.6275577545166016,0.0001355508503593228
431,1344,1344,2688,0.6292388439178467,0.00013459265687743027
432,1346,1346,2692,0.6302587985992432,0.0001195597285459371
433,1350,1350,2700,0.6319301128387451,0.00011874423330482387
434,1352,1352,2704,0.6330139636993408,8.351353392299643e-05
435,1356,1356,2712,0.6347377300262451,8.322630367274542e-05
436,1358,1358,2716,0.6357967853546143,5.609129743788799e-05
437,1362,1362,2724,0.6374220848083496,5.577578212978551e-05
438,1364,1364,2728,0.6384670734405518,3.922211465123837e-05
439,1368,1368,2736,0.6400139331817627,3.8842967455821054e-05
440,1370,1370,2740,0.6409897804260254,2.082645346490608e-05
441,1374,1374,2748,0.6424939632415771,2.1080664055261877e-05
442,1376,1376,2752,0.6434929370880127,1.9879524643329205e-05
443,1378,1378,2756,0.6445460319519043,1.5597757396790257e-05
444,1380,1380,2760,0.6455578804016113,1.2831606795771222e-05
445,1384,1384,2768,0.6471409797668457,1.2819439575650904e-05
446,1386,1386,2772,0.6481337547302246,1.1442085224189213e-05
447,1390,1390,2780,0.6496989727020264,1.1388267580514366e-05
448,1392,1392,2784,0.6507377624511719,8.61494572745869e-06
449,1396,1396,2792,0.6523020267486572,8.692821324984834e-06
450,1398,1398,2796,0.6533219814300537,1.1486233347568486e-05
451,1402,1402,2804,0.6549417972564697,1.1611519198595488e-05
452,1404,1404,2808,0.6560509204864502,9.78488253622345e-06
453,1408,1408,2816,0.6576719284057617,9.746538466970378e-06
454,1410,1410,2820,0.6586987972259521,4.3941130343228e-06
455,1414,1414,2828,0.6604530811309814,4.340223995313863e-06
456,1416,1416,2832,0.6615748405456543,9.697744189907098e-07
457,1418,1418,2836,0.6626338958740234,9.95300638351182e-07
458,1420,1420,2840,0.6637187004089355,4.734527010441525e-07
459,1422,1422,2844,0.664741039276123,2.6878444714384386e-07
460,1426,1426,2852,0.6663968563079834,2.6967529720423045e-07
461,1428,1428,2856,0.667515754699707,1.0036023923021276e-07
462,1432,1432,2864,0.6692500114440918,9.555753877066309e-08
463,1434,1434,2868,0.6703050136566162,6.447271516663022e-08
464,1436,1436,2872,0.6713290214538574,1.7600518731342163e-07
465,1440,1440,2880,0.6728477478027344,1.7922491224453552e-07
466,1442,1442,2884,0.6738460063934326,3.1787078569323057e-07
467,1446,1446,2892,0.6753509044647217,3.1926504107104847e-07
468,1448,1448,2896,0.676318883895874,2.570556034697802e-07
469,1452,1452,2904,0.6778719425201416,2.586766640888527e-07
470,1454,1454,2908,0.6788840293884277,2.982908426929498e-07
471,1456,1456,2912,0.6798808574676514,2.6638349481800105e-07
472,1460,1460,2920,0.6814918518066406,2.6620455173542723e-07
473,1462,1462,2924,0.6825180053710938,2.716778908506967e-07
474,1466,1466,2932,0.6840648651123047,2.708458168854122e-07
475,1468,1468,2936,0.6850826740264893,2.448339273541933e-07
476,1472,1472,2944,0.6866180896759033,2.388965185673442e-07
477,1474,1474,2948,0.6876001358032227,2.0013283119624248e-07
478,1478,1478,2956,0.6892688274383545,1.9955996322096325e-07
479,1480,1480,2960,0.6903998851776123,1.6573096672800602e-07
480,1484,1484,2968,0.692180871963501,1.6619446796539705e-07
481,1486,1486,2972,0.6932089328765869,1.402786438120529e-07
482,1490,1490,2980,0.6948719024658203,1.4062914033274865e-07
483,1492,1492,2984,0.6959989070892334,1.4943191217753338e-07
484,1494,1494,2988,0.697145938873291,1.57984800353006e-07
485,1498,1498,2996,0.6989238262176514,1.5818750398466364e-07
486,1500,1500,3000,0.7000119686126709,1.3792487152386457e-07
487,1504,1504,3008,0.7017068862915039,1.3722990388487233e-07
488,1506,1506,3012,0.7028217315673828,1.1580789305298822e-07
489,1510,1510,3020,0.7045228481292725,1.1562065083126072e-07
490,1512,1512,3024,0.7055940628051758,1.0055430266220355e-07
491,1516,1516,3032,0.7073509693145752,1.0022256446973188e-07
492,1518,1518,3036,0.708488941192627,9.07494950297405e-08
493,1520,1520,3040,0.7095599174499512,7.892776920925826e-08
494,1524,1524,3048,0.7112476825714111,7.849166649975814e-08
495,1526,1526,3052,0.7123351097106934,5.926051471760729e-08
496,1530,1530,3060,0.7139897346496582,5.915183010074543e-08
497,1532,1532,3064,0.7150099277496338,5.117976797919255e-08
498,1536,1536,3072,0.7166488170623779,5.1282086133142e-08
499,1538,1538,3076,0.7177300453186035,4.882883786194725e-08
500,1542,1542,3084,0.7193589210510254,4.8791207518661395e-08
501,1544,1544,3088,0.7203638553619385,5.1002302825509105e-08
502,1548,1548,3096,0.7220079898834229,5.125855295773363e-08
503,1550,1550,3100,0.7231459617614746,5.200149644224439e-08
504,1554,1554,3108,0.7248361110687256,5.1883830565202516e-08
505,1556,1556,3112,0.7258780002593994,4.9352024689142127e-08
506,1560,1560,3120,0.7275419235229492,4.923424512526253e-08
507,1562,1562,3124,0.7285959720611572,4.8583615352981724e-08
508,1564,1564,3128,0.7296481132507324,5.1394067668297794e-08
509,1568,1568,3136,0.731285810470581,5.139384029462235e-08
510,1570,1570,3140,0.7323451042175293,5.048639195592841e-08
511,1574,1574,3148,0.7339560985565186,5.024367055739276e-08
512,1576,1576,3152,0.7351059913635254,4.620892468665261e-08
513,1580,1580,3160,0.7368428707122803,4.616254045686219e-08
514,1582,1582,3164,0.7382907867431641,4.4338889892969746e-08
515,1586,1586,3172,0.7402360439300537,4.428125066624489e-08
516,1588,1588,3176,0.7414429187774658,4.0221152630692814e-08
517,1592,1592,3184,0.7434649467468262,4.0172039916797075e-08
518,1594,1594,3188,0.7447090148925781,3.649518021120457e-08
519,1598,1598,3196,0.7466080188751221,3.641366674855817e-08
520,1600,1600,3200,0.7477827072143555,3.2361072044295724e-08
521,1604,1604,3208,0.7497110366821289,3.239711077185348e-08
522,1606,1606,3212,0.7510168552398682,3.105628820776474e-08
523,1610,1610,3220,0.7527139186859131,3.09861434288905e-08
524,1612,1612,3224,0.7539377212524414,2.7630335353023838e-08
525,1616,1616,3232,0.7558038234710693,2.7509713618201204e-08
526,1618,1618,3236,0.7569899559020996,2.6181510293099564e-08
527,1622,1622,3244,0.758793830871582,2.58745558312512e-08
528,1626,1626,3252,0.7607729434967041,2.548756583564682e-08
529,1628,1628,3256,0.7623388767242432,2.3176994545792695e-08
530,1632,1632,3264,0.7641468048095703,2.301283075212268e-08
531,1636,1636,3272,0.7658827304840088,2.2868903215567116e-08
532,1638,1638,3276,0.7672328948974609,2.14466808756697e-08
533,1642,1642,3284,0.7693109512329102,2.1369942260207608e-08
534,1646,1646,3292,0.7714920043945312,2.1190885490796063e-08
535,1648,1648,3296,0.7729299068450928,2.1677237782569136e-08
536,1652,1652,3304,0.7753961086273193,2.167257662222255e-08
537,1656,1656,3312,0.777379035949707,2.170077095797751e-08
538,1660,1660,3320,0.7794308662414551,2.1776145331386942e-08
539,1664,1664,3328,0.7815148830413818,2.182230218750192e-08
540,1668,1668,3336,0.7834417819976807,2.1855726117792074e-08
541,1670,1670,3340,0.7845509052276611,2.1796154214825947e-08
542,1674,1674,3348,0.7867147922515869,2.1760001800430473e-08
543,1678,1678,3356,0.788672924041748,2.166893864341546e-08
544,1682,1682,3364,0.7904648780822754,2.160084022762021e-08
545,1686,1686,3372,0.7922537326812744,2.1553432816290297e-08
546,1688,1688,3376,0.7935528755187988,2.1363575797295198e-08
547,1692,1692,3384,0.7954549789428711,2.1364940039347857e-08
548,1696,1696,3392,0.7975778579711914,2.1345158529584296e-08
549,1700,1700,3400,0.7996447086334229,2.1219193513388745e-08
550,1704,1704,3408,0.8018128871917725,2.1121195459272712e-08
551,1708,1708,3416,0.803865909576416,2.103377028106479e-08
552,1712,1712,3424,0.8057169914245605,2.0959760149708018e-08
553,1716,1716,3432,0.8077778816223145,2.0901325115119107e-08
554,1720,1720,3440,0.809751033782959,2.0824359125981573e-08
555,1724,1724,3448,0.8115129470825195,2.075375959975645e-08
556,1728,1728,3456,0.8134660720825195,2.0626771402021404e-08
557,1732,1732,3464,0.8154327869415283,2.0541506273730192e-08
558,1736,1736,3472,0.8173727989196777,2.0509446585492697e-08
559,1740,1740,3480,0.8192570209503174,2.045135261141695e-08
560,1744,1744,3488,0.8211019039154053,2.0329366634541657e-08
561,1748,1748,3496,0.8230819702148438,2.023455181188183e-08
562,1752,1752,3504,0.8248398303985596,2.009880972764222e-08
563,1756,1756,3512,0.8268420696258545,2.001240773097379e-08
564,1760,1760,3520,0.8288378715515137,1.9916342353099026e-08
565,1764,1764,3528,0.8306670188903809,1.979572061827639e-08
566,1768,1768,3536,0.832460880279541,1.9626440916908905e-08
567,1772,1772,3544,0.8345730304718018,1.9470121515041683e-08
568,1776,1776,3552,0.8366110324859619,1.9124740902043413e-08
569,1780,1780,3560,0.8384718894958496,1.887121925392421e-08
570,1784,1784,3568,0.840634822845459,1.8325522432860453e-08
571,1788,1788,3576,0.8426821231842041,1.7929437490238342e-08
572,1792,1792,3584,0.8444609642028809,1.733349108690163e-08
573,1796,1796,3592,0.8465089797973633,1.6911712918954436e-08
574,1798,1798,3596,0.8479509353637695,1.468401933379937e-08
575,1802,1802,3604,0.8498799800872803,1.4437546269618906e-08
576,1806,1806,3612,0.851815938949585,1.4285546967585105e-08
577,1810,1810,3620,0.8538920879364014,1.4034185369382612e-08
578,1814,1814,3628,0.8558859825134277,1.3768953976978082e-08
579,1818,1818,3636,0.8576908111572266,1.3317730918060988e-08
580,1822,1822,3644,0.8596620559692383,1.290425188926747e-08
581,1826,1826,3652,0.8615458011627197,1.2113673619751353e-08
582,1830,1830,3660,0.8633708953857422,1.1212819117645267e-08
583,1832,1832,3664,0.8645498752593994,6.931600182724651e-09
584,1836,1836,3672,0.8670179843902588,6.8890813054167666e-09
585,1838,1838,3676,0.8683187961578369,3.9202632251544856e-09
586,1842,1842,3684,0.8700878620147705,3.88752141589066e-09
587,1846,1846,3692,0.8721320629119873,3.5196308090235107e-09
588,1848,1848,3696,0.8740339279174805,6.559730536537245e-10


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.00524592399597168,7527.142345757873
1001,2004,1002,3006,6.168606996536255,16.46376997585321
2002,4006,2003,6009,12.14425015449524,8.48514545168473
3003,6008,3004,9012,18.24251127243042,5.4522030773732695
4004,8010,4005,12015,24.106975078582764,3.9980777974433295
5005,10012,5006,15018,29.91569423675537,3.2173101267435413
6006,12014,6007,18021,35.73200798034668,2.7275645622394222
7007,14016,7008,21024,41.512919187545776,2.38735138289303
8008,16018,8009,24027,47.32386517524719,2.137019590698401
9009,18020,9010,27030,53.11449313163757,1.9399264741477964
10010,20022,10011,30033,58.97867703437805,1.7806732271183137
11011,22024,11012,33036,64.76487708091736,1.64475708925238
12012,24026,12013,36039,70.53877305984497,1.5329695017062477
13013,26028,13014,39042,76.28334903717041,1.4313600407931517
14014,28030,14015,42045,82.13335514068604,1.3467990983663185
15015,30032,15016,45048,87.98540592193604,1.2695771070029878
16016,32034,16017,48051,93.76351428031921,1.2018053093252092
17017,34036,17018,51054,99.60527801513672,1.1412659763827833
18018,36038,18019,54057,105.37843012809753,1.0865616033352126
19019,38040,19020,57060,111.21037697792053,1.0363326272981794
20020,40042,20021,60063,116.97914600372314,0.9916556226835382
21021,42044,21022,63066,122.7497091293335,0.9495090873260779
22022,44046,22023,66069,128.66459393501282,0.9115858801906143
23023,46048,23024,69072,134.3967580795288,0.877056067380181
24024,48050,24025,72075,140.2061471939087,0.8451090230355476
25025,50052,25026,75078,145.9766411781311,0.8151736349973362
26026,52054,26027,78081,151.76988124847412,0.7869517771960091
27027,54056,27028,81084,157.5638689994812,0.7602290669910872
28028,56058,28029,84087,163.4388620853424,0.735708273246928
29029,58060,29030,87090,169.26375722885132,0.7121296809018531
30030,60062,30031,90093,175.04315185546875,0.6905402140364458
31031,62064,31032,93096,180.84079504013062,0.6703500710937078
32032,64066,32033,96099,186.63061213493347,0.6510288220470102
33033,66068,33034,99102,192.45882201194763,0.6329364259781869
34034,68070,34035,102105,198.23517107963562,0.6157365104427299
35035,70072,35036,105108,203.9878900051117,0.5997400469223066
36036,72074,36037,108111,209.87749814987183,0.5843394932417141
37037,74076,37038,111114,215.65209817886353,0.5701002409387002
38038,76078,38039,114117,221.43722200393677,0.5562435481333523
39039,78080,39040,117120,227.19230103492737,0.5430425883459975
40040,80082,40041,120123,233.01116108894348,0.5305780116959795
41041,82084,41042,123126,238.94111013412476,0.5185390485494281
42042,84086,42043,126129,244.76317715644836,0.5072552916171844
43043,86088,43044,129132,250.5651650428772,0.4962846578055178
44044,88090,44045,132135,256.3382570743561,0.48589304602319316
45045,90092,45046,135138,262.2057890892029,0.4758671649124153
46046,92094,46047,138141,267.9462721347809,0.4663324039956933
47047,94096,47048,141144,273.74216508865356,0.4569982888951927
48048,96098,48049,144147,279.5212941169739,0.4481513049413479
49049,98100,49050,147150,285.2787630558014,0.43959602992799773
50050,100102,50051,150153,291.09027004241943,0.431607653537867
51051,102104,51052,153156,297.9381971359253,0.4236732652934734
52052,104106,52053,156159,303.48277401924133,0.41604045004532964
53053,106108,53054,159162,309.9316899776459,0.40859352535517246
54054,108110,54055,162165,316.2691740989685,0.40153939770425495
55055,110112,55056,165168,322.24494218826294,0.39457191845758643
56056,112114,56057,168171,328.1630132198334,0.38793356851783756
57057,114116,57058,171174,334.04368710517883,0.381523024305352
58058,116118,58059,174177,339.9151072502136,0.37542893896170426
59059,118120,59060,177180,345.74056100845337,0.3694781871927262
60060,120122,60061,180183,351.6556251049042,0.3637528583785752
61061,122124,61062,183186,357.6218190193176,0.35815365635426133
62062,124126,62063,186189,363.54300713539124,0.3527254153850663
63063,126128,63064,189192,369.41697907447815,0.3475516497474018
64064,128130,64065,192195,375.2745580673218,0.34242750683188206
65065,130132,65066,195198,381.07727909088135,0.3374594798333419
66066,132134,66067,198201,386.9293520450592,0.33262222276789544
67067,134136,67068,201204,392.7728269100189,0.3279226611593913
68068,136138,68069,204207,398.6041691303253,0.3234091668509791
69069,138140,69070,207210,404.70667123794556,0.3189813873850653
70070,140142,70071,210213,410.66291403770447,0.31460257780418033
71071,142144,71072,213216,416.9275121688843,0.31034069715497026
72072,144146,72073,216219,423.00449109077454,0.3062337285737158
73073,146148,73074,219222,428.8713710308075,0.30216377187934995
74074,148150,74075,222225,434.77087211608887,0.2983859369469428
75075,150152,75076,225228,440.6241149902344,0.29462508189499204
76076,152154,76077,228231,446.56535816192627,0.29096924982150085
77077,154156,77078,231234,452.37340211868286,0.28738530382725
78078,156158,78079,234237,458.14507508277893,0.28395255386385543
79079,158160,79080,237240,463.93813824653625,0.28057875588820025
80080,160162,80081,240243,469.7409780025482,0.2773005547169305
81081,162164,81082,243246,475.649729013443,0.27411371492962644
82082,164166,82083,246249,481.6122341156006,0.2709244806155766
83083,166168,83084,249252,487.4238700866699,0.26782627534339554
84084,168170,84085,252255,493.2290802001953,0.26481245578725066
85085,170172,85086,255258,499.08647990226746,0.26189055474242195
86086,172174,86087,258261,504.90303897857666,0.2589671402984095
87087,174176,87088,261264,510.8341152667999,0.25615314841525105
88088,176178,88089,264267,516.8106181621552,0.25336892163068114
89089,178180,89090,267270,522.6526551246643,0.2506037342845957
90090,180182,90091,270273,528.4534130096436,0.2479660567078099
91091,182184,91092,273276,534.2943832874298,0.24535204203675676
92092,184186,92093,276279,540.1380190849304,0.24281136033641815
93093,186188,93094,279282,545.9092390537262,0.24031717427533295
94094,188190,94095,282285,551.7672262191772,0.23791486212758173
95095,190192,95096,285288,557.5621240139008,0.23557761193478655
96096,192194,96097,288291,563.5387961864471,0.23322848237330618
97097,194196,97098,291294,569.3846161365509,0.23097349975250836
98098,196198,98099,294297,575.1747100353241,0.22871175598447735
99099,198200,99100,297300,580.9693460464478,0.22651056759787025
100100,200202,100101,300303,586.7766761779785,0.2243398152604641
101101,202204,101102,303306,592.6336052417755,0.22225886511296267
102102,204206,102103,306309,598.587249994278,0.2201789136215666
103103,206208,103104,309312,604.403774023056,0.21813595217281545
104104,208210,104105,312315,610.1745111942291,0.21609461194384494
105105,210212,105106,315318,616.0392909049988,0.21412555549977697
106106,212214,106107,318321,621.863254070282,0.21220098950834654
107107,214216,107108,321324,627.7097799777985,0.21033715482553816
108108,216218,108109,324327,633.5544030666351,0.20848555167685845
109109,218220,109110,327330,639.4589982032776,0.206694627444449
110110,220222,110111,330333,645.4049742221832,0.20489045552494645
111111,222224,111112,333336,651.2468740940094,0.20314364079422376
112112,224226,112113,336339,657.0266292095184,0.2014319482823339
113113,226228,113114,339342,662.8539600372314,0.1997364304279472
114114,228230,114115,342345,668.6839220523834,0.19806727497052634
115115,230232,115116,345348,674.580982208252,0.1964416926384729
116116,232234,116117,348351,680.4787971973419,0.19482293022156227
117117,234236,117118,351354,686.2968010902405,0.19323625365541375
118118,236238,118119,354357,692.1360692977905,0.19167494523935602
119119,238240,119120,357360,698.0135760307312,0.19015523517919064
120120,240242,120121,360363,703.972188949585,0.18865374462438922
121121,242244,121122,363366,709.875324010849,0.1871780400415446
122122,244246,122123,366369,715.6924180984497,0.18570897196696023
123123,246248,123124,369372,721.5590920448303,0.1842725486476411
124124,248250,124125,372375,727.3816781044006,0.1828258320256282
125125,250252,125126,375378,733.2056610584259,0.18138803901274514
126126,252254,126127,378381,739.2799570560455,0.18003050685183553
127127,254256,127128,381384,745.5255081653595,0.1786724548037455
128128,256258,128129,384387,751.3979971408844,0.1773289959110116
129129,258260,129130,387390,757.2427341938019,0.17602107230050024
130130,260262,130131,390393,763.0745980739594,0.1747086486338958
131131,262264,131132,393396,768.9903528690338,0.1734299444106
132132,264266,132133,396399,774.8265380859375,0.1721219385508448
133133,266268,133134,399402,780.6700301170349,0.17089104805381794
134134,268270,134135,402405,786.5174779891968,0.16968282992820605
135135,270272,135136,405408,792.45055103302,0.1684859566648811
136136,272274,136137,408411,798.2634990215302,0.16730126798756828
137137,274276,137138,411414,804.1004440784454,0.16612494951368717
138138,276278,138139,414417,809.884485244751,0.1649727831572818
139139,278280,139140,417420,815.7493410110474,0.1638340034878638
140140,280282,140141,420423,821.5696032047272,0.16272632714390056
141141,282284,141142,423426,827.3581142425537,0.16161944784835214
142142,284286,142143,426429,833.1705439090729,0.16054115742372232
143143,286288,143144,429432,839.0296010971069,0.15947271819823072
144144,288290,144145,432435,844.7957079410553,0.1584072389141511
145145,290292,145146,435438,850.4965331554413,0.15736335196379514
146146,292294,146147,438441,856.3133089542389,0.15631539871174027
147147,294296,147148,441444,862.1683280467987,0.15528106102101447
148148,296298,148149,444447,868.0054430961609,0.15427053528219403
149149,298300,149150,447450,873.8361251354218,0.15326301211644022
150150,300302,150151,450453,879.6572659015656,0.15227312663591874
151151,302304,151152,453456,885.4280421733856,0.15129672681177908
152152,304306,152153,456459,891.2643671035767,0.15033360670167895
153153,306308,153154,459462,897.0654480457306,0.14939380004580016
154154,308310,154155,462465,902.858724117279,0.14847284101051628
155155,310312,155156,465468,908.7203199863434,0.1475671823573066
156156,312314,156157,468471,914.6176111698151,0.14666071593092056
157157,314316,157158,471474,920.4799330234528,0.14574198285481543
158158,316318,158159,474477,926.3533620834351,0.1448546393057768
159159,318320,159160,477480,932.2089102268219,0.1439816642068763
160160,320322,160161,480483,938.1609301567078,0.14311205737976707
161161,322324,161162,483486,944.1884090900421,0.14225166074902518
162162,324326,162163,486489,950.0822122097015,0.14140785408199008
163163,326328,163164,489492,955.968670129776,0.14058788203874428
164164,328330,164165,492495,961.7843980789185,0.1397537621378433
165165,330332,165166,495498,967.5312662124634,0.13892438611219404
166166,332334,166167,498501,973.4250330924988,0.13812109531863825
167167,334336,167168,501504,979.319258928299,0.1373220195146132
168168,336338,168169,504507,985.1604082584381,0.1365360792278807
169169,338340,169170,507510,991.0741770267487,0.13576560800174775
170170,340342,170171,510513,996.895809173584,0.13500098550503026
171171,342344,171172,513516,1002.8029279708862,0.13424315989141178
172172,344346,172173,516519,1008.7429718971252,0.1334929506538174
173173,346348,173174,519522,1014.589497089386,0.13274187100614654
174174,348350,174175,522525,1020.5476880073547,0.13201288876734907
175175,350352,175176,525528,1026.4447031021118,0.13128923337535525
176176,352354,176177,528531,1032.3322150707245,0.13057848890275636
177177,354356,177178,531534,1038.1987462043762,0.12986629625629575
178178,356358,178179,534537,1044.0202810764313,0.12915547236116254
179179,358360,179180,537540,1049.9380490779877,0.12844716732979578
180180,360362,180181,540543,1055.821984052658,0.1277780954605987
181181,362364,181182,543546,1061.6632919311523,0.12707861620219774
182182,364366,182183,546549,1067.5321350097656,0.12640898462632322
183183,366368,183184,549552,1073.388952255249,0.12572043267573463
184184,368370,184185,552555,1079.400316953659,0.1250525660761923
185185,370372,185186,555558,1085.283503293991,0.12438902801113727
186186,372374,186187,558561,1091.1273910999298,0.12373923060658854
187187,374376,187188,561564,1097.0987479686737,0.12308724256945425
188188,376378,188189,564567,1102.96107006073,0.12244923271828156
189189,378380,189190,567570,1108.9395761489868,0.12180293255005381
190190,380382,190191,570573,1114.8520991802216,0.12117851017137582
191191,382384,191192,573576,1120.8473238945007,0.12054525416897377
192192,384386,192193,576579,1126.7932271957397,0.11993042180074553
193193,386388,193194,579582,1132.6801800727844,0.11930579677937203
194194,388390,194195,582585,1138.6787781715393,0.11867665530371596
195195,390392,195196,585588,1144.6325929164886,0.11808030541033077
196196,392394,196197,588591,1150.6567749977112,0.1174868297039211
197197,394396,197198,591594,1156.7400221824646,0.11687776174039755
198198,396398,198199,594597,1162.7759351730347,0.11630022701683629
199199,398400,199200,597600,1168.7674300670624,0.11572282843917492
200200,400402,200201,600603,1174.7755601406097,0.11514303961484984
201201,402404,201202,603606,1180.8318181037903,0.11457309933575743
202202,404406,202203,606609,1186.9059360027313,0.114010908317141
203203,406408,203204,609612,1192.9139821529388,0.11344295977323782
204204,408410,204205,612615,1198.9909970760345,0.11291881792385539
205205,410412,205206,615618,1204.9287309646606,0.11236807519344438
206206,412414,206207,618621,1210.997976064682,0.11183847311440331
207207,414416,207208,621624,1217.000277042389,0.11130251501344901
208208,416418,208209,624627,1222.9151151180267,0.11081021855898143
209209,418420,209210,627630,1228.8720951080322,0.11032931312001892
210210,420422,210211,630633,1234.8411331176758,0.10985254619845364
211211,422424,211212,633636,1240.7472982406616,0.10937979298796563
212212,424426,212213,636639,1246.6459341049194,0.10891093902864668
213213,426428,213214,639642,1252.6315469741821,0.10844587018618768
214214,428430,214215,642645,1258.6628329753876,0.10798446310400323
215215,430432,215216,645648,1264.594978094101,0.10752847626281437
216216,432434,216217,648651,1270.5260150432587,0.10707407495101506
217217,434436,217218,651654,1276.4392330646515,0.10662463740845851
218218,436438,218219,654657,1282.4797179698944,0.10617938954965211
219219,438440,219220,657660,1288.4002392292023,0.1057380052661756
220220,440442,220221,660663,1294.2937080860138,0.10530145844677463
221221,442444,221222,663666,1300.2251431941986,0.10484576932503842
222222,444446,222223,666669,1306.1267850399017,0.10435579082513868
223223,446448,223224,669672,1311.997267961502,0.10388100361160468
224224,448450,224225,672675,1317.9537770748138,0.10341459934170416
225225,450452,225226,675678,1323.8784720897675,0.10295467936884961
226226,452454,226227,678681,1329.8209171295166,0.10249081004440086
227227,454456,227228,681684,1335.763337135315,0.10202284718252486
228228,456458,228229,684687,1341.7797739505768,0.10157631143374601
229229,458460,229230,687690,1347.705164194107,0.10113154560349358
230230,460462,230231,690693,1353.5927832126617,0.10072797022257873
231231,462464,231232,693696,1359.5377600193024,0.10032745263197285
232232,464466,232233,696699,1365.449522972107,0.09992631787645223
233233,466468,233234,699702,1371.4506969451904,0.09952902292752697
234234,468470,234235,702705,1377.5097212791443,0.09913757622780395
235235,470472,235236,705708,1383.4411380290985,0.09875438753078924
236236,472474,236237,708711,1389.5388760566711,0.09832427443325287
237237,474476,237238,711714,1395.5064570903778,0.09790229306236142
238238,476478,238239,714717,1401.4664211273193,0.09747594391046732
239239,478480,239240,717720,1407.5031850337982,0.09705977148951206
240240,480482,240241,720723,1413.4592640399933,0.09663849666321767
241241,482484,241242,723726,1419.4675650596619,0.09622808482163236
242242,484486,242243,726729,1425.402330160141,0.09582709879214235
243243,486488,243244,729732,1431.3182458877563,0.09543003208818845
244244,488490,244245,732735,1437.3187379837036,0.09504475825815462
245245,490492,245246,735738,1443.2808289527893,0.09466365915614006
246246,492494,246247,738741,1449.2068700790405,0.09428639578982256
247247,494496,247248,741744,1455.1236202716827,0.09391276008136629
248248,496498,248249,744747,1461.071527004242,0.0935426774667576
249249,498500,249250,747750,1467.0196371078491,0.09317689506679017
250250,500502,250251,750753,1472.9241499900818,0.09281490913963353
251251,502504,251252,753756,1478.8638000488281,0.0924558951119252
252252,504506,252253,756759,1484.8179032802582,0.09210093125511776
253253,506508,253254,759762,1490.8700449466705,0.09174903343046026
254254,508510,254255,762765,1496.7930450439453,0.09139891977974912
255255,510512,255256,765768,1502.811734199524,0.09103830885760544
256256,512514,256257,768771,1508.724797964096,0.09067902943206718
257257,514516,257258,771774,1514.6530921459198,0.09032073061644041
258258,516518,258259,774777,1520.6287100315094,0.08996952444613271
259259,518520,259260,777780,1526.5969212055206,0.08962440159120888
260260,520522,260261,780783,1532.680652141571,0.08930525962932734
261261,522524,261262,783786,1538.6755661964417,0.08898871089695604
262262,524526,262263,786789,1544.7528729438782,0.0886754129514884
263263,526528,263264,789792,1550.788110256195,0.08836552932916675
264264,528530,264265,792795,1556.843961238861,0.08805941365972103
265265,530532,265266,795798,1562.8320331573486,0.08774605611870356
266266,532534,266267,798801,1568.8394770622253,0.08742265405817307
267267,534536,267268,801804,1574.833547115326,0.08708969907820574
268268,536538,268269,804807,1580.8308591842651,0.08676268521776365
269269,538540,269270,807810,1586.6785650253296,0.086432469990541
270270,540542,270271,810813,1592.585371017456,0.08610809290257748
271271,542544,271272,813816,1598.5943429470062,0.08578260872855026
272272,544546,272273,816819,1604.490956068039,0.08546084996305581
273273,546548,273274,819822,1610.413066148758,0.08513591253176855
274274,548550,274275,822825,1616.326093196869,0.08481708764338691
275275,550552,275276,825828,1622.2342081069946,0.08450090117185027
276276,552554,276277,828831,1628.0799779891968,0.0841862701709033
277277,554556,277278,831834,1633.9400792121887,0.08387538214810775
278278,556558,278279,834837,1639.869933128357,0.08355503254642827
279279,558560,279280,837840,1645.7473359107971,0.08324913440264936
280280,560562,280281,840843,1651.6712760925293,0.08293985928503389
281281,562564,281282,843846,1657.6738390922546,0.08263716535293497
282282,564566,282283,846849,1663.5592761039734,0.08233613666379824
283283,566568,283284,849852,1669.4589629173279,0.0820272650289553
284284,568570,284285,852855,1675.3732821941376,0.08173515734779357
285285,570572,285286,855858,1681.3507242202759,0.08144499394620652
286286,572574,286287,858861,1687.2704389095306,0.08116325298760785
287287,574576,287288,861864,1693.2577753067017,0.08087118736875709
288288,576578,288289,864867,1699.1739621162415,0.08059296972896846
289289,578580,289290,867870,1704.505851984024,0.08030881610466167
290290,580582,290291,870873,1709.628072977066,0.08002719546675507
291291,582584,291292,873876,1715.301931142807,0.07974968731286936
292292,584586,292293,876879,1721.3011021614075,0.0794773135894502
293293,586588,293294,879882,1727.2347221374512,0.07920218691106129
294294,588590,294295,882885,1733.1739451885223,0.07892955125680601
295295,590592,295296,885888,1739.1086852550507,0.07866142302736989
296296,592594,296297,888891,1745.0239770412445,0.07839333750052901
297297,594596,297298,891894,1750.9227540493011,0.0781235255599313
298298,596598,298299,894897,1756.8907611370087,0.07786317162572232
299299,598600,299300,897900,1762.8684811592102,0.07760599644825561
300300,600602,300301,900903,1768.8545689582825,0.07734371792685124
301301,602604,301302,903906,1774.6548750400543,0.07708481636473152
302302,604606,302303,906909,1780.6342680454254,0.07683821329737839
303303,606608,303304,909912,1786.5210859775543,0.07657845477660885
304304,608610,304305,912915,1792.4065222740173,0.0763233019188192
305305,610612,305306,915918,1798.3217549324036,0.07607083349284949
306306,612614,306307,918921,1804.1827290058136,0.0758287567714433
307307,614616,307308,921924,1810.098687171936,0.0755809684706037
308308,616618,308309,924927,1816.0868968963623,0.07533095331018558
309309,618620,309310,927930,1821.9811289310455,0.07508620026055723
310310,620622,310311,930933,1827.8422951698303,0.07484861741068016
311311,622624,311312,933936,1833.9309849739075,0.07461206399784714
312312,624626,312313,936939,1839.9085240364075,0.07437094065608107
313313,626628,313314,939942,1845.8512151241302,0.0741304615385161
314314,628630,314315,942945,1851.7970950603485,0.07389385086753464
315315,630632,315316,945948,1857.9082400798798,0.07365278374163609
316316,632634,316317,948951,1864.3657631874084,0.07341957479002303
317317,634636,317318,951954,1870.3236110210419,0.07319258436837117
318318,636638,318319,954957,1876.2774951457977,0.0729652427653491
319319,638640,319320,957960,1882.1805529594421,0.07273982718288607
320320,640642,320321,960963,1888.0865211486816,0.0725208781332185
321321,642644,321322,963966,1894.0013890266418,0.07229974071560719
322322,644646,322323,966969,1899.8574981689453,0.07207615140396229
323323,646648,323324,969972,1905.7969710826874,0.07184895607315411
324324,648650,324325,972975,1911.763034105301,0.07163645474975056
325325,650652,325326,975978,1917.7012190818787,0.07141815992326883
326326,652654,326327,978981,1923.6718490123749,0.07119859490376257
327327,654656,327328,981984,1929.5698170661926,0.07098062742807087
328328,656658,328329,984987,1935.4837939739227,0.07076166092883795
329329,658660,329330,987990,1941.3302690982819,0.07054840333148604
330330,660662,330331,990993,1947.2470469474792,0.07033354612758558
331331,662664,331332,993996,1953.1199660301208,0.07012106515321648
332332,664666,332333,996999,1958.995414018631,0.06991313997423276
333333,666668,333334,1000002,1964.9297530651093,0.0697044514818117
334334,668670,334335,1003005,1970.873946905136,0.06949276062186982
335335,670672,335336,1006008,1976.7221100330353,0.06928862006679992
336336,672674,336337,1009011,1982.6042120456696,0.06908105703405454
337337,674676,337338,1012014,1988.5642802715302,0.06887636077408388
338338,676678,338339,1015017,1994.5668742656708,0.06867409212100029
339339,678680,339340,1018020,2000.4918069839478,0.0684678822526621
340340,680682,340341,1021023,2006.4442460536957,0.06826474136323668
341341,682684,341342,1024026,2012.3350450992584,0.0680618735968892
342342,684686,342343,1027029,2018.3486022949219,0.06786254041799111
343343,686688,343344,1030032,2024.4026391506195,0.0676639480261656
344344,688690,344345,1033035,2030.3523721694946,0.06746002767977188
345345,690692,345346,1036038,2036.3521921634674,0.06726198054639099
346346,692694,346347,1039041,2042.280667066574,0.06706750419471064
347347,694696,347348,1042044,2048.326975107193,0.066876542978207
348348,696698,348349,1045047,2054.294336080551,0.06668445972900372
349349,698700,349350,1048050,2060.2489941120148,0.06648998583114007
350350,700702,350351,1051053,2066.280365228653,0.06630165760361706
351351,702704,351352,1054056,2072.227772951126,0.0661092765367357
352352,704706,352353,1057059,2078.148968935013,0.06591861234846874
353353,706708,353354,1060062,2084.042031288147,0.06572941586273373
354354,708710,354355,1063065,2089.964005947113,0.06553960581368301
355355,710712,355356,1066068,2095.904265165329,0.06535486467146256
356356,712714,356357,1069071,2101.795996904373,0.06517242415975488
357357,714716,357358,1072074,2107.6846611499786,0.06499041770075564
358358,716718,358359,1075077,2113.598596096039,0.06480684388588998
359359,718720,359360,1078080,2119.5634639263153,0.06462413651570387
360360,720722,360361,1081083,2125.8356630802155,0.0644431909568084
361361,722724,361362,1084086,2131.844194173813,0.06426216645741079
362362,724726,362363,1087089,2137.916430234909,0.06408413041936001
363363,726728,363364,1090092,2144.131779193878,0.0639103135872574
364364,728730,364365,1093095,2150.118113040924,0.06373443791198952
365365,730732,365366,1096098,2156.081029891968,0.06355856878872146
366366,732734,366367,1099101,2162.126820087433,0.06338433353448636
367367,734736,367368,1102104,2168.161299943924,0.06321349834433931
368368,736738,368369,1105107,2174.1346802711487,0.06303813353588339
369369,738740,369370,1108110,2180.003762960434,0.06286396560244611
370370,740742,370371,1111113,2185.9210419654846,0.0626958566281246
371371,742744,371372,1114116,2191.818237066269,0.06253027038292203
372372,744746,372373,1117119,2197.7643570899963,0.062364386749322875
373373,746748,373374,1120122,2203.665239095688,0.06219609163053974
374374,748750,374375,1123125,2209.553209066391,0.06203069273033179
375375,750752,375376,1126128,2215.4358270168304,0.06186887847434264
376376,752754,376377,1129131,2221.3088772296906,0.06170462828413292
377377,754756,377378,1132134,2227.2660870552063,0.0615429263907572
378378,756758,378379,1135137,2233.176374197006,0.06138324157655006
379379,758760,379380,1138140,2239.078533887863,0.06122056769163464
380380,760762,380381,1141143,2244.98286318779,0.061060298274242086
381381,762764,381382,1144146,2250.9499220848083,0.06089997234994371
382382,764766,382383,1147149,2256.8421483039856,0.06074177138725645
383383,766768,383384,1150152,2262.726500272751,0.06058353701882879
384384,768770,384385,1153155,2268.732104063034,0.060425492674767156
385385,770772,385386,1156158,2274.6438250541687,0.06027115297183627
386386,772774,386387,1159161,2280.6497790813446,0.06011649212632619
387387,774776,387388,1162164,2286.562005996704,0.05996089937252691
388388,776778,388389,1165167,2292.5477471351624,0.05981137978233164
389389,778780,389390,1168170,2298.5685069561005,0.0596585690836946
390390,780782,390391,1171173,2304.5329480171204,0.059503706952455104
391391,782784,391392,1174176,2310.478861093521,0.05935099839916802
392392,784786,392393,1177179,2316.526116132736,0.05920296025396965
393393,786788,393394,1180182,2322.5645229816437,0.05905186197742296
394394,788790,394395,1183185,2328.503087282181,0.058905144844175084
395395,790792,395396,1186188,2334.487225294113,0.05876187886497064
396396,792794,396397,1189191,2340.4059200286865,0.05861598527008027
397397,794796,397398,1192194,2346.3096170425415,0.05846905468933983
398398,796798,398399,1195197,2352.311109304428,0.05831840244172781
399399,798800,399400,1198200,2358.2245061397552,0.05817658436171769
400400,800802,400401,1201203,2364.1550509929657,0.05802870439947583
401401,802804,401402,1204206,2370.3334851264954,0.05788594532714342
402402,804806,402403,1207209,2375.9354209899902,0.05774257010125439
403403,806808,403404,1210212,2381.9594881534576,0.05759940478128556
404404,808810,404405,1213215,2387.930227994919,0.05745639806809777
405405,810812,405406,1216218,2393.793522119522,0.05731584597560868
406406,812814,406407,1219221,2399.81667304039,0.0571784624717111
407407,814816,407408,1222224,2405.698226928711,0.057049580123930355
408408,816818,408409,1225227,2411.54251909256,0.05692172511771787
409409,818820,409410,1228230,2417.625330924988,0.05679364110255847
410410,820822,410411,1231233,2423.5695021152496,0.056659400535863824
411411,822824,411412,1234236,2429.4947090148926,0.05652243381518929
412412,824826,412413,1237239,2435.557604074478,0.056386978956652456
413413,826828,413414,1240242,2441.456197977066,0.05625231519297813
414414,828830,414415,1243245,2447.376570224762,0.05611906938429456
415415,830832,415416,1246248,2453.292067050934,0.05598508734328789
416416,832834,416417,1249251,2459.4163432121277,0.05585262438034988
417417,834836,417418,1252254,2465.6939358711243,0.055722046352457255
418418,836838,418419,1255257,2472.204980134964,0.05558753363038704
419419,838840,419420,1258260,2478.288994073868,0.055454057293900405
420420,840842,420421,1261263,2484.2081310749054,0.05532098433468491
421421,842844,421422,1264266,2490.228786945343,0.055191688170452835
422422,844846,422423,1267269,2496.140745162964,0.055061135533833294
423423,846848,423424,1270272,2502.0654039382935,0.05493047750314872
424424,848850,424425,1273275,2507.9692721366882,0.054796986101791845
425425,850852,425426,1276278,2513.899752140045,0.05466918545971566
426426,852854,426427,1279281,2519.7959990501404,0.05454144629584334
427427,854856,427428,1282284,2525.8249349594116,0.05441804957445129
428428,856858,428429,1285287,2531.7623341083527,0.05429119392465509
429429,858860,429430,1288290,2537.7739520072937,0.05416661803974421
430430,860862,430431,1291293,2543.712461233139,0.054043663358243066
431431,862864,431432,1294296,2549.6032910346985,0.05391968598814856
432432,864866,432433,1297299,2555.561559200287,0.05379620611347491
433433,866868,433434,1300302,2561.5595421791077,0.05367155381463817
434434,868870,434435,1303305,2567.541130065918,0.0535490793408826
435435,870872,435436,1306308,2573.645776987076,0.053427838580319076
436436,872874,436437,1309311,2579.61509513855,0.05330431428956217
437437,874876,437438,1312314,2586.204750061035,0.05318313080533699
438438,876878,438439,1315317,2592.486512899399,0.05306278195894265
439439,878880,439440,1318320,2598.5104882717133,0.052942825943318894
440440,880882,440441,1321323,2604.5373220443726,0.052823980167886475
441441,882884,441442,1324326,2610.451952934265,0.05270596471564204
442442,884886,442443,1327329,2616.5132019519806,0.05258934214543842
443443,886888,443444,1330332,2622.555340051651,0.05247370304095966
444444,888890,444445,1333335,2628.5203750133514,0.05235644180538657
445445,890892,445446,1336338,2634.568125963211,0.05224011053542199
446446,892894,446447,1339341,2640.506739139557,0.05212522271358466
447447,894896,447448,1342344,2646.43731713295,0.05201096651580883
448448,896898,448449,1345347,2652.365769147873,0.05189496102684643
449449,898900,449450,1348350,2658.3147761821747,0.051778363953417283
450450,900902,450451,1351353,2664.2338712215424,0.051660210634508985
451451,902904,451452,1354356,2670.1961691379547,0.0515450945658813
452452,904906,452453,1357359,2676.141201019287,0.05143007588958426
453453,906908,453454,1360362,2682.0624051094055,0.05131820099632023
454454,908910,454455,1363365,2688.0651609897614,0.0512041421388858
455455,910912,455456,1366368,2694.0498299598694,0.05109185014953255
456456,912914,456457,1369371,2699.9741411209106,0.05098231719057367
457457,914916,457458,1372374,2705.9529852867126,0.050869180200606934
458458,916918,458459,1375377,2711.9189240932465,0.05075763394597743
459459,918920,459460,1378380,2717.8745369911194,0.05064701748415246
460460,920922,460461,1381383,2723.7996139526367,0.05053605537250405
461461,922924,461462,1384386,2729.8111340999603,0.05042898747342406
462462,924926,462463,1387389,2735.7359750270844,0.05032007618319767
463463,926928,463464,1390392,2741.6631529331207,0.05021441101234814
464464,928930,464465,1393395,2747.601678133011,0.05010577284701867
465465,930932,465466,1396398,2753.585291147232,0.04999945967392705
466466,932934,466467,1399401,2759.522177219391,0.04989252874474914
467467,934936,467468,1402404,2765.521878004074,0.04978796054820123
468468,936938,468469,1405407,2771.6038661003113,0.0496800280543539
469469,938940,469470,1408410,2777.6479501724243,0.04957539384668053
470470,940942,470471,1411413,2783.581712961197,0.049470438911157544
471471,942944,471472,1414416,2789.5636942386627,0.04936513062239101
472472,944946,472473,1417419,2795.595946073532,0.04926036002325418
473473,946948,473474,1420422,2801.6048760414124,0.04915806332064676
474474,948950,474475,1423425,2807.6218461990356,0.049053221877329634
475475,950952,475476,1426428,2813.5619621276855,0.04894980538119853
476476,952954,476477,1429431,2819.5252690315247,0.04884890140601783
477477,954956,477478,1432434,2825.453663110733,0.048745033867817256
478478,956958,478479,1435437,2831.3599491119385,0.0486444588204904
479479,958960,479480,1438440,2837.3357231616974,0.04854375630202412
480480,960962,480481,1441443,2843.35387301445,0.04844336047426623
481481,962964,481482,1444446,2849.323438167572,0.04834425718217972
482482,964966,482483,1447449,2855.332137107849,0.048243377215840155
483483,966968,483484,1450452,2861.26104927063,0.04814451791025931
484484,968970,484485,1453455,2867.155457019806,0.04804587716898823
485485,970972,485486,1456458,2873.0426802635193,0.04794755062357581
486486,972974,486487,1459461,2879.060882091522,0.047846943754848326
487487,974976,487488,1462464,2884.981786251068,0.04774991593694722
488488,976978,488489,1465467,2890.8400959968567,0.04765333165778429
489489,978980,489490,1468470,2896.7757980823517,0.04755554369694437
490490,980982,490491,1471473,2902.729198217392,0.04746093716858013
491491,982984,491492,1474476,2908.681568145752,0.047363138421133044
492492,984986,492493,1477479,2914.6368551254272,0.04726773676520679
493493,986988,493494,1480482,2920.6555330753326,0.04717168743991351
494494,988990,494495,1483485,2926.680925130844,0.04707814436915214
495495,990992,495496,1486488,2932.625396966934,0.04698609881961602
496496,992994,496497,1489491,2938.680324077606,0.046890938649085
497497,994996,497498,1492494,2944.6044211387634,0.04679628144731396
498498,996998,498499,1495497,2950.5620970726013,0.04670223916036775
499499,999000,499500,1498500,2956.5766983032227,0.04660974746548163
500501,1001004,500502,1501506,2962.597633123398,0.04651927880695439
501502,1003006,501503,1504509,2968.6872720718384,0.04642597649944946
502503,1005008,502504,1507512,2974.710160970688,0.0463352082970232
503504,1007010,503505,1510515,2980.6756801605225,0.04624382005385996
504505,1009012,504506,1513518,2986.6660590171814,0.04615378849848639
505506,1011014,505507,1516521,2992.6281139850616,0.04606142116972478
506507,1013016,506508,1519524,2998.64391207695,0.045971269168148865
507508,1015018,507509,1522527,3004.696156978607,0.04588234182665474
508509,1017020,508510,1525530,3010.6606442928314,0.04579399585418287
509510,1019022,509511,1528533,3016.6237618923187,0.04570254935606499
510511,1021024,510512,1531536,3022.7137820720673,0.045613799842612934
511512,1023026,511513,1534539,3028.7531020641327,0.04552274275920354
512513,1025028,512514,1537542,3034.7768211364746,0.04543297012060066
513514,1027030,513515,1540545,3040.8221950531006,0.04534179734218924
514515,1029032,514516,1543548,3046.802710056305,0.04525303141599579
515516,1031034,515517,1546551,3052.940104007721,0.04516509465247509
516517,1033036,516518,1549554,3060.7394630908966,0.04507798487065884
517518,1035038,517519,1552557,3068.93558716774,0.04499163968102948
518519,1037040,518520,1555560,3075.189688205719,0.04490560801968968
519520,1039042,519521,1558563,3081.330871105194,0.04482093913611607
520521,1041044,520522,1561566,3087.3282220363617,0.044736689582350664
521522,1043046,521523,1564569,3093.2577650547028,0.044650701243881485
522523,1045048,522524,1567572,3099.2191441059113,0.044564141773662413
523524,1047050,523525,1570575,3105.1614983081818,0.044480151003881474
524525,1049052,524526,1573578,3111.228073120117,0.04439505249138165
525526,1051054,525527,1576581,3117.5531611442566,0.04430925250380824
526527,1053056,526528,1579584,3123.6795320510864,0.04422400847033714
527528,1055058,527529,1582587,3129.5421481132507,0.044140438754766365
528529,1057060,528530,1585590,3135.4115750789642,0.04405879720252415
529530,1059062,529531,1588593,3141.277333021164,0.043975636775940075
530531,1061064,530532,1591596,3147.123090028763,0.04389280712894106
531532,1063066,531533,1594599,3153.0453419685364,0.043810574961753446
532533,1065068,532534,1597602,3159.0395143032074,0.04372939316635893
533534,1067070,533535,1600605,3165.0097501277924,0.043646740710755694
534535,1069072,534536,1603608,3170.902859210968,0.04356577650651161
535536,1071074,535537,1606611,3176.80842089653,0.043482897390276776
536537,1073076,536538,1609614,3183.115599155426,0.04340059301102883
537538,1075078,537539,1612617,3188.967120885849,0.043319837386661675
538539,1077080,538540,1615620,3194.3522090911865,0.04323661750277097
539540,1079082,539541,1618623,3199.5302650928497,0.04315767664957093
540541,1081084,540542,1621626,3204.618373155594,0.04307813871673716
541542,1083086,541543,1624629,3210.0585169792175,0.04299865288521687
542543,1085088,542544,1627632,3215.3828942775726,0.042919059298583306
543544,1087090,543545,1630635,3220.449171066284,0.042839948859182186
544545,1089092,544546,1633638,3225.5497410297394,0.042761939017509576
545546,1091094,545547,1636641,3231.0326931476593,0.0426828709878464
546547,1093096,546548,1639644,3237.0173971652985,0.04260394779339549
547548,1095098,547549,1642647,3242.901556968689,0.04252577901570476
548549,1097100,548550,1645650,3248.781718015671,0.04244736576038122
549550,1099102,549551,1648653,3254.671226978302,0.04237075705532334
550551,1101104,550552,1651656,3260.807384252548,0.042294648359529674
551552,1103106,551553,1654659,3267.04052901268,0.04221873370624962
552553,1105108,552554,1657662,3273.6114370822906,0.042141632120547
553554,1107110,553555,1660665,3281.308922290802,0.04206663368677255
554555,1109112,554556,1663668,3290.4779970645905,0.041990930014435435
555556,1111114,555557,1666671,3297.7542741298676,0.041915997077012435
556557,1113116,556558,1669674,3304.0784919261932,0.041839885840090574
557558,1115118,557559,1672677,3310.0311748981476,0.04176452657338814
558559,1117120,558560,1675680,3316.412852048874,0.04168990253128868
559560,1119122,559561,1678683,3322.325664997101,0.04161502056012978
560561,1121124,560562,1681686,3328.1804769039154,0.041541722717738594
561562,1123126,561563,1684689,3334.039618253708,0.04146762393247627
562563,1125128,562564,1687692,3339.8243799209595,0.04139204547027475
563564,1127130,563565,1690695,3345.6376490592957,0.04131918354869413
564565,1129132,564566,1693698,3351.477730035782,0.04124503537605051
565566,1131134,565567,1696701,3357.3558530807495,0.04117223726643715
566567,1133136,566568,1699704,3363.208976984024,0.04109838510157715
567568,1135138,567569,1702707,3369.040143251419,0.04102657316434488
568569,1137140,568570,1705710,3374.8628540039062,0.04095401260929066
569570,1139142,569571,1708713,3380.712666988373,0.04088268140912987
570571,1141144,570572,1711716,3386.849002122879,0.0408090242453909
571572,1143146,571573,1714719,3393.157539129257,0.04073773085838184
572573,1145148,572574,1717722,3399.211822271347,0.04066773316844774
573574,1147150,573575,1720725,3405.23007106781,0.04059669014532119
574575,1149152,574576,1723728,3410.8854129314423,0.040526132070226595
575576,1151154,575577,1726731,3416.692671060562,0.04045477314684831
576577,1153156,576578,1729734,3423.2906510829926,0.04038436875816842
577578,1155158,577579,1732737,3429.6005430221558,0.04031454216237762
578579,1157160,578580,1735740,3435.2574441432953,0.040244934789370745
579580,1159162,579581,1738743,3441.461201906204,0.04017431148713513
580581,1161164,580582,1741746,3447.2433862686157,0.04010398217542388
581582,1163166,581583,1744749,3453.2972979545593,0.0400354791963764
582583,1165168,582584,1747752,3459.8349142074585,0.039967050917766755
583584,1167170,583585,1750755,3464.972188949585,0.03989679811456881
584585,1169172,584586,1753758,3470.0490181446075,0.0398273567607248
585586,1171174,585587,1756761,3474.984283924103,0.039758144364896
586587,1173176,586588,1759764,3479.970865011215,0.03969003244674241
587588,1175178,587589,1762767,3484.888617038727,0.03962125495127111
588589,1177180,588590,1765770,3489.79319190979,0.03955461458645004
589590,1179182,589591,1768773,3495.0798070430756,0.03948578804374847
590591,1181184,590592,1771776,3500.033272266388,0.039418102483978146
591592,1183186,591593,1774779,3504.804344177246,0.039350858805846656
592593,1185188,592594,1777782,3509.9119670391083,0.03928486871882342
593594,1187190,593595,1780785,3514.9147679805756,0.03922026494910824
594595,1189192,594596,1783788,3519.8796060085297,0.03915428199979942
595596,1191194,595597,1786791,3524.892657995224,0.03908748959656805
596597,1193196,596598,1789794,3529.8984611034393,0.03902138136618305
597598,1195198,597599,1792797,3534.8296031951904,0.03895522800667095
598599,1197200,598600,1795800,3539.941635131836,0.03889025263379153
599600,1199202,599601,1798803,3544.9198982715607,0.03882451456411218
600601,1201204,600602,1801806,3549.932694196701,0.03876126591785578
601602,1203206,601603,1804809,3554.944319009781,0.038697125726685044
602603,1205208,602604,1807812,3559.9051790237427,0.03863249888672726
603604,1207210,603605,1810815,3564.8627891540527,0.03856902177903976
604605,1209212,604606,1813818,3569.922315120697,0.038504064939843374
605606,1211214,605607,1816821,3574.86705994606,0.03843962889732211
606607,1213216,606608,1819824,3579.847232103348,0.038374294177629054
607608,1215218,607609,1822827,3584.8146851062775,0.038309556292006164
608609,1217220,608610,1825830,3589.86168718338,0.03824494420769042
609610,1219222,609611,1828833,3594.885017156601,0.03818227692863729
610611,1221224,610612,1831836,3599.9008209705353,0.0381183478548337
611612,1223226,611613,1834839,3604.853245973587,0.03805729300074745
612613,1225228,612614,1837842,3609.9081571102142,0.03799485308263684
613614,1227230,613615,1840845,3614.850135087967,0.03793247570138192
614615,1229232,614616,1843848,3619.8242061138153,0.03786974236209062
615616,1231234,615617,1846851,3624.828330039978,0.03780796174942225
616617,1233236,616618,1849854,3629.974016189575,0.03774673260159034
617618,1235238,617619,1852857,3634.977156162262,0.03768504082472646
618619,1237240,618620,1855860,3639.948770046234,0.0376238577591721
619620,1239242,619621,1858863,3644.9480600357056,0.03756248648642213
620621,1241244,620622,1861866,3649.9010860919952,0.03750292582481052
621622,1243246,621623,1864869,3654.8406021595,0.03744205867042183
622623,1245248,622624,1867872,3659.816605091095,0.03738188605711912
623624,1247250,623625,1870875,3664.7868621349335,0.037321148189221276
624625,1249252,624626,1873878,3669.86771607399,0.03726170134359563
625626,1251254,625627,1876881,3674.8679690361023,0.03720386716850044
626627,1253256,626628,1879884,3679.8450360298157,0.0371443303720298
627628,1255258,627629,1882887,3684.9833459854126,0.03708497950901801
628629,1257260,628630,1885890,3690.050763130188,0.03702515874283563
629630,1259262,629631,1888893,3695.003566265106,0.03696585418219911
630631,1261264,630632,1891896,3699.9915022850037,0.036906734450894874
631632,1263266,631633,1894899,3705.062937259674,0.036848843345069326
632633,1265268,632634,1897902,3710.144896030426,0.0367906207775377
633634,1267270,633635,1900905,3715.1525592803955,0.03673170460751862
634635,1269272,634636,1903908,3720.1598279476166,0.03667492161366681
635636,1271274,635637,1906911,3724.9630489349365,0.036615999135392485
636637,1273276,636638,1909914,3729.3396430015564,0.03655905003142834
637638,1275278,637639,1912917,3734.592716217041,0.036500347288892954
638639,1277280,638640,1915920,3739.8798789978027,0.03644093954244454
639640,1279282,639641,1918923,3744.9856810569763,0.03638373286048591
640641,1281284,640642,1921926,3750.261799097061,0.03632488367111364
641642,1283286,641643,1924929,3755.3219542503357,0.036267289413444814
642643,1285288,642644,1927932,3760.295408964157,0.03620929890348634
643644,1287290,643645,1930935,3765.313574075699,0.03615273427203647
644645,1289292,644646,1933938,3770.2671802043915,0.03609747410155251
645646,1291294,645647,1936941,3775.182234287262,0.036040248718563817
646647,1293296,646648,1939944,3779.179750919342,0.035985487107609515
647648,1295298,647649,1942947,3784.522015094757,0.035929204312196816
648649,1297300,648650,1945950,3790.2499561309814,0.03587385927312425
649650,1299302,649651,1948953,3794.720137119293,0.03581786298127554
650651,1301304,650652,1951956,3798.322278022766,0.0357628915735404
651652,1303306,651653,1954959,3801.897190093994,0.035706998212845065
652653,1305308,652654,1957962,3805.469624042511,0.035651909027365036
653654,1307310,653655,1960965,3809.180104970932,0.03559651347131876
654655,1309312,654656,1963968,3812.7691881656647,0.035541880042728735
655656,1311314,655657,1966971,3816.3537380695343,0.03548729385875049
656657,1313316,656658,1969974,3819.932151079178,0.035432135193332215
657658,1315318,657659,1972977,3823.5282020568848,0.03537762440646475
658659,1317320,658660,1975980,3827.176442861557,0.03532349710621929
659660,1319322,659661,1978983,3830.8345742225647,0.03527096624202386
660661,1321324,660662,1981986,3834.4140009880066,0.03521660938895366
661662,1323326,661663,1984989,3837.9917771816254,0.03516227993895882
662663,1325328,662664,1987992,3841.652914047241,0.03510879472560191
663664,1327330,663665,1990995,3845.2410340309143,0.03505533102361369
664665,1329332,664666,1993998,3848.8887600898743,0.03500235488900216
665666,1331334,665667,1997001,3852.5195031166077,0.03494961107389827
666667,1333336,666668,2000004,3856.1175990104675,0.03489756725866755
667668,1335338,667669,2003007,3859.6956810951233,0.03484419893902668
668669,1337340,668670,2006010,3863.2507519721985,0.03479176240398374
669670,1339342,669671,2009013,3866.921201944351,0.03473989867234195
670671,1341344,670672,2012016,3870.5876631736755,0.034687625024162116
671672,1343346,671673,2015019,3874.1893079280853,0.03463577711954713
672673,1345348,672674,2018022,3877.74209523201,0.0345833372866764
673674,1347350,673675,2021025,3881.3364160060883,0.03453101173545292
674675,1349352,674676,2024028,3884.921741247177,0.034479148793252534
675676,1351354,675677,2027031,3888.6097869873047,0.03442735407043074
676677,1353356,676678,2030034,3892.1978759765625,0.034376209005131386
677678,1355358,677679,2033037,3895.844412088394,0.03432541850088455
678679,1357360,678680,2036040,3899.436177968979,0.03427407752315048
679680,1359362,679681,2039043,3903.0028779506683,0.03422227082046447
680681,1361364,680682,2042046,3906.5942752361298,0.034171408085967414
681682,1363366,681683,2045049,3910.2904081344604,0.03412190058224951
682683,1365368,682684,2048052,3913.9116880893707,0.03407152524050616
683684,1367370,683685,2051055,3917.4707729816437,0.034022073581581935
684685,1369372,684686,2054058,3921.05179810524,0.033971513801589026
685686,1371374,685687,2057061,3924.62278008461,0.03392190391969052
686687,1373376,686688,2060064,3928.269376039505,0.0338713330693281
687688,1375378,687689,2063067,3931.8962099552155,0.03382123881056032
688689,1377380,688690,2066070,3935.4907031059265,0.033772317112379824
689690,1379382,689691,2069073,3939.0546209812164,0.03372232394031016
690691,1381384,690692,2072076,3942.662842988968,0.03367301553043944
691692,1383386,691693,2075079,3946.326719045639,0.03362414431285288
692693,1385388,692694,2078082,3949.736554145813,0.0335757369230123
693694,1387390,693695,2081085,3954.087690114975,0.03352559458289761
694695,1389392,694696,2084088,3957.8777759075165,0.03347580746594758
695696,1391394,695697,2087091,3961.3489060401917,0.03342715415783459
696697,1393396,696698,2090094,3965.9299001693726,0.03337950893910602
697698,1395398,697699,2093097,3969.8125581741333,0.0333302716826438
698699,1397400,698700,2096100,3973.391210079193,0.03328111193695804
699700,1399402,699701,2099103,3976.9803841114044,0.033233744754397776
700701,1401404,700702,2102106,3980.549947977066,0.03318540135296644
701702,1403406,701703,2105109,3984.1973209381104,0.033137995093056816
702703,1405408,702704,2108112,3987.790521144867,0.033090087432356086
703704,1407410,703705,2111115,3991.372794151306,0.033042679458958446
704705,1409412,704706,2114118,3995.047255039215,0.032995245541314944
705706,1411414,705707,2117121,3998.6774320602417,0.03294828297839558
706707,1413416,706708,2120124,4002.299446105957,0.03290090647533361
707708,1415418,707709,2123127,4005.9148881435394,0.0328532822913985
708709,1417420,708710,2126130,4009.488953113556,0.032806645220262
709710,1419422,709711,2129133,4013.16197514534,0.03275998151366366
710711,1421424,710712,2132136,4018.6254370212555,0.03271373637835495
711712,1423426,711713,2135139,4024.0498089790344,0.03266729754250264
712713,1425428,712714,2138142,4028.4197912216187,0.032620248219245696
713714,1427430,713715,2141145,4032.0693509578705,0.032574063987340196
714715,1429432,714716,2144148,4035.9808461666107,0.03252797515960992
715716,1431434,715717,2147151,4040.574961900711,0.03248125507343502
716717,1433436,716718,2150154,4044.203872203827,0.03243399290840898
717718,1435438,717719,2153157,4047.837806224823,0.03238773170232889
718719,1437440,718720,2156160,4051.434667110443,0.032342027850972954
719720,1439442,719721,2159163,4055.033942222595,0.03229668805579422
720721,1441444,720722,2162166,4058.6165311336517,0.03225027805092395
721722,1443446,721723,2165169,4062.269697189331,0.03220450383014395
722723,1445448,722724,2168172,4065.989180088043,0.032158765503481845
723724,1447450,723725,2171175,4069.604840993881,0.03211377090701717
724725,1449452,724726,2174178,4073.2188811302185,0.03206855945791176
725726,1451454,725727,2177181,4076.784049987793,0.03202356756264635
726727,1453456,726728,2180184,4080.370714902878,0.03197844439819164
727728,1455458,727729,2183187,4084.036473274231,0.03193410393214435
728729,1457460,728730,2186190,4087.628781080246,0.03188968467657105
729730,1459462,729731,2189193,4091.251706123352,0.03184536077969824
730731,1461464,730732,2192196,4094.845039129257,0.03180217220506165
731732,1463466,731733,2195199,4098.459404230118,0.03175699846178759
732733,1465468,732734,2198202,4102.079535245895,0.03171261962779681
733734,1467470,733735,2201205,4105.638279914856,0.031668460704167956
734735,1469472,734736,2204208,4109.322656154633,0.03162467572838068
735736,1471474,735737,2207211,4113.026906967163,0.03157988480597851
736737,1473476,736738,2210214,4119.672650098801,0.03153676075999101
737738,1475478,737739,2213217,4124.923684120178,0.031492611202338594
738739,1477480,738740,2216220,4128.705730199814,0.03144864854584739
739740,1479482,739741,2219223,4132.309056997299,0.031405190984514775
740741,1481484,740742,2222226,4135.930690050125,0.03136206588897039
741742,1483486,741743,2225229,4139.701677083969,0.03131866979674669
742743,1485488,742744,2228232,4144.594056129456,0.03127602793756523
743744,1487490,743745,2231235,4149.519585132599,0.031233284926202032
744745,1489492,744746,2234238,4152.899504899979,0.031189918463496724
745746,1491494,745747,2237241,4156.429121017456,0.031147912213782547
746747,1493496,746748,2240244,4159.844330072403,0.03110482552438043
747748,1495498,747749,2243247,4163.374892234802,0.03106261358516349
748749,1497500,748750,2246250,4166.796897172928,0.031020719645312056
749750,1499502,749751,2249253,4170.722193956375,0.030977630412962753
750751,1501504,750752,2252256,4173.965283155441,0.03093589600393898
751752,1503506,751753,2255259,4177.448105096817,0.030893564591679024
752753,1505508,752754,2258262,4180.82533621788,0.030851305280521046
753754,1507510,753755,2261265,4184.985679149628,0.030810338374067214
754755,1509512,754756,2264268,4188.756808042526,0.030769264871196356
755756,1511514,755757,2267271,4192.892903089523,0.030728456817087135
756757,1513516,756758,2270274,4197.732096195221,0.030687421623952105
757758,1515518,757759,2273277,4202.446989059448,0.030646543185866904
758759,1517520,758760,2276280,4206.427613019943,0.030606144880948705
759760,1519522,759761,2279283,4210.71933221817,0.030564764552764245
760761,1521524,760762,2282286,4214.413261175156,0.030523228671881952
761762,1523526,761763,2285289,4218.199321269989,0.03048246585058223
762763,1525528,762764,2288292,4221.847665071487,0.03044177800802572
763764,1527530,763765,2291295,4225.397885084152,0.030401466938201338
764765,1529532,764766,2294298,4229.007274150848,0.030361044611709076
765766,1531534,765767,2297301,4232.621928930283,0.030320635980388033
766767,1533536,766768,2300304,4236.309000968933,0.0302812890313362
767768,1535538,767769,2303307,4239.882209062576,0.03024033648216573
768769,1537540,768770,2306310,4243.5003299713135,0.030200168655937887
769770,1539542,769771,2309313,4247.076085090637,0.030160407741277595
770771,1541544,770772,2312316,4250.649662971497,0.030120785053441068
771772,1543546,771773,2315319,4254.263866186142,0.030080464073762414
772773,1545548,772774,2318322,4257.917149066925,0.03004099044846953
773774,1547550,773775,2321325,4261.510010957718,0.030002337489349884
774775,1549552,774776,2324328,4265.076647043228,0.02996239400090417
775776,1551554,775777,2327331,4268.666544914246,0.02992353288209415
776777,1553556,776778,2330334,4272.260832071304,0.029884098257753067
777778,1555558,777779,2333337,4275.903802871704,0.029845524031770765
778779,1557560,778780,2336340,4279.490857124329,0.02980578282949864
779780,1559562,779781,2339343,4283.089323043823,0.02976624719121901
780781,1561564,780782,2342346,4286.679002285004,0.02972726225380029
781782,1563566,781783,2345349,4290.265934228897,0.029687995174754178
782783,1565568,782784,2348352,4293.927709102631,0.029649402988070506
783784,1567570,783785,2351355,4297.503190040588,0.029611687128635822
784785,1569572,784786,2354358,4301.089002132416,0.029573247014923254
785786,1571574,785787,2357361,4304.642335176468,0.02953563631126599
786787,1573576,786788,2360364,4308.219429016113,0.029496589235350257
787788,1575578,787789,2363367,4311.799654006958,0.029458239556333865
788789,1577580,788790,2366370,4315.422714948654,0.029420633405607077
789790,1579582,789791,2369373,4319.043575048447,0.029382691307546338
790791,1581584,790792,2372376,4322.626110076904,0.029344969278099597
791792,1583586,791793,2375379,4326.210574150085,0.029307458138646325
792793,1585588,792794,2378382,4330.626047134399,0.029269639440826722
793794,1587590,793795,2381385,4334.95227599144,0.029232788941953913
794795,1589592,794796,2384388,4339.125622034073,0.029194866532634478
795796,1591594,795797,2387391,4343.207997083664,0.029157567279980867
796797,1593596,796798,2390394,4347.131598234177,0.029120417346348404
797798,1595598,797799,2393397,4352.285303115845,0.029082540379022248
798799,1597600,798800,2396400,4357.946164131165,0.02904538314396632
799800,1599602,799801,2399403,4362.781071186066,0.029008655959842145
800801,1601604,800802,2402406,4366.384109258652,0.028972201303986367
801802,1603606,801803,2405409,4369.966699123383,0.028935925334735657
802803,1605608,802804,2408412,4374.159439086914,0.02889885690274241
803804,1607610,803805,2411415,4377.98385310173,0.02886278370351647
804805,1609612,804806,2414418,4381.969658136368,0.02882671425504668
805806,1611614,805807,2417421,4385.888370037079,0.028790058628146653
806807,1613616,806808,2420424,4389.779484987259,0.028753928461810574
807808,1615618,807809,2423427,4393.976613044739,0.02871681458054809
808809,1617620,808810,2426430,4397.549754858017,0.028680867129878607
809810,1619622,809811,2429433,4401.202252149582,0.028645083899391466
810811,1621624,810812,2432436,4404.840502023697,0.028609389144548913
811812,1623626,811813,2435439,4408.207571983337,0.02857410686374351
812813,1625628,812814,2438442,4411.604612112045,0.02853784403487225
813814,1627630,813815,2441445,4415.160931110382,0.02850289754314872
814815,1629632,814816,2444448,4418.697242975235,0.028468024589528795
815816,1631634,815817,2447451,4422.301651954651,0.028432329334464157
816817,1633636,816818,2450454,4425.84777712822,0.028396529885867494
817818,1635638,817819,2453457,4429.402448892593,0.02836179203586653
818819,1637640,818820,2456460,4432.671159029007,0.02832652885808784
819820,1639642,819821,2459463,4435.962363958359,0.028291282345890068
820821,1641644,820822,2462466,4439.311402082443,0.028257048636078252
821822,1643646,821823,2465469,4442.725155115128,0.028221540480444673
822823,1645648,822824,2468472,4446.620952129364,0.02818674418995215
823824,1647650,823825,2471475,4450.2669241428375,0.02815279149945127
824825,1649652,824826,2474478,4454.040655136108,0.028117997868321254
825826,1651654,825827,2477481,4458.658642053604,0.02808372097388201
826827,1653656,826828,2480484,4463.514562129974,0.02804975960862066
827828,1655658,827829,2483487,4469.0709619522095,0.028015166044497164
828829,1657660,828830,2486490,4473.948231935501,0.027981202791124815
829830,1659662,829831,2489493,4477.930210113525,0.027947399321419653
830831,1661664,830832,2492496,4481.57168006897,0.027913223073483096
831832,1663666,831833,2495499,4485.203506946564,0.027878806587978033
832833,1665668,832834,2498502,4488.885416030884,0.027845638192957267
833834,1667670,833835,2501505,4492.478076934814,0.02781180359670543
834835,1669672,834836,2504508,4496.076204061508,0.027778600011515664
835836,1671674,835837,2507511,4499.664499044418,0.02774370598672249
836837,1673676,836838,2510514,4503.3763909339905,0.027709159128789906
837838,1675678,837839,2513517,4506.907581090927,0.02767625791602768
838839,1677680,838840,2516520,4510.722527980804,0.027642571127216797
839840,1679682,839841,2519523,4514.300089120865,0.02760839692382433
840841,1681684,840842,2522526,4517.856367111206,0.02757462366571417
841842,1683686,841843,2525529,4521.572192192078,0.027540894827325246
842843,1685688,842844,2528532,4525.129437923431,0.027507952589076012
843844,1687690,843845,2531535,4529.403312921524,0.027475255559693323
844845,1689692,844846,2534538,4534.493212938309,0.027441441818155
845846,1691694,845847,2537541,4539.7282700538635,0.02740847794302681
846847,1693696,846848,2540544,4543.79484128952,0.027375959391065408
847848,1695698,847849,2543547,4547.508487939835,0.02734312558277452
848849,1697700,848850,2546550,4551.436943292618,0.027310940829920582
849850,1699702,849851,2549553,4555.214987039566,0.027278374349407386
850851,1701704,850852,2552556,4559.015660047531,0.02724591011974553
851852,1703706,851853,2555559,4562.76570391655,0.027213732077143504
852853,1705708,852854,2558562,4567.345380067825,0.02718130352877779
853854,1707710,853855,2561565,4571.145060300827,0.027148380542712403
854855,1709712,854856,2564568,4574.941719055176,0.027115387303638272
855856,1711714,855857,2567571,4578.7973918914795,0.0270829662840697
856857,1713716,856858,2570574,4582.626019239426,0.027051095785282087
857858,1715718,857859,2573577,4586.307020187378,0.02701863534275617
858859,1717720,858860,2576580,4590.2198531627655,0.026986877945091692
859860,1719722,859861,2579583,4593.9253718853,0.02695485682306753
860861,1721724,860862,2582586,4597.581705093384,0.02692260160438309
861862,1723726,861863,2585589,4601.39927315712,0.026891748299021856
862863,1725728,862864,2588592,4605.12947511673,0.02685989568090008
863864,1727730,863865,2591595,4608.854748010635,0.026829102062038146
864865,1729732,864866,2594598,4612.569361925125,0.026797994039952755
865866,1731734,865867,2597601,4616.304666996002,0.02676655764662428
866867,1733736,866868,2600604,4620.047667980194,0.026734968179880525
867868,1735738,867869,2603607,4623.841938972473,0.026704339203206473
868869,1737740,868870,2606610,4627.49610209465,0.026672670583138824
869870,1739742,869871,2609613,4631.2522439956665,0.02664165132046037
870871,1741744,870872,2612616,4634.960279226303,0.02661014045588672
871872,1743746,871873,2615619,4638.777961969376,0.026578657027130248
872873,1745748,872874,2618622,4642.632286071777,0.026547404797383933
873874,1747750,873875,2621625,4646.310128927231,0.026515854773606407
874875,1749752,874876,2624628,4650.024657964706,0.02648472005603253
875876,1751754,875877,2627631,4653.806225061417,0.02645349900558358
876877,1753756,876878,2630634,4657.6344220638275,0.026422780167195015
877878,1755758,877879,2633637,4661.311137199402,0.02639261246076785
878879,1757760,878880,2636640,4665.000982046127,0.02636187588905159
879880,1759762,879881,2639643,4668.752292871475,0.026331345523431082
880881,1761764,880882,2642646,4672.644864082336,0.026301501060515875
881882,1763766,881883,2645649,4676.3353753089905,0.02627106645013555
882883,1765768,882884,2648652,4679.993856191635,0.026241193067107815
883884,1767770,883885,2651655,4683.861720085144,0.02621045593332383
884885,1769772,884886,2654658,4687.536553144455,0.026180433203990106
885886,1771774,885887,2657661,4691.203224182129,0.02615049416453985
886887,1773776,886888,2660664,4695.066570043564,0.026120216803974472
887888,1775778,887889,2663667,4698.69656920433,0.026090061794093344
888889,1777780,888890,2666670,4702.3798542022705,0.026060275251438725
889890,1779782,889891,2669673,4706.151015996933,0.0260303523773473
890891,1781784,890892,2672676,4709.876564025879,0.026000741621828638
891892,1783786,891893,2675679,4713.529413223267,0.025970742643039557
892893,1785788,892894,2678682,4717.283397197723,0.02594119860805222
893894,1787790,893895,2681685,4720.96982884407,0.025911559503583703
894895,1789792,894896,2684688,4724.741505146027,0.025881861643938464
895896,1791794,895897,2687691,4728.3938331604,0.025852184580799076
896897,1793796,896898,2690694,4732.061085939407,0.025822433477515006
897898,1795798,897899,2693697,4735.85856795311,0.02579313690876006
898899,1797800,898900,2696700,4739.525421142578,0.025764049745703232
899900,1799802,899901,2699703,4743.213356018066,0.025734495948199765
900901,1801804,900902,2702706,4746.886339187622,0.025705258842208423
901902,1803806,901903,2705709,4750.578782081604,0.025675716085970635
902903,1805808,902904,2708712,4754.389224052429,0.025647219026723178
903904,1807810,903905,2711715,4758.07917714119,0.025617633926231065
904905,1809812,904906,2714718,4761.772860050201,0.025589115308321198
905906,1811814,905907,2717721,4765.44914317131,0.02555991779991018
906907,1813816,906908,2720724,4769.23005604744,0.02553125327176531
907908,1815818,907909,2723727,4772.918917179108,0.025502671547656064
908909,1817820,908910,2726730,4777.303389072418,0.025474426804066752
909910,1819822,909911,2729733,4781.086198091507,0.025445867899179575
910911,1821824,910912,2732736,4784.8488211631775,0.02541725882474566
911912,1823826,911913,2735739,4788.637771129608,0.025389071266545216
912913,1825828,912914,2738742,4792.456444978714,0.025360730824104394
913914,1827830,913915,2741745,4796.184367179871,0.025332704908578307
914915,1829832,914916,2744748,4799.870671272278,0.025305264920461923
915916,1831834,915917,2747751,4803.640620231628,0.02527741539051931
916917,1833836,916918,2750754,4807.468856096268,0.025248604448279366
917918,1835838,917919,2753757,4811.116362094879,0.025220773424734944
918919,1837840,918920,2756760,4814.811038017273,0.025192452581904945
919920,1839842,919921,2759763,4818.6436722278595,0.02516463818574266
920921,1841844,920922,2762766,4822.302489280701,0.025136675027169986
921922,1843846,921923,2765769,4826.082097053528,0.025108809568337165
922923,1845848,922924,2768772,4829.846273183823,0.02508108781876217
923924,1847850,923925,2771775,4833.548337936401,0.02505373193343985
924925,1849852,924926,2774778,4837.355832099915,0.02502573387391749
925926,1851854,925927,2777781,4841.129842996597,0.024998258260893635
926927,1853856,926928,2780784,4844.875138044357,0.024970584106995375
927928,1855858,927929,2783787,4848.557536125183,0.024943225438619265
928929,1857860,928930,2786790,4852.2311198711395,0.024915269197663292
929930,1859862,929931,2789793,4856.051962137222,0.024887839459552197
930931,1861864,930932,2792796,4859.757344007492,0.02486039706855081
931932,1863866,931933,2795799,4863.448132276535,0.024832908477037563
932933,1865868,932934,2798802,4867.239864110947,0.0248059333407582
933934,1867870,933935,2801805,4870.956741094589,0.024778717333902023
934935,1869872,934936,2804808,4874.659809112549,0.02475142345429049
935936,1871874,935937,2807811,4878.448730230331,0.024724156224692706
936937,1873876,936938,2810814,4882.191586256027,0.024697388929780573
937938,1875878,937939,2813817,4886.031396150589,0.024670113394677173
938939,1877880,938940,2816820,4889.709015130997,0.02464344445616007
939940,1879882,939941,2819823,4893.382992982864,0.024617199731437722
940941,1881884,940942,2822826,4897.247956037521,0.02459010093480174
941942,1883886,941943,2825829,4900.903735160828,0.024563086837588344
942943,1885888,942944,2828832,4904.591940164566,0.024536793574952753
943944,1887890,943945,2831835,4908.480502128601,0.02450975140891387
944945,1889892,944946,2834838,4912.146596908569,0.024482913369865855
945946,1891894,945947,2837841,4915.956915140152,0.024456681183437468
946947,1893896,946948,2840844,4919.665652990341,0.024429952914942987
947948,1895898,947949,2843847,4923.4818110466,0.024402969553193543
948949,1897900,948950,2846850,4927.174900054932,0.02437625419588585
949950,1899902,949951,2849853,4930.82301402092,0.02434994446048222
950951,1901904,950952,2852856,4934.633033037186,0.024323165485839127
951952,1903906,951953,2855859,4938.32973408699,0.02429730932453822
952953,1905908,952954,2858862,4942.064171075821,0.024271154748930712
953954,1907910,953955,2861865,4945.8258900642395,0.02424570813855098
954955,1909912,954956,2864868,4949.552706241608,0.02421965439680207
955956,1911914,955957,2867871,4953.313402891159,0.024193515455408487
956957,1913916,956958,2870874,4957.031565189362,0.024167328074327088
957958,1915918,957959,2873877,4960.699559926987,0.02414125892391894
958959,1917920,958960,2876880,4964.466386079788,0.02411569212199538
959960,1919922,959961,2879883,4968.185683965683,0.02408966661823797
960961,1921924,960962,2882886,4971.94556593895,0.024063639642918133
961962,1923926,961963,2885889,4975.620868206024,0.024038041116000386
962963,1925928,962964,2888892,4979.35409116745,0.024012575542656123
963964,1927930,963965,2891895,4983.000254154205,0.023987057526028366
964965,1929932,964966,2894898,4986.827459096909,0.023960556374731823
965966,1931934,965967,2897901,4990.488069295883,0.023935065257319366
966967,1933936,966968,2900904,4994.21648311615,0.023909504558105255
967968,1935938,967969,2903907,4997.974556922913,0.023884036345407367
968969,1937940,968970,2906910,5001.718122005463,0.02385872192644456
969970,1939942,969971,2909913,5005.409561157227,0.023833660690797842
970971,1941944,970972,2912916,5009.1232850551605,0.023808650783394114
971972,1943946,971973,2915919,5012.80522608757,0.023783421644111513
972973,1945948,972974,2918922,5016.610530138016,0.023758656629070174
973974,1947950,973975,2921925,5020.285452127457,0.023733277888823068
974975,1949952,974976,2924928,5024.058039188385,0.023708601394901052
975976,1951954,975977,2927931,5027.916615009308,0.023683605004407582
976977,1953956,976978,2930934,5031.580004930496,0.023658651851292234
977978,1955958,977979,2933937,5035.264101982117,0.02363346529818955
978979,1957960,978980,2936940,5039.127950191498,0.02360826427138818
979980,1959962,979981,2939943,5042.804676294327,0.023583294152558665
980981,1961964,980982,2942946,5046.502676010132,0.02355855132373108
981982,1963966,981983,2945949,5050.205860137939,0.023534480093076127
982983,1965968,982984,2948952,5053.976587057114,0.023509312872192822
983984,1967970,983985,2951955,5057.706377029419,0.02348480928048957
984985,1969972,984986,2954958,5061.337983131409,0.023460669017367763
985986,1971974,985987,2957961,5065.2006669044495,0.023436362060238025
986987,1973976,986988,2960964,5068.982138156891,0.02341205194898066
987988,1975978,987989,2963967,5072.631860971451,0.02338804069950129
988989,1977980,988990,2966970,5076.368000030518,0.02336411053147458
989990,1979982,989991,2969973,5080.156015872955,0.023340401214227313
990991,1981984,990992,2972976,5083.8304080963135,0.023316197022722918
991992,1983986,991993,2975979,5087.664262056351,0.023292363533983007
992993,1985988,992994,2978982,5091.329741239548,0.023268210605237982
993994,1987990,993995,2981985,5095.034898996353,0.023244042795340647
994995,1989992,994996,2984988,5098.715714216232,0.023220461753226118
995996,1991994,995997,2987991,5102.453720092773,0.023196308142360067
996997,1993996,996998,2990994,5106.294678211212,0.023172641293058405
997998,1995998,997999,2993997,5109.997317314148,0.023148600263084518
998999,1998000,999000,2997000,5113.611717224121,0.023124757975892862
1000000,2000002,1000001,3000003,5117.328367233276,0.023100391506886808


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.004189968109130859,12064.682476916567
1001,2003,2002,4005,8.30136489868164,21.074205127015375
2002,4005,4004,8009,15.927466869354248,19.073870623178664
3003,6007,6006,12013,23.074182748794556,17.372289908553284
4004,8009,8008,16017,30.281173944473267,15.906416381691088
5005,10011,10010,20021,37.65772008895874,14.631373993082889
6006,12013,12012,24025,44.682780742645264,13.513770899064184
7007,14015,14014,28029,52.491440773010254,12.527948884469879
8008,16017,16016,32033,62.14308977127075,11.653690998691673
9009,18019,18018,36037,71.10923886299133,10.874759810885735
10010,20021,20020,40041,78.67453169822693,10.177905979244315
11011,22023,22022,44045,87.9383270740509,9.552195649228452
12012,24025,24024,48049,95.80628609657288,8.988508349106269
13013,26027,26026,52053,103.72835779190063,8.479162481939056
14014,28029,28028,56057,110.53839468955994,8.01764140909836
15015,30031,30030,60061,117.89408683776855,7.598376535466741
16016,32033,32032,64065,125.22865796089172,7.216579546493449
17017,34035,34034,68069,132.52957892417908,6.868110005661947
18018,36037,36036,72073,139.1241810321808,6.549369756421584
19019,38039,38038,76077,146.08205485343933,6.257217886137369
20020,40041,40040,80081,153.92426586151123,5.988901629101747
21021,42043,42042,84085,163.27503776550293,5.741999743026099
22022,44045,44044,88089,171.18074798583984,5.514375734454006
23023,46047,46046,92093,179.05488991737366,5.304138927249369
24024,48049,48048,96097,187.14773869514465,5.109611828725974
25025,50051,50050,100101,195.37233090400696,4.9293025931237935
26026,52053,52052,104105,203.86585903167725,4.761881643187735
27027,54055,54054,108109,212.100919008255,4.606161709418302
28028,56057,56056,112113,219.7493109703064,4.461080698725709
29029,58059,58058,116117,227.4102840423584,4.325686921823944
30030,60061,60060,120121,234.46836304664612,4.199126299894488
31031,62063,62062,124125,241.40039587020874,4.080631242317395
32032,64065,64064,128129,248.7141261100769,3.969510943410569
33033,66067,66066,132133,255.9957938194275,3.8651428904740897
34034,68069,68068,136137,263.55916476249695,3.7669654109831754
35035,70071,70070,140141,270.62190198898315,3.674471241138235
36036,72073,72072,144145,277.51358675956726,3.587202720804271
37037,74075,74074,148149,284.7069969177246,3.5047429227015527
38038,76077,76076,152153,290.4854168891907,3.426715212297495
39039,78079,78078,156157,296.1500039100647,3.352777808724568
40040,80081,80080,160161,302.11019372940063,3.2826202209816984
41041,82083,82082,164165,309.6185758113861,3.2159600781378685
42042,84085,84084,168169,316.68725085258484,3.1525403063260455
43043,86087,86086,172173,323.8046588897705,3.092126611547428
44044,88089,88088,176177,331.01623797416687,3.034505232655647
45045,90091,90090,180181,338.35906410217285,2.9794809333798185
46046,92093,92092,184185,346.2917449474335,2.9268752062034764
47047,94095,94094,188189,355.2039988040924,2.8765246641833073
48048,96097,96096,192193,363.5561237335205,2.828279599785674
49049,98099,98098,196197,371.91515588760376,2.782002692199967
50050,100101,100100,200201,380.1844427585602,2.7375678469179547
51051,102103,102102,204205,388.294481754303,2.694859153121797
52052,104105,104104,208209,396.07781505584717,2.6537699462169257
53053,106107,106106,212213,404.23581886291504,2.6142019641883962
54054,108109,108108,216217,412.4059898853302,2.5760645878381183
55055,110111,110110,220221,420.50004386901855,2.539274155977182
56056,112113,112112,224225,428.81853890419006,2.503753347766178
57057,114115,114114,228229,436.6989607810974,2.469430625116729
58058,116117,116116,232233,444.89650678634644,2.436239729006047
59059,118119,118118,236237,453.67577171325684,2.404119224038368
60060,120121,120120,240241,461.0327408313751,2.3730120864292985
61061,122123,122122,244245,468.5896198749542,2.3428653309092624
62062,124125,124124,248249,475.77110505104065,2.313629672593379
63063,126127,126126,252253,483.36392092704773,2.285259220368971
64064,128129,128128,256257,492.8873689174652,2.2577111985938245
65065,130131,130130,260261,501.6746039390564,2.230945694287584
66066,132133,132132,264265,508.87274384498596,2.2049254273388215
67067,134135,134134,268269,515.7422018051147,2.179615541406747
68068,136137,136136,272273,522.6874008178711,2.154983501384777
69069,138139,138138,276277,529.8552989959717,2.13099871806844
70070,140141,140140,280281,537.1611950397491,2.1076324649147864
71071,142143,142142,284285,543.9829177856445,2.084857838044627
72072,144145,144144,288289,550.903990983963,2.062649558934936
73073,146147,146146,292293,558.7449977397919,2.040983853754369
74074,148149,148148,296297,566.9037058353424,2.0198383430015383
75075,150151,150150,300301,575.182835817337,1.9991919404128566
76076,152153,152152,304305,582.8094449043274,1.9790247603032185
77077,154155,154154,308309,590.5639827251434,1.9593180325755384
78078,156157,156156,312313,598.47407579422,1.9400540246715536
79079,158159,158158,316317,607.0114529132843,1.9212159698709002
80080,160161,160160,320321,615.0390219688416,1.9027880013363756
81081,162163,162162,324325,623.2447097301483,1.8847550913924351
82082,164165,164164,328329,630.5478389263153,1.86710299562219
83083,166167,166166,332333,638.0472497940063,1.8498182012772304
84084,168169,168168,336337,645.0450789928436,1.83288787971469
85085,170171,170170,340341,652.0925979614258,1.8162998424377292
86086,172173,172172,344345,659.8896586894989,1.8000425004720455
87087,174175,174174,348349,666.8113317489624,1.7841048267910082
88088,176177,176176,352353,673.6370806694031,1.76847632152203
89089,178179,178178,356357,680.4130239486694,1.7531469796958845
90090,180181,180180,360361,687.2037508487701,1.7381072613607103
91091,182183,182182,364365,693.8783898353577,1.7233481458606548
92092,184185,184184,368369,700.5123288631439,1.7088610304945178
93093,186187,186186,372373,707.5383260250092,1.694637423783206
94094,188189,188188,376377,714.3466558456421,1.6806693880425883
95095,190191,190190,380381,721.142808675766,1.6669493300269096
96096,192193,192192,384385,727.905280828476,1.6534699815711065
97097,194195,194194,388389,734.6147871017456,1.6402243815464317
98098,196197,196196,392393,741.2673869132996,1.6272058590493543
99099,198199,198198,396397,748.0748229026794,1.6144080176491116
100100,200201,200200,400401,754.8537647724152,1.601824720717559
101101,202203,202202,404405,761.588773727417,1.5894500776666973
102102,204205,204204,408409,768.6166708469391,1.5772784310938732
103103,206207,206206,412413,775.5905108451843,1.5653043447346136
104104,208209,208208,416417,782.5295779705048,1.5535225921557867
105105,210211,210210,420421,789.5153048038483,1.5419281461745413
106106,212213,212212,424425,796.4884097576141,1.5305161689084343
107107,214215,214214,428429,803.5625598430634,1.5192820024331013
108108,216217,216216,432433,810.5919427871704,1.5082211600129085
109109,218219,218218,436437,817.5104179382324,1.4973293178409222
110110,220221,220220,440441,824.5563488006592,1.4866023072627286
111111,222223,222222,444445,831.6251127719879,1.4760361074731918
112112,224225,224224,448449,838.7160696983337,1.4656268386097508
113113,226227,226226,452453,845.83846783638,1.4553707552640844
114114,228229,228228,456457,853.0078799724579,1.4452642403321079
115115,230231,230230,460461,859.9611048698425,1.4353037992441386
116116,232233,232232,464465,867.2763137817383,1.4254860544806434
117117,234235,234234,468469,874.242947101593,1.4158077404135838
118118,236237,236236,472473,880.9569756984711,1.4062656984133355
119119,238239,238238,476477,887.7838599681854,1.3968568722229975
120120,240241,240240,480481,894.1781990528107,1.387578303583723
121121,242243,242242,484485,899.8523859977722,1.3784271280837856
122122,244245,244244,488489,905.6481840610504,1.3694005712332
123123,246247,246246,492493,911.3355550765991,1.3604959447238798
124124,248249,248248,496497,917.1957318782806,1.351710642908074
125125,250251,250250,500501,924.288569688797,1.343042139436875
126126,252253,252252,504505,931.2487668991089,1.3344879840642534
127127,254255,254254,508509,938.1364316940308,1.3260457996238983
128128,256257,256256,512513,945.6963038444519,1.317713279151576
129129,258259,258258,516517,952.6517288684845,1.3094881831402745
130130,260261,260260,520521,958.5363237857819,1.3013683369390492
131131,262263,262262,524525,964.4033210277557,1.293351628268283
132132,264265,264264,528529,970.4707009792328,1.2854360048550006
133133,266267,266266,532533,976.3616578578949,1.2776194721827778
134134,268269,268268,536537,982.4331629276276,1.2699000913435157
135135,270271,270270,540541,988.2086520195007,1.2622759769983531
136136,272273,272272,544545,993.9072439670563,1.2547452954040637
137137,274275,274274,548549,999.6759181022644,1.2473062625722378
138138,276277,276276,552553,1005.4893729686737,1.2399571424630267
139139,278279,278278,556557,1011.3122508525848,1.2326962453098531
140140,280281,280280,560561,1017.084657907486,1.2255219259714067
141141,282283,282282,564565,1022.8709268569946,1.2184325823855033
142142,284285,284284,568569,1028.6567690372467,1.2114266540902463
143143,286287,286286,572573,1034.556035041809,1.2045027606709482
144144,288289,288288,576577,1040.988868713379,1.197659305862544
145145,290291,290290,580581,1046.8827159404755,1.1908948186337511
146146,292293,292292,584585,1052.873368024826,1.1842078912741272
147147,294295,294294,588589,1058.766343832016,1.1775971511269745
148148,296297,296296,592593,1064.7733418941498,1.171061259447015
149149,298299,298298,596597,1070.629968881607,1.164598910288987
150150,300301,300300,600601,1076.4115579128265,1.158208829450814
151151,302303,302302,604605,1082.3193588256836,1.1518897734658822
152152,304305,304304,608609,1088.1043388843536,1.1456405286280642
153153,306307,306306,612613,1093.9288198947906,1.1394599100531195
154154,308309,308308,616617,1099.766821861267,1.13334676078739
155155,310311,310310,620621,1105.498780965805,1.1272999509346846
156156,312313,312312,624625,1111.4390199184418,1.1213183768340969
157157,314315,314314,628629,1117.680814743042,1.1154009602614678
158158,316317,316316,632633,1123.4046049118042,1.109546647659954
159159,318319,318318,636637,1129.907450914383,1.1037544094033365
160160,320321,320320,640641,1135.805564880371,1.098023239081158
161161,322323,322322,644645,1141.9288036823273,1.092352152818421
162162,324325,324324,648649,1148.2590010166168,1.0867401886116568
163163,326327,326326,652653,1154.3172600269318,1.0811864057050116
164164,328329,328328,656657,1162.240609884262,1.0756898839645146
165165,330331,330330,660661,1169.3623349666595,1.0702497232960013
166166,332333,332332,664665,1175.0795488357544,1.0648650430666748
167167,334335,334334,668669,1180.962542772293,1.059534981581237
168168,336337,336336,672673,1187.7405717372894,1.0542586955216393
169169,338339,338338,676677,1193.9802458286285,1.0490353594468615
170170,340341,340340,680681,1200.0482790470123,1.0438641653181548
171171,342343,342342,684685,1205.9776079654694,1.038744321997001
172172,344345,344344,688689,1211.8845608234406,1.0336750547940028
173173,346347,346346,692693,1217.5689647197723,1.028655605035965
174174,348349,348348,696697,1223.3929719924927,1.0236852296202414
175175,350351,350350,700701,1229.2020018100739,1.0187632006091007
176176,352353,352352,704705,1234.9946689605713,1.0138888048295485
177177,354355,354354,708709,1240.8251078128815,1.0090613434804254
178178,356357,356356,712713,1247.6121878623962,1.004280131757696
179179,358359,358358,716717,1253.3846499919891,0.9995444984961068
180180,360361,360360,720721,1259.876529932022,0.9948537858144846
181181,362363,362362,724725,1266.1140069961548,0.9902073487810412
182182,364365,364364,728729,1272.3825018405914,0.9856045550732233
183183,366367,366366,732733,1278.3329448699951,0.9810447846684838
184184,368369,368368,736737,1284.53120303154,0.9765274295295967
185185,370371,370370,740741,1290.9129710197449,0.972051893320895
186186,372373,372372,744745,1296.7471318244934,0.9676175910917664
187187,374375,374374,748749,1302.7276957035065,0.9632239490201755
188188,376377,376376,752753,1308.9362790584564,0.958870404134359
189189,378379,378378,756757,1316.0921647548676,0.9545564040290628
190190,380381,380380,760761,1322.2539467811584,0.9502814066436258
191191,382383,382382,764765,1327.977217912674,0.946044879996407
192192,384385,384384,768769,1333.3731639385223,0.9418463019264891
193193,386387,386386,772773,1337.4626388549805,0.937685159897228
194194,388389,388388,776777,1341.5590467453003,0.9335609507361369
195195,390391,390390,780781,1345.7934198379517,0.9294731804384355
196196,392393,392392,784785,1349.7289500236511,0.9254213639342197
197197,394395,394394,788789,1354.0186479091644,0.9214050248956482
198198,396397,396396,792793,1357.9686410427094,0.9174236955295783
199199,398399,398398,796797,1361.8793530464172,0.9134769163792953
200200,400401,400400,800801,1365.7839710712433,0.9095642361335194
201201,402403,402402,804805,1369.7208168506622,0.9056852114554204
202202,404405,404404,808809,1373.7575869560242,0.9018394067788904
203203,406407,406406,812813,1377.7433898448944,0.8980263941539306
204204,408409,408408,816817,1381.5905079841614,0.8942457530720276
205205,410411,410410,820821,1385.4559507369995,0.8904970702933497
206206,412413,412412,824825,1389.3261868953705,0.8867799396957707
207207,414415,414414,828829,1394.256987810135,0.8830939621093421
208208,416417,416416,832833,1399.1770658493042,0.8794387451762304
209209,418419,418418,836837,1404.447501897812,0.8758139031888277
210210,420421,420420,840841,1409.3415658473969,0.8722190569606028
211211,422423,422422,844845,1414.174068927765,0.8686538336696685
212212,424425,424424,848849,1418.528615951538,0.8651178667350905
213213,426427,426426,852853,1423.4587128162384,0.8616107956822816
214214,428429,428428,856857,1428.2553327083588,0.858132266004759
215215,430431,430430,860861,1432.7594769001007,0.8546819290495478
216216,432433,432432,864865,1437.0802569389343,0.8512594418916706
217217,434435,434434,868869,1441.4116468429565,0.8478644672049995
218218,436437,436436,872873,1445.7897720336914,0.8444966731585737
219219,438439,438438,876877,1450.4798109531403,0.8411557332947268
220220,440441,440440,880881,1454.3725807666779,0.837841326425405
221221,442443,442442,884885,1459.755581855774,0.8345531365193892
222222,444445,444444,888889,1465.4932720661163,0.8312908525931562
223223,446447,446446,892893,1471.2488429546356,0.8280541686217475
224224,448449,448448,896897,1562.9826560020447,0.8248427834205359
225225,450451,450450,900901,1571.6620559692383,0.8216564005688269
226226,452453,452452,904905,1579.9600608348846,0.8184947282934445
227227,454455,454454,908909,1586.2999148368835,0.8153574793959706
228228,456457,456456,912913,1592.466080904007,0.8122443711454252
229229,458459,458458,916917,1597.7359569072723,0.80915512520005
230230,460461,460460,920921,1806.2405087947845,0.8060894675163581
231231,462463,462462,924925,1811.9891970157623,0.8030471282709186
232232,464465,464464,928929,1846.9234437942505,0.8000278417712252
233233,466467,466466,932933,1852.623939037323,0.7970313463756611
234234,468469,468468,936937,1860.418004989624,0.7940573844261962
235235,470471,470470,940941,1880.5764558315277,0.7911057021610759
236236,472473,472472,944945,1885.7446358203888,0.7881760496347852
237237,474475,474474,948949,1925.3699538707733,0.7852681806671171
238238,476477,476476,952953,1930.5370926856995,0.7823818527522235
239239,478479,478478,956957,1959.0680696964264,0.77951682699495
240240,480481,480480,960961,1964.2145388126373,0.7766728680453525
241241,482483,482482,964965,2436.757938861847,0.773849744027757
242242,484485,484484,968969,2441.8848638534546,0.7710472264843702
243243,486487,486486,972973,2449.2419028282166,0.7682650902988826
244244,488489,488488,976977,2456.4609699249268,0.7655031136491743
245245,490491,490490,980981,2461.6792047023773,0.762761077932737
246246,492493,492492,984985,2493.508116006851,0.7600387677193794
247247,494495,494494,988989,2498.6519799232483,0.7573359706857445
248248,496497,496496,992993,2505.9153850078583,0.7546524775661965
249249,498499,498498,996997,2511.075485944748,0.7519880820873368
250250,500501,500500,1001001,2518.374282836914,0.7493425809170731
251251,502503,502502,1005005,2523.5202028751373,0.7467157736191439
252252,504505,504504,1009009,2530.976210832596,0.7441074625985493
253253,506507,506506,1013013,2536.2180738449097,0.7415174530397053
254254,508509,508508,1017017,2543.569240808487,0.7389455528737017
255255,510511,510510,1021021,2548.7147488594055,0.7363915727200947
256256,512513,512512,1025025,2556.0581669807434,0.7338553258377942
257257,514515,514514,1029029,2561.1971237659454,0.731336628081408
258258,516517,516516,1033033,2568.5709187984467,0.7288352978684998
259259,518519,518518,1037037,2575.868574857712,0.7263511561068299
260260,520521,520520,1041041,2581.0806200504303,0.7238840261779842
261261,522523,522522,1045045,2588.425889968872,0.7214337338809855
262262,524525,524524,1049049,2593.661980867386,0.7190001073940948
263263,526527,526526,1053053,2601.373480796814,0.7165829772275174
264264,528529,528528,1057057,2606.7065467834473,0.7141821762070322
265265,530531,530530,1061061,2614.228712797165,0.7117975393975939
266266,532533,532532,1065065,2619.5162386894226,0.7094289040942385
267267,534535,534534,1069069,2627.0641379356384,0.707076126955144
268268,536537,536536,1073073,2632.1853597164154,0.7047390621501108
269269,538539,538538,1077077,2641.5878739356995,0.7024175234546419
270270,540541,540540,1081081,2646.7282700538635,0.700111356578418
271271,542543,542542,1085085,2654.1836709976196,0.6978204093720706
272272,544545,544544,1089089,2659.476749897003,0.6955445316889382
273273,546547,546546,1093093,2666.878012895584,0.6932835753632389
274274,548549,548548,1097097,2674.0783627033234,0.6910373941718717
275275,550551,550550,1101101,2679.5808367729187,0.6888058437925793
276276,552553,552552,1105105,2687.007374048233,0.6865887817857583
277277,554555,554554,1109109,2693.1337428092957,0.6843860675617179
278278,556557,556556,1113113,2700.8993978500366,0.6821975623352046
279279,558559,558558,1117117,2706.0386068820953,0.6800231291272212
280280,560561,560560,1121121,2713.4031937122345,0.6778626326995436
281281,562563,562562,1125125,2718.541023015976,0.6757159395547205
282282,564565,564564,1129129,2725.920329809189,0.6735829178978747
283283,566567,566566,1133133,2733.301367044449,0.6714634376039612
284284,568569,568568,1137137,2738.631938934326,0.6693573701977584
285285,570571,570570,1141141,2745.9373569488525,0.6672645888302213
286286,572573,572572,1145145,2751.115911960602,0.6651849682475586
287287,574575,574574,1149149,2758.46856880188,0.6631183847675857
288288,576577,576576,1153153,2764.062446117401,0.6610647162578971
289289,578579,578578,1157157,2771.518534898758,0.6590243013652071
290290,580581,580580,1161161,2776.840364933014,0.6569965880917152
291291,582583,582582,1165165,2784.2907218933105,0.654981430285261
292292,584585,584584,1169169,2789.4427649974823,0.6529787113868224
293293,586587,586586,1173173,2809.218505859375,0.6509883164253552
294294,588589,588588,1177177,2814.3507487773895,0.6490101319341193
295295,590591,590590,1181181,2885.1757209300995,0.6470440458924713
296296,592593,592592,1185185,2972.5932829380035,0.6450899476822087
297297,594595,594594,1189189,2977.8180301189423,0.6431477280475519
298298,596597,596596,1193193,2985.2168729305267,0.6412172790733166
299299,598599,598598,1197197,2990.3255150318146,0.6392984941521718
300300,600601,600600,1201201,2997.6324968338013,0.6373912679755449
301301,602603,602602,1205205,3002.743400812149,0.6354956016457436
302302,604605,604604,1209209,3010.078024864197,0.6336116482852958
303303,606607,606606,1213213,3015.163904905319,0.6317389440155239
304304,608609,608608,1217217,3033.1421868801117,0.629877387529632
305305,610611,610610,1221221,3038.260062932968,0.628026879267054
306306,612613,612612,1225225,3045.5628559589386,0.6261873210733029
307307,614615,614614,1229229,3050.6629848480225,0.62435861605627
308308,616617,616616,1233233,3057.956748008728,0.6225406685043708
309309,618619,618618,1237237,3063.072910785675,0.6207333838501654
310310,620621,620620,1241241,3070.366963863373,0.6189366686394351
311311,622623,622622,1245245,3075.493805885315,0.6171504305093549
312312,624625,624624,1249249,3082.776666879654,0.6153745781757607
313313,626627,626626,1253253,3087.8614547252655,0.613609021405864
314314,628629,628628,1257257,3095.2053139209747,0.6118536710218905
315315,630631,630630,1261261,3102.3695878982544,0.6101084388610616
316316,632633,632632,1265265,3107.6202487945557,0.608373237781052
317317,634635,634634,1269269,3114.8246309757233,0.6066479816345236
318318,636637,636636,1273273,3119.981657743454,0.6049325852563925
319319,638639,638638,1277277,3127.2696208953857,0.6032269644529151
320320,640641,640640,1281281,3132.432270050049,0.6015310359853174
321321,642643,642642,1285285,3139.666771888733,0.5998447175643378
322322,644645,644644,1289289,3144.7857599258423,0.5981679278138472
323323,646647,646646,1293293,3152.1177427768707,0.5965005862890393
324324,648649,648648,1297297,3157.343514919281,0.5948426134382316
325325,650651,650650,1301301,3164.768364906311,0.5931939306046843
326326,652653,652652,1305305,3170.1240158081055,0.5915544600065914
327327,654655,654654,1309309,3180.499778985977,0.5899241279730632
328328,656657,656656,1313313,3186.07879281044,0.5883028676744289
329329,658659,658658,1317317,3195.14310503006,0.5866905915427196
330330,660661,660660,1321321,3200.7489309310913,0.585087225164898
331331,662663,662662,1325325,3209.787137031555,0.5834926949537476
332332,664665,664664,1329329,3215.3638319969177,0.5819069281278644
333333,666667,666666,1333333,3224.387204885483,0.5803298527025618
334334,668669,668668,1337337,3229.617287874222,0.5787613974880514
335335,670671,670670,1341341,3438.2792670726776,0.5772014920585207
336336,672673,672672,1345345,3443.404467821121,0.5756500667594082
337337,674675,674674,1349349,3564.963096857071,0.5741070526873955
338338,676677,676676,1353353,3570.320767879486,0.5725723816958634
339339,678679,678678,1357357,3623.9655590057373,0.5710459863512369
340340,680681,680680,1361361,3629.584832906723,0.5695277999639075
341341,682683,682682,1365365,3746.456429004669,0.5680177565554914
342342,684685,684684,1369369,3752.1463339328766,0.56651579084064
343343,686687,686686,1373373,3760.7083308696747,0.5650218382434105
344344,688689,688688,1377377,3766.3376319408417,0.5635358348663431
345345,690691,690690,1381381,3925.3817789554596,0.562057717495918
346346,692693,692692,1385385,3930.9548258781433,0.5605874235807278
347347,694695,694694,1389389,3990.750072002411,0.5591248912296578
348348,696697,696696,1393393,3996.326826810837,0.5576700592082489
349349,698699,698698,1397397,4004.957382917404,0.5562228669186879
350350,700701,700700,1401401,4010.5531549453735,0.5547832543979894
351351,702703,702702,1405405,4085.1901519298553,0.5533511623088998
352352,704705,704704,1409409,4090.845739841461,0.5519265319344413
353353,706707,706706,1413413,4162.6697199344635,0.5505093051597214
354354,708709,708708,1417417,4168.445954084396,0.5490994244828471
355355,710711,710710,1421421,4232.722606658936,0.547696832984002
356356,712713,712712,1425425,4238.371393918991,0.5463014743363601
357357,714715,714714,1429429,4415.196980953217,0.5449132927878964
358358,716717,716716,1433433,4420.838457107544,0.5435322331577481
359359,718719,718718,1437437,4475.404349803925,0.5421582408380345
360360,720721,720720,1441441,4481.056569099426,0.5407912617592956
361361,722723,722722,1445445,4597.889928817749,0.5394312424214149
362362,724725,724724,1449449,4603.510618686676,0.5380781298536021
363363,726727,726726,1453453,4612.07719874382,0.5367318716198497
364364,728729,728728,1457457,4617.684996843338,0.5353924158243899
365365,730731,730730,1461461,4770.349407911301,0.5340597110825911
366366,732733,732732,1465465,4775.942314863205,0.5327337065318716
367367,734735,734734,1469469,4841.549667835236,0.5314143518171477
368368,736737,736736,1473473,4847.228066921234,0.5301015970835579
369369,738739,738738,1477477,4897.919805765152,0.5287953929764626
370370,740741,740740,1481481,4902.733299970627,0.5274956906305306
371371,742743,742742,1485485,4907.967903852463,0.5262024416624627
372372,744745,744744,1489489,4911.957054853439,0.5249155981709919
373373,746747,746746,1493493,4915.42110991478,0.5236351127223315
374374,748749,748748,1497497,4920.075690984726,0.5223609383574512
375375,750751,750750,1501501,4924.144910812378,0.5210930285666109
376376,752753,752752,1505505,4928.299319028854,0.5198313373057317
377377,754755,754754,1509509,4932.170143842697,0.5185758189782064
378378,756757,756756,1513513,4935.971458911896,0.5173264284239849
379379,758759,758758,1517517,4940.6628448963165,0.5160831209304888
380380,760761,760760,1521521,4944.939577102661,0.514845852218059
381381,762763,762762,1525525,4948.995139837265,0.513614578429042
382382,764765,764764,1529529,4952.917819738388,0.5123892561332468
383383,766767,766766,1533533,4957.030835866928,0.51116984231885
384384,768769,768768,1537537,4960.594947814941,0.5099562943869387
385385,770771,770770,1541541,4964.280186891556,0.5087485701405967
386386,772773,772772,1545545,4967.886094093323,0.5075466277994565
387387,774775,774774,1549549,4971.399572849274,0.5063504259615002
388388,776777,776776,1553553,4975.6549417972565,0.5051599236394395
389389,778779,778778,1557557,4979.203172683716,0.5039750802206981
390390,780781,780780,1561561,4982.708149909973,0.5027958554837824
391391,782783,782782,1565565,4986.073929786682,0.5016222095819103
392392,784785,784784,1569569,4989.379288673401,0.5004541030466498
393393,786787,786786,1573573,4992.816177845001,0.49929149678246176
394394,788789,788788,1577577,4996.133076906204,0.4981343520539667
395395,790791,790790,1581581,4999.383946895599,0.4969826304968592
396396,792793,792792,1585585,5002.826259851456,0.49583629409607965
397397,794795,794794,1589589,5006.184198856354,0.49469530519309046
398398,796797,796796,1593593,5009.6004049777985,0.4935596264876949
399399,798799,798798,1597597,5012.913302898407,0.4924292210089334
400400,800801,800800,1601601,5016.596334695816,0.4913040521387302
401401,802803,802802,1605605,5020.064617872238,0.49018408359916066
402402,804805,804804,1609609,5023.383249759674,0.48906927943971823
403403,806807,806806,1613613,5026.750888824463,0.4879596040391334
404404,808809,808808,1617617,5030.316337823868,0.4868550221053738
405405,810811,810810,1621621,5033.618598937988,0.48575549867200607
406406,812813,812812,1625625,5036.904784917831,0.48466099908364413
407407,814815,814814,1629629,5040.172940015793,0.48357148900868197
408408,816817,816816,1633633,5043.405771970749,0.4824869344192848
409409,818819,818818,1637637,5046.658061027527,0.48140730160048406
410410,820821,820820,1641641,5049.889401674271,0.48033255714290135
411411,822823,822822,1645645,5074.112232923508,0.4792626679318346
412412,824825,824824,1649649,5078.391801118851,0.4781976011581719
413413,826827,826826,1653653,5081.872451066971,0.4771373243038397
414414,828829,828828,1657657,5085.267144918442,0.47608180513998377
415415,830831,830830,1661661,5088.592904806137,0.47503101173060713
416416,832833,832832,1665665,5091.924836874008,0.4739849124180182
417417,834835,834834,1669669,5095.19616484642,0.47294347583374474
418418,836837,836836,1673673,5098.572375059128,0.4719066708803439
419419,838839,838838,1677677,5101.875315904617,0.47087446674049716
420420,840841,840840,1681681,5105.336683034897,0.46984683286245854
421421,842843,842842,1685685,5109.460011005402,0.46882373897824436
422422,844845,844844,1689689,5113.872211933136,0.4678051550690725
423423,846847,846846,1693693,5117.904023885727,0.4667910513908282
424424,848849,848848,1697697,5121.830605983734,0.4657813984540553
425425,850851,850850,1701701,5126.251508951187,0.46477616702941305
426426,852853,852852,1705705,5130.431729793549,0.4637753281476762
427427,854855,854854,1709709,5134.57128071785,0.4627788530815451
428428,856857,856856,1713713,5138.749388933182,0.4617867133583786
429429,858859,858858,1717717,5142.526726722717,0.4607988807510992
430430,860861,860860,1721721,5146.179615974426,0.45981532728001184
431431,862863,862862,1725725,5150.161900997162,0.45883602520007116
432432,864865,864864,1729729,5153.819809913635,0.45786094701361435
433433,866867,866866,1733733,5157.6517329216,0.45689006545035227
434434,868869,868868,1737737,5161.47345995903,0.4559233534782834
435435,870871,870870,1741741,5165.2692239284515,0.4549607843018748
436436,872873,872872,1745745,5169.096889734268,0.45400233134205337
437437,874875,874874,1749749,5193.39716386795,0.45304796825439553
438438,876877,876876,1753753,5197.841199874878,0.4520976689145755
439439,878879,878878,1757757,5202.181715965271,0.4511514074256411
440440,880881,880880,1761761,5205.9233548641205,0.45020915810528095
441441,882883,882882,1765765,5209.423542022705,0.44927089548218646
442442,884885,884884,1769769,5212.909881830215,0.44833659431424167
443443,886887,886886,1773773,5216.359706878662,0.44740622956123843
444444,888889,888888,1777777,5219.890236854553,0.4464797763903334
445445,890891,890890,1781781,5223.316337823868,0.44555721018696204
446446,892893,892892,1785785,5226.870623826981,0.4446385065366485
447447,894895,894894,1789789,5230.476490020752,0.44372364122318686
448448,896897,896896,1793793,5234.003228902817,0.442812590241374
449449,898899,898898,1797797,5237.770333766937,0.4419053297788196
450450,900901,900900,1801801,5241.202861070633,0.4410018362250412
451451,902903,902902,1805805,5244.672209739685,0.44010208616236923
452452,904905,904904,1809809,5248.299788951874,0.439206056362309
453453,906907,906906,1813813,5251.78440284729,0.4383137237982737
454454,908909,908908,1817817,5255.193441867828,0.4374250656219374
455455,910911,910910,1821821,5258.5715799331665,0.43654005917778704
456456,912913,912912,1825825,5262.043044805527,0.4356586819940276
457457,914915,914914,1829829,5265.453236818314,0.4347809117862198
458458,916917,916916,1833833,5268.986791849136,0.43390672644272854
459459,918919,918918,1837837,5272.491621732712,0.4330361040429125
460460,920921,920920,1841841,5276.0849609375,0.4321690228389343
461461,922923,922922,1845845,5279.648858785629,0.43130546125212277
462462,924925,924924,1849849,5283.229228973389,0.4304453978929814
463463,926927,926926,1853853,5286.697560071945,0.42958881153208495
464464,928929,928928,1857857,5290.094116687775,0.42873568111645
465465,930931,930930,1861861,5293.513497829437,0.4278859857622592
466466,932933,932932,1865865,5297.077081680298,0.4270397047512233
467467,934935,934934,1869869,5300.520126819611,0.42619681753058103
468468,936937,936936,1873873,5304.006173849106,0.4253573037167371
469469,938939,938938,1877877,5307.382255792618,0.4245211430843483
470470,940941,940940,1881881,5310.694012880325,0.4236883155645046
471471,942943,942942,1885885,5313.992281675339,0.4228588012574619
472472,944945,944944,1889889,5317.403005838394,0.42203258041627123
473473,946947,946946,1893893,5839.910350799561,0.42120963344859774
474474,948949,948948,1897897,5845.910577774048,0.42038994091853965
475475,950951,950950,1901901,5849.9435958862305,0.4195734835448093
476476,952953,952952,1905905,5856.055681943893,0.41876024219709507
477477,954955,954954,1909909,5860.91623878479,0.4179501978887856
478478,956957,956956,1913913,5865.13990187645,0.4171433317933406
479479,958959,958958,1917917,5869.286950826645,0.4163396252242819
480480,960961,960960,1921921,5872.846890926361,0.4155390596406505
481481,962963,962962,1925925,5876.390865802765,0.4147416166433686
482482,964965,964964,1929929,5880.165536880493,0.4139472779879725
483483,966967,966966,1933933,5883.8159947395325,0.41315602556096565
484484,968969,968968,1937937,5887.478606700897,0.40913828767043015
485485,970971,970970,1941941,5891.22571182251,0.40836570218561974
486486,972973,972972,1945945,5894.679506778717,0.4075960772934195
487487,974975,974974,1949949,5898.206205844879,0.40682939598445955
488488,976977,976976,1953953,5901.693073749542,0.4060656413803372
489489,978979,978978,1957957,5905.499679803848,0.40530479673361697
490490,980981,980980,1961961,5910.173569917679,0.40454684542237374
491491,982983,982982,1965965,5913.698553800583,0.4037917709483736
492492,984985,984984,1969969,5917.234534740448,0.4030395569443499
493493,986987,986986,1973973,5920.637149810791,0.4022901871630893
494494,988989,988988,1977977,5923.967542886734,0.40154364547379373
495495,990991,990990,1981981,5927.3744258880615,0.4007999158820894
496496,992993,992992,1985985,5930.748508930206,0.4000589824936469
497497,994995,994994,1989989,5934.049243927002,0.39932082955238
498498,996997,996996,1993993,5937.424050807953,0.3985854414058849
499499,998999,998998,1997997,5940.8154718875885,0.39785280253090605
500501,1001003,1001002,2002005,5944.210108757019,0.39712216969564906
501502,1003005,1003004,2006009,5947.544004678726,0.39639498593351163
502503,1005007,1005006,2010013,5950.889709949493,0.3956705055279599
503504,1007009,1007008,2014017,5954.289076805115,0.3949487134013907
504505,1009011,1009010,2018021,5957.625372886658,0.3942295945907972
505506,1011013,1011012,2022025,5961.138489723206,0.3935131342514069
506507,1013015,1013014,2026029,5964.466423034668,0.39279931763849163
507508,1015017,1015016,2030033,5967.722323894501,0.3920881301146437
508509,1017019,1017018,2034037,5971.029246807098,0.3913795571625087
509510,1019021,1019020,2038041,5974.374305009842,0.3906735843520437
510511,1021023,1021022,2042045,5977.68994307518,0.389970197375078
511512,1023025,1023024,2046049,5981.0524559021,0.3892693820234854
512513,1025027,1025026,2050053,5984.433490753174,0.38857112419100304
513514,1027029,1027028,2054057,5987.793662786484,0.38787540987141256
514515,1029031,1029030,2058061,5991.174389839172,0.3871822251639969
515516,1031033,1031032,2062065,5994.443053007126,0.3864915562717215
516517,1033035,1033034,2066069,5997.66711807251,0.3858033894921391
517518,1035037,1035036,2070073,6000.880594968796,0.385117711221028
518519,1037039,1037038,2074077,6004.131744861603,0.38443450795602985
519520,1039041,1039040,2078081,6007.316657781601,0.3837537662930117
520521,1041043,1041042,2082085,6010.554130792618,0.3830754729169712
521522,1043045,1043044,2086089,6013.762428760529,0.3823996146184072
522523,1045047,1045046,2090093,6016.974718809128,0.38172617827331123
523524,1047049,1047048,2094097,6020.174700021744,0.38105515085590014
524525,1049051,1049050,2098101,6023.400803089142,0.38038651943315926
525526,1051053,1051052,2102105,6026.783857822418,0.3797202711648424
526527,1053055,1053054,2106109,6029.997453927994,0.3790563932980149
527528,1055057,1055056,2110113,6033.208475828171,0.3783948731779674
528529,1057059,1057058,2114117,6036.3901998996735,0.37773569823184516
529530,1059061,1059060,2118121,6039.599805831909,0.37707885597774293
530531,1061063,1061062,2122125,6042.81046295166,0.3764243340247049
531532,1063065,1063064,2126129,6046.01531291008,0.3757721200636297
532533,1065067,1065066,2130133,6049.207731962204,0.37512220188000356
533534,1067069,1067068,2134137,6052.424901723862,0.37447456733752915
534535,1069071,1069070,2138141,6055.64915394783,0.37382920439267764
535536,1071073,1071072,2142145,6058.8744859695435,0.37318610107467975
536537,1073075,1073074,2146149,6062.1035788059235,0.3725452455055347
537538,1075077,1075076,2150153,6065.26314496994,0.37190662589091517
538539,1077079,1077078,2154157,6068.461692810059,0.3712702305147104
539540,1079081,1079080,2158161,6071.652441740036,0.37063604774084524
540541,1081083,1081082,2162165,6074.856686830521,0.37000406601509894
541542,1083085,1083084,2166169,6078.112847805023,0.36937427386692434
542543,1085087,1085086,2170173,6081.352867841721,0.3687466599039908
543544,1087089,1087088,2174177,6084.521222829819,0.3681212128049083
544545,1089091,1089090,2178181,6087.775859832764,0.3674979213410552
545546,1091093,1091092,2182185,6090.985559940338,0.3668767743438366
546547,1093095,1093094,2186189,6094.185478925705,0.366257760735607
547548,1095097,1095096,2190193,6097.4688448905945,0.3656408695042046
548549,1097099,1097098,2194197,6100.7093460559845,0.365026089724779
549550,1099101,1099100,2198201,6103.997699737549,0.36441341053250653
550551,1101103,1101102,2202205,6107.273837089539,0.36380282114805595
551552,1103105,1103104,2206209,6110.560940027237,0.3631943108612177
552553,1105107,1105106,2210213,6113.7539138793945,0.36258786903636064
553554,1107109,1107108,2214217,6116.996536016464,0.36198348510333744
554555,1109111,1109110,2218221,6120.235594987869,0.3613811485720362
555556,1111113,1111112,2222225,6123.41188287735,0.36078084902146657
556557,1113115,1113114,2226229,6126.597050905228,0.3601825760961219
557558,1115117,1115116,2230233,6129.976842880249,0.3595863195187121
558559,1117119,1117118,2234237,6133.399132966995,0.3589920690719737
559560,1119121,1119120,2238241,6136.629125833511,0.3583998146114027
560561,1121123,1121122,2242245,6139.880853891373,0.35780954605979787
561562,1123125,1123124,2246249,6143.161561727524,0.3572212534145365
562563,1125127,1125126,2250253,6146.4429268836975,0.35663492672756547
563564,1127129,1127128,2254257,6149.665116786957,0.35605055612541037
564565,1129131,1129130,2258261,6152.861638784409,0.35546813179280434
565566,1131133,1131132,2262265,6156.115131855011,0.3548876439945161
566567,1133135,1133134,2266269,6159.32959985733,0.3543090830444271
567568,1135137,1135136,2270273,6162.573276758194,0.3537324393309973
568569,1137139,1137138,2274277,6165.82018995285,0.3531577032954374
569570,1139141,1139140,2278281,6169.0782787799835,0.3525848654535366
570571,1141143,1141142,2282285,6172.296472787857,0.35201391637565393
571572,1143145,1143144,2286289,6175.489850759506,0.35144484670308884
572573,1145147,1145146,2290293,6178.742830038071,0.35087764712989156
573574,1147149,1147148,2294297,6181.979769706726,0.35031230840831995
574575,1149151,1149150,2298301,6185.219214677811,0.34974882137066743
575576,1151153,1151152,2302305,6188.372344017029,0.3491871768819692
576577,1153155,1153154,2306309,6191.590375900269,0.348627365892753
577578,1155157,1155156,2310313,6194.959495782852,0.3480693793899263
578579,1157159,1157158,2314317,6198.444140911102,0.3475132084386132
579580,1159161,1159160,2318321,6201.6735780239105,0.3469588441457745
580581,1161163,1161162,2322325,6204.864759922028,0.34640627768931154
581582,1163165,1163164,2326329,6208.097781896591,0.34585550029805745
582583,1165167,1165166,2330333,6211.400600671768,0.345306503253596
583584,1167169,1167168,2334337,6214.622406721115,0.34475927790117566
584585,1169171,1169170,2338341,6217.820101737976,0.3442138156387955
585586,1171173,1171172,2342345,6221.043345928192,0.34367010792448127
586587,1173175,1173174,2346349,6224.281507730484,0.3431281462580955
587588,1175177,1175176,2350353,6227.512709856033,0.3425879222104413
588589,1177179,1177178,2354357,6230.962674856186,0.34204942739233957
589590,1179181,1179180,2358361,6234.1771068573,0.34151265347827575
590591,1181183,1181182,2362365,6237.41570186615,0.3409775921936671
591592,1183185,1183184,2366369,6240.615739822388,0.3404442353112245
592593,1185187,1185186,2370373,6243.839738845825,0.3399125746636855
593594,1187189,1187188,2374377,6247.120523929596,0.3393826021292625
594595,1189191,1189190,2378381,6250.342760801315,0.3388543096407375
595596,1191193,1191192,2382385,6253.549154043198,0.33832768918728107
596597,1193195,1193194,2386389,6256.81320977211,0.3378027327944437
597598,1195197,1195196,2390393,6260.209843873978,0.33727943255507853
598599,1197199,1197198,2394397,6263.479825735092,0.3367577806020563
599600,1199201,1199200,2398401,6266.744500875473,0.3362377691173606
600601,1201203,1201202,2402405,6269.956709861755,0.33571939033390663
601602,1203205,1203204,2406409,6273.188636779785,0.3352026365355414
602603,1205207,1205206,2410413,6276.400862932205,0.3346875000552245
603604,1207209,1207208,2414417,6279.711944818497,0.3341739732713904
604605,1209211,1209210,2418421,6282.955922842026,0.33366204860794824
605606,1211213,1211212,2422425,6286.146018028259,0.3331517185379198
606607,1213215,1213214,2426429,6289.427794933319,0.3326429755834397
607608,1215217,1215216,2430433,6292.6889128685,0.3321358123102982
608609,1217219,1217218,2434437,6295.912497758865,0.33163022133521736
609610,1219221,1219220,2438441,6299.107882976532,0.3311261953149369
610611,1221223,1221222,2442445,6302.366129875183,0.3306237269534904
611612,1223225,1223224,2446449,6305.575927972794,0.33012280900220503
612613,1225227,1225226,2450453,6308.835145950317,0.3296234342524258
613614,1227229,1227228,2454457,6312.046718835831,0.3291255955464294
614615,1229231,1229230,2458461,6315.237732887268,0.3286292857646913
615616,1231233,1231232,2462465,6318.461894750595,0.3281344978367997
616617,1233235,1233234,2466469,6321.708469867706,0.3276412247305416
617618,1235237,1235236,2470473,6324.9146900177,0.3271494594609976
618619,1237239,1237238,2474477,6328.185785770416,0.32665919507962826
619620,1239241,1239240,2478481,6331.4122149944305,0.3261704246924637
620621,1241243,1241242,2482485,6334.635227918625,0.32568314143281896
621622,1243245,1243244,2486489,6337.834729909897,0.3251973384849407
622623,1245247,1245246,2490493,6341.081655025482,0.3247130090803694
623624,1247249,1247248,2494497,6344.309793949127,0.3242301464706543
624625,1249251,1249250,2498501,6347.517513990402,0.3237487439691904
625626,1251253,1251252,2502505,6350.761841773987,0.32326879492393346
626627,1253255,1253254,2506509,6354.012522935867,0.3227902927174
627628,1255257,1255256,2510513,6357.262953996658,0.32231323077758134
628629,1257259,1257258,2514517,6360.4809148311615,0.3218376025724865
629630,1259261,1259260,2518521,6363.692576885223,0.32136340160468535
630631,1261263,1261262,2522525,6366.932471036911,0.3208906214185845
631632,1263265,1263264,2526529,6370.246226787567,0.32041925560224627
632633,1265267,1265266,2530533,6373.4180018901825,0.3199492977710179
633634,1267269,1267268,2534537,6376.623393058777,0.31948074158572126
634635,1269271,1269270,2538541,6379.939043045044,0.3190135807490151
635636,1271273,1271272,2542545,6383.160787820816,0.3185478089944809
636637,1273275,1273274,2546549,6386.538491725922,0.3180834200920799
637638,1275277,1275276,2550553,6389.907367944717,0.31762040785179124
638639,1277279,1277278,2554557,6393.127936840057,0.3171587661236117
639640,1279281,1279280,2558561,6396.317310810089,0.31669848878846096
640641,1281283,1281282,2562565,6399.509551763535,0.31623956976363843
641642,1283285,1283284,2566569,6402.811353683472,0.3157820030119183
642643,1285287,1285286,2570573,6406.053098917007,0.3153257825124456
643644,1287289,1287288,2574577,6409.274647951126,0.3148709023007541
644645,1289291,1289290,2578581,6412.528207778931,0.3144173564396624
645646,1291293,1291292,2582585,6415.737134695053,0.31396513901745493
646647,1293295,1293294,2586589,6418.979748725891,0.31351424417152884
647648,1295297,1295296,2590593,6422.231261968613,0.31306466606474714
648649,1297299,1297298,2594597,6425.441141843796,0.3126163988999906
649650,1299301,1299300,2598601,6428.682209968567,0.31216943690378685
650651,1301303,1301302,2602605,6431.892110824585,0.3117237743535952
651652,1303305,1303304,2606609,6435.106912851334,0.31127940554506495
652653,1305307,1305306,2610613,6438.329462051392,0.31083632481204404
653654,1307309,1307308,2614617,6441.532304763794,0.3103945265211223
654655,1309311,1309310,2618621,6444.724603891373,0.3099540050716314
655656,1311313,1311312,2622625,6447.949589967728,0.3095147548974637
656657,1313315,1313314,2626629,6451.129544973373,0.3090767704652535
657658,1315317,1315316,2630633,6454.343020915985,0.30864004626528185
658659,1317319,1317318,2634637,6457.554259777069,0.30820457682784763
659660,1319321,1319320,2638641,6460.776715993881,0.3077703567178105
660661,1321323,1321322,2642645,6463.993994951248,0.307337380520039
661662,1323325,1323324,2646649,6467.226259946823,0.30690564285760047
662663,1325327,1325326,2650653,6470.5184898376465,0.306475138386304
663664,1327329,1327328,2654657,6473.774406909943,0.30604586178742466
664665,1329331,1329330,2658661,6476.995199918747,0.30561780777316017
665666,1331333,1331332,2662665,6480.23034787178,0.30519097109208815
666667,1333335,1333334,2666669,6483.479514837265,0.30476534651825204
667668,1335337,1335336,2670673,6486.716841936111,0.30434092885116115
668669,1337339,1337338,2674677,6489.907314777374,0.30391771293034253
669670,1339341,1339340,2678681,6493.131296873093,0.30349569361351314
670671,1341343,1341342,2682685,6496.347007989883,0.3030748657984077
671672,1343345,1343344,2686689,6499.599467992783,0.30265522440095083
672673,1345347,1345346,2690693,6502.848871946335,0.30223676437162794
673674,1347349,1347348,2694697,6506.342273950577,0.30181948069366626
674675,1349351,1349350,2698701,6509.680008888245,0.3014033683684829
675676,1351353,1351352,2702705,6512.877530813217,0.3009884224356938
676677,1353355,1353354,2706709,6516.227329969406,0.3005746379549237
677678,1355357,1355356,2710713,6519.473402738571,0.30016201001853915
678679,1357359,1357358,2714717,6522.698508024216,0.29975053374255367
679680,1359361,1359360,2718721,6525.908246040344,0.2993402042757225
680681,1361363,1361362,2722725,6529.12406873703,0.29893101679044776
681682,1363365,1363364,2726729,6532.34984087944,0.29852296648095944
682683,1365367,1365366,2730733,6535.596340894699,0.2981160485833243
683684,1367369,1367368,2734737,6538.853027820587,0.297710258344523
684685,1369371,1369370,2738741,6542.072066068649,0.2943088959909801
685686,1371373,1371372,2742745,6545.343966960907,0.29391358124485123
686687,1373375,1373374,2746749,6548.542407751083,0.2935193459052243
687688,1375377,1375376,2750753,6551.766793966293,0.29312618551375635
688689,1377379,1377378,2754757,6554.9666249752045,0.2927340956466651
689690,1379381,1379380,2758761,6558.185345888138,0.2923430718965392
690691,1381383,1381382,2762765,6561.483507871628,0.2919531098814332
691692,1383385,1383384,2766769,6564.695964813232,0.2915642052430485
692693,1385387,1385386,2770773,6567.965763092041,0.2911763536540093
693694,1387389,1387388,2774777,6571.159235715866,0.29078955079785374
694695,1389391,1389390,2778781,6574.377707958221,0.29040379239268077
695696,1391393,1391392,2782785,6577.629420995712,0.29001907417477923
696697,1393395,1393394,2786789,6580.940805912018,0.2896353919040848
697698,1395397,1395396,2790793,6584.301732778549,0.2892527413623611
698699,1397399,1397398,2794797,6587.5180468559265,0.28887111835865653
699700,1399401,1399400,2798801,6590.718092918396,0.28849051872020937
700701,1401403,1401402,2802805,6593.955326795578,0.2881109382997238
701702,1403405,1403404,2806809,6597.3157868385315,0.28773237296809384
702703,1405407,1405406,2810813,6600.527693986893,0.28735481862349843
703704,1407409,1407408,2814817,6603.7732837200165,0.2869782711859443
704705,1409411,1409410,2818821,6606.971773862839,0.2866027265881712
705706,1411413,1411412,2822825,6610.196675777435,0.2862281807974796
706707,1413415,1413414,2826829,6613.3851749897,0.28585462979572185
707708,1415417,1415416,2830833,6616.615641832352,0.2854820695883973
708709,1417419,1417418,2834837,6619.8359088897705,0.28511049620101403
709710,1419421,1419420,2838841,6623.053678035736,0.28473990567908913
710711,1421423,1421422,2842845,6626.321953058243,0.2843702940936055
711712,1423425,1423424,2846849,6629.537410020828,0.28400165753191686
712713,1425427,1425426,2850853,6632.773181915283,0.28363399210502394
713714,1427429,1427428,2854857,6636.152781009674,0.2832672939457552
714715,1429431,1429430,2858861,6639.485549926758,0.2829015591996722
715716,1431433,1431432,2862865,6642.716091871262,0.2825367840450781
716717,1433435,1433434,2866869,6645.925002813339,0.28217296466755215
717718,1435437,1435436,2870873,6649.341100931168,0.2818100972835964
718719,1437439,1437438,2874877,6652.769978761673,0.28144817812062684
719720,1439441,1439440,2878881,6656.115115880966,0.28108720343516325
720721,1441443,1441442,2882885,6659.440594911575,0.2807271694964584
721722,1443445,1443444,2886889,6662.85814499855,0.2803680725955928
722723,1445447,1445446,2890893,6666.239275932312,0.2800099090418371
723724,1447449,1447448,2894897,6669.56826376915,0.27965267516628955
724725,1449451,1449450,2898901,6672.920606851578,0.2792963673182385
725726,1451453,1451452,2902905,6676.202261924744,0.27894098186516203
726727,1453455,1453454,2906909,6679.644003868103,0.27858651519454725
727728,1455457,1455456,2910913,6682.9373087883,0.2782329637102521
728729,1457459,1457458,2914917,6686.205605745316,0.27788032384160033
729730,1459461,1459460,2918921,6689.518411874771,0.27752859202701075
730731,1461463,1461462,2922925,6692.831146001816,0.2771777647303679
731732,1463465,1463464,2926929,6696.110265016556,0.2768278384319274
732733,1465467,1465466,2930933,6699.52019572258,0.2764788096264965
733734,1467469,1467468,2934937,6702.927377939224,0.2761306748343486
734735,1469471,1469470,2938941,6706.31231880188,0.27578343058848986
735736,1471473,1471472,2942945,6709.699546813965,0.27543707344193535
736737,1473475,1473474,2946949,6713.0672607421875,0.27509159996407107
737738,1475477,1475476,2950953,6716.548014879227,0.2747470067388349
738739,1477479,1477478,2954957,6720.012903928757,0.2744032903792686
739740,1479481,1479480,2958961,6723.420598983765,0.27406044750205183
740741,1481483,1481482,2962965,6726.849880695343,0.2737184747475112
741742,1483485,1483484,2966969,6730.505563735962,0.27337736877780117
742743,1485487,1485486,2970973,6733.952852964401,0.2730371262587141
743744,1487489,1487488,2974977,6737.376483678818,0.2726977438887843
744745,1489491,1489490,2978981,6740.862755060196,0.27235921837200294
745746,1491493,1491492,2982985,6744.236685991287,0.27202154643600807
746747,1493495,1493494,2986989,6747.6382830142975,0.2716847248211707
747748,1495497,1495496,2990993,6750.997195959091,0.27134875028605165
748749,1497499,1497498,2994997,6754.522047996521,0.2710136196037638
749750,1499501,1499500,2999001,6757.997802972794,0.2706793295674288
750751,1501503,1501502,3003005,6761.363619804382,0.27034587698108226
751752,1503505,1503504,3007009,6764.7736740112305,0.27001325867240666
752753,1505507,1505506,3011013,6768.152971982956,0.26968147147817945
753754,1507509,1507508,3015017,6771.540175676346,0.26935051225154893
754755,1509511,1509510,3019021,6774.97492980957,0.26902037786749133
755756,1511513,1511512,3023025,6778.631997823715,0.2686910652100778
756757,1513515,1513514,3027029,6782.131858825684,0.26836257118702633
757758,1515517,1515516,3031033,6785.53738284111,0.26803489271151193
758759,1517519,1517518,3035037,6788.921717882156,0.26770802671671845
759760,1519521,1519520,3039041,6792.331095933914,0.26738197015765763
760761,1521523,1521522,3043045,6795.730521678925,0.2670567199911602
761762,1523525,1523524,3047049,6799.064050912857,0.26673227319770376
762763,1525527,1525526,3051053,6802.419593811035,0.26640862677959376
763764,1527529,1527528,3055057,6805.847347974777,0.2660857777354977
764765,1529531,1529530,3059061,6809.422199010849,0.26576372309682483
765766,1531533,1531532,3063065,6812.928192853928,0.26544245990226045
766767,1533535,1533534,3067069,6816.334022760391,0.2651219852032227
767768,1535537,1535536,3071073,6819.649785757065,0.26480229606568173
768769,1537539,1537538,3075077,6823.013012886047,0.2644833895810734
769770,1539541,1539540,3079081,6826.380821943283,0.26416526283719577
770771,1541543,1541542,3083085,6829.84002995491,0.2638479129564075
771772,1543545,1543544,3087089,6833.374109983444,0.2635313370556105
772773,1545547,1545546,3091093,6836.833458900452,0.2632155322753533
773774,1547549,1547548,3095097,6840.274219989777,0.26290049577619357
774775,1549551,1549550,3099101,6843.728978872299,0.2625862247241457
775776,1551553,1551552,3103105,6847.100841999054,0.26227271629613824
776777,1553555,1553554,3107109,6850.50843000412,0.2619599676945654
777778,1555557,1555556,3111113,6853.967331647873,0.26164797612545954
778779,1557559,1557558,3115117,6857.373530864716,0.2613367388184997
779780,1559561,1559560,3119121,6860.836153745651,0.26102625299972715
780781,1561563,1561562,3123125,6864.2968780994415,0.26071651592974376
781782,1563565,1563564,3127129,6867.664527893066,0.26040752486915153
782783,1565567,1565566,3131133,6870.937626838684,0.26009927709128533
783784,1567569,1567568,3135137,6874.227132797241,0.2597917698913079
784785,1569571,1569570,3139141,6877.512289047241,0.259485000573477
785786,1571573,1571572,3143145,6880.795767068863,0.25917896645114524
786787,1573575,1573574,3147149,6884.065416812897,0.25887366485585517
787788,1575577,1575576,3151153,6887.391956806183,0.25856909313006327
788789,1577579,1577578,3155157,6890.71123790741,0.25826524862895894
789790,1579581,1579580,3159161,6894.022766113281,0.2579621287222835
790791,1581583,1581582,3163165,6897.340112924576,0.25765973079069227
791792,1583585,1583584,3167169,6900.66024184227,0.25735805222575436
792793,1585587,1585586,3171173,6903.975282907486,0.2570570904354099
793794,1587589,1587588,3175177,6907.269498825073,0.256756842836694
794795,1589591,1589590,3179181,6910.546430826187,0.25645730686665047
795796,1591593,1591592,3183185,6913.8371069431305,0.25615847996050434
796797,1593595,1593594,3187189,6917.123598098755,0.2558603595771274
797798,1595597,1595596,3191193,6920.378448724747,0.25556294318630535
798799,1597599,1597598,3195197,6923.673295736313,0.2552662282669189
799800,1599601,1599600,3199201,6926.985529661179,0.2549702123124007
800801,1601603,1601602,3203205,6930.261360883713,0.25467489282164024
801802,1603605,1603604,3207209,6933.62789773941,0.254380267315355
802803,1605607,1605606,3211213,6937.160803794861,0.2540863333197194
803804,1607609,1607608,3215217,6940.572773694992,0.2537930883736408
804805,1609611,1609610,3219221,6943.974435091019,0.2535005300269404
805806,1611613,1611612,3223225,6947.374233722687,0.2532086558476294
806807,1613615,1613614,3227229,6950.796676874161,0.252917463407357
807808,1615617,1615616,3231233,6954.181272029877,0.2526269502886862
808809,1617619,1617618,3235237,6957.625860691071,0.25233711409055104
809810,1619621,1619620,3239241,6961.150424718857,0.2520479524227994
810811,1621623,1621622,3243245,6964.561151981354,0.2517594629061932
811812,1623625,1623624,3247249,6967.938083648682,0.25147164316695125
812813,1625627,1625626,3251253,6971.343863964081,0.2511844908531202
813814,1627629,1627628,3255257,6974.71529173851,0.2508980036163848
814815,1629631,1629630,3259261,6978.114489078522,0.25061217911388667
815816,1631633,1631632,3263265,6981.457641839981,0.2503270150300523
816817,1633635,1633634,3267269,6984.750149726868,0.2500425090511271
817818,1635637,1635636,3271273,6988.030082941055,0.24975865886699467
818819,1637639,1637638,3275277,6991.314100980759,0.24947546218754724
819820,1639641,1639640,3279281,6994.778747797012,0.24919291673359112
820821,1641643,1641642,3283285,6998.22082567215,0.24891102023138956
821822,1643645,1643644,3287289,7001.5148549079895,0.2486297704253957
822823,1645647,1645646,3291293,7004.813850879669,0.24834916506188165
823824,1647649,1647648,3295297,7008.0989990234375,0.24806920190167148
824825,1649651,1649650,3299301,7011.406094074249,0.24778987871650315
825826,1651653,1651652,3303305,7014.843783855438,0.24751119328357163
826827,1653655,1653654,3307309,7018.318301916122,0.24723314340008073
827828,1655657,1655656,3311313,7021.867427825928,0.24695572686687228
828829,1657659,1657658,3315317,7025.278573036194,0.24667894149570202
829830,1659661,1659660,3319321,7028.67537689209,0.24640278510378266
830831,1661663,1661662,3323325,7032.120250701904,0.2461272555301548
831832,1663665,1663664,3327329,7035.519524812698,0.24585235061204003
832833,1665667,1665666,3331333,7038.943743944168,0.24557806820303085
833834,1667669,1667668,3335337,7042.335615873337,0.24530440616763372
834835,1669671,1669670,3339341,7045.780867099762,0.24503136237035505
835836,1671673,1671672,3343345,7049.195443868637,0.24475893469934817
836837,1673675,1673674,3347349,7052.57124876976,0.24448712104276638
837838,1675677,1675676,3351353,7055.927235841751,0.24421591930513387
838839,1677679,1677678,3355357,7059.262759923935,0.24394532738915586
839840,1679681,1679680,3359361,7062.552314758301,0.24367534322118445
840841,1681683,1681682,3363365,7065.834446668625,0.2434059647275717
841842,1683685,1683684,3367369,7069.360991001129,0.2431371898492216
842843,1685687,1685686,3371373,7072.8025987148285,0.24286901653249515
843844,1687689,1687688,3375377,7076.181993961334,0.2426014427364862
844845,1689691,1689690,3379381,7079.61301779747,0.24233446642574563
845846,1691693,1691692,3383385,7083.019444942474,0.2420680855793762
846847,1693695,1693694,3387389,7086.445501804352,0.24180229817829968
847848,1695697,1695696,3391393,7089.926592826843,0.24153710221798974
848849,1697699,1697698,3395397,7093.325985908508,0.241272495704834
849850,1699701,1699700,3399401,7096.899954795837,0.24100847664885805
850851,1701703,1701702,3403405,7100.40446472168,0.24074504307100142
851852,1703705,1703704,3407409,7103.898104906082,0.24048219300129858
852853,1705707,1705706,3411413,7107.4116678237915,0.24021992447887897
853854,1707709,1707708,3415417,7110.813421964645,0.23995823555560492
854855,1709711,1709710,3419421,7114.2797498703,0.2396971242815198
855856,1711713,1711712,3423425,7117.6988480091095,0.23943658872485685
856857,1713715,1713714,3427429,7121.128174781799,0.2391766269593063
857858,1715717,1715716,3431433,7124.550998926163,0.2389172370712913
858859,1717719,1717718,3435437,7127.963385105133,0.238658417147235
859860,1719721,1719720,3439441,7131.329593896866,0.2384001652862935
860861,1721723,1721722,3443445,7134.624567985535,0.23814247960035573
861862,1723725,1723724,3447449,7137.9521317481995,0.23788535820312973
862863,1725727,1725726,3451453,7141.255993843079,0.2376287992210564
863864,1727729,1727728,3455457,7144.549635648727,0.23737280078603362
864865,1729731,1729730,3459461,7147.964555978775,0.23711736104087322
865866,1731733,1731732,3463465,7151.406725883484,0.23686247813748196
866867,1733735,1733734,3467469,7154.836664915085,0.2366081502259476
867868,1735737,1735736,3471473,7158.244302034378,0.2363543754836428
868869,1737739,1737738,3475477,7161.871914863586,0.2361011520752072
869870,1739741,1739740,3479481,7165.368805885315,0.2358484781889274
870871,1741743,1741742,3483485,7168.755460739136,0.23559635201127094
871872,1743745,1743744,3487489,7172.217801809311,0.2353447717450763
872873,1745747,1745746,3491493,7175.641801834106,0.23509373559136293
873874,1747749,1747748,3495497,7179.0511820316315,0.23484324176752125
874875,1749751,1749750,3499501,7182.453596830368,0.2345932884963986
875876,1751753,1751752,3503505,7186.105235815048,0.23434387400084233
876877,1753755,1753754,3507509,7189.614628791809,0.23409499653098464
877878,1755757,1755756,3511513,7193.03270483017,0.23384665431876783
878879,1757759,1757758,3515517,7196.519917011261,0.23359884562523803
879880,1759761,1759760,3519521,7200.024370908737,0.23335156870780338
880881,1761763,1761762,3523525,7203.473123788834,0.23310482183842396
881882,1763765,1763764,3527529,7206.973905801773,0.23285860328724084
882883,1765767,1765766,3531533,7210.420163869858,0.232612911340766
883884,1767769,1767768,3535537,7213.92503285408,0.2323677442909684
884885,1769771,1769770,3539541,7217.360615968704,0.232123100429817
885886,1771773,1771772,3543545,7220.756438970566,0.2318789780692896
886887,1773775,1773774,3547549,7224.155162811279,0.23163537551954505
887888,1775777,1775776,3551553,7227.567172765732,0.23139229110165616
888889,1777779,1777778,3555557,7230.971856832504,0.23114972314033366
889890,1779781,1779780,3559561,7234.387432813644,0.23090766997302126
890891,1781783,1781782,3563565,7237.8413009643555,0.2306661299408006
891892,1783785,1783784,3567569,7241.263599872589,0.2304251013938483
892893,1785787,1785786,3571573,7244.7037088871,0.23018458268597897
893894,1787789,1787788,3575577,7248.1442539691925,0.2299445721801021
894895,1789791,1789790,3579581,7251.574720859528,0.22970506824640324
895896,1791793,1791792,3583585,7255.141051769257,0.2294660692641628
896897,1793795,1793794,3587589,7258.70156288147,0.2292275736162992
897898,1795797,1795796,3591593,7262.122880935669,0.2289895796966448
898899,1797799,1797798,3595597,7265.580028772354,0.22875208589721296
899900,1799801,1799800,3599601,7269.008943796158,0.22851509062820696
900901,1801803,1801802,3603605,7272.45382976532,0.22827859229619207
901902,1803805,1803804,3607609,7275.888356685638,0.22804258932410448
902903,1805807,1805806,3611613,7279.349608898163,0.22780708013488038
903904,1807809,1807808,3615617,7282.85325884819,0.2275720631605509
904905,1809811,1809810,3619621,7286.256347894669,0.22733753684042313
905906,1811813,1811812,3623625,7289.685081720352,0.22710349961744214
906907,1813815,1813814,3627629,7293.11092877388,0.22686994994728593
907908,1815817,1815816,3631633,7296.525981903076,0.2266368862838135
908909,1817819,1817818,3635637,7299.9357488155365,0.2264043070954358
909910,1819821,1819820,3639641,7303.340199947357,0.22617221085056372
910911,1821823,1821822,3643645,7306.92357301712,0.2259405960303411
911912,1823825,1823824,3647649,7310.452172994614,0.22570946111409285
912913,1825827,1825826,3651653,7313.867506980896,0.22547880459933367
913914,1827829,1827828,3655657,7317.3484308719635,0.22524862497630238
914915,1829831,1829830,3659661,7320.755743980408,0.22501892074978969
915916,1831833,1831832,3663665,7324.1989569664,0.22478969043004327
916917,1833835,1833834,3667669,7327.611304998398,0.22456093253640574
917918,1835837,1835836,3671673,7331.061192989349,0.22433264558640076
918919,1837839,1837838,3675677,7334.5588138103485,0.22410482810846588
919920,1839841,1839840,3679681,7337.9814016819,0.22387747864013363
920921,1841843,1841842,3683685,7341.733428955078,0.22365059571893653
921922,1843845,1843844,3687689,7345.153155088425,0.22342417789150204
922923,1845847,1845846,3691693,7348.615777015686,0.22319822371355258
923924,1847849,1847848,3695697,7352.017814874649,0.22297273174081056
924925,1849851,1849850,3699701,7355.4517476558685,0.22274770053991233
925926,1851853,1851852,3703705,7358.877898931503,0.22252312868113222
926927,1853855,1853854,3707709,7362.342315912247,0.22229901473838254
927928,1855857,1855856,3711713,7365.930358886719,0.22207535729830852
928929,1857859,1857858,3715717,7369.6276948452,0.2218521549475554
929930,1859861,1859860,3719721,7373.036388874054,0.22162940628004435
930931,1861863,1861862,3723725,7376.31768488884,0.22140710989879153
931932,1863865,1863864,3727729,7379.64874792099,0.2211852644031751
932933,1865867,1865866,3731733,7383.005628824234,0.2209638684107631
933934,1867869,1867868,3735737,7386.392657756805,0.22074292054094258
934935,1869871,1869870,3739741,7389.742038965225,0.2205224194094626
935936,1871873,1871872,3743745,7393.066790819168,0.22030236365026212
936937,1873875,1873874,3747749,7396.380449056625,0.22008275189182314
937938,1875877,1875876,3751753,7399.683681964874,0.2198635827826365
938939,1877879,1877878,3755757,7402.986771821976,0.21964485496209818
939940,1879881,1879880,3759761,7406.270724773407,0.21942656708415598
940941,1881883,1881882,3763765,7409.590646028519,0.21920871780639573
941942,1883885,1883884,3767769,7412.8522918224335,0.21899130578640325
942943,1885887,1885886,3771773,7416.166306018829,0.21877432969631627
943944,1887889,1887888,3775777,7419.445437908173,0.21855778820645355
944945,1889891,1889890,3779781,7422.74461889267,0.21834167999804777
945946,1891893,1891892,3783785,7426.233456850052,0.2181260037541506
946947,1893895,1893894,3787789,7429.687852859497,0.21791075816145167
947948,1895897,1895896,3791793,7433.128411769867,0.2176959419157356
948949,1897899,1897898,3795797,7436.812018871307,0.21748155372188194
949950,1899901,1899900,3799801,7440.471703052521,0.21726759227749426
950951,1901903,1901902,3803805,7444.065665960312,0.21705405629472807
951952,1903905,1903904,3807809,7447.68877696991,0.21684094449483382
952953,1905907,1905906,3811813,7451.211894035339,0.216628255593605
953954,1907909,1907908,3815817,7454.708169937134,0.216415988317749
954955,1909911,1909910,3819821,7458.259516954422,0.21620414139761124
955956,1911913,1911912,3823825,7461.886417865753,0.21599271357263206
956957,1913915,1913914,3827829,7465.564654827118,0.2157817035804328
957958,1915917,1915916,3831833,7469.161808729172,0.21557111016954877
958959,1917919,1917918,3835837,7472.877789974213,0.21536093209215323
959960,1919921,1919920,3839841,7476.55583691597,0.21515116810587642
960961,1921923,1921922,3843845,7480.20828795433,0.2149418169665296
961962,1923925,1923924,3847849,7483.843883037567,0.2147328774444759
962963,1925927,1925926,3851853,7487.241086959839,0.21452434831371647
963964,1927929,1927928,3855857,7490.697666883469,0.2143162283446145
964965,1929931,1929930,3859861,7494.080336809158,0.21410851632572303
965966,1931933,1931932,3863865,7497.6062977313995,0.21390121103650017
966967,1933935,1933934,3867869,7501.236473798752,0.21369431127095595
967968,1935937,1935936,3871873,7504.773106813431,0.21348781582491938
968969,1937939,1937938,3875877,7508.254099845886,0.21328172349785746
969970,1939941,1939940,3879881,7511.818331718445,0.21307603309469414
970971,1941943,1941942,3883885,7515.309058904648,0.21287074342944834
971972,1943945,1943944,3887889,7518.741774082184,0.21266585331250099
972973,1945947,1945946,3891893,7522.062552690506,0.21246136156332796
973974,1947949,1947948,3895897,7525.328372001648,0.21225726700868108
974975,1949951,1949950,3899901,7528.599142789841,0.2120535684753122
975976,1951953,1951952,3903905,7531.811594009399,0.2118502648008871
976977,1953955,1953954,3907909,7535.079395771027,0.21164735481943353
977978,1955957,1955956,3911913,7538.300035715103,0.21144483737407427
978979,1957959,1957958,3915917,7541.503690004349,0.21124271131157002
979980,1959961,1959960,3919921,7544.688993930817,0.21104097548777645
980981,1961963,1961962,3923925,7547.890095710754,0.21083962875491125
981982,1963965,1963964,3927929,7551.141891717911,0.21063866997428704
982983,1965967,1965966,3931933,7554.406288862228,0.21043809801267344
983984,1967969,1967968,3935937,7557.700528860092,0.21023791173684003
984985,1969971,1969970,3939941,7560.961875915527,0.21003811002447037
985986,1971973,1971972,3943945,7564.241085767746,0.20983869175324799
986987,1973975,1973974,3947949,7567.5286729335785,0.20963965580813237
987988,1975977,1975976,3951953,7570.840570688248,0.20944100107226404
988989,1977979,1977978,3955957,7574.133271932602,0.20924272643969744
989990,1979981,1979980,3959961,7577.419539928436,0.209044830804487
990991,1981983,1981982,3963965,7580.703362941742,0.2088473130697821
991992,1983985,1983984,3967969,7584.000538825989,0.20865017213873216
992993,1985987,1985986,3971973,7587.327582836151,0.20845340691994352
993994,1987989,1987988,3975977,7590.598361730576,0.2082570163274795
994995,1989991,1989990,3979981,7593.900473117828,0.20806099927540345
995996,1991993,1991992,3983985,7597.216379880905,0.20786535469233058
996997,1993995,1993994,3987989,7600.53817987442,0.20767008149596222
997998,1995997,1995996,3991993,7603.865211725235,0.20747517862218956
998999,1997999,1997998,3995997,7607.157012939453,0.20728064500144683
1000000,2000001,2000000,4000001,7610.409976005554,0.2070864795750822


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002474069595336914,12064.682476916567
1001,2003,2002,4005,3.6562042236328125,65.52576608160416
2002,4005,4004,8009,7.248206853866577,42.34509678336872
3003,6007,6006,12013,11.04786491394043,34.023520514219854
4004,8009,8008,16017,14.50561809539795,28.958911805193566
5005,10011,10010,20021,18.777812957763672,25.333523203886216
6006,12013,12012,24025,22.469918966293335,22.527300385168928
7007,14015,14014,28029,25.92417597770691,20.253121634779745
8008,16017,16016,32033,29.24285912513733,18.355877411981055
9009,18019,18018,36037,32.58391785621643,16.742261724328273
10010,20021,20020,40041,35.91790509223938,15.35118558117756
11011,22023,22022,44045,39.232887983322144,14.139884765472743
12012,24025,24024,48049,42.51778697967529,13.076857731883138
13013,26027,26026,52053,45.83771800994873,12.138017055509408
14014,28029,28028,56057,49.15849304199219,11.30442975218466
15015,30031,30030,60061,52.627357959747314,10.560884002585226
16016,32033,32032,64065,56.25014519691467,9.894970055029262
17017,34035,34034,68069,59.66333293914795,9.296433581814199
18018,36037,36036,72073,63.050535917282104,8.756706160584145
19019,38039,38038,76077,66.3240110874176,8.26856343260988
20020,40041,40040,80081,69.58702301979065,7.825866925420996
21021,42043,42042,84085,72.88530492782593,7.423363869536843
22022,44045,44044,88089,76.24873995780945,7.0565315885924065
23023,46047,46046,92093,79.6149959564209,6.721454575370444
24024,48049,48048,96097,82.89304304122925,6.414726327160679
25025,50051,50050,100101,86.15027785301208,6.133370176887183
26026,52053,52052,104105,89.4551408290863,5.874774859685203
27027,54055,54054,108109,92.77283215522766,5.636641623708783
28028,56057,56056,112113,96.0748679637909,5.4169404684380424
29029,58059,58058,116117,99.35476207733154,5.213873662669357
30030,60061,60060,120121,102.65840482711792,5.025845117053905
31031,62063,62062,124125,105.96915698051453,4.851434503312703
32032,64065,64064,128129,109.25755000114441,4.689375251909951
33033,66067,66066,132133,112.52728700637817,4.5385357427494455
34034,68069,68068,136137,115.8041181564331,4.397903143561052
35035,70071,70070,140141,119.08533096313477,4.266569458923186
36036,72073,72072,144145,122.33660697937012,4.143719436893662
37037,74075,74074,148149,125.63575887680054,4.028620046206925
38038,76077,76076,152153,128.90019488334656,3.920611288767759
39039,78079,78078,156157,132.17271399497986,3.8190981533571176
40040,80081,80080,160161,135.43414902687073,3.723543549363967
41041,82083,82082,164165,138.6763458251953,3.633462985213555
42042,84085,84084,168169,141.95461201667786,3.548416926021673
43043,86087,86086,172173,145.1573121547699,3.4680069331843697
44044,88089,88088,176177,148.52698612213135,3.3918722434391384
45045,90091,90090,180181,151.79118299484253,3.3196853393728816
46046,92093,92092,184185,155.0806930065155,3.251148560690126
47047,94095,94094,188189,158.55242800712585,3.185991089043455
48048,96097,96096,192193,161.91575694084167,3.123966261749956
49049,98099,98098,196197,165.22131204605103,3.0648491757310694
50050,100101,100100,200201,168.47206902503967,3.0084345479244803
51051,102103,102102,204205,171.7801821231842,2.9545348027186265
52052,104105,104104,208209,175.0591859817505,2.9029783606383717
53053,106107,106106,212213,178.31591987609863,2.8536081056681724
54054,108109,108108,216217,181.64597415924072,2.8062800112911646
55055,110111,110110,220221,184.99818086624146,2.760861907792787
56056,112113,112112,224225,188.2722098827362,2.7172323753002274
57057,114115,114114,228229,191.54824090003967,2.6752797489734803
58058,116117,116116,232233,194.83267307281494,2.634901224208079
59059,118119,118118,236237,198.1087019443512,2.5960020512011397
60060,120121,120120,240241,201.37652587890625,2.558494809345575
61061,122123,122122,244245,204.6800661087036,2.5222987530560204
62062,124125,124124,248249,207.94788098335266,2.4873392215158674
63063,126127,126126,252253,211.24517583847046,2.453547105709731
64064,128129,128128,256257,214.52350497245789,2.4208583667805215
65065,130131,130130,260261,217.7814919948578,2.3892136004760687
66066,132133,132132,264265,221.07138323783875,2.358557642886808
67067,134135,134134,268269,224.34233713150024,2.328839213394531
68068,136137,136136,272273,227.66224598884583,2.30001059096503
69069,138139,138138,276277,230.92909598350525,2.2720273204940895
70070,140141,140140,280281,234.21257305145264,2.244847946203663
71071,142143,142142,284285,237.47074484825134,2.2184337693543057
72072,144145,144144,288289,240.73543310165405,2.1927486279837467
73073,146147,146146,292293,243.99914717674255,2.16775870678066
74074,148149,148148,296297,247.25601482391357,2.1434324638539692
75075,150151,150150,300301,250.5529329776764,2.119740070320404
76076,152153,152152,304305,253.84342098236084,2.0966536762553005
77077,154155,154154,308309,257.14520502090454,2.074147128711047
78078,156157,156156,312313,260.4210031032562,2.052195844546077
79079,158159,158158,316317,263.70937395095825,2.0307766945152252
80080,160161,160160,320321,266.9841728210449,2.0098678971498884
81081,162163,162162,324325,270.24792313575745,1.9894489215548674
82082,164165,164164,328329,273.5666389465332,1.9695003982669732
83083,166167,166166,332333,276.8556070327759,1.9500040374550736
84084,168169,168168,336337,280.13468980789185,1.9309425537958305
85085,170171,170170,340341,283.3652811050415,1.9122995973975776
86086,172173,172172,344345,286.6167039871216,1.8940596902666584
87087,174175,174174,348349,289.8852550983429,1.876208167801451
88088,176177,176176,352353,293.12982511520386,1.8587311248629703
89089,178179,178178,356357,296.40201711654663,1.8416153660473356
90090,180181,180180,360361,299.9115159511566,1.82484835977084
91091,182183,182182,364365,303.32374000549316,1.808418195856575
92092,184185,184184,368369,306.59454798698425,1.7923135463061044
93093,186187,186186,372373,309.84522819519043,1.77652362900335
94094,188189,188188,376377,313.13743019104004,1.7610381741033052
95095,190191,190190,380381,316.41469407081604,1.7458473928472813
96096,192193,192192,384385,319.70901107788086,1.730941948671898
97097,194195,194194,388389,323.07644295692444,1.716313168311899
98098,196197,196196,392393,326.41600799560547,1.7019523075414327
99099,198199,198198,396397,329.7309579849243,1.6878512114781188
100100,200201,200200,400401,332.9953360557556,1.6740021029290801
101101,202203,202202,404405,336.29006814956665,1.6603975401721982
102102,204205,204204,408409,339.59982895851135,1.6470303982314363
103103,206207,206206,412413,342.89549493789673,1.6338938513763424
104104,208209,208208,416417,346.1728069782257,1.6209813568148093
105105,210211,210210,420421,349.4274709224701,1.6082866394281154
106106,212213,212212,424425,352.9198589324951,1.595803677533695
107107,214215,214214,428429,356.2989320755005,1.5835266895282984
108108,216217,216216,432433,359.5523750782013,1.5714501214133634
109109,218219,218218,436437,362.8417270183563,1.5595686350789038
110110,220221,220220,440441,366.06811714172363,1.5478770973513747
111111,222223,222222,444445,369.3235430717468,1.5363705696745455
112112,224225,224224,448449,372.5838689804077,1.525044298477951
113113,226227,226226,452453,375.9017939567566,1.5138937060619355
114114,228229,228228,456457,379.28878021240234,1.50291438208842
115115,230231,230230,460461,382.55477690696716,1.492102075528237
116116,232233,232232,464465,385.8574140071869,1.4814526871195994
117117,234235,234234,468469,389.130487203598,1.4709622622413008
118118,236237,236236,472473,392.3820071220398,1.4606269841842732
119119,238239,238238,476477,395.664932012558,1.450443167841513
120120,240241,240240,480481,398.93274307250977,1.440407253730882
121121,242243,242242,484485,402.25536489486694,1.430515802341688
122122,244245,244244,488489,405.5646619796753,1.4207654888195975
123123,246247,246246,492493,408.8249568939209,1.411153097913484
124124,248249,248248,496497,412.0990080833435,1.4016755192224082
125125,250251,250250,500501,415.3806710243225,1.3923297426754289
126126,252253,252252,504505,418.6388928890228,1.3831128542660736
127127,254255,254254,508509,421.9202241897583,1.3740220320014487
128128,256257,256256,512513,425.23567605018616,1.365054542065991
129129,258259,258258,516517,428.4683349132538,1.3562077351853077
130130,260261,260260,520521,431.7616879940033,1.3474790431719157
131131,262263,262262,524525,435.08780908584595,1.3388659756383277
132132,264265,264264,528529,438.50223302841187,1.330366116897494
133133,266267,266266,532533,441.7632899284363,1.3219771229923936
134134,268269,268268,536537,445.1087188720703,1.3136967188820563
135135,270271,270270,540541,448.43822598457336,1.3055226957658306
136136,272273,272272,544545,451.7961280345917,1.2974529085367976
137137,274275,274274,548549,455.1235649585724,1.2894852733516018
138138,276277,276276,552553,458.41097712516785,1.281617765320334
139139,278279,278278,556557,461.70008993148804,1.2738484163073736
140140,280281,280280,560561,465.00318598747253,1.2661753128159035
141141,282283,282282,564565,468.2995309829712,1.258596594005212
142142,284285,284284,568569,471.5778839588165,1.2511104497643828
143143,286287,286286,572573,474.8299810886383,1.2437151188787539
144144,288289,288288,576577,478.10858821868896,1.2364088873127912
145145,290291,290290,580581,481.3888268470764,1.229190086514791
146146,292293,292292,584585,484.6915080547333,1.2220570918361773
147147,294295,294294,588589,488.1047189235687,1.2150083210181037
148148,296297,296296,592593,491.56655383110046,1.208042283073155
149149,298299,298298,596597,494.9070348739624,1.2011575415090192
150150,300301,300300,600601,498.1964280605316,1.1943525150909409
151151,302303,302302,604605,501.44788002967834,1.187625777127323
152152,304305,304304,608609,504.74811911582947,1.180975936629693
153153,306307,306306,612613,508.0012879371643,1.1744016371158068
154154,308309,308308,616617,511.32931113243103,1.167901555494609
155155,310311,310310,620621,514.7023069858551,1.1614744009748392
156156,312313,312312,624625,518.0369141101837,1.1551189140373026
157157,314315,314314,628629,521.3588199615479,1.148833865438064
158158,316317,316316,632633,524.606173992157,1.142618055238927
159159,318319,318318,636637,527.8979170322418,1.1364703119179467
160160,320321,320320,640641,531.2918429374695,1.1303894914599368
161161,322323,322322,644645,534.659049987793,1.1243744765251904
162162,324325,324324,648649,537.9546790122986,1.1184241756291158
163163,326327,326326,652653,541.2264919281006,1.1125375223582523
164164,328329,328328,656657,544.5571799278259,1.1067134746172087
165165,330331,330330,660661,547.8248820304871,1.1009510139065242
166166,332333,332332,664665,551.2407691478729,1.0952491446150816
167167,334335,334334,668669,554.6758668422699,1.0896068933579954
168168,336337,336336,672673,557.9796187877655,1.0840233083272324
169169,338339,338338,676677,561.4323000907898,1.0784974586531462
170170,340341,340340,680681,564.7022368907928,1.073028433827858
171171,342343,342342,684685,568.0147080421448,1.0676153430977138
172172,344345,344344,688689,571.3126649856567,1.0622573149266827
173173,346347,346346,692693,574.827455997467,1.0569534964452032
174174,348349,348348,696697,578.1247460842133,1.0517030529299518
175175,350351,350350,700701,581.4054050445557,1.0465051673072594
176176,352353,352352,704705,584.7265040874481,1.0413590396601649
177177,354355,354354,708709,587.9840610027313,1.0362638867682108
178178,356357,356356,712713,591.2906489372253,1.0312189416436013
179179,358359,358358,716717,594.5910730361938,1.0262234531091963
180180,360361,360360,720721,597.9029960632324,1.0212766853655921
181181,362363,362362,724725,601.162572145462,1.016377917583668
182182,364365,364364,728729,604.4481348991394,1.0115264435098652
183183,366367,366366,732733,607.6983277797699,1.0067215710932942
184184,368369,368368,736737,610.9646019935608,1.001962622100109
185185,370371,370370,740741,614.2318758964539,0.9972489317715372
186186,372373,372372,744745,617.5393629074097,0.9925798484691768
187187,374375,374374,748749,620.7853138446808,0.9879547333403025
188188,376377,376376,752753,624.1564428806305,0.9833729599995422
189189,378379,378378,756757,627.5263910293579,0.9788339142123732
190190,380381,380380,760761,630.8961727619171,0.9743369935858937
191191,382383,382382,764765,634.2168669700623,0.9698816072850605
192192,384385,384384,768769,637.4863519668579,0.9654671757307369
193193,386387,386386,772773,640.8159608840942,0.9610931303413963
194194,388389,388388,776777,644.1124927997589,0.9567589132529974
195195,390391,390390,780781,647.4065208435059,0.9524639770606882
196196,392393,392392,784785,650.690623998642,0.9482077845750609
197197,394395,394394,788789,653.9536578655243,0.9439898085620371
198198,396397,396396,792793,657.2507309913635,0.9398095315154933
199199,398399,398398,796797,660.5189960002899,0.935666445429888
200200,400401,400400,800801,663.8212819099426,0.9315600515710685
201201,402403,402402,804805,667.1472988128662,0.9274898602525354
202202,404405,404404,808809,670.4779851436615,0.923455390638992
203203,406407,406406,812813,674.010124206543,0.9194561705353408
204204,408409,408408,816817,677.3476119041443,0.9154917361811385
205205,410411,410410,820821,680.636491060257,0.9115616320723348
206206,412413,412412,824825,683.9164659976959,0.907665410755726
207207,414415,414414,828829,687.1774809360504,0.9038026326543331
208208,416417,416416,832833,690.5222940444946,0.8999728659055108
209209,418419,418418,836837,693.956573009491,0.8961756861554022
210210,420421,420420,840841,697.3416700363159,0.8924106764297903
211211,422423,422422,844845,700.6394441127777,0.8886774269285524
212212,424425,424424,848849,703.910028219223,0.8849755349092447
213213,426427,426426,852853,707.2069058418274,0.8813046045052033
214214,428429,428428,856857,710.6217727661133,0.877664246585482
215215,430431,430430,860861,713.9312012195587,0.8740540786038764
216216,432433,432432,864865,717.3069670200348,0.8704737244624994
217217,434435,434434,868869,720.5840120315552,0.8669228143717191
218218,436437,436436,872873,723.8806071281433,0.8634009847173729
219219,438439,438438,876877,727.1975498199463,0.8599078779152478
220220,440441,440440,880881,730.4769208431244,0.8564431423092174
221221,442443,442442,884885,733.7769510746002,0.8530064320239035
222222,444445,444444,888889,737.0808839797974,0.849597406855537
223223,446447,446446,892893,740.3854911327362,0.8462157321482664
224224,448449,448448,896897,743.6926460266113,0.8428610786850186
225225,450451,450450,900901,746.9683649539948,0.8395331225656264
226226,452453,452452,904905,750.2578899860382,0.8362315451086033
227227,454455,454454,908909,753.6104731559753,0.8329560327347281
228228,456457,456456,912913,756.8961911201477,0.8297062768779142
229229,458459,458458,916917,760.1512269973755,0.8264819738633378
230230,460461,460460,920921,763.4508399963379,0.8232828248237638
231231,462463,462462,924925,766.7120530605316,0.8201085355995019
232232,464465,464464,928929,770.0832190513611,0.8169588166456379
233233,466467,466466,932933,773.5204660892487,0.813833382931989
234234,468469,468468,936937,776.954124212265,0.810731953864888
235235,470471,470470,940941,780.2987380027771,0.8076542531980522
236236,472473,472472,944945,783.59605884552,0.8046000089398149
237237,474475,474474,948949,786.8860719203949,0.8015689532767283
238238,476477,476476,952953,790.1826918125153,0.7985608224898897
239239,478479,478478,956957,793.4451529979706,0.795575356876725
240240,480481,480480,960961,796.8555150032043,0.7926123006782291
241241,482483,482482,964965,800.1606860160828,0.7896714019898354
242242,484485,484484,968969,803.4596259593964,0.7867524127013894
243243,486487,486486,972973,806.7077641487122,0.7838550884225697
244244,488489,488488,976977,810.0101981163025,0.7809791884028527
245245,490491,490490,980981,813.3696401119232,0.7781244754769432
246246,492493,492492,984985,816.6929080486298,0.7752907159938331
247247,494495,494494,988989,819.999959230423,0.7724776797349477
248248,496497,496496,992993,823.3164310455322,0.7696851398723084
249249,498499,498498,996997,826.6246738433838,0.766912872903049
250250,500501,500500,1001001,829.9313428401947,0.7641606585639238
251251,502503,502502,1005005,833.2326738834381,0.7614282798076601
252252,504505,504504,1009009,836.5013918876648,0.7587155227156472
253253,506507,506506,1013013,839.7979819774628,0.7560221764597372
254254,508509,508508,1017017,843.1445560455322,0.7533480332222098
255255,510511,510510,1021021,846.4197859764099,0.7506928881757631
256256,512513,512512,1025025,849.7902119159698,0.7480565393962024
257257,514515,514514,1029029,853.1425409317017,0.7454387878351554
258258,516517,516516,1033033,856.4272630214691,0.7428394372509501
259259,518519,518518,1037037,859.718887090683,0.7402582941722358
260260,520521,520520,1041041,862.9994320869446,0.7376951678379555
261261,522523,522522,1045045,866.2624289989471,0.7351498701555101
262262,524525,524524,1049049,869.5451219081879,0.7326222156552831
263263,526527,526526,1053053,872.8391489982605,0.7301120214397088
264264,528529,528528,1057057,876.137423992157,0.727619107139617
265265,530531,530530,1061061,879.3808100223541,0.7251432948760339
266266,532533,532532,1065065,882.6922309398651,0.7226844092056126
267267,534535,534534,1069069,885.9509038925171,0.7202422770878911
268268,536537,536536,1073073,889.239394903183,0.7178167278489127
269269,538539,538538,1077077,892.5410759449005,0.7154075931230182
270270,540541,540540,1081081,895.8130419254303,0.71301470682738
271271,542543,542542,1085085,899.1141121387482,0.7106379051183467
272272,544545,544544,1089089,902.3746058940887,0.7082770263587008
273273,546547,546546,1093093,905.6782448291779,0.7059319534273527
274274,548549,548548,1097097,908.8927597999573,0.7036024911103596
275275,550551,550550,1101101,912.1759219169617,0.7012884793366538
276276,552553,552552,1105105,915.4459409713745,0.698989764910948
277277,554555,554554,1109109,918.7596490383148,0.6967061966679466
278278,556557,556556,1113113,922.0627160072327,0.6944376254268718
279279,558559,558558,1117117,925.3326869010925,0.6921839039696351
280280,560561,560560,1121121,928.6086821556091,0.689944887004458
281281,562563,562562,1125125,931.9109210968018,0.6877204311258538
282282,564565,564564,1129129,935.2593381404877,0.685510394801895
283283,566567,566566,1133133,938.5244538784027,0.6833146383214626
284284,568569,568568,1137137,941.7877020835876,0.6811330237869697
285285,570571,570570,1141141,945.2825191020966,0.6789654150634306
286286,572573,572572,1145145,948.6165959835052,0.6768116777693649
287287,574575,574574,1149149,951.8775579929352,0.6746716792385996
288288,576577,576576,1153153,955.1650719642639,0.6725452884893457
289289,578579,578578,1157157,958.4299039840698,0.6704323762041895
290290,580581,580580,1161161,961.7261579036713,0.6683328147100838
291291,582583,582582,1165165,965.0805780887604,0.666246477927416
292292,584585,584584,1169169,968.4569721221924,0.6641732413772843
293293,586587,586586,1173173,971.8021199703217,0.6621129821323848
294294,588589,588588,1177177,975.073310136795,0.6600657826620591
295295,590591,590590,1181181,978.3883719444275,0.6580316018898884
296296,592593,592592,1185185,981.678230047226,0.6560100369242718
297297,594595,594594,1189189,985.0679979324341,0.6540009703348915
298298,596597,596596,1193193,988.3392310142517,0.6520042863485287
299299,598599,598598,1197197,991.5850510597229,0.650019870732649
300300,600601,600600,1201201,994.9405248165131,0.6480476107299182
301301,602603,602602,1205205,998.1988508701324,0.646087395010909
302302,604605,604604,1209209,1001.4539439678192,0.6441391136231687
303303,606607,606606,1213213,1004.7140440940857,0.642202657963935
304304,608609,608608,1217217,1008.1826639175415,0.640277920763765
305305,610611,610610,1221221,1011.5717670917511,0.6383647960501548
306306,612613,612612,1225225,1014.8374290466309,0.6364631791238935
307307,614615,614614,1229229,1018.1456201076508,0.6345732934460102
308308,616617,616616,1233233,1021.3960800170898,0.6326948488494963
309309,618619,618618,1237237,1024.7827038764954,0.6308276036452298
310310,620621,620620,1241241,1028.056895017624,0.6289714574322716
311311,622623,622622,1245245,1031.3908469676971,0.6271263113558234
312312,624625,624624,1249249,1034.8128311634064,0.6252920678944065
313313,626627,626626,1253253,1038.0985870361328,0.6234686307343509
314314,628629,628628,1257257,1041.3853709697723,0.6216559047243209
315315,630631,630630,1261261,1044.6636848449707,0.6198537958462111
316316,632633,632632,1265265,1047.97096991539,0.6180622111733101
317317,634635,634634,1269269,1051.261761188507,0.6162810588775756
318318,636637,636636,1273273,1054.6512248516083,0.6145102481896174
319319,638639,638638,1277277,1057.9627878665924,0.6127496893896023
320320,640641,640640,1281281,1061.2546899318695,0.6109992937981588
321321,642643,642642,1285285,1064.5492079257965,0.6092589737509115
322322,644645,644644,1289289,1068.1564371585846,0.6075286425930244
323323,646647,646646,1293293,1071.4963538646698,0.6058082146591914
324324,648649,648648,1297297,1074.7999169826508,0.604097605260904
325325,650651,650650,1301301,1078.077208995819,0.6023967306682607
326326,652653,652652,1305305,1081.3415229320526,0.6007055081099679
327327,654655,654654,1309309,1084.6526579856873,0.5990238557405974
328328,656657,656656,1313313,1087.9153008460999,0.5973516926442244
329329,658659,658658,1317317,1091.299950838089,0.5956889388107811
330330,660661,660660,1321321,1094.6236701011658,0.5940355151287804
331331,662663,662662,1325325,1097.9460439682007,0.592391343365307
332332,664665,664664,1329329,1101.2601389884949,0.5907563461696554
333333,666667,666666,1333333,1104.4982709884644,0.5891304577180563
334334,668669,668668,1337337,1107.7899050712585,0.5875135967944516
335335,670671,670670,1341341,1111.0678339004517,0.5859056835888623
336336,672673,672672,1345345,1114.3810420036316,0.5843066441011615
337337,674675,674674,1349349,1117.7056760787964,0.5827164051297586
338338,676677,676676,1353353,1121.0055360794067,0.5811348942879704
339339,678679,678678,1357357,1124.2931849956512,0.5795620399767358
340340,680681,680680,1361361,1127.589278936386,0.5779977713809785
341341,682683,682682,1365365,1130.899069070816,0.5764420184568735
342342,684685,684684,1369369,1134.1866598129272,0.5748947119136574
343343,686687,686686,1373373,1137.47021818161,0.5733557832172664
344344,688689,688688,1377377,1140.806035041809,0.5718251645776036
345345,690691,690690,1381381,1144.07732796669,0.5703027889194345
346346,692693,692692,1385385,1147.3843281269073,0.5687885899005778
347347,694695,694694,1389389,1150.6597950458527,0.5672825018846197
348348,696697,696696,1393393,1153.9313960075378,0.5657844599336386
349349,698699,698698,1397397,1157.1908929347992,0.5642943998045666
350350,700701,700700,1401401,1160.4759078025818,0.5628122579328192
351351,702703,702702,1405405,1163.7382860183716,0.5613379714286566
352352,704705,704704,1409409,1167.0201721191406,0.5598714780680893
353353,706707,706706,1413413,1170.2929830551147,0.5584127162765071
354354,708709,708708,1417417,1173.5695040225983,0.5569616251377738
355355,710711,710710,1421421,1176.8560650348663,0.5555181443560286
356356,712713,712712,1425425,1180.1523458957672,0.5540822142829711
357357,714715,714714,1429429,1183.4239571094513,0.5526537758833001
358358,716717,716716,1433433,1186.732558965683,0.551232770729257
359359,718719,718718,1437437,1190.1017169952393,0.5498191410133586
360360,720721,720720,1441441,1193.528963804245,0.5484128295156552
361361,722723,722722,1445445,1196.8889071941376,0.5470137796073686
362362,724725,724724,1449449,1200.2176887989044,0.5456219352417975
363363,726727,726726,1453453,1203.5243520736694,0.5442372409506788
364364,728729,728728,1457457,1206.7876241207123,0.5428596418296365
365365,730731,730730,1461461,1210.09667801857,0.5414890835345432
366366,732733,732732,1465465,1213.3304419517517,0.5401255122760631
367367,734735,734734,1469469,1216.6955709457397,0.5387688748141954
368368,736737,736736,1473473,1220.0235381126404,0.5374191184400843
369369,738739,738738,1477477,1223.2705161571503,0.5360761909814755
370370,740741,740740,1481481,1226.5366051197052,0.534740040793622
371371,742743,742742,1485485,1229.7918980121613,0.5334106167465507
372372,744745,744744,1489489,1233.0772738456726,0.5320878682268813
373373,746747,746746,1493493,1236.3449440002441,0.5307717451250937
374374,748749,748748,1497497,1239.6407718658447,0.5294621978318901
375375,750751,750750,1501501,1242.9194629192352,0.5281591772290994
376376,752753,752752,1505505,1246.2100429534912,0.5268626346878591
377377,754755,754754,1509509,1249.4997961521149,0.5255725220667955
378378,756757,756756,1513513,1252.7248888015747,0.5242887916883774
379379,758759,758758,1517517,1256.0234298706055,0.5230113963534677
380380,760761,760760,1521521,1259.2814719676971,0.5217402893213148
381381,762763,762762,1525525,1262.572590827942,0.5204754243131902
382382,764765,764764,1529529,1265.8325610160828,0.5192167555014748
383383,766767,766766,1533533,1269.1327900886536,0.5179642375023832
384384,768769,768768,1537537,1272.3999121189117,0.516717825379601
385385,770771,770770,1541541,1275.6531009674072,0.5154774746297335
386386,772773,772772,1545545,1278.9608981609344,0.5142431411786674
387387,774775,774774,1549549,1282.2128238677979,0.5130147813797521
388388,776777,776776,1553553,1285.4765529632568,0.5117923520083423
389389,778779,778778,1557557,1288.7756690979004,0.5105758102545224
390390,780781,780780,1561561,1292.063244819641,0.5093651137176494
391391,782783,782782,1565565,1295.376363992691,0.5081602203990769
392392,784785,784784,1569569,1298.6666851043701,0.5069610887112503
393393,786787,786786,1573573,1302.0223441123962,0.5057676774504216
394394,788789,788788,1577577,1305.2824411392212,0.5045799458166584
395395,790791,790790,1581581,1308.5956370830536,0.5033978533847403
396396,792793,792792,1585585,1312.1432027816772,0.5022213601205294
397397,794795,794794,1589589,1315.562399148941,0.5010504263591429
398398,796797,796796,1593593,1318.8288269042969,0.4998850128158665
399399,798799,798798,1597597,1322.1407370567322,0.498725080573422
400400,800801,800800,1601601,1325.4324760437012,0.49757059107651
401401,802803,802802,1605605,1328.7596571445465,0.49642150613181
402402,804805,804804,1609609,1332.0393459796906,0.4952777879025234
403403,806807,806806,1613613,1335.3689720630646,0.4941393988992786
404404,808809,808808,1617617,1338.7363669872284,0.4930063019874069
405405,810811,810810,1621621,1342.0315778255463,0.4918784603705717
406406,812813,812812,1625625,1345.3218939304352,0.4907558375962253
407407,814815,814814,1629629,1348.6033430099487,0.4896383975410572
408408,816817,816816,1633633,1351.925036907196,0.4885261044200888
409409,818819,818818,1637637,1355.258022069931,0.4874189227775787
410410,820821,820820,1641641,1358.5484399795532,0.48631681747428956
411411,822823,822822,1645645,1361.8691289424896,0.4852197536984022
412412,824825,824824,1649649,1365.2151560783386,0.48412769695278257
413413,826827,826826,1653653,1368.546136856079,0.4830406130586198
414414,828829,828828,1657657,1371.8271760940552,0.4819584681354172
415415,830831,830830,1661661,1375.181401014328,0.48088122862100136
416416,832833,832832,1665665,1378.472242116928,0.479808861249694
417417,834835,834834,1669669,1381.7680740356445,0.4787413330577692
418418,836837,836836,1673673,1385.1020901203156,0.4776786113779963
419419,838839,838838,1677677,1388.3906269073486,0.4766206638341828
420420,840841,840840,1681681,1391.713989019394,0.47556745833753666
421421,842843,842842,1685685,1395.0151591300964,0.47451896309576114
422422,844845,844844,1689689,1398.3271489143372,0.47347514658395085
423423,846847,846846,1693693,1401.6547889709473,0.4724359775718767
424424,848849,848848,1697697,1404.9349598884583,0.4714014250985201
425425,850851,850850,1701701,1408.2370898723602,0.4703714584775298
426426,852853,852852,1705705,1411.543184041977,0.46934604729540297
427427,854855,854854,1709709,1414.8309562206268,0.4683251614042092
428428,856857,856856,1713713,1418.1490278244019,0.4673087709215906
429429,858859,858858,1717717,1421.4646151065826,0.46629684623076173
430430,860861,860860,1721721,1424.7360458374023,0.4652893579641386
431431,862863,862862,1725725,1428.0370419025421,0.46428627702698577
432432,864865,864864,1729729,1431.3225870132446,0.4632875745592173
433433,866867,866866,1733733,1434.6039791107178,0.46229322196450084
434434,868869,868868,1737737,1437.8653810024261,0.4613031908884295
435435,870871,870870,1741741,1441.1679780483246,0.4603174532276171
436436,872873,872872,1745745,1444.4654200077057,0.45933598111514584
437437,874875,874874,1749749,1447.8399949073792,0.4583587469296617
438438,876877,876876,1753753,1451.26629114151,0.4573857232808223
439439,878879,878878,1757757,1454.6199398040771,0.4564168830165727
440440,880881,880880,1761761,1457.926020860672,0.4554521992231457
441441,882883,882882,1765765,1461.1980209350586,0.4544916452068719
442442,884885,884884,1769769,1464.4963040351868,0.4535351945069124
443443,886887,886886,1773773,1467.7922158241272,0.452582820886164
444444,888889,888888,1777777,1471.1071639060974,0.4516344983330782
445445,890891,890890,1781781,1474.50084400177,0.4506902010507474
446446,892893,892892,1785785,1477.8856449127197,0.4497499034659995
447447,894895,894894,1789789,1481.173982143402,0.4488135802166653
448448,896897,896896,1793793,1484.467406988144,0.44788120616249216
449449,898899,898898,1797797,1487.78151512146,0.44695275635785947
450450,900901,900900,1801801,1491.098820924759,0.4460282060827012
451451,902903,902902,1805805,1494.4893219470978,0.4451075308206782
452452,904905,904904,1809809,1497.9173610210419,0.44419070625190216
453453,906907,906906,1813813,1501.4753530025482,0.44327770826748747
454454,908909,908908,1817817,1504.7931969165802,0.4423685129513615
455455,910911,910910,1821821,1508.062628030777,0.4414630965929973
456456,912913,912912,1825825,1511.3499989509583,0.44056143567649997
457457,914915,914914,1829829,1514.6561870574951,0.4396635068751493
458458,916917,916916,1833833,1517.930615901947,0.4387692870623141
459459,918919,918918,1837837,1521.2129528522491,0.437878753293262
460460,920921,920920,1841841,1524.4604160785675,0.43699188282153045
461461,922923,922922,1845845,1527.8166921138763,0.43610865307528
462462,924925,924924,1849849,1531.0856959819794,0.435229041679122
463463,926927,926926,1853853,1534.3834850788116,0.4343530264304718
464464,928929,928928,1857857,1537.7184238433838,0.4334805853122816
465465,930931,930930,1861861,1540.975214958191,0.4326116964875837
466466,932933,932932,1865865,1544.286880016327,0.4317463382903952
467467,934935,934934,1869869,1547.577880859375,0.43088448924027034
468468,936937,936936,1873873,1550.8253769874573,0.43002612802047224
469469,938939,938938,1877877,1554.1496210098267,0.4291712334888871
470470,940941,940940,1881881,1557.4290339946747,0.428319784678024
471471,942943,942942,1885885,1560.7145297527313,0.4274717607822822
472472,944945,944944,1889889,1563.984990119934,0.42662714116522693
473473,946947,946946,1893893,1567.280506849289,0.4257859053577704
474474,948949,948948,1897897,1570.7772459983826,0.4249480330545339
475475,950951,950950,1901901,1574.1513969898224,0.4241135041029338
476476,952953,952952,1905905,1577.5807518959045,0.42328229852137156
477477,954955,954954,1909909,1581.0066499710083,0.42245439648468164
478478,956957,956956,1913913,1584.3785939216614,0.42162977831685566
479479,958959,958958,1917917,1587.6629450321198,0.4208084245055943
480480,960961,960960,1921921,1590.9512050151825,0.41999031569139333
481481,962963,962962,1925925,1594.253121137619,0.41917543266572466
482482,964965,964964,1929929,1597.581001996994,0.4183637563710363
483483,966967,966966,1933933,1600.8572480678558,0.4175552678952954
484484,968969,968968,1937937,1604.1759040355682,0.41674994848290225
485485,970971,970970,1941941,1607.5175938606262,0.4159477795165003
486486,972973,972972,1945945,1610.819407939911,0.4151487425297091
487487,974975,974974,1949949,1614.1022589206696,0.4143528191943915
488488,976977,976976,1953953,1617.4484858512878,0.4135599913333863
489489,978979,978978,1957957,1620.782742023468,0.41277024089686165
490490,980981,980980,1961961,1624.1220359802246,0.41198364838601265
491491,982983,982982,1965965,1627.4005279541016,0.4112001088888064
492492,984985,984984,1969969,1630.6570200920105,0.41041959323047195
493493,986987,986986,1973973,1633.9365730285645,0.40964208389414125
494494,988989,988988,1977977,1637.229609966278,0.4088675635175605
495495,990991,990990,1981981,1640.4990510940552,0.408096014871262
496496,992993,992992,1985985,1643.806482076645,0.4073274208640214
497497,994995,994994,1989989,1647.0738561153412,0.4065617645301245
498498,996997,996996,1993993,1650.3430018424988,0.4057990290421003
499499,998999,998998,1997997,1653.6238539218903,0.4050391976888932
500501,1001003,1001002,2002005,1656.970232963562,0.40428149914805545
501502,1003005,1003004,2006009,1660.2373991012573,0.40352742932554975
502503,1005007,1005006,2010013,1663.4718978404999,0.40277621426503174
503504,1007009,1007008,2014017,1666.8958489894867,0.4020278377665818
504505,1009011,1009010,2018021,1670.4100408554077,0.40128228374305763
505506,1011013,1011012,2022025,1673.728754043579,0.4005395362364652
506507,1013015,1013014,2026029,1677.0145909786224,0.3997995794034068
507508,1015017,1015016,2030033,1680.276673078537,0.39906239752235706
508509,1017019,1017018,2034037,1683.6103110313416,0.39832797498638683
509510,1019021,1019020,2038041,1686.8711009025574,0.3975962963049824
510511,1021023,1021022,2042045,1690.162439107895,0.39686734610586427
511512,1023025,1023024,2046049,1693.5087850093842,0.3961411091295304
512513,1025027,1025026,2050053,1696.8600101470947,0.39541757023107493
513514,1027029,1027028,2054057,1700.1370341777802,0.3946967143747315
514515,1029031,1029030,2058061,1703.4135100841522,0.3939785266375111
515516,1031033,1031032,2062065,1706.731833934784,0.3932629922073829
516517,1033035,1033034,2066069,1710.0031387805939,0.3925500963778177
517518,1035037,1035036,2070073,1713.2992079257965,0.3918398245550634
518519,1037039,1037038,2074077,1716.5879318714142,0.39113216225268843
519520,1039041,1039040,2078081,1719.8648209571838,0.3904270950843056
520521,1041043,1041042,2082085,1723.1468408107758,0.3897246087763051
521522,1043045,1043044,2086089,1726.4437971115112,0.38902468915148347
522523,1045047,1045046,2090093,1729.7412509918213,0.3883273221417767
523524,1047049,1047048,2094097,1732.9976468086243,0.3876324937791651
524525,1049051,1049050,2098101,1736.2815771102905,0.38694019020113046
525526,1051053,1051052,2102105,1739.5826539993286,0.386250397637923
526527,1053055,1053054,2106109,1742.8602890968323,0.38556310242529435
527528,1055057,1055056,2110113,1746.164234161377,0.3848782909954025
528529,1057059,1057058,2114117,1749.4030239582062,0.38419594987499295
529530,1059061,1059060,2118121,1752.7074120044708,0.3835160656963126
530531,1061063,1061062,2122125,1755.9678449630737,0.38283862518073875
531532,1063065,1063064,2126129,1759.2487378120422,0.38216361514605524
532533,1065067,1065066,2130133,1762.5306839942932,0.3814910225046333
533534,1067069,1067068,2134137,1765.778797864914,0.3808208342652506
534535,1069071,1069070,2138141,1769.0447881221771,0.38015303752217733
535536,1071073,1071072,2142145,1772.301841020584,0.3794876194697281
536537,1073075,1073074,2146149,1775.5975539684296,0.37882456738771
537538,1075077,1075076,2150153,1778.8684220314026,0.37816386864869855
538539,1077079,1077078,2154157,1782.165342092514,0.37750551071621885
539540,1079081,1079080,2158161,1785.4093539714813,0.3768494811356504
540541,1081083,1081082,2162165,1788.7299201488495,0.37619576754696027
541542,1083085,1083084,2166169,1792.0359539985657,0.3755443576756079
542543,1085087,1085086,2170173,1795.3011310100555,0.3748952393307263
543544,1087089,1087088,2174177,1798.6221981048584,0.37424840040876006
544545,1089091,1089090,2178181,1801.8823239803314,0.3736038288916461
545546,1091093,1091092,2182185,1805.315880060196,0.372961512844995
546547,1093095,1093094,2186189,1808.6755018234253,0.3723214404180908
547548,1095097,1095096,2190193,1811.939637184143,0.37168359984571
548549,1097099,1097098,2194197,1815.256551027298,0.3710479794317507
549550,1099101,1099100,2198201,1818.5206730365753,0.3704145675783366
550551,1101103,1101102,2202205,1821.832909822464,0.3697833527567127
551552,1103105,1103104,2206209,1825.2071161270142,0.3691543235217978
552553,1105107,1105106,2210213,1828.4535508155823,0.368527468510365
553554,1107109,1107108,2214217,1831.7700581550598,0.36790277643012814
554555,1109111,1109110,2218221,1835.102795124054,0.3672802360724745
555556,1111113,1111112,2222225,1838.3737711906433,0.36665983630700794
556557,1113115,1113114,2226229,1841.6521670818329,0.36604156607063487
557558,1115117,1115116,2230233,1844.9536101818085,0.36542541438939224
558559,1117119,1117118,2234237,1848.2653000354767,0.3648113703529816
559560,1119121,1119120,2238241,1851.7224099636078,0.36419942313295905
560561,1121123,1121122,2242245,1855.1653761863708,0.36358956197000225
561562,1123125,1123124,2246249,1858.4269080162048,0.36298177617936744
562563,1125127,1125126,2250253,1861.739557981491,0.3623760551454325
563564,1127129,1127128,2254257,1865.0956399440765,0.3617723883344297
564565,1129131,1129130,2258261,1868.4067521095276,0.36117076527625613
565566,1131133,1131132,2262265,1871.7554697990417,0.36057117557174934
566567,1133135,1133134,2266269,1875.0627768039703,0.35997360889450647
567568,1135137,1135136,2270273,1878.550908088684,0.3593780549854273
568569,1137139,1137138,2274277,1881.8516309261322,0.35878450365817116
569570,1139141,1139140,2278281,1885.1641600131989,0.35819294478642405
570571,1141143,1141142,2282285,1888.491447210312,0.3576033683257265
571572,1143145,1143144,2286289,1891.7264499664307,0.3570157642807317
572573,1145147,1145146,2290293,1895.077800989151,0.3564301227397664
573574,1147149,1147148,2294297,1898.3563060760498,0.355846433847546
574575,1149151,1149150,2298301,1901.6166081428528,0.35526468781790754
575576,1151153,1151152,2302305,1904.892233133316,0.35468487492653367
576577,1153155,1153154,2306309,1908.1709699630737,0.3541069855200476
577578,1155157,1155156,2310313,1911.5322089195251,0.35353101000146125
578579,1157159,1157158,2314317,1914.836716890335,0.35295693884108914
579580,1159161,1159160,2318321,1918.1146461963654,0.3523847625747294
580581,1161163,1161162,2322325,1921.4078710079193,0.35181447179093084
581582,1163165,1163164,2326329,1924.7044949531555,0.35124605715645885
582583,1165167,1165166,2330333,1928.006511926651,0.35067950938173453
583584,1167169,1167168,2334337,1931.2734589576721,0.35011481925357657
584585,1169171,1169170,2338341,1934.624027967453,0.3495519776024594
585586,1171173,1171172,2342345,1937.8694689273834,0.3489909753370739
586587,1173175,1173174,2346349,1941.1563091278076,0.34843180341158586
587588,1175177,1175176,2350353,1944.433249950409,0.34787445284564456
588589,1177179,1177178,2354357,1947.7365939617157,0.34731891471710696
589590,1179181,1179180,2358361,1950.9982089996338,0.34676518015658075
590591,1181183,1181182,2362365,1954.2984659671783,0.3462132403619762
591592,1183185,1183184,2366369,1957.6311709880829,0.3456630865784973
592593,1185187,1185186,2370373,1960.8885679244995,0.3451147101131937
593594,1187189,1187188,2374377,1964.1660299301147,0.34456810232950374
594595,1189191,1189190,2378381,1967.4036581516266,0.3440232546399784
595596,1191193,1191192,2382385,1970.795692205429,0.34348015852265235
596597,1193195,1193194,2386389,1974.2411751747131,0.34293880550285394
597598,1195197,1195196,2390393,1977.5241680145264,0.3423991871641192
598599,1197199,1197198,2394397,1980.7874729633331,0.3418612951390969
599600,1199201,1199200,2398401,1984.0923669338226,0.3413251211204624
600601,1201203,1201202,2402405,1987.3215928077698,0.34079065685182286
601602,1203205,1203204,2406409,1990.6322240829468,0.34025789412407903
602603,1205207,1205206,2410413,1993.9730219841003,0.33972682478452043
603604,1207209,1207208,2414417,1997.2353138923645,0.3391974407386442
604605,1209211,1209210,2418421,2000.5061919689178,0.33866973392832733
605606,1211213,1211212,2422425,2003.7420060634613,0.3381436963645683
606607,1213215,1213214,2426429,2007.0293459892273,0.3376193200892885
607608,1215217,1215216,2430433,2010.3082389831543,0.3370965972135309
608609,1217219,1217218,2434437,2013.6408910751343,0.33657551988471823
609610,1219221,1219220,2438441,2016.9168620109558,0.3360560803066619
610611,1221223,1221222,2442445,2020.181156873703,0.33553827072864806
611612,1223225,1223224,2446449,2023.4669630527496,0.33502208345089457
612613,1225227,1225226,2450453,2026.7258250713348,0.334507510819094
613614,1227229,1227228,2454457,2030.0121281147003,0.3339945452316897
614615,1229231,1229230,2458461,2033.2877221107483,0.33348317912714265
615616,1231233,1231232,2462465,2036.544970035553,0.3329734050003026
616617,1233235,1233234,2466469,2039.7966830730438,0.332465215386037
617618,1235237,1235236,2470473,2043.0928900241852,0.33195860286650714
618619,1237239,1237238,2474477,2046.3745670318604,0.3314535600729869
619620,1239241,1239240,2478481,2049.627187013626,0.3309500796785869
620621,1241243,1241242,2482485,2052.8880331516266,0.33044815440371167
621622,1243245,1243244,2486489,2056.1825659275055,0.32994777701787825
622623,1245247,1245246,2490493,2059.4481320381165,0.3294489403251646
623624,1247249,1247248,2494497,2062.7127480506897,0.32895163718421827
624625,1249251,1249250,2498501,2065.984852075577,0.3284558604900667
625626,1251253,1251252,2502505,2069.26845908165,0.32796160318684997
626627,1253255,1253254,2506509,2072.5665209293365,0.32746885825690697
627628,1255257,1255256,2510513,2075.8380270004272,0.3269776187335083
628629,1257259,1257258,2514517,2079.0971081256866,0.3264878776844853
629630,1259261,1259260,2518521,2082.3690991401672,0.3259996282249631
630631,1261263,1261262,2522525,2085.628154039383,0.3255128635064466
631632,1263265,1263264,2526529,2088.8884329795837,0.32502757672409643
632633,1265267,1265266,2530533,2092.1679549217224,0.32454376112582395
633634,1267269,1267268,2534537,2095.4226450920105,0.32406140997954935
634635,1269271,1269270,2538541,2098.7055299282074,0.3235805166168575
635636,1271273,1271272,2542545,2101.9123759269714,0.3231010743857041
636637,1273275,1273274,2546549,2105.2184870243073,0.32262307669589063
637638,1275277,1275276,2550553,2108.447530031204,0.32214651698450325
638639,1277279,1277278,2554557,2111.986167192459,0.32167138873046497
639640,1279281,1279280,2558561,2115.4592010974884,0.32119768545453553
640641,1281283,1281282,2562565,2118.6824321746826,0.32072540071749245
641642,1283285,1283284,2566569,2121.9435851573944,0.32025452810921706
642643,1285287,1285286,2570573,2125.2157049179077,0.31978506126870343
643644,1287289,1287288,2574577,2128.5158360004425,0.3193169938695064
644645,1289291,1289290,2578581,2131.7717509269714,0.31885031962156063
645646,1291293,1291292,2582585,2135.050948858261,0.3183850322729995
646647,1293295,1293294,2586589,2138.4400510787964,0.31792112561379327
647648,1295297,1295296,2590593,2141.724233150482,0.3174585934593779
648649,1297299,1297298,2594597,2145.0112500190735,0.3169974296761211
649650,1299301,1299300,2598601,2148.3021631240845,0.3165376281558565
650651,1301303,1301302,2602605,2151.5755620002747,0.31607918282861647
651652,1303305,1303304,2606609,2154.846652984619,0.3156220876680891
652653,1305307,1305306,2610613,2158.079924106598,0.3151663366734283
653654,1307309,1307308,2614617,2161.419888973236,0.3147119238819869
654655,1309311,1309310,2618621,2164.700478076935,0.3142588433711353
655656,1311313,1311312,2622625,2167.9830269813538,0.3138070892491669
656657,1313315,1313314,2626629,2171.2604508399963,0.3133566556571168
657658,1315317,1315316,2630633,2174.523545026779,0.3129075367742189
658659,1317319,1317318,2634637,2177.7969160079956,0.3124597268142679
659660,1319321,1319320,2638641,2181.0273830890656,0.31201322001652443
660661,1321323,1321322,2642645,2184.30274105072,0.3115680106657237
661662,1323325,1323324,2646649,2187.52970290184,0.3111240930720669
662663,1325327,1325326,2650653,2190.8254721164703,0.31068146158213494
663664,1327329,1327328,2654657,2194.10595703125,0.3102401105734316
664665,1329331,1329330,2658661,2197.3752360343933,0.3098000344562024
665666,1331333,1331332,2662665,2200.6729130744934,0.30936122767707275
666667,1333335,1333334,2666669,2203.949064016342,0.3089236847099528
667668,1335337,1335336,2670673,2207.2597880363464,0.3084874000578566
668669,1337339,1337338,2674677,2210.5166800022125,0.30805236826745386
669670,1339341,1339340,2678681,2213.8000688552856,0.3076185839054233
670671,1341343,1341342,2682685,2217.1622920036316,0.30718604157300433
671672,1343345,1343344,2686689,2220.5594120025635,0.30675473590417823
672673,1345347,1345346,2690693,2223.8801729679108,0.3063246615638491
673674,1347349,1347348,2694697,2227.1791911125183,0.3058958132423868
674675,1349351,1349350,2698701,2230.7408521175385,0.3054681856701791
675676,1351353,1351352,2702705,2234.091798067093,0.3050417735976225
676677,1353355,1353354,2706709,2237.340656042099,0.3046165718133125
677678,1355357,1355356,2710713,2240.6020390987396,0.30419257512767217
678679,1357359,1357358,2714717,2243.842849969864,0.30376977838568564
679680,1359361,1359360,2718721,2247.107396841049,0.30334817646325973
680681,1361363,1361362,2722725,2250.401249885559,0.30292776425994816
681682,1363365,1363364,2726729,2253.9253420829773,0.30250853670622746
682683,1365367,1365366,2730733,2257.397234916687,0.302090488763497
683684,1367369,1367368,2734737,2260.6762640476227,0.3016736154222599
684685,1369371,1369370,2738741,2263.9469311237335,0.3012579116948473
685686,1371373,1371372,2742745,2267.215760946274,0.30084337263178895
686687,1373375,1373374,2746749,2270.5279891490936,0.30042999330180464
687688,1375377,1375376,2750753,2273.9872760772705,0.3000177688045369
688689,1377379,1377378,2754757,2277.350861787796,0.2996066942669131
689690,1379381,1379380,2758761,2280.6216430664062,0.29919676485042146
690691,1381383,1381382,2762765,2283.932062149048,0.29878797573110205
691692,1383385,1383384,2766769,2287.253452062607,0.29838032212319376
692693,1385387,1385386,2770773,2290.5718290805817,0.2979737992554874
693694,1387389,1387388,2774777,2293.8365919589996,0.29756840299160103
694695,1389391,1389390,2778781,2297.219447851181,0.29716412939160364
695696,1391393,1391392,2782785,2300.464823961258,0.2967609726747469
696697,1393395,1393394,2786789,2303.7656950950623,0.29635892798432906
697698,1395397,1395396,2790793,2307.010807991028,0.29595799063645245
698699,1397399,1397398,2794797,2310.314491033554,0.295558156007246
699700,1399401,1399400,2798801,2313.660129070282,0.29515941950558044
700701,1401403,1401402,2802805,2316.944627046585,0.29476177657488734
701702,1403405,1403404,2806809,2320.2303869724274,0.2943652226767881
702703,1405407,1405406,2810813,2323.5191571712494,0.293969753305646
703704,1407409,1407408,2814817,2326.818810939789,0.2935753639831091
704705,1409411,1409410,2818821,2330.1714367866516,0.29318205024719646
705706,1411413,1411412,2822825,2333.5005888938904,0.2927898076650308
706707,1413415,1413414,2826829,2336.7860198020935,0.2923986318310199
707708,1415417,1415416,2830833,2340.057065010071,0.2920085183595802
708709,1417419,1417418,2834837,2343.338068008423,0.29161946288877516
709710,1419421,1419420,2838841,2346.610072851181,0.291231461085772
710711,1421423,1421422,2842845,2349.8764889240265,0.29084450863228994
711712,1423425,1423424,2846849,2353.154340028763,0.2904586012427899
712713,1425427,1425426,2850853,2356.4235711097717,0.2900737346517417
713714,1427429,1427428,2854857,2359.69206905365,0.2896899046118051
714715,1429431,1429430,2858861,2362.9416449069977,0.2893071069065627
715716,1431433,1431432,2862865,2366.233868122101,0.2889253373396059
716717,1433435,1433434,2866869,2369.505882024765,0.2885445917308971
717718,1435437,1435436,2870873,2373.061560869217,0.2881648659331404
718719,1437439,1437438,2874877,2376.457388162613,0.2877861558172299
719720,1439441,1439440,2878881,2379.7345130443573,0.2874084572758875
720721,1441443,1441442,2882885,2383.021094083786,0.287031766221844
721722,1443445,1443444,2886889,2386.4217879772186,0.2866560785932961
722723,1445447,1445446,2890893,2389.734097957611,0.28628139034663036
723724,1447449,1447448,2894897,2393.0426268577576,0.28590769746369915
724725,1449451,1449450,2898901,2396.4944038391113,0.2855349959445448
725726,1451453,1451452,2902905,2399.7927329540253,0.28516328181467543
726727,1453455,1453454,2906909,2403.088795900345,0.2847925511159701
727728,1455457,1455456,2910913,2406.2962651252747,0.2844227999157738
728729,1457459,1457458,2914917,2409.4754781723022,0.28405402429962123
729730,1459461,1459460,2918921,2412.6737570762634,0.2836862203748751
730731,1461463,1461462,2922925,2415.907392024994,0.283319384267088
731732,1463465,1463464,2926929,2419.1125090122223,0.2829535121272784
732733,1465467,1465466,2930933,2422.3320169448853,0.2825886001246545
733734,1467469,1467468,2934937,2425.5419311523438,0.28222464444479556
734735,1469471,1469470,2938941,2428.802092075348,0.2818616412969277
735736,1471473,1471472,2942945,2431.9710059165955,0.28149958691392385
736737,1473475,1473474,2946949,2435.219055891037,0.2811384775395709
737738,1475477,1475476,2950953,2438.8001589775085,0.2807783094467595
738739,1477479,1477478,2954957,2442.5116250514984,0.2804190789211134
739740,1479481,1479480,2958961,2445.8218429088593,0.280060782273722
740741,1481483,1481482,2962965,2449.1774921417236,0.27970341582658875
741742,1483485,1483484,2966969,2452.7440049648285,0.27934697592900193
742743,1485487,1485486,2970973,2456.315383911133,0.2789914589448017
743744,1487489,1487488,2974977,2459.6964869499207,0.2786368612632941
744745,1489491,1489490,2978981,2462.985577106476,0.2782831792792422
745746,1491493,1491492,2982985,2466.3845789432526,0.27793040942196967
746747,1493495,1493494,2986989,2469.7966301441193,0.2775785481262574
747748,1495497,1495496,2990993,2473.243639230728,0.2772275918559899
748749,1497499,1497498,2994997,2476.7831530570984,0.27687753708596574
749750,1499501,1499500,2999001,2480.2710201740265,0.27652838031099236
750751,1501503,1501502,3003005,2483.717260122299,0.27618011804770504
751752,1503505,1503504,3007009,2487.124382019043,0.275832746825472
752753,1505507,1505506,3011013,2490.4684171676636,0.2754862631936703
753754,1507509,1507508,3015017,2493.9391651153564,0.275140663721686
754755,1509511,1509510,3019021,2497.405412912369,0.27479594499163795
755756,1511513,1511512,3023025,2500.862226963043,0.27445210360929195
756757,1513515,1513514,3027029,2504.3584349155426,0.2741091361949657
757758,1515517,1515516,3031033,2507.7956659793854,0.27376703938534774
758759,1517519,1517518,3035037,2511.160124063492,0.2734258098334976
759760,1519521,1519520,3039041,2514.617882013321,0.2730854442124837
760761,1521523,1521522,3043045,2518.031502008438,0.2727459392099263
761762,1523525,1523524,3047049,2521.4637389183044,0.27240729153345455
762763,1525527,1525526,3051053,2524.894127845764,0.2720694979052496
763764,1527529,1527528,3055057,2528.3734369277954,0.2717325550656824
764765,1529531,1529530,3059061,2531.881576061249,0.2713964597642189
765766,1531533,1531532,3063065,2535.3336839675903,0.27106120878124784
766767,1533535,1533534,3067069,2538.7821300029755,0.270726798900796
767768,1535537,1535536,3071073,2542.224748849869,0.2703932269287179
768769,1537539,1537538,3075077,2545.6595549583435,0.2700604896836012
769770,1539541,1539540,3079081,2549.073093891144,0.2697285840076802
770771,1541543,1541542,3083085,2552.5134239196777,0.26939750675046525
771772,1543545,1543544,3087089,2556.126156806946,0.26906725478147564
772773,1545547,1545546,3091093,2559.6398758888245,0.2687378249847825
773774,1547549,1547548,3095097,2563.0575590133667,0.26840921426446585
774775,1549551,1549550,3099101,2566.514638900757,0.2680814195318817
775776,1551553,1551552,3103105,2569.9122610092163,0.2677544377202139
776777,1553555,1553554,3107109,2573.353273868561,0.26742826577537926
777778,1555557,1555556,3111113,2576.7634150981903,0.26710290065966547
778779,1557559,1557558,3115117,2580.1852581501007,0.2667783393535501
779780,1559561,1559560,3119121,2583.6028230190277,0.26645457884296775
780781,1561563,1561562,3123125,2586.9680919647217,0.2661316161429568
781782,1563565,1563564,3127129,2590.3084077835083,0.26580944826855557
782783,1565567,1565566,3131133,2593.697254896164,0.26548807226208737
783784,1567569,1567568,3135137,2597.12259888649,0.2651674851713324
784785,1569571,1569570,3139141,2600.5763380527496,0.26484768406589865
785786,1571573,1571572,3143145,2604.0331978797913,0.2645286660244892
786787,1573575,1573574,3147149,2607.459276199341,0.264210428142178
787788,1575577,1575576,3151153,2610.876424074173,0.2638929675304098
788789,1577579,1577578,3155157,2614.3600730895996,0.2635762813133624
789790,1579581,1579580,3159161,2617.8066890239716,0.2632603666279465
790791,1581583,1581582,3163165,2621.2701358795166,0.26294522062562464
791792,1583585,1583584,3167169,2624.726408958435,0.26263084047604934
792793,1585587,1585586,3171173,2628.1672310829163,0.26231722335614904
793794,1587589,1587588,3175177,2631.624083995819,0.2620043664592231
794795,1589591,1589590,3179181,2635.0928070545197,0.26169226699676074
795796,1591593,1591592,3183185,2638.5184211730957,0.26138092219116515
796797,1593595,1593594,3187189,2641.9872200489044,0.2610703292702965
797798,1595597,1595596,3191193,2645.440707921982,0.26076048548929975
798799,1597599,1597598,3195197,2648.956475019455,0.2604513881069579
799800,1599601,1599600,3199201,2652.525983095169,0.26014303440206277
800801,1601603,1601602,3203205,2656.038185119629,0.2598354216588632
801802,1603605,1603604,3207209,2659.4779291152954,0.2595285471834359
802803,1605607,1605606,3211213,2662.9558658599854,0.2592224082854955
803804,1607609,1607608,3215217,2666.4823150634766,0.25891700229658454
804805,1609611,1609610,3219221,2669.957128047943,0.25861232655734057
805806,1611613,1611612,3223225,2673.5765368938446,0.25830837842113397
806807,1613615,1613614,3227229,2677.0332429409027,0.2580051552540681
807808,1615617,1615616,3231233,2680.4905030727386,0.2577026544349792
808809,1617619,1617618,3235237,2683.947464942932,0.2574008733572555
809810,1619621,1619620,3239241,2687.3736641407013,0.25709980942519906
810811,1621623,1621622,3243245,2690.8136038780212,0.256799460055845
811812,1623625,1623624,3247249,2694.2427458763123,0.25649982267532323
812813,1625627,1625626,3251253,2697.6971690654755,0.2562008947297727
813814,1627629,1627628,3255257,2701.131061077118,0.25590267366897024
814815,1629631,1629630,3259261,2704.549940109253,0.2556051569627016
815816,1631633,1631632,3263265,2708.065313100815,0.25530834208620945
816817,1633635,1633634,3267269,2711.4464950561523,0.25501222653110744
817818,1635637,1635636,3271273,2714.924288034439,0.2547168077999231
818819,1637639,1637638,3275277,2718.377935886383,0.25442208340791694
819820,1639641,1639640,3279281,2721.7951471805573,0.25412805087762536
820821,1641643,1641642,3283285,2725.221936941147,0.2538347077497747
821822,1643645,1643644,3287289,2728.584846019745,0.2535420515760052
822823,1645647,1645646,3291293,2732.1771750450134,0.2532500799097761
823824,1647649,1647648,3295297,2736.7276759147644,0.25295879033001256
824825,1649651,1649650,3299301,2740.8574678897858,0.25266818041745864
825826,1651653,1651652,3303305,2744.41517496109,0.2523782477728673
826827,1653655,1653654,3307309,2747.7884590625763,0.2520889899988106
827828,1655657,1655656,3311313,2751.6885759830475,0.2518004047124123
828829,1657659,1657658,3315317,2755.1227390766144,0.2515124895471672
829830,1659661,1659660,3319321,2758.7074661254883,0.25122524213838915
830831,1661663,1661662,3323325,2762.0647189617157,0.25093866014321975
831832,1663665,1663664,3327329,2765.345705986023,0.25065274121880066
832833,1665667,1665666,3331333,2768.7592520713806,0.2503674830441014
833834,1667669,1667668,3335337,2772.048662185669,0.25008288330172945
834835,1669671,1669670,3339341,2775.2867469787598,0.24979893968520628
835836,1671673,1671672,3343345,2778.4956040382385,0.24951564990078623
836837,1673675,1673674,3347349,2781.6973400115967,0.24923301166927558
837838,1675677,1675676,3351353,2784.895306110382,0.2489510227151186
838839,1677679,1677678,3355357,2788.5442152023315,0.24866968077913043
839840,1679681,1679680,3359361,2791.7896630764008,0.24838898360212625
840841,1681683,1681682,3363365,2795.051162004471,0.24810892895038705
841842,1683685,1683684,3367369,2798.5029530525208,0.24782951459383185
842843,1685687,1685686,3371373,2801.9423592090607,0.2475507383060176
843844,1687689,1687688,3375377,2805.277256965637,0.24727259788414813
844845,1689691,1689690,3379381,2808.5828869342804,0.24699509112542728
845846,1691693,1691692,3383385,2811.9412710666656,0.24671821583797282
846847,1693695,1693694,3387389,2815.304136991501,0.2464419698480924
847848,1695697,1695696,3391393,2818.6467900276184,0.24616635097845574
848849,1697699,1697698,3395397,2821.9730298519135,0.24589135707901733
849850,1699701,1699700,3399401,2825.3482599258423,0.24561698599063675
850851,1701703,1701702,3403405,2828.7054789066315,0.24534323557963944
851852,1703705,1703704,3407409,2832.0701670646667,0.2450701037178078
852853,1705707,1705706,3411413,2835.4206280708313,0.2447975882787432
853854,1707709,1707708,3415417,2838.7724220752716,0.24452568715969392
854855,1709711,1709710,3419421,2842.1449270248413,0.2442543982542702
855856,1711713,1711712,3423425,2845.5071029663086,0.24398371947427222
856857,1713715,1713714,3427429,2848.867033958435,0.24371364873513812
857858,1715717,1715716,3431433,2852.255541086197,0.24344418397049594
858859,1717719,1717718,3435437,2855.636610031128,0.24317532311215473
859860,1719721,1719720,3439441,2859.119554042816,0.24290706410829443
860861,1721723,1721722,3443445,2862.518436908722,0.24263940491800895
861862,1723725,1723724,3447449,2865.9016761779785,0.24237234350221115
862863,1725727,1725726,3451453,2869.3265209198,0.24210587783818482
863864,1727729,1727728,3455457,2872.7009041309357,0.2418400059123087
864865,1729731,1729730,3459461,2876.109340906143,0.2415747257109615
865866,1731733,1731732,3463465,2879.472095012665,0.24131003524053085
866867,1733735,1733734,3467469,2882.8737511634827,0.24104593251286133
867868,1735737,1735736,3471473,2886.2600989341736,0.24078241554525448
868869,1737739,1737738,3475477,2889.6218869686127,0.24051948236774479
869870,1739741,1739740,3479481,2893.1398050785065,0.24025713101946167
870871,1741743,1741742,3483485,2896.6309971809387,0.23999535954317253
871872,1743745,1743744,3487489,2899.9751360416412,0.23973416599619668
872873,1745747,1745746,3491493,2903.351081132889,0.23947354844676738
873874,1747749,1747748,3495497,2906.7461519241333,0.2392135049612989
874875,1749751,1749750,3499501,2910.0903520584106,0.23895403362439538
875876,1751753,1751752,3503505,2913.514666080475,0.23869513252429897
876877,1753755,1753754,3507509,2916.870234966278,0.23843679976198473
877878,1755757,1755756,3511513,2920.2173278331757,0.2381790334420657
878879,1757759,1757758,3515517,2923.5965299606323,0.23792183168188785
879880,1759761,1759760,3519521,2926.970386981964,0.23766519260061614
880881,1761763,1761762,3523525,2930.492058992386,0.2374091143356054
881882,1763765,1763764,3527529,2934.0336468219757,0.2371535950260295
882883,1765767,1765766,3531533,2937.4193308353424,0.2368986328219762
883884,1767769,1767768,3535537,2940.776755094528,0.23664422587535228
884885,1769771,1769770,3539541,2944.1778151988983,0.23639037235443539
885886,1771773,1771772,3543545,2947.512226819992,0.23613707043114118
886887,1773775,1773774,3547549,2950.9002890586853,0.23588431828829926
887888,1775777,1775776,3551553,2954.248444080353,0.23563211411783413
888889,1777779,1777778,3555557,2957.7537689208984,0.23538045610803238
889890,1779781,1779780,3559561,2961.2255828380585,0.23512934247264639
890891,1781783,1781782,3563565,2964.601397037506,0.2348787714181526
891892,1783785,1783784,3567569,2967.9865159988403,0.2346287411692174
892893,1785787,1785786,3571573,2971.366229057312,0.23437924995596404
893894,1787789,1787788,3575577,2974.763421058655,0.23413029601215385
894895,1789791,1789790,3579581,2978.139976978302,0.23388187758246204
895896,1791793,1791792,3583585,2981.473958969116,0.2336339929188398
896897,1793795,1793794,3587589,2984.867394924164,0.23338664027869527
897898,1795797,1795796,3591593,2988.3475658893585,0.23313981793216954
898899,1797799,1797798,3595597,2991.8769450187683,0.23289352415304165
899900,1799801,1799800,3599601,2995.272336959839,0.23264775722236664
900901,1801803,1801802,3603605,2998.6482660770416,0.23240251543211343
901902,1803805,1803804,3607609,3002.029134988785,0.23215779707606998
902903,1805807,1805806,3611613,3005.4292809963226,0.23191360046075715
903904,1807809,1807808,3615617,3008.8109929561615,0.2316699238945148
904905,1809811,1809810,3619621,3012.179976940155,0.23142676570023468
905906,1811813,1811812,3623625,3015.545902967453,0.23118412420444656
906907,1813815,1813814,3627629,3018.9031801223755,0.23094199774095614
907908,1815817,1815816,3631633,3022.3222150802612,0.2307003846453881
908909,1817819,1817818,3635637,3025.6988549232483,0.23045928327155707
909910,1819821,1819820,3639641,3029.052722930908,0.2302186919732776
910911,1821823,1821822,3643645,3032.4138708114624,0.22997860910982126
911912,1823825,1823824,3647649,3035.808445930481,0.22973903305319254
912913,1825827,1825826,3651653,3039.1714210510254,0.2294999621790339
913914,1827829,1827828,3655657,3042.771243095398,0.22926139487026376
914915,1829831,1829830,3659661,3046.2581839561462,0.2290233295134385
915916,1831833,1831832,3663665,3049.595854997635,0.22878576451148547
916917,1833835,1833834,3667669,3053.0297989845276,0.22854869826369395
917918,1835837,1835836,3671673,3056.4009160995483,0.2283121291857242
918919,1837839,1837838,3675677,3059.768310070038,0.22807605568777944
919920,1839841,1839840,3679681,3063.2395548820496,0.22784047620007186
920921,1841843,1841842,3683685,3066.646488904953,0.2276053891509946
921922,1843845,1843844,3687689,3070.0205330848694,0.22737079297621676
922923,1845847,1845846,3691693,3073.3919591903687,0.22713668612595939
923924,1847849,1847848,3695697,3076.7440769672394,0.22690306704680552
924925,1849851,1849850,3699701,3080.0957651138306,0.22666993419261416
925926,1851853,1851852,3703705,3083.452296972275,0.22643728603179625
926927,1853855,1853854,3707709,3086.8584809303284,0.22620512103821966
927928,1855857,1855856,3711713,3090.2506980895996,0.22597343768029532
928929,1857859,1857858,3715717,3093.6555531024933,0.22574223444644304
929930,1859861,1859860,3719721,3097.0327620506287,0.2255115098250826
930931,1861863,1861862,3723725,3100.6893751621246,0.2252812623155478
931932,1863865,1863864,3727729,3104.227262020111,0.22505149041535333
932933,1865867,1865866,3731733,3107.5995841026306,0.2248221926329279
933934,1867869,1867868,3735737,3110.9644770622253,0.22459336748761416
934935,1869871,1869870,3739741,3114.346028804779,0.22436501349693572
935936,1871873,1871872,3743745,3117.7614319324493,0.22413712918933015
936937,1873875,1873874,3747749,3121.141902923584,0.223909713100511
937938,1875877,1875876,3751753,3124.5246200561523,0.22368276376801077
938939,1877879,1877878,3755757,3127.977847099304,0.22345627973663795
939940,1879881,1879880,3759761,3131.485990047455,0.22323025956029596
940941,1881883,1881882,3763765,3134.9101469516754,0.2230047017965262
941942,1883885,1883884,3767769,3138.3042390346527,0.22277960500650806
942943,1885887,1885886,3771773,3141.6707680225372,0.22255496776233485
943944,1887889,1887888,3775777,3145.044795036316,0.22233078864155686
944945,1889891,1889890,3779781,3148.501277923584,0.22210706622172438
945946,1891893,1891892,3783785,3151.832813978195,0.2218837990967586
946947,1893895,1893894,3787789,3155.31289601326,0.22166098585148575
947948,1895897,1895896,3791793,3158.715129852295,0.22143862509255996
948949,1897899,1897898,3795797,3162.088783979416,0.22121671542117838
949950,1899901,1899900,3799801,3165.473489046097,0.2209952554494521
950951,1901903,1901902,3803805,3168.9777669906616,0.22077424379494914
951952,1903905,1903904,3807809,3172.542151927948,0.22055367907705659
952953,1905907,1905906,3811813,3176.104173898697,0.22033355992789438
953954,1907909,1907908,3815817,3179.6442019939423,0.22011388497594453
954955,1909911,1909910,3819821,3183.250837087631,0.21989465286605991
955956,1911913,1911912,3823825,3186.7790229320526,0.21967586223763647
956957,1913915,1913914,3827829,3190.3302841186523,0.21945751174280304
957958,1915917,1915916,3831833,3193.863079071045,0.21923960004096443
958959,1917919,1917918,3835837,3197.4199628829956,0.21902212578970648
959960,1919921,1919920,3839841,3200.9888610839844,0.21880508765570994
960961,1921923,1921922,3843845,3204.533315896988,0.21858848431475053
961962,1923925,1923924,3847849,3208.165143966675,0.21837231444078498
962963,1925927,1925926,3851853,3211.708139181137,0.21815657672050293
963964,1927929,1927928,3855857,3215.2688710689545,0.21794126983513706
964965,1929931,1929930,3859861,3218.8349800109863,0.21772639248774794
965966,1931933,1931932,3863865,3222.3853969573975,0.21751194337412016
966967,1933935,1933934,3867869,3225.9300780296326,0.21729792119913327
967968,1935937,1935936,3871873,3229.4806611537933,0.2170843246676668
968969,1937939,1937938,3875877,3233.045751094818,0.21687115249915223
969970,1939941,1939940,3879881,3236.439852952957,0.216658403413021
970971,1941943,1941942,3883885,3239.8045399188995,0.21644607613598055
971972,1943945,1943944,3887889,3243.2018010616302,0.21623416939473827
972973,1945947,1945946,3891893,3246.59277009964,0.21602268193055352
973974,1947949,1947948,3895897,3249.9691169261932,0.21581161247740965
974975,1949951,1949950,3899901,3253.536642074585,0.21560095978202298
975976,1951953,1951952,3903905,3256.990730047226,0.21539072260384273
976977,1953955,1953954,3907909,3260.379774093628,0.21518089968776621
977978,1955957,1955956,3911913,3263.7804901599884,0.21497148979869962
978979,1957959,1957958,3915917,3267.1444220542908,0.21476249170518713
979980,1959961,1959960,3919921,3270.515394926071,0.2145539041757729
980981,1961963,1961962,3923925,3273.907637119293,0.21434572598263912
981982,1963965,1963964,3927929,3277.34232711792,0.21413795590888185
982983,1965967,1965966,3931933,3280.800950050354,0.21393059274487314
983984,1967969,1967968,3935937,3284.2156660556793,0.21372363527552807
984985,1969971,1969970,3939941,3287.600070953369,0.21351708229667565
985986,1971973,1971972,3943945,3290.9870748519897,0.2133109326077829
986987,1973975,1973974,3947949,3294.3648970127106,0.21310518501377373
987988,1975977,1975976,3951953,3297.7394251823425,0.21289983832502912
988989,1977979,1977978,3955957,3301.141799926758,0.21269489135556796
989990,1979981,1979980,3959961,3304.541310071945,0.21249034292304714
990991,1981983,1981982,3963965,3307.910754919052,0.2122861918505805
991992,1983985,1983984,3967969,3311.268275976181,0.21208243697219586
992993,1985987,1985986,3971973,3314.645651102066,0.21187907711282605
993994,1987989,1987988,3975977,3318.026892900467,0.21167611111377482
994995,1989991,1989990,3979981,3321.392380952835,0.21147353781634592
995996,1991993,1991992,3983985,3324.764140844345,0.21127135606730008
996997,1993995,1993994,3987989,3328.1265869140625,0.21106956471885496
997998,1995997,1995996,3991993,3331.6670711040497,0.21086816262504726
998999,1997999,1997998,3995997,3335.1974658966064,0.2106671486471896
1000000,2000001,2000000,4000001,3338.5692281723022,0.2104665216502326


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002852916717529297,12064.682476916567
775,1551,775,2326,2.745640993118286,1.7677786603617278
1550,3101,1550,4651,5.344280242919922,0.4014025325795956
2324,4649,2324,6973,7.957818031311035,0.1667746777930006
3099,6199,3099,9298,10.606822967529297,0.09114737647360016
3874,7749,3874,11623,13.439836025238037,0.056166856207710225
4649,9299,4649,13948,16.61601996421814,0.038495066579343984
5423,10847,5423,16270,19.813029050827026,0.02792227615827869
6198,12397,6198,18595,22.94659113883972,0.021325745914509753
6973,13947,6973,20920,25.835829973220825,0.016638080285702017
7748,15497,7748,23245,28.67917227745056,0.013368418583922903
8522,17045,8522,25567,31.304814100265503,0.010898089672991773
9297,18595,9297,27892,33.93050503730774,0.009102592601266224
10072,20145,10072,30217,36.53684210777283,0.007663005782887922
10847,21695,10847,32542,39.180908203125,0.006520347500554635
11621,23243,11621,34864,41.821572065353394,0.005626610769468243
12396,24793,12396,37189,44.44194006919861,0.004873611356742913
13171,26343,13171,39514,47.07123517990112,0.004269268079951871
13946,27893,13946,41839,49.74748921394348,0.003744532736163819
14721,29443,14721,44164,52.383578300476074,0.0033283825341641204
15495,30991,15495,46486,55.01123309135437,0.002958919632874313
16270,32541,16270,48811,57.63287925720215,0.002667349132025265
17045,34091,17045,51136,60.283698081970215,0.0023996528834686615
17820,35641,17820,53461,62.8657500743866,0.0021793110136059113
18594,37189,18594,55783,65.47942209243774,0.0019711316981556593
19369,38739,19369,58108,68.09490513801575,0.0017870550473162439
20144,40289,20144,60433,70.78429126739502,0.001615925328223966
20919,41839,20919,62758,73.67022013664246,0.0014607805514970096
21693,43387,21693,65080,76.42484784126282,0.001323564780250308
22468,44937,22468,67405,79.11635994911194,0.0011996704797638813
23243,46487,23243,69730,81.74084806442261,0.001092055576009443
24018,48037,24018,72055,84.34089303016663,0.000993107409158256
24792,49585,24792,74377,86.92521095275879,0.0008996737778943498
25567,51135,25567,76702,89.5535581111908,0.0008043631096370518
26342,52685,26342,79027,92.136953830719,0.0007156788597058039
27117,54235,27117,81352,94.80945897102356,0.0006237916804820998
27891,55783,27891,83674,97.48084092140198,0.000548225898455712
28666,57333,28666,85999,100.0959370136261,0.0004942133909935364
29441,58883,29441,88324,102.68812489509583,0.0004488420545385452
30216,60433,30216,90649,105.29028511047363,0.00040464819358021487
30991,61983,30991,92974,107.91358804702759,0.00036244392140361015
31765,63531,31765,95296,110.51516389846802,0.00032371085399063304
32540,65081,32540,97621,113.1130690574646,0.00028519438637886196
33315,66631,33315,99946,115.78718495368958,0.0002489538055669982
34090,68181,34090,102271,118.40932106971741,0.00021314061450539157
34864,69729,34864,104593,121.02134418487549,0.00018004104822466616
35639,71279,35639,106918,123.6182951927185,0.00014671289864054415
36414,72829,36414,109243,126.24045395851135,0.00012676610640482977
37189,74379,37189,111568,128.89652609825134,0.0001274834849027684
37963,75927,37963,113890,131.5113890171051,0.0001277419341931818
38738,77477,38738,116215,134.2838830947876,0.00012497166244429536
39513,79027,39513,118540,137.03791689872742,0.00012021554903185461
40288,80577,40288,120865,139.66226601600647,0.00011699726201186422
41062,82125,41062,123187,142.28595805168152,0.0001147355305874953
41837,83675,41837,125512,144.8837640285492,0.00011100803021690808
42612,85225,42612,127837,147.5332748889923,0.00010569814003247302
43387,86775,43387,130162,150.1225061416626,0.0001025164128805045
44162,88325,44162,132487,152.73624396324158,9.874528768705204e-05
44936,89873,44936,134809,155.32544898986816,9.786390546651091e-05
45711,91423,45711,137134,157.95757508277893,0.00010074950660055038
46486,92973,46486,139459,160.556654214859,0.0001031169140333077
47261,94523,47261,141784,163.14953303337097,0.00010510779611649923
48035,96071,48035,144106,165.88540387153625,0.0001062755545717664
48810,97621,48810,146431,168.64868903160095,0.00010579736044746824
49585,99171,49585,148756,171.47142004966736,0.00010525467405386735
50360,100721,50360,151081,174.22674417495728,0.00010384920642536599
51134,102269,51134,153403,176.99540615081787,0.00010185028804698959
51909,103819,51909,155728,179.73317408561707,9.897376185108442e-05
52684,105369,52684,158053,182.45862817764282,9.735794446896762e-05
53459,106919,53459,160378,185.2087481021881,9.82797791948542e-05
54233,108467,54233,162700,187.93822503089905,9.620645687391516e-05
55008,110017,55008,165025,190.6682391166687,9.431776379642542e-05
55783,111567,55783,167350,193.41566395759583,9.302177386416588e-05
56558,113117,56558,169675,196.16140818595886,9.342872363049537e-05
57333,114667,57333,172000,198.94582509994507,9.326197323389351e-05
58107,116215,58107,174322,201.67475199699402,9.177753236144781e-05
58882,117765,58882,176647,204.40849208831787,8.81782834767364e-05
59657,119315,59657,178972,207.1083242893219,8.425397209066432e-05
60432,120865,60432,181297,209.84565830230713,7.942208867461886e-05
61206,122413,61206,183619,212.55731105804443,7.564453881059308e-05
61981,123963,61981,185944,215.5026319026947,7.00463951943675e-05
62756,125513,62756,188269,218.32217502593994,6.581307934538927e-05
63531,127063,63531,190594,221.06718015670776,6.39132395008346e-05
64305,128611,64305,192916,223.8058681488037,6.276919884840026e-05
65080,130161,65080,195241,226.55526614189148,6.202607255545445e-05
65855,131711,65855,197566,229.26593899726868,6.137341733847279e-05
66630,133261,66630,199891,231.99581503868103,6.0511027186294086e-05
67404,134809,67404,202213,234.63794803619385,5.852079266333021e-05
68179,136359,68179,204538,237.37354397773743,5.621965647151228e-05
68954,137909,68954,206863,240.0160551071167,5.2604791562771425e-05
69729,139459,69729,209188,242.59821915626526,4.84391948702978e-05
70504,141009,70504,211513,245.19819712638855,4.3721418478526175e-05
71278,142557,71278,213835,247.82261610031128,4.0510372855351306e-05
72053,144107,72053,216160,250.4334590435028,4.003081267001107e-05
72828,145657,72828,218485,253.0189130306244,3.860147080558818e-05
73603,147207,73603,220810,255.62403106689453,3.656563785625622e-05
74377,148755,74377,223132,258.2696180343628,3.3460652048233896e-05
75152,150305,75152,225457,260.88443303108215,3.157551145704929e-05
75927,151855,75927,227782,263.4843740463257,2.8666167054325342e-05
76702,153405,76702,230107,266.09620904922485,2.693700480449479e-05
77476,154953,77476,232429,268.72795009613037,2.351377952436451e-05
78251,156503,78251,234754,271.3304650783539,2.454014975228347e-05
79026,158053,79026,237079,273.9328589439392,2.6714507839642465e-05
79801,159603,79801,239404,276.54637694358826,2.717930510698352e-05
80575,161151,80575,241726,279.182639837265,3.0102628443273716e-05
81350,162701,81350,244051,281.87464904785156,3.119765460724011e-05
82125,164251,82125,246376,284.4688210487366,3.097036460530944e-05
82900,165801,82900,248701,287.0893020629883,2.8824342734878883e-05
83674,167349,83674,251023,289.7398989200592,2.403824510111008e-05
84449,168899,84449,253348,292.35095620155334,2.073369614663534e-05
85224,170449,85224,255673,294.96246099472046,1.5199153494904749e-05
85999,171999,85999,257998,297.56201910972595,1.183923268399667e-05
86774,173549,86774,260323,300.25460505485535,1.1765241652028635e-05
87548,175097,87548,262645,302.8561010360718,1.2892120139440522e-05
88323,176647,88323,264970,305.4631612300873,1.5386647646664642e-05
89098,178197,89098,267295,308.09879994392395,1.8569018720882013e-05
89873,179747,89873,269620,310.7483949661255,2.1210846171015874e-05
90647,181295,90647,271942,313.35808205604553,2.2328007617034018e-05
91422,182845,91422,274267,315.9660301208496,2.2831973183201626e-05
92197,184395,92197,276592,318.6076989173889,2.1542937247431837e-05
92972,185945,92972,278917,321.2079482078552,1.9815743144135922e-05
93746,187493,93746,281239,323.83251690864563,2.1108891814947128e-05
94521,189043,94521,283564,326.4411871433258,2.292700082762167e-05
95296,190593,95296,285889,329.03459310531616,2.3089714886737056e-05
96071,192143,96071,288214,331.6668691635132,2.246791700599715e-05
96845,193691,96845,290536,334.27379989624023,2.3058833903633058e-05
97620,195241,97620,292861,336.86903190612793,2.2195834390004165e-05
98395,196791,98395,295186,339.4646589756012,1.9949737179558724e-05
99170,198341,99170,297511,342.0730769634247,2.0219467842252925e-05
99945,199891,99945,299836,344.68992805480957,2.0540855985018425e-05
100719,201439,100719,302158,347.3261489868164,1.991930002986919e-05
101494,202989,101494,304483,349.94937205314636,1.855997834354639e-05
102269,204539,102269,306808,352.5736620426178,1.7686255887383595e-05
103044,206089,103044,309133,355.18724727630615,1.7531572666484863e-05
103818,207637,103818,311455,357.8209240436554,1.6314696040353738e-05
104593,209187,104593,313780,360.48984003067017,1.2627886462723836e-05
105368,210737,105368,316105,363.09752106666565,9.35580101213418e-06
106143,212287,106143,318430,365.70304703712463,8.440449164481834e-06
106917,213835,106917,320752,368.35013723373413,1.210491063829977e-05
107692,215385,107692,323077,371.1088709831238,1.5667346815462224e-05
108467,216935,108467,325402,373.79383087158203,1.88503363460768e-05
109242,218485,109242,327727,376.6077380180359,1.9234568753745407e-05
110016,220033,110016,330049,379.3425438404083,1.8051121514872648e-05
110791,221583,110791,332374,381.95368099212646,1.5811820048838854e-05
111566,223133,111566,334699,384.5488269329071,1.324856566498056e-05
112341,224683,112341,337024,387.1522262096405,9.278041034121998e-06
113116,226233,113116,339349,389.7857758998871,6.417565600713715e-06
113890,227781,113890,341671,392.3829951286316,7.554262992925942e-06
114665,229331,114665,343996,394.9729549884796,1.026120298774913e-05
115440,230881,115440,346321,397.59638714790344,1.170631730929017e-05
116215,232431,116215,348646,400.25602197647095,1.198944664793089e-05
116989,233979,116989,350968,402.941232919693,1.2242708180565387e-05
117764,235529,117764,353293,405.5837490558624,1.219591467815917e-05
118539,237079,118539,355618,408.210333108902,1.2919916116516106e-05
119314,238629,119314,357943,410.8298602104187,1.3319102436071262e-05
120088,240177,120088,360265,413.4221131801605,1.3684311852557585e-05
120863,241727,120863,362590,416.04121708869934,1.2838274415116757e-05
121638,243277,121638,364915,418.6422860622406,1.2584298019646667e-05
122413,244827,122413,367240,421.28537106513977,1.0868310710065998e-05
123187,246375,123187,369562,423.870078086853,1.0482979632797651e-05
123962,247925,123962,371887,426.4902489185333,1.0073383236886002e-05
124737,249475,124737,374212,429.11045002937317,9.443641829420812e-06
125512,251025,125512,376537,431.7575891017914,9.667259291745722e-06
126286,252573,126286,378859,434.3851752281189,8.75638761499431e-06
127061,254123,127061,381184,437.14276790618896,6.131020199973136e-06
127836,255673,127836,383509,439.88828706741333,4.857853127759881e-06
128611,257223,128611,385834,442.4880909919739,4.247289325576276e-06
129386,258773,129386,388159,445.09362602233887,5.760231942986138e-06
130160,260321,130160,390481,447.70531606674194,8.511267878930084e-06
130935,261871,130935,392806,450.3397591114044,9.231502190232277e-06
131710,263421,131710,395131,452.93116307258606,9.867173503153026e-06
132485,264971,132485,397456,455.79060411453247,8.60466025187634e-06
133259,266519,133259,399778,458.48410820961,7.827222361811437e-06
134034,268069,134034,402103,461.10670018196106,5.042500561103225e-06
134809,269619,134809,404428,463.73003125190735,3.978726454079151e-06
135584,271169,135584,406753,466.3415639400482,5.256886652205139e-06
136358,272717,136358,409075,468.9438819885254,7.024626029306091e-06
137133,274267,137133,411400,471.5861608982086,7.304419341380708e-06
137908,275817,137908,413725,474.22146010398865,8.054643330979161e-06
138683,277367,138683,416050,476.82519721984863,8.78046193975024e-06
139457,278915,139457,418372,479.46450901031494,9.842533472692594e-06
140232,280465,140232,420697,482.2165541648865,1.0234269211650826e-05
141007,282015,141007,423022,484.8849501609802,9.010669600684196e-06
141782,283565,141782,425347,487.4891040325165,9.318553566117771e-06
142557,285115,142557,427672,490.1180500984192,9.162075002677739e-06
143331,286663,143331,429994,492.72211623191833,9.685210898169316e-06
144106,288213,144106,432319,495.3201632499695,9.174023944069631e-06
144881,289763,144881,434644,497.9609811306,9.238789061782882e-06
145656,291313,145656,436969,500.5933539867401,8.904356946004555e-06
146430,292861,146430,439291,503.20531606674194,7.72114253777545e-06
147205,294411,147205,441616,505.82760190963745,6.9441466621356085e-06
147980,295961,147980,443941,508.44168615341187,6.386082532117143e-06
148755,297511,148755,446266,511.0604159832001,5.5658565543126315e-06
149529,299059,149529,448588,513.6633100509644,4.209445251035504e-06
150304,300609,150304,450913,516.2868769168854,4.235032974975184e-06
151079,302159,151079,453238,518.9262721538544,6.225107426871546e-06
151854,303709,151854,455563,521.5352499485016,7.973192623467185e-06
152628,305257,152628,457885,524.1618921756744,8.497781891492195e-06
153403,306807,153403,460210,526.8418691158295,7.045169695629738e-06
154178,308357,154178,462535,529.4907321929932,4.977049684384838e-06
154953,309907,154953,464860,532.0958580970764,3.5085158742731437e-06
155728,311457,155728,467185,534.7237720489502,4.484696546569467e-06
156502,313005,156502,469507,537.3432719707489,5.256684744381346e-06
157277,314555,157277,471832,539.9644250869751,5.337660695658997e-06
158052,316105,158052,474157,542.5941309928894,5.4241845646174625e-06
158827,317655,158827,476482,545.205824136734,6.3309653342003e-06
159601,319203,159601,478804,547.8125472068787,6.3345851231133565e-06
160376,320753,160376,481129,550.4250130653381,6.526486686198041e-06
161151,322303,161151,483454,553.0365929603577,6.161477358546108e-06
161926,323853,161926,485779,555.6616299152374,6.674170435871929e-06
162700,325401,162700,488101,558.2926280498505,7.045575330266729e-06
163475,326951,163475,490426,560.9237780570984,6.345706424326636e-06
164250,328501,164250,492751,563.614825963974,5.786556357634254e-06
165025,330051,165025,495076,566.3376798629761,5.389196303440258e-06
165799,331599,165799,497398,569.0307359695435,4.6584918891312554e-06
166574,333149,166574,499723,571.7780170440674,3.6330420698504895e-06
167349,334699,167349,502048,574.4995651245117,2.848033545888029e-06
168124,336249,168124,504373,577.195739030838,1.456073732697405e-06
168899,337799,168899,506698,579.918331861496,2.708091415115632e-06
169673,339347,169673,509020,582.6349132061005,4.7812463890295476e-06
170448,340897,170448,511345,585.3622379302979,5.865429557161406e-06
171223,342447,171223,513670,588.1242849826813,5.558526027016342e-06
171998,343997,171998,515995,590.8497550487518,4.096244083484635e-06
172772,345545,172772,518317,593.6097390651703,2.726032107602805e-06
173547,347095,173547,520642,596.5480411052704,2.0210372895235196e-06
174322,348645,174322,522967,599.3574368953705,3.115877916570753e-06
175097,350195,175097,525292,602.0838751792908,3.316006768727675e-06
175871,351743,175871,527614,604.8349521160126,3.619450581027195e-06
176646,353293,176646,529939,607.558039188385,4.899149644188583e-06
177421,354843,177421,532264,610.2897641658783,5.4596675909124315e-06
178196,356393,178196,534589,613.0065290927887,5.28391137777362e-06
178970,357941,178970,536911,615.7746601104736,5.458885425468907e-06
179745,359491,179745,539236,618.5325441360474,5.85163252253551e-06
180520,361041,180520,541561,621.3339149951935,5.327563485479914e-06
181295,362591,181295,543886,624.0878391265869,4.272387741366401e-06
182069,364139,182069,546208,626.8048191070557,4.0225095290225e-06
182844,365689,182844,548533,629.5146200656891,3.2339048630092293e-06
183619,367239,183619,550858,632.1370460987091,2.0082443370483816e-06
184394,368789,184394,553183,634.7678029537201,2.217908331658691e-06
185169,370339,185169,555508,637.400139093399,3.4299555409234017e-06
185943,371887,185943,557830,640.0287871360779,4.501951480051503e-06
186718,373437,186718,560155,642.6331031322479,5.0911821745103225e-06
187493,374987,187493,562480,645.2510778903961,4.863744834437966e-06
188268,376537,188268,564805,647.8905642032623,3.0397422960959375e-06
189042,378085,189042,567127,650.4947230815887,2.188049620599486e-06
189817,379635,189817,569452,653.1078128814697,1.8584632925922051e-06
190592,381185,190592,571777,655.7045991420746,2.6758079911815003e-06
191367,382735,191367,574102,658.3114252090454,3.881936208927073e-06
192141,384283,192141,576424,660.9094860553741,4.059833372593857e-06
192916,385833,192916,578749,663.5393459796906,4.547073331195861e-06
193691,387383,193691,581074,666.1638770103455,4.733479727292433e-06
194466,388933,194466,583399,668.7777349948883,4.469198756851256e-06
195240,390481,195240,585721,671.3601140975952,4.205299774184823e-06
196015,392031,196015,588046,673.981153011322,3.7490990507649258e-06
196790,393581,196790,590371,676.6062998771667,3.012604793184437e-06
197565,395131,197565,592696,679.1994712352753,2.66384995484259e-06
198340,396681,198340,595021,681.7963840961456,1.8449372873874381e-06
199114,398229,199114,597343,684.3965640068054,1.8850805645342916e-06
199889,399779,199889,599668,687.0088400840759,2.7780679374700412e-06
200664,401329,200664,601993,689.6142420768738,3.475443008937873e-06
201439,402879,201439,604318,692.2077419757843,3.866776751237921e-06
202213,404427,202213,606640,694.8251020908356,3.1757299439050257e-06
202988,405977,202988,608965,697.4199891090393,1.928192432387732e-06
203763,407527,203763,611290,700.035236120224,1.1906759027624503e-06
204538,409077,204538,613615,702.6316821575165,1.6950525605352595e-06
205312,410625,205312,615937,705.2388410568237,2.5117169570876285e-06
206087,412175,206087,618262,707.8800342082977,2.5970457500079647e-06
206862,413725,206862,620587,710.4810869693756,3.4032764233415946e-06
207637,415275,207637,622912,713.0749220848083,3.4921995393233374e-06
208411,416823,208411,625234,715.8064610958099,3.0635728762717918e-06
209186,418373,209186,627559,718.5024859905243,3.0633582355221733e-06
209961,419923,209961,629884,721.1435351371765,3.140450644423254e-06
210736,421473,210736,632209,723.7795991897583,2.422924808342941e-06
211511,423023,211511,634534,726.4078950881958,2.4518139980500564e-06
212285,424571,212285,636856,729.0143141746521,1.6804660845082253e-06
213060,426121,213060,639181,731.7661321163177,1.2220298231113702e-06
213835,427671,213835,641506,734.4210121631622,2.1001033019274473e-06
214610,429221,214610,643831,737.0478370189667,2.259856046293862e-06
215384,430769,215384,646153,739.6393330097198,2.910957846324891e-06
216159,432319,216159,648478,742.387197971344,2.776447217911482e-06
216934,433869,216934,650803,745.1688561439514,2.1613195713143796e-06
217709,435419,217709,653128,747.8839602470398,1.625297954888083e-06
218483,436967,218483,655450,750.5355131626129,1.5734949556645006e-06
219258,438517,219258,657775,753.1657538414001,1.932410668814555e-06
220033,440067,220033,660100,755.7832200527191,2.36985033552628e-06
220808,441617,220808,662425,758.4568982124329,2.7162168407812715e-06
221582,443165,221582,664747,761.0529069900513,2.7323985705152154e-06
222357,444715,222357,667072,763.6542201042175,3.105347786913626e-06
223132,446265,223132,669397,766.2873330116272,3.2005154935177416e-06
223907,447815,223907,671722,768.8883430957794,2.730794221861288e-06
224681,449363,224681,674044,771.4799518585205,2.713639332796447e-06
225456,450913,225456,676369,774.0975959300995,2.086566382786259e-06
226231,452463,226231,678694,776.7039110660553,1.2512246030382812e-06
227006,454013,227006,681019,779.302953004837,1.3244534784462303e-06
227781,455563,227781,683344,781.912143945694,1.9272520148660988e-06
228555,457111,228555,685666,784.5509650707245,2.5354092940688133e-06
229330,458661,229330,687991,787.6050498485565,3.075872882618569e-06
230105,460211,230105,690316,790.4109740257263,2.5841418391792104e-06
230880,461761,230880,692641,793.2167320251465,2.3318953026318923e-06
231654,463309,231654,694963,795.9507138729095,1.6092180885607377e-06
232429,464859,232429,697288,798.7141242027283,7.67555320635438e-07
233204,466409,233204,699613,801.6599502563477,1.7249531083507463e-06
233979,467959,233979,701938,804.513069152832,1.9996004994027317e-06
234753,469507,234753,704260,807.3050911426544,2.544309609220363e-06
235528,471057,235528,706585,810.0514183044434,2.734899680945091e-06
236303,472607,236303,708910,812.7864971160889,2.3797183530405164e-06
237078,474157,237078,711235,815.5141232013702,2.5498247850919142e-06
237852,475705,237852,713557,818.2902801036835,2.1228406694717705e-06
238627,477255,238627,715882,821.0325410366058,1.8442297005094588e-06
239402,478805,239402,718207,823.7864201068878,1.6523754311492667e-06
240177,480355,240177,720532,826.5912530422211,8.154602255672216e-07
240952,481905,240952,722857,829.4441180229187,1.417502062395215e-06
241726,483453,241726,725179,832.1755731105804,1.7854072211775929e-06
242501,485003,242501,727504,834.9186398983002,1.969034201465547e-06
243276,486553,243276,729829,837.6561350822449,2.1786181605421007e-06
244051,488103,244051,732154,840.3922460079193,2.0307670638430864e-06
244825,489651,244825,734476,843.1557919979095,2.1912710508331656e-06
245600,491201,245600,736801,845.9046499729156,1.7875863704830408e-06
246375,492751,246375,739126,848.653158903122,1.4039505913387984e-06
247150,494301,247150,741451,851.3505439758301,7.132694008760154e-07
247924,495849,247924,743773,853.987722158432,9.008908818941563e-07
248699,497399,248699,746098,856.6152260303497,1.5033947420306504e-06
249474,498949,249474,748423,859.2446510791779,1.7441125237382948e-06
250249,500499,250249,750748,861.8809411525726,2.178852810175158e-06
251023,502047,251023,753070,864.4866991043091,2.0372553990455344e-06
251798,503597,251798,755395,867.0862550735474,2.0124789443798363e-06
252573,505147,252573,757720,869.7130219936371,1.554924892843701e-06
253348,506697,253348,760045,872.3150322437286,1.113297912525013e-06
254123,508247,254123,762370,874.9225862026215,7.488251867471263e-07
254897,509795,254897,764692,877.5160050392151,9.504674380877987e-07
255672,511345,255672,767017,880.1173911094666,1.5907789929769933e-06
256447,512895,256447,769342,882.7944431304932,1.635335138416849e-06
257222,514445,257222,771667,885.3958129882812,1.9297913240734488e-06
257996,515993,257996,773989,888.0245051383972,1.6469839465571567e-06
258771,517543,258771,776314,890.6313989162445,1.8146311049349606e-06
259546,519093,259546,778639,893.2430069446564,1.5965651982696727e-06
260321,520643,260321,780964,895.8388290405273,1.2821419659303501e-06
261095,522191,261095,783286,898.423173904419,7.454855222022161e-07
261870,523741,261870,785611,901.007269859314,1.107126081478782e-06
262645,525291,262645,787936,903.6254191398621,1.4240686141420156e-06
263420,526841,263420,790261,906.2506530284882,1.7107540770666674e-06
264194,528389,264194,792583,908.8697621822357,1.9630369934020564e-06
264969,529939,264969,794908,911.4970502853394,1.9011258700629696e-06
265744,531489,265744,797233,914.1162109375,1.7795537132769823e-06
266519,533039,266519,799558,916.7361118793488,1.2761447578668594e-06
267293,534587,267293,801880,919.343138217926,7.379330781986937e-07
268068,536137,268068,804205,921.9333808422089,8.929164323490113e-07
268843,537687,268843,806530,924.5354981422424,1.4916931831976399e-06
269618,539237,269618,808855,927.1493890285492,1.6785743355285376e-06
270393,540787,270393,811180,929.7446842193604,1.9136223272653297e-06
271167,542335,271167,813502,932.3443038463593,1.7436304915463552e-06
271942,543885,271942,815827,934.9860382080078,1.5834393707336858e-06
272717,545435,272717,818152,937.6153371334076,1.2692635209532455e-06
273492,546985,273492,820477,940.2072870731354,1.0622552508721128e-06
274266,548533,274266,822799,942.798770904541,7.447797543136403e-07
275041,550083,275041,825124,945.4128589630127,1.2474138202378526e-06
275816,551633,275816,827449,948.0390651226044,1.4484066923614591e-06
276591,553183,276591,829774,950.6528930664062,1.5054756659083068e-06
277365,554731,277365,832096,953.260645866394,1.6171525203390047e-06
278140,556281,278140,834421,955.8567440509796,1.5355926734628156e-06
278915,557831,278915,836746,958.4743571281433,1.2757154763676226e-06
279690,559381,279690,839071,961.0752410888672,7.530543371103704e-07
280464,560929,280464,841393,963.6622641086578,7.252965588122606e-07
281239,562479,281239,843718,966.2741351127625,9.727591532282531e-07
282014,564029,282014,846043,968.8832290172577,1.4184097381075844e-06
282789,565579,282789,848368,971.4852170944214,1.4555262168869376e-06
283564,567129,283564,850693,974.0844612121582,1.5753412299090996e-06
284338,568677,284338,853015,976.7026591300964,1.2215987226227298e-06
285113,570227,285113,855340,979.3257710933685,9.713348845252767e-07
285888,571777,285888,857665,981.962856054306,5.241272447165102e-07
286663,573327,286663,859990,984.6902952194214,7.220696716103703e-07
287437,574875,287437,862312,987.4323210716248,1.1276424629613757e-06
288212,576425,288212,864637,990.066890001297,1.3166572898626328e-06
288987,577975,288987,866962,992.6536159515381,1.3655080692842603e-06
289762,579525,289762,869287,995.2723960876465,1.1217925930395722e-06
290536,581073,290536,871609,997.8841800689697,1.1381798685761169e-06
291311,582623,291311,873934,1000.4899652004242,7.048220140859485e-07
292086,584173,292086,876259,1003.0706608295441,5.175334081286564e-07
292861,585723,292861,878584,1005.6525690555573,8.390252332901582e-07
293635,587271,293635,880906,1008.2909970283508,1.0274343367200345e-06
294410,588821,294410,883231,1010.9721779823303,1.279362550121732e-06
295185,590371,295185,885556,1013.6102101802826,1.2548171071102843e-06
295960,591921,295960,887881,1016.3691022396088,1.2532054824987426e-06
296735,593471,296735,890206,1018.9981510639191,8.916340448195115e-07
297509,595019,297509,892528,1021.6157791614532,3.979912435170263e-07
298284,596569,298284,894853,1024.2000210285187,6.737609510309994e-07
299059,598119,299059,897178,1026.8613090515137,9.866071195574477e-07
299834,599669,299834,899503,1029.5226299762726,1.32853165268898e-06
300608,601217,300608,901825,1032.128428220749,1.3305361790116876e-06
301383,602767,301383,904150,1034.7577538490295,1.1399151844670996e-06
302158,604317,302158,906475,1037.4094049930573,9.277209755964577e-07
302933,605867,302933,908800,1040.0223019123077,6.060035957489163e-07
303707,607415,303707,911122,1042.6992211341858,6.841819413239136e-07
304482,608965,304482,913447,1045.417032957077,1.0632138582877815e-06
305257,610515,305257,915772,1048.0898802280426,1.098418579204008e-06
306032,612065,306032,918097,1050.6801090240479,1.1998999980278313e-06
306806,613613,306806,920419,1053.2878699302673,1.211268681799993e-06
307581,615163,307581,922744,1055.8704981803894,9.348405001219362e-07
308356,616713,308356,925069,1058.5126330852509,6.299978849710897e-07
309131,618263,309131,927394,1061.2354640960693,6.724876584485173e-07
309906,619813,309906,929719,1063.8729538917542,8.267688826890662e-07
310680,621361,310680,932041,1066.5040199756622,1.1991214705631137e-06
311455,622911,311455,934366,1069.0954539775848,1.2862183211836964e-06
312230,624461,312230,936691,1071.6934931278229,1.1059837561333552e-06
313005,626011,313005,939016,1074.3039691448212,8.704973879503086e-07
313779,627559,313779,941338,1076.933392047882,4.924495442537591e-07
314554,629109,314554,943663,1079.541981935501,6.377558747772127e-07
315329,630659,315329,945988,1082.12970495224,9.773393685463816e-07
316104,632209,316104,948313,1084.7042078971863,1.1708852980518714e-06
316878,633757,316878,950635,1087.327430009842,1.0996827768394724e-06
317653,635307,317653,952960,1089.9455261230469,8.959941624198109e-07
318428,636857,318428,955285,1092.5408289432526,7.023481884971261e-07
319203,638407,319203,957610,1095.151554107666,4.3998807086609304e-07
319977,639955,319977,959932,1097.7849791049957,7.65929144108668e-07
320752,641505,320752,962257,1100.4096291065216,8.771530701778829e-07
321527,643055,321527,964582,1103.0200729370117,9.806590242078528e-07
322302,644605,322302,966907,1105.6157629489899,1.0331714292988181e-06
323076,646153,323076,969229,1108.2150909900665,8.83344910107553e-07
323851,647703,323851,971554,1110.8268649578094,5.297024472383782e-07
324626,649253,324626,973879,1113.4278030395508,3.235763870179653e-07
325401,650803,325401,976204,1116.347004890442,7.319085852941498e-07
326176,652353,326176,978529,1119.1206440925598,9.288251021644101e-07
326950,653901,326950,980851,1121.7215361595154,9.270861482946202e-07
327725,655451,327725,983176,1124.3302669525146,7.659727998543531e-07
328500,657001,328500,985501,1126.9660859107971,5.16602085554041e-07
329275,658551,329275,987826,1129.5697548389435,2.8878639568574727e-07
330049,660099,330049,990148,1132.192633152008,6.544541975017637e-07
330824,661649,330824,992473,1134.8950769901276,8.231254469137639e-07
331599,663199,331599,994798,1137.5126490592957,8.132701623253524e-07
332374,664749,332374,997123,1140.1283621788025,8.334573067259043e-07
333148,666297,333148,999445,1142.7497990131378,6.589161785086617e-07
333923,667847,333923,1001770,1145.3451120853424,2.90938260150142e-07
334698,669397,334698,1004095,1147.9580450057983,4.6051536628510803e-07
335473,670947,335473,1006420,1150.564973115921,7.281887519638985e-07
336247,672495,336247,1008742,1153.1676330566406,8.656825229991227e-07
337022,674045,337022,1011067,1155.7823832035065,8.025090210139751e-07
337797,675595,337797,1013392,1158.4099140167236,5.367110134102404e-07
338572,677145,338572,1015717,1161.008670091629,1.9807521312031895e-07
339347,678695,339347,1018042,1163.6160049438477,5.402198439696804e-07
340121,680243,340121,1020364,1166.2361290454865,7.846210792195052e-07
340896,681793,340896,1022689,1168.8604581356049,8.110764611046761e-07
341671,683343,341671,1025014,1171.4627652168274,7.066992111504078e-07
342446,684893,342446,1027339,1174.1985681056976,5.828787834616378e-07
343220,686441,343220,1029661,1176.9205901622772,2.7056194085162133e-07
343995,687991,343995,1031986,1179.6214580535889,5.207366484683007e-07
344770,689541,344770,1034311,1182.2078258991241,7.164417183957994e-07
345545,691091,345545,1036636,1184.7978792190552,8.230090315919369e-07
346319,692639,346319,1038958,1187.4134330749512,7.36457877792418e-07
347094,694189,347094,1041283,1190.0466902256012,4.5780689106322825e-07
347869,695739,347869,1043608,1192.667044878006,2.8940849006175995e-07
348644,697289,348644,1045933,1195.3384990692139,6.452428351622075e-07
349418,698837,349418,1048255,1197.9420280456543,7.663002179469913e-07
350193,700387,350193,1050580,1200.6052701473236,6.953196134418249e-07
350968,701937,350968,1052905,1203.2615630626678,6.182563083712012e-07
351743,703487,351743,1055230,1205.8444809913635,3.536424628691748e-07
352518,705037,352518,1057555,1208.4673421382904,4.352750693215057e-07
353292,706585,353292,1059877,1211.0588240623474,6.355476216413081e-07
354067,708135,354067,1062202,1213.675784111023,7.601520337630063e-07
354842,709685,354842,1064527,1216.27787399292,7.008602551650256e-07
355617,711235,355617,1066852,1218.9456520080566,4.323337634559721e-07
356391,712783,356391,1069174,1221.5581650733948,2.2262793208938092e-07
357166,714333,357166,1071499,1224.1616020202637,5.511683411896229e-07
357941,715883,357941,1073824,1226.7643189430237,6.774043868063018e-07
358716,717433,358716,1076149,1229.396686077118,6.258305802475661e-07
359490,718981,359490,1078471,1231.985778093338,5.409001460066065e-07
360265,720531,360265,1080796,1234.5906870365143,2.531032805563882e-07
361040,722081,361040,1083121,1237.2122812271118,3.852692316286266e-07
361815,723631,361815,1085446,1239.83726811409,5.665788194164634e-07
362589,725179,362589,1087768,1242.457594871521,6.441241566790268e-07
363364,726729,363364,1090093,1245.0747010707855,5.312667781254277e-07
364139,728279,364139,1092418,1247.7199010849,2.544566086726263e-07
364914,729829,364914,1094743,1250.3499519824982,3.0892442737240344e-07
365688,731377,365688,1097065,1253.094575881958,5.193596734898165e-07
366463,732927,366463,1099390,1255.8030421733856,5.280871846480295e-07
367238,734477,367238,1101715,1258.4480509757996,4.833073035115376e-07
368013,736027,368013,1104040,1261.0680301189423,2.602118911454454e-07
368788,737577,368788,1106365,1263.6735439300537,2.811393642332405e-07
369562,739125,369562,1108687,1266.2817080020905,4.800731403520331e-07
370337,740675,370337,1111012,1268.8710551261902,5.593246896751225e-07
371112,742225,371112,1113337,1271.5171661376953,4.5938577386550605e-07
371887,743775,371887,1115662,1274.1262691020966,1.964235707418993e-07
372661,745323,372661,1117984,1276.7715060710907,2.989345375681296e-07
373436,746873,373436,1120309,1279.4950699806213,4.7160210669972e-07
374211,748423,374211,1122634,1282.1276450157166,4.547855496639386e-07
374986,749973,374986,1124959,1284.7400760650635,4.164521669736132e-07
375760,751521,375760,1127281,1287.364166021347,1.7229467630386353e-07
376535,753071,376535,1129606,1289.9951729774475,2.847646101145074e-07
377310,754621,377310,1131931,1292.596313238144,4.711928340839222e-07
378085,756171,378085,1134256,1295.2334380149841,4.87883880850859e-07
378859,757719,378859,1136578,1297.8456320762634,2.963715814985335e-07
379634,759269,379634,1138903,1300.4785211086273,1.7541060515213758e-07
380409,760819,380409,1141228,1303.0967519283295,4.208359314361587e-07
381184,762369,381184,1143553,1305.7118651866913,4.657431418308988e-07
381959,763919,381959,1145878,1308.3325741291046,4.114626790396869e-07
382733,765467,382733,1148200,1310.9559319019318,2.2677704691886902e-07
383508,767017,383508,1150525,1313.5763399600983,2.99962266581133e-07
384283,768567,384283,1152850,1316.2066791057587,4.605135472957045e-07
385058,770117,385058,1155175,1318.8339021205902,4.765388439409435e-07
385832,771665,385832,1157497,1321.4510080814362,3.021959855686873e-07
386607,773215,386607,1159822,1324.0690660476685,2.2558560885954648e-07
387382,774765,387382,1162147,1326.6810810565948,4.332359822001308e-07
388157,776315,388157,1164472,1329.2954471111298,4.4064290705136955e-07
388931,777863,388931,1166794,1331.9481852054596,3.9312908484134823e-07
389706,779413,389706,1169119,1334.5581080913544,1.7840829968918115e-07
390481,780963,390481,1171444,1337.2016341686249,3.371187631273642e-07
391256,782513,391256,1173769,1339.9692602157593,4.651556082535535e-07
392030,784061,392030,1176091,1342.7373189926147,3.8699363358318806e-07
392805,785611,392805,1178416,1345.396388053894,2.0647166820708662e-07
393580,787161,393580,1180741,1348.0715589523315,3.1155468604993075e-07
394355,788711,394355,1183066,1350.7872650623322,4.118992364965379e-07
395130,790261,395130,1185391,1353.5803022384644,4.045159585075453e-07
395904,791809,395904,1187713,1356.294909954071,2.0527841115836054e-07
396679,793359,396679,1190038,1358.990739107132,2.825199771905318e-07
397454,794909,397454,1192363,1361.6311151981354,3.745790309039876e-07
398229,796459,398229,1194688,1364.2357079982758,3.5390803532209247e-07
399003,798007,399003,1197010,1366.8649621009827,1.7287857190240175e-07
399778,799557,399778,1199335,1369.4745001792908,2.5831832317635417e-07
400553,801107,400553,1201660,1372.0916390419006,3.4123695513699204e-07
401328,802657,401328,1203985,1374.799269914627,2.503147698007524e-07
402102,804205,402102,1206307,1377.417948961258,1.2431701179593801e-07
402877,805755,402877,1208632,1380.0546550750732,2.4598921299912035e-07
403652,807305,403652,1210957,1382.6813750267029,2.696524461498484e-07
404427,808855,404427,1213282,1385.3001201152802,1.0805524652823806e-07
405201,810403,405201,1215604,1387.9297349452972,2.255947038065642e-07
405976,811953,405976,1217929,1390.5644810199738,2.2660424292553216e-07
406751,813503,406751,1220254,1393.1682450771332,1.1245901987422258e-07
407526,815053,407526,1222579,1395.8167049884796,2.1851155906915665e-07
408301,816603,408301,1224904,1398.4715640544891,2.20945366891101e-07
409075,818151,409075,1227226,1401.0782091617584,7.456947059836239e-08
409850,819701,409850,1229551,1403.8200840950012,2.1099003788549453e-07
410625,821251,410625,1231876,1406.4773271083832,1.6345074982382357e-07
411400,822801,411400,1234201,1409.1005260944366,1.0473377187736332e-07
412174,824349,412174,1236523,1411.6908769607544,1.6247031453531235e-07
412949,825899,412949,1238848,1414.3312299251556,1.0256189852952957e-07
413724,827449,413724,1241173,1416.9285068511963,1.3928547559771687e-07
414499,828999,414499,1243498,1419.6768279075623,1.473545125918463e-07
415273,830547,415273,1245820,1422.4201030731201,9.31977410800755e-08
416048,832097,416048,1248145,1425.1307001113892,1.503340172348544e-07
416823,833647,416823,1250470,1427.818174123764,7.322341843973845e-08
417598,835197,417598,1252795,1430.470137834549,1.4516990631818771e-07
418372,836745,418372,1255117,1433.350641965866,1.2420605344232172e-07
419147,838295,419147,1257442,1436.0495512485504,1.320477167610079e-07
419922,839845,419922,1259767,1438.6693940162659,1.5126897778827697e-07
420697,841395,420697,1262092,1441.2789361476898,6.770642357878387e-08
421471,842943,421471,1264414,1443.9011640548706,1.539556251373142e-07
422246,844493,422246,1266739,1446.5470931529999,8.453207556158304e-08
423021,846043,423021,1269064,1449.181205034256,1.3989119906909764e-07
423796,847593,423796,1271389,1451.9040808677673,8.861934475135058e-08
424571,849143,424571,1273714,1454.6514530181885,1.352163963019848e-07
425345,850691,425345,1276036,1457.330715894699,7.382550393231213e-08
426120,852241,426120,1278361,1459.9468400478363,1.2643977242987603e-07
426895,853791,426895,1280686,1462.5553119182587,8.491588232573122e-08
427670,855341,427670,1283011,1465.275505065918,1.2619602784980088e-07
428444,856889,428444,1285333,1468.004019021988,9.929317457135767e-08
429219,858439,429219,1287658,1470.860671043396,8.980350685305893e-08
429994,859989,429994,1289983,1473.5991060733795,1.3150565791875124e-07
430769,861539,430769,1292308,1476.2160730361938,1.080607034964487e-07
431543,863087,431543,1294630,1478.85751414299,9.378527465742081e-08
432318,864637,432318,1296955,1481.465658903122,1.193893695017323e-07
433093,866187,433093,1299280,1484.0991780757904,1.0887197277043015e-07
433868,867737,433868,1301605,1486.786583185196,8.99963197298348e-08
434642,869285,434642,1303927,1489.4118139743805,1.0194526112172753e-07
435417,870835,435417,1306252,1492.102447271347,1.1013071343768388e-07
436192,872385,436192,1308577,1494.7534580230713,9.375798981636763e-08
436967,873935,436967,1310902,1497.369166135788,7.643211574759334e-08
437742,875485,437742,1313227,1499.9729690551758,8.664574124850333e-08
438516,877033,438516,1315549,1502.5764529705048,8.962160791270435e-08
439291,878583,439291,1317874,1505.1877870559692,7.788366929162294e-08
440066,880133,440066,1320199,1507.8096070289612,7.176822691690177e-08
440841,881683,440841,1322524,1510.4193470478058,7.814560376573354e-08
441615,883231,441615,1324846,1513.0346660614014,6.762638804502785e-08
442390,884781,442390,1327171,1515.662309885025,5.716719897463918e-08
443165,886331,443165,1329496,1518.316545009613,5.312722350936383e-08
443940,887881,443940,1331821,1520.918622970581,5.5402779253199697e-08
444714,889429,444714,1334143,1523.543033838272,4.33956302003935e-08
445489,890979,445489,1336468,1526.1882150173187,4.518551577348262e-08
446264,892529,446264,1338793,1528.8102469444275,5.127913027536124e-08
447039,894079,447039,1341118,1531.496992111206,4.174398782197386e-08
447813,895627,447813,1343440,1534.1954791545868,3.458990249782801e-08
448588,897177,448588,1345765,1536.8210492134094,3.97740222979337e-08
449363,898727,449363,1348090,1539.4318170547485,3.876812115777284e-08
450138,900277,450138,1350415,1542.036906003952,3.3940523280762136e-08
450913,901827,450913,1352740,1544.6555709838867,2.89292074739933e-08
451687,903375,451687,1355062,1547.2837481498718,3.5701305023394525e-08
452462,904925,452462,1357387,1549.9101169109344,3.460627340245992e-08
453237,906475,453237,1359712,1552.5049250125885,2.4334440240636468e-08
454012,908025,454012,1362037,1555.1604380607605,3.097557055298239e-08
454786,909573,454786,1364359,1557.7792909145355,3.331842890474945e-08
455561,911123,455561,1366684,1560.4086999893188,2.7746864361688495e-08
456336,912673,456336,1369009,1563.0096790790558,2.6488123694434762e-08
457111,914223,457111,1371334,1565.6316192150116,3.199784259777516e-08
457885,915771,457885,1373656,1568.223887205124,3.425884642638266e-08
458660,917321,458660,1375981,1570.825433254242,2.734486770350486e-08
459435,918871,459435,1378306,1573.4481010437012,3.2487150747328997e-08
460210,920421,460210,1380631,1576.0786690711975,3.9661244954913855e-08
460984,921969,460984,1382953,1578.7470421791077,3.499553713481873e-08
461759,923519,461759,1385278,1581.3519940376282,3.5837729228660464e-08
462534,925069,462534,1387603,1583.9570980072021,4.294270183891058e-08
463309,926619,463309,1389928,1586.5917670726776,4.579305823426694e-08
464083,928167,464083,1392250,1589.1940941810608,4.2145984480157495e-08
464858,929717,464858,1394575,1591.8073091506958,4.555840860120952e-08
465633,931267,465633,1396900,1594.4276940822601,5.3756593842990696e-08
466408,932817,466408,1399225,1597.0496981143951,5.019137461204082e-08
467183,934367,467183,1401550,1599.6606311798096,4.903085937257856e-08
467957,935915,467957,1403872,1602.2737019062042,5.589754437096417e-08
468732,937465,468732,1406197,1604.8767082691193,5.717447493225336e-08
469507,939015,469507,1408522,1607.5256369113922,5.314541340339929e-08
470282,940565,470282,1410847,1610.1331462860107,5.417132342699915e-08
471056,942113,471056,1413169,1612.733834028244,5.99011400481686e-08
471831,943663,471831,1415494,1615.343677997589,5.65414666198194e-08
472606,945213,472606,1417819,1617.9949488639832,5.232504918240011e-08
473381,946763,473381,1420144,1620.5853970050812,5.728361429646611e-08
474155,948311,474155,1422466,1623.1943349838257,5.766742106061429e-08
474930,949861,474930,1424791,1625.810917854309,5.1948518375866115e-08
475705,951411,475705,1427116,1628.4246101379395,5.174842954147607e-08
476480,952961,476480,1429441,1631.050784111023,5.519177648238838e-08
477254,954509,477254,1431763,1633.6788139343262,5.1935785450041294e-08
478029,956059,478029,1434088,1636.323410987854,4.6566128730773926e-08
478804,957609,478804,1436413,1638.9684329032898,4.924731911160052e-08
479579,959159,479579,1438738,1641.5738761425018,4.9876689445227385e-08
480354,960709,480354,1441063,1644.1803798675537,4.315734258852899e-08
481128,962257,481128,1443385,1646.8054521083832,4.1680323192849755e-08
481903,963807,481903,1445710,1649.4570829868317,4.4177795643918216e-08
482678,965357,482678,1448035,1652.1378660202026,4.0363374864682555e-08
483453,966907,483453,1450360,1654.8798170089722,3.47681634593755e-08
484227,968455,484227,1452682,1657.5867831707,3.5608536563813686e-08
485002,970005,485002,1455007,1660.2345201969147,3.613786248024553e-08
485777,971555,485777,1457332,1662.8474431037903,2.9756847652606666e-08
486552,973105,486552,1459657,1665.478904247284,2.68664734903723e-08
487326,974653,487326,1461979,1668.3256211280823,2.964588929899037e-08
488101,976203,488101,1464304,1671.0528309345245,2.6231646188534796e-08
488876,977753,488876,1466629,1673.7839081287384,2.0983861759305e-08
489651,979303,489651,1468954,1676.4993999004364,2.2149833966977894e-08
490425,980851,490425,1471276,1679.2572820186615,2.32448655879125e-08
491200,982401,491200,1473601,1682.0291690826416,1.8935679690912366e-08
491975,983951,491975,1475926,1684.763640165329,1.660737325437367e-08
492750,985501,492750,1478251,1687.4539561271667,2.0349034457467496e-08
493525,987051,493525,1480576,1690.1592478752136,1.9523213268257678e-08
494299,988599,494299,1482898,1692.888060092926,1.5455952961929142e-08
495074,990149,495074,1485223,1695.5832269191742,1.8075297703035176e-08
495849,991699,495849,1487548,1698.3278000354767,2.0925654098391533e-08
496624,993249,496624,1489873,1701.0517382621765,1.8575519789010286e-08
497398,994797,497398,1492195,1703.9554262161255,1.7851562006399035e-08
498173,996347,498173,1494520,1706.6526448726654,2.216438588220626e-08
498948,997897,498948,1496845,1709.395262002945,2.355227479711175e-08
499723,999447,499723,1499170,1712.1154351234436,2.072556526400149e-08
500497,1000995,500497,1501492,1714.8233759403229,2.3575921659357846e-08
501272,1002545,501272,1503817,1717.540889263153,2.7783244149759412e-08
502047,1004095,502047,1506142,1720.2667260169983,2.6231646188534796e-08
502822,1005645,502822,1508467,1722.9536740779877,2.6104316930286586e-08
503596,1007193,503596,1510789,1725.650407075882,3.038621798623353e-08
504371,1008743,504371,1513114,1728.4129750728607,3.235982148908079e-08
505146,1010293,505146,1515439,1731.1071560382843,3.0257069738581777e-08
505921,1011843,505921,1517764,1733.7339761257172,3.234526957385242e-08
506696,1013393,506696,1520089,1736.338900089264,3.6781784729100764e-08
507470,1014941,507470,1522411,1738.962720155716,3.552304406184703e-08
508245,1016491,508245,1524736,1741.5715131759644,3.487730282358825e-08
509020,1018041,509020,1527061,1744.1597290039062,3.866625775117427e-08
509795,1019591,509795,1529386,1746.7518842220306,4.024332156404853e-08
510569,1021139,510569,1531708,1749.3666551113129,3.810782800428569e-08
511344,1022689,511344,1534033,1751.969773054123,3.8915459299460053e-08
512119,1024239,512119,1536358,1754.5777008533478,4.2462488636374474e-08
512894,1025789,512894,1538683,1757.1767029762268,4.097637429367751e-08
513668,1027337,513668,1541005,1759.80095911026,3.882814780808985e-08
514443,1028887,514443,1543330,1762.4038531780243,4.140929377172142e-08
515218,1030437,515218,1545655,1765.013482093811,4.186586011201143e-08
515993,1031987,515993,1547980,1767.6220800876617,3.874083631671965e-08
516767,1033535,516767,1550302,1770.2497291564941,3.797686076723039e-08
517542,1035085,517542,1552627,1772.8457689285278,3.980494511779398e-08
518317,1036635,518317,1554952,1775.6856710910797,3.7698555388487875e-08
519092,1038185,519092,1557277,1778.401239156723,3.400054993107915e-08
519866,1039733,519866,1559599,1781.040297985077,3.496461431495845e-08
520641,1041283,520641,1561924,1783.6348259449005,3.468812792561948e-08
521416,1042833,521416,1564249,1786.2818729877472,3.0573573894798756e-08
522191,1044383,522191,1566574,1788.9341180324554,2.8823706088587642e-08
522966,1045933,522966,1568899,1791.5237481594086,2.9602233553305268e-08
523740,1047481,523740,1571221,1794.1104369163513,2.734486770350486e-08
524515,1049031,524515,1573546,1796.8091452121735,2.337219484616071e-08
525290,1050581,525290,1575871,1799.4454910755157,2.3426764528267086e-08
526065,1052131,526065,1578196,1802.058884859085,2.350861905142665e-08
526839,1053679,526839,1580518,1804.6870620250702,1.9615981727838516e-08
527614,1055229,527614,1582843,1807.310429096222,1.780608727131039e-08
528389,1056779,528389,1585168,1809.9230952262878,1.885928213596344e-08
529164,1058329,529164,1587493,1812.5094799995422,1.726948539726436e-08
529938,1059877,529938,1589815,1815.1198060512543,1.4084434951655567e-08
530713,1061427,530713,1592140,1817.7612528800964,1.4348188415169716e-08
531488,1062977,531488,1594465,1820.3975791931152,1.5319528756663203e-08
532263,1064527,532263,1596790,1823.0011761188507,1.2674718163907528e-08
533037,1066075,533037,1599112,1825.6003260612488,1.1401425581425428e-08
533812,1067625,533812,1601437,1828.2172422409058,1.3335011317394674e-08
534587,1069175,534587,1603762,1830.812684059143,1.2994860298931599e-08
535362,1070725,535362,1606087,1833.4502520561218,1.0928488336503506e-08
536137,1072275,536137,1608412,1836.050017118454,1.1990778148174286e-08
536911,1073823,536911,1610734,1838.6952772140503,1.3998942449688911e-08
537686,1075373,537686,1613059,1841.3164329528809,1.2860255083069205e-08
538461,1076923,538461,1615384,1843.8796999454498,1.2400050763972104e-08
539236,1078473,539236,1617709,1846.5039989948273,1.5183104551397264e-08
540010,1080021,540010,1620031,1849.0967218875885,1.617263478692621e-08
540785,1081571,540785,1622356,1851.707675933838,1.5104888007044792e-08
541560,1083121,541560,1624681,1854.3018090724945,1.6827470972202718e-08
542335,1084671,542335,1627006,1856.8756680488586,1.9625076674856246e-08
543109,1086219,543109,1629328,1859.474927186966,1.9501385395415127e-08
543884,1087769,543884,1631653,1862.1450719833374,1.9519575289450586e-08
544659,1089319,544659,1633978,1864.8682749271393,2.2519088815897703e-08
545434,1090869,545434,1636303,1867.3329269886017,2.4130713427439332e-08
546208,1092417,546208,1638625,1869.8474650382996,2.337219484616071e-08
546983,1093967,546983,1640950,1872.3513460159302,2.4880137061700225e-08
547758,1095517,547758,1643275,1874.9700429439545,2.7619535103440285e-08
548533,1097067,548533,1645600,1878.882327079773,2.752130967564881e-08
549308,1098617,549308,1647925,1882.7803809642792,2.7137502911500633e-08
550082,1100165,550082,1650247,1886.6666178703308,2.938577381428331e-08
550857,1101715,550857,1652572,1890.550763130188,3.060631570406258e-08
551632,1103265,551632,1654897,1893.8375749588013,2.9340299079194665e-08
552407,1104815,552407,1657222,1896.2952210903168,2.9762304620817304e-08
553181,1106363,553181,1659544,1898.7100820541382,3.1641320674680173e-08
553956,1107913,553956,1661869,1901.125836133957,3.086279320996255e-08
554731,1109463,554731,1664194,1903.5977311134338,2.9476723284460604e-08
555506,1111013,555506,1666519,1906.053871870041,3.0508090276271105e-08
556280,1112561,556280,1668841,1908.5065560340881,3.086279320996255e-08
557055,1114111,557055,1671166,1911.7695271968842,2.878914528992027e-08
557830,1115661,557830,1673491,1914.2046921253204,2.8008798835799098e-08
558605,1117211,558605,1675816,1916.823646068573,2.8827344067394733e-08
559379,1118759,559379,1678138,1919.3593952655792,2.741035132203251e-08
560154,1120309,560154,1680463,1921.7709078788757,2.5091139832511544e-08
560929,1121859,560929,1682788,1924.2025711536407,2.5120243662968278e-08
561704,1123409,561704,1685113,1926.713723897934,2.482920535840094e-08
562478,1124957,562478,1687435,1929.2732381820679,2.224805939476937e-08
563253,1126507,563253,1689760,1931.7388870716095,2.0749212126247585e-08
564028,1128057,564028,1692085,1934.1810839176178,2.0929292077198625e-08
564803,1129607,564803,1694410,1936.6182680130005,1.9379513105377555e-08
565578,1131157,565578,1696735,1939.058188199997,1.676016836427152e-08
566352,1132705,566352,1699057,1941.4793601036072,1.6378180589526892e-08
567127,1134255,567127,1701382,1943.9794130325317,1.611988409422338e-08
567902,1135805,567902,1703707,1946.48965716362,1.3733369996771216e-08
568677,1137355,568677,1706032,1948.9138140678406,1.2236341717652977e-08
569451,1138903,569451,1708354,1951.31134390831,1.257285475730896e-08
570226,1140453,570226,1710679,1953.741827249527,1.1557858670130372e-08
571001,1142003,571001,1713004,1956.191812992096,9.471477824263275e-09
571776,1143553,571776,1715329,1958.6353740692139,9.405994205735624e-09
572550,1145101,572550,1717651,1961.0487968921661,9.871655493043363e-09
573325,1146651,573325,1719976,1963.449203968048,8.394636097364128e-09
574100,1148201,574100,1722301,1965.8597340583801,7.536073098890483e-09
574875,1149751,574875,1724626,1968.283998966217,8.620190783403814e-09
575649,1151299,575649,1726948,1970.7182312011719,8.618371794000268e-09
576424,1152849,576424,1729273,1973.1269581317902,7.523340173065662e-09
577199,1154399,577199,1731598,1975.548122882843,8.172719390131533e-09
577974,1155949,577974,1733923,1977.9588391780853,9.56606527324766e-09
578749,1157499,578749,1736248,1980.3673431873322,9.185896487906575e-09
579523,1159047,579523,1738570,1982.8007941246033,9.07857611309737e-09
580298,1160597,580298,1740895,1985.2608740329742,1.0863004717975855e-08
581073,1162147,581073,1743220,1987.6891419887543,1.178705133497715e-08
581848,1163697,581848,1745545,1990.7133960723877,1.1465090210549533e-08
582622,1165245,582622,1747867,1995.4645781517029,1.2598320608958602e-08
583397,1166795,583397,1750192,1999.495033979416,1.4528268366120756e-08
584172,1168345,584172,1752517,2002.1752951145172,1.4799297787249088e-08
584947,1169895,584947,1754842,2004.8151681423187,1.5006662579253316e-08
585721,1171443,585721,1757164,2007.3204469680786,1.692387741059065e-08
586496,1172993,586496,1759489,2010.041160106659,1.8175342120230198e-08
587271,1174543,587271,1761814,2014.4834079742432,1.7993443179875612e-08
588046,1176093,588046,1764139,2017.2173252105713,1.8975697457790375e-08
588820,1177641,588820,1766461,2019.783716917038,2.0754669094458222e-08
589595,1179191,589595,1768786,2023.641662120819,2.097476681228727e-08
590370,1180741,590370,1771111,2027.4772679805756,2.0838342607021332e-08
591145,1182291,591145,1773436,2032.008952140808,2.2200765670277178e-08
591920,1183841,591920,1775761,2037.5540130138397,2.3097527446225286e-08
592694,1185389,592694,1778083,2040.9094150066376,2.244087227154523e-08
593469,1186939,593469,1780408,2044.3356540203094,2.267006493639201e-08
594244,1188489,594244,1782733,2047.8490362167358,2.373599272686988e-08
595019,1190039,595019,1785058,2051.6053869724274,2.3370375856757164e-08
595793,1191587,595793,1787380,2055.2977979183197,2.2453605197370052e-08
596568,1193137,596568,1789705,2059.280351161957,2.2886524675413966e-08
597343,1194687,597343,1792030,2062.642212867737,2.3039319785311818e-08
598118,1196237,598118,1794355,2066.618895292282,2.1698724594898522e-08
598892,1197785,598892,1796677,2070.5891880989075,2.0985680748708546e-08
599667,1199335,599667,1799002,2074.4344091415405,2.1233063307590783e-08
600442,1200885,600442,1801327,2078.4973871707916,2.0243533072061837e-08
601217,1202435,601217,1803652,2082.51348900795,1.861371856648475e-08
601991,1203983,601991,1805974,2086.575275182724,1.8268110579811037e-08
602766,1205533,602766,1808299,2090.7866151332855,1.7869751900434494e-08
603541,1207083,603541,1810624,2094.952605009079,1.6123522073030472e-08
604316,1208633,604316,1812949,2099.5947201251984,1.4850229490548372e-08
605090,1210181,605090,1815271,2104.438299894333,1.4673787518404424e-08
605865,1211731,605865,1817596,2109.0159361362457,1.3526005204766989e-08
606640,1213281,606640,1819921,2113.443778038025,1.1730662663467228e-08
607415,1214831,607415,1822246,2117.858983039856,1.1161318980157375e-08
608190,1216381,608190,1824571,2122.149496078491,1.0806616046465933e-08
608964,1217929,608964,1826893,2127.372107028961,9.260475053451955e-09
609739,1219479,609739,1829218,2131.9710490703583,8.107235771603882e-09
610514,1221029,610514,1831543,2135.741697072983,8.119968697428703e-09
611289,1222579,611289,1833868,2139.683396100998,7.452399586327374e-09
612063,1224127,612063,1836190,2145.014429092407,6.119080353528261e-09
612838,1225677,612838,1838515,2149.896196126938,5.9371814131736755e-09
613613,1227227,613613,1840840,2154.5180230140686,6.184563972055912e-09
614388,1228777,614388,1843165,2158.842262029648,5.360561772249639e-09
615162,1230325,615162,1845487,2163.491833925247,4.823959898203611e-09
615937,1231875,615937,1847812,2167.8377940654755,5.458787200041115e-09
616712,1233425,616712,1850137,2172.4419322013855,5.618858267553151e-09
617487,1234975,617487,1852462,2176.863035917282,5.0640664994716644e-09
618261,1236523,618261,1854784,2180.904286146164,5.527908797375858e-09
619036,1238073,619036,1857109,2184.732808113098,6.51016307529062e-09
619811,1239623,619811,1859434,2188.580407142639,6.517439032904804e-09
620586,1241173,620586,1861759,2193.7113020420074,6.6211214289069176e-09
621361,1242723,621361,1864084,2197.782562017441,7.82711140345782e-09
622135,1244271,622135,1866406,2201.970932006836,8.671122486703098e-09
622910,1245821,622910,1868731,2206.1604840755463,8.712959242984653e-09
623685,1247371,623685,1871056,2209.9077639579773,9.567884262651205e-09
624460,1248921,624460,1873381,2213.1929869651794,1.0953954188153148e-08
625234,1250469,625234,1875703,2216.910593032837,1.1408701539039612e-08
626009,1252019,626009,1878028,2220.1674501895905,1.173430064227432e-08
626784,1253569,626784,1880353,2223.584347009659,1.3047610991634429e-08
627559,1255119,627559,1882678,2227.5024840831757,1.4046236174181104e-08
628333,1256667,628333,1885000,2231.137754917145,1.4162651496008039e-08
629108,1258217,629108,1887325,2234.3670332431793,1.485568645875901e-08
629883,1259767,629883,1889650,2237.78378200531,1.6072590369731188e-08
630658,1261317,630658,1891975,2242.033210992813,1.638727553654462e-08
631432,1262865,631432,1894297,2245.5069031715393,1.638727553654462e-08
632207,1264415,632207,1896622,2249.0440080165863,1.7236743588000536e-08
632982,1265965,632982,1898947,2252.3779740333557,1.7842467059381306e-08
633757,1267515,633757,1901272,2255.863466978073,1.752414391376078e-08
634532,1269065,634532,1903597,2259.6011340618134,1.7584170564077795e-08
635306,1270613,635306,1905919,2264.205605983734,1.8184437067247927e-08
636081,1272163,636081,1908244,2269.162405014038,1.7949787434190512e-08
636856,1273713,636856,1910569,2274.1514041423798,1.7304046195931733e-08
637631,1275263,637631,1912894,2279.051768064499,1.7394995666109025e-08
638405,1276811,638405,1915216,2283.68141913414,1.7378624761477113e-08
639180,1278361,639180,1917541,2288.231355905533,1.6450940165668726e-08
639955,1279911,639955,1919866,2292.7585532665253,1.5801560948602855e-08
640730,1281461,640730,1922191,2297.2433140277863,1.5736077330075204e-08
641504,1283009,641504,1924513,2301.8853051662445,1.4984834706410766e-08
642279,1284559,642279,1926838,2306.421198129654,1.3791577657684684e-08
643054,1286109,643054,1929163,2310.951793909073,1.3302269508130848e-08
643829,1287659,643829,1931488,2315.4658901691437,1.2865712051279843e-08
644603,1289207,644603,1933810,2319.938945055008,1.161606633104384e-08
645378,1290757,645378,1936135,2324.521651983261,1.0601070243865252e-08
646153,1292307,646153,1938460,2329.0696489810944,1.0240910341963172e-08
646928,1293857,646928,1940785,2333.575016975403,9.391442290507257e-09
647703,1295407,647703,1943110,2338.061334133148,8.107235771603882e-09
648477,1296955,648477,1945432,2342.5641660690308,7.536073098890483e-09
649252,1298505,649252,1947757,2347.12312912941,7.163180271163583e-09
650027,1300055,650027,1950082,2351.6489431858063,6.1154423747211695e-09
650802,1301605,650802,1952407,2356.2831571102142,5.2532413974404335e-09
651576,1303153,651576,1954729,2360.7726900577545,5.133188096806407e-09
652351,1304703,652351,1957054,2365.3584661483765,4.672983777709305e-09
653126,1306253,653126,1959379,2369.856442928314,3.794411895796657e-09
653901,1307803,653901,1961704,2374.3774342536926,3.5943230614066124e-09
654675,1309351,654675,1964026,2378.969983100891,3.7180143408477306e-09
655450,1310901,655450,1966351,2383.44052195549,3.2669049687683582e-09
656225,1312451,656225,1968676,2387.968015909195,2.9303919291123748e-09
657000,1314001,657000,1971001,2392.4547250270844,3.332388587296009e-09
657774,1315549,657774,1973323,2397.0294840335846,3.523382474668324e-09
658549,1317099,658549,1975648,2401.564512014389,3.2905518310144544e-09
659324,1318649,659324,1977973,2406.0657081604004,3.6325218388810754e-09
660099,1320199,660099,1980298,2410.523325920105,4.349203663878143e-09
660873,1321747,660873,1982620,2414.977280139923,4.529283614829183e-09
661648,1323297,661648,1984945,2419.4757981300354,4.723915481008589e-09
662423,1324847,662423,1987270,2424.0137300491333,5.589754437096417e-09
663198,1326397,663198,1989595,2428.528783082962,6.295522325672209e-09
663973,1327947,663973,1991920,2433.0068459510803,6.51925802230835e-09
664747,1329495,664747,1994242,2437.478741168976,7.172275218181312e-09
665522,1331045,665522,1996567,2442.0443000793457,8.19636625237763e-09
666297,1332595,666297,1998892,2446.6600770950317,8.680217433720827e-09
667072,1334145,667072,2001217,2451.125673055649,9.044015314429998e-09
667846,1335693,667846,2003539,2455.6436760425568,9.968061931431293e-09
668621,1337243,668621,2005864,2460.238617181778,1.075568434316665e-08
669396,1338793,669396,2008189,2464.7532732486725,1.0988514986820519e-08
670171,1340343,670171,2010514,2469.2570979595184,1.150146999862045e-08
670945,1341891,670945,2012836,2473.716975212097,1.2343662092462182e-08
671720,1343441,671720,2015161,2478.2208211421967,1.2658347259275615e-08
672495,1344991,672495,2017486,2482.821130990982,1.2729287846013904e-08
673270,1346541,673270,2019811,2487.2805840969086,1.3258613762445748e-08
674044,1348089,674044,2022133,2491.7528860569,1.3682438293471932e-08
674819,1349639,674819,2024458,2496.242030143738,1.3511453289538622e-08
675594,1351189,675594,2026783,2500.749503135681,1.3511453289538622e-08
676369,1352739,676369,2029108,2505.3138670921326,1.3822500477544963e-08
677144,1354289,677144,2031433,2509.7925980091095,1.3662429410032928e-08
677918,1355837,677918,2033755,2514.2710399627686,1.3182216207496822e-08
678693,1357387,678693,2036080,2518.8136808872223,1.3116732588969171e-08
679468,1358937,679468,2038405,2523.395586013794,1.3002136256545782e-08
680243,1360487,680243,2040730,2527.869104862213,1.2332748156040907e-08
681017,1362035,681017,2043052,2532.3399629592896,1.1768861440941691e-08
681792,1363585,681792,2045377,2536.9233610630035,1.155422069132328e-08
682567,1365135,682567,2047702,2541.458778142929,1.0959411156363785e-08
683342,1366685,683342,2050027,2545.990532875061,1.0051735443994403e-08
684116,1368233,684116,2052349,2550.480310201645,9.5478753792122e-09
684891,1369783,684891,2054674,2554.9797582626343,9.098584996536374e-09
685666,1371333,685666,2056999,2559.524477005005,8.179995347745717e-09
686441,1372883,686441,2059324,2564.096251010895,7.346898200921714e-09
687215,1374431,687215,2061646,2568.6158430576324,6.933987606316805e-09
687990,1375981,687990,2063971,2573.028463125229,6.260961527004838e-09
688765,1377531,688765,2066296,2577.5476381778717,5.318725015968084e-09
689540,1379081,689540,2068621,2582.227005004883,4.782123141922057e-09
690315,1380631,690315,2070946,2586.7615439891815,4.420144250616431e-09
691089,1382179,691089,2073268,2591.2595660686493,3.677996573969722e-09
691864,1383729,691864,2075593,2595.798727989197,3.0249793780967593e-09
692639,1385279,692639,2077918,2600.358561038971,2.837623469531536e-09
693414,1386829,693414,2080243,2604.8640661239624,2.508386387489736e-09
694188,1388377,694188,2082565,2609.366068124771,1.940861693583429e-09
694963,1389927,694963,2084890,2613.87481713295,1.762600732035935e-09
695738,1391477,695738,2087215,2618.380690097809,1.8408172763884068e-09
696513,1393027,696513,2089540,2622.923243999481,1.6025296645238996e-09
697287,1394575,697287,2091862,2627.4600059986115,1.4279066817834973e-09
698062,1396125,698062,2094187,2631.9108521938324,1.7080310499295592e-09
698837,1397675,698837,2096512,2636.380527973175,1.926309778355062e-09
699612,1399225,699612,2098837,2640.8936409950256,1.889929990284145e-09
700386,1400773,700386,2101159,2645.3792049884796,2.1864252630621195e-09
701161,1402323,701161,2103484,2649.8582870960236,2.752130967564881e-09
701936,1403873,701936,2105809,2654.4187021255493,3.0213413992896676e-09
702711,1405423,702711,2108134,2658.9517719745636,3.2796378945931792e-09
703485,1406971,703485,2110456,2663.470216989517,3.938112058676779e-09
704260,1408521,704260,2112781,2667.958894252777,4.549292498268187e-09
705035,1410071,705035,2115106,2672.455075263977,4.858520696870983e-09
705810,1411621,705810,2117431,2677.103073120117,5.40421751793474e-09
706585,1413171,706585,2119756,2681.6738471984863,6.1791070038452744e-09
707359,1414719,707359,2122078,2686.2554030418396,6.655682227574289e-09
708134,1416269,708134,2124403,2690.8453080654144,7.0158421294763684e-09
708909,1417819,708909,2126728,2695.389216184616,7.703420124016702e-09
709684,1419369,709684,2129053,2699.956083059311,8.32369551062584e-09
710458,1420917,710458,2131375,2704.4268250465393,8.594724931754172e-09
711233,1422467,711233,2133700,2708.9351711273193,8.989445632323623e-09
712008,1424017,712008,2136025,2713.4558169841766,9.582436177879572e-09
712783,1425567,712783,2138350,2717.9750809669495,9.862560546025634e-09
713557,1427115,713557,2140672,2722.555022239685,9.948053047992289e-09
714332,1428665,714332,2142997,2727.023542165756,1.0288204066455364e-08
715107,1430215,715107,2145322,2731.5582370758057,1.0562871466390789e-08
715882,1431765,715882,2147647,2736.0620832443237,1.047010300680995e-08
716656,1433313,716656,2149969,2740.59742808342,1.0422809282317758e-08
717431,1434863,717431,2152294,2745.095188140869,1.0561052476987243e-08
718206,1436413,718206,2154619,2749.6640362739563,1.0410076356492937e-08
718981,1437963,718981,2156944,2754.1477591991425,1.003536453936249e-08
719756,1439513,719756,2159269,2758.6513962745667,9.877112461254e-09
720530,1441061,720530,2161591,2763.240662097931,9.704308467917144e-09
721305,1442611,721305,2163916,2767.7522649765015,9.182258509099483e-09
722080,1444161,722080,2166241,2772.2757132053375,8.682036423124373e-09
722855,1445711,722855,2168566,2776.8132400512695,8.39827407617122e-09
723629,1447259,723629,2170888,2781.342038154602,7.896233000792563e-09
724404,1448809,724404,2173213,2785.852485895157,7.183189154602587e-09
725179,1450359,725179,2175538,2790.368443965912,6.693881005048752e-09
725954,1451909,725954,2177863,2794.917077064514,6.26459950581193e-09
726728,1453457,726728,2180185,2799.367926120758,5.555193638429046e-09
727503,1455007,727503,2182510,2803.9016740322113,4.880348569713533e-09
728278,1456557,728278,2184835,2808.4169640541077,4.461981006897986e-09
729053,1458107,729053,2187160,2812.9658608436584,3.927198122255504e-09
729827,1459655,729827,2189482,2817.472995042801,3.219611244276166e-09
730602,1461205,730602,2191807,2821.968369960785,2.7539499569684267e-09
731377,1462755,731377,2194132,2826.4886910915375,2.4283508537337184e-09
732152,1464305,732152,2196457,2831.036728143692,1.8953869584947824e-09
732927,1465855,732927,2198782,2835.620947122574,1.407897798344493e-09
733701,1467403,733701,2201104,2840.1132550239563,1.216903910972178e-09
734476,1468953,734476,2203429,2844.692458152771,9.840732673183084e-10
735251,1470503,735251,2205754,2849.2079181671143,6.093614501878619e-10
736026,1472053,736026,2208079,2853.70321893692,4.747562343254685e-10
736800,1473601,736800,2210401,2858.1508009433746,5.238689482212067e-10
737575,1475151,737575,2212726,2862.7185311317444,4.147295840084553e-10
738350,1476701,738350,2215051,2867.2629430294037,3.3287506084889174e-10
739125,1478251,739125,2217376,2871.7518990039825,5.475158104673028e-10
739899,1479799,739899,2219698,2876.38503408432,7.548806024715304e-10
740674,1481349,740674,2222023,2880.9075951576233,8.203642209991813e-10
741449,1482899,741449,2224348,2885.4713549613953,1.0822986951097846e-09
742224,1484449,742224,2226673,2890.02325296402,1.5261321095749736e-09
742998,1485997,742998,2228995,2894.5820429325104,1.8189894035458565e-09
743773,1487547,743773,2231320,2899.1100239753723,2.0881998352706432e-09
744548,1489097,744548,2233645,2903.586959838867,2.610249794088304e-09
745323,1490647,745323,2235970,2908.084860086441,3.1213858164846897e-09
746098,1492197,746098,2238295,2912.569230079651,3.4524418879300356e-09
746872,1493745,746872,2240617,2917.0358250141144,3.901732270605862e-09
747647,1495295,747647,2242942,2921.5453090667725,4.507455741986632e-09
748422,1496845,748422,2245267,2926.075931072235,4.933099262416363e-09
749197,1498395,749197,2247592,2930.5744829177856,5.275069270282984e-09
749971,1499943,749971,2249914,2935.0724959373474,5.791662260890007e-09
750746,1501493,750746,2252239,2939.541831970215,6.282789399847388e-09
751521,1503043,751521,2254564,2944.0434839725494,6.548361852765083e-09
752296,1504593,752296,2256889,2948.535675048828,6.859409040771425e-09
753070,1506141,753070,2259211,2953.017170906067,7.285052561201155e-09
753845,1507691,753845,2261536,2957.4882559776306,7.516064215451479e-09
754620,1509241,754620,2263861,2961.9684591293335,7.605194696225226e-09
755395,1510791,755395,2266186,2966.5554740428925,7.818016456440091e-09
756169,1512339,756169,2268508,2971.1176199913025,7.999915396794677e-09
756944,1513889,756944,2270833,2975.60573387146,7.93261278886348e-09
757719,1515439,757719,2273158,2980.1211149692535,7.86712917033583e-09
758494,1516989,758494,2275483,2984.728908061981,7.899870979599655e-09
759268,1518537,759268,2277805,2989.237370967865,7.763446774333715e-09
760043,1520087,760043,2280130,2993.6680541038513,7.456037565134466e-09
760818,1521637,760818,2282455,2998.1523790359497,7.263224688358605e-09
761593,1523187,761593,2284780,3002.6383199691772,7.057678885757923e-09
762368,1524737,762368,2287105,3007.162068128586,6.6356733441352844e-09
763142,1526285,763142,2289427,3011.6413702964783,6.2045728554949164e-09
763917,1527835,763917,2291752,3016.1111590862274,5.895344656892121e-09
764692,1529385,764692,2294077,3020.6602811813354,5.4678821470588446e-09
765467,1530935,765467,2296402,3025.125888109207,4.893081495538354e-09
766241,1532483,766241,2298724,3029.6471519470215,4.443791112862527e-09
767016,1534033,767016,2301049,3034.351683139801,4.043613444082439e-09
767791,1535583,767791,2303374,3038.9575419425964,3.4797267289832234e-09
768566,1537133,768566,2305699,3043.5254039764404,2.9249349609017372e-09
769340,1538681,769340,2308021,3048.0572440624237,2.5374902179464698e-09
770115,1540231,770115,2310346,3052.5682549476624,2.091837814077735e-09
770890,1541781,770890,2312671,3057.067466020584,1.5497789718210697e-09
771665,1543331,771665,2314996,3061.5271339416504,1.1514202924445271e-09
772439,1544879,772439,2317318,3066.069405078888,8.62200977280736e-10
773214,1546429,773214,2319643,3070.6150500774384,4.656612873077393e-10
773989,1547979,773989,2321968,3075.100857257843,9.822542779147625e-11


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0024199485778808594,12064.682476916567
2002,2003,2002,4005,5.172716856002808,60.659557687866254
4004,4005,4004,8009,10.17728304862976,40.01013285976478
6006,6007,6006,12013,15.386091947555542,32.122823954647174
8008,8009,8008,16017,20.587572813034058,27.232249265985956
10010,10011,10010,20021,25.848038911819458,23.709264738188722
12012,12013,12012,24025,30.755960702896118,20.97624637750596
14014,14015,14014,28029,35.772347927093506,18.762942711508003
16016,16017,16016,32033,40.77490568161011,16.921908606920624
18018,18019,18018,36037,45.719876766204834,15.3630753883117
20020,20021,20020,40041,50.87304377555847,14.026422174050822
22022,22023,22022,44045,55.86635184288025,12.869279116112011
24024,24025,24024,48049,60.838228940963745,11.859884815996338
26026,26027,26026,52053,65.72886991500854,10.973807613236204
28028,28029,28028,56057,70.45732498168945,10.191772110585589
30030,30031,30030,60061,75.28628993034363,9.49831038087541
32032,32033,32032,64065,80.07366991043091,8.880821937249493
34034,34035,34034,68069,84.80838084220886,8.32891496922457
36036,36037,36036,72073,89.51976585388184,7.833935179643959
38038,38039,38038,76077,94.2336368560791,7.388610457366667
40040,40041,40040,80081,98.95079493522644,6.986782983762168
42042,42043,42042,84085,103.68086981773376,6.62320315895704
44044,44045,44044,88089,108.36869883537292,6.29336894071821
46046,46047,46046,92093,113.09729790687561,5.993399070212035
48048,48049,48048,96097,117.77982783317566,5.7199319244773505
50050,50051,50050,100101,122.51098275184631,5.470043981698836
52052,52053,52052,104105,127.17121362686157,5.241183463827838
54054,54055,54054,108109,131.89265203475952,5.031115848094487
56056,56057,56056,112113,136.58025193214417,4.837878754167832
58058,58059,58058,116117,141.3129117488861,4.659744309799862
60060,60061,60060,120121,146.00278973579407,4.495187537451784
62062,62063,62062,124125,150.69809579849243,4.342859631875399
64064,64065,64064,128129,155.48066091537476,4.201565244247831
66066,66067,66066,132133,160.13977909088135,4.0702430743695
68068,68069,68068,136137,164.84128093719482,3.947949214345499
70070,70071,70070,140141,169.5170590877533,3.83384279620077
72072,72073,72072,144145,174.28276681900024,3.7271735806662036
74074,74075,74074,148149,178.9806158542633,3.6272721958848706
76076,76077,76076,152153,183.6696548461914,3.53353834322661
78078,78079,78078,156157,188.4683277606964,3.445433793713164
80080,80081,80080,160161,193.34247875213623,3.3624761818246043
82082,82083,82082,164165,198.04426169395447,3.2842320765794284
84084,84085,84084,168169,202.82017874717712,3.210311494196503
86086,86087,86086,172173,207.5563247203827,3.140363075232017
88088,88089,88088,176177,212.2366750240326,3.074069839265576
90090,90091,90090,180181,217.0563566684723,3.011145442724228
92092,92093,92092,184185,221.77789902687073,2.9513308758487256
94094,94095,94094,188189,226.48492789268494,2.8943915437066607
96096,96097,96096,192193,231.19119477272034,2.840114683553111
98098,98099,98098,196197,235.92206001281738,2.7883070772695646
100100,100101,100100,200201,240.61104893684387,2.738793022943355
102102,102103,102102,204205,245.34230089187622,2.691412534448318
104104,104105,104104,208209,250.0317039489746,2.646019741678174
106106,106107,106106,212213,254.81864285469055,2.602481467751204
108108,108109,108108,216217,259.56136870384216,2.5606759623242397
110110,110111,110110,220221,264.31130599975586,2.5204917728224245
112112,112113,112112,224225,268.9788227081299,2.4818267375703726
114114,114115,114114,228229,273.68713784217834,2.444587086867614
116116,116117,116116,232233,278.36722683906555,2.408686639580992
118118,118119,118118,236237,283.12001299858093,2.3740460844965128
120120,120121,120120,240241,288.0113537311554,2.3405923368300137
122122,122123,122122,244245,292.8991389274597,2.3082579615002032
124124,124125,124124,248249,297.59548687934875,2.276980655711668
126126,126127,126126,252253,302.31019496917725,2.2467027843285905
128128,128129,128128,256257,307.0411629676819,2.2173709622347815
130130,130131,130130,260261,312.0076367855072,2.188935678534108
132132,132133,132132,264265,316.931129693985,2.161351008073325
134134,134135,134134,268269,321.87547278404236,2.1345742730918573
136136,136137,136136,272273,326.830689907074,2.1085655631977716
138138,138139,138138,276277,331.78523993492126,2.083287795738215
140140,140141,140140,280281,336.43759274482727,2.0587063696129917
142142,142143,142142,284285,340.9312376976013,2.034788961527738
144144,144145,144144,288289,345.38750100135803,2.0115053414428985
146146,146147,146146,292293,349.8347098827362,1.9888272051666718
148148,148149,148148,296297,354.3421368598938,1.9667280223657144
150150,150151,150150,300301,358.7761697769165,1.9451828983583255
152152,152153,152152,304305,363.3234508037567,1.9241684484150028
154154,154155,154154,308309,367.81097984313965,1.9036626832057664
156156,156157,156156,312313,372.3192718029022,1.8836449043810717
158158,158159,158158,316317,376.8059628009796,1.864095609249489
160160,160161,160160,320321,381.2854928970337,1.8449964036772144
162162,162163,162162,324325,385.79009985923767,1.8263299224126968
164164,164165,164164,328329,390.32827496528625,1.8080797561506188
166166,166167,166166,332333,394.7906799316406,1.79023038466039
168168,168169,168168,336337,399.2742488384247,1.772767115448005
170170,170171,170170,340341,404.05829882621765,1.7556760274110275
172172,172173,172172,344345,408.5186779499054,1.7389439190428675
174174,174175,174174,348349,412.9988007545471,1.7225583894924057
176176,176177,176176,352353,417.39266777038574,1.7065075560640253
178178,178179,178178,356357,421.96313977241516,1.6907799361633806
180180,180181,180180,360361,426.44036197662354,1.6753647669811471
182182,182183,182182,364365,430.8607428073883,1.6602518012787186
184184,184185,184184,368369,435.3015558719635,1.6454312754412967
186186,186187,186186,372373,439.8396170139313,1.6308938799375028
188188,188189,188188,376377,444.3333878517151,1.6166307319199404
190190,190191,190190,380381,448.76127195358276,1.6026333498321037
192192,192193,192192,384385,453.39943385124207,1.5888936298288172
194194,194195,194194,388389,457.9937627315521,1.5754038238846988
196196,196197,196196,392393,462.41339087486267,1.5621565194142022
198198,198199,198198,396397,466.8201730251312,1.5491446203395753
200200,200201,200200,400401,471.5895879268646,1.5363613294102834
202202,202203,202202,404405,476.2631359100342,1.5238001317684393
204204,204205,204204,408409,480.7883110046387,1.5114547795783437
206206,206207,206206,412413,485.38422989845276,1.499319277701943
208208,208209,208208,416417,490.39082980155945,1.4873878702819638
210210,210211,210210,420421,495.035826921463,1.4756550282218086
212212,212213,212212,424425,499.61464500427246,1.4641154374512553
214214,214215,214214,428429,504.4472498893738,1.4527639879343042
216216,216217,216216,432433,509.4147448539734,1.441595763377336
218218,218219,218218,436437,514.4516479969025,1.430606031555726
220220,220221,220220,440441,519.4096279144287,1.4197902352516394
222222,222223,222222,444445,524.3104927539825,1.40914398372297
224224,224225,224224,448449,529.0412929058075,1.3986630447034258
226226,226227,226226,452453,533.7500488758087,1.3883433368464466
228228,228229,228228,456457,538.409138917923,1.3781809226420592
230230,230231,230230,460461,543.0932638645172,1.3681720017357293
232232,232233,232232,464465,547.7499897480011,1.3583129046128306
234234,234235,234234,468469,552.4804139137268,1.3486000866632821
236236,236237,236236,472473,557.181765794754,1.3390301225754229
238238,238239,238238,476477,561.8875119686127,1.3295997010263818
240240,240241,240240,480481,566.5442008972168,1.320305619681676
242242,242243,242242,484485,571.1893849372864,1.3111447804585623
244244,244245,244244,488489,575.8557648658752,1.3021141850495042
246246,246247,246246,492493,580.5159428119659,1.2932109306748316
248248,248249,248248,496497,585.1758139133453,1.2844322060682316
250250,250251,250250,500501,589.8485717773438,1.2757752876696031
252252,252253,252252,504505,594.5028438568115,1.2672375360161823
254254,254255,254254,508509,599.1448707580566,1.2588163923082902
256256,256257,256256,512513,603.8060920238495,1.2505093751697132
258258,258259,258258,516517,608.6617708206177,1.2423140775463253
260260,260261,260260,520521,613.5248649120331,1.234228163773878
262262,262263,262262,524525,618.1910746097565,1.2262493667949457
264264,264265,264264,528529,622.8730418682098,1.2183754854941071
266266,266267,266266,532533,627.6471128463745,1.2106043821695494
268268,268269,268268,536537,632.3013107776642,1.202934153698152
270270,270271,270270,540541,637.0600759983063,1.1953626175982208
272272,272273,272272,544545,641.7243218421936,1.1878878010356857
274274,274275,274274,548549,646.3962647914886,1.1805077970748243
276276,276277,276276,552553,651.1146759986877,1.173220751243207
278278,278279,278278,556557,655.7257947921753,1.16602485963449
280280,280281,280280,560561,660.3696568012238,1.1589183670912462
282282,282283,282282,564565,665.0342099666595,1.151899565489657
284284,284285,284284,568569,669.6538558006287,1.1449667920660431
286286,286287,286286,572573,674.3150749206543,1.1381184278561705
288288,288289,288288,576577,678.9854609966278,1.131352896165481
290290,290291,290290,580581,683.7026789188385,1.124668661135729
292292,292293,292292,584585,688.3547866344452,1.1180642263516347
294294,294295,294294,588589,693.0857207775116,1.1115381335239363
296296,296297,296296,592593,697.753476858139,1.1050889612033643
298298,298299,298298,596597,702.6349680423737,1.0987153235892038
300300,300301,300300,600601,707.378616809845,1.092415869328761
302302,302303,302302,604605,712.0587389469147,1.0861892804277886
304304,304305,304304,608609,716.7120356559753,1.0800342711645499
306306,306307,306306,612613,721.4807198047638,1.0739495870548126
308308,308309,308308,616617,726.1133780479431,1.0679340038659575
310310,310311,310310,620621,730.7672169208527,1.0619863266729226
312312,312313,312312,624625,735.4493837356567,1.0561053889396135
314314,314315,314314,628629,740.1438248157501,1.0502900516348745
316316,316317,316316,632633,744.8246319293976,1.0445392024066678
318318,318319,318318,636637,749.7022426128387,1.0388517547507945
320320,320321,320320,640641,754.4954669475555,1.033226647243282
322322,322323,322322,644645,759.1546258926392,1.027662842783684
324324,324325,324324,648649,763.8460879325867,1.0221593278838554
326326,326327,326326,652653,768.516863822937,1.016715111945814
328328,328329,328328,656657,773.332879781723,1.0113292266214557
330330,330331,330330,660661,778.0000047683716,1.006000725141348
332332,332333,332332,664665,782.6441359519958,1.0007286817126442
334334,334335,334334,668669,787.2837629318237,0.9955121909024456
336336,336337,336336,672673,791.9317367076874,0.9903503670720966
338338,338339,338338,676677,796.5961027145386,0.9852423438060214
340340,340341,340340,680681,801.30402302742,0.9801872733787604
342342,342343,342342,684685,805.9291026592255,0.9751843262420152
344344,344345,344344,688689,810.8498198986053,0.9702326905080554
346346,346347,346346,692693,815.6836709976196,0.9653315714858763
348348,348349,348348,696697,820.3886368274689,0.9604801911827963
350350,350351,350350,700701,825.0294208526611,0.9556777878806315
352352,352353,352352,704705,829.7076318264008,0.9509236156845873
354354,354355,354354,708709,834.4448037147522,0.946216944103071
356356,356357,356356,712713,839.1285088062286,0.9415570576402388
358358,358359,358358,716717,843.7914397716522,0.9369432553939987
360360,360361,360360,720721,848.4395010471344,0.932374850688575
362362,362363,362362,724725,853.0795028209686,0.9278511706888821
364364,364365,364364,728729,857.7003738880157,0.9233715560549172
366366,366367,366366,732733,862.4178128242493,0.9189353605834185
368368,368369,368368,736737,867.1766629219055,0.914541950884086
370370,370371,370370,740741,871.984885931015,0.9101907060467056
372372,372373,372372,744745,876.6599538326263,0.9058810173319216
374374,374375,374374,748749,881.3133890628815,0.9016122878601891
376376,376377,376376,752753,886.0971558094025,0.8973839323189168
378378,378379,378378,756757,890.75221991539,0.8931953766841616
380380,380381,380380,760761,895.4906878471375,0.8890460579259525
382382,382383,382382,764765,900.1400289535522,0.8849354237590887
384384,384385,384384,768769,904.796868801117,0.8808629323648347
386386,386387,386386,772773,909.4653129577637,0.8768280521453562
388388,388389,388388,776777,914.0924398899078,0.8728302614854329
390390,390391,390390,780781,918.744414806366,0.8688690484923427
392392,392393,392392,784785,923.438071012497,0.8649439107939543
394394,394395,394394,788789,928.2786726951599,0.8610543552840682
396396,396397,396396,792793,933.0997738838196,0.857199897931423
398398,398399,398398,796797,937.7471768856049,0.8533800635486841
400400,400401,400400,800801,942.4403088092804,0.8495943855905352
402402,402403,402402,804805,947.1006078720093,0.845842405960866
404404,404405,404404,808809,951.9225389957428,0.842123674821778
406406,406407,406406,812813,956.570506811142,0.8384377503807627
408408,408409,408408,816817,961.2389848232269,0.834784198736088
410410,410411,410410,820821,965.8648838996887,0.8311625936839846
412412,412413,412412,824825,970.5104019641876,0.8275725165476615
414414,414415,414414,828829,975.2861549854279,0.8240135560081399
416416,416417,416416,832833,979.9538547992706,0.8204853079405439
418418,418419,418418,836837,984.6948857307434,0.8169873752631247
420420,420421,420420,840841,989.3410978317261,0.8135193677608186
422422,422423,422422,844845,994.0158467292786,0.8100809019579174
424424,424425,424424,848849,998.6874878406525,0.8066716009598167
426426,426427,426426,852853,1003.3254647254944,0.8032910943129536
428428,428429,428428,856857,1008.1348979473114,0.7999390178556496
430430,430431,430430,860861,1012.9378659725189,0.796615013599876
432432,432433,432432,864865,1017.6105048656464,0.7933187295839161
434434,434435,434434,868869,1022.4016849994659,0.790049819761407
436436,436437,436436,872873,1027.037977695465,0.7868079438521818
438438,438439,438438,876877,1031.8803668022156,0.7835927672422258
440440,440441,440440,880881,1036.5449159145355,0.7804039608508901
442442,442443,442442,884885,1041.2361946105957,0.7772412010272092
444444,444445,444444,888889,1045.9294548034668,0.7741041694280284
446446,446447,446446,892893,1050.5844888687134,0.7709925529015891
448448,448449,448448,896897,1055.2781088352203,0.7679060434020357
450450,450451,450450,900901,1059.91947889328,0.7648443378657248
452452,452453,452452,904905,1064.596291065216,0.7618071381148184
454454,454455,454454,908909,1069.2512118816376,0.7587941507681535
456456,456457,456456,912913,1073.9104309082031,0.755805087123008
458458,458459,458458,916917,1078.573865890503,0.7528396630841598
460460,460461,460460,920921,1083.2425520420074,0.7498975990456529
462462,462463,462462,924925,1087.9283850193024,0.7469786198362272
464464,464465,464464,928929,1092.591373682022,0.7440824545919895
466466,466467,466466,932933,1097.2412610054016,0.7412088367036631
468468,468469,468468,936937,1101.9237208366394,0.7383575037074479
470470,470471,470470,940941,1106.5770030021667,0.735528197230451
472472,472473,472472,944945,1111.2213706970215,0.7327206628760905
474474,474475,474474,948949,1115.8924448490143,0.7299346501913533
476476,476477,476476,952953,1120.5632548332214,0.7271699125376472
478478,478479,478478,956957,1125.2131807804108,0.7244262070726109
480480,480481,480480,960961,1129.8408498764038,0.7217032946264226
482482,482483,482482,964965,1134.517068862915,0.7190009396708774
484484,484485,484484,968969,1139.1597917079926,0.7163189102266188
486486,486487,486486,972973,1143.8224868774414,0.7136569778031117
488488,488489,488488,976977,1148.5849027633667,0.7110149173386162
490490,490491,490490,980981,1153.49329996109,0.708392507125609
492492,492493,492492,984985,1158.108981847763,0.7057895739853848
494494,494495,494494,988989,1162.795738697052,0.7032058642289485
496496,496497,496496,992993,1167.444524049759,0.7006411587281036
498498,498499,498498,996997,1172.0982949733734,0.698095248597383
500501,500502,500501,1001003,1176.8449668884277,0.6955666702251619
502503,502504,502503,1005007,1181.5380418300629,0.6930577454986633
504505,504506,504505,1009011,1186.223639011383,0.6905670075175294
506507,506508,506507,1013015,1190.8903639316559,0.6880942593106738
508509,508510,508509,1017019,1195.540267944336,0.6856393067355384
510511,510512,510511,1021023,1200.3979749679565,0.683201958438076
512513,512514,512513,1025027,1205.1801946163177,0.6807820258145512
514515,514516,514515,1029031,1210.0953719615936,0.6783793229406001
516517,516518,516517,1033035,1214.8797647953033,0.6759936665384885
518519,518520,518519,1037039,1219.5170948505402,0.6736248759243608
520521,520522,520521,1041043,1224.222039937973,0.6712727729627659
522523,522524,522523,1045047,1228.9095387458801,0.6689371820211818
524525,524526,524525,1049051,1233.6153600215912,0.6666179299318173
526527,526528,526527,1053055,1238.3745830059052,0.6643148459388613
528529,528530,528529,1057059,1243.0673768520355,0.6620277616566455
530531,530532,530531,1061063,1247.7044270038605,0.6597567888566118
532533,532534,532533,1065067,1252.3975937366486,0.6575017478335212
534535,534536,534535,1069071,1257.0911569595337,0.6552622127728682
536537,536538,536537,1073075,1261.9705348014832,0.6530380238073121
538539,538540,538539,1077079,1267.1222758293152,0.6508290235015011
540541,540542,540541,1081083,1272.0703349113464,0.6486350567247428
542543,542544,542543,1085087,1276.818282842636,0.6464559705345891
544545,544546,544545,1089091,1281.4993579387665,0.6442916140949819
546547,546548,546547,1093095,1286.2461559772491,0.6421418386398727
548549,548550,548549,1097099,1290.940016746521,0.6400064974113775
550551,550552,550551,1101103,1295.6373329162598,0.6378854456324916
552553,552554,552553,1105107,1300.290991783142,0.6357785697509826
554555,554556,554555,1109111,1304.9719789028168,0.6336861877607589
556557,556558,556557,1113115,1309.6656110286713,0.6316076709699701
558559,558560,558559,1117119,1314.3618278503418,0.6295428808189172
560561,560562,560561,1121123,1319.0469329357147,0.6274916813799791
562563,562564,562563,1125127,1323.728938817978,0.6254539388355624
564565,564566,564565,1129131,1328.3751428127289,0.6234295212234429
566567,566568,566567,1133135,1333.036367893219,0.6214182983621868
568569,568570,568569,1137139,1337.669065952301,0.6194201417802105
570571,570572,570571,1141143,1342.4198677539825,0.6174349246757629
572573,572574,572573,1145147,1347.0880329608917,0.6154625218860019
574575,574576,574575,1149151,1351.8378999233246,0.6135028098597104
576577,576578,576577,1153155,1356.5417199134827,0.6115556666281918
578579,578580,578579,1157159,1361.2214078903198,0.6096209717816237
580581,580582,580581,1161163,1365.8840289115906,0.6076986064508674
582583,582584,582583,1165167,1370.5450019836426,0.6057884532638127
584585,584586,584585,1169171,1375.193205833435,0.6038903963417397
586587,586588,586587,1173175,1379.8531308174133,0.6020043212629389
588589,588590,588589,1177179,1384.504109621048,0.6001301150427025
590591,590592,590591,1181183,1389.1815128326416,0.5982676661205915
592593,592594,592593,1185187,1393.8724510669708,0.5964168643240555
594595,594596,594595,1189191,1398.5260426998138,0.5945776008466055
596597,596598,596597,1193195,1403.2093107700348,0.5927497682459943
598599,598600,598599,1197199,1407.9872777462006,0.5909332603969233
600601,600602,600601,1201203,1412.6532537937164,0.5891279831848806
602603,602604,602603,1205207,1417.3133277893066,0.5873338292240078
604605,604606,604605,1209211,1421.956414937973,0.5855506895659346
606607,606608,606607,1213215,1426.6389486789703,0.5837784631821705
608609,608610,608609,1217219,1431.4347069263458,0.582017050275681
610611,610612,610611,1221223,1436.2134518623352,0.5802663522626972
612613,612614,612613,1225227,1440.8628509044647,0.5785262717581645
614615,614616,614615,1229231,1445.5614190101624,0.5767967125484574
616617,616618,616617,1233235,1450.2625379562378,0.5750775795841037
618619,618620,618619,1237239,1454.925316810608,0.5733687789579562
620621,620622,620621,1241243,1459.6795568466187,0.5716702178797277
622623,622624,622623,1245247,1464.3710038661957,0.5699818046796281
624625,624626,624625,1249251,1469.0291018486023,0.5683034487665282
626627,626628,626627,1253255,1473.7424638271332,0.5666350606315973
628629,628630,628629,1257259,1478.3872158527374,0.5649765518264758
630631,630632,630631,1261263,1483.096650838852,0.5633278349378088
632633,632634,632633,1265267,1487.7696540355682,0.5616888235854276
634635,634636,634635,1269271,1492.4245097637177,0.5600594324041595
636637,636638,636637,1273275,1497.090539932251,0.5584395770201809
638639,638640,638639,1277279,1501.7714607715607,0.5568291740546556
640641,640642,640641,1281283,1506.4445617198944,0.5552281410818978
642643,642644,642643,1285287,1511.1164238452911,0.553636396640286
644645,644646,644645,1289291,1515.782450914383,0.5520538602140732
646647,646648,646647,1293295,1520.4314849376678,0.5504804522024642
648649,648650,648649,1297299,1525.1435968875885,0.5489160939305293
650651,650652,650651,1301303,1529.9334697723389,0.5473607076146436
652653,652654,652653,1305307,1534.8150808811188,0.545814216369763
654655,654656,654655,1309311,1539.4454357624054,0.5442765441748634
656657,656658,656657,1313315,1544.132019996643,0.5427476158838545
658659,658660,658659,1317319,1548.824623823166,0.5412273571910191
660661,660662,660661,1321323,1553.6997587680817,0.5397156946346513
662663,662664,662663,1325327,1558.510776758194,0.5382125555788662
664665,664666,664665,1329331,1563.178645849228,0.5367178682045051
666667,666668,666667,1333335,1567.9506497383118,0.5352315614945837
668669,668670,668669,1337339,1572.9449808597565,0.5337535652251972
670671,670672,670671,1341343,1577.8541827201843,0.5322838099527871
672673,672674,672673,1345347,1582.601542711258,0.5308222270068654
674675,674676,674675,1349351,1587.4177577495575,0.5293687484791008
676677,676678,676677,1353355,1592.193060874939,0.5279233072033094
678679,678680,678679,1357359,1596.8944878578186,0.5264858367572742
680681,680682,680681,1361363,1601.5978360176086,0.525056271450012
682683,682684,682683,1365367,1606.2842197418213,0.5236345463054022
684685,684686,684685,1369371,1610.9681327342987,0.5222205970585492
686687,686688,686687,1373375,1615.6838908195496,0.5208143601466872
688689,688690,688689,1377379,1620.326239824295,0.5194157726909907
690691,690692,690691,1381383,1625.0662457942963,0.5180247724965739
692693,692694,692693,1385387,1629.7469367980957,0.5166412980433961
694695,694696,694695,1389391,1634.4088797569275,0.5152652884717099
696697,696698,696697,1393395,1639.1387848854065,0.5138966835693282
698699,698700,698699,1397399,1644.081367969513,0.5125354237807187
700701,700702,700701,1401403,1648.8433117866516,0.5111814501742629
702703,702704,702703,1405407,1653.5139698982239,0.5098347044568072
704705,704706,704705,1409411,1658.2185699939728,0.5084951289445598
706707,706708,706707,1413415,1662.9036538600922,0.5071626665776421
708709,708710,708709,1417419,1667.5488197803497,0.5058372608873469
710711,710712,710711,1421423,1672.2424788475037,0.5045188560034148
712713,712714,712713,1425427,1676.8884580135345,0.5032073966449389
714715,714716,714715,1429431,1681.5999248027802,0.5019028281112696
716717,716718,716717,1433435,1686.2412867546082,0.5006050962747395
718719,718720,718719,1437439,1690.8932039737701,0.4993141475661105
720721,720722,720721,1441443,1695.5503208637238,0.49802992897457443
722723,722724,722723,1445447,1700.1956977844238,0.4967523880513909
724725,724726,724725,1449451,1704.8564517498016,0.4954814728753263
726727,726728,726727,1453455,1709.5380578041077,0.49421713206720597
728729,728730,728729,1457459,1714.2414288520813,0.4929593147808191
730731,730732,730731,1461463,1718.9100768566132,0.49170797068290995
732733,732734,732733,1465467,1723.5568189620972,0.49046304996227263
734735,734736,734735,1469471,1728.357349872589,0.4892245033188374
736737,736738,736737,1473475,1733.1665179729462,0.4879922819472995
738739,738740,738739,1477479,1737.834378004074,0.48676633754439536
740741,740742,740741,1481483,1742.5537989139557,0.4855466222979885
742743,742744,742743,1485487,1747.2394287586212,0.4843330888706987
744745,744746,744745,1489491,1751.931447982788,0.48312569041445386
746747,746748,746747,1493495,1756.7122938632965,0.4819243805432052
748749,748750,748749,1497499,1761.4195828437805,0.4807291133402032
750751,750752,750751,1501503,1766.0675067901611,0.47953984334708366
752753,752754,752753,1505507,1770.7199838161469,0.4783565255620488
754755,754756,754755,1509511,1775.4081280231476,0.4771791154271341
756757,756758,756757,1513515,1780.1476888656616,0.47600756883548456
758759,758760,758759,1517519,1784.8835628032684,0.4748418421095266
760761,760762,760761,1521523,1789.5655386447906,0.4736818920046062
762763,762764,762763,1525527,1794.2431390285492,0.4725276757053507
764765,764766,764765,1529531,1798.909117937088,0.4713791508147551
766767,766768,766767,1533535,1803.5958907604218,0.470236275356001
768769,768770,768769,1537539,1808.2626519203186,0.46909900775972346
770771,770772,770771,1541543,1812.933974981308,0.4679673068658303
772773,772774,772773,1545547,1817.6174988746643,0.46684113191076904
774775,774776,774775,1549551,1822.2810130119324,0.4657204425329837
776777,776778,776777,1553555,1826.9726629257202,0.4646051987529063
778779,778780,778779,1557559,1831.687847852707,0.4634953609893273
780781,780782,780781,1561563,1836.3466138839722,0.4623908900339302
782783,782784,782783,1565567,1841.0295288562775,0.4612917470640241
784785,784786,784785,1569571,1845.746610879898,0.46019789362071606
786787,786788,786787,1573575,1850.4230227470398,0.45910929161800595
788789,788790,788789,1577579,1855.1288130283356,0.45802590333369153
790791,790792,790791,1581583,1859.7534000873566,0.45694769140573044
792793,792794,792793,1585587,1864.562032699585,0.45587461883042124
794795,794796,794795,1589591,1869.3386437892914,0.4548066489460325
796797,796798,796797,1593595,1873.9905018806458,0.45374374544917373
798799,798800,798799,1597599,1878.640707731247,0.45268587236751046
800801,800802,800801,1601603,1883.3278529644012,0.4516329940797732
802803,802804,802803,1605607,1888.0074009895325,0.45058507529211056
804805,804806,804805,1609611,1892.7875907421112,0.4495420810399082
806807,806808,806807,1613615,1897.4312357902527,0.44850397669142694
808809,808810,808809,1617619,1902.1387798786163,0.4474707279368886
810811,810812,810811,1621623,1906.79590177536,0.44644230078301916
812813,812814,812813,1625627,1911.4909608364105,0.44541866155486787
814815,814816,814815,1629631,1916.2655427455902,0.44439977688853105
816817,816818,816817,1633635,1920.918684720993,0.44338561372933327
818819,818820,818819,1637639,1925.606008052826,0.4423761393263703
820821,820822,820821,1641643,1930.5066738128662,0.4413713212325092
822823,822824,822823,1645647,1935.2333507537842,0.44037112729711225
824825,824826,824825,1649651,1939.8878200054169,0.439375525662399
826827,826828,826827,1653655,1944.5895838737488,0.43838448476526537
828829,828830,828829,1657659,1949.2600660324097,0.4373979733281885
830831,830832,830831,1661663,1954.0092358589172,0.43641596035922703
832833,832834,832833,1665667,1958.7530159950256,0.4354384151483828
834835,834836,834835,1669671,1963.5110697746277,0.43446530726032506
836837,836838,836837,1673675,1968.4026370048523,0.43349660654348554
838839,838840,838839,1677679,1973.1159448623657,0.43253228310459235
840841,840842,840841,1681683,1977.8078598976135,0.431572307332317
842843,842844,842843,1685687,1982.4603219032288,0.43061664987544646
844845,844846,844845,1689691,1987.1454319953918,0.4296652816428832
846847,846848,846847,1693695,1991.8266518115997,0.42871817381092114
848849,848850,848849,1697699,1996.4676480293274,0.42777529780505574
850851,850852,850851,1701703,2001.1461598873138,0.42683662531271693
852853,852854,852853,1705707,2005.826751947403,0.4259021282668982
854855,854856,854855,1709711,2010.4880578517914,0.42497177884979465
856857,856858,856857,1713715,2015.2318618297577,0.42404554948734585
858859,858860,858859,1717719,2019.9441268444061,0.423123412861969
860861,860862,860861,1721723,2024.633276939392,0.42220534187981684
862863,862864,862863,1725727,2029.2641746997833,0.4212913096907869
864865,864866,864865,1729731,2033.9725449085236,0.4203812896848831
866867,866868,866867,1733735,2038.6341319084167,0.4194752554776642
868869,868870,868869,1737739,2043.2893838882446,0.4185731809193385
870871,870872,870871,1741743,2047.9515960216522,0.417675040087488
872873,872874,872873,1745747,2052.6087398529053,0.4167808072816115
874875,874876,874875,1749751,2057.2653110027313,0.4158904570267623
876877,876878,876877,1753755,2061.93084692955,0.4150039640699106
878879,878880,878879,1757759,2066.5655286312103,0.4141213033708482
880881,880882,880881,1761763,2071.226672887802,0.4132424501058267
882883,882884,882883,1765767,2075.9032418727875,0.4123674244929134
884885,884886,884885,1769771,2080.612375020981,0.41149623426099424
886887,886888,886887,1773775,2085.3327968120575,0.410628777994134
888889,888890,888889,1777779,2089.9639418125153,0.40976503159618005
890891,890892,890891,1781783,2094.6928718090057,0.408904971278389
892893,892894,892893,1785787,2099.3567197322845,0.40804857346302015
894895,894896,894895,1789791,2104.023468017578,0.40719581476878375
896897,896898,896897,1793795,2108.67493391037,0.4063466720235738
898899,898900,898899,1797799,2113.331813812256,0.4055011222444591
900901,900902,900901,1801803,2117.982396841049,0.4046591426431405
902903,902904,902903,1805807,2122.6378479003906,0.4038207106223126
904905,904906,904905,1809811,2127.272843837738,0.4029858037811209
906907,906908,906907,1813815,2132.0563547611237,0.4021543998969719
908909,908910,908909,1817819,2136.866231918335,0.4013264769419038
910911,910912,910911,1821823,2141.5535707473755,0.40050201306257804
912913,912914,912913,1825827,2146.5325009822845,0.39968098659483076
914915,914916,914915,1829831,2150.9987177848816,0.3988633760563971
916917,916918,916917,1833835,2155.4913408756256,0.39804916012872127
918919,918920,918919,1837839,2160.084345817566,0.3972383176933363
920921,920922,920921,1841843,2164.5674607753754,0.3964308277827513
922923,922924,922923,1845847,2169.012887954712,0.39562666961501236
924925,924926,924925,1849851,2173.463747024536,0.3948258225755126
926927,926928,926927,1853855,2177.9280738830566,0.39402826622063003
928929,928930,928929,1857859,2182.448409795761,0.39323398027408984
930931,930932,930931,1861863,2186.90589594841,0.3924429446196882
932933,932934,932933,1865867,2191.3673300743103,0.3916551393158443
934935,934936,934935,1869871,2195.8082349300385,0.39087054457195336
936937,936938,936937,1873875,2200.252068758011,0.39008914076657675
938939,938940,938939,1877879,2204.7198157310486,0.3893109084365278
940941,940942,940941,1881883,2209.447165966034,0.3885358282677771
942943,942944,942943,1885887,2214.0623936653137,0.38776388111364213
944945,944946,944945,1889891,2218.49378991127,0.38699504797477857
946947,946948,946947,1893895,2222.903634786606,0.3862293100046372
948949,948950,948949,1897899,2227.4186198711395,0.385466648511283
950951,950952,950951,1901903,2231.883796930313,0.38470704495193786
952953,952954,952953,1905907,2236.4311497211456,0.383950480931162
954955,954956,954955,1909911,2240.9157297611237,0.3831969381953968
956957,956958,956957,1913915,2245.3766436576843,0.38244639864387864
958959,958960,958959,1917919,2249.7989118099213,0.38169884431954415
960961,960962,960961,1921923,2254.237858772278,0.38095425739993516
962963,962964,962963,1925927,2258.814796924591,0.3802126202153886
964965,964966,964965,1929931,2263.432856798172,0.37947391522175167
966967,966968,966967,1933935,2267.8893377780914,0.3787381250240287
968969,968970,968969,1937939,2272.369024991989,0.37800523236364825
970971,970972,970971,1941943,2276.806174993515,0.3772752201093681
972973,972974,972973,1945947,2281.3840239048004,0.3765480712736462
974975,974976,974975,1949951,2285.812519788742,0.3758237689962698
976977,976978,976977,1953955,2290.249300956726,0.3751022965479933
978979,978980,978979,1957959,2294.6878876686096,0.37438363733599545
980981,980982,980981,1961963,2299.1176567077637,0.3736677748893271
982983,982984,982983,1965967,2303.5781686306,0.3729546928698255
984985,984986,984985,1969971,2308.0430159568787,0.3722443750648381
986987,986988,986987,1973975,2312.4643597602844,0.37153680538540357
988989,988990,988989,1977979,2316.877180814743,0.37083196786625194
990991,990992,990991,1981983,2321.369585752487,0.3701298466658045
992993,992994,992993,1985987,2325.8580408096313,0.3694304260716308
994995,994996,994995,1989991,2330.329499721527,0.3687336904786207
996997,996998,996997,1993995,2334.794766664505,0.3680396244089934
998999,999000,998999,1997999,2339.236051797867,0.36734821250502137
1001001,1001002,1001001,2002003,2343.697945833206,0.3666594395235734
1003003,1003004,1003003,2006007,2348.3210277557373,0.3659732903342956
1005005,1005006,1005005,2010011,2352.992758989334,0.3652897499232495
1007007,1007008,1007007,2014015,2357.444658756256,0.36460880339836876
1009009,1009010,1009009,2018019,2361.998591899872,0.3639304359694506
1011011,1011012,1011011,2022023,2366.413864850998,0.36325463296452654
1013013,1013014,1013013,2026027,2370.9647669792175,0.36258137981894834
1015015,1015016,1015015,2030031,2375.465591907501,0.3619106620808452
1017017,1017018,1017017,2034035,2379.901015996933,0.36124246540202876
1019019,1019020,1019019,2038039,2384.361448764801,0.36057677555254486
1021021,1021022,1021021,2042043,2388.809471845627,0.3599135783952079
1023023,1023024,1023023,2046047,2393.3146460056305,0.3592528599056095
1025025,1025026,1025025,2050051,2397.7913637161255,0.35859460616484284
1027027,1027028,1027027,2054055,2402.198184967041,0.35793880335768335
1029029,1029030,1029029,2058059,2406.6403138637543,0.35728543776713195
1031031,1031032,1031031,2062063,2411.066788673401,0.3566344957853289
1033033,1033034,1033033,2066067,2415.484804868698,0.35598596389536397
1035035,1035036,1035035,2070071,2419.9010138511658,0.35533982868946623
1037037,1037038,1037037,2074075,2424.395686864853,0.35469607685445226
1039039,1039040,1039039,2078079,2428.8467288017273,0.354054695177183
1041041,1041042,1041041,2082083,2433.341367006302,0.35341567053728795
1043043,1043044,1043043,2086087,2437.7458589076996,0.3527789899144409
1045045,1045046,1045045,2090091,2442.169888973236,0.35214464038472215
1047047,1047048,1047047,2094095,2446.5976808071136,0.35151260911516147
1049049,1049050,1049049,2098099,2451.066989660263,0.35088288336919504
1051051,1051052,1051051,2102103,2455.52005982399,0.3502554505048465
1053053,1053054,1053053,2106107,2460.01008272171,0.34963029796381306
1055055,1055056,1055055,2110111,2464.4518809318542,0.34900741328783624
1057057,1057058,1057057,2114115,2468.9018857479095,0.34838678410415014
1059059,1059060,1059059,2118119,2473.3463039398193,0.3477683981327573
1061061,1061062,1061061,2122123,2477.7820518016815,0.3471522431791527
1063063,1063064,1063063,2126127,2482.232603788376,0.34653830713978095
1065065,1065066,1065065,2130131,2486.6657316684723,0.345926577992941
1067067,1067068,1067067,2134135,2491.1359798908234,0.3453170438115194
1069069,1069070,1069069,2138139,2495.5834918022156,0.3447096927466191
1071071,1071072,1071071,2142143,2500.00102686882,0.3441045130348357
1073073,1073074,1073073,2146147,2504.4899609088898,0.34350149300371413
1075075,1075076,1075075,2150151,2508.908465862274,0.342900621055378
1077077,1077078,1077077,2154155,2513.37645983696,0.34230188567926234
1079079,1079080,1079079,2158159,2517.8571088314056,0.34170527544483775
1081081,1081082,1081081,2162163,2522.3272478580475,0.34111077900524833
1083083,1083084,1083083,2166167,2526.7967908382416,0.34051838509003574
1085085,1085086,1085085,2170171,2531.5959117412567,0.33992808251241513
1087087,1087088,1087087,2174175,2536.1107230186462,0.33933986016018025
1089089,1089090,1089089,2178179,2540.587994813919,0.3387537070084363
1091091,1091092,1091091,2182183,2545.057801961899,0.3381696120941342
1093093,1093094,1093093,2186187,2549.5080230236053,0.33758756454699324
1095095,1095096,1095095,2190191,2554.0196237564087,0.33700755356039735
1097097,1097098,1097097,2194195,2558.5173478126526,0.336429568415042
1099099,1099100,1099099,2198199,2562.95832490921,0.33585359845892526
1101101,1101102,1101101,2202203,2567.392063856125,0.3352796331146237
1103103,1103104,1103103,2206207,2571.8755548000336,0.33470766188293055
1105105,1105106,1105105,2210211,2576.3674759864807,0.33413767433012254
1107107,1107108,1107107,2214215,2581.239311695099,0.333569660104331
1109109,1109110,1109109,2218219,2585.84863781929,0.33300360891189484
1111111,1111112,1111111,2222223,2590.458212852478,0.33243951055010257
1113113,1113114,1113113,2226227,2595.088709831238,0.3318773548671743
1115115,1115116,1115115,2230231,2599.582547903061,0.33131713179318467
1117117,1117118,1117117,2234235,2604.0553648471832,0.330758831320054
1119119,1119120,1119119,2238239,2608.5850858688354,0.3302024435124622
1121121,1121122,1121121,2242243,2613.056032896042,0.3296479585060297
1123123,1123124,1123123,2246247,2617.5193479061127,0.32909536650004156
1125125,1125126,1125125,2250251,2621.9640667438507,0.32854465775744757
1127127,1127128,1127127,2254255,2626.389930009842,0.32799582261759497
1129129,1129130,1129129,2258259,2630.9395220279694,0.32744885147258174
1131131,1131132,1131131,2262263,2635.4279108047485,0.3269037347909034
1133133,1133134,1133133,2266267,2640.1792356967926,0.3263604631029011
1135135,1135136,1135135,2270271,2644.7370369434357,0.32581902699712373
1137137,1137138,1137137,2274275,2649.2118027210236,0.32527941713306063
1139139,1139140,1139139,2278279,2653.676242828369,0.3247416242284089
1141141,1141142,1141141,2282283,2658.147668838501,0.3242056390718062
1143143,1143144,1143143,2286287,2662.6458168029785,0.32367145250100293
1145145,1145146,1145145,2290291,2667.170012950897,0.32313905542469
1147147,1147148,1147147,2294295,2671.665428876877,0.3226084388115851
1149149,1149150,1149149,2298299,2676.3211958408356,0.3220795936849754
1151151,1151152,1151151,2302303,2680.763462781906,0.3215525111372699
1153153,1153154,1153153,2306307,2685.221663951874,0.32102718230999017
1155155,1155156,1155155,2310311,2689.7104358673096,0.3205035984137794
1157157,1157158,1157157,2314315,2694.1950318813324,0.3199817507102125
1159159,1159160,1159159,2318319,2698.671891927719,0.31946163052271004
1161161,1161162,1161161,2322323,2703.1511178016663,0.3189432292347192
1163163,1163164,1163163,2326327,2707.584002017975,0.31842653828061884
1165165,1165166,1165165,2330331,2712.0589559078217,0.3179115491493576
1167167,1167168,1167167,2334335,2716.5739970207214,0.3173982533990056
1169169,1169170,1169169,2338339,2721.069772005081,0.31688664263310784
1171171,1171172,1171171,2342343,2725.609422683716,0.31637670850977884
1173173,1173174,1173173,2346347,2730.0865218639374,0.31586844274534087
1175175,1175176,1175175,2350351,2734.527319908142,0.3153618371106859
1177177,1177178,1177177,2354355,2738.9672219753265,0.3148568834294565
1179179,1179180,1179179,2358359,2743.4491798877716,0.3143535735744081
1181181,1181182,1181181,2362363,2747.9322040081024,0.31385189948741754
1183183,1183184,1183183,2366367,2752.406874895096,0.3133518531376467
1185185,1185186,1185185,2370371,2756.865383863449,0.31285342657247384
1187187,1187188,1187187,2374375,2761.3118607997894,0.31235661186838115
1189189,1189190,1189189,2378379,2765.7905609607697,0.3118614011709724
1191191,1191192,1191191,2382383,2770.235067844391,0.3113677866640501
1193193,1193194,1193193,2386387,2774.7361238002777,0.3108757605896244
1195195,1195196,1195195,2390391,2779.173821926117,0.3103853152351803
1197197,1197198,1197197,2394395,2783.6712770462036,0.3098964429427724
1199199,1199200,1199199,2398399,2788.2751338481903,0.30940913609811105
1201201,1201202,1201201,2402403,2792.847596883774,0.30892338714147627
1203203,1203204,1203203,2406407,2797.32484292984,0.30843918855498487
1205205,1205206,1205205,2410411,2801.8131499290466,0.3079565328771423
1207207,1207208,1207207,2414415,2806.2703337669373,0.3074754126882908
1209209,1209210,1209209,2418419,2810.752275943756,0.30699582061242836
1211211,1211212,1211211,2422423,2815.3075778484344,0.30651774933176057
1213213,1213214,1213213,2426427,2819.7509849071503,0.30604119156669185
1215215,1215216,1215215,2430431,2824.1857867240906,0.3055661400885583
1217217,1217218,1217217,2434435,2828.6890017986298,0.30509258770871384
1219219,1219220,1219219,2438439,2833.142375946045,0.304620527289444
1221221,1221222,1221221,2442443,2837.6155269145966,0.30414995173487114
1223223,1223224,1223223,2446447,2842.066946029663,0.3036808539964113
1225225,1225226,1225225,2450451,2846.5214116573334,0.30321322706731735
1227227,1227228,1227227,2454455,2851.2481818199158,0.3027470639881358
1229229,1229230,1229229,2458459,2855.789037704468,0.3022823578394309
1231231,1231232,1231231,2462463,2860.2342178821564,0.3018191017490608
1233233,1233234,1233233,2466467,2864.6641368865967,0.3013572888885392
1235235,1235236,1235235,2470471,2869.1509528160095,0.3008969124639407
1237237,1237238,1237237,2474475,2873.606034755707,0.30043796573227155
1239239,1239240,1239239,2478479,2878.151398897171,0.29998044199055585
1241241,1241242,1241241,2482483,2882.5994539260864,0.2995243345758354
1243243,1243244,1243243,2486487,2887.0407490730286,0.29906963686698873
1245245,1245246,1245245,2490491,2891.668032884598,0.2986163422847312
1247247,1247248,1247247,2494495,2896.0951437950134,0.2981644442916149
1249249,1249250,1249249,2498499,2900.582629919052,0.29771393648479716
1251251,1251252,1251251,2502503,2905.033144712448,0.29726481415309536
1253253,1253254,1253253,2506507,2909.47181892395,0.2968170695457957
1255255,1255256,1255255,2510511,2913.9085228443146,0.2963706958835246
1257257,1257258,1257257,2514515,2918.370110988617,0.2959256867507065
1259259,1259260,1259259,2518519,2922.8093860149384,0.29548203582089627
1261261,1261262,1261261,2522523,2927.323118686676,0.2950397368203994
1263263,1263264,1263263,2526527,2931.9846098423004,0.2945987835282722
1265265,1265266,1265265,2530531,2936.461989879608,0.29415916975085565
1267267,1267268,1267267,2534535,2940.9172258377075,0.29372088934178464
1269269,1269270,1269269,2538539,2945.3237318992615,0.29328393619107374
1271271,1271272,1271271,2542543,2949.8751690387726,0.2928483042287553
1273273,1273274,1273273,2546547,2954.407628059387,0.2924139874139655
1275275,1275276,1275275,2550551,2958.884541749954,0.2919809797494963
1277277,1277278,1277277,2554555,2963.3274188041687,0.2915492752690625
1279279,1279280,1279279,2558559,2967.8090858459473,0.2911188680536725
1281281,1281282,1281281,2562563,2972.2768199443817,0.2906897522043437
1283283,1283284,1283283,2566567,2976.7649488449097,0.29026192186938715
1285285,1285286,1285285,2570571,2981.2191627025604,0.2898353712298558
1287287,1287288,1287287,2574575,2985.6787338256836,0.28941009449772537
1289289,1289290,1289289,2578579,2990.144015789032,0.2889860859249893
1291291,1291292,1291291,2582583,2994.638478755951,0.28856333979456394
1293293,1293294,1293293,2586587,2999.1226308345795,0.28814185042392637
1295295,1295296,1295295,2590591,3003.580544948578,0.28772161216875247
1297297,1297298,1297297,2594595,3008.185703754425,0.28730261941382196
1299299,1299300,1299299,2598599,3012.8843507766724,0.28688486657847534
1301301,1301302,1301301,2602603,3017.308227777481,0.28646834811297595
1303303,1303304,1303303,2606607,3021.832177877426,0.28605305850942386
1305305,1305306,1305305,2610611,3026.2987728118896,0.28563899227992806
1307307,1307308,1307307,2614615,3030.746532678604,0.28522614398025325
1309309,1309310,1309309,2618619,3035.328012943268,0.284814508189811
1311311,1311312,1311311,2622623,3039.8187098503113,0.2844040795280307
1313313,1313314,1313313,2626627,3044.255057811737,0.2839948526434455
1315315,1315316,1315315,2630631,3048.716886997223,0.2835868222082354
1317317,1317318,1317317,2634635,3053.198595046997,0.2831799829400552
1319319,1319320,1319319,2638639,3057.6096477508545,0.28277432957474957
1321321,1321322,1321321,2642643,3062.3259558677673,0.28236985688636196
1323323,1323324,1323323,2646647,3066.791298866272,0.28196655967803963
1325325,1325326,1325325,2650651,3071.2643859386444,0.2815644327820337
1327327,1327328,1327327,2654655,3075.730829000473,0.28116347106697503
1329329,1329330,1329329,2658659,3080.173615694046,0.28076366941604647
1331331,1331332,1331331,2662663,3084.705451965332,0.2803650227615435
1333333,1333334,1333333,2666667,3089.180013656616,0.2799675260521326
1335335,1335336,1335335,2670671,3093.639797925949,0.27957117427285993
1337337,1337338,1337337,2674675,3098.1150999069214,0.2791759624324186
1339339,1339340,1339339,2678679,3102.591778755188,0.2787818855704245
1341341,1341342,1341341,2682683,3107.021948814392,0.2783889387592353
1343343,1343344,1343343,2686687,3111.518703699112,0.27799711709303665
1345345,1345346,1345345,2690691,3115.9676308631897,0.2776064156987559
1347347,1347348,1347347,2694695,3120.433316707611,0.27721682973060524
1349349,1349350,1349349,2698699,3124.8522827625275,0.2768283543682628
1351351,1351352,1351351,2702703,3129.3126430511475,0.2764409848223295
1353353,1353354,1353353,2706707,3133.79487490654,0.276054716330691
1355355,1355356,1355355,2710711,3138.2469868659973,0.275669544156699
1357357,1357358,1357357,2714715,3142.712154865265,0.2752854635928088
1359359,1359360,1359359,2718719,3147.1673159599304,0.2749024699569418
1361361,1361362,1361361,2722723,3151.609225988388,0.27452055859248503
1363363,1363364,1363363,2726727,3156.0798857212067,0.2741397248719295
1365365,1365366,1365365,2730731,3160.57941198349,0.273759964191413
1367367,1367368,1367367,2734735,3165.0814328193665,0.2733812719798152
1369369,1369370,1369369,2738739,3169.536469936371,0.2730036436805676
1371371,1371372,1371371,2742743,3174.033433675766,0.27262707477530057
1373373,1373374,1373373,2746747,3178.4821577072144,0.2722515607638343
1375375,1375376,1375375,2750751,3183.287090778351,0.2718770971696358
1377377,1377378,1377377,2754755,3187.8675198554993,0.2715036795470951
1379379,1379380,1379379,2758759,3192.3326630592346,0.27113130347424885
1381381,1381382,1381381,2762763,3196.7774698734283,0.2707599645545997
1383383,1383384,1383383,2766767,3201.2511427402496,0.2703896584116592
1385385,1385386,1385385,2770771,3205.712343931198,0.2700203806980426
1387387,1387388,1387387,2774775,3210.2566328048706,0.2696521270900121
1389389,1389390,1389389,2778779,3214.6987047195435,0.26928489328565774
1391391,1391392,1391391,2782783,3219.168876886368,0.2689186750103545
1393393,1393394,1393393,2786787,3223.6353657245636,0.26855346801676205
1395395,1395396,1395395,2790791,3228.094409942627,0.2681892680666351
1397397,1397398,1397397,2794795,3232.614804983139,0.26782607096174615
1399399,1399400,1399399,2798799,3237.0947058200836,0.26746387251660053
1401401,1401402,1401401,2802803,3241.558257818222,0.26710266857844545
1403403,1403404,1403403,2806807,3246.119950771332,0.26674245500908
1405405,1405406,1405405,2810811,3250.5675098896027,0.26638322769576916
1407407,1407408,1407407,2814815,3255.01078081131,0.26602498254942475
1409409,1409410,1409409,2818819,3259.428906917572,0.26566771550096746
1411411,1411412,1411411,2822823,3263.922521829605,0.26531142251042183
1413413,1413414,1413413,2826827,3268.3604307174683,0.2649560995560023
1415415,1415416,1415415,2830831,3272.8025467395782,0.2646017426304752
1417417,1417418,1417417,2834835,3277.234585762024,0.26424834776298667
1419419,1419420,1419419,2838839,3281.719790697098,0.26389591099359677
1421421,1421422,1421421,2842843,3286.2273919582367,0.26354442838783143
1423423,1423424,1423423,2846847,3290.700642824173,0.26319389603486343
1425425,1425426,1425425,2850851,3295.1578707695007,0.26284431004205544
1427427,1427428,1427427,2854855,3299.6257269382477,0.262495666538598
1429429,1429430,1429429,2858859,3304.20663189888,0.2621479616736906
1431431,1431432,1431431,2862863,3308.808266878128,0.26180119162199844
1433433,1433434,1433433,2866867,3313.2908647060394,0.26145535257455776
1435435,1435436,1435435,2870871,3317.7687468528748,0.26111044074241363
1437437,1437438,1437437,2874875,3322.236357688904,0.26076645236389595
1439439,1439440,1439439,2878879,3326.665105819702,0.2604233836864296
1441441,1441442,1441441,2882883,3331.330327987671,0.2600812309920002
1443443,1443444,1443443,2886887,3335.802985906601,0.2597399905680504
1445445,1445446,1445445,2890891,3340.2821497917175,0.25939965873840265
1447447,1447448,1447447,2894895,3344.7186057567596,0.2590602318250603
1449449,1449450,1449449,2898899,3349.1912047863007,0.2587217061936826
1451451,1451452,1451451,2902903,3353.806581020355,0.2583840782062907
1453453,1453454,1453453,2906907,3358.711338996887,0.2580473442667426
1455455,1455456,1455455,2910911,3363.1987776756287,0.25771150077889615
1457457,1457458,1457457,2914915,3367.6707026958466,0.25737654418298916
1459459,1459460,1459459,2918919,3372.248925924301,0.25704247092107835
1461461,1461462,1461461,2922923,3376.6718797683716,0.25670927746614325
1463463,1463464,1463463,2926927,3381.1500039100647,0.2563769603093533
1465465,1465466,1465465,2930931,3385.6510620117188,0.2560455159527919
1467467,1467468,1467467,2934935,3390.4568688869476,0.25571494092764624
1469469,1469470,1469469,2938939,3394.932543992996,0.2553852317723795
1471471,1471472,1471471,2942943,3399.321400642395,0.25505638505455863
1473473,1473474,1473473,2946947,3403.7524399757385,0.2547283973508456
1475475,1475476,1475475,2950951,3408.265925884247,0.25440126526336826
1477477,1477478,1477477,2954955,3412.948385953903,0.25407498540516826
1479479,1479480,1479479,2958959,3417.609045982361,0.2537495544147532
1481481,1481482,1481481,2962963,3422.2699949741364,0.25342496894154465
1483483,1483484,1483483,2966967,3426.923640012741,0.25310122565679194
1485485,1485486,1485485,2970971,3431.884080886841,0.2527783212481154
1487487,1487488,1487487,2974975,3436.709265947342,0.2524562524158682
1489489,1489490,1489489,2978979,3441.4602649211884,0.2521350158895075
1491491,1491492,1491491,2982983,3446.1580736637115,0.2518146084057662
1493493,1493494,1493493,2986987,3450.819674730301,0.25149502671774826
1495495,1495496,1495495,2990991,3455.5373587608337,0.25117626760038547
1497497,1497498,1497497,2994995,3460.264173746109,0.25085832784316153
1499499,1499500,1499499,2998999,3464.936582803726,0.250541204257388
1501502,1501503,1501502,3003005,3469.6490869522095,0.2502247358661407
1503504,1503505,1503504,3007009,3474.4458558559418,0.24990923550649313
1505506,1505507,1505506,3011013,3479.1443870067596,0.24959454183044727
1507508,1507509,1507508,3015017,3483.8048796653748,0.2492806517129793
1509510,1509511,1509510,3019021,3488.468822002411,0.24896756204361736
1511512,1511513,1511512,3023025,3493.174114704132,0.24865526972644147
1513514,1513515,1513514,3027029,3497.8956480026245,0.24834377168372157
1515516,1515517,1515516,3031033,3502.605334997177,0.24803306484682253
1517518,1517519,1517518,3035037,3507.305291891098,0.24772314617439406
1519520,1519521,1519520,3039041,3512.034862756729,0.24741401263418084
1521522,1521523,1521522,3043045,3516.7338438034058,0.24710566120666044
1523524,1523525,1523524,3047049,3521.428538799286,0.24679808889050037
1525526,1525527,1525526,3051053,3526.115233898163,0.24649129270619596
1527528,1527529,1527528,3055057,3530.817332983017,0.24618526967788057
1529530,1529531,1529530,3059061,3535.5280346870422,0.24588001685333438
1531532,1531533,1531532,3063065,3540.525541782379,0.24557553129125154
1533534,1533535,1533534,3067069,3545.4337668418884,0.24527181006669707
1535536,1535537,1535536,3071073,3550.359096765518,0.24496885027110693
1537538,1537539,1537538,3075077,3555.2632019519806,0.24466664900864998
1539540,1539541,1539540,3079081,3560.1814210414886,0.24436520339804702
1541542,1541543,1541542,3083085,3565.128075838089,0.24406451057438971
1543544,1543545,1543544,3087089,3570.2238597869873,0.2437645676873217
1545546,1545547,1545546,3091093,3575.2498359680176,0.24346537189740047
1547548,1547549,1547548,3095097,3580.18790602684,0.2431669203833735
1549550,1549551,1549550,3099101,3585.157889842987,0.24286921033672115
1551552,1551553,1551552,3103105,3590.075889825821,0.24257223896347568
1553554,1553555,1553554,3107109,3595.1521756649017,0.2422760034842213
1555556,1555557,1555556,3111113,3600.170257806778,0.2419805011322751
1557558,1557559,1557558,3115117,3605.0259828567505,0.2416857291573251
1559560,1559561,1559560,3119121,3609.764796733856,0.24139168481633533
1561562,1561563,1561562,3123125,3614.4399547576904,0.2410983653862786
1563564,1563565,1563564,3127129,3619.134809732437,0.2408057681604987
1565566,1565567,1565566,3131133,3623.82928276062,0.24051389043415838
1567568,1567569,1567568,3135137,3628.5455837249756,0.24022272953152424
1569570,1569571,1569570,3139141,3633.2114386558533,0.23993228277322487
1571572,1571573,1571572,3143145,3637.892250776291,0.23964254750899272
1573574,1573575,1573574,3147149,3642.567534685135,0.23935352109037922
1575576,1575577,1575576,3151153,3647.2247087955475,0.23906520088894467
1577578,1577579,1577578,3155157,3651.9149780273438,0.23877758428534435
1579580,1579581,1579580,3159161,3656.601791858673,0.2384906686784234
1581582,1581583,1581582,3163165,3661.261646747589,0.23820445146884595
1583584,1583585,1583584,3167169,3665.925223827362,0.23791893008092302
1585586,1585587,1585586,3171173,3670.9029376506805,0.23763410194806056
1587588,1587589,1587588,3175177,3675.6335048675537,0.23734996452003543
1589590,1589591,1589590,3179181,3680.318754673004,0.23706651525208144
1591592,1591593,1591592,3183185,3685.0491178035736,0.23678375161398435
1593594,1593595,1593594,3187189,3689.7823219299316,0.23650167109371978
1595596,1595597,1595596,3191193,3694.529932975769,0.23622027117926336
1597598,1597599,1597598,3195197,3699.1636888980865,0.23593954939133255
1599600,1599601,1599600,3199201,3703.8488409519196,0.23565950323973084
1601602,1601603,1601602,3203205,3708.483408689499,0.23538013026154658
1603604,1603605,1603604,3207209,3713.189651966095,0.2351014279993251
1605606,1605607,1605606,3211213,3717.8287539482117,0.2348233940119826
1607608,1607609,1607608,3215217,3722.490757703781,0.23454602586753026
1609610,1609611,1609610,3219221,3727.173594713211,0.23426932114671217
1611612,1611613,1611612,3223225,3731.9652638435364,0.23399327743754839
1613614,1613615,1613614,3227229,3736.6589188575745,0.2337178923517058
1615616,1615617,1615616,3231233,3741.4009437561035,0.23344316349903238
1617618,1617619,1617618,3235237,3746.0912578105927,0.23316908850392792
1619620,1619621,1619620,3239241,3750.7954139709473,0.23289566501080117
1621622,1621623,1621622,3243245,3755.4746758937836,0.2326228906695178
1623624,1623625,1623624,3247249,3760.1713337898254,0.23235076313903846
1625626,1625627,1625626,3251253,3764.8579268455505,0.23207928008741874
1627628,1627629,1627628,3255257,3769.502546787262,0.23180843920818006
1629630,1629631,1629630,3259261,3774.213552713394,0.2315382381912059
1631632,1631633,1631632,3263265,3778.889302968979,0.23126867473729362
1633634,1633635,1633634,3267269,3783.571063041687,0.2309997465708875
1635636,1635637,1635636,3271273,3788.2354488372803,0.2307314514182508
1637638,1637639,1637638,3275277,3792.906177997589,0.23046378701656067
1639640,1639641,1639640,3279281,3797.6448769569397,0.23019675111572724
1641642,1641643,1641642,3283285,3802.364015817642,0.22993034147839353
1643644,1643645,1643644,3287289,3807.0252809524536,0.22966455587265955
1645646,1645647,1645646,3291293,3811.7056138515472,0.22939939207935822
1647648,1647649,1647648,3295297,3816.3765058517456,0.2291348478938744
1649650,1649651,1649650,3299301,3821.053472995758,0.22887092111704987
1651652,1651653,1651652,3303305,3825.753942012787,0.2286076095606404
1653654,1653655,1653654,3307309,3830.5788626670837,0.22834491105459165
1655656,1655657,1655656,3311313,3835.3774189949036,0.22808282342339226
1657658,1657659,1657658,3315317,3840.2758548259735,0.22782134451881575
1659660,1659661,1659660,3319321,3845.0484018325806,0.22756047219081665
1661662,1661663,1661662,3323325,3849.8083448410034,0.2273002043039014
1663664,1663665,1663664,3327329,3854.6193828582764,0.22704053873530938
1665666,1665667,1665666,3331333,3859.5406336784363,0.22678147336591792
1667668,1667669,1667668,3335337,3864.270015001297,0.22652300609297527
1669670,1669671,1669670,3339341,3868.9443187713623,0.22626513481918664
1671672,1671673,1671672,3343345,3873.65487575531,0.2260078574581712
1673674,1673675,1673674,3347349,3878.3260538578033,0.22575117193446204
1675676,1675677,1675676,3351353,3883.075122833252,0.22549507618350617
1677678,1677679,1677678,3355357,3887.7547528743744,0.2252395681462076
1679680,1679681,1679680,3359361,3892.4480550289154,0.22498464577620325
1681682,1681683,1681682,3363365,3897.110958814621,0.22473030703804397
1683684,1683685,1683684,3367369,3901.8263030052185,0.22447654989809962
1685686,1685687,1685686,3371373,3906.5600419044495,0.2242233723445679
1687688,1687689,1687688,3375377,3911.2784378528595,0.22397077236382756
1689690,1689691,1689690,3379381,3916.007281780243,0.22371874795499025
1691692,1691693,1691692,3383385,3920.7038538455963,0.22346729712990054
1693694,1693695,1693694,3387389,3925.4380390644073,0.223216417907679
1695696,1695697,1695696,3391393,3930.097498893738,0.22296610831836006
1697698,1697699,1697698,3395397,3934.7512168884277,0.22271636639015924
1699700,1699701,1699700,3399401,3939.4036819934845,0.22246719017493888
1701702,1701703,1701702,3403405,3944.0867397785187,0.2222185777300183
1703704,1703705,1703704,3407409,3948.7450597286224,0.22197052711089782
1705706,1705707,1705706,3411413,3953.3997797966003,0.22172303640036262
1707708,1707709,1707708,3415417,3958.089661836624,0.2214761036757409
1709710,1709711,1709710,3419421,3962.801261663437,0.22122972702709376
1711712,1711713,1711712,3423425,3967.4663937091827,0.2209839045553963
1713714,1713715,1713714,3427429,3972.397640943527,0.22073863436344254
1715716,1715717,1715716,3431433,3977.106405735016,0.22049391457403544
1717718,1717719,1717718,3435437,3981.8229088783264,0.22024974330997793
1719720,1719721,1719720,3439441,3986.545358657837,0.2200061187013489
1721722,1721723,1721722,3443445,3991.2401757240295,0.21976303889823612
1723724,1723725,1723724,3447449,3996.1274988651276,0.2195205020452704
1725726,1725727,1725726,3451453,4000.7784440517426,0.21927850630527246
1727728,1727729,1727728,3455457,4005.439834833145,0.21903704984288197
1729730,1729731,1729730,3459461,4010.104943752289,0.21879613083365257
1731732,1731733,1731732,3463465,4014.8202917575836,0.2185557474658708
1733734,1733735,1733734,3467469,4019.510566711426,0.21831589792600425
1735736,1735737,1735736,3471473,4024.192091703415,0.21807658041871036
1737738,1737739,1737738,3475477,4028.9968798160553,0.21783779315592255
1739740,1739741,1739740,3479481,4033.947783946991,0.21759953434593626
1741742,1741743,1741742,3483485,4038.67791891098,0.2173618022170558
1743744,1743745,1743744,3487489,4043.4069187641144,0.21712459500486148
1745746,1745747,1745746,3491493,4048.118446826935,0.21688791094857152
1747748,1747749,1747748,3495497,4053.0235397815704,0.21665174829286116
1749750,1749751,1749750,3499501,4057.7224340438843,0.21641610530059552
1751752,1751753,1751752,3503505,4062.389865875244,0.21618098023100174
1753754,1753755,1753754,3507509,4067.1055529117584,0.21594637135785888
1755756,1755757,1755756,3511513,4071.825695991516,0.21571227696404094
1757758,1757759,1757758,3515517,4076.5072000026703,0.21547869533242192
1759760,1759761,1759760,3519521,4081.183007001877,0.21524562475860876
1761762,1761763,1761762,3523525,4085.8580327033997,0.2150130635509413
1763764,1763765,1763764,3527529,4090.535224676132,0.21478101001412142
1765766,1765767,1765766,3531533,4095.1890847682953,0.21454946246558393
1767768,1767769,1767768,3535537,4099.872920751572,0.21431841923367756
1769770,1769771,1769770,3539541,4104.588335752487,0.21408787865038903
1771772,1771773,1771772,3543545,4109.492630958557,0.213857839054981
1773774,1773775,1773774,3547549,4114.1963267326355,0.21362829879581113
1775776,1775777,1775776,3551553,4118.880134820938,0.21339925622669398
1777778,1777779,1777778,3555557,4123.579489946365,0.21317070971053909
1779780,1779781,1779780,3559561,4128.259147882462,0.21294265761571296
1781782,1781783,1781782,3563565,4133.076135873795,0.21271509831967705
1783784,1783785,1783784,3567569,4137.762216806412,0.21248803020898777
1785786,1785787,1785786,3571573,4142.4690680503845,0.21226145166656352
1787788,1787789,1787788,3575577,4147.186219930649,0.2120353610971506
1789790,1789791,1789790,3579581,4151.872799873352,0.21180975690185733
1791792,1791793,1791792,3583585,4156.800961017609,0.21158463749270595
1793794,1793795,1793794,3587589,4161.532459020615,0.21136000129263266
1795796,1795797,1795796,3591593,4166.203691959381,0.21113584672275465
1797798,1797799,1797798,3595597,4170.864436864853,0.21091217222056002
1799800,1799801,1799800,3599601,4175.5562748909,0.2106889762217179
1801802,1801803,1801802,3603605,4180.24162197113,0.2104662571728113
1803804,1803805,1803804,3607609,4184.920549869537,0.2102440135240613
1805806,1805807,1805806,3611613,4189.614594936371,0.2100222437402408
1807808,1807809,1807808,3615617,4194.315562963486,0.20980094628612278
1809810,1809811,1809810,3619621,4198.975764989853,0.2095801196373941
1811812,1811813,1811812,3623625,4203.6538598537445,0.20935976226792263
1813814,1813815,1813814,3627629,4208.481523990631,0.2091398726679472
1815816,1815817,1815816,3631633,4213.372496843338,0.20892044933134457
1817818,1817819,1817818,3635637,4218.0571320056915,0.2087014907538105
1819820,1819821,1819820,3639641,4222.802263021469,0.2084829954437737
1821822,1821823,1821822,3643645,4227.543690919876,0.2082649619133008
1823824,1823825,1823824,3647649,4232.327835798264,0.20804738867991546
1825826,1825827,1825826,3651653,4237.050398826599,0.20783027427387424
1827828,1827829,1827828,3655657,4241.862065792084,0.20761361721997673
1829830,1829831,1829830,3659661,4246.560670852661,0.20739741605939344
1831832,1831833,1831832,3663665,4251.236578702927,0.20718166933147586
1833834,1833835,1833834,3667669,4255.91992688179,0.2069663755937654
1835836,1835837,1835836,3671673,4260.62118601799,0.2067515334019845
1837838,1837839,1837838,3675677,4265.317982912064,0.20653714131003653
1839840,1839841,1839840,3679681,4270.0027866363525,0.2063231978972908
1841842,1841843,1841842,3683685,4274.844573974609,0.20610970173402166
1843844,1843845,1843844,3687689,4279.60024189949,0.20589665140141733
1845846,1845847,1845846,3691693,4284.448192834854,0.20568404548430408
1847848,1847849,1847848,3695697,4289.178664922714,0.20547188258024107
1849850,1849851,1849850,3699701,4294.065109968185,0.20526016128678748
1851852,1851853,1851852,3703705,4298.8365046978,0.20504888020695944
1853854,1853855,1853854,3707709,4303.498212814331,0.204838037956506
1855856,1855857,1855856,3711713,4308.197332859039,0.2046276331439003
1857858,1857859,1857858,3715717,4312.895216703415,0.2044176643994433
1859860,1859861,1859860,3719721,4317.603075027466,0.20420813034797902
1861862,1861863,1861862,3723725,4322.2865216732025,0.20399908705439884
1863864,1863865,1863864,3727729,4326.954115867615,0.20379047929782246
1865866,1865867,1865866,3731733,4331.652066707611,0.20358230218516837
1867868,1867869,1867868,3735737,4336.380632638931,0.20337455427034
1869870,1869871,1869870,3739741,4341.04328083992,0.2031672341763624
1871872,1871873,1871872,3743745,4345.726496934891,0.20296034054990741
1873874,1873875,1873874,3747749,4350.4202439785,0.20275387205765583
1875876,1875877,1875876,3751753,4355.103662729263,0.2025478273681074
1877878,1877879,1877878,3755757,4359.798361778259,0.2023422051606758
1879880,1879881,1879880,3759761,4364.502913951874,0.20213700412023172
1881882,1881883,1881882,3763765,4369.349982976913,0.20193222293710278
1883884,1883885,1883884,3767769,4374.150562763214,0.20172786030889256
1885886,1885887,1885886,3771773,4378.8143928050995,0.20152391493684263
1887888,1887889,1887888,3775777,4383.474269866943,0.20132038552583253
1889890,1889891,1889890,3779781,4388.25438284874,0.20111727079347475
1891892,1891893,1891892,3783785,4393.071036815643,0.20091456945374375
1893894,1893895,1893894,3787789,4397.719272851944,0.200712280229709
1895896,1895897,1895896,3791793,4402.414701700211,0.20051040185353486
1897898,1897899,1897898,3795797,4407.203769683838,0.20030893305556674
1899900,1899901,1899900,3799801,4411.8634197711945,0.20010787257706397
1901902,1901903,1901902,3803805,4416.58296585083,0.1999072191592859
1903904,1903905,1903904,3807809,4421.239204883575,0.19970697155804373
1905906,1905907,1905906,3811813,4425.924760818481,0.1995071285218728
1907908,1907909,1907908,3815817,4430.66232085228,0.1993076888120413
1909910,1909911,1909910,3819821,4435.3265788555145,0.19910865119527443
1911912,1911913,1911912,3823825,4439.981735944748,0.19891001444193535
1913914,1913915,1913914,3827829,4444.654137849808,0.1987117773223872
1915916,1915917,1915916,3831833,4449.332108974457,0.1985139386197261
1917918,1917919,1917918,3835837,4453.990757703781,0.1983164971225051
1919920,1919921,1919920,3839841,4458.6505398750305,0.19811945161745825
1921922,1921923,1921922,3843845,4463.394885778427,0.1979228008967766
1923924,1923925,1923924,3847849,4468.091209888458,0.1977265437672031
1925926,1925927,1925926,3851853,4472.811666965485,0.19753067902638577
1927928,1927929,1927928,3855857,4477.502029657364,0.1973352054883435
1929930,1929931,1929930,3859861,4482.197198867798,0.19714012196891417
1931932,1931933,1931932,3863865,4486.910160779953,0.19694542728393571
1933934,1933935,1933934,3867869,4491.604638814926,0.19675112025834096
1935936,1935937,1935936,3871873,4496.256569862366,0.19655719972251973
1937938,1937939,1937938,3875877,4501.150429964066,0.1963636645104998
1939940,1939941,1939940,3879881,4506.013249874115,0.19617051345812797
1941942,1941943,1941942,3883885,4510.668590784073,0.19597774541216495
1943944,1943945,1943944,3887889,4515.35954284668,0.19578535921755247
1945946,1945947,1945946,3891893,4520.051909685135,0.1955933537265082
1947948,1947949,1947948,3895897,4524.741318941116,0.19540172780034482
1949950,1949951,1949950,3899901,4529.542201757431,0.19521048029673693
1951952,1951953,1951952,3903905,4534.295393943787,0.19501961008427315
1953954,1953955,1953954,3907909,4538.979073047638,0.19482911602972308
1955956,1955957,1955956,3911913,4543.660290956497,0.19463899701440823
1957958,1957959,1957958,3915917,4548.305842876434,0.19444925191601214
1959960,1959961,1959960,3919921,4553.001691818237,0.1942598796194943
1961962,1961963,1961962,3923925,4557.732643842697,0.19407087901163322
1963964,1963965,1963964,3927929,4562.405180931091,0.19388224898466433
1965966,1965967,1965966,3931933,4567.069809913635,0.19369398844173702
1967968,1967969,1967968,3935937,4571.752575874329,0.19350609628054372
1969970,1969971,1969970,3939941,4576.472797870636,0.19331857141150977
1971972,1971973,1971972,3943945,4581.231864690781,0.19313141274324153
1973974,1973975,1973974,3947949,4585.995335817337,0.1929446191916213
1975976,1975977,1975976,3951953,4590.6841106414795,0.19275818967435043
1977978,1977979,1977978,3955957,4595.349401712418,0.19257212312004413
1979980,1979981,1979980,3959961,4600.051933765411,0.19238641845004167
1981982,1981983,1981982,3963965,4604.69038271904,0.19220107460205327
1983984,1983985,1983984,3967969,4609.349477767944,0.1920160905119701
1985986,1985987,1985986,3971973,4614.056988954544,0.19183146512295934
1987988,1987989,1987988,3975977,4618.719107866287,0.19164719737273117
1989990,1989991,1989990,3979981,4623.5196878910065,0.19146328621718567
1991992,1991993,1991992,3983985,4628.310809850693,0.19127973060858494
1993994,1993995,1993994,3987989,4633.000715970993,0.19109652950101008
1995996,1995997,1995996,3991993,4637.736422777176,0.1909136818612751
1997998,1997999,1997998,3995997,4642.414333820343,0.19073118665073707
2000000,2000001,2000000,4000001,4647.114407777786,0.19054904284166696


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0036039352416992188,12064.682476916567
1001,7376,7376,14752,18.16280508041382,0.2185577111922612
2002,15100,15100,30200,36.29642605781555,0.10515795791798155
3003,22762,22762,45524,55.961483001708984,0.006310511173069244
4004,30610,30610,61220,74.9745442867279,0.006166181057778886
5005,38584,38584,77168,93.57754707336426,0.0061183757625258295
6006,46568,46568,93136,113.38448905944824,0.006105341291913646
7007,54562,54562,109124,142.87890005111694,0.00609804192208685
8008,62554,62554,125108,177.2360281944275,0.006088372179874568
9009,70554,70554,141108,210.6262331008911,0.006084384294808842
10010,78552,78552,157104,243.88585495948792,0.006078809925384121
11011,86552,86552,173104,278.44044494628906,0.006076112389564514
12012,94546,94546,189092,312.65111804008484,0.006070468207326485
13013,102538,102538,205076,345.7434480190277,0.006055822785128839
14014,110542,110542,221084,382.3908441066742,0.006053901757695712
15015,118536,118536,237072,415.9855511188507,0.006029809774190653
16016,126516,126516,253032,449.01793217658997,0.004569394761347212
17017,134398,134398,268796,483.2819230556488,0.004537211319984635
18018,142386,142386,284772,518.3921480178833,0.004532146278506843
19019,150372,150372,300744,550.1638860702515,0.0045086469981470145
20020,158360,158360,316720,585.198468208313,0.004502913083342719
21021,166356,166356,332712,620.999340057373,0.004497499165154295
22022,174358,174358,348716,656.4476721286774,0.0044958962134842295
23023,182354,182354,364708,688.4954319000244,0.0044931493648618925
24024,190356,190356,380712,721.382621049881,0.004491351395699894
25025,198360,198360,396720,754.6736462116241,0.004490362911383272
26026,206346,206346,412692,787.703507900238,0.004464074212592095
27027,214348,214348,428696,821.9748229980469,0.004462264327230514
28028,222332,222332,444664,853.145613193512,0.004413959157318459
29029,230332,230332,460664,888.7861461639404,0.004411526042531477
30030,238336,238336,476672,925.3950181007385,0.004410199748235755
31031,246304,246304,492608,961.8196110725403,0.004038582866996876
32032,254300,254300,508600,998.8853759765625,0.004037275894006598
33033,262298,262298,524596,1035.3081619739532,0.0040345481647818815
34034,270300,270300,540600,1063.3009731769562,0.004032811650176882
35035,278302,278302,556604,1088.452163219452,0.004031622900583898
36036,286300,286300,572600,1111.8984880447388,0.004029210433145636
37037,294304,294304,588608,1134.603765964508,0.004028389123050147
38038,302298,302298,604596,1157.0772511959076,0.004018111469122232
39039,310298,310298,620596,1177.961655139923,0.004015640271973098
40040,318298,318298,636596,1203.168092250824,0.004013682415461517
41041,326304,326304,652608,1226.8443021774292,0.004012846737168729
42042,334300,334300,668600,1251.3533720970154,0.004012456953205401
43043,342298,342298,684596,1276.49449300766,0.004009942063930794
44044,350296,350296,700592,1301.2952420711517,0.004008084464658168
45045,358296,358296,716592,1325.3093860149384,0.004005187915026909
46046,366300,366300,732600,1350.2774209976196,0.0040041729207587196
47047,374302,374302,748604,1374.5554602146149,0.0040025338930718135
48048,382304,382304,764608,1393.232134103775,0.0040008795804169495
49049,390306,390306,780612,1410.6644310951233,0.00399958563320979
50050,398308,398308,796616,1428.066192150116,0.0039986009724088944
51051,406304,406304,812608,1445.5209431648254,0.003989975157310255
52052,414306,414306,828612,1462.8963301181793,0.003988224792919937
53053,422306,422306,844612,1480.2903361320496,0.003987019848864293
54054,430308,430308,860616,1497.4659650325775,0.003985179098890512
55055,438312,438312,876624,1514.6665861606598,0.003984542921898537
56056,446288,446288,892576,1531.6646001338959,0.003814730836893432
57057,454290,454290,908580,1548.7969889640808,0.003813430144873564
58058,462292,462292,924584,1566.6821298599243,0.0038122364749142434
59059,470294,470294,940588,1585.9281451702118,0.003806719418207649
60060,478294,478294,956588,1606.2770760059357,0.003803654752118746
61061,486292,486292,972584,1626.6950058937073,0.0038021814816602273
62062,494294,494294,988588,1647.4440021514893,0.0037996505343471654
63063,502296,502296,1004592,1667.8569700717926,0.0037984243499522563
64064,510298,510298,1020596,1688.225051164627,0.003797217659666785
65065,518264,518264,1036528,1708.464273929596,0.0035975307418993907
66066,526258,526258,1052516,1728.7690172195435,0.0035961042067356175
67067,534260,534260,1068520,1749.1775941848755,0.003594583062294987
68068,542260,542260,1084520,1769.2913711071014,0.0035922969909734093
69069,550268,550268,1100536,1789.5549800395966,0.003592217495679506
70070,558276,558276,1116552,1809.7798941135406,0.0035921380040235817
71071,566284,566284,1132568,1829.6877582073212,0.003592058514186647
72072,574288,574288,1148576,1849.6127271652222,0.0035918797038902994
73073,582290,582290,1164580,1869.8222362995148,0.0035910830865759635
74074,590280,590280,1180560,1890.259345293045,0.0035819142285618
75075,598278,598278,1196556,1910.4130811691284,0.0035802942929876735
76076,606280,606280,1212560,1930.5707750320435,0.0035784086903731804
77077,614280,614280,1228560,1950.6553170681,0.003576421018806286
78078,622282,622282,1244564,1970.8327660560608,0.0035756251272687223
79079,630286,630286,1260572,1990.9458129405975,0.003574803167794016
80080,638290,638290,1276580,2011.2244679927826,0.0035741694264288526
81081,646290,646290,1292580,2031.4125671386719,0.003571700503016473
82082,654292,654292,1308584,2051.3261392116547,0.003571106868548668
83083,662294,662294,1324588,2071.5119721889496,0.0035698300307558384
84084,670236,670236,1340472,2091.689558982849,0.00321327148230921
85085,678226,678226,1356452,2111.838219165802,0.0032118226099555613
86086,686218,686218,1372436,2132.3470990657806,0.0032042105194705073
87087,694216,694216,1388432,2152.5454251766205,0.0032011193652579095
88088,702216,702216,1404432,2172.865375995636,0.0031999948023440083
89089,710212,710212,1420424,2193.246793985367,0.0031940356275299564
90090,718208,718208,1436416,2213.7653822898865,0.0031919295124680502
91091,726210,726210,1452420,2233.684655189514,0.0031905471587378997
92092,734214,734214,1468428,2253.8622431755066,0.003189582421327941
93093,742218,742218,1484436,2274.2748651504517,0.0031887740315141855
94094,750220,750220,1500440,2294.7043042182922,0.003187344154866878
95095,758226,758226,1516452,2315.1024639606476,0.003187178283042158
96096,766222,766222,1532444,2335.378538131714,0.003175734944306896
97097,774226,774226,1548452,2355.9910740852356,0.0031753908915561624
98098,782230,782230,1564460,2376.6198251247406,0.0031747442990308627
99099,790236,790236,1580472,2397.168914079666,0.0031742060837132158
100100,798240,798240,1596480,2417.4661922454834,0.003173520406562602
101101,806244,806244,1612488,2437.890110015869,0.0031727931418572553
102102,814244,814244,1628488,2458.343760251999,0.0031697189806436654
103103,822246,822246,1644492,2478.8211481571198,0.003168674218613887
104104,830254,830254,1660508,2499.3358421325684,0.0031686091006122297
105105,838258,838258,1676516,2519.7117083072662,0.003167554779793136
106106,846258,846258,1692516,2540.084396123886,0.003165012063618633
107107,854264,854264,1708528,2560.4339730739594,0.003164593297697138
108108,862270,862270,1724540,2580.6224040985107,0.003163373959978344
109109,870274,870274,1740548,2601.0163803100586,0.003162213311952655
110110,878278,878278,1756556,2621.4079349040985,0.0031614803992852103
111111,886272,886272,1772544,2641.696823120117,0.003141903876894503
112112,894276,894276,1788552,2662.101217985153,0.0031413617871294264
113113,902282,902282,1804564,2683.194875240326,0.0031409441344294464
114114,910288,910288,1820576,2703.6829130649567,0.0031389806372317253
115115,918296,918296,1836592,2724.13276219368,0.003138916350508225
116116,926288,926288,1852576,2744.5488460063934,0.0031327863871410955
117117,934290,934290,1868580,2765.029587984085,0.0031321677033702144
118118,942288,942288,1884576,2785.4293920993805,0.0031239426625688793
119119,950294,950294,1900588,2805.724534034729,0.003123813610727666
120120,958296,958296,1916592,2826.111825942993,0.003122707012153114
121121,966300,966300,1932600,2846.4586210250854,0.0031217578343785135
122122,974308,974308,1948616,2866.8674092292786,0.003121695872323471
123123,982310,982310,1964620,2886.4738640785217,0.003117781319815549
124124,990314,990314,1980628,2903.5492658615112,0.003117078096693149
125125,998312,998312,1996624,2919.2882690429688,0.0030978669001342496
126126,1006314,1006314,2012628,2940.340908050537,0.0030973435186751885
127127,1014302,1014302,2028604,2956.7732491493225,0.003073490926908562
128128,1022306,1022306,2044612,2974.314189195633,0.0030728936126251938
129129,1030312,1030312,2060624,2991.304661989212,0.003072279901971342
130130,1038312,1038312,2076624,3008.705105304718,0.0030692137333971914
131131,1046312,1046312,2092624,3025.747143983841,0.0030628718395746546
132132,1054316,1054316,2108632,3042.5695600509644,0.0030626049683633028
133133,1062318,1062318,2124636,3059.319144010544,0.0030614239349233685
134134,1070324,1070324,2140648,3076.082262992859,0.0030607663411501562
135135,1078326,1078326,2156652,3092.8240311145782,0.003056192163057858
136136,1086330,1086330,2172660,3109.6917581558228,0.0030554855493392097
137137,1094332,1094332,2188664,3126.3019211292267,0.0030528913102898514
138138,1102336,1102336,2204672,3143.1099841594696,0.0030524231387971668
139139,1110320,1110320,2220640,3159.7179460525513,0.0029932763609394897
140140,1118322,1118322,2236644,3176.5145070552826,0.002992038129377761
141141,1126322,1126322,2252644,3193.6119890213013,0.0029907684875070117
142142,1134326,1134326,2268652,3210.2704231739044,0.0029904134062235244
143143,1142334,1142334,2284668,3227.2503321170807,0.002990355054862448
144144,1150274,1150274,2300548,3243.9866881370544,0.002012816312344512
145145,1158270,1158270,2316540,3261.2793600559235,0.0020119406653975602
146146,1166272,1166272,2332544,3278.0441200733185,0.002011584019783186
147147,1174272,1174272,2348544,3294.758646965027,0.002011063528698287
148148,1182274,1182274,2364548,3311.7303080558777,0.0020094083811272867
149149,1190278,1190278,2380556,3328.7029650211334,0.002008088009461062
150150,1198278,1198278,2396556,3345.64887714386,0.0020074933490832336
151151,1206278,1206278,2412556,3362.53417801857,0.0020013584198750323
152152,1214280,1214280,2428560,3379.6189329624176,0.0020009602176287444
153153,1222278,1222278,2444556,3396.2066271305084,0.0020004824400530197
154154,1230280,1230280,2460560,3413.147203207016,0.001999698710278608
155155,1238282,1238282,2476564,3429.8134059906006,0.0019974819515482523
156156,1246284,1246284,2492568,3446.621251106262,0.0019954700001107994
157157,1254288,1254288,2508576,3466.7952089309692,0.0019949774505221285
158158,1262294,1262294,2524588,3483.4357781410217,0.0019948639728681883
159159,1270296,1270296,2540592,3500.193377017975,0.001992493851503241
160160,1278296,1278296,2556592,3516.9355058670044,0.0019910818828066112
161161,1286296,1286296,2572592,3533.3914999961853,0.001990525974179036
162162,1294298,1294298,2588596,3549.932160139084,0.0019899763447028818
163163,1302304,1302304,2604608,3566.5633840560913,0.001989778033021139
164164,1310306,1310306,2620612,3582.951446056366,0.001987860594454105
165165,1318310,1318310,2636620,3599.49537730217,0.0019856102735502645
166166,1326314,1326314,2652628,3616.3786959648132,0.0019853122539643664
167167,1334294,1334294,2668588,3633.034252166748,0.0019845467122650007
168168,1342296,1342296,2684592,3649.7457191944122,0.001983988999199937
169169,1350296,1350296,2700592,3666.3260910511017,0.0019832599737128476
170170,1358296,1358296,2716592,3683.2027299404144,0.0019822367485176073
171171,1366302,1366302,2732604,3700.259552001953,0.0019820038542093243
172172,1374296,1374296,2748592,3717.1768839359283,0.001975770999706583
173173,1382298,1382298,2764596,3733.780612230301,0.0019751653635466937
174174,1390306,1390306,2780612,3750.534632921219,0.001975131224753568
175175,1398308,1398308,2796616,3767.1775040626526,0.0019732179353013635
176176,1406314,1406314,2812628,3783.911733150482,0.0019730018630070845
177177,1414314,1414314,2828628,3800.538777112961,0.00197175693938334
178178,1422318,1422318,2844636,3817.0367748737335,0.001971350076928502
179179,1430294,1430294,2860588,3833.829648256302,0.0019710092110472033
180180,1438296,1438296,2876592,3850.5510590076447,0.001970497571164742
181181,1446300,1446300,2892600,3867.3309450149536,0.001970207800695789
182182,1454302,1454302,2908604,3884.154228925705,0.0019698553005582653
183183,1462304,1462304,2924608,3900.8747022151947,0.0019684526305354666
184184,1470304,1470304,2940608,3917.8294270038605,0.0019675469575304305
185185,1478304,1478304,2956608,3934.805018186569,0.001961568781553069
186186,1486304,1486304,2972608,3951.380027294159,0.0019609681348811137
187187,1494304,1494304,2988608,3968.293745994568,0.0019605961279012263
188188,1502308,1502308,3004616,3985.004536151886,0.001960414721907
189189,1510304,1510304,3020608,4001.6913232803345,0.001955682830157457
190190,1518288,1518288,3036576,4018.4278621673584,0.0018290587649971712
191191,1526288,1526288,3052576,4035.2328720092773,0.0018285622536495794
192192,1534286,1534286,3068572,4052.7553882598877,0.0018279729501955444
193193,1542290,1542290,3084580,4069.5769662857056,0.0018277351427968824
194194,1550292,1550292,3100584,4086.3071212768555,0.0018274786398251308
195195,1558286,1558286,3116572,4103.909521102905,0.0018202762457804056
196196,1566288,1566288,3132576,4120.583676099777,0.0018199382229795447
197197,1574284,1574284,3148568,4137.250628232956,0.0018194191143265925
198198,1582282,1582282,3164564,4154.219115018845,0.0018179514390794793
199199,1590284,1590284,3180568,4170.845966100693,0.0018174982797063421
200200,1598286,1598286,3196572,4187.5428121089935,0.001817199250581325
201201,1606286,1606286,3212572,4203.965481996536,0.0018155416782974498
202202,1614286,1614286,3228572,4220.402921915054,0.0018150635587517172
203203,1622284,1622284,3244568,4237.092982053757,0.0018146104102925165
204204,1630282,1630282,3260564,4254.077873945236,0.0018138481937057804
205205,1638282,1638282,3276564,4270.717393159866,0.0018134473648387939
206206,1646282,1646282,3292564,4289.295325994492,0.0018130039461539127
207207,1654282,1654282,3308564,4308.083702087402,0.0018124156431440497
208208,1662282,1662282,3324564,4323.234523296356,0.0018118684238288552
209209,1670288,1670288,3340576,4344.794780254364,0.0018116208175342763
210210,1678278,1678278,3356556,4363.229255914688,0.0017842487068264745
211211,1686276,1686276,3372552,4381.167537927628,0.0017837964369391557
212212,1694274,1694274,3388548,4398.137850046158,0.0017833512392826378
213213,1702274,1702274,3404548,4415.227951049805,0.0017829008011176484
214214,1710278,1710278,3420556,4432.079571008682,0.0017825575887400191
215215,1718280,1718280,3436560,4449.0188620090485,0.0017822324680309976
216216,1726282,1726282,3452564,4465.793895959854,0.0017819373169913888
217217,1734282,1734282,3468564,4482.597526073456,0.0017811731831898214
218218,1742270,1742270,3484540,4499.925736904144,0.0017736832469381625
219219,1750268,1750268,3500536,4516.836786031723,0.0017728162365528988
220220,1758270,1758270,3516540,4533.880578041077,0.0017723042274155887
221221,1766274,1766274,3532548,4551.235173225403,0.001772128845914267
222222,1774268,1774268,3548536,4568.29233789444,0.0017555912017996889
223223,1782274,1782274,3564548,4585.513379096985,0.001755460407366627
224224,1790278,1790278,3580556,4602.482076883316,0.001755268820488709
225225,1798270,1798270,3596540,4619.510792970657,0.0017527921991131734
226226,1806270,1806270,3612540,4636.596781015396,0.0017524571885587648
227227,1814270,1814270,3628540,4653.705342054367,0.0017520185338071315
228228,1822270,1822270,3644540,4670.732409238815,0.0017516719944978831
229229,1830270,1830270,3660540,4687.642586231232,0.00175064630820998
230230,1838260,1838260,3676520,4704.435386180878,0.0017384937400493072
231231,1846260,1846260,3692520,4721.3544199466705,0.0017382769292453304
232232,1854262,1854262,3708524,4738.21338391304,0.0017375549614371266
233233,1862262,1862262,3724524,4754.949258089066,0.001737171793138259
234234,1870264,1870264,3740528,4771.908514022827,0.0017368439876008779
235235,1878258,1878258,3756516,4789.064076185226,0.001719924743156298
236236,1886256,1886256,3772512,4806.272969961166,0.0017192213144880952
237237,1894254,1894254,3788508,4823.683954954147,0.0017184096759592649
238238,1902254,1902254,3804508,4841.083744049072,0.0017177561403514119
239239,1910256,1910256,3820512,4858.519937038422,0.0017174608619825449
240240,1918256,1918256,3836512,4876.424715995789,0.0017168429912999272
241241,1926258,1926258,3852516,4893.527106046677,0.0017165755270980299
242242,1934258,1934258,3868516,4911.228709220886,0.0017115326518251095
243243,1942258,1942258,3884516,4928.559731006622,0.0017110288117692107
244244,1950258,1950258,3900516,4947.375263929367,0.0017106643608713057
245245,1958262,1958262,3916524,4964.439789056778,0.0017102404053730424
246246,1966262,1966262,3932524,4981.468001127243,0.00170963441269123
247247,1974262,1974262,3948524,4998.767392158508,0.0017078480959753506
248248,1982260,1982260,3964520,5015.841014146805,0.001707385063127731
249249,1990264,1990264,3980528,5032.906541109085,0.0017068949509848608
250250,1998272,1998272,3996544,5050.085644006729,0.0017068657853087643
251251,2006280,2006280,4012560,5067.311565160751,0.0017068366214516573
252252,2014280,2014280,4028560,5084.548743963242,0.0017067675798898563
253253,2022276,2022276,4044552,5101.971196174622,0.001706244436718407
254254,2030278,2030278,4060556,5119.445343971252,0.0017060651443898678
255255,2038274,2038274,4076548,5136.672102212906,0.0017034619177138666
256256,2046276,2046276,4092552,5153.91082906723,0.001703102683677571
257257,2054280,2054280,4108560,5171.499056100845,0.0017029346654453548
258258,2062280,2062280,4124560,5188.6377210617065,0.0017009885996230878
259259,2070278,2070278,4140556,5205.955778121948,0.001700369903119281
260260,2078282,2078282,4156564,5223.03466296196,0.0016999990621116012
261261,2086280,2086280,4172560,5240.277059078217,0.001696808276392403
262262,2094280,2094280,4188560,5257.764703989029,0.0016963875477813417
263263,2102280,2102280,4204560,5275.112316131592,0.0016959879958449164
264264,2110266,2110266,4220532,5292.422820091248,0.0016304316395689966
265265,2118268,2118268,4236536,5309.677940130234,0.0016300593688356457
266266,2126266,2126266,4252532,5327.434041023254,0.0016292834352498176
267267,2134268,2134268,4268536,5345.005412101746,0.0016291520678350935
268268,2142268,2142268,4284536,5362.532751083374,0.0016285408582916716
269269,2150270,2150270,4300540,5379.830721139908,0.0016279315768770175
270270,2158270,2158270,4316540,5397.139317035675,0.0016276572932838462
271271,2166270,2166270,4332540,5414.611145019531,0.0016271129170490894
272272,2174276,2174276,4348552,5435.4828979969025,0.0016270623927994166
273273,2182272,2182272,4364544,5453.294513940811,0.0016238256575888954
274274,2190272,2190272,4380544,5470.736958026886,0.0016232460602623178
275275,2198274,2198274,4396548,5487.744978904724,0.001619024551473558
276276,2206276,2206276,4412552,5504.918660163879,0.0016186785196623532
277277,2214278,2214278,4428556,5522.032348155975,0.0016184256310225464
278278,2222282,2222282,4444564,5539.12607216835,0.0016151934614754282
279279,2230286,2230286,4460572,5556.24990105629,0.0016149238745128969
280280,2238290,2238290,4476580,5573.244082927704,0.0016147779751918279
281281,2246290,2246290,4492580,5590.692441225052,0.0016115047747007338
282282,2254288,2254288,4508576,5607.719774007797,0.0016109825774037745
283283,2262290,2262290,4524580,5624.587826967239,0.0016105822505778633
284284,2270294,2270294,4540588,5641.221815109253,0.0016103760590340244
285285,2278294,2278294,4556588,5658.000732898712,0.001607112399142352
286286,2286296,2286296,4572592,5674.791819095612,0.0016067559117800556
287287,2294294,2294294,4588588,5691.802468061447,0.0016060873331298353
288288,2302298,2302298,4604596,5706.12522816658,0.0016058877008617856
289289,2310304,2310304,4620608,5720.3622789382935,0.0016057356206147233
290290,2318304,2318304,4636608,5734.615180015564,0.0016045548145484645
291291,2326304,2326304,4652608,5748.958498001099,0.001604182996743475
292292,2334304,2334304,4668608,5763.07520198822,0.0016038216544984607
293293,2342306,2342306,4684612,5777.285624027252,0.0016035226526582846
294294,2350310,2350310,4700620,5791.413829088211,0.0016032215899031144
295295,2358306,2358306,4716612,5805.5444622039795,0.0015998240323824575
296296,2366308,2366308,4732616,5819.955288171768,0.001599470564542571
297297,2374306,2374306,4748612,5834.293165206909,0.001598995724634733
298298,2382310,2382310,4764620,5848.977005004883,0.0015988195591489784
299299,2390316,2390316,4780632,5863.121335029602,0.0015985606041795108
300300,2398316,2398316,4796632,5877.2717361450195,0.001591165439094766
301301,2406318,2406318,4812636,5891.117640972137,0.001590890218722052
302302,2414322,2414322,4828644,5905.160263299942,0.0015896857512416318
303303,2422320,2422320,4844640,5919.1743841171265,0.0015891138937149663
304304,2430326,2430326,4860652,5933.477260112762,0.0015889955320744775
305305,2438334,2438334,4876668,5947.5183029174805,0.0015889690876065288
306306,2446340,2446340,4892680,5961.813734292984,0.0015889305341261206
307307,2454348,2454348,4908696,5976.074901103973,0.0015889040896581719
308308,2462356,2462356,4924712,5990.2950320243835,0.0015888776451902231
309309,2470364,2470364,4940728,6004.4217710494995,0.0015888512025412638
310310,2478372,2478372,4956744,6018.487023115158,0.0015888247617112938
311311,2486358,2486358,4972716,6032.93607711792,0.0015884447802818613
312312,2494360,2494360,4988720,6047.2323660850525,0.0015882031184446532
313313,2502360,2502360,5004720,6061.608931064606,0.0015876603010838153
314314,2510360,2510360,5020720,6082.786150217056,0.0015873239844950149
315315,2518362,2518362,5036724,6098.6028571128845,0.001587023130923626
316316,2526364,2526364,5052728,6113.883697271347,0.0015843082201172365
317317,2534360,2534360,5068720,6130.986830234528,0.0015821121123735793
318318,2542364,2542364,5084728,6147.470840215683,0.001581909700689721
319319,2550366,2550366,5100732,6162.920146942139,0.0015816230297787115
320320,2558366,2558366,5116732,6177.846074104309,0.001581221898959484
321321,2566368,2566368,5132736,6193.280166149139,0.0015809911437827395
322322,2574370,2574370,5148740,6208.609596252441,0.0015805898983671796
323323,2582372,2582372,5164744,6223.669548034668,0.001580210380780045
324324,2590372,2590372,5180744,6240.285578966141,0.0015794757582625607
325325,2598374,2598374,5196748,6261.034747123718,0.0015786115036462434
326326,2606376,2606376,5212752,6281.012468099594,0.0015783915932843229
327327,2614380,2614380,5228760,6297.827601909637,0.0015779262357682455
328328,2622382,2622382,5244764,6314.458093166351,0.0015761101349198725
329329,2630382,2630382,5260764,6331.048300981522,0.0015738257479824824
330330,2638384,2638384,5276768,6347.67218708992,0.001573407114847214
331331,2646382,2646382,5292764,6364.542471885681,0.0015729379829281243
332332,2654384,2654384,5308768,6381.197369098663,0.0015699497344030533
333333,2662384,2662384,5324768,6398.05962395668,0.0015693794903199887
334334,2670388,2670388,5340776,6415.056812047958,0.0015690304262534482
335335,2678390,2678390,5356780,6432.367347955704,0.0015656094219593797
336336,2686392,2686392,5372784,6448.893322944641,0.0015654728395020356
337337,2694380,2694380,5388760,6465.169562101364,0.0015273121334757889
338338,2702380,2702380,5404760,6481.716746091843,0.001526631205706508
339339,2710380,2710380,5420760,6498.221784114838,0.0015262289543898078
340340,2718382,2718382,5436764,6514.7818722724915,0.001525617808511015
341341,2726384,2726384,5452768,6531.204698085785,0.0015250881988322362
342342,2734384,2734384,5468768,6547.587015867233,0.0015214038467092905
343343,2742382,2742382,5484764,6564.125246047974,0.0015210888577712467
344344,2750382,2750382,5500764,6580.590044260025,0.0015207139440462925
345345,2758386,2758386,5516772,6597.162959098816,0.0015175961143540917
346346,2766388,2766388,5532776,6613.452949047089,0.0015174393429333577
347347,2774390,2774390,5548780,6630.442687034607,0.0015164504893618869
348348,2782388,2782388,5564776,6647.356224060059,0.0015159080267039826
349349,2790378,2790378,5580756,6664.287879943848,0.0014498840791929979
350350,2798378,2798378,5596756,6681.013375043869,0.001449638717531343
351351,2806382,2806382,5612764,6697.5081951618195,0.0014475410043814918
352352,2814384,2814384,5628768,6714.145865917206,0.0014472559469140833
353353,2822388,2822388,5644776,6730.593089103699,0.0014468089793808758
354354,2830392,2830392,5660784,6747.419090986252,0.0014466271350102033
355355,2838396,2838396,5676792,6763.923634052277,0.0014459622179856524
356356,2846400,2846400,5692800,6780.54120016098,0.001445618658181047
357357,2854404,2854404,5708808,6797.100882053375,0.0014453617131948704
358358,2862406,2862406,5724812,6813.816833972931,0.0014429976654355414
359359,2870410,2870410,5740820,6829.9813911914825,0.0014426911966438638
360360,2878414,2878414,5756828,6846.2686240673065,0.0014414297038456425
361361,2886418,2886418,5772836,6862.638086080551,0.0014413742846954847
362362,2894422,2894422,5788844,6879.103418111801,0.0014411463871510932
363363,2902422,2902422,5804844,6895.7084720134735,0.001440830734281917
364364,2910414,2910414,5820828,6912.146491289139,0.001423713274562033
365365,2918416,2918416,5836832,6928.87047123909,0.0014233820620574988
366366,2926418,2926418,5852836,6945.911933898926,0.0014229860480554635
367367,2934420,2934420,5868840,6962.763422966003,0.0014224668320821365
368368,2942420,2942420,5884840,6979.451199054718,0.0014221154469851172
369369,2950420,2950420,5900840,6996.133891105652,0.0014214807051757816
370370,2958420,2958420,5916840,7012.702589035034,0.0014212034038791899
371371,2966426,2966426,5932852,7029.49631524086,0.0014209827877493808
372372,2974426,2974426,5948852,7046.232782125473,0.0014177400043990929
373373,2982428,2982428,5964856,7062.976998090744,0.0014174136085784994
374374,2990430,2990430,5980860,7079.657286167145,0.001417136205418501
375375,2998432,2998432,5996864,7096.292495250702,0.0014169327459967462
376376,3006434,3006434,6012868,7112.931990146637,0.0014167562585498672
377377,3014438,3014438,6028876,7129.852472066879,0.0014161132839944912
378378,3022444,3022444,6044888,7146.961318254471,0.0014160477185214404
379379,3030450,3030450,6060900,7164.131192207336,0.001415953744071885
380380,3038458,3038458,6076916,7181.032028198242,0.0014159303373162402
381381,3046466,3046466,6092932,7197.704263210297,0.001415906928741606
382382,3054448,3054448,6108896,7214.210344076157,0.001091110903871595
383383,3062442,3062442,6124884,7230.553340911865,0.0010908970216405578
384384,3070440,3070440,6140880,7247.001633167267,0.0010904486116487533
385385,3078442,3078442,6156884,7263.255464076996,0.0010902238100243267
386386,3086444,3086444,6172888,7279.616072893143,0.0010897791744355345
387387,3094448,3094448,6188896,7296.124223947525,0.0010882545248023234
388388,3102456,3102456,6204912,7312.5552570819855,0.0010882354035857134
389389,3110458,3110458,6220916,7329.119206190109,0.001086270769519615
390390,3118462,3118462,6236924,7345.767804861069,0.0010859486683330033
391391,3126466,3126466,6252932,7362.300738096237,0.00108435772563098
392392,3134466,3134466,6268932,7379.657177209854,0.0010841186303878203
393393,3142472,3142472,6284944,7396.274076223373,0.0010839623300853418
394394,3150476,3150476,6300952,7412.931876182556,0.0010824661985679995
395395,3158482,3158482,6316964,7429.9169862270355,0.0010808389924932271
396396,3166484,3166484,6332968,7446.371974229813,0.0010806159607454902
397397,3174484,3174484,6348968,7462.836834192276,0.0010803574386955006
398398,3182488,3182488,6364976,7479.322140216827,0.001077916791473399
399399,3190494,3190494,6380988,7495.821266889572,0.0010778878422570415
400400,3198496,3198496,6396992,7512.261138916016,0.001076239044778049
401401,3206504,3206504,6413008,7528.891694068909,0.001076220027243835
402402,3214510,3214510,6429020,7545.3054258823395,0.001076162110621226
403403,3222512,3222512,6445024,7561.8538200855255,0.0010746818861662177
404404,3230516,3230516,6461032,7578.46585226059,0.001074563164365827
405405,3238516,3238516,6477032,7593.082453012466,0.0010714926611399278
406406,3246520,3246520,6493040,7607.215425014496,0.001071327524186927
407407,3254524,3254524,6509048,7621.2485382556915,0.001071103415597463
408408,3262532,3262532,6525064,7635.2091290950775,0.0010710844417189946
409409,3270526,3270526,6541052,7649.197813034058,0.0010488872685527895
410410,3278528,3278528,6557056,7663.3746790885925,0.001048572488798527
411411,3286532,3286532,6573064,7677.331822156906,0.0010484558133612154
412412,3294534,3294534,6589068,7691.325779914856,0.0010467718948348192
413413,3302542,3302542,6605084,7705.382393121719,0.0010467531174072064
414414,3310546,3310546,6621092,7719.521688222885,0.001046351333570783
415415,3318550,3318550,6637100,7733.6123032569885,0.0010462118807481602
416416,3326554,3326554,6653108,7747.658348083496,0.0010458358192408923
417417,3334558,3334558,6669116,7761.783930063248,0.0010456346044520615
418418,3342564,3342564,6685128,7776.630259037018,0.0010455685260239989
419419,3350566,3350566,6701132,7790.840553998947,0.0010443323062645504
420420,3358566,3358566,6717132,7804.037887096405,0.001040607676259242
421421,3366572,3366572,6733144,7816.821014165878,0.0010394996734248707
422422,3374576,3374576,6749152,7828.644674062729,0.0010394340370112332
423423,3382578,3382578,6765156,7840.061057090759,0.0010390969546278939
424424,3390582,3390582,6781164,8730.009188175201,0.0010383519584138412
425425,3398586,3398586,6797172,8770.025446176529,0.0010381912361481227
426426,3406592,3406592,6813184,9708.871412992477,0.0010381021638750099
427427,3414598,3414598,6829196,9760.416160106659,0.0010364648824179312
428428,3422604,3422604,6845208,9809.55641913414,0.0010364300615037791
429429,3430612,3430612,6861224,9856.093774080276,0.0010364113713876577
430430,3438582,3438582,6877164,10793.070572137833,0.001035652005157317
431431,3446574,3446574,6893148,11731.227354049683,0.0010354389087297022
432432,3454572,3454572,6909144,11779.0992770195,0.0010352147255616728
433433,3462572,3462572,6925144,11827.287668943405,0.0010349030962970573
434434,3470574,3470574,6941148,11875.54084610939,0.001034762117342325
435435,3478578,3478578,6957156,11923.957799911499,0.0010304359821020626
436436,3486578,3486578,6973156,11969.206002950668,0.001030145276672556
437437,3494578,3494578,6989156,12008.625719070435,0.001029986282446771
438438,3502578,3502578,7005156,12047.917563199997,0.0010296831369487336
439439,3510578,3510578,7021156,12087.398347139359,0.0010294921066815732
440440,3518580,3518580,7037160,12126.831684112549,0.0010292169099557213
441441,3526586,3526586,7053172,12166.268202066422,0.0010281007762387162
442442,3534584,3534584,7069168,12207.354279994965,0.0010278287845721934
443443,3542588,3542588,7085176,12255.768394947052,0.001027759466524003
444444,3550588,3550588,7101176,12303.986257076263,0.0010273242187395226
445445,3558588,3558588,7117176,12343.947348117828,0.0010269018202961888
446446,3566592,3566592,7133184,12383.657984972,0.0010258773691020906
447447,3574600,3574600,7149200,12423.346771001816,0.001025862839014735
448448,3582600,3582600,7165200,12462.77928185463,0.001025500294417725
449449,3590604,3590604,7181208,12502.207864046097,0.0010253737618768355
450450,3598606,3598606,7197212,12549.487977981567,0.0010248327107547084
451451,3606608,3606608,7213216,12598.053055047989,0.0010245113480777945
452452,3614612,3614612,7229224,12640.942888975143,0.0010243594733765349
453453,3622614,3622614,7245228,12680.503710985184,0.001023686965709203
454454,3630612,3630612,7261224,12719.856669902802,0.001020976276777219
455455,3638614,3638614,7277228,12759.254215240479,0.0010208529365627328
456456,3646618,3646618,7293236,12798.718556880951,0.0010193845118919853
457457,3654624,3654624,7309248,12844.793382167816,0.0010193434627581155
458458,3662624,3662624,7325248,12892.995398283005,0.0010178529701079242
459459,3670624,3670624,7341248,12939.046565055847,0.0010176196847169194
460460,3678626,3678626,7357252,12978.418396234512,0.0010159905068576336
461461,3686630,3686630,7373260,13018.143195152283,0.0010158222321479116
462462,3694632,3694632,7389264,13057.54843711853,0.0010153273069590796
463463,3702630,3702630,7405260,13096.957174062729,0.0010134018884855323
464464,3710632,3710632,7421264,13142.07751917839,0.0010132872776011936
465465,3718638,3718638,7437276,13190.421263217926,0.0010129373767995276
466466,3726638,3726638,7453276,13236.221063137054,0.0010112805157405091
467467,3734640,3734640,7469280,13275.669817209244,0.0010112105101143243
468468,3742642,3742642,7485284,13315.23275899887,0.0010110324474226218
469469,3750644,3750644,7501288,13354.53630900383,0.0010108584974659607
470470,3758648,3758648,7517296,13394.379642248154,0.0010088782419188647
471471,3766654,3766654,7533308,13440.969098091125,0.0010081726832140703
472472,3774654,3774654,7549308,13489.46995306015,0.0010064310172310797
473473,3782652,3782652,7565304,13534.901252031326,0.0010042013782367576
474474,3790654,3790654,7581308,13574.33845615387,0.0010039999378932407
475475,3798654,3798654,7597308,13613.698937177658,0.0010037285992439138
476476,3806658,3806658,7613316,13653.040405035019,0.0010029168206528993
477477,3814664,3814664,7629328,13692.688824176788,0.0010028201540990267
478478,3822668,3822668,7645336,13738.137032032013,0.0010025952869909815
479479,3830674,3830674,7661348,13786.835989952087,0.0010024546627391828
480480,3838678,3838678,7677356,13832.195088148117,0.0010017106360464823
481481,3846682,3846682,7693364,13871.704196214676,0.0010015435291279573
482482,3854682,3854682,7709364,13911.20905303955,0.0010009937996073859
483483,3862686,3862686,7725372,13950.973443031311,0.001000810059849755
484484,3870690,3870690,7741380,13990.26261305809,0.0009995849741244456
485485,3878698,3878698,7757396,14036.033931970596,0.0009995707259804476
486486,3886700,3886700,7773400,14085.651568174362,0.0009975938992283773
487487,3894704,3894704,7789408,14134.4519469738,0.0009975597204174846
488488,3902708,3902708,7805416,14175.69886302948,0.0009969372786144959
489489,3910712,3910712,7821424,14215.298135995865,0.000996853421384003
490490,3918716,3918716,7837432,14254.853105306625,0.0009966324960259954
491491,3926712,3926712,7853424,14294.288234949112,0.000990809581708163
492492,3934708,3934708,7869416,14336.167111873627,0.000990558761259308
493493,3942710,3942710,7885420,14384.636595964432,0.0009899303477141075
494494,3950714,3950714,7901428,14433.421742200851,0.0009898680509650148
495495,3958718,3958718,7917436,14477.014634132385,0.000988856379990466
496496,3966718,3966718,7933436,14516.625042915344,0.0009883805414574454
497497,3974726,3974726,7949452,14556.115123033524,0.0009883664170047268
498498,3982730,3982730,7965460,14595.625297307968,0.0009871443271549651
499499,3990732,3990732,7981464,14639.716610193253,0.000986959392321296
500501,3998746,3998746,7997492,14688.38225197792,0.0009855586376943393
501502,4006746,4006746,8013492,14736.436348199844,0.0009854153340711491
502503,4014748,4014748,8029496,14775.886017084122,0.0009852476432570256
503504,4022752,4022752,8045504,14815.269476175308,0.000985146298262407
504505,4030754,4030754,8061508,14854.807982206345,0.000984854386842926
505506,4038758,4038758,8077516,14894.257657051086,0.000983491805527592
506507,4046758,4046758,8093516,14939.122663974762,0.000983297810307704
507508,4054760,4054760,8109520,14987.845247983932,0.0009831162606133148
508509,4062766,4062766,8125532,15035.81881403923,0.0009829304417507956
509510,4070766,4070766,8141532,15075.281742095947,0.0009806921661947854
510511,4078772,4078772,8157544,15114.572703123093,0.0009805874269659398
511512,4086772,4086772,8173544,15153.960842132568,0.000979198752247612
512513,4094774,4094774,8189548,15193.79343008995,0.000978812102403026
513514,4102774,4102774,8205548,15238.883230924606,0.0009764142669155262
514515,4110776,4110776,8221552,15287.32487821579,0.0009762646113813389
515516,4118778,4118778,8237556,15334.306031227112,0.0009761278070072876
516517,4126774,4126774,8253548,15373.730783939362,0.0009493963825661922
517518,4134776,4134776,8269552,15413.074673891068,0.0009493280758761102
518519,4142776,4142776,8285552,15452.600355148315,0.0009491663367953151
519520,4150776,4150776,8301552,15492.551743984222,0.0009487139668635791
520521,4158782,4158782,8317564,15539.289608001709,0.0009486762191954767
521522,4166782,4166782,8333564,15587.677145242691,0.0009469208653172245
522523,4174788,4174788,8349576,15633.250422000885,0.0009461805584578542
523524,4182794,4182794,8365588,15672.554786205292,0.000946139318330097
524525,4190794,4190794,8381588,15711.975147008896,0.0009450095403735759
525526,4198796,4198796,8397592,15751.490264177322,0.0009439536206627963
526527,4206804,4206804,8413608,15790.880368232727,0.0009439399509574287
527528,4214806,4214806,8429612,15838.177994012833,0.0009437927019462222
528529,4222806,4222806,8445612,15886.932890176773,0.0009434334406250855
529530,4230812,4230812,8461624,15931.936845064163,0.0009433613413420971
530531,4238812,4238812,8477624,15971.316534996033,0.0009428736811969429
531532,4246816,4246816,8493632,16011.182700157166,0.0009416256616532337
532533,4254820,4254820,8509640,16050.566263198853,0.0009415099575562635
533534,4262826,4262826,8525652,16090.129743099213,0.0009414267424290301
534535,4270828,4270828,8541656,16138.262183904648,0.0009396855257364223
535536,4278832,4278832,8557664,16186.984627962112,0.000939561026825686
536537,4286834,4286834,8573668,16232.412539243698,0.0009386116234963993
537538,4294838,4294838,8589676,16271.939949035645,0.0009385178182128584
538539,4302836,4302836,8605672,16311.244721889496,0.0009383368796989089
539540,4310842,4310842,8621684,16350.637172937393,0.0009360353487863904
540541,4318848,4318848,8637696,16390.202007055283,0.0009360047461086651
541542,4326852,4326852,8653704,16438.25026512146,0.0009355818092444679
542543,4334860,4334860,8669720,16487.070801258087,0.0009355682213936234
543544,4342850,4342850,8685700,16531.854471206665,0.0009354416870337445
544545,4350834,4350834,8701668,16571.07764315605,0.000935287396714557
545546,4358832,4358832,8717664,16610.857329130173,0.0009350223735964391
546547,4366836,4366836,8733672,16650.336185216904,0.0009348607400170295
547548,4374838,4374838,8749676,16692.475993156433,0.0009347176037408644
548549,4382842,4382842,8765684,16740.713244199753,0.0009332767294836231
549550,4390844,4390844,8781688,16789.11185312271,0.00093230374113773
550551,4398842,4398842,8797684,16831.128580093384,0.0009321678335254546
551552,4406838,4406838,8813676,16870.413310050964,0.0009291510104958434
552553,4414840,4414840,8829680,16909.731667995453,0.0009290200960094808
553554,4422844,4422844,8845688,16949.12661910057,0.0009281726743211038
554555,4430844,4430844,8861688,16990.59442305565,0.000927965518712881
555556,4438842,4438842,8877684,17038.834884166718,0.0009273104151361622
556557,4446844,4446844,8893688,17087.18335199356,0.0009257304718630621
557558,4454840,4454840,8909680,17129.83329319954,0.0009256047742383089
558559,4462840,4462840,8925680,17169.407524108887,0.0009255074110114947
559560,4470842,4470842,8941684,17208.812999248505,0.000925225440369104
560561,4478840,4478840,8957680,17248.395651102066,0.0009249370123143308
561562,4486842,4486842,8973684,17291.429239034653,0.0009247395591955865
562563,4494840,4494840,8989680,17339.64773106575,0.0009246206700481707
563564,4502842,4502842,9005684,17388.235463142395,0.0009234883455064846
564565,4510842,4510842,9021684,17429.31130504608,0.0009232895154127618
565566,4518842,4518842,9037684,17468.646822929382,0.0009230931336787762
566567,4526844,4526844,9053688,17508.084364175797,0.0009226015536114573
567568,4534834,4534834,9069668,17547.47334098816,0.0009093751996260835
568569,4542830,4542830,9085660,17590.0454351902,0.0009090259063668782
569570,4550836,4550836,9101672,17638.339558124542,0.0009089821687666699
570571,4558832,4558832,9117664,17687.25378894806,0.0009077969625650439
571572,4566838,4566838,9133676,17728.868302106857,0.0009077349477593089
572573,4574840,4574840,9149680,17768.480419158936,0.000907627885680995
573574,4582842,4582842,9165684,17808.16235113144,0.0009074847821466392
574575,4590846,4590846,9181692,17847.45920729637,0.0009073822875507176
575576,4598846,4598846,9197692,17889.758854150772,0.0009070969517779304
576577,4606852,4606852,9213704,17938.07600212097,0.0009059835974767338
577578,4614850,4614850,9229700,17986.487910985947,0.0009057977022166597
578579,4622854,4622854,9245708,18028.23484802246,0.0009056051912921248
579580,4630850,4630850,9261700,18067.61696410179,0.0009054635393113131
580581,4638850,4638850,9277700,18107.045896053314,0.0009052756449818844
581582,4646850,4646850,9293700,18146.507389068604,0.0009051240485860035
582583,4654846,4654846,9309692,18190.627222061157,0.0009049640957528027
583584,4662844,4662844,9325688,18238.9017059803,0.0009046371869771974
584585,4670846,4670846,9341692,18287.39178299904,0.0009037327199621359
585586,4678850,4678850,9357700,18327.765547037125,0.0009030440633068793
586587,4686850,4686850,9373700,18367.29949903488,0.0009029394441313343
587588,4694852,4694852,9389704,18406.56869506836,0.0009012899208755698
588589,4702852,4702852,9405704,18446.252885103226,0.0009002403166959994
589590,4710852,4710852,9421704,18490.810840129852,0.0009000735590234399
590591,4718852,4718852,9437704,18538.938153982162,0.0008999248875625199
591592,4726856,4726856,9453712,18587.309746026993,0.0008989851230580825
592593,4734862,4734862,9469724,18626.829208135605,0.0008989316320366925
593594,4742864,4742864,9485728,18666.270438194275,0.0008979182421171572
594595,4750864,4750864,9501728,18706.19402909279,0.0008977720117400168
595596,4758866,4758866,9517732,18745.713248968124,0.0008974718984973151
596597,4766868,4766868,9533736,18792.327729940414,0.0008973958811111515
597598,4774870,4774870,9549740,18840.436472177505,0.0008972552841441939
598599,4782872,4782872,9565744,18887.298187971115,0.0008970335384219652
599600,4790878,4790878,9581756,18926.95513010025,0.0008969699683802901
600601,4798882,4798882,9597764,18966.635987997055,0.0008968444672063924
601602,4806884,4806884,9613768,19005.992882966995,0.000896765533980215
602603,4814888,4814888,9629776,19045.520119190216,0.0008965864526544465
603604,4822890,4822890,9645780,19093.829936265945,0.0008964149019448087
604605,4830890,4830890,9661780,19142.140773057938,0.0008963353120634565
605606,4838892,4838892,9677784,19186.25747203827,0.0008962576703197556
606607,4846890,4846890,9693780,19225.554188013077,0.0008960813520388911
607608,4854890,4854890,9709780,19265.489710092545,0.0008958977268775925
608609,4862890,4862890,9725780,19304.965707063675,0.0008933877070376184
609610,4870888,4870888,9741776,19346.698933124542,0.0008932143391575664
610611,4878886,4878886,9757772,19395.215715169907,0.0008930918029363966
611612,4886886,4886886,9773772,19443.59343099594,0.0008928334718802944
612613,4894888,4894888,9789776,19485.716962099075,0.0008927152248361381
613614,4902888,4902888,9805776,19525.29750919342,0.0008862561899150023
614615,4910890,4910890,9821780,19564.82728409767,0.0008860937487042975
615616,4918896,4918896,9837792,19604.282044887543,0.0008860358138917945
616617,4926892,4926892,9853784,19649.401239156723,0.0008853000799717847
617618,4934894,4934894,9869788,19697.715180158615,0.0008844625026540598
618619,4942898,4942898,9885796,19745.33118224144,0.0008837350615067407
619620,4950902,4950902,9901804,19785.261074066162,0.0008837142704578582
620621,4958902,4958902,9917804,19825.039817094803,0.0008833849715301767
621622,4966904,4966904,9933808,19864.631578207016,0.0008832604999042815
622623,4974900,4974900,9949800,19905.731548309326,0.0008830837014102144
623624,4982904,4982904,9965808,19954.145275115967,0.0008828892132441979
624625,4990908,4990908,9981816,20002.590667963028,0.0008827619203657378
625626,4998908,4998908,9997816,20045.16315817833,0.0008825513741612667
626627,5006912,5006912,10013824,20084.91286087036,0.0008809281607682351
627628,5014920,5014920,10029840,20124.54239010811,0.0008809176779323025
628629,5022922,5022922,10045844,20164.23545408249,0.0008799858769634739
629630,5030930,5030930,10061860,20209.403027057648,0.0008799754050414776
630631,5038900,5038900,10077800,20258.08243727684,0.0008798092694632942
631632,5046898,5046898,10093796,20306.86972308159,0.0008796283636911539
632633,5054900,5054900,10109800,20347.23977613449,0.000879393139257445
633634,5062898,5062898,10125796,20386.791515111923,0.0008792235166765749
634635,5070896,5070896,10141792,20426.25981593132,0.0008791056843620026
635636,5078898,5078898,10157796,20465.761579990387,0.0008790046504145721
636637,5086902,5086902,10173804,20511.32465004921,0.0008780426087469095
637638,5094902,5094902,10189804,20559.88543200493,0.0008770557324169204
638639,5102902,5102902,10205804,20607.79978609085,0.0008768895768298535
639640,5110902,5110902,10221804,20647.26097726822,0.0008767732306296239
640641,5118906,5118906,10237812,21663.786453962326,0.0008764566446188837
641642,5126904,5126904,10253808,21695.78417992592,0.0008746307976252865
642643,5134902,5134902,10269804,21743.99830198288,0.0008737235275475541
643644,5142906,5142906,10285812,21792.2275390625,0.000873631979629863
644645,5150906,5150906,10301812,21840.549160003662,0.0008734312286833301
645646,5158910,5158910,10317820,21889.302610874176,0.0008724294184503378
646647,5166908,5166908,10333816,21932.939080953598,0.000872187460117857
647648,5174906,5174906,10349812,21972.494771003723,0.000871749676662148
648649,5182906,5182906,10365812,22012.128821134567,0.0008715918702364434
649650,5190906,5190906,10381812,22051.619173049927,0.0008692684477864532
650651,5198906,5198906,10397812,22091.025842905045,0.000869158599016373
651652,5206906,5206906,10413812,22132.831834077835,0.0008690624326845864
652653,5214908,5214908,10429816,22181.221370220184,0.0008688734214956639
653654,5222910,5222910,10445820,22229.79891705513,0.0008685203174536582
654655,5230912,5230912,10461824,22269.61724805832,0.0008684024614922237
655656,5238912,5238912,10477824,22309.140522003174,0.0008682145980856149
656657,5246916,5246916,10493832,22348.568348169327,0.0008678165577293839
657658,5254916,5254916,10509832,22388.423590898514,0.0008657190392113989
658659,5262916,5262916,10525832,22436.50910305977,0.0008656089521537069
659660,5270916,5270916,10541832,22484.769936084747,0.0008652367814647732
660661,5278916,5278916,10557832,22527.49671125412,0.0008650515519548208
661662,5286918,5286918,10573836,22567.17841887474,0.0008649126048112521
662663,5294920,5294920,10589840,22606.575864076614,0.0008647572740301257
663664,5302920,5302920,10605840,22646.312976121902,0.0008646683036204195
664665,5310920,5310920,10621840,22685.683002233505,0.0008631138698547147
665666,5318924,5318924,10637848,22733.211273908615,0.000862997374497354
666667,5326930,5326930,10653860,22781.427723169327,0.000862903365487
667668,5334930,5334930,10669860,22825.06713604927,0.000862723010868649
668669,5342932,5342932,10685864,22864.707436084747,0.0008625970876892097
669670,5350936,5350936,10701872,22904.225986003876,0.0008623064386483748
670671,5358936,5358936,10717872,22944.10759305954,0.0008620862809038954
671672,5366940,5366940,10733880,22983.551233053207,0.0008611601115262602
672673,5374942,5374942,10749884,23032.01819396019,0.0008610875465819845
673674,5382942,5382942,10765884,23080.413093090057,0.0008597278501838446
674675,5390946,5390946,10781892,23125.59328007698,0.000859617584865191
675676,5398948,5398948,10797896,23165.163246154785,0.0008594294940849068
676677,5406956,5406956,10813912,23204.715538978577,0.0008594196442572866
677678,5414958,5414958,10829916,23244.0772690773,0.0008581901365687372
678679,5422954,5422954,10845908,23284.42505812645,0.0008567920831410447
679680,5430956,5430956,10861912,23332.729908943176,0.0008566836386307841
680681,5438964,5438964,10877928,23380.98162007332,0.000856673825182952
681682,5446968,5446968,10893936,23423.146461963654,0.0008565980115236016
682683,5454968,5454968,10909936,23463.579627990723,0.0008563179580960423
683684,5462972,5462972,10925944,23503.13823413849,0.0008562543807784095
684685,5470976,5470976,10941952,23542.74988102913,0.0008561832255509216
685686,5478954,5478954,10957908,23585.623568058014,0.0004885468133579707
686687,5486954,5486954,10973908,23633.885631084442,0.0004885312555416021
687688,5494952,5494952,10989904,23682.26042699814,0.0004884694008069346
688689,5502956,5502956,11005912,23722.32472205162,0.0004884330282948213
689690,5510962,5510962,11021924,23762.13770699501,0.0004883275323663838
690691,5518970,5518970,11037940,23801.409679174423,0.0004883214969595429
691692,5526970,5526970,11053940,23840.733636140823,0.0004873328980465885
692693,5534974,5534974,11069948,23885.93261694908,0.0004872557437920477
693694,5542982,5542982,11085964,23934.489269018173,0.00048724971384217497
694695,5550988,5550988,11101976,23981.76428604126,0.00048690404582885094
695696,5558994,5558994,11117988,24021.24706196785,0.0004868499036092544
696697,5567000,5567000,11134000,24061.17277121544,0.00048683418754080776
697698,5575000,5575000,11150000,24100.782286167145,0.00048621058522257954
698699,5583008,5583008,11166016,24140.307128190994,0.0004862045643676538
699700,5591012,5591012,11182024,24187.985157251358,0.000486090570120723
700701,5599020,5599020,11198040,24236.37485909462,0.00048608454562781844
701702,5607026,5607026,11214052,24280.99907398224,0.00048585191871097777
702703,5615034,5615034,11230068,24320.529563188553,0.00048584589785605203
703704,5623038,5623038,11246076,24360.013911008835,0.0004857917065237416
704705,5631044,5631044,11262088,24399.715486049652,0.0004854812359553762
705706,5639052,5639052,11278104,24439.067890882492,0.00048547521873842925
706707,5647060,5647060,11294120,24487.72128510475,0.0004854691997024929
707708,5655066,5655066,11310132,24536.313909053802,0.00048529997729929164
708709,5663074,5663074,11326148,24581.787434101105,0.0004852939564443659
709710,5671080,5671080,11342160,24621.20397901535,0.0004852351630688645
710711,5679088,5679088,11358176,24660.72308921814,0.00048522914403292816
711712,5687094,5687094,11374188,24700.160380125046,0.00048503872312721796
712713,5695102,5695102,11390204,24739.835705041885,0.00048503270591027103
713714,5703110,5703110,11406220,24787.944179058075,0.0004850266886933241
714715,5711114,5711114,11422228,24836.970885276794,0.0004847092968702782
715716,5719120,5719120,11438240,24882.158541202545,0.0004843901679123519
716717,5727124,5727124,11454248,24921.597280979156,0.0004843768219870981
717718,5735132,5735132,11470264,24961.07811999321,0.00048437080840812996
718719,5743136,5743136,11486272,25000.571092128754,0.00048433721349283587
719720,5751140,5751140,11502280,25041.83252310753,0.00048311265345546417
720721,5759144,5759144,11518288,25090.192164182663,0.00048307914585166145
721722,5767152,5767152,11534304,25138.52984714508,0.00048307314136764035
722723,5775156,5775156,11550312,25181.760250091553,0.00048262222117045894
723724,5783158,5783158,11566316,25221.393742084503,0.0004825814648938831
724725,5791164,5791164,11582328,25261.01671719551,0.00048252823398797773
725726,5799168,5799168,11598336,25301.10906815529,0.00048247813720081467
726727,5807172,5807172,11614344,25345.975255012512,0.00048178317774727475
727728,5815178,5815178,11630356,25394.2626349926,0.0004812698589375941
728729,5823182,5823182,11646364,25441.943697929382,0.0004812419902009424
729730,5831188,5831188,11662376,25481.329730033875,0.0004811980288650375
730731,5839192,5839192,11678384,25520.82314491272,0.00048099536797963083
731732,5847196,5847196,11694392,25560.677588939667,0.0004809245747310342
732733,5855204,5855204,11710408,25600.01916217804,0.00048091858297993895
733734,5863210,5863210,11726420,25646.80811023712,0.00048083722685987595
734735,5871218,5871218,11742436,25695.021356105804,0.00048083123328979127
735736,5879222,5879222,11758444,25740.965832948685,0.0004803054871445056
736737,5887226,5887226,11774452,29149.92858695984,0.00048027525372162927
737738,5895232,5895232,11790464,30200.600572109222,0.00048020040958363097
738739,5903240,5903240,11806480,30227.800886154175,0.0004801944214705145
739740,5911244,5911244,11822488,30275.708631038666,0.0004796868815901689
740741,5919248,5919248,11838496,30323.439146995544,0.0004796551111212466
741742,5927256,5927256,11854512,31385.643567085266,0.0004796491230081301
742743,5935262,5935262,11870524,31425.515169143677,0.0004795731802005321
743744,5943270,5943270,11886540,31473.194390058517,0.000479567193906405
744745,5951276,5951276,11902552,31520.384471178055,0.0004794590076926397
745746,5959284,5959284,11918568,31559.34072613716,0.00047945301957952324
746747,5967290,5967290,11934580,31597.95636987686,0.0004794220094481716
747748,5975298,5975298,11950596,31632.23523902893,0.0004794160231540445
748749,5983300,5983300,11966600,31663.130172252655,0.0004786897825397318
749750,5991306,5991306,11982612,31693.100288152695,0.0004784565062436741
750751,5999314,5999314,11998628,31723.066598892212,0.00047845052722550463
751752,6007320,6007320,12014640,32801.68294906616,0.00047842448293522466
752753,6015328,6015328,12030656,32838.65291810036,0.0004784185002790764
753754,6023330,6023330,12046660,32886.27066612244,0.0004782024880114477
754755,6031336,6031336,12062672,32934.14724826813,0.00047818013081268873
755756,6039342,6039342,12078684,32973.397439956665,0.000478114903671667
756757,6047348,6047348,12094696,33012.13684415817,0.0004775594024977181
757758,6055352,6055352,12110704,33047.01950216293,0.000477536990729277
758759,6063356,6063356,12126712,33078.31833910942,0.0004774937842739746
759760,6071362,6071362,12142724,33108.33161020279,0.00047733319661347196
760761,6079370,6079370,12158740,33138.37141919136,0.0004773272248712601
761762,6087378,6087378,12174756,33168.27379608154,0.00047732124767208006
762763,6095384,6095384,12190768,33197.89035105705,0.0004773046548507409
763764,6103388,6103388,12206776,33228.596640110016,0.0004772537104145158
764765,6111396,6111396,12222792,33260.991595983505,0.00047724773685331456
765766,6119400,6119400,12238800,33293.88696408272,0.00047597509728802834
766767,6127408,6127408,12254816,33326.22133517265,0.0004759691291837953
767768,6135410,6135410,12270820,33356.29237604141,0.00047550812632835004
768769,6143416,6143416,12286832,33386.195674180984,0.00047549355986120645
769770,6151422,6151422,12302844,33416.04671216011,0.00047541476124024484
770771,6159428,6159428,12318856,34472.45931601524,0.0004753730972879566
771772,6167432,6167432,12334864,34500.42791008949,0.00047413084575964604
772773,6175440,6175440,12350880,34548.32572412491,0.0004741248885693494
773774,6183448,6183448,12366896,34596.17824792862,0.0004741189313790528
774775,6191456,6191456,12382912,34637.55771112442,0.0004741129760077456
775776,6199462,6199462,12398924,34676.552289009094,0.0004740321764984401
776777,6207470,6207470,12414940,34712.897887945175,0.0004740262211271329
777778,6215478,6215478,12430956,34744.813343048096,0.0004740202657558257
778779,6223484,6223484,12446968,34774.848922252655,0.00047364079910039436
779780,6231492,6231492,12462984,34804.91082215309,0.00047363484554807656
780781,6239500,6239500,12479000,34834.89660692215,0.00047362889017676935
781782,6247508,6247508,12495016,34865.18705511093,0.00047362293480546214
782783,6255514,6255514,12511028,34896.32366323471,0.00047358666961372364
783784,6263518,6263518,12527036,34928.728654146194,0.0004733412861241959
784785,6271522,6271522,12543044,34961.08521223068,0.0004733148161903955
785786,6279526,6279526,12559052,34992.64360499382,0.00047244069719454274
786787,6287534,6287534,12575068,35022.43455004692,0.00047243474909919314
787788,6295540,6295540,12591080,35052.335506916046,0.0004724247737613041
788789,6303542,6303542,12607084,35082.378151893616,0.0004723448619188275
789790,6311550,6311550,12623100,35114.129553079605,0.00047233891564246733
790791,6319554,6319554,12639108,35146.760196208954,0.0004722750327346148
791792,6327558,6327558,12655116,35179.38994216919,0.00047174390238069464
792793,6335564,6335564,12671128,35211.77236914635,0.00047171995356620755
793794,6343572,6343572,12687144,35243.83094501495,0.00047171400910883676
794795,6351578,6351578,12703156,35273.66798520088,0.0004716630937764421
795796,6359584,6359584,12719168,35303.4870390892,0.0004716340627055615
796797,6367592,6367592,12735184,35333.19844913483,0.00047162812006718013
797798,6375596,6375596,12751192,35363.188175201416,0.00047129185804806184
798799,6383604,6383604,12767208,35395.39837408066,0.00047128591722866986
799800,6391608,6391608,12783216,36337.24374914169,0.0004709599725174485
800801,6399612,6399612,12799224,36385.55161809921,0.00047090317275433335
801802,6407618,6407618,12815236,36433.87005996704,0.00047078953139134683
802803,6415626,6415626,12831252,36482.2177400589,0.00047078359239094425
803804,6423632,6423632,12847264,36530.5534620285,0.0004707266180048464
804805,6431636,6431636,12863272,36573.57706284523,0.0004703165432147216
805806,6439642,6439642,12879284,36613.74948811531,0.00047030903078848496
806807,6447650,6447650,12895300,36653.38501000404,0.0004703030917880824
807808,6455654,6455654,12911308,36692.977993011475,0.0004698860793723725
808809,6463662,6463662,12927324,36732.50613617897,0.0004698801458289381
809810,6471668,6471668,12943336,36774.69319701195,0.00046983763058960903
810811,6479676,6479676,12959352,36823.01365303993,0.00046983169704617467
811812,6487682,6487682,12975364,36872.10605597496,0.0004697885269706603
812813,6495688,6495688,12991376,36911.74848198891,0.00046963768545538187
813814,6503692,6503692,13007384,36951.19838690758,0.00046960089275671635
814815,6511698,6511698,13023396,36990.966296195984,0.00046929976997489575
815816,6519702,6519702,13039404,37030.37082219124,0.00046929093514336273
816817,6527706,6527706,13055412,37074.81984901428,0.00046860758811817504
817818,6535708,6535708,13071416,37123.73140621185,0.0004685616495407885
818819,6543712,6543712,13087424,37170.25539302826,0.0004683084898715606
819820,6551720,6551720,13103440,37210.0817630291,0.00046830256542307325
820821,6559726,6559726,13119452,37249.71259903908,0.0004682098478951957
821822,6567732,6567732,13135464,37289.512909173965,0.00046817872316751163
822823,6575740,6575740,13151480,37328.96297597885,0.0004681727987190243
823824,6583744,6583744,13167488,37372.588475227356,0.0004677721080952324
824825,6591750,6591750,13183500,37420.902664899826,0.000467756217403803
825826,6599758,6599758,13199516,37467.78899717331,0.0004677502947743051
826827,6607762,6607762,13215524,37507.26983189583,0.00046771320194238797
827828,6615766,6615766,13231532,37546.963905096054,0.00046739810386497993
828829,6623774,6623774,13247548,37586.57736802101,0.000467392181235482
829830,6631782,6631782,13263564,37626.69105005264,0.00046738626224396285
830831,6639788,6639788,13279576,37670.54360294342,0.0004668547244364163
831832,6647790,6647790,13295580,37718.924666166306,0.000466841764136916
832833,6655798,6655798,13311596,37765.75266313553,0.0004668358451453969
833834,6663800,6663800,13327600,37805.28789305687,0.0004661294660763815
834835,6671808,6671808,13343616,37844.944184064865,0.0004661235525418306
835836,6679814,6679814,13359628,37884.61462020874,0.0004661142920667771
836837,6687818,6687818,13375636,37924.281635046005,0.0004660368213080801
837838,6695826,6695826,13391652,37969.28200125694,0.0004660309077735292
838839,6703832,6703832,13407664,38017.747608184814,0.00046569005280616693
839840,6711840,6711840,13423680,38063.87196588516,0.000465684139271616
840841,6719846,6719846,13439692,38103.38572502136,0.0004656423843698576
841842,6727854,6727854,13455708,38142.914021253586,0.0004656364744732855
842843,6735858,6735858,13471716,38182.99486017227,0.00046499368727381807
843844,6743864,6743864,13487728,38222.675729990005,0.00046494998241541907
844845,6751868,6751868,13503736,38270.165424108505,0.00046484943231916986
845846,6759876,6759876,13519752,38318.64678311348,0.00046484352606057655
846847,6767884,6767884,13535768,38362.882246255875,0.00046483761798299383
847848,6775888,6775888,13551776,38402.36021518707,0.0004646759643947007
848849,6783894,6783894,13567788,38442.0363881588,0.0004646504676202312
849850,6791900,6791900,13583800,38481.7661011219,0.0004646014676836785
850851,6799904,6799904,13599808,38521.38666296005,0.0004638901991711464
851852,6807912,6807912,13615824,38569.967900276184,0.00046388429655053187
852853,6815918,6815918,13631836,38618.37799119949,0.00046354498226719443
853854,6823926,6823926,13647852,38661.56035900116,0.0004635390814655693
854855,6831932,6831932,13663864,38701.16893410683,0.0004635135082935449
855856,6839940,6839940,13679880,38740.95467209816,0.00046350760567293037
856857,6847946,6847946,13695892,38780.49541401863,0.0004632935597328469
857858,6855952,6855952,13711904,38821.10061907768,0.0004632747641153401
858859,6863958,6863958,13727916,38869.41204094887,0.0004632297441276023
859860,6871960,6871960,13743920,38917.90443611145,0.0004619726132659707
860861,6879966,6879966,13759932,38960.276305913925,0.00046195883260224946
861862,6887972,6887972,13775944,38999.613234996796,0.00046192014451662544
862863,6895980,6895980,13791960,39039.210487127304,0.00046191425280994736
863864,6903986,6903986,13807972,39078.93575191498,0.0004617027152562514
864865,6911990,6911990,13823980,39120.89724493027,0.00046168705557647627
865866,6919996,6919996,13839992,39169.371166944504,0.00046164057130226865
866867,6928002,6928002,13856004,39217.75461292267,0.0004616121314029442
867868,6936010,6936010,13872020,39258.92408800125,0.00046160624151525553
868869,6944016,6944016,13888032,39298.40399622917,0.0004614663357642712
869870,6952024,6952024,13904048,39338.00872921944,0.0004614604458765825
870871,6960030,6960030,13920060,39377.59418606758,0.00046140736230881885
871872,6968036,6968036,13936072,39419.82843327522,0.0004609444586094469
872873,6976044,6976044,13952088,39468.28677916527,0.000460938572359737
873874,6984052,6984052,13968104,39516.48235321045,0.00046093268611002713
874875,6992058,6992058,13984116,39557.06812500954,0.0004608896797435591
875876,7000062,7000062,14000124,39596.56774020195,0.00046082148219284136
876877,7008068,7008068,14016136,39636.04406619072,0.0004608111503330292
877878,7016076,7016076,14032152,39675.644517183304,0.00046080526590230875
878879,7024078,7024078,14048156,39718.4975001812,0.0004603683210007148
879880,7032086,7032086,14064172,39766.85031700134,0.0004603624383889837
880881,7040092,7040092,14080184,39815.12604999542,0.000460332306829514
881882,7048100,7048100,14096200,39855.802861213684,0.0004603264242177829
882883,7056106,7056106,14112212,39895.26611304283,0.0004601882246788591
883884,7064110,7064110,14128220,39934.93170619011,0.0004598875566443894
884885,7072118,7072118,14144236,39974.374791145325,0.00045988167403265834
885886,7080126,7080126,14160252,40019.02478790283,0.0004598757950589061
886887,7088130,7088130,14176260,40067.45554304123,0.00045964288256072905
887888,7096138,7096138,14192276,40115.22585296631,0.000459636999948998
888889,7104144,7104144,14208288,40154.8656129837,0.00045962293916090857
889890,7112150,7112150,14224300,40194.27179002762,0.0004595528334903065
890891,7120158,7120158,14240316,40233.821918964386,0.00045954695451655425
891892,7128166,7128166,14256332,40273.97229528427,0.000459541075542802
892893,7136172,7136172,14272344,40322.37455415726,0.00045949985906190705
893894,7144180,7144180,14288360,40370.95243501663,0.0004594939819071442
894895,7152188,7152188,14304376,40415.059591293335,0.00045948810475238133
895896,7160190,7160190,14320380,40454.80555224419,0.0004591798842739081
896897,7168198,7168198,14336396,40494.34504389763,0.00045917400711914524
897898,7176202,7176202,14352404,40534.1350672245,0.00045883221355325077
898899,7184204,7184204,14368408,40579.71904420853,0.00045849767957406584
899900,7192212,7192212,14384424,40627.980384111404,0.000458491802419303
900901,7200216,7200216,14400432,40675.388337135315,0.00045845372005715035
901902,7208222,7208222,14416444,40715.0090470314,0.00045841156315873377
902903,7216230,7216230,14432460,40754.600716114044,0.0004584056878229603
903904,7224236,7224236,14448472,40794.468662023544,0.00045809027324139606
904905,7232240,7232240,14464480,40834.33956003189,0.0004580686036206316
905906,7240242,7240242,14480484,40882.62641787529,0.00045609796688950155
906907,7248244,7248244,14496488,40930.9399061203,0.0004560612051136559
907908,7256250,7256250,14512500,40975.41834115982,0.000455464027254493
908909,7264258,7264258,14528516,41014.77144026756,0.00045545816828962415
909910,7272266,7272266,14544532,41054.24870014191,0.00045545231114374474
910911,7280274,7280274,14560548,41093.64589905739,0.0004554464521788759
911912,7288280,7288280,14576560,41134.8017270565,0.00045531292926170863
912913,7296286,7296286,14592572,41183.27155303955,0.0004552902282739524
913914,7304292,7304292,14608584,41231.74224901199,0.00045524379311245866
914915,7312300,7312300,14624600,41274.37511920929,0.00045523793778556865
915916,7320302,7320302,14640604,41313.750338077545,0.00045452674021362327
916917,7328308,7328308,14656616,41353.36093211174,0.00045451333789969794
917918,7336314,7336314,14672628,41392.82120394707,0.0004544685798464343
918919,7344320,7344320,14688640,41436.0244140625,0.0004544409894151613
919920,7352328,7352328,14704656,41484.639545202255,0.0004544351377262501
920921,7360330,7360330,14720660,42934.942090034485,0.00045409766062221024
921922,7368336,7368336,14736672,42974.26832795143,0.00045369234248937573
922923,7376342,7376342,14752684,43022.640416145325,0.00045368374412646517
923924,7384350,7384350,14768700,43071.0513279438,0.00045367789425654337
924925,7392356,7392356,14784712,43119.4507830143,0.0004531659997155657
925926,7400362,7400362,14800724,43167.73885798454,0.00045314658200368285
926927,7408368,7408368,14816736,43208.39494013786,0.0004527355940808775
927928,7416374,7416374,14832748,43248.05476307869,0.0004527189685177291
928929,7424380,7424380,14848760,43287.58693408966,0.0004526313605310861
929930,7432386,7432386,14864772,43327.11792206764,0.0004526073917077156
930931,7440392,7440392,14880784,43366.68169403076,0.00045254325232235715
931932,7448400,7448400,14896800,43406.90069723129,0.00045253740790940356
932933,7456406,7456406,14912812,43455.30004811287,0.000452276415671804
933934,7464410,7464410,14928820,43503.989349126816,0.00045225372741697356
934935,7472416,7472416,14944832,43544.86364507675,0.0004520683032751549
935936,7480422,7480422,14960844,43584.384154081345,0.00045206196773506235
936937,7488428,7488428,14976856,43624.11368393898,0.0004520454658631934
937938,7496436,7496436,14992872,43663.62138915062,0.0004520396250882186
938939,7504442,7504442,15008884,43709.17789912224,0.0004516753633652115
939940,7512450,7512450,15024900,43757.484850883484,0.00045166952440922614
940941,7520456,7520456,15040912,43802.36233115196,0.00045165317533246707
941942,7528460,7528460,15056920,43842.05725693703,0.0004514023512456333
942943,7536466,7536466,15072932,43881.64790511131,0.000451385460110032
943944,7544474,7544474,15088948,43921.16597414017,0.0004513796247920254
944945,7552480,7552480,15104960,43960.502808094025,0.0004513426283665467
945946,7560484,7560484,15120968,44004.88704299927,0.0004506638324528467
946947,7568490,7568490,15136980,44053.31239295006,0.00045060885895509273
947948,7576496,7576496,15152992,44099.642952919006,0.0004505939650698565
948949,7584502,7584502,15169004,44139.38607907295,0.0004504659118538257
949950,7592510,7592510,15185020,44178.97829914093,0.0004504600783548085
950951,7600514,7600514,15201028,44218.53163123131,0.0004503800446400419
951952,7608522,7608522,15217044,44258.057749032974,0.0004503742129600141
952953,7616524,7616524,15233048,44305.11050701141,0.0004499941278481856
953954,7624528,7624528,15249056,44353.3977971077,0.00044946618072572164
954955,7632532,7632532,15265064,44397.61898112297,0.0004494289805734297
955956,7640536,7640536,15281072,44437.19870519638,0.00044814360444433987
956957,7648538,7648538,15297076,44476.842803001404,0.00044809312021243386
957958,7656546,7656546,15313092,44516.31602811813,0.0004480873012653319
958959,7664552,7664552,15329104,44555.99882221222,0.000447990290922462
959960,7672558,7672558,15345116,44602.55081009865,0.0004479553590499563
960961,7680566,7680566,15361132,44651.010788202286,0.00044794954010285437
961962,7688570,7688570,15377140,44696.34128808975,0.0004476327812881209
962963,7696576,7696576,15393152,44736.59025621414,0.0004476048379729036
963964,7704578,7704578,15409156,44775.99540805817,0.0004468033857847331
964965,7712584,7712584,15425168,44815.5469250679,0.0004467752769414801
965966,7720588,7720588,15441176,44857.48396420479,0.00044629945114138536
966967,7728592,7728592,15457184,44905.65909194946,0.0004462654651433695
967968,7736600,7736600,15473200,44954.1609249115,0.0004462596534722252
968969,7744606,7744606,15489212,44995.49449300766,0.0004462425695237471
969970,7752614,7752614,15505228,45035.01245903969,0.00044623675785260275
970971,7760620,7760620,15521240,45074.56973528862,0.0004462031174625736
971972,7768624,7768624,15537248,45114.179303884506,0.00044564121708390303
972973,7776632,7776632,15553264,45158.33217716217,0.0004456354108697269
973974,7784634,7784634,15569268,45206.72168803215,0.00044560562855622265
974975,7792640,7792640,15585280,45255.26041817665,0.0004454491390788462
975976,7800648,7800648,15601296,45295.24021100998,0.0004454433346836595
976977,7808654,7808654,15617308,45334.96514201164,0.00044540714588947594
977978,7816660,7816660,15633320,45374.48662495613,0.000445006946392823
978979,7824668,7824668,15649336,45414.03167104721,0.0004450011401786469
979980,7832676,7832676,15665352,45460.17820811272,0.0004449953376024496
980981,7840682,7840682,15681364,45508.8426630497,0.00044494704707176425
981982,7848690,7848690,15697380,45556.08993721008,0.00044494124267657753
982983,7856692,7856692,15713384,45595.68620419502,0.0004446292168722721
983984,7864700,7864700,15729400,45635.46771931648,0.00044462341429607477
984985,7872704,7872704,15745408,45674.88216614723,0.00044437059477786534
985986,7880712,7880712,15761424,45714.36330699921,0.00044436479583964683
986987,7888718,7888718,15777436,45762.33430600166,0.00044432829054130707
987988,7896726,7896726,15793452,45810.85006594658,0.00044432249160308857
988989,7904732,7904732,15809464,45855.591551065445,0.0004443028610694455
989990,7912736,7912736,15825472,45895.28424715996,0.0004442529534571804
990991,7920742,7920742,15841484,45934.95069217682,0.0004436001818248769
991992,7928750,7928750,15857500,45974.63481593132,0.0004435943847056478
992993,7936756,7936756,15873512,46016.14853310585,0.00044358460581861436
993994,7944760,7944760,15889520,46064.543909072876,0.00044323750444164034
994995,7952768,7952768,15905536,46112.77650523186,0.00044323170914140064
995996,7960774,7960774,15921548,46155.12911105156,0.00044319241715129465
996997,7968782,7968782,15937564,46194.678168058395,0.00044318662185105495
997998,7976788,7976788,15953576,46234.39041519165,0.00044311551937425975
998999,7984796,7984796,15969592,46273.96345615387,0.00044310972225503065
1000000,7992802,7992802,15985604,46319.63829302788,0.0004430947101354832


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.03208613395690918,12064.682476916567
36,146,146,292,1.104646921157837,52.30500082631261
71,248,248,496,1.7445580959320068,27.141848262002895
107,358,358,716,2.4315409660339355,11.933394474070155
142,466,466,932,3.2864770889282227,5.197580163256134
178,578,578,1156,4.076996088027954,3.1365870973932033
213,694,694,1388,4.858889102935791,2.479279129920542
249,822,822,1644,5.696300029754639,1.9649261214290163
284,950,950,1900,6.5995259284973145,1.594074333557728
320,1082,1082,2164,7.5958662033081055,1.3089532206158765
355,1214,1214,2428,8.631164073944092,1.0862390728598257
391,1358,1358,2716,9.67017912864685,0.9758987308323412
426,1482,1482,2964,10.545928001403809,0.7592629871105601
462,1610,1610,3220,11.465901136398315,0.5564759814660647
497,1740,1740,3480,12.333163976669312,0.45034559544728836
533,1860,1860,3720,13.108394145965576,0.3600335182836716
568,1998,1998,3996,13.907964944839478,0.33296849535690853
604,2128,2128,4256,14.744874000549316,0.29890755062479
640,2262,2262,4524,15.617071151733398,0.2696009202318237
675,2398,2398,4796,16.509824991226196,0.25181713265556027
711,2546,2546,5092,17.45164918899536,0.2370260315692576
746,2696,2696,5392,18.447766065597534,0.21919866958705825
782,2842,2842,5684,19.3876211643219,0.20245800934753788
817,3000,3000,6000,20.478121042251587,0.1781729139165691
853,3148,3148,6296,21.358756065368652,0.16321093675651355
888,3280,3280,6560,22.214028120040894,0.1559341810625483
924,3420,3420,6840,23.102277994155884,0.13586458643294463
959,3570,3570,7140,24.13960599899292,0.13091624469780072
995,3730,3730,7460,25.187839031219482,0.12349765578619554
1030,3884,3884,7768,26.132794857025146,0.11849342138339125
1066,4048,4048,8096,27.16092300415039,0.10630610299085674
1101,4208,4208,8416,28.1181161403656,0.09892259914158785
1137,4358,4358,8716,29.156046152114868,0.09272213218901015
1172,4500,4500,9000,30.16516900062561,0.08255026140250266
1208,4636,4636,9272,31.005311012268066,0.07082356795945088
1243,4768,4768,9536,31.811548948287964,0.06478122332555358
1279,4904,4904,9808,32.59728002548218,0.05939617703006661
1315,5048,5048,10096,33.41242504119873,0.05768445014109602
1350,5188,5188,10376,34.17873692512512,0.05684824076524819
1386,5332,5332,10664,34.998881101608276,0.05624914616055321
1421,5476,5476,10952,35.82648801803589,0.05355406722628686
1457,5622,5622,11244,36.617778062820435,0.052311414408904966
1492,5766,5766,11532,37.40172219276428,0.051610537126180134
1528,5914,5914,11828,38.248316049575806,0.04937863067971193
1563,6066,6066,12132,39.09885501861572,0.0477488277683733
1599,6214,6214,12428,39.93120789527893,0.04581970052822726
1634,6362,6362,12724,40.74213886260986,0.04461492495283892
1670,6526,6526,13052,41.63882398605347,0.04234772918061935
1705,6670,6670,13340,42.44318413734436,0.04154595709769637
1741,6818,6818,13636,43.30479598045349,0.039951398543053074
1776,6976,6976,13952,44.32193422317505,0.0359954647901759
1812,7138,7138,14276,45.511444091796875,0.03286750309962372
1847,7298,7298,14596,46.57936906814575,0.030447379613178782
1883,7448,7448,14896,47.660573959350586,0.029233557401312282
1919,7600,7600,15200,48.62986612319946,0.028034453900545486
1954,7740,7740,15480,49.65371918678284,0.02645723446221382
1990,7888,7888,15776,50.73527503013611,0.025766663024114678
2025,8028,8028,16056,51.90542793273926,0.024019976142881205
2061,8176,8176,16352,52.893226146698,0.023371382972982246
2096,8320,8320,16640,53.8654248714447,0.021384484238296864
2132,8472,8472,16944,54.86685013771057,0.018939170169687713
2167,8616,8616,17232,55.813512086868286,0.01702903140176204
2203,8754,8754,17508,56.6920599937439,0.015818984978977824
2238,8886,8886,17772,57.546345949172974,0.014432462732656859
2274,9018,9018,18036,58.40186405181885,0.012594293077199836
2309,9136,9136,18272,59.17098307609558,0.010613960239425069
2345,9278,9278,18556,60.07165813446045,0.010183783877437236
2380,9416,9416,18832,60.969993114471436,0.010048247655504383
2416,9568,9568,19136,62.066365003585815,0.009763846617715899
2451,9708,9708,19416,62.98412227630615,0.009689518954473897
2487,9852,9852,19704,63.876370906829834,0.009570026200890425
2523,9996,9996,19992,64.79013204574585,0.009380069606777397
2558,10142,10142,20284,65.73026609420776,0.009068069241038756
2594,10286,10286,20572,66.69977807998657,0.008748620521146222
2629,10434,10434,20868,67.61970686912537,0.008185995955500402
2665,10578,10578,21156,68.62773704528809,0.00782466590317199
2700,10718,10718,21436,69.53133916854858,0.007446860960044432
2736,10868,10868,21736,70.46383500099182,0.007046232585707912
2771,11008,11008,22016,71.34814429283142,0.00693053121540288
2807,11152,11152,22304,72.22943496704102,0.0067140253268007655
2842,11292,11292,22584,73.1023371219635,0.006437039834054303
2878,11440,11440,22880,74.01475501060486,0.0062620754943054635
2913,11586,11586,23172,74.91496515274048,0.0058995115159632405
2949,11730,11730,23460,75.81179189682007,0.005695157999070943
2984,11898,11898,23796,76.80902004241943,0.0053690798977186205
3020,12054,12054,24108,77.76813316345215,0.005062888469183235
3055,12194,12194,24388,78.62640309333801,0.004969327535945922
3091,12344,12344,24688,79.55316090583801,0.004836234316826449
3127,12488,12488,24976,80.43757915496826,0.004683102752096602
3162,12650,12650,25300,81.42260408401489,0.00473930924636079
3198,12804,12804,25608,82.38449692726135,0.004562167545373086
3233,12960,12960,25920,83.34723114967346,0.004274073586202576
3269,13116,13116,26232,84.31581807136536,0.004068812771947705
3304,13274,13274,26548,85.27389311790466,0.003883218527334975
3340,13438,13438,26876,86.26750898361206,0.0038821205071144504
3375,13578,13578,27156,87.12845492362976,0.0038947400698816637
3411,13724,13724,27448,88.03743410110474,0.003816092304987251
3446,13906,13906,27812,89.12543892860413,0.0037578973860945553
3482,14050,14050,28100,90.00696802139282,0.0037565188613370992
3517,14190,14190,28380,90.88628005981445,0.0037543962007475784
3553,14338,14338,28676,91.7997829914093,0.0037514242121687857
3588,14478,14478,28956,92.66328716278076,0.0037494813332159538
3624,14622,14622,29244,93.54816794395447,0.003745963149413001
3659,14762,14762,29524,94.42831492424011,0.003743111263247556
3695,14906,14906,29812,95.33014106750488,0.0037407408435683465
3730,15046,15046,30092,96.17762899398804,0.0037378223987616366
3766,15190,15190,30380,97.08587217330933,0.0037363583651313093
3802,15334,15334,30668,97.98681497573853,0.0037332647352741333
3837,15474,15474,30948,98.86529302597046,0.0037288173698470928
3873,15618,15618,31236,99.76038718223572,0.003713581434567459
3908,15758,15758,31516,100.62114691734314,0.003703098724145093
3944,15902,15902,31804,101.52966618537903,0.003681254169350723
3979,16054,16054,32108,102.46317601203918,0.003656962589957402
4015,16318,16318,32636,103.9655659198761,0.003656882081486401
4050,16544,16544,33088,105.26955699920654,0.0036566635717463214
4086,16688,16688,33376,106.15908622741699,0.0036551536122715333
4121,16832,16832,33664,107.0423948764801,0.0036533609636535402
4157,16976,16976,33952,107.94294500350952,0.0036508849552774336
4192,17116,17116,34232,108.81288814544678,0.0036476998757279944
4228,17262,17262,34524,109.71074509620667,0.003645095661340747
4263,17402,17402,34804,110.59325218200684,0.0036397482072061393
4299,17546,17546,35092,111.4796371459961,0.00362737919385836
4334,17686,17686,35372,112.36199498176575,0.0036172536802041577
4370,17872,17872,35744,113.44809913635254,0.0035850278072757646
4406,18132,18132,36264,114.92898607254028,0.003584899804991437
4441,18272,18272,36544,115.79930806159973,0.0035840696746163303
4477,18416,18416,36832,116.69552707672119,0.003582414514312404
4512,18556,18556,37112,117.58247923851013,0.003581278200726956
4548,18712,18712,37424,118.5514121055603,0.003579207803340978
4583,18852,18852,37704,119.44892406463623,0.003570682845747797
4619,18996,18996,37992,120.32674098014832,0.00356289674891741
4654,19136,19136,38272,121.22235703468323,0.0035573807053879136
4690,19280,19280,38560,122.12768602371216,0.003545022293110378
4725,19420,19420,38840,123.02446103096008,0.0035297159611218376
4761,19564,19564,39128,123.92833995819092,0.0035118006217089714
4796,19712,19712,39424,124.85492420196533,0.0034756314562400803
4832,19856,19856,39712,125.7763991355896,0.0034357377317064675
4867,19996,19996,39992,126.67367100715637,0.0033659067048574798
4903,20140,20140,40280,127.59209084510803,0.0033095090020651696
4938,20280,20280,40560,128.53000903129578,0.00319638389373722
4974,20470,20470,40940,129.71346616744995,0.0030951334920246154
5010,20710,20710,41420,131.22660398483276,0.0030948050916776992
5045,20854,20854,41708,132.18880891799927,0.0030931337514630286
5081,20998,20998,41996,133.12825202941895,0.003092151633609319
5116,21138,21138,42276,134.05877208709717,0.003090305155637907
5152,21282,21282,42564,135.07595920562744,0.0030883272593200672
5187,21422,21422,42844,135.9528350830078,0.0030852728596073575
5223,21566,21566,43132,136.852117061615,0.003082822047872469
5258,21706,21706,43412,137.71050906181335,0.003078379540966125
5294,21850,21850,43700,138.61057305335999,0.003072112704103347
5329,21990,21990,43980,139.47025513648987,0.003066566250709002
5365,22134,22134,44268,140.37233805656433,0.003063400699829799
5400,22274,22274,44548,141.23498010635376,0.0030616551339335274
5436,22418,22418,44836,142.14519095420837,0.003058913742279401
5471,22558,22558,45116,143.03204894065857,0.0030563251330022467
5507,22702,22702,45404,143.9253330230713,0.0030514060526911635
5542,22842,22842,45684,144.79886603355408,0.0030458132969215512
5578,22986,22986,45972,145.6841950416565,0.003039917199203046
5614,23130,23130,46260,146.65081906318665,0.003030993642823887
5649,23270,23270,46540,147.54149103164673,0.003018508243258111
5685,23414,23414,46828,148.47120904922485,0.002988317455674405
5720,23562,23562,47124,149.40033602714539,0.002954209969175281
5756,23706,23706,47412,150.34441089630127,0.0029217158335086424
5791,23860,23860,47720,151.28673911094666,0.0028629561802517856
5827,24104,24104,48208,152.70320010185242,0.0028557965761137893
5862,24340,24340,48680,154.0757350921631,0.0028554710315802367
5898,24560,24560,49120,155.34880995750427,0.002854980975826038
5933,24700,24700,49400,156.22162699699402,0.002852415153029142
5969,24844,24844,49688,157.11573004722595,0.0028493060563050676
6004,24984,24984,49968,157.9887261390686,0.0028459463483159197
6040,25128,25128,50256,158.8951771259308,0.0028437577620934462
6075,25268,25268,50536,159.7431812286377,0.0028428046134649776
6111,25412,25412,50824,160.65216898918152,0.0028398008635122096
6146,25552,25552,51104,161.50905084609985,0.0028370811087370384
6182,25696,25696,51392,162.41626906394958,0.002834510669345036
6217,25836,25836,51672,163.27114129066467,0.002830455829098355
6253,25980,25980,51960,164.15022897720337,0.0028284136787988245
6289,26126,26126,52252,165.04987716674805,0.002821279918862274
6324,26266,26266,52532,165.92557311058044,0.002817903916366049
6360,26410,26410,52820,166.8236858844757,0.0028127750738349278
6395,26550,26550,53100,167.6943109035492,0.002805656227792497
6431,26698,26698,53396,168.60294818878174,0.0027996928765787743
6466,26838,26838,53676,169.48104596138,0.002787332679872634
6502,26982,26982,53964,170.37532114982605,0.0027754692600865383
6537,27122,27122,54244,171.26277613639832,0.002772653764623101
6573,27266,27266,54532,172.1568021774292,0.002750843319518026
6608,27406,27406,54812,173.0144820213318,0.002691053387025022
6644,27552,27552,55104,173.93100214004517,0.0025960621551348595
6679,27730,27730,55460,174.9847710132599,0.0025365621950186323
6715,27954,27954,55908,176.29271912574768,0.002532480610170751
6750,28212,28212,56424,177.75188207626343,0.002532415219320683
6786,28492,28492,56984,179.32645416259766,0.0025324154557893053
6821,28640,28640,57280,180.24219918251038,0.002531931311750668
6857,28784,28784,57568,181.1188521385193,0.0025303665079263737
6893,28928,28928,57856,182.00891017913818,0.002529323848648346
6928,29068,29068,58136,182.89486384391785,0.0025286474792665103
6964,29212,29212,58424,183.78021717071533,0.0025278985303884838
6999,29352,29352,58704,184.67504596710205,0.0025265511030738708
7035,29496,29496,58992,185.58211612701416,0.002524901912693167
7070,29636,29636,59272,186.48955392837524,0.002522097245673649
7106,29780,29780,59560,187.40388417243958,0.002519368734283489
7141,29920,29920,59840,188.2943480014801,0.0025151253958028974
7177,30064,30064,60128,189.21166896820068,0.002513175311833038
7212,30206,30206,60412,190.097186088562,0.002510475269446033
7248,30356,30356,60712,191.04460906982422,0.0025065897880267585
7283,30496,30496,60992,191.92031598091125,0.0025011808465933427
7319,30642,30642,61284,192.8343071937561,0.002496802608220605
7354,30782,30782,61564,193.72205591201782,0.0024816540390020236
7390,30932,30932,61864,194.66074109077454,0.0024687676268513314
7425,31152,31152,62304,196.22542905807495,0.0024633146585983923
7461,31296,31296,62592,197.12376403808594,0.002464988090650877
7497,31444,31444,62888,198.05002117156982,0.002463416003593011
7532,31682,31682,63364,199.42306518554688,0.0024631916367070517
7568,31964,31964,63928,200.99514293670654,0.002463185905071441
7603,32244,32244,64488,202.5653510093689,0.002463184395310236
7639,32412,32412,64824,203.57759594917297,0.0024628251248941524
7674,32556,32556,65112,204.4762260913849,0.00246228561445605
7710,32704,32704,65408,205.4077160358429,0.002460658508425695
7745,32844,32844,65688,206.27986693382263,0.0024568783101130975
7781,32988,32988,65976,207.14893007278442,0.002452804577842471
7816,33128,33128,66256,208.01439905166626,0.0024519094531569863
7852,33272,33272,66544,208.9209921360016,0.002449375466312631
7887,33412,33412,66824,209.79807996749878,0.0024446945335512282
7923,33556,33556,67112,210.69050407409668,0.002439139609123231
7958,33696,33696,67392,211.56187295913696,0.002432211877021473
7994,33844,33844,67688,212.4968409538269,0.002430910331895575
8029,33984,33984,67968,213.38281917572021,0.002425083823254681
8065,34128,34128,68256,214.2828779220581,0.002419044778434909
8101,34272,34272,68544,215.18962407112122,0.002405657658528071
8136,34412,34412,68824,216.04854822158813,0.002395466170128202
8172,34558,34558,69116,216.97581911087036,0.00237367108638864
8207,34702,34702,69404,217.86104702949524,0.002331731629965361
8243,34854,34854,69708,218.79799604415894,0.002287804083607625
8278,34994,34994,69988,219.6745090484619,0.0022566417246707715
8314,35138,35138,70276,220.56731915473938,0.002237276148662204
8349,35280,35280,70560,221.46218609809875,0.0022076580517023103
8385,35428,35428,70856,222.37927198410034,0.0021749030602222774
8420,35574,35574,71148,223.29532384872437,0.002140520055036177
8456,35718,35718,71436,224.1865029335022,0.002043104204858537
8491,35890,35890,71780,225.2233669757843,0.0019191782903362764
8527,36102,36102,72204,226.48554110527039,0.001920222819535411
8562,36242,36242,72484,227.36492609977722,0.0019198070713173365
8598,36386,36386,72772,228.2613880634308,0.0019191296287317527
8633,36606,36606,73212,229.53957104682922,0.001918803944136016
8669,36894,36894,73788,231.16737699508667,0.0019188027326890733
8704,37120,37120,74240,232.47927713394165,0.0019185881774319569
8740,37264,37264,74528,233.36627793312073,0.0019181656007276615
8776,37408,37408,74816,234.26480412483215,0.001916736035127542
8811,37548,37548,75096,235.13935899734497,0.0019137909966957523
8847,37692,37692,75384,236.04197812080383,0.0019117132032988593
8882,37832,37832,75664,236.93503999710083,0.0019107345833617728
8918,37976,37976,75952,237.84375,0.0019097655276709702
8953,38120,38120,76240,238.72317504882812,0.0019084439245489193
8989,38264,38264,76528,239.6087350845337,0.0019066924342041602
9024,38404,38404,76808,240.48671221733093,0.0019055826796829933
9060,38552,38552,77104,241.40228414535522,0.0019046861034439644
9095,38692,38692,77384,242.27103996276855,0.0019039550807065098
9131,38846,38846,77692,243.22152495384216,0.001902968459035037
9166,38998,38998,77996,244.13879108428955,0.0019016964270122116
9202,39150,39150,78300,245.071946144104,0.001900381392260897
9237,39292,39292,78584,245.95686197280884,0.0018997961778950412
9273,39438,39438,78876,246.86858296394348,0.001898207250633277
9308,39578,39578,79156,247.73864912986755,0.0018965753006341401
9344,39722,39722,79444,248.63410687446594,0.001895553441499942
9380,39866,39866,79732,249.53940725326538,0.0018949460063595325
9415,40008,40008,80016,250.4219400882721,0.001887383068606141
9451,40152,40152,80304,251.30361008644104,0.001870563692136784
9486,40292,40292,80584,252.18470811843872,0.0018289638555870624
9522,40500,40500,81000,253.40388107299805,0.0017994799145526486
9557,40674,40674,81348,254.45532298088074,0.00179931971069891
9593,40920,40920,81840,255.85915398597717,0.0017992175708059222
9628,41064,41064,82128,256.74915409088135,0.0017986045331781497
9664,41212,41212,82424,257.65878200531006,0.0017982256922550732
9699,41352,41352,82704,258.5400199890137,0.0017974116799450712
9735,41500,41500,83000,259.46763920783997,0.0017965493152587442
9770,41640,41640,83280,260.3337609767914,0.0017958725638891337
9806,41784,41784,83568,261.21817922592163,0.001795283351384569
9841,41926,41926,83852,262.08546209335327,0.001794228286598809
9877,42078,42078,84156,263.02927589416504,0.0017924155999935465
9912,42220,42220,84440,263.9046070575714,0.001790995887859026
9948,42368,42368,84736,264.82581210136414,0.0017891616698761936
9984,42520,42520,85040,265.75614309310913,0.0017864327601273544
10019,42660,42660,85320,266.6122188568115,0.0017843362693383824
10055,42804,42804,85608,267.50891399383545,0.001782202021786361
10090,42944,42944,85888,268.37538504600525,0.0017774260122678243
10126,43090,43090,86180,269.272586107254,0.0017700350617815275
10161,43230,43230,86460,270.1305179595947,0.0017627927172725322
10197,43374,43374,86748,271.0188219547272,0.0017466400440753205
10232,43518,43518,87036,271.91815996170044,0.0017260132262890693
10268,43662,43662,87324,272.8075451850891,0.0017031029383360874
10303,43802,43802,87604,273.68194007873535,0.0016817914711282356
10339,43946,43946,87892,274.5761079788208,0.0016652028371026972
10374,44088,44088,88176,275.44962787628174,0.0016424377499788534
10410,44234,44234,88468,276.3604679107666,0.0016134666020661825
10445,44386,44386,88772,277.28621220588684,0.0015634638621122576
10481,44580,44580,89160,278.46285605430603,0.0015490341993427137
10516,44776,44776,89552,279.6079740524292,0.0015478305886063026
10552,45030,45030,90060,281.0548732280731,0.0015477482447749935
10588,45318,45318,90636,282.67920112609863,0.0015477473243663553
10623,45508,45508,91016,283.800390958786,0.0015476373100682395
10659,45652,45652,91304,284.70370626449585,0.0015474062747671269
10694,45792,45792,91584,285.5681240558624,0.001546133893498336
10730,45936,45936,91872,286.4630711078644,0.0015455205411853967
10765,46076,46076,92152,287.34320521354675,0.0015442248641193146
10801,46220,46220,92440,288.2382140159607,0.0015429763370775618
10836,46360,46360,92720,289.10703587532043,0.0015414570243592607
10872,46504,46504,93008,290.00767493247986,0.0015403674115077592
10907,46646,46646,93292,290.9412660598755,0.0015395402115245815
10943,46790,46790,93580,291.83337807655334,0.0015385825481644133
10978,46934,46934,93868,292.74101400375366,0.0015381053126475308
11014,47078,47078,94156,293.6513931751251,0.0015372282796306536
11049,47226,47226,94452,294.5580701828003,0.0015368165677500656
11085,47382,47382,94764,295.5298020839691,0.001535370198325836
11120,47534,47534,95068,296.4730360507965,0.0015340912814281182
11156,47680,47680,95360,297.3829710483551,0.0015336710948758991
11191,47832,47832,95664,298.3255889415741,0.0015325987715186784
11227,47984,47984,95968,299.24793100357056,0.00153078436414944
11263,48138,48138,96276,300.20142793655396,0.0015281449032045202
11298,48282,48282,96564,301.08076000213623,0.0015260843847499928
11334,48430,48430,96860,302.00446796417236,0.0015209398825390963
11369,48570,48570,97140,302.8711349964142,0.0015182974257186288
11405,48714,48714,97428,303.7584488391876,0.0015141894728003535
11440,48858,48858,97716,304.654736995697,0.0015065234601934208
11476,49002,49002,98004,305.54757499694824,0.0014889695867168484
11511,49142,49142,98284,306.41997385025024,0.001465678429667605
11547,49290,49290,98580,307.32529616355896,0.0014444761054619448
11582,49492,49492,98984,308.53262209892273,0.0014107015940680867
11618,49644,49644,99288,309.46654319763184,0.0014104544443398481
11653,49834,49834,99668,310.5739049911499,0.0014102592176641338
11689,49986,49986,99972,311.5192201137543,0.0014101684046181617
11724,50126,50126,100252,312.39610290527344,0.0014100097760092467
11760,50280,50280,100560,313.352890253067,0.001409369682733086
11795,50420,50420,100840,314.2090561389923,0.0014086865085118916
11831,50568,50568,101136,315.19610500335693,0.0014081794579396956
11867,50712,50712,101424,316.0924742221832,0.0014076961924729403
11902,50852,50852,101704,316.9818539619446,0.0014071403493289836
11938,51006,51006,102012,317.94697308540344,0.0014062243753869552
11973,51154,51154,102308,318.89321184158325,0.0014055463689146563
12009,51302,51302,102604,319.8230631351471,0.00140475152147701
12044,51444,51444,102888,320.6924500465393,0.0014042100319784367
12080,51592,51592,103184,321.61286997795105,0.0014027993438503472
12115,51732,51732,103464,322.4907500743866,0.0014008048729010625
12151,51894,51894,103788,323.479727268219,0.001398521209921455
12186,52038,52038,104076,324.376394033432,0.0013945639511803165
12222,52186,52186,104372,325.27784299850464,0.001386781132168835
12257,52326,52326,104652,326.1429650783539,0.001379980723868357
12293,52472,52472,104944,327.0384130477905,0.0013668875544681214
12328,52612,52612,105224,327.90120816230774,0.001350243514025351
12364,52756,52756,105512,328.80106806755066,0.0013310548056324478
12399,52900,52900,105800,329.67712807655334,0.0013153708241588902
12435,53044,53044,106088,330.56179094314575,0.001306321786614717
12471,53188,53188,106376,331.4483380317688,0.0012938240906805731
12506,53330,53330,106660,332.33460521698,0.00127051024355751
12542,53474,53474,106948,333.22320008277893,0.0012283703381399391
12577,53630,53630,107260,334.1674199104309,0.001159994326371816
12613,53894,53894,107788,335.67359805107117,0.001158573404609342
12648,54128,54128,108256,337.02373719215393,0.0011578231788007542
12684,54372,54372,108744,338.4356219768524,0.001157780816356535
12719,54552,54552,109104,339.5036630630493,0.0011576911219890462
12755,54712,54712,109424,340.47427797317505,0.0011573053980100667
12790,54852,54852,109704,341.35230588912964,0.00115664251097769
12826,55000,55000,110000,342.2634310722351,0.0011563281859707786
12861,55146,55146,110292,343.157653093338,0.0011558006626728456
12897,55290,55290,110580,344.04935002326965,0.0011555685614439426
12932,55440,55440,110880,344.96781492233276,0.0011551230163604487
12968,55584,55584,111168,345.8697118759155,0.0011536069741850952
13003,55732,55732,111464,346.7555079460144,0.001152626538896584
13039,55880,55880,111760,347.66857290267944,0.0011509413689054782
13074,56020,56020,112040,348.5170040130615,0.0011498107724037254
13110,56174,56174,112348,349.45013403892517,0.001149823878222378
13146,56330,56330,112660,350.4064042568207,0.0011494933387439232
13181,56476,56476,112952,351.31025314331055,0.001149268993685837
13217,56620,56620,113240,352.210813999176,0.0011488898653624346
13252,56790,56790,113580,353.2245042324066,0.0011485161321616033
13288,56944,56944,113888,354.16133999824524,0.0011476854688226013
13323,57094,57094,114188,355.0723571777344,0.0011468758530099876
13359,57246,57246,114492,355.99517798423767,0.0011456203737907344
13394,57396,57396,114792,356.93265199661255,0.0011437150442361599
13430,57544,57544,115088,357.84765005111694,0.0011373132310836809
13465,57684,57684,115368,358.72493386268616,0.0011313970771880122
13501,57830,57830,115660,359.58426308631897,0.0011216721541131847
13536,57970,57970,115940,360.212877035141,0.0011119094015157316
13572,58120,58120,116240,361.22081995010376,0.0011043647991755279
13607,58264,58264,116528,362.21690607070923,0.00109003792204021
13643,58408,58408,116816,363.1649420261383,0.001075515921911574
13678,58548,58548,117096,364.06456089019775,0.0010630689012032235
13714,58692,58692,117384,364.99498295783997,0.0010317157393728849
13750,58848,58848,117696,366.02529525756836,0.0009753078757057665
13785,59000,59000,118000,366.9986078739166,0.0009217417646141257
13821,59178,59178,118356,368.11111307144165,0.000876567160958075
13856,59422,59422,118844,369.7033140659332,0.0008718551125639351
13892,59614,59614,119228,370.7241380214691,0.0008717142136447364
13927,59808,59808,119616,372.1806721687317,0.000871590160386404
13963,60090,60090,120180,373.9531149864197,0.0008715886633581249
13998,60294,60294,120588,375.28170704841614,0.0008712292201380478
14034,60508,60508,121016,376.63396406173706,0.0008711725495231804
14069,60752,60752,121504,378.12901306152344,0.0008711500540812267
14105,60904,60904,121808,379.14373207092285,0.0008710767870070413
14140,61048,61048,122096,380.10202717781067,0.000870794488946558
14176,61198,61198,122396,381.1296100616455,0.0008705038271727972
14211,61340,61340,122680,382.07332825660706,0.0008700071593921166
14247,61484,61484,122968,383.041286945343,0.0008696159620740218
14282,61624,61624,123248,383.978728055954,0.0008690341455803718
14318,61774,61774,123548,384.9817259311676,0.0008680535502207931
14354,61924,61924,123848,385.97040605545044,0.0008676141878822818
14389,62082,62082,124164,386.987272977829,0.0008670919305586722
14425,62234,62234,124468,387.98608207702637,0.0008667775528010679
14460,62378,62378,124756,388.9240720272064,0.0008664475881232647
14496,62522,62522,125044,389.89109206199646,0.00086580146853521
14531,62676,62676,125352,390.88768315315247,0.0008654939338157419
14567,62832,62832,125664,391.9288160800934,0.0008653524237161037
14602,62982,62982,125964,392.9455180168152,0.000865078571223421
14638,63128,63128,126256,393.93148708343506,0.0008647949198348215
14673,63280,63280,126560,394.89767718315125,0.0008643649653095054
14709,63444,63444,126888,395.9426500797272,0.0008639083716843743
14744,63608,63608,127216,396.97042298316956,0.0008626619091955945
14780,63758,63758,127516,397.93960404396057,0.0008619263317086734
14815,63912,63912,127824,398.94891715049744,0.0008601469544373685
14851,64060,64060,128120,399.9003930091858,0.0008577746266382746
14886,64204,64204,128408,400.8407139778137,0.0008548058285668958
14922,64362,64362,128724,401.871857881546,0.0008512019885529298
14958,64508,64508,129016,402.8333692550659,0.0008464883740089135
14993,64648,64648,129296,403.7692120075226,0.000840872709886753
15029,64792,64792,129584,404.703919172287,0.0008330266064149328
15064,64932,64932,129864,405.59987711906433,0.0008200189240596956
15100,65116,65116,130232,406.77286410331726,0.0007934779860079288
15135,65272,65272,130544,407.75723695755005,0.0007933604556455975
15171,65458,65458,130916,408.9121558666229,0.000793252849689452
15206,65736,65736,131472,410.597088098526,0.000793252038420178
15242,66022,66022,132044,412.3048379421234,0.0007932515836728271
15277,66274,66274,132548,413.81386494636536,0.000793174698628718
15313,66442,66442,132884,414.8944170475006,0.0007931519121484598
15348,66582,66582,133164,415.8341271877289,0.000793090372098959
15384,66730,66730,133460,416.8054881095886,0.0007930336614663247
15419,66876,66876,133752,417.76847410202026,0.0007929456132842461
15455,67044,67044,134088,418.8572700023651,0.0007928152463136939
15490,67192,67192,134384,419.84128522872925,0.0007925200843601488
15526,67358,67358,134716,420.89489698410034,0.000792381488281535
15561,67510,67510,135020,421.88320112228394,0.000792295115388697
15597,67668,67668,135336,422.91631412506104,0.000792222877862514
15633,67830,67830,135660,423.95100116729736,0.0007918994160718285
15668,67984,67984,135968,424.97617626190186,0.0007911427292128792
15704,68168,68168,136336,426.1376881599426,0.0007907089748186991
15739,68336,68336,136672,427.2196249961853,0.0007904125031927833
15775,68588,68588,137176,428.75132489204407,0.0007902957386249909
15810,68866,68866,137732,430.39924788475037,0.0007902963734522928
15846,69146,69146,138292,432.08061695098877,0.000790242131188279
15881,69316,69316,138632,433.1773121356964,0.0007899823394836858
15917,69472,69472,138944,434.19479393959045,0.0007896952756709652
15952,69618,69618,139236,435.19223499298096,0.0007891203240433242
15988,69784,69784,139568,436.27079820632935,0.0007887449919508072
16023,69940,69940,139880,437.28167510032654,0.0007880558878241573
16059,70104,70104,140208,438.3361761569977,0.0007875109295127913
16094,70250,70250,140500,439.27746510505676,0.0007867722506489372
16130,70434,70434,140868,440.4412591457367,0.0007862883394409437
16165,70588,70588,141176,441.4419050216675,0.0007853523202356882
16201,70742,70742,141484,442.4378590583801,0.000784387057137792
16237,70886,70886,141772,443.3769931793213,0.000780425329139689
16272,71026,71026,142052,444.3026921749115,0.0007741904628346674
16308,71170,71170,142340,445.23135900497437,0.0007665427492611343
16343,71358,71358,142716,446.4185690879822,0.0007573926322947955
16379,71590,71590,143180,447.85360527038574,0.0007573648490506457
16414,71866,71866,143732,449.56836891174316,0.000757363552111201
16450,72012,72012,144024,450.68078207969666,0.0007573140355816577
16485,72152,72152,144304,451.64428210258484,0.0007572242902824655
16521,72298,72298,144596,452.59803009033203,0.00075714361264545
16556,72438,72438,144876,453.525887966156,0.0007569837453047512
16592,72596,72596,145192,454.55489706993103,0.0007568677719973493
16627,72746,72746,145492,455.47075724601746,0.0007565531614091014
16663,72898,72898,145796,456.37541818618774,0.0007560886224382557
16698,73050,73050,146100,457.318706035614,0.000756025883674738
16734,73208,73208,146416,458.2639329433441,0.0007559745208709501
16769,73364,73364,146728,459.1914849281311,0.0007557963417639257
16805,73518,73518,147036,460.1480882167816,0.0007556748241768219
16841,73704,73704,147408,461.2363929748535,0.0007555411266366718
16876,73896,73896,147792,462.31389021873474,0.0007553483301308006
16912,74054,74054,148108,463.2265040874481,0.0007551603739557322
16947,74328,74328,148656,464.6767590045929,0.0007551529870397644
16983,74608,74608,149216,466.2133800983429,0.0007551270664407639
17018,74888,74888,149776,467.723237991333,0.0007551267935923534
17054,75176,75176,150352,469.36522817611694,0.0007551265116489958
17089,75438,75438,150876,470.7835099697113,0.0007549210567958653
17125,75718,75718,151436,472.51305508613586,0.0007549148431280628
17160,75990,75990,151980,474.1272692680359,0.0007548773901362438
17196,76152,76152,152304,475.10847210884094,0.000753906188037945
17231,76300,76300,152600,476.02570128440857,0.0007521703519159928
17267,76450,76450,152900,476.94904708862305,0.0007465476737706922
17302,76592,76592,153184,477.8714950084686,0.0007400250869977754
17338,76740,76740,153480,478.834450006485,0.0007341337695834227
17373,76882,76882,153764,479.75919008255005,0.0007057567981973989
17409,77028,77028,154056,480.6993169784546,0.000658199169265572
17445,77184,77184,154368,481.63893723487854,0.0005368545735109365
17480,77324,77324,154648,482.5096700191498,0.00045682035124627873
17516,77480,77480,154960,483.50274419784546,0.00033321647424600087
17551,77648,77648,155296,484.50692987442017,0.0003331626739964122
17587,77792,77792,155584,485.4536461830139,0.0003330655235913582
17622,77932,77932,155864,486.37695503234863,0.0003329723695060238
17658,78080,78080,156160,487.3413550853729,0.0003329050068714423
17693,78224,78224,156448,488.26430106163025,0.0003328265102027217
17729,78368,78368,156736,489.1875419616699,0.00033269743107666727
17764,78516,78516,157032,490.13150119781494,0.0003326567730255192
17800,78712,78712,157424,491.3398220539093,0.00033260867166973185
17835,78864,78864,157728,492.3450679779053,0.00033259224983339664
17871,79012,79012,158024,493.34601497650146,0.000332562785843038
17906,79158,79158,158316,494.2562401294708,0.00033249258194700815
17942,79310,79310,158620,495.2454719543457,0.0003324521476315567
17977,79482,79482,158964,496.3263580799103,0.000332381610860466
18013,79648,79648,159296,497.4181959629059,0.00033223013269889634
18048,79796,79796,159592,498.4085490703583,0.00033207080196007155
18084,79958,79958,159916,499.4639871120453,0.0003317828868603101
18120,80114,80114,160228,500.4032452106476,0.0003316403726785211
18155,80268,80268,160536,501.34233808517456,0.0003314697605674155
18191,80484,80484,160968,502.55318212509155,0.0003312473854748532
18226,80652,80652,161304,503.555242061615,0.00033104846806963906
18262,80818,80818,161636,504.55547404289246,0.000330868491801084
18297,80970,80970,161940,505.4825279712677,0.0003307550068711862
18333,81152,81152,162304,506.5396611690521,0.00033067843469325453
18368,81322,81322,162644,507.5657489299774,0.00033056470965675544
18404,81520,81520,163040,508.7188789844513,0.0003304949259472778
18439,81706,81706,163412,509.8210859298706,0.00033036440254363697
18475,81908,81908,163816,510.96884512901306,0.0003301705619378481
18510,82180,82180,164360,512.4593999385834,0.00033015811095538083
18546,82466,82466,164932,514.0313658714294,0.0003301572342024883
18581,82742,82742,165484,515.5138781070709,0.00033014853215718176
18617,83028,83028,166056,517.0771460533142,0.0003301464348623995
18652,83308,83308,166616,518.5872042179108,0.0003301462948002154
18688,83586,83586,167172,520.1058571338654,0.0003301249653304694
18724,83872,83872,167744,521.6545281410217,0.00033012317726388574
18759,84148,84148,168296,523.1495649814606,0.000330069340634509
18795,84426,84426,168852,524.6499330997467,0.0003300520584161859
18830,84704,84704,169408,526.152890920639,0.00033005161276378203
18866,84992,84992,169984,527.7112550735474,0.00033005146724462975
18901,85270,85270,170540,529.2028002738953,0.0003300498392491136
18937,85554,85554,171108,530.7536189556122,0.0003300344724266324
18972,85832,85832,171664,532.2658140659332,0.00033003298995026853
19008,86120,86120,172240,533.8652439117432,0.00033003284443111625
19043,86396,86396,172792,535.3672981262207,0.0003300300995761063
19079,86624,86624,173248,536.6573650836945,0.00032961020951916
19114,86780,86780,173560,537.5652050971985,0.0003291168868599925
19150,86986,86986,173972,538.8229739665985,0.0003289350097475108
19185,87260,87260,174520,540.312059879303,0.0003289156247774372
19221,87546,87546,175092,541.8794219493866,0.0003289137948740972
19256,87810,87810,175620,543.4115340709686,0.00032888467649172526
19292,88080,88080,176160,545.1471841335297,0.00032875575016078074
19328,88320,88320,176640,546.6507329940796,0.0003286690443928819
19363,88594,88594,177188,548.1289041042328,0.0003286519931862131
19399,88878,88878,177756,549.6748449802399,0.00032864905369933695
19434,89152,89152,178304,551.1246700286865,0.0003286399951321073
19470,89438,89438,178876,552.6487090587616,0.0003286392839072505
19505,89716,89716,179432,554.1385600566864,0.00032863218257261906
19541,90002,90002,180004,555.7101340293884,0.00032863136038940866
19576,90280,90280,180560,557.2965710163116,0.00032862899024621584
19612,90488,90488,180976,558.5122141838074,0.00032846094109117985
19647,90768,90768,181536,560.0198311805725,0.0003284608028479852
19683,91054,91054,182108,561.592766046524,0.0003284582962805871
19718,91324,91324,182648,563.04030418396,0.00032841384199855383
19754,91610,91610,183220,564.5658838748932,0.00032841209576872643
19789,91888,91888,183776,566.0483441352844,0.00032841040592757054
19825,92172,92172,184344,567.5470089912415,0.00032840537642186973
19860,92452,92452,184904,569.0131788253784,0.00032840523635968566
19896,92712,92712,185424,570.4064419269562,0.0003279142856627004
19932,92870,92870,185740,571.319561958313,0.0003271659843449015
19967,93012,93012,186024,572.1395320892334,0.00032605271735519636
20003,93156,93156,186312,573.009889125824,0.0003184883953508688
20038,93296,93296,186592,573.8358931541443,0.00030322079328470863
20074,93474,93474,186948,574.8507578372955,0.00028257546364329755
20109,93736,93736,187472,576.2397949695587,0.00028262783416721504
20145,93976,93976,187952,577.5557971000671,0.00028135393949924037
20180,94176,94176,188352,578.7005891799927,0.00028133085470471997
20216,94454,94454,188908,580.1960020065308,0.00028132448278483935
20251,94620,94620,189240,581.129243850708,0.00028128353915235493
20287,94780,94780,189560,582.0546209812164,0.00028126810684625525
20322,94928,94928,189856,582.9146590232849,0.0002812103593896609
20358,95072,95072,190144,583.770072221756,0.00028107353500672616
20393,95216,95216,190432,584.5952372550964,0.0002810182049870491
20429,95360,95360,190720,585.4485561847687,0.00028098078109906055
20464,95502,95502,191004,586.3000020980835,0.0002809525285556447
20500,95658,95658,191316,587.200926065445,0.00028090259911550675
20535,95822,95822,191644,588.1471061706543,0.00028080467018298805
20571,95986,95986,191972,589.0902469158173,0.0002807378532452276
20607,96156,96156,192312,590.0999190807343,0.00028069298423361033
20642,96324,96324,192648,591.0452480316162,0.0002806162246997701
20678,96490,96490,192980,591.9914691448212,0.000280529166047927
20713,96710,96710,193420,593.1787750720978,0.00028044004102412146
20749,96896,96896,193792,594.2347021102905,0.00028033462695020717
20784,97172,97172,194344,595.6912560462952,0.00028032348927808926
20820,97458,97458,194916,597.2071740627289,0.0002803200677590212
20855,97732,97732,195464,598.6452639102936,0.00028030743305862416
20891,98016,98016,196032,600.1238679885864,0.0002803047318593599
20926,98296,98296,196592,601.595715045929,0.00028030461362504866
20962,98578,98578,197156,603.0703780651093,0.0002802610233629821
20997,98852,98852,197704,604.4955809116364,0.00028025581923429854
21033,99134,99134,198268,605.999922990799,0.0002802543058351148
21068,99400,99400,198800,607.428092956543,0.00028019267665513325
21104,99674,99674,199348,608.8791010379791,0.00028014189774694387
21139,99952,99952,199904,610.3556401729584,0.0002801376122079091
21175,100238,100238,200476,611.8609600067139,0.0002801362170430366
21211,100526,100526,201052,613.3831300735474,0.00028013609517074656
21246,100800,100800,201600,614.8441541194916,0.00028012171969749033
21282,101086,101086,202172,616.34330701828,0.00028011787435389124
21317,101366,101366,202732,617.819066286087,0.0002801177579385694
21353,101654,101654,203308,619.3303401470184,0.0002801176360662794
21388,101930,101930,203860,620.7932720184326,0.00028011531867377926
21424,102206,102206,204412,622.2343900203705,0.0002798901787173236
21459,102364,102364,204728,623.1472451686859,0.00027856525957759004
21495,102524,102524,205048,624.0592350959778,0.0002782040028250776
21530,102722,102722,205444,625.1783859729767,0.0002777410063572461
21566,102994,102994,205988,626.6209390163422,0.00027773078909376636
21601,103260,103260,206520,628.0485260486603,0.0002777292265818687
21637,103540,103540,207080,629.547581911087,0.00027771735221904237
21672,103816,103816,207632,631.0310881137848,0.00027771528039011173
21708,104054,104054,208108,632.3372161388397,0.0002774967924779048
21743,104210,104210,208420,633.2279198169708,0.0002773677570075961
21779,104412,104412,208824,634.3605530261993,0.0002772553234535735
21815,104644,104644,209288,635.6164391040802,0.00027725302606995683
21850,104922,104922,209844,637.0846180915833,0.000277250033832388
21886,105204,105204,210408,638.5937190055847,0.00027723153289116453
21921,105482,105482,210964,640.0589509010315,0.0002772312491288176
21957,105768,105768,211536,641.5587320327759,0.0002772294574242551
21992,106046,106046,212092,643.0234000682831,0.00027722849699785
22028,106334,106334,212668,644.5673279762268,0.00027722837512556
22063,106602,106602,213204,645.9801480770111,0.00027719106401491445
22099,106886,106886,213772,647.4942910671234,0.00027718968158296775
22134,107160,107160,214320,648.9683170318604,0.0002771861618384719
22170,107446,107446,214892,650.4771399497986,0.00027717938064597547
22205,107670,107670,215340,651.6959049701691,0.00027697801488102414
22241,107850,107850,215700,652.7108669281006,0.00027646533635561354
22276,108064,108064,216128,653.8942432403564,0.00027613635575107764
22312,108346,108346,216692,655.3815131187439,0.00027613103338808287
22347,108610,108610,217220,656.7640142440796,0.0002760947882052278
22383,108782,108782,217564,657.7504179477692,0.0002759216386039043
22419,109064,109064,218128,659.243330001831,0.00027591543039307
22454,109342,109342,218684,660.7198829650879,0.00027591089565248694
22490,109630,109630,219260,662.2372710704803,0.0002759107755991863
22525,109904,109904,219808,663.6684310436249,0.00027590786885411944
22561,110188,110188,220376,665.1753630638123,0.0002758825557975797
22596,110464,110464,220928,666.6519401073456,0.00027588124430621974
22632,110744,110744,221488,668.1253390312195,0.00027585005773289595
22667,111020,111020,222040,669.5596082210541,0.00027584840790950693
22703,111306,111306,222612,671.058266878128,0.00027584600502450485
22738,111584,111584,223168,672.5986320972443,0.00027584421695792116
22774,111866,111866,223732,674.4829361438751,0.0002758024656941416
22809,112142,112142,224284,676.0438048839569,0.00027579772722674534
22845,112430,112430,224860,677.5698320865631,0.0002757976053544553
22880,112708,112708,225416,679.04176902771,0.00027579310699366033
22916,112992,112992,225984,680.8619542121887,0.00027578917615755927
22951,113272,113272,226544,682.5563032627106,0.00027578905792324804
22987,113560,113560,227120,684.3253729343414,0.0002757889396889368
23022,113832,113832,227664,685.9020500183105,0.0002756656740530161
23058,114116,114116,228232,687.5277290344238,0.00027566256358113606
23094,114402,114402,228804,689.1952068805695,0.00027566096287046093
23129,114682,114682,229364,690.6864860057831,0.0002756608482741285
23165,114968,114968,229936,692.2176692485809,0.00027565799609874375
23200,115248,115248,230496,693.6836440563202,0.0002756578796834219
23236,115534,115534,231068,695.1952798366547,0.00027565754498937167
23271,115812,115812,231624,696.6747479438782,0.0002756511439656606
23307,116098,116098,232196,698.1899650096893,0.00027564820447878446
23342,116370,116370,232740,699.707967042923,0.0002755734367383411
23378,116652,116652,233304,701.4463429450989,0.0002755682980932761
23413,116932,116932,233864,703.0456631183624,0.00027556818167795427
23449,117218,117218,234436,704.8415911197662,0.00027555879205465317
23484,117496,117496,234992,706.379830121994,0.0002755576679192018
23520,117782,117782,235564,708.0224261283875,0.00027555606720852666
23555,118062,118062,236124,709.6002979278564,0.0002755559489742154
23591,118348,118348,236696,711.1994450092316,0.0002755543937382754
23626,118626,118626,237252,712.7316429615021,0.0002755525965767447
23662,118912,118912,237824,714.2360162734985,0.0002755492678261362
23698,119200,119200,238400,715.7135128974915,0.00027554914595384616
23733,119480,119480,238960,717.3891389369965,0.00027554902953852434
23769,119766,119766,239532,718.9026260375977,0.00027554431289900094
23804,120044,120044,240088,720.4995121955872,0.0002755418718152214
23840,120332,120332,240664,722.14102602005,0.00027554174994293135
23875,120572,120572,241144,723.5056481361389,0.00027208445499127265
23911,120720,120720,241440,724.3978409767151,0.0002451450982334791
23946,120918,120918,241836,725.4910349845886,0.0001651966285862727
23982,121062,121062,242124,726.3953878879547,0.00016517563381057698
24017,121206,121206,242412,727.3203730583191,0.00016515474271727726
24053,121360,121360,242720,728.3121762275696,0.00016512355250597466
24088,121514,121514,243028,729.2083189487457,0.0001651019829296274
24124,121664,121664,243328,730.0926668643951,0.0001650670383241959
24159,121818,121818,243636,730.9835450649261,0.00016501960453751963
24195,121980,121980,243960,731.910628080368,0.00016496559510414954
24230,122142,122142,244284,732.8192760944366,0.00016490327834617347
24266,122294,122294,244588,733.6966941356659,0.0001648143388592871
24302,122476,122476,244952,734.7158660888672,0.0001647347344260197
24337,122662,122662,245324,735.7418439388275,0.00016470454829686787
24373,122866,122866,245732,736.8580000400543,0.00016467767454741988
24408,123132,123132,246264,738.2662038803101,0.0001646727650950197
24444,123420,123420,246840,739.7972030639648,0.0001646726559556555
24479,123700,123700,247400,741.27499127388,0.0001646725468162913
24515,123988,123988,247976,742.818498134613,0.00016467243767692707
24550,124264,124264,248528,744.2700412273407,0.00016466919259983115
24586,124548,124548,249096,745.9274611473083,0.00016463872270833235
24621,124824,124824,249648,747.5298681259155,0.00016463620704598725
24657,125106,125106,250212,749.1548049449921,0.00016461609629914165
24692,125384,125384,250768,750.6868731975555,0.00016461485211038962
24728,125672,125672,251344,752.3599760532379,0.000164614741152036
24763,125952,125952,251904,753.9029331207275,0.0001646146338316612
24799,126238,126238,252476,755.4086890220642,0.0001646086329856189
24834,126516,126516,253032,756.8446180820465,0.0001646083328523673
24870,126804,126804,253608,758.4532680511475,0.0001646082237130031
24905,127072,127072,254144,759.8947122097015,0.00016449688337161206
24941,127340,127340,254680,761.2917370796204,0.0001644527874304913
24977,127626,127626,255252,762.8098530769348,0.0001644520252739312
25012,127904,127904,255808,764.2621750831604,0.00016445118308183737
25048,128186,128186,256372,765.6912460327148,0.00016444392531411722
25083,128464,128464,256928,767.1431679725647,0.0001644436124479398
25119,128742,128742,257484,768.5972480773926,0.0001643420873733703
25154,129018,129018,258036,770.0300920009613,0.00016433951168437488
25190,129304,129304,258608,771.5384211540222,0.00016433817290817387
25225,129580,129580,259160,772.9913420677185,0.00016433016389783006
25261,129864,129864,259728,774.4551260471344,0.00016432706615887582
25296,130144,130144,260288,775.891175031662,0.00016432695883850101
25332,130432,130432,260864,777.389543056488,0.0001643268496991368
25367,130708,130708,261416,778.8203821182251,0.00016431769472546875
25403,130996,130996,261992,780.3088059425354,0.00016431758194812573
25438,131274,131274,262548,781.7666659355164,0.0001643118666834198
25474,131562,131562,263124,783.2401731014252,0.00016431175572506618
25509,131842,131842,263684,784.7006001472473,0.00016431165022368077
25545,132130,132130,264260,786.1888520717621,0.00016431154108431656
25581,132366,132366,264732,787.4494771957397,0.00016336169392161537
25616,132596,132596,265192,788.6923069953918,0.00016345269432349596
25652,132864,132864,265728,790.093090057373,0.00016334732754330616
25687,133144,133144,266288,791.5372490882874,0.00016334722204192076
25723,133426,133426,266852,793.0284328460693,0.00016334552856278606
25758,133704,133704,267408,794.4773650169373,0.00016334351312252693
25794,133992,133992,267984,795.9578812122345,0.0001633434021641733
25829,134272,134272,268544,797.3979241847992,0.0001633432948437985
25865,134558,134558,269116,798.8924958705902,0.0001633425781619735
25900,134838,134838,269676,800.3399200439453,0.0001633424708415987
25936,135126,135126,270252,801.8529851436615,0.00016334236170223448
25971,135406,135406,270812,803.3136692047119,0.00016334225438185968
26007,135694,135694,271388,804.8131730556488,0.00016334214342350606
26042,135974,135974,271948,806.2793111801147,0.00016334203610313125
26078,136262,136262,272524,807.7841711044312,0.00016334192696376704
26113,136510,136510,273020,809.0712180137634,0.0001633375431993045
26149,136720,136720,273440,810.2109251022339,0.00016332817904185504
26185,137006,137006,274012,811.6808750629425,0.0001633265637792647
26220,137286,137286,274572,813.1362502574921,0.00016332645827787928
26256,137572,137572,275144,814.6388108730316,0.00016332425184373278
26291,137848,137848,275696,816.0716469287872,0.00016331624283338897
26327,138134,138134,276268,817.5529391765594,0.00016331580809492152
26362,138412,138412,276824,819.0296719074249,0.00016331530423485674
26398,138694,138694,277388,820.5426502227783,0.00016330737162206788
26433,138972,138972,277944,822.0846831798553,0.0001633030260563828
26469,139256,139256,278512,823.6734561920166,0.00016329521895386279
26504,139532,139532,279064,825.2330861091614,0.00016326451623172034
26540,139818,139818,279636,827.0403578281403,0.00016326205332006793
26575,140098,140098,280196,828.6689960956573,0.00016326194418070372
26611,140380,140380,280760,830.1599960327148,0.00016325559772667475
26646,140660,140660,281320,831.8042261600494,0.00016325549222528934
26682,140946,140946,281892,833.3947021961212,0.00016325343312928453
26717,141226,141226,282452,834.9151329994202,0.00016325332580890972
26753,141510,141510,283020,836.4997041225433,0.00016324908028764185
26789,141798,141798,283596,838.3131620883942,0.00016324897114827763
26824,142078,142078,284156,839.9009459018707,0.00016324886382790282
26860,142364,142364,284728,841.4655921459198,0.00016324262651323806
26895,142642,142642,285284,843.1139562129974,0.00016324219359376002
26931,142928,142928,285856,844.6386210918427,0.00016324185344274156
26966,143206,143206,286412,846.0946459770203,0.00016324013995472342
27002,143492,143492,286984,847.5937721729279,0.0001632381845411146
27037,143770,143770,287540,849.0518450737,0.00016323661111528054
27073,144058,144058,288116,850.5510149002075,0.00016323650197591633
27108,144338,144338,288676,852.0206878185272,0.00016323639465554152
27144,144626,144626,289252,853.5365839004517,0.0001632362836971879
27179,144862,144862,289724,854.8003950119019,0.00016108207273646258
27215,145038,145038,290076,855.7959549427032,0.00015968974912539124
27250,145186,145186,290372,856.6259920597076,0.00015755853928567376
27286,145338,145338,290676,857.5004422664642,0.00015133642773434985
27321,145482,145482,290964,858.3307280540466,0.00014751198978046887
27357,145630,145630,291260,859.1862530708313,0.00013984514589537866
27392,145770,145770,291540,860.0101251602173,0.00013453066640067846
27428,145930,145930,291860,860.9205939769745,0.00010811994798132218
27464,146172,146172,292344,862.2089960575104,0.00010798941184475552
27499,146380,146380,292760,863.3392939567566,0.00010797447794175241
27535,146614,146614,293228,864.5947070121765,0.00010794083209475502
27570,146758,146758,293516,865.4661099910736,0.00010793457295221742
27606,146902,146902,293804,866.475438117981,0.00010792350985866506
27641,147046,147046,294092,867.3869760036469,0.0001079116809705738
27677,147198,147198,294396,868.414489030838,0.00010790164196805563
27712,147354,147354,294708,869.3067572116852,0.00010789155930979177
27748,147508,147508,295016,870.1737291812897,0.00010785147424030583
27783,147652,147652,295304,871.0092730522156,0.0001077630204235902
27819,147806,147806,295612,871.8894729614258,0.00010773610847536474
27854,147964,147964,295928,872.9349410533905,0.00010772030691441614
27890,148194,148194,296388,874.3481631278992,0.00010769538675958756
27925,148382,148382,296764,875.3886280059814,0.0001076535445463378
27961,148574,148574,297148,876.4558100700378,0.00010761284283944406
27996,148844,148844,297688,877.8843882083893,0.00010758796815935057
28032,149126,149126,298252,879.3661539554596,0.000107585725345416
28068,149406,149406,298812,880.8232178688049,0.00010758327152871061
28103,149684,149684,299368,882.2708611488342,0.00010758159260149114
28139,149972,149972,299944,883.7730638980865,0.00010758153621281963
28174,150248,150248,300496,885.206433057785,0.00010757987001852598
28210,150506,150506,301012,886.5724930763245,0.00010752199523267336
28245,150742,150742,301484,887.8202090263367,0.00010747186024673283
28281,151022,151022,302044,889.2861561775208,0.00010747059604909737
28316,151290,151290,302580,890.6588742733002,0.00010746643238235265
28352,151480,151480,302960,891.69944190979,0.00010744267638074234
28387,151728,151728,303456,893.0057010650635,0.00010743314305727836
28423,152010,152010,304020,894.4833731651306,0.00010742913400463294
28458,152286,152286,304572,895.912623167038,0.000107427624243428
28494,152570,152570,305140,897.3867330551147,0.00010742721860879101
28529,152850,152850,305700,898.8333210945129,0.0001074271622201195
28565,153134,153134,306268,900.3005890846252,0.00010741703590610996
28600,153412,153412,306824,901.752424955368,0.000107416648461367
28636,153696,153696,307392,903.2179090976715,0.00010741595360741485
28672,153926,153926,307852,904.4477560520172,0.00010718928569986019
28707,154144,154144,308288,905.6178991794586,0.0001065936576196691
28743,154298,154298,308596,906.4943220615387,0.00010540259063418489
28778,154450,154450,308900,907.3687932491302,0.00010425148684589658
28814,154616,154616,309232,908.3261299133301,0.00010364617264713161
28849,154758,154758,309516,909.1438610553741,0.00010265979835821781
28885,154912,154912,309824,910.0290172100067,0.00010052404468297027
28920,155052,155052,310104,910.8488600254059,9.682539348432329e-05
28956,155208,155208,310416,911.7476532459259,9.327813677373342e-05
28991,155416,155416,310832,912.8853430747986,9.044095168064814e-05
29027,155658,155658,311316,914.1833591461182,9.045602746482473e-05
29062,155854,155854,311708,915.2320051193237,9.110439896176104e-05
29098,156018,156018,312036,916.1730461120605,9.133392268267926e-05
29133,156204,156204,312408,917.1910600662231,9.044445141626056e-05
29169,156424,156424,312848,918.3795690536499,9.043940190167632e-05
29204,156684,156684,313368,919.7517590522766,9.043870522873476e-05
29240,156960,156960,313920,921.197765827179,9.043286081578117e-05
29276,157104,157104,314208,922.0276050567627,9.038857751875184e-05
29311,157248,157248,314496,922.875333070755,9.037871132022701e-05
29347,157410,157410,314820,923.7963171005249,9.036941082740668e-05
29382,157564,157564,315128,924.6763589382172,9.03603940969333e-05
29418,157756,157756,315512,925.7259268760681,9.034822141984478e-05
29453,157922,157922,315844,926.6625680923462,9.031598528963514e-05
29489,158088,158088,316176,927.6001920700073,9.02789251995273e-05
29524,158288,158288,316576,928.6881589889526,9.024742212204728e-05
29560,158566,158566,317132,930.1572329998016,9.024472819874063e-05
29595,158758,158758,317516,931.220269203186,9.022899757837877e-05
29631,158936,158936,317872,932.22043800354,9.021211008075625e-05
29666,159106,159106,318212,933.1719648838043,9.017368392960634e-05
29702,159284,159284,318568,934.1984980106354,9.014409079100005e-05
29737,159494,159494,318988,935.4034402370453,9.004246203403454e-05
29773,159660,159660,319320,936.3915300369263,8.995393181976397e-05
29808,159818,159818,319636,937.3887870311737,8.991580943984445e-05
29844,159998,159998,319996,938.4992158412933,8.985047497844789e-05
29879,160252,160252,320504,939.9374599456787,8.984288251667749e-05
29915,160530,160530,321060,941.5449900627136,8.984059422800783e-05
29951,160778,160778,321556,943.0003509521484,8.982973849924747e-05
29986,161052,161052,322104,944.4302752017975,8.982756480691023e-05
30022,161314,161314,322628,945.7899429798126,8.978385631053243e-05
30057,161532,161532,323064,946.9469990730286,8.975057062343694e-05
30093,161818,161818,323636,948.4103670120239,8.974756747193169e-05
30128,162096,162096,324192,949.8670279979706,8.974716729426291e-05
30164,162376,162376,324752,951.3175821304321,8.974402408057358e-05
30199,162650,162650,325300,952.6964921951294,8.973258445621468e-05
30235,162936,162936,325872,954.1893770694733,8.973213698482141e-05
30270,163216,163216,326432,955.7333319187164,8.973208787210751e-05
30306,163498,163498,326996,957.4574029445648,8.97313620953355e-05
30341,163768,163768,327536,958.9743430614471,8.972138675744645e-05
30377,164054,164054,328108,960.5655879974365,8.972128125606105e-05
30412,164334,164334,328668,962.1552929878235,8.972123396233656e-05
30448,164614,164614,329228,963.6502740383148,8.971893657871988e-05
30483,164892,164892,329784,965.1243619918823,8.971857459982857e-05
30519,165176,165176,330352,966.6252150535583,8.97165919013787e-05
30555,165462,165462,330924,968.1411280632019,8.971537499746773e-05
30590,165738,165738,331476,969.5925529003143,8.97135632840218e-05
30626,166020,166020,332040,971.0920362472534,8.96962719707517e-05
30661,166216,166216,332432,972.1578931808472,8.926158807298634e-05
30697,166390,166390,332780,973.1381850242615,8.889622040442191e-05
30732,166538,166538,333076,973.9854872226715,8.742079626244958e-05
30768,166694,166694,333388,974.9518721103668,8.659271588840056e-05
30803,166862,166862,333724,975.8849761486053,8.557085129723419e-05
30839,167012,167012,334024,976.7612009048462,8.457644617010374e-05
30874,167166,167166,334332,977.8043200969696,8.28973115858389e-05
30910,167326,167326,334652,978.8115479946136,8.18791268102359e-05
30945,167474,167474,334948,979.7536981105804,7.989959158294369e-05
30981,167622,167622,335244,980.6190259456635,7.759575601085089e-05
31016,167764,167764,335528,981.4475772380829,7.133524195523933e-05
31052,167908,167908,335816,982.2933912277222,6.398268124030437e-05
31087,168052,168052,336104,983.1262350082397,5.544068153540138e-05
31123,168204,168204,336408,984.0084049701691,4.810762402485125e-05
31159,168348,168348,336696,984.894453048706,4.722105950349942e-05
31194,168488,168488,336976,985.7154240608215,4.670799171435647e-05
31230,168636,168636,337272,986.5814049243927,3.694379665830638e-05
31265,168780,168780,337560,987.4342601299286,2.5973920855903998e-05
31301,169026,169026,338052,988.7599229812622,2.4093949832604267e-05
31336,169268,169268,338536,990.0421171188354,2.4077779016806744e-05
31372,169544,169544,339088,991.4487071037292,2.4076680347207002e-05
31407,169734,169734,339468,992.5084159374237,2.4069247956504114e-05
31443,169874,169874,339748,993.3290500640869,2.4062655938905664e-05
31478,170012,170012,340024,994.1480441093445,2.4056591428234242e-05
31514,170158,170158,340316,994.9972422122955,2.405471241218038e-05
31549,170298,170298,340596,995.8022210597992,2.4047281840466894e-05
31585,170450,170450,340900,996.6628749370575,2.4036713512032293e-05
31620,170642,170642,341284,997.6937611103058,2.4033104637055658e-05
31656,170840,170840,341680,998.8111202716827,2.403055077593308e-05
31691,171000,171000,342000,999.7218198776245,2.4027265681070276e-05
31727,171154,171154,342308,1000.608724117279,2.401739766355604e-05
31763,171302,171302,342604,1001.4846980571747,2.3989288820303045e-05
31798,171454,171454,342908,1002.3470611572266,2.3974309442564845e-05
31834,171602,171602,343204,1003.2104299068451,2.395953742961865e-05
31869,171748,171748,343496,1004.0547158718109,2.3953465642989613e-05
31905,171894,171894,343788,1004.9022221565247,2.3945827706484124e-05
31940,172046,172046,344092,1005.7817878723145,2.3938049707794562e-05
31976,172206,172206,344412,1006.6928472518921,2.39265264099231e-05
32011,172370,172370,344740,1007.6309361457825,2.3921957108541392e-05
32047,172528,172528,345056,1008.5332000255585,2.391491216258146e-05
32082,172696,172696,345392,1009.4785301685333,2.390510962868575e-05
32118,172884,172884,345768,1010.5028109550476,2.3895872800494544e-05
32153,173092,173092,346184,1011.6321210861206,2.3890439479146153e-05
32189,173260,173260,346520,1012.5800859928131,2.3882495952420868e-05
32224,173436,173436,346872,1013.5407092571259,2.3869981305324472e-05
32260,173658,173658,347316,1014.7396841049194,2.3860529836383648e-05
32295,173892,173892,347784,1015.9962041378021,2.385781226621475e-05
32331,174078,174078,348156,1017.033774137497,2.3855927793192677e-05
32366,174244,174244,348488,1017.9705650806427,2.3847605916671455e-05
32402,174442,174442,348884,1019.0751402378082,2.3840004359954037e-05
32438,174690,174690,349380,1020.3930051326752,2.3838674678700045e-05
32473,174890,174890,349780,1021.4828870296478,2.3835536921978928e-05
32509,175082,175082,350164,1022.5528891086578,2.3832229999243282e-05
32544,175264,175264,350528,1023.5632441043854,2.3816837710910477e-05
32580,175488,175488,350976,1024.7917921543121,2.3793281798134558e-05
32615,175676,175676,351352,1025.8266010284424,2.3746413717162795e-05
32651,175828,175828,351656,1026.6829681396484,2.3613276425749063e-05
32686,175980,175980,351960,1027.5502121448517,2.3393035007757135e-05
32722,176128,176128,352256,1028.4084658622742,2.2880887627252378e-05
32757,176270,176270,352540,1029.229653120041,2.2628655642620288e-05
32793,176452,176452,352904,1030.2391710281372,2.2616892238147557e-05
32828,176604,176604,353208,1031.1086132526398,2.2673591956845485e-05
32864,176776,176776,353552,1032.0717260837555,2.2474443539977074e-05
32899,176924,176924,353848,1032.9249889850616,2.2062220523366705e-05
32935,177072,177072,354144,1033.7922520637512,2.1260408175294288e-05
32970,177218,177218,354436,1034.6462779045105,2.0862469682469964e-05
33006,177370,177370,354740,1035.5412049293518,2.0435671103768982e-05
33042,177522,177522,355044,1036.4125719070435,1.9987739506177604e-05
33077,177662,177662,355324,1037.2107660770416,1.8585862562758848e-05
33113,177810,177810,355620,1038.0864441394806,1.6498257537023164e-05
33148,177950,177950,355900,1038.901848077774,1.3833710909239016e-05
33184,178094,178094,356188,1039.7326200008392,1.1092590284533799e-05
33219,178304,178304,356608,1040.902459859848,9.296847565565258e-06
33255,178452,178452,356904,1041.8055412769318,9.294295523432083e-06
33290,178688,178688,357376,1043.1544120311737,9.293486073147506e-06
33326,178892,178892,357784,1044.3715488910675,9.292183676734567e-06
33361,179040,179040,358080,1045.2542231082916,9.291470632888377e-06
33397,179192,179192,358384,1046.1843130588531,9.28945155465044e-06
33432,179332,179332,358664,1047.0602071285248,9.281438906327821e-06
33468,179484,179484,358968,1048.113186120987,9.277795470552519e-06
33503,179640,179640,359280,1049.0178079605103,9.276740456698462e-06
33539,179792,179792,359584,1049.888128042221,9.272436727769673e-06
33574,179936,179936,359872,1050.7143139839172,9.266364941140637e-06
33610,180084,180084,360168,1051.5857601165771,9.261624654754996e-06
33646,180244,180244,360488,1052.5018730163574,9.256689736503176e-06
33681,180396,180396,360792,1053.3897001743317,9.250194125343114e-06
33717,180578,180578,361156,1054.4118490219116,9.2491609393619e-06
33752,180768,180768,361536,1055.4603550434113,9.245957699022256e-06
33788,180960,180960,361920,1056.5077571868896,9.244871762348339e-06
33823,181118,181118,362236,1057.4068710803986,9.242849046131596e-06
33859,181300,181300,362600,1058.4204621315002,9.240729923476465e-06
33894,181470,181470,362940,1059.4634492397308,9.238050552085042e-06
33930,181638,181638,363276,1060.3929979801178,9.234880053554662e-06
33965,181820,181820,363640,1061.7893152236938,9.233343007508665e-06
34001,182008,182008,364016,1062.9329640865326,9.231542207999155e-06
34036,182194,182194,364388,1064.2836139202118,9.229972420143895e-06
34072,182380,182380,364760,1065.7131509780884,9.228157068719156e-06
34107,182584,182584,365168,1066.9047801494598,9.226279871654697e-06
34143,182764,182764,365528,1068.0649752616882,9.222578228218481e-06
34178,182962,182962,365924,1069.5507760047913,9.2179707280593e-06
34214,183162,183162,366324,1070.9113790988922,9.214796591550112e-06
34250,183346,183346,366692,1072.0582389831543,9.205450623994693e-06
34285,183544,183544,367088,1073.3558950424194,9.192144716507755e-06
34321,183724,183724,367448,1074.6268830299377,9.179966582451016e-06
34356,183896,183896,367792,1075.6584131717682,9.159835826721974e-06
34392,184114,184114,368228,1076.8889548778534,9.136914741247892e-06
34427,184290,184290,368580,1077.8833589553833,9.105069693760015e-06
34463,184450,184450,368900,1078.9108889102936,9.080462405108847e-06
34498,184608,184608,369216,1080.1639811992645,9.054776455741376e-06
34534,184792,184792,369584,1082.107535123825,9.006025720736943e-06
34569,184950,184950,369900,1083.6726121902466,8.947052265284583e-06
34605,185104,185104,370208,1084.5707468986511,8.881632311386056e-06
34640,185276,185276,370552,1085.548525094986,8.774855814408511e-06
34676,185426,185426,370852,1086.4212369918823,8.636183338239789e-06
34711,185580,185580,371160,1087.304003238678,8.497418093611486e-06
34747,185732,185732,371464,1088.1913521289825,8.489394531352445e-06
34782,185888,185888,371776,1089.0712461471558,8.386341505683959e-06
34818,186040,186040,372080,1089.953663110733,8.057473678491078e-06
34853,186180,186180,372360,1090.7673921585083,7.74579712015111e-06
34889,186336,186336,372672,1091.6751170158386,7.492490112781525e-06
34925,186484,186484,372968,1092.5469450950623,7.093291060300544e-06
34960,186626,186626,373252,1093.3903832435608,6.706481144647114e-06
34996,186770,186770,373540,1094.2188129425049,6.0691127146128565e-06
35031,186914,186914,373828,1095.0699081420898,4.952315066475421e-06
35067,187064,187064,374128,1095.9133050441742,3.961758920922875e-06
35102,187206,187206,374412,1096.746433019638,3.022982127731666e-06
35138,187342,187342,374684,1097.5592651367188,1.8929567886516452e-06
35173,187460,187460,374920,1098.283075094223,7.780054147588089e-07
35209,187584,187584,375168,1099.050499200821,2.426950231892988e-07
35244,187700,187700,375400,1099.7601511478424,1.7196725821122527e-08
35280,187824,187824,375648,1100.4983401298523,1.0649091564118862e-07
35315,187942,187942,375884,1101.2272820472717,1.713851816020906e-08
35351,188064,188064,376128,1101.9810190200806,7.952621672302485e-09
35386,188188,188188,376376,1102.7342040538788,6.801201379857957e-09
35422,188332,188332,376664,1103.5915460586548,5.178662831895053e-09
35457,188472,188472,376944,1104.4045979976654,3.5324774216860533e-09
35493,188616,188616,377232,1105.2502081394196,6.45741238258779e-11


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.0013380050659179688,848.0296294260013
26,54,27,81,0.03875422477722168,64.55440294495315
52,106,53,159,0.07812714576721191,54.22509003574646
78,158,79,237,0.11524724960327148,51.2969092672995
104,210,105,315,0.16167616844177246,48.72297871866749
129,260,130,390,0.19779610633850098,46.74075616746313
155,312,156,468,0.2304689884185791,44.43631605511496
181,364,182,546,0.2641868591308594,42.71364398680453
207,416,208,624,0.29657506942749023,40.73060747976024
233,468,234,702,0.3298759460449219,39.087079665765486
259,520,260,780,0.36219024658203125,37.332305536422155
285,572,286,858,0.3932528495788574,36.03472597627729
311,624,312,936,0.4252650737762451,34.861416548359784
337,676,338,1014,0.4582381248474121,33.65773857761383
363,728,364,1092,0.48850321769714355,32.58253864491621
388,778,389,1167,0.5180909633636475,31.644703310142177
414,830,415,1245,0.5485019683837891,30.658344269839517
440,882,441,1323,0.5788891315460205,29.76121898938527
466,934,467,1401,0.6091899871826172,28.893073472229844
492,986,493,1479,0.6394820213317871,27.98442518028901
518,1038,519,1557,0.6700711250305176,27.27382269331838
544,1090,545,1635,0.7010071277618408,26.632419444260677
570,1142,571,1713,0.7323331832885742,25.776650215247628
596,1194,597,1791,0.7643001079559326,25.033858078960748
621,1244,622,1866,0.7956140041351318,24.38877585334626
647,1296,648,1944,0.8287889957427979,23.884737122102933
673,1348,674,2022,0.861004114151001,23.14966530322249
699,1400,700,2100,0.8920278549194336,22.523100178724917
725,1452,726,2178,0.9245262145996094,22.017996133548422
751,1504,752,2256,0.9587399959564209,21.464858332583844
777,1556,778,2334,0.9931089878082275,20.98192310671834
803,1608,804,2412,1.0267038345336914,20.460179121105284
829,1660,830,2490,1.060230016708374,19.99264850112104
855,1712,856,2568,1.0920259952545166,19.496596493037487
880,1762,881,2643,1.1272971630096436,19.096591161775223
906,1814,907,2721,1.1602060794830322,18.63602398024318
932,1866,933,2799,1.1920130252838135,18.217339574553534
958,1918,959,2877,1.223886251449585,17.743323062224817
984,1970,985,2955,1.2553470134735107,17.39954682883058
1010,2022,1011,3033,1.2863199710845947,16.899319557106082
1036,2074,1037,3111,1.317944049835205,16.544207100359245
1062,2126,1063,3189,1.3498179912567139,16.156176624285536
1088,2178,1089,3267,1.381343126296997,15.796283555119203
1113,2228,1114,3342,1.4142279624938965,15.413354952006898
1139,2280,1140,3420,1.4463071823120117,15.079879678087877
1165,2332,1166,3498,1.479072093963623,14.671344576619276
1191,2384,1192,3576,1.5109572410583496,14.321231743000794
1217,2436,1218,3654,1.5425889492034912,13.974641827623486
1243,2488,1244,3732,1.5741472244262695,13.691403627591512
1269,2540,1270,3810,1.6067490577697754,13.345334473184494
1295,2592,1296,3888,1.6377081871032715,13.056265189725991
1321,2644,1322,3966,1.669348955154419,12.756130723805086
1347,2696,1348,4044,1.7003378868103027,12.465504141307633
1372,2746,1373,4119,1.7315011024475098,12.179080601483747
1398,2798,1399,4197,1.7634949684143066,11.879805570098256
1424,2850,1425,4275,1.7955269813537598,11.573713554482993
1450,2902,1451,4353,1.8277971744537354,11.31738306363411
1476,2954,1477,4431,1.8599040508270264,11.010097380303932
1502,3006,1503,4509,1.8917372226715088,10.808895255114635
1528,3058,1529,4587,1.9249138832092285,10.510792807917142
1554,3110,1555,4665,1.9578461647033691,10.291354840989584
1580,3162,1581,4743,1.9896290302276611,10.072079031799376
1605,3212,1606,4818,2.020695209503174,9.826333154595545
1631,3264,1632,4896,2.053359270095825,9.5662735381718
1657,3316,1658,4974,2.087393045425415,9.377416467291368
1683,3368,1684,5052,2.1211960315704346,9.161177453901587
1709,3420,1710,5130,2.1535820960998535,8.954672917738094
1735,3472,1736,5208,2.1854941844940186,8.755777858355145
1761,3524,1762,5286,2.222170829772949,8.547245145683632
1787,3576,1788,5364,2.2604410648345947,8.365212184241841
1813,3628,1814,5442,2.296041965484619,8.176834833998214
1839,3680,1840,5520,2.3287570476531982,7.9789181397180755
1864,3730,1865,5595,2.3717310428619385,7.779077630457323
1890,3782,1891,5673,2.403496026992798,7.597797091993698
1916,3834,1917,5751,2.43458890914917,7.417125140957069
1942,3886,1943,5829,2.465837240219116,7.271273415001019
1968,3938,1969,5907,2.4967780113220215,7.100406416774035
1994,3990,1995,5985,2.5292410850524902,6.971343847407866
2020,4042,2021,6063,2.5706288814544678,6.794730799243325
2046,4094,2047,6141,2.6034839153289795,6.667588717332023
2072,4146,2073,6219,2.6346702575683594,6.518530663246111
2097,4196,2098,6294,2.66723895072937,6.395856717360402
2123,4248,2124,6372,2.702852249145508,6.249954589872232
2149,4300,2150,6450,2.7347099781036377,6.1285117852759186
2175,4352,2176,6528,2.7669310569763184,6.007991640511818
2201,4404,2202,6606,2.798927068710327,5.871239533860603
2227,4456,2228,6684,2.8321008682250977,5.741786242539092
2253,4508,2254,6762,2.865093946456909,5.595760754569483
2279,4560,2280,6840,2.897611141204834,5.4877420492554165
2305,4612,2306,6918,2.9300990104675293,5.381440312968493
2331,4664,2332,6996,2.962351083755493,5.2657242542974245
2356,4714,2357,7071,2.9924230575561523,5.164887049658773
2382,4766,2383,7149,3.0255730152130127,5.053946727879747
2408,4818,2409,7227,3.0620691776275635,4.934487992532581
2434,4870,2435,7305,3.09454607963562,4.830610095022735
2460,4922,2461,7383,3.126134157180786,4.723752453326824
2486,4974,2487,7461,3.1594879627227783,4.635206789783524
2512,5026,2513,7539,3.1907169818878174,4.534577580845621
2538,5078,2539,7617,3.2242910861968994,4.435307488862691
2564,5130,2565,7695,3.2558341026306152,4.343919424261458
2589,5180,2590,7770,3.28741717338562,4.248667728689838
2615,5232,2616,7848,3.320863962173462,4.1543978278222085
2641,5284,2642,7926,3.3543481826782227,4.06360321614261
2667,5336,2668,8004,3.3863251209259033,3.984443010754717
2693,5388,2694,8082,3.420681953430176,3.896648972354569
2719,5440,2720,8160,3.455435037612915,3.8055699341405216
2745,5492,2746,8238,3.4883241653442383,3.7277595080684023
2771,5544,2772,8316,3.522062063217163,3.643820797674721
2797,5596,2798,8394,3.5641160011291504,3.573484532991415
2823,5648,2824,8472,3.5975260734558105,3.5006644175980455
2848,5698,2849,8547,3.630237102508545,3.426478353845596
2874,5750,2875,8625,3.673424005508423,3.3493800544190435
2900,5802,2901,8703,3.714553117752075,3.2742872959531724
2926,5854,2927,8781,3.7573490142822266,3.1942545933353585
2952,5906,2953,8859,3.791774034500122,3.1325427138531268
2978,5958,2979,8937,3.8243770599365234,3.06671029882898
3004,6010,3005,9015,3.862215042114258,3.00314073330685
3030,6062,3031,9093,3.8950350284576416,2.9499246011569085
3056,6114,3057,9171,3.9272570610046387,2.876919439614767
3081,6164,3082,9246,3.9581000804901123,2.8235996358640705
3107,6216,3108,9324,3.99005389213562,2.761865547683101
3133,6268,3134,9402,4.026061058044434,2.711254818505722
3159,6320,3160,9480,4.067285060882568,2.65476738661323
3185,6372,3186,9558,4.101819038391113,2.6076291315226854
3211,6424,3212,9636,4.136611223220825,2.5537932540888733
3237,6476,3238,9714,4.1849470138549805,2.508017372308359
3263,6528,3264,9792,4.22446608543396,2.456689298007859
3289,6580,3290,9870,4.259695291519165,2.4017173389752315
3315,6632,3316,9948,4.302698135375977,2.358619146934643
3340,6682,3341,10023,4.3410749435424805,2.3102868630620605
3366,6734,3367,10101,4.380881071090698,2.2600065238076468
3392,6786,3393,10179,4.434319257736206,2.2192334923530552
3418,6838,3419,10257,4.478191137313843,2.171428242212528
3444,6890,3445,10335,4.522029161453247,2.130923903506414
3470,6942,3471,10413,4.569005012512207,2.089940858676073
3496,6994,3497,10491,4.609097957611084,2.0517985539448773
3522,7046,3523,10569,4.649423837661743,2.0101641931411223
3548,7098,3549,10647,4.691973924636841,1.9713055262566286
3573,7148,3574,10722,4.734377145767212,1.9326929940564241
3599,7200,3600,10800,4.7766640186309814,1.8920624705403952
3625,7252,3626,10878,4.820632219314575,1.8559192969501055
3651,7304,3652,10956,4.862404823303223,1.8169066127536553
3677,7356,3678,11034,4.904090166091919,1.7795488150221672
3703,7408,3704,11112,4.941892862319946,1.7432217596507371
3729,7460,3730,11190,4.980417013168335,1.7090260225927523
3755,7512,3756,11268,5.019272089004517,1.6775808948925715
3781,7564,3782,11346,5.062787055969238,1.6452358593304552
3807,7616,3808,11424,5.1071391105651855,1.6166003574123806
3832,7666,3833,11499,5.139852046966553,1.5823864060167807
3858,7718,3859,11577,5.175869941711426,1.5564857210861192
3884,7770,3885,11655,5.2115678787231445,1.523059778140805
3910,7822,3911,11733,5.248098134994507,1.4925730139952975
3936,7874,3937,11811,5.2874979972839355,1.456877339508651
3962,7926,3963,11889,5.32738995552063,1.4273020682762763
3988,7978,3989,11967,5.386125087738037,1.3935744952474352
4014,8030,4015,12045,5.448139190673828,1.364236196827278
4040,8082,4041,12123,5.506074905395508,1.3377185652051367
4065,8132,4066,12198,5.5661211013793945,1.3142417650691414
4091,8184,4092,12276,5.605145215988159,1.2865148508889206
4117,8236,4118,12354,5.643064022064209,1.2647977159991797
4143,8288,4144,12432,5.680459022521973,1.233356781428597
4169,8340,4170,12510,5.7168920040130615,1.2122239562174855
4195,8392,4196,12588,5.748471021652222,1.1857824146770781
4221,8444,4222,12666,5.7812340259552,1.1658052585477208
4247,8496,4248,12744,5.813474178314209,1.1409037775135857
4273,8548,4274,12822,5.844692945480347,1.1221698918147922
4299,8600,4300,12900,5.877887010574341,1.0983877708569025
4324,8650,4325,12975,5.909085988998413,1.0784264927693812
4350,8702,4351,13053,5.940519094467163,1.0575797244581508
4376,8754,4377,13131,5.9726879596710205,1.0411863819617793
4402,8806,4403,13209,6.004653215408325,1.0184627887803117
4428,8858,4429,13287,6.03909707069397,0.9996042567518089
4454,8910,4455,13365,6.071835994720459,0.9810410080719976
4480,8962,4481,13443,6.103454113006592,0.9619839900936995
4506,9014,4507,13521,6.136389970779419,0.9457512061624129
4532,9066,4533,13599,6.170150995254517,0.9263325188439921
4558,9118,4559,13677,6.2021472454071045,0.9078027159144995
4583,9168,4584,13752,6.232576131820679,0.8938890073335415
4609,9220,4610,13830,6.264657020568848,0.87397436363824
4635,9272,4636,13908,6.29597282409668,0.8554724705459194
4661,9324,4662,13986,6.328663110733032,0.8394402454010788
4687,9376,4688,14064,6.360320091247559,0.8211654535648449
4713,9428,4714,14142,6.391748905181885,0.8056871818102991
4739,9480,4740,14220,6.422648191452026,0.790487812439892
4765,9532,4766,14298,6.453912019729614,0.7766888413459583
4791,9584,4792,14376,6.484600067138672,0.7600927170526575
4816,9634,4817,14451,6.514842987060547,0.7482223485787927
4842,9686,4843,14529,6.545650959014893,0.7334171972430568
4868,9738,4869,14607,6.584417104721069,0.7206435594777076
4894,9790,4895,14685,6.617176055908203,0.7058119215914758
4920,9842,4921,14763,6.648874998092651,0.6934073755485315
4946,9894,4947,14841,6.682165145874023,0.6772689686090416
4972,9946,4973,14919,6.714212894439697,0.6654689520771626
4998,9998,4999,14997,6.749465227127075,0.6505907214433364
5024,10050,5025,15075,6.782247066497803,0.6392163299052527
5050,10102,5051,15153,6.813384056091309,0.6284885096171138
5075,10152,5076,15228,6.842666149139404,0.6198768841419451
5101,10204,5102,15306,6.874150991439819,0.6057195174215622
5127,10256,5128,15384,6.90506911277771,0.5933908032951649
5153,10308,5154,15462,6.935479164123535,0.5800412660561278
5179,10360,5180,15540,6.9665422439575195,0.5697731497725727
5205,10412,5206,15618,6.996830940246582,0.5604054627007145
5231,10464,5232,15696,7.028916120529175,0.5497396805941435
5257,10516,5258,15774,7.065083026885986,0.5400916386435028
5283,10568,5284,15852,7.098427057266235,0.529425072618892
5308,10618,5309,15927,7.129975080490112,0.5192307388290374
5334,10670,5335,16005,7.163006067276001,0.5084733481963895
5360,10722,5361,16083,7.1944899559021,0.4996620600282995
5386,10774,5387,16161,7.226233959197998,0.4891552348897221
5412,10826,5413,16239,7.2573230266571045,0.48046308450091146
5438,10878,5439,16317,7.2879040241241455,0.4730683393485151
5464,10930,5465,16395,7.319252967834473,0.4634995210934676
5490,10982,5491,16473,7.351169109344482,0.4550512076898485
5516,11034,5517,16551,7.3830389976501465,0.4461184943892249
5542,11086,5543,16629,7.413646221160889,0.43835492213122507
5567,11136,5568,16704,7.442866086959839,0.43029951304083625
5593,11188,5594,16782,7.474086046218872,0.4220698081852561
5619,11240,5620,16860,7.506273031234741,0.41429418135555807
5645,11292,5646,16938,7.53666615486145,0.406263227637055
5671,11344,5672,17016,7.568187952041626,0.39831266493195017
5697,11396,5698,17094,7.598288059234619,0.39144347363765064
5723,11448,5724,17172,7.628852128982544,0.38356540071458767
5749,11500,5750,17250,7.661334991455078,0.37719250395423387
5775,11552,5776,17328,7.691876173019409,0.3695133301864644
5800,11602,5801,17403,7.721864938735962,0.36341741761555113
5826,11654,5827,17481,7.754679203033447,0.35803129569615066
5852,11706,5853,17559,7.790459871292114,0.35017904103233377
5878,11758,5879,17637,7.82219123840332,0.3432850277616808
5904,11810,5905,17715,7.853384017944336,0.33790890550551467
5930,11862,5931,17793,7.883949041366577,0.3310126231664299
5956,11914,5957,17871,7.915164947509766,0.32562192316697747
5982,11966,5983,17949,7.951730012893677,0.3194317769539339
6008,12018,6009,18027,7.982860088348389,0.3134580888745404
6034,12070,6035,18105,8.014262199401855,0.31026669042546473
6059,12120,6060,18180,8.04348111152649,0.3013958757809405
6085,12172,6086,18258,8.074532270431519,0.29560097974763266
6111,12224,6112,18336,8.105309009552002,0.2904883282373021
6137,12276,6138,18414,8.135422945022583,0.28513431574469905
6163,12328,6164,18492,8.16641902923584,0.27949042546197234
6189,12380,6190,18570,8.19684886932373,0.27410297070389333
6215,12432,6216,18648,8.227320194244385,0.2689549259449677
6241,12484,6242,18726,8.258277893066406,0.2643893131931918
6267,12536,6268,18804,8.28885817527771,0.2601505303699696
6292,12586,6293,18879,8.318470001220703,0.2556296813726249
6318,12638,6319,18957,8.34899616241455,0.25120188370647156
6344,12690,6345,19035,8.379424095153809,0.24675192368317767
6370,12742,6371,19113,8.410167217254639,0.24266488816840592
6396,12794,6397,19191,8.440705060958862,0.23732272684583222
6422,12846,6423,19269,8.471289873123169,0.23353019644559936
6448,12898,6449,19347,8.501838207244873,0.22900756368039765
6474,12950,6475,19425,8.533529043197632,0.22534696479601735
6500,13002,6501,19503,8.564593076705933,0.22164246765498774
6526,13054,6527,19581,8.59515905380249,0.216779313194138
6551,13104,6552,19656,8.624577045440674,0.21277307556920277
6577,13156,6578,19734,8.65477204322815,0.2089080946749391
6603,13208,6604,19812,8.685086965560913,0.20526864150463098
6629,13260,6630,19890,8.71708607673645,0.2018618774618517
6655,13312,6656,19968,8.749024152755737,0.19852576664084154
6681,13364,6682,20046,8.781252145767212,0.1944866645727643
6707,13416,6708,20124,8.813515186309814,0.19108265468082664
6733,13468,6734,20202,8.846405029296875,0.18737646087186022
6759,13520,6760,20280,8.877554893493652,0.18362913660030245
6784,13570,6785,20355,8.908313274383545,0.18081628602567434
6810,13622,6811,20433,8.938575267791748,0.17728046171612277
6836,13674,6837,20511,8.978691101074219,0.17433096632760225
6862,13726,6863,20589,9.010382175445557,0.17085793207343158
6888,13778,6889,20667,9.040748119354248,0.1682536162836641
6914,13830,6915,20745,9.072538137435913,0.16524878835843992
6940,13882,6941,20823,9.104083061218262,0.1624781614237918
6966,13934,6967,20901,9.135408878326416,0.1596503243825964
6992,13986,6993,20979,9.170900106430054,0.15663714237769
7018,14038,7019,21057,9.201458930969238,0.15385398634043668
7043,14088,7044,21132,9.231657981872559,0.15123893502902774
7069,14140,7070,21210,9.263738870620728,0.14856723224352208
7095,14192,7096,21288,9.29410696029663,0.1459266517136939
7121,14244,7122,21366,9.325904846191406,0.14362365628551288
7147,14296,7148,21444,9.357009887695312,0.14089123533744896
7173,14348,7174,21522,9.387184858322144,0.13849925984618494
7199,14400,7200,21600,9.418501853942871,0.1364500228014549
7225,14452,7226,21678,9.449609994888306,0.1336749764037677
7251,14504,7252,21756,9.48045802116394,0.1312543777993369
7276,14554,7277,21831,9.511228084564209,0.12903376321617088
7302,14606,7303,21909,9.540970087051392,0.12691582243155608
7328,14658,7329,21987,9.571884155273438,0.12457272855192514
7354,14710,7355,22065,9.603344917297363,0.12234990420915892
7380,14762,7381,22143,9.633495092391968,0.11982795105268451
7406,14814,7407,22221,9.668429136276245,0.11836645006621893
7432,14866,7433,22299,9.700257062911987,0.11551027425093707
7458,14918,7459,22377,9.732004880905151,0.1135903207531328
7484,14970,7485,22455,9.765011072158813,0.11139088498134697
7510,15022,7511,22533,9.795522212982178,0.10923038313273992
7535,15072,7536,22608,9.825860261917114,0.10751843489549628
7561,15124,7562,22686,9.856727123260498,0.10563597551674775
7587,15176,7588,22764,9.887155055999756,0.10382577600159948
7613,15228,7614,22842,9.918303966522217,0.10190771639599916
7639,15280,7640,22920,9.949528217315674,0.10024671122994278
7665,15332,7666,22998,9.9810152053833,0.09821081722657254
7691,15384,7692,23076,10.012201070785522,0.09667445127365681
7717,15436,7718,23154,10.042577028274536,0.0949773691286282
7743,15488,7744,23232,10.073722839355469,0.09334166025507784
7768,15538,7769,23307,10.104496002197266,0.0914395299203079
7794,15590,7795,23385,10.135421991348267,0.09000832377398638
7820,15642,7821,23463,10.168284893035889,0.08821049298592243
7846,15694,7847,23541,10.198944091796875,0.08688784100627345
7872,15746,7873,23619,10.229673147201538,0.0852108892755723
7898,15798,7899,23697,10.260113954544067,0.08385603584338241
7924,15850,7925,23775,10.290777206420898,0.08236800755719287
7950,15902,7951,23853,10.321797847747803,0.08095640097985779
7976,15954,7977,23931,10.352734088897705,0.07955399309082622
8002,16006,8003,24009,10.384180068969727,0.07813762648243028
8027,16056,8028,24084,10.413737058639526,0.0768167213217339
8053,16108,8054,24162,10.444293975830078,0.07549074667952027
8079,16160,8080,24240,10.474820137023926,0.07427761329927307
8105,16212,8106,24318,10.505427122116089,0.07284356812783699
8131,16264,8132,24396,10.536548137664795,0.07170150689682941
8157,16316,8158,24474,10.572134971618652,0.07065221995492266
8183,16368,8184,24552,10.603354215621948,0.0693029813406838
8209,16420,8210,24630,10.633738040924072,0.06819869160460712
8235,16472,8236,24708,10.6651132106781,0.06688002723535647
8260,16522,8261,24783,10.69429612159729,0.0657233426794619
8286,16574,8287,24861,10.725342035293579,0.06466895018968444
8312,16626,8313,24939,10.7617769241333,0.06333753011460885
8338,16678,8339,25017,10.793783187866211,0.062332041616627976
8364,16730,8365,25095,10.823992013931274,0.06113743933747173
8390,16782,8391,25173,10.85550308227539,0.060142929059907146
8416,16834,8417,25251,10.888203144073486,0.059269714121342076
8442,16886,8443,25329,10.92152190208435,0.05791886051406436
8468,16938,8469,25407,10.960988998413086,0.0568997644712681
8494,16990,8495,25485,10.993587970733643,0.05590027288599231
8519,17040,8520,25560,11.02311396598816,0.05515550559607618
8545,17092,8546,25638,11.053644180297852,0.05393906585084096
8571,17144,8572,25716,11.083796977996826,0.05284338288629442
8597,17196,8598,25794,11.114490032196045,0.05193314175426167
8623,17248,8624,25872,11.144582033157349,0.05101799121325712
8649,17300,8650,25950,11.174890995025635,0.05020240031160483
8675,17352,8676,26028,11.205685138702393,0.04936630678423626
8701,17404,8702,26106,11.235870122909546,0.04854413220425613
8727,17456,8728,26184,11.26642107963562,0.04790934937500424
8752,17506,8753,26259,11.295475959777832,0.04688676432476768
8778,17558,8779,26337,11.326232194900513,0.04596797504132155
8804,17610,8805,26415,11.356861114501953,0.04516417242348325
8830,17662,8831,26493,11.386819124221802,0.044296912075537875
8856,17714,8857,26571,11.417515993118286,0.04362886433841595
8882,17766,8883,26649,11.447992086410522,0.042793640350055284
8908,17818,8909,26727,11.478531122207642,0.042059266734781886
8934,17870,8935,26805,11.509286880493164,0.041291289643709206
8960,17922,8961,26883,11.540311098098755,0.04053342329837051
8986,17974,8987,26961,11.571524143218994,0.03974861347410297
9011,18024,9012,27036,11.601087093353271,0.03917826547638015
9037,18076,9038,27114,11.631710052490234,0.03836834242167697
9063,18128,9064,27192,11.662652015686035,0.03766118792555062
9089,18180,9090,27270,11.692776918411255,0.03703914113600604
9115,18232,9116,27348,11.723703145980835,0.0363858990655217
9141,18284,9142,27426,11.754188060760498,0.0358210637641605
9167,18336,9168,27504,11.78414011001587,0.0352000306802438
9193,18388,9194,27582,11.815783977508545,0.0346211053188199
9219,18440,9220,27660,11.846233129501343,0.03400375144008194
9244,18490,9245,27735,11.875578880310059,0.033478040623435845
9270,18542,9271,27813,11.906332969665527,0.032895995827857405
9296,18594,9297,27891,11.936691999435425,0.03230258671419506
9322,18646,9323,27969,11.973550081253052,0.031799628180465334
9348,18698,9349,28047,12.004029035568237,0.031214365682330936
9374,18750,9375,28125,12.034533023834229,0.030741325615963433
9400,18802,9401,28203,12.064696073532104,0.03023488643179917
9426,18854,9427,28281,12.09466814994812,0.029666275324188973
9452,18906,9453,28359,12.1252760887146,0.02908188232743214
9478,18958,9479,28437,12.162349224090576,0.02854833405467616
9503,19008,9504,28512,12.1914381980896,0.02812304227700224
9529,19060,9530,28590,12.222298860549927,0.02746606777816396
9555,19112,9556,28668,12.252938985824585,0.027022938015306863
9581,19164,9582,28746,12.283424139022827,0.026583341293530793
9607,19216,9608,28824,12.313188076019287,0.02613677861177166
9633,19268,9634,28902,12.34334397315979,0.02569708863654796
9659,19320,9660,28980,12.374081134796143,0.025270543125884615
9685,19372,9686,29058,12.404804229736328,0.024759149780265943
9711,19424,9712,29136,12.435090065002441,0.024293315238196556
9736,19474,9737,29211,12.465342998504639,0.023931737920406704
9762,19526,9763,29289,12.494917869567871,0.023404925495242423
9788,19578,9789,29367,12.525799036026001,0.023025224281013834
9814,19630,9815,29445,12.556762218475342,0.022599532819299384
9840,19682,9841,29523,12.587041139602661,0.02226170270591865
9866,19734,9867,29601,12.617784023284912,0.021829928242937058
9892,19786,9893,29679,12.648612260818481,0.021476581578099285
9918,19838,9919,29757,12.679304122924805,0.021078265449887112
9944,19890,9945,29835,12.710097074508667,0.020740171298371024
9970,19942,9971,29913,12.74108600616455,0.020390993968476323
9995,19992,9996,29988,12.771228075027466,0.020013467702483467
10021,20044,10022,30066,12.802489042282104,0.019681002626839472
10047,20096,10048,30144,12.832722902297974,0.01932828532358144
10073,20148,10074,30222,12.86355209350586,0.019010603154697492
10099,20200,10100,30300,12.893818855285645,0.018657433395787848
10125,20252,10126,30378,12.92487096786499,0.018347040048865892
10151,20304,10152,30456,12.95596194267273,0.01801004488959279
10177,20356,10178,30534,12.986147165298462,0.017680436428236135
10203,20408,10204,30612,13.019095182418823,0.017375437133409832
10228,20458,10229,30687,13.050580978393555,0.01707532332034134
10254,20510,10255,30765,13.083285093307495,0.01677967606258335
10280,20562,10281,30843,13.115063190460205,0.01649467428603657
10306,20614,10307,30921,13.1478590965271,0.016255091361472296
10332,20666,10333,30999,13.18457293510437,0.01591705623161488
10358,20718,10359,31077,13.214852094650269,0.015661216963962943
10384,20770,10385,31155,13.244529008865356,0.015376889925391879
10410,20822,10411,31233,13.27544093132019,0.015142790237518966
10436,20874,10437,31311,13.305552959442139,0.01479123535295912
10462,20926,10463,31389,13.336405038833618,0.014563033815875315
10487,20976,10488,31464,13.375133991241455,0.014303746190421407
10513,21028,10514,31542,13.409913063049316,0.014092527382103981
10539,21080,10540,31620,13.446355104446411,0.013814872370403464
10565,21132,10566,31698,13.479172945022583,0.013590072667966524
10591,21184,10592,31776,13.513798952102661,0.013359083919795012
10617,21236,10618,31854,13.547969102859497,0.013139345458512253
10643,21288,10644,31932,13.585669994354248,0.012906688703083091
10669,21340,10670,32010,13.618137121200562,0.012691061606460607
10695,21392,10696,32088,13.651823282241821,0.012483065453807285
10720,21442,10721,32163,13.683304071426392,0.012264032322377716
10746,21494,10747,32241,13.71633505821228,0.012004634519371393
10772,21546,10773,32319,13.747781991958618,0.011827200856487252
10798,21598,10799,32397,13.779568910598755,0.011635777564379168
10824,21650,10825,32475,13.811958074569702,0.01142715072808187
10850,21702,10851,32553,13.842761993408203,0.011225133074503901
10876,21754,10877,32631,13.875174045562744,0.011041331547630762
10902,21806,10903,32709,13.906822919845581,0.01087053747050959
10928,21858,10929,32787,13.939275026321411,0.010692556481785687
10954,21910,10955,32865,13.97217583656311,0.010509707522487588
10979,21960,10980,32940,14.00613784790039,0.010356923756489778
11005,22012,11006,33018,14.037988901138306,0.010152342212450094
11031,22064,11032,33096,14.070021867752075,0.00996833453882573
11057,22116,11058,33174,14.10096001625061,0.009811577173877595
11083,22168,11084,33252,14.131911039352417,0.009657919374262747
11109,22220,11110,33330,14.1632399559021,0.009488174136322414
11135,22272,11136,33408,14.193786859512329,0.009313262999626204
11161,22324,11162,33486,14.225318908691406,0.009160491175180141
11187,22376,11188,33564,14.25690507888794,0.008970335886942848
11212,22426,11213,33639,14.285807847976685,0.008843064980851523
11238,22478,11239,33717,14.32391905784607,0.008682853099458043
11264,22530,11265,33795,14.358705043792725,0.00854350121483094
11290,22582,11291,33873,14.389219045639038,0.008414982245540159
11316,22634,11317,33951,14.420860052108765,0.0082333506205714
11342,22686,11343,34029,14.452591896057129,0.00810521157131916
11368,22738,11369,34107,14.483716249465942,0.007969246775132888
11394,22790,11395,34185,14.51593804359436,0.007830760895785716
11420,22842,11421,34263,14.547425031661987,0.007714161799299291
11446,22894,11447,34341,14.579077959060669,0.00756788392470753
11471,22944,11472,34416,14.609691858291626,0.007449795882848775
11497,22996,11498,34494,14.640176057815552,0.0072965499113024634
11523,23048,11524,34572,14.671756029129028,0.007177397455620849
11549,23100,11550,34650,14.703339099884033,0.007050978693087018
11575,23152,11576,34728,14.734235048294067,0.006932605383099144
11601,23204,11602,34806,14.766571998596191,0.006821257484261878
11627,23256,11628,34884,14.79712700843811,0.006686408589303028
11653,23308,11654,34962,14.828416109085083,0.00657920099013154
11679,23360,11680,35040,14.860100269317627,0.006461520536277021
11704,23410,11705,35115,14.889414072036743,0.006356209283126191
11730,23462,11731,35193,14.921099185943604,0.006235775411482791
11756,23514,11757,35271,14.953815221786499,0.006137127859119573
11782,23566,11783,35349,14.99067497253418,0.006024985869430566
11808,23618,11809,35427,15.022137880325317,0.005936524459002612
11834,23670,11835,35505,15.053898096084595,0.005846092722890717
11860,23722,11861,35583,15.08487606048584,0.00573886227971343
11886,23774,11887,35661,15.116288185119629,0.005639487441499114
11912,23826,11913,35739,15.154311895370483,0.005555319445988971
11938,23878,11939,35817,15.18673300743103,0.005454064652099078
11963,23928,11964,35892,15.21906304359436,0.005360395066190904
11989,23980,11990,35970,15.252618074417114,0.005257677990698539
12015,24032,12016,36048,15.284868955612183,0.005163561825611396
12041,24084,12042,36126,15.317935228347778,0.005087033223844628
12067,24136,12068,36204,15.349120140075684,0.004983408815178336
12093,24188,12094,36282,15.379763126373291,0.00488642962159247
12119,24240,12120,36360,15.411994218826294,0.004810679003981022
12145,24292,12146,36438,15.442528009414673,0.004721199541677379
12171,24344,12172,36516,15.473392963409424,0.0046527722281553
12196,24394,12197,36591,15.5031418800354,0.004565850845551722
12222,24446,12223,36669,15.534450054168701,0.0044964471441062415
12248,24498,12249,36747,15.566343069076538,0.00441222593542534
12274,24550,12275,36825,15.597445011138916,0.004342536301919608
12300,24602,12301,36903,15.62986707687378,0.004254985085935914
12326,24654,12327,36981,15.662904024124146,0.004190286872699289
12352,24706,12353,37059,15.694442987442017,0.004110031910045109
12378,24758,12379,37137,15.728109121322632,0.004048852140840609
12404,24810,12405,37215,15.7620849609375,0.003978238187073657
12430,24862,12431,37293,15.795981168746948,0.003911539194291436
12455,24912,12456,37368,15.827062129974365,0.003850522916764021
12481,24964,12482,37446,15.860130071640015,0.0037862932073267075
12507,25016,12508,37524,15.89181900024414,0.0037168048676221588
12533,25068,12534,37602,15.925425052642822,0.0036548769562614325
12559,25120,12560,37680,15.959191083908081,0.0035880679495221557
12585,25172,12586,37758,15.990777969360352,0.0035301488982213414
12611,25224,12612,37836,16.02352213859558,0.003470356710863598
12637,25276,12638,37914,16.056539058685303,0.003408599240174226
12663,25328,12664,37992,16.088608980178833,0.0033459062743759205
12688,25378,12689,38067,16.119502067565918,0.0032951458695151814
12714,25430,12715,38145,16.152495861053467,0.003236614031834506
12740,25482,12741,38223,16.189857006072998,0.003182480789860165
12766,25534,12767,38301,16.22245192527771,0.0031237987016083935
12792,25586,12793,38379,16.255038022994995,0.0030747391740533203
12818,25638,12819,38457,16.28677988052368,0.0029978725812043194
12844,25690,12845,38535,16.319273948669434,0.0029507449305583577
12870,25742,12871,38613,16.356736183166504,0.0028955946045243763
12896,25794,12897,38691,16.38817310333252,0.002848093405873442
12922,25846,12923,38769,16.420879125595093,0.002802428180075367
12947,25896,12948,38844,16.452434062957764,0.0027546552959165638
12973,25948,12974,38922,16.484699010849,0.002711363245339271
12999,26000,13000,39000,16.516448974609375,0.002656862336039012
13025,26052,13026,39078,16.54872703552246,0.0026131133471380963
13051,26104,13052,39156,16.58052706718445,0.002570924205542724
13077,26156,13078,39234,16.612727165222168,0.0025279558130932855
13103,26208,13104,39312,16.644158124923706,0.0024814658199829864
13129,26260,13130,39390,16.67659306526184,0.0024434735064460256
13155,26312,13156,39468,16.711310148239136,0.0023956342065503122
13181,26364,13182,39546,16.743946075439453,0.002358512733508178
13206,26414,13207,39621,16.77544903755188,0.002317422680562231
13232,26466,13233,39699,16.809290170669556,0.002278618679497413
13258,26518,13259,39777,16.840691089630127,0.0022392836966673713
13284,26570,13285,39855,16.873876094818115,0.002203797256811413
13310,26622,13311,39933,16.91006898880005,0.002162679286243474
13336,26674,13337,40011,16.94671320915222,0.0021293268722502035
13362,26726,13363,40089,16.98097586631775,0.002085144127931926
13388,26778,13389,40167,17.01611614227295,0.0020497139330473146
13414,26830,13415,40245,17.050270080566406,0.0020077260222706172
13439,26880,13440,40320,17.080480098724365,0.0019765827487390197
13465,26932,13466,40398,17.112277030944824,0.0019404413759502859
13491,26984,13492,40476,17.145787000656128,0.001910817721636704
13517,27036,13518,40554,17.180392026901245,0.0018808437780535314
13543,27088,13544,40632,17.213758945465088,0.0018481225050663852
13569,27140,13570,40710,17.245203018188477,0.0018186100908224034
13595,27192,13596,40788,17.27731704711914,0.0017839203208041
13621,27244,13622,40866,17.309764862060547,0.0017556195775796368
13647,27296,13648,40944,17.342955112457275,0.0017258100094750262
13673,27348,13674,41022,17.383996963500977,0.0016955061553289852
13698,27398,13699,41097,17.420538902282715,0.0016685563064129383
13724,27450,13725,41175,17.45999503135681,0.001641278772581245
13750,27502,13751,41253,17.494537115097046,0.0016147518276738992
13776,27554,13777,41331,17.52865695953369,0.0015822476742641811
13802,27606,13803,41409,17.566219091415405,0.0015565303061748637
13828,27658,13829,41487,17.598275184631348,0.0015297767223501069
13854,27710,13855,41565,17.63078808784485,0.0015027839568801937
13880,27762,13881,41643,17.665621042251587,0.001480048818962132
13906,27814,13907,41721,17.69742703437805,0.0014538053601427237
13931,27864,13932,41796,17.729629039764404,0.001432686805060257
13957,27916,13958,41874,17.76350998878479,0.0014072575995669467
13983,27968,13984,41952,17.797078132629395,0.0013762775458872056
14009,28020,14010,42030,17.831095218658447,0.0013568801160772637
14035,28072,14036,42108,17.86595606803894,0.001337236535619013
14061,28124,14062,42186,17.89841103553772,0.0013123803050802962
14087,28176,14088,42264,17.933094024658203,0.0012859949274570681
14113,28228,14114,42342,17.967563152313232,0.0012576245312629908
14139,28280,14140,42420,18.000375032424927,0.0012368451411930437
14165,28332,14166,42498,18.033594846725464,0.0012158557126440428
14190,28382,14191,42573,18.066556930541992,0.0011966560147129712
14216,28434,14217,42651,18.09949493408203,0.0011789361757337247
14242,28486,14243,42729,18.13431406021118,0.0011584958865569206
14268,28538,14269,42807,18.16724705696106,0.001141411858156971
14294,28590,14295,42885,18.201123237609863,0.0011202227985904756
14320,28642,14321,42963,18.23424792289734,0.0011022361328514307
14346,28694,14347,43041,18.2671480178833,0.0010838162270374596
14372,28746,14373,43119,18.30093216896057,0.001064037906530757
14398,28798,14399,43197,18.333919048309326,0.0010450978261360433
14423,28848,14424,43272,18.370234966278076,0.0010274209313365645
14449,28900,14450,43350,18.405349016189575,0.001009280687071623
14475,28952,14476,43428,18.43839693069458,0.0009924006051278411
14501,29004,14502,43506,18.472310066223145,0.0009788924076019612
14527,29056,14528,43584,18.506025075912476,0.0009580769183230586
14553,29108,14554,43662,18.538919925689697,0.0009406149125652519
14579,29160,14580,43740,18.572550058364868,0.000926533401298002
14605,29212,14606,43818,18.60586404800415,0.0009110320947911532
14631,29264,14632,43896,18.638272047042847,0.0008970984659981696
14657,29316,14658,43974,18.672482013702393,0.0008784171370734839
14682,29366,14683,44049,18.70553493499756,0.0008654957712224132
14708,29418,14709,44127,18.73911190032959,0.0008512253687058546
14734,29470,14735,44205,18.772320985794067,0.0008373083999231312
14760,29522,14761,44283,18.806869983673096,0.0008213506112042523
14786,29574,14787,44361,18.839653968811035,0.0008067576836765511
14812,29626,14813,44439,18.873560190200806,0.000792709897154964
14838,29678,14839,44517,18.905848026275635,0.0007803520857123658
14864,29730,14865,44595,18.938150882720947,0.0007652168468439413
14890,29782,14891,44673,18.971673250198364,0.0007539618085274924
14915,29832,14916,44748,19.003669023513794,0.0007404363559544436
14941,29884,14942,44826,19.036749124526978,0.0007270728746107125
14967,29936,14968,44904,19.069746017456055,0.0007140752090890601
14993,29988,14994,44982,19.102909088134766,0.0007031706185216535
15019,30040,15020,45060,19.13551902770996,0.0006900519621240164
15045,30092,15046,45138,19.168477058410645,0.0006797213910658684
15071,30144,15072,45216,19.20217514038086,0.00066697577267405
15097,30196,15098,45294,19.235471963882446,0.0006560787992384576
15123,30248,15124,45372,19.26852297782898,0.0006433095808233702
15149,30300,15150,45450,19.30143904685974,0.000633780734233369
15174,30350,15175,45525,19.334988117218018,0.0006222038973646704
15200,30402,15201,45603,19.373268127441406,0.0006128595854306695
15226,30454,15227,45681,19.410969257354736,0.000600846615611772
15252,30506,15253,45759,19.44485306739807,0.0005919546129007358
15278,30558,15279,45837,19.47978711128235,0.0005815335188117388
15304,30610,15305,45915,19.51742911338806,0.0005720944028553276
15330,30662,15331,45993,19.554498195648193,0.0005601757876547708
15356,30714,15357,46071,19.589177131652832,0.0005520507027085841
15382,30766,15383,46149,19.626582145690918,0.00054274747776617
15407,30816,15408,46224,19.658899068832397,0.0005336890841363129
15433,30868,15434,46302,19.69252109527588,0.0005241264302640047
15459,30920,15460,46380,19.726678133010864,0.0005157512883897653
15485,30972,15486,46458,19.76072096824646,0.0005075492072137422
15511,31024,15512,46536,19.7934250831604,0.0004981384769280339
15537,31076,15538,46614,19.826837062835693,0.0004890732818694232
15563,31128,15564,46692,19.860857248306274,0.00048097141382186237
15589,31180,15590,46770,19.894383192062378,0.0004727696658619607
15615,31232,15616,46848,19.929664134979248,0.00046507855540767196
15641,31284,15642,46926,19.963623046875,0.00045768465827222826
15666,31334,15667,47001,19.99545192718506,0.0004498248670188332
15692,31386,15693,47079,20.029343128204346,0.0004406004142083475
15718,31438,15719,47157,20.06278395652771,0.0004336775575666252
15744,31490,15745,47235,20.095980167388916,0.0004246105698939573
15770,31542,15771,47313,20.128690004348755,0.00041815239183051744
15796,31594,15797,47391,20.162756204605103,0.000409532020057668
15822,31646,15823,47469,20.196599006652832,0.0004010824964097992
15848,31698,15849,47547,20.230576038360596,0.0003939326740010074
15874,31750,15875,47625,20.263972282409668,0.0003877538731558161
15899,31800,15900,47700,20.296192169189453,0.00037978768443736044
15925,31852,15926,47778,20.330169200897217,0.000373302116031482
15951,31904,15952,47856,20.3631591796875,0.0003670270197062564
15977,31956,15978,47934,20.394917964935303,0.0003595786688492808
16003,32008,16004,48012,20.4274001121521,0.0003531611300786608
16029,32060,16030,48090,20.46025514602661,0.00034789733990692184
16055,32112,16056,48168,20.49196195602417,0.0003426742314331932
16081,32164,16082,48246,20.529855012893677,0.00033623242302383005
16107,32216,16108,48324,20.565150022506714,0.0003300533549008833
16133,32268,16134,48402,20.597334146499634,0.0003246704164894254
16158,32318,16159,48477,20.62870502471924,0.0003193652048594231
16184,32370,16185,48555,20.662626028060913,0.00031417050752224895
16210,32422,16211,48633,20.694857120513916,0.00030657097886432894
16236,32474,16237,48711,20.72712802886963,0.00030203626283764606
16262,32526,16263,48789,20.760184049606323,0.00029660940367648436
16288,32578,16289,48867,20.792006015777588,0.00029182425237195275
16314,32630,16315,48945,20.82429003715515,0.0002860978212311238
16340,32682,16341,49023,20.856747150421143,0.00028128496830959193
16366,32734,16367,49101,20.888381958007812,0.00027635744970666565
16391,32784,16392,49176,20.920006036758423,0.0002723520291283421
16417,32836,16418,49254,20.95384407043457,0.00026721196445578244
16443,32888,16444,49332,20.98541021347046,0.000262622246623323
16469,32940,16470,49410,21.01759099960327,0.00025775804124350543
16495,32992,16496,49488,21.049934148788452,0.00025361646521560033
16521,33044,16522,49566,21.081594944000244,0.00024917842074501095
16547,33096,16548,49644,21.11382508277893,0.00024506939109869563
16573,33148,16574,49722,21.145965099334717,0.00024062748082087637
16599,33200,16600,49800,21.177900075912476,0.00023653398545775417
16625,33252,16626,49878,21.210937976837158,0.00023226828648148512
16650,33302,16651,49953,21.241266012191772,0.00022855755548789602
16676,33354,16677,50031,21.27336812019348,0.0002248712985419843
16702,33406,16703,50109,21.305028200149536,0.00022111702924121346
16728,33458,16729,50187,21.337467908859253,0.00021796760950110183
16754,33510,16755,50265,21.368711948394775,0.00021296670968240505
16780,33562,16781,50343,21.400701999664307,0.00020875049949609092
16806,33614,16807,50421,21.432175159454346,0.00020542755726182804
16832,33666,16833,50499,21.46498417854309,0.00020198928984882514
16858,33718,16859,50577,21.497062921524048,0.0001991035236414973
16883,33768,16884,50652,21.528600215911865,0.00019613767244663904
16909,33820,16910,50730,21.561717987060547,0.00019253902360105712
16935,33872,16936,50808,21.593322038650513,0.0001889501857021969
16961,33924,16962,50886,21.628345251083374,0.00018625712277753337
16987,33976,16988,50964,21.663854122161865,0.00018310947882582695
17013,34028,17014,51042,21.698981046676636,0.00017975032835693128
17039,34080,17040,51120,21.733476161956787,0.00017614666148801916
17065,34132,17066,51198,21.770212173461914,0.00017356420437408815
17091,34184,17092,51276,21.80280089378357,0.00017055847820302006
17117,34236,17118,51354,21.83460307121277,0.0001676049846537353
17142,34286,17143,51429,21.866401195526123,0.00016514305718828837
17168,34338,17169,51507,21.898977041244507,0.00016229607365403353
17194,34390,17195,51585,21.931533098220825,0.00015957859784521133
17220,34442,17221,51663,21.96495008468628,0.0001569298648291806
17246,34494,17247,51741,21.997112035751343,0.00015410941239224485
17272,34546,17273,51819,22.029680967330933,0.0001512229010813826
17298,34598,17299,51897,22.06237006187439,0.0001488838669274628
17324,34650,17325,51975,22.09410786628723,0.00014636542243806616
17350,34702,17351,52053,22.12656307220459,0.00014364376545472624
17375,34752,17376,52128,22.156574964523315,0.00014064075628539285
17401,34804,17402,52206,22.188540935516357,0.00013861914851531765
17427,34856,17428,52284,22.22163200378418,0.00013576760875366745
17453,34908,17454,52362,22.253568172454834,0.00013368190866458463
17479,34960,17480,52440,22.288538217544556,0.0001314727325052445
17505,35012,17506,52518,22.321282148361206,0.00012880786641744635
17531,35064,17532,52596,22.353265047073364,0.00012624313887954486
17557,35116,17558,52674,22.38567090034485,0.00012417779794304806
17583,35168,17584,52752,22.418192863464355,0.00012181891145246482
17609,35220,17610,52830,22.450764179229736,0.00011986526521923224
17634,35270,17635,52905,22.481189012527466,0.00011771791332648718
17660,35322,17661,52983,22.51244020462036,0.00011578313569771126
17686,35374,17687,53061,22.544515132904053,0.0001137265238639884
17712,35426,17713,53139,22.577373027801514,0.00011200072185602039
17738,35478,17739,53217,22.60900092124939,0.00010997036986282183
17764,35530,17765,53295,22.64039707183838,0.0001080382829741211
17790,35582,17791,53373,22.673527002334595,0.00010620553302942426
17816,35634,17817,53451,22.70666193962097,0.00010443406745253014
17842,35686,17843,53529,22.737812042236328,0.0001026604508069795
17867,35736,17868,53604,22.769157886505127,0.00010095425341205555
17893,35788,17894,53682,22.80122709274292,9.937124002590281e-05
17919,35840,17920,53760,22.83355402946472,9.798083533496538e-05
17945,35892,17946,53838,22.86468195915222,9.566887274559122e-05
17971,35944,17972,53916,22.896272897720337,9.408141170297313e-05
17997,35996,17998,53994,22.928390979766846,9.245000194368913e-05
18023,36048,18024,54072,22.9624240398407,9.084858356800396e-05
18049,36100,18050,54150,22.99393582344055,8.940538407387066e-05
18075,36152,18076,54228,23.02626895904541,8.776112304076378e-05
18101,36204,18102,54306,23.059298038482666,8.627798865745717e-05
18126,36254,18127,54381,23.08929204940796,8.48965439672611e-05
18152,36306,18153,54459,23.12153196334839,8.339927489942056e-05
18178,36358,18179,54537,23.153871059417725,8.202980768601265e-05
18204,36410,18205,54615,23.18528699874878,8.042582089728967e-05
18230,36462,18231,54693,23.217693090438843,7.915411242720438e-05
18256,36514,18257,54771,23.249068021774292,7.798577803441731e-05
18282,36566,18283,54849,23.281136989593506,7.670317904739932e-05
18308,36618,18309,54927,23.31364417076111,7.494939063690254e-05
18334,36670,18335,55005,23.345088005065918,7.361170901276637e-05
18359,36720,18360,55080,23.37605094909668,7.24123977988711e-05
18385,36772,18386,55158,23.408290147781372,7.109099738045188e-05
18411,36824,18412,55236,23.439574003219604,6.97894703307611e-05
18437,36876,18438,55314,23.472261905670166,6.861415931780357e-05
18463,36928,18464,55392,23.504162073135376,6.751249793524039e-05
18489,36980,18490,55470,23.536739110946655,6.630114842209878e-05
18515,37032,18516,55548,23.5688898563385,6.533378291351255e-05
18541,37084,18542,55626,23.60118818283081,6.420158740638726e-05
18567,37136,18568,55704,23.63349986076355,6.293739750162786e-05
18593,37188,18594,55782,23.665749073028564,6.184569144807028e-05
18618,37238,18619,55857,23.696133852005005,6.0689494489452045e-05
18644,37290,18645,55935,23.72866415977478,5.961065380688524e-05
18670,37342,18671,56013,23.75974202156067,5.857711562384793e-05
18696,37394,18697,56091,23.79300308227539,5.7545357208255155e-05
18722,37446,18723,56169,23.828017950057983,5.6461845247213205e-05
18748,37498,18749,56247,23.862712144851685,5.556156861530326e-05
18774,37550,18775,56325,23.897247076034546,5.4731140608055284e-05
18800,37602,18801,56403,23.93175196647644,5.382215908866783e-05
18826,37654,18827,56481,23.96419095993042,5.2915868195668736e-05
18851,37704,18852,56556,23.995087146759033,5.1912887215621595e-05
18877,37756,18878,56634,24.027705907821655,5.111762300202827e-05
18903,37808,18904,56712,24.060132265090942,5.0376209969726915e-05
18929,37860,18930,56790,24.091233015060425,4.9419330252931104e-05
18955,37912,18956,56868,24.122716903686523,4.8371384536949336e-05
18981,37964,18982,56946,24.155609130859375,4.765074254464707e-05
19007,38016,19008,57024,24.18674898147583,4.674921547120903e-05
19033,38068,19034,57102,24.219347953796387,4.600112367825204e-05
19059,38120,19060,57180,24.251133918762207,4.5085550823387166e-05
19085,38172,19086,57258,24.282383918762207,4.42265148876686e-05
19110,38222,19111,57333,24.312673091888428,4.348735558323824e-05
19136,38274,19137,57411,24.343836069107056,4.277742311842303e-05
19162,38326,19163,57489,24.374540090560913,4.200563512313238e-05
19188,38378,19189,57567,24.40586495399475,4.13318133496432e-05
19214,38430,19215,57645,24.43804121017456,4.054839291711687e-05
19240,38482,19241,57723,24.469967126846313,3.971561989146721e-05
19266,38534,19267,57801,24.50182008743286,3.9115031768233166e-05
19292,38586,19293,57879,24.53355121612549,3.8473109384540294e-05
19318,38638,19319,57957,24.56610417366028,3.792988536588382e-05
19343,38688,19344,58032,24.59641408920288,3.7094285971761565e-05
19369,38740,19370,58110,24.628525018692017,3.6474966236710316e-05
19395,38792,19396,58188,24.661184072494507,3.5841492945110076e-05
19421,38844,19422,58266,24.692875146865845,3.5164323094249994e-05
19447,38896,19448,58344,24.725085973739624,3.4589957408570626e-05
19473,38948,19474,58422,24.757659912109375,3.403075129426725e-05
19499,39000,19500,58500,24.788881063461304,3.340468265378149e-05
19525,39052,19526,58578,24.820831060409546,3.278047245203197e-05
19551,39104,19552,58656,24.852609157562256,3.2265038271361846e-05
19577,39156,19578,58734,24.8844051361084,3.167471663800825e-05
19602,39206,19603,58809,24.91564917564392,3.1186903356683615e-05
19628,39258,19629,58887,24.947247982025146,3.061799986880942e-05
19654,39310,19655,58965,24.98053503036499,3.0093367058725562e-05
19680,39362,19681,59043,25.012463092803955,2.9552527394116623e-05
19706,39414,19707,59121,25.044109106063843,2.9058033533146954e-05
19732,39466,19733,59199,25.076029062271118,2.8526927394523227e-05
19758,39518,19759,59277,25.107373237609863,2.8070367989130318e-05
19784,39570,19785,59355,25.138806104660034,2.7519663717612275e-05
19810,39622,19811,59433,25.17009997367859,2.7089129616797436e-05
19835,39672,19836,59508,25.20008087158203,2.662818008047907e-05
19861,39724,19862,59586,25.23134708404541,2.6185044134763302e-05
19887,39776,19888,59664,25.262574195861816,2.563856673987175e-05
19913,39828,19914,59742,25.29349398612976,2.5232223038074153e-05
19939,39880,19940,59820,25.325413942337036,2.4751777004894393e-05
19965,39932,19966,59898,25.357008934020996,2.4348534452656168e-05
19991,39984,19992,59976,25.388087034225464,2.393093882346875e-05
20017,40036,20018,60054,25.419734001159668,2.350764498260105e-05
20043,40088,20044,60132,25.452057123184204,2.309686101398256e-05
20069,40140,20070,60210,25.484391927719116,2.2626115082857723e-05
20094,40190,20095,60285,25.514739990234375,2.225254331733595e-05
20120,40242,20121,60363,25.546425104141235,2.1857551701032207e-05
20146,40294,20147,60441,25.579647064208984,2.149140448182152e-05
20172,40346,20173,60519,25.613224029541016,2.1168064563426015e-05
20198,40398,20199,60597,25.645785093307495,2.0781482817255892e-05
20224,40450,20225,60675,25.67806601524353,2.0419873862920213e-05
20250,40502,20251,60753,25.710953950881958,2.0022770399918954e-05
20276,40554,20277,60831,25.742909908294678,1.9725864831343642e-05
20302,40606,20303,60909,25.776950120925903,1.9366018591426837e-05
20327,40656,20328,60984,25.809123039245605,1.905482952224702e-05
20353,40708,20354,61062,25.839969158172607,1.8716415297603817e-05
20379,40760,20380,61140,25.87345600128174,1.8382160192231822e-05
20405,40812,20406,61218,25.90627408027649,1.8097475503964233e-05
20431,40864,20432,61296,25.940934896469116,1.7804077742766822e-05
20457,40916,20458,61374,25.976934909820557,1.7546697108627995e-05
20483,40968,20484,61452,26.0127911567688,1.7214119793607097e-05
20509,41020,20510,61530,26.04624104499817,1.6949267205745855e-05
20535,41072,20536,61608,26.079782009124756,1.663240664129262e-05
20561,41124,20562,61686,26.11162805557251,1.6312739262502873e-05
20586,41174,20587,61761,26.141690969467163,1.6042366723922896e-05
20612,41226,20613,61839,26.17421293258667,1.5782168020450626e-05
20638,41278,20639,61917,26.206942081451416,1.5498265270252887e-05
20664,41330,20665,61995,26.23791003227234,1.5238915580084722e-05
20690,41382,20691,62073,26.270101070404053,1.4956110248931509e-05
20716,41434,20717,62151,26.301403045654297,1.4686063764202117e-05
20742,41486,20743,62229,26.332777976989746,1.4409842833629227e-05
20768,41538,20769,62307,26.36825919151306,1.4172841247273027e-05
20794,41590,20795,62385,26.40144419670105,1.3929108831689518e-05
20819,41640,20820,62460,26.430752992630005,1.3698751445190283e-05
20845,41692,20846,62538,26.46259093284607,1.3436642689157452e-05
20871,41744,20872,62616,26.49243712425232,1.3211187820161285e-05
20897,41796,20898,62694,26.524386167526245,1.2951835060448502e-05
20923,41848,20924,62772,26.556143283843994,1.2737311976707133e-05
20949,41900,20950,62850,26.58753204345703,1.2505927998063271e-05
20975,41952,20976,62928,26.61952018737793,1.2326378396210202e-05
21001,42004,21002,63006,26.65385913848877,1.2037769806738652e-05
21027,42056,21028,63084,26.68629002571106,1.179014952867874e-05
21053,42108,21054,63162,26.718799114227295,1.159461464794731e-05
21078,42158,21079,63237,26.75181293487549,1.1380250725778751e-05
21104,42210,21105,63315,26.78491497039795,1.1153421496601368e-05
21130,42262,21131,63393,26.81762409210205,1.0961390444208519e-05
21156,42314,21157,63471,26.850370168685913,1.074154670277494e-05
21182,42366,21183,63549,26.88209104537964,1.0563505497884762e-05
21208,42418,21209,63627,26.913472175598145,1.0393869956715207e-05
21234,42470,21235,63705,26.94416904449463,1.0213098448730307e-05
21260,42522,21261,63783,26.97500491142273,1.0016055966843851e-05
21286,42574,21287,63861,27.00599503517151,9.854829954747402e-06
21311,42624,21312,63936,27.03641700744629,9.670447298049112e-06
21337,42676,21338,64014,27.06831121444702,9.466421261095093e-06
21363,42728,21364,64092,27.098660945892334,9.29859788811882e-06
21389,42780,21390,64170,27.129671096801758,9.129918453254504e-06
21415,42832,21416,64248,27.160601139068604,8.946463253778347e-06
21441,42884,21442,64326,27.191213130950928,8.76481783507188e-06
21467,42936,21468,64404,27.222373962402344,8.568847306378302e-06
21493,42988,21494,64482,27.257911205291748,8.424915677096578e-06
21519,43040,21520,64560,27.288227081298828,8.269112186098937e-06
21545,43092,21546,64638,27.323076963424683,8.136678957271215e-06
21570,43142,21571,64713,27.35242199897766,7.967171882228286e-06
21596,43194,21597,64791,27.383033275604248,7.831996299501043e-06
21622,43246,21623,64869,27.41522216796875,7.688757932555745e-06
21648,43298,21649,64947,27.445794105529785,7.557011372227862e-06
21674,43350,21675,65025,27.477864980697632,7.4350333534312085e-06
21700,43402,21701,65103,27.51306390762329,7.295066211554513e-06
21726,43454,21727,65181,27.544484853744507,7.141498940654856e-06
21752,43506,21753,65259,27.57526206970215,7.001655148997088e-06
21778,43558,21779,65337,27.606364011764526,6.883322839712491e-06
21804,43610,21805,65415,27.637315034866333,6.751334126420261e-06
21829,43660,21830,65490,27.66739320755005,6.644710310865776e-06
21855,43712,21856,65568,27.697923183441162,6.515463724099391e-06
21881,43764,21882,65646,27.728703022003174,6.383901336448616e-06
21907,43816,21908,65724,27.76020908355713,6.265399406402139e-06
21933,43868,21934,65802,27.79248809814453,6.143393306956568e-06
21959,43920,21960,65880,27.826112031936646,6.031316047483415e-06
21985,43972,21986,65958,27.859282970428467,5.924355605202436e-06
22011,44024,22012,66036,27.892917156219482,5.821351123813656e-06
22037,44076,22038,66114,27.926521062850952,5.713848963750934e-06
22062,44126,22063,66189,27.958402156829834,5.611108917946694e-06
22088,44178,22089,66267,27.989854097366333,5.494281140272506e-06
22114,44230,22115,66345,28.021735906600952,5.407694743553293e-06
22140,44282,22141,66423,28.05405020713806,5.301464966578351e-06
22166,44334,22167,66501,28.088818073272705,5.206987225392368e-06
22192,44386,22193,66579,28.131327152252197,5.115011845191475e-06
22218,44438,22219,66657,28.16543483734131,5.0145768000220414e-06
22244,44490,22245,66735,28.198216915130615,4.915693239126995e-06
22270,44542,22271,66813,28.232664108276367,4.828286819247296e-06
22296,44594,22297,66891,28.26366114616394,4.7446378630411346e-06
22321,44644,22322,66966,28.29282522201538,4.671740612138819e-06
22347,44696,22348,67044,28.324196100234985,4.571311137624434e-06
22373,44748,22374,67122,28.355286121368408,4.4723226437781705e-06
22399,44800,22400,67200,28.385683059692383,4.391114998725243e-06
22425,44852,22426,67278,28.416927099227905,4.302809088585491e-06
22451,44904,22452,67356,28.44733214378357,4.22887774220726e-06
22477,44956,22478,67434,28.479076862335205,4.140867304158746e-06
22503,45008,22504,67512,28.514111042022705,4.068127623213513e-06
22529,45060,22530,67590,28.550308227539062,4.005916821370192e-06
22554,45110,22555,67665,28.596687078475952,3.916299306183646e-06
22580,45162,22581,67743,28.635507106781006,3.839096166302625e-06
22606,45214,22607,67821,28.673890113830566,3.7722295473940903e-06
22632,45266,22633,67899,28.71074628829956,3.703553488776379e-06
22658,45318,22659,67977,28.758610010147095,3.6280893027651473e-06
22684,45370,22685,68055,28.818695068359375,3.5515275840225513e-06
22710,45422,22711,68133,28.878320932388306,3.488090214887052e-06
22736,45474,22737,68211,28.91875195503235,3.4222997555843904e-06
22762,45526,22763,68289,28.971123933792114,3.3582855394342914e-06
22788,45578,22789,68367,29.006953954696655,3.2919856494117994e-06
22813,45628,22814,68442,29.039157152175903,3.2225281074715895e-06
22839,45680,22840,68520,29.07364797592163,3.156274146931537e-06
22865,45732,22866,68598,29.111225843429565,3.1005556593299843e-06
22891,45784,22892,68676,29.144922971725464,3.0335565952555044e-06
22917,45836,22918,68754,29.182029008865356,2.977498297696002e-06
22943,45888,22944,68832,29.21767497062683,2.9200780318205943e-06
22969,45940,22970,68910,29.252753973007202,2.858090851987072e-06
22995,45992,22996,68988,29.288986921310425,2.794861416077765e-06
23021,46044,23022,69066,29.326136112213135,2.7346633260094677e-06
23046,46094,23047,69141,29.36091899871826,2.6780809321280685e-06
23072,46146,23073,69219,29.39700412750244,2.629160235301242e-06
23098,46198,23099,69297,29.43955111503601,2.5768873683773563e-06
23124,46250,23125,69375,29.479537963867188,2.5270014702982735e-06
23150,46302,23151,69453,29.518079042434692,2.4734132466619485e-06
23176,46354,23177,69531,29.555366039276123,2.4154541051757406e-06
23202,46406,23203,69609,29.587049961090088,2.3677886247241986e-06
23228,46458,23229,69687,29.619357109069824,2.3305319700739346e-06
23254,46510,23255,69765,29.65213108062744,2.2697624899592483e-06
23280,46562,23281,69843,29.683940887451172,2.221603494945157e-06
23305,46612,23306,69918,29.71599006652832,2.1781587520308676e-06
23331,46664,23332,69996,29.74809193611145,2.1305742166077835e-06
23357,46716,23358,70074,29.782469034194946,2.0864955558863585e-06
23383,46768,23384,70152,29.81895613670349,2.0401610072440235e-06
23409,46820,23410,70230,29.851744174957275,1.9995359252789058e-06
23435,46872,23436,70308,29.88494896888733,1.957455765477789e-06
23461,46924,23462,70386,29.918181896209717,1.920405793498503e-06
23487,46976,23488,70464,29.950226068496704,1.879597448350978e-06
23513,47028,23514,70542,29.987940073013306,1.840377763073775e-06
23538,47078,23539,70617,30.021027088165283,1.8020361949311337e-06
23564,47130,23565,70695,30.065834045410156,1.7558055560584762e-06
23590,47182,23591,70773,30.104421854019165,1.7130890910266316e-06
23616,47234,23617,70851,30.15819025039673,1.6743888409109786e-06
23642,47286,23643,70929,30.209542989730835,1.639341007830808e-06
23668,47338,23669,71007,30.260426998138428,1.5967901845215238e-06
23694,47390,23695,71085,30.295520067214966,1.5659148857594118e-06
23720,47442,23721,71163,30.331125020980835,1.5309266245822073e-06
23746,47494,23747,71241,30.36556601524353,1.4914692201273283e-06
23772,47546,23773,71319,30.3988139629364,1.4584801419914584e-06
23797,47596,23798,71394,30.42951512336731,1.4292339756138972e-06
23823,47648,23824,71472,30.4632670879364,1.393855995956983e-06
23849,47700,23850,71550,30.49472427368164,1.3621984180645086e-06
23875,47752,23876,71628,30.526526927947998,1.3333291235539946e-06
23901,47804,23902,71706,30.55902600288391,1.30162914047105e-06
23927,47856,23928,71784,30.590593099594116,1.273122506972868e-06
23953,47908,23954,71862,30.622488021850586,1.2417161769917584e-06
23979,47960,23980,71940,30.654165029525757,1.212790266436059e-06
24005,48012,24006,72018,30.685538053512573,1.183671429316746e-06
24030,48062,24031,72093,30.716930150985718,1.157612246061035e-06
24056,48114,24057,72171,30.749495029449463,1.13179476102232e-06
24082,48166,24083,72249,30.78168511390686,1.1052758281948627e-06
24108,48218,24109,72327,30.81438708305359,1.0723682635216392e-06
24134,48270,24135,72405,30.845826148986816,1.0476088618815993e-06
24160,48322,24161,72483,30.877935886383057,1.0210823120360146e-06
24186,48374,24187,72561,30.909879207611084,9.944538987838314e-07
24212,48426,24213,72639,30.94123601913452,9.684745236882009e-07
24238,48478,24239,72717,30.97362518310547,9.465003358855029e-07
24264,48530,24265,72795,31.005450010299683,9.169284567178693e-07
24289,48580,24290,72870,31.036245107650757,8.933877779782051e-07
24315,48632,24316,72948,31.068325996398926,8.718997150936048e-07
24341,48684,24342,73026,31.100815057754517,8.500346666551195e-07
24367,48736,24368,73104,31.132527828216553,8.261747552751331e-07
24393,48788,24394,73182,31.170735120773315,8.044958121899981e-07
24419,48840,24420,73260,31.202575206756592,7.812500371073838e-07
24445,48892,24446,73338,31.234498023986816,7.618443760293303e-07
24471,48944,24472,73416,31.266802072525024,7.407340945064789e-07
24497,48996,24498,73494,31.29812788963318,7.182901526903152e-07
24522,49046,24523,73569,31.328931093215942,6.978056035222835e-07
24548,49098,24549,73647,31.36557102203369,6.803019232393126e-07
24574,49150,24575,73725,31.397248029708862,6.60963678456028e-07
24600,49202,24601,73803,31.429153203964233,6.428820142900804e-07
24626,49254,24627,73881,31.4614360332489,6.245109034352936e-07
24652,49306,24653,73959,31.49251627922058,6.063894488761434e-07
24678,49358,24679,74037,31.525731086730957,5.861014642505324e-07
24704,49410,24705,74115,31.557834148406982,5.678460865965462e-07
24730,49462,24731,74193,31.588830947875977,5.501856321643572e-07
24756,49514,24757,74271,31.62035608291626,5.317201612342615e-07
24781,49564,24782,74346,31.65095806121826,5.158362910151482e-07
24807,49616,24808,74424,31.68239688873291,4.989358330931282e-07
24833,49668,24834,74502,31.71449303627014,4.838346967517282e-07
24859,49720,24860,74580,31.74561905860901,4.692857373811421e-07
24885,49772,24886,74658,31.778218030929565,4.528282033788855e-07
24911,49824,24912,74736,31.810578107833862,4.2581200432323385e-07
24937,49876,24938,74814,31.842052221298218,4.123734242966748e-07
24963,49928,24964,74892,31.87377119064331,3.973790398958954e-07
24989,49980,24990,74970,31.905500888824463,3.8015650716261007e-07
25014,50030,25015,75045,31.93712592124939,3.6362507671583444e-07
25040,50082,25041,75123,31.969285011291504,3.503733978504897e-07
25066,50134,25067,75201,32.000710010528564,3.370250851730816e-07
25092,50186,25093,75279,32.03239822387695,3.189474000464543e-07
25118,50238,25119,75357,32.064424991607666,3.074263759117457e-07
25144,50290,25145,75435,32.09587788581848,2.9265936518640956e-07
25170,50342,25171,75513,32.1274151802063,2.806186785164755e-07
25196,50394,25197,75591,32.1604528427124,2.6791701657202793e-07
25222,50446,25223,75669,32.19258093833923,2.5538702175254e-07
25248,50498,25249,75747,32.22501516342163,2.415548578937887e-07
25273,50548,25274,75822,32.255680084228516,2.2963467927183956e-07
25299,50600,25300,75900,32.28741788864136,2.186054643971147e-07
25325,50652,25326,75978,32.31970691680908,2.0620791474357247e-07
25351,50704,25352,76056,32.351582050323486,1.965318006114103e-07
25377,50756,25378,76134,32.388777017593384,1.834591785154771e-07
25403,50808,25404,76212,32.423717975616455,1.7281399777857587e-07
25429,50860,25430,76290,32.45933389663696,1.6034198324632598e-07
25455,50912,25456,76368,32.4913969039917,1.510413767391583e-07
25481,50964,25482,76446,32.526543855667114,1.396880406900891e-07
25506,51014,25507,76521,32.563157081604004,1.2865132248407463e-07
25532,51066,25533,76599,32.59444999694824,1.191674527944997e-07
25558,51118,25559,76677,32.62686491012573,1.1406268640712369e-07
25584,51170,25585,76755,32.659334897994995,9.815710200200556e-08
25610,51222,25611,76833,32.69051003456116,8.64830553837237e-08
25636,51274,25637,76911,32.72359108924866,7.685571290494408e-08
25662,51326,25663,76989,32.755436182022095,6.954621767363278e-08
25688,51378,25689,77067,32.7870659828186,5.97801772528328e-08
25714,51430,25715,77145,32.819663286209106,5.122092261444777e-08
25740,51482,25741,77223,32.85837912559509,4.1632574721006677e-08
25765,51532,25766,77298,32.88984990119934,3.353909505676711e-08
25791,51584,25792,77376,32.924575090408325,2.540116383897839e-08
25817,51636,25818,77454,32.9577260017395,1.8109062693838496e-08
25843,51688,25844,77532,32.988577127456665,8.459892342216335e-09
25869,51740,25870,77610,33.02084803581238,8.503775461576879e-11


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0005269050598144531,2181.2938132599165
1001,2003,2002,4005,0.846794843673706,44.348860614599744
2002,4005,4004,8009,1.651149034500122,42.70063180611464
3003,6007,6006,12013,2.4800140857696533,41.168996973026196
4004,8009,8008,16017,3.480733871459961,39.74206310087607
5005,10011,10010,20021,4.483521938323975,38.41004779718355
6006,12013,12012,24025,5.221987009048462,37.164448983126476
7007,14015,14014,28029,5.988049745559692,35.99760366567284
8008,16017,16016,32033,6.831360816955566,34.902471575462414
9009,18019,18018,36037,7.552431106567383,33.872542806958336
10010,20021,20020,40041,8.32486081123352,32.90180687460929
11011,22023,22022,44045,9.032744884490967,31.984745863677517
12012,24025,24024,48049,9.78105092048645,31.11633127426262
13013,26027,26026,52053,10.633514881134033,30.29201507749076
14014,28029,28028,56057,11.476765871047974,29.507712053032492
15015,30031,30030,60061,12.202636957168579,28.75977398425357
16016,32033,32032,64065,12.939412832260132,28.04495782384788
17017,34035,34034,68069,13.64516806602478,27.360390316515804
18018,36037,36036,72073,14.372004985809326,26.70353133521121
19019,38039,38038,76077,15.072341918945312,26.07213770811404
20020,40041,40040,80081,15.74144983291626,25.464228788021728
21021,42043,42042,84085,16.445328950881958,24.878054546039948
22022,44045,44044,88089,17.13111686706543,24.312066596662817
23023,46047,46046,92093,17.816312074661255,23.764892286299073
24024,48049,48048,96097,18.494430780410767,23.235311790254627
25025,50051,50050,100101,19.183851957321167,22.722238046277653
26026,52053,52052,104105,19.88132905960083,22.224699288077773
27027,54055,54054,108109,20.619349002838135,21.741823914088855
28028,56057,56056,112113,21.315129041671753,21.272827422812497
29029,58059,58058,116117,22.028686046600342,20.81700115708236
30030,60061,60060,120121,22.742612838745117,20.373702619029018
31031,62063,62062,124125,23.42637300491333,19.942347140904758
32032,64065,64064,128129,24.11462378501892,19.522400721436952
33033,66067,66066,132133,24.86072587966919,19.113373861213176
34034,68069,68068,136137,25.565565824508667,18.71481625280444
35035,70071,70070,140141,26.25200891494751,18.326333749942933
36036,72073,72072,144145,26.933076858520508,17.947587045890714
37037,74075,74074,148149,27.60494899749756,17.57814805843327
38038,76077,76076,152153,28.280616760253906,17.217683326783117
39039,78079,78078,156157,28.97985601425171,16.8658811226353
40040,80081,80080,160161,29.64040994644165,16.52244917089979
41041,82083,82082,164165,30.31555986404419,16.187112688565094
42042,84085,84084,168169,30.978113889694214,15.859612674460664
43043,86087,86086,172173,31.681318044662476,15.539704411808543
44044,88089,88088,176177,32.34742283821106,15.227156153677015
45045,90091,90090,180181,33.03373885154724,14.921747966216799
46046,92093,92092,184185,33.72959876060486,14.623270708275413
47047,94095,94094,188189,34.408020973205566,14.331525129123861
48048,96097,96096,192193,35.095386028289795,14.04632106865813
49049,98099,98098,196197,35.79289484024048,13.767476746700595
50050,100101,100100,200201,36.49651098251343,13.494818129884152
51051,102103,102102,204205,37.199769020080566,13.228178366263819
52052,104105,104104,208209,37.946556091308594,12.967397279129386
53053,106107,106106,212213,38.751953125,12.71232091268189
54054,108109,108108,216217,39.52462887763977,12.462801123215854
55055,110111,110110,220221,40.29127097129822,12.218695210313967
56056,112113,112112,224225,41.063923835754395,11.979865583273522
57057,114115,114114,228229,42.30094790458679,11.746179458620531
58058,116117,116116,232233,43.449862003326416,11.517508585095584
59059,118119,118118,236237,44.58692383766174,11.293728992957654
60060,120121,120120,240241,45.70150279998779,11.074720764855897
61061,122123,122122,244245,47.03110599517822,10.860367825858475
62062,124125,124124,248249,48.17832803726196,10.650557750528947
63063,126127,126126,252253,49.3016459941864,10.445181585200203
64064,128129,128128,256257,50.3967490196228,10.244133683819769
65065,130131,130130,260261,51.480828046798706,10.04731155594402
66066,132133,132132,264265,52.56254506111145,9.85461572562349
67067,134135,134134,268269,53.67476296424866,9.665949600080012
68068,136137,136136,272273,54.71813893318176,9.481219347208025
69069,138139,138138,276277,55.75368690490723,9.30033378104747
70070,140141,140140,280281,56.86208772659302,9.12320425448354
71071,142143,142142,284285,57.93423295021057,8.949744558516727
72072,144145,144144,288289,59.04012489318848,8.779870827529066
73073,146147,146146,292293,60.17039608955383,8.613501450040417
74074,148149,148148,296297,61.29886984825134,8.450556984516084
75075,150151,150150,300301,62.37877082824707,8.290960079832871
76076,152153,152152,304305,63.465874910354614,8.134635400064326
77077,154155,154154,308309,64.54682111740112,7.981509553280148
78078,156157,156156,312313,65.6387288570404,7.831511024092947
79079,158159,158158,316317,66.72039794921875,7.684570109708716
80080,160161,160160,320321,67.7974328994751,7.540618859264441
81081,162163,162162,324325,68.85248494148254,7.399591016251065
82082,164165,164164,328329,69.89071607589722,7.261421963840689
83083,166167,166166,332333,70.92979502677917,7.126048672941238
84084,168169,168168,336337,72.02668309211731,6.993409652816922
85085,170171,170170,340341,73.10998487472534,6.863444904121366
86086,172173,172172,344345,74.22541689872742,6.736095874190255
87087,174175,174174,348349,75.3312418460846,6.611305414454705
88088,176177,176176,352353,76.44131088256836,6.489017739834253
89089,178179,178178,356357,77.52353286743164,6.369178389982608
90090,180181,180180,360361,78.603111743927,6.251734192253366
91091,182183,182182,364365,79.67991089820862,6.136633226273489
92092,184185,184184,368369,80.77050375938416,6.023824790005165
93093,186187,186186,372373,81.83539700508118,5.913259367192836
94094,188189,188188,376377,82.91001200675964,5.804888596094656
95095,190191,190190,380381,83.98654413223267,5.698665239408797
96096,192193,192192,384385,85.10086798667908,5.594543155305814
97097,194195,194194,388389,86.18544507026672,5.492477269492724
98098,196197,196196,392393,87.27712512016296,5.392423548238185
99099,198199,198198,396397,88.37706112861633,5.294338972292962
100100,200201,200200,400401,89.46467304229736,5.1981815116484995
101101,202203,202202,404405,90.55713391304016,5.10391010108367
102102,204205,204204,408409,91.65128898620605,5.011484616449707
103103,206207,206206,412413,92.73247599601746,4.920865851654412
104104,208209,208208,416417,93.96526980400085,4.8320154963057576
105105,210211,210210,420421,95.08342909812927,4.744896113984282
106106,212213,212212,424425,96.50510311126709,4.659471121108595
107107,214215,214214,428429,97.69749999046326,4.5757047663745425
108108,216217,216216,432433,98.82585000991821,4.493562110734729
109109,218219,218218,436437,100.01825499534607,4.413009007904293
110110,220221,220220,440441,101.18522310256958,4.334012085366339
111111,222223,222222,444445,102.59965586662292,4.256538725862697
112112,224225,224224,448449,103.77772688865662,4.180557049350909
113113,226227,226226,452453,104.99876093864441,4.106035895413925
114114,228229,228228,456457,106.41098213195801,4.032944806104979
115115,230231,230230,460461,107.63742995262146,3.9612540092181234
116116,232233,232232,464465,108.75116205215454,3.8909344019692753
117117,234235,234234,468469,109.87004494667053,3.8219575350775585
118118,236237,236236,472473,111.22925090789795,3.754295597233977
119119,238239,238238,476477,112.57147002220154,3.6879213999512785
120120,240241,240240,480481,113.75300812721252,3.6228083627790966
121121,242243,242242,484485,114.9441089630127,3.558930498880727
122122,244245,244244,488489,116.10821795463562,3.496262400958358
123123,246247,246246,492493,117.27981901168823,3.434779227520835
124124,248249,248248,496497,118.58339500427246,3.3744566894844183
125125,250251,250250,500501,119.87305903434753,3.315271037097318
126126,252253,252252,504505,120.9057970046997,3.2571990471838035
127127,254255,254254,508509,122.10547590255737,3.2002180106949254
128128,256257,256256,512513,123.18758296966553,3.144305720565626
129129,258259,258258,516517,124.31336688995361,3.089440459862317
130130,260261,260260,520521,125.39931797981262,3.035600990223429
131131,262263,262262,524525,126.52951502799988,2.982766540576449
132132,264265,264264,528529,127.6680498123169,2.930916796134966
133133,266267,266266,532533,128.79627585411072,2.880031887659129
134134,268269,268268,536537,129.87450098991394,2.8300923809808864
135135,270271,270270,540541,130.93505597114563,2.7810792667846727
136136,272273,272272,544545,132.0209457874298,2.7329739506359374
137137,274275,274274,548549,133.08933186531067,2.685758243255691
138138,276277,276276,552553,134.14940881729126,2.6394143510302683
139139,278279,278278,556557,135.22863793373108,2.593924866756197
140140,280281,280280,560561,136.45536184310913,2.5492727606089147
141141,282283,282282,564565,137.79334497451782,2.5054413713336317
142142,284285,284284,568569,139.11210894584656,2.4624143976521964
143143,286287,286286,572573,140.24226188659668,2.420175889879829
144144,288289,288288,576577,141.35783910751343,2.3787102417468304
145145,290291,290290,580581,142.45982003211975,2.3380021824222013
146146,292293,292292,584585,143.6945219039917,2.2980367687310945
147147,294295,294294,588589,145.07604503631592,2.2587993775630366
148148,296297,296296,592593,146.39265084266663,2.22027569846648
149149,298299,298298,596597,147.70488286018372,2.182451726424688
150150,300301,300300,600601,148.97782397270203,2.1453137548091945
151151,302303,302302,604605,150.24796795845032,2.108848368502663
152152,304305,304304,608609,151.49884295463562,2.07304243719409
153153,306307,306306,612613,152.74403882026672,2.037883108834535
154154,308309,308308,616617,153.99236607551575,2.003357803255426
155155,310311,310310,620621,155.2470200061798,1.9694542059398827
156156,312313,312312,624625,156.499351978302,1.9361602619483165
157157,314315,314314,628629,157.752427816391,1.9034641699915937
158158,316317,316316,632633,159.02469491958618,1.871354376648128
159159,318319,318318,636637,160.28739285469055,1.8398195707213745
160160,320321,320320,640641,161.5766577720642,1.8088486777367052
161161,322323,322322,644645,162.90400290489197,1.7784308545694785
162162,324325,324324,648649,164.15260410308838,1.7485554842052125
163163,326327,326326,652653,165.4223358631134,1.719212170626406
164164,328329,328328,656657,166.72118091583252,1.690390733823051
165165,330331,330330,660661,168.24943614006042,1.662081204923993
166166,332333,332332,664665,169.64585280418396,1.6342738214468682
167167,334335,334334,668669,171.10904788970947,1.6069590226618402
168168,336337,336336,672673,172.48027205467224,1.580127445066978
169169,338339,338338,676677,173.78836297988892,1.553769917974023
170170,340341,340340,680681,175.11111998558044,1.527877459199317
171171,342343,342342,684685,176.42052388191223,1.5024412708579575
172172,344345,344344,688689,177.7157130241394,1.4774527352608402
173173,346347,346346,692693,179.00280594825745,1.4529034109074246
174174,348349,348348,696697,180.32335782051086,1.428785028577181
175175,350351,350350,700701,181.62084794044495,1.4050894875124413
176176,352353,352352,704705,182.9992549419403,1.3818088516933358
177177,354355,354354,708709,184.34137988090515,1.3589353462011786
178178,356357,356356,712713,185.69275212287903,1.3364613536689376
179179,358359,358358,716717,187.0290470123291,1.3143794108159454
180180,360361,360360,720721,188.3356249332428,1.2926822050642386
181181,362363,362362,724725,189.6662518978119,1.2713625712364092
182182,364365,364364,728729,191.02089476585388,1.2504134883299685
183183,366367,366366,732733,192.34613704681396,1.229828076369813
184184,368369,368368,736737,193.65900683403015,1.2095995933327686
185185,370371,370370,740741,194.96078777313232,1.189721432147735
186186,372373,372372,744745,196.25232410430908,1.1701871177619978
187187,374375,374374,748749,197.56072115898132,1.150990304281322
188188,376377,376376,752753,198.8249499797821,1.1321247721730288
189189,378379,378378,756757,200.30167603492737,1.1135844255376242
190190,380381,380380,760761,201.80094981193542,1.0953632894415932
191191,382383,382382,764765,203.61433100700378,1.0774555073140846
192192,384385,384384,768769,205.0859980583191,1.0598553384048728
193193,386387,386386,772773,206.84682488441467,1.0425571552982547
194194,388389,388388,776777,208.68223595619202,1.0255554414889048
195195,390391,390390,780781,210.39403796195984,1.008844789010709
196196,392393,392392,784785,211.83275699615479,0.9924198961223283
197197,394395,394394,788789,213.22413897514343,0.9762755650442614
198198,396397,396396,792793,214.7055139541626,0.9604066997504788
199199,398399,398398,796797,216.55212998390198,0.9448083038091681
200200,400401,400400,800801,218.61302185058594,0.9294754782741848
201201,402403,402402,804805,220.05260396003723,0.9144034196234543
202202,404405,404404,808809,221.7380039691925,0.8995874177467158
203203,406407,406406,812813,223.12113499641418,0.8850228539769205
204204,408409,408408,816817,225.086040019989,0.8707051991681283
205205,410411,410410,820821,227.37898683547974,0.8566300118170602
206206,412413,412412,824825,229.68154311180115,0.842792936226715
207207,414415,414414,828829,231.85626792907715,0.8291897007117086
208208,416417,416416,832833,233.53342199325562,0.8158161158454504
209209,418419,418418,836837,235.13550686836243,0.8026680727455187
210210,420421,420420,840841,236.74081778526306,0.7897415413980298
211211,422423,422422,844845,238.23452997207642,0.7770325690207756
212212,424425,424424,848849,239.714262008667,0.764537278462285
213213,426427,426426,852853,241.21420407295227,0.7522518666371525
214214,428429,428428,856857,242.7296178340912,0.7401726029958127
215215,430431,430430,860861,244.1941258907318,0.7282958280300136
216216,432433,432432,864865,245.70529985427856,0.7166179518098943
217217,434435,434434,868869,247.26502299308777,0.705135452555055
218218,436437,436436,872873,248.84980082511902,0.6938448752368913
219219,438439,438438,876877,250.42459988594055,0.6827428302120779
220220,440441,440440,880881,251.93534088134766,0.671825991885953
221221,442443,442442,884885,253.42588591575623,0.66109109740637
222222,444445,444444,888889,254.90464401245117,0.6505349453856297
223223,446447,446446,892893,256.4673430919647,0.6401543946510628
224224,448449,448448,896897,257.9990828037262,0.6299463630225546
225225,450451,450450,900901,259.5130181312561,0.6199078261178101
226226,452453,452452,904905,261.1006729602814,0.6100358161830854
227227,454455,454454,908909,262.64175510406494,0.6003274209499523
228228,456457,456456,912913,264.1684970855713,0.5907797825167336
229229,458459,458458,916917,265.7041208744049,0.5813900962547223
230230,460461,460460,920921,267.185644865036,0.5721556097379334
231231,462463,462462,924925,268.69317388534546,0.5630736216965033
232232,464465,464464,928929,270.18683886528015,0.5541414809916887
233233,466467,466466,932933,271.679811000824,0.5453565856150817
234234,468469,468468,936937,273.2292070388794,0.5367163817076062
235235,470471,470470,940941,274.76948595046997,0.5282183626003416
236236,472473,472472,944945,276.2932929992676,0.519860067876607
237237,474475,474474,948949,277.8598120212555,0.5116390824531436
238238,476477,476476,952953,279.37238597869873,0.5035530356821027
239239,478479,478478,956957,280.8810019493103,0.4955996004711096
240240,480481,480480,960961,282.4030649662018,0.4877764924232224
241241,482483,482482,964965,283.9249289035797,0.4800814689957633
242242,484485,484484,968969,285.4462299346924,0.47251232867358794
243243,486487,486486,972973,287.01737904548645,0.46506691016577406
244244,488489,488488,976977,288.54580187797546,0.4577430916137928
245245,490491,490490,980981,290.0644679069519,0.45053878981980233
246246,492493,492492,984985,291.57761788368225,0.4434519594899484
247247,494495,494494,988989,293.0996677875519,0.436480592494604
248248,496497,496496,992993,294.60480308532715,0.4296227171433884
249249,498499,498498,996997,296.09216499328613,0.4228763974749654
250250,500501,500500,1001001,297.6021099090576,0.41623973256366753
251251,502503,502502,1005005,299.15310502052307,0.4097108558388527
252252,504505,504504,1009009,300.6987769603729,0.4032879344192679
253253,506507,506506,1013013,302.46104097366333,0.39696916846162367
254254,508509,508508,1017017,304.178270816803,0.3907527905217876
255255,510511,510510,1021021,305.8065640926361,0.38463706493075733
256256,512513,512512,1025025,307.57814502716064,0.37862028718188867
257257,514515,514514,1029029,309.28645181655884,0.37270078333222045
258258,516517,516516,1033033,310.8214781284332,0.3668769094165327
259259,518519,518518,1037037,312.33701395988464,0.3611470508702723
260260,520521,520520,1041041,313.8286838531494,0.3555096219703273
261261,522523,522522,1045045,315.3206388950348,0.34996306528069
262262,524525,524524,1049049,316.81392192840576,0.34450585111505916
263263,526527,526526,1053053,318.3845839500427,0.33913647700683214
264264,528529,528528,1057057,320.08091378211975,0.3338534671918296
265265,530531,530530,1061061,321.74983191490173,0.3286553721013661
266266,532533,532532,1065065,323.5185980796814,0.3235407678643014
267267,534535,534534,1069069,325.2097840309143,0.31850825582239395
268268,536537,536536,1073073,327.6420819759369,0.31355646205099674
269269,538539,538538,1077077,329.31807684898376,0.30868403689476054
270270,540541,540540,1081081,330.8071868419647,0.3038896545076568
271271,542543,542542,1085085,332.2753028869629,0.29917201240675695
272272,544545,544544,1089089,333.7654068470001,0.294529831031241
273273,546547,546546,1093093,335.26084184646606,0.28996185331322977
274274,548549,548548,1097097,336.73279786109924,0.2854668442564616
275275,550551,550550,1101101,338.23401379585266,0.2810435905222448
276276,552553,552552,1105105,339.6953980922699,0.2766909000247324
277277,554555,554554,1109109,341.1678738594055,0.2724076015351784
278278,556557,556556,1113113,342.67791509628296,0.26819254429233297
279279,558559,558558,1117117,344.16903591156006,0.26404459762204624
280280,560561,560560,1121121,345.6755139827728,0.259962650563466
281281,562563,562562,1125125,347.1594169139862,0.255945611504103
282282,564565,564564,1129129,348.646595954895,0.2519924078196709
283283,566567,566566,1133133,350.13740491867065,0.24810198552449947
284284,568569,568568,1137137,351.63466787338257,0.24427330892581267
285285,570571,570570,1141141,353.1371068954468,0.24050536028676106
286286,572573,572572,1145145,354.61867594718933,0.23679713949513825
287287,574575,574574,1149149,356.15162682533264,0.2331476637390324
288288,576577,576576,1153153,357.6463620662689,0.22955596718907145
289289,578579,578578,1157157,359.430716753006,0.2260211006865802
290290,580581,580580,1161161,361.09396290779114,0.22254213143799007
291291,582583,582582,1165165,362.8301627635956,0.21911814271493313
292292,584585,584584,1169169,364.48519587516785,0.215748233561726
293293,586587,586586,1173173,366.25773882865906,0.21243151850558206
294294,588589,588588,1177177,367.9345829486847,0.2091671272758049
295295,590591,590590,1181181,369.7898690700531,0.2059542045268472
296296,592593,592592,1185185,371.4723608493805,0.20279190956568982
297297,594595,594594,1189189,373.0910029411316,0.19967941608717865
298298,596597,596596,1193193,374.6895089149475,0.19661591191220396
299299,598599,598598,1197197,376.34150290489197,0.19360059873235969
300300,600601,600600,1201201,377.9531829357147,0.19063269185835452
301301,602603,602602,1205205,379.4543001651764,0.18771141997456198
302302,604605,604604,1209209,381.18099904060364,0.18483602489766326
303303,606607,606606,1213213,383.09646582603455,0.18200576133949653
304304,608609,608608,1217217,384.7024927139282,0.17921989667513571
305305,610611,610610,1221221,386.28163504600525,0.17647771071597163
306306,612613,612612,1225225,388.0269179344177,0.17377849548529412
307307,614615,614614,1229229,389.55559182167053,0.17112155500012705
308308,616617,616616,1233233,391.1168580055237,0.16850620505613279
309309,618619,618618,1237237,392.7620279788971,0.1659317730169505
310310,620621,620620,1241241,394.3363609313965,0.16339759760762718
311311,622623,622622,1245245,395.82070899009705,0.16090302871191398
312312,624625,624624,1249249,397.3330399990082,0.15844742717342797
313313,626627,626626,1253253,398.89075899124146,0.15603016459999708
314314,628629,628628,1257257,400.64159393310547,0.15365062317323464
315315,630631,630630,1261261,402.84445881843567,0.15130819546038765
316316,632633,632632,1265265,404.51822996139526,0.1490022842298231
317317,634635,634634,1269269,406.3373899459839,0.14673230227060685
318318,636637,636636,1273273,408.9023537635803,0.14449767221549337
319319,638639,638638,1277277,411.1798577308655,0.14229782636630262
320320,640641,640640,1281281,413.05169701576233,0.14013220652384462
321321,642643,642642,1285285,414.8720381259918,0.13800026381989028
322322,644645,644644,1289289,416.89326000213623,0.13590145855368974
323323,646647,646646,1293293,418.84522581100464,0.1338352600298549
324324,648649,648648,1297297,420.44632601737976,0.13180114640022111
325325,650651,650650,1301301,422.10391902923584,0.12979860450877823
326326,652653,652652,1305305,423.72987699508667,0.12782712974035348
327327,654655,654654,1309309,425.75492095947266,0.1258862258687259
328328,656657,656656,1313313,429.33060908317566,0.12397540491235759
329329,658659,658658,1317317,431.94296383857727,0.12209418698785157
330330,660661,660660,1321321,434.48207998275757,0.12024210017114001
331331,662663,662662,1325325,437.0490930080414,0.11841868035708103
332332,664665,664664,1329329,439.08752393722534,0.11662347112428506
333333,666667,666666,1333333,440.6355068683624,0.11485602360028224
334334,668669,668668,1337337,442.11727595329285,0.11311589633112362
335335,670671,670670,1341341,443.6087279319763,0.11140265515336978
336336,672673,672672,1345345,445.08628702163696,0.10971587306619313
337337,674675,674674,1349349,446.63984298706055,0.10805513010814138
338338,676677,676676,1353353,448.107106924057,0.10642001323537897
339339,678679,678678,1357357,449.64779901504517,0.1048101162017474
340340,680681,680680,1361361,451.29511284828186,0.10322503944223627
341341,682683,682682,1365365,452.84851813316345,0.10166438995679528
342342,684685,684684,1369369,454.35548305511475,0.10012778119744326
343343,686687,686686,1373373,455.8563051223755,0.09861483295810558
344344,688689,688688,1377377,457.35503792762756,0.09712517126433795
345345,690691,690690,1381381,458.8663969039917,0.09565842826748394
346346,692693,692692,1385385,460.3587329387665,0.09421424213826413
347347,694695,694694,1389389,461.84613704681396,0.09279225696502635
348348,696697,696696,1393393,463.3741660118103,0.0913921226514276
349349,698699,698698,1397397,464.95909905433655,0.09001349481741272
350350,700701,700700,1401401,466.64223885536194,0.08865603470178485
351351,702703,702702,1405405,468.1814298629761,0.08731940906511682
352352,704705,704704,1409409,469.92056012153625,0.08600329009766483
353353,706707,706706,1413413,471.4287278652191,0.0847073553240989
354354,708709,708708,1417417,472.9346179962158,0.08343128751607765
355355,710711,710710,1421421,475.11684799194336,0.08217477459970723
356356,712713,712712,1425425,477.6604039669037,0.08093750957027623
357357,714715,714714,1429429,479.47885513305664,0.0797191904051715
358358,716717,716716,1433433,481.09445691108704,0.07851951998020468
359359,718719,718718,1437437,482.629497051239,0.07733820598582497
360360,720721,720720,1441441,484.21379494667053,0.07617496084617414
361361,722723,722722,1445445,485.8023090362549,0.07502950163870992
362362,724725,724724,1449449,487.35829281806946,0.07390155001598941
363363,726727,726726,1453453,488.8801441192627,0.07279083212836213
364364,728729,728728,1457457,490.52039790153503,0.07169707854814078
365365,730731,730730,1461461,492.0639238357544,0.0706200241947954
366366,732733,732732,1465465,493.6206157207489,0.06955940826287588
367367,734735,734734,1469469,495.2520899772644,0.06851497414834284
368368,736737,736736,1473473,496.88177490234375,0.06748646937990088
369369,738739,738738,1477477,498.433002948761,0.06647364554862634
370370,740741,740740,1481481,499.9630661010742,0.06547625824032366
371371,742743,742742,1485485,501.5270240306854,0.06449406696742699
372372,744745,744744,1489489,503.129900932312,0.06352683510544921
373373,746747,746746,1493493,504.6562180519104,0.06257432982658884
374374,748749,748748,1497497,506.1606249809265,0.06163632203663383
375375,750751,750750,1501501,507.7278130054474,0.06071258631368437
376376,752753,752752,1505505,509.28214502334595,0.05980290084551143
377377,754755,754754,1509509,510.8286168575287,0.0589070473705533
378378,756757,756756,1513513,512.5875911712646,0.05802481111788893
379379,758759,758758,1517517,514.2447347640991,0.057155980749826085
380380,760761,760760,1521521,515.7849359512329,0.0563003483052853
381381,762763,762762,1525525,517.279501914978,0.05545770914181958
382382,764765,764764,1529529,518.941535949707,0.05462786188320479
383383,766767,766766,1533533,520.5773229598999,0.0538106083627099
384384,768769,768768,1537537,522.2372739315033,0.05300575357239268
385385,770771,770770,1541541,524.2917490005493,0.05221310560887105
386386,772773,772772,1545545,525.9052519798279,0.05143247562295983
387387,774775,774774,1549549,527.5095739364624,0.05066367776930747
388388,776777,776776,1553553,529.1405379772186,0.04990652915614646
389389,778779,778778,1557557,531.18425989151,0.049160849796976436
390390,780781,780780,1561561,532.8758981227875,0.04842646256292937
391391,782783,782782,1565565,534.4842119216919,0.0477031931353622
392392,784785,784784,1569569,536.0370547771454,0.04699086995969992
393393,786787,786786,1573573,538.0319328308105,0.046289324199847215
394394,788789,788788,1577577,540.0401329994202,0.0455983896943053
395395,790791,790790,1581581,541.6302790641785,0.04491790291081088
396396,792793,792792,1585585,543.1159439086914,0.04424770290518154
397397,794795,794794,1589589,544.872386932373,0.04358763127675047
398398,796797,796796,1593593,546.7623109817505,0.04293753212812135
399399,798799,798798,1597597,548.263298034668,0.04229725202424106
400400,800801,800800,1601601,549.7577500343323,0.0416666399511314
401401,802803,802802,1605605,551.2693648338318,0.04104554727757659
402402,804805,804804,1609609,552.7632608413696,0.040433827715219195
403403,806807,806806,1613613,554.2432260513306,0.03983133728070243
404404,808809,808808,1617617,555.7903280258179,0.03923793425860822
405405,810811,810810,1621621,557.3045279979706,0.03865347916325845
406406,812813,812812,1625625,558.7985508441925,0.03807783470404047
407407,814815,814814,1629629,560.2633588314056,0.037510865748117794
408408,816817,816816,1633633,561.7557349205017,0.03695243928666514
409409,818819,818818,1637637,563.4130959510803,0.0364024243995118
410410,820821,820820,1641641,565.4595999717712,0.035860692221831414
411411,822823,822822,1645645,567.3577988147736,0.035327115910263274
412412,824825,824824,1649649,569.1763119697571,0.0348015706103979
413413,826827,826826,1653653,571.9908010959625,0.03428393342517211
414414,828829,828828,1657657,573.7430799007416,0.03377408338144505
415415,830831,830830,1661661,575.6660869121552,0.033271901401121795
416416,832833,832832,1665665,577.4904499053955,0.03277727026932098
417417,834835,834834,1669669,579.2128307819366,0.032290074603679386
418418,836837,836836,1673673,580.7289960384369,0.031810200826612345
419419,838839,838838,1677677,582.196939945221,0.03133753713427723
420420,840841,840840,1681681,583.6870000362396,0.030871973469174918
421421,842843,842842,1685685,585.5821008682251,0.03041340149172811
422422,844845,844844,1689689,587.3647909164429,0.029961714552200647
423423,846847,846846,1693693,589.2385137081146,0.029516807664663247
424424,848849,848848,1697697,590.9570558071136,0.029078577478912848
425425,850851,850850,1701701,592.5800549983978,0.028646922254665697
426426,852853,852852,1705705,594.1970059871674,0.028221741836887304
427427,854855,854854,1709709,595.7936818599701,0.027802937627598112
428428,856857,856856,1713713,597.3500018119812,0.027390412564159305
429429,858859,858858,1717717,598.860239982605,0.02698407109244272
430430,860861,860860,1721721,600.3816409111023,0.026583819143411347
431431,862863,862862,1725725,601.9327578544617,0.02618956410969986
432432,864865,864864,1729729,603.5519490242004,0.025801214821512986
433433,866867,866866,1733733,605.178386926651,0.0254186815243429
434434,868869,868868,1737737,606.7482171058655,0.025041875855549733
435435,870871,870870,1741741,608.3374979496002,0.024670710823215813
436436,872873,872872,1745745,609.8530600070953,0.024305100783180933
437437,874875,874874,1749749,611.487795829773,0.0239449614186924
438438,876877,876876,1753753,613.0445721149445,0.023590209718349797
439439,878879,878878,1757757,614.6252219676971,0.023240763955413968
440440,880881,880880,1761761,616.2474977970123,0.022896543668025515
441441,882883,882882,1765765,617.816422700882,0.022557469638400107
442442,884885,884884,1769769,619.3814699649811,0.022223463873501714
443443,886887,886886,1773773,620.9302139282227,0.021894449585374787
444444,888889,888888,1777777,622.4981050491333,0.021570351171703805
445445,890891,890890,1781781,624.129723072052,0.02125109419796445
446446,892893,892892,1785785,625.6006979942322,0.020936605377869455
447447,894895,894894,1789789,627.1644718647003,0.02062681255551979
448448,896897,896896,1793793,628.7417368888855,0.020321644688351626
449449,898899,898898,1797797,630.6282768249512,0.020021031827582192
450450,900901,900900,1801801,632.2428667545319,0.01972490510308944
451451,902903,902902,1805805,634.1037368774414,0.019433196704881084
452452,904905,904904,1809809,637.0621438026428,0.01914583986706475
453453,906907,906906,1813813,640.0089898109436,0.01886276885090865
454454,908909,908908,1817817,642.2620298862457,0.018583918929266474
455455,910911,910910,1821821,644.3019948005676,0.018309226369183307
456456,912913,912912,1825825,645.9022209644318,0.018038628418480585
457457,914915,914914,1829829,647.4462268352509,0.017772063288475692
458458,916917,916916,1833833,649.0100920200348,0.017509470138975303
459459,918919,918918,1837837,650.6450469493866,0.017250789064974015
460460,920921,920920,1841841,652.202488899231,0.016995961079487643
461461,922923,922922,1845845,654.0951879024506,0.016744928100933976
462462,924925,924924,1849849,656.5506417751312,0.01649763293869455
463463,926927,926926,1853853,659.054918050766,0.016254019277880616
464464,928929,928928,1857857,662.0500888824463,0.016014031667168638
465465,930931,930930,1861861,665.3566670417786,0.01577761550447576
466466,932933,932932,1865865,667.4539377689362,0.015544717023544763
467467,934935,934934,1869869,669.1303369998932,0.01531528328132481
468468,936937,936936,1873873,671.3541460037231,0.015089262144215354
469469,938939,938938,1877877,673.4626758098602,0.014866602276811136
470470,940941,940940,1881881,675.5602600574493,0.014647253127577642
471471,942943,942942,1885885,677.4817168712616,0.014431164918846662
472472,944945,944944,1889889,679.1405549049377,0.014218288631809628
473473,946947,946946,1893893,681.5804440975189,0.014008575997650041
474474,948949,948948,1897897,683.2143950462341,0.01380197948424211
475475,950951,950950,1901901,684.6816439628601,0.013598452284213636
476476,952953,952952,1905905,686.2081871032715,0.013397948305168939
477477,954955,954954,1909909,687.7571461200714,0.01320042215684225
478478,956957,956956,1913913,689.2572009563446,0.013005829141775394
479479,958959,958958,1917917,690.7744328975677,0.012814125243380659
480480,960961,960960,1921921,692.2692210674286,0.012625267115936367
481481,962963,962962,1925925,693.8132750988007,0.0124392120731045
482482,964965,964964,1929929,695.6267371177673,0.012255918079745243
483483,966967,966966,1933933,697.2128179073334,0.012075343739525124
484484,968969,968968,1937937,699.041601896286,0.0118974482863905
485485,970971,970970,1941941,701.311164855957,0.011722191574222052
486486,972973,972972,1945945,702.9249861240387,0.011549534067739842
487487,974975,974974,1949949,704.5183401107788,0.011379436832271494
488488,976977,976976,1953953,706.3022549152374,0.011211861524657252
489489,978979,978978,1957957,707.8298778533936,0.011046770384609772
490490,980981,980980,1961961,709.3504319190979,0.010884126225278123
491491,982983,982982,1965965,711.0725758075714,0.01072389242403915
492492,984985,984984,1969969,712.593003988266,0.010566032914425705
493493,986987,986986,1973973,714.1360139846802,0.010410512176804332
494494,988989,988988,1977977,715.6908760070801,0.010257295230985619
495495,990991,990990,1981981,717.3047578334808,0.010106347626560819
496496,992993,992992,1985985,718.8944199085236,0.009957635435398515
497497,994995,994994,1989989,720.5185770988464,0.009811125244027608
498498,996997,996996,1993993,722.2114880084991,0.009666784144428675
499499,998999,998998,1997997,723.8643350601196,0.009524579727553828
500501,1001003,1001002,2002005,725.3938930034637,0.009384341157101517
501502,1003005,1003004,2006009,726.9445719718933,0.009246316888834372
502503,1005007,1005006,2010013,728.6314129829407,0.00911033495913216
503504,1007009,1007008,2014017,730.3314549922943,0.008976364876616572
504505,1009011,1009010,2018021,732.0776591300964,0.008844376611818916
505506,1011013,1011012,2022025,733.7866628170013,0.0087143405887673
506507,1013015,1013014,2026029,735.3026208877563,0.008586227678847536
507508,1015017,1015016,2030033,736.7969899177551,0.008460009193527185
508509,1017019,1017018,2034037,738.3090558052063,0.00833565687742066
509510,1019021,1019020,2038041,739.7793960571289,0.008213142902036452
510511,1021023,1021022,2042045,741.4289269447327,0.008092439858955913
511512,1023025,1023024,2046049,743.0194957256317,0.0079735207534668
512513,1025027,1025026,2050053,744.5682528018951,0.007856358998424184
513514,1027029,1027028,2054057,746.0737881660461,0.007740928407542924
514515,1029031,1029030,2058061,747.6613109111786,0.00762720318925858
515516,1031033,1031032,2062065,749.1550278663635,0.007515157941384132
516517,1033035,1033034,2066069,750.7064599990845,0.007404767644402455
517518,1035037,1035036,2070073,752.3603849411011,0.0072960076557819775
518519,1037039,1037038,2074077,754.0009109973907,0.007188853704064968
519520,1039041,1039040,2078081,755.610906124115,0.007083281883865311
520521,1041043,1041042,2082085,757.163213968277,0.0069792686492746725
521522,1043045,1043044,2086089,758.6527390480042,0.006876790809087652
522523,1045047,1045046,2090093,760.3182849884033,0.006775825521231127
523524,1047049,1047048,2094097,762.0338799953461,0.006676350287079913
524525,1049051,1049050,2098101,763.9876368045807,0.006578342946681914
525526,1051053,1051052,2102105,765.836226940155,0.006481781673073783
526527,1053055,1053054,2106109,767.9393708705902,0.006386644967733446
527528,1055057,1055056,2110113,769.9480118751526,0.0062929116551231346
528529,1057059,1057058,2114117,772.0404388904572,0.006200560878255601
529530,1059061,1059060,2118121,774.312924861908,0.006109572093009774
530531,1061063,1061062,2122125,776.5035948753357,0.006019925064265408
531532,1063065,1063064,2126129,779.3583889007568,0.0059315998605598
532533,1065067,1065066,2130133,782.0983099937439,0.005844576849654004
533534,1067069,1067068,2134137,783.9435520172119,0.005758836694099045
534535,1069071,1069070,2138141,786.6034009456635,0.005674360346802132
535536,1071073,1071072,2142145,789.0228018760681,0.0055911290460244345
536537,1073075,1073074,2146149,791.4830539226532,0.005509124311970481
537538,1075077,1075076,2150153,795.7295439243317,0.005428327941444877
538539,1077079,1077078,2154157,798.3904480934143,0.005348722004441697
539540,1079081,1079080,2158161,801.574285030365,0.005270288839710702
540541,1081083,1081082,2162165,803.248391866684,0.005193011050778296
541542,1083085,1083084,2166169,806.4006147384644,0.005116871501627429
542543,1085087,1085086,2170173,809.7725319862366,0.005041853312945932
543544,1087089,1087088,2174177,811.708582162857,0.004967939858261161
544545,1089091,1089090,2178181,813.672492980957,0.004895114760074648
545546,1091093,1091092,2182185,815.1961917877197,0.004823361886337807
546547,1093095,1093094,2186189,817.2457981109619,0.004752665345790774
547548,1095097,1095096,2190193,819.4475560188293,0.004683009485461298
548549,1097099,1097098,2194197,823.0283398628235,0.004614378886344639
549550,1099101,1099100,2198201,825.8486571311951,0.004546758360447711
550551,1101103,1101102,2202205,828.7495260238647,0.004480132946127924
551552,1103105,1103104,2206209,831.5472049713135,0.0044144879061605025
552553,1105107,1105106,2210213,833.410336971283,0.0043498087233047045
553554,1107109,1107108,2214217,835.0187849998474,0.004286081097234273
554555,1109111,1109110,2218221,836.8512959480286,0.004223290941467894
555556,1111113,1111112,2222225,838.334734916687,0.004161424379958589
556557,1113115,1113114,2226229,839.9075119495392,0.004100467743569425
557558,1115117,1115116,2230233,841.9142661094666,0.0040404075676860884
558559,1117119,1117118,2234237,843.6806309223175,0.00398123058857891
559560,1119121,1119120,2238241,845.5677280426025,0.003922923740560691
560561,1121123,1121122,2242245,847.3796279430389,0.003865474152689785
561562,1123125,1123124,2246249,849.2972929477692,0.0038088691462689894
562563,1125127,1125126,2250253,851.0920498371124,0.0037530962320033723
563564,1127129,1127128,2254257,852.8526599407196,0.003698143106362295
564565,1129131,1129130,2258261,854.8698830604553,0.0036439976494193616
565566,1131133,1131132,2262265,856.6073188781738,0.0035906479225786825
566567,1133135,1133134,2266269,858.3591327667236,0.0035380821641410876
567568,1135137,1135136,2270273,860.3096640110016,0.003486288788735692
568569,1137139,1137138,2274277,861.8617568016052,0.0034352563827724225
569570,1139141,1139140,2278281,863.3516368865967,0.0033849737034188365
570571,1141143,1141142,2282285,864.9593887329102,0.0033354296750758294
571572,1143145,1143144,2286289,866.9591310024261,0.0032866133864217772
572573,1145147,1145146,2290293,868.9856507778168,0.0032385140902988496
573574,1147149,1147148,2294297,870.5239789485931,0.0031911211975739207
574575,1149151,1149150,2298301,872.0383059978485,0.0031444242779343767
575576,1151153,1151152,2302305,873.5541348457336,0.003098413056136451
576577,1153155,1153154,2306309,875.0910770893097,0.0030530774096177993
577578,1155157,1155156,2310313,876.6360628604889,0.003008407366451138
578579,1157159,1157158,2314317,878.1541638374329,0.00296439310329788
579580,1159161,1159160,2318321,879.674339056015,0.0029210249423385903
580581,1161163,1161162,2322325,881.3871788978577,0.002878293350477179
581582,1163165,1163164,2326329,883.0122580528259,0.0028361889357029213
582583,1165167,1165166,2330333,884.6341459751129,0.0027947024461809633
583584,1167169,1167168,2334337,886.5595738887787,0.0027538247667280302
584585,1169171,1169170,2338341,888.2986800670624,0.0027135469185850525
585586,1171173,1171172,2342345,889.8467009067535,0.002673860055892874
586587,1173175,1173174,2346349,891.4872989654541,0.0026347554638732618
587588,1175177,1175176,2350353,892.993616104126,0.0025962245578057264
588589,1177179,1177178,2354357,894.6195409297943,0.002558258880299036
589590,1179181,1179180,2358361,896.20490193367,0.002520850099699601
590591,1181183,1181182,2362365,898.2905178070068,0.0024839900073629906
591592,1183185,1183184,2366369,900.3018698692322,0.0024476705170854984
592593,1185187,1185186,2370373,902.3751919269562,0.0024118836624893447
593594,1187189,1187188,2374377,904.9989428520203,0.0023766215957721215
594595,1189191,1189190,2378381,907.2902429103851,0.0023418765849783085
595596,1191193,1191192,2382385,908.9466700553894,0.0023076410130897784
596597,1193195,1193194,2386389,910.6148369312286,0.0022739073759794337
597598,1195197,1195196,2390393,912.1993980407715,0.0022406682812743384
598599,1197199,1197198,2394397,913.7500488758087,0.0022079164458546074
599600,1199201,1199200,2398401,915.385725736618,0.0021756446942617913
600601,1201203,1201202,2402405,916.9582769870758,0.0021438459579030678
601602,1203205,1203204,2406409,918.4857220649719,0.002112513273004879
602603,1205207,1205206,2410413,920.0872669219971,0.002081639778339195
603604,1207209,1207208,2414417,921.6497919559479,0.0020512187148824523
604605,1209211,1209210,2418421,923.2264668941498,0.0020212434237691923
605606,1211213,1211212,2422425,924.903443813324,0.001991707344700444
606607,1213215,1213214,2426429,926.4481687545776,0.0019626040144657964
607608,1215217,1215216,2430433,928.0093250274658,0.0019339270651244078
608609,1217219,1217218,2434437,929.5077338218689,0.0019056702238913203
609610,1219221,1219220,2438441,931.0429339408875,0.0018778273104089749
610611,1221223,1221222,2442445,932.6964039802551,0.001850392235610343
611612,1223225,1223224,2446449,934.282812833786,0.0018233590010368061
612613,1225227,1225226,2450453,935.7817659378052,0.0017967216963370447
613614,1227229,1227228,2454457,937.2670350074768,0.0017704744994944122
614615,1229231,1229230,2458461,938.765636920929,0.0017446116735300166
615616,1231233,1231232,2462465,940.5371329784393,0.0017191275674122153
616617,1233235,1233234,2466469,942.2548987865448,0.0016940166131007572
617618,1235237,1235236,2470473,944.33345079422,0.0016692733248646618
618619,1237239,1237238,2474477,945.972058057785,0.0016448922983727243
619620,1239241,1239240,2478481,947.911994934082,0.0016208682089882132
620621,1241243,1241242,2482485,950.6945838928223,0.0015971958108593753
621622,1243245,1243244,2486489,953.5133128166199,0.0015738699355551944
622623,1245247,1245246,2490493,956.0412049293518,0.001550885491496956
623624,1247249,1247248,2494497,958.304929971695,0.0015282374616845118
624625,1249251,1249250,2498501,960.7490148544312,0.0015059209034689047
625626,1251253,1251252,2502505,962.5501239299774,0.0014839309475291884
626627,1253255,1253254,2506509,964.274612903595,0.001462262796280811
627628,1255257,1255256,2510513,965.8648297786713,0.0014409117228524337
628629,1257259,1257258,2514517,967.4341180324554,0.0014198730701764362
629630,1259261,1259260,2518521,969.0035057067871,0.001399142250420482
630631,1261263,1261262,2522525,970.4820909500122,0.0013787147428274693
631632,1263265,1263264,2526529,971.9749097824097,0.0013585860938292171
632633,1265267,1265266,2530533,973.5043697357178,0.0013387519156822236
633634,1267269,1267268,2534537,975.4554390907288,0.0013192078846486766
634635,1269271,1269270,2538541,977.2738809585571,0.0012999497421333217
635636,1271273,1271272,2542545,979.0880239009857,0.0012809732908181104
636637,1273275,1273274,2546549,981.090213060379,0.0012622743965948757
637638,1275277,1275276,2550553,983.0610549449921,0.0012438489856094748
638639,1277279,1277278,2554557,984.635027885437,0.0012256930443754754
639640,1279281,1279280,2558561,986.1482379436493,0.001207802618750975
640641,1281283,1281282,2562565,987.7350850105286,0.001190173812346984
641642,1283285,1283284,2566569,989.2881908416748,0.0011728027869821744
642643,1285287,1285286,2570573,990.8536260128021,0.0011556857605228288
643644,1287289,1287288,2574577,992.3587999343872,0.001138819006769154
644645,1289291,1289290,2578581,993.866409778595,0.0011221988544320993
645646,1291293,1291292,2582585,995.3348867893219,0.001105821686451236
646647,1293295,1293294,2586589,996.986839056015,0.0010896839389715751
647648,1295297,1295296,2590593,998.5650427341461,0.0010737821003203862
648649,1297299,1297298,2594597,1000.1319448947906,0.0010581127112345712
649650,1299301,1299300,2598601,1001.6401419639587,0.0010426723632690482
650651,1301303,1301302,2602605,1003.1106128692627,0.0010274576978872574
651652,1303305,1303304,2606609,1004.6295168399811,0.0010124654058927263
652653,1305307,1305306,2610613,1006.1474030017853,0.00099769222742907
653654,1307309,1307308,2614617,1007.7550208568573,0.0009831349500473152
654655,1309311,1309310,2618621,1009.3748750686646,0.000968790409160647
655656,1311313,1311312,2622625,1011.0618150234222,0.0009546554864527934
656657,1313315,1313314,2626629,1012.6146337985992,0.0009407271093095915
657658,1315317,1315316,2630633,1014.5787398815155,0.0009270022509326736
658659,1317319,1317318,2634637,1016.9014329910278,0.0009134779285204786
659660,1319321,1319320,2638641,1018.6717929840088,0.0009001512034956249
660661,1321323,1321322,2642645,1020.846107006073,0.0008870191804817296
661662,1323325,1323324,2646649,1022.3842630386353,0.0008740790067349735
662663,1325327,1325326,2650653,1024.1450979709625,0.0008613278713482941
663664,1327329,1327328,2654657,1025.8875739574432,0.0008487630046829509
664665,1329331,1329330,2658661,1027.6364018917084,0.0008363816782548383
665666,1331333,1331332,2662665,1029.1591620445251,0.0008241812034839313
666667,1333335,1333334,2666669,1030.7429249286652,0.000812158931353224
667668,1335337,1335336,2670673,1032.504135131836,0.0008003122516129224
668669,1337339,1337338,2674677,1034.259377002716,0.0007886385925530703
669670,1339341,1339340,2678681,1035.938050031662,0.0007771354205488024
670671,1341343,1341342,2682685,1038.7895758152008,0.0007658002389234753
671672,1343345,1343344,2686689,1040.8018689155579,0.0007546305876076076
672673,1345347,1345346,2690693,1042.7336089611053,0.0007436240430251928
673674,1347349,1347348,2694697,1044.5449068546295,0.0007327782170705177
674675,1349351,1349350,2698701,1046.485694885254,0.0007220907565397283
675676,1351353,1351352,2702705,1048.7934310436249,0.0007115593431308298
676677,1353355,1353354,2706709,1051.5267729759216,0.0007011816927615655
677678,1355357,1355356,2710713,1053.9452548027039,0.0006909555543188617
678679,1357359,1357358,2714717,1055.801011800766,0.0006808787101135749
679680,1359361,1359360,2718721,1057.872503042221,0.0006709489750846842
680681,1361363,1361362,2722725,1059.877275943756,0.0006611641963445436
681682,1363365,1363364,2726729,1062.1330118179321,0.0006515222521557007
682683,1365367,1365366,2730733,1064.2749407291412,0.0006420210526130177
683684,1367369,1367368,2734737,1066.1940658092499,0.0006326585380520555
684685,1369371,1369370,2738741,1068.2363839149475,0.0006234326790490741
685686,1371373,1371372,2742745,1070.0838119983673,0.0006143414766484057
686687,1373375,1373374,2746749,1072.0394189357758,0.0006053829602024052
687688,1375377,1375376,2750753,1074.0964739322662,0.0005965551885083187
688689,1377379,1377378,2754757,1076.078132867813,0.0005878562491261619
689690,1379381,1379380,2758761,1078.0096580982208,0.0005792842574692258
690691,1381383,1381382,2762765,1079.808315038681,0.0005708373563493296
691692,1383385,1383384,2766769,1082.09028506279,0.0005625137160905069
692693,1385387,1385386,2770773,1084.0513038635254,0.0005543115341879457
693694,1387389,1387388,2774777,1086.3357429504395,0.000546229033830059
694695,1389391,1389390,2778781,1088.072126865387,0.0005382644650353541
695696,1391393,1391392,2782785,1089.6511409282684,0.0005304161030608157
696697,1393395,1393394,2786789,1091.6884257793427,0.0005226822486292804
697698,1395397,1395396,2790793,1093.5865178108215,0.0005150612272473154
698699,1397399,1397398,2794797,1095.286180973053,0.0005075513890915317
699700,1399401,1399400,2798801,1097.4419589042664,0.0005001511087812105
700701,1401403,1401402,2802805,1099.4427418708801,0.0004928587841277476
701702,1403405,1403404,2806809,1101.4005889892578,0.0004856728371578356
702703,1405407,1405406,2810813,1103.2842168807983,0.0004785917127492212
703704,1407409,1407408,2814817,1105.7644128799438,0.0004716138786307056
704705,1409411,1409410,2818821,1108.0766360759735,0.00046473782470002334
705706,1411413,1411412,2822825,1110.1058900356293,0.000457962063251216
706707,1413415,1413414,2826829,1112.263935804367,0.0004512851285198849
707708,1415417,1415416,2830833,1114.5132579803467,0.00044470557600106986
708709,1417419,1417418,2834837,1116.8761987686157,0.00043822198279031
709710,1419421,1419420,2838841,1119.3086698055267,0.00043183294610571465
710711,1421423,1421422,2842845,1121.7822880744934,0.00042553708442483185
711712,1423425,1423424,2846849,1123.565771818161,0.00041933303600671934
712713,1425427,1425426,2850853,1125.235633134842,0.00041321945911931834
713714,1427429,1427428,2854857,1127.4223818778992,0.0004071950322668272
714715,1429431,1429430,2858861,1129.499587059021,0.00040125845248439873
715716,1431433,1431432,2862865,1131.538594007492,0.00039540843636132195
716717,1433435,1433434,2866869,1133.3374569416046,0.00038964371958627453
717718,1435437,1435436,2870873,1135.4620079994202,0.0003839630553557072
718719,1437439,1437438,2874877,1137.4616298675537,0.00037836521653389354
719720,1439441,1439440,2878881,1139.5894589424133,0.0003728489924696987
720721,1441443,1441442,2882885,1141.6089899539948,0.0003674131914976897
721722,1443445,1443444,2886889,1143.6977598667145,0.00036205663877808547
722723,1445447,1445446,2890893,1145.6153509616852,0.00035677817675150436
723724,1447449,1447448,2894897,1147.370540857315,0.00035157666491159034
724725,1449451,1449450,2898901,1149.0188429355621,0.0003464509795776394
725726,1451453,1451452,2902905,1150.7432868480682,0.00034140001309879153
726727,1453455,1453454,2906909,1152.6495740413666,0.00033642267430877837
727728,1455457,1455456,2910913,1154.4542157649994,0.0003315178882985492
728729,1457459,1457458,2914917,1156.3145110607147,0.00032668459527940286
729730,1459461,1459460,2918921,1157.93581199646,0.0003219217513787953
730731,1461463,1461462,2922925,1160.1331088542938,0.00031722832818559255
731732,1463465,1463464,2926929,1162.171236038208,0.00031260331184057577
732733,1465467,1465466,2930933,1164.2199311256409,0.00030804570371856244
733734,1467469,1467468,2934937,1166.010407924652,0.00030355451951891155
734735,1469471,1469470,2938941,1167.6926429271698,0.0002991287899476447
735736,1471473,1471472,2942945,1169.6534860134125,0.00029476755901214347
736737,1473475,1473474,2946949,1171.574001789093,0.0002904698849306442
737738,1475477,1475476,2950953,1173.3555917739868,0.00028623484070067207
738739,1477479,1477478,2954957,1175.639055967331,0.00028206151171161764
739740,1479481,1479480,2958961,1177.772929906845,0.0002779489967679183
740741,1481483,1481482,2962965,1179.5903499126434,0.0002738964088848661
741742,1483485,1483484,2966969,1181.8399019241333,0.00026990287301487115
742743,1485487,1485486,2970973,1183.953290939331,0.0002659675275253903
743744,1487489,1487488,2974977,1185.9528968334198,0.0002620895227209985
744745,1489491,1489490,2978981,1187.7914559841156,0.0002582680223213174
745746,1491493,1491492,2982985,1190.0292310714722,0.0002545022014146525
746747,1493495,1493494,2986989,1191.882756948471,0.0002507912477085483
747748,1495497,1495496,2990993,1193.9159348011017,0.0002471343602792331
748749,1497499,1497498,2994997,1196.0919868946075,0.0002435307504811135
749750,1499501,1499500,2999001,1198.482300043106,0.00023997964080990641
750751,1501503,1501502,3003005,1200.1978950500488,0.00023648026490263874
751752,1503505,1503504,3007009,1202.153268814087,0.0002330318684471422
752753,1505507,1505506,3011013,1203.9267377853394,0.0002296337077041244
753754,1507509,1507508,3015017,1205.9810090065002,0.0002262850492797952
754755,1509511,1509510,3019021,1208.2191369533539,0.0002229851712627351
755756,1511513,1511512,3023025,1210.457477092743,0.00021973336197333992
756757,1513515,1513514,3027029,1212.916958808899,0.0002165289204185683
757758,1515517,1515516,3031033,1215.1418988704681,0.00021337115526876005
758759,1517519,1517518,3035037,1217.0084338188171,0.00021025938576713088
759760,1519521,1519520,3039041,1219.009686946869,0.0002071929410476514
760761,1521523,1521522,3043045,1220.6902680397034,0.00020417116002136027
761762,1523525,1523524,3047049,1222.352149963379,0.00020119339114899049
762763,1525527,1525526,3051053,1224.4275588989258,0.0001982589925546563
763764,1527529,1527528,3055057,1226.2191388607025,0.0001953673316847926
764765,1529531,1529530,3059061,1228.0005548000336,0.000192517785308155
765766,1531533,1531532,3063065,1229.670408964157,0.00018970973894738563
766767,1533535,1533534,3067069,1231.2094478607178,0.00018694258790219465
767768,1535537,1535536,3071073,1233.1523067951202,0.000184215735316684
768769,1537539,1537538,3075077,1235.809308052063,0.00018152859365727636
769770,1539541,1539540,3079081,1237.8355560302734,0.00017888058403059404
770771,1541543,1541542,3083085,1239.4434039592743,0.00017627113561502483
771772,1543545,1543544,3087089,1241.4177379608154,0.00017369968634284305
772773,1545547,1545546,3091093,1243.0251219272614,0.00017116568187702796
773774,1547549,1547548,3095097,1244.586613893509,0.00016866857640707167
774775,1549551,1549550,3099101,1246.6996488571167,0.00016620783219423174
775776,1551553,1551552,3103105,1249.365905046463,0.0001637829185483497
776777,1553555,1553554,3107109,1250.8773968219757,0.00016139331353315356
777778,1555557,1555556,3111113,1252.379448890686,0.00015903850214726845
778779,1557559,1557558,3115117,1253.8862807750702,0.00015671797723371128
779780,1559561,1559560,3119121,1255.3517470359802,0.00015443123902514344
780781,1561563,1561562,3123125,1256.9633519649506,0.00015217779503018392
781782,1563565,1563564,3127129,1258.548124074936,0.0001499571596923488
782783,1565567,1565566,3131133,1260.046600818634,0.00014776885495848546
783784,1567569,1567568,3135137,1261.559494972229,0.00014561240948296472
784785,1569571,1569570,3139141,1263.0458028316498,0.00014348735874136764
785786,1571573,1571572,3143145,1264.551974773407,0.0001413932454852329
786787,1573575,1573574,3147149,1266.0270149707794,0.00013932961860518844
787788,1575577,1575576,3151153,1267.505994796753,0.0001372960336993856
788789,1577579,1577578,3155157,1268.9965589046478,0.0001352920527324386
789790,1579581,1579580,3159161,1270.4853711128235,0.0001333172447175457
790791,1581583,1581582,3163165,1271.9631941318512,0.0001313711842385601
791792,1583585,1583584,3167169,1273.4438908100128,0.00012945345224579796
792793,1585587,1585586,3171173,1274.9034609794617,0.00012756363605603838
793794,1587589,1587588,3175177,1276.3936460018158,0.00012570132889777597
794795,1589591,1589590,3179181,1277.8780999183655,0.00012386612979753409
795796,1591593,1591592,3183185,1279.3542461395264,0.00012205764357986482
796797,1593595,1593594,3187189,1280.8320360183716,0.00012027548143578315
797798,1595597,1595596,3191193,1282.307846069336,0.00011851925921746442
798799,1597599,1597598,3195197,1283.7918298244476,0.00011678859937092056
799800,1599601,1599600,3199201,1285.270614862442,0.00011508312934438436
800801,1601603,1601602,3203205,1286.7935719490051,0.00011340248204305681
801802,1603605,1603604,3207209,1288.2892870903015,0.00011174629582910711
802803,1605607,1605606,3211213,1289.8050079345703,0.00011011421440798586
803804,1607609,1607608,3215217,1291.2809047698975,0.00010850588648736448
804805,1609611,1609610,3219221,1292.7582697868347,0.00010692096577713528
805806,1611613,1611612,3223225,1294.2292709350586,0.00010535911189890612
806807,1613615,1613614,3227229,1295.5240581035614,0.00010381998811226367
807808,1615617,1615616,3231233,1296.8411371707916,0.00010230326358851016
808809,1617619,1617618,3235237,1298.0839309692383,0.00010080861204642133
809810,1619621,1619620,3239241,1299.7081561088562,9.933571209330694e-05
810811,1621623,1621622,3243245,1301.4576649665833,9.78842464292029e-05
811812,1623625,1623624,3247249,1303.0418558120728,9.645390309742652e-05
812813,1625627,1625626,3251253,1304.65642786026,9.504437457508175e-05
813814,1627629,1627628,3255257,1306.327605009079,9.365535743199871e-05
814815,1629631,1629630,3259261,1307.8896570205688,9.228655289916787e-05
815816,1631633,1631632,3263265,1310.126643896103,9.093766664136638e-05
816817,1633635,1633634,3267269,1312.2132778167725,8.960840875715803e-05
817818,1635637,1635636,3271273,1313.8423500061035,8.829849286939861e-05
818819,1637639,1637638,3275277,1315.543293952942,8.700763760316477e-05
819820,1639641,1639640,3279281,1317.2821400165558,8.573556544888561e-05
820821,1641643,1641642,3283285,1318.780128955841,8.448200264865591e-05
821822,1643645,1643644,3287289,1320.2525088787079,8.324667942360975e-05
822823,1645647,1645646,3291293,1321.7966890335083,8.202933088341524e-05
823824,1647649,1647648,3295297,1323.2708089351654,8.082969452516409e-05
824825,1649651,1649650,3299301,1324.801232099533,7.964751250710833e-05
825826,1651653,1651652,3303305,1326.3721630573273,7.84825308528525e-05
826827,1653655,1653654,3307309,1327.9408581256866,7.733449911029311e-05
827828,1655657,1655656,3311313,1329.4162299633026,7.620317046530545e-05
828829,1657659,1657658,3315317,1330.9128019809723,7.508830140068312e-05
829830,1659661,1659660,3319321,1332.3906757831573,7.398965271931957e-05
830831,1661663,1661662,3323325,1333.8535799980164,7.290698772521864e-05
831832,1663665,1663664,3327329,1335.3884809017181,7.184007404248405e-05
832833,1665667,1665666,3331333,1336.8644618988037,7.078868213739042e-05
833834,1667669,1667668,3335337,1338.3443338871002,6.975258600050438e-05
834835,1669671,1669670,3339341,1339.8374450206757,6.873156303299766e-05
835836,1671673,1671672,3343345,1341.3246159553528,6.772539393296029e-05
836837,1673675,1673674,3347349,1342.7975449562073,6.673386189959274e-05
837838,1675677,1675676,3351353,1344.2859869003296,6.575675422482163e-05
838839,1677679,1677678,3355357,1345.7579708099365,6.479386070168403e-05
839840,1679681,1679680,3359361,1347.2893469333649,6.384497476119577e-05
840841,1681683,1681682,3363365,1348.7530658245087,6.290989222179633e-05
841842,1683685,1683684,3367369,1350.2690329551697,6.19884120851566e-05
842843,1685687,1685686,3371373,1351.7446870803833,6.108033630880527e-05
843844,1687689,1687688,3375377,1353.234512090683,6.018546980612882e-05
844845,1689691,1689690,3379381,1354.6878299713135,5.930362033268466e-05
845846,1691693,1691692,3383385,1356.1617777347565,5.843459848620114e-05
846847,1693695,1693694,3387389,1357.6684441566467,5.757821725183021e-05
847848,1695697,1695696,3391393,1359.1272299289703,5.673429279795528e-05
848849,1697699,1697698,3395397,1360.594969034195,5.5902643680383335e-05
849850,1699701,1699700,3399401,1362.0549519062042,5.5083091524466e-05
850851,1701703,1701702,3403405,1363.524003982544,5.427546000191796e-05
851852,1703705,1703704,3407409,1365.019569158554,5.347957551293803e-05
852853,1705707,1705706,3411413,1366.508148908615,5.2695267186209094e-05
853854,1707709,1707708,3415417,1367.9620220661163,5.192236653783766e-05
854855,1709711,1709710,3419421,1369.4443318843842,5.116070747135382e-05
855856,1711713,1711712,3423425,1370.952998161316,5.041012650508492e-05
856857,1713715,1713714,3427429,1372.4531779289246,4.967046209003456e-05
857858,1715717,1715716,3431433,1373.9150450229645,4.8941555633064127e-05
858859,1717719,1717718,3435437,1375.395026922226,4.822325070108491e-05
859860,1719721,1719720,3439441,1376.8651597499847,4.7515392679997603e-05
860861,1721723,1721722,3443445,1378.4070000648499,4.681782957050018e-05
861862,1723725,1723724,3447449,1379.9049689769745,4.613041153334052e-05
862863,1725727,1725726,3451453,1381.4221527576447,4.545299100300326e-05
863864,1727729,1727728,3455457,1382.8603377342224,4.478542246033612e-05
864865,1729731,1729730,3459461,1384.3347160816193,4.412756254623673e-05
865866,1731733,1731732,3463465,1385.8313629627228,4.347927006165264e-05
866867,1733735,1733734,3467469,1387.3279378414154,4.284040539914713e-05
867868,1735737,1735736,3471473,1388.785562992096,4.2210831907141255e-05
868869,1737739,1737738,3475477,1390.2688879966736,4.159041407092445e-05
869870,1739741,1739740,3479481,1391.715134859085,4.0979018649522914e-05
870871,1741743,1741742,3483485,1393.17950797081,4.0376514448325906e-05
871872,1743745,1743744,3487489,1394.6642599105835,3.9782772091712104e-05
872873,1745747,1745746,3491493,1396.1291718482971,3.919766379567591e-05
873874,1747749,1747748,3495497,1397.6149969100952,3.862106427732215e-05
874875,1749751,1749750,3499501,1399.113177061081,3.805284950431087e-05
875876,1751753,1751752,3503505,1400.6049449443817,3.7492897718038876e-05
876877,1753755,1753754,3507509,1402.0638608932495,3.6941088524145016e-05
877878,1755757,1755756,3511513,1403.5429890155792,3.639730334725755e-05
878879,1757759,1757758,3515517,1405.008817911148,3.5861425772054645e-05
879880,1759761,1759760,3519521,1406.479462146759,3.533334017902234e-05
880881,1761763,1761762,3523525,1407.979481935501,3.481293390450446e-05
881882,1763765,1763764,3527529,1409.6434428691864,3.430009462590533e-05
882883,1765767,1765766,3531533,1411.484699010849,3.3794712408052874e-05
883884,1767769,1767768,3535537,1413.5515389442444,3.329667913476442e-05
884885,1769771,1769770,3539541,1415.3629260063171,3.2805887371978315e-05
885886,1771773,1771772,3543545,1417.0535979270935,3.2322231845682836e-05
886887,1773775,1773774,3547549,1418.89950299263,3.1845608987168816e-05
887888,1775777,1775776,3551553,1420.8304669857025,3.137591625090863e-05
888889,1777779,1777778,3555557,1422.7317538261414,3.0913053137737734e-05
889890,1779781,1779780,3559561,1424.4330179691315,3.0456919830612605e-05
890891,1781783,1781782,3563565,1426.4975008964539,3.000741878622648e-05
891892,1783785,1783784,3567569,1428.2268159389496,2.9564453484454134e-05
892893,1785787,1785786,3571573,1430.4156420230865,2.912792842835188e-05
893894,1787789,1787788,3575577,1432.608125925064,2.8697750508399622e-05
894895,1789791,1789790,3579581,1434.7758378982544,2.8273827183511457e-05
895896,1791793,1791792,3583585,1437.3878519535065,2.7856067163156695e-05
896897,1793795,1793794,3587589,1439.9935519695282,2.7444381089480885e-05
897898,1795797,1795796,3591593,1441.7882459163666,2.7038680741497956e-05
898899,1797799,1797798,3595597,1443.655101776123,2.66388786940297e-05
899900,1799801,1799800,3599601,1445.8020498752594,2.6244889568260987e-05
900901,1801803,1801802,3603605,1447.7065749168396,2.5856628326437203e-05
901902,1803805,1803804,3607609,1450.1367328166962,2.5474011863479973e-05
902903,1805807,1805806,3611613,1451.8983829021454,2.50969582111793e-05
903904,1807809,1807808,3615617,1453.7612237930298,2.4725386424506723e-05
904905,1809811,1809810,3619621,1455.4466898441315,2.435921646792849e-05
905906,1811813,1811812,3623625,1457.2737147808075,2.3998370124900248e-05
906907,1813815,1813814,3627629,1459.1950969696045,2.364276986099867e-05
907908,1815817,1815816,3631633,1461.0484640598297,2.329233905129513e-05
908909,1817819,1817818,3635637,1462.7725780010223,2.2947003117224085e-05
909910,1819821,1819820,3639641,1464.5728459358215,2.2606687252846314e-05
910911,1821823,1821822,3643645,1466.3411450386047,2.2271319039646187e-05
911912,1823825,1823824,3647649,1468.1213910579681,2.194082628648175e-05
912913,1825827,1825826,3651653,1469.8348479270935,2.1615138166453107e-05
913914,1827829,1827828,3655657,1471.501788854599,2.1294184421094542e-05
914915,1829831,1829830,3659661,1473.4300210475922,2.0977896610929747e-05
915916,1831833,1831832,3663665,1475.1637349128723,2.0666206864916603e-05
916917,1833835,1833834,3667669,1477.0059559345245,2.0359048107820854e-05
917918,1835837,1835836,3671673,1478.9961309432983,2.0056354628650297e-05
918919,1837839,1837838,3675677,1480.5535039901733,1.975806117116008e-05
919920,1839841,1839840,3679681,1482.054827928543,1.9464104070721078e-05
920921,1841843,1841842,3683685,1483.614336013794,1.917442011745152e-05
921922,1843845,1843844,3687689,1485.1221470832825,1.8888947238338005e-05
922923,1845847,1845846,3691693,1486.632465839386,1.8607624269861844e-05
923924,1847849,1847848,3695697,1488.2514958381653,1.833039061693853e-05
924925,1849851,1849850,3699701,1489.789640903473,1.805718693503877e-05
925926,1851853,1851852,3703705,1491.274535894394,1.7787954675441142e-05
926927,1853855,1853854,3707709,1492.7660269737244,1.7522635971545242e-05
927928,1855857,1855856,3711713,1494.402529001236,1.726117397993221e-05
928929,1857859,1857858,3715717,1496.004823923111,1.7003512766677886e-05
929930,1859861,1859860,3719721,1497.5203218460083,1.674959662523179e-05
930931,1861863,1861862,3723725,1499.0119609832764,1.6499371554346e-05
931932,1863865,1863864,3727729,1500.5245537757874,1.62527835527726e-05
932933,1865867,1865866,3731733,1502.0019161701202,1.600978009719256e-05
933934,1867869,1867868,3735737,1503.7539639472961,1.577030855060002e-05
934935,1869871,1869870,3739741,1505.3386080265045,1.553431798129168e-05
935936,1871873,1871872,3743745,1506.864744901657,1.530175779862475e-05
936937,1873875,1873874,3747749,1508.3411228656769,1.5072577753016958e-05
937938,1875877,1875876,3751753,1509.8231809139252,1.4846728959128086e-05
938939,1877879,1877878,3755757,1511.507642030716,1.4624162758991588e-05
939940,1879881,1879880,3759761,1513.1447808742523,1.4404831745196134e-05
940941,1881883,1881882,3763765,1515.1914248466492,1.418868873770407e-05
941942,1883885,1883884,3767769,1516.7725749015808,1.3975687238598766e-05
942943,1885887,1885886,3771773,1518.4249818325043,1.3765781886831974e-05
943944,1887889,1887888,3775777,1519.9867010116577,1.3558927207668603e-05
944945,1889891,1889890,3779781,1521.6185750961304,1.3355079204302456e-05
945946,1891893,1891892,3783785,1523.4909060001373,1.315419410730101e-05
946947,1893895,1893894,3787789,1525.1843528747559,1.2956228601979092e-05
947948,1895897,1895896,3791793,1526.7677628993988,1.276114039683307e-05
948949,1897899,1897898,3795797,1528.5656139850616,1.2568888109854015e-05
949950,1899901,1899900,3799801,1530.2737839221954,1.237942956322513e-05
950951,1901903,1901902,3803805,1531.8696899414062,1.2192724966553214e-05
951952,1903905,1903904,3807809,1533.361788034439,1.2008733961010876e-05
952953,1905907,1905906,3811813,1534.8970580101013,1.182741686989175e-05
953954,1907909,1907908,3815817,1536.4033398628235,1.1648735153357848e-05
954955,1909911,1909910,3819821,1537.8795640468597,1.1472650498944859e-05
955956,1911913,1911912,3823825,1539.3513669967651,1.1299124821562145e-05
956957,1913915,1913914,3827829,1540.8749599456787,1.1128121172987449e-05
957958,1915917,1915916,3831833,1542.9959218502045,1.0959602946059022e-05
958959,1917919,1917918,3835837,1544.4957098960876,1.0793533760988794e-05
959960,1919921,1919920,3839841,1545.997329711914,1.0629878374857071e-05
960961,1921923,1921922,3843845,1547.4839498996735,1.0468601317370485e-05
961962,1923925,1923924,3847849,1549.0703799724579,1.0309668141417205e-05
962963,1925927,1925926,3851853,1550.6637721061707,1.0153044968319591e-05
963964,1927929,1927928,3855857,1552.1954097747803,9.998697805713164e-06
964965,1929931,1929930,3859861,1553.9368197917938,9.84659391178866e-06
965966,1931933,1931932,3863865,1555.8108568191528,9.696700658423651e-06
966967,1933935,1933934,3867869,1557.610366821289,9.54898564486939e-06
967968,1935937,1935936,3871873,1559.2241530418396,9.403417607245501e-06
968969,1937939,1937938,3875877,1560.7563989162445,9.259964713237423e-06
969970,1939941,1939940,3879881,1562.2928581237793,9.118596949519997e-06
970971,1941943,1941942,3883885,1563.8049409389496,8.979283620647038e-06
971972,1943945,1943944,3887889,1565.3481130599976,8.841994826980226e-06
972973,1945947,1945946,3891893,1566.8839600086212,8.706701237315428e-06
973974,1947949,1947948,3895897,1568.3782880306244,8.573373747822188e-06
974975,1949951,1949950,3899901,1569.8461270332336,8.441984050477913e-06
975976,1951953,1951952,3903905,1571.332997083664,8.312503496199497e-06
976977,1953955,1953954,3907909,1572.8247969150543,8.184904800145887e-06
977978,1955957,1955956,3911913,1574.3030829429626,8.059160336415516e-06
978979,1957959,1957958,3915917,1575.8027210235596,7.935243274914683e-06
979980,1959961,1959960,3919921,1577.2860589027405,7.81312701292336e-06
980981,1961963,1961962,3923925,1578.7963848114014,7.692785402468871e-06
981982,1963965,1963964,3927929,1580.2737619876862,7.574192409265379e-06
982983,1965967,1965966,3931933,1581.7904689311981,7.457322908521746e-06
983984,1967969,1967968,3935937,1583.3085758686066,7.3421518891336746e-06
984985,1969971,1969970,3939941,1584.7897918224335,7.228654339996865e-06
985986,1971973,1971972,3943945,1586.2635250091553,7.116806273188558e-06
986987,1973975,1973974,3947949,1587.7530798912048,7.00658347341232e-06
987988,1975977,1975976,3951953,1589.26691198349,6.897962521179579e-06
988989,1977979,1977978,3955957,1590.8007128238678,6.7909198833149276e-06
989990,1979981,1979980,3959961,1592.2923929691315,6.6854329361376585e-06
990991,1981983,1981982,3963965,1593.7760949134827,6.581478714906552e-06
991992,1983985,1983984,3967969,1595.2771549224854,6.479035164375091e-06
992993,1985987,1985986,3971973,1596.7735741138458,6.378080342983594e-06
993994,1987989,1987988,3975977,1598.2848460674286,6.278592422859219e-06
994995,1989991,1989990,3979981,1599.7650439739227,6.180550144563313e-06
995996,1991993,1991992,3983985,1601.247636795044,6.083932703404571e-06
996997,1993995,1993994,3987989,1602.7304220199585,5.988719067318016e-06
997998,1995997,1995996,3991993,1604.2101349830627,5.894889341107046e-06
998999,1997999,1997998,3995997,1605.7003049850464,5.8024224927066825e-06
1000000,2000001,2000000,4000001,1607.2158608436584,5.71129987747554e-06


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0009839534759521484,2181.2938132599165
1001,2003,2002,4005,1.6696579456329346,60.24885261358577
2002,4005,4004,8009,3.163712978363037,53.77859451869858
3003,6007,6006,12013,4.62731409072876,50.92243883003266
4004,8009,8008,16017,6.096297025680542,48.68494381511141
5005,10011,10010,20021,7.580941915512085,46.691969112691595
6006,12013,12012,24025,9.183863878250122,44.867160963980496
7007,14015,14014,28029,10.767898082733154,43.181007680888115
8008,16017,16016,32033,12.238910913467407,41.61577992971229
9009,18019,18018,36037,13.820996046066284,40.15858680114866
10010,20021,20020,40041,15.4914391040802,38.79909674755504
11011,22023,22022,44045,17.152826070785522,37.52847409324636
12012,24025,24024,48049,18.724649906158447,36.33883035729923
13013,26027,26026,52053,20.533782958984375,35.2229502662276
14014,28029,28028,56057,23.683632135391235,34.1741690618162
15015,30031,30030,60061,26.24609398841858,33.18632746839512
16016,32033,32032,64065,28.800775051116943,32.25376010823106
17017,34035,34034,68069,33.07889199256897,31.37129247508051
18018,36037,36036,72073,35.663373947143555,30.53423417371664
19019,38039,38038,76077,37.959240198135376,29.738363873788558
20020,40041,40040,80081,40.03615880012512,28.979905736756564
21021,42043,42042,84085,41.761090993881226,28.25549911295866
22022,44045,44044,88089,43.41641116142273,27.562163962825935
23023,46047,46046,92093,45.28204679489136,26.89726436380988
24024,48049,48048,96097,47.56490993499756,26.258472033869566
25025,50051,50050,100101,49.6177818775177,25.643731276923745
26026,52053,52052,104105,51.827003955841064,25.051226263215085
27027,54055,54054,108109,53.89559483528137,24.479351152850313
28028,56057,56056,112113,55.691056966781616,23.926683266755163
29029,58059,58058,116117,57.354275941848755,23.39195929771222
30030,60061,60060,120121,59.27090501785278,22.874054418249216
31031,62063,62062,124125,60.738879919052124,22.371964063629093
32032,64065,64064,128129,62.19211792945862,21.884788130571906
33033,66067,66066,132133,63.73110294342041,21.411717322285085
34034,68069,68068,136137,65.61202192306519,20.952021377713663
35035,70071,70070,140141,67.58785915374756,20.50503894039116
36036,72073,72072,144145,69.29348587989807,20.07016884483687
37037,74075,74074,148149,71.3541350364685,19.64686262284613
38038,76077,76076,152153,72.82718992233276,19.234618056184672
39039,78079,78078,156157,75.12943410873413,18.83297362496819
40040,80081,80080,160161,77.26256799697876,18.441503721751815
41041,82083,82082,164165,79.28955101966858,18.05989871991801
42042,84085,84084,168169,81.48197388648987,17.687711314216813
43043,86087,86086,172173,83.38214206695557,17.324595528035616
44044,88089,88088,176177,85.22617602348328,16.970233388048655
45045,90091,90090,180181,87.12790012359619,16.624327017803125
46046,92093,92092,184185,88.88261008262634,16.286596591251737
47047,94095,94094,188189,90.73016595840454,15.956778552026663
48048,96097,96096,192193,92.43196105957031,15.634624055713857
49049,98099,98098,196197,94.17009615898132,15.319897603406503
50050,100101,100100,200201,95.90395998954773,15.012375840133245
51051,102103,102102,204205,97.52496290206909,14.711846495718419
52052,104105,104104,208209,99.13337111473083,14.41810744892257
53053,106107,106106,212213,100.94622302055359,14.130965898484192
54054,108109,108108,216217,102.57635283470154,13.850237627052593
55055,110111,110110,220221,104.16241908073425,13.575746345965399
56056,112113,112112,224225,105.95493006706238,13.307323110548623
57057,114115,114114,228229,107.89903998374939,13.04480579704034
58058,116117,116116,232233,110.09079313278198,12.7880386334582
59059,118119,118118,236237,111.93464493751526,12.53687177778204
60060,120121,120120,240241,113.83798384666443,12.29116093771006
61061,122123,122122,244245,115.77823305130005,12.05076702700751
62062,124125,124124,248249,118.05190801620483,11.815555854122408
63063,126127,126126,252253,119.99100995063782,11.585397839303027
64064,128129,128128,256257,121.97187304496765,11.360167756933265
65065,130131,130130,260261,123.87839818000793,11.139744500219308
66066,132133,132132,264265,125.80260181427002,10.924010865721812
67067,134135,134134,268269,127.77046489715576,10.71285335553739
68068,136137,136136,272273,130.0548231601715,10.506161995206185
69069,138139,138138,276277,132.1311650276184,10.303830165656109
70070,140141,140140,280281,133.686420917511,10.105754447699951
71071,142143,142142,284285,135.21967196464539,9.911834477786101
72072,144145,144144,288289,136.73435997962952,9.721972813853085
73073,146147,146146,292293,138.29225420951843,9.536074810285413
74074,148149,148148,296297,139.75850582122803,9.354048501084549
75075,150151,150150,300301,141.22966694831848,9.175804490479663
76076,152153,152152,304305,142.67782282829285,9.001255850295024
77077,154155,154154,308309,144.1162040233612,8.83031802347898
78078,156157,156156,312313,145.59844708442688,8.662908733267386
79079,158159,158158,316317,147.1055290699005,8.498947897522385
80080,160161,160160,320321,149.5407431125641,8.338357547842861
81081,162163,162162,324325,151.11949396133423,8.181061753091512
82082,164165,164164,328329,152.829745054245,8.026986547022261
83083,166167,166166,332333,154.31337094306946,7.876059859733232
84084,168169,168168,336337,155.8827109336853,7.728211452692335
85085,170171,170170,340341,157.418527841568,7.583372857113432
86086,172173,172172,344345,158.95857906341553,7.441477315476504
87087,174175,174174,348349,160.39903807640076,7.302459726004599
88088,176177,176176,352353,161.83521509170532,7.166256589919158
89089,178179,178178,356357,163.3163230419159,7.032805961311624
90090,180181,180180,360361,165.3139591217041,6.902047399468074
91091,182183,182182,364365,166.83787989616394,6.773921923503281
92092,184185,184184,368369,168.6047878265381,6.64837196915289
93093,186187,186186,372373,170.0907051563263,6.525341347589574
94094,188189,188188,376377,172.08157515525818,6.404775206126601
95095,190191,190190,380381,173.73494601249695,6.286619990683107
96096,192193,192192,384385,175.29993414878845,6.170823409888385
97097,194195,194194,388389,176.77869510650635,6.057334400709124
98098,196197,196196,392393,178.56967210769653,5.9461030954939815
99099,198199,198198,396397,180.102303981781,5.837080790330106
100100,200201,200200,400401,182.4148828983307,5.730219914621898
101101,202203,202202,404405,184.00730800628662,5.625474001799489
102102,204205,204204,408409,185.44154524803162,5.522797661083928
103103,206207,206206,412413,186.90417098999023,5.422146550230082
104104,208209,208208,416417,188.3450710773468,5.3234773491861915
105105,210211,210210,420421,189.9736499786377,5.226747734608239
106106,212213,212212,424425,191.66082406044006,5.13191635517444
107107,214215,214214,428429,193.21473288536072,5.038942807655303
108108,216217,216216,432433,194.71286392211914,4.947787613692412
109109,218219,218218,436437,196.14271807670593,4.858412197248072
110110,220221,220220,440441,197.6390199661255,4.770778862692964
111111,222223,222222,444445,199.1283299922943,4.684850773497942
112112,224225,224224,448449,200.55268812179565,4.600591931503573
113113,226227,226226,452453,202.03079199790955,4.517967156740497
114114,228229,228228,456457,203.4871039390564,4.436942067780137
115115,230231,230230,460461,205.2219340801239,4.357483062592337
116116,232233,232232,464465,207.0720920562744,4.279557299893895
117117,234235,234234,468469,208.4624490737915,4.203132680966178
118118,236237,236236,472473,210.04730415344238,4.128177831932135
119119,238239,238238,476477,212.11453199386597,4.054662086471467
120120,240241,240240,480481,214.04526710510254,3.9825554689664386
121121,242243,242242,484485,215.4211459159851,3.9118286780598055
122122,244245,244244,488489,216.66057801246643,3.8424530706188307
123123,246247,246246,492493,219.16006803512573,3.7744006460890205
124124,248249,248248,496497,220.7719509601593,3.707644031230302
125125,250251,250250,500501,222.6248300075531,3.6421564652243887
126126,252253,252252,504505,225.8530468940735,3.5779117851444653
127127,254255,254254,508509,227.52686715126038,3.514884411777075
128128,256257,256256,512513,229.13877391815186,3.4530493357879095
129129,258259,258258,516517,230.9864330291748,3.392382104223998
130130,260261,260260,520521,232.8015341758728,3.3328588073426317
131131,262263,262262,524525,234.53265190124512,3.274456065760205
132132,264265,264264,528529,237.09429502487183,3.2171510179119878
133133,266267,266266,532533,239.28882503509521,3.1609213078180574
134134,268269,268268,536537,241.07564616203308,3.1057450731461813
135135,270271,270270,540541,242.73439502716064,3.051600933563236
136136,272273,272272,544545,244.28627490997314,2.998467979372208
137137,274275,274274,548549,245.80334305763245,2.94632576042477
138138,276277,276276,552553,247.29093503952026,2.895154275304776
139139,278279,278278,556557,248.88128995895386,2.844933960773915
140140,280281,280280,560561,250.40132904052734,2.795645681476799
141141,282283,282282,564565,251.88988995552063,2.7472707198971875
142142,284285,284284,568569,253.35518598556519,2.6997907665570438
143143,286287,286286,572573,254.90525007247925,2.6531879104605878
144144,288289,288288,576577,256.31336402893066,2.6074446297644727
145145,290291,290290,580581,257.7615761756897,2.5625437826835196
146146,292293,292292,584585,259.1866829395294,2.5184685986150726
147147,294295,294294,588589,260.608873128891,2.475202669481064
148148,296297,296296,592593,262.13785004615784,2.432729941282787
149149,298299,298298,596597,263.67859506607056,2.3910347058625803
150150,300301,300300,600601,265.21803092956543,2.350101592866622
151151,302303,302302,604605,266.75970005989075,2.309915561904859
152152,304305,304304,608609,268.63935804367065,2.2704618949030646
153153,306307,306306,612613,270.14275002479553,2.231726188642824
154154,308309,308308,616617,271.55128598213196,2.193694347482392
155155,310311,310310,620621,272.97471499443054,2.1563525762577456
156156,312313,312312,624625,274.6565852165222,2.119687373355873
157157,314315,314314,628629,276.13836097717285,2.0836855239583656
158158,316317,316316,632633,278.0097289085388,2.048334093449739
159159,318319,318318,636637,280.2850179672241,2.0136204209876496
160160,320321,320320,640641,282.0237910747528,1.9795321132280606
161161,322323,322322,644645,283.4800832271576,1.9460570382061633
162162,324325,324324,648649,284.91242694854736,1.9131833193656576
163163,326327,326326,652653,286.3386940956116,1.8808993297316192
164164,328329,328328,656657,288.0149040222168,1.8491936862288867
165165,330331,330330,660661,290.1029438972473,1.8180552441358486
166166,332333,332332,664665,292.3770809173584,1.7874730916739736
167167,334335,334334,668669,294.1020550727844,1.7574365447288756
168168,336337,336336,672673,295.7968502044678,1.7279351416999589
169169,338339,338338,676677,297.94375491142273,1.6989586384734139
170170,340341,340340,680681,299.9653389453888,1.6704970035186761
171171,342343,342342,684685,301.5440249443054,1.64254041310312
172172,344345,344344,688689,303.13552594184875,1.6150792466210078
173173,346347,346346,692693,304.6358880996704,1.5881040820366934
174174,348349,348348,696697,306.5122961997986,1.5616056914379897
175175,350351,350350,700701,308.1090998649597,1.5355750366945813
176176,352353,352352,704705,309.8981499671936,1.5100032652231903
177177,354355,354354,708709,312.41674304008484,1.484881705852672
178178,356357,356356,712713,314.35854601860046,1.460201864789724
179179,358359,358358,716717,315.8666977882385,1.4359554216796369
180180,360361,360360,720721,317.7357540130615,1.412134225763566
181181,362363,362362,724725,319.356586933136,1.3887302921250466
182182,364365,364364,728729,321.00889587402344,1.3657357980270035
183183,366367,366366,732733,322.57368302345276,1.343143079338006
184184,368369,368368,736737,324.13319993019104,1.3209446270398075
185185,370371,370370,740741,325.6753680706024,1.29913308382163
186186,372373,372372,744745,327.37358713150024,1.277701240752208
187187,374375,374374,748749,328.9097800254822,1.2566420340319837
188188,376377,376376,752753,330.46217584609985,1.235948541822836
189189,378379,378378,756757,332.12954902648926,1.2156139811509092
190190,380381,380380,760761,333.7189300060272,1.1956317048839082
191191,382383,382382,764765,335.3153929710388,1.1759951987791055
192192,384385,384384,768769,336.94352197647095,1.1566980785999021
193193,386387,386386,772773,338.43749499320984,1.137734087301169
194194,388389,388388,776777,339.8766419887543,1.1190970922805263
195195,390391,390390,780781,341.2344710826874,1.1007810826930609
196196,392393,392392,784785,342.53058409690857,1.0827801668285701
197197,394395,394394,788789,343.8428809642792,1.0650885695516763
198198,396397,396396,792793,345.1029019355774,1.0477006297995786
199199,398399,398398,796797,346.41079807281494,1.0306107981385821
200200,400401,400400,800801,347.74329113960266,1.0138136343782662
201201,402403,402402,804805,349.0555281639099,0.99730380523863
202202,404405,404404,808809,350.77065992355347,0.9810760820740825
203203,406407,406406,812813,352.4964859485626,0.9651253386472263
204204,408409,408408,816817,354.17509484291077,0.9494465489558479
205205,410411,410410,820821,356.0206320285797,0.9340347851087927
206206,412413,412412,824825,357.8198239803314,0.9188852152507252
207207,414415,414414,828829,359.66778206825256,0.9039931015354341
208208,416417,416416,832833,361.4510099887848,0.8893537981438158
209209,418419,418418,836837,363.2014911174774,0.8749627493481285
210210,420421,420420,840841,364.94093894958496,0.860815487621494
211211,422423,422422,844845,366.6757228374481,0.8469076317869622
212212,424425,424424,848849,368.6792092323303,0.8332348852131872
213213,426427,426426,852853,370.2458710670471,0.819793034046711
214214,428429,428428,856857,371.8934509754181,0.80657794548722
215215,430431,430430,860861,373.462033033371,0.7935855661008873
216216,432433,432432,864865,375.11010098457336,0.7808119201708905
217217,434435,434434,868869,376.93531107902527,0.7682531080861281
218218,436437,436436,872873,378.54048919677734,0.7559053047658608
219219,438439,438438,876877,380.1064670085907,0.7437647581198235
220220,440441,440440,880881,381.7310380935669,0.7318277875419881
221221,442443,442442,884885,383.29565620422363,0.7200907824393425
222222,444445,444444,888889,384.830952167511,0.7085502007923878
223223,446447,446446,892893,386.39608502388,0.6972025677483771
224224,448449,448448,896897,387.9812870025635,0.6860444742450227
225225,450451,450450,900901,389.8032958507538,0.6750725756654674
226226,452453,452452,904905,391.34513306617737,0.6642835905234961
227227,454455,454454,908909,393.08430004119873,0.6536742991762594
228228,456457,456456,912913,394.7148640155792,0.6432415425667841
229229,458459,458458,916917,396.19312596321106,0.6329822209938811
230230,460461,460460,920921,397.7707030773163,0.6228932929084294
231231,462463,462462,924925,399.29266905784607,0.6129717737373994
232232,464465,464464,928929,401.29933404922485,0.6032147347319778
233233,466467,466466,932933,403.229159116745,0.5936193018420681
234234,468469,468468,936937,405.00232911109924,0.5841826546159155
235235,470471,470470,940941,406.90173411369324,0.5749020251213324
236236,472473,472472,944945,408.5433487892151,0.5657746968934134
237237,474475,474474,948949,410.01588702201843,0.5567980039025997
238238,476477,476476,952953,411.4559841156006,0.5479693295466177
239239,478479,478478,956957,412.91487407684326,0.5392861056643596
240240,480481,480480,960961,414.3854429721832,0.5307458115685222
241241,482483,482482,964965,415.81877398490906,0.5223459731035973
242242,484485,484484,968969,417.26158809661865,0.5140841617194383
243243,486487,486486,972973,418.70071601867676,0.5059579935683587
244244,488489,488488,976977,420.20594906806946,0.49796512861928477
245245,490491,490490,980981,421.7397108078003,0.4901032697921437
246246,492493,492492,984985,423.23574209213257,0.48237016211021455
247247,494495,494494,988989,424.8937478065491,0.4747635918703281
248248,496497,496496,992993,426.5734930038452,0.46728138583216605
249249,498499,498498,996997,428.159282207489,0.45992141042222556
250250,500501,500500,1001001,429.7604720592499,0.4526815709575658
251251,502503,502502,1005005,431.52616691589355,0.44555981088353747
252252,504505,504504,1009009,433.17100405693054,0.4385541110293616
253253,506507,506506,1013013,434.68461513519287,0.43166248887848724
254254,508509,508508,1017017,436.2947781085968,0.4248829978549793
255255,510511,510510,1021021,437.92327213287354,0.41821372662400336
256256,512513,512512,1025025,439.5201289653778,0.411652798407772
257257,514515,514514,1029029,440.9994468688965,0.4051983703160431
258258,516517,516516,1033033,442.63205909729004,0.3988486326893508
259259,518519,518518,1037037,444.43250799179077,0.3926018084574707
260260,520521,520520,1041041,446.0130658149719,0.3864561525105046
261261,522523,522522,1045045,447.52954506874084,0.38040995108281095
262262,524525,524524,1049049,449.13062596321106,0.37446152115069253
263263,526527,526526,1053053,450.8875710964203,0.3686092098409972
264264,528529,528528,1057057,452.4840760231018,0.36285139385404364
265265,530531,530530,1061061,454.1752419471741,0.357186478896665
266266,532533,532532,1065065,455.85459184646606,0.35161289912787197
267267,534535,534534,1069069,457.6705560684204,0.3461291166159981
268268,536537,536536,1073073,459.33516693115234,0.34073362080619063
269269,538539,538538,1077077,461.1102559566498,0.33542492800006585
270270,540541,540540,1081081,463.0643298625946,0.33020158084468676
271271,542543,542542,1085085,464.5750410556793,0.3250621478332505
272272,544545,544544,1089089,466.03645610809326,0.32000522281487065
273273,546547,546546,1093093,467.6741669178009,0.31502942451572835
274274,548549,548548,1097097,469.3930480480194,0.3101333960685224
275275,550551,550550,1101101,470.95694398880005,0.305315804551924
276276,552553,552552,1105105,472.3938479423523,0.3005753405401492
277277,554555,554554,1109109,473.80244398117065,0.29591071766071764
278278,556557,556556,1113113,475.17788887023926,0.2913206721618735
279279,558559,558558,1117117,476.5411071777344,0.286803962487852
280280,560561,560560,1121121,477.88575410842896,0.2823593688640358
281281,562563,562562,1125125,479.22669506073,0.2779856928882509
282282,564565,564564,1129129,480.61730694770813,0.27368175713434084
283283,566567,566566,1133133,482.1757779121399,0.2694464047575593
284284,568569,568568,1137137,483.75297713279724,0.2652784991145154
285285,570571,570570,1141141,485.3954339027405,0.26117692338573306
286286,572573,572572,1145145,487.31657791137695,0.2571405802082154
287287,574575,574574,1149149,488.94406485557556,0.25316839131471625
288288,576577,576576,1153153,490.4817090034485,0.24925929718017414
289289,578579,578578,1157157,492.12048506736755,0.2454122566754222
290290,580581,580580,1161161,493.83285999298096,0.24162624672635502
291291,582583,582582,1165165,495.8299889564514,0.23790026198321357
292292,584585,584584,1169169,497.68215322494507,0.23423331449180296
293293,586587,586586,1173173,499.38504219055176,0.23062443337573768
294294,588589,588588,1177177,501.8713300228119,0.22707266452164276
295295,590591,590590,1181181,503.52168583869934,0.2235770702712898
296296,592593,592592,1185185,505.22984409332275,0.22013672912214588
297297,594595,594594,1189189,506.9760990142822,0.2167507354299687
298298,596597,596596,1193193,508.6503999233246,0.21341819912038318
299299,598599,598598,1197197,510.3311870098114,0.21013824540432324
300300,600601,600600,1201201,511.8785240650177,0.20691001449984014
301301,602603,602602,1205205,513.5470499992371,0.20373266135857193
302302,604605,604604,1209209,515.0871589183807,0.20060535539880675
303303,606607,606606,1213213,516.7402820587158,0.19752728024297994
304304,608609,608608,1217217,518.3992919921875,0.19449763345937754
305305,610611,610610,1221221,520.1949229240417,0.19151562631088836
306306,612613,612612,1225225,521.9581279754639,0.18858048350625722
307307,614615,614614,1229229,523.4217681884766,0.18569144295884144
308308,616617,616616,1233233,524.8570930957794,0.18284775554730004
309309,618619,618618,1237237,526.2965159416199,0.18004868488264947
310310,620621,620620,1241241,527.777557849884,0.17729350707929825
311311,622623,622622,1245245,529.2083430290222,0.1745815105307429
312312,624625,624624,1249249,530.6974198818207,0.17191199568833326
313313,626627,626626,1253253,532.1526761054993,0.16928427484674557
314314,628629,628628,1257257,533.6883990764618,0.1666976719309332
315315,630631,630630,1261261,535.125,0.16415152228807983
316316,632633,632632,1265265,536.5987901687622,0.16164517248546417
317317,634635,634634,1269269,538.0160109996796,0.15917798010809747
318318,636637,636636,1273273,539.5131828784943,0.1567493135642053
319319,638639,638638,1277277,541.0694680213928,0.1543585518920736
320320,640641,640640,1281281,542.6053149700165,0.15200508457144224
321321,642643,642642,1285285,544.2889561653137,0.14968831133785443
322322,644645,644644,1289289,545.986964225769,0.14740764200178091
323323,646647,646646,1293293,547.6532771587372,0.14516249626922217
324324,648649,648648,1297297,549.3766748905182,0.14295230356788124
325325,650651,650650,1301301,550.9445478916168,0.14077650287424603
326326,652653,652652,1305305,552.4848330020905,0.13863454254658336
327327,654655,654654,1309309,553.9793000221252,0.13652588015827405
328328,656657,656656,1313313,555.4910790920258,0.13444998233683236
329329,658659,658658,1317317,557.0482621192932,0.13240632460349389
330330,660661,660660,1321321,558.472804069519,0.1303943912188288
331331,662663,662662,1325325,559.9250028133392,0.12841367502767298
332332,664665,664664,1329329,561.3666439056396,0.12646367731008468
333333,666667,666666,1333333,562.7959489822388,0.12454390763298306
334334,668669,668668,1337337,564.2064440250397,0.1226538837059934
335335,670671,670670,1341341,565.6534790992737,0.12079313123842894
336336,672673,672672,1345345,567.1709840297699,0.118961183800252
337337,674675,674674,1349349,568.6026740074158,0.117157582685536
338338,676677,676676,1353353,570.0475978851318,0.11538187677740552
339339,678679,678678,1357357,571.4838471412659,0.11363362241672803
340340,680681,680680,1361361,572.9574601650238,0.11191238327194242
341341,682683,682682,1365365,574.4048690795898,0.11021773021286663
342342,684685,684684,1369369,575.8666501045227,0.10854924118461895
343343,686687,686686,1373373,577.3488941192627,0.10690650108722366
344344,688689,688688,1377377,578.797091960907,0.1052891016530566
345345,690691,690690,1381381,580.2893621921539,0.10369664133042988
346346,692693,692692,1385385,581.8208889961243,0.1021287251674039
347347,694695,694694,1389389,583.3374769687653,0.10058496469798683
348348,696697,696696,1393393,584.8461689949036,0.09906497782992574
349349,698699,698698,1397397,586.4084389209747,0.09756838873602192
350350,700701,700700,1401401,587.9082269668579,0.09609482774612843
351351,702703,702702,1405405,589.3546249866486,0.09464393124153503
352352,704705,704704,1409409,590.8081498146057,0.09321534155037625
353353,706707,706706,1413413,592.2702281475067,0.09180870684758702
354354,708709,708708,1417417,593.770182132721,0.09042368105338028
355355,710711,710710,1421421,595.2783370018005,0.08905992373559002
356356,712713,712712,1425425,596.7645599842072,0.08771710001315114
357357,714715,714714,1429429,598.492458820343,0.08639488046162569
358358,716717,716716,1433433,600.0350000858307,0.08509294101952491
359359,718719,718718,1437437,601.4958040714264,0.08381096289792822
360360,720721,720720,1441441,602.945139169693,0.08254863249078426
361361,722723,722722,1445445,604.3713519573212,0.08130564128532569
362362,724725,724724,1449449,605.8207380771637,0.08008168577828201
363363,726727,726726,1453453,607.2572090625763,0.07887646738856802
364364,728729,728728,1457457,608.762629032135,0.07768969237451984
365365,730731,730730,1461461,610.3029429912567,0.07652107175306355
366366,732733,732732,1465465,611.8888008594513,0.07537032121763332
367367,734735,734734,1469469,613.6215999126434,0.07423716106063694
368368,736737,736736,1473473,615.3494729995728,0.07312131609421613
369369,738739,738738,1477477,616.9775190353394,0.07202251557657746
370370,740741,740740,1481481,618.5902388095856,0.0709404931338895
371371,742743,742742,1485485,620.2123072147369,0.0698749866895696
372372,744745,744744,1489489,621.6367220878601,0.06882573839016004
373373,746747,746746,1493493,623.0945010185242,0.06779249453552438
374374,748749,748748,1497497,624.5372588634491,0.06677500550847526
375375,750751,750750,1501501,626.0132751464844,0.06577302570667598
376376,752753,752752,1505505,627.4589359760284,0.06478631347522423
377377,754755,754754,1509509,628.8710279464722,0.06381463104060003
378378,756757,756756,1513513,630.3584260940552,0.06285774444563685
379379,758759,758758,1517517,631.9238178730011,0.061915423486425425
380380,760761,760760,1521521,633.4860048294067,0.06098744164864911
381381,762763,762762,1525525,635.161367893219,0.0600735760463067
382382,764765,764764,1529529,636.6593909263611,0.059173607362026814
383383,766767,766766,1533533,638.1915829181671,0.058287319787154956
384384,768769,768768,1537537,639.6464040279388,0.05741450096252265
385385,770771,770770,1541541,641.0625400543213,0.05655494192308197
386386,772773,772772,1545545,642.5540599822998,0.055708437039356795
387387,774775,774774,1549549,643.9835119247437,0.05487478396366896
388388,776777,776776,1553553,645.4862229824066,0.05405378357488644
389389,778779,778778,1557557,646.9780042171478,0.05324523992567265
390390,780781,780780,1561561,648.4641110897064,0.05244896018916734
391391,782783,782782,1565565,649.9340319633484,0.051664754608054864
392392,784785,784784,1569569,651.3830277919769,0.05089243644351882
393393,786787,786786,1573573,652.8975739479065,0.05013182192499244
394394,788789,788788,1577577,654.3818590641022,0.04938273020229644
395395,790791,790790,1581581,655.9312360286713,0.048644983296867395
396396,792793,792792,1585585,657.401789188385,0.04791840605378184
397397,794795,794794,1589589,658.8330299854279,0.04720282609673632
398398,796797,796796,1593593,660.2873740196228,0.04649807378098103
399399,798799,798798,1597597,661.7559909820557,0.04580398214955039
400400,800801,800800,1601601,663.2076749801636,0.04512038688824305
401401,802803,802802,1605605,664.6898150444031,0.0444471262829893
402402,804805,804804,1609609,666.1517980098724,0.04378404117642276
403403,806807,806806,1613613,667.6000380516052,0.04313097492718043
404404,808809,808808,1617617,669.0415840148926,0.04248777336749754
405405,810811,810810,1621621,670.4828510284424,0.04185428476341713
406406,812813,812812,1625625,671.9608948230743,0.041230359774772296
407407,814815,814814,1629629,673.3998591899872,0.040615851416646365
408408,816817,816816,1633633,674.8461050987244,0.040010615019923534
409409,818819,818818,1637637,676.3115549087524,0.03941450819479542
410410,820821,820820,1641641,677.8078439235687,0.03882739079244857
411411,822823,822822,1645645,679.2971251010895,0.03824912486879839
412412,824825,824824,1649649,680.7185609340668,0.0376795746501557
413413,826827,826826,1653653,682.1737430095673,0.03711860649514165
414414,828829,828828,1657657,683.6113698482513,0.036566088862855395
415415,830831,830830,1661661,685.0468828678131,0.036021892276608014
416416,832833,832832,1665665,686.570060968399,0.03548588929231755
417417,834835,834834,1669669,689.2098321914673,0.03495795446349348
418418,836837,836836,1673673,690.9753849506378,0.034437964310995994
419419,838839,838838,1677677,692.6462140083313,0.03392579728972578
420420,840841,840840,1681681,694.4051649570465,0.03342133375770118
421421,842843,842842,1685685,696.1382439136505,0.032924455945590125
422422,844845,844844,1689689,697.6633570194244,0.03243504792646945
423423,846847,846846,1693693,699.1464660167694,0.03195299558547049
424424,848849,848848,1697697,700.6245868206024,0.03147818659147106
425425,850851,850850,1701701,702.0994689464569,0.03101051036719582
426426,852853,852852,1705705,703.6021540164948,0.030549858062272506
427427,854855,854854,1709709,705.0634100437164,0.030096122524582825
428428,856857,856856,1713713,706.6144869327545,0.029649198272750255
429429,858859,858858,1717717,708.2113530635834,0.02920898147021944
430430,860861,860860,1721721,709.878662109375,0.028775369898085046
431431,862863,862862,1725725,711.452586889267,0.028348262929171142
432432,864865,864864,1729729,713.1466720104218,0.02792756150279274
433433,866867,866866,1733733,714.6638031005859,0.027513168099631002
434434,868869,868868,1737737,716.1408429145813,0.027104986716722124
435435,870871,870870,1741741,717.582967042923,0.026702922843355736
436436,872873,872872,1745745,719.0356919765472,0.026306883437200668
437437,874875,874874,1749749,720.524374961853,0.025916776900885452
438438,876877,876876,1753753,722.0119321346283,0.025532513058919903
439439,878879,878878,1757757,723.4512269496918,0.025154003134503
440440,880881,880880,1761761,724.9574339389801,0.024781159728036073
441441,882883,882882,1765765,726.4278008937836,0.024413896794840184
442442,884885,884884,1769769,727.913323879242,0.024052129622873508
443443,886887,886886,1773773,729.430125951767,0.02369577481260876
444444,888889,888888,1777777,730.9219810962677,0.02334475025475058
445445,890891,890890,1781781,732.3799939155579,0.02299897511193194
446446,892893,892892,1785785,733.8626580238342,0.022658369795408362
447447,894895,894894,1789789,735.300201177597,0.022322855948686993
448448,896897,896896,1793793,736.772381067276,0.021992356424334503
449449,898899,898898,1797797,738.234601020813,0.021666795268288297
450450,900901,900900,1801801,739.7017419338226,0.02134609769814233
451451,902903,902902,1805805,741.2144930362701,0.02103019008609408
452452,904905,904904,1809809,742.6780059337616,0.020718999940072536
453453,906907,906906,1813813,744.1905798912048,0.020412455886003045
454454,908909,908908,1817817,745.6756520271301,0.020110487650072173
455455,910911,910910,1821821,747.149729013443,0.019813026041333615
456456,912913,912912,1825825,748.6158480644226,0.01952000293420042
457457,914915,914914,1829829,750.1117749214172,0.01923135125218778
458458,916917,916916,1833833,751.6019570827484,0.018947004950973678
459459,918919,918918,1837837,753.070004940033,0.018666899002369064
460460,920921,920920,1841841,754.5317118167877,0.018390969378174304
461461,922923,922922,1845845,755.9819691181183,0.01811915303414935
462462,924925,924924,1849849,757.4750790596008,0.017851387894552317
463463,926927,926926,1853853,758.9985311031342,0.017587612837587585
464464,928929,928928,1857857,760.4652781486511,0.017327767679944373
465465,930931,930930,1861861,761.9680449962616,0.01707179316122165
466466,932933,932932,1865865,763.4194002151489,0.016819630930967833
467467,934935,934934,1869869,764.8900499343872,0.016571223532992008
468468,936937,936936,1873873,766.4562449455261,0.016326514391948876
469469,938939,938938,1877877,767.9157190322876,0.016085447800264774
470470,940941,940940,1881881,769.3799841403961,0.01584796890256257
471471,942943,942942,1885885,770.9816439151764,0.015614023683951928
472472,944945,944944,1889889,772.5915930271149,0.015383558956727938
473473,946947,946946,1893893,774.2524840831757,0.015156522346501333
474474,948949,948948,1897897,775.9143130779266,0.014932862280147674
475475,950951,950950,1901901,777.595263004303,0.01471252797307443
476476,952953,952952,1905905,779.232006072998,0.014495469417397544
477477,954955,954954,1909909,780.703910112381,0.014281637368299016
478478,956957,956956,1913913,782.292023897171,0.014070983334477205
479479,958959,958958,1917917,783.7792038917542,0.013863459563935976
480480,960961,960960,1921921,785.2403402328491,0.013659019033980258
481481,962963,962962,1925925,786.7404689788818,0.013457615439506299
482482,964965,964964,1929929,788.2042038440704,0.01325920318140561
483483,966967,966966,1933933,789.8063237667084,0.013063737356105776
484484,968969,968968,1937937,791.3390340805054,0.012871173744088082
485485,970971,970970,1941941,792.912966966629,0.012681468800565199
486486,972973,972972,1945945,794.4055359363556,0.01249457964274825
487487,974975,974974,1949949,795.8648648262024,0.012310464041775049
488488,976977,976976,1953953,797.3643610477448,0.012129080411227733
489489,978979,978978,1957957,798.8611829280853,0.011950387797696749
490490,980981,980980,1961961,800.3559029102325,0.011774345870776415
491491,982983,982982,1965965,801.9685900211334,0.011600914912946791
492492,984985,984984,1969969,803.5017139911652,0.011430055810933482
493493,986987,986986,1973973,805.0025889873505,0.01126173004604425
494494,988989,988988,1977977,806.481164932251,0.011095899684391952
495495,990991,990990,1981981,807.9949688911438,0.010932527368254341
496496,992993,992992,1985985,809.4249520301819,0.010771576307206487
497497,994995,994994,1989989,810.893639087677,0.010613010269480583
498498,996997,996996,1993993,812.4361848831177,0.010456793572757306
499499,998999,998998,1997997,813.9162600040436,0.01030289107632143
500501,1001003,1001002,2002005,815.4065730571747,0.010151117828968381
501502,1003005,1003004,2006009,816.8923711776733,0.010001742659937918
502503,1005007,1005006,2010013,818.4386148452759,0.009854579399416252
503504,1007009,1007008,2014017,819.9042501449585,0.009709594990113146
504505,1009011,1009010,2018021,821.3893020153046,0.009566756874619387
505506,1011013,1011012,2022025,822.8900690078735,0.009426032988926636
506507,1013015,1013014,2026029,824.3536620140076,0.009287391754696728
507508,1015017,1015016,2030033,825.7930040359497,0.009150802070962527
508509,1017019,1017018,2034037,827.3069770336151,0.00901623330730672
509510,1019021,1019020,2038041,828.7627370357513,0.008883655296926918
510511,1021023,1021022,2042045,830.2559690475464,0.008753038329018636
511512,1023025,1023024,2046049,831.7478840351105,0.008624353141499341
512513,1025027,1025026,2050053,833.2845289707184,0.008497570914983044
513514,1027029,1027028,2054057,835.7876358032227,0.008372663265390656
514515,1029031,1029030,2058061,837.7868030071259,0.00824960223724247
515516,1031033,1031032,2062065,839.9445850849152,0.008128360297064319
516517,1033035,1033034,2066069,841.7072658538818,0.008008910326907426
517518,1035037,1035036,2070073,843.3236300945282,0.007891225618664066
518519,1037039,1037038,2074077,844.806036233902,0.007775279866336859
519520,1039041,1039040,2078081,846.3156588077545,0.0076610471616049836
520521,1041043,1041042,2082085,847.7583639621735,0.007548501985752409
521522,1043045,1043044,2086089,849.2749171257019,0.007437619205575174
522523,1045047,1045046,2090093,850.740510225296,0.007328374066446486
523524,1047049,1047048,2094097,852.2233719825745,0.007220742186859752
524525,1049051,1049050,2098101,853.7247619628906,0.00711469955172106
525526,1051053,1051052,2102105,855.3491880893707,0.007010222509052255
526527,1053055,1053054,2106109,856.9446449279785,0.006907287761464431
527528,1055057,1055056,2110113,858.4131319522858,0.00680587236320207
528529,1057059,1057058,2114117,859.8070387840271,0.006705953713321833
529530,1059061,1059060,2118121,861.2618319988251,0.006607509551372459
530531,1061063,1061062,2122125,862.7345309257507,0.006510517951255679
531532,1063065,1063064,2126129,864.211315870285,0.006414957316451364
532533,1065067,1065066,2130133,865.7080838680267,0.006320806375924803
533534,1067069,1067068,2134137,867.1753840446472,0.006228044177078118
534535,1069071,1069070,2138141,868.6521461009979,0.006136650083362838
535536,1071073,1071072,2142145,870.1315848827362,0.006046603767231318
536537,1073075,1073074,2146149,871.596687078476,0.0059578852072945665
537538,1075077,1075076,2150153,873.0787448883057,0.005870474682069471
538539,1077079,1077078,2154157,874.5608150959015,0.005784352766454504
539540,1079081,1079080,2158161,876.0117301940918,0.005699500326954876
540541,1081083,1081082,2162165,877.4779171943665,0.005615898517021378
541542,1083085,1083084,2166169,879.0255579948425,0.005533528772502905
542543,1085087,1085086,2170173,880.4559378623962,0.005452372808349537
543544,1087089,1087088,2174177,881.9250128269196,0.005372412613382949
544545,1089091,1089090,2178181,883.4006109237671,0.005293630445976305
545546,1091093,1091092,2182185,884.8798758983612,0.0052160088310984065
546547,1093095,1093094,2186189,886.3863840103149,0.005139530555311467
547548,1095097,1095096,2190193,887.9234819412231,0.005064178662678387
548549,1097099,1097098,2194197,889.5155827999115,0.004989936451806898
549550,1099101,1099100,2198201,891.0734620094299,0.004916787470733652
550551,1101103,1101102,2202205,892.6367011070251,0.004844715514764175
551552,1103105,1103104,2206209,894.2100839614868,0.004773704620561148
552553,1105107,1105106,2210213,895.8042430877686,0.004703739064666479
553554,1107109,1107108,2214217,897.2574388980865,0.004634803358499084
554555,1109111,1109110,2218221,898.7972378730774,0.004566882244603221
555556,1111113,1111112,2222225,900.3925218582153,0.004499960694829497
556557,1113115,1113114,2226229,901.9729990959167,0.004434023904764217
557558,1115117,1115116,2230233,903.6478490829468,0.004369057291910394
558559,1117119,1117118,2234237,905.3089320659637,0.004305046491253961
559560,1119121,1119120,2238241,906.9878799915314,0.004241977352535287
560561,1121123,1121122,2242245,908.6601960659027,0.004179835937293319
561562,1123125,1123124,2246249,910.2162971496582,0.004118608515000233
562563,1125127,1125126,2250253,911.7885820865631,0.004058281559991883
563564,1127129,1127128,2254257,913.2641661167145,0.00399884174851195
564565,1129131,1129130,2258261,914.733980178833,0.003940275956210826
565566,1131133,1131132,2262265,916.1966319084167,0.003882571254280265
566567,1133135,1133134,2266269,917.6605370044708,0.0038257149067248974
567568,1135137,1135136,2270273,919.1953361034393,0.0037696943677474337
568569,1137139,1137138,2274277,920.7724120616913,0.0037144972787928054
569570,1139141,1139140,2278281,922.3909401893616,0.003660111465251248
570571,1141143,1141142,2282285,923.8896570205688,0.0036065249342982497
571572,1143145,1143144,2286289,925.391438961029,0.0035537258718250087
572573,1145147,1145146,2290293,926.8707740306854,0.0035017026400510076
573574,1147149,1147148,2294297,928.4001331329346,0.0034504437742270966
574575,1149151,1149150,2298301,929.9638948440552,0.0033999379805891294
575576,1151153,1151152,2302305,931.5485119819641,0.0033501741337431667
576577,1153155,1153154,2306309,933.1118359565735,0.0033011412740506785
577578,1155157,1155156,2310313,934.6601948738098,0.0032528286045589994
578579,1157159,1157158,2314317,936.17067694664,0.003205225489637087
579580,1159161,1159160,2318321,937.6384098529816,0.0031583214519059766
580581,1161163,1161162,2322325,939.1339681148529,0.003112106169623985
581582,1163165,1163164,2326329,940.6095700263977,0.0030665694748677197
582583,1165167,1165166,2330333,942.1545219421387,0.00302170135103097
583584,1167169,1167168,2334337,943.6729960441589,0.0029774919304372816
584585,1169171,1169170,2338341,945.1663022041321,0.002933931492066222
585586,1171173,1171172,2342345,946.6570389270782,0.002891010459620702
586587,1173175,1173174,2346349,948.161553144455,0.002848719399366928
587588,1175177,1175176,2350353,949.6589920520782,0.002807049017292229
588589,1177179,1177178,2354357,951.1646339893341,0.00276599015796819
589590,1179181,1179180,2358361,952.6601808071136,0.0027255338018221664
590591,1181183,1181182,2362365,954.1357970237732,0.0026856710634319825
591592,1183185,1183184,2366369,955.6106588840485,0.002646393189252194
592593,1185187,1185186,2370373,957.0940709114075,0.0026076915557950997
593594,1187189,1187188,2374377,958.5478270053864,0.0025695576675843768
594595,1189191,1189190,2378381,960.0569751262665,0.00253198315579084
595596,1191193,1191192,2382385,961.6514971256256,0.0024949597748218366
596597,1193195,1193194,2386389,963.1564462184906,0.002458479402434932
597598,1195197,1195196,2390393,964.6486802101135,0.00242253403655468
598599,1197199,1197198,2394397,966.2585179805756,0.002387115793681005
599600,1199201,1199200,2398401,967.8026249408722,0.002352216907638649
600601,1201203,1201202,2402405,969.3474850654602,0.00231782972741712
601602,1203205,1203204,2406409,970.8424701690674,0.00228394671512433
602603,1205207,1205206,2410413,972.3074510097504,0.002250560445077099
603604,1207209,1207208,2414417,973.7870481014252,0.0022176636016411067
604605,1209211,1209210,2418421,975.2220280170441,0.002185248977411902
605606,1211213,1211212,2422425,976.7442281246185,0.002153309471850662
606607,1213215,1213214,2426429,978.2978310585022,0.002121838090147321
607608,1215217,1215216,2430433,979.8226430416107,0.0020908279406057773
608609,1217219,1217218,2434437,981.3593471050262,0.002060272233620708
609610,1219221,1219220,2438441,982.8812279701233,0.0020301642806543896
610611,1221223,1221222,2442445,984.36075091362,0.0020004974918492735
611612,1223225,1223224,2446449,985.8173680305481,0.001971265375459552
612613,1225227,1225226,2450453,987.2959480285645,0.0019424615347816143
613614,1227229,1227228,2454457,988.800507068634,0.0019140796691772266
614615,1229231,1229230,2458461,990.2631731033325,0.0018861135704355547
615616,1231233,1231232,2462465,991.7486598491669,0.0018585571222047292
616617,1233235,1233234,2466469,993.2999711036682,0.001831404299650785
617618,1235237,1235236,2470473,994.8137030601501,0.001804649165705996
618619,1237239,1237238,2474477,996.3613679409027,0.0017782858720920558
619620,1239241,1239240,2478481,997.8944029808044,0.0017523086569326551
620621,1241243,1241242,2482485,999.585776090622,0.0017267118431618655
621622,1243245,1243244,2486489,1001.2174649238586,0.0017014898380693921
622623,1245247,1245246,2490493,1003.1474840641022,0.001676637131708958
623624,1247249,1247248,2494497,1004.8228390216827,0.0016521482954203748
624625,1249251,1249250,2498501,1006.5412588119507,0.0016280179806926753
625626,1251253,1251252,2502505,1008.2175619602203,0.0016042409184819917
626627,1253255,1253254,2506509,1009.9228200912476,0.0015808119170515056
627628,1255257,1255256,2510513,1011.591854095459,0.0015577258619714485
628629,1257259,1257258,2514517,1013.1071579456329,0.0015349777144137988
629630,1259261,1259260,2518521,1014.5970752239227,0.0015125625093332928
630631,1261263,1261262,2522525,1016.8391320705414,0.0014904753555811112
631632,1263265,1263264,2526529,1018.8105208873749,0.0014687114340858898
632633,1265267,1265266,2530533,1020.5700809955597,0.0014472659971715984
633634,1267269,1267268,2534537,1022.2356698513031,0.0014261343671932991
634635,1269271,1269270,2538541,1023.9776301383972,0.0014053119351729038
635636,1271273,1271272,2542545,1025.6909868717194,0.0013847941606854874
636637,1273275,1273274,2546549,1027.3549621105194,0.0013645765702676727
637638,1275277,1275276,2550553,1028.9505569934845,0.0013446547563944478
638639,1277279,1277278,2554557,1030.5611670017242,0.0013250243764559855
639640,1279281,1279280,2558561,1032.241248846054,0.0013056811523028955
640641,1281283,1281282,2562565,1033.9475739002228,0.0012866208684272351
641642,1283285,1283284,2566569,1035.7794229984283,0.001267839372076196
642643,1285287,1285286,2570573,1037.633069038391,0.0012493325712057413
643644,1287289,1287288,2574577,1039.3415441513062,0.0012310964344806052
644645,1289291,1289290,2578581,1041.2948169708252,0.0012131269902511121
645646,1291293,1291292,2582585,1043.07150888443,0.0011954203246204997
646647,1293295,1293294,2586589,1044.7521052360535,0.001177972582354414
647648,1295297,1295296,2590593,1046.6623229980469,0.0011607799644934857
648649,1297299,1297298,2594597,1048.5111269950867,0.0011438387282396434
649650,1299301,1299300,2598601,1050.3828461170197,0.0011271451859329318
650651,1301303,1301302,2602605,1052.0471119880676,0.0011106957044830779
651652,1303305,1303304,2606609,1053.759477853775,0.0010944867040052486
652653,1305307,1305306,2610613,1055.4681930541992,0.001078514657820051
653654,1307309,1307308,2614617,1057.3323440551758,0.001062776090520856
654655,1309311,1309310,2618621,1059.206670999527,0.0010472675785422325
655656,1311313,1311312,2622625,1060.9619119167328,0.0010319857484546446
656657,1313315,1313314,2626629,1062.7591080665588,0.0010169272768507653
657658,1315317,1315316,2630633,1064.4725120067596,0.001002088888981234
658659,1317319,1317318,2634637,1066.0700809955597,0.0009874673579588489
659660,1319321,1319320,2638641,1067.6720650196075,0.0009730595053270008
660661,1321323,1321322,2642645,1069.298763036728,0.0009588621986722501
661662,1323325,1323324,2646649,1070.7653040885925,0.0009448723523064473
662663,1325327,1325326,2650653,1072.5233058929443,0.0009310869254477439
663664,1327329,1327328,2654657,1074.1142508983612,0.0009175029219932185
664665,1329331,1329330,2658661,1075.7679278850555,0.0009041173907462507
665666,1331333,1331332,2662665,1077.350042104721,0.0008909274230290976
666667,1333335,1333334,2666669,1078.9097349643707,0.0008779301535923878
667668,1335337,1335336,2670673,1080.411316871643,0.0008651227589098198
668669,1337339,1337338,2674677,1082.1776449680328,0.0008525024574055351
669670,1339341,1339340,2678681,1083.8216140270233,0.0008400665080898762
670671,1341343,1341342,2682685,1085.6235859394073,0.0008278122105593866
671672,1343345,1343344,2686689,1087.3318800926208,0.0008157369039736295
672673,1345347,1345346,2690693,1088.9311411380768,0.0008038379664867534
673674,1347349,1347348,2694697,1090.516657114029,0.0007921128150201184
674675,1349351,1349350,2698701,1092.0328760147095,0.000780558904807549
675676,1351353,1351352,2702705,1093.5442159175873,0.0007691737279174049
676677,1353355,1353354,2706709,1095.0189521312714,0.0007579548133662684
677678,1355357,1355356,2710713,1096.5820498466492,0.0007468997271189437
678679,1357359,1357358,2714717,1098.0759961605072,0.0007360060698147208
679680,1359361,1359360,2718721,1099.5886061191559,0.000725271478245304
680681,1361363,1361362,2722725,1101.0619370937347,0.0007146936242179436
681682,1363365,1363364,2726729,1102.5467290878296,0.0007042702125090727
682683,1365367,1365366,2730733,1104.1392030715942,0.0006939989826832971
683684,1367369,1367368,2734737,1105.6231789588928,0.0006838777071607183
684685,1369371,1369370,2738741,1107.565763950348,0.0006739041912169341
685686,1371373,1371372,2742745,1109.0655300617218,0.0006640762721872306
686687,1373375,1373374,2746749,1110.5355660915375,0.0006543918191255216
687688,1375377,1375376,2750753,1112.038321018219,0.0006448487328043484
688689,1377379,1377378,2754757,1113.529718875885,0.0006354449443506383
689690,1379381,1379380,2758761,1115.039491891861,0.0006261784153593908
690691,1381383,1381382,2762765,1116.667321920395,0.0006170471378936782
691692,1383385,1383384,2766769,1118.2892980575562,0.0006080491327793425
692693,1385387,1385386,2770773,1120.008414030075,0.00059918245017343
693694,1387389,1387388,2774777,1121.9042122364044,0.0005904451691094437
694695,1389391,1389390,2778781,1123.369271993637,0.0005818353967015355
695696,1391393,1391392,2782785,1125.0185780525208,0.0005733512673486985
696697,1393395,1393394,2786789,1127.022430896759,0.0005649909434168876
697698,1395397,1395396,2790793,1128.5270030498505,0.0005567526143295254
698699,1397399,1397398,2794797,1130.0200140476227,0.0005486344956580069
699700,1399401,1399400,2798801,1131.503798007965,0.0005406348292353869
700701,1401403,1401402,2802805,1132.9693942070007,0.0005327518828153188
701702,1403405,1403404,2806809,1134.4839599132538,0.0005249839498446818
702703,1405407,1405406,2810813,1135.9575440883636,0.0005173293483267116
703704,1407409,1407408,2814817,1137.4364259243011,0.0005097864207073144
704705,1409411,1409410,2818821,1138.9336380958557,0.0005023535347845609
705706,1411413,1411412,2822825,1140.4129419326782,0.0004950290814349501
706707,1413415,1413414,2826829,1141.9875328540802,0.00048781147540921665
707708,1415417,1415416,2830833,1143.501435995102,0.0004806991548775841
708709,1417419,1417418,2834837,1144.9736909866333,0.00047369058017920906
709710,1419421,1419420,2838841,1146.5002977848053,0.00046678423518642376
710711,1421423,1421422,2842845,1148.155044078827,0.00045997862571312
711712,1423425,1423424,2846849,1149.8434898853302,0.00045327227917368873
712713,1425427,1425426,2850853,1151.883367061615,0.00044666374481039384
713714,1427429,1427428,2854857,1154.275778055191,0.00044015159301125095
714715,1429431,1429430,2858861,1155.8585150241852,0.00043373441531002754
715716,1431433,1431432,2862865,1157.5141229629517,0.0004274108234767482
716717,1433435,1433434,2866869,1159.2696959972382,0.00042117945031350246
717718,1435437,1435436,2870873,1160.858808040619,0.0004150389482902028
718719,1437439,1437438,2874877,1162.4335479736328,0.00040898798931721103
719720,1439441,1439440,2878881,1163.9753680229187,0.0004030252652000854
720721,1441443,1441442,2882885,1165.513657093048,0.00039714948684377305
721722,1443445,1443444,2886889,1166.9901311397552,0.00039135938368417555
722723,1445447,1445446,2890893,1168.4439289569855,0.00038565370471133065
723724,1447449,1447448,2894897,1170.0548479557037,0.0003800312159683017
724725,1449451,1449450,2898901,1171.6928219795227,0.0003744907022564803
725726,1451453,1451452,2902905,1173.3579330444336,0.00036903096656715206
726727,1453455,1453454,2906909,1175.2281930446625,0.0003636508286035678
727728,1455457,1455456,2910913,1177.176595211029,0.0003583491258041249
728729,1457459,1457458,2914917,1178.9514548778534,0.0003531247126602466
729730,1459461,1459460,2918921,1180.571585893631,0.0003479764604890079
730731,1461463,1461462,2922925,1181.996768951416,0.00034290325675101485
731732,1463465,1463464,2926929,1183.3228919506073,0.0003379040056188387
732733,1465467,1465466,2930933,1184.8598408699036,0.0003329776267264606
733734,1467469,1467468,2934937,1186.8980882167816,0.0003281230565335136
734735,1469471,1469470,2938941,1188.3104848861694,0.00032333924627891975
735736,1471473,1471472,2942945,1190.0961380004883,0.00031862516254932416
736737,1473475,1473474,2946949,1191.7077071666718,0.00031397978739278187
737738,1475477,1475476,2950953,1193.345645904541,0.00030940211763663683
738739,1477479,1477478,2954957,1195.2483780384064,0.0003048911650012087
739740,1479481,1479480,2958961,1197.1071400642395,0.0003004459553039851
740741,1481483,1481482,2962965,1198.979387998581,0.0002960655286869951
741742,1483485,1483484,2966969,1200.8533370494843,0.00029174893927574885
742743,1485487,1485486,2970973,1202.7056438922882,0.00028749525574767176
743744,1487489,1487488,2974977,1204.5859160423279,0.00028330355928574136
744745,1489491,1489490,2978981,1206.9804329872131,0.0002791729453974767
745746,1491493,1491492,2982985,1209.1443297863007,0.00027510252255069645
746747,1493495,1493494,2986989,1210.8260688781738,0.00027109141194614494
747748,1495497,1495496,2990993,1212.7238850593567,0.0002671387481996135
748749,1497499,1497498,2994997,1214.3146409988403,0.0002632436782050718
749750,1499501,1499500,2999001,1215.8375022411346,0.0002594053612483549
750751,1501503,1501502,3003005,1217.6403529644012,0.0002556229693482237
751752,1503505,1503504,3007009,1219.2114589214325,0.0002518956863468702
752753,1505507,1505506,3011013,1220.794103860855,0.0002482227081372912
753754,1507509,1507508,3015017,1222.5017478466034,0.00024460324209485407
754755,1509511,1509510,3019021,1225.1106479167938,0.00024103650764573104
755756,1511513,1511512,3023025,1226.9152390956879,0.00023752173524371756
756757,1513515,1513514,3027029,1228.6737949848175,0.0002340581664839192
757758,1515517,1515516,3031033,1230.3884599208832,0.00023064505489855947
758759,1517519,1517518,3035037,1231.8597211837769,0.00022728166379692993
759760,1519521,1519520,3039041,1233.503175020218,0.00022396726819806645
760761,1521523,1521522,3043045,1235.006767988205,0.00022070115301175974
761762,1523525,1523524,3047049,1236.7943091392517,0.00021748261394805013
762763,1525527,1525526,3051053,1238.4712948799133,0.00021431095740354067
763764,1527529,1527528,3055057,1240.1956040859222,0.00021118549886978144
764765,1529531,1529530,3059061,1241.7940781116486,0.00020810556497963262
765766,1531533,1531532,3063065,1243.5371308326721,0.00020507049134721456
766767,1533535,1533534,3067069,1245.2883648872375,0.00020207962393214984
767768,1535537,1535536,3071073,1246.752291917801,0.00019913231767532125
768769,1537539,1537538,3075077,1248.4789669513702,0.00019622793752205325
769770,1539541,1539540,3079081,1250.1149821281433,0.00019336585717155685
770771,1541543,1541542,3083085,1251.7151770591736,0.0001905454598727374
771772,1543545,1543544,3087089,1253.424766778946,0.00018776613785576046
772773,1545547,1545546,3091093,1255.318983078003,0.0001850272916499307
773774,1547549,1547548,3095097,1256.9496638774872,0.00018232833156162087
774775,1549551,1549550,3099101,1259.1508529186249,0.00017966867585528234
775776,1551553,1551552,3103105,1260.9582860469818,0.00017704775086713198
776777,1553555,1553554,3107109,1262.462172985077,0.000174464992483081
777778,1555557,1555556,3111113,1263.9454700946808,0.00017191984386499826
778779,1557559,1557558,3115117,1265.6718680858612,0.00016941175692863908
779780,1559561,1559560,3119121,1267.2464711666107,0.00016694019086571643
780781,1561563,1561562,3123125,1269.1255300045013,0.00016450461350814294
781782,1563565,1563564,3127129,1270.8656768798828,0.00016210450007747568
782783,1565567,1565566,3131133,1272.5179450511932,0.00015973933363966353
783784,1567569,1567568,3135137,1274.0074779987335,0.00015740860465029982
784785,1569571,1569570,3139141,1275.5792210102081,0.00015511181095462234
785786,1571573,1571572,3143145,1277.0950560569763,0.00015284845812857384
786787,1573575,1573574,3147149,1278.6672611236572,0.00015061805834193365
787788,1575577,1575576,3151153,1280.291393995285,0.0001484201316088729
788789,1577579,1577578,3155157,1281.838761806488,0.00014625420431002567
789790,1579581,1579580,3159161,1283.5442049503326,0.00014411980998829677
790791,1581583,1581582,3163165,1285.3039419651031,0.00014201648946254863
791792,1583585,1583584,3167169,1287.2043330669403,0.0001399437892359856
792793,1585587,1585586,3171173,1288.7272958755493,0.0001379012633151433
793794,1587589,1587588,3175177,1290.2767369747162,0.00013588847184564656
794795,1589591,1589590,3179181,1291.8697781562805,0.0001339049816806437
795796,1591593,1591592,3183185,1293.7605381011963,0.00013195036535762483
796797,1593595,1593594,3187189,1295.372601032257,0.0001300242024626641
797798,1595597,1595596,3191193,1296.8628311157227,0.00012812607803880383
798799,1597599,1597598,3195197,1298.480129957199,0.0001262555837229229
799800,1599601,1599600,3199201,1300.2618479728699,0.00012441231660886842
800801,1601603,1601602,3203205,1302.296646118164,0.00012259588038432412
801802,1603605,1603604,3207209,1304.1042549610138,0.00012080588373919454
802803,1605607,1605606,3211213,1306.377802848816,0.00011904194150247349
803804,1607609,1607608,3215217,1307.9250900745392,0.00011730367384643614
804805,1609611,1609610,3219221,1309.4803829193115,0.00011559070696876006
805806,1611613,1611612,3223225,1311.2937581539154,0.00011390267206934368
806807,1613615,1613614,3227229,1313.5900111198425,0.00011223920580505364
807808,1615617,1615616,3231233,1316.098177909851,0.00011059995040341164
808809,1617619,1617618,3235237,1317.976224899292,0.00010898455286678654
809810,1619621,1619620,3239241,1319.6125988960266,0.00010739266610926279
810811,1621623,1621622,3243245,1321.3019318580627,0.00010582394702396414
811812,1623625,1623624,3247249,1322.9292168617249,0.00010427805830204306
812813,1625627,1625626,3251253,1324.393975019455,0.00010275466752318607
813814,1627629,1627628,3255257,1325.837590932846,0.00010125344681455317
814815,1629631,1629630,3259261,1327.2775039672852,9.977407307815156e-05
815816,1631633,1631632,3263265,1328.7261180877686,9.831622833189613e-05
816817,1633635,1633634,3267269,1330.1838262081146,9.687959880011476e-05
817818,1635637,1635636,3271273,1331.6372141838074,9.546387525460887e-05
818819,1637639,1637638,3275277,1333.7879300117493,9.406875346940069e-05
819820,1639641,1639640,3279281,1335.3626689910889,9.269393342492549e-05
820821,1641643,1641642,3283285,1336.9690890312195,9.133911919434468e-05
821822,1643645,1643644,3287289,1338.6724960803986,9.000401962566684e-05
822823,1645647,1645646,3291293,1340.1430869102478,8.868834731856623e-05
823824,1647649,1647648,3295297,1341.6152758598328,8.739181930650375e-05
824825,1649651,1649650,3299301,1343.1883518695831,8.611415694304014e-05
825826,1651653,1651652,3303305,1344.9554929733276,8.485508521971497e-05
826827,1653655,1653654,3307309,1346.7319989204407,8.361433378922811e-05
827828,1655657,1655656,3311313,1348.335212945938,8.239163548751094e-05
828829,1657659,1657658,3315317,1350.297730922699,8.118672769796831e-05
829830,1659661,1659660,3319321,1352.157086133957,7.999935110092338e-05
830831,1661663,1661662,3323325,1353.7375299930573,7.882925046942546e-05
831832,1663665,1663664,3327329,1355.1858348846436,7.7676173987129e-05
832833,1665667,1665666,3331333,1356.6340351104736,7.653987427147513e-05
833834,1667669,1667668,3335337,1358.2225329875946,7.542010655470222e-05
834835,1669671,1669670,3339341,1359.861876964569,7.431663038914849e-05
835836,1671673,1671672,3343345,1361.7233929634094,7.322920839669678e-05
836837,1673675,1673674,3347349,1363.2341449260712,7.215760683720873e-05
837838,1675677,1675676,3351353,1364.6535761356354,7.110159526746429e-05
838839,1677679,1677678,3355357,1366.1047458648682,7.006094699590903e-05
839840,1679681,1679680,3359361,1367.5489430427551,6.903543794578582e-05
840841,1681683,1681682,3363365,1368.9801199436188,6.80248480193768e-05
841842,1683685,1683684,3367369,1370.418783903122,6.702895984744828e-05
842843,1685687,1685686,3371373,1371.8683199882507,6.604755924399797e-05
843844,1687689,1687688,3375377,1373.3431839942932,6.508043543362874e-05
844845,1689691,1689690,3379381,1375.0546779632568,6.412738059680123e-05
845846,1691693,1691692,3383385,1377.0982871055603,6.318818986983388e-05
846847,1693695,1693694,3387389,1379.2729589939117,6.226266134490288e-05
847848,1695697,1695696,3391393,1381.176687002182,6.135059618372907e-05
848849,1697699,1697698,3395397,1383.4383490085602,6.045179850389104e-05
849850,1699701,1699700,3399401,1385.3560738563538,5.956607492407784e-05
850851,1701703,1701702,3403405,1387.0850999355316,5.869323547358363e-05
851852,1703705,1703704,3407409,1389.1415431499481,5.7833092114378815e-05
852853,1705707,1705706,3411413,1391.0924849510193,5.698546021903894e-05
853854,1707709,1707708,3415417,1392.9645080566406,5.6150157774936815e-05
854855,1709711,1709710,3419421,1395.9931600093842,5.5327005270555674e-05
855856,1711713,1711712,3423425,1398.1661868095398,5.45158260365497e-05
856857,1713715,1713714,3427429,1400.7975718975067,5.371644533624931e-05
857858,1715717,1715716,3431433,1402.8558249473572,5.292869184359006e-05
858859,1717719,1717718,3435437,1404.7230818271637,5.215239593781007e-05
859860,1719721,1719720,3439441,1406.7374789714813,5.1387391181378916e-05
860861,1721723,1721722,3443445,1408.7279419898987,5.063351329681609e-05
861862,1723725,1723724,3447449,1410.413722038269,4.9890600053004164e-05
862863,1725727,1725726,3451453,1411.965980052948,4.9158491833622975e-05
863864,1727729,1727728,3455457,1413.7008879184723,4.843703163714963e-05
864865,1729731,1729730,3459461,1415.3007969856262,4.772606439473748e-05
865866,1731733,1731732,3463465,1417.0062010288239,4.702543719758978e-05
866867,1733735,1733734,3467469,1419.0358970165253,4.633499986539391e-05
867868,1735737,1735736,3471473,1421.4312269687653,4.565460403682664e-05
868869,1737739,1737738,3475477,1423.3431611061096,4.498410339692782e-05
869870,1739741,1739740,3479481,1425.7673099040985,4.43233540181609e-05
870871,1741743,1741742,3483485,1427.5726308822632,4.3672214019352396e-05
871872,1743745,1743744,3487489,1429.7888958454132,4.3030543565691914e-05
872873,1745747,1745746,3491493,1432.0448858737946,4.23982047550453e-05
873874,1747749,1747748,3495497,1433.7473289966583,4.177506218638882e-05
874875,1749751,1749750,3499501,1435.4610199928284,4.11609814818803e-05
875876,1751753,1751752,3503505,1436.9235849380493,4.055583110584848e-05
876877,1753755,1753754,3507509,1438.3565249443054,3.9959480886864185e-05
877878,1755757,1755756,3511513,1439.829843044281,3.937180292723497e-05
878879,1757759,1757758,3515517,1441.2785708904266,3.879267103457096e-05
879880,1759761,1759760,3519521,1442.7362079620361,3.822196094915853e-05
880881,1761763,1761762,3523525,1444.9763679504395,3.765954988921294e-05
881882,1763765,1763764,3527529,1446.555813074112,3.710531723299937e-05
882883,1765767,1765766,3531533,1448.0586330890656,3.655914395039872e-05
883884,1767769,1767768,3535537,1449.622901916504,3.6020912830281304e-05
884885,1769771,1769770,3539541,1451.1217639446259,3.5490508366819995e-05
885886,1771773,1771772,3543545,1452.6513671875,3.4967816645803396e-05
886887,1773775,1773774,3547549,1454.5357291698456,3.4452725230949e-05
887888,1775777,1775776,3551553,1456.047613143921,3.394512373233738e-05
888889,1777779,1777778,3555557,1457.5973489284515,3.3444903237977996e-05
889890,1779781,1779780,3559561,1458.9955921173096,3.2951956313809205e-05
890891,1781783,1781782,3563565,1460.3394348621368,3.246617700369825e-05
891892,1783785,1783784,3567569,1461.8611371517181,3.19874609431281e-05
892893,1785787,1785786,3571573,1463.4121570587158,3.1515705813944805e-05
893894,1787789,1787788,3575577,1464.8973548412323,3.105080986642861e-05
894895,1789791,1789790,3579581,1466.337084054947,3.059267373828334e-05
895896,1791793,1791792,3583585,1467.8620829582214,3.014119897670753e-05
896897,1793795,1793794,3587589,1469.5185589790344,2.969628826576809e-05
897898,1795797,1795796,3591593,1471.3058359622955,2.9257846449581848e-05
898899,1797799,1797798,3595597,1472.954502105713,2.8825779736507684e-05
899900,1799801,1799800,3599601,1474.5004630088806,2.8399994789651828e-05
900901,1801803,1801802,3603605,1475.934121131897,2.7980400432170427e-05
901902,1803805,1803804,3607609,1477.362009048462,2.7566906737774843e-05
902903,1805807,1805806,3611613,1478.8305339813232,2.7159424917044817e-05
903904,1807809,1807808,3615617,1480.240014076233,2.675786754480214e-05
904905,1809811,1809810,3619621,1481.7307569980621,2.636214821905014e-05
905906,1811813,1811812,3623625,1483.146893978119,2.597218224309472e-05
906907,1813815,1813814,3627629,1484.555231809616,2.5587885943423316e-05
907908,1815817,1815816,3631633,1485.9812469482422,2.5209176669704902e-05
908909,1817819,1817818,3635637,1487.41832113266,2.4835973363224184e-05
909910,1819821,1819820,3639641,1488.8361320495605,2.4468195647386892e-05
910911,1821823,1821822,3643645,1490.3094320297241,2.410576496458816e-05
911912,1823825,1823824,3647649,1491.7587418556213,2.3748603211970476e-05
912913,1825827,1825826,3651653,1493.2060539722443,2.3396633991978888e-05
913914,1827829,1827828,3655657,1495.7261900901794,2.3049781702866312e-05
914915,1829831,1829830,3659661,1497.6433079242706,2.2707971766067203e-05
915916,1831833,1831832,3663665,1500.1190149784088,2.2371131194631744e-05
916917,1833835,1833834,3667669,1501.7877202033997,2.203918734267063e-05
917918,1835837,1835836,3671673,1503.5394768714905,2.1712069269597123e-05
918919,1837839,1837838,3675677,1505.7765438556671,2.1389706603258674e-05
919920,1839841,1839840,3679681,1507.538514137268,2.107202999468427e-05
920921,1841843,1841842,3683685,1509.0094120502472,2.0758971686518635e-05
921922,1843845,1843844,3687689,1510.442549943924,2.0450464603527507e-05
922923,1845847,1845846,3691693,1511.8903441429138,2.0146442011537147e-05
923924,1847849,1847848,3695697,1513.3440301418304,1.984683922273689e-05
924925,1849851,1849850,3699701,1514.7679798603058,1.9551591435629234e-05
925926,1851853,1851852,3703705,1516.7352831363678,1.926063578139292e-05
926927,1853855,1853854,3707709,1518.5433549880981,1.8973909618580365e-05
927928,1855857,1855856,3711713,1520.3625741004944,1.869135132892552e-05
928929,1857859,1857858,3715717,1522.3968801498413,1.8412900658404396e-05
929930,1859861,1859860,3719721,1525.2045831680298,1.8138497580366675e-05
930931,1861863,1861862,3723725,1528.2453429698944,1.786808354609093e-05
931932,1863865,1863864,3727729,1530.600214958191,1.7601600006855733e-05
932933,1865867,1865866,3731733,1532.4748170375824,1.7338990232929063e-05
933934,1867869,1867868,3735737,1534.1894659996033,1.7080197608265735e-05
934935,1869871,1869870,3739741,1535.9362120628357,1.6825166994749452e-05
935936,1871873,1871872,3743745,1537.404571056366,1.6573843367950758e-05
936937,1873875,1873874,3747749,1538.9803500175476,1.632617295399541e-05
937938,1875877,1875876,3751753,1540.8347299098969,1.6082102547443355e-05
938939,1877879,1877878,3755757,1542.5065791606903,1.584157985234924e-05
939940,1879881,1879880,3759761,1544.191143989563,1.560455336857558e-05
940941,1881883,1881882,3763765,1545.7862989902496,1.5370972164419072e-05
941942,1883885,1883884,3767769,1547.439936876297,1.5140786103984283e-05
942943,1885887,1885886,3771773,1548.892860174179,1.4913945960870478e-05
943944,1887889,1887888,3775777,1550.347697019577,1.46904027360506e-05
944945,1889891,1889890,3779781,1551.7736489772797,1.447010902211332e-05
945946,1891893,1891892,3783785,1553.4858889579773,1.425301718427363e-05
946947,1893895,1893894,3787789,1556.367651939392,1.4039080610928067e-05
947948,1895897,1895896,3791793,1558.4059100151062,1.3828253713654703e-05
948949,1897899,1897898,3795797,1560.4602599143982,1.3620491245092126e-05
949950,1899901,1899900,3799801,1561.9566910266876,1.3415748298939434e-05
950951,1901903,1901902,3803805,1563.4720940589905,1.3213981333137781e-05
951952,1903905,1903904,3807809,1564.9214429855347,1.3015147033001995e-05
952953,1905907,1905906,3811813,1567.4624650478363,1.2819202538594254e-05
953954,1907909,1907908,3815817,1569.2502369880676,1.2626106240531954e-05
954955,1909911,1909910,3819821,1571.2601640224457,1.2435816188371973e-05
955956,1911913,1911912,3823825,1572.7562358379364,1.2248292023286922e-05
956957,1913915,1913914,3827829,1574.2586369514465,1.2063493159075733e-05
957958,1915917,1915916,3831833,1575.7403030395508,1.1881380373779393e-05
958959,1917919,1917918,3835837,1577.2474138736725,1.1701914445438888e-05
959960,1919921,1919920,3839841,1578.8314390182495,1.1525056606842554e-05
960961,1921923,1921922,3843845,1581.0295221805573,1.1350769341333944e-05
961962,1923925,1923924,3847849,1582.5015668869019,1.1179015245943447e-05
962963,1925927,1925926,3851853,1583.9675960540771,1.1009757258761965e-05
963964,1927929,1927928,3855857,1585.5025119781494,1.0842959341061942e-05
964965,1929931,1929930,3859861,1586.9421200752258,1.0678585454115819e-05
965966,1931933,1931932,3863865,1588.411530971527,1.0516600582377578e-05
966967,1933935,1933934,3867869,1589.8875088691711,1.03569697103012e-05
967968,1935937,1935936,3871873,1591.3322970867157,1.0199659072895884e-05
968969,1937939,1937938,3875877,1592.7966549396515,1.0044634450423473e-05
969970,1939941,1939940,3879881,1594.2917149066925,9.891863101074705e-06
970971,1941943,1941942,3883885,1595.818659067154,9.741311941979802e-06
971972,1943945,1943944,3887889,1597.7190470695496,9.592948572390014e-06
972973,1945947,1945946,3891893,1599.494525194168,9.446741387364455e-06
973974,1947949,1947948,3895897,1602.4662098884583,9.302659236709587e-06
974975,1949951,1949950,3899901,1604.8130490779877,9.160670742858201e-06
975976,1951953,1951952,3903905,1606.8410160541534,9.020746119858813e-06
976977,1953955,1953954,3907909,1608.9003820419312,8.882854785952077e-06
977978,1955957,1955956,3911913,1611.233325958252,8.746967409933859e-06
978979,1957959,1957958,3915917,1612.8197829723358,8.613054660600028e-06
979980,1959961,1959960,3919921,1614.4832410812378,8.481088116241153e-06
980981,1961963,1961962,3923925,1616.0267088413239,8.351039468834642e-06
981982,1963965,1963964,3927929,1617.5113949775696,8.222880751418415e-06
982983,1965967,1965966,3931933,1618.986032962799,8.096584338090906e-06
983984,1967969,1967968,3935937,1620.8723409175873,7.97212351244525e-06
984985,1969971,1969970,3939941,1622.5403249263763,7.84947121701407e-06
985986,1971973,1971972,3943945,1624.5484068393707,7.72860130382469e-06
986987,1973975,1973974,3947949,1626.0817620754242,7.609488079651783e-06
987988,1975977,1975976,3951953,1628.0829770565033,7.492105737583188e-06
988989,1977979,1977978,3955957,1629.944734096527,7.376429266514606e-06
989990,1979981,1979980,3959961,1632.0998351573944,7.2624335416549e-06
990991,1981983,1981982,3963965,1633.8196840286255,7.150094575081312e-06
991992,1983985,1983984,3967969,1635.632374048233,7.039388037810568e-06
992993,1985987,1985986,3971973,1637.225596189499,6.930290169293585e-06
993994,1987989,1987988,3975977,1638.7887001037598,6.822777891102305e-06
994995,1989991,1989990,3979981,1640.396103143692,6.716827897434996e-06
995996,1991993,1991992,3983985,1642.0104250907898,6.612417564610951e-06
996997,1993995,1993994,3987989,1643.4547271728516,6.509524496323138e-06
997998,1995997,1995996,3991993,1645.269896030426,6.408126409951365e-06
998999,1997999,1997998,3995997,1646.998386144638,6.308201932370139e-06
1000000,2000001,2000000,4000001,1648.6927552223206,6.2097294630802935e-06


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0008897781372070312,2181.2938132599165
5,11,5,16,0.01314091682434082,551.6572936697758
9,19,9,28,0.018110990524291992,328.55966978448737
14,29,14,43,0.02493596076965332,210.09838993014114
18,37,18,55,0.030296802520751953,162.94770294226828
23,47,23,70,0.0363919734954834,128.02251159792422
27,55,27,82,0.04106593132019043,110.32071588270901
32,65,32,97,0.04689788818359375,95.32596105537482
36,73,36,109,0.05164909362792969,86.95884698182999
41,83,41,124,0.05733299255371094,79.58223819698173
46,93,46,139,0.06327390670776367,74.41726328357527
50,101,50,151,0.06794977188110352,71.2249660873008
55,111,55,166,0.07413101196289062,67.97957715833968
59,119,59,178,0.0791168212890625,65.82527310965133
64,129,64,193,0.08534407615661621,63.51994542126204
68,137,68,205,0.09254574775695801,61.885768455410926
73,147,73,220,0.09832191467285156,60.05414066981007
78,157,78,235,0.10694575309753418,58.48128388845657
82,165,82,247,0.11159896850585938,57.42541371166362
87,175,87,262,0.11749410629272461,56.337611548024825
91,183,91,274,0.12215614318847656,55.62582065774427
96,193,96,289,0.12974286079406738,54.903526621526225
100,201,100,301,0.13481497764587402,54.43580853555068
105,211,105,316,0.14109587669372559,53.95288888748814
109,219,109,328,0.14622282981872559,53.62066620994665
114,229,114,343,0.15337872505187988,53.23500935584639
119,239,119,358,0.1608419418334961,52.84674502919029
123,247,123,370,0.16715383529663086,52.51999195501844
128,257,128,385,0.1759939193725586,52.086835235855006
132,265,132,397,0.18344402313232422,51.722205659494875
137,275,137,412,0.1916518211364746,51.247821407905576
141,283,141,424,0.1981799602508545,50.8552389243423
146,293,146,439,0.20527386665344238,50.34828483045567
150,301,150,451,0.2113800048828125,49.92927072969201
155,311,155,466,0.21968793869018555,49.38915824350374
160,321,160,481,0.22803378105163574,48.83349698253892
164,329,164,493,0.23465204238891602,48.38066761506502
169,339,169,508,0.2427070140838623,47.808346037700176
173,347,173,520,0.25225305557250977,47.34865389378115
178,357,178,535,0.2617518901824951,46.77607651772769
182,365,182,547,0.26886677742004395,46.32248067424712
187,375,187,562,0.2780628204345703,45.76350953952533
192,385,192,577,0.28694677352905273,45.2139030816802
196,393,196,589,0.2934868335723877,44.779953190588685
201,403,201,604,0.30580997467041016,44.242660525023666
205,411,205,616,0.3157539367675781,43.815568779795285
210,421,210,631,0.32678890228271484,43.28382497862117
214,429,214,643,0.33498406410217285,42.8594880498008
219,439,219,658,0.34273791313171387,42.32973697368698
223,447,223,670,0.3491659164428711,41.906030828599114
228,457,228,685,0.35684990882873535,41.37594521439587
233,467,233,700,0.36447691917419434,40.84477224257489
237,475,237,712,0.3710191249847412,40.41869288449129
242,485,242,727,0.3817627429962158,39.88436746223124
246,493,246,739,0.38876795768737793,39.45548068444032
251,503,251,754,0.3971569538116455,38.91787524273991
255,511,255,766,0.40354490280151367,38.48710832692518
260,521,260,781,0.4116690158843994,37.94886614165375
265,531,265,796,0.4197659492492676,37.41232836878453
269,539,269,808,0.42676472663879395,36.9853949270489
274,549,274,823,0.43463683128356934,36.45572776871859
278,557,278,835,0.4408390522003174,36.035777873435336
283,567,283,850,0.4486348628997803,35.515977090220304
287,575,287,862,0.4546818733215332,35.104302450518844
292,585,292,877,0.4623398780822754,34.59476542014545
296,593,296,889,0.46848487854003906,34.1909875643305
301,603,301,904,0.47624778747558594,33.690831385122465
306,613,306,919,0.4840869903564453,33.195588629829444
310,621,310,931,0.490386962890625,32.802918095914265
315,631,315,946,0.49816083908081055,32.31655594594258
319,639,319,958,0.5040369033813477,31.931099714866377
324,649,324,973,0.5114378929138184,31.453811173767008
328,657,328,985,0.5182418823242188,31.075512708542874
333,667,333,1000,0.5291850566864014,30.60683691556187
337,675,337,1012,0.535559892654419,30.235068553143492
342,685,342,1027,0.5432078838348389,29.774116420396467
347,695,347,1042,0.5506210327148438,29.31722515055685
351,703,351,1054,0.556704044342041,28.95464893458916
356,713,356,1069,0.5645039081573486,28.50522798750285
360,721,360,1081,0.571448802947998,28.14887581576454
365,731,365,1096,0.583000898361206,27.70762615880153
369,739,369,1108,0.5890870094299316,27.358109050643407
374,749,374,1123,0.5965650081634521,26.92567026992174
379,759,379,1138,0.603538990020752,26.49820389088518
383,767,383,1150,0.6085379123687744,26.159769815116306
388,777,388,1165,0.6157279014587402,25.741057686879458
392,785,392,1177,0.6225359439849854,25.409475980466596
397,795,397,1192,0.6317269802093506,24.99914032670722
401,803,401,1204,0.6385118961334229,24.674124810152307
406,813,406,1219,0.647406816482544,24.271844947119916
410,821,410,1231,0.6541519165039062,23.953150333218446
415,831,415,1246,0.6619091033935547,23.558594156326535
420,841,420,1261,0.6690230369567871,23.16814416867078
424,849,424,1273,0.6747877597808838,22.858640213780063
429,859,429,1288,0.6824090480804443,22.475208243453153
433,867,433,1300,0.6870858669281006,22.171142587771783
438,877,438,1315,0.6928339004516602,21.79433103128008
442,885,442,1327,0.6974759101867676,21.495461233985452
447,895,447,1342,0.7033600807189941,21.12507498190871
451,903,451,1354,0.7079470157623291,20.83132344287833
456,913,456,1369,0.7139449119567871,20.46733606873454
461,923,461,1384,0.7197918891906738,20.106915813559453
465,931,465,1396,0.7246799468994141,19.821154891500782
470,941,470,1411,0.7345118522644043,19.467183120473464
474,949,474,1423,0.7411129474639893,19.186627262391312
479,959,479,1438,0.7471029758453369,18.839202110637416
483,967,483,1450,0.7517929077148438,18.563890703470634
488,977,488,1465,0.7575778961181641,18.22306292194753
493,987,493,1480,0.7633848190307617,17.885935216414964
497,995,497,1492,0.7681689262390137,17.618901135066608
502,1005,502,1507,0.7794640064239502,17.28842966477191
506,1013,506,1519,0.7851049900054932,17.026685481543154
511,1023,511,1534,0.7906818389892578,16.70275075904965
515,1031,515,1546,0.795191764831543,16.44616116392035
520,1041,520,1561,0.8008899688720703,16.128573898694867
524,1049,524,1573,0.8053348064422607,15.876996022481421
529,1059,529,1588,0.8110549449920654,15.565615100192645
534,1069,534,1603,0.8165929317474365,15.257658010921318
538,1077,538,1615,0.8210890293121338,15.013756043115563
543,1087,543,1630,0.8268020153045654,14.711958585836442
547,1095,547,1642,0.831981897354126,14.472982681018607
552,1105,552,1657,0.8375980854034424,14.177332639971041
556,1113,556,1669,0.8419489860534668,13.943259897983125
561,1123,561,1684,0.8476920127868652,13.653716932658654
566,1133,566,1699,0.853212833404541,13.36755499194328
570,1141,570,1711,0.8576920032501221,13.141063913062453
575,1151,575,1726,0.8631899356842041,12.861015855374035
579,1159,579,1738,0.8676979541778564,12.639450753999768
584,1169,584,1753,0.8737390041351318,12.365619523619443
588,1177,588,1765,0.8789031505584717,12.149079416987888
593,1187,593,1780,0.8846840858459473,11.881587944614353
597,1195,597,1792,0.889319896697998,11.670155076153492
602,1205,602,1807,0.8948848247528076,11.409071201653092
607,1215,607,1822,0.9005169868469238,11.151546047860506
611,1223,611,1834,0.9052670001983643,10.948077843647297
616,1233,616,1849,0.9110219478607178,10.69691315106013
620,1241,620,1861,0.9176018238067627,10.498500710600865
625,1251,625,1876,0.9262869358062744,10.253609254923049
629,1259,629,1888,0.9314048290252686,10.060176215003025
634,1269,634,1903,0.9371569156646729,9.821459751648604
638,1277,638,1915,0.9417328834533691,9.632928987784112
643,1287,643,1930,0.9474470615386963,9.400298575587271
648,1297,648,1945,0.9532818794250488,9.171022312944388
652,1305,652,1957,0.957838773727417,8.990010283336233
657,1315,657,1972,0.9633948802947998,8.766756701320787
661,1323,661,1984,0.968193769454956,8.590568141575318
666,1333,666,1999,0.974635124206543,8.373362138447987
670,1341,670,2011,0.9792039394378662,8.202031703210878
675,1351,675,2026,0.9849889278411865,7.990925689911251
680,1361,680,2041,0.9905989170074463,7.783229145637279
684,1369,684,2053,0.9951379299163818,7.619532821557755
689,1379,689,2068,1.0007050037384033,7.4179915223913895
693,1387,693,2080,1.0051679611206055,7.25922078543033
698,1397,698,2095,1.0108129978179932,7.06383002618486
702,1405,702,2107,1.0155839920043945,6.909968999084981
707,1415,707,2122,1.0216331481933594,6.720694806746678
711,1423,711,2134,1.026425838470459,6.571705137752133
716,1433,716,2149,1.0323069095611572,6.388485076060192
721,1443,721,2164,1.0380299091339111,6.208590475753454
725,1451,725,2176,1.042454719543457,6.067047308662836
730,1461,730,2191,1.0480749607086182,5.893054672673429
734,1469,734,2203,1.0525970458984375,5.756187601161514
739,1479,739,2218,1.058218002319336,5.587984272487688
743,1487,743,2230,1.0627260208129883,5.455707011671279
748,1497,748,2245,1.068444013595581,5.293195162420261
752,1505,752,2257,1.074145793914795,5.1654398938167105
757,1515,757,2272,1.0811328887939453,5.008548666132242
762,1525,762,2287,1.0869340896606445,4.854758117711185
766,1533,766,2299,1.0914459228515625,4.73394953278364
771,1543,771,2314,1.0970361232757568,4.585708191257709
775,1551,775,2326,1.1018540859222412,4.46932238278373
780,1561,780,2341,1.1073479652404785,4.326586556777897
784,1569,784,2353,1.1118619441986084,4.21458400679262
789,1579,789,2368,1.1176810264587402,4.0772958951991995
794,1589,794,2383,1.1236238479614258,3.9430015662455844
798,1597,798,2395,1.1283111572265625,3.8377027762541047
803,1607,803,2410,1.134186029434204,3.7087239211547285
807,1615,807,2422,1.1387898921966553,3.607635713046193
812,1625,812,2437,1.1444838047027588,3.4838650531818303
816,1633,816,2449,1.1490728855133057,3.3868986091982833
821,1643,821,2464,1.1546781063079834,3.268224791989155
825,1651,825,2476,1.1592469215393066,3.175292937862878
830,1661,830,2491,1.1649549007415771,3.061611277554448
835,1671,835,2506,1.1708159446716309,2.9506612982884235
839,1679,839,2518,1.1754648685455322,2.8638489584936906
844,1689,844,2533,1.181152105331421,2.7577442638909133
848,1697,848,2545,1.1855719089508057,2.674771098145243
853,1707,853,2560,1.1912047863006592,2.5734178712216362
857,1715,857,2572,1.1957488059997559,2.4942065686138903
862,1725,862,2587,1.2014808654785156,2.397504537380655
867,1735,867,2602,1.2072038650512695,2.3033404339682875
871,1743,871,2614,1.211824893951416,2.229813512816918
876,1753,876,2629,1.2175350189208984,2.140131120316596
880,1761,880,2641,1.222689151763916,2.070144362877045
885,1771,885,2656,1.2291457653045654,1.9848304953585512
889,1779,889,2668,1.2345249652862549,1.918293465458646
894,1789,894,2683,1.2402808666229248,1.8372361760960985
898,1797,898,2695,1.2448740005493164,1.7740607564173843
903,1807,903,2710,1.250601053237915,1.6971520945412522
908,1817,908,2725,1.2562110424041748,1.6225030310066586
912,1825,912,2737,1.260706901550293,1.564389189575877
917,1835,917,2752,1.2663748264312744,1.4937264601271636
921,1843,921,2764,1.2716097831726074,1.4387592172002996
926,1853,926,2779,1.2778599262237549,1.371974918841488
930,1861,930,2791,1.2825889587402344,1.3200648891820492
935,1871,935,2806,1.2882587909698486,1.2570426954473533
939,1879,939,2818,1.2927989959716797,1.2080930153356348
944,1889,944,2833,1.298487901687622,1.1487075278225802
949,1899,949,2848,1.3042020797729492,1.0912859938341626
953,1907,953,2860,1.3085949420928955,1.0467354776787943
958,1917,958,2875,1.3141670227050781,0.9927469211850166
962,1925,962,2887,1.318711757659912,0.9508912458189798
967,1935,967,2902,1.3250908851623535,0.9002088814869467
971,1943,971,2914,1.3301539421081543,0.8609503786333335
976,1953,976,2929,1.3359529972076416,0.8134581379129031
981,1963,981,2944,1.3418629169464111,0.767693079837386
985,1971,985,2956,1.346506118774414,0.7323047735238788
990,1981,990,2971,1.3526217937469482,0.6895755773830388
994,1989,994,2983,1.3573870658874512,0.656580220521505
999,1999,999,2998,1.3635740280151367,0.6167982410213426
1003,2007,1003,3010,1.3682167530059814,0.586125093566011
1008,2017,1008,3025,1.3742239475250244,0.5491998170975876
1012,2025,1012,3037,1.3799450397491455,0.5207734104808424
1017,2035,1017,3052,1.3858540058135986,0.4866055213284426
1022,2045,1022,3067,1.391706943511963,0.45392276140569265
1026,2053,1026,3079,1.39652681350708,0.4288222652414788
1031,2063,1031,3094,1.4023487567901611,0.3987237195681246
1035,2071,1035,3106,1.4068498611450195,0.3756441261219834
1040,2081,1040,3121,1.4125518798828125,0.3480138088195872
1044,2089,1044,3133,1.4175560474395752,0.32686314270824823
1049,2099,1049,3148,1.4237167835235596,0.30158829718675406
1053,2107,1053,3160,1.4288179874420166,0.28227865297367316
1058,2117,1058,3175,1.435241937637329,0.25925244438667505
1063,2127,1063,3190,1.441270112991333,0.23743119141022362
1067,2135,1067,3202,1.4462201595306396,0.22082086604859796
1072,2145,1072,3217,1.4522850513458252,0.20109022528572496
1076,2153,1076,3229,1.4569988250732422,0.18611205532022268
1081,2163,1081,3244,1.4633679389953613,0.1683709090151524
1085,2171,1085,3256,1.4684059619903564,0.15494364473022415
1090,2181,1090,3271,1.4744579792022705,0.13909050431061587
1095,2191,1095,3286,1.480578899383545,0.12424346140062426
1099,2199,1099,3298,1.4852187633514404,0.11307068200221693
1104,2209,1104,3313,1.4920458793640137,0.09996278264441116
1108,2217,1108,3325,1.4966418743133545,0.09014696674057632
1113,2227,1113,3340,1.5024700164794922,0.07869531592541534
1117,2235,1117,3352,1.5079219341278076,0.0701745379312797
1122,2245,1122,3367,1.5135319232940674,0.06030626747985934
1126,2253,1126,3379,1.5182170867919922,0.053024685727223186
1131,2263,1131,3394,1.5243017673492432,0.044671098483036076
1136,2273,1136,3409,1.530411958694458,0.03712834739292248
1140,2281,1140,3421,1.5350759029388428,0.03166222405980079
1145,2291,1145,3436,1.5408987998962402,0.025518793508467752
1149,2299,1149,3448,1.5454089641571045,0.021139105461088548
1154,2309,1154,3463,1.551048994064331,0.01631047345006209
1158,2317,1158,3475,1.5555920600891113,0.012946987328632531
1163,2327,1163,3490,1.5614349842071533,0.009343420959226023
1168,2337,1168,3505,1.567288875579834,0.0063816761188491
1172,2345,1172,3517,1.5720510482788086,0.00445641465614699
1177,2355,1177,3532,1.5778439044952393,0.0025835270397465138
1181,2363,1181,3544,1.582615852355957,0.0014970074001894318
1186,2373,1186,3559,1.5883710384368896,0.0006342480769490066
1190,2381,1190,3571,1.5929317474365234,0.0003266816243012727
1195,2391,1195,3586,1.5987091064453125,0.00040287007766437455
1199,2399,1199,3598,1.603261947631836,0.0008196230595558518
1204,2409,1204,3613,1.6088998317718506,0.0017685459372387413
1209,2419,1209,3628,1.6146299839019775,0.0031746293495871214
1213,2427,1213,3640,1.6192739009857178,0.004615571170688781
1218,2437,1218,3655,1.625791072845459,0.00679574581408815
1222,2445,1222,3667,1.6307017803192139,0.008831391092144258
1227,2455,1227,3682,1.6364197731018066,0.011725085590342132
1231,2463,1231,3694,1.640854835510254,0.014308477568761191
1236,2473,1236,3709,1.6464331150054932,0.01785928385106672
1240,2481,1240,3721,1.6509368419647217,0.020947263164089236
1245,2491,1245,3736,1.6565239429473877,0.02510355709966916
1250,2501,1250,3751,1.6621809005737305,0.029575179728453804
1254,2509,1254,3763,1.6667537689208984,0.03336955365045924
1259,2519,1259,3778,1.67252779006958,0.038371251428884534
1263,2527,1263,3790,1.6774730682373047,0.042569975265678295
1268,2537,1268,3805,1.6838629245758057,0.0480517101316309
1272,2545,1272,3817,1.688429832458496,0.052613508742410886
1277,2555,1277,3832,1.694303035736084,0.058522141630078295
1282,2565,1282,3847,1.7001910209655762,0.06464421919508823
1286,2573,1286,3859,1.7047100067138672,0.06968419402062409
1291,2583,1291,3874,1.7105748653411865,0.07614816373165922
1295,2591,1295,3886,1.7152600288391113,0.08144059136623127
1300,2601,1300,3901,1.7214338779449463,0.08819492369377713
1304,2609,1304,3913,1.7302470207214355,0.09370044486752249
1309,2619,1309,3928,1.7365119457244873,0.10069847189652137
1313,2627,1313,3940,1.7411751747131348,0.10638171384505313
1318,2637,1318,3955,1.746971845626831,0.11358136338003533
1323,2647,1323,3970,1.752701997756958,0.12087603521740675
1327,2655,1327,3982,1.7572789192199707,0.12677232587384424
1332,2665,1332,3997,1.7629518508911133,0.13420878094859745
1336,2673,1336,4009,1.767552137374878,0.1402038656235618
1341,2683,1341,4024,1.7769339084625244,0.14774607083938918
1345,2691,1345,4036,1.781944751739502,0.15381208087603682
1350,2701,1350,4051,1.7875988483428955,0.16142670521389846
1354,2709,1354,4063,1.792184829711914,0.1675383765857532
1359,2719,1359,4078,1.7978699207305908,0.17519571084449126
1364,2729,1364,4093,1.8036308288574219,0.18286519955302083
1368,2737,1368,4105,1.8080329895019531,0.18900430370717913
1373,2747,1373,4120,1.8137400150299072,0.19667613300839548
1377,2755,1377,4132,1.8182649612426758,0.20280713000909145
1382,2765,1382,4147,1.8244900703430176,0.21045612525608703
1386,2773,1386,4159,1.8295259475708008,0.21655839510458463
1391,2783,1391,4174,1.835669994354248,0.2241579444777244
1396,2793,1396,4189,1.8413138389587402,0.23171794608254004
1400,2801,1400,4201,1.845716953277588,0.23773158453570886
1405,2811,1405,4216,1.8525588512420654,0.24519840295840822
1409,2819,1409,4228,1.8571209907531738,0.25112642921499173
1414,2829,1414,4243,1.8627779483795166,0.25847294605819116
1418,2837,1418,4255,1.8672678470611572,0.26429464730347263
1423,2847,1423,4270,1.8741869926452637,0.27149649591933667
1427,2855,1427,4282,1.8789761066436768,0.27719369913472747
1432,2865,1432,4297,1.885037899017334,0.2842297925882349
1437,2875,1437,4312,1.8906638622283936,0.2911657427000591
1441,2883,1441,4324,1.895164966583252,0.2966388357388041
1446,2893,1446,4339,1.9007837772369385,0.30338138255899594
1450,2901,1450,4351,1.9052281379699707,0.308693344463677
1455,2911,1455,4366,1.9109320640563965,0.31522679332988446
1459,2919,1459,4378,1.9155139923095703,0.3203655661409357
1464,2929,1464,4393,1.9220287799835205,0.3266754834620542
1469,2939,1469,4408,1.9300718307495117,0.33285551201515773
1473,2947,1473,4420,1.9380578994750977,0.3377035089565652
1478,2957,1478,4435,1.9443888664245605,0.34364057182256147
1482,2965,1482,4447,1.9489538669586182,0.3482898710412883
1487,2975,1487,4462,1.9546990394592285,0.35397352773134116
1491,2983,1491,4474,1.9591879844665527,0.35841629670835573
1496,2993,1496,4489,1.9650850296020508,0.36383724781910587
1500,3001,1500,4501,1.9697070121765137,0.36806631788851973
1505,3011,1505,4516,1.9760048389434814,0.37321580295986223
1510,3021,1510,4531,1.9816999435424805,0.37821076651937346
1514,3029,1514,4543,1.9862017631530762,0.3820937344437425
1519,3039,1519,4558,1.991832971572876,0.3868040668027106
1523,3047,1523,4570,1.9963138103485107,0.3904561182243924
1528,3057,1528,4585,2.0021488666534424,0.39487399577137694
1532,3065,1532,4597,2.0067217350006104,0.39828922579761183
1537,3075,1537,4612,2.012410879135132,0.40240779158216355
1541,3083,1541,4624,2.017190933227539,0.40558116428962876
1546,3093,1546,4639,2.0230910778045654,0.40939468349733943
1551,3103,1551,4654,2.0290608406066895,0.41303663236908505
1555,3111,1555,4666,2.0339109897613525,0.41582577682163446
1560,3121,1560,4681,2.0397651195526123,0.41915569812363174
1564,3129,1564,4693,2.0442121028900146,0.4216937773585414
1569,3139,1569,4708,2.049907922744751,0.4247083125989093
1573,3147,1573,4720,2.0544850826263428,0.42699305678752353
1578,3157,1578,4735,2.0601518154144287,0.42968998489152455
1583,3167,1583,4750,2.065903902053833,0.43221004483336856
1587,3175,1587,4762,2.0707569122314453,0.4340987761671613
1592,3185,1592,4777,2.07686185836792,0.43630079786066744
1596,3193,1596,4789,2.081799030303955,0.43793562395899244
1601,3203,1601,4804,2.0874650478363037,0.4398212441248006
1605,3211,1605,4816,2.0920729637145996,0.44120391145406757
1610,3221,1610,4831,2.0978949069976807,0.44277568641837206
1614,3229,1614,4843,2.102555990219116,0.4439084102241395
1619,3239,1619,4858,2.108350992202759,0.44516917572673265
1624,3249,1624,4873,2.1155669689178467,0.446258350743733
1628,3257,1628,4885,2.122663974761963,0.4470066969166737
1633,3267,1633,4900,2.1289138793945312,0.447789072085925
1637,3275,1637,4912,2.1335837841033936,0.4482930471818918
1642,3285,1642,4927,2.1392440795898438,0.4487713497868526
1646,3293,1646,4939,2.143808126449585,0.44903325114171366
1651,3303,1651,4954,2.149472951889038,0.4492105709310863
1655,3311,1655,4966,2.1541409492492676,0.4492330864864016
1660,3321,1660,4981,2.1597959995269775,0.4491130902065379
1665,3331,1665,4996,2.1654469966888428,0.4488297460480908
1669,3339,1669,5008,2.1703057289123535,0.4484864354686806
1674,3349,1674,5023,2.176527976989746,0.447912824377795
1678,3357,1678,5035,2.1813488006591797,0.44733941641140973
1683,3367,1683,5050,2.1869897842407227,0.4464810472999261
1687,3375,1687,5062,2.191577911376953,0.44568229885919664
1692,3385,1692,5077,2.1971800327301025,0.4445455839611441
1697,3395,1697,5092,2.2029359340667725,0.44325735464622085
1701,3403,1701,5104,2.207468032836914,0.4421193022105854
1706,3413,1706,5119,2.213181972503662,0.44056452103268384
1710,3421,1710,5131,2.2176709175109863,0.4392165436019013
1715,3431,1715,5146,2.2237179279327393,0.43740358965953874
1719,3439,1719,5158,2.2284088134765625,0.4358524794832874
1724,3449,1724,5173,2.234375,0.4337898357315453
1728,3457,1728,5185,2.238968849182129,0.43204230142430333
1733,3467,1733,5200,2.2446439266204834,0.42973819667065527
1738,3477,1738,5215,2.2504630088806152,0.4273033811781488
1742,3485,1742,5227,2.2550108432769775,0.4252630400681028
1747,3495,1747,5242,2.2606987953186035,0.42259903989588565
1751,3503,1751,5254,2.265220880508423,0.42037852079306504
1756,3513,1756,5269,2.2709670066833496,0.4174933574967099
1760,3521,1760,5281,2.2756638526916504,0.41509925916716384
1765,3531,1765,5296,2.281571865081787,0.4120014772199738
1769,3539,1769,5308,2.286026954650879,0.40944089836148123
1774,3549,1774,5323,2.291680097579956,0.4061397001214573
1779,3559,1779,5338,2.2975308895111084,0.4027296806686991
1783,3567,1783,5350,2.302053928375244,0.39992538149545
1788,3577,1788,5365,2.3077011108398438,0.3963272736733643
1792,3585,1792,5377,2.313264846801758,0.39337656406496535
1797,3595,1797,5392,2.3189408779144287,0.3896005575121535
1801,3603,1801,5404,2.3236968517303467,0.38651164262705606
1806,3613,1806,5419,2.3297390937805176,0.38256804949946854
1811,3623,1811,5434,2.3355050086975098,0.37853584958168085
1815,3631,1815,5446,2.3400259017944336,0.37524846713608895
1820,3641,1820,5461,2.3456709384918213,0.3710649405835511
1824,3649,1824,5473,2.350245952606201,0.36766071136719347
1829,3659,1829,5488,2.3558928966522217,0.3633363931299982
1833,3667,1833,5500,2.3604679107666016,0.3598237281088359
1838,3677,1838,5515,2.3661229610443115,0.3553690708274644
1842,3685,1842,5527,2.370837926864624,0.35175625698957447
1847,3695,1847,5542,2.3765339851379395,0.34718150272419734
1852,3705,1852,5557,2.3823559284210205,0.3425443666509409
1856,3713,1856,5569,2.3868439197540283,0.33879180263829767
1861,3723,1861,5584,2.3923699855804443,0.334050097346676
1865,3731,1865,5596,2.3969268798828125,0.3302178471616344
1870,3741,1870,5611,2.4026451110839844,0.3253815244249836
1874,3749,1874,5623,2.4070990085601807,0.3214776090663918
1879,3759,1879,5638,2.4128270149230957,0.316556801614297
1884,3769,1884,5653,2.4185149669647217,0.3115935236100995
1888,3777,1888,5665,2.423103094100952,0.30759449273102746
1893,3787,1893,5680,2.4287660121917725,0.3025629206360918
1897,3795,1897,5692,2.433612823486328,0.2985134642676712
1902,3805,1902,5707,2.439350128173828,0.29342411963455106
1906,3813,1906,5719,2.443833827972412,0.28933263953592814
1911,3823,1911,5734,2.4495980739593506,0.28419598208324715
1915,3831,1915,5746,2.454103946685791,0.28007080456404765
1920,3841,1920,5761,2.459714889526367,0.2748971922496821
1925,3851,1925,5776,2.4653000831604004,0.269707497589593
1929,3859,1929,5788,2.46972393989563,0.26554629120164464
1934,3869,1934,5803,2.4754638671875,0.2603356234359353
1938,3877,1938,5815,2.480093002319336,0.2561617236268603
1943,3887,1943,5830,2.48579478263855,0.2509402620989931
1947,3895,1947,5842,2.490295171737671,0.24676174566263853
1952,3905,1952,5857,2.4959559440612793,0.24153945803357146
1956,3913,1956,5869,2.5005829334259033,0.23736416012184236
1961,3923,1961,5884,2.5062568187713623,0.23215062168685563
1966,3933,1966,5899,2.5120248794555664,0.22694589265461218
1970,3941,1970,5911,2.5171427726745605,0.22279027250556283
1975,3951,1975,5926,2.5228397846221924,0.21760816056382737
1979,3959,1979,5938,2.5274529457092285,0.21347400449394627
1984,3969,1984,5953,2.533313035964966,0.20832284584491845
1988,3977,1988,5965,2.5377800464630127,0.20421670430994254
1993,3987,1993,5980,2.543332815170288,0.1991045921922705
1998,3997,1998,5995,2.5490479469299316,0.19401764204917527
2002,4005,2002,6007,2.55351185798645,0.18996786670015808
2007,4015,2007,6022,2.5591378211975098,0.18493247041101313
2011,4023,2011,6034,2.5637331008911133,0.18092716959370136
2016,4033,2016,6049,2.569563865661621,0.17595141248796153
2020,4041,2020,6061,2.574144124984741,0.1719970583559416
2025,4051,2025,6076,2.5799827575683594,0.16708901617960237
2029,4059,2029,6088,2.584510087966919,0.16319204172452828
2034,4069,2034,6103,2.590287923812866,0.1583596996132428
2039,4079,2039,6118,2.5958800315856934,0.1535728035696593
2043,4087,2043,6130,2.6004600524902344,0.14977760383112582
2048,4097,2048,6145,2.6060569286346436,0.14507845615889892
2052,4105,2052,6157,2.6105339527130127,0.14135643885231275
2057,4115,2057,6172,2.616209030151367,0.13675239938538652
2061,4123,2061,6184,2.6208059787750244,0.13310928483133466
2066,4133,2066,6199,2.6268019676208496,0.12860725600876322
2070,4141,2070,6211,2.6315829753875732,0.12504833950413285
2075,4151,2075,6226,2.637249708175659,0.12065462391012716
2080,4161,2080,6241,2.643018960952759,0.11632355302288033
2084,4169,2084,6253,2.6475889682769775,0.11290488851648206
2089,4179,2089,6268,2.653204917907715,0.10869056901185559
2093,4187,2093,6280,2.657721996307373,0.10536721063851928
2098,4197,2098,6295,2.663367986679077,0.10127426710664622
2102,4205,2102,6307,2.6679229736328125,0.09804972014558189
2107,4215,2107,6322,2.6736998558044434,0.0940823419177832
2112,4225,2112,6337,2.679642915725708,0.09018643478816557
2116,4233,2116,6349,2.6844959259033203,0.08712196955161744
2121,4243,2121,6364,2.6901509761810303,0.0833577031941104
2125,4251,2125,6376,2.6947360038757324,0.08040007077829614
2130,4261,2130,6391,2.700612783432007,0.07677122758855148
2134,4269,2134,6403,2.70544171333313,0.07392342414675568
2139,4279,2139,6418,2.7115049362182617,0.07043370412202421
2143,4287,2143,6430,2.716114044189453,0.06769864410557602
2148,4297,2148,6445,2.7218990325927734,0.06435161865647387
2153,4307,2153,6460,2.7277328968048096,0.06108534486315875
2157,4315,2157,6472,2.7325329780578613,0.05853114448029828
2162,4325,2162,6487,2.738111972808838,0.05541272778657458
2166,4333,2166,6499,2.742609977722168,0.05297803409609969
2171,4343,2171,6514,2.7482528686523438,0.050010441499011904
2175,4351,2175,6526,2.7527198791503906,0.047697486161382585
2180,4361,2180,6541,2.7583377361297607,0.04488330102731197
2185,4371,2185,6556,2.764216899871826,0.04215527814176312
2189,4379,2189,6568,2.768803834915161,0.040035264190919406
2194,4389,2194,6583,2.774867057800293,0.03746362324545771
2198,4397,2198,6595,2.779520034790039,0.03546922236671435
2203,4407,2203,6610,2.7851641178131104,0.03305505675064069
2207,4415,2207,6622,2.789700984954834,0.03118687458959357
2212,4425,2212,6637,2.795320749282837,0.02893061570921418
2216,4433,2216,6649,2.7999298572540283,0.027188753694531442
2221,4443,2221,6664,2.8056068420410156,0.025090256255111854
2226,4453,2226,6679,2.81123685836792,0.02307917680798255
2230,4461,2230,6691,2.8157310485839844,0.021533099941962064
2235,4471,2235,6706,2.821603775024414,0.01967876361322851
2239,4479,2239,6718,2.8263649940490723,0.01825772059260089
2244,4489,2244,6733,2.8322629928588867,0.01655918961535008
2248,4497,2248,6745,2.8368120193481445,0.015262381673551317
2253,4507,2253,6760,2.8423879146575928,0.013718612215939174
2257,4515,2257,6772,2.846949815750122,0.012545173648163654
2262,4525,2262,6787,2.8526108264923096,0.011155045998975766
2267,4535,2267,6802,2.85829496383667,0.009849757899473843
2271,4543,2271,6814,2.8627641201019287,0.00886634595576652
2276,4553,2276,6829,2.869572877883911,0.00771274803344113
2280,4561,2280,6841,2.874551773071289,0.0068501175799156044
2285,4571,2285,6856,2.880380868911743,0.005846719507076159
2289,4579,2289,6868,2.884855031967163,0.005103569820334997
2294,4589,2294,6883,2.8904950618743896,0.004248582176387572
2299,4599,2299,6898,2.8961679935455322,0.0034751263308407943
2303,4607,2303,6910,2.900702953338623,0.0029145584115894962
2308,4617,2308,6925,2.9065070152282715,0.002285892548911761
2312,4625,2312,6937,2.910989761352539,0.0018400238277536118
2317,4635,2317,6952,2.916653871536255,0.001353182938714781
2321,4643,2321,6964,2.9213907718658447,0.0010194396409133333
2326,4653,2326,6979,2.927323818206787,0.0006709685461601111
2330,4661,2330,6991,2.9319069385528564,0.00044641321198923833
2335,4671,2335,7006,2.9376368522644043,0.0002324530382793455
2340,4681,2340,7021,2.9432787895202637,9.144633145297121e-05
2344,4689,2344,7033,2.9477410316467285,3.0288557468338695e-05
2349,4699,2349,7048,2.953263998031616,1.728579854898271e-05
2353,4707,2353,7060,2.9577369689941406,5.6803480561029573e-05
2358,4717,2358,7075,2.963418960571289,0.00016746933476952108
2362,4725,2362,7087,2.9679927825927734,0.0003041736218847291
2367,4735,2367,7102,2.9743409156799316,0.0005341293931451219
2371,4743,2371,7114,2.979033946990967,0.000764504842209135
2376,4753,2376,7129,2.984807014465332,0.0011093380454667567
2381,4763,2381,7144,2.990431070327759,0.001516066194085397
2385,4771,2385,7156,2.9949378967285156,0.0018850775865075775
2390,4781,2390,7171,3.0004889965057373,0.002399694086989257
2394,4789,2394,7183,3.0051138401031494,0.0028531773432405316
2399,4799,2399,7198,3.0107178688049316,0.0034710490223233137
2403,4807,2403,7210,3.0153439044952393,0.004005237663591288
2408,4817,2408,7225,3.0210719108581543,0.004721570465221703
2413,4827,2413,7240,3.0269358158111572,0.005490460180908485
2417,4835,2417,7252,3.0315659046173096,0.006142353299196657
2422,4845,2422,7267,3.037226915359497,0.007001840708085183
2426,4853,2426,7279,3.0417869091033936,0.007724098692506232
2431,4863,2431,7294,3.047287940979004,0.008668843684404237
2435,4871,2435,7306,3.0518698692321777,0.00945710961389068
2440,4881,2440,7321,3.057485818862915,0.01048156996034777
2444,4889,2444,7333,3.0620779991149902,0.011331343281199224
2449,4899,2449,7348,3.0677058696746826,0.012429826024913382
2454,4909,2454,7363,3.0737040042877197,0.01356693868444836
2458,4917,2458,7375,3.0783729553222656,0.014503239653208766
2463,4927,2463,7390,3.084047794342041,0.015705375538914268
2467,4935,2467,7402,3.088510036468506,0.016691376745143316
2472,4945,2472,7417,3.094241142272949,0.01795274754726961
2476,4953,2476,7429,3.098855972290039,0.018983832999765582
2481,4963,2481,7444,3.1044528484344482,0.020298694050438826
2486,4973,2486,7459,3.110037088394165,0.021640812573650692
2490,4981,2490,7471,3.1145098209381104,0.022732962256668543
2495,4991,2495,7486,3.120450735092163,0.0241197650121876
2499,4999,2499,7498,3.125549793243408,0.02524542763512727
2504,5009,2504,7513,3.1348938941955566,0.02667134762123169
2508,5017,2508,7525,3.1411657333374023,0.0278260983278642
2513,5027,2513,7540,3.1469359397888184,0.02928563756472613
2517,5035,2517,7552,3.1515719890594482,0.030465101103573033
2522,5045,2522,7567,3.1571080684661865,0.031952813396401325
2527,5055,2527,7582,3.1627390384674072,0.03345383436897009
2531,5063,2531,7594,3.167263984680176,0.03466310951819196
2536,5073,2536,7609,3.1731419563293457,0.03618387015387725
2540,5081,2540,7621,3.1776540279388428,0.03740676567849732
2545,5091,2545,7636,3.1832997798919678,0.03894183295210496
2549,5099,2549,7648,3.187757730484009,0.0401739958148255
2554,5109,2554,7663,3.1934139728546143,0.04171792349200132
2558,5117,2558,7675,3.1979708671569824,0.042954997922720395
2563,5127,2563,7690,3.203721046447754,0.04450235307808725
2568,5137,2568,7705,3.2093489170074463,0.04604928540629771
2572,5145,2572,7717,3.2137937545776367,0.047285423996072495
2577,5155,2577,7732,3.219489812850952,0.04882747878173177
2581,5163,2581,7744,3.224416971206665,0.0500576343706598
2586,5173,2586,7759,3.230199098587036,0.05158965652367442
2590,5181,2590,7771,3.234750986099243,0.05280978251471424
2595,5191,2595,7786,3.2403600215911865,0.05432682134721745
2600,5201,2600,7801,3.245987892150879,0.055833482869502404
2604,5209,2604,7813,3.2506461143493652,0.05703038912292868
2609,5219,2609,7828,3.2563648223876953,0.058514837277584775
2613,5227,2613,7840,3.260793924331665,0.059692211854212474
2618,5237,2618,7855,3.266469955444336,0.06115010288181111
2622,5245,2622,7867,3.2712059020996094,0.06230455823640568
2627,5255,2627,7882,3.2771849632263184,0.063731757773553
2631,5263,2631,7894,3.281888008117676,0.06486005855515486
2636,5273,2636,7909,3.2875258922576904,0.06625260145017364
2641,5283,2641,7924,3.2932469844818115,0.06762422617248376
2645,5291,2645,7936,3.297929048538208,0.06870568119200016
2650,5301,2650,7951,3.3037240505218506,0.07003672798282423
2654,5309,2654,7963,3.30834698677063,0.07108423983447665
2659,5319,2659,7978,3.315074920654297,0.07237103370516706
2663,5327,2663,7990,3.32318377494812,0.0733817064460709
2668,5337,2668,8005,3.3302109241485596,0.0746206903016855
2672,5345,2672,8017,3.3349249362945557,0.07559173636491323
2677,5355,2677,8032,3.3406829833984375,0.07677951081120682
2682,5365,2682,8047,3.346273899078369,0.07793744122977841
2686,5373,2686,8059,3.3509247303009033,0.07884166214500965
2691,5383,2691,8074,3.3565549850463867,0.07994352565106055
2695,5391,2695,8086,3.361158847808838,0.08080174991198419
2700,5401,2700,8101,3.3668220043182373,0.08184476227108917
2704,5409,2704,8113,3.371884822845459,0.08265487706250951
2709,5419,2709,8128,3.3775429725646973,0.08363654185143332
2714,5429,2714,8143,3.3832719326019287,0.0845831508363517
2718,5437,2718,8155,3.38798189163208,0.08531476845735142
2723,5447,2723,8170,3.3935139179229736,0.08619670153620973
2727,5455,2727,8182,3.398198127746582,0.08687582684024164
2732,5465,2732,8197,3.403860092163086,0.0876912645592256
2736,5473,2736,8209,3.408342123031616,0.08831653077436386
2741,5483,2741,8224,3.4138739109039307,0.08906386776084219
2745,5491,2745,8236,3.4184348583221436,0.08963406783288974
2750,5501,2750,8251,3.424499034881592,0.09031188610276786
2755,5511,2755,8266,3.4302449226379395,0.09095053367207129
2759,5519,2759,8278,3.4348130226135254,0.09143300888194972
2764,5529,2764,8293,3.4404890537261963,0.0920002730467786
2768,5537,2768,8305,3.44508695602417,0.09242523259104019
2773,5547,2773,8320,3.4508650302886963,0.09292013896163098
2777,5555,2777,8332,3.455387830734253,0.09328687935862945
2782,5565,2782,8347,3.4609038829803467,0.09370864934510337
2787,5575,2787,8362,3.4666199684143066,0.09408953108231799
2791,5583,2791,8374,3.471695899963379,0.09436470609591652
2796,5593,2796,8389,3.478257894515991,0.0946716814029287
2800,5601,2800,8401,3.4830169677734375,0.09488763077422391
2805,5611,2805,8416,3.488837957382202,0.09512051233139118
2809,5619,2809,8428,3.4935450553894043,0.0952771847855729
2814,5629,2814,8443,3.4994709491729736,0.09543603086626717
2818,5637,2818,8455,3.504450798034668,0.09553356928847734
2823,5647,2823,8470,3.510241746902466,0.09561867555635217
2828,5657,2828,8485,3.5167088508605957,0.09566302545067629
2832,5665,2832,8497,3.521451950073242,0.09566929112611433
2837,5675,2837,8512,3.5281169414520264,0.09564079544190918
2841,5683,2841,8524,3.5329558849334717,0.09558909599820709
2846,5693,2846,8539,3.539255142211914,0.0954885808932886
2850,5701,2850,8551,3.543980121612549,0.0953796494574135
2855,5711,2855,8566,3.5497379302978516,0.09520811765491999
2859,5719,2859,8578,3.554403781890869,0.09504282287582555
2864,5729,2864,8593,3.560241937637329,0.09480144029282656
2869,5739,2869,8608,3.566066026687622,0.0945218123374616
2873,5747,2873,8620,3.5707709789276123,0.0942708633182292
2878,5757,2878,8635,3.5767529010772705,0.09392350128166527
2882,5765,2882,8647,3.5815370082855225,0.09361896921484458
2887,5775,2887,8662,3.589263916015625,0.09320542123543873
2891,5783,2891,8674,3.593965768814087,0.09284860258776462
2896,5793,2896,8689,3.6000759601593018,0.09237056166853108
2901,5803,2901,8704,3.605865955352783,0.09185747631147478
2905,5811,2905,8716,3.610862970352173,0.09142217321459611
2910,5821,2910,8731,3.6170239448547363,0.09084751716977735
2914,5829,2914,8743,3.6218509674072266,0.09036376803328494
2919,5839,2919,8758,3.627586841583252,0.08972960465303004
2923,5847,2923,8770,3.632222890853882,0.08919911687223703
2928,5857,2928,8785,3.6379411220550537,0.08850764968872227
2932,5865,2932,8797,3.6423799991607666,0.08793223990949173
2937,5875,2937,8812,3.6481800079345703,0.08718580428899259
2942,5885,2942,8827,3.6538538932800293,0.08640988435058716
2946,5893,2946,8839,3.6584229469299316,0.08576844092294778
2951,5903,2951,8854,3.664155960083008,0.08494141754988505
2955,5911,2955,8866,3.6686758995056152,0.08426012666348015
2960,5921,2960,8881,3.6746819019317627,0.08338461104119688
2964,5929,2964,8893,3.6794159412384033,0.08266559570859044
2969,5939,2969,8908,3.6851608753204346,0.08174428068980433
2973,5947,2973,8920,3.6897048950195312,0.08098972415848493
2978,5957,2978,8935,3.6954410076141357,0.08002537235665841
2983,5967,2983,8950,3.7011258602142334,0.07903832777287789
2987,5975,2987,8962,3.705620050430298,0.07823294530658131
2992,5985,2992,8977,3.7112619876861572,0.07720728126059839
2996,5993,2996,8989,3.7158589363098145,0.07637216173327488
3001,6003,3001,9004,3.7216148376464844,0.0753107882576387
3005,6011,3005,9016,3.726285934448242,0.0744482806983342
3010,6021,3010,9031,3.732095956802368,0.07335415965599168
3015,6031,3015,9046,3.737783908843994,0.07224314334087012
3019,6039,3019,9058,3.7422099113464355,0.07134279492504447
3024,6049,3024,9073,3.747936964035034,0.07020373212333197
3028,6057,3028,9085,3.7523488998413086,0.06928217156200844
3033,6067,3033,9100,3.758063793182373,0.0681181326119713
3037,6075,3037,9112,3.7626569271087646,0.06717782662269656
3042,6085,3042,9127,3.768317937850952,0.06599190372935482
3046,6093,3046,9139,3.772979974746704,0.06503532962926784
3051,6103,3051,9154,3.7789688110351562,0.06383061892654496
3056,6113,3056,9169,3.7848339080810547,0.06261680359227739
3060,6121,3060,9181,3.7892749309539795,0.0616398321702718
3065,6131,3065,9196,3.7949440479278564,0.060412009349192886
3069,6139,3069,9208,3.7995219230651855,0.05942504753443245
3074,6149,3074,9223,3.8051180839538574,0.05818624539335815
3078,6157,3078,9235,3.809609889984131,0.05719169863425577
3083,6167,3083,9250,3.8152430057525635,0.05594490207386116
3087,6175,3087,9262,3.819689989089966,0.054945140994050234
3092,6185,3092,9277,3.82542085647583,0.05369329266352452
3097,6195,3097,9292,3.83123779296875,0.05243989545408567
3101,6203,3101,9304,3.835783004760742,0.05143666156618565
3106,6213,3106,9319,3.841491937637329,0.05018271886228831
3110,6221,3110,9331,3.8459479808807373,0.04918019501042181
3115,6231,3115,9346,3.8516199588775635,0.047928565633924336
3119,6239,3119,9358,3.856096029281616,0.04692902754675288
3124,6249,3124,9373,3.8616750240325928,0.04568254122887083
3129,6259,3129,9388,3.8674609661102295,0.044440122368996526
3133,6267,3133,9400,3.8720319271087646,0.0434496908710571
3138,6277,3138,9415,3.8778817653656006,0.0422167427605018
3142,6285,3142,9427,3.8826968669891357,0.04123498026820016
3147,6295,3147,9442,3.888439178466797,0.0400142171929474
3151,6303,3151,9454,3.8929879665374756,0.03904326751001008
3156,6313,3156,9469,3.898800849914551,0.037837329755802784
3160,6321,3160,9481,3.9034907817840576,0.03687926985787726
3165,6331,3165,9496,3.909661054611206,0.03569070481125891
3170,6341,3170,9511,3.9154069423675537,0.034512852191483034
3174,6349,3174,9523,3.9200119972229004,0.033578775682485684
3179,6359,3179,9538,3.9261510372161865,0.03242203581078229
3183,6367,3183,9550,3.930975914001465,0.03150576111909231
3188,6377,3188,9565,3.9366719722747803,0.030372380095968765
3192,6385,3192,9577,3.9411678314208984,0.029475653352847075
3197,6395,3197,9592,3.9467568397521973,0.028367751092901017
3202,6405,3202,9607,3.9524857997894287,0.027274875004764
3206,6413,3206,9619,3.956990957260132,0.026411795202307076
3211,6423,3211,9634,3.9627299308776855,0.025347460008333655
3215,6431,3215,9646,3.967345952987671,0.024507956559546074
3220,6441,3220,9661,3.9730279445648193,0.02347399625057278
3224,6449,3224,9673,3.977465867996216,0.02265949870241002
3229,6459,3229,9688,3.9831130504608154,0.021657655830949807
3233,6467,3233,9700,3.9876580238342285,0.020869524267936868
3238,6477,3238,9715,3.993346929550171,0.019901457792798283
3243,6487,3243,9730,3.9991397857666016,0.01895284272529807
3247,6495,3247,9742,4.003619909286499,0.01820827342260145
3252,6505,3252,9757,4.009365081787109,0.017295849927791096
3256,6513,3256,9769,4.013974905014038,0.016580817938461223
3261,6523,3261,9784,4.0198280811309814,0.015706019525850934
3265,6531,3265,9796,4.024526834487915,0.015021628858676195
3270,6541,3270,9811,4.0304200649261475,0.014185777264060562
3274,6549,3274,9823,4.034980773925781,0.01353303501434766
3279,6559,3279,9838,4.040509939193726,0.012737321444546978
3284,6569,3284,9853,4.046156883239746,0.01196436790394273
3288,6577,3288,9865,4.050766944885254,0.011362591919464649
3293,6587,3293,9880,4.056441783905029,0.010631333294213619
3297,6595,3297,9892,4.060895919799805,0.010063249392374018
3302,6605,3302,9907,4.066538095474243,0.0093744851867541
3306,6613,3306,9919,4.0713160037994385,0.008840670621339086
3311,6623,3311,9934,4.07725191116333,0.008195046960054242
3316,6633,3316,9949,4.083354949951172,0.007573617208208816
3320,6641,3320,9961,4.087865829467773,0.00709398393689753
3325,6651,3325,9976,4.093545913696289,0.006516428314853329
3329,6659,3329,9988,4.0982489585876465,0.006072035057854919
3334,6669,3334,10003,4.103919982910156,0.0055386790934335295
3338,6677,3338,10015,4.108475923538208,0.005129747361252157
3343,6687,3343,10030,4.114236831665039,0.004640823155568796
3347,6695,3347,10042,4.118780851364136,0.004267504988206383
3352,6705,3352,10057,4.124696969985962,0.0038231624175750767
3357,6715,3357,10072,4.130875825881958,0.0034036230855463145
3361,6723,3361,10084,4.135429859161377,0.003085855606741461
3366,6733,3366,10099,4.141134977340698,0.002710971304281884
3370,6741,3370,10111,4.145676136016846,0.002428911142146717
3375,6751,3375,10126,4.1514739990234375,0.002098614644182817
3379,6759,3379,10138,4.155967950820923,0.001852167274819294
3384,6769,3384,10153,4.161581754684448,0.0015662855385016883
3388,6777,3388,10165,4.166181802749634,0.0013552657732134321
3393,6787,3393,10180,4.172039031982422,0.0011135054741089334
3398,6797,3398,10195,4.177984952926636,0.0008960825165331698
3402,6805,3402,10207,4.182761907577515,0.0007395644672669732
3407,6815,3407,10222,4.188498020172119,0.0005655458226101473
3411,6823,3411,10234,4.19298791885376,0.00044351266149078583
3416,6833,3416,10249,4.19874382019043,0.0003122687481891262
3420,6841,3420,10261,4.203297853469849,0.00022416673220959638
3425,6851,3425,10276,4.208791732788086,0.00013494614722731058
3430,6861,3430,10291,4.214511871337891,6.870724894270097e-05
3434,6869,3434,10303,4.21896505355835,3.2074598607323423e-05
3439,6879,3439,10318,4.224740982055664,6.485020435320621e-06
3443,6887,3443,10330,4.229359865188599,1.9837827949231723e-06
3448,6897,3448,10345,4.235170841217041,1.6055097717071476e-05
3452,6905,3452,10357,4.239731073379517,4.286767057237739e-05
3457,6915,3457,10372,4.245463848114014,9.554777193443442e-05
3461,6923,3461,10384,4.250020980834961,0.00015281049559234816
3466,6933,3466,10399,4.255573034286499,0.00024299447920839157
3471,6943,3471,10414,4.261337995529175,0.0003535190323873394
3475,6951,3475,10426,4.266077995300293,0.00045633981744686025
3480,6961,3480,10441,4.2720348834991455,0.0006025556048143699
3484,6969,3484,10453,4.276839017868042,0.0007334437607369182
3489,6979,3489,10468,4.282676935195923,0.0009141233346099398
3493,6987,3493,10480,4.2871928215026855,0.0010720755832380746
3498,6997,3498,10495,4.292857885360718,0.001285936407043664
3503,7007,3503,10510,4.298450946807861,0.0015176544865198593
3507,7015,3507,10522,4.3028810024261475,0.0017156000367322122
3512,7025,3512,10537,4.3086419105529785,0.0019783786929110647
3516,7033,3516,10549,4.3133158683776855,0.0022005994887877023
3521,7043,3521,10564,4.319093942642212,0.002492987471782726
3525,7051,3525,10576,4.324351072311401,0.0027382945659155666
3530,7061,3530,10591,4.333079814910889,0.003058771502082891
3534,7069,3534,10603,4.33965277671814,0.0033259222951755874
3539,7079,3539,10618,4.345654010772705,0.00367290411486465
3544,7089,3544,10633,4.351223945617676,0.004033906138488419
3548,7097,3548,10645,4.355699062347412,0.004332457670898293
3553,7107,3553,10660,4.361399173736572,0.0047173987544510965
3557,7115,3557,10672,4.365966796875,0.0050344265492867635
3562,7125,3562,10687,4.371692895889282,0.005441612880190405
3566,7133,3566,10699,4.376415967941284,0.005775753498596714
3571,7143,3571,10714,4.382375955581665,0.006203473946584381
3575,7151,3575,10726,4.38692307472229,0.006553355494361313
3580,7161,3580,10741,4.392685890197754,0.006999894336217949
3585,7171,3585,10756,4.3984479904174805,0.00745614784227655
3589,7179,3589,10768,4.402869939804077,0.00782779110033971
3594,7189,3594,10783,4.408568859100342,0.008300204321130877
3598,7197,3598,10795,4.413088083267212,0.008684095088938193
3603,7207,3603,10810,4.418657064437866,0.00917096923490135
3607,7215,3607,10822,4.423407793045044,0.009565750927777117
3612,7225,3612,10837,4.429343938827515,0.010065391987041039
3617,7235,3617,10852,4.435171842575073,0.010571393609097868
3621,7243,3621,10864,4.439511775970459,0.010980422323541461
3626,7253,3626,10879,4.4451069831848145,0.011496551064396954
3630,7261,3630,10891,4.44962477684021,0.011912999433207005
3635,7271,3635,10906,4.455413103103638,0.012437547489412282
3639,7279,3639,10918,4.459909915924072,0.012860045166462442
3644,7289,3644,10933,4.465657949447632,0.013391295014343996
3648,7297,3648,10945,4.470308780670166,0.013818465236226984
3653,7307,3653,10960,4.476037979125977,0.014354694428220682
3658,7317,3658,10975,4.481836795806885,0.014892946917257177
3662,7325,3662,10987,4.486655950546265,0.015324650839261267
3667,7335,3667,11002,4.492396116256714,0.015865217581335855
3671,7343,3671,11014,4.496914863586426,0.016298095947604452
3676,7353,3676,11029,4.502892732620239,0.016839292915278747
3680,7361,3680,11041,4.507595062255859,0.017272012616331267
3685,7371,3685,11056,4.5135087966918945,0.017812194077805543
3689,7379,3689,11068,4.522937774658203,0.01824345692443785
3694,7389,3694,11083,4.529381990432739,0.01878102505907009
3699,7399,3699,11098,4.535445928573608,0.01931647030221484
3703,7407,3703,11110,4.540010929107666,0.019742983409855697
3708,7417,3708,11125,4.545757055282593,0.020273434794262357
3712,7425,3712,11137,4.550341844558716,0.02069536182614229
3717,7435,3717,11152,4.556116104125977,0.021219354329787166
3721,7443,3721,11164,4.56053900718689,0.021635541858586294
3726,7453,3726,11179,4.566209077835083,0.022151655217953703
3731,7463,3731,11194,4.572041034698486,0.022662791888251377
3735,7471,3735,11206,4.57706093788147,0.02306783514836752
3740,7481,3740,11221,4.583226919174194,0.023568957462998696
3744,7489,3744,11233,4.587682723999023,0.02396545356839397
3749,7499,3749,11248,4.593336820602417,0.024455230616126755
3753,7507,3753,11260,4.597933769226074,0.02484212780325379
3758,7517,3758,11275,4.603526830673218,0.02531926196149925
3762,7525,3762,11287,4.608072996139526,0.02569553686043946
3767,7535,3767,11302,4.613703966140747,0.02615876924312488
3772,7545,3772,11317,4.619338035583496,0.026613751526156193
3776,7553,3776,11329,4.623962879180908,0.02697155196233325
3781,7563,3781,11344,4.629780054092407,0.027410772460484623
3785,7571,3785,11356,4.634382963180542,0.02775550958438089
3790,7581,3790,11371,4.640069961547852,0.028177851313898827
3794,7589,3794,11383,4.644670009613037,0.028508659681619974
3799,7599,3799,11398,4.650478839874268,0.02891307794163822
3804,7609,3804,11413,4.656207799911499,0.029307115872597933
3808,7617,3808,11425,4.660664796829224,0.029614680602094268
3813,7627,3813,11440,4.6662819385528564,0.029989325690053192
3817,7635,3817,11452,4.670721769332886,0.030281030698347422
3822,7645,3822,11467,4.676459074020386,0.030635439424713695
3826,7653,3826,11479,4.681077003479004,0.030910640444062665
3831,7663,3831,11494,4.686809778213501,0.031244044255799963
3835,7671,3835,11506,4.6913957595825195,0.03150215463551831
3840,7681,3840,11521,4.6970908641815186,0.03181385365269307
3845,7691,3845,11536,4.7028419971466064,0.03211321500509712
3849,7699,3849,11548,4.707414865493774,0.032343694891437735
3854,7709,3854,11563,4.713059902191162,0.032620383062180736
3858,7717,3858,11575,4.717684030532837,0.032832497714252895
3863,7727,3863,11590,4.7236528396606445,0.03308595941621206
3867,7735,3867,11602,4.728827953338623,0.033279286835863786
3872,7745,3872,11617,4.734868049621582,0.03350902033048442
3876,7753,3876,11629,4.739430904388428,0.03368318004129378
3881,7763,3881,11644,4.7451090812683105,0.03388873670883186
3886,7773,3886,11659,4.750925779342651,0.034080688939639
3890,7781,3890,11671,4.75547194480896,0.03422438120298921
3895,7791,3895,11686,4.761180877685547,0.0343915757873674
3899,7799,3899,11698,4.7656049728393555,0.034515339309223236
3904,7809,3904,11713,4.771320819854736,0.0346574882596542
3908,7817,3908,11725,4.776141881942749,0.034761121915153126
3913,7827,3913,11740,4.7820470333099365,0.03487801191431572
3918,7837,3918,11755,4.787709951400757,0.034980806053454216
3922,7845,3922,11767,4.7922587394714355,0.03505287338737162
3927,7855,3927,11782,4.797987937927246,0.03513023494792833
3931,7863,3931,11794,4.802602052688599,0.03518194440266598
3936,7873,3936,11809,4.808336973190308,0.035233864248652935
3940,7881,3940,11821,4.812812805175781,0.03526523954133154
3945,7891,3945,11836,4.818547010421753,0.03529178469045746
3949,7899,3949,11848,4.823302984237671,0.035302908045423465
3954,7909,3954,11863,4.82926082611084,0.03530421508150994
3959,7919,3959,11878,4.835078954696655,0.03529158297158119
3963,7927,3963,11890,4.839572906494141,0.035271488385205885
3968,7937,3968,11905,4.845262765884399,0.035233950221368104
3972,7945,3972,11917,4.849900007247925,0.035194037607425344
3977,7955,3977,11932,4.855568885803223,0.03513187275348173
3981,7963,3981,11944,4.860028982162476,0.03507238424754178
3986,7973,3986,11959,4.8657097816467285,0.034985917882636386
3990,7981,3990,11971,4.87034797668457,0.034907131344198206
3995,7991,3995,11986,4.876342058181763,0.034796732940776565
4000,8001,4000,12001,4.882279872894287,0.03467321528466982
4004,8009,4004,12013,4.886948823928833,0.03456504660414339
4009,8019,4009,12028,4.89254093170166,0.03441826355901867
4013,8027,4013,12040,4.897027969360352,0.0342916743021533
4018,8037,4018,12055,4.902761936187744,0.03412211907175333
4022,8045,4022,12067,4.907330751419067,0.033977525570207945
4027,8055,4027,12082,4.912970066070557,0.03378574669466161
4032,8065,4032,12097,4.918720960617065,0.03358187965648085
4036,8073,4036,12109,4.923840045928955,0.03341021474727768
4041,8083,4041,12124,4.929879903793335,0.03318509268615344
4045,8091,4045,12136,4.934544801712036,0.03299669638158775
4050,8101,4050,12151,4.940047979354858,0.032751015220128465
4054,8109,4054,12163,4.944534778594971,0.03254646595155464
4059,8119,4059,12178,4.950243949890137,0.03228097442854505
4063,8127,4063,12190,4.95480489730835,0.032060890496040884
4068,8137,4068,12205,4.960470914840698,0.03177638374484104
4073,8147,4073,12220,4.966249942779541,0.03148167114795797
4077,8155,4077,12232,4.970946788787842,0.031238729519259323
4082,8165,4082,12247,4.977046012878418,0.030926312850738213
4086,8173,4086,12259,4.981997728347778,0.030669557302189787
4091,8183,4091,12274,4.987775087356567,0.030340316270212497
4095,8191,4095,12286,4.992316961288452,0.03007045993297197
4100,8201,4100,12301,4.998031854629517,0.02972529658916301
4105,8211,4105,12316,5.003523826599121,0.029371684492161876
4109,8219,4109,12328,5.008039951324463,0.029082904872211657
4114,8229,4114,12343,5.013797998428345,0.0287148119413132
4118,8237,4118,12355,5.018548011779785,0.028414826018320127
4123,8247,4123,12370,5.0245137214660645,0.028033203327140654
4127,8255,4127,12382,5.03088903427124,0.02772278011502749
4132,8265,4132,12397,5.036526918411255,0.02732859965226453
4136,8273,4136,12409,5.041043996810913,0.027008525713085874
4141,8283,4141,12424,5.0467369556427,0.026602782354189003
4146,8293,4146,12439,5.05239200592041,0.026191053906586603
4150,8301,4150,12451,5.056995868682861,0.02585757586894033
4155,8311,4155,12466,5.062658786773682,0.025435879895667313
4159,8319,4159,12478,5.067378997802734,0.025094847564673728
4164,8329,4164,12493,5.07336688041687,0.024664238831405783
4168,8337,4168,12505,5.078426837921143,0.024316504008879747
4173,8347,4173,12520,5.084453821182251,0.02387805600642423
4177,8355,4177,12532,5.08905291557312,0.023524483377514116
4182,8365,4182,12547,5.094682931900024,0.023079282667708867
4187,8375,4187,12562,5.100566864013672,0.022630802549770124
4191,8383,4191,12574,5.105597019195557,0.022269884123261363
4196,8393,4196,12589,5.111530065536499,0.02181635135673332
4200,8401,4200,12601,5.116055727005005,0.02145182715730698
4205,8411,4205,12616,5.121944904327393,0.02099433074033641
4209,8419,4209,12628,5.126662015914917,0.020627068621138278
4214,8429,4214,12643,5.133074998855591,0.020166688070958116
4219,8439,4219,12658,5.138661861419678,0.01970516706512626
4223,8447,4223,12670,5.143268823623657,0.019335348873710245
4228,8457,4228,12685,5.148940086364746,0.01887259715590517
4232,8465,4232,12697,5.153432846069336,0.018502213897022557
4237,8475,4237,12712,5.159105062484741,0.018039276753938793
4241,8483,4241,12724,5.163651943206787,0.017669159442334603
4246,8493,4246,12739,5.169305801391602,0.017207069517894524
4250,8501,4250,12751,5.1743550300598145,0.01683803967341646
4255,8511,4255,12766,5.180311918258667,0.016377818480464157
4260,8521,4260,12781,5.186117887496948,0.015919073096029024
4264,8529,4264,12793,5.19071102142334,0.01555334799047614
4269,8539,4269,12808,5.196444034576416,0.015098039866529689
4273,8547,4273,12820,5.201129913330078,0.014735463374108804
4278,8557,4278,12835,5.206787824630737,0.014284586093140206
4282,8565,4282,12847,5.211146116256714,0.013925947418783835
4287,8575,4287,12862,5.2168238162994385,0.013480479314694094
4291,8583,4291,12874,5.221527814865112,0.013126553645633976
4296,8593,4296,12889,5.227380990982056,0.012687452961017698
4301,8603,4301,12904,5.233222961425781,0.01225229457372734
4305,8611,4305,12916,5.237810850143433,0.01190719654618988
4310,8621,4310,12931,5.243499040603638,0.01147984320687101
4314,8629,4314,12943,5.248058795928955,0.011141345896589883
4319,8639,4319,12958,5.253619909286499,0.01072268009693289
4323,8647,4323,12970,5.258116960525513,0.010391475007395456
4328,8657,4328,12985,5.2637619972229,0.009982342365219665
4333,8667,4333,13000,5.2693798542022705,0.009578857165138288
4337,8675,4337,13012,5.274013996124268,0.009260298334083927
4342,8685,4342,13027,5.279994964599609,0.008867585183907067
4346,8693,4346,13039,5.284553050994873,0.008557946978271502
4351,8703,4351,13054,5.290333032608032,0.00817675369501103
4355,8711,4355,13066,5.294864892959595,0.007876619640342142
4360,8721,4360,13081,5.30068302154541,0.007507657633368581
4364,8729,4364,13093,5.305328845977783,0.0072175827406226745
4369,8739,4369,13108,5.31090784072876,0.00686152842536103
4374,8749,4374,13123,5.316529989242554,0.006512924695130096
4378,8757,4378,13135,5.321155786514282,0.006239535532017726
4383,8767,4383,13150,5.327126741409302,0.005904823294031303
4387,8775,4387,13162,5.331899881362915,0.0056427859788072965
4392,8785,4392,13177,5.337547063827515,0.005322552329403152
4396,8793,4396,13189,5.342095851898193,0.005072321557690884
4401,8803,4401,13204,5.347858905792236,0.004767115371350883
4406,8813,4406,13219,5.353478908538818,0.0044704798169732385
4410,8821,4410,13231,5.358019828796387,0.004239442674361271
4415,8831,4415,13246,5.363781929016113,0.0039586046394788355
4419,8839,4419,13258,5.368330955505371,0.003740384946922859
4424,8849,4424,13273,5.3740198612213135,0.0034757805157141775
4428,8857,4428,13285,5.378657102584839,0.0032707076237556976
4433,8867,4433,13300,5.3843019008636475,0.0030227235509983075
4437,8875,4437,13312,5.388844013214111,0.0028310866359788633
4442,8885,4442,13327,5.394654035568237,0.00260005890265802
4447,8895,4447,13342,5.400353908538818,0.00237857776699002
4451,8903,4451,13354,5.405027866363525,0.0022083200204860987
4456,8913,4456,13369,5.4106409549713135,0.002004217049830004
4460,8921,4460,13381,5.415151834487915,0.0018479501561614597
4465,8931,4465,13396,5.4213340282440186,0.001661433786125599
4469,8939,4469,13408,5.426390886306763,0.0015193056494808843
4474,8949,4474,13423,5.432598114013672,0.001350537845951294
4478,8957,4478,13435,5.4370808601379395,0.0012226601816109905
4483,8967,4483,13450,5.442764759063721,0.0010717588678517131
4488,8977,4488,13465,5.448657035827637,0.0009308188117529426
4492,8985,4492,13477,5.453467845916748,0.0008252501247625332
4497,8995,4497,13492,5.45907998085022,0.0007022769854074795
4501,9003,4501,13504,5.463624954223633,0.0006110910863981189
4506,9013,4506,13519,5.469280958175659,0.0005060974921207162
4510,9021,4510,13531,5.474126815795898,0.0004292882116487817
4515,9031,4515,13546,5.479684829711914,0.00034224589137465955
4520,9041,4520,13561,5.485306978225708,0.0002651488470064578
4524,9049,4524,13573,5.489876985549927,0.00021061248082787642
4529,9059,4529,13588,5.49551796913147,0.0001513383763267484
4533,9067,4533,13600,5.500058889389038,0.00011100935807917267
4538,9077,4538,13615,5.505795955657959,6.941884998923342e-05
4542,9085,4542,13627,5.510303020477295,4.316731974540744e-05
4547,9095,4547,13642,5.516205787658691,1.9074816236752667e-05
4551,9103,4551,13654,5.520921945571899,6.733567715855315e-06
4556,9113,4556,13669,5.527065992355347,9.337225037597818e-09


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0011000633239746094,2181.2938132599165
2002,2003,2002,4005,2.280527114868164,58.98939413564449
4004,4005,4004,8009,4.509216070175171,53.03643300809222
6006,6007,6006,12013,6.557736396789551,50.14448564934969
8008,8009,8008,16017,9.011595010757446,47.78238326053793
10010,10011,10010,20021,11.676583290100098,45.667972303392844
12012,12013,12012,24025,13.8959321975708,43.73827157437995
14014,14015,14014,28029,17.115005254745483,41.96421429747534
16016,16017,16016,32033,19.955968141555786,40.326626752231505
18018,18019,18018,36037,22.13455104827881,38.81085736169712
20020,20021,20020,40041,24.704042196273804,37.404696941323664
22022,22023,22022,44045,27.0596821308136,36.09739520430389
24024,24025,24024,48049,29.155108213424683,34.87920504021599
26026,26027,26026,52053,31.147736072540283,33.741197391877904
28028,28029,28028,56057,33.136481046676636,32.675202996515736
30030,30031,30030,60061,35.19402813911438,31.67380030947197
32032,32033,32032,64065,37.19806528091431,30.730308340338524
34034,34035,34034,68069,39.248173236846924,29.83876717643193
36036,36037,36036,72073,41.24838399887085,28.99390239063723
38038,38039,38038,76077,43.24014639854431,28.191075966046128
40040,40041,40040,80081,45.24280023574829,27.426228613720923
42042,42043,42042,84085,47.260823249816895,26.69581838396789
44044,44045,44044,88089,49.3740131855011,25.99675953070073
46046,46047,46046,92093,51.942129373550415,25.326364396208646
48048,48049,48048,96097,54.37241721153259,24.682289990762683
50050,50051,50050,100101,56.312294244766235,24.062490081422084
52052,52053,52052,104105,58.327967405319214,23.465172994981003
54054,54055,54054,108109,60.33034825325012,22.888764946980018
56056,56057,56056,112113,62.29389023780823,22.331878481869126
58058,58059,58058,116117,64.30425119400024,21.793285499888043
60060,60061,60060,120121,66.25876307487488,21.271894313895928
62062,62063,62062,124125,68.21049332618713,20.76673019411305
64064,64065,64064,128129,70.2581512928009,20.27691889943162
66066,66067,66066,132133,72.92543721199036,19.801672746742724
68068,68069,68068,136137,75.38293027877808,19.340278825864743
70070,70071,70070,140141,77.42764639854431,18.892089022114533
72072,72073,72072,144145,79.48442029953003,18.456511558652437
74074,74075,74074,148149,81.4573004245758,18.033094262313625
76076,76077,76076,152153,83.39859938621521,17.621252501791332
78078,78079,78078,156157,85.35580229759216,17.220515531400224
80080,80081,80080,160161,87.27231526374817,16.83045515125127
82082,82083,82082,164165,89.22171115875244,16.45067273713653
84084,84085,84084,168169,91.16441917419434,16.080795952795256
86086,86087,86086,172173,93.06998825073242,15.720475925140931
88088,88089,88088,176177,95.00507020950317,15.369384805435402
90090,90091,90090,180181,96.97749829292297,15.027213657072139
92092,92093,92092,184185,98.89448118209839,14.69367062078129
94094,94095,94094,188189,101.39060306549072,14.368479316052458
96096,96097,96096,192193,103.7192862033844,14.051377444162767
98098,98099,98098,196197,106.59745216369629,13.742115563676407
100100,100101,100100,200201,108.68919515609741,13.440456013834478
102102,102103,102102,204205,110.87200832366943,13.146171965067651
104104,104105,104104,208209,113.02520513534546,12.85904657902438
106106,106107,106106,212213,115.11272120475769,12.578872263163817
108108,108109,108108,216217,117.22778534889221,12.30545000719394
110110,110111,110110,220221,119.23177218437195,12.038588790493577
112112,112113,112112,224225,121.39110016822815,11.778105051239208
114114,114115,114114,228229,123.82145023345947,11.523822209284504
116116,116117,116116,232233,126.87766718864441,11.275570235959549
118118,118119,118118,236237,129.08838033676147,11.033185264917847
120120,120121,120120,240241,131.08825016021729,10.79650923896861
122122,122123,122122,244245,133.07888531684875,10.565389588519793
124124,124125,124124,248249,135.25730109214783,10.339678937857911
126126,126127,126126,252253,137.34092116355896,10.119234835991392
128128,128129,128128,256257,139.30051040649414,9.903919509231628
130130,130131,130130,260261,141.35481333732605,9.693599633051008
132132,132133,132132,264265,143.39034914970398,9.488146121100954
134134,134135,134134,268269,145.55514645576477,9.287433929541862
136136,136137,136136,272273,147.500794172287,9.091341875098124
138138,138139,138138,276277,149.50001215934753,8.899752465451002
140140,140141,140140,280281,151.48497009277344,8.71255174078658
142142,142143,142142,284285,153.50501823425293,8.529629125458314
144144,144145,144144,288289,155.49493718147278,8.350877288881179
146146,146147,146146,292293,157.45935535430908,8.176192014876847
148148,148149,148148,296297,159.41884422302246,8.005472078803791
150150,150151,150150,300301,161.35276627540588,7.838619131879341
152152,152153,152152,304305,163.26719737052917,7.675537592176283
154154,154155,154154,308309,165.20732736587524,7.516134541831548
156156,156157,156156,312313,167.14945816993713,7.36031963004632
158158,158159,158158,316317,169.07266306877136,7.208004981495151
160160,160161,160160,320321,171.03576135635376,7.0591051097869695
162162,162163,162162,324325,173.0136570930481,6.913536835643868
164164,164165,164164,328329,174.9808051586151,6.771219209477181
166166,166167,166166,332333,177.0032093524933,6.6320734380631166
168168,168169,168168,336337,179.2143042087555,6.496022815018591
170170,170171,170170,340341,181.37208223342896,6.362992654809773
172172,172173,172172,344345,183.30688738822937,6.23291023002173
174174,174175,174174,348349,185.1022481918335,6.1057047116416925
176176,176177,176176,352353,187.153626203537,5.981307112122522
178178,178179,178178,356357,189.83672332763672,5.859650231003798
180180,180181,180180,360361,192.7216193675995,5.740668602889286
182182,182183,182182,364365,195.54861903190613,5.624298447595493
184184,184185,184184,368369,200.29076409339905,5.510477622299618
186186,186187,186186,372373,204.16207718849182,5.399145575536409
188188,188189,188188,376377,207.190580368042,5.29024330290531
190190,190191,190190,380381,209.3960452079773,5.18371330436446
192192,192193,192192,384385,211.77341318130493,5.079499543003408
194194,194195,194194,388389,214.6214473247528,4.977547405196333
196196,196197,196196,392393,217.24164199829102,4.877803662050042
198198,198199,198198,396397,219.55877017974854,4.780216432071825
200200,200201,200200,400401,222.1956160068512,4.684735144986007
202202,202203,202202,404405,224.66296815872192,4.591310506644277
204204,204205,204204,408409,227.89457726478577,4.4998944649712485
206206,206207,206206,412413,230.519287109375,4.410440176899783
208208,208209,208208,416417,232.87555313110352,4.322901976254116
210210,210211,210210,420421,235.27060914039612,4.237235342538952
212212,212213,212212,424425,237.4436752796173,4.15339687060316
214214,214215,214214,428429,239.74439334869385,4.071344241143038
216216,216217,216216,432433,242.01642322540283,3.9910361920165087
218218,218219,218218,436437,244.2860233783722,3.912432490343349
220220,220221,220220,440441,246.9726321697235,3.835493905362455
222222,222223,222222,444445,249.60929107666016,3.7601821820259147
224224,224225,224224,448449,252.18155908584595,3.686460015306807
226226,226227,226226,452453,254.5910611152649,3.6142910251994635
228228,228229,228228,456457,256.90168499946594,3.543639732393899
230230,230231,230230,460461,259.2921531200409,3.474471534603026
232232,232233,232232,464465,261.60894322395325,3.406752683528225
234234,234235,234234,468469,264.0016140937805,3.3404502624438237
236236,236237,236236,472473,266.22930932044983,3.2755321643836623
238238,238239,238238,476477,268.5235741138458,3.2119670709150796
240240,240241,240240,480481,270.8299193382263,3.1497244314853106
242242,242243,242242,484485,273.05086731910706,3.0887744433214266
244244,244245,244244,488489,275.30400943756104,3.029088031875631
246246,246247,246246,492493,277.490745306015,2.9706368317948773
248248,248249,248248,496497,279.67144441604614,2.913393168406401
250250,250251,250250,500501,281.7946791648865,2.857330039702674
252252,252253,252252,504505,284.1916801929474,2.802421098813852
254254,254255,254254,508509,286.74918127059937,2.748640636953496
256256,256257,256256,512513,289.03922510147095,2.695963566828027
258258,258259,258258,516517,291.3203992843628,2.6443654064930797
260260,260261,260260,520521,293.5571184158325,2.5938222636509636
262262,262263,262262,524525,295.67409110069275,2.5443108203701286
264264,264265,264264,528529,297.7807421684265,2.495808318222089
266266,266267,266266,532533,299.9380271434784,2.448292543821026
268268,268269,268268,536537,302.1294152736664,2.401741814754587
270270,270271,270270,540541,304.3083493709564,2.356134965899514
272272,272273,272272,544545,306.53968715667725,2.311451336105165
274274,274275,274274,548549,308.7385711669922,2.2676707552419657
276276,276277,276276,552553,310.5774493217468,2.224773531599226
278278,278279,278278,556557,312.49559020996094,2.1827404396258316
280280,280281,280280,560561,314.4184892177582,2.1415527080039283
282282,282283,282282,564565,316.39019322395325,2.101192008044791
284284,284285,284284,568569,318.83321237564087,2.0616404424014263
286286,286287,286286,572573,321.46911215782166,2.022880534084493
288288,288289,288288,576577,324.10483026504517,1.9848952157772146
290290,290291,290290,580581,326.41622018814087,1.9476678194395163
292292,292293,292292,584585,328.7427752017975,1.911182066193419
294294,294295,294294,588589,331.26284742355347,1.8754220564800335
296296,296297,296296,592593,333.7288682460785,1.8403722604844006
298298,298299,298298,596597,336.25238132476807,1.8060175088176038
300300,300301,300300,600601,339.1867341995239,1.772342983450244
302302,302303,302302,604605,341.35476517677307,1.7393342088901136
304304,304305,304304,608609,344.01371121406555,1.7069770435959981
306306,306307,306306,612613,346.2194492816925,1.67525767162374
308308,308309,308308,616617,348.35729217529297,1.6441625944964926
310310,310311,310310,620621,350.61172318458557,1.613678623289843
312312,312313,312312,624625,352.7996280193329,1.5837928709333937
314314,314315,314314,628629,355.0008943080902,1.5544927447135706
316316,316317,316316,632633,357.20956110954285,1.5257659389803848
318318,318319,318318,636637,359.4140112400055,1.4976004280460984
320320,320321,320320,640641,361.53443217277527,1.469984459273178
322322,322323,322322,644645,363.851202249527,1.442906546347558
324324,324325,324324,648649,366.0624713897705,1.4163554627282338
326326,326327,326326,652653,368.3244574069977,1.39032023527227
328328,328329,328328,656657,370.55968618392944,1.3647901380272742
330330,330331,330330,660661,372.73890924453735,1.3397546861889396
332332,332333,332332,664665,374.89173221588135,1.3152036302162742
334334,334335,334334,668669,377.0877151489258,1.2911269501040579
336336,336337,336336,672673,379.3066921234131,1.2675148498030921
338338,338339,338338,676677,381.56870126724243,1.2443577517899485
340340,340341,340340,680681,383.8343753814697,1.2216462917768922
342342,342343,342342,684685,386.08393812179565,1.1993713135598227
344344,344345,344344,688689,388.22800731658936,1.1775238640028647
346346,346347,346346,692693,390.37486124038696,1.1560951881518804
348348,348349,348348,696697,392.5259392261505,1.1350767244754252
350350,350351,350350,700701,394.6692941188812,1.1144601002298486
352352,352353,352352,704705,396.9231712818146,1.0942371269436535
354354,354355,354354,708709,399.16297912597656,1.0743997960207707
356356,356357,356356,712713,401.39498019218445,1.0549402744535428
358358,358359,358358,716717,403.532594203949,1.035850900650189
360360,360361,360360,720721,405.68697023391724,1.0171241803682278
362362,362363,362362,724725,407.84594202041626,0.9987527827502163
364364,364365,364364,728729,409.9949543476105,0.9807295364646507
366366,366367,366366,732733,412.20164728164673,0.9630474259445236
368368,368369,368368,736737,414.411758184433,0.9456995877191048
370370,370371,370370,740741,416.6313850879669,0.9286793068434918
372372,372373,372372,744745,418.7895312309265,0.9119800134162688
374374,374375,374374,748749,420.93669724464417,0.8955952791862956
376376,376377,376376,752753,423.14165139198303,0.8795188142456709
378378,378379,378378,756757,425.2813892364502,0.8637444638062561
380380,380381,380380,760761,427.50364112854004,0.8482662050566887
382382,382383,382382,764765,429.9995450973511,0.8330781441009094
384384,384385,384384,768769,432.4473121166229,0.8181745129711544
386386,386387,386386,772773,434.88395643234253,0.8035496667167763
388388,388389,388388,776777,437.0434682369232,0.7891980805663934
390390,390391,390390,780781,439.2408893108368,0.7751143471609794
392392,392393,392392,784785,441.40874433517456,0.7612931738555062
394394,394395,394394,788789,443.7613422870636,0.7477293800875486
396396,396397,396396,792793,446.09405732154846,0.7344178948120543
398398,398399,398398,796797,448.4175581932068,0.7213537539995514
400400,400401,400400,800801,451.1283950805664,0.7085320981955192
402402,402403,402402,804805,453.3295621871948,0.6959481701414916
404404,404405,404404,808809,455.61966824531555,0.6835973124530028
406406,406407,406406,812813,458.6070191860199,0.6714749653556282
408408,408409,408408,816817,460.9824540615082,0.6595766644778678
410410,410411,410410,820821,463.8608922958374,0.6478980386950752
412412,412413,412412,824825,466.99742913246155,0.6364348080288664
414414,414415,414414,828829,469.372278213501,0.6251827815967772
416416,416417,416416,832833,472.1209032535553,0.6141378556114887
418418,418419,418418,836837,474.63309121131897,0.6032960114295065
420420,420421,420420,840841,477.5071883201599,0.592653313646224
422422,422423,422422,844845,480.06218338012695,0.5822059082381656
424424,424425,424424,848849,482.59731221199036,0.5719500207495685
426426,426427,426426,852853,484.87687611579895,0.561881954522164
428428,428429,428428,856857,487.1634781360626,0.5519980889691851
430430,430431,430430,860861,489.80267214775085,0.5422948778884802
432432,432433,432432,864865,492.63965010643005,0.5327688478187156
434434,434435,434434,868869,495.16024827957153,0.5234165964325257
436436,436437,436436,872873,497.38088512420654,0.514234790970022
438438,438439,438438,876877,499.71570205688477,0.5052201667078862
440440,440441,440440,880881,502.07758021354675,0.4963695254656386
442442,442443,442442,884885,504.41562700271606,0.4876797341486281
444444,444445,444444,888889,506.8121783733368,0.4791477233228534
446446,446447,446446,892893,509.7759323120117,0.4707704858262787
448448,448449,448448,896897,512.1807641983032,0.46254507541061685
450450,450451,450450,900901,514.4484901428223,0.4544686054163094
452452,452453,452452,904905,516.6929180622101,0.44653824747888393
454454,454455,454454,908909,520.1527051925659,0.43875123026509755
456456,456457,456456,912913,522.7159082889557,0.4311048382385252
458458,458459,458458,916917,526.3622181415558,0.4235964104550476
460460,460461,460460,920921,528.605954170227,0.41622333938380507
462462,462463,462462,924925,530.8338313102722,0.40898306975930154
464464,464465,464464,928929,533.2190222740173,0.4018730974578375
466466,466467,466466,932933,535.3428022861481,0.3948909684006594
468468,468469,468468,936937,537.5182473659515,0.3880342774820065
470470,470471,470470,940941,539.7465121746063,0.3813006675221686
472472,472473,472472,944945,542.7762553691864,0.3746878282454418
474474,474475,474474,948949,545.779871225357,0.3681934952804795
476476,476477,476476,952953,548.3522622585297,0.3618154491836094
478478,478479,478478,956957,550.8147630691528,0.35555151448670586
480480,480481,480480,960961,553.2092442512512,0.34939955876257045
482482,482483,482482,964965,555.5505821704865,0.34335749171657426
484484,484485,484484,968969,557.8801143169403,0.3374232642958077
486486,486487,486486,972973,560.1277832984924,0.33159486781914893
488488,488489,488488,976977,562.3495674133301,0.3258703331274546
490490,490491,490490,980981,564.6058423519135,0.32024772975341875
492492,492493,492492,984985,566.7961840629578,0.3147251651088254
494494,494495,494494,988989,569.0588612556458,0.30930078369181047
496496,496497,496496,992993,571.4414401054382,0.30397276631060777
498498,498499,498498,996997,573.6954801082611,0.2987393293255991
500501,500502,500501,1001003,576.0817263126373,0.29359617908278324
502503,502504,502503,1005007,578.6133742332458,0.2885467355815763
504505,504506,504505,1009011,580.9033694267273,0.28358672671083696
506507,506508,506507,1013015,583.148674249649,0.27871450380882834
508509,508510,508509,1017019,585.3261330127716,0.2739284502213195
510511,510512,510511,1021023,587.5307881832123,0.26922698064151973
512513,512514,512513,1025027,589.7034661769867,0.2646085404610403
514515,514516,514515,1029031,591.9396753311157,0.26007160513745475
516517,516518,516517,1033035,594.2188580036163,0.25561467957606965
518519,518520,518519,1037039,596.4036910533905,0.2512362975239739
520521,520522,520521,1041043,598.6829633712769,0.24693502097875353
522523,522524,522523,1045047,601.0072402954102,0.242709439608916
524525,524526,524525,1049051,603.2054162025452,0.23855817018852576
526527,526528,526527,1053055,605.3442471027374,0.23447985604343557
528529,528530,528529,1057059,607.664694070816,0.23047316650911398
530531,530532,530531,1061063,610.113908290863,0.22653679640177415
532533,532534,532533,1065067,612.3015501499176,0.22266946549984823
534535,534536,534535,1069071,614.5506553649902,0.21886991803648925
536537,536538,536537,1073075,616.7895321846008,0.2151369222053745
538539,538540,538539,1077079,618.9889574050903,0.2114692696743532
540541,540542,540541,1081083,621.1697402000427,0.20786577511080395
542543,542544,542543,1085087,623.3381969928741,0.20432527571858827
544545,544546,544545,1089091,625.5037953853607,0.2008466307826211
546547,546548,546547,1093095,627.6978192329407,0.1974287212251511
548549,548550,548549,1097099,631.7730123996735,0.1940704491702263
550551,550552,550551,1101103,635.4469921588898,0.19077073751941498
552553,552554,552553,1105107,638.7513401508331,0.18752852953400634
554555,554556,554555,1109111,641.6557660102844,0.18434278842835283
556557,556558,556557,1113115,644.653813123703,0.18121249697105668
558559,558560,558559,1117119,647.6599612236023,0.17813665709468296
560561,560562,560561,1121123,650.0309331417084,0.17511428951388552
562563,562564,562563,1125127,652.9414081573486,0.17214443335160468
564565,564566,564565,1129131,655.4789571762085,0.16922614577322292
566567,566568,566567,1133135,658.0934841632843,0.16635850162856514
568569,568570,568569,1137139,660.7127523422241,0.16354059310185676
570571,570572,570571,1141143,663.1169700622559,0.16077152936702532
572573,572574,572573,1145147,665.3642492294312,0.1580504362540296
574575,574576,574575,1149151,667.7867403030396,0.15537645591984983
576577,576578,576577,1153155,670.0775122642517,0.1527487465239119
578579,578580,578579,1157159,672.4831931591034,0.15016648191715376
580581,580582,580581,1161163,675.0320391654968,0.14762885133040982
582583,582584,582583,1165167,677.345516204834,0.14513505907359558
584585,584586,584585,1169171,680.6651730537415,0.14268432424034927
586587,586588,586587,1173175,683.5891242027283,0.14027588041824401
588589,588590,588589,1177179,687.1192502975464,0.13790897540491187
590591,590592,590591,1181183,689.9932742118835,0.13558287093098897
592593,592594,592593,1185187,692.5203251838684,0.133296842388404
594595,594596,594595,1189191,695.0658891201019,0.13105017856389622
596597,596598,596597,1193195,697.3772521018982,0.1288421813783316
598599,598600,598599,1197199,699.7898092269897,0.12667216563181682
600601,600602,600601,1201203,702.058158159256,0.12453945875347472
602603,602604,602603,1205207,704.1847453117371,0.12244340055735847
604605,604606,604605,1209211,706.4317293167114,0.12038334300086717
606607,606608,606607,1213215,708.5378880500793,0.11835864995236989
608609,608610,608609,1217219,710.6442742347717,0.11636869695905716
610611,610612,610611,1221223,712.6991612911224,0.1144128710232053
612613,612614,612613,1225227,714.8778781890869,0.11249057038048704
614615,614616,614615,1229231,717.8242073059082,0.11060120428396658
616617,616618,616617,1233235,720.0798079967499,0.10874419279309677
618619,618620,618619,1237239,722.4911532402039,0.10691896656533117
620621,620622,620621,1241243,725.1507792472839,0.10512496665330673
622623,622624,622623,1245247,727.6183743476868,0.10336164430600547
624625,624626,624625,1249251,729.9712052345276,0.10162846077366794
626627,626628,626627,1253255,732.2853412628174,0.0999248871155487
628629,628630,628629,1257259,734.4443602561951,0.09825040401517526
630631,630632,630631,1261263,736.6192932128906,0.09660450159412903
632633,632634,632633,1265267,738.7559270858765,0.0949866792341254
634635,634636,634635,1269271,740.8064341545105,0.09339644540068548
636637,636638,636637,1273275,742.8956632614136,0.09183331746964996
638639,638640,638639,1277279,744.9786150455475,0.09029682155903629
640641,640642,640641,1281283,747.8188033103943,0.08878649236351066
642643,642644,642643,1285287,750.380588054657,0.08730187299045156
644645,644646,644645,1289291,753.1330771446228,0.0858425148024935
646647,646648,646647,1293295,755.6508421897888,0.08440797726143501
648649,648650,648649,1297299,758.0724983215332,0.08299782777407927
650651,650652,650651,1301303,760.278626203537,0.08161164154398648
652653,652654,652653,1305307,762.526703119278,0.08024900142345359
654655,654656,654655,1309311,764.6561300754547,0.07890949777060996
656657,656658,656657,1313315,766.9492542743683,0.07759272830821828
658659,658660,658659,1317319,769.9158172607422,0.07629829798429455
660661,660662,660661,1321323,772.6503133773804,0.07502581883818493
662663,662664,662663,1325327,774.7968833446503,0.07377490986709745
664665,664666,664665,1329331,777.1520662307739,0.07254519689581684
666667,666668,666667,1333335,779.5232162475586,0.0713363124488069
668669,668670,668669,1337339,781.8077912330627,0.07014789562629176
670671,670672,670671,1341343,784.1723403930664,0.06897959197976888
672673,672674,672673,1345347,786.3725283145905,0.06783105339354734
674675,674676,674675,1349351,788.6038901805878,0.06670193796583135
676677,676678,676677,1353355,790.7531950473785,0.06559190989378294
678679,678680,678679,1357359,792.8319232463837,0.06450063935915296
680681,680682,680681,1361363,795.4258103370667,0.06342780241891433
682683,682684,682683,1365367,798.0314831733704,0.06237308089464477
684685,684686,684685,1369371,800.3602240085602,0.061336162266456995
686687,686688,686687,1373375,802.4398562908173,0.060316739568747835
688689,688690,688689,1377379,804.5168471336365,0.05931451128685694
690691,690692,690691,1381383,807.1927270889282,0.05832918125656761
692693,692694,692693,1385387,810.2920732498169,0.05736045856531291
694695,694696,694695,1389391,812.4362523555756,0.056408057455882954
696697,696698,696697,1393395,814.6637661457062,0.055471697230359496
698699,698700,698699,1397399,817.2813854217529,0.05455110215825698
700701,700702,700701,1401403,819.3962984085083,0.05364600138489095
702703,702704,702703,1405407,822.0847780704498,0.05275612884133807
704705,704706,704705,1409411,824.8512473106384,0.051881223156669876
706707,706708,706707,1413415,827.3357102870941,0.0510210275724603
708709,708710,708709,1417419,830.1340301036835,0.05017528985797526
710711,710712,710711,1421423,832.5101964473724,0.0493437622270676
712713,712714,712713,1425427,835.077977180481,0.04852620125723206
714715,714716,714715,1429431,837.7951462268829,0.04772236781025185
716717,716718,716717,1433435,840.676726102829,0.04693202695261789
718719,718720,718719,1437439,843.6999621391296,0.0461549478809502
720721,720722,720721,1441443,846.312328338623,0.04539090384514566
722723,722724,722723,1445447,848.7464911937714,0.044639672074822556
724725,724726,724725,1449451,851.1684243679047,0.04390103370781162
726727,726728,726727,1453455,853.6141083240509,0.043174773718305914
728729,728730,728729,1457459,856.7274880409241,0.04246068084739818
730731,730732,730731,1461463,858.9982330799103,0.0417585475352098
732733,732734,732733,1465467,861.2908091545105,0.04106816985313344
734735,734736,734735,1469471,863.7580642700195,0.04038934743869049
736737,736738,736737,1473475,866.2815833091736,0.039721883430729577
738739,738740,738739,1477479,868.5672721862793,0.039065584405989284
740741,740742,740741,1481483,871.1519622802734,0.0384202603175936
742743,742744,742743,1485487,873.3691310882568,0.03778572443320627
744745,744746,744745,1489491,875.7861602306366,0.037161793276141
746747,746748,746747,1493495,878.1556541919708,0.03654828656613063
748749,748750,748749,1497499,880.4102311134338,0.03594502716225634
750751,750752,750751,1501503,882.6596722602844,0.03535184100587685
752753,752754,752753,1505507,884.8993191719055,0.03476855706549031
754755,754756,754755,1509511,887.1186890602112,0.034195007283187806
756757,756758,756757,1513515,889.3675122261047,0.03363102651928784
758759,758760,758759,1517519,891.6070022583008,0.03307645250220048
760761,760762,760761,1521523,894.2188742160797,0.03253112577601769
762763,762764,762763,1525527,896.5224120616913,0.03199488964912689
764765,764766,764765,1529531,898.870599269867,0.03146759014748568
766767,766768,766767,1533535,901.828889131546,0.030949075962553252
768769,768770,768769,1537539,904.2061061859131,0.030439198407066215
770771,770772,770771,1541543,906.7617621421814,0.029937811365471134
772773,772774,772773,1545547,909.2577061653137,0.02944477124981404
774775,774776,774775,1549551,911.8690280914307,0.028959936953469878
776777,776778,776777,1553555,914.3366751670837,0.028483169808509956
778779,778780,778779,1557559,916.7592771053314,0.028014333540454572
780781,780782,780781,1561563,918.9011824131012,0.027553294227118386
782783,782784,782783,1565567,921.0057482719421,0.027099920256205223
784785,784786,784785,1569571,923.1587612628937,0.026654082284267133
786787,786788,786787,1573575,925.3511083126068,0.026215653197027677
788789,788790,788789,1577579,927.4370181560516,0.025784508068227296
790791,790792,790791,1581583,929.5456891059875,0.02536052412290246
792793,792794,792793,1585587,931.6995022296906,0.024943580698504775
794795,794796,794795,1589591,933.8020441532135,0.024533559206929567
796797,796798,796797,1593595,936.287611246109,0.024130343098022422
798799,798800,798799,1597599,938.7676253318787,0.023733817824677317
800801,800802,800801,1601603,941.7240424156189,0.023343870805661027
802803,802804,802803,1605607,944.3097610473633,0.02296039139275763
804805,804806,804805,1609611,946.9785442352295,0.022583270834957148
806807,806808,806807,1613615,949.6639621257782,0.02221240224628218
808809,808810,808809,1617619,952.3301951885223,0.02184768057270503
810811,810812,810811,1621623,954.9525442123413,0.021489002558837456
812813,812814,812813,1625627,957.5048551559448,0.021136266718031038
814815,814816,814815,1629631,959.7971813678741,0.020789373300203806
816817,816818,816817,1633635,962.9384210109711,0.0204482242610311
818819,818820,818819,1637639,965.2153122425079,0.020112723232841745
820821,820822,820821,1641643,967.9581742286682,0.019782775495286842
822823,822824,822823,1645647,970.2733671665192,0.019458287945099073
824825,824826,824825,1649651,972.6289422512054,0.01913916906880786
826827,826828,826827,1653655,975.061083316803,0.01882532891579558
828829,828830,828829,1657659,977.8074612617493,0.018516679068625308
830831,830832,830831,1661663,980.2935152053833,0.018213132618257077
832833,832834,832833,1665667,982.9183690547943,0.017914604136763046
834835,834836,834835,1669671,985.5453882217407,0.017621009651293207
836837,836838,836837,1673675,988.2239072322845,0.017332266619405345
838839,838840,838839,1677679,990.7405412197113,0.017048293903712874
840841,840842,840841,1681683,993.2250213623047,0.016769011746760043
842843,842844,842843,1685687,995.7901401519775,0.016494341748511943
844845,844846,844845,1689691,998.4864392280579,0.01622420684077497
846847,846848,846847,1693695,1000.9518871307373,0.015958531265710008
848849,848850,848849,1697699,1003.5630593299866,0.015697240551958203
850851,850852,850851,1701703,1006.6260132789612,0.01544026149315414
852853,852854,852853,1705707,1009.5331110954285,0.015187522124620045
854855,854856,854855,1709711,1012.6389412879944,0.014938951703470593
856857,856858,856857,1713715,1015.0803942680359,0.01469448068598922
858859,858860,858859,1717719,1017.1668684482574,0.014454040707278182
860861,860862,860861,1721723,1019.8613471984863,0.01421756456136336
862863,862864,862863,1725727,1021.8713982105255,0.01398498618073063
864865,864866,864865,1729731,1023.9511752128601,0.013756240615862225
866867,866868,866867,1733735,1026.0243122577667,0.013531264016819478
868869,868870,868869,1737739,1028.0646772384644,0.01330999361493923
870871,870872,870871,1741743,1030.25617313385,0.01309236770168809
872873,872874,872873,1745747,1032.66561627388,0.012878325612518893
874875,874876,874875,1749751,1035.0195252895355,0.012667807708339751
876877,876878,876877,1753755,1037.4585993289948,0.012460755357096787
878879,878880,878879,1757759,1040.189501285553,0.012257110917289538
880881,880882,880881,1761763,1042.7785501480103,0.0120568177203495
882883,882884,882883,1765767,1044.8989412784576,0.011859820053700787
884885,884886,884885,1769771,1047.0762922763824,0.011666063145298722
886887,886888,886887,1773775,1049.2554762363434,0.011475493146122062
888889,888890,888889,1777779,1051.5690841674805,0.011288057115052652
890891,890892,890891,1781783,1053.7508301734924,0.011103703003186638
892893,892894,892893,1785787,1056.0808942317963,0.01092237963871412
894895,894896,894895,1789791,1058.242612361908,0.010744036710889304
896897,896898,896897,1793795,1060.388503074646,0.01056862475638809
898899,898900,898899,1797799,1062.8307571411133,0.010396095143732964
900901,900902,900901,1801803,1065.183517217636,0.010226400060332708
902903,902904,902903,1805807,1067.4650371074677,0.010059492496907296
904905,904906,904905,1809811,1069.9576740264893,0.009895326234868662
906907,906908,906907,1813815,1072.115023136139,0.009733855832109839
908909,908910,908909,1817819,1074.2861912250519,0.009575036610385723
910911,910912,910911,1821823,1076.6954312324524,0.009418824640874845
912913,912914,912913,1825827,1078.9345662593842,0.009265176733379121
914915,914916,914915,1829831,1081.1637501716614,0.009114050422226683
916917,916918,916917,1833835,1083.4214141368866,0.008965403953538953
918919,918920,918919,1837839,1085.6101722717285,0.00881919627465777
920921,920922,920921,1841843,1087.8518080711365,0.008675387021071401
922923,922924,922923,1845847,1090.1127161979675,0.008533936504363737
924925,924926,924925,1849851,1092.2748003005981,0.008394805702209851
926927,926928,926927,1853855,1094.5097181797028,0.008257956244733577
928929,928930,928929,1857859,1096.676872253418,0.008123350405753627
930931,930932,930931,1861863,1098.8551461696625,0.007990951089709597
932933,932934,932933,1865867,1101.078092098236,0.007860721822680716
934935,934936,934935,1869871,1103.264434337616,0.007732626740789783
936937,936938,936937,1873875,1105.493455171585,0.007606630579971352
938939,938940,938939,1877879,1107.699901342392,0.007482698665626231
940941,940942,940941,1881883,1109.880618095398,0.0073607969032991605
942943,942944,942943,1885887,1112.0994591712952,0.007240891768105939
944945,944946,944945,1889891,1114.311867237091,0.007122950295070041
946947,946948,946947,1893895,1116.487262248993,0.007006940069800294
948949,948950,948949,1897899,1118.7396092414856,0.006892829219850682
950951,950952,950951,1901903,1120.981308221817,0.006780586403920097
952953,952954,952953,1905907,1123.355089187622,0.0066701808045763755
954955,954956,954955,1909911,1125.859590291977,0.006561582117683429
956957,956958,956957,1913915,1128.3449063301086,0.006454760545238969
958959,958960,958959,1917919,1130.6240193843842,0.006349686785711128
960961,960962,960961,1921923,1132.9203741550446,0.006246332026194068
962963,962964,962963,1925927,1135.2311441898346,0.006144667934108838
964965,964966,964965,1929931,1137.448587179184,0.006044666648790553
966967,966968,966967,1933935,1139.7379393577576,0.005946300773643998
968969,968970,968969,1937939,1142.1387922763824,0.005849543368071863
970971,970972,970971,1941943,1144.4334683418274,0.005754367940539851
972973,972974,972973,1945947,1146.7833292484283,0.005660748440163843
974975,974976,974975,1949951,1149.1001162528992,0.005568659248979202
976977,976978,976977,1953955,1151.2019410133362,0.005478075176256425
978979,978980,978979,1957959,1153.36696600914,0.005388971449406199
980981,980982,980981,1961963,1155.5345242023468,0.005301323707953998
982983,982984,982983,1965967,1157.7218461036682,0.005215107996605184
984985,984986,984985,1969971,1159.986251115799,0.005130300757855366
986987,986988,986987,1973975,1162.3003220558167,0.005046878825737622
988989,988990,988989,1977979,1164.5331263542175,0.004964819419001287
990991,990992,990991,1981983,1166.5959582328796,0.0048841001349728685
992993,992994,992993,1985987,1168.673971414566,0.004804698942507457
994995,994996,994995,1989991,1170.8736691474915,0.004726594176531762
996997,996998,996997,1993995,1173.3665699958801,0.0046497645313365865
998999,999000,998999,1997999,1175.6867713928223,0.004574189054778799
1001001,1001002,1001001,2002003,1177.774393081665,0.004499847142142244
1003003,1003004,1003003,2006007,1179.850726366043,0.004426718530226026
1005005,1005006,1005005,2010011,1181.9119024276733,0.004354783292228603
1007007,1007008,1007007,2014015,1183.971194267273,0.004284021831495011
1009009,1009010,1009009,2018019,1186.1942842006683,0.004214414875946204
1011011,1011012,1011011,2022023,1188.2506031990051,0.00414594347273578
1013013,1013014,1013013,2026027,1190.2954270839691,0.004078588983475129
1015015,1015016,1015015,2030031,1192.3620202541351,0.0040123330779806565
1017017,1017018,1017017,2034035,1194.4503452777863,0.003947157729840001
1019019,1019020,1019019,2038039,1196.5653183460236,0.003883045210614
1021021,1021022,1021021,2042043,1198.6140401363373,0.003819978085743969
1023023,1023024,1023023,2046047,1200.6841552257538,0.0037579392089810426
1025025,1025026,1025025,2050051,1202.7662951946259,0.0036969117178387023
1027027,1027028,1027027,2054055,1204.8290991783142,0.003636879028590556
1029029,1029030,1029029,2058059,1207.2673852443695,0.003577824831381804
1031031,1031032,1031031,2062063,1209.8429923057556,0.0035197330871596932
1033033,1033034,1033033,2066067,1212.3476321697235,0.003462588020624935
1035035,1035036,1035035,2070071,1214.930447101593,0.0034063741180716534
1037037,1037038,1037037,2074075,1217.236325263977,0.0033510761218167318
1039039,1039040,1039039,2078079,1219.4045813083649,0.0032966790261070855
1041041,1041042,1041041,2082083,1222.002221107483,0.003243168073140623
1043043,1043044,1043043,2086087,1224.4227221012115,0.003190528749200894
1045045,1045046,1045045,2090091,1226.647140264511,0.0031387467795411794
1047047,1047048,1047047,2094095,1229.685678243637,0.003087808125428637
1049049,1049050,1049049,2098099,1231.8885962963104,0.0030376989797105125
1051051,1051052,1051051,2102103,1233.9673600196838,0.002988405763062474
1053053,1053054,1053053,2106107,1236.0173292160034,0.002939915120009573
1055055,1055056,1055055,2110111,1238.3990151882172,0.002892213915743014
1057057,1057058,1057057,2114115,1240.9705312252045,0.0028452892318000522
1059059,1059060,1059059,2118119,1243.783529996872,0.002799128362880765
1061061,1061062,1061061,2122123,1246.8645193576813,0.0027537188126416368
1063063,1063064,1063063,2126127,1249.0577883720398,0.002709048291194449
1065065,1065066,1065065,2130131,1251.2715373039246,0.0026651047113546156
1067067,1067068,1067067,2134135,1253.43514919281,0.0026218761843210814
1069069,1069070,1069069,2138139,1255.6487910747528,0.002579351017971021
1071071,1071072,1071071,2142143,1257.7626621723175,0.002537517712198678
1073073,1073074,1073073,2146147,1260.868046283722,0.0024963649563005674
1075075,1075076,1075075,2150151,1263.2794790267944,0.002455881626133305
1077077,1077078,1077077,2154155,1265.409235239029,0.0024160567803619415
1079079,1079080,1079079,2158159,1267.5299272537231,0.0023768796578451656
1081081,1081082,1081081,2162163,1269.6797981262207,0.0023383396744520724
1083083,1083084,1083083,2166167,1271.8288624286652,0.0023004264204473657
1085085,1085086,1085085,2170171,1273.90585231781,0.0022631296569670667
1087087,1087088,1087087,2174175,1276.1896872520447,0.0022264393138584637
1089089,1089090,1089089,2178179,1278.3698601722717,0.0021903454861558203
1091091,1091092,1091091,2182183,1280.4737792015076,0.0021548384321476988
1093093,1093094,1093093,2186187,1282.6487562656403,0.002119908570421103
1095095,1095096,1095095,2190191,1284.8034722805023,0.0020855464765645593
1097097,1097098,1097097,2194195,1286.8998172283173,0.0020517428810080673
1099099,1099100,1099099,2198199,1289.0790011882782,0.0020184886672041102
1101101,1101102,1101101,2202203,1291.2192842960358,0.0019857748676486153
1103103,1103104,1103103,2206207,1293.330527305603,0.001953592662630399
1105105,1105106,1105105,2210211,1295.3929982185364,0.0019219333767068747
1107107,1107108,1107107,2214215,1297.5064051151276,0.0018907884775671846
1109109,1109110,1109109,2218219,1299.6047611236572,0.0018601495726215944
1111111,1111112,1111111,2222223,1301.7095732688904,0.0018300084070688172
1113113,1113114,1113113,2226227,1303.8632152080536,0.0018003568616222765
1115115,1115116,1115115,2230231,1305.973120212555,0.0017711869504637434
1117117,1117118,1117117,2234235,1308.7422363758087,0.0017424908182874788
1119119,1119120,1119119,2238239,1311.4054503440857,0.0017142607393907383
1121121,1121122,1121121,2242243,1314.1377391815186,0.0016864891141494809
1123123,1123124,1123123,2246247,1316.4774022102356,0.0016591684677678131
1125125,1125126,1125125,2250251,1319.4115703105927,0.001632291448459
1127127,1127128,1127127,2254255,1322.2251591682434,0.001605850824148547
1129129,1129130,1129129,2258259,1324.7641642093658,0.0015798394820194517
1131131,1131132,1131131,2262263,1327.4848561286926,0.0015542504260110945
1133133,1133134,1133133,2266267,1329.8284912109375,0.0015290767739770672
1135135,1135136,1135135,2270271,1331.92906332016,0.0015043117572304254
1137137,1137138,1137137,2274275,1334.0707740783691,0.0014799487171330838
1139139,1139140,1139139,2278279,1336.6770460605621,0.0014559811053231897
1141141,1141142,1141141,2282283,1339.3219583034515,0.0014324024797360835
1143143,1143144,1143143,2286287,1341.83047914505,0.0014092065043769253
1145145,1145146,1145145,2290291,1344.5716841220856,0.0013863869468195844
1147147,1147148,1147147,2294295,1347.0847663879395,0.0013639376765013367
1149149,1149150,1149149,2298299,1349.610433101654,0.0013418526635859962
1151151,1151152,1151151,2302303,1352.2749981880188,0.0013201259766901785
1153153,1153154,1153153,2306307,1355.02982711792,0.0012987517817464322
1155155,1155156,1155155,2310311,1357.370970249176,0.001277724339956876
1157157,1157158,1157157,2314315,1359.6908390522003,0.0012570380064289566
1159159,1159160,1159159,2318319,1362.0371870994568,0.0012366872286975195
1161161,1161162,1161161,2322323,1364.3398714065552,0.0012166665453605674
1163163,1163164,1163163,2326327,1366.8538250923157,0.001196970584032897
1165165,1165166,1165165,2330331,1369.5436911582947,0.0011775940604366042
1167167,1167168,1167167,2334335,1371.803655385971,0.001158531776241034
1169169,1169170,1169169,2338339,1374.1668872833252,0.0011397786189490944
1171171,1171172,1171171,2342343,1376.513501405716,0.00112132955848665
1173173,1173174,1173173,2346347,1378.9101071357727,0.0011031796485667655
1175175,1175176,1175175,2350351,1381.3461632728577,0.0010853240223696048
1177177,1177178,1177177,2354355,1383.7353904247284,0.0010677578929971787
1179179,1179180,1179179,2358359,1385.944708108902,0.0010504765523364767
1181181,1181182,1181181,2362363,1388.1594061851501,0.0010334753685583564
1183183,1183184,1183183,2366367,1390.7836751937866,0.001016749785662796
1185185,1185186,1185185,2370371,1392.8468582630157,0.0010002953225694
1187187,1187188,1187187,2374375,1395.0906312465668,0.0009841075706162883
1189189,1189190,1189189,2378379,1397.5147902965546,0.0009681821935600965
1191191,1191192,1191191,2382383,1399.7620811462402,0.000952514926098047
1193193,1193194,1193193,2386387,1401.903643131256,0.0009371015722763332
1195195,1195196,1195195,2390391,1404.7322239875793,0.0009219380049216852
1197197,1197198,1197197,2394395,1406.752248287201,0.0009070201640497544
1199199,1199200,1199199,2398399,1408.8260543346405,0.0008923440558419315
1201201,1201202,1201201,2402403,1410.9907641410828,0.0008779057521905997
1203203,1203204,1203203,2406407,1413.0556771755219,0.0008637013886527711
1205205,1205206,1205205,2410411,1415.1061372756958,0.0008497271636542791
1207207,1207208,1207207,2414415,1417.2387850284576,0.0008359793382624048
1209209,1209210,1209209,2418419,1419.52041721344,0.0008224542341395136
1211211,1211212,1211211,2422423,1421.6978843212128,0.0008091482330883082
1213213,1213214,1213213,2426427,1424.0260710716248,0.0007960577758012732
1215215,1215216,1215215,2430431,1426.1781241893768,0.0007831793614059279
1217217,1217218,1217217,2434435,1428.5249571800232,0.0007705095453047761
1219219,1219220,1219219,2438439,1431.0999352931976,0.0007580449401984879
1221221,1221222,1221221,2442443,1433.3085162639618,0.0007457822131300418
1223223,1223224,1223223,2446447,1436.1381351947784,0.0007337180857120984
1225225,1225226,1225225,2450451,1438.5207459926605,0.0007218493333311926
1227227,1227228,1227227,2454455,1440.6575272083282,0.0007101727833287441
1229229,1229230,1229229,2458459,1443.5975041389465,0.0006986853155694916
1231231,1231232,1231231,2462463,1445.9995551109314,0.0006873838600540694
1233233,1233234,1233233,2466467,1448.0356884002686,0.0006762653969190069
1235235,1235236,1235235,2470471,1450.1062741279602,0.0006653269560956687
1237237,1237238,1237237,2474475,1452.1511392593384,0.0006545656151502044
1239239,1239240,1239239,2478479,1454.1978542804718,0.0006439784997382958
1241241,1241242,1241241,2482483,1456.228104352951,0.000633562782354602
1243243,1243244,1243243,2486487,1458.300802230835,0.0006233156808548301
1245245,1245246,1245245,2490491,1460.3504803180695,0.0006132344594789174
1247247,1247248,1247247,2494495,1462.5428822040558,0.0006033164263499202
1249249,1249250,1249249,2498499,1464.6127643585205,0.0005935589334740143
1251251,1251252,1251251,2502503,1466.670684337616,0.0005839593761720607
1253253,1253254,1253253,2506507,1470.0493791103363,0.0005745151921701108
1255255,1255256,1255255,2510511,1472.3459503650665,0.0005652238604625381
1257257,1257258,1257257,2514515,1474.5605483055115,0.0005560829017667857
1259259,1259260,1259259,2518519,1476.823545217514,0.0005470898767043764
1261261,1261262,1261261,2522523,1479.0509622097015,0.0005382423858009133
1263263,1263264,1263263,2526527,1481.3452532291412,0.0005295380683492112
1265265,1265266,1265265,2530531,1483.5569252967834,0.0005209746025229833
1267267,1267268,1267267,2534535,1485.6987102031708,0.0005125497036715387
1269269,1269270,1269269,2538539,1487.8953912258148,0.0005042611252292772
1271271,1271272,1271271,2542543,1490.3106801509857,0.0004961066563282657
1273273,1273274,1273273,2546547,1492.5212581157684,0.00048808412225298525
1275275,1275276,1275275,2550551,1494.7605073451996,0.0004801913837582106
1277277,1277278,1277277,2554555,1497.0795540809631,0.0004724263367279491
1279279,1279280,1279279,2558559,1499.1460900306702,0.0004647869105838254
1281281,1281282,1281281,2562563,1501.0579822063446,0.0004572710688535153
1283283,1283284,1283283,2566567,1502.9112162590027,0.00044987680837493826
1285285,1285286,1285285,2570571,1504.7442910671234,0.00044260215815938864
1287287,1287288,1287287,2574575,1506.629809141159,0.00043544517939153593
1289289,1289290,1289289,2578579,1508.79945230484,0.0004284039647473037
1291291,1291292,1291291,2582583,1510.7311780452728,0.000421476638052809
1293293,1293294,1293293,2586587,1512.8236072063446,0.0004146613534885546
1295295,1295296,1295295,2590591,1515.0292873382568,0.0004079562952483684
1297297,1297298,1297297,2594595,1517.4373021125793,0.00040135967742571665
1299299,1299300,1299299,2598599,1519.9045441150665,0.00039486974242208817
1301301,1301302,1301301,2602603,1522.3494262695312,0.0003884847616291154
1303303,1303304,1303303,2606607,1524.687905073166,0.00038220303440539283
1305305,1305306,1305305,2610611,1527.1193704605103,0.0003760228880764771
1307307,1307308,1307307,2614615,1529.6985154151917,0.0003699426767980185
1309309,1309310,1309309,2618619,1532.3572952747345,0.0003639607814420742
1311311,1311312,1311311,2622623,1534.7233390808105,0.0003580756093697346
1313313,1313314,1313313,2626627,1537.0912082195282,0.00035228559374900215
1315315,1315316,1315315,2630631,1539.5750153064728,0.00034658919321373105
1317317,1317318,1317317,2634635,1542.2963662147522,0.0003409848914088798
1319319,1319320,1319319,2638639,1544.9848492145538,0.0003354711966494506
1321321,1321322,1321321,2642643,1547.9361851215363,0.00033004664112468163
1323323,1323324,1323323,2646647,1550.59761428833,0.00032470978158016806
1325325,1325326,1325325,2650651,1553.4033222198486,0.00031945919761255936
1327327,1327328,1327327,2654655,1555.9572632312775,0.00031429349201061996
1329329,1329330,1329329,2658659,1558.6016011238098,0.0003092112904141686
1331331,1331332,1331331,2662663,1560.8804302215576,0.00030421124051827064
1333333,1333334,1333333,2666667,1562.9870212078094,0.00029929201230061153
1335335,1335336,1335335,2670671,1565.1478819847107,0.0002944522968846286
1337337,1337338,1337337,2674675,1567.3077671527863,0.0002896908069942583
1339339,1339340,1339339,2678679,1569.8125212192535,0.00028500627638550213
1341341,1341342,1341341,2682683,1572.4234974384308,0.0002803974587095581
1343343,1343344,1343343,2686687,1575.6725702285767,0.0002758631286496893
1345345,1345346,1345345,2690691,1577.9861900806427,0.00027140208021592116
1347347,1347348,1347347,2694695,1580.406016111374,0.00026701312708610203
1349349,1349350,1349349,2698699,1582.9955923557281,0.0002626951022648427
1351351,1351352,1351351,2702703,1585.515729188919,0.00025844685785614274
1353353,1353354,1353353,2706707,1587.5506403446198,0.00025426726438126934
1355355,1355356,1355355,2710711,1589.4715282917023,0.0002501552103240101
1357357,1357358,1357357,2714715,1591.379295349121,0.0002461096032675414
1359359,1359360,1359359,2718719,1593.2415311336517,0.0002421293673933178
1361361,1361362,1361361,2722723,1595.0947132110596,0.0002382134449590012
1363363,1363364,1363363,2726727,1596.8882853984833,0.00023436079538896593
1365365,1365366,1365365,2730731,1598.7015211582184,0.00023057039425111725
1367367,1367368,1367367,2734735,1600.5233809947968,0.00022684123462113348
1369369,1369370,1369369,2738739,1602.3526620864868,0.00022317232560453704
1371371,1371372,1371371,2742743,1604.2465453147888,0.00021956269222300762
1373373,1373374,1373373,2746747,1606.0925283432007,0.00021601137564175588
1375375,1375376,1375375,2750751,1607.9399712085724,0.00021251743203265505
1377377,1377378,1377377,2754755,1609.70428109169,0.00020907993337004882
1379379,1379380,1379379,2758759,1611.5087523460388,0.00020569796629388293
1381381,1381382,1381381,2762763,1613.3511281013489,0.00020237063267813937
1383383,1383384,1383383,2766767,1615.2471103668213,0.00019909704883502854
1385385,1385386,1385385,2770771,1618.0580060482025,0.00019587634494655504
1387387,1387388,1387387,2774775,1619.8613412380219,0.0001927076658603255
1389389,1389390,1389389,2778779,1621.6037890911102,0.0001895901699526803
1391391,1391392,1391391,2782783,1623.5735292434692,0.0001865230295834408
1393393,1393394,1393393,2786787,1625.4161632061005,0.00018350542984535423
1395395,1395396,1395395,2790791,1627.5291702747345,0.00018053656992833567
1397397,1397398,1397397,2794795,1630.4436402320862,0.00017761566141416552
1399399,1399400,1399399,2798799,1633.034897327423,0.00017474192884492368
1401401,1401402,1401401,2802803,1635.3506972789764,0.00017191460915455536
1403403,1403404,1403403,2806807,1637.4393222332,0.00016913295178255794
1405405,1405406,1405405,2810811,1639.4759571552277,0.00016639621844660724
1407407,1407408,1407407,2814815,1641.528052330017,0.00016370368268781021
1409409,1409410,1409409,2818819,1643.5809993743896,0.00016105462987070496
1411411,1411412,1411411,2822823,1645.6447343826294,0.00015844835684220016
1413413,1413414,1413413,2826827,1647.747724056244,0.00015588417181788827
1415415,1415416,1415415,2830831,1650.1337983608246,0.00015336139449573238
1417417,1417418,1417417,2834835,1652.7635781764984,0.00015087935503288463
1419419,1419420,1419419,2838839,1655.4879863262177,0.00014843739506886777
1421421,1421422,1421421,2842843,1657.635371208191,0.0001460348665887068
1423423,1423424,1423423,2846847,1660.0935411453247,0.00014367113203661575
1425425,1425426,1425425,2850851,1662.505666255951,0.00014134556465705828
1427427,1427428,1427427,2854855,1664.8571512699127,0.00013905754690313188
1429429,1429430,1429429,2858859,1666.9413242340088,0.00013680647214187047
1431431,1431432,1431431,2862863,1668.987386226654,0.00013459174294894183
1433433,1433434,1433433,2866867,1671.021960258484,0.00013241277190445544
1435435,1435436,1435435,2870871,1673.0615322589874,0.00013026898136558884
1437437,1437438,1437437,2874875,1675.0829071998596,0.0001281598022160324
1439439,1439440,1439439,2878879,1677.081208229065,0.0001260846750028577
1441441,1441442,1441441,2882883,1679.0259373188019,0.00012404304982283065
1443443,1443444,1443443,2886887,1680.9149980545044,0.0001220343848444827
1445445,1445446,1445445,2890891,1683.0184733867645,0.00012005814755866595
1447447,1447448,1447447,2894895,1685.5044062137604,0.0001181138138690585
1449449,1449450,1449449,2898899,1687.8065302371979,0.00011620086797847762
1451451,1451452,1451451,2902903,1690.113754272461,0.00011431880307100073
1453453,1453454,1453453,2906907,1692.4521181583405,0.00011246711960666289
1455455,1455456,1455455,2910911,1694.5121850967407,0.00011064532714044617
1457457,1457458,1457457,2914915,1697.0491321086884,0.00010885294193485606
1459459,1459460,1459459,2918919,1699.1728911399841,0.00010708948968840559
1461461,1461462,1461461,2922923,1701.1586964130402,0.00010535450235238386
1463463,1463464,1463463,2926927,1703.230004310608,0.00010364752017721912
1465465,1465466,1465465,2930931,1705.4771211147308,0.00010196809046192357
1467467,1467468,1467467,2934935,1707.6564161777496,0.00010031576823621435
1469469,1469470,1469469,2938939,1710.2295260429382,9.869011569207942e-05
1471471,1471472,1471471,2942943,1712.0737221240997,9.709070161534328e-05
1473473,1473474,1473473,2946947,1714.0463581085205,9.551710195410124e-05
1475475,1475476,1475475,2950951,1716.1741650104523,9.396890015977988e-05
1477477,1477478,1477477,2954955,1718.2360210418701,9.244568582289503e-05
1479479,1479480,1479479,2958959,1720.2599790096283,9.094705490042543e-05
1481481,1481482,1481481,2962963,1722.273742198944,8.947261062530742e-05
1483483,1483484,1483483,2966967,1724.354097366333,8.80219620285061e-05
1485485,1485486,1485485,2970971,1727.161472082138,8.659472484850994e-05
1487487,1487488,1487487,2974975,1729.5509660243988,8.519052107658354e-05
1489489,1489490,1489489,2978979,1731.785696029663,8.380897838833334e-05
1491491,1491492,1491491,2982983,1734.4206492900848,8.244973082582874e-05
1493493,1493494,1493493,2986987,1737.3196663856506,8.111241834285465e-05
1495495,1495496,1495495,2990991,1739.5852732658386,7.979668646385107e-05
1497497,1497498,1497497,2994995,1741.703839302063,7.85021870797209e-05
1499499,1499500,1499499,2998999,1743.6919343471527,7.722857674252737e-05
1501502,1501503,1501502,3003005,1745.634693145752,7.597489752697584e-05
1503504,1503505,1503504,3007009,1748.4528892040253,7.474206904589664e-05
1505506,1505507,1505506,3011013,1750.8261213302612,7.352913394242933e-05
1507508,1507509,1507508,3015017,1753.1792314052582,7.233577071019681e-05
1509510,1509511,1509510,3019021,1755.3055233955383,7.11616631861034e-05
1511512,1511513,1511512,3023025,1757.4166300296783,7.000650055033475e-05
1513514,1513515,1513514,3027029,1759.7181980609894,6.886997709898424e-05
1515516,1515517,1515516,3031033,1762.4113693237305,6.77517915619319e-05
1517518,1517519,1517518,3035037,1764.5850553512573,6.665164778496546e-05
1519520,1519521,1519520,3039041,1766.7494382858276,6.55692548434672e-05
1521522,1521523,1521522,3043045,1768.9783790111542,6.45043254507982e-05
1523524,1523525,1523524,3047049,1771.5284931659698,6.345657811834826e-05
1525526,1525527,1525526,3051053,1774.1410291194916,6.242573510917282e-05
1527528,1527529,1527528,3055057,1777.491051197052,6.141152380223502e-05
1529530,1529531,1529530,3059061,1780.6108992099762,6.0413675214476825e-05
1531532,1531533,1531532,3063065,1783.2649822235107,5.943192559243471e-05
1533534,1533535,1533534,3067069,1785.8170611858368,5.846601482062397e-05
1535536,1535537,1535536,3071073,1788.3684341907501,5.751568710365973e-05
1537538,1537539,1537538,3075077,1790.8419442176819,5.658069107994379e-05
1539540,1539541,1539540,3079081,1793.5088651180267,5.566077868479624e-05
1541542,1541543,1541542,3083085,1796.2326772212982,5.475570708313171e-05
1543544,1543545,1543544,3087089,1798.9553401470184,5.3865236395722604e-05
1545546,1545547,1545546,3091093,1801.5745091438293,5.298913060869381e-05
1547548,1547549,1547548,3095097,1805.4417552947998,5.212715836933057e-05
1549550,1549551,1549550,3099101,1809.172503232956,5.1279091053402226e-05
1551552,1551553,1551552,3103105,1812.9658932685852,5.0444704470464785e-05
1553554,1553555,1553554,3107109,1816.8152551651,4.962377772699256e-05
1555556,1555557,1555556,3111113,1820.4010922908783,4.8816093567438656e-05
1557558,1557559,1557558,3115117,1823.9436581134796,4.8021437805800815e-05
1559560,1559561,1559560,3119121,1827.5003063678741,4.7239600803550275e-05
1561562,1561563,1561562,3123125,1830.5213131904602,4.647037519589503e-05
1563564,1563565,1563564,3127129,1832.3818311691284,4.571355748339556e-05
1565566,1565567,1565566,3131133,1834.352697134018,4.4968947690904315e-05
1567568,1567569,1567568,3135137,1836.5257182121277,4.423634834438417e-05
1569570,1569571,1569570,3139141,1838.8547751903534,4.3515565721463645e-05
1571572,1571573,1571572,3143145,1840.941976070404,4.280640939668956e-05
1573574,1573575,1573574,3147149,1843.2303140163422,4.210869144571916e-05
1575576,1575577,1575576,3151153,1846.2252180576324,4.142222712744115e-05
1577578,1577579,1577578,3155157,1848.6949744224548,4.074683488397568e-05
1579580,1579581,1579580,3159161,1850.9575061798096,4.0082336340674374e-05
1581582,1581583,1581582,3163165,1852.798572063446,3.942855528293876e-05
1583584,1583585,1583584,3167169,1854.688448190689,3.87853189067755e-05
1585586,1585587,1585586,3171173,1856.6810281276703,3.815245690930169e-05
1587588,1587589,1587588,3175177,1858.644525051117,3.7529802284552716e-05
1589590,1589591,1589590,3179181,1860.802555322647,3.6917189959240204e-05
1591592,1591593,1591592,3183185,1862.6173791885376,3.6314457815933565e-05
1593594,1593595,1593594,3187189,1864.6354081630707,3.5721446351999475e-05
1595596,1595597,1595596,3191193,1866.601565361023,3.513799913434923e-05
1597598,1597599,1597598,3195197,1868.5113162994385,3.456396143519669e-05
1599600,1599601,1599600,3199201,1870.4600882530212,3.3999181482613494e-05
1601602,1601603,1601602,3203205,1872.5083122253418,3.344350977840804e-05
1603604,1603605,1603604,3207209,1874.4601011276245,3.289679978024651e-05
1605606,1605607,1605606,3211213,1876.346577167511,3.2358906423723965e-05
1607608,1607609,1607608,3215217,1878.206199169159,3.182968794135377e-05
1609610,1609611,1609610,3219221,1880.0757644176483,3.130900370251766e-05
1611612,1611613,1611612,3223225,1881.970165014267,3.079671625982883e-05
1613614,1613615,1613614,3227229,1883.8153421878815,3.029269032595039e-05
1615616,1615617,1615616,3231233,1885.6860060691833,2.9796792546221695e-05
1617618,1617619,1617618,3235237,1887.5701911449432,2.9308891612345178e-05
1619620,1619621,1619620,3239241,1889.4650511741638,2.8828858489760023e-05
1621622,1621623,1621622,3243245,1891.4452941417694,2.8356566531329008e-05
1623624,1623625,1623624,3247249,1893.4140622615814,2.7891890454156965e-05
1625626,1625627,1625626,3251253,1895.366698026657,2.743470759014599e-05
1627628,1627629,1627628,3255257,1897.232880115509,2.6984897090187587e-05
1629630,1629631,1629630,3259261,1899.0768761634827,2.654233992416266e-05
1631632,1631633,1631632,3263265,1900.9224331378937,2.610691899462836e-05
1633634,1633635,1633634,3267269,1902.7820122241974,2.5678519250504905e-05
1635636,1635637,1635636,3271273,1904.739518404007,2.525702757338877e-05
1637638,1637639,1637638,3275277,1906.6861753463745,2.4842332209118467e-05
1639640,1639641,1639640,3279281,1908.6711752414703,2.4434323790956114e-05
1641642,1641643,1641642,3283285,1910.615079164505,2.4032894089032197e-05
1643644,1643645,1643644,3287289,1912.52614402771,2.3637937488274474e-05
1645646,1645647,1645646,3291293,1914.3797192573547,2.3249349055731727e-05
1647648,1647649,1647648,3295297,1916.2234580516815,2.2867026473250007e-05
1649650,1649651,1649650,3299301,1918.0870792865753,2.249086821848323e-05
1651652,1651653,1651652,3303305,1919.9768242835999,2.2120775270195736e-05
1653654,1653655,1653654,3307309,1921.8475341796875,2.1756649630333413e-05
1655656,1655657,1655656,3311313,1923.819895029068,2.139839500614471e-05
1657658,1657659,1657658,3315317,1925.774109363556,2.104591692386748e-05
1659660,1659661,1659660,3319321,1927.6749923229218,2.0699121478173765e-05
1661662,1661663,1661662,3323325,1929.5790331363678,2.0357917946967063e-05
1663664,1663665,1663664,3327329,1931.4817831516266,2.0022215494464035e-05
1665666,1665667,1665666,3331333,1933.4063034057617,1.9691925672304933e-05
1667668,1667669,1667668,3335337,1935.2010560035706,1.9366961168998387e-05
1669670,1669671,1669670,3339341,1937.0464770793915,1.9047235809921403e-05
1671672,1671673,1671672,3343345,1938.868833065033,1.873266546681407e-05
1673674,1673675,1673674,3347349,1940.8094232082367,1.8423166807224334e-05
1675676,1675677,1675676,3351353,1942.633530139923,1.8118658090315876e-05
1677678,1677679,1677678,3355357,1944.4654173851013,1.781905871212075e-05
1679680,1679681,1679680,3359361,1946.2377500534058,1.752428920553939e-05
1681682,1681683,1681682,3363365,1948.0849232673645,1.7234272604582657e-05
1683684,1683685,1683684,3367369,1949.9322481155396,1.6948931261140388e-05
1685686,1685687,1685686,3371373,1951.8331673145294,1.666819036927336e-05
1687688,1687689,1687688,3375377,1953.704602241516,1.639197546410287e-05
1689690,1689691,1689690,3379381,1955.5689914226532,1.6120213672365935e-05
1691692,1691693,1691692,3383385,1957.4447112083435,1.585283291660744e-05
1693694,1693695,1693694,3387389,1959.319253206253,1.558976305204851e-05
1695696,1695697,1695696,3391393,1961.1962661743164,1.5330933933910273e-05
1697698,1697699,1697698,3395397,1963.0417392253876,1.5076277691150608e-05
1699700,1699701,1699700,3399401,1964.873375415802,1.482572668010107e-05
1701702,1701703,1701702,3403405,1966.8039500713348,1.4579215076082619e-05
1703704,1703705,1703704,3407409,1969.4445323944092,1.4336677054416214e-05
1705706,1705707,1705706,3411413,1972.0321652889252,1.4098049405220081e-05
1707708,1707709,1707708,3415417,1974.3623502254486,1.386326835017826e-05
1709710,1709711,1709710,3419421,1976.557597398758,1.3632272157337866e-05
1711712,1711713,1711712,3423425,1978.7060720920563,1.3404999890553881e-05
1713714,1713715,1713714,3427429,1980.8700354099274,1.3181391182115476e-05
1715716,1715717,1715716,3431433,1982.9430310726166,1.2961387255927548e-05
1717718,1717719,1717718,3435437,1984.9495553970337,1.274493001801602e-05
1719720,1719721,1719720,3439441,1986.8413853645325,1.2531961942841008e-05
1721722,1721723,1721722,3443445,1988.769944190979,1.2322426869104675e-05
1723724,1723725,1723724,3447449,1990.5789651870728,1.2116269658690726e-05
1725726,1725727,1725726,3451453,1992.553304195404,1.1913435741917056e-05
1727728,1727729,1727728,3455457,1994.6934731006622,1.1713871117535746e-05
1729730,1729731,1729730,3459461,1996.5574142932892,1.1517523603288282e-05
1731732,1731733,1731732,3463465,1998.454291343689,1.1324341357976664e-05
1733734,1733735,1733734,3467469,2000.321393251419,1.1134272881463403e-05
1735736,1735737,1735736,3471473,2002.133599281311,1.0947268492600415e-05
1737738,1737739,1737738,3475477,2004.2353973388672,1.076327828286594e-05
1739740,1739741,1739740,3479481,2006.592785358429,1.0582253707980271e-05
1741742,1741743,1741742,3483485,2009.023389339447,1.0404147474218917e-05
1743744,1743745,1743744,3487489,2011.2386491298676,1.0228912060483708e-05
1745746,1745747,1745746,3491493,2013.3526504039764,1.0056501196231693e-05
1747748,1747749,1747748,3495497,2015.5162591934204,9.886869406727783e-06
1749750,1749751,1749750,3499501,2017.7110702991486,9.719971899357915e-06
1751752,1751753,1751752,3503505,2019.8375353813171,9.555764563629054e-06
1753754,1753755,1753754,3507509,2021.869430065155,9.394204198542866e-06
1755756,1755757,1755756,3511513,2024.2191181182861,9.235247603101016e-06
1757758,1757759,1757758,3515517,2026.0087022781372,9.078853622668248e-06
1759760,1759761,1759760,3519521,2027.906836271286,8.924980193114607e-06
1761762,1761763,1761762,3523525,2029.9431381225586,8.773587182986375e-06
1763764,1763765,1763764,3527529,2031.992567062378,8.624634119769325e-06
1765766,1765767,1765766,3531533,2033.9042212963104,8.47808189519128e-06
1767768,1767769,1767768,3535537,2035.8724331855774,8.333891855727416e-06
1769770,1769771,1769770,3539541,2037.7473771572113,8.192026143660769e-06
1771772,1771773,1771772,3543545,2039.6825802326202,8.052446787587542e-06
1773774,1773775,1773774,3547549,2041.6023533344269,7.915117180345987e-06
1775776,1775777,1775776,3551553,2043.4609372615814,7.780001055834873e-06
1777778,1777779,1777778,3555557,2045.3093492984772,7.647062830073992e-06
1779780,1779781,1779780,3559561,2047.1458129882812,7.51626726014365e-06
1781782,1781783,1781782,3563565,2049.0132281780243,7.387579557871504e-06
1783784,1783785,1783784,3567569,2050.8603451251984,7.260966185640427e-06
1785786,1785787,1785786,3571573,2052.768976211548,7.136393378459616e-06
1787788,1787789,1787788,3575577,2054.6828322410583,7.013828508206643e-06
1789790,1789791,1789790,3579581,2056.6280751228333,6.893238946759084e-06
1791792,1791793,1791792,3583585,2058.568966150284,6.774593089176051e-06
1793794,1793795,1793794,3587589,2060.4307692050934,6.657859330516658e-06
1795796,1795797,1795796,3591593,2062.2971770763397,6.54300697533472e-06
1797798,1797799,1797798,3595597,2064.2885291576385,6.430006010305078e-06
1799800,1799801,1799800,3599601,2066.1327612400055,6.318825967355224e-06
1801802,1801803,1801802,3603605,2067.9729363918304,6.2094378563415376e-06
1803804,1803805,1803804,3607609,2069.7562041282654,6.101812800807238e-06
1805806,1805807,1805806,3611613,2071.5303761959076,5.995922379042895e-06
1807808,1807809,1807808,3615617,2073.3151910305023,5.891738283025916e-06
1809810,1809811,1809810,3619621,2075.145938396454,5.789233455288922e-06
1811812,1811813,1811812,3623625,2076.965705394745,5.688380838364537e-06
1813814,1813815,1813814,3627629,2078.751083135605,5.589153374785383e-06
1815816,1815817,1815816,3631633,2080.5045642852783,5.4915250302656204e-06
1817818,1817819,1817818,3635637,2082.266384124756,5.3954704526404385e-06
1819820,1819821,1819820,3639641,2084.0162732601166,5.300963834997674e-06
1821822,1821823,1821822,3643645,2085.716944217682,5.207980166233028e-06
1823824,1823825,1823824,3647649,2087.3996522426605,5.116495003676391e-06
1825826,1825827,1825826,3651653,2089.0967993736267,5.026484473091841e-06
1827828,1827829,1827828,3655657,2090.8549041748047,4.937924245496106e-06
1829830,1829831,1829830,3659661,2092.6116983890533,4.850791469834803e-06
1831832,1831833,1831832,3663665,2094.3946533203125,4.7650630676798755e-06
1833834,1833835,1833834,3667669,2096.126430273056,4.6807159606032656e-06
1835836,1835837,1835836,3671673,2097.822911262512,4.597728207045293e-06
1837838,1837839,1837838,3675677,2099.5206611156464,4.516077979133115e-06
1839840,1839841,1839840,3679681,2101.2820003032684,4.435743676367565e-06
1841842,1841843,1841842,3683685,2103.1355521678925,4.356703811936313e-06
1843844,1843845,1843844,3687689,2105.0850973129272,4.27893792220857e-06
1845846,1845847,1845846,3691693,2106.966100215912,4.202425202493032e-06
1847848,1847849,1847848,3695697,2108.862169265747,4.127145530219423e-06
1849850,1849851,1849850,3699701,2110.5499591827393,4.053078896504303e-06
1851852,1851853,1851852,3703705,2112.2491822242737,3.980206088272098e-06
1853854,1853855,1853854,3707709,2114.051525115967,3.9085075513867196e-06
1855856,1855857,1855856,3711713,2115.8875272274017,3.837964413833106e-06
1857858,1857859,1857858,3715717,2117.7193484306335,3.7685581446567085e-06
1859860,1859861,1859860,3719721,2119.4642980098724,3.700270440276654e-06
1861862,1861863,1861862,3723725,2121.2356543540955,3.6330829971120693e-06
1863864,1863865,1863864,3727729,2122.9612152576447,3.566978421076783e-06
1865866,1865867,1865866,3731733,2124.65288233757,3.501939204397786e-06
1867868,1867869,1867868,3735737,2126.332998275757,3.4379479529889068e-06
1869870,1869871,1869870,3739741,2128.0520782470703,3.3749879548850004e-06
1871872,1871873,1871872,3743745,2129.7804222106934,3.3130424981209217e-06
1873874,1873875,1873874,3747749,2131.5558621883392,3.2520953254788765e-06
1875876,1875877,1875876,3751753,2133.301965236664,3.192130407114746e-06
1877878,1877879,1877878,3755757,2135.084784269333,3.1331317131844116e-06
1879880,1879881,1879880,3759761,2136.763393163681,3.075083782277943e-06
1881882,1881883,1881882,3763765,2138.4687070846558,3.0179713803590857e-06
1883884,1883885,1883884,3767769,2140.1770632267,2.961779159704747e-06
1885886,1885887,1885886,3771773,2141.8552281856537,2.906492568399699e-06
1887888,1887889,1887888,3775777,2143.5832302570343,2.8520968271550373e-06
1889890,1889891,1889890,3779781,2145.3363950252533,2.7985774977423716e-06
1891892,1891893,1891892,3783785,2147.121174097061,2.7459208240543376e-06
1893894,1893895,1893894,3787789,2148.8340673446655,2.69411259523622e-06
1895896,1895897,1895896,3791793,2150.5287911891937,2.6431393962411676e-06
1897898,1897899,1897898,3795797,2152.2158482074738,2.5929873572749784e-06
1899900,1899901,1899900,3799801,2153.9326951503754,2.5436434043513145e-06
1901902,1901903,1901902,3803805,2155.6022703647614,2.495094804544351e-06
1903904,1903905,1903904,3807809,2157.329725265503,2.44732848386775e-06
1905906,1905907,1905906,3811813,2159.0463490486145,2.4003318230825244e-06
1907908,1907909,1907908,3815817,2160.7503912448883,2.3540924303233624e-06
1909910,1909911,1909910,3819821,2162.505942106247,2.308598141098628e-06
1911912,1911913,1911912,3823825,2164.258505344391,2.26383701829036e-06
1913914,1913915,1913914,3827829,2165.956210374832,2.219797124780598e-06
1915916,1915917,1915916,3831833,2167.650395154953,2.1764669781987322e-06
1917918,1917919,1917918,3835837,2169.2945952415466,2.133834982487315e-06
1919920,1919921,1919920,3839841,2170.9742062091827,2.091890110023087e-06
1921922,1921923,1921922,3843845,2172.7679150104523,2.0506208784354385e-06
1923924,1923925,1923924,3847849,2174.5235781669617,2.0100167148484616e-06
1925926,1925927,1925926,3851853,2176.2663311958313,1.970066705325735e-06
1927928,1927929,1927928,3855857,2177.969206094742,1.9307605043650256e-06
1929930,1929931,1929930,3859861,2179.6455051898956,1.8920877664641012e-06
1931932,1931933,1931932,3863865,2181.3498392105103,1.854038146120729e-06
1933934,1933935,1933934,3867869,2183.050270318985,1.816601752580027e-06
1935936,1935937,1935936,3871873,2184.752712249756,1.7797683540266007e-06
1937938,1937939,1937938,3875877,2186.4471900463104,1.743528514452919e-06
1939940,1939941,1939940,3879881,2188.203058242798,1.707872684164613e-06
1941942,1941943,1941942,3883885,2189.932178258896,1.67279154084099e-06
1943944,1943945,1943944,3887889,2191.6336681842804,1.638275534787681e-06
1945946,1945947,1945946,3891893,2193.3277072906494,1.6043156847445061e-06
1947948,1947949,1947948,3895897,2195.041783094406,1.5709031231381232e-06
1949950,1949951,1949950,3899901,2196.7351381778717,1.5380287550215144e-06
1951952,1951953,1951952,3903905,2198.4211101531982,1.505684281255526e-06
1953954,1953955,1953954,3907909,2200.1235201358795,1.4738608342668158e-06
1955956,1955957,1955956,3911913,2201.808427095413,1.4425503422899055e-06
1957958,1957959,1957958,3915917,2203.4814841747284,1.411744278811966e-06
1959960,1959961,1959960,3919921,2205.2077622413635,1.3814345720675192e-06
1961962,1961963,1961962,3923925,2206.971328020096,1.3516131502910866e-06
1963964,1963965,1963964,3927929,2208.69366812706,1.3222722827777034e-06
1965966,1965967,1965966,3931933,2210.376985311508,1.2934042388224043e-06
1967968,1967969,1967968,3935937,2212.064583301544,1.2650012877202244e-06
1969970,1969971,1969970,3939941,2213.754531145096,1.2370561535135494e-06
1971972,1971973,1971972,3943945,2215.4443802833557,1.2095609918105765e-06
1973974,1973975,1973974,3947949,2217.152451276779,1.1825089814010425e-06
1975976,1975977,1975976,3951953,2218.838847398758,1.1558930737010087e-06
1977978,1977979,1977978,3955957,2220.533839225769,1.129705879066023e-06
1979980,1979981,1979980,3959961,2222.253467321396,1.1039404625989846e-06
1981982,1981983,1981982,3963965,2223.96085524559,1.0785903441501432e-06
1983984,1983985,1983984,3967969,2225.6381413936615,1.0536487025092356e-06
1985986,1985987,1985986,3971973,2227.341639280319,1.0291088301528362e-06
1987988,1987989,1987988,3975977,2229.3334143161774,1.0049644743048702e-06
1989990,1989991,1989990,3979981,2231.2624881267548,9.812091548155877e-07
1991992,1991993,1991992,3983985,2233.1158192157745,9.57836505222076e-07
1993994,1993995,1993994,3987989,2234.992618083954,9.348403864350985e-07
1995996,1995997,1995996,3991993,2236.679386138916,9.122148867390933e-07
1997998,1997999,1997998,3995997,2238.3879251480103,8.899539807316614e-07
2000000,2000001,2000000,4000001,2240.1321170330048,8.680516430104035e-07


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0005650520324707031,2181.2938132599165
1,4,4,8,0.0019378662109375,1650.9600894919724
2,6,6,12,0.0030868053436279297,786.9009567073322
3,8,8,16,0.004029989242553711,443.58608911943384
4,12,12,24,0.005432844161987305,300.56155646592265
5,20,20,40,0.007476091384887695,289.3974206603966
6,24,24,48,0.008771181106567383,223.69526839628975
7,32,32,64,0.010661840438842773,220.72167943146133
8,36,36,72,0.011862993240356445,183.69180242892548
9,44,44,88,0.014126062393188477,182.02986018160618
10,50,50,100,0.01618790626525879,181.17567132880208
11,56,56,112,0.018147945404052734,170.03638269693147
12,60,60,120,0.01933002471923828,148.57486999488424
13,64,64,128,0.020489931106567383,133.65412768561646
14,70,70,140,0.022565841674804688,109.77584992925767
15,72,72,144,0.02368903160095215,82.14485419750099
16,76,76,152,0.025273799896240234,80.83922421752368
17,80,80,160,0.026824951171875,78.96080307353009
18,88,88,176,0.029392004013061523,78.7719300343806
19,92,92,184,0.03115081787109375,75.49803880435866
20,96,96,192,0.032891035079956055,73.83934276444575
21,102,102,204,0.03518104553222656,73.37869766012068
22,106,106,212,0.036707162857055664,70.68360968449633
23,110,110,220,0.03832602500915527,69.18156561569117
24,116,116,232,0.04058504104614258,68.41646619118296
25,124,124,248,0.04332709312438965,68.3663813211524
26,128,128,256,0.044970035552978516,65.3897452770234
27,134,134,268,0.047178030014038086,64.9236398858518
28,138,138,276,0.04865312576293945,62.985472947437074
29,146,146,292,0.05112409591674805,62.95210477775822
30,150,150,300,0.052577972412109375,60.535359788497544
31,158,158,316,0.05451393127441406,60.50873240431133
32,162,162,324,0.0559239387512207,58.29827656607495
33,168,168,336,0.05773186683654785,57.92439847378023
34,172,172,344,0.05887198448181152,56.76619974948835
35,180,180,360,0.06115579605102539,56.754147744358306
36,184,184,368,0.06280875205993652,55.729978746412826
37,188,188,376,0.06395912170410156,55.19744382774138
38,196,196,392,0.06624889373779297,55.19050256349988
39,200,200,400,0.06739997863769531,54.64523022558342
40,208,208,416,0.06950712203979492,54.640314439927806
41,212,212,424,0.07103395462036133,54.108094140376124
42,220,220,440,0.07371020317077637,54.10375604936826
43,226,226,452,0.0758049488067627,53.877086292780405
44,234,234,468,0.07831001281738281,53.87330472012718
45,240,240,480,0.08030200004577637,53.49811888471481
46,248,248,496,0.0827641487121582,53.49460341009626
47,254,254,508,0.09033918380737305,52.9254795429415
48,262,262,524,0.09487295150756836,52.92221640965681
49,268,268,536,0.09690499305725098,52.26786738777196
50,276,276,552,0.09890580177307129,52.26485072563719
51,282,282,564,0.10049891471862793,51.44443076873904
52,290,290,580,0.10249495506286621,51.44147432892464
53,298,298,596,0.10501599311828613,51.438536470135205
54,306,306,612,0.10766386985778809,51.435615587362236
55,312,312,624,0.10930681228637695,49.7136069230437
56,320,320,640,0.1113119125366211,49.71073909746406
57,328,328,656,0.1140749454498291,49.70791406796411
58,336,336,672,0.11710000038146973,49.7051272194808
59,342,342,684,0.11895895004272461,47.47352121865515
60,350,350,700,0.1216888427734375,47.47091040218811
61,358,358,716,0.12419414520263672,47.468338978416114
62,366,366,732,0.1266341209411621,47.46580319891996
63,372,372,744,0.12841510772705078,44.90985403410468
64,380,380,760,0.13109779357910156,44.90739089077556
65,388,388,776,0.13387298583984375,44.90496943583321
66,396,396,792,0.13707709312438965,44.90258587415542
67,404,404,808,0.13986992835998535,44.90023677588715
68,410,410,820,0.14169907569885254,41.79387968652577
69,418,418,836,0.14455819129943848,41.79184236490073
70,424,424,848,0.1465449333190918,38.947228266797765
71,432,432,864,0.1487410068511963,38.94540290101531
72,440,440,880,0.15136003494262695,38.9435920282051
73,448,448,896,0.15386199951171875,38.941794501922686
74,454,454,908,0.15588998794555664,35.960261131487414
75,462,462,924,0.15852022171020508,35.95861437940107
76,468,468,936,0.160567045211792,33.287248377427886
77,476,476,952,0.16292095184326172,33.28577475992529
78,482,482,964,0.1645510196685791,30.539653791511455
79,488,488,976,0.16628098487854004,29.615008422158553
80,496,496,992,0.1684858798980713,29.61365911296957
81,502,502,1004,0.17035913467407227,27.041313078749454
82,510,510,1020,0.1724071502685547,27.040106249533892
83,516,516,1032,0.17441201210021973,24.651822871100194
84,524,524,1048,0.17693710327148438,24.650662686907026
85,530,530,1060,0.17895889282226562,21.926916595581133
86,538,538,1076,0.18155384063720703,21.925876387494327
87,544,544,1088,0.1838829517364502,19.38987887854023
88,552,552,1104,0.18660902976989746,19.388930271255276
89,558,558,1116,0.18898987770080566,16.608093985512596
90,566,566,1132,0.1918489933013916,16.60720854258807
91,572,572,1144,0.19408202171325684,14.340721007916954
92,580,580,1160,0.19652891159057617,14.339894160041126
93,586,586,1172,0.19814395904541016,12.296962068950279
94,594,594,1188,0.20064306259155273,12.29616325254949
95,600,600,1200,0.20230889320373535,10.510741953040451
96,608,608,1216,0.20458292961120605,10.510010324363634
97,614,614,1228,0.2061781883239746,9.014298594634283
98,622,622,1244,0.2081458568572998,9.013638444774529
99,630,630,1260,0.2100968360900879,9.01298080384538
100,638,638,1276,0.21232891082763672,9.012325589257216
101,644,644,1288,0.2139129638671875,7.780570310155326
102,652,652,1304,0.21584391593933105,7.779951526052514
103,658,658,1316,0.21737194061279297,6.819609936315487
104,666,666,1332,0.21929502487182617,6.819035208742889
105,674,674,1348,0.22133517265319824,6.818470923337259
106,682,682,1364,0.22345495223999023,6.817916235665393
107,688,688,1376,0.2255251407623291,5.9367486603406405
108,696,696,1392,0.22815585136413574,5.936211169413809
109,702,702,1404,0.2298288345336914,5.174314634658003
110,710,710,1420,0.23187994956970215,5.173815290662105
111,716,716,1432,0.23352813720703125,4.494302502301821
112,724,724,1448,0.23577284812927246,4.493820308759155
113,730,730,1460,0.23806285858154297,3.8866757925634374
114,738,738,1476,0.24089717864990234,3.8862466840530487
115,744,744,1488,0.24311399459838867,3.3576534065056194
116,752,752,1504,0.24571919441223145,3.357269581602168
117,758,758,1516,0.24735116958618164,2.880300846288719
118,766,766,1532,0.24935102462768555,2.8799550688476074
119,772,772,1544,0.25095391273498535,2.471740110092469
120,780,780,1560,0.2529909610748291,2.47143597397735
121,786,786,1572,0.25462794303894043,2.112352332036494
122,792,792,1584,0.25630688667297363,1.8133498744381313
123,798,798,1596,0.2578911781311035,1.4925185789629722
124,806,806,1612,0.259829044342041,1.4922642545719782
125,812,812,1624,0.2613718509674072,1.2760333677532572
126,820,820,1640,0.2639601230621338,1.2758055117387812
127,826,826,1652,0.26598095893859863,1.0747965742291399
128,834,834,1668,0.26834583282470703,1.0745936419660893
129,838,838,1676,0.26966094970703125,0.5794730414766036
130,846,846,1692,0.2723050117492676,0.5792765367091306
131,850,850,1700,0.27399516105651855,0.31190445181914583
132,858,858,1716,0.27664899826049805,0.3117665257838098
133,862,862,1724,0.278270959854126,0.16648912514040148
134,866,866,1732,0.27990293502807617,0.09332014461233484
135,872,872,1744,0.2821509838104248,0.0809951449637083
136,876,876,1752,0.28388404846191406,0.050160142572963196
137,880,880,1760,0.2853879928588867,0.032760873621782594
138,884,884,1768,0.28720998764038086,0.025375763368288062
139,888,888,1776,0.2887740135192871,0.021377153048092623
140,896,896,1792,0.29086995124816895,0.02133605104631897
141,900,900,1800,0.29208803176879883,0.016293070737106063
142,908,908,1816,0.2947530746459961,0.016264277908248914
143,912,912,1824,0.2962930202484131,0.012659173853762695
144,920,920,1840,0.29937005043029785,0.01263847739414814
145,924,924,1848,0.30092597007751465,0.009445123849559423
146,928,928,1856,0.30254483222961426,0.006891616261100353
147,936,936,1872,0.30533504486083984,0.0068789167659133454
148,940,940,1880,0.3071911334991455,0.0055435354696555805
149,948,948,1896,0.3099949359893799,0.00553332780089022
150,952,952,1904,0.3112339973449707,0.004343211079117282
151,960,960,1920,0.31325292587280273,0.0043347196871081906
152,964,964,1928,0.3144259452819824,0.0033238844248444366
153,970,970,1940,0.3169548511505127,0.003086398933987766
154,976,976,1952,0.31873393058776855,0.002892278228387113
155,980,980,1960,0.32044291496276855,0.0022202596724127943
156,988,988,1976,0.3235180377960205,0.0022151515900077356
157,992,992,1984,0.3251199722290039,0.0016091770994535182
158,1000,1000,2000,0.3271369934082031,0.0016054316405416102
159,1004,1004,2008,0.3290250301361084,0.0011430153840592538
160,1010,1010,2020,0.3312230110168457,0.001062806116806314
161,1014,1014,2028,0.33281898498535156,0.0007474035813856972
162,1020,1020,2040,0.33504486083984375,0.0006953956898314573
163,1024,1024,2048,0.33707189559936523,0.0005246692453511059
164,1030,1030,2060,0.33965110778808594,0.0004972708296691053
165,1034,1034,2068,0.34188389778137207,0.0003823883920404114
166,1042,1042,2084,0.3446199893951416,0.0003814495393044126
167,1046,1046,2092,0.3464689254760742,0.0002918856743008291
168,1052,1052,2104,0.34845900535583496,0.0002755629951707306
169,1058,1058,2116,0.3505978584289551,0.00026029314460629394
170,1062,1062,2124,0.35228705406188965,0.00019450272384347045
171,1068,1068,2136,0.3545229434967041,0.00018278977529462281
172,1074,1074,2148,0.35698699951171875,0.0001719445128856023
173,1078,1078,2156,0.35836195945739746,0.00013496233327714435
174,1084,1084,2168,0.36000895500183105,0.00012825582348341413
175,1088,1088,2176,0.36167311668395996,0.00010706492435019754
176,1094,1094,2188,0.36350202560424805,0.00010324783352189115
177,1098,1098,2196,0.36501502990722656,8.610767258687702e-05
178,1106,1106,2212,0.3678560256958008,8.592472920554428e-05
179,1110,1110,2220,0.36959290504455566,6.744613813225442e-05
180,1116,1116,2232,0.37186098098754883,6.424260652693192e-05
181,1120,1120,2240,0.3738870620727539,5.4416926218436856e-05
182,1126,1126,2252,0.37631702423095703,5.254078371308424e-05
183,1132,1132,2264,0.3785128593444824,5.0766687422765244e-05
184,1136,1136,2272,0.3802361488342285,4.44698126784715e-05
185,1140,1140,2280,0.38187599182128906,3.9589785956195556e-05
186,1148,1148,2296,0.3843238353729248,3.953774364617857e-05
187,1152,1152,2304,0.3861660957336426,3.3837318710538966e-05
188,1156,1156,2312,0.38814496994018555,2.9217035148576542e-05
189,1164,1164,2328,0.39218902587890625,2.9172171366553812e-05
190,1168,1168,2336,0.3940460681915283,2.4958050175882818e-05
191,1172,1172,2344,0.3957839012145996,2.0890831137876376e-05
192,1180,1180,2360,0.39831089973449707,2.085558344333549e-05
193,1184,1184,2368,0.3999481201171875,1.7467220004618866e-05
194,1192,1192,2384,0.40252017974853516,1.743914924645651e-05
195,1196,1196,2392,0.4037439823150635,1.3840700148648466e-05
196,1204,1204,2408,0.40649914741516113,1.381813206080551e-05
197,1208,1208,2416,0.40824389457702637,1.0393337561254157e-05
198,1216,1216,2432,0.41069793701171875,1.0377167541264498e-05
199,1220,1220,2440,0.41185688972473145,7.665222938157967e-06
200,1228,1228,2456,0.4138450622558594,7.651546525266895e-06
201,1232,1232,2464,0.4152719974517822,5.4896534038562095e-06
202,1240,1240,2480,0.417525053024292,5.48006596545747e-06
203,1244,1244,2488,0.41887497901916504,3.9288286188821075e-06
204,1252,1252,2504,0.42142391204833984,3.922081987184356e-06
205,1256,1256,2512,0.42308616638183594,2.8830952487624018e-06
206,1264,1264,2528,0.4250919818878174,2.878218651858333e-06
207,1268,1268,2536,0.42624497413635254,2.181166337322793e-06
208,1274,1274,2548,0.42781591415405273,2.059618964267429e-06
209,1278,1278,2556,0.4289522171020508,1.7095497923946823e-06
210,1286,1286,2572,0.43091678619384766,1.7063545101336786e-06
211,1290,1290,2580,0.4323158264160156,1.4161586250338587e-06
212,1296,1296,2592,0.4346041679382324,1.3648367485075141e-06
213,1302,1302,2604,0.437391996383667,1.3123968756190152e-06
214,1308,1308,2616,0.43955397605895996,1.2613271564987372e-06
215,1312,1312,2624,0.4408130645751953,1.0993429668815224e-06
216,1320,1320,2640,0.4428081512451172,1.0975418263114989e-06
217,1324,1324,2648,0.44460201263427734,9.043033060152084e-07
218,1332,1332,2664,0.4470038414001465,9.028540262079332e-07
219,1336,1336,2672,0.44831013679504395,7.182483159340336e-07
220,1344,1344,2688,0.4504368305206299,7.169280706875725e-07
221,1348,1348,2696,0.4518458843231201,5.373093472371693e-07
222,1352,1352,2704,0.45310282707214355,3.997984094894491e-07
223,1360,1360,2720,0.4551889896392822,3.9905967241793405e-07
224,1364,1364,2728,0.4566640853881836,2.8994077183597255e-07
225,1368,1368,2736,0.45785093307495117,1.970372522919206e-07
226,1376,1376,2752,0.4597897529602051,1.9649212390504545e-07
227,1380,1380,2760,0.46093010902404785,1.259768396266736e-07
228,1386,1386,2772,0.462507963180542,1.1362101304257521e-07
229,1392,1392,2784,0.4641149044036865,1.0229246072412934e-07
230,1398,1398,2796,0.4659850597381592,9.046414106705924e-08
231,1404,1404,2808,0.4677917957305908,7.983339855854865e-08
232,1410,1410,2820,0.469512939453125,6.987067990849027e-08
233,1416,1416,2832,0.47113990783691406,5.772221811639611e-08
234,1422,1422,2844,0.47311902046203613,4.715229806606658e-08
235,1426,1426,2852,0.4743349552154541,1.4687429938931018e-08
236,1434,1434,2868,0.4763360023498535,1.4476313481281977e-08
237,1438,1438,2876,0.47750210762023926,9.40292466111714e-09


==> extragradient/plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0013971328735351562,2181.2938132599165
1,4,4,8,0.0028219223022460938,1650.9600894919724
2,6,6,12,0.00410914421081543,811.2562314125337
3,8,8,16,0.0052759647369384766,540.4289308351636
4,10,10,20,0.006644010543823242,340.4672839375705
5,12,12,24,0.007918834686279297,246.045559467972
6,14,14,28,0.009087085723876953,179.15645943945333
7,18,18,36,0.010715961456298828,176.09590819170626
8,22,22,44,0.012698888778686523,179.49204530230872
9,24,24,48,0.014139890670776367,132.26997085802282
10,26,26,52,0.01567816734313965,127.41736922878476
11,28,28,56,0.017106056213378906,131.37556663863074
12,32,32,64,0.019366025924682617,126.84435295539743
13,34,34,68,0.021001100540161133,106.30186430969206
14,36,36,72,0.023188114166259766,102.88115960850382
15,40,40,80,0.024930238723754883,102.47618365977314
16,44,44,88,0.026534080505371094,101.82312920170057
17,46,46,92,0.027615070343017578,97.15490589928982
18,50,50,100,0.029797077178955078,94.33019338730924
19,52,52,104,0.031145095825195312,80.4903442751745
20,54,54,108,0.03242802619934082,81.31254268609837
21,56,56,112,0.03369498252868652,81.88121702865942
22,58,58,116,0.03488326072692871,81.27086783594427
23,60,60,120,0.036536216735839844,76.74140494959192
24,62,62,124,0.037748098373413086,76.99510499544522
25,64,64,128,0.03890204429626465,74.5431711425615
26,66,66,132,0.04004526138305664,74.69278249642502
27,70,70,140,0.041754961013793945,74.56441781853619
28,72,72,144,0.04288220405578613,69.9782011093198
29,76,76,152,0.04479217529296875,69.91225327359734
30,78,78,156,0.0460970401763916,66.26838141079611
31,82,82,164,0.04790902137756348,66.27073562276814
32,84,84,168,0.049139976501464844,63.481344845964486
33,86,86,172,0.05089592933654785,63.7190912540359
34,88,88,176,0.05202007293701172,63.90336556497323
35,92,92,184,0.05359387397766113,63.807608879668805
36,94,94,188,0.05482196807861328,61.566793292530974
37,98,98,196,0.056558847427368164,61.52688100814953
38,100,100,200,0.05767107009887695,58.904292568147866
39,104,104,208,0.059439897537231445,58.88762163541469
40,106,106,212,0.06048011779785156,57.717888333730116
41,108,108,216,0.061654090881347656,57.62514878141383
42,110,110,220,0.06323695182800293,57.529530762268905
43,112,112,224,0.06441497802734375,57.41867547769448
44,116,116,232,0.06638288497924805,57.40215875999911
45,118,118,236,0.06744813919067383,56.81739714880291
46,120,120,240,0.06854510307312012,56.67589043198427
47,122,122,244,0.0696871280670166,56.457494112811446
48,126,126,252,0.0712900161743164,56.43205628063629
49,128,128,256,0.07230210304260254,55.982180017030714
50,132,132,264,0.07402706146240234,55.978461192982195
51,134,134,268,0.0751039981842041,54.69553390432793
52,138,138,276,0.07675719261169434,54.695983044795184
53,140,140,280,0.07784104347229004,54.45590175028951
54,144,144,288,0.07990217208862305,54.445062997060404
55,146,146,292,0.08104991912841797,53.8193328940863
56,150,150,300,0.08283305168151855,53.816132750525185
57,152,152,304,0.08396601676940918,53.525672145477074
58,156,156,312,0.08564519882202148,53.522790263717525
59,158,158,316,0.08673906326293945,53.34773220655529
60,162,162,324,0.08842921257019043,53.3207535877018
61,166,166,332,0.09010791778564453,53.25856436054846
62,170,170,340,0.09172201156616211,53.21180002390997
63,174,174,348,0.09336090087890625,53.17560667429029
64,176,176,352,0.09455108642578125,52.7891853756953
65,180,180,360,0.09660601615905762,52.77928969535628
66,182,182,364,0.09778308868408203,52.141518450020385
67,186,186,372,0.09964799880981445,52.1379852390578
68,188,188,376,0.10070419311523438,51.74794340898188
69,192,192,384,0.10232400894165039,51.745726125558804
70,194,194,388,0.10334300994873047,51.15281829385094
71,198,198,396,0.1049339771270752,51.139004666116534
72,200,200,400,0.10595011711120605,50.32606022315281
73,204,204,408,0.10756421089172363,50.33210907284115
74,206,206,412,0.1086130142211914,49.111912121295745
75,210,210,420,0.11024308204650879,49.106148589788745
76,212,212,424,0.11138415336608887,47.88341765867813
77,216,216,432,0.11345696449279785,47.873716808252766
78,220,220,440,0.11541199684143066,47.70529594795198
79,224,224,448,0.11733007431030273,47.56986665540762
80,228,228,456,0.11951112747192383,47.28607925363235
81,232,232,464,0.12119197845458984,47.21691307390756
82,240,240,480,0.12413406372070312,47.21483184032263
83,242,242,484,0.12527227401733398,45.974385723906835
84,246,246,492,0.12691116333007812,45.98467424968453
85,248,248,496,0.12813305854797363,44.98403881979198
86,252,252,504,0.1300640106201172,44.84044553590729
87,254,254,508,0.13176512718200684,43.57311045395045
88,256,256,512,0.1331479549407959,43.32134127210816
89,258,258,516,0.13443899154663086,42.342862578362656
90,262,262,524,0.1362619400024414,42.33275773240484
91,264,264,528,0.13752007484436035,42.11980298516801
92,268,268,536,0.13942885398864746,42.05487165395766
93,272,272,544,0.1410691738128662,41.98342412577972
94,276,276,552,0.1426830291748047,41.95492980523932
95,280,280,560,0.14431285858154297,41.998682712158825
96,284,284,568,0.1460728645324707,42.03792059843636
97,288,288,576,0.14788007736206055,42.06259545623175
98,290,290,580,0.14911103248596191,40.89056747301629
99,294,294,588,0.15101122856140137,40.87964705566492
100,296,296,592,0.15222406387329102,39.316257281756634
101,300,300,600,0.15388703346252441,39.274169876181304
102,302,302,604,0.15489506721496582,35.405214141751
103,306,306,612,0.15662407875061035,35.4526896313962
104,308,308,616,0.15768718719482422,34.17626727254515
105,312,312,624,0.15938591957092285,34.08729856638297
106,314,314,628,0.16045308113098145,32.95671528036314
107,318,318,636,0.16222500801086426,32.903598214128806
108,320,320,640,0.16338419914245605,32.15058893076093
109,324,324,648,0.16543126106262207,32.12697971344028
110,326,326,652,0.16662216186523438,29.92015578753194
111,330,330,660,0.16829919815063477,30.164880333014025
112,336,336,672,0.17041897773742676,30.182399399707037
113,340,340,680,0.17208409309387207,30.278798013638152
114,342,342,684,0.17313814163208008,29.63007955622834
115,346,346,692,0.17479991912841797,29.612355075034657
116,350,350,700,0.17661190032958984,29.630230023401282
117,352,352,704,0.17769908905029297,27.97622078695099
118,356,356,712,0.17951393127441406,28.03753285133712
119,358,358,716,0.18062400817871094,25.34843114369278
120,362,362,724,0.18231892585754395,25.453168551075578
121,366,366,732,0.18402314186096191,25.61177984731262
122,370,370,740,0.18565893173217773,25.78289374467704
123,372,372,744,0.18681716918945312,24.741572168414905
124,376,376,752,0.18849587440490723,24.835083425723724
125,378,378,756,0.1895618438720703,23.201882124629265
126,384,384,768,0.1917891502380371,23.195321246401818
127,390,390,780,0.19399094581604004,23.190550630701864
128,394,394,788,0.19556522369384766,23.23954731937738
129,396,396,792,0.19663119316101074,21.477107215243223
130,400,400,800,0.1981830596923828,21.570661583075434
131,402,402,804,0.1991729736328125,18.75149452098526
132,404,404,808,0.20022201538085938,20.331368843071232
133,410,410,820,0.2023160457611084,20.289049794597076
134,414,414,828,0.204024076461792,20.259360509390262
135,416,416,832,0.2050950527191162,19.527335682313606
136,420,420,840,0.2068009376525879,19.31077388472636
137,422,422,844,0.2079000473022461,17.956819459640883
138,426,426,852,0.2095041275024414,17.856707193638385
139,428,428,856,0.21053194999694824,14.142350177945218
140,432,432,864,0.2122809886932373,14.31766783192188
141,434,434,868,0.21345019340515137,13.324780552837069
142,438,438,876,0.2151482105255127,13.310923761402364
143,440,440,880,0.21629118919372559,11.853973581573541
144,444,444,888,0.2181541919708252,11.851520433455335
145,446,446,892,0.2195441722869873,11.008395336379749
146,450,450,900,0.22134804725646973,11.001379314050155
147,452,452,904,0.22255492210388184,10.008559577545952
148,458,458,916,0.2251279354095459,10.005290165935207
149,460,460,920,0.2263929843902588,9.572443249941443
150,464,464,928,0.22814488410949707,9.596939655818119
151,466,466,932,0.22922801971435547,9.501403702039966
152,470,470,940,0.23094987869262695,9.529918725749667
153,474,474,948,0.2328352928161621,9.546865253024748
154,478,478,956,0.23476696014404297,9.511269318368022
155,482,482,964,0.23661303520202637,9.435407092256355
156,486,486,972,0.2385101318359375,9.372193541336173
157,490,490,980,0.24045705795288086,9.34112863310213
158,492,492,984,0.2416400909423828,9.059318130712654
159,496,496,992,0.24331307411193848,9.067817113954902
160,498,498,996,0.24442410469055176,9.309412886534005
161,502,502,1004,0.24605393409729004,9.306294905412415
162,504,504,1008,0.24713397026062012,9.112889958891401
163,508,508,1016,0.2492051124572754,9.113831830920162
164,512,512,1024,0.25108909606933594,9.145918857784068
165,516,516,1032,0.25270724296569824,9.152418629197996
166,520,520,1040,0.25433826446533203,9.126671737871675
167,524,524,1048,0.2559840679168701,9.107646881023356
168,526,526,1052,0.2570970058441162,8.887666278525217
169,530,530,1060,0.258695125579834,8.888872054371518
170,532,532,1064,0.25972700119018555,8.831460499300647
171,536,536,1072,0.2614438533782959,8.831135469752098
172,538,538,1076,0.26259422302246094,8.806414540025685
173,542,542,1084,0.26430296897888184,8.804508373655949
174,546,546,1092,0.2661151885986328,8.809391401525659
175,550,550,1100,0.26778721809387207,8.81244743946877
176,554,554,1108,0.2695350646972656,8.781167101496862
177,558,558,1116,0.27118802070617676,8.758025714379869
178,562,562,1124,0.2728562355041504,8.744175941929825
179,566,566,1132,0.2745780944824219,8.727422997158556
180,570,570,1140,0.27627015113830566,8.71349668746609
181,572,572,1144,0.2776200771331787,8.559660649393322
182,576,576,1152,0.2792551517486572,8.556050719222526
183,578,578,1156,0.2803061008453369,8.120320403448432
184,582,582,1164,0.2818901538848877,8.118140655766751
185,586,586,1172,0.2835102081298828,8.097061699317692
186,588,588,1176,0.284534215927124,7.638968283079407
187,592,592,1184,0.2861809730529785,7.63701218152994
188,594,594,1188,0.28722596168518066,7.353176989130134
189,598,598,1196,0.28884100914001465,7.325656119624114
190,600,600,1200,0.289870023727417,7.107522423550449
191,604,604,1208,0.29145002365112305,7.079946429809297
192,608,608,1216,0.29299306869506836,7.035260657666413
193,612,612,1224,0.2945291996002197,6.951647145329503
194,614,614,1228,0.2955000400543213,6.525980611676346
195,618,618,1236,0.2970290184020996,6.523306809489782
196,620,620,1240,0.2981741428375244,6.498802229173634
197,624,624,1248,0.2998340129852295,6.469163069517094
198,628,628,1256,0.3015110492706299,6.40372465905466
199,630,630,1260,0.3026089668273926,6.186357278876812
200,634,634,1268,0.3043348789215088,6.184725097541332
201,638,638,1276,0.306016206741333,6.185192167299647
202,642,642,1284,0.3077688217163086,6.187958140872411
203,644,644,1288,0.30895304679870605,6.1556371626192
204,648,648,1296,0.3106980323791504,6.154659520064456
205,652,652,1304,0.3122990131378174,6.122803056083626
206,656,656,1312,0.3139619827270508,6.086306495836766
207,660,660,1320,0.315748929977417,6.053306006324647
208,664,664,1328,0.31756019592285156,6.025096303950022
209,666,666,1332,0.31868410110473633,5.798054297496378
210,670,670,1340,0.3203890323638916,5.797900965092822
211,672,672,1344,0.3214550018310547,5.602075518953484
212,676,676,1352,0.3231229782104492,5.57997056848501
213,680,680,1360,0.32476186752319336,5.538105909563342
214,682,682,1364,0.32584500312805176,5.3108229842841865
215,686,686,1372,0.32756996154785156,5.306829539099567
216,688,688,1376,0.3286271095275879,4.991279274022531
217,692,692,1384,0.3301961421966553,4.990579558520039
218,694,694,1388,0.33126091957092285,4.717796943624194
219,698,698,1396,0.3329010009765625,4.713725845544218
220,700,700,1400,0.33397889137268066,4.322210476406326
221,704,704,1408,0.33563804626464844,4.319442490166352
222,706,706,1412,0.3367161750793457,3.9093038090592245
223,710,710,1420,0.3384690284729004,3.9085605554630547
224,712,712,1424,0.3396000862121582,3.3354202805128352
225,716,716,1432,0.341292142868042,3.331588269776944
226,718,718,1436,0.3423490524291992,3.278931829186945
227,722,722,1444,0.3440840244293213,3.28295372409184
228,724,724,1448,0.3451499938964844,3.2680930311757947
229,728,728,1456,0.34676218032836914,3.2653658951552416
230,730,730,1460,0.34785914421081543,3.1596591317619414
231,734,734,1468,0.34949421882629395,3.1459867146380702
232,736,736,1472,0.35057711601257324,2.4502152909810775
233,740,740,1480,0.352154016494751,2.4552495830514545
234,746,746,1492,0.35443687438964844,2.456700108505629
235,748,748,1496,0.3555269241333008,2.019811086411096
236,752,752,1504,0.35715699195861816,2.0057954623284786
237,756,756,1512,0.35881924629211426,2.009358050776882
238,760,760,1520,0.3604700565338135,2.036791336063061
239,762,762,1524,0.36158013343811035,1.8439571018624292
240,766,766,1532,0.3632171154022217,1.8630425920786138
241,768,768,1536,0.36428308486938477,1.827822798031434
242,772,772,1544,0.366199254989624,1.8250014728048427
243,774,774,1548,0.36765027046203613,1.6477378561447722
244,778,778,1556,0.36964893341064453,1.6118088731888065
245,782,782,1564,0.3714790344238281,1.5812240359842917
246,784,784,1568,0.3726348876953125,1.290214586696834
247,788,788,1576,0.3745460510253906,1.2914685086590225
248,790,790,1580,0.37578415870666504,1.0163974565576837
249,794,794,1588,0.3776381015777588,1.017424727608386
250,796,796,1592,0.3787689208984375,0.7479697458059036
251,800,800,1600,0.3807680606842041,0.7096804343055965
252,804,804,1608,0.38249921798706055,0.6929855648535295
253,806,806,1612,0.38369011878967285,0.5517213756771753
254,810,810,1620,0.38541507720947266,0.5575003055440675
255,812,812,1624,0.38651204109191895,0.5673350545134781
256,816,816,1632,0.38815999031066895,0.5829821477813084
257,820,820,1640,0.38983726501464844,0.5492117036698119
258,822,822,1644,0.3909640312194824,0.5674136864449792
259,824,824,1648,0.3920910358428955,0.6022248134764823
260,828,828,1656,0.3937849998474121,0.6022857185520252
261,830,830,1660,0.39485597610473633,0.6029297948713292
262,834,834,1668,0.39661192893981934,0.6042666790599469
263,836,836,1672,0.3977930545806885,0.6037096523263017
264,840,840,1680,0.3994791507720947,0.6014428256117981
265,842,842,1684,0.4004960060119629,0.4955061188460377
266,846,846,1692,0.4021289348602295,0.49578811805201894
267,848,848,1696,0.4031980037689209,0.44338681278406966
268,852,852,1704,0.4050140380859375,0.4428736433408176
269,854,854,1708,0.40606021881103516,0.4044965840674877
270,858,858,1716,0.40769314765930176,0.40525008389533923
271,860,860,1720,0.40874814987182617,0.3835060524143046
272,864,864,1728,0.4104001522064209,0.3832871030462002
273,866,866,1732,0.4114861488342285,0.3740392699842232
274,870,870,1740,0.41320204734802246,0.37565488012990045
275,872,872,1744,0.41434407234191895,0.37932126942143896
276,874,874,1748,0.4154829978942871,0.37356102010255654
277,878,878,1756,0.41716504096984863,0.3732297696498108
278,880,880,1760,0.41829609870910645,0.33418124959405304
279,884,884,1768,0.42021703720092773,0.3327602733977528
280,886,886,1772,0.421550989151001,0.2798861456830082
281,890,890,1780,0.4233999252319336,0.2795847396685076
282,892,892,1784,0.42461705207824707,0.23199679874130652
283,896,896,1792,0.4265151023864746,0.23207750620747447
284,898,898,1796,0.42762207984924316,0.212408526532613
285,900,900,1800,0.4286980628967285,0.19286934914362064
286,902,902,1804,0.4297139644622803,0.17449745533690475
287,906,906,1812,0.4313790798187256,0.17456751069198617
288,908,908,1816,0.43244409561157227,0.16215965463322846
289,912,912,1824,0.434124231338501,0.1613955835964589
290,914,914,1828,0.43523216247558594,0.1493501761636935
291,918,918,1836,0.43691515922546387,0.1493805642537609
292,920,920,1840,0.43801212310791016,0.11171676347350967
293,924,924,1848,0.4397621154785156,0.1115529805516644
294,926,926,1852,0.4408590793609619,0.08162637693294528
295,928,928,1856,0.4418818950653076,0.0828565976568143
296,930,930,1860,0.44298291206359863,0.07206259370286716
297,934,934,1868,0.4447000026702881,0.07234785134426147
298,936,936,1872,0.44577693939208984,0.06168422863106571
299,940,940,1880,0.44738101959228516,0.06189443671325989
300,942,942,1884,0.4484832286834717,0.046178134508977564
301,946,946,1892,0.45012593269348145,0.04596172622905215
302,948,948,1896,0.4511990547180176,0.029541864734937917
303,952,952,1904,0.45286011695861816,0.029724443279405932
304,954,954,1908,0.4538919925689697,0.022532327907015315
305,958,958,1916,0.4556281566619873,0.022917943325410306
306,960,960,1920,0.4567420482635498,0.01926410588453109
307,964,964,1928,0.4583902359008789,0.01922022466942508
308,966,966,1932,0.4593989849090576,0.02156623313055661
309,970,970,1940,0.46103811264038086,0.02171415449288361
310,972,972,1944,0.4621269702911377,0.021410740155829444
311,976,976,1952,0.4639921188354492,0.021355873551556215
312,978,978,1956,0.46503710746765137,0.01983446218412155
313,982,982,1964,0.4667999744415283,0.019561435280706974
314,984,984,1968,0.46788525581359863,0.019240220238316397
315,988,988,1976,0.4695320129394531,0.019248891018833092
316,990,990,1980,0.4706110954284668,0.01825672119673527
317,994,994,1988,0.472182035446167,0.018251538474714835
318,996,996,1992,0.4732060432434082,0.01700770229376758
319,1000,1000,2000,0.47484707832336426,0.017006194679538567
320,1002,1002,2004,0.47594714164733887,0.01603262340756828
321,1006,1006,2012,0.47768306732177734,0.016032147362807336
322,1008,1008,2016,0.47876524925231934,0.01609032041108094
323,1012,1012,2024,0.48046302795410156,0.016117452411776867
324,1016,1016,2032,0.48215198516845703,0.016087364900272405
325,1018,1018,2036,0.48318004608154297,0.014296818934099065
326,1022,1022,2044,0.48485684394836426,0.014248860139446151
327,1024,1024,2048,0.48597097396850586,0.011040098057833347
328,1028,1028,2056,0.4875972270965576,0.01100542209167088
329,1030,1030,2060,0.48862218856811523,0.010542782407355844
330,1034,1034,2068,0.4902510643005371,0.010517195022430315
331,1036,1036,2072,0.4913311004638672,0.009299755029132939
332,1040,1040,2080,0.49298691749572754,0.009304263468493446
333,1042,1042,2084,0.493988037109375,0.009127783435928905
334,1046,1046,2092,0.4957289695739746,0.009081414456659331
335,1048,1048,2096,0.49688100814819336,0.00798224164691419
336,1052,1052,2104,0.4985480308532715,0.007938130389902653
337,1054,1054,2108,0.49959707260131836,0.0069563307821454146
338,1058,1058,2116,0.5011940002441406,0.006970629959710095
339,1060,1060,2120,0.5023181438446045,0.005672720931443109
340,1064,1064,2128,0.503960132598877,0.005666005518264683
341,1066,1066,2132,0.5051670074462891,0.004778024959932736
342,1070,1070,2140,0.5068199634552002,0.004720877503245902
343,1072,1072,2144,0.5080950260162354,0.003940335587685695
344,1076,1076,2152,0.5101230144500732,0.003920145292909183
345,1078,1078,2156,0.5113842487335205,0.003252791416571199
346,1082,1082,2164,0.5131778717041016,0.0032066053751123036
347,1084,1084,2168,0.5142779350280762,0.002060805143514699
348,1086,1086,2172,0.5153930187225342,0.0020762528387194834
349,1090,1090,2180,0.5170350074768066,0.002074150917565021
350,1092,1092,2184,0.5180270671844482,0.0016353320189637088
351,1096,1096,2192,0.5196502208709717,0.0016411882188549498
352,1098,1098,2196,0.5207481384277344,0.00140246701482738
353,1102,1102,2204,0.5225000381469727,0.0014011639553928035
354,1104,1104,2208,0.5235171318054199,0.0012840434646932408
355,1108,1108,2216,0.5252339839935303,0.0012698938805897342
356,1110,1110,2220,0.5263490676879883,0.0009335636337937103
357,1114,1114,2228,0.5281879901885986,0.000926087654534058
358,1116,1116,2232,0.5295040607452393,0.0004949704189129989
359,1120,1120,2240,0.5314939022064209,0.000491747709588708
360,1122,1122,2244,0.5329632759094238,0.00031222802385855175
361,1124,1124,2248,0.534217119216919,0.00029867265118355135
362,1126,1126,2252,0.5354142189025879,0.0002910417830435108
363,1128,1128,2256,0.5369000434875488,0.00031855913027811766
364,1130,1130,2260,0.5382061004638672,0.0003182371951879759
365,1134,1134,2268,0.5401911735534668,0.00031528889780929603
366,1136,1136,2272,0.5418350696563721,0.0002161586321562936
367,1140,1140,2280,0.5437378883361816,0.00021501508001620095
368,1142,1142,2284,0.5450069904327393,0.0001950005012076872
369,1146,1146,2292,0.5469472408294678,0.0001972571157011771
370,1148,1148,2296,0.5480620861053467,0.000199267083075938
371,1150,1150,2300,0.5490992069244385,0.00018486439364551188
372,1154,1154,2308,0.5509111881256104,0.0001845257603463324
373,1156,1156,2312,0.5522620677947998,0.00013986493524953403
374,1160,1160,2320,0.5544211864471436,0.0001391813964346511
375,1162,1162,2324,0.5560588836669922,0.0001190870791560883
376,1166,1166,2332,0.5577659606933594,0.00011815179539098608
377,1168,1168,2336,0.5588181018829346,0.00011121725003704341
378,1172,1172,2344,0.5604500770568848,0.00011156364223552373
379,1174,1174,2348,0.5617170333862305,0.00012034744838729239
380,1176,1176,2352,0.5630228519439697,0.00010178264938076609
381,1180,1180,2360,0.564716100692749,0.00010160878730403056
382,1182,1182,2364,0.5658929347991943,9.410487052718963e-05
383,1186,1186,2372,0.5676529407501221,9.411341716258903e-05
384,1188,1188,2376,0.5689601898193359,9.531269802209863e-05
385,1192,1192,2384,0.570742130279541,9.569605526849045e-05
386,1194,1194,2388,0.5719940662384033,0.00010350215222842962
387,1198,1198,2396,0.574038028717041,0.00010379710988672741
388,1200,1200,2400,0.5753281116485596,0.00011244544703004067
389,1204,1204,2408,0.5769801139831543,0.00011235226213557326
390,1206,1206,2412,0.5780930519104004,0.00010487260578884161
391,1210,1210,2420,0.5799980163574219,0.00010473333077243296
392,1214,1214,2428,0.5819389820098877,0.00010448377804550546
393,1216,1216,2432,0.5832860469818115,9.642943803100934e-05
394,1220,1220,2440,0.5850310325622559,9.66584063917253e-05
395,1222,1222,2444,0.5861730575561523,0.00010222293019523931
396,1226,1226,2452,0.5880279541015625,0.00010229895690372359
397,1228,1228,2456,0.5893731117248535,9.712099961234344e-05
398,1232,1232,2464,0.5913209915161133,9.709247365208284e-05
399,1234,1234,2468,0.5924282073974609,9.497492396803864e-05
400,1238,1238,2476,0.594202995300293,9.486244243817055e-05
401,1240,1240,2480,0.5955290794372559,9.316556213434524e-05
402,1244,1244,2488,0.5974302291870117,9.266903987281694e-05
403,1248,1248,2496,0.5991501808166504,9.192468712626578e-05
404,1250,1250,2500,0.6002869606018066,9.049078994394222e-05
405,1254,1254,2508,0.6019301414489746,9.051392487435805e-05
406,1256,1256,2512,0.6029400825500488,8.872369699020055e-05
407,1260,1260,2520,0.6046061515808105,8.868292786701204e-05
408,1262,1262,2524,0.6058609485626221,8.379445591799595e-05
409,1266,1266,2532,0.6078019142150879,8.372608749596111e-05
410,1268,1268,2536,0.6089141368865967,7.62700962013696e-05
411,1272,1272,2544,0.6106178760528564,7.620928124651982e-05
412,1274,1274,2548,0.6120378971099854,7.241388300371909e-05
413,1278,1278,2556,0.6138520240783691,7.240144964271167e-05
414,1280,1280,2560,0.6149570941925049,7.100073287347186e-05
415,1284,1284,2568,0.6166191101074219,7.137628438158572e-05
416,1288,1288,2576,0.6182689666748047,7.163369082263671e-05
417,1290,1290,2580,0.6193511486053467,7.038043213469791e-05
418,1294,1294,2588,0.6210000514984131,7.021803298812301e-05
419,1296,1296,2592,0.6220402717590332,7.00948013445668e-05
420,1300,1300,2600,0.623967170715332,7.00070338552905e-05
421,1302,1302,2604,0.625208854675293,6.884790320782486e-05
422,1306,1306,2612,0.6268520355224609,6.88379196844835e-05
423,1308,1308,2616,0.6279261112213135,6.5211362766604e-05
424,1312,1312,2624,0.6298189163208008,6.52715557407646e-05
425,1316,1316,2632,0.6315310001373291,6.547877808316116e-05
426,1318,1318,2636,0.6326169967651367,6.465522938015056e-05
427,1322,1322,2644,0.6342780590057373,6.46174287339818e-05
428,1324,1324,2648,0.6353280544281006,6.121993772012502e-05
429,1328,1328,2656,0.6369650363922119,6.111951825005235e-05
430,1330,1330,2660,0.6380281448364258,5.8583519262356276e-05
431,1334,1334,2668,0.6399250030517578,5.861908255155868e-05
432,1336,1336,2672,0.6413111686706543,5.739698303841578e-05
433,1340,1340,2680,0.643090009689331,5.7299880950267834e-05
434,1344,1344,2688,0.645205020904541,5.7125263765556156e-05
435,1346,1346,2692,0.6463680267333984,5.182343738852069e-05
436,1350,1350,2700,0.6482410430908203,5.1692963779714773e-05
437,1354,1354,2708,0.6501390933990479,5.1158379278604116e-05
438,1356,1356,2712,0.6514651775360107,4.739037046874728e-05
439,1360,1360,2720,0.6532449722290039,4.7183627202684875e-05
440,1364,1364,2728,0.6551141738891602,4.692515426540922e-05
441,1366,1366,2732,0.6564948558807373,4.4366618340063724e-05
442,1370,1370,2740,0.6582961082458496,4.4450283326114004e-05
443,1374,1374,2748,0.6599140167236328,4.4482193516159896e-05
444,1378,1378,2756,0.6618850231170654,4.4373274249664973e-05
445,1380,1380,2760,0.6631810665130615,4.067750273861748e-05
446,1384,1384,2768,0.6649959087371826,4.064291078975657e-05
447,1386,1386,2772,0.6662640571594238,3.774675224121893e-05
448,1388,1388,2776,0.6674580574035645,3.451606323778833e-05
449,1392,1392,2784,0.6693031787872314,3.4462799817447376e-05
450,1394,1394,2788,0.6706631183624268,2.8432274007172964e-05
451,1398,1398,2796,0.6724529266357422,2.838170598806755e-05
452,1400,1400,2800,0.6737251281738281,2.7917560487367155e-05
453,1404,1404,2808,0.67557692527771,2.799368962769222e-05
454,1406,1406,2812,0.6767439842224121,2.7524226993591583e-05
455,1410,1410,2820,0.6786360740661621,2.7576465640777315e-05
456,1414,1414,2828,0.6804540157318115,2.7570889642447582e-05
457,1416,1416,2832,0.6815590858459473,2.137369745014439e-05
458,1420,1420,2840,0.6833171844482422,2.1337815496735857e-05
459,1422,1422,2844,0.6843559741973877,1.9828219365081168e-05
460,1426,1426,2852,0.6860392093658447,1.9811542529168946e-05
461,1428,1428,2856,0.6871230602264404,2.0101483414691756e-05
462,1432,1432,2864,0.6890289783477783,2.0151911940047285e-05
463,1434,1434,2868,0.6902720928192139,1.994448155073769e-05
464,1438,1438,2876,0.6919710636138916,1.9983800029876875e-05
465,1440,1440,2880,0.6930551528930664,2.100303765928402e-05
466,1444,1444,2888,0.6950259208679199,2.0954252022420405e-05
467,1446,1446,2892,0.6963710784912109,1.8538703102422005e-05
468,1448,1448,2896,0.6974532604217529,1.4263347679843719e-05
469,1452,1452,2904,0.6992552280426025,1.4224318533706537e-05
470,1454,1454,2908,0.7003872394561768,8.322856956510805e-06
471,1458,1458,2916,0.7020831108093262,8.240959800787095e-06
472,1460,1460,2920,0.7031009197235107,4.159401441938826e-06
473,1462,1462,2924,0.7042140960693359,3.996809368800314e-06
474,1466,1466,2932,0.7061760425567627,3.9991510902837035e-06
475,1468,1468,2936,0.7074599266052246,2.073418500003754e-06
476,1472,1472,2944,0.7091710567474365,2.03850606794731e-06
477,1474,1474,2948,0.710219144821167,6.880076171000837e-07
478,1478,1478,2956,0.7122058868408203,6.513462267321302e-07
479,1480,1480,2960,0.7135241031646729,3.070175580432988e-07
480,1482,1482,2964,0.7145822048187256,9.288919500249904e-08
481,1486,1486,2972,0.7162730693817139,8.245660865213722e-08
482,1488,1488,2976,0.7173662185668945,2.145142161680269e-09


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.005098819732666016,7527.1682254052175
1001,2004,1002,3006,3.6467480659484863,16.497806269995635
2002,4006,2003,6009,7.238240957260132,8.493645480455598
3003,6008,3004,9012,10.868703842163086,5.458411064455504
4004,8010,4005,12015,14.944911003112793,4.0183071345327335
5005,10012,5006,15018,18.747506141662598,3.22679212312687
6006,12014,6007,18021,23.342329025268555,2.7412246159965434
7007,14016,7008,21024,28.049583911895752,2.4010585392661596
8008,16018,8009,24027,32.46620798110962,2.1473435429415986
9009,18020,9010,27030,36.59423875808716,1.9510757904063212
10010,20022,10011,30033,40.99786901473999,1.7860873272093158
11011,22024,11012,33036,44.91871500015259,1.6496502359241276
12012,24026,12013,36039,48.269286155700684,1.5356632292659924
13013,26028,13014,39042,53.206477880477905,1.4379722296016553
14014,28030,14015,42045,58.65890097618103,1.3520213924985
15015,30032,15016,45048,63.3932728767395,1.2742289145662653
16016,32034,16017,48051,66.61575698852539,1.207127379722806
17017,34036,17018,51054,70.00086998939514,1.146283669553668
18018,36038,18019,54057,74.22565603256226,1.0918120883015945
19019,38040,19020,57060,78.23007702827454,1.0424478336863103
20020,40042,20021,60063,81.88735604286194,0.9969560017580079
21021,42044,21022,63066,85.60669207572937,0.9558615275109332
22022,44046,22023,66069,89.36515092849731,0.9176484019026248
23023,46048,23024,69072,92.91565299034119,0.8819220992099872
24024,48050,24025,72075,96.25085091590881,0.8492827874051727
25025,50052,25026,75078,99.81518411636353,0.8197084285638994
26026,52054,26027,78081,103.37525296211243,0.7915118778582837
27027,54056,27028,81084,106.68792700767517,0.7649407176704699
28028,56058,28029,84087,109.89806199073792,0.7406526523391221
29029,58060,29030,87090,113.24599385261536,0.717516735978279
30030,60062,30031,90093,116.53232097625732,0.6960358251853904
31031,62064,31032,93096,119.81329298019409,0.6761034219180146
32032,64066,32033,96099,123.53746390342712,0.6566625917566853
33033,66068,33034,99102,127.02709794044495,0.6385920771299425
34034,68070,34035,102105,130.5686318874359,0.6213090652981919
35035,70072,35036,105108,133.9097719192505,0.6054368420846004
36036,72074,36037,108111,137.51473593711853,0.5899539575129893
37037,74076,37038,111114,140.93576383590698,0.575850874904063
38038,76078,38039,114117,144.5266411304474,0.5620418065409467
39039,78080,39040,117120,148.02537393569946,0.5489631221644231
40040,80082,40041,120123,151.34961700439453,0.5365798114016798
41041,82084,41042,123126,154.6927888393402,0.5247631347301649
42042,84086,42043,126129,158.01648998260498,0.5134134385461948
43043,86088,43044,129132,161.33764791488647,0.5022046245594538
44044,88090,44045,132135,164.70172691345215,0.4917957345551258
45045,90092,45046,135138,168.0752658843994,0.48152754926195485
46046,92094,46047,138141,173.13305377960205,0.47210523306603136
47047,94096,47048,141144,177.7668809890747,0.4630634162167553
48048,96098,48049,144147,182.45351481437683,0.45412089460296556
49049,98100,49050,147150,186.21646690368652,0.44561378928301565
50050,100102,50051,150153,189.73361086845398,0.43731890040362487
51051,102104,51052,153156,193.15243697166443,0.42939628356361936
52052,104106,52053,156159,196.5193920135498,0.421768821477599
53053,106108,53054,159162,199.83905696868896,0.41448086035052256
54054,108110,54055,162165,203.1999819278717,0.407511265570065
55055,110112,55056,165168,206.60861778259277,0.4005870653199963
56056,112114,56057,168171,209.92689394950867,0.393895394881838
57057,114116,57058,171174,213.25325894355774,0.38750695320595696
58058,116118,58059,174177,216.53420686721802,0.3814584564534016
59059,118120,59060,177180,219.7956600189209,0.3754735273141705
60060,120122,60061,180183,223.07716703414917,0.36974671455391217
61061,122124,61062,183186,226.45909190177917,0.36410737318692554
62062,124126,62063,186189,229.7380998134613,0.3586352511738369
63063,126128,63064,189192,233.04684901237488,0.3533858682058053
64064,128130,64065,192195,236.37164998054504,0.3483475837238075
65065,130132,65066,195198,239.5901539325714,0.34344225045606436
66066,132134,66067,198201,242.8056890964508,0.33863474435929675
67067,134136,67068,201204,246.01495790481567,0.3339623388565087
68068,136138,68069,204207,249.1772849559784,0.32942746442495263
69069,138140,69070,207210,252.3767011165619,0.32502469818791724
70070,140142,70071,210213,255.62268090248108,0.3207800291311287
71071,142144,71072,213216,258.807904958725,0.316658925908996
72072,144146,72073,216219,262.03289580345154,0.3124673175279895
73073,146148,73074,219222,265.2709319591522,0.30851173182782077
74074,148150,74075,222225,268.52366304397583,0.30464353173738346
75075,150152,75076,225228,271.7283990383148,0.3008890543515008
76076,152154,76077,228231,274.9656958580017,0.2972730325109296
77077,154156,77078,231234,278.1803369522095,0.29374264490434143
78078,156158,78079,234237,281.3559069633484,0.29019346320274053
79079,158160,79080,237240,284.6501941680908,0.28683214347802277
80080,160162,80081,240243,287.94939494132996,0.2835663693567767
81081,162164,81082,243246,291.13415002822876,0.28031315655607614
82082,164166,82083,246249,294.4020938873291,0.27707980180275626
83083,166168,83084,249252,297.5976128578186,0.27401483678659133
84084,168170,84085,252255,300.8032109737396,0.2710367277104524
85085,170172,85086,255258,303.970458984375,0.2680502941548184
86086,172174,86087,258261,307.20662808418274,0.2651336481958424
87087,174176,87088,261264,310.3590729236603,0.2623141853382549
88088,176178,88089,264267,313.5144839286804,0.2595501636806148
89089,178180,89090,267270,316.732253074646,0.2567464036401361
90090,180182,90091,270273,319.8972489833832,0.25406428346104803
91091,182184,91092,273276,323.1377079486847,0.2515219147080643
92092,184186,92093,276279,326.31721782684326,0.24902016379746783
93093,186188,93094,279282,329.65363097190857,0.24649716358726437
94094,188190,94095,282285,332.83149695396423,0.2439996516022802
95095,190192,95096,285288,336.0214488506317,0.24160324150398083
96096,192194,96097,288291,339.24643182754517,0.2392263167312194
97097,194196,97098,291294,342.4238488674164,0.23690407795038482
98098,196198,98099,294297,345.6061179637909,0.23467143730340467
99099,198200,99100,297300,348.8476028442383,0.23250848719362693
100100,200202,100101,300303,352.0409257411957,0.23028648278705077
101101,202204,101102,303306,355.26041316986084,0.228118407081638
102102,204206,102103,306309,358.4614100456238,0.2260358890016505
103103,206208,103104,309312,361.63514375686646,0.22399632231827127
104104,208210,104105,312315,364.84763407707214,0.2220149036620569
105105,210212,105106,315318,368.0416350364685,0.2200313745524909
106106,212214,106107,318321,371.2205328941345,0.21806712200850598
107107,214216,107108,321324,374.39325618743896,0.21616051192722807
108108,216218,108109,324327,377.6301329135895,0.21432161974189512
109109,218220,109110,327330,380.8391079902649,0.2125081885878899
110110,220222,110111,330333,384.05106806755066,0.2106970793720393
111111,222224,111112,333336,387.2442989349365,0.20893583075303468
112112,224226,112113,336339,390.4198808670044,0.20717976369996904
113113,226228,113114,339342,393.59871888160706,0.20549386142738513
114114,228230,114115,342345,396.78173089027405,0.2037603152293741
115115,230232,115116,345348,399.9455761909485,0.20212424049896072
116116,232234,116117,348351,403.13218092918396,0.20051385473016126
117117,234236,117118,351354,406.2981858253479,0.19894357516204764
118118,236238,118119,354357,409.52019596099854,0.19739563831899432
119119,238240,119120,357360,412.72762989997864,0.1958393422428344
120120,240242,120121,360363,415.89733600616455,0.1943071466866968
121121,242244,121122,363366,419.08821392059326,0.19279230246502266
122122,244246,122123,366369,422.25520610809326,0.19132446379262547
123123,246248,123124,369372,425.449257850647,0.1898995523715712
124124,248250,124125,372375,428.66551208496094,0.188462773552601
125125,250252,125126,375378,432.10064816474915,0.18705085916735698
126126,252254,126127,378381,435.4713649749756,0.18567268950937432
127127,254256,127128,381384,438.6673460006714,0.18433589931919414
128128,256258,128129,384387,441.8621621131897,0.18301034322576015
129129,258260,129130,387390,445.09716296195984,0.18167717431424535
130130,260262,130131,390393,448.28959703445435,0.18036237830892787
131131,262264,131132,393396,451.45953607559204,0.17907697554619517
132132,264266,132133,396399,454.70990204811096,0.1778225380294316
133133,266268,133134,399402,457.87704491615295,0.17658395933904103
134134,268270,134135,402405,461.1218979358673,0.17533394904421584
135135,270272,135136,405408,464.3357059955597,0.17413790986938693
136136,272274,136137,408411,467.4982359409332,0.17296563084528316
137137,274276,137138,411414,470.6668930053711,0.1718038296457962
138138,276278,138139,414417,473.841117143631,0.1706309357268765
139139,278280,139140,417420,477.0297088623047,0.1694840832387854
140140,280282,140141,420423,480.2375011444092,0.1683483669967245
141141,282284,141142,423426,483.41571283340454,0.1672327166688774
142142,284286,142143,426429,486.5437159538269,0.16613368243270088
143143,286288,143144,429432,489.69209384918213,0.16504226253346133
144144,288290,144145,432435,492.86531591415405,0.16398136337556934
145145,290292,145146,435438,496.05629992485046,0.16290896101418184
146146,292294,146147,438441,499.18534803390503,0.1618791703003808
147147,294296,147148,441444,502.3563549518585,0.1608572646655375
148148,296298,148149,444447,505.52002811431885,0.1598246188932535
149149,298300,149150,447450,508.7181248664856,0.1588046500182827
150150,300302,150151,450453,511.9009430408478,0.15781925526425766
151151,302304,151152,453456,515.1044819355011,0.15684078941740154
152152,304306,152153,456459,518.29065990448,0.15585675163492851
153153,306308,153154,459462,521.5037169456482,0.15492164332681568
154154,308310,154155,462465,524.6643087863922,0.15399009380962525
155155,310312,155156,465468,527.8446090221405,0.1530835003213724
156156,312314,156157,468471,531.0353388786316,0.1521651426119206
157157,314316,157158,471474,534.2558360099792,0.15124965226459608
158158,316318,158159,474477,537.4476919174194,0.15034279609426449
159159,318320,159160,477480,540.630481004715,0.14945472571707796
160160,320322,160161,480483,543.8682630062103,0.14857372365440824
161161,322324,161162,483486,547.2040810585022,0.14770831501300563
162162,324326,162163,486489,550.6126449108124,0.14685379122238373
163163,326328,163164,489492,554.0195429325104,0.1460215353017702
164164,328330,164165,492495,557.4643218517303,0.14519077583099715
165165,330332,165166,495498,560.8990938663483,0.14436370925795927
166166,332334,166167,498501,564.3367741107941,0.1435555053049029
167167,334336,167168,501504,567.77610206604,0.1427298386588518
168168,336338,168169,504507,571.1640181541443,0.14196044045274903
169169,338340,169170,507510,574.4781329631805,0.1411670707675512
170170,340342,170171,510513,577.6874988079071,0.14038354423792043
171171,342344,171172,513516,580.7995729446411,0.13961192019451119
172172,344346,172173,516519,583.9452850818634,0.13885429314905195
173173,346348,173174,519522,587.06369805336,0.13811171433189884
174174,348350,174175,522525,590.2492949962616,0.13735427009305567
175175,350352,175176,525528,593.428386926651,0.13662850934088056
176176,352354,176177,528531,596.5940027236938,0.13591056288714753
177177,354356,177178,531534,599.7376408576965,0.1351865487813484
178178,356358,178179,534537,602.8921618461609,0.13447545955204987
179179,358360,179180,537540,606.035441160202,0.1337655631123198
180180,360362,180181,540543,609.2303321361542,0.13307280397384602
181181,362364,181182,543546,612.4699728488922,0.13238329144041927
182182,364366,182183,546549,615.6785697937012,0.13170566990811494
183183,366368,183184,549552,618.8857898712158,0.1310416895776143
184184,368370,184185,552555,622.0636730194092,0.13036930579801265
185185,370372,185186,555558,625.2788639068604,0.12971068968545296
186186,372374,186187,558561,628.4346311092377,0.12905034065079235
187187,374376,187188,561564,631.6070199012756,0.12841976679374056
188188,376378,188189,564567,634.7437138557434,0.12779184837381763
189189,378380,189190,567570,637.8933091163635,0.1271694866427424
190190,380382,190191,570573,641.0608038902283,0.12654655516234925
191191,382384,191192,573576,644.237566947937,0.1259342502344225
192192,384386,192193,576579,647.38201379776,0.12532487717726326
193193,386388,193194,579582,650.531140089035,0.12470222717638535
194194,388390,194195,582585,653.9036450386047,0.12410089484183118
195195,390392,195196,585588,657.0541400909424,0.12350029504887061
196196,392394,196197,588591,660.1912980079651,0.12291293228372524
197197,394396,197198,591594,663.3209798336029,0.12231943448387028
198198,396398,198199,594597,666.4549510478973,0.12175190807647596
199199,398400,199200,597600,669.5998129844666,0.12118687697147834
200200,400402,200201,600603,672.7565670013428,0.12061233546410222
201201,402404,201202,603606,675.9349510669708,0.12004874657577602
202202,404406,202203,606609,679.0705268383026,0.11948765349734458
203203,406408,203204,609612,682.2094571590424,0.11894012164884771
204204,408410,204205,612615,685.3995339870453,0.1183956219592801
205205,410412,205206,615618,688.5217139720917,0.11785534625960281
206206,412414,206207,618621,691.6576619148254,0.11731828563097224
207207,414416,207208,621624,694.7807238101959,0.11678281152489944
208208,416418,208209,624627,697.9185147285461,0.11626146294292994
209209,418420,209210,627630,701.0755279064178,0.11574160594864225
210210,420422,210211,630633,704.2321040630341,0.11523256568943907
211211,422424,211212,633636,707.3968820571899,0.11472187432264036
212212,424426,212213,636639,710.5501358509064,0.11422107158250583
213213,426428,213214,639642,713.7352747917175,0.11371435881119396
214214,428430,214215,642645,716.9237909317017,0.11321671213590889
215215,430432,215216,645648,720.0480799674988,0.11272944273150642
216216,432434,216217,648651,723.1866850852966,0.11224269904414541
217217,434436,217218,651654,726.3152668476105,0.11175924310009577
218218,436438,218219,654657,729.4552800655365,0.1112829644298472
219219,438440,219220,657660,732.5716519355774,0.11081129226113262
220220,440442,220221,660663,735.7539701461792,0.11033430244788178
221221,442444,221222,663666,738.9620459079742,0.10985945648280904
222222,444446,222223,666669,742.1441488265991,0.10939786878043378
223223,446448,223224,669672,745.2741270065308,0.1089359788584261
224224,448450,224225,672675,748.4127910137177,0.10848241558960581
225225,450452,225226,675678,751.5352728366852,0.10803518534703471
226226,452454,226227,678681,754.6787188053131,0.10758411192000494
227227,454456,227228,681684,757.8724939823151,0.10714659151926753
228228,456458,228229,684687,761.0392611026764,0.10669520751616801
229229,458460,229230,687690,764.1762900352478,0.10626105517258111
230230,460462,230231,690693,767.3196640014648,0.10583009994843451
231231,462464,231232,693696,770.4563999176025,0.10540205221695942
232232,464466,232233,696699,773.6540987491608,0.10497622477305413
233233,466468,233234,699702,776.793182849884,0.10454209768977307
234234,468470,234235,702705,779.8808088302612,0.10412440362051711
235235,470472,235236,705708,783.0679867267609,0.10371492617196054
236236,472474,236237,708711,786.3616271018982,0.10330418657758855
237237,474476,237238,711714,789.488972902298,0.10289304848811298
238238,476478,238239,714717,792.5707049369812,0.1024892195546272
239239,478480,239240,717720,795.6998698711395,0.10209433690215519
240240,480482,240241,720723,798.8064379692078,0.1016947977059317
241241,482484,241242,723726,801.9685130119324,0.10128805645217653
242242,484486,242243,726729,805.1658160686493,0.10089610746217659
243243,486488,243244,729732,808.296709060669,0.10050745449370879
244244,488490,244245,732735,811.4073798656464,0.10011470221616037
245245,490492,245246,735738,814.5615110397339,0.09974203425008454
246246,492494,246247,738741,817.9421601295471,0.09935096413573774
247247,494496,247248,741744,821.1507251262665,0.09896969855253701
248248,496498,248249,744747,824.2744839191437,0.09859599244009587
249249,498500,249250,747750,827.4189789295197,0.0982161902320513
250250,500502,250251,750753,830.5472359657288,0.09785341511633305
251251,502504,251252,753756,833.7593369483948,0.09748814200611378
252252,504506,252253,756759,836.9172310829163,0.09709963740533567
253253,506508,253254,759762,840.0551159381866,0.0967417145948275
254254,508510,254255,762765,843.1779289245605,0.09638311707203684
255255,510512,255256,765768,846.334212064743,0.09602736738088424
256256,512514,256257,768771,849.474179983139,0.09567076871462632
257257,514516,257258,771774,852.6718518733978,0.09532250081429083
258258,516518,258259,774777,855.8559300899506,0.09497640523477457
259259,518520,259260,777780,858.9822278022766,0.09463343617062492
260260,520522,260261,780783,862.1382477283478,0.09429415298291133
261261,522524,261262,783786,865.3556168079376,0.09395859171672782
262262,524526,262263,786789,868.5151238441467,0.09361903066383093
263263,526528,263264,789792,871.6857960224152,0.09327822893101256
264264,528530,264265,792795,874.8217258453369,0.09294339048028633
265265,530532,265266,795798,877.9517290592194,0.09261626479928964
266266,532534,266267,798801,881.0879940986633,0.0922886057451251
267267,534536,267268,801804,884.2346091270447,0.0919639932053542
268268,536538,268269,804807,887.4438738822937,0.09163259724482486
269269,538540,269270,807810,890.5758669376373,0.09131221627285413
270270,540542,270271,810813,893.7761240005493,0.09099100371713575
271271,542544,271272,813816,896.9406960010529,0.09067776039228193
272272,544546,272273,816819,900.1109931468964,0.09035981666056614
273273,546548,273274,819822,903.3106389045715,0.09004430209279235
274274,548550,274275,822825,906.4885458946228,0.08973193009478564
275275,550552,275276,825828,909.6213209629059,0.08942181523525505
276276,552554,276277,828831,912.8073999881744,0.08911729145438585
277277,554556,277278,831834,915.9503200054169,0.08881903215115017
278278,556558,278279,834837,919.1320748329163,0.08851720266466145
279279,558560,279280,837840,922.2844667434692,0.08821582500240766
280280,560562,280281,840843,925.4756660461426,0.087919444687941
281281,562564,281282,843846,928.5954778194427,0.08761950703410548
282282,564566,282283,846849,931.8302681446075,0.08732924613650539
283283,566568,283284,849852,935.0987920761108,0.08703904316462285
284284,568570,284285,852855,938.2216219902039,0.08675181585203973
285285,570572,285286,855858,941.385605096817,0.08646448038052768
286286,572574,286287,858861,944.4996740818024,0.08618096503050765
287287,574576,287288,861864,948.0349569320679,0.08590201172228262
288288,576578,288289,864867,952.3668761253357,0.08561937550803123
289289,578580,289290,867870,957.4778048992157,0.08534126657286834
290290,580582,290291,870873,961.3578081130981,0.08506259887872147
291291,582584,291292,873876,964.6262040138245,0.08478989211107546
292292,584586,292293,876879,967.85888504982,0.08451946561035584
293293,586588,293294,879882,971.2927799224854,0.08424756777640141
294294,588590,294295,882885,974.7476987838745,0.08398369482893031
295295,590592,295296,885888,977.9843509197235,0.08370801241107984
296296,592594,296297,888891,981.133003950119,0.08343828658144048
297297,594596,297298,891894,984.3124058246613,0.08317414516386634
298298,596598,298299,894897,987.525074005127,0.08291341662516061
299299,598600,299300,897900,990.6627340316772,0.08265382449098979
300300,600602,300301,900903,993.7990419864655,0.0823981085941341
301301,602604,301302,903906,996.9474239349365,0.08214311643678229
302302,604606,302303,906909,1000.1062309741974,0.08188884889204928
303303,606608,303304,909912,1003.2295730113983,0.08163511414386448
304304,608610,304305,912915,1006.373685836792,0.08138010504808335
305305,610612,305306,915918,1009.4914600849152,0.08112451448869251
306306,612614,306307,918921,1012.7236630916595,0.08087314273325319
307307,614616,307308,921924,1015.8449268341064,0.0806254348535731
308308,616618,308309,924927,1019.0316488742828,0.08038052174197219
309309,618620,309310,927930,1022.1696648597717,0.08014079315034905
310310,620622,310311,930933,1025.32039809227,0.0798958136474539
311311,622624,311312,933936,1028.6442930698395,0.07965374562627403
312312,624626,312313,936939,1031.856763124466,0.07941650450811721
313313,626628,313314,939942,1035.0306799411774,0.07917364170862129
314314,628630,314315,942945,1038.2588820457458,0.07893356873864832
315315,630632,315316,945948,1041.408164024353,0.0786947631095245
316316,632634,316317,948951,1044.5740451812744,0.07845986047323095
317317,634636,317318,951954,1047.7258217334747,0.07822849031981605
318318,636638,318319,954957,1050.8688280582428,0.0779890043540945
319319,638640,319320,957960,1054.0289468765259,0.077759381290889
320320,640642,320321,960963,1057.1611387729645,0.07753257944204961
321321,642644,321322,963966,1060.3174169063568,0.07730391225413769
322322,644646,322323,966969,1063.4688119888306,0.07708046329935314
323323,646648,323324,969972,1066.61727309227,0.07685706888696586
324324,648650,324325,972975,1069.7187161445618,0.07663479043912957
325325,650652,325326,975978,1072.8897609710693,0.07641355826490326
326326,652654,326327,978981,1076.0706589221954,0.07619351641187677
327327,654656,327328,981984,1079.228903055191,0.07597313282894902
328328,656658,328329,984987,1082.3447289466858,0.07575552177695499
329329,658660,329330,987990,1085.5218570232391,0.07554059549511294
330330,660662,330331,990993,1088.660579919815,0.07532256937702186
331331,662664,331332,993996,1091.8191878795624,0.07511143944975629
332332,664666,332333,996999,1094.9780180454254,0.07489736709612771
333333,666668,333334,1000002,1098.1688838005066,0.07468470936328231
334334,668670,334335,1003005,1101.3640060424805,0.07447105111532437
335335,670672,335336,1006008,1104.5445611476898,0.07426070514884486
336336,672674,336337,1009011,1107.6880958080292,0.07404844286611478
337337,674676,337338,1012014,1110.8434658050537,0.07384173696118523
338338,676678,338339,1015017,1114.1088519096375,0.07363414524115797
339339,678680,339340,1018020,1117.3491039276123,0.07343024728106684
340340,680682,340341,1021023,1120.5147659778595,0.07322976654359081
341341,682684,341342,1024026,1123.6640198230743,0.07302279608848039
342342,684686,342343,1027029,1126.8021171092987,0.07282086288978462
343343,686688,343344,1030032,1129.951975107193,0.07262342461581284
344344,688690,344345,1033035,1133.1409430503845,0.07242868881257891
345345,690692,345346,1036038,1136.2924358844757,0.07223064821300795
346346,692694,346347,1039041,1139.4480559825897,0.07203473163099261
347347,694696,347348,1042044,1142.5617518424988,0.07183832311056904
348348,696698,348349,1045047,1145.7275018692017,0.07164758330873156
349349,698700,349350,1048050,1148.8503370285034,0.07145429295269423
350350,700702,350351,1051053,1151.9947879314423,0.0712635462587059
351351,702704,351352,1054056,1155.1176590919495,0.07107359631481813
352352,704706,352353,1057059,1158.3974869251251,0.07088419655701728
353353,706708,353354,1060062,1161.59099984169,0.0706947094622592
354354,708710,354355,1063065,1164.7735409736633,0.07050756635180733
355355,710712,355356,1066068,1167.8992140293121,0.0703207417154772
356356,712714,356357,1069071,1171.0375158786774,0.07013308282694197
357357,714716,357358,1072074,1174.2046599388123,0.06994539621518925
358358,716718,358359,1075077,1177.3646428585052,0.06976274001863203
359359,718720,359360,1078080,1180.4949469566345,0.06958119714181521
360360,720722,360361,1081083,1183.6241948604584,0.06939953422806866
361361,722724,361362,1084086,1186.7589139938354,0.06921925193455536
362362,724726,362363,1087089,1189.892410993576,0.06903808879542339
363363,726728,363364,1090092,1193.0656869411469,0.06886187490272278
364364,728730,364365,1093095,1196.2309129238129,0.06868252303502231
365365,730732,365366,1096098,1199.3492209911346,0.06850604022110929
366366,732734,366367,1099101,1202.5111229419708,0.06833199484026409
367367,734736,367368,1102104,1205.638504743576,0.068157335239448
368368,736738,368369,1105107,1208.7921650409698,0.06798055420767923
369369,738740,369370,1108110,1212.053109884262,0.06780760223591642
370370,740742,370371,1111113,1215.1984629631042,0.0676334252457309
371371,742744,371372,1114116,1218.3798689842224,0.06745809260974056
372372,744746,372373,1117119,1221.523586988449,0.06728626407311822
373373,746748,373374,1120122,1224.6928868293762,0.06711427075242682
374374,748750,374375,1123125,1227.8433787822723,0.06694299407718063
375375,750752,375376,1126128,1231.0147960186005,0.0667714860446722
376376,752754,376377,1129131,1234.1425108909607,0.06660223213839345
377377,754756,377378,1132134,1237.2790579795837,0.06643522535705415
378378,756758,378379,1135137,1240.4251279830933,0.06627135087182978
379379,758760,379380,1138140,1243.6027150154114,0.06610417648153089
380380,760762,380381,1141143,1246.746120929718,0.06594335816225794
381381,762764,381382,1144146,1249.9132409095764,0.06577952658335562
382382,764766,382383,1147149,1253.0877759456635,0.06561648188289837
383383,766768,383384,1150152,1256.2583458423615,0.06545250448471052
384384,768770,384385,1153155,1259.3971219062805,0.06529538741415308
385385,770772,385386,1156158,1262.5495109558105,0.06513237012222817
386386,772774,386387,1159161,1265.7043778896332,0.0649750957127253
387387,774776,387388,1162164,1268.8419868946075,0.06481972266374214
388388,776778,388389,1165167,1271.9635009765625,0.06465900004877767
389389,778780,389390,1168170,1275.1324877738953,0.06450198187485512
390390,780782,390391,1171173,1278.3456780910492,0.0643454819019098
391391,782784,391392,1174176,1281.5098719596863,0.06418672602376319
392392,784786,392393,1177179,1284.6665320396423,0.06403159612455056
393393,786788,393394,1180182,1287.8135669231415,0.06388071266883344
394394,788790,394395,1183185,1290.9587960243225,0.06372715586439881
395395,790792,395396,1186188,1294.0847549438477,0.06357453322561923
396396,792794,396397,1189191,1297.255756855011,0.06342363000658224
397397,794796,397398,1192194,1300.4047219753265,0.06327064707147656
398398,796798,398399,1195197,1303.5434629917145,0.06312170886849344
399399,798800,399400,1198200,1306.6934039592743,0.06297276787518058
400400,800802,400401,1201203,1309.8496308326721,0.06282351444315282
401401,802804,401402,1204206,1313.018019914627,0.06267517084597785
402402,804806,402403,1207209,1316.1373829841614,0.06252440000935167
403403,806808,403404,1210212,1319.2914869785309,0.062379969471294316
404404,808810,404405,1213215,1322.4530851840973,0.062234104161689174
405405,810812,405406,1216218,1325.585079908371,0.06209096334896458
406406,812814,406407,1219221,1328.7728979587555,0.06194253749708878
407407,814816,407408,1222224,1331.8665919303894,0.06179840485492605
408408,816818,408409,1225227,1335.0195748806,0.06165560378212831
409409,818820,409410,1228230,1338.168741941452,0.061514495904702926
410410,820822,410411,1231233,1341.3231389522552,0.06137498021053034
411411,822824,411412,1234236,1344.5648109912872,0.06123610360373277
412412,824826,412413,1237239,1347.7482688426971,0.06109562876918062
413413,826828,413414,1240242,1350.8960118293762,0.06095525485761755
414414,828830,414415,1243245,1354.0299980640411,0.06081667955004377
415415,830832,415416,1246248,1357.2066740989685,0.06067929220807855
416416,832834,416417,1249251,1360.3707330226898,0.06054175743884116
417417,834836,417418,1252254,1363.5078928470612,0.06040306264185347
418418,836838,418419,1255257,1366.6694560050964,0.06026871407630097
419419,838840,419420,1258260,1369.7905468940735,0.060132589233035105
420420,840842,420421,1261263,1372.954931974411,0.05999803644772328
421421,842844,421422,1264266,1376.1227538585663,0.05986405484327406
422422,844846,422423,1267269,1379.2579560279846,0.05972991670569172
423423,846848,423424,1270272,1382.3799679279327,0.059596150245852186
424424,848850,424425,1273275,1385.5554909706116,0.05946374485756678
425425,850852,425426,1276278,1388.7404849529266,0.05933206732515828
426426,852854,426427,1279281,1391.8855049610138,0.05919907424504345
427427,854856,427428,1282284,1395.0169899463654,0.05906868835882051
428428,856858,428429,1285287,1398.2213830947876,0.05893881947486079
429429,858860,429430,1288290,1401.3907208442688,0.0588066089530912
430430,860862,430431,1291293,1404.5791800022125,0.058678364806837635
431431,862864,431432,1294296,1407.767154932022,0.05854971923326957
432432,864866,432433,1297299,1410.9271049499512,0.058421492043635226
433433,866868,433434,1300302,1414.1489069461823,0.058294382941312506
434434,868870,434435,1303305,1417.3319220542908,0.058168406303593656
435435,870872,435436,1306308,1420.4515607357025,0.05804166982488823
436436,872874,436437,1309311,1423.5834748744965,0.05791795457844273
437437,874876,437438,1312314,1426.7358350753784,0.05779200810866314
438438,876878,438439,1315317,1429.844561100006,0.05766726786714571
439439,878880,439440,1318320,1433.0183520317078,0.05754391759910504
440440,880882,440441,1321323,1436.1316289901733,0.05741835710068699
441441,882884,441442,1324326,1439.2818179130554,0.057293671981824446
442442,884886,442443,1327329,1442.4150879383087,0.057172790215190616
443443,886888,443444,1330332,1445.5766909122467,0.05705300022418669
444444,888890,444445,1333335,1448.7415080070496,0.05693163285468472
445445,890892,445446,1336338,1451.9121367931366,0.05681374396044703
446446,892894,446447,1339341,1455.0398120880127,0.05669458049851528
447447,894896,447448,1342344,1458.198961019516,0.056576138915261254
448448,896898,448449,1345347,1461.32870388031,0.056457972974385484
449449,898900,449450,1348350,1464.5179629325867,0.05633830330771161
450450,900902,450451,1351353,1467.6450951099396,0.0562211262404162
451451,902904,451452,1354356,1470.9008359909058,0.056105323768861126
452452,904906,452453,1357359,1474.010354757309,0.05598744606686523
453453,906908,453454,1360362,1477.1540248394012,0.055871996311907424
454454,908910,454455,1363365,1480.300742149353,0.05575627851067111
455455,910912,455456,1366368,1483.421777009964,0.055639961998167564
456456,912914,456457,1369371,1486.5619759559631,0.055526395844935905
457457,914916,457458,1372374,1489.7044169902802,0.055411639623343945
458458,916918,458459,1375377,1492.8452908992767,0.05529790212676744
459459,918920,459460,1378380,1495.9965109825134,0.05518290323743713
460460,920922,460461,1381383,1499.2333381175995,0.05506938186044863
461461,922924,461462,1384386,1502.392716884613,0.05495822140619566
462462,924926,462463,1387389,1505.5476450920105,0.054844704227434704
463463,926928,463464,1390392,1508.7012090682983,0.05473243259257288
464464,928930,464465,1393395,1511.864578962326,0.05462007967435056
465465,930932,465466,1396398,1515.0244450569153,0.054511328489752486
466466,932934,466467,1399401,1518.1916131973267,0.054401612462243065
467467,934936,467468,1402404,1521.3799879550934,0.0542896384067717
468468,936938,468469,1405407,1524.5458080768585,0.05418094660853967
469469,938940,469470,1408410,1527.676080942154,0.054072229790108395
470470,940942,470471,1411413,1530.8868429660797,0.05396303886118403
471471,942944,471472,1414416,1534.0368402004242,0.053853469020396005
472472,944946,472473,1417419,1537.194760799408,0.053747301191833685
473473,946948,473474,1420422,1540.361130952835,0.053639915444364306
474474,948950,474475,1423425,1543.5116708278656,0.053533352469457895
475475,950952,475476,1426428,1546.630312204361,0.05342485800247232
476476,952954,476477,1429431,1549.8271751403809,0.05332076743616199
477477,954956,477478,1432434,1553.329232931137,0.053215817744785454
478478,956958,478479,1435437,1556.5475628376007,0.05310885204016813
479479,958960,479480,1438440,1559.668445110321,0.05300600652844878
480480,960962,480481,1441443,1562.8337488174438,0.052900794871675316
481481,962964,481482,1444446,1566.0634150505066,0.05279814907044056
482482,964966,482483,1447449,1569.2521698474884,0.05269305521687784
483483,966968,483484,1450452,1572.4843838214874,0.05259018527249282
484484,968970,484485,1453455,1575.718924999237,0.05248831227982009
485485,970972,485486,1456458,1578.9396629333496,0.052386169705641805
486486,972974,486487,1459461,1582.0803740024567,0.052283488354078145
487487,974976,487488,1462464,1585.2690658569336,0.052181147098963265
488488,976978,488489,1465467,1588.5091669559479,0.05207966296984523
489489,978980,489490,1468470,1591.748496055603,0.051980278207338415
490490,980982,490491,1471473,1594.8946959972382,0.051877976351534016
491491,982984,491492,1474476,1598.0711369514465,0.0517795587056753
492492,984986,492493,1477479,1601.2313709259033,0.05167965121290763
493493,986988,493494,1480482,1604.4182629585266,0.05158046599171939
494494,988990,494495,1483485,1607.6814849376678,0.05148222935349622
495495,990992,495496,1486488,1610.8185770511627,0.05138407037702564
496496,992994,496497,1489491,1613.998888015747,0.05128688516197144
497497,994996,497498,1492494,1617.1515748500824,0.05118980230508896
498498,996998,498499,1495497,1620.2715528011322,0.05109390031793737
499499,999000,499500,1498500,1623.4381759166718,0.050995432646232075
500501,1001004,500502,1501506,1626.583009004593,0.05090035688954231
501502,1003006,501503,1504509,1629.7402868270874,0.050805758639398846
502503,1005008,502504,1507512,1632.8726329803467,0.05071089473676693
503504,1007010,503505,1510515,1636.0216839313507,0.050615932341315784
504505,1009012,504506,1513518,1639.2338647842407,0.050521713827038184
505506,1011014,505507,1516521,1642.3657879829407,0.05042548369419819
506507,1013016,506508,1519524,1645.5556840896606,0.05033082427326008
507508,1015018,507509,1522527,1648.728436946869,0.05023666063607379
508509,1017020,508510,1525530,1651.8732669353485,0.05014328451215988
509510,1019022,509511,1528533,1655.0135951042175,0.05005090968552395
510511,1021024,510512,1531536,1658.1827890872955,0.049959424357439275
511512,1023026,511513,1534539,1661.31210398674,0.049867271964103566
512513,1025028,512514,1537542,1664.4548168182373,0.049773681414080784
513514,1027030,513515,1540545,1667.5774660110474,0.04968110229674494
514515,1029032,514516,1543548,1670.7137019634247,0.049589778822337394
515516,1031034,515517,1546551,1673.851751089096,0.04949589047100744
516517,1033036,516518,1549554,1677.0397238731384,0.04940552661719266
517518,1035038,517519,1552557,1680.1724331378937,0.049314870724629145
518519,1037040,518520,1555560,1683.3217520713806,0.04922398920825799
519520,1039042,519521,1558563,1686.452054977417,0.04913330849376507
520521,1041044,520522,1561566,1689.621505022049,0.049043751543649705
521522,1043046,521523,1564569,1692.8119859695435,0.0489543357216462
522523,1045048,522524,1567572,1695.9999539852142,0.04886592671937251
523524,1047050,523525,1570575,1699.155601978302,0.04877819638750225
524525,1049052,524526,1573578,1702.2986080646515,0.0486907016402256
525526,1051054,525527,1576581,1705.4767138957977,0.04860325131994614
526527,1053056,526528,1579584,1708.62118601799,0.04851394532852282
527528,1055058,527529,1582587,1711.7446508407593,0.04842633028783894
528529,1057060,528530,1585590,1714.8936820030212,0.04833868170862843
529530,1059062,529531,1588593,1718.072138786316,0.048251480924591306
530531,1061064,530532,1591596,1721.2370779514313,0.048163793258936494
531532,1063066,531533,1594599,1724.3970611095428,0.04807844823153573
532533,1065068,532534,1597602,1727.5854759216309,0.04799239403473621
533534,1067070,533535,1600605,1730.7109339237213,0.04790563487949839
534535,1069072,534536,1603608,1733.9016089439392,0.0478212656944379
535536,1071074,535537,1606611,1737.0146729946136,0.047737461207361775
536537,1073076,536538,1609614,1740.1617279052734,0.047654560577939264
537538,1075078,537539,1612617,1743.3033530712128,0.047569475282216445
538539,1077080,538540,1615620,1746.4674808979034,0.04748495266176178
539540,1079082,539541,1618623,1749.5907890796661,0.04740149079771072
540541,1081084,540542,1621626,1752.7552528381348,0.04731940388046496
541542,1083086,541543,1624629,1755.8993680477142,0.0472373421798693
542543,1085088,542544,1627632,1759.065689086914,0.04715322945776279
543544,1087090,543545,1630635,1762.1999127864838,0.047069958251086064
544545,1089092,544546,1633638,1765.362576007843,0.04698887720769562
545546,1091094,545547,1636641,1768.494961977005,0.046906223375117406
546547,1093096,546548,1639644,1771.6578459739685,0.046825318539049476
547548,1095098,547549,1642647,1775.227998971939,0.046742959562834585
548549,1097100,548550,1645650,1778.8756058216095,0.04666254513358581
549550,1099102,549551,1648653,1782.4012069702148,0.046581631675508106
550551,1101104,550552,1651656,1786.225327014923,0.04650192002009135
551552,1103106,551553,1654659,1789.835035085678,0.04642086829881009
552553,1105108,552554,1657662,1793.8439300060272,0.04634116964916757
553554,1107110,553555,1660665,1797.7989249229431,0.04626296538663155
554555,1109112,554556,1663668,1801.1518869400024,0.046185372442778316
555556,1111114,555557,1666671,1804.663337945938,0.046107495783871855
556557,1113116,556558,1669674,1808.100370168686,0.04603011263498047
557558,1115118,557559,1672677,1811.6722049713135,0.04595306099508889
558559,1117120,558560,1675680,1814.9623777866364,0.0458741017318971
559560,1119122,559561,1678683,1818.1772468090057,0.04579636055495939
560561,1121124,560562,1681686,1821.3694241046906,0.045718708366621286
561562,1123126,561563,1684689,1824.8428359031677,0.04564223754823615
562563,1125128,562564,1687692,1828.3851580619812,0.04556606764163007
563564,1127130,563565,1690695,1831.8375887870789,0.0454895422590198
564565,1129132,564566,1693698,1835.0059559345245,0.045412774130454636
565566,1131134,565567,1696701,1838.2205259799957,0.04533767696375435
566567,1133136,566568,1699704,1841.3831651210785,0.04526180666107393
567568,1135138,567569,1702707,1844.9258279800415,0.04518569262836536
568569,1137140,568570,1705710,1848.3076379299164,0.04511015470052371
569570,1139142,569571,1708713,1851.7804069519043,0.04503496786310279
570571,1141144,570572,1711716,1855.3732059001923,0.044959556576941395
571572,1143146,571573,1714719,1858.8313419818878,0.04488413905346533
572573,1145148,572574,1717722,1862.3637919425964,0.0448101383390167
573574,1147150,573575,1720725,1866.334076166153,0.04473666089506878
574575,1149152,574576,1723728,1870.2870519161224,0.04466009384850622
575576,1151154,575577,1726731,1874.3534178733826,0.044587020616745576
576577,1153156,576578,1729734,1878.1478769779205,0.04451414503819251
577578,1155158,577579,1732737,1881.9773280620575,0.04444091132245376
578579,1157160,578580,1735740,1885.3233659267426,0.04436869539131294
579580,1159162,579581,1738743,1888.5962400436401,0.04429689074822818
580581,1161164,580582,1741746,1891.8755869865417,0.04422357928160636
581582,1163166,581583,1744749,1895.4415469169617,0.04414986156371015
582583,1165168,582584,1747752,1898.611743927002,0.04407581319355813
583584,1167170,583585,1750755,1901.9417929649353,0.044004772847983986
584585,1169172,584586,1753758,1905.3456118106842,0.04393424596310069
585586,1171174,585587,1756761,1908.7309720516205,0.043862658416401246
586587,1173176,586588,1759764,1911.9918749332428,0.043793404369353084
587588,1175178,587589,1762767,1915.2745609283447,0.0437222551117884
588589,1177180,588590,1765770,1918.5419878959656,0.043650132005495834
589590,1179182,589591,1768773,1922.4201440811157,0.04358097710064612
590591,1181184,590592,1771776,1925.621423959732,0.04351138607125904
591592,1183186,591593,1774779,1928.8603188991547,0.043441357111078105
592593,1185188,592594,1777782,1932.5221920013428,0.04337170409417013
593594,1187190,593595,1780785,1936.6794199943542,0.043302403446432436
594595,1189192,594596,1783788,1941.9770851135254,0.04323324109282112
595596,1191194,595597,1786791,1948.2553520202637,0.04316388510778779
596597,1193196,596598,1789794,1955.093554019928,0.04309501779061975
597598,1195198,597599,1792797,1959.2258758544922,0.043026458381064
598599,1197200,598600,1795800,1963.5981090068817,0.04295820854531485
599600,1199202,599601,1798803,1968.2218689918518,0.042889869093414745
600601,1201204,600602,1801806,1972.311040878296,0.04282092554967676
601602,1203206,601603,1804809,1977.5238199234009,0.04275241000868846
602603,1205208,602604,1807812,1985.064659833908,0.04268527343265305
603604,1207210,603605,1810815,1991.0554311275482,0.04261758642496716
604605,1209212,604606,1813818,1997.0010690689087,0.04255037713301135
605606,1211214,605607,1816821,2003.3884608745575,0.04248414690846403
606607,1213216,606608,1819824,2007.9060881137848,0.042415345551489736
607608,1215218,607609,1822827,2012.2413218021393,0.04234929137965082
608609,1217220,608610,1825830,2015.62043094635,0.042283609795049415
609610,1219222,609611,1828833,2018.9647438526154,0.04221700195193989
610611,1221224,610612,1831836,2022.8233420848846,0.0421519214505679
611612,1223226,611613,1834839,2028.2265319824219,0.04208638289310329
612613,1225228,612614,1837842,2032.9879038333893,0.04202031037857523
613614,1227230,613615,1840845,2037.1618638038635,0.04195546826667851
614615,1229232,614616,1843848,2042.976124048233,0.04188987466477556
615616,1231234,615617,1846851,2048.7355608940125,0.04182607431539509
616617,1233236,616618,1849854,2054.129898786545,0.04176243709480332
617618,1235238,617619,1852857,2059.7739288806915,0.04169758628268028
618619,1237240,618620,1855860,2066.0419318675995,0.041635043040514574
619620,1239242,619621,1858863,2071.8875029087067,0.041571202125851414
620621,1241244,620622,1861866,2077.994777917862,0.04150764776204596
621622,1243246,621623,1864869,2084.0906269550323,0.04144455976529571
622623,1245248,622624,1867872,2089.212607860565,0.041379930669791065
623624,1247250,623625,1870875,2094.5463128089905,0.04131724388207658
624625,1249252,624626,1873878,2100.0910229682922,0.04125405273771321
625626,1251254,625627,1876881,2105.7901339530945,0.041191075797542
626627,1253256,626628,1879884,2111.277456998825,0.04112834275838395
627628,1255258,627629,1882887,2116.9726309776306,0.04106545570175513
628629,1257260,628630,1885890,2122.2987360954285,0.04100408538033662
629630,1259262,629631,1888893,2127.5815529823303,0.04094285784049134
630631,1261264,630632,1891896,2132.7739329338074,0.040880973521780106
631632,1263266,631633,1894899,2138.2709300518036,0.04081938163108134
632633,1265268,632634,1897902,2143.6012799739838,0.040758221462965594
633634,1267270,633635,1900905,2148.7185609340668,0.04069696935403044
634635,1269272,634636,1903908,2154.0890579223633,0.04063567369848897
635636,1271274,635637,1906911,2159.37774682045,0.04057409816959989
636637,1273276,636638,1909914,2164.5885627269745,0.04051328544301214
637638,1275278,637639,1912917,2169.7127211093903,0.04045297698030481
638639,1277280,638640,1915920,2175.095111131668,0.040392912771494593
639640,1279282,639641,1918923,2180.4443418979645,0.04033282272575889
640641,1281284,640642,1921926,2185.747433900833,0.040273815397085855
641642,1283286,641643,1924929,2191.419862985611,0.04021324417772121
642643,1285288,642644,1927932,2197.247104883194,0.04015354650255176
643644,1287290,643645,1930935,2202.5706741809845,0.04009462554677157
644645,1289292,644646,1933938,2207.7880580425262,0.04003443870533374
645646,1291294,645647,1936941,2213.2182669639587,0.039974716908545815
646647,1293296,646648,1939944,2218.617031097412,0.03991660761857929
647648,1295298,647649,1942947,2223.803519964218,0.03985788689351466
648649,1297300,648650,1945950,2229.237277030945,0.03979905945743667
649650,1299302,649651,1948953,2234.788936853409,0.03974067712260876
650651,1301304,650652,1951956,2240.141368865967,0.03968275122679188
651652,1303306,651653,1954959,2246.0997400283813,0.039624319100767025
652653,1305308,652654,1957962,2251.525661945343,0.03956645934158587
653654,1307310,653655,1960965,2257.1946709156036,0.0395078811179701
654655,1309312,654656,1963968,2264.332941055298,0.0394513010069204
655656,1311314,655657,1966971,2270.2472448349,0.039392405155012966
656657,1313316,656658,1969974,2275.903461933136,0.03933641526600695
657658,1315318,657659,1972977,2282.0164959430695,0.03927874493456329
658659,1317320,658660,1975980,2287.0984721183777,0.03922197036808939
659660,1319322,659661,1978983,2292.211678981781,0.03916570541150577
660661,1321324,660662,1981986,2297.267026901245,0.0391096770454169
661662,1323326,661663,1984989,2302.3890538215637,0.03905399721770664
662663,1325328,662664,1987992,2307.511715888977,0.03899830144291627
663664,1327330,663665,1990995,2312.5932998657227,0.03894232297534472
664665,1329332,664666,1993998,2317.6712868213654,0.0388862266754586
665666,1331334,665667,1997001,2322.7218039035797,0.03883053954450588
666667,1333336,666668,2000004,2327.828311920166,0.03877456749432895
667668,1335338,667669,2003007,4091.698336839676,0.03871932228321384
668669,1337340,668670,2006010,4099.084939956665,0.03866480605756806
669670,1339342,669671,2009013,4115.691527843475,0.03860982913101907
670671,1341344,670672,2012016,4139.026416063309,0.038555029375856975
671672,1343346,671673,2015019,4142.970368862152,0.038501210930917296
672673,1345348,672674,2018022,4146.455374956131,0.03844708491305937
673674,1347350,673675,2021025,4149.963955879211,0.038393645039832336
674675,1349352,674676,2024028,4153.836854934692,0.038339206021191785
675676,1351354,675677,2027031,4157.450986862183,0.03828540522954427
676677,1353356,676678,2030034,4161.239151000977,0.03823104801631416
677678,1355358,677679,2033037,4164.6348531246185,0.03817709151735471
678679,1357360,678680,2036040,4168.356494903564,0.03812284182095027
679680,1359362,679681,2039043,4171.726599931717,0.0380702406855562
680681,1361364,680682,2042046,4175.091633081436,0.03801742582800216
681682,1363366,681683,2045049,4178.780520915985,0.03796415519173024
682683,1365368,682684,2048052,4182.156746864319,0.03791121947506326
683684,1367370,683685,2051055,4185.515522003174,0.0378580127726309
684685,1369372,684686,2054058,4188.905415058136,0.037805041449246346
685686,1371374,685687,2057061,4192.562621831894,0.037752692680442124
686687,1373376,686688,2060064,4195.947293043137,0.03770106526098971
687688,1375378,687689,2063067,4199.137413978577,0.03764945925831853
688689,1377380,688690,2066070,4202.27200293541,0.03759599534532754
689690,1379382,689691,2069073,4205.992250919342,0.03754296102488297
690691,1381384,690692,2072076,4210.528977155685,0.03749097446416272
691692,1383386,691693,2075079,4215.187668800354,0.03743898047832772
692693,1385388,692694,2078082,4219.946036815643,0.03738743566827907
693694,1387390,693695,2081085,4223.696805000305,0.03733618166188535
694695,1389392,694696,2084088,4227.292818784714,0.03728485861392983
695696,1391394,695697,2087091,4231.148254871368,0.037233469729471835
696697,1393396,696698,2090094,4235.161218881607,0.03718269662203966
697698,1395398,697699,2093097,4238.718869924545,0.03713197352226416
698699,1397400,698700,2096100,4242.424997091293,0.03708065932369209
699700,1399402,699701,2099103,4246.540647983551,0.0370299874975899
700701,1401404,700702,2102106,4250.353470802307,0.03698010499647353
701702,1403406,701703,2105109,4254.4948699474335,0.03692995557867107
702703,1405408,702704,2108112,4258.967711925507,0.03688004927789734
703704,1407410,703705,2111115,4262.817600011826,0.036830290944635635
704705,1409412,704706,2114118,4267.033741950989,0.03678107391351659
705706,1411414,705707,2117121,4270.729420900345,0.036731516043801093
706707,1413416,706708,2120124,4274.544628858566,0.03668132059829077
707708,1415418,707709,2123127,4278.190690994263,0.036631594459322514
708709,1417420,708710,2126130,4282.122334957123,0.0365823926840676
709710,1419422,709711,2129133,4285.968441963196,0.03653395191213349
710711,1421424,710712,2132136,4290.232913970947,0.0364840890179039
711712,1423426,711713,2135139,4293.940696001053,0.03643541640849435
712713,1425428,712714,2138142,4297.519789934158,0.036386769426826504
713714,1427430,713715,2141145,4301.173377990723,0.03633834562606353
714715,1429432,714716,2144148,4304.812829017639,0.03629088347770448
715716,1431434,715717,2147151,4308.091698169708,0.03624298957220162
716717,1433436,716718,2150154,4312.041035890579,0.03619523824454518
717718,1435438,717719,2153157,4316.284625053406,0.036146624142929795
718719,1437440,718720,2156160,4320.174027919769,0.03609831373796624
719720,1439442,719721,2159163,4324.289486885071,0.03604966674538446
720721,1441444,720722,2162166,4328.527805089951,0.03600229898984253
721722,1443446,721723,2165169,4332.483278989792,0.03595412662616582
722723,1445448,722724,2168172,4336.397146940231,0.03590584421908716
723724,1447450,723725,2171175,4340.613430023193,0.03585837710306805
724725,1449452,724726,2174178,4344.800122022629,0.03581201867746131
725726,1451454,725727,2177181,4349.157467126846,0.03576470997359138
726727,1453456,726728,2180184,4352.994756937027,0.03571860784177261
727728,1455458,727729,2183187,4356.68745303154,0.035671457491844194
728729,1457460,728730,2186190,4360.579021930695,0.03562449936907797
729730,1459462,729731,2189193,4364.03465795517,0.03557748882667511
730731,1461464,730732,2192196,4367.6006100177765,0.03553088889566425
731732,1463466,731733,2195199,4371.755285978317,0.03548482366022654
732733,1465468,732734,2198202,4375.239307880402,0.0354382008772518
733734,1467470,733735,2201205,4379.271016120911,0.0353913798717258
734735,1469472,734736,2204208,4382.708813905716,0.03534572712669615
735736,1471474,735737,2207211,4385.886002063751,0.035300097420986276
736737,1473476,736738,2210214,4389.246035814285,0.035254299034932046
737738,1475478,737739,2213217,4392.560343980789,0.03520932006176736
738739,1477480,738740,2216220,4395.858367919922,0.03516398169085733
739740,1479482,739741,2219223,4399.202148914337,0.03511880136284162
740741,1481484,740742,2222226,4402.778849840164,0.03507275264200871
741742,1483486,741743,2225229,4406.3883509635925,0.035027042191359214
742743,1485488,742744,2228232,4410.389400005341,0.034981531938683474
743744,1487490,743745,2231235,4413.91626906395,0.03493698836427939
744745,1489492,744746,2234238,4417.088963031769,0.03489175106733455
745746,1491494,745747,2237241,4420.768791913986,0.034847662844185834
746747,1493496,746748,2240244,4423.96058678627,0.034803178792572
747748,1495498,747749,2243247,4427.193526029587,0.034758711204631254
748749,1497500,748750,2246250,4430.559084892273,0.03471424038798432
749750,1499502,749751,2249253,4434.830430984497,0.034669603393922444
750751,1501504,750752,2252256,4439.1307208538055,0.03462416969705373
751752,1503506,751753,2255259,4444.241780996323,0.034579417819259106
752753,1505508,752754,2258262,4449.22009396553,0.03453658034231921
753754,1507510,753755,2261265,4453.3006939888,0.03449279608321376
754755,1509512,754756,2264268,4458.001098871231,0.03444845521153184
755756,1511514,755757,2267271,4461.740766763687,0.03440501668410434
756757,1513516,756758,2270274,4465.388877868652,0.034362663063802756
757758,1515518,757759,2273277,4468.905707836151,0.034319789137953194
758759,1517520,758760,2276280,4472.3062398433685,0.03427602720330469
759760,1519522,759761,2279283,4475.762804985046,0.03423261836542224
760761,1521524,760762,2282286,4479.246771812439,0.03418961277930066
761762,1523526,761763,2285289,4482.66813993454,0.03414665835589403
762763,1525528,762764,2288292,4486.4732620716095,0.03410442505264655
763764,1527530,763765,2291295,4490.102833986282,0.03406161260136287
764765,1529532,764766,2294298,4493.757650136948,0.034019160661046044
765766,1531534,765767,2297301,4497.602061033249,0.03397746815608116
766767,1533536,766768,2300304,4501.4056391716,0.03393495422460546
767768,1535538,767769,2303307,4505.053637981415,0.03389227359184588
768769,1537540,768770,2306310,4508.750738859177,0.03384961175106582
769770,1539542,769771,2309313,4513.403367996216,0.03380806336281239
770771,1541544,770772,2312316,4517.763236045837,0.033766449540053145
771772,1543546,771773,2315319,4522.182215929031,0.033724763938153046
772773,1545548,772774,2318322,4526.025736808777,0.033683460769680096
773774,1547550,773775,2321325,4530.470230817795,0.03364172602232429
774775,1549552,774776,2324328,4534.898781776428,0.033599998056160985
775776,1551554,775777,2327331,4539.649871110916,0.0335584021104296
776777,1553556,776778,2330334,4544.470153808594,0.033517257137646084
777778,1555558,777779,2333337,4549.37979888916,0.03347643734377925
778779,1557560,778780,2336340,4554.1906089782715,0.03343526779462991
779780,1559562,779781,2339343,4558.6956288814545,0.03339471659819537
780781,1561564,780782,2342346,4562.211613893509,0.03335386601793289
781782,1563566,781783,2345349,4566.618706941605,0.033313104533590376
782783,1565568,782784,2348352,4570.546141862869,0.03327247619199625
783784,1567570,783785,2351355,4574.593616962433,0.033232224981475156
784785,1569572,784786,2354358,4578.544322967529,0.033192340004461585
785786,1571574,785787,2357361,4582.22572517395,0.033151528046801104
786787,1573576,786788,2360364,4585.520621061325,0.03311041713459417
787788,1575578,787789,2363367,4589.391371011734,0.03307095599666354
788789,1577580,788790,2366370,4592.958515882492,0.03303067898377776
789790,1579582,789791,2369373,4597.24237203598,0.03299129588231153
790791,1581584,790792,2372376,4600.510750770569,0.0329518017861119
791792,1583586,791793,2375379,4604.293848991394,0.03291252976850956
792793,1585588,792794,2378382,4608.062875032425,0.03287402156456665
793794,1587590,793795,2381385,4612.048408985138,0.03283395802100131
794795,1589592,794796,2384388,4615.508891105652,0.032795438206449035
795796,1591594,795797,2387391,4619.783047914505,0.032755821781393024
796797,1593596,796798,2390394,4623.007378816605,0.03271525218951865
797798,1595598,797799,2393397,4626.2900149822235,0.032676240287401015
798799,1597600,798800,2396400,4629.5637748241425,0.03263684814919543
799800,1599602,799801,2399403,4632.871695995331,0.032597626335700625
800801,1601604,800802,2402406,4636.373883962631,0.032558924927798216
801802,1603606,801803,2405409,4640.025093078613,0.032519601638341555
802803,1605608,802804,2408412,4643.816245794296,0.03248162298950774
803804,1607610,803805,2411415,4647.103326797485,0.032443141304611345
804805,1609612,804806,2414418,4650.2938940525055,0.03240454524893721
805806,1611614,805807,2417421,4653.539753913879,0.03236644182834425
806807,1613616,806808,2420424,4656.701565742493,0.03232829934131587
807808,1615618,807809,2423427,4660.016810894012,0.032289791975927074
808809,1617620,808810,2426430,4663.346800088882,0.03225160025067453
809810,1619622,809811,2429433,4666.582525014877,0.032214089267654344
810811,1621624,810812,2432436,4670.813022851944,0.032175778036616975
811812,1623626,811813,2435439,4674.429881095886,0.0321390231129044
812813,1625628,812814,2438442,4677.726385116577,0.032100406100653345
813814,1627630,813815,2441445,4681.018491029739,0.0320630025016726
814815,1629632,814816,2444448,4684.411664009094,0.03202519233309431
815816,1631634,815817,2447451,4687.647872924805,0.03198814424467855
816817,1633636,816818,2450454,4691.246066093445,0.03195124947524164
817818,1635638,817819,2453457,4694.548254966736,0.03191364057784085
818819,1637640,818820,2456460,4697.689256191254,0.03187679375332664
819820,1639642,819821,2459463,4700.970524072647,0.03183907057973556
820821,1641644,820822,2462466,4704.184775114059,0.03180179355695145
821822,1643646,821823,2465469,4707.555480957031,0.03176509848526621
822823,1645648,822824,2468472,4711.077173948288,0.03172879615340207
823824,1647650,823825,2471475,4714.901731014252,0.03169159653407405
824825,1649652,824826,2474478,4718.409392118454,0.031654371681725024
825826,1651654,825827,2477481,4722.380391120911,0.031617933373127016
826827,1653656,826828,2480484,4726.011096000671,0.031581702236508136
827828,1655658,827829,2483487,4729.288881063461,0.03154470658955688
828829,1657660,828830,2486490,4733.088234901428,0.03150773511879379
829830,1659662,829831,2489493,4737.078544139862,0.031471800484723644
830831,1661664,830832,2492496,4741.203775882721,0.03143545958118921
831832,1663666,831833,2495499,4744.547883987427,0.031399543542647734
832833,1665668,832834,2498502,4747.984932899475,0.03136315700430714
833834,1667670,833835,2501505,4751.371357917786,0.03132686094795645
834835,1669672,834836,2504508,4755.237520933151,0.03129095609074284
835836,1671674,835837,2507511,4758.935166835785,0.031255343315933715
836837,1673676,836838,2510514,4762.238480091095,0.031219599479300086
837838,1675678,837839,2513517,4765.484871149063,0.031183902519842377
838839,1677680,838840,2516520,4768.997900009155,0.03114803342759842
839840,1679682,839841,2519523,4772.540303945541,0.03111256327247247
840841,1681684,840842,2522526,4776.287311077118,0.031077125167939812
841842,1683686,841843,2525529,4780.122676849365,0.031042275073559722
842843,1685688,842844,2528532,4783.873647928238,0.031006753735709935
843844,1687690,843845,2531535,4787.852553844452,0.03097192180393904
844845,1689692,844846,2534538,4791.620132923126,0.030935997239794233
845846,1691694,845847,2537541,4795.152317047119,0.03090112885547569
846847,1693696,846848,2540544,4798.642001152039,0.030866403350955807
847848,1695698,847849,2543547,4802.349472999573,0.030832054626444005
848849,1697700,848850,2546550,4806.017889022827,0.03079660007824714
849850,1699702,849851,2549553,4809.739509820938,0.030761423760850448
850851,1701704,850852,2552556,4813.272099018097,0.03072729557788989
851852,1703706,851853,2555559,4817.237803936005,0.030693142069139867
852853,1705708,852854,2558562,4821.143630981445,0.030659198517241748
853854,1707710,853855,2561565,4825.088047027588,0.030624860501120565
854855,1709712,854856,2564568,4829.578109025955,0.030590744057917618
855856,1711714,855857,2567571,4834.420916795731,0.030556371528291493
856857,1713716,856858,2570574,4838.682142972946,0.030522578983436688
857858,1715718,857859,2573577,4843.063844919205,0.03048810725158546
858859,1717720,858860,2576580,4847.023699760437,0.030453990892056026
859860,1719722,859861,2579583,4850.397127151489,0.030420116816458176
860861,1721724,860862,2582586,4853.847176790237,0.03038651472161291
861862,1723726,861863,2585589,4857.14200592041,0.03035241820725787
862863,1725728,862864,2588592,4860.75612783432,0.03031901862777886
863864,1727730,863865,2591595,4864.114503145218,0.030285821374491206
864865,1729732,864866,2594598,4867.571174144745,0.03025216152491339
865866,1731734,865867,2597601,4871.000324964523,0.03021919363163761
866867,1733736,866868,2600604,4874.585211992264,0.03018562353645393
867868,1735738,867869,2603607,4878.970557928085,0.030152297469612677
868869,1737740,868870,2606610,4883.050940990448,0.030119596720396657
869870,1739742,869871,2609613,4887.415110111237,0.030085728130870848
870871,1741744,870872,2612616,4891.133594989777,0.030053000888074166
871872,1743746,871873,2615619,4894.926430940628,0.030019500361959217
872873,1745748,872874,2618622,4898.790283918381,0.029986421606736258
873874,1747750,873875,2621625,4902.595242977142,0.029953411200040136
874875,1749752,874876,2624628,4906.043792009354,0.02992070059553953
875876,1751754,875877,2627631,4909.304524898529,0.02988757572893519
876877,1753756,876878,2630634,4912.70180606842,0.029854832333512604
877878,1755758,877879,2633637,4916.000274181366,0.029822144668287365
878879,1757760,878880,2636640,4919.192974090576,0.029788771171297412
879880,1759762,879881,2639643,4922.645506858826,0.029755646672128933
880881,1761764,880882,2642646,4926.638334989548,0.02972325278642529
881882,1763766,881883,2645649,4930.629602909088,0.02969039900926873
882883,1765768,882884,2648652,4934.19583773613,0.02965827065963822
883884,1767770,883885,2651655,4937.6632759571075,0.029626119685417507
884885,1769772,884886,2654658,4941.138813734055,0.02959422837739112
885886,1771774,885887,2657661,4944.8299198150635,0.02956127459037816
886887,1773776,886888,2660664,4948.827579975128,0.029529615469073178
887888,1775778,887889,2663667,4952.210072994232,0.029497455796445138
888889,1777780,888890,2666670,4956.627835035324,0.029466116100593354
889890,1779782,889891,2669673,4960.03732585907,0.029434167181534576
890891,1781784,890892,2672676,4963.6160678863525,0.029402903041045647
891892,1783786,891893,2675679,4967.133340120316,0.02937107244906656
892893,1785788,892894,2678682,4970.79675412178,0.02933935275177646
893894,1787790,893895,2681685,4974.499418973923,0.029308029457752127
894895,1789792,894896,2684688,4978.276323080063,0.029276658033268177
895896,1791794,895897,2687691,4982.086149930954,0.029245277168229222
896897,1793796,896898,2690694,4985.691527843475,0.02921408079964749
897898,1795798,897899,2693697,4990.41171503067,0.02918310409222613
898899,1797800,898900,2696700,4995.1042239665985,0.029152423341656686
899900,1799802,899901,2699703,4999.972170829773,0.029120745462932973
900901,1801804,900902,2702706,5004.972925901413,0.029089889752867748
901902,1803806,901903,2705709,5009.674431800842,0.02905919281693059
902903,1805808,902904,2708712,5014.780626773834,0.02902849067322677
903904,1807810,903905,2711715,5019.504405975342,0.02899744144269789
904905,1809812,904906,2714718,5023.838215112686,0.028966995763767045
905906,1811814,905907,2717721,5027.703917980194,0.028935690175785567
906907,1813816,906908,2720724,5032.816445827484,0.028905024228151888
907908,1815818,907909,2723727,5037.032786130905,0.028873939025288564
908909,1817820,908910,2726730,5041.019506931305,0.028843062413216103
909910,1819822,909911,2729733,5045.392885923386,0.028812653026761836
910911,1821824,910912,2732736,5049.725791931152,0.028782113158740685
911912,1823826,911913,2735739,5054.0988137722015,0.028752115731549566
912913,1825828,912914,2738742,5058.239325761795,0.0287215346161247
913914,1827830,913915,2741745,5061.927144050598,0.0286915788128681
914915,1829832,914916,2744748,5065.9133858680725,0.02866078713122988
915916,1831834,915917,2747751,5069.776775121689,0.028630538579818676
916917,1833836,916918,2750754,5073.357801914215,0.028600612144145998
917918,1835838,917919,2753757,5076.794517993927,0.028571161084983032
918919,1837840,918920,2756760,5080.489871025085,0.0285411127970292
919920,1839842,919921,2759763,5084.144505977631,0.02851063468551729
920921,1841844,920922,2762766,5087.993330955505,0.028481110790380626
921922,1843846,921923,2765769,5091.740677118301,0.028451663374653435
922923,1845848,922924,2768772,5095.515827894211,0.028422044808394276
923924,1847850,923925,2771775,5099.532336950302,0.028392245980285225
924925,1849852,924926,2774778,5103.799822092056,0.02836262343225826
925926,1851854,925927,2777781,5107.682447910309,0.028332986248642555
926927,1853856,926928,2780784,5111.133094072342,0.028303642857281375
927928,1855858,927929,2783787,5114.9874448776245,0.028274421334572253
928929,1857860,928930,2786790,5118.735208749771,0.028245034223800758
929930,1859862,929931,2789793,5122.1567368507385,0.028216122886078665
930931,1861864,930932,2792796,5125.937621831894,0.028186402099890984
931932,1863866,931933,2795799,5130.151705026627,0.028157841501524672
932933,1865868,932934,2798802,5133.598215103149,0.028128996576924692
933934,1867870,933935,2801805,5137.055328845978,0.028100239693230833
934935,1869872,934936,2804808,5140.480310916901,0.028071228734916076
935936,1871874,935937,2807811,5144.828907966614,0.028042384305081214
936937,1873876,936938,2810814,5149.025298833847,0.028013755325446255
937938,1875878,937939,2813817,5152.712814092636,0.02798347389943956
938939,1877880,938940,2816820,5156.892079114914,0.027954690285696415
939940,1879882,939941,2819823,5160.875806808472,0.02792558804321743
940941,1881884,940942,2822826,5164.415240764618,0.027897375875909347
941942,1883886,941943,2825829,5168.497157096863,0.02786889989693009
942943,1885888,942944,2828832,5172.118111848831,0.027840701995955897
943944,1887890,943945,2831835,5175.662349939346,0.02781281352508813
944945,1889892,944946,2834838,5179.312213897705,0.02778388583283231
945946,1891894,945947,2837841,5183.339426994324,0.027755733230151236
946947,1893896,946948,2840844,5187.590912818909,0.02772779733459174
947948,1895898,947949,2843847,5192.227419137955,0.027699891033989843
948949,1897900,948950,2846850,5196.816307783127,0.02767230679455679
949950,1899902,949951,2849853,5201.191655158997,0.02764438150006754
950951,1901904,950952,2852856,5205.3339149951935,0.02761588063913223
951952,1903906,951953,2855859,5209.415547132492,0.027587947281062952
952953,1905908,952954,2858862,5213.032489776611,0.027560153686863487
953954,1907910,953955,2861865,5216.4420347213745,0.02753220568592951
954955,1909912,954956,2864868,5219.830653190613,0.02750450854000519
955956,1911914,955957,2867871,5223.474904060364,0.027477171661303146
956957,1913916,956958,2870874,5227.610511064529,0.027449873845398542
957958,1915918,957959,2873877,5231.658034801483,0.02742221693188185
958959,1917920,958960,2876880,5236.212136030197,0.027394678072596435
959960,1919922,959961,2879883,5240.1828100681305,0.027366760514269117
960961,1921924,960962,2882886,5244.601906776428,0.02733927430017502
961962,1923926,961963,2885889,5248.613600969315,0.027310930887324503
962963,1925928,962964,2888892,5252.506670951843,0.027284040668746457
963964,1927930,963965,2891895,5256.091553926468,0.027256460296484875
964965,1929932,964966,2894898,5259.645341157913,0.027229739702306688
965966,1931934,965967,2897901,5263.401695966721,0.027202205023058923
966967,1933936,966968,2900904,5267.032893896103,0.02717545553423406
967968,1935938,967969,2903907,5271.464231014252,0.027148316801685723
968969,1937940,968970,2906910,5276.753186941147,0.027121235867525684
969970,1939942,969971,2909913,5280.941751003265,0.027094575749288197
970971,1941944,970972,2912916,5285.699464797974,0.027067925462688436
971972,1943946,971973,2915919,5289.779031038284,0.027041320225180243
972973,1945948,972974,2918922,5294.023982048035,0.02701479605093482
973974,1947950,973975,2921925,5298.48277592659,0.026988092213287018
974975,1949952,974976,2924928,5302.789623975754,0.02696152322096168
975976,1951954,975977,2927931,5307.030978918076,0.02693498028384056
976977,1953956,976978,2930934,5312.0432250499725,0.0269079985555436
977978,1955958,977979,2933937,5316.7024738788605,0.026881365693043335
978979,1957960,978980,2936940,5320.38431596756,0.026854754205487552
979980,1959962,979981,2939943,5324.378356933594,0.026828830190424924
980981,1961964,980982,2942946,5328.16979598999,0.02680286422400968
981982,1963966,981983,2945949,5332.5676419734955,0.02677618648885982
982983,1965968,982984,2948952,5337.038569927216,0.026750973735033767
983984,1967970,983985,2951955,5341.830600738525,0.026724187275249278
984985,1969972,984986,2954958,5346.262991905212,0.0266975292324787
985986,1971974,985987,2957961,5350.712601900101,0.026671626230381662
986987,1973976,986988,2960964,5354.621773004532,0.026645260586519726
987988,1975978,987989,2963967,5358.698045015335,0.026619375119480537
988989,1977980,988990,2966970,5362.769677877426,0.02659372013840766
989990,1979982,989991,2969973,5366.420922994614,0.02656835868037888
990991,1981984,990992,2972976,5370.021301984787,0.026542259774942067
991992,1983986,991993,2975979,5373.730073928833,0.02651684874763305
992993,1985988,992994,2978982,5377.596878051758,0.026490979760637856
993994,1987990,993995,2981985,5381.801306962967,0.026465454793651588
994995,1989992,994996,2984988,5385.666743040085,0.026439945575475576
995996,1991994,995997,2987991,5389.418166875839,0.026414401523652487
996997,1993996,996998,2990994,5393.604700088501,0.026389493952592602
997998,1995998,997999,2993997,5398.450407981873,0.02636395296030969
998999,1998000,999000,2997000,5402.246125936508,0.026338771709561115
1000000,2000002,1000001,3000003,5406.496776819229,0.026313360594940605


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0026559829711914062,12064.709122577777
1001,2003,2002,4005,3.4950649738311768,12.835124349569014
2002,4005,4004,8009,6.758717060089111,11.944634412788218
3003,6007,6006,12013,10.094599962234497,11.148884621363322
4004,8009,8008,16017,13.44087290763855,10.435206510481294
5005,10011,10010,20021,16.938480138778687,9.793065177316748
6006,12013,12012,24025,20.515602111816406,9.213598608499524
7007,14015,14014,28029,23.948411226272583,8.689284992171451
8008,16017,16016,32033,27.571858882904053,8.213692023180556
9009,18019,18018,36037,30.72619891166687,7.781284697110095
10010,20021,20020,40041,33.880789041519165,7.387273657386686
11011,22023,22022,44045,37.06355810165405,7.0274945171859144
12012,24025,24024,48049,40.28280997276306,6.698310615191076
13013,26027,26026,52053,43.56460523605347,6.396533875067689
14014,28029,28028,56057,46.711780071258545,6.119359828790039
15015,30031,30030,60061,49.841068983078,5.864313836927977
16016,32033,32032,64065,53.03543210029602,5.629206242432701
17017,34035,34034,68069,56.18182396888733,5.412094713119586
18018,36037,36036,72073,59.378933906555176,5.211252415772833
19019,38039,38038,76077,62.53703022003174,5.025140957832264
20020,40041,40040,80081,65.71999502182007,4.852387255838039
21021,42043,42042,84085,68.95322394371033,4.691763661241566
22022,44045,44044,88089,72.13115692138672,4.54217080665876
23023,46047,46046,92093,75.29652905464172,4.402622738787613
24024,48049,48048,96097,78.45367217063904,4.272233984846025
25025,50051,50050,100101,81.62401103973389,4.150208263214154
26026,52053,52052,104105,84.79374194145203,4.035828599335218
27027,54055,54054,108109,87.96549391746521,3.928448648466656
28028,56057,56056,112113,91.10581016540527,3.8274850593079464
29029,58059,58058,116117,94.28150796890259,3.7324107388485572
30030,60061,60060,120121,97.44615387916565,3.6427489597372187
31031,62063,62062,124125,100.64060807228088,3.5580680003768066
32032,64065,64064,128129,103.80441808700562,3.4779763806545816
33033,66067,66066,132133,106.97126603126526,3.4021189303530264
34034,68069,68068,136137,110.12469911575317,3.330173004356766
35035,70071,70070,140141,113.37465000152588,3.261845197301227
36036,72073,72072,144145,116.55617618560791,3.196868415008794
37037,74075,74074,148149,119.75825500488281,3.134999261199482
38038,76077,76076,152153,122.90700197219849,3.0760157031345443
39039,78079,78078,156157,126.14792490005493,3.019714984460734
40040,80081,80080,160161,129.35842204093933,2.9659117573555704
41041,82083,82082,164165,132.52135109901428,2.9144364094536286
42042,84085,84084,168169,135.70116806030273,2.8651335640315665
43043,86087,86086,172173,138.98321723937988,2.817860734363421
44044,88089,88088,176177,142.3063349723816,2.7724871154441644
45045,90091,90090,180181,145.49201822280884,2.728892498254936
46046,92093,92092,184185,148.72013902664185,2.686966293324076
47047,94095,94094,188189,151.9368860721588,2.646606651966067
48048,96097,96096,192193,155.15496802330017,2.6077196748356073
49049,98099,98098,196197,158.39673805236816,2.570218698523604
50050,100101,100100,200201,161.65513706207275,2.5340236520896724
51051,102103,102102,204205,165.02342104911804,2.4990604762260773
52052,104105,104104,208209,168.24806809425354,2.4652605985138507
53053,106107,106106,212213,171.52575707435608,2.4325604590794683
54054,108109,108108,216217,174.77418494224548,2.4009010814006615
55055,110111,110110,220221,177.9986071586609,2.3702276837466343
56056,112113,112112,224225,181.1837830543518,2.340489327089017
57057,114115,114114,228229,184.3813018798828,2.3116385958164756
58058,116117,116116,232233,187.56935906410217,2.283631308006079
59059,118119,118118,236237,190.80045318603516,2.256426252261008
60060,120121,120120,240241,194.0019040107727,2.229984948551646
61061,122123,122122,244245,197.1868028640747,2.2042714306189737
62062,124125,124124,248249,200.38405799865723,2.1792520479211817
63063,126127,126126,252253,203.54104709625244,2.154895285159
64064,128129,128128,256257,206.7100269794464,2.1311716044274363
65065,130131,130130,260261,209.87272906303406,2.1080532828345895
66066,132133,132132,264265,213.11961793899536,2.085514271404463
67067,134135,134134,268269,216.2877230644226,2.0635300874073437
68068,136137,136136,272273,219.8714780807495,2.0420776913888403
69069,138139,138138,276277,223.0088551044464,2.0211353821541707
70070,140141,140140,280281,226.22470808029175,2.000682700532707
71071,142143,142142,284285,229.79627203941345,1.9807003410987818
72072,144145,144144,288289,233.03378295898438,1.9611700711611775
73073,146147,146146,292293,236.3176350593567,1.9420746563246212
74074,148149,148148,296297,239.5995969772339,1.9233977920503094
75075,150151,150150,300301,242.7890968322754,1.9051240406824945
76076,152153,152152,304305,245.9729609489441,1.887238773439094
77077,154155,154154,308309,249.51617407798767,1.869728116933402
78078,156157,156156,312313,252.71622109413147,1.8525789038649236
79079,158159,158158,316317,255.89196515083313,1.835778627450054
80080,160161,160160,320321,259.04586696624756,1.8193153993506712
81081,162163,162162,324325,262.25056409835815,1.8031779107404873
82082,164165,164164,328329,265.4277548789978,1.7873553962654114
83083,166167,166166,332333,268.905779838562,1.7718376006723702
84084,168169,168168,336337,272.1653790473938,1.756614747859203
85085,170171,170170,340341,275.33785700798035,1.741677512147362
86086,172173,172172,344345,278.5904519557953,1.7270169934363366
87087,174175,174174,348349,281.7684950828552,1.7126247108662938
88088,176177,176176,352353,284.9200351238251,1.6984925117903913
89089,178179,178178,356357,288.17061018943787,1.6846126237414865
90090,180181,180180,360361,291.47307109832764,1.670977608717294
91091,182183,182182,364365,294.66961002349854,1.657580344548478
92092,184185,184184,368369,297.83230686187744,1.6444140075036557
93093,186187,186186,372373,301.0050401687622,1.6314720560567366
94094,188189,188188,376377,304.19787406921387,1.6187482157110935
95095,190191,190190,380381,307.3924241065979,1.6062364648114453
96096,192193,192192,384385,310.7349691390991,1.5939310212797864
97097,194195,194194,388389,314.0838692188263,1.5818263301625848
98098,196197,196196,392393,317.4551730155945,1.5699170520074404
99099,198199,198198,396397,320.7851400375366,1.5581980519127683
100100,200201,200200,400401,324.1468458175659,1.5466643892923457
101101,202203,202202,404405,327.50811791419983,1.535311308240125
102102,204205,204204,408409,330.83103108406067,1.5241342284916755
103103,206207,206206,412413,334.1876459121704,1.5131287369113124
104104,208209,208208,416417,337.5370988845825,1.5022905794921826
105105,210211,210210,420421,340.91296792030334,1.4916156538165524
106106,212213,212212,424425,344.2813711166382,1.4811000019744824
107107,214215,214214,428429,347.65298986434937,1.4707398038408428
108108,216217,216216,432433,351.0458869934082,1.4605313707943424
109109,218219,218218,436437,354.3879339694977,1.4504711397494248
110110,220221,220220,440441,357.73757219314575,1.4405556675119442
111111,222223,222222,444445,361.11696195602417,1.4307816254950012
112112,224225,224224,448449,364.49558115005493,1.4211457946712471
113113,226227,226226,452453,367.8432331085205,1.4116450608235027
114114,228229,228228,456457,371.33100509643555,1.4022764100354834
115115,230231,230230,460461,374.70840215682983,1.3930369244499161
116116,232233,232232,464465,378.0592701435089,1.3839237782067357
117117,234235,234234,468469,381.40681505203247,1.3749342336286645
118118,236237,236236,472473,384.76181197166443,1.3660656375814142
119119,238239,238238,476477,388.10665488243103,1.3573154180212441
120120,240241,240240,480481,391.4586720466614,1.3486810807407892
121121,242243,242242,484485,394.80032205581665,1.3401602062367601
122122,244245,244244,488489,398.1534209251404,1.3317504467686376
123123,246247,246246,492493,401.53087615966797,1.3234495235356007
124124,248249,248248,496497,404.8978831768036,1.3152552240135265
125125,250251,250250,500501,408.2493019104004,1.3071653994102235
126126,252253,252252,504505,411.6285629272461,1.2991779622261674
127127,254255,254254,508509,414.98873710632324,1.2912908839571173
128128,256257,256256,512513,418.5522770881653,1.2835021928895003
129129,258259,258258,516517,422.00322818756104,1.2758099720067548
130130,260261,260260,520521,425.4120318889618,1.2682123569720716
131131,262263,262262,524525,428.82167506217957,1.2607075342330063
132132,264265,264264,528529,432.25367283821106,1.2532937391861196
133133,266267,266266,532533,435.60822916030884,1.2459692544434802
134134,268269,268268,536537,438.95588302612305,1.2387324081482802
135135,270271,270270,540541,442.3473961353302,1.231581572406867
136136,272273,272272,544545,445.66022181510925,1.2245151617444208
137137,274275,274274,548549,449.0396149158478,1.2175316316606768
138138,276277,276276,552553,452.4190709590912,1.210629477231123
139139,278279,278278,556557,455.80640721321106,1.203807234252963
140140,280281,280280,560561,459.22365617752075,1.1970634843455628
141141,282283,282282,564565,462.57851219177246,1.1903968195019843
142142,284285,284284,568569,465.9542200565338,1.183805880296859
143143,286287,286286,572573,469.28914308547974,1.1772893407342053
144144,288289,288288,576577,472.66038608551025,1.1708459071760444
145145,290291,290290,580581,476.03202295303345,1.1644743172982999
146146,292293,292292,584585,479.38637804985046,1.1581733390994486
147147,294295,294294,588589,482.7508201599121,1.1519417699346377
148148,296297,296296,592593,486.1625039577484,1.1457784356171032
149149,298299,298298,596597,489.549467086792,1.139682189517771
150150,300301,300300,600601,492.9353940486908,1.1336519117212447
151151,302303,302302,604605,496.2657699584961,1.1276865082163567
152152,304305,304304,608609,499.63904213905334,1.1217849101067259
153153,306307,306306,612613,503.0036988258362,1.115946072854058
154154,308309,308308,616617,506.3337049484253,1.1101689755687403
155155,310311,310310,620621,509.69115591049194,1.1044526202786074
156156,312313,312312,624625,513.0185780525208,1.098796031288657
157157,314315,314314,628629,516.3923871517181,1.0931982545134815
158158,316317,316316,632633,519.7780499458313,1.0876583568588103
159159,318319,318318,636637,523.1113500595093,1.0821754256157874
160160,320321,320320,640641,526.6372430324554,1.0767485678879893
161161,322323,322322,644645,530.2866480350494,1.0713769100166246
162162,324325,324324,648649,533.878231048584,1.0660595970548457
163163,326327,326326,652653,537.6256220340729,1.060795792242061
164164,328329,328328,656657,541.4047222137451,1.0555846765000751
165165,330331,330330,660661,545.1133921146393,1.0504254479437805
166166,332333,332332,664665,548.7627398967743,1.0453173214173148
167167,334335,334334,668669,552.4034941196442,1.0402595280393143
168168,336337,336336,672673,556.0032680034637,1.0352513147627178
169169,338339,338338,676677,559.6603090763092,1.0302919439618563
170170,340341,340340,680681,563.2963900566101,1.0253806930068095
171171,342343,342342,684685,567.0131320953369,1.0205168538759608
172172,344345,344344,688689,570.6321818828583,1.015699732788562
173173,346347,346346,692693,574.2754790782928,1.010928649802736
174174,348349,348348,696697,577.9002590179443,1.0062029384862399
175175,350351,350350,700701,581.7117428779602,1.0015219455617625
176176,352353,352352,704705,585.4709711074829,0.996885030557678
177177,354355,354354,708709,589.0779950618744,0.9922915655006364
178178,356357,356356,712713,592.5787830352783,0.987740934604517
179179,358359,358358,716717,595.9621629714966,0.9832325339393719
180180,360361,360360,720721,599.3490009307861,0.9787657711694919
181181,362363,362362,724725,602.7297511100769,0.9743400652423588
182182,364365,364364,728729,606.2850348949432,0.9699548461194354
183183,366367,366366,732733,609.7261140346527,0.9656095545160497
184184,368369,368368,736737,613.0896182060242,0.9613036416285468
185185,370371,370370,740741,616.4897201061249,0.957036568885087
186186,372373,372372,744745,619.8710510730743,0.9528078077019018
187187,374375,374374,748749,623.2484550476074,0.9486168392577383
188188,376377,376376,752753,626.6407558917999,0.9444631542228308
189189,378379,378378,756757,630.0046188831329,0.9403462525897339
190190,380381,380380,760761,633.3550472259521,0.9362656434132077
191191,382383,382382,764765,636.6993730068207,0.9322208446174045
192192,384385,384384,768769,640.3359401226044,0.9282113827885041
193193,386387,386386,772773,643.7729740142822,0.9242367929746251
194194,388389,388388,776777,647.1301369667053,0.9202966184930119
195195,390391,390390,780781,650.4735469818115,0.9163904107372218
196196,392393,392392,784785,653.8405690193176,0.9125177290006832
197197,394395,394394,788789,657.2041940689087,0.9086781402911583
198198,396397,396396,792793,660.7060961723328,0.9048712191724917
199199,398399,398398,796797,664.1229629516602,0.9010965475772537
200200,400401,400400,800801,667.507698059082,0.8973537146557646
201201,402403,402402,804805,670.9252579212189,0.8936423166214809
202202,404405,404404,808809,674.2963480949402,0.8899619565836474
203203,406407,406406,812813,677.6612520217896,0.88631224439996
204204,408409,408408,816817,681.0209541320801,0.882692796538322
205205,410411,410410,820821,684.391340970993,0.8791032359258679
206206,412413,412412,824825,687.7638339996338,0.8755431918143586
207207,414415,414414,828829,691.1254751682281,0.8720122996455757
208208,416417,416416,832833,694.4621019363403,0.8685102009185357
209209,418419,418418,836837,697.8485040664673,0.8650365430548845
210210,420421,420420,840841,701.2496249675751,0.8615909792915772
211211,422423,422422,844845,704.6236679553986,0.8581731685408158
212212,424425,424424,848849,707.9734320640564,0.8547827752809098
213213,426427,426426,852853,711.3267171382904,0.8514194694416801
214214,428429,428428,856857,714.6813411712646,0.8480829262825864
215215,430431,430430,860861,718.0193269252777,0.844772826303597
216216,432433,432432,864865,721.374655008316,0.8414888551142212
217217,434435,434434,868869,724.8528828620911,0.8382307033425604
218218,436437,436436,872873,728.2444851398468,0.8349980665370822
219219,438439,438438,876877,731.6246929168701,0.831790645052024
220220,440441,440440,880881,735.2273609638214,0.828608143970996
221221,442443,442442,884885,738.6914300918579,0.8254502729978412
222222,444445,444444,888889,742.071918964386,0.8223167463711434
223223,446447,446446,892893,745.4358310699463,0.8192072827696393
224224,448449,448448,896897,748.7924220561981,0.8161216052340023
225225,450451,450450,900901,752.1633489131927,0.8130594410704362
226226,452453,452452,904905,755.5266008377075,0.8100205217797338
227227,454455,454454,908909,758.9174199104309,0.8070045829590526
228228,456457,456456,912913,762.2965738773346,0.8040113642418873
229229,458459,458458,916917,765.6575651168823,0.8010406092053017
230230,460461,460460,920921,769.0280282497406,0.798092065298988
231231,462463,462462,924925,772.4061622619629,0.7951654837706883
232232,464465,464464,928929,776.0323550701141,0.7922606196116249
233233,466467,466466,932933,779.5280990600586,0.7893772314455418
234234,468469,468468,936937,782.934005022049,0.7865150815032393
235235,470471,470470,940941,786.3252739906311,0.783673935526167
236236,472473,472472,944945,789.7139010429382,0.7808535627118545
237237,474475,474474,948949,793.0507960319519,0.7780537356538844
238238,476477,476476,952953,796.4339051246643,0.7752742302673141
239239,478479,478478,956957,799.8545939922333,0.7725148257377441
240240,480481,480480,960961,803.2699508666992,0.769775304450377
241241,482483,482482,964965,806.603226184845,0.7670554519481811
242242,484485,484484,968969,809.969969034195,0.7643550568573119
243243,486487,486486,972973,813.3335962295532,0.7616739108398178
244244,488489,488488,976977,816.7069182395935,0.7590118085390714
245245,490491,490490,980981,820.069827079773,0.7563685475179227
246246,492493,492492,984985,823.4068689346313,0.7537439282223204
247247,494495,494494,988989,826.8085732460022,0.7511377539121895
248248,496497,496496,992993,830.1401269435883,0.748549830617776
249249,498499,498498,996997,833.4972290992737,0.74597996709781
250250,500501,500500,1001001,836.8569231033325,0.7434279747849359
251251,502503,502502,1005005,840.5072209835052,0.7408936677329621
252252,504505,504504,1009009,843.9825720787048,0.7383768625822995
253253,506507,506506,1013013,847.4141201972961,0.7358773785126687
254254,508509,508508,1017017,850.7863600254059,0.7333950371867104
255255,510511,510510,1021021,854.1509220600128,0.7309296627227013
256256,512513,512512,1025025,857.5424630641937,0.728481081643622
257257,514515,514514,1029029,860.9196321964264,0.7260491228407773
258258,516517,516516,1033033,864.3220951557159,0.7236336175210454
259259,518519,518518,1037037,867.7470850944519,0.7212343991923262
260260,520521,520520,1041041,871.1157691478729,0.7188513035907818
261261,522523,522522,1045045,874.4563910961151,0.7164841686735599
262262,524525,524524,1049049,877.8185470104218,0.714132834564225
263263,526527,526526,1053053,881.2118310928345,0.7117971435236541
264264,528529,528528,1057057,884.523276090622,0.7094769399063807
265265,530531,530530,1061061,887.9046928882599,0.7071720701314916
266266,532533,532532,1065065,891.2346270084381,0.7048823826535227
267267,534535,534534,1069069,894.6149108409882,0.702607727915165
268268,536537,536536,1073073,897.9661061763763,0.7003479583236185
269269,538539,538538,1077077,901.308473110199,0.6981029282214877
270270,540541,540540,1081081,904.6992540359497,0.695872493841307
271271,542543,542542,1085085,908.2305750846863,0.6936565150772367
272272,544545,544544,1089089,911.732106924057,0.69145485284389
273273,546547,546546,1093093,915.1183550357819,0.6892673660986475
274274,548549,548548,1097097,918.6996750831604,0.6870939183736482
275275,550551,550550,1101101,922.2091271877289,0.684934374947261
276276,552553,552552,1105105,925.6223840713501,0.6827886028167995
277277,554555,554554,1109109,928.9731011390686,0.6806564706785139
278278,556557,556556,1113113,932.3276772499084,0.6785378488893912
279279,558559,558558,1117117,935.700660943985,0.6764326094489661
280280,560561,560560,1121121,939.1026139259338,0.6743406259774929
281281,562563,562562,1125125,942.4821639060974,0.6722617736741086
282282,564565,564564,1129129,945.8599548339844,0.670195929309557
283283,566567,566566,1133133,949.2152800559998,0.66814297118799
284284,568569,568568,1137137,952.6197249889374,0.6661028262296895
285285,570571,570570,1141141,956.0046892166138,0.6640753303618112
286286,572573,572572,1145145,959.3911850452423,0.6620603643441427
287287,574575,574574,1149149,962.763631105423,0.6600578124071035
288288,576577,576576,1153153,966.1357228755951,0.6580675601999246
289289,578579,578578,1157157,969.6664550304413,0.6560894947760971
290290,580581,580580,1161161,973.099356174469,0.6541235045751819
291291,582583,582582,1165165,976.526504278183,0.6521694793882489
292292,584585,584584,1169169,980.1560461521149,0.6502273103469633
293293,586587,586586,1173173,983.5919020175934,0.6482968899035768
294294,588589,588588,1177177,987.0322108268738,0.6463781118072802
295295,590591,590590,1181181,990.3867492675781,0.6444708710805571
296296,592593,592592,1185185,993.8054051399231,0.642575076311914
297297,594595,594594,1189189,997.1776139736176,0.640690647485826
298298,596597,596596,1193193,1000.591185092926,0.6388174483072362
299299,598599,598598,1197197,1003.963583946228,0.6369553787262703
300300,600601,600600,1201201,1007.3335862159729,0.6351043398735783
301301,602603,602602,1205205,1010.7249929904938,0.6332642340585153
302302,604605,604604,1209209,1014.0856392383575,0.6314349647345807
303303,606607,606606,1213213,1017.4567999839783,0.6296164364957804
304304,608609,608608,1217217,1020.8205301761627,0.6278085550547985
305305,610611,610610,1221221,1024.2042899131775,0.626011227213894
306306,612613,612612,1225225,1027.6432240009308,0.6242243608703575
307307,614615,614614,1229229,1031.0600640773773,0.6224478649855882
308308,616617,616616,1233233,1034.4196569919586,0.6206816495796375
309309,618619,618618,1237237,1037.800148010254,0.6189256257039233
310310,620621,620620,1241241,1041.2755720615387,0.6171797054375929
311311,622623,622622,1245245,1044.7565970420837,0.6154438018693327
312312,624625,624624,1249249,1048.1521210670471,0.6137178290755401
313313,626627,626626,1253253,1051.5177121162415,0.6120017021166859
314314,628629,628628,1257257,1054.9014410972595,0.6102953370227624
315315,630631,630630,1261261,1058.3065609931946,0.6085986507696362
316316,632633,632632,1265265,1061.6930689811707,0.6069115612717724
317317,634635,634634,1269269,1065.08141207695,0.6052339873767778
318318,636637,636636,1273273,1068.5339801311493,0.6035658488362969
319319,638639,638638,1277277,1071.9323508739471,0.601907066304193
320320,640641,640640,1281281,1075.285269021988,0.600257561321996
321321,642643,642642,1285285,1078.618835926056,0.598617256309808
322322,644645,644644,1289289,1082.011085987091,0.5969860745371989
323323,646647,646646,1293293,1085.4230251312256,0.5953639401413966
324324,648649,648648,1297297,1088.8410642147064,0.5937507780836313
325325,650651,650650,1301301,1092.2596819400787,0.5921465141636872
326326,652653,652652,1305305,1095.597468137741,0.59055107498898
327327,654655,654654,1309309,1098.9957301616669,0.5889643879727373
328328,656657,656656,1313313,1102.391086101532,0.5873863813285425
329329,658659,658658,1317317,1105.7198450565338,0.5858169840430492
330330,660661,660660,1321321,1109.084200143814,0.5842561258796195
331331,662663,662662,1325325,1112.4535059928894,0.5827037373655912
332332,664665,664664,1329329,1115.8434429168701,0.5811597497722687
333333,666667,666666,1333333,1119.262332201004,0.579624096817497
334334,668669,668668,1337337,1122.6017799377441,0.5780967098526162
335335,670671,670670,1341341,1125.9576160907745,0.5765775220243086
336336,672673,672672,1345345,1129.3167350292206,0.5750664675160806
337337,674675,674674,1349349,1132.7102301120758,0.5735634812099306
338338,676677,676676,1353353,1136.0885019302368,0.5720684986827109
339339,678679,678678,1357357,1139.4493429660797,0.5705814561933948
340340,680681,680680,1361361,1142.8282051086426,0.5691022906794387
341341,682683,682682,1365365,1146.2347598075867,0.5676309397367731
342342,684685,684684,1369369,1149.6499891281128,0.5661673416252597
343343,686687,686686,1373373,1153.2633850574493,0.5647114352486824
344344,688689,688688,1377377,1156.700112104416,0.5632631601565663
345345,690691,690690,1381381,1160.0933949947357,0.561822456516893
346346,692693,692692,1385385,1163.651391029358,0.5603892651361093
347347,694695,694694,1389389,1167.113940000534,0.5589635274282045
348348,696697,696696,1393393,1170.505089044571,0.5575451854147104
349349,698699,698698,1397397,1173.8741590976715,0.5561341817137873
350350,700701,700700,1401401,1177.2280750274658,0.5547304595420428
351351,702703,702702,1405405,1180.6470310688019,0.5533339626927045
352352,704705,704704,1409409,1184.025645017624,0.5519446355392574
353353,706707,706706,1413413,1187.407263994217,0.5505624230263493
354354,708709,708708,1417417,1190.9242029190063,0.5491872706552385
355355,710711,710710,1421421,1194.3252770900726,0.5478191244856134
356356,712713,712712,1425425,1197.747689962387,0.546457931124678
357357,714715,714714,1429429,1201.155117034912,0.5451036377162382
358358,716717,716716,1433433,1204.535180091858,0.5437561919443397
359359,718719,718718,1437437,1207.9677481651306,0.5424155420096213
360360,720721,720720,1441441,1211.4043881893158,0.5410816366511426
361361,722723,722722,1445445,1214.7837669849396,0.5397544251045474
362362,724725,724724,1449449,1218.1864140033722,0.5384338571184344
363363,726727,726726,1453453,1221.5774099826813,0.5371198829452624
364364,728729,728728,1457457,1224.936005115509,0.5358124533304363
365365,730731,730730,1461461,1228.3306999206543,0.5345115195086692
366366,732733,732732,1465465,1231.7320351600647,0.5332170331967063
367367,734735,734734,1469469,1235.1118111610413,0.5319289465933252
368368,736737,736736,1473473,1238.5176088809967,0.5306472123538697
369369,738739,738738,1477477,1241.9018650054932,0.5293717836175347
370370,740741,740740,1481481,1245.311653137207,0.5281026139691676
371371,742743,742742,1485485,1248.7815110683441,0.5268396574556391
372372,744745,744744,1489489,1252.2536931037903,0.5255828685676533
373373,746747,746746,1493493,1255.6491861343384,0.5243322022361099
374374,748749,748748,1497497,1258.9972231388092,0.5230876138375606
375375,750751,750750,1501501,1262.3740680217743,0.5218490591742011
376376,752753,752752,1505505,1265.7638750076294,0.5206164944756893
377377,754755,754754,1509509,1269.1721048355103,0.5193898763991456
378378,756757,756756,1513513,1272.6650390625,0.5181691620091442
379379,758759,758758,1517517,1276.0815060138702,0.5169543087922648
380380,760761,760760,1521521,1279.4894251823425,0.5157452746316267
381381,762763,762762,1525525,1282.8786540031433,0.5145420178196218
382382,764765,764764,1529529,1286.265172958374,0.5133444970433629
383383,766767,766766,1533533,1289.6290171146393,0.5121526713846833
384384,768769,768768,1537537,1293.0072009563446,0.5109665003074042
385385,770771,770770,1541541,1296.3908989429474,0.5097859436627914
386386,772773,772772,1545545,1299.7843210697174,0.5086109616822796
387387,774775,774774,1549549,1303.1494460105896,0.5074415149701963
388388,776777,776776,1553553,1306.5282800197601,0.5062775644964859
389389,778779,778778,1557557,1309.9305529594421,0.5051190716003475
390390,780781,780780,1561561,1313.298245191574,0.5039659979847784
391391,782783,782782,1565565,1316.6457741260529,0.5028183057038405
392392,784785,784784,1569569,1320.0241179466248,0.5016759571699367
393393,786787,786786,1573573,1323.3949010372162,0.5005389151428972
394394,788789,788788,1577577,1326.8907070159912,0.4994071427208837
395395,790791,790790,1581581,1330.2834889888763,0.4982806033567613
396396,792793,792792,1585585,1333.6571769714355,0.4971592608235369
397397,794795,794794,1589589,1337.079801082611,0.4960430792380066
398398,796797,796796,1593593,1340.4579050540924,0.49493202304438455
399399,798799,798798,1597597,1343.820692062378,0.49382605701430293
400400,800801,800800,1601601,1347.1832721233368,0.49272514623226016
401401,802803,802802,1605605,1350.5456838607788,0.49162925610653474
402402,804805,804804,1609609,1353.9066090583801,0.49053835236372834
403403,806807,806806,1613613,1357.3299131393433,0.4894524010378518
404404,808809,808808,1617617,1360.708335161209,0.48837136846850626
405405,810811,810810,1621621,1364.08145403862,0.487295221297245
406406,812813,812812,1625625,1367.4637911319733,0.4862239264712116
407407,814815,814814,1629629,1370.8378620147705,0.48515745123586385
408408,816817,816816,1633633,1374.2190399169922,0.4840957631222409
409409,818819,818818,1637637,1377.5917942523956,0.48303882995787717
410410,820821,820820,1641641,1380.9593279361725,0.4819866198595264
411411,822823,822822,1645645,1384.3283610343933,0.4809391012222477
412412,824825,824824,1649649,1387.7027230262756,0.47989624272122455
413413,826827,826826,1653653,1391.1043419837952,0.4788580133172218
414414,828829,828828,1657657,1394.5759179592133,0.47782438223657664
415415,830831,830830,1661661,1398.1670560836792,0.47679531898756977
416416,832833,832832,1665665,1401.5765590667725,0.4757707933349593
417417,834835,834834,1669669,1404.94952917099,0.47475077531998977
418418,836837,836836,1673673,1408.333503961563,0.4737352352367452
419419,838839,838838,1677677,1411.88250207901,0.4727241436503391
420420,840841,840840,1681681,1415.2967541217804,0.47171747137326747
421421,842843,842842,1685685,1418.6966540813446,0.47071518947632285
422422,844845,844844,1689689,1422.0706779956818,0.4697172692813183
423423,846847,846846,1693693,1425.4447238445282,0.4687236823610874
424424,848849,848848,1697697,1428.8106470108032,0.4677344005303894
425425,850851,850850,1701701,1432.3180830478668,0.466749395849547
426426,852853,852852,1705705,1435.74964594841,0.4657686406208086
427427,854855,854854,1709709,1439.1310300827026,0.4647921073847101
428428,856857,856856,1713713,1442.5005822181702,0.4638197689109802
429429,858859,858858,1717717,1445.8947441577911,0.4628515982112731
430430,860861,860860,1721721,1449.3246488571167,0.46188756852461665
431431,862863,862862,1725725,1452.665402173996,0.4609276533155935
432432,864865,864864,1729729,1456.1401541233063,0.45997182627615985
433433,866867,866866,1733733,1459.7335422039032,0.45902006132564566
434434,868869,868868,1737737,1463.0926389694214,0.4580723325998406
435435,870871,870870,1741741,1466.4601788520813,0.45712861445099406
436436,872873,872872,1745745,1469.8692269325256,0.4561888814550912
437437,874875,874874,1749749,1473.2491850852966,0.45525310839548183
438438,876877,876876,1753753,1476.621304988861,0.45432127027197566
439439,878879,878878,1757757,1480.016680240631,0.4533933422899281
440440,880881,880880,1761761,1483.3832612037659,0.4524692998602404
441441,882883,882882,1765765,1486.7476551532745,0.4515491186102736
442442,884885,884884,1769769,1490.132167816162,0.45063277436020144
443443,886887,886886,1773773,1493.510525226593,0.4497202431321057
444444,888889,888888,1777777,1496.8557019233704,0.4488115011517948
445445,890891,890890,1781781,1500.2177908420563,0.4479065248378902
446446,892893,892892,1785785,1503.599837064743,0.44700529080182605
447447,894895,894894,1789789,1506.9877400398254,0.4461077758551255
448448,896897,896896,1793793,1510.3705899715424,0.44521395699484856
449449,898899,898898,1797797,1513.742301940918,0.4443238114090491
450450,900901,900900,1801801,1517.3394010066986,0.44343731646586093
451451,902903,902902,1805805,1520.8537871837616,0.44255444973350677
452452,904905,904904,1809809,1524.2098789215088,0.4416751889493753
453453,906907,906906,1813813,1527.5746638774872,0.4407995120345731
454454,908909,908908,1817817,1530.9773349761963,0.4399273970957438
455455,910911,910910,1821821,1534.3181371688843,0.43905882241051586
456456,912913,912912,1825825,1537.693589925766,0.4381937664365978
457457,914915,914914,1829829,1541.1089782714844,0.4373322078045021
458458,916917,916916,1833833,1544.4412100315094,0.43647412531572627
459459,918919,918918,1837837,1547.7976701259613,0.43561949794639077
460460,920921,920920,1841841,1551.3545660972595,0.43476830483268714
461461,922923,922922,1845845,1554.7896182537079,0.4339205252890679
462462,924925,924924,1849849,1558.1657631397247,0.4330761387864186
463463,926927,926926,1853853,1561.5341351032257,0.4322351249647909
464464,928929,928928,1857857,1564.9183349609375,0.4313974636261264
465465,930931,930930,1861861,1568.3503921031952,0.43056313472698093
466466,932933,932932,1865865,1571.7117512226105,0.4297321183948952
467467,934935,934934,1869869,1575.0979239940643,0.4289043948992912
468468,936937,936936,1873873,1578.5756721496582,0.4280799446769379
469469,938939,938938,1877877,1581.9469921588898,0.4272587483173993
470470,940941,940940,1881881,1585.3254890441895,0.42644078655757767
471471,942943,942942,1885885,1588.688971042633,0.4256260402926273
472472,944945,944944,1889889,1592.0791511535645,0.42481449056140264
473473,946947,946946,1893893,1595.430163860321,0.42400611855555326
474474,948949,948948,1897897,1598.8222980499268,0.4232009056122479
475475,950951,950950,1901901,1602.2013220787048,0.4223988332123554
476476,952953,952952,1905905,1605.5527811050415,0.4215998829822638
477477,954955,954954,1909909,1608.9235849380493,0.42080403669388033
478478,956957,956956,1913913,1612.2911150455475,0.42001127625553636
479479,958959,958958,1917917,1615.7177629470825,0.41922158371380647
480480,960961,960960,1921921,1619.217199087143,0.4184349477854994
481481,962963,962962,1925925,1622.626827955246,0.41765134872730414
482482,964965,964964,1929929,1625.9582540988922,0.416870764514897
483483,966967,966966,1933933,1629.4169840812683,0.4160931777423684
484484,968969,968968,1937937,1632.787768125534,0.41531857114023296
485485,970971,970970,1941941,1636.1376218795776,0.41454692757179146
486486,972973,972972,1945945,1639.5582990646362,0.413778230025855
487487,974975,974974,1949949,1642.981761932373,0.4130124616294779
488488,976977,976976,1953953,1646.4137270450592,0.41224960563158675
489489,978979,978978,1957957,1649.7780630588531,0.41148964540661837
490490,980981,980980,1961961,1653.1470499038696,0.41073256446361484
491491,982983,982982,1965965,1656.556146144867,0.40997834642803355
492492,984985,984984,1969969,1659.9266090393066,0.40922697505084216
493493,986987,986986,1973973,1663.2873899936676,0.4084784342085186
494494,988989,988988,1977977,1666.666246175766,0.4077327078957751
495495,990991,990990,1981981,1670.05025100708,0.4069897802291962
496496,992993,992992,1985985,1673.4470179080963,0.40624963543996273
497497,994995,994994,1989989,1677.0118010044098,0.40551225788294687
498498,996997,996996,1993993,1680.4127180576324,0.4047776320276171
499499,998999,998998,1997997,1683.7947421073914,0.40404574245985714
500501,1001003,1001002,2002005,1687.1817910671234,0.40331584678824584
501502,1003005,1003004,2006009,1690.5530202388763,0.4025893866964907
502503,1005007,1005006,2010013,1693.931361913681,0.4018656173157069
503504,1007009,1007008,2014017,1697.275573015213,0.4011445236774307
504505,1009011,1009010,2018021,1700.7595779895782,0.40042609093325154
505506,1011013,1011012,2022025,1704.159070968628,0.39971030433662236
506507,1013015,1013014,2026029,1707.5012340545654,0.3989971492537734
507508,1015017,1015016,2030033,1710.8516750335693,0.39828661115825525
508509,1017019,1017018,2034037,1714.2338600158691,0.397578675627301
509510,1019021,1019020,2038041,1717.5996358394623,0.39687332834910194
510511,1021023,1021022,2042045,1720.9947061538696,0.39617055510643695
511512,1023025,1023024,2046049,1724.4365780353546,0.39547034179668117
512513,1025027,1025026,2050053,1727.8214619159698,0.3947726744117972
513514,1027029,1027028,2054057,1731.1880459785461,0.39407753904743004
514515,1029031,1029030,2058061,1734.5438680648804,0.39338492190472607
515516,1031033,1031032,2062065,1737.890098810196,0.39269480927941913
516517,1033035,1033034,2066069,1741.23983502388,0.3920071875636495
517518,1035037,1035036,2070073,1744.6083459854126,0.3913220432586968
518519,1037039,1037038,2074077,1748.0133900642395,0.3906393629476952
519520,1039041,1039040,2078081,1751.3971590995789,0.3899591333247372
520521,1041043,1041042,2082085,1754.7799479961395,0.3892813411694078
521522,1043045,1043044,2086089,1758.1474349498749,0.3886059733613365
522523,1045047,1045046,2090093,1761.508173942566,0.38793301686928316
523524,1047049,1047048,2094097,1764.895262002945,0.38726245875841414
524525,1049051,1049050,2098101,1768.2391290664673,0.38659428618302627
525526,1051053,1051052,2102105,1771.6108231544495,0.3859284863956418
526527,1053055,1053054,2106109,1775.0224702358246,0.38526504672881856
527528,1055057,1055056,2110113,1778.4600219726562,0.38460395461333974
528529,1057059,1057058,2114117,1781.8041641712189,0.38394519756548107
529530,1059061,1059060,2118121,1785.1538980007172,0.3832887631870108
530531,1061063,1061062,2122125,1788.4889421463013,0.38263463917064655
531532,1063065,1063064,2126129,1791.859111070633,0.3819828132964176
532533,1065067,1065066,2130133,1795.2098460197449,0.3813332734280266
533534,1067069,1067068,2134137,1798.5597059726715,0.38068600751103077
534535,1069071,1069070,2138141,1801.920240163803,0.3800410035819368
535536,1071073,1071072,2142145,1805.2724740505219,0.379398249757287
536537,1073075,1073074,2146149,1808.8733191490173,0.378757734237297
537538,1075077,1075076,2150153,1812.2304000854492,0.3781194453022181
538539,1077079,1077078,2154157,1815.5827980041504,0.3774833713177941
539540,1079081,1079080,2158161,1818.9522202014923,0.3768495007225283
540541,1081083,1081082,2162165,1822.3107991218567,0.37621782204405463
541542,1083085,1083084,2166169,1825.6728081703186,0.3755883238845854
542543,1085087,1085086,2170173,1829.034420967102,0.3749609949281876
543544,1087089,1087088,2174177,1832.3787188529968,0.37433582393168763
544545,1089091,1089090,2178181,1835.7401220798492,0.3737127997319476
545546,1091093,1091092,2182185,1839.1343200206757,0.37309191124404606
546547,1093095,1093094,2186189,1842.5074679851532,0.3724731474540022
547548,1095097,1095096,2190193,1845.8994369506836,0.3718564974333276
548549,1097099,1097098,2194197,1849.2351830005646,0.37124195031537965
549550,1099101,1099100,2198201,1852.5999548435211,0.37062949531537015
550551,1101103,1101102,2202205,1856.098776102066,0.3700191217194515
551552,1103105,1103104,2206209,1859.6253590583801,0.3694108188901737
552553,1105107,1105106,2210213,1863.234887123108,0.36880457625738927
553554,1107109,1107108,2214217,1866.7449898719788,0.3682003833237104
554555,1109111,1109110,2218221,1870.1096940040588,0.36759822966450884
555556,1111113,1111112,2222225,1873.4557139873505,0.3669981049224589
556557,1113115,1113114,2226229,1876.8299272060394,0.36639999881299445
557558,1115117,1115116,2230233,1880.2174680233002,0.36580390112067107
558559,1117119,1117118,2234237,1883.6823971271515,0.36520980169734685
559560,1119121,1119120,2238241,1887.0877480506897,0.3646176904621825
560561,1121123,1121122,2242245,1890.4485051631927,0.3640275574016414
561562,1123125,1123124,2246249,1893.791172027588,0.3634393925731274
562563,1125127,1125126,2250253,1897.1706840991974,0.3628531860958901
563564,1127129,1127128,2254257,1900.5642449855804,0.3622689281583007
564565,1129131,1129130,2258261,1903.9287440776825,0.3616866090105759
565566,1131133,1131132,2262265,1907.2722401618958,0.3611062189684162
566567,1133135,1133134,2266269,1910.6520040035248,0.3605277484111866
567568,1135137,1135136,2270273,1914.0281131267548,0.3599511877873738
568569,1137139,1137138,2274277,1917.3933959007263,0.359376527603672
569570,1139141,1139140,2278281,1920.7192702293396,0.35880375842680223
570571,1141143,1141142,2282285,1924.134595155716,0.358232870892607
571572,1143145,1143144,2286289,1927.5581622123718,0.3576638556914986
572573,1145147,1145146,2290293,1930.923723936081,0.35709670357937284
573574,1147149,1147148,2294297,1934.2613968849182,0.3565314053739712
574575,1149151,1149150,2298301,1937.639820098877,0.3559679519457859
575576,1151153,1151152,2302305,1941.0033469200134,0.3554063342326117
576577,1153155,1153154,2306309,1944.3695652484894,0.35484654323227005
577578,1155157,1155156,2310313,1947.7161540985107,0.35428856998805713
578579,1157159,1157158,2314317,1951.0659592151642,0.35373240562148567
579580,1159161,1159160,2318321,1954.4286110401154,0.35317804129226715
580581,1161163,1161162,2322325,1957.7855741977692,0.3526254682274157
581582,1163165,1163164,2326329,1961.1701180934906,0.35207467771215306
582583,1165167,1165166,2330333,1964.5303490161896,0.3515256610880897
583584,1167169,1167168,2334337,1967.9034061431885,0.35097840974231076
584585,1169171,1169170,2338341,1971.279303073883,0.35043291512920405
585586,1171173,1171172,2342345,1974.6387860774994,0.34988916875227005
586587,1173175,1173174,2346349,1978.0740330219269,0.34934716216957895
587588,1175177,1175176,2350353,1981.588702917099,0.34880688699922757
588589,1177179,1177178,2354357,1984.9506101608276,0.3482683349029685
589590,1179181,1179180,2358361,1988.397912979126,0.3477314976043999
590591,1181183,1181182,2362365,1991.7318680286407,0.3471963668744138
591592,1183185,1183184,2366369,1995.0759191513062,0.3466629345421097
592593,1185187,1185186,2370373,1998.445270061493,0.34613119247842405
593594,1187189,1187188,2374377,2001.792839050293,0.3456011326161388
594595,1189191,1189190,2378381,2005.227833032608,0.3450727469371486
595596,1191193,1191192,2382385,2008.6343100070953,0.344546027468823
596597,1193195,1193194,2386389,2011.9763250350952,0.34402096629492007
597598,1195197,1195196,2390393,2015.3509600162506,0.34349755554467265
598599,1197199,1197198,2394397,2018.731775045395,0.3429757873964263
599600,1199201,1199200,2398401,2022.1155200004578,0.3424556540867343
600601,1201203,1201202,2402405,2025.4644401073456,0.3419371478885296
601602,1203205,1203204,2406409,2028.8533251285553,0.3414202611293149
602603,1205207,1205206,2410413,2032.3412871360779,0.34090498618570564
603604,1207209,1207208,2414417,2035.984040260315,0.34039131547979196
604605,1209211,1209210,2418421,2039.3360719680786,0.3398792414791387
605606,1211213,1211212,2422425,2042.8997418880463,0.33936875670224254
606607,1213215,1213214,2426429,2046.400285243988,0.3388598537130747
607608,1215217,1215216,2430433,2049.9058690071106,0.3383525251192623
608609,1217219,1217218,2434437,2053.5013670921326,0.33784676358118304
609610,1219221,1219220,2438441,2056.9407448768616,0.33734256179377553
610611,1221223,1221222,2442445,2060.284926891327,0.336839912501091
611612,1223225,1223224,2446449,2063.6505908966064,0.33633880850356945
612613,1225227,1225226,2450453,2067.0431730747223,0.33583924262529763
613614,1227229,1227228,2454457,2070.412915945053,0.335341207754027
614615,1229231,1229230,2458461,2073.779750108719,0.3348446968066128
615616,1231233,1231232,2462465,2077.14878988266,0.334349702749023
616617,1233235,1233234,2466469,2080.555762052536,0.3338562185981573
617618,1235237,1235236,2470473,2083.9463160037994,0.3333642374000192
618619,1237239,1237238,2474477,2087.267650127411,0.33287375224790594
619620,1239241,1239240,2478481,2090.6233110427856,0.3323847562824085
620621,1241243,1241242,2482485,2093.9820070266724,0.3318972426804976
621622,1243245,1243244,2486489,2097.339067220688,0.3314112046627997
622623,1245247,1245246,2490493,2100.678771018982,0.33092663548995915
623624,1247249,1247248,2494497,2104.021341085434,0.3304435284644569
624625,1249251,1249250,2498501,2107.419296979904,0.32996187692697276
625626,1251253,1251252,2502505,2110.7946910858154,0.32948167426366126
626627,1253255,1253254,2506509,2114.139986038208,0.32900291388978076
627628,1255257,1255256,2510513,2117.4896681308746,0.32852558927879727
628629,1257259,1257258,2514517,2121.024085044861,0.3280496939241857
629630,1259261,1259260,2518521,2124.465791940689,0.3275752213667147
630631,1261263,1261262,2522525,2127.860044002533,0.3271021651908086
631632,1263265,1263264,2526529,2131.213238954544,0.3266305190118146
632633,1265267,1265266,2530533,2134.566848039627,0.3261602764832787
633634,1267269,1267268,2534537,2137.8767850399017,0.3256914313042216
634635,1269271,1269270,2538541,2141.266860961914,0.32522397720276786
635636,1271273,1271272,2542545,2144.640009880066,0.3247579079470597
636637,1273275,1273274,2546549,2148.1144580841064,0.3242932173452573
637638,1275277,1275276,2550553,2151.4587371349335,0.32382989924008143
638639,1277279,1277278,2554557,2154.801856994629,0.3233679475088138
639640,1279281,1279280,2558561,2158.328602075577,0.32290735606875387
640641,1281283,1281282,2562565,2161.8712430000305,0.3224481188735808
641642,1283285,1283284,2566569,2165.250603914261,0.32199022990425874
642643,1285287,1285286,2570573,2168.695286989212,0.3215336831872264
643644,1287289,1287288,2574577,2172.0821759700775,0.32107847278166446
644645,1289291,1289290,2578581,2175.410719871521,0.3206245927776763
645646,1291293,1291292,2582585,2178.8270609378815,0.32017203730538313
646647,1293295,1293294,2586589,2182.17210316658,0.319720800522191
647648,1295297,1295296,2590593,2185.5873651504517,0.31927087662734266
648649,1297299,1297298,2594597,2188.9961841106415,0.31882225985100376
649650,1299301,1299300,2598601,2192.333983898163,0.3183749444579007
650651,1301303,1301302,2602605,2195.665757894516,0.31792892474004475
651652,1303305,1303304,2606609,2199.08566904068,0.3174841950312839
652653,1305307,1305306,2610613,2202.4744679927826,0.31704074969638896
653654,1307309,1307308,2614617,2205.8266520500183,0.3165985831274156
654655,1309311,1309310,2618621,2209.205556869507,0.3161576897564373
655656,1311313,1311312,2622625,2212.557543039322,0.31571806404099334
656657,1313315,1313314,2626629,2215.9236381053925,0.31527970047318377
657658,1315317,1315316,2630633,2219.254872083664,0.3148425935814885
658659,1317319,1317318,2634637,2222.6059839725494,0.3144067379180342
659660,1319321,1319320,2638641,2226.013684988022,0.31397212807314645
660661,1321323,1321322,2642645,2229.454020023346,0.3135387586626166
661662,1323325,1323324,2646649,2232.8413190841675,0.3131066243367968
662663,1325327,1325326,2650653,2236.157840013504,0.3126757197751431
663664,1327329,1327328,2654657,2239.506791114807,0.3122460396916722
664665,1329331,1329330,2658661,2242.912905931473,0.31181757882040984
665666,1331333,1331332,2662665,2246.2385201454163,0.31139033193539944
666667,1333335,1333334,2666669,2249.7143778800964,0.3109642938379693
667668,1335337,1335336,2670673,2253.204118013382,0.31053945935491356
668669,1337339,1337338,2674677,2256.5722510814667,0.31011582334940613
669670,1339341,1339340,2678681,2259.972468852997,0.3096933807100868
670671,1341343,1341342,2682685,2263.3332200050354,0.30927212634924217
671672,1343345,1343344,2686689,2266.697729110718,0.3088520552173577
672673,1345347,1345346,2690693,2270.0625789165497,0.30843316229038464
673674,1347349,1347348,2694697,2273.423803091049,0.3080154425679211
674675,1349351,1349350,2698701,2276.9188120365143,0.3075988910823071
675676,1351353,1351352,2702705,2280.2916688919067,0.3071835028949863
676677,1353355,1353354,2706709,2283.6352281570435,0.3067692730928684
677678,1355357,1355356,2710713,2287.0023560523987,0.3063561967865098
678679,1357359,1357358,2714717,2290.52419090271,0.3059442691210279
679680,1359361,1359360,2718721,2293.896686077118,0.30553348526336777
680681,1361363,1361362,2722725,2297.2694520950317,0.3051238404150354
681682,1363365,1363364,2726729,2300.633684873581,0.3047153297939076
682683,1365367,1365366,2730733,2303.9877190589905,0.30430794865242206
683684,1367369,1367368,2734737,2307.3513741493225,0.3039016922630253
684685,1369371,1369370,2738741,2310.707309961319,0.3034965559345437
685686,1371373,1371372,2742745,2314.0936958789825,0.3030925349867175
686687,1373375,1373374,2746749,2317.4495549201965,0.3026896247829427
687688,1375377,1375376,2750753,2320.869183063507,0.30228782069752924
688689,1377379,1377378,2754757,2324.212774038315,0.3018871181375289
689690,1379381,1379380,2758761,2327.5507140159607,0.30148751253182127
690691,1381383,1381382,2762765,2330.93310213089,0.30108899934020883
691692,1383385,1383384,2766769,2334.2760100364685,0.3006915740443219
692693,1385387,1385386,2770773,2337.6308290958405,0.3002952321457997
693694,1387389,1387388,2774777,2340.991136074066,0.2998999691753852
694695,1389391,1389390,2778781,2344.3373968601227,0.2995057806947443
695696,1391393,1391392,2782785,2347.712677001953,0.29911266227645683
696697,1393395,1393394,2786789,2351.0798461437225,0.2987206095276633
697698,1395397,1395396,2790793,2354.4177589416504,0.2983296180755133
698699,1397399,1397398,2794797,2357.7702808380127,0.297939683572622
699700,1399401,1399400,2798801,2361.131005048752,0.29755080169161374
700701,1401403,1401402,2802805,2364.4767541885376,0.2971629681360355
701702,1403405,1403404,2806809,2367.8547780513763,0.2967761786221672
702703,1405407,1405406,2810813,2371.204808950424,0.2963904288972117
703704,1407409,1407408,2814817,2374.5740809440613,0.2960057147338375
704705,1409411,1409410,2818821,2377.9120790958405,0.2956220319174463
705706,1411413,1411412,2822825,2381.3382320404053,0.29523937626800034
706707,1413415,1413414,2826829,2384.7183549404144,0.29485774361819495
707708,1415417,1415416,2830833,2388.0639169216156,0.29447712982619123
708709,1417419,1417418,2834837,2391.651927947998,0.29409753077925416
709710,1419421,1419420,2838841,2395.1327199935913,0.29371894237192464
710711,1421423,1421422,2842845,2398.5071761608124,0.29334136054058035
711712,1423425,1423424,2846849,2402.081199169159,0.29296478122341796
712713,1425427,1425426,2850853,2405.6084489822388,0.2925892003950139
713714,1427429,1427428,2854857,2409.0300059318542,0.29221461404631555
714715,1429431,1429430,2858861,2412.392151117325,0.28934317169296264
715716,1431433,1431432,2862865,2415.7891709804535,0.2889771243899304
716717,1433435,1433434,2866869,2419.216155052185,0.28861203355882026
717718,1435437,1435436,2870873,2422.610813856125,0.2882478954070393
718719,1437439,1437438,2874877,2425.969412088394,0.2878847061692795
719720,1439441,1439440,2878881,2429.3452010154724,0.2875224620984227
720721,1441443,1441442,2882885,2432.717878103256,0.28716115946917853
721722,1443445,1443444,2886889,2436.090409040451,0.28680079457262764
722723,1445447,1445446,2890893,2439.503361940384,0.2864413637216785
723724,1447449,1447448,2894897,2442.898943901062,0.28608286325106747
724725,1449451,1449450,2898901,2446.271213054657,0.28572528950462583
725726,1451453,1451452,2902905,2449.633125066757,0.2853686388571077
726727,1453455,1453454,2906909,2453.0142681598663,0.2850129076978192
727728,1455457,1455456,2910913,2456.3657462596893,0.2846580924306181
728729,1457459,1457458,2914917,2459.7601788043976,0.2843041894848284
729730,1459461,1459460,2918921,2463.1284441947937,0.28395119530432567
730731,1461463,1461462,2922925,2466.490084171295,0.28359910635481356
731732,1463465,1463464,2926929,2470.0240280628204,0.2832479191110906
732733,1465467,1465466,2930933,2473.6027760505676,0.28289763007705915
733734,1467469,1467468,2934937,2476.9943709373474,0.2825482357711735
734735,1469471,1469470,2938941,2480.340672016144,0.2821997327300778
735736,1471473,1471472,2942945,2483.7059800624847,0.2818521175049682
736737,1473475,1473474,2946949,2487.084962129593,0.2815053866652306
737738,1475477,1475476,2950953,2490.4406900405884,0.2811595368057169
738739,1477479,1477478,2954957,2493.7940349578857,0.2808145645303739
739740,1479481,1479480,2958961,2497.1569719314575,0.2804704664613382
740741,1481483,1481482,2962965,2500.5731461048126,0.28012723924075544
741742,1483485,1483484,2966969,2503.946943998337,0.27978487952896103
742743,1485487,1485486,2970973,2507.2911059856415,0.27944338399902335
743744,1487489,1487488,2974977,2510.685173034668,0.2791027493458387
744745,1489491,1489490,2978981,2514.080318927765,0.27876297227703617
745746,1491493,1491492,2982985,2517.6956651210785,0.2784240495184349
746747,1493495,1493494,2986989,2521.1871070861816,0.27808597781586286
747748,1495497,1495496,2990993,2524.6107420921326,0.2777487539242429
748749,1497499,1497498,2994997,2527.9800980091095,0.27741237462396384
749750,1499501,1499500,2999001,2531.3771991729736,0.27707683670269034
750751,1501503,1501502,3003005,2534.7858860492706,0.276742136971734
751752,1503505,1503504,3007009,2538.16086602211,0.2764082722533203
752753,1505507,1505506,3011013,2541.553727865219,0.2760752393896837
753754,1507509,1507508,3015017,2545.0043001174927,0.27574303523942945
754755,1509511,1509510,3019021,2548.383980035782,0.27541165666480083
755756,1511513,1511512,3023025,2552.0661318302155,0.2750811005662399
756757,1513515,1513514,3027029,2555.7843730449677,0.27475136384236976
757758,1515517,1515516,3031033,2559.533720970154,0.2744224434118223
758759,1517519,1517518,3035037,2563.157033920288,0.27409433620778145
759760,1519521,1519520,3039041,2566.7588169574738,0.27376703918162093
760761,1521523,1521522,3043045,2570.3411650657654,0.2734405493010854
761762,1523525,1523524,3047049,2573.9864749908447,0.2731148635430145
762763,1525527,1525526,3051053,2577.5588459968567,0.2727899789042567
763764,1527529,1527528,3055057,2581.1544020175934,0.27246589239439345
764765,1529531,1529530,3059061,2584.8474581241608,0.27214260103937704
765766,1531533,1531532,3063065,2588.482245206833,0.27182010187789274
766767,1533535,1533534,3067069,2592.0653080940247,0.2714983919668157
767768,1535537,1535536,3071073,2595.622400045395,0.271177468372116
768769,1537539,1537538,3075077,2599.2273259162903,0.2708573281815916
769770,1539541,1539540,3079081,2602.817052125931,0.2705379684921354
770771,1541543,1541542,3083085,2606.3905210494995,0.2702193864133733
771772,1543545,1543544,3087089,2609.959550857544,0.2699015790785779
772773,1545547,1545546,3091093,2613.535094022751,0.269584543622841
773774,1547549,1547548,3095097,2617.1148788928986,0.26926827719944413
774775,1549551,1549550,3099101,2620.513969182968,0.2689527769853157
775776,1551553,1551552,3103105,2624.1668961048126,0.26863804015920323
776777,1553555,1553554,3107109,2627.6366720199585,0.268324063912587
777778,1555557,1555556,3111113,2631.012889146805,0.26801084546423226
778779,1557559,1557558,3115117,2634.414423942566,0.2676983820329042
779780,1559561,1559560,3119121,2637.798586130142,0.26738667086101486
780781,1561563,1561562,3123125,2641.1510379314423,0.2670757091946143
781782,1563565,1563564,3127129,2644.6304800510406,0.2667654943015805
782783,1565567,1565566,3131133,2648.093371152878,0.2664560234588862
783784,1567569,1567568,3135137,2651.4855558872223,0.26614729395623726
784785,1569571,1569570,3139141,2654.877767801285,0.2658393030978914
785786,1571573,1571572,3143145,2658.2160880565643,0.26553204820629617
786787,1573575,1573574,3147149,2661.5844221115112,0.2652255266020802
787788,1575577,1575576,3151153,2664.9734477996826,0.26491973563861393
788789,1577579,1577578,3155157,2668.321923971176,0.26461467266562977
789790,1579581,1579580,3159161,2671.6683492660522,0.26431033505286905
790791,1581583,1581582,3163165,2675.041624069214,0.264006720186444
791792,1583585,1583584,3167169,2678.453145980835,0.26370382545064786
792793,1585587,1585586,3171173,2681.886066198349,0.26340164826251566
793794,1587589,1587588,3175177,2685.2425808906555,0.2631001860390825
794795,1589591,1589590,3179181,2688.6257140636444,0.2627994362064783
795796,1591593,1591592,3183185,2691.992795228958,0.26249939621447993
796797,1593595,1593594,3187189,2695.3476898670197,0.2622000635146833
797798,1595597,1595596,3191193,2698.742287158966,0.26190143557869305
798799,1597599,1597598,3195197,2702.1220898628235,0.26160350988175196
799800,1599601,1599600,3199201,2705.5115308761597,0.26130628392274957
800801,1601603,1601602,3203205,2709.114045858383,0.26100975520239444
801802,1603605,1603604,3207209,2712.5057520866394,0.26071392123776604
802803,1605607,1605606,3211213,2715.9632561206818,0.26041877955867676
803804,1607609,1607608,3215217,2719.510101079941,0.26012432770039595
804805,1609611,1609610,3219221,2722.8868222236633,0.25983056321638287
805806,1611613,1611612,3223225,2726.254946947098,0.2595374836728297
806807,1613615,1613614,3227229,2729.62198805809,0.2592450866395666
807808,1615617,1615616,3231233,2732.9595189094543,0.2589533697046136
808809,1617619,1617618,3235237,2736.3227529525757,0.25866233046872367
809810,1619621,1619620,3239241,2739.7530510425568,0.2583719665362878
810811,1621623,1621622,3243245,2743.119817018509,0.25808227552624885
811812,1623625,1623624,3247249,2746.495525121689,0.2577932550721016
812813,1625627,1625626,3251253,2749.864701271057,0.25750490282007377
813814,1627629,1627628,3255257,2753.2695829868317,0.25721721641457407
814815,1629631,1629630,3259261,2756.6644401550293,0.25693019353093405
815816,1631633,1631632,3263265,2760.0347290039062,0.2566438318353903
816817,1633635,1633634,3267269,2763.4291739463806,0.2563581290178263
817818,1635637,1635636,3271273,2766.778920173645,0.2560730827790394
818819,1637639,1637638,3275277,2770.243138074875,0.25578869081800804
819820,1639641,1639640,3279281,2773.596997022629,0.25550495085917646
820821,1641643,1641642,3283285,2776.974799156189,0.2552218606324459
821822,1643645,1643644,3287289,2780.536544084549,0.2549394178768125
822823,1645647,1645646,3291293,2784.2056272029877,0.25465762033854844
823824,1647649,1647648,3295297,2787.771963119507,0.2543764657857537
824825,1649651,1649650,3299301,2791.3208181858063,0.25409595198107127
825826,1651653,1651652,3303305,2794.877569913864,0.2538160767107911
826827,1653655,1653654,3307309,2798.4840519428253,0.25353683776666003
827828,1655657,1655656,3311313,2802.053514957428,0.2532582329495199
828829,1657659,1657658,3315317,2805.7568719387054,0.2529802600693074
829830,1659661,1659660,3319321,2809.335478067398,0.25270291695233027
830831,1661663,1661662,3323325,2812.935727119446,0.2524262014285341
831832,1663665,1663664,3327329,2816.4685518741608,0.2521501113387785
832833,1665667,1665666,3331333,2820.0489361286163,0.251874644536656
833834,1667669,1667668,3335337,2823.6223850250244,0.25159979888485395
834835,1669671,1669670,3339341,2827.18758392334,0.25132557224969787
835836,1671673,1671672,3343345,2830.84211397171,0.251051962522979
836837,1673675,1673674,3347349,2834.39319896698,0.2507789675855747
837838,1675677,1675676,3351353,2837.9633798599243,0.2505065853438282
838839,1677679,1677678,3355357,2841.5120120048523,0.2502348137059016
839840,1679681,1679680,3359361,2845.074695110321,0.24996365058905212
840841,1681683,1681682,3363365,2848.455286026001,0.24969309393054573
841842,1683685,1683684,3367369,2851.840231180191,0.24942314166401047
842843,1685687,1685686,3371373,2855.2074699401855,0.24915379173216934
843844,1687689,1687688,3375377,2858.903932094574,0.24888504210321116
844845,1689691,1689690,3379381,2862.35196518898,0.2486168907398678
845846,1691693,1691692,3383385,2865.7138521671295,0.24834933561214712
846847,1693695,1693694,3387389,2869.087804079056,0.24808237471188477
847848,1695697,1695696,3391393,2872.4946789741516,0.24781600603091647
848849,1697699,1697698,3395397,2875.876361846924,0.24755022757381084
849850,1699701,1699700,3399401,2879.227727174759,0.24728503735241247
850851,1701703,1701702,3403405,2882.6669738292694,0.2470204333840229
851852,1703705,1703704,3407409,2886.10262799263,0.2467564137041336
852853,1705707,1705706,3411413,2889.508544921875,0.24649297634823597
853854,1707709,1707708,3415417,2892.8544108867645,0.2462301193663734
854855,1709711,1709710,3419421,2896.2153131961823,0.24596784081222722
855856,1711713,1711712,3423425,2899.5756368637085,0.2457061387522117
856857,1713715,1713714,3427429,2902.9609389305115,0.24544501126001705
857858,1715717,1715716,3431433,2906.4732961654663,0.24518445642206643
858859,1717719,1717718,3435437,2910.158936023712,0.244924472322964
859860,1719721,1719720,3439441,2913.565801858902,0.2446650570655038
860861,1721723,1721722,3443445,2916.9705350399017,0.24440620875611785
861862,1723725,1723724,3447449,2920.649252176285,0.24414792551579012
862863,1725727,1725726,3451453,2924.299450159073,0.24389020546186657
863864,1727729,1727728,3455457,2927.7765159606934,0.24363304673534003
864865,1729731,1729730,3459461,2931.1547708511353,0.24337644746992737
865866,1731733,1731732,3463465,2934.577708005905,0.24312040582117334
866867,1733735,1733734,3467469,2938.113774061203,0.24286491994280368
867868,1735737,1735736,3471473,2941.6182289123535,0.24260998800673406
868869,1737739,1737738,3475477,2944.964996099472,0.24235560818124213
869870,1739741,1739740,3479481,2948.381824016571,0.2421017786473385
870871,1741743,1741742,3483485,2951.7802770137787,0.2418484976005857
871872,1743745,1743744,3487489,2955.1686398983,0.2415957632347272
872873,1745747,1745746,3491493,2958.513554096222,0.24134357376169646
873874,1747749,1747748,3495497,2961.9157350063324,0.24109192738433194
874875,1749751,1749750,3499501,2965.2595829963684,0.24084082233639492
875876,1751753,1751752,3503505,2968.6483080387115,0.24059025684255175
876877,1753755,1753754,3507509,2972.0087530612946,0.24034022913474473
877878,1755757,1755756,3511513,2975.343014240265,0.24009073746674403
878879,1757759,1757758,3515517,2978.744162082672,0.23984178008504387
879880,1759761,1759760,3519521,2982.1257650852203,0.23959335525432834
880881,1761763,1761762,3523525,2985.4951322078705,0.23934546123928158
881882,1763765,1763764,3527529,2988.860116004944,0.2390980963155016
882883,1765767,1765766,3531533,2992.2203409671783,0.23885125876950042
883884,1767769,1767768,3535537,2995.6163198947906,0.238604946885971
884885,1769771,1769770,3539541,2999.009019136429,0.23835915896779625
885886,1771773,1771772,3543545,3002.3643629550934,0.23811389331785904
886887,1773775,1773774,3547549,3005.7057461738586,0.23786914824631822
887888,1775777,1775776,3551553,3009.138664960861,0.23762492207788455
888889,1777779,1777778,3555557,3012.528477191925,0.2373812131354498
889890,1779781,1779780,3559561,3015.891725063324,0.23713801975463866
890891,1781783,1781782,3563565,3019.220498085022,0.2368953402765328
891892,1783785,1783784,3567569,3022.587347984314,0.23665317305312783
892893,1785787,1785786,3571573,3025.9815311431885,0.23641151643641933
893894,1787789,1787788,3575577,3029.3529160022736,0.23617036878931685
894895,1789791,1789790,3579581,3032.712224960327,0.23592972848200588
895896,1791793,1791792,3583585,3036.057865858078,0.23568959389194788
896897,1793795,1793794,3587589,3039.463362932205,0.23544996340569924
897898,1795797,1795796,3591593,3042.8477540016174,0.23521083540799737
898899,1797799,1797798,3595597,3046.3736460208893,0.23497220830176957
899900,1799801,1799800,3599601,3049.8093209266663,0.23473408048630517
900901,1801803,1801802,3603605,3053.1747801303864,0.2344964503772644
901902,1803805,1803804,3607609,3056.5394620895386,0.2342593163903075
902903,1805807,1805806,3611613,3059.944967985153,0.23402267695018963
903904,1807809,1807808,3615617,3063.2847821712494,0.23378653048894193
904905,1809811,1809810,3619621,3066.6354229450226,0.2335508754476905
905906,1811813,1811812,3623625,3070.1548578739166,0.2333157102639234
906907,1813815,1813814,3627629,3073.540121078491,0.23308103339695663
907908,1815817,1815816,3631633,3076.9200870990753,0.2328468432988302
908909,1817819,1817818,3635637,3080.251261949539,0.23261313843613607
909910,1819821,1819820,3639641,3083.6423161029816,0.2323799172809231
910911,1821823,1821822,3643645,3087.1383221149445,0.2321471783088782
911912,1823825,1823824,3647649,3090.7086141109467,0.2319149200029642
912913,1825827,1825826,3651653,3094.0689730644226,0.2316831408552389
913914,1827829,1827828,3655657,3097.4375212192535,0.23145183936139802
914915,1829831,1829830,3659661,3100.83478808403,0.2312210140262323
915916,1831833,1831832,3663665,3104.2272429466248,0.23099066335817042
916917,1833835,1833834,3667669,3107.609139919281,0.23076078586927906
917918,1835837,1835836,3671673,3110.962013244629,0.23053138008253882
918919,1837839,1837838,3675677,3114.331378221512,0.23030244452638726
919920,1839841,1839840,3679681,3117.9142651557922,0.23007397773835692
920921,1841843,1841842,3683685,3121.3513531684875,0.2298459782541613
921922,1843845,1843844,3687689,3124.7688291072845,0.2296184446204279
922923,1845847,1845846,3691693,3128.118273973465,0.22939137538924115
923924,1847849,1847848,3695697,3131.5618538856506,0.2291647691217804
924925,1849851,1849850,3699701,3134.918431997299,0.22893862437740609
925926,1851853,1851852,3703705,3138.370385169983,0.22871293973184947
926927,1853855,1853854,3707709,3141.775608062744,0.2284877137572039
927928,1855857,1855856,3711713,3145.139678955078,0.22826294504011457
928929,1857859,1857858,3715717,3148.491338968277,0.22803863216358877
929930,1859861,1859860,3719721,3151.94731426239,0.22781477372336667
930931,1861863,1861862,3723725,3155.3844521045685,0.22759136831700744
931932,1863865,1863864,3727729,3158.8422582149506,0.22736841455662216
932933,1865867,1865866,3731733,3162.407623052597,0.22714591104522697
933934,1867869,1867868,3735737,3165.8304691314697,0.2269238564040279
934935,1869871,1869870,3739741,3169.202308177948,0.22670224925604998
935936,1871873,1871872,3743745,3172.5799281597137,0.2264810882279562
936937,1873875,1873874,3747749,3175.9571919441223,0.22626037195368554
937938,1875877,1875876,3751753,3179.3137781620026,0.2260400990726339
938939,1877879,1877878,3755757,3182.6905930042267,0.22582026823147316
939940,1879881,1879880,3759761,3186.057844877243,0.22560087807869422
940941,1881883,1881882,3763765,3189.4725620746613,0.22538192727370188
941942,1883885,1883884,3767769,3192.829383134842,0.22516341447590094
942943,1885887,1885886,3771773,3196.190205812454,0.22494533835197217
943944,1887889,1887888,3775777,3199.5729641914368,0.2247276975758723
944945,1889891,1889890,3779781,3202.9171121120453,0.22451049082519603
945946,1891893,1891892,3783785,3206.2884800434113,0.22429371678299503
946947,1893895,1893894,3787789,3209.6302630901337,0.22407737413777795
947948,1895897,1895896,3791793,3213.1376209259033,0.2238614615835104
948949,1897899,1897898,3795797,3216.5382339954376,0.22364597782143392
949950,1899901,1899900,3799801,3219.885540008545,0.2234309215509711
950951,1901903,1901902,3803805,3223.2454750537872,0.22321629148791544
951952,1903905,1903904,3807809,3226.6568369865417,0.2230020863498794
952953,1905907,1905906,3811813,3230.033149957657,0.22278830484719947
953954,1907909,1907908,3815817,3233.4755251407623,0.22257494571204006
954955,1909911,1909910,3819821,3236.980283021927,0.22236200767656555
955956,1911913,1911912,3823825,3240.3493859767914,0.22214948947112134
956957,1913915,1913914,3827829,3243.696568965912,0.22193738983878575
957958,1915917,1915916,3831833,3247.0573019981384,0.22172570752627507
958959,1917919,1917918,3835837,3250.4922029972076,0.2215144412857626
959960,1919921,1919920,3839841,3253.862202167511,0.22130358987305954
960961,1921923,1921922,3843845,3257.199594974518,0.22109315204397717
961962,1923925,1923924,3847849,3260.647348880768,0.22088312656887865
962963,1925927,1925926,3851853,3264.041425228119,0.22067351221812714
963964,1927929,1927928,3855857,3267.3921089172363,0.22046430776936177
964965,1929931,1929930,3859861,3270.7364590168,0.22025551200022164
965966,1931933,1931932,3863865,3274.103410243988,0.22004712369744084
966967,1933935,1933934,3867869,3277.4797308444977,0.2198391416513914
967968,1935937,1935936,3871873,3280.911952018738,0.21963156465790235
968969,1937939,1937938,3875877,3284.2707710266113,0.21942439151644066
969970,1939941,1939940,3879881,3287.655741214752,0.21921762103011133
970971,1941943,1941942,3883885,3291.02024102211,0.21901125200929528
971972,1943945,1943944,3887889,3294.388871908188,0.2188052832698304
972973,1945947,1945946,3891893,3297.903604030609,0.21859971363119257
973974,1947949,1947948,3895897,3301.3627030849457,0.21839454191285768
974975,1949951,1949950,3899901,3304.72096991539,0.2181897669488535
975976,1951953,1951952,3903905,3308.1044149398804,0.21798538756956987
976977,1953955,1953954,3907909,3311.5009689331055,0.21778140261085355
977978,1955957,1955956,3911913,3314.882644891739,0.21757781091582729
978979,1957959,1957958,3915917,3318.2991049289703,0.2173746113312518
979980,1959961,1959960,3919921,3321.702966928482,0.21717180270934477
980981,1961963,1961962,3923925,3325.0656559467316,0.2169693839041429
981982,1963965,1963964,3927929,3328.4125230312347,0.21676735377877776
982983,1965967,1965966,3931933,3331.7745089530945,0.21656571119274304
983984,1967969,1967968,3935937,3335.1324331760406,0.21636445502190327
984985,1969971,1969970,3939941,3338.50740814209,0.21616358413666603
985986,1971973,1971972,3943945,3341.8888082504272,0.21596309741289588
986987,1973975,1973974,3947949,3345.242119073868,0.21576299373191432
987988,1975977,1975976,3951953,3348.6237099170685,0.2155632719877758
988989,1977979,1977978,3955957,3351.9927201271057,0.21536393106725882
989990,1979981,1979980,3959961,3355.4347681999207,0.2151649698644178
990991,1981983,1981982,3963965,3359.0268342494965,0.21496638727876416
991992,1983985,1983984,3967969,3362.434376001358,0.21476818222072325
992993,1985987,1985986,3971973,3365.8001849651337,0.21457035358980647
993994,1987989,1987988,3975977,3369.1948342323303,0.21437290030553413
994995,1989991,1989990,3979981,3372.5652000904083,0.21417582128196955
995996,1991993,1991992,3983985,3375.9365379810333,0.21397911543499504
996997,1993995,1993994,3987989,3379.316915035248,0.2137827816986828
997998,1995997,1995996,3991993,3382.652661085129,0.21358681899619114
998999,1997999,1997998,3995997,3385.994081020355,0.21339122626341123
1000000,2000001,2000000,4000001,3389.333256006241,0.21319600243805326


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0027458667755126953,12064.709122577777
1001,2003,2002,4005,3.6115479469299316,65.54308581374062
2002,4005,4004,8009,7.196931838989258,42.36125675350013
3003,6007,6006,12013,10.735725164413452,34.03888935166469
4004,8009,8008,16017,14.49898099899292,28.9736744604088
5005,10011,10010,20021,18.256932020187378,25.347796528210893
6006,12013,12012,24025,22.094247102737427,22.541154451162583
7007,14015,14014,28029,25.44001603126526,20.266618657631625
8008,16017,16016,32033,28.789549827575684,18.369066826699054
9009,18019,18018,36037,32.211326122283936,16.75518334221306
10010,20021,20020,40041,35.59293293952942,15.363866328221775
11011,22023,22022,44045,39.035109996795654,14.152344435575287
12012,24025,24024,48049,42.55358123779297,13.089117171617545
13013,26027,26026,52053,46.08311414718628,12.150095046214119
14014,28029,28028,56057,49.516438007354736,11.316336767915345
15015,30031,30030,60061,52.99904203414917,10.572633315323401
16016,32033,32032,64065,56.371178150177,9.906575041453834
17017,34035,34034,68069,59.71449899673462,9.30790492201595
18018,36037,36036,72073,63.01842379570007,8.768053615920508
19019,38039,38038,76077,66.41734886169434,8.279796333541526
20020,40041,40040,80081,69.74904108047485,7.83699363989399
21021,42043,42042,84085,73.06229400634766,7.434391921489805
22022,44045,44044,88089,76.45601320266724,7.0674677593142405
23023,46047,46046,92093,79.86075496673584,6.732304990688135
24024,48049,48048,96097,83.18646001815796,6.425496532749094
25025,50051,50050,100101,86.52707099914551,6.144065203598075
26026,52053,52052,104105,89.86694502830505,5.885399280419733
27027,54055,54054,108109,93.20168399810791,5.647199603103218
28028,56057,56056,112113,96.58000111579895,5.42743580638853
29029,58059,58058,116117,99.95947599411011,5.224309832568906
30030,60061,60060,120121,103.30021214485168,5.036225299478247
31031,62063,62062,124125,106.6273250579834,4.861761615753494
32032,64065,64064,128129,109.949383020401,4.699651975070083
33033,66067,66066,132133,113.29242396354675,4.5487645438679465
34034,68069,68068,136137,116.62531900405884,4.408086297122281
35035,70071,70070,140141,119.94893288612366,4.276709065070463
36036,72073,72072,144145,123.2637460231781,4.153817437863836
37037,74075,74074,148149,126.88334703445435,4.038678240984154
38038,76077,76076,152153,130.3403868675232,3.9306313461856917
39039,78079,78078,156157,133.66798901557922,3.829081623838647
40040,80081,80080,160161,137.01576709747314,3.7334918754459068
41041,82083,82082,164165,140.35639786720276,3.643376690981313
42042,84085,84084,168169,143.7153570652008,3.5582967863683734
43043,86087,86086,172173,147.20238590240479,3.4778541834857606
44044,88089,88088,176177,150.5920910835266,3.4016880430081073
45045,90091,90090,180181,153.91083407402039,3.3294707772256515
46046,92093,92092,184185,157.3594582080841,3.2609046608413337
47047,94095,94094,188189,160.69124603271484,3.1957188153337484
48048,96097,96096,192193,164.0047812461853,3.1336665222806914
49049,98099,98098,196197,167.33908200263977,3.0745228269388463
50050,100101,100100,200201,170.66259479522705,3.018082398313709
51051,102103,102102,204205,173.99177503585815,2.96415761627577
52052,104105,104104,208209,177.49394011497498,2.912576859982437
53053,106107,106106,212213,180.93330693244934,2.8631829749247117
54054,108109,108108,216217,184.28635001182556,2.8158318987552775
55055,110111,110110,220221,187.62109899520874,2.7703914283592894
56056,112113,112112,224225,190.93987202644348,2.726740112721018
57057,114115,114114,228229,194.25598120689392,2.6847662579166354
58058,116117,116116,232233,197.5934500694275,2.6443670321714308
59059,118119,118118,236237,201.05178713798523,2.6054476602639625
60060,120121,120120,240241,204.36580300331116,2.5679206978093134
61061,122123,122122,244245,207.69349694252014,2.531705376924947
62062,124125,124124,248249,210.9986629486084,2.4967270159067994
63063,126127,126126,252253,214.33691000938416,2.462916486127142
64064,128129,128128,256257,217.92963314056396,2.430209730318893
65065,130131,130130,260261,221.2511329650879,2.3985473269094655
66066,132133,132132,264265,224.5895709991455,2.3678740957093396
67067,134135,134134,268269,227.93601894378662,2.338138740768045
68068,136137,136136,272273,231.25413584709167,2.309293526604961
69069,138139,138138,276277,234.591126203537,2.281293984502554
70070,140141,140140,280281,237.9416139125824,2.2540986458207044
71071,142143,142142,284285,241.27411484718323,2.227668799694584
72072,144145,144144,288289,244.57360291481018,2.2019682726804604
73073,146147,146146,292293,247.926029920578,2.1769632282048406
74074,148149,148148,296297,251.27779006958008,2.15262198390883
75075,150151,150150,300301,254.58129906654358,2.1289148527066573
76076,152153,152152,304305,257.9308590888977,2.1058139750857663
77077,154155,154154,308309,261.25280117988586,2.0832931818367797
78078,156157,156156,312313,264.592472076416,2.061327881379839
79079,158159,158158,316317,268.0914239883423,2.039894936457131
80080,160161,160160,320321,271.58864402770996,2.018972557998495
81081,162163,162162,324325,274.91818499565125,1.998540207881888
82082,164165,164164,328329,278.2998969554901,1.9785785097737971
83083,166167,166166,332333,281.6118631362915,1.9590691673110996
84084,168169,168168,336337,284.9523799419403,1.9399948889404186
85085,170171,170170,340341,288.28871297836304,1.9213393188474583
86086,172173,172172,344345,291.6226840019226,1.9030869733906002
87087,174175,174174,348349,294.9464840888977,1.8852231825749186
88088,176177,176176,352353,298.2528610229492,1.8677340361209644
89089,178179,178178,356357,301.5746760368347,1.8506063337190426
90090,180181,180180,360361,304.8728840351105,1.8338275390888157
91091,182183,182182,364365,308.23843908309937,1.817385737575023
92092,184185,184184,368369,311.5676119327545,1.8012695968864136
93093,186187,186186,372373,314.8887288570404,1.785468330806907
94094,188189,188188,376377,318.22092604637146,1.7699716655552038
95095,190191,190190,380381,321.6007330417633,1.7547698086145829
96096,192193,192192,384385,325.2059290409088,1.739853419818246
97097,194195,194194,388389,328.62334394454956,1.7252135934522812
98098,196197,196196,392393,331.9477400779724,1.7108418227326183
99099,198199,198198,396397,335.30570101737976,1.6967299528078001
100100,200201,200200,400401,338.6727252006531,1.6828702026996325
101101,202203,202202,404405,341.98027205467224,1.669255127055294
102102,204205,204204,408409,345.3311839103699,1.6558775974026503
103103,206207,206206,412413,348.69270610809326,1.642730784647938
104104,208209,208208,416417,352.08227491378784,1.6298081427630677
105105,210211,210210,420421,355.4292480945587,1.6171033935170271
106106,212213,212212,424425,358.74741411209106,1.6046105122277368
107107,214215,214214,428429,362.11046409606934,1.59232371440703
108108,216217,216216,432433,365.4399619102478,1.5802374432769284
109109,218219,218218,436437,368.7953109741211,1.5683463580535317
110110,220221,220220,440441,372.1017942428589,1.556645322982149
111111,222223,222222,444445,375.4348828792572,1.5451293970290862
112112,224225,224224,448449,378.8297791481018,1.533793824222812
113113,226227,226226,452453,382.1812801361084,1.5226340245644678
114114,228229,228228,456457,385.5349860191345,1.5116455854858941
115115,230231,230230,460461,388.8596041202545,1.5008242538187915
116116,232233,232232,464465,392.1724669933319,1.490165928233182
117117,234235,234234,468469,395.7134358882904,1.479666652103333
118118,236237,236236,472473,399.17777705192566,1.4693226068011427
119119,238239,238238,476477,402.5410759449005,1.4591301053660573
120120,240241,240240,480481,405.878201007843,1.4490855865096819
121121,242243,242242,484485,409.20735001564026,1.4391856089932844
122122,244245,244244,488489,412.55543780326843,1.4294268462854234
123123,246247,246246,492493,415.8822720050812,1.4198060815215285
124124,248249,248248,496497,419.19719314575195,1.4103202027345105
125125,250251,250250,500501,422.6311550140381,1.4009661983382102
126126,252253,252252,504505,426.11056113243103,1.3917411528709636
127127,254255,254254,508509,429.5118041038513,1.3826422429174272
128128,256257,256256,512513,432.86035418510437,1.3736667332977959
129129,258259,258258,516517,436.1562850475311,1.3648119734116335
130130,260261,260260,520521,439.476930141449,1.3560753937872505
131131,262263,262262,524525,443.0320370197296,1.3474545027966087
132132,264265,264264,528529,446.453556060791,1.3389468835503067
133133,266267,266266,532533,449.80646896362305,1.3305501909198938
134134,268269,268268,536537,453.10089087486267,1.3222621487366268
135135,270271,270270,540541,456.54367899894714,1.3140805471084605
136136,272273,272272,544545,459.9613130092621,1.306003239860729
137137,274275,274274,548549,463.29757595062256,1.298028142120529
138138,276277,276276,552553,466.65905809402466,1.2901532279938692
139139,278279,278278,556557,469.9887840747833,1.2823765283756074
140140,280281,280280,560561,473.3273561000824,1.2746961288285092
141141,282283,282282,564565,476.66826915740967,1.2671101675914542
142142,284285,284284,568569,480.01656103134155,1.2596168336549454
143143,286287,286286,572573,483.364511013031,1.2522143649566715
144144,288289,288288,576577,486.73221802711487,1.2449010466061736
145145,290291,290290,580581,490.1623661518097,1.2376752092404786
146146,292293,292292,584585,493.6927111148834,1.2305352274124743
147147,294295,294294,588589,496.9171669483185,1.2234795180866058
148148,296297,296296,592593,500.12242698669434,1.2165065391636745
149149,298299,298298,596597,503.3312110900879,1.2096147880965873
150150,300301,300300,600601,506.55142307281494,1.2028028043223458
151151,302303,302302,604605,509.74848794937134,1.1960691691729153
152152,304305,304304,608609,512.9500560760498,1.1894124782338622
153153,306307,306306,612613,516.4713459014893,1.1828313743353647
154154,308309,308308,616617,519.7609858512878,1.1763245337078843
155155,310311,310310,620621,523.055046081543,1.1698906649071432
156156,312313,312312,624625,526.2859840393066,1.1635285077663866
157157,314315,314314,628629,529.5528709888458,1.157236832412309
158158,316317,316316,632633,532.7953858375549,1.1510144383028091
159159,318319,318318,636637,536.0421772003174,1.1448601533138572
160160,320321,320320,640641,539.3095922470093,1.1387728328445519
161161,322323,322322,644645,542.549586057663,1.1327513589876617
162162,324325,324324,648649,545.8652429580688,1.1267946397001651
163163,326327,326326,652653,549.1072850227356,1.1209016080265428
164164,328329,328328,656657,552.3695530891418,1.1150712213402585
165165,330331,330330,660661,555.5514221191406,1.1093024606143445
166166,332333,332332,664665,558.7142670154572,1.1035943297374615
167167,334335,334334,668669,561.8681931495667,1.097945854824502
168168,336337,336336,672673,565.0409061908722,1.0923560835744865
169169,338339,338338,676677,568.2156939506531,1.0868240846521076
170170,340341,340340,680681,571.3433890342712,1.081348947069273
171171,342343,342342,684685,574.474879026413,1.0759297796266765
172172,344345,344344,688689,577.7494280338287,1.0705657103389967
173173,346347,346346,692693,580.9045510292053,1.0652558858946577
174174,348349,348348,696697,584.0928280353546,1.0599994711446925
175175,350351,350350,700701,587.446527004242,1.0547956485916075
176176,352353,352352,704705,590.6675798892975,1.0496436179073498
177177,354355,354354,708709,593.8532218933105,1.0445425954712846
178178,356357,356356,712713,597.040491104126,1.039491813895438
179179,358359,358358,716717,600.2323830127716,1.0344905216134066
180180,360361,360360,720721,603.40469622612,1.0295379824492557
181181,362363,362362,724725,606.5847351551056,1.0246334751936956
182182,364365,364364,728729,609.7925200462341,1.0197762932348269
183183,366367,366366,732733,613.0582580566406,1.014965744156143
184184,368369,368368,736737,616.3752660751343,1.0102011493727332
185185,370371,370370,740741,619.5536730289459,1.005481843776579
186186,372373,372372,744745,622.7067139148712,1.0008071753909462
187187,374375,374374,748749,625.838446855545,0.9961765050302347
188188,376377,376376,752753,629.0214080810547,0.9915892059816542
189189,378379,378378,756757,632.3122670650482,0.9870446636869019
190190,380381,380380,760761,635.5990869998932,0.9825422754347528
191191,382383,382382,764765,638.8089511394501,0.9780814500791166
192192,384385,384384,768769,642.5077829360962,0.9736616077352664
193193,386387,386386,772773,645.7466490268707,0.9692821795251803
194194,388389,388388,776777,648.9055140018463,0.9649426072846836
195195,390391,390390,780781,652.6495079994202,0.9606423433233431
196196,392393,392392,784785,655.7805562019348,0.9563808501588937
197197,394395,394394,788789,658.9455320835114,0.9521576002844085
198198,396397,396396,792793,662.1219940185547,0.9479720759136399
199199,398399,398398,796797,665.3484590053558,0.9438237687681976
200200,400401,400400,800801,668.5847098827362,0.9397121798483568
201201,402403,402402,804805,671.998370885849,0.9356368192056834
202202,404405,404404,808809,675.6364891529083,0.9315972057484032
203203,406407,406406,812813,679.2813808917999,0.9275928670176654
204204,408409,408408,816817,682.8770830631256,0.923623339014739
205205,410411,410410,820821,686.5120389461517,0.9196881659772771
206206,412413,412412,824825,690.1731789112091,0.9157869002174266
207207,414415,414414,828829,693.7825491428375,0.9119191019217396
208208,416417,416416,832833,697.4097290039062,0.9080843389820075
209209,418419,418418,836837,701.0849230289459,0.9042821868206374
210210,420421,420420,840841,704.7403750419617,0.900512228228763
211211,422423,422422,844845,708.2710890769958,0.8967740531879826
212212,424425,424424,848849,711.6555879116058,0.8930672587339359
213213,426427,426426,852853,715.0450599193573,0.8893914487725851
214214,428429,428428,856857,718.4124600887299,0.8857462339674385
215215,430431,430430,860861,721.7871551513672,0.8821312315576506
216216,432433,432432,864865,725.2795331478119,0.8785460652397887
217217,434435,434434,868869,728.7489638328552,0.8749903650132183
218218,436437,436436,872873,732.162034034729,0.8714637670618686
219219,438439,438438,876877,735.5371630191803,0.8679659136068949
220220,440441,440440,880881,738.9014959335327,0.864496452788444
221221,442443,442442,884885,742.3597829341888,0.8610550385401439
222222,444445,444444,888889,745.7370221614838,0.8576413304654125
223223,446447,446446,892893,749.1372859477997,0.8542549937228614
224224,448449,448448,896897,752.6482629776001,0.8508956989026046
225225,450451,450450,900901,756.0742311477661,0.8475631219280331
226226,452453,452452,904905,759.5109450817108,0.8442569439303043
227227,454455,454454,908909,762.9657161235809,0.8409768511610309
228228,456457,456456,912913,766.3406639099121,0.8377225348667707
229229,458459,458458,916917,769.7556009292603,0.8344936912017147
230230,460461,460460,920921,773.1973671913147,0.8312900211312808
231231,462463,462462,924925,776.5642919540405,0.8281112303247937
232232,464465,464464,928929,779.9815609455109,0.8249570290663542
233233,466467,466466,932933,783.4262778759003,0.8218271321657085
234234,468469,468468,936937,786.8488590717316,0.8187212588654802
235235,470471,470470,940941,790.271586894989,0.8156391327556776
236236,472473,472472,944945,793.6467130184174,0.81258048169002
237237,474475,474474,948949,797.0499222278595,0.8095450376949884
238238,476477,476476,952953,800.4667541980743,0.8065325369007041
239239,478479,478478,956957,803.9899048805237,0.8035427194517979
240240,480481,480480,960961,807.4905638694763,0.8005753294364695
241241,482483,482482,964965,810.8975381851196,0.7976301148009952
242242,484485,484484,968969,814.2920110225677,0.7947068272915203
243243,486487,486486,972973,817.7078800201416,0.7918052223703853
244244,488489,488488,976977,821.1208200454712,0.7889250591488235
245245,490491,490490,980981,824.4939091205597,0.7860661003123823
246246,492493,492492,984985,827.8624970912933,0.7832281120736297
247247,494495,494494,988989,831.3651919364929,0.7804108640757477
248248,496497,496496,992993,834.8811340332031,0.7776141293597902
249249,498499,498498,996997,838.3510000705719,0.7748376842810103
250250,500501,500500,1001001,841.9991068840027,0.7720813084488327
251251,502503,502502,1005005,845.4920961856842,0.7693447846813797
252252,504505,504504,1009009,848.8632941246033,0.7666278989308921
253253,506507,506506,1013013,852.2363610267639,0.763930440236436
254254,508509,508508,1017017,855.6353099346161,0.7612522006638756
255255,510511,510510,1021021,859.0238389968872,0.7585929752513039
256256,512513,512512,1025025,862.389769077301,0.7559525619562919
257257,514515,514514,1029029,866.0402891635895,0.7533307616049569
258258,516517,516516,1033033,869.4684629440308,0.7507273778392118
259259,518519,518518,1037037,872.8657150268555,0.7481422170640144
260260,520521,520520,1041041,876.2912058830261,0.7455750883982546
261261,522523,522522,1045045,879.7592189311981,0.7430258036383748
262262,524525,524524,1049049,883.134360074997,0.7404941771965241
263263,526527,526526,1053053,886.511265039444,0.7379800260605407
264264,528529,528528,1057057,889.960294008255,0.7354831697502959
265265,530531,530530,1061061,893.6581389904022,0.7330034302722197
266266,532533,532532,1065065,897.2671382427216,0.7305406320756447
267267,534535,534534,1069069,900.6978042125702,0.7280946020146075
268268,536537,536536,1073073,904.0962510108948,0.7256651692987361
269269,538539,538538,1077077,907.5549640655518,0.723252165458689
270270,540541,540540,1081081,910.9708528518677,0.7208554243061371
271271,542543,542542,1085085,914.3955221176147,0.7184747819010227
272272,544545,544544,1089089,917.840667963028,0.7161100764933508
273273,546547,546546,1093093,921.2866830825806,0.7137611485068192
274274,548549,548548,1097097,924.6662180423737,0.711427840495162
275275,550551,550550,1101101,928.0584621429443,0.7091099971075892
276276,552553,552552,1105105,931.504096031189,0.7068074650469498
277277,554555,554554,1109109,934.9576258659363,0.7045200930479041
278278,556557,556556,1113113,938.3366038799286,0.7022477318314486
279279,558559,558558,1117117,941.7191770076752,0.6999902340776316
280280,560561,560560,1121121,945.0752568244934,0.697747454396449
281281,562563,562562,1125125,948.4369850158691,0.6955192492878268
282282,564565,564564,1129129,951.7694611549377,0.6933054793025804
283283,566567,566566,1133133,955.1079289913177,0.691106004809626
284284,568569,568568,1137137,958.4317462444305,0.6889206854284566
285285,570571,570570,1141141,961.8354041576385,0.6867493849331368
286286,572573,572572,1145145,965.1882529258728,0.6845919688494178
287287,574575,574574,1149149,968.5334990024567,0.68244830441472
288288,576577,576576,1153153,971.9027719497681,0.6803182605690381
289289,578579,578578,1157157,975.2426450252533,0.6782017078985518
290290,580581,580580,1161161,978.568706035614,0.6760985186410835
291291,582583,582582,1165165,981.9179878234863,0.6740085666351661
292292,584585,584584,1169169,985.235239982605,0.6719317273091292
293293,586587,586586,1173173,988.5746409893036,0.6698678776519955
294294,588589,588588,1177177,991.9277892112732,0.6678168983071373
295295,590591,590590,1181181,995.3125970363617,0.6657787141703011
296296,592593,592592,1185185,998.7930729389191,0.6637531594824395
297297,594595,594594,1189189,1002.3182020187378,0.6617401172316022
298298,596597,596596,1193193,1005.7436108589172,0.6597394718501164
299299,598599,598598,1197197,1009.0787000656128,0.657751109196397
300300,600601,600600,1201201,1012.4099810123444,0.6557749165203859
301301,602603,602602,1205205,1015.7497491836548,0.6538107824580948
302302,604605,604604,1209209,1019.2070200443268,0.6518585969934065
303303,606607,606606,1213213,1022.6190841197968,0.6499182514544373
304304,608609,608608,1217217,1026.019133090973,0.6479896384771564
305305,610611,610610,1221221,1029.344228029251,0.6460726519944728
306306,612613,612612,1225225,1032.7197000980377,0.644167187219864
307307,614615,614614,1229229,1036.0940589904785,0.6422731568873132
308308,616617,616616,1233233,1039.5050129890442,0.640390473196021
309309,618619,618618,1237237,1043.018481016159,0.6385190040255111
310310,620621,620620,1241241,1046.3672170639038,0.6366586494896183
311311,622623,622622,1245245,1049.7305731773376,0.6348093108972535
312312,624625,624624,1249249,1053.0961339473724,0.6329708907196618
313313,626627,626626,1253253,1056.4675650596619,0.6311432925867848
314314,628629,628628,1257257,1059.874668121338,0.6293264212454233
315315,630631,630630,1261261,1063.2511188983917,0.6275201825737895
316316,632633,632632,1265265,1066.580050945282,0.6257244835323945
317317,634635,634634,1269269,1069.9690079689026,0.6239392321804189
318318,636637,636636,1273273,1073.3535199165344,0.6221643376284192
319319,638639,638638,1277277,1076.7227339744568,0.6203997100510605
320320,640641,640640,1281281,1080.0645530223846,0.6186452606507373
321321,642643,642642,1285285,1083.3890488147736,0.6169009016557538
322322,644645,644644,1289289,1086.766359090805,0.6151665462966776
323323,646647,646646,1293293,1090.1095099449158,0.6134421088008821
324324,648649,648648,1297297,1093.5041711330414,0.6117275043689006
325325,650651,650650,1301301,1096.87619805336,0.6100226491689682
326326,652653,652652,1305305,1100.248962879181,0.6083274603170139
327327,654655,654654,1309309,1103.6225020885468,0.606641855865746
328328,656657,656656,1313313,1106.965805053711,0.6049657547991956
329329,658659,658658,1317317,1110.3094611167908,0.6032990769963362
330330,660661,660660,1321321,1113.660024881363,0.6016417432419985
331331,662663,662662,1325325,1117.216826915741,0.5999936752177746
332332,664665,664664,1329329,1120.5926520824432,0.5983547954583628
333333,666667,666666,1333333,1123.954663991928,0.5967250273733953
334334,668669,668668,1337337,1127.2945129871368,0.5951042952128773
335335,670671,670670,1341341,1130.6222269535065,0.5934925240671873
336336,672673,672672,1345345,1133.9703178405762,0.5918896398543438
337337,674675,674674,1349349,1137.5168640613556,0.5902955693036347
338338,676677,676676,1353353,1140.9837429523468,0.5887102399447031
339339,678679,678678,1357357,1144.3260049819946,0.5871335801057285
340340,680681,680680,1361361,1147.7395160198212,0.5855655188934179
341341,682683,682682,1365365,1151.2611169815063,0.5840059861820919
342342,684685,684684,1369369,1154.6709089279175,0.5824549126082275
343343,686687,686686,1373373,1158.3702569007874,0.5809122295595444
344344,688689,688688,1377377,1161.9739410877228,0.5793778711395134
345345,690691,690690,1381381,1165.5708141326904,0.5778517682447273
346346,692693,692692,1385385,1169.1811769008636,0.5763338544093131
347347,694695,694694,1389389,1172.7778041362762,0.5748240639222786
348348,696697,696696,1393393,1176.422446012497,0.5733223317729426
349349,698699,698698,1397397,1180.0047919750214,0.5718285936382017
350350,700701,700700,1401401,1183.1609799861908,0.5703427858770738
351351,702703,702702,1405405,1186.3101570606232,0.5688648455270595
352352,704705,704704,1409409,1189.4931061267853,0.5673947102804959
353353,706707,706706,1413413,1192.6500759124756,0.5659323184972891
354354,708709,708708,1417417,1195.8117730617523,0.5644776091758104
355355,710711,710710,1421421,1198.9464600086212,0.5630305219583533
356356,712713,712712,1425425,1202.1192150115967,0.561590997111125
357357,714715,714714,1429429,1205.2685639858246,0.5601589755297027
358358,716717,716716,1433433,1208.4606401920319,0.5587343987208442
359359,718719,718718,1437437,1211.6057801246643,0.5573172087915736
360360,720721,720720,1441441,1214.707925081253,0.5559073484546388
361361,722723,722722,1445445,1217.8486790657043,0.5545047610121401
362362,724725,724724,1449449,1221.059063911438,0.5531093903446163
363363,726727,726726,1453453,1224.3586010932922,0.5517211809110449
364364,728729,728728,1457457,1227.6056220531464,0.5503400777397474
365365,730731,730730,1461461,1230.749393939972,0.5489660264156555
366366,732733,732732,1465465,1233.924565076828,0.5475989730821311
367367,734735,734734,1469469,1237.08429813385,0.5462388644245948
368368,736737,736736,1473473,1240.2210109233856,0.5448856476723449
369369,738739,738738,1477477,1243.2904238700867,0.5435392705821869
370370,740741,740740,1481481,1246.3863871097565,0.5421996814420709
371371,742743,742742,1485485,1249.584510087967,0.5408668290601781
372372,744745,744744,1489489,1252.6912741661072,0.5395406627503689
373373,746747,746746,1493493,1255.7679319381714,0.5382211323412776
374374,748749,748748,1497497,1258.8746881484985,0.5369081881544844
375375,750751,750750,1501501,1262.0022959709167,0.5356017810172489
376376,752753,752752,1505505,1265.1338398456573,0.5343018622279487
377377,754755,754754,1509509,1268.3101079463959,0.5330083835815458
378378,756757,756756,1513513,1271.6724948883057,0.5317212973423011
379379,758759,758758,1517517,1274.8845739364624,0.530440556247413
380380,760761,760760,1521521,1278.024444103241,0.5291661134906462
381381,762763,762762,1525525,1281.2477090358734,0.5278979227368836
382382,764765,764764,1529529,1284.4703559875488,0.5266359380930226
383383,766767,766766,1533533,1287.5914840698242,0.5253801141225267
384384,768769,768768,1537537,1290.7622230052948,0.5241304058199603
385385,770771,770770,1541541,1293.9105942249298,0.5228867686255398
386386,772773,772772,1545545,1297.0769171714783,0.5216491584124014
387387,774775,774774,1549549,1300.24662399292,0.5204175314684107
388388,776777,776776,1553553,1303.366641998291,0.5191918445161718
389389,778779,778778,1557557,1306.4572291374207,0.5179720546821045
390390,780781,780780,1561561,1309.6176452636719,0.516758119510996
391391,782783,782782,1565565,1312.7488470077515,0.5155499969532684
392392,784785,784784,1569569,1315.8861429691315,0.5143476453595213
393393,786787,786786,1573573,1319.0464689731598,0.5131510234750749
394394,788789,788788,1577577,1322.1617789268494,0.5119600904381514
395395,790791,790790,1581581,1325.2983701229095,0.5107748057780555
396396,792793,792792,1585585,1328.4767649173737,0.5095951293951657
397397,794795,794794,1589589,1331.61021900177,0.5084210215845815
398398,796797,796796,1593593,1334.7305591106415,0.5072524430033809
399399,798799,798798,1597597,1337.8480360507965,0.5060893546760781
400400,800801,800800,1601601,1340.9693357944489,0.5049317180018988
401401,802803,802802,1605605,1344.0920150279999,0.503779494732953
402402,804805,804804,1609609,1347.1904101371765,0.5026326469778724
403403,806807,806806,1613613,1350.2925221920013,0.5014911372054485
404404,808809,808808,1617617,1353.429370880127,0.500354928220986
405405,810811,810810,1621621,1356.5733149051666,0.4992239831844927
406406,812813,812812,1625625,1359.730456829071,0.4980982655870321
407407,814815,814814,1629629,1362.8380460739136,0.4969777392670949
408408,816817,816816,1633633,1365.9621279239655,0.4958623683814949
409409,818819,818818,1637637,1369.0772199630737,0.4947521174290159
410410,820821,820820,1641641,1372.217148065567,0.49364695122494595
411411,822823,822822,1645645,1375.3320710659027,0.49254683490653406
412412,824825,824824,1649649,1378.455905199051,0.49145173393299046
413413,826827,826826,1653653,1381.5749070644379,0.4903616140709346
414414,828829,828828,1657657,1384.6991591453552,0.48927644140349
415415,830831,830830,1661661,1387.8254261016846,0.4881961823157326
416416,832833,832832,1665665,1391.0018730163574,0.4871208035019663
417417,834835,834834,1669669,1394.125610113144,0.4860502719475335
418418,836837,836836,1673673,1397.2281548976898,0.48498455494518566
419419,838839,838838,1677677,1400.3499081134796,0.48392362006961775
420420,840841,840840,1681681,1403.5775151252747,0.4828674351938389
421421,842843,842842,1685685,1406.8717341423035,0.4818159684746206
422422,844845,844844,1689689,1410.022915840149,0.4807691883524967
423423,846847,846846,1693693,1413.173063993454,0.47972706354448746
424424,848849,848848,1697697,1416.3342821598053,0.4786895630550134
425425,850851,850850,1701701,1419.4821479320526,0.47765665614861064
426426,852853,852852,1705705,1422.6253290176392,0.4766283123735775
427427,854855,854854,1709709,1425.7580380439758,0.4756045015401469
428428,856857,856856,1713713,1428.9753711223602,0.4745851937295811
429429,858859,858858,1717717,1432.1455261707306,0.47357035927052493
430430,860861,860860,1721721,1435.2793319225311,0.47255996877174766
431431,862863,862862,1725725,1438.4169759750366,0.4715539930821251
432432,864865,864864,1729729,1441.5286779403687,0.4705524033142865
433433,866867,866866,1733733,1444.734009027481,0.46955517082642473
434434,868869,868868,1737737,1447.8961281776428,0.4685622672259342
435435,870871,870870,1741741,1451.029901266098,0.46757366436941084
436436,872873,872872,1745745,1454.1878108978271,0.4665893343517382
437437,874875,874874,1749749,1457.3082041740417,0.4656092495115445
438438,876877,876876,1753753,1460.491811990738,0.4646333824239264
439439,878879,878878,1757757,1463.6077950000763,0.4636617058986303
440440,880881,880880,1761761,1466.7307970523834,0.4626941929800523
441441,882883,882882,1765765,1469.821758031845,0.4617308169417811
442442,884885,884884,1769769,1472.9597120285034,0.46077155128296
443443,886887,886886,1773773,1476.084702014923,0.45981636973556306
444444,888889,888888,1777777,1479.2342631816864,0.4588652462425671
445445,890891,890890,1781781,1482.4565830230713,0.4579181549761415
446446,892893,892892,1785785,1485.5780189037323,0.45697507033037255
447447,894895,894894,1789789,1488.6904730796814,0.45603596690125414
448448,896897,896896,1793793,1491.7945051193237,0.45510081951397297
449449,898899,898898,1797797,1494.9414868354797,0.4541696031956235
450450,900901,900900,1801801,1498.1076259613037,0.45324229318612197
451451,902903,902902,1805805,1501.2376940250397,0.45231886492911144
452452,904905,904904,1809809,1504.375195980072,0.45139929407923773
453453,906907,906906,1813813,1507.563043832779,0.4504835564894165
454454,908909,908908,1817817,1510.6869552135468,0.4495716282126523
455455,910911,910910,1821821,1513.8116879463196,0.44866348550567636
456456,912913,912912,1825825,1516.9490780830383,0.44775910481257597
457457,914915,914914,1829829,1520.098128080368,0.44685846277752717
458458,916917,916916,1833833,1523.3485720157623,0.44596153624479484
459459,918919,918918,1837837,1526.6128568649292,0.44506830223508587
460460,920921,920920,1841841,1529.7845079898834,0.44417873796373897
461461,922923,922922,1845845,1532.9357159137726,0.44329282083890575
462462,924925,924924,1849849,1536.0722179412842,0.44241052844154183
463463,926927,926926,1853853,1539.2427039146423,0.44153183854541567
464464,928929,928928,1857857,1542.538264989853,0.44065672909891873
465465,930931,930930,1861861,1545.7185559272766,0.4397851782359794
466466,932933,932932,1865865,1548.7998979091644,0.43891716425969207
467467,934935,934934,1869869,1551.9651679992676,0.4380526656532311
468468,936937,936936,1873873,1555.0831520557404,0.43719166107621277
469469,938939,938938,1877877,1558.230463027954,0.43633412935923843
470470,940941,940940,1881881,1561.4068810939789,0.43548004949298047
471471,942943,942942,1885885,1564.5454709529877,0.4346294006536482
472472,944945,944944,1889889,1567.8896470069885,0.433782162173884
473473,946947,946946,1893893,1571.1389141082764,0.4329383135482203
474474,948949,948948,1897897,1574.2778351306915,0.43209783444399363
475475,950951,950950,1901901,1577.4018378257751,0.43126070468861144
476476,952953,952952,1905905,1580.53178191185,0.43042690426409536
477477,954955,954954,1909909,1583.6582968235016,0.42959641331435705
478478,956957,956956,1913913,1586.779145002365,0.42876921214519825
479479,958959,958958,1917917,1589.8959000110626,0.42794528120975883
480480,960961,960960,1921921,1593.0997321605682,0.4271246011212497
481481,962963,962962,1925925,1596.254832983017,0.426307152642039
482482,964965,964964,1929929,1599.399167060852,0.42549291668728983
483483,966967,966966,1933933,1602.5744888782501,0.42468187432314153
484484,968969,968968,1937937,1605.7575500011444,0.42387400676125253
485485,970971,970970,1941941,1608.8805751800537,0.42306929535698146
486486,972973,972972,1945945,1612.014477968216,0.42226772162212
487487,974975,974974,1949949,1615.1437380313873,0.4214692671994271
488488,976977,976976,1953953,1618.282154083252,0.42067391388263786
489489,978979,978978,1957957,1621.4354000091553,0.4198816436019115
490490,980981,980980,1961961,1624.5485861301422,0.41909243843110744
491491,982983,982982,1965965,1627.669986963272,0.41830628873140085
492492,984985,984984,1969969,1630.7920169830322,0.41752317151804164
493493,986987,986986,1973973,1633.9336550235748,0.41674306641834846
494494,988989,988988,1977977,1637.059382200241,0.4159659560518776
495495,990991,990990,1981981,1640.1830830574036,0.4151918231709715
496496,992993,992992,1985985,1643.5108890533447,0.4144206506516639
497497,994995,994994,1989989,1646.7800180912018,0.41365242151005077
498498,996997,996996,1993993,1649.9586489200592,0.4128871188895573
499499,998999,998998,1997997,1653.0769369602203,0.4121247260573
500501,1001003,1001002,2002005,1656.284439086914,0.41136446911150415
501502,1003005,1003004,2006009,1659.4209570884705,0.4106078490440268
502503,1005007,1005006,2010013,1662.6401789188385,0.40985408931555867
503504,1007009,1007008,2014017,1665.880213022232,0.40910317369889526
504505,1009011,1009010,2018021,1669.012097120285,0.4083550860905234
505506,1011013,1011012,2022025,1672.1195549964905,0.40760981049788825
506507,1013015,1013014,2026029,1675.240730047226,0.4068673310612212
507508,1015017,1015016,2030033,1678.386167049408,0.406127632029893
508509,1017019,1017018,2034037,1681.5109939575195,0.4053906977733277
509510,1019021,1019020,2038041,1684.6169791221619,0.4046565127810027
510511,1021023,1021022,2042045,1687.7972960472107,0.4039250616569916
511512,1023025,1023024,2046049,1690.9412989616394,0.4031963291163265
512513,1025027,1025026,2050053,1694.0589439868927,0.4024702999886358
513514,1027029,1027028,2054057,1697.2396922111511,0.4017469592163252
514515,1029031,1029030,2058061,1700.4065759181976,0.4010262918545777
515516,1031033,1031032,2062065,1703.5231919288635,0.4003082830695348
516517,1033035,1033034,2066069,1706.6259360313416,0.39959291813283926
517518,1035037,1035036,2070073,1709.7793979644775,0.39888018242345424
518519,1037039,1037038,2074077,1712.8950560092926,0.3981700614331203
519520,1039041,1039040,2078081,1716.0563850402832,0.3974625407572603
520521,1041043,1041042,2082085,1719.1881470680237,0.39675760609497956
521522,1043045,1043044,2086089,1722.3586361408234,0.3960552432527038
522523,1045047,1045046,2090093,1725.4819960594177,0.3953554381387221
523524,1047049,1047048,2094097,1728.6162419319153,0.39465817675954895
524525,1049051,1049050,2098101,1731.7088010311127,0.39396344523265725
525526,1051053,1051052,2102105,1734.879277229309,0.3932712297682883
526527,1053055,1053054,2106109,1738.0274698734283,0.3925815166785469
527528,1055057,1055056,2110113,1741.1445000171661,0.39189429237558215
528529,1057059,1057058,2114117,1744.260754108429,0.39120954336976865
529530,1059061,1059060,2118121,1747.4505760669708,0.39052725626424944
530531,1061063,1061062,2122125,1750.57945394516,0.389847417762212
531532,1063065,1063064,2126129,1753.7238399982452,0.3891700146614312
532533,1065067,1065066,2130133,1756.8565032482147,0.3884950338560884
533534,1067069,1067068,2134137,1759.9954450130463,0.3878224623276765
534535,1069071,1069070,2138141,1763.111664056778,0.38715228715773264
535536,1071073,1071072,2142145,1766.2569580078125,0.38648449551510566
536537,1073075,1073074,2146149,1769.4203989505768,0.38581907466323173
537538,1075077,1075076,2150153,1772.5440452098846,0.38515601195103955
538539,1077079,1077078,2154157,1775.675409078598,0.38449529482022626
539540,1079081,1079080,2158161,1778.7942957878113,0.3838369108070765
540541,1081083,1081082,2162165,1781.955978155136,0.3831808475188154
541542,1083085,1083084,2166169,1785.230796098709,0.38252709266998863
542543,1085087,1085086,2170173,1788.5393319129944,0.3818756340442633
543544,1087089,1087088,2174177,1791.6827220916748,0.38122645952535095
544545,1089091,1089090,2178181,1794.7995479106903,0.3805795570697228
545546,1091093,1091092,2182185,1797.9232971668243,0.3799349147302564
546547,1093095,1093094,2186189,1801.0389430522919,0.379292520632589
547548,1095097,1095096,2190193,1804.1647939682007,0.3786523629896692
548549,1097099,1097098,2194197,1807.3196589946747,0.3780144300944812
549550,1099101,1099100,2198201,1810.5179960727692,0.37737871032550174
550551,1101103,1101102,2202205,1813.6635301113129,0.37674519213760504
551552,1103105,1103104,2206209,1816.8117461204529,0.3761138640638819
552553,1105107,1105106,2210213,1819.9421031475067,0.37548471472655365
553554,1107109,1107108,2214217,1823.0652329921722,0.37485773281332513
554555,1109111,1109110,2218221,1826.231498003006,0.37423290709739376
555556,1111113,1111112,2222225,1829.380441904068,0.3736102264301735
556557,1113115,1113114,2226229,1832.5903708934784,0.37298967973583785
557558,1115117,1115116,2230233,1835.746726989746,0.37237125601131993
558559,1117119,1117118,2234237,1838.8692932128906,0.37175494433722633
559560,1119121,1119120,2238241,1842.026883840561,0.37114073386510427
560561,1121123,1121122,2242245,1845.1260170936584,0.3705286138174415
561562,1123125,1123124,2246249,1848.3123281002045,0.3699185734931234
562563,1125127,1125126,2250253,1851.4391491413116,0.3693106022619759
563564,1127129,1127128,2254257,1854.6136400699615,0.3687046895702224
564565,1129131,1129130,2258261,1857.759437084198,0.3681008249277511
565566,1131133,1131132,2262265,1860.8816771507263,0.3674989979226666
566567,1133135,1133134,2266269,1864.003713130951,0.3668991982103762
567568,1135137,1135136,2270273,1867.1561181545258,0.36630141551540873
568569,1137139,1137138,2274277,1870.2904450893402,0.36570563963141467
569570,1139141,1139140,2278281,1873.4177911281586,0.36511186042116606
570571,1141143,1141142,2282285,1876.5319900512695,0.36452006781655655
571572,1143145,1143144,2286289,1879.6743738651276,0.3639302518149634
572573,1145147,1145146,2290293,1882.9006159305573,0.36334240248106653
573574,1147149,1147148,2294297,1886.1595721244812,0.3627565099468484
574575,1149151,1149150,2298301,1889.3576400279999,0.3621725644061371
575576,1151153,1151152,2302305,1892.4875979423523,0.3615905561218824
576577,1153155,1153154,2306309,1895.6466541290283,0.3610104754243366
577578,1155157,1155156,2310313,1898.7334659099579,0.36043231269832177
578579,1157159,1157158,2314317,1901.9162690639496,0.3598560584050574
579580,1159161,1159160,2318321,1905.0359802246094,0.35928170305305684
580581,1161163,1161162,2322325,1908.1982719898224,0.3587092372290499
581582,1163165,1163164,2326329,1911.4130189418793,0.35813865157069813
582583,1165167,1165166,2330333,1914.573634147644,0.35756993678296567
583584,1167169,1167168,2334337,1917.692223072052,0.35700308362902433
584585,1169171,1169170,2338341,1920.8162529468536,0.35643808293934853
585586,1171173,1171172,2342345,1923.9656689167023,0.35587492558806844
586587,1173175,1173174,2346349,1927.1689660549164,0.35531360252571176
587588,1175177,1175176,2350353,1930.2921659946442,0.3547541047537379
588589,1177179,1177178,2354357,1933.4266510009766,0.354196423335452
589590,1179181,1179180,2358361,1936.567710161209,0.3536405493887287
590591,1181183,1181182,2362365,1939.7808530330658,0.3530864740914694
591592,1183185,1183184,2366369,1942.9930069446564,0.35253418867978326
592593,1185187,1185186,2370373,1946.1632809638977,0.35198368444071093
593594,1187189,1187188,2374377,1949.3129959106445,0.3514349527285958
594595,1189191,1189190,2378381,1952.4529581069946,0.350887984943256
595596,1191193,1191192,2382385,1955.6330041885376,0.3503427725372603
596597,1193195,1193194,2386389,1958.8973350524902,0.3497993070304801
597598,1195197,1195196,2390393,1962.0493819713593,0.34925757999189955
598599,1197199,1197198,2394397,1965.1541020870209,0.34871758303597744
599600,1199201,1199200,2398401,1968.2661159038544,0.34817930784629425
600601,1201203,1201202,2402405,1971.4339048862457,0.3476427461482672
601602,1203205,1203204,2406409,1974.565680027008,0.3471078897200641
602603,1205207,1205206,2410413,1977.7154169082642,0.34657473039806064
603604,1207209,1207208,2414417,1980.8863849639893,0.346043260067745
604605,1209211,1209210,2418421,1984.0054650306702,0.34551347066553717
605606,1211213,1211212,2422425,1987.176884174347,0.34498535418060783
606607,1213215,1213214,2426429,1990.2835211753845,0.34445890264942136
607608,1215217,1215216,2430433,1993.4371128082275,0.34393410816301184
608609,1217219,1217218,2434437,1996.5836019515991,0.3434109628578881
609610,1219221,1219220,2438441,1999.757719039917,0.3428894589233096
610611,1221223,1221222,2442445,2002.9930489063263,0.34236958859764854
611612,1223225,1223224,2446449,2006.2955479621887,0.34185134416475194
612613,1225227,1225226,2450453,2009.4958741664886,0.3413347179593984
613614,1227229,1227228,2454457,2012.7490890026093,0.3408197023672983
614615,1229231,1229230,2458461,2016.1362390518188,0.34030628981417976
615616,1231233,1231232,2462465,2019.2929091453552,0.3397944727803406
616617,1233235,1233234,2466469,2022.4767761230469,0.3392842437897343
617618,1235237,1235236,2470473,2025.6299121379852,0.33877559540997026
618619,1237239,1237238,2474477,2028.7320120334625,0.3382685202595894
619620,1239241,1239240,2478481,2031.8635761737823,0.33776301099896955
620621,1241243,1241242,2482485,2034.9988720417023,0.3372590603412391
621622,1243245,1243244,2486489,2038.11989402771,0.3367566610304493
622623,1245247,1245246,2490493,2041.282516002655,0.33625580587431614
623624,1247249,1247248,2494497,2044.4289638996124,0.3357564877060213
624625,1249251,1249250,2498501,2047.5937149524689,0.3352586994169542
625626,1251253,1251252,2502505,2050.7111802101135,0.334762433936703
626627,1253255,1253254,2506509,2053.8790969848633,0.33426768423487374
627628,1255257,1255256,2510513,2056.9948949813843,0.333774443330185
628629,1257259,1257258,2514517,2060.130650997162,0.3332827042831923
629630,1259261,1259260,2518521,2063.2598621845245,0.33279246018901176
630631,1261263,1261262,2522525,2066.415102958679,0.33230370419551036
631632,1263265,1263264,2526529,2069.5454030036926,0.3318164294887538
632633,1265267,1265266,2530533,2072.6637489795685,0.3313306292893685
633634,1267269,1267268,2534537,2075.805119037628,0.33084629687255074
634635,1269271,1269270,2538541,2078.925341129303,0.33036342554078146
635636,1271273,1271272,2542545,2082.076539039612,0.3298820086456544
636637,1273275,1273274,2546549,2085.2640058994293,0.32940203957514314
637638,1275277,1275276,2550553,2088.375237941742,0.3289235117572389
638639,1277279,1277278,2554557,2091.4781110286713,0.3284464186617697
639640,1279281,1279280,2558561,2094.629280090332,0.3279707537985814
640641,1281283,1281282,2562565,2097.7560770511627,0.32749651070844266
641642,1283285,1283284,2566569,2100.853175878525,0.32702368298305373
642643,1285287,1285286,2570573,2103.9923000335693,0.3265522642413998
643644,1287289,1287288,2574577,2107.1477031707764,0.32608224814975983
644645,1289291,1289290,2578581,2110.319983959198,0.32561362840715447
645646,1291293,1291292,2582585,2113.4114830493927,0.3251463987489842
646647,1293295,1293294,2586589,2116.542226076126,0.32468055295066733
647648,1295297,1295296,2590593,2119.7070281505585,0.3242160848240019
648649,1297299,1297298,2594597,2122.8501031398773,0.3237529882171657
649650,1299301,1299300,2598601,2125.941927909851,0.3232912570165354
650651,1301303,1301302,2602605,2129.06333899498,0.32283088514304836
651652,1303305,1303304,2606609,2132.233170032501,0.32237186655220285
652653,1305307,1305306,2610613,2135.416501045227,0.3219141952376958
653654,1307309,1307308,2614617,2138.5707879066467,0.3214578652259661
654655,1309311,1309310,2618621,2141.7341310977936,0.3210028705852892
655656,1311313,1311312,2622625,2145.0452921390533,0.32054920540940657
656657,1313315,1313314,2626629,2148.3026168346405,0.32009686383389635
657658,1315317,1315316,2630633,2151.407438993454,0.31964584001980256
658659,1317319,1317318,2634637,2154.5390980243683,0.31919612817546295
659660,1319321,1319320,2638641,2157.6689450740814,0.3187477225346811
660661,1321323,1321322,2642645,2160.794415950775,0.3183006173640024
661662,1323325,1323324,2646649,2163.9211840629578,0.31785480696999
662663,1325327,1325326,2650653,2167.088392972946,0.317410285682854
663664,1327329,1327328,2654657,2170.3101241588593,0.31696704787282215
664665,1329331,1329330,2658661,2173.4371869564056,0.31652508794286405
665666,1331333,1331332,2662665,2176.5390520095825,0.31608440032323415
666667,1333335,1333334,2666669,2179.6888139247894,0.3156449794805667
667668,1335337,1335336,2670673,2182.820550918579,0.3152068199142377
668669,1337339,1337338,2674677,2185.945657014847,0.3147699161545461
669670,1339341,1339340,2678681,2189.0639810562134,0.3143342627554375
670671,1341343,1341342,2682685,2192.1908481121063,0.3138998543181515
671672,1343345,1343344,2686689,2195.321835041046,0.3134666854602983
672673,1345347,1345346,2690693,2198.493592262268,0.31303475083950616
673674,1347349,1347348,2694697,2201.66530585289,0.312604045135231
674675,1349351,1349350,2698701,2204.8179070949554,0.3121745630669466
675676,1351353,1351352,2702705,2207.977371931076,0.31174629937777354
676677,1353355,1353354,2706709,2211.0657300949097,0.3113192488453933
677678,1355357,1355356,2710713,2214.1845037937164,0.31089340627113415
678679,1357359,1357358,2714717,2217.3177769184113,0.31046876649452315
679680,1359361,1359360,2718721,2220.464648962021,0.31004532437509624
680681,1361363,1361362,2722725,2223.5903010368347,0.30962307481058815
681682,1363365,1363364,2726729,2226.7808232307434,0.3092020127187425
682683,1365367,1365366,2730733,2229.898520231247,0.30878213305186364
683684,1367369,1367368,2734737,2233.034812927246,0.3083634307877219
684685,1369371,1369370,2738741,2236.164892911911,0.30794590093864826
685686,1371373,1371372,2742745,2239.3342118263245,0.30752953853334475
686687,1373375,1373374,2746749,2242.447783946991,0.30711433863871207
687688,1375377,1375376,2750753,2245.888589859009,0.3067002963489358
688689,1377379,1377378,2754757,2249.1608130931854,0.3062874067818484
689690,1379381,1379380,2758761,2252.282473087311,0.30587566508256714
690691,1381383,1381382,2762765,2255.4674570560455,0.30546506642167515
691692,1383385,1383384,2766769,2258.616019964218,0.30505560600613535
692693,1385387,1385386,2770773,2261.777065038681,0.3046472790574626
693694,1387389,1387388,2774777,2264.988615989685,0.3042400808317325
694695,1389391,1389390,2778781,2268.172660112381,0.30383400660684856
695696,1391393,1391392,2782785,2271.3075029850006,0.30342905169345613
696697,1393395,1393394,2786789,2274.4245131015778,0.3030252114240284
697698,1395397,1395396,2790793,2277.5784668922424,0.3026224811528664
698699,1397399,1397398,2794797,2280.7039802074432,0.302220856268832
699700,1399401,1399400,2798801,2283.8259930610657,0.30182033217352
700701,1401403,1401402,2802805,2287.0144279003143,0.30142090431218094
701702,1403405,1403404,2806809,2290.160742998123,0.3010225681373413
702703,1405407,1405406,2810813,2293.262759923935,0.30062531913790735
703704,1407409,1407408,2814817,2296.3882989883423,0.3002291528227943
704705,1409411,1409410,2818821,2299.4864132404327,0.2998340647263831
705706,1411413,1411412,2822825,2302.668058872223,0.29944005040488264
706707,1413415,1413414,2826829,2305.7834901809692,0.2990471054454247
707708,1415417,1415416,2830833,2308.922350883484,0.29865522545878775
708709,1417419,1417418,2834837,2312.036199092865,0.29826440606848337
709710,1419421,1419420,2838841,2315.1882750988007,0.2978746429325838
710711,1421423,1421422,2842845,2318.3429760932922,0.29748593173462723
711712,1423425,1423424,2846849,2321.5268528461456,0.2970982681708847
712713,1425427,1425426,2850853,2324.6794440746307,0.29671164797400706
713714,1427429,1427428,2854857,2327.8286349773407,0.29632606688574015
714715,1429431,1429430,2858861,2330.9466400146484,0.29594152068239055
715716,1431433,1431432,2862865,2334.0895750522614,0.2955580051566358
716717,1433435,1433434,2866869,2337.2434589862823,0.29517551613025717
717718,1435437,1435436,2870873,2340.357619047165,0.29479404944140697
718719,1437439,1437438,2874877,2343.5122530460358,0.2944136009500653
719720,1439441,1439440,2878881,2346.6705610752106,0.2940341665453161
720721,1441443,1441442,2882885,2349.8194279670715,0.29365574213079526
721722,1443445,1443444,2886889,2352.9435868263245,0.29327832363560447
722723,1445447,1445446,2890893,2356.0795509815216,0.2929019070143113
723724,1447449,1447448,2894897,2359.1982412338257,0.2925264882378542
724725,1449451,1449450,2898901,2362.349165916443,0.2921520632971806
725726,1451453,1451452,2902905,2365.4747710227966,0.29177862843789626
726727,1453455,1453454,2906909,2368.6388082504272,0.2914061795709131
727728,1455457,1455456,2910913,2371.774528026581,0.2910347126507986
728729,1457459,1457458,2914917,2374.9204199314117,0.29066422376126866
729730,1459461,1459460,2918921,2378.0538079738617,0.290294708995134
730731,1461463,1461462,2922925,2381.216304063797,0.2899261644761282
731732,1463465,1463464,2926929,2384.370092153549,0.2895585863479937
732733,1465467,1465466,2930933,2387.672618150711,0.28919197076538694
733734,1467469,1467468,2934937,2390.8832421302795,0.28882631391388713
734735,1469471,1469470,2938941,2394.005537033081,0.2884616119972634
735736,1471473,1471472,2942945,2397.126242160797,0.28809786123019876
736737,1473475,1473474,2946949,2400.2531809806824,0.2877350578619371
737738,1475477,1475476,2950953,2403.3699259757996,0.2873731981489982
738739,1477479,1477478,2954957,2406.5326709747314,0.2870122783770057
739740,1479481,1479480,2958961,2409.702203989029,0.2866522948424972
740741,1481483,1481482,2962965,2412.903831243515,0.2862932438674761
741742,1483485,1483484,2966969,2416.0326538085938,0.28593512179031677
742743,1485487,1485486,2970973,2419.1554231643677,0.2855779249694024
743744,1487489,1487488,2974977,2422.2840139865875,0.28522164978312503
744745,1489491,1489490,2978981,2425.423793077469,0.28486629262806673
745746,1491493,1491492,2982985,2428.5716800689697,0.28451184991718037
746747,1493495,1493494,2986989,2431.7404561042786,0.2841583180870657
747748,1495497,1495496,2990993,2434.9427359104156,0.2838056935888744
748749,1497499,1497498,2994997,2438.1269631385803,0.2834539728901291
749750,1499501,1499500,2999001,2441.265424013138,0.28310315248199913
750751,1501503,1501502,3003005,2444.41659617424,0.2827532288720249
751752,1503505,1503504,3007009,2447.529319047928,0.2824041985841177
752753,1505507,1505506,3011013,2450.68238902092,0.2820560581640166
753754,1507509,1507508,3015017,2453.8245849609375,0.2817088041701936
754755,1509511,1509510,3019021,2456.9661571979523,0.28136243317931076
755756,1511513,1511512,3023025,2460.11749792099,0.2810169417934958
756757,1513515,1513514,3027029,2463.2386140823364,0.2806723266185145
757758,1515517,1515516,3031033,2466.382683992386,0.28032858429105545
758759,1517519,1517518,3035037,2469.504660129547,0.2799857114569022
759760,1519521,1519520,3039041,2472.6445360183716,0.2796437047818472
760761,1521523,1521522,3043045,2475.794676065445,0.2793025609516917
761762,1523525,1523524,3047049,2478.90354013443,0.278962276659513
762763,1525527,1525526,3051053,2482.067677974701,0.27862284862203524
763764,1527529,1527528,3055057,2485.189106941223,0.27828427357962937
764765,1529531,1529530,3059061,2488.312432050705,0.2779465482726664
765766,1531533,1531532,3063065,2491.4400589466095,0.27760966947244015
766767,1533535,1533534,3067069,2494.5412380695343,0.27727363396115834
767768,1535537,1535536,3071073,2497.6977360248566,0.27693843853376165
768769,1537539,1537538,3075077,2500.7906761169434,0.2766040800088376
769770,1539541,1539540,3079081,2503.979259967804,0.2762705552158877
770771,1541543,1541542,3083085,2507.1164441108704,0.27593786099896533
771772,1543545,1543544,3087089,2510.24178314209,0.27560599423122767
772773,1545547,1545546,3091093,2513.3728709220886,0.275274951776737
773774,1547549,1547548,3095097,2516.530506134033,0.27494473053775437
774775,1549551,1549550,3099101,2519.6567120552063,0.27461532742745476
775776,1551553,1551552,3103105,2522.781137943268,0.2742867393644701
776777,1553555,1553554,3107109,2526.125235080719,0.27395896329107927
777778,1555557,1555556,3111113,2529.426398038864,0.2736319961659319
778779,1557559,1557558,3115117,2532.5576169490814,0.27330583495677274
779780,1559561,1559560,3119121,2535.7424330711365,0.27298047665499325
780781,1561563,1561562,3123125,2538.8794651031494,0.27265591825562296
781782,1563565,1563564,3127129,2542.06085896492,0.2723321567809762
782783,1565567,1565566,3131133,2545.177093029022,0.2720091892606433
783784,1567569,1567568,3135137,2548.3196680545807,0.2716870127351285
784785,1569571,1569570,3139141,2551.4955899715424,0.2713656242740399
785786,1571573,1571572,3143145,2554.6601390838623,0.2710450209433475
786787,1573575,1573574,3147149,2557.8105590343475,0.27072519984176324
787788,1575577,1575576,3151153,2560.9534780979156,0.27040615806618007
788789,1577579,1577578,3155157,2564.0952401161194,0.27008789273713774
789790,1579581,1579580,3159161,2567.245115995407,0.26977040098972793
790791,1581583,1581582,3163165,2570.394743204117,0.2694536799663183
791792,1583585,1583584,3167169,2573.5445079803467,0.2691377268292854
792793,1585587,1585586,3171173,2576.7340371608734,0.2688225387555576
793794,1587589,1587588,3175177,2579.952406167984,0.2685081129293394
794795,1589591,1589590,3179181,2583.0732519626617,0.26819444655484403
795796,1591593,1591592,3183185,2586.26127910614,0.2678815368508367
796797,1593595,1593594,3187189,2589.405543088913,0.2675693810433586
797798,1595597,1595596,3191193,2592.536509990692,0.26725797637482174
798799,1597599,1597598,3195197,2595.6550171375275,0.2669473201058281
799800,1599601,1599600,3199201,2598.7627971172333,0.26663740950243664
800801,1601603,1601602,3203205,2601.9204380512238,0.26632824184889614
801802,1603605,1603604,3207209,2605.3009791374207,0.26601981444582634
802803,1605607,1605606,3211213,2608.55672621727,0.26571212459384697
803804,1607609,1607608,3215217,2611.701003074646,0.26540516962268157
804805,1609611,1609610,3219221,2614.8715641498566,0.2650989468656917
805806,1611613,1611612,3223225,2618.038733959198,0.2647934536689718
806807,1613615,1613614,3227229,2621.2504642009735,0.2644886874004442
807808,1615617,1615616,3231233,2624.4814291000366,0.26418464542621223
808809,1617619,1617618,3235237,2627.6138050556183,0.2638813251378451
809810,1619621,1619620,3239241,2630.7219960689545,0.26357872393236903
810811,1621623,1621622,3243245,2633.8733241558075,0.263276839223181
811812,1623625,1623624,3247249,2636.985948085785,0.2629756684345921
812813,1625627,1625626,3251253,2640.1370561122894,0.2626752090000082
813814,1627629,1627628,3255257,2643.2748959064484,0.26237545836920617
814815,1629631,1629630,3259261,2646.4392552375793,0.2620764140065148
815816,1631633,1631632,3263265,2649.5352940559387,0.2617780733817199
816817,1633635,1633634,3267269,2652.6658141613007,0.261480433980978
817818,1635637,1635636,3271273,2655.7987110614777,0.2611834933013597
818819,1637639,1637638,3275277,2658.9482851028442,0.26088724885448755
819820,1639641,1639640,3279281,2662.095563173294,0.26059169815926
820821,1641643,1641642,3283285,2665.5040459632874,0.26029683874548937
821822,1643645,1643644,3287289,2668.7300679683685,0.260002668161178
822823,1645647,1645646,3291293,2671.8082242012024,0.25970918395978515
823824,1647649,1647648,3295297,2674.960009098053,0.25941638371295994
824825,1649651,1649650,3299301,2678.1148500442505,0.2591242649996275
825826,1651653,1651652,3303305,2681.239593029022,0.25883282540416985
826827,1653655,1653654,3307309,2684.413675069809,0.25854206253643497
827828,1655657,1655656,3311313,2687.528727054596,0.25825197400627076
828829,1657659,1657658,3315317,2690.726443052292,0.25796255743807706
829830,1659661,1659660,3319321,2693.889322042465,0.2576738104708056
830831,1661663,1661662,3323325,2696.993621110916,0.2573857307434082
831832,1663665,1663664,3327329,2700.1247730255127,0.2570983159203024
832833,1665667,1665666,3331333,2703.2572298049927,0.25681156366954383
833834,1667669,1667668,3335337,2706.4227850437164,0.256525471670102
834835,1669671,1669670,3339341,2709.54309797287,0.2562400376118603
835836,1671673,1671672,3343345,2712.819538116455,0.2559552591974352
836837,1673675,1673674,3347349,2716.185425043106,0.25567113413853804
837838,1675677,1675676,3351353,2719.398089170456,0.255387660157794
838839,1677679,1677678,3355357,2722.52449798584,0.25510483499056136
839840,1679681,1679680,3359361,2725.6684172153473,0.2548226563776552
840841,1681683,1681682,3363365,2728.776460170746,0.2545411220744427
841842,1683685,1683684,3367369,2731.898810863495,0.25426022985084273
842843,1685687,1685686,3371373,2735.242849111557,0.2539799774731364
843844,1687689,1687688,3375377,2738.481708049774,0.2537003627312515
844845,1689691,1689690,3379381,2741.617441177368,0.25342138342239195
845846,1691693,1691692,3383385,2744.753441095352,0.2531430373492185
846847,1693695,1693694,3387389,2747.9112989902496,0.25286532233440084
847848,1695697,1695696,3391393,2751.0471000671387,0.2525882361951517
848849,1697699,1697698,3395397,2754.2194278240204,0.2523117767759686
849850,1699701,1699700,3399401,2757.3616411685944,0.2520359419140732
850851,1701703,1701702,3403405,2760.548420906067,0.2517607294739719
851852,1703705,1703704,3407409,2763.718403816223,0.25148613731471414
852853,1705707,1705706,3411413,2766.892637014389,0.2512121633189963
853854,1707709,1707708,3415417,2769.9895498752594,0.25093880536405777
854855,1709711,1709710,3419421,2773.154402256012,0.2506660613526037
855856,1711713,1711712,3423425,2776.2506268024445,0.2503939291818824
856857,1713715,1713714,3427429,2779.4572830200195,0.25012240677097
857858,1715717,1715716,3431433,2782.6283128261566,0.2498514920425805
858859,1717719,1717718,3435437,2785.777922153473,0.24958118293034204
859860,1719721,1719720,3439441,2788.9110720157623,0.24931147737333959
860861,1721723,1721722,3443445,2792.0710339546204,0.24904237332884804
861862,1723725,1723724,3447449,2795.184536933899,0.2487738687541423
862863,1725727,1725726,3451453,2798.345316886902,0.2485059616228682
863864,1727729,1727728,3455457,2801.46950006485,0.2482386499104905
864865,1729731,1729730,3459461,2804.7553770542145,0.24797193160520692
865866,1731733,1731732,3463465,2808.0416860580444,0.2477058047097671
866867,1733735,1733734,3467469,2811.1813700199127,0.24744026723055867
867868,1735737,1735736,3471473,2814.3051459789276,0.2471753171794262
868869,1737739,1737738,3475477,2817.434007167816,0.24691095258276619
869870,1739741,1739740,3479481,2820.565299987793,0.24664717147607007
870871,1741743,1741742,3483485,2823.7294840812683,0.24638397190210526
871872,1743745,1743744,3487489,2826.894401073456,0.24612135190727713
872873,1745747,1745746,3491493,2830.108241081238,0.24585930955618096
873874,1747749,1747748,3495497,2833.2601039409637,0.24559784291705
874875,1749751,1749750,3499501,2836.408117055893,0.24533695006357448
875876,1751753,1751752,3503505,2839.5480301380157,0.2450766290858155
876877,1753755,1753754,3507509,2842.6724710464478,0.2448168780774722
877878,1755757,1755756,3511513,2845.800358057022,0.24455769513951964
878879,1757759,1757758,3515517,2848.9573760032654,0.24429907838566578
879880,1759761,1759760,3519521,2852.0851500034332,0.2440410259332566
880881,1761763,1761762,3523525,2855.210900068283,0.243783535912371
881882,1763765,1763764,3527529,2858.3726329803467,0.24352660645854485
882883,1765767,1765766,3531533,2861.4872410297394,0.24327023571640893
883884,1767769,1767768,3535537,2864.6749992370605,0.243014421841508
884885,1769771,1769770,3539541,2867.7640199661255,0.24275916298938682
885886,1771773,1771772,3543545,2870.9114830493927,0.242504457335599
886887,1773775,1773774,3547549,2874.0208480358124,0.2422503030520602
887888,1775777,1775776,3551553,2877.1455430984497,0.24199669832887594
888889,1777779,1777778,3555557,2880.2685861587524,0.2417436413543328
889890,1779781,1779780,3559561,2883.421200990677,0.2414911303367262
890891,1781783,1781782,3563565,2886.6207571029663,0.24123916347707564
891892,1783785,1783784,3567569,2889.7640120983124,0.24098773899822845
892893,1785787,1785786,3571573,2893.0581908226013,0.240736855121213
893894,1787789,1787788,3575577,2896.3701169490814,0.24048651008342858
894895,1789791,1789790,3579581,2899.5963048934937,0.24023670212045545
895896,1791793,1791792,3583585,2902.740494966507,0.2399874294824258
896897,1793795,1793794,3587589,2905.8592689037323,0.23973869042674778
897898,1795797,1795796,3591593,2909.003231048584,0.23949048321264854
898899,1797799,1797798,3595597,2912.1081070899963,0.23924280611572613
899900,1799801,1799800,3599601,2915.3624358177185,0.2389956574097596
900901,1801803,1801802,3603605,2918.6244370937347,0.2387490353848989
901902,1803805,1803804,3607609,2921.8278641700745,0.23850293833311298
902903,1805807,1805806,3611613,2924.9723269939423,0.23825736455182778
903904,1807809,1807808,3615617,2928.1134610176086,0.23801231235302112
904905,1809811,1809810,3619621,2931.224671125412,0.2377677800523088
905906,1811813,1811812,3623625,2934.3796820640564,0.23752376596894464
906907,1813815,1813814,3627629,2937.540514230728,0.23728026843673433
907908,1815817,1815816,3631633,2940.694048166275,0.23703728579130257
908909,1817819,1817818,3635637,2943.867718935013,0.23679481637918798
909910,1819821,1819820,3639641,2947.060217857361,0.2365528585451102
910911,1821823,1821822,3643645,2950.1815440654755,0.23631141065561678
911912,1823825,1823824,3647649,2953.3035731315613,0.23607047107179824
912913,1825827,1825826,3651653,2956.447986125946,0.23583003816747805
913914,1827829,1827828,3655657,2959.6224360466003,0.23559011032193666
914915,1829831,1829830,3659661,2962.7672760486603,0.23535068592354946
915916,1831833,1831832,3663665,2965.8940761089325,0.23511176336432982
916917,1833835,1833834,3667669,2969.257822036743,0.23487334104356705
917918,1835837,1835836,3671673,2972.4134001731873,0.23463541736964544
918919,1837839,1837838,3675677,2975.5912668704987,0.23439799075640622
919920,1839841,1839840,3679681,2978.707733154297,0.23416105962496658
920921,1841843,1841842,3683685,2981.835058927536,0.2339246224019007
921922,1843845,1843844,3687689,2985.03227186203,0.2336886775210587
922923,1845847,1845846,3691693,2988.20494389534,0.23345322342720465
923924,1847849,1847848,3695697,2991.2994079589844,0.23321825855964562
924925,1849851,1849850,3699701,2994.4383850097656,0.23298378137951659
925926,1851853,1851852,3703705,2997.5458691120148,0.23274979034613352
926927,1853855,1853854,3707709,3000.7041029930115,0.23251628392608836
927928,1855857,1855856,3711713,3003.853234052658,0.23228326058961102
928929,1857859,1857858,3715717,3007.077802181244,0.23205071882148331
929930,1859861,1859860,3719721,3010.1696860790253,0.2318186571028491
930931,1861863,1861862,3723725,3013.2959520816803,0.23158707393304212
931932,1863865,1863864,3727729,3016.5216131210327,0.23135596780775813
932933,1865867,1865866,3731733,3019.86638712883,0.23112533722814987
933934,1867869,1867868,3735737,3023.081181049347,0.23089518071174098
934935,1869871,1869870,3739741,3026.241136074066,0.23066549677787407
935936,1871873,1871872,3743745,3029.3889269828796,0.23043628394589177
936937,1873875,1873874,3747749,3032.5254559516907,0.23020754074605065
937938,1875877,1875876,3751753,3035.7653279304504,0.2299792657195212
938939,1877879,1877878,3755757,3038.8831429481506,0.22975145740019798
939940,1879881,1879880,3759761,3042.043555021286,0.22952411434562237
940941,1881883,1881882,3763765,3045.3150169849396,0.2292972351078788
941942,1883885,1883884,3767769,3048.4541771411896,0.22907081824814668
942943,1885887,1885886,3771773,3051.5835371017456,0.22884486233124335
943944,1887889,1887888,3775777,3054.7131128311157,0.22861936592926213
944945,1889891,1889890,3779781,3057.852516889572,0.22839432762521028
945946,1891893,1891892,3783785,3060.971694946289,0.22816974599845707
946947,1893895,1893894,3787789,3064.081295967102,0.22794561963928572
947948,1895897,1895896,3791793,3067.271776199341,0.22772194714889338
948949,1897899,1897898,3795797,3070.438849210739,0.2274987271248392
949950,1899901,1899900,3799801,3073.578472137451,0.22727595817559632
950951,1901903,1901902,3803805,3076.7565310001373,0.22705363891691377
951952,1903905,1903904,3807809,3080.0741641521454,0.22683176796635962
952953,1905907,1905906,3811813,3083.260200023651,0.22661034395059687
953954,1907909,1907908,3815817,3086.4427120685577,0.22638936549628852
954955,1909911,1909910,3819821,3089.5866298675537,0.22616883124464948
955956,1911913,1911912,3823825,3092.7177970409393,0.2259487398332567
956957,1913915,1913914,3827829,3095.9360988140106,0.22572908991060103
957958,1915917,1915916,3831833,3099.1507160663605,0.22550988013063034
958959,1917919,1917918,3835837,3102.347825050354,0.22529110914911143
959960,1919921,1919920,3839841,3105.5874769687653,0.2250727756345441
960961,1921923,1921922,3843845,3109.056415081024,0.22485487825179007
961962,1923925,1923924,3847849,3112.246376991272,0.22463741568026308
962963,1925927,1925926,3851853,3115.3837389945984,0.22442038659573882
963964,1927929,1927928,3855857,3118.502692937851,0.22420378968490695
964965,1929931,1929930,3859861,3121.6567089557648,0.2239876236399141
965966,1931933,1931932,3863865,3124.7923011779785,0.22377188715836382
966967,1933935,1933934,3867869,3127.9908318519592,0.22355657893604075
967968,1935937,1935936,3871873,3131.1776089668274,0.22334169768510037
968969,1937939,1937938,3875877,3134.302939891815,0.2231272421158792
969970,1939941,1939940,3879881,3137.4310171604156,0.2229132109459897
970971,1941943,1941942,3883885,3140.598300933838,0.22269960289668234
971972,1943945,1943944,3887889,3143.8412630558014,0.2224864166964835
972973,1945947,1945946,3891893,3147.134532928467,0.22227365107937658
973974,1947949,1947948,3895897,3150.242141008377,0.22206130477934494
974975,1949951,1949950,3899901,3153.499256849289,0.22184937654492387
975976,1951953,1951952,3903905,3156.7019867897034,0.2216378651191917
976977,1953955,1953954,3907909,3159.8160421848297,0.2214267692543217
977978,1955957,1955956,3911913,3163.0062930583954,0.22121608771522006
978979,1957959,1957958,3915917,3166.122011899948,0.221005819259517
979980,1959961,1959960,3919921,3169.2861409187317,0.22079596265211876
980981,1961963,1961962,3923925,3172.404706954956,0.2205865166743024
981982,1963965,1963964,3927929,3175.546851873398,0.2203774800982501
982983,1965967,1965966,3931933,3178.6548340320587,0.2201688517088769
983984,1967969,1967968,3935937,3181.795439004898,0.21996063028927892
984985,1969971,1969970,3939941,3184.9175820350647,0.21975281463892316
985986,1971973,1971972,3943945,3188.098969936371,0.21954540355000063
986987,1973975,1973974,3947949,3191.246320962906,0.21933839582561632
987988,1975977,1975976,3951953,3194.400829076767,0.21913179027251317
988989,1977979,1977978,3955957,3197.487025976181,0.2189255857028911
989990,1979981,1979980,3959961,3200.64662194252,0.21871978093076905
990991,1981983,1981982,3963965,3203.85978102684,0.21851437477926083
991992,1983985,1983984,3967969,3207.151419878006,0.21830936607329932
992993,1985987,1985986,3971973,3210.3389620780945,0.2181047536432743
993994,1987989,1987988,3975977,3213.5356738567352,0.2179005363232136
994995,1989991,1989990,3979981,3216.726588010788,0.21769671295260196
995996,1991993,1991992,3983985,3219.8757379055023,0.2174932823763811
996997,1993995,1993994,3987989,3223.101881980896,0.21729024344313075
997998,1995997,1995996,3991993,3226.2371332645416,0.2170875950014306
998999,1997999,1997998,3995997,3229.360999107361,0.21688533591441228
1000000,2000001,2000000,4000001,3232.502713918686,0.2166834650452074


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0029349327087402344,12064.709122577777
1001,2003,1001,3004,3.814255714416504,1.081112418198245
2002,4005,2002,6007,7.438738822937012,0.23651446568328538
3003,6007,3003,9010,11.312902688980103,0.1033214599101484
4004,8009,4004,12013,15.392501831054688,0.05736764844004938
5005,10011,5005,15016,19.37235188484192,0.03677323784904729
6006,12013,6006,18019,23.76543092727661,0.026102900248588412
7007,14015,7007,21022,27.416931867599487,0.019222093715143274
8008,16017,8008,24025,31.04142689704895,0.014864625576592516
9009,18019,9009,27028,34.61112594604492,0.011805651212853263
10010,20021,10010,30031,38.26709985733032,0.009544548203848535
11011,22023,11011,33034,41.95066690444946,0.007896683888247935
12012,24025,12012,36037,45.69839000701904,0.00659135574096581
13013,26027,13013,39040,49.17533588409424,0.0055896630001370795
14014,28029,14014,42043,52.33380699157715,0.004792524105141638
15015,30031,15015,45046,55.53766393661499,0.00414137494226452
16016,32033,16016,48049,58.72829270362854,0.0036119735123065766
17017,34035,17017,51052,61.91007995605469,0.003173069149852381
18018,36037,18018,54055,65.07790780067444,0.0028111199808336096
19019,38039,19019,57058,68.23487091064453,0.0025028508498508018
20020,40041,20020,60061,71.38699698448181,0.002241971844341606
21021,42043,21021,63064,74.56941795349121,0.0020186352958262432
22022,44045,22022,66067,77.75248980522156,0.0018273158493684605
23023,46047,23023,69070,81.33155608177185,0.0016630015616101446
24024,48049,24024,72073,84.46893286705017,0.001516828224339406
25025,50051,25025,75076,87.64894890785217,0.001391092575431685
26026,52053,26026,78079,90.76573204994202,0.0012795733364328044
27027,54055,27027,81082,93.92856788635254,0.0011810493560915347
28028,56057,28028,84085,97.03047704696655,0.001094615952752065
29029,58059,29029,87088,100.59425973892212,0.001015768211800605
30030,60061,30030,90091,103.72895193099976,0.0009469393517065328
31031,62063,31031,93094,107.10560894012451,0.0008845652610034449
32032,64065,32032,96097,110.34594202041626,0.0008282670551125193
33033,66067,33033,99100,113.45813870429993,0.0007780286869092379
34034,68069,34034,102103,116.61467480659485,0.0007316113315027906
35035,70071,35035,105106,120.15351486206055,0.0006906106282258406
36036,72073,36036,108109,123.32692670822144,0.0006527325913339155
37037,74075,37037,111112,126.45845603942871,0.0006181628468766576
38038,76077,38038,114115,129.59396195411682,0.0005869194174010772
39039,78079,39039,117118,132.80724382400513,0.0005577117262873799
40040,80081,40040,120121,136.04245781898499,0.0005314653353707399
41041,82083,41041,123124,139.56394791603088,0.0005068210066383472
42042,84085,42042,126127,142.7154097557068,0.0004841958561883075
43043,86087,43043,129130,145.84037590026855,0.0004633940479834564
44044,88089,44044,132133,149.01714992523193,0.00044364019595377613
45045,90091,45045,135136,152.22818565368652,0.0004259109864506172
46046,92093,46046,138139,155.35653686523438,0.0004090492693649139
47047,94095,47047,141142,158.5482497215271,0.00039354062573693227
48048,96097,48048,144145,161.74791598320007,0.0003790990340348799
49049,98099,49049,147148,164.9419538974762,0.00036568315226759296
50050,100101,50050,150151,168.03075289726257,0.00035356161060917657
51051,102103,51051,153154,171.18036603927612,0.0003419875865802169
52052,104105,52052,156157,174.31843495368958,0.0003315274152555503
53053,106107,53053,159160,177.4928686618805,0.00032163729156309273
54054,108109,54054,162163,180.80200386047363,0.00031195291740004905
55055,110111,55055,165166,184.16376972198486,0.00030303633684525266
56056,112113,56056,168169,187.50724697113037,0.00029428337620629463
57057,114115,57057,171172,190.840922832489,0.0002860368258552626
58058,116117,58058,174175,194.18677687644958,0.00027807352307718247
59059,118119,59059,177178,197.55430793762207,0.0002701857392821694
60060,120121,60060,180181,200.8835198879242,0.0002628112088132184
61061,122123,61061,183184,204.2026298046112,0.00025547312725393567
62062,124125,62062,186187,207.6540768146515,0.0002485995792085305
63063,126127,63063,189190,211.1269018650055,0.00024188053248508368
64064,128129,64064,192193,214.45727682113647,0.00023525397409684956
65065,130131,65065,195196,217.8007128238678,0.00022901087868376635
66066,132133,66066,198199,221.1649148464203,0.0002227404202130856
67067,134135,67067,201202,224.49698567390442,0.00021670449314115103
68068,136137,68068,204205,227.9295196533203,0.00021082127204863355
69069,138139,69069,207208,231.30770683288574,0.0002050726816378301
70070,140141,70070,210211,234.6520698070526,0.00019969312415923923
71071,142143,71071,213214,238.00091171264648,0.000194501235455391
72072,144145,72072,216217,241.3759458065033,0.00018948895194625948
73073,146147,73073,219220,244.75707697868347,0.00018453031589160673
74074,148149,74074,222223,248.10691285133362,0.00017973863577935845
75075,150151,75075,225226,251.42265582084656,0.00017511609621578828
76076,152153,76076,228229,254.79598474502563,0.0001703733159956755
77077,154155,77077,231232,258.14615178108215,0.00016573125503782649
78078,156157,78078,234235,261.49320578575134,0.00016107034934975673
79079,158159,79079,237238,264.83274579048157,0.00015636643183825072
80080,160161,80080,240241,268.1673209667206,0.00015177652494458016
81081,162163,81081,243244,271.58967900276184,0.0001470652441639686
82082,164165,82082,246247,274.89964985847473,0.00014241270764614455
83083,166167,83083,249250,278.25491094589233,0.00013771186604571994
84084,168169,84084,252253,281.6021807193756,0.00013294586642587092
85085,170171,85085,255256,284.97570991516113,0.00012838259135605767
86086,172173,86086,258259,288.2978847026825,0.00012396969032124616
87087,174175,87087,261262,291.6038718223572,0.0001199091893795412
88088,176177,88088,264265,294.94205474853516,0.00011582251863728743
89089,178179,89089,267268,298.3127727508545,0.0001116852381528588
90090,180181,90090,270271,301.6616897583008,0.00010794173613248859
91091,182183,91091,273274,304.99639892578125,0.00010416499026177917
92092,184185,92092,276277,308.30326795578003,0.00010040933193522505
93093,186187,93093,279280,311.67064690589905,9.660917021392379e-05
94094,188189,94094,282283,315.0936577320099,9.30845199036412e-05
95095,190191,95095,285286,318.4010429382324,8.960674313129857e-05
96096,192193,96096,288289,321.7499167919159,8.611644989287015e-05
97097,194195,97097,291292,325.05195903778076,8.262146366178058e-05
98098,196197,98098,294295,328.4229817390442,7.912145338195842e-05
99099,198199,99099,297298,331.7641179561615,7.559852929261979e-05
100100,200201,100100,300301,335.07679200172424,7.205719703051727e-05
101101,202203,101101,303304,338.3998749256134,6.842176298960112e-05
102102,204205,102102,306307,341.78729581832886,6.477458373410627e-05
103103,206207,103103,309310,345.1681399345398,6.125335858087055e-05
104104,208209,104104,312313,348.64675092697144,5.774228884547483e-05
105105,210211,105105,315316,352.035612821579,5.4209758673096076e-05
106106,212213,106106,318319,355.3739969730377,5.0599051974131726e-05
107107,214215,107107,321322,358.70293498039246,4.697754229709972e-05
108108,216217,108108,324325,362.06733107566833,4.3422898670542054e-05
109109,218219,109109,327328,365.39985179901123,4.0078059100778773e-05
110110,220221,110110,330331,368.7344298362732,3.748267590708565e-05
111111,222223,111111,333334,372.1106958389282,3.537140219123103e-05
112112,224225,112112,336337,375.5574028491974,3.357582500029821e-05
113113,226227,113113,339340,378.8812258243561,3.1772888178238645e-05
114114,228229,114114,342343,382.2576549053192,2.9990122129675e-05
115115,230231,115115,345346,385.59646677970886,2.8210008167661726e-05
116116,232233,116116,348349,388.90149688720703,2.6607442123349756e-05
117117,234235,117117,351352,392.3258008956909,2.5210547391907312e-05
118118,236237,118118,354355,395.6301758289337,2.4026487153605558e-05
119119,238239,119119,357358,398.98450994491577,2.2831371097709052e-05
120120,240241,120120,360361,402.29383277893066,2.160562689823564e-05
121121,242243,121121,363364,405.6561598777771,2.0328161554061808e-05
122122,244245,122122,366367,408.99699783325195,1.904594319057651e-05
123123,246247,123123,369370,412.30432987213135,1.7725013094604947e-05
124124,248249,124124,372373,415.6840078830719,1.6412392142228782e-05
125125,250251,125125,375376,419.01412868499756,1.5090223314473405e-05
126126,252253,126126,378379,422.38878202438354,1.3727494660997763e-05
127127,254255,127127,381382,425.708438873291,1.2336744475760497e-05
128128,256257,128128,384385,429.0252888202667,1.0928586561931297e-05
129129,258259,129129,387388,432.36354875564575,1.0320472938474268e-05
130130,260261,130130,390391,435.7038109302521,1.0474112059455365e-05
131131,262263,131131,393394,439.0241367816925,1.0559393558651209e-05
132132,264265,132132,396397,442.36266684532166,1.0672009011614136e-05
133133,266267,133133,399400,445.68483781814575,1.0802243195939809e-05
134134,268269,134134,402403,449.02320408821106,1.0829622624441981e-05
135135,270271,135135,405406,452.3699357509613,1.086459269572515e-05
136136,272273,136136,408409,455.72707986831665,1.0883411960094236e-05
137137,274275,137137,411412,459.08720993995667,1.0955009202007204e-05
138138,276277,138138,414415,462.4105839729309,1.1034875569748692e-05
139139,278279,139139,417418,465.9713110923767,1.1150621503475122e-05
140140,280281,140140,420421,469.3424618244171,1.1223884939681739e-05
141141,282283,141141,423424,472.69530177116394,1.1599138815654442e-05
142142,284285,142142,426427,476.0490050315857,1.1976573659921996e-05
143143,286287,143143,429430,479.40621995925903,1.2380098269204609e-05
144144,288289,144144,432433,482.79568099975586,1.2766464351443574e-05
145145,290291,145145,435436,486.1354479789734,1.3119279174134135e-05
146146,292293,146146,438439,489.4423348903656,1.3451714039547369e-05
147147,294295,147147,441442,492.7888607978821,1.3696615496883169e-05
148148,296297,148148,444445,496.11070585250854,1.3847000445821323e-05
149149,298299,149149,447448,499.47171783447266,1.3993787433719262e-05
150150,300301,150150,450451,502.8089747428894,1.4115632438915782e-05
151151,302303,151151,453454,506.15341687202454,1.4210754670784809e-05
152152,304305,152152,456457,509.59619975090027,1.4354545783135109e-05
153153,306307,153153,459460,512.9294037818909,1.4484479834209196e-05
154154,308309,154154,462463,516.2736339569092,1.4583352822228335e-05
155155,310311,155155,465466,519.617429971695,1.4637349522672594e-05
156156,312313,156156,468469,523.0572509765625,1.4653125617769547e-05
157157,314315,157157,471472,526.7601459026337,1.4636614650953561e-05
158158,316317,158158,474475,530.2126529216766,1.4575163731933571e-05
159159,318319,159159,477478,533.6957569122314,1.4486724467133172e-05
160160,320321,160160,480481,537.2894577980042,1.4357654436025769e-05
161161,322323,161161,483484,540.6742849349976,1.4269962775870226e-05
162162,324325,162162,486487,544.0044898986816,1.4257257134886459e-05
163163,326327,163163,489490,547.3764758110046,1.4179584468365647e-05
164164,328329,164164,492493,550.6997907161713,1.4053466657060198e-05
165165,330331,165165,495496,554.0121078491211,1.3907894754083827e-05
166166,332333,166166,498499,557.3871648311615,1.377645821776241e-05
167167,334335,167167,501502,560.7088539600372,1.364433228445705e-05
168168,336337,168168,504505,564.0494267940521,1.3492142898030579e-05
169169,338339,169169,507508,567.3824338912964,1.3317734556039795e-05
170170,340341,170170,510511,570.7157878875732,1.312246240559034e-05
171171,342343,171171,513514,574.06112408638,1.2983542546862736e-05
172172,344345,172172,516517,577.411367893219,1.2859434718848206e-05
173173,346347,173173,519520,580.7428948879242,1.272346344194375e-05
174174,348349,174174,522523,584.1290926933289,1.2572952982736751e-05
175175,350351,175175,525526,587.5089237689972,1.2476049960241653e-05
176176,352353,176176,528529,590.9020719528198,1.2432832591002807e-05
177177,354355,177177,531532,594.2229979038239,1.2351960322121158e-05
178178,356357,178178,534535,597.5662467479706,1.224707011715509e-05
179179,358359,179179,537538,600.9158546924591,1.2188620530650951e-05
180180,360361,180180,540541,604.3209338188171,1.212014103657566e-05
181181,362363,181181,543544,607.8925149440765,1.2015820175292902e-05
182182,364365,182182,546547,611.5372858047485,1.2069956937921233e-05
183183,366367,183183,549550,614.9840829372406,1.2110856914659962e-05
184184,368369,184184,552553,618.2901418209076,1.2129296010243706e-05
185185,370371,185185,555556,621.6284708976746,1.2110966054024175e-05
186186,372373,186186,558559,624.9476528167725,1.2064434486092068e-05
187187,374375,187187,561562,628.3228468894958,1.2021759175695479e-05
188188,376377,188188,564565,631.7325277328491,1.1993388397968374e-05
189189,378379,189189,567568,635.1056518554688,1.1950985935982317e-05
190190,380381,190190,570571,638.4269580841064,1.1862079190905206e-05
191191,382383,191191,573574,641.7528870105743,1.173504460894037e-05
192192,384385,192192,576577,645.1538717746735,1.1593821909627877e-05
193193,386387,193193,579580,648.4800839424133,1.1523246939759701e-05
194194,388389,194194,582583,651.8114159107208,1.1469845048850402e-05
195195,390391,195195,585586,655.1387858390808,1.1459602319519036e-05
196196,392393,196196,588589,658.6610469818115,1.1395313777029514e-05
197197,394395,197197,591592,662.3081579208374,1.1274125427007675e-05
198198,396397,198198,594595,665.6531209945679,1.1095880836364813e-05
199199,398399,199199,597598,669.0092267990112,1.0954718163702637e-05
200200,400401,200200,600601,672.3306539058685,1.0793333785841241e-05
201201,402403,201201,603604,675.7038760185242,1.0594234481686726e-05
202202,404405,202202,606607,679.0326566696167,1.0328327334718779e-05
203203,406407,203203,609610,682.3896179199219,1.0044968803413212e-05
204204,408409,204204,612613,685.7092978954315,9.769933967618272e-06
205205,410411,205205,615616,689.0650098323822,9.577008313499391e-06
206206,412413,206206,618619,692.4045879840851,9.36941069085151e-06
207207,414415,207207,621622,695.7768688201904,9.169636541628279e-06
208208,416417,208208,624625,699.1443419456482,9.167442840407602e-06
209209,418419,209209,627628,702.4342188835144,9.144721843767911e-06
210210,420421,210210,630631,705.7912459373474,9.269573638448492e-06
211211,422423,211211,633634,709.1162009239197,9.479865184403025e-06
212212,424425,212212,636637,712.467033624649,9.657325790612958e-06
213213,426427,213213,639640,715.7965228557587,9.824527296586893e-06
214214,428429,214214,642643,719.1251540184021,9.948824299499393e-06
215215,430431,215215,645646,722.5003917217255,1.0038198524853215e-05
216216,432433,216216,648649,725.9528429508209,1.0118543286807835e-05
217217,434435,217217,651652,729.4012620449066,1.0160847523366101e-05
218218,436437,218218,654655,732.7392299175262,1.0173929695156403e-05
219219,438439,219219,657658,736.0814008712769,1.0182093319599517e-05
220220,440441,220220,660661,739.4111688137054,1.0162881153519265e-05
221221,442443,221221,663664,742.8036968708038,1.0115567420143634e-05
222222,444445,222222,666667,746.1364059448242,1.005233389150817e-05
223223,446447,223223,669670,749.505735874176,1.0034797014668584e-05
224224,448449,224224,672673,752.9181706905365,9.999335816246457e-06
225225,450451,225225,675676,756.2699477672577,9.981815310311504e-06
226226,452453,226226,678679,759.6034557819366,9.946337740984745e-06
227227,454455,227227,681682,762.9045088291168,9.913868780131452e-06
228228,456457,228228,684685,766.2734699249268,9.851315553532913e-06
229229,458459,229229,687688,769.6029009819031,9.769606549525633e-06
230230,460461,230230,690691,772.9707777500153,9.652023436501622e-06
231231,462463,231231,693694,776.2916059494019,9.528990631224588e-06
232232,464465,232232,696697,779.6078717708588,9.395289453095756e-06
233233,466467,233233,699700,782.9761078357697,9.233734090230428e-06
234234,468469,234234,702703,786.4788358211517,9.044029866345227e-06
235235,470471,235235,705706,790.063622713089,8.881406756700017e-06
236236,472473,236236,708709,793.4085297584534,8.8175820565084e-06
237237,474475,237237,711712,796.7687909603119,8.766035534790717e-06
238238,476477,238238,714715,800.0891649723053,8.702108971192501e-06
239239,478479,239239,717718,803.6825699806213,8.605853508925065e-06
240240,480481,240240,720721,807.1729388237,8.473409252474084e-06
241241,482483,241241,723724,810.5188808441162,8.423858162132092e-06
242242,484485,242242,726727,813.8676588535309,8.39754102344159e-06
243243,486487,243243,729730,817.2206358909607,8.34877573652193e-06
244244,488489,244244,732733,820.5577960014343,8.273405910586007e-06
245245,490491,245245,735736,823.8717539310455,8.198960131267086e-06
246246,492493,246246,738739,827.2304680347443,8.104163498501293e-06
247247,494495,247247,741742,830.5810668468475,7.997790817171335e-06
248248,496497,248248,744745,833.913899898529,7.887101673986763e-06
249249,498499,249249,747748,837.2460289001465,7.77301102061756e-06
250250,500501,250250,750751,840.5897529125214,7.641227057320066e-06
251251,502503,251251,753754,843.970901966095,7.485370588256046e-06
252252,504505,252252,756757,847.2884979248047,7.390346581814811e-06
253253,506507,253253,759760,850.6402926445007,7.32052831153851e-06
254254,508509,254254,762763,853.9739739894867,7.249809641507454e-06
255255,510511,255255,765766,857.3537290096283,7.184977221186273e-06
256256,512513,256256,768769,860.7015027999878,7.0972819230519235e-06
257257,514515,257257,771772,864.0465288162231,6.9711786636617035e-06
258258,516517,258258,774775,867.6080360412598,6.8284807639429346e-06
259259,518519,259259,777778,871.0444247722626,6.651449439232238e-06
260260,520521,260260,780781,874.3662960529327,6.481550371972844e-06
261261,522523,261261,783784,877.7107787132263,6.362381100188941e-06
262262,524525,262262,786787,881.1603009700775,6.189329724293202e-06
263263,526527,263263,789790,884.5851838588715,6.0123493312858045e-06
264264,528529,264264,792793,887.8922898769379,5.834255716763437e-06
265265,530531,265265,795796,891.2272658348083,5.663012416334823e-06
266266,532533,266266,798799,894.5707256793976,5.5310301831923425e-06
267267,534535,267267,801802,897.8928470611572,5.467592927743681e-06
268268,536537,268268,804805,901.1927788257599,5.3929106798022985e-06
269269,538539,269269,807808,904.5846607685089,5.2999275794718415e-06
270270,540541,270270,810811,908.0076367855072,5.212314135860652e-06
271271,542543,271271,813814,911.3812079429626,5.119109118822962e-06
272272,544545,272272,816817,914.8058207035065,5.031963155488484e-06
273273,546547,273273,819820,918.2219467163086,4.958632416673936e-06
274274,548549,274274,822823,921.6386480331421,4.895338861388154e-06
275275,550551,275275,825826,925.0344197750092,4.835595973418094e-06
276276,552553,276276,828829,928.4277009963989,4.796809662366286e-06
277277,554555,277277,831832,931.923907995224,4.7560370148858055e-06
278278,556557,278278,834835,935.4918987751007,4.683135557570495e-06
279279,558559,279279,837838,938.9420049190521,4.5607375795952976e-06
280280,560561,280280,840841,942.3253428936005,4.4021235225955024e-06
281281,562563,281281,843844,945.744827747345,4.341678504715674e-06
282282,564565,282282,846847,949.1093847751617,4.2766405385918915e-06
283283,566567,283283,849850,952.477324962616,4.174371497356333e-06
284284,568569,284284,852853,955.8420269489288,4.017383616883308e-06
285285,570571,285285,855856,959.2673966884613,3.848637788905762e-06
286286,572573,286286,858859,962.694531917572,3.7437639548443258e-06
287287,574575,287287,861862,966.0308678150177,3.624089004006237e-06
288288,576577,288288,864865,969.3539979457855,3.4889872040366754e-06
289289,578579,289289,867868,972.7194306850433,3.3229298423975706e-06
290290,580581,290290,870871,976.0718877315521,3.1422132451552898e-06
291291,582583,291291,873874,979.4537718296051,2.949536792584695e-06
292292,584585,292292,876877,982.7865519523621,2.725329977693036e-06
293293,586587,293293,879880,986.1787629127502,2.5238059606635943e-06
294294,588589,294294,882883,989.5125260353088,2.3968968889676034e-06
295295,590591,295295,885886,992.9529099464417,2.2871900000609457e-06
296296,592593,296296,888889,996.4254419803619,2.1858813852304593e-06
297297,594595,297297,891892,999.7711389064789,2.1874620870221406e-06
298298,596597,298298,894895,1003.1137657165527,2.1570813260041177e-06
299299,598599,299299,897898,1006.4760687351227,2.110265995725058e-06
300300,600601,300300,900901,1009.9053559303284,2.233306076959707e-06
301301,602603,301301,903904,1013.3038928508759,2.469563696649857e-06
302302,604605,302302,906907,1016.6757309436798,2.771812432911247e-06
303303,606607,303303,909910,1020.011109828949,3.0406226869672537e-06
304304,608609,304304,912913,1023.3969779014587,3.2796724553918466e-06
305305,610611,305305,915916,1026.752457857132,3.4826334740500897e-06
306306,612613,306306,918919,1030.1110787391663,3.6382243706611916e-06
307307,614615,307307,921922,1033.468223810196,3.814613592112437e-06
308308,616617,308308,924925,1036.7991547584534,3.969178578699939e-06
309309,618619,309309,927928,1040.1444590091705,4.089159119757824e-06
310310,620621,310310,930931,1043.504737854004,4.1845141822705045e-06
311311,622623,311311,933934,1046.8516509532928,4.2293977458029985e-06
312312,624625,312312,936937,1050.2060840129852,4.250014171702787e-06
313313,626627,313313,939940,1053.54052400589,4.241168426233344e-06
314314,628629,314314,942943,1056.8740289211273,4.188181264908053e-06
315315,630631,315315,945946,1060.2295258045197,4.1021812648978084e-06
316316,632633,316316,948949,1063.5809168815613,4.009960321127437e-06
317317,634635,317317,951952,1066.9521598815918,3.8939124351600185e-06
318318,636637,318318,954955,1070.2808697223663,3.7397439882624894e-06
319319,638639,319319,957958,1073.6043338775635,3.535209543770179e-06
320320,640641,320320,960961,1076.9896550178528,3.3147316571557894e-06
321321,642643,321321,963964,1080.3130569458008,3.083461706410162e-06
322322,644645,322322,966967,1083.6907629966736,2.81617212749552e-06
323323,646647,323323,969970,1087.0480890274048,2.537301043048501e-06
324324,648649,324324,972973,1090.408846616745,2.2167023416841403e-06
325325,650651,325325,975976,1093.7741348743439,1.8671689758775756e-06
326326,652653,326326,978979,1097.1228637695312,1.5037512639537454e-06
327327,654655,327327,981982,1100.4728167057037,1.1532720236573368e-06
328328,656657,328328,984985,1103.8202607631683,8.763690857449546e-07
329329,658659,329329,987988,1107.1961357593536,7.159287633839995e-07
330330,660661,330330,990991,1110.5384650230408,6.59683792036958e-07
331331,662663,331331,993994,1113.9083659648895,7.533944881288335e-07
332332,664665,332332,996997,1117.2786588668823,8.688311936566606e-07
333333,666667,333333,1000000,1120.6150126457214,1.0025778465205804e-06
334334,668669,334334,1003003,1123.951416015625,1.1639422154985368e-06
335335,670671,335335,1006006,1127.3154170513153,1.3204553397372365e-06
336336,672673,336336,1009009,1130.793212890625,1.4539291441906244e-06
337337,674675,337337,1012012,1134.2515850067139,1.5897858247626573e-06
338338,676677,338338,1015015,1137.622044801712,1.7138590919785202e-06
339339,678679,339339,1018018,1140.9750108718872,1.8533355614636093e-06
340340,680681,340340,1021021,1144.346629858017,1.959233486559242e-06
341341,682683,341341,1024024,1147.6610589027405,2.0517945813480765e-06
342342,684685,342342,1027027,1151.0197548866272,2.1340347302611917e-06
343343,686687,343343,1030030,1154.4215247631073,2.2115436877356842e-06
344344,688689,344344,1033033,1158.0482659339905,2.293598299729638e-06
345345,690691,345345,1036036,1161.587035894394,2.3623033484909683e-06
346346,692693,346346,1039039,1164.9686629772186,2.4093733372865245e-06
347347,694695,347347,1042042,1168.2979168891907,2.4502351152477786e-06
348348,696697,348348,1045045,1171.7239909172058,2.4703222152311355e-06
349349,698699,349349,1048048,1175.207018852234,2.4765195121290162e-06
350350,700701,350350,1051051,1178.5377168655396,2.485039658495225e-06
351351,702703,351351,1054054,1181.8910439014435,2.5610315788071603e-06
352352,704705,352352,1057057,1185.328992843628,2.6949292077915743e-06
353353,706707,353353,1060060,1188.6668729782104,2.8116555768065155e-06
354354,708709,354354,1063063,1192.0462279319763,2.8918057068949565e-06
355355,710711,355355,1066066,1195.4120199680328,2.9452894523274153e-06
356356,712713,356356,1069069,1198.7705657482147,2.9837647161912173e-06
357357,714715,357357,1072072,1202.151743888855,3.0224600777728483e-06
358358,716717,358358,1075075,1205.5277779102325,3.027787897735834e-06
359359,718719,359359,1078078,1208.8678257465363,3.0140236049192026e-06
360360,720721,360360,1081081,1212.2227199077606,3.0133542168186978e-06
361361,722723,361361,1084084,1215.625593662262,2.9917700885562226e-06
362362,724725,362362,1087087,1218.9781448841095,2.9467737476807088e-06
363363,726727,363363,1090090,1222.3312418460846,2.945664164144546e-06
364364,728729,364364,1093093,1225.6973958015442,2.94938035949599e-06
365365,730731,365365,1096096,1229.030357837677,2.9307684599189088e-06
366366,732733,366366,1099099,1232.3928067684174,2.9243001335998997e-06
367367,734735,367367,1102102,1235.7583448886871,2.994120222865604e-06
368368,736737,368368,1105105,1239.1040897369385,3.0471510399365798e-06
369369,738739,369369,1108108,1242.4618048667908,3.0915944080334157e-06
370370,740741,370370,1111111,1245.821303844452,3.115628715022467e-06
371371,742743,371371,1114114,1249.1858177185059,3.1134677556110546e-06
372372,744745,372372,1117117,1252.652923822403,3.1332947401097044e-06
373373,746747,373373,1120120,1256.108426809311,3.1225554266711697e-06
374374,748749,374374,1123123,1259.5330867767334,3.074070264119655e-06
375375,750751,375375,1126126,1263.0479888916016,3.00070496450644e-06
376376,752753,376376,1129129,1266.419133901596,2.8865106287412345e-06
377377,754755,377377,1132132,1269.7808020114899,2.7965143090113997e-06
378378,756757,378378,1135135,1273.1297907829285,2.677992597455159e-06
379379,758759,379379,1138138,1276.5130288600922,2.5500994524918497e-06
380380,760761,380380,1141141,1279.8554828166962,2.4359687813557684e-06
381381,762763,381381,1144144,1283.2226297855377,2.3961765691637993e-06
382382,764765,382382,1147147,1286.5506927967072,2.3273278202395886e-06
383383,766767,383383,1150150,1289.8936018943787,2.247985321446322e-06
384384,768769,384384,1153153,1293.234939813614,2.170521838706918e-06
385385,770771,385385,1156156,1296.5831289291382,2.063832653220743e-06
386386,772773,386386,1159159,1299.9253160953522,1.9462549971649423e-06
387387,774775,387387,1162162,1303.2607579231262,1.8174432625528425e-06
388388,776777,388388,1165165,1306.6335418224335,1.7261427274206653e-06
389389,778779,389389,1168168,1309.9993467330933,1.6256071830866858e-06
390390,780781,390390,1171171,1313.3997519016266,1.5638997865607962e-06
391391,782783,391391,1174174,1316.741133928299,1.503300154581666e-06
392392,784785,392392,1177177,1320.0930478572845,1.4173911040415987e-06
393393,786787,393393,1180180,1323.4775638580322,1.319504008279182e-06
394394,788789,394394,1183183,1326.8288009166718,1.189375325338915e-06
395395,790791,395395,1186186,1330.1814818382263,1.075808540917933e-06
396396,792793,396396,1189189,1333.5122528076172,9.248433343600482e-07
397397,794795,397397,1192192,1336.883817911148,9.066170605365187e-07
398398,796797,398398,1195195,1340.2487318515778,1.033664375427179e-06
399399,798799,399399,1198198,1343.5914816856384,1.249947672476992e-06
400400,800801,400400,1201201,1346.979084968567,1.5053101378725842e-06
401401,802803,401401,1204204,1350.3491559028625,1.7325746739516035e-06
402402,804805,402402,1207207,1353.9483749866486,1.932068698806688e-06
403403,806807,403403,1210210,1357.3750829696655,2.092370777972974e-06
404404,808809,404404,1213213,1360.7178709506989,2.2465374058810994e-06
405405,810811,405405,1216216,1364.1132097244263,2.3605352907907218e-06
406406,812813,406406,1219219,1367.6514286994934,2.4354067136300728e-06
407407,814815,407407,1222222,1370.9678928852081,2.4825549189699814e-06
408408,816817,408408,1225225,1374.4283456802368,2.5080917112063617e-06
409409,818819,409409,1228228,1377.9031789302826,2.497043169569224e-06
410410,820821,410410,1231231,1381.289393901825,2.4591117835370824e-06
411411,822823,411411,1234234,1384.6841378211975,2.4030050553847104e-06
412412,824825,412412,1237237,1388.036409854889,2.3115480871638283e-06
413413,826827,413413,1240240,1391.4858758449554,2.217371729784645e-06
414414,828829,414414,1243243,1394.960828781128,2.120159479090944e-06
415415,830831,415415,1246246,1398.3132190704346,1.9803428585873917e-06
416416,832833,416416,1249249,1401.6560637950897,1.8595055735204369e-06
417417,834835,417417,1252252,1404.9977159500122,1.787253495422192e-06
418418,836837,418418,1255255,1408.3680157661438,1.6923204384511337e-06
419419,838839,419419,1258258,1411.7155678272247,1.5642672224203125e-06
420420,840841,420420,1261261,1415.0672907829285,1.4160177670419216e-06
421421,842843,421421,1264264,1418.4186789989471,1.2300843081902713e-06
422422,844845,422422,1267267,1421.7534277439117,1.0174280760111287e-06
423423,846847,423423,1270270,1425.1149706840515,9.150171536020935e-07
424424,848849,424424,1273273,1428.4694797992706,8.341703505720943e-07
425425,850851,425425,1276276,1431.803748846054,8.79475919646211e-07
426426,852853,426426,1279279,1435.1791727542877,9.35486241360195e-07
427427,854855,427427,1282282,1438.5126807689667,9.944833436748013e-07
428428,856857,428428,1285285,1441.8691837787628,1.024516677716747e-06
429429,858859,429429,1288288,1445.258241891861,1.0420444596093148e-06
430430,860861,430430,1291291,1448.6020889282227,1.0496169124962762e-06
431431,862863,431431,1294294,1451.930547952652,1.0582298273220658e-06
432432,864865,432432,1297297,1455.3351616859436,1.0364547051722184e-06
433433,866867,433433,1300300,1458.6876528263092,1.0507901606615633e-06
434434,868869,434434,1303303,1462.1555578708649,1.0903713700827211e-06
435435,870871,435435,1306306,1465.7338407039642,1.1330957931932062e-06
436436,872873,436436,1309309,1469.1101558208466,1.1501379049150273e-06
437437,874875,437437,1312312,1472.6928486824036,1.2226300896145403e-06
438438,876877,438438,1315315,1476.0992786884308,1.3042226782999933e-06
439439,878879,439439,1318318,1479.4394388198853,1.3615353964269161e-06
440440,880881,440440,1321321,1482.8049018383026,1.3968874554848298e-06
441441,882883,441441,1324324,1486.1920669078827,1.4527868188451976e-06
442442,884885,442442,1327327,1489.5469827651978,1.5028854249976575e-06
443443,886887,443443,1330330,1492.9009437561035,1.538326614536345e-06
444444,888889,444444,1333333,1496.337611913681,1.5755013009766117e-06
445445,890891,445445,1336336,1499.738872051239,1.6295616660499945e-06
446446,892893,446446,1339339,1503.139102935791,1.6479007172165439e-06
447447,894895,447447,1342342,1506.4594478607178,1.6463563952129334e-06
448448,896897,448448,1345345,1509.7914378643036,1.6522444639122114e-06
449449,898899,449449,1348348,1513.1633007526398,1.6330050129909068e-06
450450,900901,450450,1351351,1516.538115978241,1.6610028978902847e-06
451451,902903,451451,1354354,1520.0267970561981,1.6698722902219743e-06
452452,904905,452452,1357357,1523.4486148357391,1.68760925589595e-06
453453,906907,453453,1360360,1526.8397817611694,1.688105840003118e-06
454454,908909,454454,1363363,1530.5248308181763,1.6890717233764008e-06
455455,910911,455455,1366366,1533.8186378479004,1.73511216416955e-06
456456,912913,456456,1369369,1537.1591737270355,1.7539259715704247e-06
457457,914915,457457,1372372,1540.495284795761,1.7374295566696674e-06
458458,916917,458458,1375375,1543.8501498699188,1.6869907994987443e-06
459459,918919,459459,1378378,1547.3053867816925,1.6128433344420046e-06
460460,920921,460460,1381381,1550.649300813675,1.5148543752729893e-06
461461,922923,461461,1384384,1554.0779089927673,1.4555680536432192e-06
462462,924925,462462,1387387,1557.6713976860046,1.3882909115636721e-06
463463,926927,463463,1390390,1561.057196855545,1.3177868822822347e-06
464464,928929,464464,1393393,1564.4337408542633,1.279382559005171e-06
465465,930931,465465,1396396,1567.786212682724,1.2828932085540146e-06
466466,932933,466466,1399399,1571.1953828334808,1.2964119378011674e-06
467467,934935,467467,1402402,1574.935798883438,1.2888285709777847e-06
468468,936937,468468,1405405,1578.4480979442596,1.2931322999065742e-06
469469,938939,469469,1408408,1581.8742547035217,1.3040680642006919e-06
470470,940941,470470,1411411,1585.4478168487549,1.3001390470890328e-06
471471,942943,471471,1414414,1589.0360298156738,1.2508844520198181e-06
472472,944945,472472,1417417,1592.5759608745575,1.1698830348905176e-06
473473,946947,473473,1420420,1596.2191317081451,1.066371623892337e-06
474474,948949,474474,1423423,1599.8163468837738,1.0172898328164592e-06
475475,950951,475475,1426426,1603.4016058444977,9.76524461293593e-07
476476,952953,476476,1429429,1606.9812037944794,9.487393981544301e-07
477477,954955,477477,1432432,1610.5790567398071,9.210234566126019e-07
478478,956957,478478,1435435,1614.1448156833649,9.104660421144217e-07
479479,958959,479479,1438438,1617.7227058410645,8.906517905415967e-07
480480,960961,480480,1441441,1621.2713210582733,8.648676157463342e-07
481481,962963,481481,1444444,1624.9001598358154,8.145907486323267e-07
482482,964965,482482,1447447,1628.4777839183807,7.615763024659827e-07
483483,966967,483483,1450450,1632.0169169902802,6.94213667884469e-07
484484,968969,484484,1453453,1635.6428399085999,6.419904821086675e-07
485485,970971,485485,1456456,1639.2199668884277,5.709298420697451e-07
486486,972973,486486,1459459,1642.7874038219452,5.238525773165748e-07
487487,974975,487487,1462462,1646.3371849060059,5.879574018763378e-07
488488,976977,488488,1465465,1649.8282296657562,7.245089364005253e-07
489489,978979,489489,1468468,1653.210031747818,9.51731635723263e-07
490490,980981,490490,1471471,1656.7757649421692,1.1303254723316059e-06
491491,982983,491491,1474474,1660.2323739528656,1.2946984497830272e-06
492492,984985,492492,1477477,1663.5812227725983,1.4227844076231122e-06
493493,986987,493493,1480480,1666.976727962494,1.4949982869438827e-06
494494,988989,494494,1483483,1670.3101286888123,1.5264686226146296e-06
495495,990991,495495,1486486,1673.6454010009766,1.5633449947927147e-06
496496,992993,496496,1489489,1676.9914937019348,1.5772657206980512e-06
497497,994995,497497,1492492,1680.3583657741547,1.5534842532360926e-06
498498,996997,498498,1495495,1683.7450287342072,1.4919114619260654e-06
499499,998999,499499,1498498,1687.1049647331238,1.3830449461238459e-06
500501,1001003,500501,1501504,1690.440439939499,1.2711061572190374e-06
501502,1003005,501502,1504507,1693.8102598190308,1.1860283848363906e-06
502503,1005007,502503,1507510,1697.1986408233643,1.0752573871286586e-06
503504,1007009,503504,1510513,1700.5076637268066,9.182240319205448e-07
504505,1009011,504505,1513516,1703.829598903656,8.20789864519611e-07
505506,1011013,505506,1516519,1707.2152798175812,7.458565960405394e-07
506507,1013015,506507,1519522,1710.5520839691162,6.44828105578199e-07
507508,1015017,507508,1522525,1713.868754863739,6.762347766198218e-07
508509,1017019,508509,1525528,1717.2132139205933,6.831705832155421e-07
509510,1019021,509510,1528531,1720.5662808418274,6.578811735380441e-07
510511,1021023,510511,1531534,1723.892669916153,6.90424712956883e-07
511512,1023025,511512,1534537,1727.2690598964691,7.355902198469266e-07
512513,1025027,512513,1537540,1730.6333377361298,7.776143320370466e-07
513514,1027029,513514,1540543,1734.3563289642334,8.332299330504611e-07
514515,1029031,514515,1543546,1737.8736219406128,8.971583156380802e-07
515516,1031033,515516,1546549,1741.22256398201,1.0056628525489941e-06
516517,1033035,516517,1549552,1744.5801467895508,1.099255314329639e-06
517518,1035037,517518,1552555,1747.9335627555847,1.1458741937531158e-06
518519,1037039,518519,1555558,1751.258365869522,1.1448737495811656e-06
519520,1039041,519520,1558561,1754.6519610881805,1.1624888429651037e-06
520521,1041043,520521,1561564,1758.034278869629,1.1759348126361147e-06
521522,1043045,521522,1564567,1761.462001800537,1.1601950973272324e-06
522523,1045047,522523,1567570,1764.7983937263489,1.1760603229049593e-06
523524,1047049,523524,1570573,1768.1620609760284,1.2184082152089104e-06
524525,1049051,524525,1573576,1771.5116307735443,1.2701002560788766e-06
525526,1051053,525526,1576579,1774.851173877716,1.2830896594095975e-06
526527,1053055,526527,1579582,1778.1896660327911,1.273350790143013e-06
527528,1055057,527528,1582585,1781.5296638011932,1.3168191799195483e-06
528529,1057059,528529,1585588,1785.0137708187103,1.339338268735446e-06
529530,1059061,529530,1588591,1788.3502707481384,1.337015419267118e-06
530531,1061063,530531,1591594,1791.6910157203674,1.340364178759046e-06
531532,1063065,531532,1594597,1795.0262808799744,1.3240241969469935e-06
532533,1065067,532533,1597600,1798.3706529140472,1.2683176464634016e-06
533534,1067069,533534,1600603,1801.708378791809,1.2682576198130846e-06
534535,1069071,534535,1603606,1805.0695569515228,1.3152202882338315e-06
535536,1071073,535536,1606609,1808.4268736839294,1.3295793905854225e-06
536537,1073075,536537,1609612,1811.7360796928406,1.3324479368748143e-06
537538,1075077,537538,1612615,1815.096028804779,1.3270146155264229e-06
538539,1077079,538539,1615618,1818.4342877864838,1.3184926501708105e-06
539540,1079081,539540,1618621,1821.7534849643707,1.2881209840998054e-06
540541,1081083,540541,1621624,1825.1447138786316,1.2450182111933827e-06
541542,1083085,541542,1624627,1829.0308198928833,1.2111941032344475e-06
542543,1085087,542543,1627630,1832.7048797607422,1.175376382889226e-06
543544,1087089,543544,1630633,1836.2744498252869,1.1344127415213734e-06
544545,1089091,544545,1633636,1839.8244128227234,1.1037591320928186e-06
545546,1091093,545546,1636639,1843.4225678443909,1.0659023246262223e-06
546547,1093095,546547,1639642,1847.0046017169952,9.839059202931821e-07
547548,1095097,547548,1642645,1850.5912828445435,9.251343726646155e-07
548549,1097099,548549,1645648,1854.244045972824,9.044761100085452e-07
549550,1099101,549550,1648651,1857.969765663147,8.611823432147503e-07
550551,1101103,550551,1651654,1861.547415971756,8.710612746654078e-07
551552,1103105,551552,1654657,1865.3772447109222,8.560582500649616e-07
552553,1105107,552553,1657660,1868.9707119464874,8.199131116271019e-07
553554,1107109,553554,1660663,1872.5500128269196,8.013648766791448e-07
554555,1109111,554555,1663666,1876.1348519325256,7.747639756416902e-07
555556,1111113,555556,1666669,1879.697401046753,7.14740963303484e-07
556557,1113115,556557,1669672,1883.291358947754,6.37686753179878e-07
557558,1115117,557558,1672675,1886.9000680446625,5.446763680083677e-07
558559,1117119,558559,1675678,1890.3446078300476,5.183101166039705e-07
559560,1119121,559560,1678681,1893.7146890163422,5.141864676261321e-07
560561,1121123,560561,1681684,1897.173444032669,5.020574462832883e-07
561562,1123125,561562,1684687,1900.756313085556,4.869471013080329e-07
562563,1125127,562563,1687690,1904.097263097763,4.428657121025026e-07
563564,1127129,563564,1690693,1907.4749329090118,4.98417648486793e-07
564565,1129131,564565,1693696,1910.8147559165955,5.234105628915131e-07
565566,1131133,565566,1696699,1914.1497430801392,5.412111931946129e-07
566567,1133135,566567,1699702,1917.51784491539,6.340833351714537e-07
567568,1135137,567568,1702705,1920.8426847457886,7.214894139906392e-07
568569,1137139,568569,1705708,1924.2038819789886,8.507049642503262e-07
569570,1139141,569570,1708711,1927.579905986786,9.48479282669723e-07
570571,1141143,570571,1711714,1930.9487400054932,1.018011971609667e-06
571572,1143145,571572,1714717,1934.3264276981354,1.045267708832398e-06
572573,1145147,572573,1717720,1937.6658809185028,1.032871296047233e-06
573574,1147149,573574,1720723,1941.0026726722717,9.72519046626985e-07
574575,1149151,574575,1723726,1944.3320617675781,9.008035704027861e-07
575576,1151153,575576,1726729,1947.7047128677368,8.477181836497039e-07
576577,1153155,576577,1729732,1951.0311708450317,7.683192961849272e-07
577578,1155157,577578,1732735,1954.5950639247894,6.268983270274475e-07
578579,1157159,578579,1735738,1957.9829769134521,4.4504668039735407e-07
579580,1159161,579580,1738741,1961.3110547065735,3.2257776183541864e-07
580581,1161163,580581,1741744,1964.6881167888641,2.6166890165768564e-07
581582,1163165,581582,1744747,1968.0011239051819,2.2870153770782053e-07
582583,1165167,582583,1747750,1971.3148567676544,2.673841663636267e-07
583584,1167169,583584,1750753,1974.6394879817963,3.3941250876523554e-07
584585,1169171,584585,1753756,1978.027109861374,3.7853715184610337e-07
585586,1171173,585586,1756759,1981.4550697803497,4.101457307115197e-07
586587,1173175,586587,1759762,1984.7994177341461,4.509183781920001e-07
587588,1175177,587588,1762765,1988.1504759788513,4.7907633415889e-07
588589,1177179,588589,1765768,1991.5143349170685,5.483452696353197e-07
589590,1179181,589590,1768771,1994.942905664444,5.967067409073934e-07
590591,1181183,590591,1771774,1998.2802398204803,6.780664989491925e-07
591592,1183185,591592,1774777,2001.5883839130402,7.216749509098008e-07
592593,1185187,592593,1777780,2004.9305768013,7.320286385947838e-07
593594,1187189,593594,1780783,2008.2615759372711,7.4403578764759e-07
594595,1189191,594595,1783786,2011.6285009384155,7.88759280112572e-07
595596,1191193,595596,1786789,2014.9456560611725,8.446386345895007e-07
596597,1193195,596597,1789792,2018.260764837265,8.803999662632123e-07
597598,1195197,597598,1792795,2021.599946975708,8.796250767773017e-07
598599,1197199,598599,1795798,2024.9433488845825,8.670522220199928e-07
599600,1199201,599600,1798801,2028.308394908905,8.6460386228282e-07
600601,1201203,600601,1801804,2031.641394853592,8.518982212990522e-07
601602,1203205,601602,1804807,2034.988823890686,8.109691407298669e-07
602603,1205207,602603,1807810,2038.3352718353271,8.249280654126778e-07
603604,1207209,603604,1810813,2041.771726846695,8.443494152743369e-07
604605,1209211,604605,1813816,2045.381008863449,8.95224729902111e-07
605606,1211213,605606,1816819,2048.7229387760162,9.099931048694998e-07
606607,1213215,606607,1819822,2052.042243003845,8.894676284398884e-07
607608,1215217,607608,1822825,2055.415969848633,8.541574061382562e-07
608609,1217219,608609,1825828,2058.7351579666138,8.271508704638109e-07
609610,1219221,609610,1828831,2062.032935857773,7.951493898872286e-07
610611,1221223,610611,1831834,2065.365784883499,7.813487172825262e-07
611612,1223225,611612,1834837,2068.7058668136597,7.571597961941734e-07
612613,1225227,612613,1837840,2072.052840948105,7.063936209306121e-07
613614,1227229,613614,1840843,2075.3719708919525,6.742320692865178e-07
614615,1229231,614615,1843846,2078.6560349464417,6.420614226954058e-07
615616,1231233,615616,1846849,2082.004513025284,5.945457814959809e-07
616617,1233235,616617,1849852,2085.365634918213,5.893525667488575e-07
617618,1235237,617618,1852855,2088.9370748996735,5.682413757313043e-07
618619,1237239,618619,1855858,2092.4977288246155,5.526453605853021e-07
619620,1239241,619620,1858861,2095.9586188793182,5.079327820567414e-07
620621,1241243,620621,1861864,2099.3011240959167,4.6135392040014267e-07
621622,1243245,621622,1864867,2102.622116804123,4.467456165002659e-07
622623,1245247,622623,1867870,2106.0446088314056,4.3051659304182976e-07
623624,1247249,623624,1870873,2109.457669734955,3.889545041602105e-07
624625,1249251,624625,1873876,2112.8323278427124,3.5802804632112384e-07
625626,1251253,625626,1876879,2116.2068729400635,4.2787723941728473e-07
626627,1253255,626627,1879882,2119.541455745697,4.604426067089662e-07
627628,1255257,627628,1882885,2122.8630146980286,4.89906597067602e-07
628629,1257259,628629,1885888,2126.2545619010925,5.902020348003134e-07
629630,1259261,629630,1888891,2129.602150917053,6.847458280390128e-07
630631,1261263,630631,1891894,2132.9243268966675,7.307571650017053e-07
631632,1263265,631632,1894897,2136.2358498573303,7.634771463926882e-07
632633,1265267,632633,1897900,2139.533787727356,7.980834197951481e-07
633634,1267269,633634,1900903,2142.8726167678833,8.451552275801077e-07
634635,1269271,634635,1903906,2146.2274668216705,8.447113941656426e-07
635636,1271273,635636,1906909,2149.5538418293,8.411152521148324e-07
636637,1273275,636637,1909912,2152.878762960434,8.049701136769727e-07
637638,1275277,637638,1912915,2156.2196159362793,7.35328285372816e-07
638639,1277279,638639,1915918,2159.568431854248,6.643003871431574e-07
639640,1279281,639640,1918921,2162.909513950348,5.662022886099294e-07
640641,1281283,640641,1921924,2166.2527170181274,4.7268986236304045e-07
641642,1283285,641642,1924927,2169.620609998703,3.8729012885596603e-07
642643,1285287,642643,1927930,2172.985394716263,2.9898365028202534e-07
643644,1287289,643644,1930933,2176.3782167434692,2.3853135644458234e-07
644645,1289291,644645,1933936,2179.7315118312836,2.9460898076649755e-07
645646,1291293,645646,1936939,2183.029653787613,3.13548298436217e-07
646647,1293295,646647,1939942,2186.6036999225616,3.949917299905792e-07
647648,1295297,647648,1942945,2190.029095888138,4.6936111175455153e-07
648649,1297299,648649,1945948,2193.344050884247,5.307374522089958e-07
649650,1299301,649650,1948951,2196.6825518608093,6.056252459529787e-07
650651,1301303,650651,1951954,2199.997492790222,6.76422132528387e-07
651652,1303305,651652,1954957,2203.3046309947968,7.171238394221291e-07
652653,1305307,652653,1957960,2206.645674943924,7.327544153667986e-07
653654,1307309,653654,1960963,2210.00697183609,7.698599802097306e-07
654655,1309311,654655,1963966,2213.5097007751465,7.973740139277652e-07
655656,1311313,655656,1966969,2216.827816963196,7.994185580173507e-07
656657,1313315,656657,1969972,2220.149223804474,7.907965482445434e-07
657658,1315317,657658,1972975,2223.479085922241,7.759426807751879e-07
658659,1317319,658659,1975978,2226.8665347099304,7.44352291803807e-07
659660,1319321,659660,1978981,2230.226181745529,7.138460205169395e-07
660661,1321323,660661,1981984,2233.534094810486,7.291055226232857e-07
661662,1323325,661662,1984987,2236.9321868419647,7.61110641178675e-07
662663,1325327,662663,1987990,2240.28164601326,7.91455022408627e-07
663664,1327329,663664,1990993,2243.59157705307,8.0551762948744e-07
664665,1329331,664665,1993996,2247.0810039043427,8.038277883315459e-07
665666,1331333,665666,1996999,2250.5114607810974,7.969410944497213e-07
666667,1333335,666667,2000002,2253.85564994812,7.727376214461401e-07
667668,1335337,667668,2003005,2257.1991329193115,7.222133717732504e-07
668669,1337339,668669,2006008,2260.517646074295,6.737918738508597e-07
669670,1339341,669670,2009011,2263.864778995514,6.061200110707432e-07
670671,1341343,670671,2012014,2267.3847358226776,5.328693077899516e-07
671672,1343345,671672,2015017,2270.7351427078247,4.440607881406322e-07
672673,1345347,672673,2018020,2274.1889657974243,4.326011548982933e-07
673674,1347349,673674,2021023,2277.5143480300903,4.314661055104807e-07
674675,1349351,674675,2024026,2280.8719437122345,4.2762076191138476e-07
675676,1351353,675676,2027029,2284.242688894272,4.061475920025259e-07
676677,1353355,676677,2030032,2287.615129709244,3.7505742511712015e-07
677678,1355357,677678,2033035,2290.9381947517395,3.4119329939130694e-07
678679,1357359,678679,2036038,2294.276841878891,2.8307294996920973e-07
679680,1359361,679680,2039041,2297.666302919388,2.322267391718924e-07
680681,1361363,680681,2042044,2301.0023186206818,2.4695691536180675e-07
681682,1363365,681682,2045047,2304.3514099121094,2.692122507141903e-07
682683,1365367,682683,2048050,2307.685874938965,3.189616109011695e-07
683684,1367369,683684,2051053,2310.994111776352,4.0827944758348167e-07
684685,1369371,684685,2054056,2314.373694896698,5.268902896204963e-07
685686,1371373,685686,2057059,2317.7792880535126,6.099726306274533e-07
686687,1373375,686687,2060062,2321.0816848278046,6.597656465601176e-07
687688,1375377,687688,2063065,2324.4388148784637,6.900027074152604e-07
688689,1377379,688689,2066068,2327.7587130069733,6.85486156726256e-07
689690,1379381,689690,2069071,2331.095268011093,6.573573045898229e-07
690691,1381383,690691,2072074,2334.4736618995667,5.813108145957813e-07
691692,1383385,691692,2075077,2337.789163827896,4.841585905523971e-07
692693,1385387,692693,2078080,2341.347208738327,3.7790596252307296e-07
693694,1387389,693694,2081083,2344.9890048503876,3.080058377236128e-07
694695,1389391,694695,2084086,2348.592976808548,2.9839247872587293e-07
695696,1391393,695696,2087089,2352.1773447990417,2.6539055397734046e-07
696697,1393395,696697,2090092,2355.801466703415,2.3361280909739435e-07
697698,1395397,697698,2093095,2359.3661799430847,2.1744017431046814e-07
698699,1397399,698699,2096098,2362.9468488693237,2.4857945390976965e-07
699700,1399401,699700,2099101,2366.4984328746796,2.7363603294361383e-07
700701,1401403,700701,2102104,2370.1990377902985,2.8847716748714447e-07
701702,1403405,701702,2105107,2373.863328933716,3.0795308703090996e-07
702703,1405407,702703,2108110,2377.567544937134,3.2571188057772815e-07
703704,1407409,703704,2111113,2381.115528821945,3.40343831339851e-07
704705,1409411,704705,2114116,2384.7564747333527,4.107369022676721e-07
705706,1411413,705706,2117119,2388.3053879737854,4.5329215936362743e-07
706707,1413415,706707,2120122,2391.856246948242,4.985831765225157e-07
707708,1415417,707708,2123125,2395.433230638504,5.283909558784217e-07
708709,1417419,708709,2126128,2399.0514726638794,5.481815605890006e-07
709710,1419421,709710,2129131,2402.6496958732605,5.704805516870692e-07
710711,1421423,710711,2132134,2406.1587777137756,5.88577677262947e-07
711712,1423425,711712,2135137,2409.637622833252,5.873098416486755e-07
712713,1425427,712713,2138140,2413.189351797104,5.749134288635105e-07
713714,1427429,713714,2141143,2416.6089310646057,5.486836016643792e-07
714715,1429431,714715,2144146,2419.9526178836823,5.769215931650251e-07
715716,1431433,715716,2147149,2423.306659936905,5.843430699314922e-07
716717,1433435,716717,2150152,2426.68963766098,5.795500328531489e-07
717718,1435437,717718,2153155,2430.0826349258423,5.680158210452646e-07
718719,1437439,718719,2156158,2433.4022829532623,5.42187990504317e-07
719720,1439441,719720,2159161,2436.7531130313873,5.33800630364567e-07
720721,1441443,720721,2162164,2440.0932598114014,5.055590008851141e-07
721722,1443445,721722,2165167,2443.451955795288,4.699904820881784e-07
722723,1445447,722723,2168170,2446.8207290172577,4.664652806241065e-07
723724,1447449,723724,2171173,2450.1726336479187,4.6810055209789425e-07
724725,1449451,724725,2174176,2453.498039960861,4.526318662101403e-07
725726,1451453,725726,2177179,2456.8234329223633,4.074881871929392e-07
726727,1453455,726727,2180182,2460.188845872879,3.810491762124002e-07
727728,1455457,727728,2183185,2463.5431518554688,3.5266930353827775e-07
728729,1457459,728729,2186188,2466.9590740203857,3.020359145011753e-07
729730,1459461,729730,2189191,2470.4060158729553,2.2588574211113155e-07
730731,1461463,730731,2192194,2473.7648968696594,2.2697531676385552e-07
731732,1463465,731732,2195197,2477.188153028488,2.4579094315413386e-07
732733,1465467,732733,2198200,2480.8320128917694,2.3497887013945729e-07
733734,1467469,733734,2201203,2484.2185728549957,2.1999949240125716e-07
734735,1469471,734735,2204206,2487.6290810108185,2.855504135368392e-07
735736,1471473,735736,2207209,2491.0138998031616,3.2210664357990026e-07
736737,1473475,736737,2210212,2494.5857939720154,3.3036121749319136e-07
737738,1475477,737738,2213215,2498.1590209007263,3.4348704502917826e-07
738739,1477479,738739,2216218,2501.733561038971,4.427547537488863e-07
739740,1479481,739740,2219221,2505.1456248760223,5.080764822196215e-07
740741,1481483,740741,2222224,2508.498571872711,5.477486411109567e-07
741742,1483485,741742,2225227,2511.822506904602,5.692563718184829e-07
742743,1485487,742743,2228230,2515.196133852005,5.830443114973605e-07
743744,1487489,743744,2231233,2518.573725938797,5.574074748437852e-07
744745,1489491,744745,2234236,2521.9184839725494,4.911689757136628e-07
745746,1491493,745746,2237239,2525.2881088256836,3.792847564909607e-07
746747,1493495,746747,2240242,2528.6429579257965,2.95500285574235e-07
747748,1495497,747748,2243245,2531.9719128608704,2.591677912278101e-07
748749,1497499,748749,2246248,2535.3872780799866,2.267843228764832e-07
749750,1499501,749750,2249251,2538.7295129299164,2.213655534433201e-07
750751,1501503,750751,2252254,2542.118523836136,2.2252061171457171e-07
751752,1503505,751752,2255257,2545.4833788871765,2.4698420020285994e-07
752753,1505507,752753,2258260,2549.056109905243,2.520482667023316e-07
753754,1507509,753754,2261263,2552.5197789669037,2.7890928322449327e-07
754755,1509511,754755,2264266,2555.8569688796997,3.052027750527486e-07
755756,1511513,755756,2267269,2559.1965548992157,3.32052877638489e-07
756757,1513515,756757,2270272,2562.572772026062,3.7790960050188005e-07
757758,1515517,757758,2273275,2565.943960905075,4.3613363231997937e-07
758759,1517519,758759,2276278,2569.3141486644745,4.6215791371650994e-07
759760,1519521,759760,2279281,2572.659614801407,4.99227098771371e-07
760761,1521523,760761,2282284,2576.081696987152,5.138244887348264e-07
761762,1523525,761762,2285287,2579.446893930435,5.147267074789852e-07
762763,1525527,762763,2288290,2582.78342795372,5.22057234775275e-07
763764,1527529,763764,2291293,2586.246752977371,5.240763130132109e-07
764765,1529531,764765,2294296,2589.790513753891,5.371948645915836e-07
765766,1531533,765766,2297299,2593.1739089488983,5.743422661907971e-07
766767,1533535,766767,2300302,2596.573703765869,5.723086360376328e-07
767768,1535537,767768,2303305,2599.939079761505,5.547735781874508e-07
768769,1537539,768769,2306308,2603.3062777519226,5.602469173027202e-07
769770,1539541,769770,2309311,2606.6534008979797,5.415658961283043e-07
770771,1541543,770771,2312314,2609.986853837967,5.032852641306818e-07
771772,1543545,771772,2315317,2613.345346927643,5.159236025065184e-07
772773,1545547,772773,2318320,2616.6866879463196,4.989396984456107e-07
773774,1547549,773774,2321323,2620.0179347991943,4.822086339117959e-07
774775,1549551,774775,2324326,2623.37238073349,4.726280167233199e-07
775776,1551553,775776,2327329,2626.776696920395,4.7640605771448463e-07
776777,1553555,776777,2330332,2630.10737490654,4.4343505578581244e-07
777778,1555557,777778,2333335,2633.485723733902,3.9537917473353446e-07
778779,1557559,778779,2336338,2636.8037028312683,3.616751200752333e-07
779780,1559561,779780,2339341,2640.2582218647003,3.718669177033007e-07
780781,1561563,780781,2342344,2643.7216498851776,3.4513686841819435e-07
781782,1563565,781782,2345347,2647.112049818039,3.333771019242704e-07
782783,1565567,782783,2348350,2650.4609427452087,3.182722139172256e-07
783784,1567569,783784,2351353,2653.8015580177307,2.9480725061148405e-07
784785,1569571,784785,2354356,2657.1919298171997,2.6485940907150507e-07
785786,1571573,785786,2357359,2660.558469772339,2.3603206500411034e-07
786787,1573575,786787,2360362,2663.9235787391663,2.421038516331464e-07
787788,1575577,787788,2363365,2667.382682800293,2.842698449967429e-07
788789,1577579,788789,2366368,2670.7651257514954,3.236782504245639e-07
789790,1579581,789790,2369371,2674.127415895462,3.4125332604162395e-07
790791,1581583,790791,2372374,2677.5025577545166,4.0368104237131774e-07
791792,1583585,791792,2375377,2680.83575963974,4.77926732855849e-07
792793,1585587,792793,2378380,2684.1878519058228,4.928369889967144e-07
793794,1587589,793794,2381383,2687.59303689003,5.038546078139916e-07
794795,1589591,794795,2384386,2690.973785638809,4.834382707485929e-07
795796,1591593,795796,2387389,2694.3182888031006,4.309513315092772e-07
796797,1593595,796797,2390392,2697.6306517124176,3.98553311242722e-07
797798,1595597,797798,2393395,2700.968964099884,3.5352968552615494e-07
798799,1597599,798799,2396398,2704.3045728206635,3.1273339118342847e-07
799800,1599601,799800,2399401,2707.690342903137,2.6143970899283886e-07
800801,1601603,800801,2402404,2711.057580947876,2.1404412109404802e-07
801802,1603605,801802,2405407,2714.455258846283,1.6667581803631037e-07
802803,1605607,802803,2408410,2718.0116958618164,1.250937202712521e-07
803804,1607609,803804,2411413,2721.404397010803,1.73185981111601e-07
804805,1609611,804805,2414416,2724.828003883362,2.430078893667087e-07
805806,1611613,805806,2417419,2728.3803420066833,2.868946467060596e-07
806807,1613615,806807,2420422,2731.7950489521027,3.166969690937549e-07
807808,1615617,807808,2423425,2735.1294298171997,3.275981725892052e-07
808809,1617619,808809,2426428,2738.482890844345,3.313216438982636e-07
809810,1619621,809810,2429431,2741.8304028511047,3.459317667875439e-07
810811,1621623,810811,2432434,2745.1932756900787,3.7838981370441616e-07
811812,1623625,811812,2435437,2748.5431637763977,4.2545070755295455e-07
812813,1625627,812813,2438440,2751.9575958251953,4.42723830929026e-07
813814,1627629,813814,2441443,2755.334326982498,4.3546606320887804e-07
814815,1629631,814815,2444446,2758.6826667785645,4.366975190350786e-07
815816,1631633,815816,2447449,2762.0093936920166,4.309858923079446e-07
816817,1633635,816817,2450452,2765.399605989456,4.0371742215938866e-07
817818,1635637,817818,2453455,2768.9500148296356,4.407484084367752e-07
818819,1637639,818819,2456458,2772.336045026779,4.38598362961784e-07
819820,1639641,819820,2459461,2775.7244367599487,4.457215254660696e-07
820821,1641643,820821,2462464,2779.0312576293945,4.366393113741651e-07
821822,1643645,821822,2465467,2782.399475812912,3.951026883441955e-07
822823,1645647,822823,2468470,2785.7665598392487,3.5291850508656353e-07
823824,1647649,823824,2471473,2789.116938829422,3.429013304412365e-07
824825,1649651,824825,2474476,2792.523750782013,3.488203219603747e-07
825826,1651653,825826,2477479,2795.931133747101,3.575351001927629e-07
826827,1653655,826827,2480482,2799.2977378368378,3.5506127460394055e-07
827828,1655657,827828,2483485,2802.658113002777,3.313780325697735e-07
828829,1657659,828829,2486488,2806.0331819057465,3.0059527489356697e-07
829830,1659661,829830,2489491,2809.3653450012207,2.546385076129809e-07
830831,1661663,830831,2492494,2812.7127289772034,2.62436515185982e-07
831832,1663665,831832,2495497,2816.0646529197693,2.417909854557365e-07
832833,1665667,832833,2498500,2819.402941942215,2.2098720364738256e-07
833834,1667669,833834,2501503,2822.7412757873535,1.9639628590084612e-07
834835,1669671,834835,2504506,2826.1210889816284,1.5691330190747976e-07
835836,1671673,835836,2507509,2829.462189912796,1.4309625839814544e-07
836837,1673675,836837,2510512,2832.972541809082,1.666376192588359e-07
837838,1675677,837838,2513515,2836.4899230003357,1.9352046365384012e-07
838839,1677679,838839,2516518,2839.8408739566803,2.3762731871102005e-07
839840,1679681,839840,2519521,2843.169455051422,2.75349520961754e-07
840841,1681683,840841,2522524,2846.535467863083,3.270633897045627e-07
841842,1683685,841842,2525527,2849.8867378234863,3.582645149435848e-07
842843,1685687,842843,2528530,2853.3397579193115,3.6044730222783983e-07
843844,1687689,843844,2531533,2856.7247507572174,3.4501863410696387e-07
844845,1689691,844845,2534536,2860.082932949066,3.260502126067877e-07
845846,1691693,845846,2537539,2863.446703672409,3.0581941246055067e-07
846847,1693695,846847,2540542,2866.7999918460846,2.5199915398843586e-07
847848,1695697,847848,2543545,2870.14604473114,2.2792482923250645e-07
848849,1697699,848849,2546548,2873.4950358867645,1.961889211088419e-07
849850,1699701,849850,2549551,2876.8115010261536,1.490570866735652e-07
850851,1701703,850851,2552554,2880.178748846054,1.1418887879699469e-07
851852,1703705,851852,2555557,2883.631045818329,1.136340870289132e-07
852853,1705707,852853,2558560,2887.0137248039246,1.4170473150443286e-07
853854,1707709,853854,2561563,2890.4934458732605,1.9376420823391527e-07
854855,1709711,854855,2564566,2894.0333647727966,2.2726271708961576e-07
855856,1711713,855856,2567569,2897.4057557582855,2.285451046191156e-07
856857,1713715,856857,2570572,2900.769302845001,2.3287248041015118e-07
857858,1715717,857858,2573575,2904.0975608825684,2.753276930889115e-07
858859,1717719,858859,2576578,2907.7439296245575,3.1017771107144654e-07
859860,1719721,859860,2579581,2911.196954727173,3.4653385228011757e-07
860861,1721723,860861,2582584,2914.53271484375,3.601217031246051e-07
861862,1723725,861862,2585587,2917.9525718688965,3.431032382650301e-07
862863,1725727,862863,2588590,2921.30867767334,3.333061613375321e-07
863864,1727729,863864,2591593,2924.6771008968353,3.3754440664779395e-07
864865,1729731,864865,2594596,2928.0406687259674,3.631557774497196e-07
865866,1731733,865866,2597599,2931.3724689483643,3.770783223444596e-07
866867,1733735,866867,2600602,2934.8189659118652,3.6369783629197627e-07
867868,1735737,867868,2603605,2938.1824939250946,3.317109076306224e-07
868869,1737739,868869,2606608,2941.5234138965607,3.0756746127735823e-07
869870,1739741,869870,2609611,2944.8628237247467,3.1139279599301517e-07
870871,1741743,870871,2612614,2948.222597837448,3.346303856233135e-07
871872,1743745,871872,2615617,2951.5836358070374,3.399945853743702e-07
872873,1745747,872873,2618620,2954.952749967575,3.353961801622063e-07
873874,1747749,873874,2621623,2958.3097746372223,3.0366936698555946e-07
874875,1749751,874875,2624626,2961.6502487659454,2.603028406156227e-07
875876,1751753,875876,2627629,2964.981602907181,2.579909050837159e-07
876877,1753755,876877,2630632,2968.336993932724,2.505057636881247e-07
877878,1755757,877878,2633635,2971.702888727188,2.3379834601655602e-07
878879,1757759,878879,2636638,2975.0580348968506,2.045107976300642e-07
879880,1759761,879880,2639641,2978.381778717041,1.6668309399392456e-07
880881,1761763,880881,2642644,2981.7144918441772,1.3501266948878765e-07
881882,1763765,881882,2645647,2985.137753009796,1.4763827493879944e-07
882883,1765767,882883,2648650,2988.4792668819427,2.0093102648388594e-07
883884,1767769,883884,2651653,2991.803330898285,2.3217762645799667e-07
884885,1769771,884885,2654656,2995.149104833603,2.3726897779852152e-07
885886,1771773,885886,2657659,2998.560354948044,2.659744495758787e-07
886887,1773775,886887,2660662,3001.959501028061,2.899978426285088e-07
887888,1775777,887888,2663665,3005.3619499206543,3.1584750104229897e-07
888889,1777779,888889,2666668,3008.703655719757,3.462882887106389e-07
889890,1779781,889890,2669671,3012.0400519371033,3.3883407013490796e-07
890891,1781783,890891,2672674,3015.4167239665985,3.098975867033005e-07
891892,1783785,891892,2675677,3018.723645925522,2.8955946618225425e-07
892893,1785787,892893,2678680,3022.10085773468,2.505257725715637e-07
893894,1787789,893894,2681683,3025.602516889572,2.275737642776221e-07
894895,1789791,894895,2684686,3028.9553320407867,1.8968239601235837e-07
895896,1791793,895896,2687689,3032.293907880783,1.7853017197921872e-07
896897,1793795,896897,2690692,3035.6256239414215,1.5821387933101505e-07
897898,1795797,897898,2693695,3038.9762217998505,1.5248951967805624e-07
898899,1797799,898899,2696698,3042.29354596138,1.9299295672681183e-07
899900,1799801,899900,2699701,3045.8574788570404,1.961179805221036e-07
900901,1801803,900901,2702704,3049.252091884613,2.3546635929960757e-07
901902,1803805,901902,2705707,3052.595841884613,2.7532587409950793e-07
902903,1805807,902903,2708710,3055.948115825653,2.7866735763382167e-07
903904,1807809,903904,2711713,3059.298274040222,3.0880619306117296e-07
904905,1809811,904905,2714716,3062.6125848293304,3.1686249712947756e-07
905906,1811813,905906,2717719,3065.9662158489227,3.1932540878187865e-07
906907,1813815,906907,2720722,3069.3295137882233,3.3487958717159927e-07
907908,1815817,907908,2723725,3072.7683777809143,3.1546551326755434e-07
908909,1817819,908909,2726728,3076.184080839157,3.385466698091477e-07
909910,1819821,909910,2729731,3079.7368218898773,3.393597580725327e-07
910911,1821823,910911,2732734,3083.285616874695,3.271306923124939e-07
911912,1823825,911912,2735737,3086.7788898944855,3.4044387575704604e-07
912913,1825827,912913,2738740,3090.3413166999817,3.310487954877317e-07
913914,1827829,913914,2741743,3093.8978548049927,3.101595211774111e-07
914915,1829831,914915,2744746,3097.4406628608704,3.198947524651885e-07
915916,1831833,915916,2747749,3100.988464832306,3.250825102441013e-07
916917,1833835,916917,2750752,3104.53076505661,3.16464138450101e-07
917918,1835837,917918,2753755,3108.1133749485016,3.0164119380060583e-07
918919,1837839,918919,2756758,3111.6317517757416,2.802444214466959e-07
919920,1839841,919920,2759761,3115.1493589878082,2.590059011708945e-07
920921,1841843,920921,2762764,3118.6722779273987,2.3258871806319803e-07
921922,1843845,921922,2765767,3122.1966960430145,2.0388506527524441e-07
922923,1845847,922923,2768770,3125.7525837421417,1.5461228031199425e-07
923924,1847849,923924,2771773,3129.2367708683014,1.1314659786876291e-07
924925,1849851,924925,2774776,3132.7631437778473,1.5072873793542385e-07
925926,1851853,925926,2777779,3136.544819831848,1.8017817637883127e-07
926927,1853855,926927,2780782,3140.119395971298,1.9045182853005826e-07
927928,1855857,927928,2783785,3143.4628326892853,2.1717460185755044e-07
928929,1857859,928929,2786788,3146.815757036209,2.2177664504852146e-07
929930,1859861,929930,2789791,3150.180845975876,2.1206506062299013e-07
930931,1861863,930931,2792794,3153.50567984581,2.5179542717523873e-07
931932,1863865,931932,2795797,3156.848834991455,2.9376860766205937e-07
932933,1865867,932933,2798800,3160.2191178798676,3.0903538572601974e-07
933934,1867869,933934,2801803,3163.922610759735,3.0839692044537514e-07
934935,1869871,934935,2804806,3167.437198638916,2.699853212106973e-07
935936,1871873,935936,2807809,3170.781240940094,2.296401362400502e-07
936937,1873875,936937,2810812,3174.1401529312134,2.2062522475607693e-07
937938,1875877,937938,2813815,3177.4584419727325,1.8323225958738476e-07
938939,1877879,938939,2816818,3180.7974169254303,1.685057213762775e-07
939940,1879881,939940,2819821,3184.132519721985,1.4436591300182045e-07
940941,1881883,940941,2822824,3187.496976852417,1.3246608432382345e-07
941942,1883885,941942,2825827,3190.845478773117,1.517419150331989e-07
942943,1885887,942943,2828830,3194.1714799404144,1.5691330190747976e-07
943944,1887889,943944,2831833,3197.556802034378,1.7155252862721682e-07
944945,1889891,944945,2834836,3200.863602876663,1.8687751435209066e-07
945946,1891893,945946,2837839,3204.192484855652,2.1764753910247236e-07
946947,1893895,946947,2840842,3207.537854909897,2.3135544324759394e-07
947948,1895897,947948,2843845,3210.864778995514,2.4248583940789104e-07
948949,1897899,948949,2846848,3214.2110798358917,2.592205419205129e-07
949950,1899901,949950,2849851,3217.529653787613,2.587003109510988e-07
950951,1901903,950951,2852854,3220.935975790024,2.600936568342149e-07
951952,1903905,951952,2855857,3224.4365496635437,2.6375164452474564e-07
952953,1905907,952953,2858860,3227.763368844986,2.5536610337439924e-07
953954,1907909,953954,2861863,3231.332232952118,2.6638554118108004e-07
954955,1909911,954955,2864866,3234.71488571167,2.9003604140598327e-07
955956,1911913,955956,2867869,3237.9009346961975,2.8636168281082064e-07
956957,1913915,956957,2870872,3241.0342268943787,2.9691000236198306e-07
957958,1915917,957958,2873875,3244.1298489570618,2.905089786509052e-07
958959,1917919,958959,2876878,3247.3357439041138,2.6062662072945386e-07
959960,1919921,959960,2879881,3251.1923367977142,2.3292523110285401e-07
960961,1921923,960961,2882884,3254.4287190437317,2.3619213607162237e-07
961962,1923925,961962,2885887,3257.905884742737,2.2354288375936449e-07
962963,1925927,962963,2888890,3262.3448498249054,1.951775630004704e-07
963964,1927929,963964,2891893,3268.1463720798492,1.775133569026366e-07
964965,1929931,964965,2894896,3273.026039838791,1.5540172171313316e-07
965966,1931933,965966,2897899,3277.053373813629,1.1267366062384099e-07
966967,1933935,966967,2900902,3281.3801758289337,8.802453521639109e-08
967968,1935937,967968,2903905,3285.6122159957886,8.866481948643923e-08
968969,1937939,968969,2906908,3289.753588914871,7.958078640513122e-08
969970,1939941,969970,2909911,3294.256540775299,1.2703640095423907e-07
970971,1941943,970971,2912914,3297.9290838241577,1.4981742424424738e-07
971972,1943945,971972,2915917,3301.7234978675842,1.782282197382301e-07
972973,1945947,972973,2918920,3305.2544119358063,2.1333471522666514e-07
973974,1947949,973974,2921923,3309.1423938274384,2.2198764781933278e-07
974975,1949951,974975,2924926,3312.9348180294037,2.520791895221919e-07
975976,1951953,975976,2927929,3316.8008377552032,2.5289591576438397e-07
976977,1953955,976977,2930932,3320.454509973526,2.6283123588655144e-07
977978,1955957,977978,2933935,3324.095536708832,2.249398676212877e-07
978979,1957959,978979,2936938,3327.9381999969482,2.2216408979147673e-07
979980,1959961,979980,2939941,3331.585175037384,2.075139491353184e-07
980981,1961963,980981,2942944,3335.5409858226776,1.8570972315501422e-07
981982,1963965,981982,2945947,3339.3902127742767,1.704411261016503e-07
982983,1965967,982983,2948950,3343.1723136901855,1.2574673746712506e-07
983984,1967969,983984,2951953,3346.7480187416077,7.755625119898468e-08
984985,1969971,984985,2954956,3350.2226927280426,8.520146366208792e-08
985986,1971973,985986,2957959,3353.805943965912,1.128009898820892e-07
986987,1973975,986987,2960962,3357.6238539218903,1.334356056759134e-07
987988,1975977,987988,2963965,3361.109556913376,1.5796103980392218e-07
988989,1977979,988989,2966968,3365.4896879196167,1.6153353499248624e-07
989990,1979981,989990,2969971,3369.824367761612,1.554435584694147e-07
990991,1981983,990991,2972974,3374.2988719940186,1.7871752788778394e-07
991992,1983985,991992,2975977,3377.9148190021515,2.1089908841531724e-07
992993,1985987,992993,2978980,3381.945502758026,2.387914719292894e-07
993994,1987989,993994,2981983,3385.275140762329,2.537417458370328e-07
994995,1989991,994995,2984986,3388.5555629730225,2.6130874175578356e-07
995996,1991993,995996,2987989,3392.094361782074,2.7021815185435116e-07
996997,1993995,996997,2990992,3395.7904148101807,2.747656253632158e-07
997998,1995997,997998,2993995,3399.44744181633,2.6434281608089805e-07
998999,1997999,998999,2996998,3403.761720895767,2.6790075935423374e-07
1000000,2000001,1000000,3000001,3407.6098589897156,2.7104761102236807e-07


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002299785614013672,12064.709122577777
2002,2003,2002,4005,4.75390100479126,60.67671186811822
4004,4005,4004,8009,9.179544925689697,40.02609617545022
6006,6007,6006,12013,13.806530952453613,32.13797708286802
8008,8009,8008,16017,18.536274909973145,27.246786066505592
10010,10011,10010,20021,23.83765196800232,23.723299817738734
12012,12013,12012,24025,28.585903882980347,20.989859030964
14014,14015,14014,28029,32.98323893547058,18.776198956609733
16016,16017,16016,32033,37.389081954956055,16.934860506264158
18018,18019,18018,36037,41.90768313407898,15.375758415093514
20020,20021,20020,40041,46.458094120025635,14.038860967322762
22022,22023,22022,44045,50.93951988220215,12.881498903649117
24024,24025,24024,48049,55.376060962677,11.871907541533801
26026,26027,26026,52053,59.79984092712402,10.98564499834174
28028,28029,28028,56057,64.16934204101562,10.20344186195689
30030,30031,30030,60061,68.58322882652283,9.509827417139604
32032,32033,32032,64065,73.0224277973175,8.89219817101548
34034,34035,34034,68069,77.4310851097107,8.340162209044138
36036,36037,36036,72073,81.85543990135193,7.845063883871262
38038,38039,38038,76077,86.2601227760315,7.399629918034407
40040,40041,40040,80081,90.88143110275269,6.997701481135664
42042,42043,42042,84085,95.27119588851929,6.634028092285007
44044,44045,44044,88089,99.68200707435608,6.304106939418489
46046,46047,46046,92093,104.10074591636658,6.004056088931975
48048,48049,48048,96097,108.60720896720886,5.730513324713684
50050,50051,50050,100101,113.03764796257019,5.480554602134362
52052,52053,52052,104105,117.41631197929382,5.251627681196624
54054,54055,54054,108109,121.85888314247131,5.041497629967125
56056,56057,56056,112113,126.2500491142273,4.848201704922758
58058,58059,58058,116117,130.64207792282104,4.670011710717517
60060,60061,60060,120121,135.01412796974182,4.505402381795648
62062,62063,62062,124125,139.41858577728271,4.353024655658373
64064,64065,64064,128129,143.82268595695496,4.211682953255149
66066,66067,66066,132133,148.24550604820251,4.080315767972934
68068,68069,68068,136137,152.6328158378601,3.9579790064890403
70070,70071,70070,140141,156.9849009513855,3.8438316339797893
72072,72073,72072,144145,161.39062309265137,3.7371232607620186
74074,74075,74074,148149,165.78386688232422,3.637183463866677
76076,76077,76076,152153,170.35667991638184,3.5434122191090864
78078,78079,78078,156157,174.70426988601685,3.455271782277123
80080,80081,80080,160161,179.05490684509277,3.372279685723697
82082,82083,82082,164165,183.42714285850525,3.2940024048857595
84084,84085,84084,168169,187.81218886375427,3.2200498701367906
86086,86087,86086,172173,192.23461890220642,3.1500706432252628
88088,88089,88088,176177,196.61578702926636,3.0837476713004435
90090,90091,90090,180181,201.02780175209045,3.0207945441597985
92092,92093,92092,184185,205.39346408843994,2.960952190687749
94094,94095,94094,188189,209.76182103157043,2.903985959379497
96096,96097,96096,192193,214.1278998851776,2.849683035279668
98098,98099,98098,196197,218.48798394203186,2.7978501520228747
100100,100101,100100,200201,222.96164512634277,2.7483115630911925
102102,102103,102102,204205,227.35588788986206,2.7009072410255612
104104,104105,104104,208209,231.71004009246826,2.6554912774245167
106106,106107,106106,212213,236.0722680091858,2.61193045985965
108108,108109,108108,216217,240.47041988372803,2.5701030049676774
110110,110111,110110,220221,244.8715558052063,2.5298974294582877
112112,112113,112112,224225,249.3859510421753,2.49121154308159
114114,114115,114114,228229,253.93149590492249,2.453951549479825
116116,116117,116116,232233,258.3166968822479,2.4180312426651653
118118,118119,118118,236237,262.70561480522156,2.3833712882224063
120120,120121,120120,240241,267.083379983902,2.34989857967048
122122,122123,122122,244245,271.49806094169617,2.3175456616263546
124124,124125,124124,248249,275.97581481933594,2.286250212287996
126126,126127,126126,252253,280.36494398117065,2.2559545787007664
128128,128129,128128,256257,284.8008179664612,2.2266053590283263
130130,130131,130130,260261,289.2810549736023,2.198153026674845
132132,132133,132132,264265,293.66827297210693,2.17055159175834
134134,134135,134134,268269,298.0662851333618,2.143758295880616
136136,136137,136136,272273,302.45581102371216,2.1177333513569465
138138,138139,138138,276277,306.82402300834656,2.092439649719381
140140,140141,140140,280281,311.2592279911041,2.0678425762762345
142142,142143,142142,284285,315.6270411014557,2.0439097965718247
144144,144145,144144,288289,320.04482793807983,2.02061107002919
146146,146147,146146,292293,324.4516439437866,1.9979180825139338
148148,148149,148148,296297,328.8220191001892,1.9758042942758038
150150,150151,150150,300301,333.22871804237366,1.9542448017436982
152152,152153,152152,304305,337.60684084892273,1.9332162117461849
154154,154155,154154,308309,342.0134038925171,1.9126965269679204
156156,156157,156156,312313,346.3915808200836,1.8926650414832693
158158,158159,158158,316317,350.782488822937,1.8731022454157937
160160,160161,160160,320321,355.13146805763245,1.8539897377941088
162162,162163,162162,324325,359.52449679374695,1.835310146883785
164164,164165,164164,328329,363.8648729324341,1.8170470572022168
166166,166167,166166,332333,368.22841691970825,1.7991849426452973
168168,168169,168168,336337,372.6263380050659,1.7817091051256284
170170,170171,170170,340341,377.02136874198914,1.7646056182147731
172172,172173,172172,344345,381.43832182884216,1.747861275312971
174174,174175,174174,348349,385.8674638271332,1.7314635419861588
176176,176177,176176,352353,390.5388789176941,1.715400538443646
178178,178179,178178,356357,394.9487929344177,1.6996609200305102
180180,180181,180180,360361,399.36937403678894,1.6842339163158613
182182,182183,182182,364365,403.7784860134125,1.6691092750515963
184184,184185,184184,368369,408.2091820240021,1.6542772278389748
186186,186187,186186,372373,412.6572849750519,1.6397284605573077
188188,188189,188188,376377,417.09700298309326,1.6254540859663393
190190,190191,190190,380381,421.4944038391113,1.6114456182913273
192192,192193,192192,384385,425.86330914497375,1.5976949496543966
194194,194195,194194,388389,430.2623689174652,1.5841943281520798
196196,196197,196196,392393,434.6337699890137,1.5709363374971872
198198,198199,198198,396397,439.03688406944275,1.5579138780340145
200200,200201,200200,400401,443.4321959018707,1.5451201491068787
202202,202203,202202,404405,448.0033800601959,1.532548632572798
204204,204205,204204,408409,452.5551071166992,1.5201930774546781
206206,206207,206206,412413,456.92317605018616,1.5080474855803914
208208,208209,208208,416417,461.32906198501587,1.496106098198652
210210,210211,210210,420421,465.7057468891144,1.484363383417076
212212,212213,212212,424425,470.16528391838074,1.4728140244824317
214214,214215,214214,428429,474.63135385513306,1.4614529087866686
216216,216217,216216,432433,479.0395667552948,1.4502751175496087
218218,218219,218218,436437,483.4170660972595,1.4392759161673894
220220,220221,220220,440441,487.7992398738861,1.4284507451247919
222222,222223,222222,444445,492.18144488334656,1.4177952114714572
224224,224225,224224,448449,496.53914403915405,1.4073050808110565
226226,226227,226226,452453,501.00561475753784,1.3969762697433907
228228,228229,228228,456457,505.4425790309906,1.386804838793978
230230,230231,230230,460461,509.88569712638855,1.3767869856928883
232232,232233,232232,464465,514.2478201389313,1.3669190390992298
234234,234235,234234,468469,518.5970029830933,1.357197452622131
236236,236237,236236,472473,523.0150117874146,1.347618799249176
238238,238239,238238,476477,527.5157949924469,1.338179766002213
240240,240241,240240,480481,532.0613729953766,1.3288771489569626
242242,242243,242242,484485,536.4400818347931,1.3197078484918165
244244,244245,244244,488489,540.8856220245361,1.310668864809486
246246,246247,246246,492493,545.3025758266449,1.3017572936932993
248248,248249,248248,496497,549.7405200004578,1.2929703224872355
250250,250251,250250,500501,554.094349861145,1.2843052262815036
252252,252253,252252,504505,558.4840829372406,1.2757593643164
254254,254255,254254,508509,562.8595368862152,1.2673301765316864
256256,256257,256256,512513,567.2532279491425,1.2590151803233312
258258,258259,258258,516517,571.6063737869263,1.2508119674639602
260260,260261,260260,520521,576.010244846344,1.2427182011360856
262262,262263,262262,524525,580.5504689216614,1.2347316131745174
264264,264265,264264,528529,584.9281978607178,1.2268500013851735
266266,266267,266266,532533,589.3509769439697,1.219071227022141
268268,268269,268268,536537,593.7068119049072,1.2113932123829727
270270,270271,270270,540541,598.0449941158295,1.203813939850079
272272,272273,272272,544545,602.4472188949585,1.1963314624736086
274274,274275,274274,548549,606.8187148571014,1.1889438553316722
276276,276277,276276,552553,611.2700209617615,1.1816492630023276
278278,278279,278278,556557,615.6358017921448,1.1744458806606417
280280,280281,280280,560561,619.9970149993896,1.1673319522542442
282282,282283,282282,564565,624.3961217403412,1.160305768786202
284284,284285,284284,568569,628.7423319816589,1.1533656666488241
286286,286287,286286,572573,633.1303060054779,1.1465100260484178
288288,288289,288288,576577,637.516704082489,1.1397372694882506
290290,290291,290290,580581,641.9389131069183,1.1330458603260922
292292,292293,292292,584585,646.311420917511,1.1264343013790494
294294,294295,294294,588589,650.7278399467468,1.1199011336175317
296296,296297,296296,592593,655.0723321437836,1.11344493487195
298298,298299,298298,596597,659.4302468299866,1.1070643186194502
300300,300301,300300,600601,663.7925679683685,1.1007579328252177
302302,302303,302302,604605,668.1835100650787,1.0945244588256173
304304,304305,304304,608609,672.5390751361847,1.0883626102331618
306306,306307,306306,612613,676.9105489253998,1.082271131921516
308308,308309,308308,616617,681.3031768798828,1.076248799030509
310310,310311,310310,620621,685.7174229621887,1.0702944160275365
312312,312313,312312,624625,690.1975729465485,1.0644068157689617
314314,314315,314314,628629,694.5925409793854,1.0585848586415523
316316,316317,316316,632633,699.0168449878693,1.0528274317221076
318318,318319,318318,636637,703.3981809616089,1.0471334479461802
320320,320321,320320,640641,707.9090218544006,1.0415018453422817
322322,322323,322322,644645,712.4492938518524,1.0359315862733638
324324,324325,324324,648649,716.7220408916473,1.0304216567219555
326326,326327,326326,652653,721.0660517215729,1.0249710655825766
328328,328329,328328,656657,725.426558971405,1.019578844003263
330330,330331,330330,660661,729.764307975769,1.0142440447234549
332332,332333,332332,664665,734.167888879776,1.0089657414646354
334334,334335,334334,668669,738.5385699272156,1.0037430283264257
336336,336337,336336,672673,742.945562839508,0.9985750192026899
338338,338339,338338,676677,747.3908109664917,0.9934608472267428
340340,340341,340340,680681,751.7743430137634,0.9883996642292914
342342,342343,342342,684685,756.1731939315796,0.9833906402254797
344344,344345,344344,688689,760.5867321491241,0.9784329629019339
346346,346347,346346,692693,765.0272047519684,0.9735258371438249
348348,348349,348348,696697,769.4548099040985,0.9686684845528362
350350,350351,350350,700701,773.8356747627258,0.9638601430033304
352352,352353,352352,704705,778.2111659049988,0.9591000662076112
354354,354355,354354,708709,782.5542118549347,0.9543875232830032
356356,356357,356356,712713,786.9037868976593,0.9497217983534938
358358,358359,358358,716717,791.3318519592285,0.9451021901440981
360360,360361,360360,720721,795.8266377449036,0.9405280116079666
362362,362363,362362,724725,800.5788087844849,0.9359985895553109
364364,364365,364364,728729,805.0265128612518,0.9315132642823301
366366,366367,366366,732733,809.4183518886566,0.9270713892492495
368368,368369,368368,736737,813.8071219921112,0.922672330712885
370370,370371,370370,740741,818.1642508506775,0.9183154674301477
372372,372373,372372,744745,822.6156969070435,0.9140001903324446
374374,374375,374374,748749,827.1003530025482,0.9097259022128128
376376,376377,376376,752753,831.5335049629211,0.9054920174439758
378378,378379,378378,756757,835.9024798870087,0.9012979616836674
380380,380381,380380,760761,840.3295738697052,0.8971431715981453
382382,382383,382382,764765,844.7072830200195,0.8930270945929806
384384,384385,384384,768769,849.0909860134125,0.8889491885511234
386386,386387,386386,772773,853.5131499767303,0.8849089215855201
388388,388389,388388,776777,857.9231760501862,0.8809057717880933
390390,390391,390390,780781,862.267523765564,0.8769392269859964
392392,392393,392392,784785,866.8803699016571,0.8730087845233356
394394,394395,394394,788789,871.3310639858246,0.8691139510210633
396396,396397,396396,792793,875.7284290790558,0.8652542421750695
398398,398399,398398,796797,880.1474330425262,0.8614291825306282
400400,400401,400400,800801,884.6075329780579,0.8576383052841265
402402,402403,402402,804805,889.002434015274,0.8538811520793388
404404,404405,404404,808809,893.3629169464111,0.8501572728164319
406406,406407,406406,812813,897.7352600097656,0.846466225462791
408408,408409,408408,816817,902.1206867694855,0.8428075758638442
410410,410411,410410,820821,906.4962041378021,0.8391808975757158
412412,412413,412412,824825,910.9148721694946,0.8355857716796891
414414,414415,414414,828829,915.3261828422546,0.8320217866221356
416416,416417,416416,832833,919.6794791221619,0.8284885380508058
418418,418419,418418,836837,924.1404778957367,0.8249856286402064
420420,420421,420420,840841,928.5249898433685,0.8215126679679088
422422,422423,422422,844845,932.904953956604,0.8180692723235552
424424,424425,424424,848849,937.2769160270691,0.8146550645979005
426426,426427,426426,852853,941.6724629402161,0.811269674115465
428428,428429,428428,856857,946.0248458385468,0.8079127365126624
430430,430431,430430,860861,950.4559328556061,0.8045838935813663
432432,432433,432432,864865,954.8530869483948,0.8012827931615902
434434,434435,434434,868869,959.2228689193726,0.7980090889923304
436436,436437,436436,872873,963.5849158763885,0.7947624406006071
438438,438439,438438,876877,967.9454128742218,0.7915425131723168
440440,440441,440440,880881,972.6091477870941,0.7883489774321788
442442,442443,442442,884885,977.0028448104858,0.7851815095327765
444444,444445,444444,888889,981.4284858703613,0.7820397909363237
446446,446447,446446,892893,985.8608529567719,0.7789235083146195
448448,448449,448448,896897,990.2463150024414,0.7758323534308147
450450,450451,450450,900901,994.6684308052063,0.7727660230393667
452452,452453,452452,904905,999.0369300842285,0.7697242187823576
454454,454455,454454,908909,1003.4034371376038,0.7667066470985446
456456,456457,456456,912913,1007.7725598812103,0.7637130191124015
458458,458459,458458,916917,1012.226814031601,0.7607430505486263
460460,460461,460460,920921,1016.5578548908234,0.7577964616448298
462462,462463,462462,924925,1020.9164500236511,0.7548729770442151
464464,464465,464464,928929,1025.2912409305573,0.7519723257282749
466466,466467,466466,932933,1029.6885449886322,0.7490942409167474
468468,468469,468468,936937,1034.0666999816895,0.7462384599875804
470470,470471,470470,940941,1038.4337029457092,0.7434047244023532
472472,472473,472472,944945,1042.779042005539,0.7405927796171454
474474,474475,474474,948949,1047.1462180614471,0.7378023750097782
476476,476477,476476,952953,1051.4985411167145,0.7350332637979591
478478,478479,478478,956957,1055.8904139995575,0.7322852029774367
480480,480481,480480,960961,1060.2620449066162,0.7295579532365082
482482,482483,482482,964965,1064.6203830242157,0.7268512788923545
484484,484485,484484,968969,1069.0078389644623,0.7241649478219188
486486,486487,486486,972973,1073.3649060726166,0.721498731390966
488488,488489,488488,976977,1077.7545139789581,0.718852404395875
490490,490491,490490,980981,1082.1159839630127,0.7162257449817844
492492,492493,492492,984985,1086.5132038593292,0.7136185345989361
494494,494495,494494,988989,1090.8888368606567,0.7110305579390115
496496,496497,496496,992993,1095.2396659851074,0.7084616028569144
498498,498499,498498,996997,1099.6360340118408,0.7059114603343914
500501,500502,500501,1001003,1104.0058579444885,0.7033786645224609
502503,502504,502503,1005007,1108.6708171367645,0.7008655413810629
504505,504506,504505,1009011,1113.2286758422852,0.698370621768845
506507,506508,506507,1013015,1117.5976388454437,0.6958937085728394
508509,508510,508509,1017019,1122.0014321804047,0.6934346094440116
510511,510512,510511,1021023,1126.367660999298,0.6909931340996991
512513,512514,512513,1025027,1130.7462258338928,0.6885690906437958
514515,514516,514515,1029031,1135.1936049461365,0.6861622930264275
516517,516518,516517,1033035,1139.5439591407776,0.6837725578443496
518519,518520,518519,1037039,1143.8742830753326,0.6813997042936535
520521,520522,520521,1041043,1148.23859500885,0.6790435541115585
522523,522524,522523,1045047,1152.6129958629608,0.6767039315491274
524525,524526,524525,1049051,1156.9944698810577,0.6743806633166969
526527,526528,526527,1053055,1161.3789761066437,0.6720735785365832
528529,528530,528529,1057059,1165.7357399463654,0.669782508717617
530531,530532,530531,1061063,1170.1701860427856,0.6675072972830094
532533,532534,532533,1065067,1174.5388419628143,0.6652478156047437
534535,534536,534535,1069071,1178.9089329242706,0.6630038568546297
536537,536538,536537,1073075,1183.2834270000458,0.660775261638264
538539,538540,538539,1077079,1187.6624789237976,0.6585618727294786
540541,540542,540541,1081083,1192.0618679523468,0.6563635350485129
542543,542544,542543,1085087,1196.4292569160461,0.6541800956256338
544545,544546,544545,1089091,1200.7837891578674,0.6520114035502047
546547,546548,546547,1093095,1205.1719739437103,0.6498573099524947
548549,548550,548549,1097099,1209.5859270095825,0.6477176679600234
550551,550552,550551,1101103,1213.9447770118713,0.645592332661181
552553,552554,552553,1105107,1218.3348009586334,0.6434811610834004
554555,554556,554555,1109111,1222.7140500545502,0.641384050657507
556557,556558,556557,1113115,1227.0945069789886,0.6393008372069744
558559,558560,558559,1117119,1231.469489812851,0.6372313694701006
560561,560562,560561,1121123,1235.829579114914,0.6351755118867004
562563,562564,562563,1125127,1240.3838000297546,0.6331331306719221
564565,564566,564565,1129131,1244.9850597381592,0.6311040937907819
566567,566568,566567,1133135,1249.380611896515,0.6290882709363359
568569,568570,568569,1137139,1253.7494831085205,0.6270855334842054
570571,570572,570571,1141143,1258.1112897396088,0.6250957544816629
572573,572574,572573,1145147,1262.5059950351715,0.6231188086057955
574575,574576,574575,1149151,1266.9867429733276,0.6211545721525908
576577,576578,576577,1153155,1271.3877518177032,0.6192029229987384
578579,578580,578579,1157159,1275.746307849884,0.6172637405852583
580581,580582,580581,1161163,1280.1639938354492,0.6153369058829412
582583,582584,582583,1165167,1284.5965769290924,0.6134223013759765
584585,584586,584585,1169171,1288.9590537548065,0.6115198110346682
586587,586588,586587,1173175,1293.3305490016937,0.6096293202881498
588589,588590,588589,1177179,1297.777816772461,0.6077507160152891
590591,590592,590591,1181183,1302.184534072876,0.605883886504671
592593,592594,592593,1185187,1306.5871269702911,0.604028721440045
594595,594596,594595,1189191,1311.0308511257172,0.602185111885774
596597,596598,596597,1193195,1315.408226966858,0.6003529502468155
598599,598600,598599,1197199,1319.7524948120117,0.5985321302723605
600601,600602,600601,1201203,1324.1073579788208,0.5967225470121775
602603,602604,602603,1205207,1328.4634220600128,0.5949240968111553
604605,604606,604605,1209211,1332.8606309890747,0.5931366772874753
606607,606608,606607,1213215,1337.2196538448334,0.5913601873016887
608609,608610,608609,1217219,1341.6508297920227,0.5895945269530785
610611,610612,610611,1221223,1346.0214099884033,0.5878395975560124
612613,612614,612613,1225227,1350.3691778182983,0.5860953016144776
614615,614616,614615,1229231,1354.7234609127045,0.5843615428111661
616617,616618,616617,1233235,1359.1204509735107,0.5826382259892853
618619,618620,618619,1237239,1363.5468831062317,0.5809252571380057
620621,620622,620621,1241243,1367.9033877849579,0.5792225455388689
622623,622624,622623,1245247,1372.5382778644562,0.577529997264719
624625,624626,624625,1249251,1376.9811918735504,0.5758475215661747
626627,626628,626627,1253255,1381.3409268856049,0.574175028827085
628629,628630,628629,1257259,1385.7185978889465,0.5725124304917699
630631,630632,630631,1261263,1390.1185417175293,0.5708596390486491
632633,632634,632633,1265267,1394.5526599884033,0.5692165680084145
634635,634636,634635,1269271,1398.9809758663177,0.5675831319022109
636637,636638,636637,1273275,1403.3548319339752,0.5659592462616274
638639,638640,638639,1277279,1407.799416065216,0.5643448275877745
640641,640642,640641,1281283,1412.1770079135895,0.5627397933694738
642643,642644,642643,1285287,1416.5217578411102,0.5611440620377834
644645,644646,644645,1289291,1420.9389340877533,0.5595575529787311
646647,646648,646647,1293295,1425.3216669559479,0.5579801864878391
648649,648650,648649,1297299,1429.7438879013062,0.5564118837937713
650651,650652,650651,1301303,1434.1217958927155,0.5548525670128583
652653,652654,652653,1305307,1438.5035359859467,0.5533021591636498
654655,654656,654655,1309311,1442.872858762741,0.551760584132353
656657,656658,656657,1313315,1447.2286260128021,0.5502277666673763
658659,658660,658659,1317319,1451.6428859233856,0.5487036323720531
660661,660662,660661,1321323,1456.0320110321045,0.5471881076937279
662663,662664,662663,1325327,1460.4066519737244,0.5456811199001095
664665,664666,664665,1329331,1464.8020799160004,0.5441825970774516
666667,666668,666667,1333335,1469.3749659061432,0.5426924681178207
668669,668670,668669,1337339,1473.8567340373993,0.5412106627063622
670671,670672,670671,1341343,1478.2321519851685,0.5397371113103873
672673,672674,672673,1345347,1482.7938740253448,0.5382717451684584
674675,674676,674675,1349351,1487.2798857688904,0.5368144962794759
676677,676678,676677,1353355,1491.7140591144562,0.5353652973935823
678679,678680,678679,1357359,1496.1529867649078,0.5339240820012492
680681,680682,680681,1361363,1500.5382008552551,0.5324907843241817
682683,682684,682683,1365367,1504.9430658817291,0.531065339297129
684685,684686,684685,1369371,1509.3504168987274,0.5296476825787977
686687,686688,686687,1373375,1513.7250900268555,0.5282377505081968
688689,688690,688689,1377379,1518.0743608474731,0.5268354801355599
690691,690692,690691,1381383,1522.5876870155334,0.525440809180509
692693,692694,692693,1385387,1526.9418680667877,0.5240536760393297
694695,694696,694695,1389391,1531.308021068573,0.5226740197667823
696697,696698,696697,1393395,1535.6677498817444,0.5213017800833768
698699,698700,698699,1397399,1540.1057019233704,0.5199368973389937
700701,700702,700701,1401403,1544.4970099925995,0.5185793125310738
702703,702704,702703,1405407,1548.8951890468597,0.5172289672882471
704705,704706,704705,1409411,1553.337699174881,0.515885803852143
706707,706708,706707,1413415,1557.6636190414429,0.5145497650737525
708709,708710,708709,1417419,1562.0651679039001,0.5132207944225229
710711,710712,710711,1421423,1566.4321410655975,0.5118988359481591
712713,712714,712713,1425427,1570.8261890411377,0.5105838342933566
714715,714716,714715,1429431,1575.1920149326324,0.5092757346847065
716717,716718,716717,1433435,1579.6368079185486,0.5079744829217816
718719,718720,718719,1437439,1584.1811828613281,0.5066800253625843
720721,720722,720721,1441443,1588.6598799228668,0.5053923089308228
722723,722724,722723,1445447,1593.130649805069,0.5041112810940831
724725,724726,724725,1449451,1597.662713766098,0.5028368898692861
726727,726728,726727,1453455,1602.3099429607391,0.5015690838063165
728729,728730,728729,1457459,1606.8094189167023,0.5003078119880229
730731,730732,730731,1461463,1611.2958278656006,0.4990530240138469
732733,732734,732733,1465467,1615.6742680072784,0.497804670010737
734735,734736,734735,1469471,1620.081717967987,0.49656270060040697
736737,736738,736737,1473475,1624.7277419567108,0.49532706692116335
738739,738740,738739,1477479,1629.0904560089111,0.49409772059880197
740741,740742,740741,1481483,1633.6739859580994,0.49287461375206476
742743,742744,742743,1485487,1638.0895738601685,0.4916576989890018
744745,744746,744745,1489491,1642.487725019455,0.4904469293887814
746747,746748,746747,1493495,1646.8583800792694,0.4892422585035092
748749,748750,748749,1497499,1651.2044007778168,0.488043640356409
750751,750752,750751,1501503,1655.604327917099,0.486851029427271
752753,752754,752753,1505507,1660.0034430027008,0.48566438065063267
754755,754756,754755,1509511,1664.416827917099,0.48448364940850297
756757,756758,756757,1513515,1668.8520488739014,0.4833087915303622
758759,758760,758759,1517519,1673.3600919246674,0.4821397632786102
760761,760762,760761,1521523,1677.7542719841003,0.48097652135402313
762763,762764,762763,1525527,1682.1441159248352,0.4798190228812018
764765,764766,764765,1529531,1686.5347797870636,0.4786672254012956
766767,766768,766767,1533535,1691.3563997745514,0.4775210868810973
768769,768770,768769,1537539,1695.7457089424133,0.47638056569485343
770771,770772,770771,1541543,1700.1193528175354,0.47524562062244513
772773,772774,772773,1545547,1704.4762449264526,0.47411621085120714
774775,774776,774775,1549551,1708.8082230091095,0.4729922959541
776777,776778,776777,1553555,1713.2858889102936,0.4718738359042618
778779,778780,778779,1557559,1717.6606941223145,0.47076079106227553
780781,780782,780781,1561563,1722.0833847522736,0.4696531221652549
782783,782784,782783,1565567,1726.517585992813,0.4685507903341204
784785,784786,784785,1569571,1731.06516289711,0.46745375706086634
786787,786788,786787,1573575,1735.547639131546,0.4663619842085609
788789,788790,788789,1577579,1739.9209899902344,0.46527543399679416
790791,790792,790791,1581583,1744.3436107635498,0.46419406901441107
792793,792794,792793,1585587,1748.8934841156006,0.4631178522049595
794795,794796,794795,1589591,1753.5992147922516,0.4620467468575953
796797,796798,796797,1593595,1758.260078907013,0.46098071661617723
798799,798800,798799,1597599,1763.1429529190063,0.4599197254592582
800801,800802,800801,1601603,1767.9065458774567,0.45886373771463695
802803,802804,802803,1605607,1772.5968379974365,0.4578127180393494
804805,804806,804805,1609611,1777.393846988678,0.45676663142148755
806807,806808,806807,1613615,1782.0800189971924,0.45572544318019936
808809,808810,808809,1617619,1786.8008739948273,0.45468911895659403
810811,810812,810811,1621623,1791.469691991806,0.45365762471010385
812813,812814,812813,1625627,1796.1205570697784,0.45263092671666527
814815,814816,814815,1629631,1800.8108959197998,0.4516089915723569
816817,816818,816817,1633635,1805.4786818027496,0.4505917861661146
818819,818820,818819,1637639,1810.192883014679,0.44957927770883543
820821,820822,820821,1641643,1814.945235967636,0.44857143370245467
822823,822824,822823,1645647,1819.5894100666046,0.44756822195449786
824825,824826,824825,1649651,1824.4976539611816,0.44656961056352884
826827,826828,826827,1653655,1829.80979514122,0.4455755679136928
828829,828830,828829,1657659,1834.9299640655518,0.4445860626947251
830831,830832,830831,1661663,1839.9719660282135,0.44360106386193365
832833,832834,832833,1665667,1845.0595610141754,0.44262054066530254
834835,834836,834835,1669671,1850.2210838794708,0.4416444626294833
836837,836838,836837,1673675,1855.3132998943329,0.4406727995501569
838839,838840,838839,1677679,1860.3463160991669,0.4397055215031287
840841,840842,840841,1681683,1865.4161548614502,0.4387425988279574
842843,842844,842843,1685687,1870.7591760158539,0.4377840021334123
844845,844846,844845,1689691,1875.8480257987976,0.43682970228837803
846847,846848,846847,1693695,1880.8763778209686,0.4358796704236738
848849,848850,848849,1697699,1885.9697709083557,0.4349338779320533
850851,850852,850851,1701703,1891.0928120613098,0.43399229645365267
852853,852854,852853,1705707,1895.8034009933472,0.4330548978814477
854855,854856,854855,1709711,1900.5568089485168,0.4321216543612536
856857,856858,856857,1713715,1905.2848467826843,0.43119253828444926
858859,858860,858859,1717719,1910.0397498607635,0.4302675222807011
860861,860862,860861,1721723,1914.7195620536804,0.4293465792252391
862863,862864,862863,1725727,1919.4182889461517,0.42842968223158095
864865,864866,864865,1729731,1924.1014878749847,0.42751680464971287
866867,866868,866867,1733735,1928.7843420505524,0.4266079200551758
868869,868870,868869,1737739,1933.50346493721,0.42570300226361724
870871,870872,870871,1741743,1938.1910347938538,0.4248020253107825
872873,872874,872873,1745747,1942.881817817688,0.42390496346342843
874875,874876,874875,1749751,1947.562933921814,0.4230117912102287
876877,876878,876877,1753755,1952.262830734253,0.4221224832563166
878879,878880,878879,1757759,1956.9463539123535,0.4212370145305613
880881,880882,880881,1761763,1961.6541068553925,0.42035536017465347
882883,882884,882883,1765767,1966.3610088825226,0.41947749554128677
884885,884886,884885,1769771,1971.0672459602356,0.41860340019411524
886887,886888,886887,1773775,1975.7960529327393,0.4177330541169795
888889,888890,888889,1777779,1980.5624949932098,0.4168664250519214
890891,890892,890891,1781783,1985.5647978782654,0.4160034891865507
892893,892894,892893,1785787,1990.3143239021301,0.415144222906747
894895,894896,894895,1789791,1994.9784851074219,0.41428860280393565
896897,896898,896897,1793795,1999.684541940689,0.4134366056714498
898899,898900,898899,1797799,2004.3187210559845,0.41258820848997857
900901,900902,900901,1801803,2008.9944970607758,0.4117433884348429
902903,902904,902903,1805807,2013.9119749069214,0.41090212288327166
904905,904906,904905,1809811,2018.6840720176697,0.4100643893907545
906907,906908,906907,1813815,2023.3778638839722,0.4092301657055941
908909,908910,908909,1817819,2028.0818219184875,0.408399429763449
910911,910912,910911,1821823,2032.7787539958954,0.40757215968551463
912913,912914,912913,1825827,2037.4935607910156,0.40674833376579045
914915,914916,914915,1829831,2042.2788848876953,0.4059279304910888
916917,916918,916917,1833835,2046.9315347671509,0.40511092851556896
918919,918920,918919,1837839,2051.616791009903,0.4042973066771083
920921,920922,920921,1841843,2056.313155889511,0.403487043986388
922923,922924,922923,1845847,2060.970543861389,0.4026801196287124
924925,924926,924925,1849851,2065.6327748298645,0.4018765129512758
926927,926928,926927,1853855,2070.3272998332977,0.4010762034849904
928929,928930,928929,1857859,2075.0031187534332,0.40027917091902054
930931,930932,930931,1861863,2079.7023627758026,0.3994853951080586
932933,932934,932933,1865867,2084.4229698181152,0.3986948560741439
934935,934936,934935,1869871,2089.1024038791656,0.3979075340066629
936937,936938,936937,1873875,2093.827845811844,0.3971234092459781
938939,938940,938939,1877879,2098.511207818985,0.3963424622979801
940941,940942,940941,1881883,2103.3977789878845,0.3955646738213545
942943,942944,942943,1885887,2108.2381739616394,0.3947900246403151
944945,944946,944945,1889891,2112.9546189308167,0.3940184957227757
946947,946948,946947,1893895,2117.643194913864,0.39325006819490227
948949,948950,948949,1897899,2122.30738902092,0.39248472333565587
950951,950952,950951,1901903,2127.1207768917084,0.3917224425713357
952953,952954,952953,1905907,2132.0061688423157,0.3909632074773981
954955,954956,954955,1909911,2136.697731733322,0.39020699977481854
956957,956958,956957,1913915,2141.361454963684,0.38945380133191065
958959,958960,958959,1917919,2146.1392769813538,0.3887035941625072
960961,960962,960961,1921923,2151.0563180446625,0.3879563604186842
962963,962964,962963,1925927,2155.7242550849915,0.3872120823980367
964965,964966,964965,1929931,2160.4131338596344,0.3864707425382221
966967,966968,966967,1933935,2165.0967218875885,0.3857323234060459
968969,968970,968969,1937939,2169.8053550720215,0.3849968077174708
970971,970972,970971,1941943,2174.507383108139,0.3842641783230647
972973,972974,972973,1945947,2179.205271959305,0.3835344181970868
974975,974976,974975,1949951,2183.8901040554047,0.3828075104574964
976977,976978,976977,1953955,2188.549073934555,0.38208343834958214
978979,978980,978979,1957959,2193.2205817699432,0.38136218525141885
980981,980982,980981,1961963,2197.9202387332916,0.38064373466477264
982983,982984,982983,1965967,2202.61794090271,0.3799280702278338
984985,984986,984985,1969971,2207.3218579292297,0.379215175702484
986987,986988,986987,1973975,2212.0614359378815,0.378505034972477
988989,988990,988989,1977979,2216.7893240451813,0.37779763204707706
990991,990992,990991,1981983,2221.462965965271,0.37709295106105856
992993,992994,992993,1985987,2226.1190259456635,0.3763909762728872
994995,994996,994995,1989991,2230.815659046173,0.37569169205380604
996997,996998,996997,1993995,2235.4539799690247,0.37499508290238737
998999,999000,998999,1997999,2240.1443209648132,0.3743011334354378
1001001,1001002,1001001,2002003,2244.7954709529877,0.3736098283825413
1003003,1003004,1003003,2006007,2249.4604148864746,0.37292115259333514
1005005,1005006,1005005,2010011,2254.11598277092,0.3722350910284149
1007007,1007008,1007007,2014015,2258.780173063278,0.3715516287684295
1009009,1009010,1009009,2018019,2263.4820940494537,0.3708707509977103
1011011,1011012,1011011,2022023,2268.135239839554,0.37019244302791776
1013013,1013014,1013013,2026027,2273.036563873291,0.369516690267119
1015015,1015016,1015015,2030031,2277.7032351493835,0.36884347823797725
1017017,1017018,1017017,2034035,2282.5632030963898,0.3681727925722953
1019019,1019020,1019019,2038039,2287.449527978897,0.3675046190091962
1021021,1021022,1021021,2042043,2292.193529844284,0.36683894339694234
1023023,1023024,1023023,2046047,2296.966068983078,0.36617575168565963
1025025,1025026,1025025,2050051,2301.6921758651733,0.36551502993461327
1027027,1027028,1027027,2054055,2306.3716638088226,0.36485676430311287
1029029,1029030,1029029,2058059,2311.019096851349,0.3642009410523315
1031031,1031032,1031031,2062063,2315.691209077835,0.3635475465471245
1033033,1033034,1033033,2066067,2320.4287729263306,0.3628965672614868
1035035,1035036,1035035,2070071,2325.102350950241,0.3622479897530866
1037037,1037038,1037037,2074075,2329.771618127823,0.36160180069600756
1039039,1039040,1039039,2078079,2334.480568885803,0.36095798684254987
1041041,1041042,1041041,2082083,2339.1411368846893,0.360316535063248
1043043,1043044,1043043,2086087,2343.80446100235,0.359677432310491
1045045,1045046,1045045,2090091,2348.5228538513184,0.3590406656403502
1047047,1047048,1047047,2094095,2353.1760199069977,0.35840622219620855
1049049,1049050,1049049,2098099,2357.8504209518433,0.35777408922331233
1051051,1051052,1051051,2102103,2362.484783887863,0.35714425405603833
1053053,1053054,1053053,2106107,2367.3237178325653,0.3565167041178938
1055055,1055056,1055055,2110111,2372.1727969646454,0.3558914269269735
1057057,1057058,1057057,2114115,2376.8310730457306,0.35526841009414056
1059059,1059060,1059059,2118119,2381.688153743744,0.35464764131393167
1061061,1061062,1061061,2122123,2386.3560090065002,0.354029108371833
1063063,1063064,1063063,2126127,2391.0675909519196,0.3534127991479181
1065065,1065066,1065065,2130131,2395.8287649154663,0.35279870159683924
1067067,1067068,1067067,2134135,2400.5197970867157,0.3521868037732929
1069069,1069070,1069069,2138139,2405.1640689373016,0.3515770938083733
1071071,1071072,1071071,2142143,2409.8303220272064,0.3509695599186671
1073073,1073074,1073073,2146147,2414.515843153,0.3503641904080723
1075075,1075076,1075075,2150151,2419.5764169692993,0.3497609736641607
1077077,1077078,1077077,2154155,2424.298017978668,0.3491598981545394
1079079,1079080,1079079,2158159,2428.9926538467407,0.3485609524359461
1081081,1081082,1081081,2162163,2433.87162399292,0.34796412513060204
1083083,1083084,1083083,2166167,2438.5234088897705,0.347369404957135
1085085,1085086,1085085,2170171,2443.2390677928925,0.3467767807051132
1087087,1087088,1087087,2174175,2447.912488937378,0.3461862412514165
1089089,1089090,1089089,2178179,2452.6133120059967,0.3455977755384083
1091091,1091092,1091091,2182183,2457.397511959076,0.3450113726012205
1093093,1093094,1093093,2186187,2462.047341108322,0.3444270215368306
1095095,1095096,1095095,2190191,2466.716356754303,0.34384471153134655
1097097,1097098,1097097,2194195,2471.4094920158386,0.343264431838179
1099099,1099100,1099099,2198199,2476.0799679756165,0.3426861717925931
1101101,1101102,1101101,2202203,2480.7985780239105,0.3421099207971565
1103103,1103104,1103103,2206207,2485.6412448883057,0.3415356683344726
1105105,1105106,1105105,2210211,2490.5547120571136,0.34096340395444713
1107107,1107108,1107107,2214215,2495.5837218761444,0.3403931172833836
1109109,1109110,1109109,2218219,2500.3340990543365,0.3398247980148881
1111111,1111112,1111111,2222223,2505.040694952011,0.33925843592624005
1113113,1113114,1113113,2226227,2509.776885032654,0.3386940208474698
1115115,1115116,1115115,2230231,2514.5077970027924,0.33813154269410006
1117117,1117118,1117117,2234235,2519.194296836853,0.33757099143804226
1119119,1119120,1119119,2238239,2523.895805835724,0.33701235713124333
1121121,1121122,1121121,2242243,2528.5691509246826,0.3364556298874959
1123123,1123124,1123123,2246247,2533.295350074768,0.33590079988607613
1125125,1125126,1125125,2250251,2537.9424130916595,0.3353478573844768
1127127,1127128,1127127,2254255,2542.630198955536,0.3347967926929414
1129129,1129130,1129129,2258259,2547.4213309288025,0.33424759619447286
1131131,1131132,1131131,2262263,2552.0888998508453,0.3337002583393769
1133133,1133134,1133133,2266267,2556.74719786644,0.33315476963798574
1135135,1135136,1135135,2270271,2561.4713368415833,0.3326111206697533
1137137,1137138,1137137,2274275,2566.1185009479523,0.3320693020723411
1139139,1139140,1139139,2278279,2570.7656078338623,0.3315293045507133
1141141,1141142,1141141,2282283,2575.504630088806,0.33099111887167965
1143143,1143144,1143143,2286287,2580.1620709896088,0.33045473586207663
1145145,1145146,1145145,2290291,2584.7994129657745,0.3299201464160433
1147147,1147148,1147147,2294295,2589.6476271152496,0.32938734147865034
1149149,1149150,1149149,2298299,2594.5234088897705,0.32885631206590915
1151151,1151152,1151151,2302303,2599.2061638832092,0.3283270492502197
1153153,1153154,1153153,2306307,2603.879212141037,0.3277995441585517
1155155,1155156,1155155,2310311,2608.562306165695,0.3272737879851775
1157157,1157158,1157157,2314315,2613.226611852646,0.32674977198075794
1159159,1159160,1159159,2318319,2617.908819913864,0.3262274874487048
1161161,1161162,1161161,2322323,2622.5998950004578,0.3257069257560943
1163163,1163164,1163163,2326327,2627.248820066452,0.3251880783227534
1165165,1165166,1165165,2330331,2631.9566509723663,0.3246709366339928
1167167,1167168,1167167,2334335,2636.600373983383,0.32415549221514084
1169169,1169170,1169169,2338339,2641.299989938736,0.32364173666246643
1171171,1171172,1171171,2342343,2645.991768836975,0.32312966162317025
1173173,1173174,1173173,2346347,2650.8339278697968,0.32261925879538467
1175175,1175176,1175175,2350351,2655.6050288677216,0.3221105199354497
1177177,1177178,1177177,2354355,2660.241914987564,0.32160343685245607
1179179,1179180,1179179,2358359,2664.8952779769897,0.32109800141006417
1181181,1181182,1181181,2362363,2669.572736978531,0.3205942055228661
1183183,1183184,1183183,2366367,2674.2630457878113,0.32009204116002365
1185185,1185186,1185185,2370371,2679.150027990341,0.3195915003434493
1187187,1187188,1187187,2374375,2683.8980510234833,0.3190925751441682
1189189,1189190,1189189,2378379,2688.554510831833,0.3185952576877753
1191191,1191192,1191191,2382383,2693.2914760112762,0.3180995401489781
1193193,1193194,1193193,2386387,2697.9451761245728,0.317605414749778
1195195,1195196,1195195,2390391,2702.6462478637695,0.3171128737685649
1197197,1197198,1197197,2394395,2707.3527870178223,0.31662190953284153
1199199,1199200,1199199,2398399,2712.084737062454,0.3161325144155853
1201201,1201202,1201201,2402403,2716.72616815567,0.3156446808407054
1203203,1203204,1203203,2406407,2721.4417259693146,0.31515840127940464
1205205,1205206,1205205,2410411,2726.066589832306,0.3146736682519986
1207207,1207208,1207207,2414415,2730.7309041023254,0.31419047433155356
1209209,1209210,1209209,2418419,2735.363065958023,0.31370881212933455
1211211,1211212,1211211,2422423,2740.0465359687805,0.3132286743093573
1213213,1213214,1213213,2426427,2744.7232551574707,0.3127500535792933
1215215,1215216,1215215,2430431,2749.404057741165,0.31227294269774575
1217217,1217218,1217217,2434435,2754.0871658325195,0.31179733446697355
1219219,1219220,1219219,2438439,2758.7597119808197,0.3113232217328914
1221221,1221222,1221221,2442443,2763.4213650226593,0.3108505973887077
1223223,1223224,1223223,2446447,2768.101241827011,0.31037945437128656
1225225,1225226,1225225,2450451,2772.8004517555237,0.3099097856611479
1227227,1227228,1227227,2454455,2777.461770057678,0.30944158428610535
1229229,1229230,1229229,2458459,2782.3608677387238,0.30897484331944725
1231231,1231232,1231231,2462463,2787.0641779899597,0.30850955586902273
1233233,1233234,1233233,2466467,2791.7194299697876,0.30804571509361267
1235235,1235236,1235235,2470471,2796.3644721508026,0.30758331419383467
1237237,1237238,1237237,2474475,2801.163707971573,0.3071223464085051
1239239,1239240,1239239,2478479,2805.9328248500824,0.3066628050255531
1241241,1241242,1241241,2482483,2810.8022499084473,0.30620468336746853
1243243,1243244,1243243,2486487,2815.7039799690247,0.30574797480585403
1245245,1245246,1245245,2490491,2820.3837399482727,0.305292672743235
1247247,1247248,1247247,2494495,2825.0937299728394,0.3048387706348876
1249249,1249250,1249249,2498499,2829.76824092865,0.3043862619651918
1251251,1251252,1251251,2502503,2834.552358865738,0.3039351402694592
1253253,1253254,1253253,2506507,2839.252716064453,0.30348539911574335
1255255,1255256,1255255,2510511,2843.937597990036,0.3030370321121154
1257257,1257258,1257257,2514515,2848.602110862732,0.3025900329084834
1259259,1259260,1259259,2518519,2853.2733449935913,0.3021443951947731
1261261,1261262,1261261,2522523,2857.9474968910217,0.30170011269365204
1263263,1263264,1263263,2526527,2862.6413209438324,0.30125717917690054
1265265,1265266,1265265,2530531,2867.3355820178986,0.3008155884381267
1267267,1267268,1267267,2534535,2872.04269695282,0.3003753343291464
1269269,1269270,1269269,2538539,2876.694761991501,0.29993641071996535
1271271,1271272,1271271,2542543,2881.4028627872467,0.2994988115315209
1273273,1273274,1273273,2546547,2886.0747079849243,0.29906253071385436
1275275,1275276,1275275,2550551,2890.767447948456,0.2986275622588437
1277277,1277278,1277277,2554555,2895.45529794693,0.2981939001911087
1279279,1279280,1279279,2558559,2900.102098941803,0.297761538575287
1281281,1281282,1281281,2562563,2904.7720110416412,0.29733047150511993
1283283,1283284,1283283,2566567,2909.633908033371,0.2969006931198237
1285285,1285286,1285285,2570571,2914.3858649730682,0.2964721975804423
1287287,1287288,1287287,2574575,2919.048696756363,0.29604497909895144
1289289,1289290,1289289,2578579,2923.728653907776,0.29561903190915473
1291291,1291292,1291291,2582583,2928.3825039863586,0.2951943502866925
1293293,1293294,1293293,2586587,2933.1167948246,0.2947709285399469
1295295,1295296,1295295,2590591,2937.8470978736877,0.2943487610118609
1297297,1297298,1297297,2594595,2942.500830888748,0.2939278420763003
1299299,1299300,1299299,2598599,2947.1847789287567,0.2935081661416916
1301301,1301302,1301301,2602603,2952.007917165756,0.29308972765102226
1303303,1303304,1303303,2606607,2956.6729769706726,0.2926725210782024
1305305,1305306,1305305,2610611,2961.365859746933,0.29225654093352205
1307307,1307308,1307307,2614615,2966.0274579524994,0.29184178193099797
1309309,1309310,1309309,2618619,2970.7801349163055,0.2914282386609557
1311311,1311312,1311311,2622623,2975.620250940323,0.2910159055409167
1313313,1313314,1313313,2626627,2980.556179046631,0.29060477720486233
1315315,1315316,1315315,2630631,2985.455636024475,0.29019484832315356
1317317,1317318,1317317,2634635,2990.3747520446777,0.28978611358797934
1319319,1319320,1319319,2638639,2995.195606946945,0.2893785677424603
1321321,1321322,1321321,2642643,2999.8764810562134,0.28897220554063097
1323323,1323324,1323323,2646647,3004.528100967407,0.2885670217801817
1325325,1325326,1325325,2650651,3009.332254886627,0.2881630112788116
1327327,1327328,1327327,2654655,3014.0587871074677,0.2877601688978757
1329329,1329330,1329329,2658659,3018.738410949707,0.2873584895150998
1331331,1331332,1331331,2662663,3023.4072258472443,0.2869579680445895
1333333,1333334,1333333,2666667,3028.129590988159,0.2865585994313733
1335335,1335336,1335335,2670671,3032.781080722809,0.28616037864776445
1337337,1337338,1337337,2674675,3037.4412820339203,0.28576330069699907
1339339,1339340,1339339,2678679,3042.166531085968,0.28536736060414114
1341341,1341342,1341341,2682683,3046.8368439674377,0.2849725534360914
1343343,1343344,1343343,2686687,3051.7030398845673,0.2845788742724835
1345345,1345346,1345345,2690691,3056.46381688118,0.2841863182384259
1347347,1347348,1347347,2694695,3061.1354517936707,0.28379488046994084
1349349,1349350,1349349,2698699,3065.8078808784485,0.28340455614852544
1351351,1351352,1351351,2702703,3070.4948279857635,0.2830153404684097
1353353,1353354,1353353,2706707,3075.2694039344788,0.2826272286565654
1355355,1355356,1355355,2710711,3080.037871837616,0.2822402159708872
1357357,1357358,1357357,2714715,3084.705682992935,0.2818542976929166
1359359,1359360,1359359,2718719,3089.442691087723,0.28146946913329884
1361361,1361362,1361361,2722723,3094.1208069324493,0.2810857256226882
1363363,1363364,1363363,2726727,3098.8579359054565,0.2807030625299376
1365365,1365366,1365365,2730731,3103.970855951309,0.28032147524208995
1367367,1367368,1367367,2734735,3109.000277042389,0.27994095917347295
1369369,1369370,1369369,2738739,3114.042366027832,0.27956150976569916
1371371,1371372,1371371,2742743,3119.0915138721466,0.279183122484028
1373373,1373374,1373373,2746747,3124.13329410553,0.2788057928210037
1375375,1375376,1375375,2750751,3129.2043809890747,0.2784295163000934
1377377,1377378,1377377,2754755,3134.242365837097,0.278054288459316
1379379,1379380,1379379,2758759,3139.2661440372467,0.2776801048694324
1381381,1381382,1381381,2762763,3144.286814928055,0.2773069611230312
1383383,1383384,1383383,2766767,3149.5890049934387,0.276934852838167
1385385,1385386,1385385,2770771,3154.7654490470886,0.2765637756601791
1387387,1387388,1387387,2774775,3159.7844009399414,0.27619372525441577
1389389,1389390,1389389,2778779,3164.821939945221,0.2758246973116911
1391391,1391392,1391391,2782783,3169.5306990146637,0.27545668754646613
1393393,1393394,1393393,2786787,3174.3348758220673,0.27508969170230557
1395395,1395396,1395395,2790791,3179.0360078811646,0.27472370554278314
1397397,1397398,1397397,2794795,3183.702610015869,0.2743587248478434
1399399,1399400,1399399,2798799,3188.430755853653,0.27399474543744873
1401401,1401402,1401401,2802803,3193.07675075531,0.2736317631370184
1403403,1403404,1403403,2806807,3197.7282240390778,0.2732697738083516
1405405,1405406,1405405,2810811,3202.4282608032227,0.2729087733277993
1407407,1407408,1407407,2814815,3207.0730240345,0.2725487575989973
1409409,1409410,1409409,2818819,3211.7446699142456,0.27218972254922846
1411411,1411412,1411411,2822823,3216.459836959839,0.2718316641239653
1413413,1413414,1413413,2826827,3221.1639969348907,0.27147457829232735
1415415,1415416,1415415,2830831,3225.8525619506836,0.27111846104526194
1417417,1417418,1417417,2834835,3230.738133907318,0.27076330840282026
1419419,1419420,1419419,2838839,3235.6006758213043,0.27040911639414844
1421421,1421422,1421421,2842843,3240.2724969387054,0.27005588107931544
1423423,1423424,1423423,2846847,3244.923999071121,0.2697035985402181
1425425,1425426,1425425,2850851,3249.6518337726593,0.2693522648733051
1427427,1427428,1427427,2854855,3254.2746369838715,0.2690018762041291
1429429,1429430,1429429,2858859,3258.952008008957,0.2686524286691565
1431431,1431432,1431431,2862863,3263.6208879947662,0.2683039184394147
1433433,1433434,1433433,2866867,3268.2649998664856,0.2679563417004829
1435435,1435436,1435435,2870871,3272.906965970993,0.2676096946524922
1437437,1437438,1437437,2874875,3277.699469804764,0.2672639735210396
1439439,1439440,1439439,2878879,3282.5502038002014,0.26691917455900693
1441441,1441442,1441441,2882883,3287.202742099762,0.26657529403019
1443443,1443444,1443443,2886887,3291.8500678539276,0.26623232822021237
1445445,1445446,1445445,2890891,3296.574812889099,0.2658902734383446
1447447,1447448,1447447,2894895,3301.258059024811,0.2655491260084091
1449449,1449450,1449449,2898899,3305.8874781131744,0.2652088822796941
1451451,1451452,1451451,2902903,3310.621230840683,0.26486953861967777
1453453,1453454,1453453,2906907,3315.292135953903,0.2645310914122092
1455455,1455456,1455455,2910911,3319.9601669311523,0.26419353705932735
1457457,1457458,1457457,2914915,3325.0481259822845,0.263856871993994
1459459,1459460,1459459,2918919,3329.7574529647827,0.2635210926509899
1461461,1461462,1461461,2922923,3334.439983844757,0.2631861954960186
1463463,1463464,1463463,2926927,3339.1146397590637,0.2628521770129737
1465465,1465466,1465465,2930931,3343.901160955429,0.2625190336966625
1467467,1467468,1467467,2934935,3348.583643913269,0.2621867620746343
1469469,1469470,1469469,2938939,3353.3184950351715,0.26185535867261933
1471471,1471472,1471471,2942943,3358.0109388828278,0.2615248200527276
1473473,1473474,1473473,2946947,3363.052706003189,0.26119514278980205
1475475,1475476,1475475,2950951,3368.084100961685,0.26086632347323757
1477477,1477478,1477477,2954955,3373.1125209331512,0.2605383587106189
1479479,1479480,1479479,2958959,3378.1479120254517,0.2602112451349967
1481481,1481482,1481481,2962963,3383.199937105179,0.2598849793866975
1483483,1483484,1483483,2966967,3388.3025028705597,0.25955955813333276
1485485,1485486,1485485,2970971,3393.3505008220673,0.2592349780516088
1487487,1487488,1487487,2974975,3398.3764810562134,0.2589112358436978
1489489,1489490,1489489,2978979,3403.4805879592896,0.25858832822268596
1491491,1491492,1491491,2982983,3408.7395210266113,0.2582662519198493
1493493,1493494,1493493,2986987,3413.855443954468,0.2579450036864728
1495495,1495496,1495495,2990991,3418.871097803116,0.25762458029203117
1497497,1497498,1497497,2994995,3424.0630910396576,0.25730497851691325
1499499,1499500,1499499,2998999,3428.9117918014526,0.2569861951578787
1501502,1501503,1501502,3003005,3433.710983991623,0.25666806841582
1503504,1503505,1503504,3007009,3438.465229034424,0.25635091277035826
1505506,1505507,1505506,3011013,3443.2849700450897,0.2560345660440362
1507508,1507509,1507508,3015017,3448.039760828018,0.25571902510273503
1509510,1509511,1509510,3019021,3453.014402151108,0.255404286826888
1511512,1511513,1511512,3023025,3457.7467629909515,0.2550903481169371
1513514,1513515,1513514,3027029,3462.430862903595,0.25477720588787633
1515516,1515517,1515516,3031033,3467.1307320594788,0.2544648570692516
1517518,1517519,1517518,3035037,3472.116180896759,0.25415329860697966
1519520,1519521,1519520,3039041,3476.912863969803,0.25384252746334823
1521522,1521523,1521522,3043045,3481.6567130088806,0.2535325406151969
1523524,1523525,1523524,3047049,3486.5130639076233,0.25322333505755523
1525526,1525527,1525526,3051053,3491.4442160129547,0.2529149077945476
1527528,1527529,1527528,3055057,3496.296814918518,0.2526072558557644
1529530,1529531,1529530,3059061,3501.0419569015503,0.2523003762762528
1531532,1531533,1531532,3063065,3505.784564971924,0.251994266112888
1533534,1533535,1533534,3067069,3510.4725110530853,0.2516889224298211
1535536,1535537,1535536,3071073,3515.183121919632,0.2513843423148501
1537538,1537539,1537538,3075077,3519.872658967972,0.2510805228703248
1539540,1539541,1539540,3079081,3524.543086051941,0.2507774612022331
1541542,1541543,1541542,3083085,3529.237979888916,0.2504751544420287
1543544,1543545,1543544,3087089,3533.9092059135437,0.2501735997320793
1545546,1545547,1545546,3091093,3538.556384086609,0.24987279422930442
1547548,1547549,1547548,3095097,3543.264643907547,0.24957273510699451
1549550,1549551,1549550,3099101,3547.965348958969,0.24927341955299198
1551552,1551553,1551552,3103105,3552.765748977661,0.24897484476059617
1553554,1553555,1553554,3107109,3557.7359340190887,0.24867700794857228
1555556,1555557,1555556,3111113,3562.406221151352,0.24837990634296148
1557558,1557559,1557558,3115117,3567.210849046707,0.2480835371898138
1559560,1559561,1559560,3119121,3572.0120408535004,0.24778789773699827
1561562,1561563,1561562,3123125,3576.707619190216,0.24749298526330676
1563564,1563565,1563564,3127129,3581.4506709575653,0.24719879704753112
1565566,1565567,1565566,3131133,3586.112761735916,0.24690533038665308
1567568,1567569,1567568,3135137,3590.7488629817963,0.2466125825922063
1569570,1569571,1569570,3139141,3595.549824953079,0.24632055098481942
1571572,1571573,1571572,3143145,3600.2223460674286,0.2460292329033109
1573574,1573575,1573574,3147149,3604.898456096649,0.24573862569923222
1575576,1575577,1575576,3151153,3609.6666860580444,0.24544872673686768
1577578,1577579,1577578,3155157,3614.3241081237793,0.24515953338959662
1579580,1579581,1579580,3159161,3619.013447999954,0.24487104304716922
1581582,1581583,1581582,3163165,3623.731173992157,0.2445832531157066
1583584,1583585,1583584,3167169,3628.3918840885162,0.24429616100860585
1585586,1585587,1585586,3171173,3633.0837240219116,0.24400976415199693
1587588,1587589,1587588,3175177,3637.7886850833893,0.24372405998656177
1589590,1589591,1589590,3179181,3642.4841599464417,0.24343904596935317
1591592,1591593,1591592,3183185,3647.13281583786,0.24315471956469992
1593594,1593595,1593594,3187189,3651.805421113968,0.2428710782496637
1595596,1595597,1595596,3191193,3656.466673851013,0.24258811951585812
1597598,1597599,1597598,3195197,3661.0804579257965,0.24230584086399176
1599600,1599601,1599600,3199201,3665.69780087471,0.24202423981478205
1601602,1601603,1601602,3203205,3670.318193912506,0.24174331388894643
1603604,1603605,1603604,3207209,3675.0031628608704,0.2414630606308492
1605606,1605607,1605606,3211213,3679.689822912216,0.24118347759031167
1607608,1607609,1607608,3215217,3684.3719370365143,0.240904562329888
1609610,1609611,1609610,3219221,3689.0434980392456,0.24062631242486532
1611612,1611613,1611612,3223225,3693.7424080371857,0.2403487254632637
1613614,1613615,1613614,3227229,3698.4767060279846,0.2400717990421981
1615616,1615617,1615616,3231233,3703.154624938965,0.23979553077515448
1617618,1617619,1617618,3235237,3707.907753944397,0.23951991828289465
1619620,1619621,1619620,3239241,3712.7496540546417,0.23924495919709443
1621622,1621623,1621622,3243245,3717.4213609695435,0.23897065116398153
1623624,1623625,1623624,3247249,3722.0534908771515,0.2386969918388786
1625626,1625627,1625626,3251253,3726.7508709430695,0.23842397888984124
1627628,1627629,1627628,3255257,3731.555704832077,0.23815160999583895
1629630,1629631,1629630,3259261,3736.2191219329834,0.2378798828467552
1631632,1631633,1631632,3263265,3740.9119050502777,0.2376087951433874
1633634,1633635,1633634,3267269,3745.636512041092,0.23733834459562786
1635636,1635637,1635636,3271273,3750.3324389457703,0.23706852893337782
1637638,1637639,1637638,3275277,3755.468142747879,0.23679934588108154
1639640,1639641,1639640,3279281,3760.260015964508,0.2365307931922871
1641642,1641643,1641642,3283285,3764.9836349487305,0.2362628686150856
1643644,1643645,1643644,3287289,3769.64817404747,0.23599556991939608
1645646,1645647,1645646,3291293,3774.3424429893494,0.23572889488423243
1647648,1647649,1647648,3295297,3779.0381088256836,0.2354628412904276
1649650,1649651,1649650,3299301,3783.669203042984,0.23519740694246138
1651652,1651653,1651652,3303305,3788.311989068985,0.23493258964845154
1653654,1653655,1653654,3307309,3793.0172939300537,0.2346683872219728
1655656,1655657,1655656,3311313,3797.6796929836273,0.23440479749478982
1657658,1657659,1657658,3315317,3802.3631360530853,0.23414181830594316
1659660,1659661,1659660,3319321,3807.169729948044,0.23387944750720635
1661662,1661663,1661662,3323325,3812.030844926834,0.23361768295580987
1663664,1663665,1663664,3327329,3816.6970250606537,0.23335652252353611
1665666,1665667,1665666,3331333,3821.385466814041,0.23309596408762445
1667668,1667669,1667668,3335337,3826.0270009040833,0.23283600553986616
1669670,1669671,1669670,3339341,3830.7997250556946,0.2325766447775095
1671672,1671673,1671672,3343345,3835.526741027832,0.2323178797159926
1673674,1673675,1673674,3347349,3840.183662891388,0.23205970826711564
1675676,1675677,1675676,3351353,3844.8350129127502,0.23180212836632563
1677678,1677679,1677678,3355357,3849.5743827819824,0.23154513794725062
1679680,1679681,1679680,3359361,3854.226826906204,0.23128873496170854
1681682,1681683,1681682,3363365,3858.861790895462,0.2310329173651553
1683684,1683685,1683684,3367369,3863.5773499011993,0.23077768312759872
1685686,1685687,1685686,3371373,3868.219352722168,0.2305230302245036
1687688,1687689,1687688,3375377,3872.881635904312,0.23026895664406766
1689690,1689691,1689690,3379381,3877.5698449611664,0.2300154603781266
1691692,1691693,1691692,3383385,3882.3573899269104,0.229762539436706
1693694,1693695,1693694,3387389,3887.0518209934235,0.22951019182983146
1695696,1695697,1695696,3391393,3891.7508301734924,0.2292584155820805
1697698,1697699,1697698,3395397,3896.468204975128,0.22900720872712554
1699700,1699701,1699700,3399401,3901.126708984375,0.22875656930409605
1701702,1701703,1701702,3403405,3905.800817966461,0.2285064953703113
1703704,1703705,1703704,3407409,3910.522572994232,0.2282569849758147
1705706,1705707,1705706,3411413,3915.2328720092773,0.22800803619247745
1707708,1707709,1707708,3415417,3919.8839790821075,0.2277596471049037
1709710,1709711,1709710,3419421,3924.599598169327,0.2275118157886027
1711712,1711713,1711712,3423425,3929.252079963684,0.22726454034273047
1713714,1713715,1713714,3427429,3933.9570429325104,0.22701781887553807
1715716,1715717,1715716,3431433,3938.6161358356476,0.2267716494952765
1717718,1717719,1717718,3435437,3943.3141570091248,0.22652603032292973
1719720,1719721,1719720,3439441,3947.957039833069,0.22628095948675764
1721722,1721723,1721722,3443445,3952.7170419692993,0.22603643512957206
1723724,1723725,1723724,3447449,3957.400239944458,0.2257924553923658
1725726,1725727,1725726,3451453,3962.038656949997,0.2255490184361406
1727728,1727729,1727728,3455457,3966.697462081909,0.2253061224200792
1729730,1729731,1729730,3459461,3971.6015717983246,0.22506376551791618
1731732,1731733,1731732,3463465,3976.333306789398,0.2248219459052052
1733734,1733735,1733734,3467469,3981.046956062317,0.2245806617775088
1735736,1735737,1735736,3471473,3985.7273559570312,0.22433991132675146
1737738,1737739,1737738,3475477,3990.391832113266,0.22409969275940966
1739740,1739741,1739740,3479481,3995.1142070293427,0.22386000428741681
1741742,1741743,1741742,3483485,3999.88302898407,0.22362084413180128
1743744,1743745,1743744,3487489,4004.5222549438477,0.22338221052086737
1745746,1745747,1745746,3491493,4009.1868238449097,0.22314410169201437
1747748,1747749,1747748,3495497,4013.8536677360535,0.22290651588627952
1749750,1749751,1749750,3499501,4018.5074520111084,0.22266945136470895
1751752,1751753,1751752,3503505,4023.3496038913727,0.22243290638107283
1753754,1753755,1753754,3507509,4028.0807271003723,0.22219687920187425
1755756,1755757,1755756,3511513,4032.770171880722,0.22196136810998723
1757758,1757759,1757758,3515517,4037.4397099018097,0.2217263713846478
1759760,1759761,1759760,3519521,4042.1206290721893,0.22149188731964387
1761762,1761763,1761762,3523525,4046.809666156769,0.22125791421058238
1763764,1763765,1763764,3527529,4051.4538300037384,0.22102445036398422
1765766,1765767,1765766,3531533,4056.1152789592743,0.22079149409728416
1767768,1767769,1767768,3535537,4060.791626930237,0.220559043729736
1769770,1769771,1769770,3539541,4065.5643589496613,0.2203270975896885
1771772,1771773,1771772,3543545,4070.2930018901825,0.2200956540145853
1773774,1773775,1773774,3547549,4075.1848998069763,0.2198647113473271
1775776,1775777,1775776,3551553,4080.05402803421,0.21963426794172847
1777778,1777779,1777778,3555557,4084.74085688591,0.21940432215342298
1779780,1779781,1779780,3559561,4089.409698009491,0.21917487235077715
1781782,1781783,1781782,3563565,4094.0908937454224,0.21894591690215748
1783784,1783785,1783784,3567569,4098.739641904831,0.2187174541886634
1785786,1785787,1785786,3571573,4103.4259259700775,0.21848948260048928
1787788,1787789,1787788,3575577,4108.252830982208,0.2182620005296485
1789790,1789791,1789790,3579581,4113.006599903107,0.21803500638088735
1791792,1791793,1791792,3583585,4117.672245979309,0.21780849855531415
1793794,1793795,1793794,3587589,4122.356248140335,0.21758247547404608
1795796,1795797,1795796,3591593,4127.001603841782,0.21735693555456237
1797798,1797799,1797798,3595597,4131.651002883911,0.21713187723071314
1799800,1799801,1799800,3599601,4136.503235816956,0.21690729893452954
1801802,1801803,1801802,3603605,4141.153810977936,0.2166831991107756
1803804,1803805,1803804,3607609,4145.800557136536,0.21645957621149137
1805806,1805807,1805806,3611613,4150.504482984543,0.21623642868871684
1807808,1807809,1807808,3615617,4155.449547052383,0.21601375500540598
1809810,1809811,1809810,3619621,4160.150623083115,0.2157915536336077
1811812,1811813,1811812,3623625,4164.804616928101,0.21556982304900885
1813814,1813815,1813814,3627629,4169.437786817551,0.2153485617309343
1815816,1815817,1815816,3631633,4174.099541902542,0.21512776817507984
1817818,1817819,1817818,3635637,4178.832950115204,0.2149074408753222
1819820,1819821,1819820,3639641,4183.813017845154,0.2146875783273572
1821822,1821823,1821822,3643645,4188.497878074646,0.2144681790505274
1823824,1823825,1823824,3647649,4193.147068977356,0.21424924155144254
1825826,1825827,1825826,3651653,4197.8661477565765,0.21403076435854018
1827828,1827829,1827828,3655657,4202.515860080719,0.2138127459984389
1829830,1829831,1829830,3659661,4207.185415029526,0.21359518500321428
1831832,1831833,1831832,3663665,4211.89159989357,0.2133780799122178
1833834,1833835,1833834,3667669,4216.709192037582,0.2131614292757149
1835836,1835837,1835836,3671673,4221.423552036285,0.21294523164579005
1837838,1837839,1837838,3675677,4226.142035961151,0.2127294855818036
1839840,1839841,1839840,3679681,4230.801050901413,0.21251418965039193
1841842,1841843,1841842,3683685,4235.468526124954,0.21229934242001036
1843844,1843845,1843844,3687689,4240.193270921707,0.21208494247184717
1845846,1845847,1845846,3691693,4244.95007109642,0.2118709883889096
1847848,1847849,1847848,3695697,4249.662735939026,0.2116574787578429
1849850,1849851,1849850,3699701,4254.392082929611,0.21144441217984422
1851852,1851853,1851852,3703705,4259.056733846664,0.2112317872524727
1853854,1853855,1853854,3707709,4263.722405910492,0.2110196025823825
1855856,1855857,1855856,3711713,4268.415844917297,0.21080785678896063
1857858,1857859,1857858,3715717,4273.0724539756775,0.21059655436511093
1859860,1859861,1859860,3719721,4277.717505931854,0.21038568840231164
1861862,1861863,1861862,3723725,4282.416085958481,0.2101752571761608
1863864,1863865,1863864,3727729,4287.1167249679565,0.20996525932605437
1865866,1865867,1865866,3731733,4291.745219945908,0.20975569349138823
1867868,1867869,1867868,3735737,4296.499185800552,0.2095465583188343
1869870,1869871,1869870,3739741,4301.280739068985,0.20933785246597836
1871872,1871873,1871872,3743745,4305.938288927078,0.20912957459040626
1873874,1873875,1873874,3747749,4310.604646921158,0.2089217233551608
1875876,1875877,1875876,3751753,4315.227801799774,0.20871429743601766
1877878,1877879,1877878,3755757,4319.886115074158,0.2085072955051146
1879880,1879881,1879880,3759761,4324.575672864914,0.20830071624732227
1881882,1881883,1881882,3763765,4329.2517030239105,0.20809455834933033
1883884,1883885,1883884,3767769,4333.947895050049,0.20788882050510438
1885886,1885887,1885886,3771773,4338.611768007278,0.20768350141042902
1887888,1887889,1887888,3775777,4343.573312997818,0.20747859977200278
1889890,1889891,1889890,3779781,4348.251757144928,0.2072741142965242
1891892,1891893,1891892,3783785,4352.928771018982,0.20707004369796778
1893894,1893895,1893894,3787789,4357.627857923508,0.20686638669940294
1895896,1895897,1895896,3791793,4362.298276901245,0.20666314202571812
1897898,1897899,1897898,3795797,4367.0987668037415,0.20646030840543972
1899900,1899901,1899900,3799801,4371.757230758667,0.2062578845761891
1901902,1901903,1901902,3803805,4376.429517745972,0.2060558692774066
1903904,1903905,1903904,3807809,4381.099759817123,0.2058542612576275
1905906,1905907,1905906,3811813,4385.783899784088,0.20565305926356814
1907908,1907909,1907908,3815817,4390.499851942062,0.2054522620564967
1909910,1909911,1909910,3819821,4395.198893070221,0.2052518683976814
1911912,1911913,1911912,3823825,4400.242692947388,0.20505187705020944
1913914,1913915,1913914,3827829,4404.961562871933,0.20485228678990097
1915916,1915917,1915916,3831833,4409.6803431510925,0.20465309638893814
1917918,1917919,1917918,3835837,4414.3159601688385,0.20445430463223602
1919920,1919921,1919920,3839841,4418.963288068771,0.20425591031198564
1921922,1921923,1921922,3843845,4423.663072109222,0.20405791220946412
1923924,1923925,1923924,3847849,4428.311846971512,0.2038603091295954
1925926,1925927,1925926,3851853,4433.019514799118,0.20366309986820852
1927928,1927929,1927928,3855857,4437.749998807907,0.2034662832338654
1929930,1929931,1929930,3859861,4442.397401809692,0.20326985804240394
1931932,1931933,1931932,3863865,4447.083482980728,0.20307382310420508
1933934,1933935,1933934,3867869,4451.794034004211,0.20287817724056367
1935936,1935937,1935936,3871873,4456.420534133911,0.20268291928005056
1937938,1937939,1937938,3875877,4461.360008955002,0.20248804805669351
1939940,1939941,1939940,3879881,4466.075471878052,0.2022935623972444
1941942,1941943,1941942,3883885,4470.728209972382,0.2020994611466449
1943944,1943945,1943944,3887889,4475.394414901733,0.2019057431480178
1945946,1945947,1945946,3891893,4480.171870946884,0.20171240725358075
1947948,1947949,1947948,3895897,4484.8787751197815,0.20151945231737045
1949950,1949951,1949950,3899901,4489.547554016113,0.20132687719342357
1951952,1951953,1951952,3903905,4494.194893121719,0.20113468074669072
1953954,1953955,1953954,3907909,4499.22262597084,0.20094286185121746
1955956,1955957,1955956,3911913,4504.0372059345245,0.2007514193701354
1957958,1957959,1957958,3915917,4508.732905864716,0.20056035218840407
1959960,1959961,1959960,3919921,4513.391453027725,0.20036965918188798
1961962,1961963,1961962,3923925,4518.073987722397,0.20017933923918463
1963964,1963965,1963964,3927929,4522.7506980896,0.19998939124889148
1965966,1965967,1965966,3931933,4527.478595018387,0.19979981410870096
1967968,1967969,1967968,3935937,4532.302670955658,0.1996106067126675
1969970,1969971,1969970,3939941,4536.935380935669,0.19942176797121647
1971972,1971973,1971972,3943945,4541.64004778862,0.19923329678567825
1973974,1973975,1973974,3947949,4546.294841766357,0.19904519207375415
1975976,1975977,1975976,3951953,4550.921060800552,0.1988574527495075
1977978,1977979,1977978,3955957,4555.73059797287,0.19867007773609657
1979980,1979981,1979980,3959961,4560.4220678806305,0.19848306595849863
1981982,1981983,1981982,3963965,4565.210164070129,0.19829641634169093
1983984,1983985,1983984,3967969,4569.902776002884,0.19811012782520265
1985986,1985987,1985986,3971973,4574.543251037598,0.19792419934128702
1987988,1987989,1987988,3975977,4579.247550010681,0.19773862983674917
1989990,1989991,1989990,3979981,4583.955366849899,0.19755341825839423
1991992,1991993,1991992,3983985,4588.607778072357,0.19736856355484633
1993994,1993995,1993994,3987989,4593.2763459682465,0.19718406468018657
1995996,1995997,1995996,3991993,4597.934273958206,0.196999920593953
1997998,1997999,1997998,3995997,4602.866447925568,0.19681613025932165
2000000,2000001,2000000,4000001,4607.572920799255,0.19663269264310657


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0058441162109375,12064.709122577777
1001,7464,7464,14928,22.337682962417603,0.20711947713971313
2002,15168,15168,30336,47.1640510559082,0.033931367774130194
3003,22980,22980,45960,74.1202540397644,0.023931723146233708
4004,30900,30900,61800,98.12813019752502,0.02163328727874614
5005,38802,38802,77604,122.24070906639099,0.021135450318979565
6006,46722,46722,93444,149.71453189849854,0.019952024764279486
7007,54656,54656,109312,176.52278113365173,0.01942558198243205
8008,62520,62520,125040,202.8719141483307,0.013227093633759068
9009,70474,70474,140948,226.82937002182007,0.013088619421978365
10010,78444,78444,156888,252.5719211101532,0.013014944728638511
11011,86268,86268,172536,278.30533504486084,0.00910960692090157
12012,94212,94212,188424,303.17382621765137,0.009079115157874185
13013,102154,102154,204308,327.07973408699036,0.008891416662663687
14014,110116,110116,220232,354.2395250797272,0.0088567284947203
15015,118072,118072,236144,378.66551518440247,0.008771253462327877
16016,126014,126014,252028,402.6845588684082,0.008301757843582891
17017,134008,134008,268016,427.63274598121643,0.008296194935610401
18018,141994,141994,283988,452.1954550743103,0.00825646351040632
19019,149980,149980,299960,478.6927869319916,0.00824022644519573
20020,157980,157980,315960,508.8689911365509,0.00823686442890903
21021,165978,165978,331956,537.063001871109,0.008231528809119482
22022,173842,173842,347684,565.1250171661377,0.003059662985833711
23023,181778,181778,363556,591.4076581001282,0.0030518880776071455
24024,189766,189766,379532,623.3845510482788,0.0030502662193612196
25025,197746,197746,395492,654.3624951839447,0.003047534855795675
26026,205726,205726,411452,684.2512891292572,0.0030448771358351223
27027,213648,213648,427296,713.8214380741119,0.0029866077293263515
28028,221624,221624,443248,743.979325056076,0.002983521453643334
29029,229606,229606,459212,771.7895171642303,0.002976289730213466
30030,237598,237598,475196,795.9876282215118,0.0029756170224572998
31031,245592,245592,491184,817.7576432228088,0.0029742751776211662
32032,253566,253566,507132,842.6080420017242,0.002952171238575829
33033,261534,261534,523068,866.9546940326691,0.0029472911410266533
34034,269530,269530,539060,890.9341552257538,0.002946503491330077
35035,277450,277450,554900,913.1285500526428,0.0027701464114215923
36036,285406,285406,570812,935.3121140003204,0.0027650704632833367
37037,293398,293398,586796,957.6555359363556,0.0027645146765280515
38038,301392,301392,602784,982.9666221141815,0.002764008646408911
39039,309348,309348,618696,1006.1300270557404,0.002746056323303492
40040,317334,317334,634668,1030.9737720489502,0.0027442900300229667
41041,325330,325330,650660,1054.8438701629639,0.0027437515473138774
42042,333324,333324,666648,1080.2317471504211,0.0027417949713708367
43043,341312,341312,682624,1104.2962839603424,0.0027409733993408736
44044,349308,349308,698616,1128.6539101600647,0.0027404856937209843
45045,357286,357286,714572,1152.5920209884644,0.002666634472916485
46046,365266,365266,730532,1177.6816930770874,0.002660747422851273
47047,373258,373258,746516,1201.565187215805,0.002660300373463542
48048,381252,381252,762504,1225.7138919830322,0.0026597569940349786
49049,389248,389248,778496,1249.7344059944153,0.0026593696256895782
50050,397240,397240,794480,1276.0980360507965,0.002658844958205009
51051,405222,405222,810444,1301.758424282074,0.0026359743296779925
52052,413200,413200,826400,1327.5116219520569,0.002632535255543189
53053,421188,421188,842376,1352.4250042438507,0.0026309112363378517
54054,429174,429174,858348,1377.1334071159363,0.0026292307666153647
55055,437168,437168,874336,1399.9464468955994,0.0026283010538463714
56056,445166,445166,890332,1422.2358238697052,0.002627841902722139
57057,453162,453162,906324,1444.6103119850159,0.002627398291224381
58058,461150,461150,922300,1466.9689311981201,0.0026252891093463404
59059,469142,469142,938284,1490.849583864212,0.0026248204776493367
60060,477132,477132,954264,1514.1772480010986,0.002624125465445104
61061,485114,485114,970228,1536.1522760391235,0.002603795901450212
62062,493108,493108,986216,1560.341313123703,0.0026032918322016485
63063,500986,500986,1001972,1585.4233832359314,0.002417935987978126
64064,508964,508964,1017928,1608.239193201065,0.002414960423266166
65065,516956,516956,1033912,1632.0857031345367,0.002414373846477247
66066,524938,524938,1049876,1654.6326229572296,0.0024099243000819115
67067,532934,532934,1065868,1677.8712179660797,0.002409630435067811
68068,540924,540924,1081848,1703.0935702323914,0.0024081805549940327
69069,548900,548900,1097800,1729.0901908874512,0.00240120117632614
70070,556884,556884,1113768,1753.0372860431671,0.00240033851514454
71071,564880,564880,1129760,1777.5402040481567,0.002399970106125693
72072,572800,572800,1145600,1801.3743340969086,0.0019959337914770003
73073,580760,580760,1161520,1824.775689125061,0.001992120876820991
74074,588746,588746,1177492,1848.7652418613434,0.0019917241879738867
75075,596740,596740,1193480,1872.3026061058044,0.0019912867046514293
76076,604734,604734,1209468,1894.961818933487,0.001991030387216597
77077,612726,612726,1225452,1919.8111009597778,0.0019898096379620256
78078,620722,620722,1241444,1943.0842580795288,0.0019895689401892014
79079,628716,628716,1257432,1965.8287591934204,0.001987739306059666
80080,636710,636710,1273420,1990.144373178482,0.001987221907256753
81081,644704,644704,1289408,2013.9782040119171,0.0019867615919793025
82082,652702,652702,1305404,2037.0974140167236,0.0019864651549141854
83083,660698,660698,1321396,2060.0347430706024,0.0019862440967699513
84084,668690,668690,1337380,2083.563383102417,0.0019841727680613985
85085,676686,676686,1353372,2107.808867931366,0.001983876085432712
86086,684682,684682,1369364,2132.569904088974,0.0019835199127555825
87087,692678,692678,1385356,2157.094587087631,0.0019832608377328143
88088,700664,700664,1401328,2181.844507932663,0.001978168438654393
89089,708662,708662,1417324,2205.641222000122,0.0019779500689764973
90090,716662,716662,1433324,2229.423267841339,0.0019775579621637007
91091,724664,724664,1449328,2253.670328140259,0.001977226547751343
92092,732660,732660,1465320,2277.9142060279846,0.001976900235604262
93093,740660,740660,1481320,2301.8443660736084,0.0019761713811021764
94094,748584,748584,1497168,2326.0803599357605,0.0005695894033124205
95095,756536,756536,1513072,2354.1624541282654,0.0005692783524864353
96096,764504,764504,1529008,2377.632511138916,0.0005688375676982105
97097,772500,772500,1545000,2400.4199590682983,0.0005688203364115907
98098,780500,780500,1561000,2424.519322872162,0.0005687448556273011
99099,788502,788502,1577004,2451.025153160095,0.0005686506519850809
100100,796500,796500,1593000,2477.57874417305,0.0005686257682100404
101101,804504,804504,1609008,2504.214476108551,0.0005686202639481053
102102,812502,812502,1625004,2530.931116104126,0.0005684430834662635
103103,820506,820506,1641012,2557.4734239578247,0.0005684193947672611
104104,828512,828512,1657024,2584.210594177246,0.0005684121115336893
105105,836518,836518,1673036,2617.5389552116394,0.0005683998097083531
106106,844520,844520,1689040,2646.881462097168,0.0005682248647644883
107107,852526,852526,1705052,2675.8297820091248,0.0005682202317984775
108108,860534,860534,1721068,2703.630844116211,0.0005682188439095626
109109,868540,868540,1737080,2732.0390820503235,0.0005682114060618915
110110,876548,876548,1753096,2763.0561010837555,0.0005682100181729766
111111,884554,884554,1769108,2791.4667870998383,0.0005682048795279115
112112,892562,892562,1785124,2820.4862921237946,0.0005682034898200072
113113,900566,900566,1801132,2848.78120303154,0.0005681140737578971
114114,908570,908570,1817140,2876.8844799995422,0.0005681019192707026
115115,916578,916578,1833156,2905.012498140335,0.0005681005332007771
116116,924582,924582,1849164,2934.2260439395905,0.0005680553858837811
117117,932586,932586,1865172,2962.71617102623,0.0005680477170244558
118118,940592,940592,1881184,2992.7264568805695,0.0005680418616975658
119119,948598,948598,1897196,3021.7596759796143,0.0005680257909261854
120120,956602,956602,1913204,3052.4582240581512,0.0005678149791492615
121121,964608,964608,1929216,3082.073147058487,0.0005678122925019125
122122,972614,972614,1945228,3112.058802127838,0.0005677955214196118
123123,980622,980622,1961244,3141.5514481067657,0.0005677941353496863
124124,988630,988630,1977260,3166.665544986725,0.0005677927510987502
125125,996638,996638,1993276,3194.68412399292,0.0005677913650288247
126126,1004644,1004644,2009288,3220.6929202079773,0.0005677715653291671
127127,1012652,1012652,2025304,3246.373591184616,0.0005677701792592416
128128,1020660,1020660,2041320,3271.727741956711,0.0005677687986462843
129129,1028666,1028666,2057332,3297.027976036072,0.0005677574390574591
130130,1036674,1036674,2073348,3322.268846988678,0.000567756054806523
131131,1044680,1044680,2089360,3347.5940461158752,0.0005676971813954879
132132,1052686,1052686,2105372,3372.6982321739197,0.000567695820791414
133133,1060694,1060694,2121388,3397.84614109993,0.0005676944365404779
134134,1068700,1068700,2137400,3422.963176012039,0.0005676761647919193
135135,1076706,1076706,2153412,3447.835060119629,0.00056767405840219
136136,1084714,1084714,2169428,3474.4516801834106,0.0005676726759702433
137137,1092720,1092720,2185440,3499.1978681087494,0.0005676524342561606
138138,1100726,1100726,2201452,3523.3239572048187,0.000567645760384039
139139,1108728,1108728,2217456,3547.232848882675,0.0005674083622579928
140140,1116736,1116736,2233472,3570.8574459552765,0.0005674069780070568
141141,1124742,1124742,2249484,3596.150938987732,0.0005673942487192107
142142,1132750,1132750,2265500,3619.6438381671906,0.000567392866287264
143143,1140758,1140758,2281516,3642.6859040260315,0.0005673914856743068
144144,1148764,1148764,2297528,3666.386463165283,0.000567361872526817
145145,1156770,1156770,2313540,3689.3496820926666,0.000567358865737333
146146,1164778,1164778,2329556,3712.741259098053,0.0005673574833053863
147147,1172784,1172784,2345568,3733.976589202881,0.0005673465384461451
148148,1180792,1180792,2361584,3754.8233318328857,0.0005673451560141984
149149,1188800,1188800,2377600,3778.5467960834503,0.0005673437735822517
150150,1196804,1196804,2393608,3801.7301251888275,0.0005673123559972737
151151,1204812,1204812,2409624,3826.8367400169373,0.000567310973565327
152152,1212820,1212820,2425640,3848.095158100128,0.0005673095929523697
153153,1220826,1220826,2441652,3869.286994934082,0.0005672511288139503
154154,1228832,1228832,2457664,3891.2339441776276,0.0005672473707818426
155155,1236840,1236840,2473680,3913.3077211380005,0.0005672459901688853
156156,1244846,1244846,2489692,3936.647040128708,0.000567186421903898
157157,1252854,1252854,2505708,3958.8262951374054,0.0005671850412909407
158158,1260862,1260862,2521724,3982.6432111263275,0.000567183658858994
159159,1268868,1268868,2537736,4007.194077014923,0.0005671322978741955
160160,1276876,1276876,2553752,4027.814261198044,0.0005671309172612382
161161,1284884,1284884,2569768,4048.779294013977,0.0005671295348292915
162162,1292888,1292888,2585776,4069.826940059662,0.0005671121234627208
163163,1300896,1300896,2601792,4090.9408688545227,0.0005671107410307741
164164,1308902,1308902,2617804,4112.266324043274,0.0005670899572578492
165165,1316910,1316910,2633820,4134.589154243469,0.0005670885748259025
166166,1324916,1324916,2649832,4158.47119307518,0.000567084520298522
167167,1332924,1332924,2665848,4179.91784620285,0.0005670831415045541
168168,1340930,1340930,2681860,4201.0581929683685,0.0005670798527717125
169169,1348938,1348938,2697876,4221.712688922882,0.0005670784703397658
170170,1356942,1356942,2713884,4244.009602069855,0.0005667703007929958
171171,1364950,1364950,2729900,4266.016750097275,0.0005667689183610491
172172,1372958,1372958,2745916,4288.282329082489,0.0005667675395670813
173173,1380966,1380966,2761932,4310.413254976273,0.0005667661607731134
174174,1388974,1388974,2777948,4332.553112268448,0.0005667647801601561
175175,1396980,1396980,2793960,4354.184633016586,0.0005667526384058874
176176,1404988,1404988,2809976,4375.371755123138,0.0005667512596119195
177177,1412996,1412996,2825992,4396.3765251636505,0.0005667498789989622
178178,1421002,1421002,2842004,4418.18977689743,0.000566614111448871
179179,1429010,1429010,2858020,4440.97998714447,0.0005666127308359137
180180,1437016,1437016,2874032,4462.494589090347,0.0005666067136189668
181181,1445024,1445024,2890048,4486.635045051575,0.0005666053348249989
182182,1453030,1453030,2906060,4511.745404958725,0.0005666018769261427
183183,1461036,1461036,2922072,4534.3164529800415,0.0005665987155225594
184184,1469042,1469042,2938084,4556.850037097931,0.0005664396685460815
185185,1477050,1477050,2954100,4579.1990921497345,0.0005664382933900924
186186,1485058,1485058,2970116,4601.487809181213,0.0005664369145961246
187187,1493066,1493066,2986132,4624.48209810257,0.0005664355339831673
188188,1501070,1501070,3002140,4648.682251214981,0.0005664225136570167
189189,1509078,1509078,3018156,4672.025053977966,0.0005664211348630488
190190,1517084,1517084,3034168,4695.335026025772,0.0005662480107275769
191191,1525092,1525092,3050184,4718.503251075745,0.0005662466355715878
192192,1533100,1533100,3066200,4741.107465028763,0.0005662452567776199
193193,1541106,1541106,3082212,4763.603976011276,0.0005662399962602649
194194,1549114,1549114,3098228,4786.138295173645,0.000566238617466297
195195,1557122,1557122,3114244,4808.520071029663,0.0005662372404913185
196196,1565130,1565130,3130260,4831.007629156113,0.00056623586351634
197197,1573136,1573136,3146272,4853.614758014679,0.0005662338953698054
198198,1581132,1581132,3162264,4876.04208111763,0.0005662275161739672
199199,1589140,1589140,3178280,4901.701044082642,0.0005662261555698933
200200,1597142,1597142,3194284,4930.377199888229,0.0005662192852469161
201201,1605148,1605148,3210296,4956.6792368888855,0.0005662100138579262
202202,1613156,1613156,3226312,4980.367117166519,0.0005662086550728418
203203,1621162,1621162,3242324,5004.1297471523285,0.0005661912018695148
204204,1629170,1629170,3258340,5027.5749771595,0.0005661898394464515
205205,1637176,1637176,3274352,5051.8860721588135,0.0005661787763528991
206206,1645184,1645184,3290368,5075.889643192291,0.0005661774157488253
207207,1653192,1653192,3306384,5099.489905118942,0.0005661760551447514
208208,1661198,1661198,3322396,5124.082407951355,0.0005661677932948805
209209,1669204,1669204,3338408,5149.380733013153,0.0005660827810061164
210210,1677212,1677212,3354424,5172.20019698143,0.0005660814204020426
211211,1685220,1685220,3370440,5192.611859083176,0.0005660800579789793
212212,1693226,1693226,3386452,5213.143200159073,0.0005659485341311665
213213,1701232,1701232,3402464,5234.301270008087,0.0005659454636770533
214214,1709240,1709240,3418480,5255.361251115799,0.0005659441012539901
215215,1717244,1717244,3434488,5276.372796058655,0.0005659038288285956
216216,1725252,1725252,3450504,5297.24125123024,0.0005659024664055323
217217,1733256,1733256,3466512,5319.0141389369965,0.0005658281243086094
218218,1741264,1741264,3482528,5340.107956171036,0.0005658267637045356
219219,1749270,1749270,3498540,5361.114171028137,0.0005658240534103243
220220,1757276,1757276,3514552,5382.113888025284,0.0005658132813550765
221221,1765284,1765284,3530568,5403.02276301384,0.000565811922569992
222222,1773290,1773290,3546580,5423.978103160858,0.0005657461006194353
223223,1781298,1781298,3562596,5444.905484199524,0.0005657447400153615
224224,1789306,1789306,3578612,5465.845276117325,0.000565743381230277
225225,1797314,1797314,3594628,5488.3710770606995,0.0005657420206262032
226226,1805320,1805320,3610640,5509.84517788887,0.0005657396377500845
227227,1813326,1813326,3626652,5530.620509147644,0.000565734762858483
228228,1821334,1821334,3642668,5551.247160196304,0.0005657334040733986
229229,1829340,1829340,3658680,5571.712069988251,0.0005657140045514097
230230,1837348,1837348,3674696,5592.338613033295,0.0005657126457663253
231231,1845354,1845354,3690708,5612.901819944382,0.000565707077839761
232232,1853362,1853362,3706724,5633.5920259952545,0.0005657057190546766
233233,1861368,1861368,3722736,5654.233741044998,0.000565699026992661
234234,1869376,1869376,3738752,5674.875977039337,0.0005656976663885871
235235,1877384,1877384,3754768,5695.446798086166,0.0005656963076035026
236236,1885390,1885390,3770780,5716.10719704628,0.000565683345485013
237237,1893398,1893398,3786796,5736.778636217117,0.0005656819885189179
238238,1901404,1901404,3802808,5757.505645275116,0.0005656717330566607
239239,1909412,1909412,3818824,5778.162847995758,0.0005656703742715763
240240,1917418,1917418,3834836,5798.85259103775,0.0005656388784700539
241241,1925426,1925426,3850852,5819.507427215576,0.00056563751786598
242242,1933432,1933432,3866864,5840.096019029617,0.0005655207223753678
243243,1941438,1941438,3882876,5857.76264500618,0.0005655187833326636
244244,1949446,1949446,3898892,5879.055466175079,0.0005655174263665685
245245,1957454,1957454,3914908,5900.095008134842,0.0005655160694004735
246246,1965460,1965460,3930920,5921.498637199402,0.0005655043678416405
247247,1973468,1973468,3946936,5942.250168085098,0.000565503009056556
248248,1981474,1981474,3962948,5962.930149078369,0.0005654526994476328
249249,1989480,1989480,3978960,5983.541618108749,0.0005654494871123461
250250,1997488,1997488,3994976,6004.076382160187,0.0005654481283272617
251251,2005494,2005494,4010988,6024.742300033569,0.00056530424990342
252252,2013500,2013500,4027000,6045.443649053574,0.0005653033913404215
253253,2021506,2021506,4043012,6066.0743932724,0.0005652899872075068
254254,2029514,2029514,4059028,6086.699536085129,0.0005652886284224223
255255,2037520,2037520,4075040,6107.283169031143,0.0005652867785101989
256256,2045528,2045528,4091056,6127.9766709804535,0.0005652854215441039
257257,2053534,2053534,4107068,6148.609053134918,0.0005652444469887996
258258,2061542,2061542,4123084,6169.252559900284,0.0005652430882037152
259259,2069548,2069548,4139096,6189.855684041977,0.0005652411418850534
260260,2077554,2077554,4155108,6210.476763963699,0.0005652316049236106
261261,2085562,2085562,4171124,6231.2409591674805,0.0005652302479575155
262262,2093568,2093568,4187136,6251.942668199539,0.0005652166582876816
263263,2101576,2101576,4203152,6272.612960100174,0.0005652153013215866
264264,2109584,2109584,4219168,6293.17991900444,0.0005652139425365021
265265,2117586,2117586,4235172,6313.799061059952,0.0005651870942529058
266266,2125594,2125594,4251188,6334.42304110527,0.0005651857391058002
267267,2133602,2133602,4267204,6355.224102973938,0.0005651843803207157
268268,2141608,2141608,4283216,6375.884599208832,0.0005651778883475345
269269,2149612,2149612,4299224,6396.444129228592,0.0005651612555084284
270270,2157620,2157620,4315240,6417.06275510788,0.0005651598985423334
271271,2165628,2165628,4331256,6437.775857925415,0.0005651585433952278
272272,2173632,2173632,4347264,6458.384489059448,0.0005651420269714436
273273,2181640,2181640,4363280,6478.942873954773,0.0005651406700053485
274274,2189646,2189646,4379292,6499.599645137787,0.0005651354676956544
275275,2197654,2197654,4395308,6520.268285989761,0.0005651341107295593
276276,2205658,2205658,4411316,6540.888388872147,0.0005651022202073364
277277,2213666,2213666,4427332,6561.451878070831,0.0005651008614222519
278278,2221668,2221668,4443336,6582.071696996689,0.0005648253754770849
279279,2229676,2229676,4459352,6602.713777065277,0.0005648240203299792
280280,2237684,2237684,4475368,6623.282380104065,0.0005648226651828736
281281,2245690,2245690,4491380,6643.880268096924,0.0005647924808727112
282282,2253698,2253698,4507396,6664.731768846512,0.0005647911257256055
283283,2261704,2261704,4523408,6685.491815090179,0.00056477308862668
284284,2269712,2269712,4539424,6706.046773195267,0.0005647717316605849
285285,2277718,2277718,4555436,6726.807579040527,0.0005647648358717561
286286,2285726,2285726,4571452,6747.359434127808,0.0005647634807246504
287287,2293732,2293732,4587464,6767.980943918228,0.0005647029702231521
288288,2301740,2301740,4603480,6788.726116895676,0.0005647016150760464
289289,2309748,2309748,4619496,6809.262233972549,0.0005647002617479302
290290,2317754,2317754,4635508,6829.717559099197,0.0005646908375638304
291291,2325760,2325760,4651520,6850.236218929291,0.0005646903318847762
292292,2333768,2333768,4667536,6870.821587085724,0.00056468897855666
293293,2341772,2341772,4683544,6891.3764860630035,0.0005646302943205228
294294,2349780,2349780,4699560,6911.931612968445,0.0005646289391734172
295295,2357788,2357788,4715576,6932.420398235321,0.0005646275840263115
296296,2365794,2365794,4731588,6952.943372249603,0.0005646169120154809
297297,2373802,2373802,4747604,6973.583778142929,0.0005646155550493859
298298,2381808,2381808,4763616,6994.187992095947,0.0005645589080813807
299299,2389816,2389816,4779632,7014.749624967575,0.000564557552934275
300300,2397824,2397824,4795648,7035.394721031189,0.0005645561996061588
301301,2405830,2405830,4811660,7055.954744100571,0.0005645527908200165
302302,2413838,2413838,4827676,7076.608287096024,0.0005645514374919003
303303,2421844,2421844,4843688,7097.158687114716,0.0005645471646857914
304304,2429848,2429848,4859696,7117.787431001663,0.0005643997901643161
305305,2437856,2437856,4875712,7138.3312022686005,0.0005643984350172104
306306,2445860,2445860,4891720,7158.850932121277,0.0005643746026180452
307307,2453868,2453868,4907736,7179.4967041015625,0.0005643732492899289
308308,2461876,2461876,4923752,7200.033607959747,0.0005643718977808021
309309,2469882,2469882,4939764,7220.562490940094,0.0005643481508741388
310310,2477890,2477890,4955780,7241.159598112106,0.0005643467975460226
311311,2485896,2485896,4971792,7261.704280138016,0.0005643426102324156
312312,2493904,2493904,4987808,7282.334745168686,0.0005643412587232888
313313,2501910,2501910,5003820,7303.010097980499,0.0005643362837872701
314314,2509918,2509918,5019836,7323.838016033173,0.0005643349304591538
315315,2517924,2517924,5035848,7344.561548233032,0.0005643209678964922
316316,2525932,2525932,5051864,7365.107692241669,0.0005643196127493866
317317,2533938,2533938,5067876,7385.793061971664,0.0005642875203193398
318318,2541946,2541946,5083892,7406.547893047333,0.000564286168810213
319319,2549954,2549954,5099908,7427.2323751449585,0.0005642848136631073
320320,2557960,2557960,5115920,7447.93826508522,0.0005640449726342922
321321,2565968,2565968,5131936,7468.4375739097595,0.0005640436174871866
322322,2573976,2573976,5147952,7489.006042957306,0.0005640422659780597
323323,2581982,2581982,5163964,7509.769611120224,0.0005640337421937147
324324,2589988,2589988,5179976,7530.4888870716095,0.000564027712243842
325325,2597996,2597996,5195992,7551.274117946625,0.0005640263607347151
326326,2606002,2606002,5212004,7571.93235707283,0.0005640212493744912
327327,2614010,2614010,5228020,7592.691522121429,0.0005640198960463749
328328,2622016,2622016,5244032,7613.267067909241,0.0005640100553137017
329329,2630024,2630024,5260048,7634.0729858875275,0.0005640087019855855
330330,2638030,2638030,5276060,7654.832286119461,0.0005639983410219429
331331,2646038,2646038,5292076,7675.437909126282,0.0005639969876938267
332332,2654044,2654044,5308088,7696.011377096176,0.0005638675484078703
333333,2662050,2662050,5324100,7716.63884806633,0.0005638633429043693
334334,2670056,2670056,5340112,7737.155470132828,0.000563849611353362
335335,2678064,2678064,5356128,7757.698152065277,0.0005638482616632245
336336,2686072,2686072,5372144,7778.369131088257,0.0005638469083351083
337337,2694078,2694078,5388156,7799.153198957443,0.0005638131242449163
338338,2702086,2702086,5404172,7819.810503959656,0.0005638117727357894
339339,2710094,2710094,5420188,7840.509802103043,0.0005638104212266626
340340,2718102,2718102,5436204,7861.3307909965515,0.0005638090678985463
341341,2726108,2726108,5452216,7881.912598133087,0.0005637887588818558
342342,2734116,2734116,5468232,7902.653048992157,0.0005637874073727289
343343,2742122,2742122,5484244,7923.298772096634,0.0005636641708406387
344344,2750128,2750128,5500256,7943.902936220169,0.00056365907403233
345345,2758136,2758136,5516272,7964.612082958221,0.0005636577225232031
346346,2766144,2766144,5532288,7985.245465993881,0.0005636563728330657
347347,2774150,2774150,5548300,8005.910399198532,0.0005636216701532248
348348,2782158,2782158,5564316,8026.545550107956,0.000563620318644098
349349,2790166,2790166,5580332,8047.114464044571,0.0005636189671349712
350350,2798172,2798172,5596344,8067.856323957443,0.0005636049336317228
351351,2806180,2806180,5612360,8088.5998520851135,0.0005636035839415854
352352,2814188,2814188,5628376,8109.37863612175,0.000563602234251448
353353,2822194,2822194,5644388,8129.992166996002,0.0005635958914353978
354354,2830200,2830200,5660400,8151.099533081055,0.0005635507059196243
355355,2838208,2838208,5676416,8172.016019105911,0.0005635493525915081
356356,2846216,2846216,5692432,8192.600439071655,0.0005635480029013706
357357,2854222,2854222,5708444,8213.260824203491,0.0005635186553263338
358358,2862230,2862230,5724460,8233.959081172943,0.0005635173056361964
359359,2870236,2870236,5740472,8254.598976135254,0.0005634988156089094
360360,2878244,2878244,5756488,8275.302379131317,0.0005634974659187719
361361,2886252,2886252,5772504,8296.08767914772,0.0005634961162286345
362362,2894260,2894260,5788520,8316.829713106155,0.0005634947647195077
363363,2902266,2902266,5804532,8337.55402302742,0.0005634852404909907
364364,2910274,2910274,5820548,8358.34604024887,0.0005634838908008533
365365,2918280,2918280,5836560,8378.978207111359,0.0005634793396893656
366366,2926286,2926286,5852572,8399.710623025894,0.0005634483459289186
367367,2934294,2934294,5868588,8420.566068172455,0.0005634469962387811
368368,2942302,2942302,5884604,8441.367510080338,0.0005634456447296543
369369,2950310,2950310,5900620,8462.136611938477,0.0005634442950395169
370370,2958316,2958316,5916632,8482.926120996475,0.0005634255812765332
371371,2966324,2966324,5932648,8503.63237786293,0.0005634242315863958
372372,2974332,2974332,5948664,8524.462369203568,0.0005634228800772689
373373,2982340,2982340,5964680,8545.360725164413,0.0005634215303871315
374374,2990344,2990344,5980688,8566.049612045288,0.0005633787422993919
375375,2998350,2998350,5996700,8586.804931163788,0.0005633766613755142
376376,3006356,3006356,6012712,8607.580316066742,0.0005633724122162675
377377,3014364,3014364,6028728,8628.436479091644,0.0005633710643451195
378378,3022372,3022372,6044744,8649.100317001343,0.0005633697128359927
379379,3030378,3030378,6060756,8669.967625141144,0.0005633389264403377
380380,3038386,3038386,6076772,8690.765652179718,0.0005633375767502002
381381,3046392,3046392,6092784,8711.411629199982,0.0005633293876599055
382382,3054400,3054400,6108800,8732.146775245667,0.000563328037969768
383383,3062406,3062406,6124812,8752.920537948608,0.0005633178807329386
384384,3070414,3070414,6140828,8773.742444038391,0.0005633165328617906
385385,3078422,3078422,6156844,8794.55757021904,0.0005633151813526638
386386,3086428,3086428,6172856,8815.308266162872,0.0005633054024656303
387387,3094436,3094436,6188872,8836.163085222244,0.0005633040564134717
388388,3102442,3102442,6204884,8856.983174085617,0.0005632794618577464
389389,3110448,3110448,6220896,8877.720340013504,0.0005632806933135726
390390,3118456,3118456,6236912,8898.450602054596,0.0005632793436234351
391391,3126462,3126462,6252924,8919.286942005157,0.0005632732318190392
392392,3134466,3134466,6268932,8940.009218215942,0.0005632477495964849
393393,3142474,3142474,6284948,8960.733129024506,0.0005632464017253369
394394,3150482,3150482,6300964,8981.618305206299,0.0005632450520351995
395395,3158486,3158486,6316972,9002.373094081879,0.0005632220818370115
396396,3166492,3166492,6332984,9023.16002202034,0.0005632154679915402
397397,3174498,3174498,6348996,9043.907086133957,0.0005631703952531097
398398,3182506,3182506,6365012,9064.711126089096,0.0005631690455629723
399399,3190514,3190514,6381028,9085.560026884079,0.0005631676995108137
400400,3198518,3198518,6397036,9106.444093942642,0.0005631502826872747
401401,3206526,3206526,6413052,9127.39488697052,0.0005631489329971373
402402,3214534,3214534,6429068,9148.219474077225,0.0005631475869449787
403403,3222540,3222540,6445080,9169.052791118622,0.0005631357744277921
404404,3230548,3230548,6461096,9189.873336076736,0.000563134426556644
405405,3238556,3238556,6477112,9210.677649974823,0.000563133078685496
406406,3246562,3246562,6493124,9231.45320725441,0.00056312815650017
407407,3254566,3254566,6509132,9252.29223895073,0.0005631043877656339
408408,3262574,3262574,6525148,9273.161142110825,0.0005631030380754964
409409,3270582,3270582,6541164,9293.951397895813,0.0005631016902043484
410410,3278588,3278588,6557176,9314.948965072632,0.0005630931991618127
411411,3286594,3286594,6573188,9335.7416369915,0.0005630895375361433
412412,3294602,3294602,6589204,9356.540503263474,0.0005630881878460059
413413,3302608,3302608,6605216,9377.68516421318,0.0005630285977531457
414414,3310616,3310616,6621232,9398.469249248505,0.0005630272517009871
415415,3318624,3318624,6637248,9419.33256816864,0.0005630259020108497
416416,3326630,3326630,6653260,9440.181385040283,0.0005630067626043456
417417,3334638,3334638,6669276,9461.209028959274,0.0005630054147331975
418418,3342646,3342646,6685292,9482.25679397583,0.0005630040668620495
419419,3350652,3350652,6701304,9503.251097917557,0.0005629979350487702
420420,3358660,3358660,6717320,9524.496133089066,0.0005629965871776221
421421,3366666,3366666,6733332,9545.649058103561,0.0005629845600196859
422422,3374674,3374674,6749348,9566.84807896614,0.0005629832121485379
423423,3382680,3382680,6765360,9587.275381088257,0.0005629612405755324
424424,3390688,3390688,6781376,9606.88846898079,0.0005629598927043844
425425,3398696,3398696,6797392,9629.188691139221,0.0005629585448332364
426426,3406702,3406702,6813404,9650.551132917404,0.0005629419156321092
427427,3414710,3414710,6829420,9671.425671100616,0.0005629405677609611
428428,3422716,3422716,6845432,9692.332818031311,0.0005629380484606372
429429,3430722,3430722,6861444,9713.248514175415,0.0005629264651361154
430430,3438730,3438730,6877460,9734.209495067596,0.0005629251190839568
431431,3446738,3446738,6893476,9755.272083044052,0.0005629237693938194
432432,3454744,3454744,6909488,9776.162467241287,0.00056284603124368
433433,3462752,3462752,6925504,9797.162575006485,0.0005628446870105108
434434,3470760,3470760,6941520,9818.204169988632,0.0005628433391393628
435435,3478766,3478766,6957532,9839.193947076797,0.0005628274884657003
436436,3486774,3486774,6973548,9860.475395917892,0.0005628261424135417
437437,3494778,3494778,6989556,9881.565455913544,0.0005628192011499777
438438,3502784,3502784,7005568,9902.727405071259,0.0005628057679132326
439439,3510792,3510792,7021584,9923.626680850983,0.0005628044182230951
440440,3518798,3518798,7037596,9944.845586061478,0.0005627856589853764
441441,3526806,3526806,7053612,9966.236128091812,0.0005627843129332177
442442,3534812,3534812,7069624,9987.581003189087,0.0005627813516184688
443443,3542816,3542816,7085632,10009.205966949463,0.0005627258888125652
444444,3550824,3550824,7101648,10030.659003019333,0.0005627245427604066
445445,3558830,3558830,7117660,10052.107459068298,0.0005627026621368714
446446,3566838,3566838,7133676,10073.550169229507,0.0005627013160847127
447447,3574846,3574846,7149692,10095.043091058731,0.0005626999682135647
448448,3582852,3582852,7165704,10116.672071933746,0.0005626953006867552
449449,3590860,3590860,7181720,10138.133357048035,0.0005626939546345966
450450,3598866,3598866,7197732,10159.545530080795,0.0005626689562632237
451451,3606874,3606874,7213748,10180.990136146545,0.000562667610211065
452452,3614882,3614882,7229764,10202.479233026505,0.000562666262339917
453453,3622884,3622884,7245768,10223.95714211464,0.000562560759135522
454454,3630892,3630892,7261784,10245.500194072723,0.0005625594130833633
455455,3638898,3638898,7277796,10266.980715036392,0.0005625530575343873
456456,3646906,3646906,7293812,10288.439663887024,0.0005625517096632393
457457,3654912,3654912,7309824,10309.892590284348,0.0005625363392027793
458458,3662920,3662920,7325840,10331.451454162598,0.0005625349931506207
459459,3670926,3670926,7341852,10353.17220902443,0.0005625310113828164
460460,3678934,3678934,7357868,10374.801097154617,0.0005625296671496471
461461,3686942,3686942,7373884,10396.279328107834,0.0005625283210974885
462462,3694948,3694948,7389896,10417.805104970932,0.0005625009544019122
463463,3702956,3702956,7405912,10439.365703105927,0.0005624996065307641
464464,3710962,3710962,7421924,10460.90938091278,0.0005624982677545631
465465,3718968,3718968,7437936,10482.450543880463,0.0005621694854198722
466466,3726976,3726976,7453952,10503.938844919205,0.000562168141186703
467467,3734984,3734984,7469968,10525.445977210999,0.0005621667987725232
468468,3742990,3742990,7485980,10547.042939901352,0.0005621577292913571
469469,3750998,3750998,7501996,10568.452178001404,0.0005621563850581879
470470,3759004,3759004,7518008,10589.9208111763,0.0005621457275992725
471471,3767012,3767012,7534024,10611.417490959167,0.0005621443833661033
472472,3775020,3775020,7550040,10632.832554101944,0.0005621430409519235
473473,3783028,3783028,7566056,10654.363636016846,0.0005621416948997648
474474,3791032,3791032,7582064,10675.801774978638,0.0005621218224405311
475475,3799040,3799040,7598080,10697.082909107208,0.0005621204763883725
476476,3807048,3807048,7614096,10718.52734708786,0.0005621191339741927
477477,3815054,3815054,7630108,10739.901991128922,0.0005621008385787718
478478,3823062,3823062,7646124,10761.292985916138,0.0005620994943456026
479479,3831070,3831070,7662140,10782.89301109314,0.0005620981501124334
480480,3839076,3839076,7678152,10804.32765507698,0.0005620841984637082
481481,3847084,3847084,7694168,10825.937088012695,0.0005620828542305389
482482,3855092,3855092,7710184,10847.322094917297,0.0005620815099973697
483483,3863098,3863098,7726196,10868.60473394394,0.0005620576757792151
484484,3871104,3871104,7742208,10889.85111618042,0.0005620581723633222
485485,3879112,3879112,7758224,10911.066288948059,0.000562056828130153
486486,3887118,3887118,7774236,10932.757343053818,0.0005620480806101114
487487,3895126,3895126,7790252,10954.123821258545,0.0005620467345579527
488488,3903132,3903132,7806264,10975.496818065643,0.0005620437332254369
489489,3911140,3911140,7822280,10996.799674034119,0.0005620423908112571
490490,3919146,3919146,7838292,11018.171192884445,0.0005620392130367691
491491,3927152,3927152,7854304,11039.366791963577,0.0005618439117824892
492492,3935160,3935160,7870320,11061.052654266357,0.0005618425693683093
493493,3943168,3943168,7886336,11082.461766958237,0.0005618412269541295
494494,3951176,3951176,7902352,11103.80333185196,0.0005618398845399497
495495,3959182,3959182,7918364,11125.102840900421,0.0005617595907096984
496496,3967190,3967190,7934380,11146.527306079865,0.0005617582482955186
497497,3975196,3975196,7950392,11167.82062125206,0.0005617517672362737
498498,3983204,3983204,7966408,11189.111525058746,0.0005617504266410833
499499,3991212,3991212,7982424,11210.372292041779,0.0005617490842269035
500501,3999224,3999224,7998448,11231.841430187225,0.0005617329461529152
501502,4007232,4007232,8014464,11253.183224916458,0.0005617316037387354
502503,4015238,4015238,8030476,11274.4611389637,0.0005617260922008427
503504,4023246,4023246,8046492,11295.911082029343,0.0005617247497866629
504505,4031248,4031248,8062496,11317.11208987236,0.00056136358580261
505506,4039256,4039256,8078512,11338.40824007988,0.0005613622433884302
506507,4047264,4047264,8094528,11359.715872049332,0.0005613609009742504
507508,4055270,4055270,8110540,11381.094637155533,0.0005612913610093528
508509,4063276,4063276,8126552,11399.857031106949,0.0005612881195702357
509510,4071284,4071284,8142568,11422.287331104279,0.0005612867789750453
510511,4079290,4079290,8158580,11445.53048825264,0.0005612601053144317
511512,4087298,4087298,8174596,11468.127820253372,0.0005612587665382307
512513,4095306,4095306,8190612,11490.234763145447,0.0005612574259430403
513514,4103312,4103312,8206624,11511.510840177536,0.0005612462027784204
514515,4111320,4111320,8222640,11532.961646080017,0.0005612448640022194
515516,4119326,4119326,8238652,11554.434489011765,0.0005612417826341698
516517,4127334,4127334,8254668,11575.817409038544,0.0005612404420389794
517518,4135340,4135340,8270680,11597.093523979187,0.0005612219301838195
518519,4143348,4143348,8286696,11618.368176937103,0.0005612205877696397
519520,4151356,4151356,8302712,11639.781184196472,0.0005612192471744493
520521,4159362,4159362,8318724,11660.980385065079,0.0005611602537101135
521522,4167368,4167368,8334736,11682.427980184555,0.0005611601591226645
522523,4175376,4175376,8350752,11703.757355213165,0.0005611588167084847
523524,4183382,4183382,8366764,11725.047538995743,0.0005610773714579409
524525,4191390,4191390,8382780,11746.4162940979,0.0005610760290437611
525526,4199396,4199396,8398792,11767.747257947922,0.0005610741682176013
526527,4207404,4207404,8414808,11789.23582291603,0.0005610728312603896
527528,4215410,4215410,8430820,11810.639725208282,0.0005610107364191208
528529,4223416,4223416,8446832,11832.023885250092,0.0005610077969322447
529530,4231424,4231424,8462848,11853.264413118362,0.0005610064563370543
530531,4239430,4239430,8478860,11874.557282209396,0.0005609936251858016
531532,4247438,4247438,8494876,11895.838522911072,0.0005609922845906112
532533,4255446,4255446,8510892,11917.157343149185,0.0005609909458144102
533534,4263452,4263452,8526904,11938.521901130676,0.0005609831896435935
534535,4271460,4271460,8542920,11959.762629032135,0.0005609818508673925
535536,4279466,4279466,8558932,11981.096887111664,0.0005609771415038267
536537,4287474,4287474,8574948,12002.359333992004,0.0005609758009086363
537538,4295480,4295480,8590960,12023.681371927261,0.0005608401934296126
538539,4303488,4303488,8606976,12045.090053081512,0.0005608388546534115
539540,4311496,4311496,8622992,12066.4121260643,0.0005608375158772105
540541,4319502,4319502,8639004,12087.74651813507,0.0005607834118563915
541542,4327510,4327510,8655020,12109.199151039124,0.0005607820730801905
542543,4335518,4335518,8671036,12130.518923044205,0.000560780732485
543544,4343524,4343524,8687048,12151.864795923233,0.0005606239810731495
544545,4351532,4351532,8703064,12173.32005405426,0.0005606226441159379
545546,4359540,4359540,8719080,12194.651724100113,0.0005606213053397369
546547,4367548,4367548,8735096,12215.9110622406,0.0005606199665635359
547548,4375554,4375554,8751108,12237.210144042969,0.0005606141567113809
548549,4383562,4383562,8767124,12258.491587162018,0.0005606128197541693
549550,4391564,4391564,8783128,12279.764876127243,0.000560502587177325
550551,4399572,4399572,8799144,12301.197077035904,0.0005605012520391028
551552,4407576,4407576,8815152,12322.77767109871,0.0005603355857601855
552553,4415582,4415582,8831164,12344.07598900795,0.0005603323970717611
553554,4423588,4423588,8847176,12365.446748971939,0.0005603315257758368
554555,4431594,4431594,8863188,12386.632560968399,0.0005603237259492744
555556,4439602,4439602,8879204,12407.959826946259,0.0005603223871730734
556557,4447610,4447610,8895220,12429.299633026123,0.0005603210538538406
557558,4455616,4455616,8911232,12450.561123132706,0.0005603067202173406
558559,4463622,4463622,8927244,12471.873590230942,0.0005603043809969677
559560,4471630,4471630,8943260,12493.07649898529,0.0005603030440397561
560561,4479636,4479636,8959272,12514.45606303215,0.0005602896635537036
561562,4487642,4487642,8975284,12535.823823928833,0.0005602243272733176
562563,4495650,4495650,8991300,12557.088521003723,0.0005602229921350954
563564,4503658,4503658,9007316,12578.504533052444,0.0005602216569968732
564565,4511662,4511662,9023324,12599.887963056564,0.0005602073579211719
565566,4519670,4519670,9039340,12621.229504108429,0.0005602060227829497
566567,4527674,4527674,9055348,12642.468924045563,0.000560185140784597
567568,4535682,4535682,9071364,12663.802961111069,0.0005601838056463748
568569,4543688,4543688,9087376,12684.981273889542,0.0005601744069281267
569570,4551696,4551696,9103392,12706.424822092056,0.0005601730699709151
570571,4559702,4559702,9119404,12727.622583150864,0.0005600345721177291
571572,4567708,4567708,9135416,12749.000848054886,0.0005600328968284884
572573,4575714,4575714,9151428,12770.278100013733,0.000560030406631995
573574,4583720,4583720,9167440,12791.512635946274,0.0005600219319603639
574575,4591728,4591728,9183456,12813.001858234406,0.0005600205968221417
575576,4599736,4599736,9199472,12834.43815112114,0.0005600192616839195
576577,4607742,4607742,9215484,12855.695513248444,0.000559996122319717
577578,4615750,4615750,9231500,12877.161375045776,0.0005599947853625054
578579,4623756,4623756,9247512,12898.439366102219,0.0005599892429017927
579580,4631764,4631764,9263528,12919.802469968796,0.00055998790958256
580581,4639772,4639772,9279544,12941.164256095886,0.0005599865726253483
581582,4647778,4647778,9295556,12962.510823011398,0.0005599792875727871
582583,4655786,4655786,9311572,12983.738310098648,0.0005599779524345649
583584,4663792,4663792,9327584,13005.048226118088,0.0005599721462203888
584585,4671798,4671798,9343596,13026.253761053085,0.0005599674714176217
585586,4679806,4679806,9359612,13047.688110113144,0.0005599661362793995
586587,4687812,4687812,9375624,13069.068948030472,0.0005599290143436519
587588,4695818,4695818,9391636,13090.476264953613,0.0005599250034720171
588589,4703826,4703826,9407652,13111.884290218353,0.0005599236701527843
589590,4711832,4711832,9423664,13133.579442024231,0.0005599163068836788
590591,4719840,4719840,9439680,13154.823230028152,0.0005599149699264672
591592,4727846,4727846,9455692,13173.011266231537,0.0005597823437710758
592593,4735854,4735854,9471708,13195.591982841492,0.0005597810086328536
593594,4743862,4743862,9487724,13217.416893959045,0.0005597796734946314
594595,4751868,4751868,9503736,13238.957117080688,0.0005595965903921751
595596,4759876,4759876,9519752,13260.142861127853,0.0005595952570729423
596597,4767882,4767882,9535764,13281.372469186783,0.0005595932325377362
597598,4775890,4775890,9551780,13302.585571289062,0.0005595918992185034
598599,4783896,4783896,9567792,13323.627796173096,0.0005595660313701956
599600,4791904,4791904,9583808,13344.771263122559,0.0005595646998699522
600601,4799912,4799912,9599824,13365.790666103363,0.0005595633665507194
601602,4807916,4807916,9615832,13386.90235209465,0.0005595565053226892
602603,4815922,4815922,9631844,13407.945425987244,0.0005594964804913616
603604,4823928,4823928,9647856,13429.060635089874,0.0005594944395852508
604605,4831932,4831932,9663864,13450.309802055359,0.0005594316244241782
605606,4839940,4839940,9679880,13471.486496210098,0.0005594302911049454
606607,4847946,4847946,9695892,13492.533714056015,0.0005594078629655996
607608,4855952,4855952,9711904,13513.737240076065,0.0005594047051999951
608609,4863960,4863960,9727920,13534.873008012772,0.0005594033718807623
609610,4871968,4871968,9743936,13555.956153869629,0.0005594020403805189
610611,4879974,4879974,9759948,13576.794688224792,0.000559339521714719
611612,4887982,4887982,9775964,13597.364100933075,0.0005593381865764968
612613,4895990,4895990,9791980,13617.796627998352,0.0005593368568952428
613614,4903998,4903998,9807996,13639.44474196434,0.00055933552357601
614615,4912002,4912002,9824004,13660.816217899323,0.0005593205733021023
615616,4920008,4920008,9840016,13682.158870220184,0.0005593179866991704
616617,4928014,4928014,9856028,13703.021155834198,0.0005593026326096151
617618,4936022,4936022,9872044,13723.430058002472,0.0005593013011093717
618619,4944030,4944030,9888060,13744.030080080032,0.0005592999696091283
619620,4952036,4952036,9904072,13764.411366939545,0.0005592915767920204
620621,4960044,4960044,9920088,13784.818148851395,0.0005592902434727876
621622,4968050,4968050,9936100,13805.315579891205,0.0005592851503024576
622623,4976058,4976058,9952116,13825.75672006607,0.0005592838188022142
623624,4984064,4984064,9968128,13846.225525140762,0.0005592741217697039
624625,4992072,4992072,9984144,13866.7356569767,0.0005592727884504711
625626,5000078,5000078,10000156,13887.282598018646,0.0005592566685663769
626627,5008086,5008086,10016172,13907.662052869797,0.0005592553370661335
627628,5016092,5016092,10032184,13928.176677942276,0.0005591731678578071
628629,5024100,5024100,10048200,13948.77150797844,0.0005591718363575637
629630,5032108,5032108,10064216,13969.206111192703,0.0005591705048573203
630631,5040114,5040114,10080228,13989.659476041794,0.0005591633780568372
631632,5048122,5048122,10096244,14010.235561132431,0.0005591620483755833
632633,5056128,5056128,10112256,14030.874912023544,0.000559141280973563
633634,5064134,5064134,10128268,14051.417819023132,0.0005591419139818754
634635,5072138,5072138,10144276,14071.893651008606,0.0005591302870016079
635636,5080146,5080146,10160292,14092.565999031067,0.0005591289555013645
636637,5088152,5088152,10176304,14113.090158939362,0.0005591258868662408
637638,5096158,5096158,10192316,14133.746115207672,0.00055901591804286
638639,5104166,5104166,10208332,14154.371490240097,0.0005590145865426166
639640,5112174,5112174,10224348,14174.85908317566,0.0005590132568613626
640641,5120182,5120182,10240364,14195.509521961212,0.0005590119253611192
641642,5128188,5128188,10256376,14216.059953927994,0.0005589267384493724
642643,5136196,5136196,10272392,14236.624608039856,0.0005589254087681184
643644,5144204,5144204,10288408,14257.157771110535,0.0005589240790868644
644645,5152210,5152210,10304420,14277.805923938751,0.0005589169868471799
645646,5160218,5160218,10320436,14298.307552099228,0.000558915657165926
646647,5168224,5168224,10336448,14318.86450791359,0.0005589073480223306
647648,5176232,5176232,10352464,14339.547157049179,0.0005589060183410766
648649,5184238,5184238,10368476,14360.054161071777,0.000558821504455409
649650,5192246,5192246,10384492,14380.83562207222,0.0005588201729551656
650651,5200254,5200254,10400508,14401.305294275284,0.0005588188432739116
651652,5208260,5208260,10416520,14421.794394016266,0.0005588088934018742
652653,5216266,5216266,10432532,14442.285388231277,0.0005588071799138561
653654,5224274,5224274,10448548,14462.763463020325,0.0005588058520515915
654655,5232280,5232280,10464560,14483.345108032227,0.0005587576979451114
655656,5240284,5240284,10480568,14503.715146064758,0.0005587536106759217
656657,5248292,5248292,10496584,14524.064434051514,0.0005587522809946677
657658,5256296,5256296,10512592,14544.653272151947,0.0005587319483311148
658659,5264300,5264300,10528600,14564.991044998169,0.0005586818188021425
659660,5272306,5272306,10544612,14585.318509101868,0.0005586142233369173
660661,5280312,5280312,10560624,14605.822670221329,0.0005586097086052177
661662,5288320,5288320,10576640,14626.23633813858,0.0005586083789239638
662663,5296328,5296328,10592656,14646.641669988632,0.0005586070474237204
663664,5304334,5304334,10608668,14667.232101917267,0.0005584726241067983
664665,5312342,5312342,10624684,14687.86184501648,0.0005584712962445337
665666,5320350,5320350,10640700,14708.504195213318,0.0005584699665632797
666667,5328356,5328356,10656712,14729.133609056473,0.0005584644222835777
667668,5336364,5336364,10672728,14749.680835962296,0.0005584630944213131
668669,5344372,5344372,10688744,14770.18403506279,0.0005584617665590486
669670,5352378,5352378,10704756,14790.76926112175,0.0005584355712926481
670671,5360386,5360386,10720772,14811.249592065811,0.0005584342416113941
671672,5368394,5368394,10736788,14831.894275903702,0.0005584329137491295
672673,5376402,5376402,10752804,14852.387320280075,0.0005584315840678755
673674,5384408,5384408,10768816,14872.890808105469,0.0005584151549555827
674675,5392414,5392414,10784828,14893.598590135574,0.000558414480110514
675676,5400420,5400420,10800840,14914.273628950119,0.000558404653929756
676677,5408428,5408428,10816856,14934.915385961533,0.0005584033260674914
677678,5416434,5416434,10832868,14955.568056106567,0.0005583968541031936
678679,5424442,5424442,10848884,14976.215747117996,0.000558395526240929
679680,5432450,5432450,10864900,14996.843131065369,0.000558394196559675
680681,5440454,5440454,10880908,15017.506839036942,0.000558320931304479
681682,5448462,5448462,10896924,15038.153373003006,0.0005583196052612038
682683,5456470,5456470,10912940,15058.777483224869,0.0005583182737609604
683684,5464476,5464476,10928952,15079.273673057556,0.0005583068304986227
684685,5472484,5472484,10944968,15099.863915205002,0.0005583055026363581
685686,5480490,5480490,10960980,15120.416965007782,0.0005582861667789984
686687,5488498,5488498,10976996,15140.931945085526,0.0005582848389167339
687688,5496506,5496506,10993012,15161.523687124252,0.0005582835110544693
688689,5504512,5504512,11009024,15182.150949001312,0.0005582783851423301
689690,5512520,5512520,11025040,15203.324906110764,0.0005582770554610761
690691,5520526,5520526,11041052,15224.176483154297,0.0005582616231549764
691692,5528532,5528532,11057064,15245.336535215378,0.0005582597259490285
692693,5536538,5536538,11073076,15266.578313112259,0.0005582468911597971
693694,5544546,5544546,11089092,15287.189496278763,0.0005582455614785431
694695,5552552,5552552,11105104,15307.804573059082,0.0005582408157351892
695696,5560560,5560560,11121120,15328.451105117798,0.0005582394878729247
696697,5568564,5568564,11137128,15349.272562980652,0.0005578256241278723
697698,5576568,5576568,11153136,15369.96224117279,0.0005578205546044046
698699,5584574,5584574,11169148,15390.697673082352,0.0005578172040259233
699700,5592580,5592580,11185160,15411.396875143051,0.0005577977262873901
700701,5600588,5600588,11201176,15431.837321043015,0.0005577964002441149
701702,5608596,5608596,11217192,15452.208405017853,0.0005577950760198291
702703,5616604,5616604,11233208,15472.64096403122,0.0005577937481575646
703704,5624608,5624608,11249216,15493.12213730812,0.0005577486099355156
704705,5632616,5632616,11265232,15511.89135813713,0.0005577472838922404
705706,5640624,5640624,11281248,15527.664354085922,0.0005577459578489652
706707,5648630,5648630,11297260,15550.043952941895,0.0005577311821980402
707708,5656636,5656636,11313272,15572.780029058456,0.0005577282699960051
708709,5664644,5664644,11329288,15594.524927139282,0.0005577269457717193
709710,5672650,5672650,11345300,15615.79426407814,0.0005577057290793164
710711,5680658,5680658,11361316,15637.141057014465,0.0005577044030360412
711712,5688666,5688666,11377332,15658.492670059204,0.000557703076992766
712713,5696672,5696672,11393344,15679.889575004578,0.0005576617350016022
713714,5704680,5704680,11409360,15701.207649230957,0.0005576604107773164
714715,5712688,5712688,11425376,15722.677951097488,0.0005576590829150518
715716,5720694,5720694,11441388,15743.926876068115,0.0005576571893470827
716717,5728698,5728698,11457396,15765.298175096512,0.0005576087023655418
717718,5736706,5736706,11473412,15786.687290906906,0.0005576073799602455
718719,5744712,5744712,11489424,15808.077404022217,0.0005575991799560143
719720,5752720,5752720,11505440,15829.378722190857,0.0005575978557317285
720721,5760728,5760728,11521456,15850.593445062637,0.0005575965296884533
721722,5768732,5768732,11537464,15871.956283092499,0.0005575611903623212
722723,5776740,5776740,11553480,15893.237607002258,0.0005575598661380354
723724,5784746,5784746,11569492,15914.652022123337,0.0005575544346356764
724725,5792754,5792754,11585508,15936.113762140274,0.0005575531085924013
725726,5800760,5800760,11601520,15957.457408189774,0.0005575445993599715
726727,5808764,5808764,11617528,15978.636646986008,0.0005573916387220379
727728,5816772,5816772,11633544,15999.818164110184,0.0005573903163167415
728729,5824778,5824778,11649556,16021.066152095795,0.0005573890739469789
729730,5832786,5832786,11665572,16042.289735078812,0.0005573877497226931
730731,5840792,5840792,11681584,16063.770280122757,0.0005573384805757087
731732,5848800,5848800,11697600,16085.058717012405,0.0005573371581704123
732733,5856808,5856808,11713616,16106.349082946777,0.0005573358357651159
733734,5864814,5864814,11729628,16127.455997943878,0.0005573336766246939
734735,5872822,5872822,11745644,16148.704091072083,0.0005573323542193975
735736,5880826,5880826,11761652,16170.038275957108,0.0005573084545176243
736737,5888832,5888832,11777664,16191.165157079697,0.0005572927602770505
737738,5896840,5896840,11793680,16212.343975067139,0.0005572914378717542
738739,5904846,5904846,11809692,16233.725379228592,0.0005572555764956633
739740,5912854,5912854,11825708,16255.15961098671,0.0005572542522713775
740741,5920862,5920862,11841724,16276.287459850311,0.0005572529298660811
741742,5928870,5928870,11857740,16297.542417049408,0.0005572516056417953
742743,5936876,5936876,11873752,16318.75981593132,0.0005572379050136078
743744,5944884,5944884,11889768,16340.08085513115,0.000557236580789322
744745,5952892,5952892,11905784,16361.291890144348,0.0005572352583840257
745746,5960898,5960898,11921796,16382.568854093552,0.0005572181544266641
746747,5968906,5968906,11937812,16403.775913000107,0.0005572168320213677
747748,5976912,5976912,11953824,16424.897862911224,0.0005572154950641561
748749,5984918,5984918,11969836,16446.240364074707,0.0005571862511715153
749750,5992924,5992924,11985848,16467.395046949387,0.0005571833698923001
750751,6000932,6000932,12001864,16488.619663000107,0.0005571820474870037
751752,6008938,6008938,12017876,16509.92524600029,0.0005571706515183905
752753,6016946,6016946,12033892,16531.159344911575,0.0005571693254751153
753754,6024952,6024952,12049904,16552.459181070328,0.0005571658857661532
754755,6032958,6032958,12065916,16573.733319997787,0.0005570422745222459
755756,6040966,6040966,12081932,16594.933836221695,0.0005570409502979601
756757,6048974,6048974,12097948,16616.139981269836,0.0005570396278926637
757758,6056980,6056980,12113960,16637.46855211258,0.0005570201556110987
758759,6064988,6064988,12129976,16658.69846200943,0.0005570188332058024
759760,6072996,6072996,12145992,16679.93086218834,0.000557017510800506
760761,6081002,6081002,12162004,16701.43485403061,0.0005570089451794047
761762,6089010,6089010,12178020,16722.71132016182,0.0005570076209551189
762763,6097014,6097014,12194028,16743.90589904785,0.0005569740860664751
763764,6105022,6105022,12210044,16765.21029806137,0.0005569727618421894
764765,6113028,6113028,12226056,16786.42991709709,0.0005569682853092672
765766,6121034,6121034,12242068,16807.58034014702,0.0005569373661273858
766767,6129042,6129042,12258084,16828.621850013733,0.0005569360419031
767768,6137050,6137050,12274100,16849.77022600174,0.000556934721316793
768769,6145056,6145056,12290112,16870.798574209213,0.0005569290024141083
769770,6153064,6153064,12306128,16891.997928142548,0.0005569276818278013
770771,6161068,6161068,12322136,16913.086729049683,0.0005568466822296614
771772,6169076,6169076,12338152,16934.137411117554,0.000556845359824365
772773,6177080,6177080,12354160,16955.14033317566,0.0005568313245021272
773774,6185088,6185088,12370176,16976.122009277344,0.0005568300039158203
774775,6193096,6193096,12386192,16997.18113708496,0.0005568286815105239
775776,6201102,6201102,12402204,17018.283600091934,0.0005568140695686452
776777,6209108,6209108,12418216,17039.35489320755,0.0005568102333199931
777778,6217114,6217114,12434228,17060.447122097015,0.0005567687476286665
778779,6225122,6225122,12450244,17081.631301879883,0.0005567674270423595
779780,6233130,6233130,12466260,17102.780472278595,0.0005567661046370631
780781,6241136,6241136,12482272,17124.123250961304,0.0005567638218053617
781782,6249142,6249142,12498284,17145.56823825836,0.0005567505922954297
782783,6257150,6257150,12514300,17167.23612189293,0.0005567492717091227
783784,6265156,6265156,12530312,17188.942546129227,0.0005567328316828934
784785,6273164,6273164,12546328,17210.36348605156,0.0005567315110965865
785786,6281172,6281172,12562344,17231.495561122894,0.0005567301905102795
786787,6289178,6289178,12578356,17253.454246997833,0.0005561807029152988
787788,6297186,6297186,12594372,17274.824746131897,0.0005561793841479812
788789,6305192,6305192,12610384,17290.9161632061,0.000556177972612204
789790,6313200,6313200,12626400,17306.368052005768,0.0005561766538448865
790791,6321206,6321206,12642412,17318.491291999817,0.0005561460966418963
791792,6329214,6329214,12658428,17330.762777090073,0.0005561447778745787
792793,6337222,6337222,12674444,17343.15977191925,0.0005561434591072612
793794,6345230,6345230,12690460,17355.70130109787,0.000556142142158933
794795,6353234,6353234,12706468,17368.33209991455,0.0005561310281336773
795796,6361240,6361240,12722480,17380.62472987175,0.0005561279504036065
796797,6369248,6369248,12738496,17393.144222974777,0.0005561266334552784
797798,6377252,6377252,12754504,17405.18899011612,0.0005560983281611698
798799,6385260,6385260,12770520,17417.147152900696,0.0005560970093938522
799800,6393266,6393266,12786532,17428.829843997955,0.0005560855588555569
800801,6401274,6401274,12802548,17441.312152147293,0.0005560842419072287
801802,6409280,6409280,12818560,17453.578601121902,0.0005560763347602915
802803,6417288,6417288,12834576,17465.342890024185,0.0005560750159929739
803804,6425294,6425294,12850588,17477.726615190506,0.000556052555111819
804805,6433302,6433302,12866604,17489.924482107162,0.000556051234525512
805806,6441310,6441310,12882620,17502.24098587036,0.0005560499175771838
806807,6449316,6449316,12898632,17514.779225111008,0.0005560442805290222
807808,6457322,6457322,12914644,17526.567630290985,0.0005560371300816769
808809,6465330,6465330,12930660,17538.632921934128,0.0005560358131333487
809810,6473336,6473336,12946672,17550.340750217438,0.000555938573597814
810811,6481344,6481344,12962688,17562.344917058945,0.0005559372566494858
811812,6489350,6489350,12978700,17574.39560198784,0.0005559363526117522
812813,6497356,6497356,12994712,17586.093092918396,0.0005557765234698309
813814,6505362,6505362,13010724,17598.385416030884,0.0005557716503972188
814815,6513370,6513370,13026740,17609.8071539402,0.0005557703334488906
815816,6521376,6521376,13042752,17621.254554986954,0.0005557541226153262
816817,6529384,6529384,13058768,17632.540198087692,0.000555752805666998
817818,6537390,6537390,13074780,17643.992000102997,0.0005556050327868434
818819,6545396,6545396,13090792,17655.514099121094,0.0005556014821195276
819820,6553404,6553404,13106808,17666.969194173813,0.0005556001651711995
820821,6561410,6561410,13122820,17678.336776018143,0.000555593122044229
821822,6569418,6569418,13138836,17689.607117176056,0.0005555918050959008
822823,6577426,6577426,13154852,17701.429347276688,0.0005555904881475726
823824,6585432,6585432,13170864,17713.054222106934,0.0005555648021982051
824825,6593440,6593440,13186880,17725.06784105301,0.0005555634870688664
825826,6601446,6601446,13202892,17736.464740037918,0.0005555573989113327
826827,6609454,6609454,13218908,17748.00027823448,0.000555556083781994
827828,6617460,6617460,13234920,17759.435483932495,0.0005555396892304998
828829,6625468,6625468,13250936,17771.095196962357,0.0005555383722821716
829830,6633476,6633476,13266952,17782.587115049362,0.0005555370553338435
830831,6641482,6641482,13282964,17794.024673223495,0.0005555306852329522
831832,6649488,6649488,13298976,17805.554134130478,0.0005555217921937583
832833,6657496,6657496,13314992,17817.061470985413,0.0005555204752454301
833834,6665504,6665504,13331008,17828.58925819397,0.000555519158297102
834835,6673510,6673510,13347020,17840.115514993668,0.0005554956514970399
835836,6681518,6681518,13363036,17851.65559196472,0.0005554943345487118
836837,6689524,6689524,13379048,17863.33158302307,0.0005554920189752011
837838,6697532,6697532,13395064,17874.597514152527,0.0005554907020268729
838839,6705538,6705538,13411076,17886.416830062866,0.0005554700674110791
839840,6713546,6713546,13427092,17897.85351204872,0.0005554687504627509
840841,6721554,6721554,13443108,17909.290267944336,0.0005554674335144227
841842,6729558,6729558,13459116,17920.69682407379,0.0005554519684665138
842843,6737564,6737564,13475128,17932.125281095505,0.0005554420768021373
843844,6745570,6745570,13491140,17943.651118278503,0.0005553559785766993
844845,6753578,6753578,13507156,17955.478218078613,0.0005553546634473605
845846,6761586,6761586,13523172,17967.187999010086,0.0005553533464990323
846847,6769592,6769592,13539184,17978.539119005203,0.0005553509272431256
847848,6777600,6777600,13555200,17990.023260116577,0.0005553496102947975
848849,6785606,6785606,13571212,18001.578545093536,0.0005553253831749316
849850,6793614,6793614,13587228,18013.472353219986,0.0005553240698645823
850851,6801620,6801620,13603240,18025.187457084656,0.000555319398699794
851852,6809628,6809628,13619256,18037.04953813553,0.0005553180835704552
852853,6817634,6817634,13635268,18048.33174109459,0.0005552991678996477
853854,6825640,6825640,13651280,18059.73415827751,0.0005552950460696593
854855,6833648,6833648,13667296,18071.140693187714,0.0005552937309403205
855856,6841654,6841654,13683308,18082.99304819107,0.0005552833590627415
856857,6849662,6849662,13699324,18094.428932905197,0.0005552820439334027
857858,6857668,6857668,13715336,18105.906336069107,0.0005552659131353721
858859,6865676,6865676,13731352,18117.280122995377,0.0005552645998250227
859860,6873682,6873682,13747364,18128.769176244736,0.0005552626680582762
860861,6881688,6881688,13763376,18140.468168973923,0.0005552427519432968
861862,6889696,6889696,13779392,18152.27138018608,0.0005552414349949686
862863,6897702,6897702,13795404,18163.676030158997,0.0005552359471039381
863864,6905708,6905708,13811416,18175.03445315361,0.0005551565245696111
864865,6913716,6913716,13827432,18186.648525238037,0.0005551552112592617
865866,6921724,6921724,13843448,18198.22676205635,0.0005551538943109335
866867,6929732,6929732,13859464,18209.710942983627,0.0005551525810005842
867868,6937738,6937738,13875476,18221.229598999023,0.000555140297365142
868869,6945746,6945746,13891492,18232.629016160965,0.0005551389840547927
869870,6953754,6953754,13907508,18244.076596021652,0.0005551376707444433
870871,6961760,6961760,13923520,18255.743447065353,0.0005551226931856945
871872,6969768,6969768,13939536,18267.255923986435,0.0005551213798753452
872873,6977774,6977774,13955548,18278.814776182175,0.0005551132180698914
873874,6985782,6985782,13971564,18290.1755259037,0.0005551119047595421
874875,6993790,6993790,13987580,18301.550868988037,0.0005551105896302033
875876,7001796,7001796,14003592,18312.949996232986,0.0005550840014620917
876877,7009802,7009802,14019604,18324.33189892769,0.0005550821497308789
877878,7017810,7017810,14035620,18335.667320251465,0.0005550808346015401
878879,7025816,7025816,14051632,18347.15996813774,0.0005550562673306558
879880,7033824,7033824,14067648,18358.580141067505,0.0005550549522013171
880881,7041832,7041832,14083664,18369.973778009415,0.0005550536388909677
881882,7049838,7049838,14099676,18381.732229948044,0.0005550494042836362
882883,7057844,7057844,14115688,18393.154477119446,0.0005550029454752803
883884,7065850,7065850,14131700,18404.79231595993,0.0005550056503125234
884885,7073858,7073858,14147716,18416.112869024277,0.000555004337002174
885886,7081864,7081864,14163728,18427.44180417061,0.0005549893285206053
886887,7089872,7089872,14179744,18438.81906914711,0.0005549880133912666
887888,7097880,7097880,14195760,18450.1294028759,0.0005549867000809172
888889,7105886,7105886,14211772,18461.550096035004,0.0005549699926632456
889890,7113894,7113894,14227788,18472.976634025574,0.0005549686793528963
890891,7121898,7121898,14243796,18484.480657100677,0.0005549055749725085
891892,7129904,7129904,14259808,18496.272314071655,0.0005549030047404813
892893,7137910,7137910,14275820,18507.750138044357,0.0005548914341488853
893894,7145918,7145918,14291836,18519.427008152008,0.000554890120838536
894895,7153924,7153924,14307848,18530.766279935837,0.0005548842909774976
895896,7161932,7161932,14323864,18542.175452947617,0.0005548829776671482
896897,7169940,7169940,14339880,18553.7858440876,0.0005548816643567989
897898,7177944,7177944,14355888,18565.322286128998,0.0005548598692257656
898899,7185952,7185952,14371904,18576.96498799324,0.0005548585559154162
899900,7193958,7193958,14387916,18588.30326604843,0.0005548564386117505
900901,7201964,7201964,14403928,18599.721262931824,0.0005547118980757659
901902,7209972,7209972,14419944,18611.198255062103,0.0005547105847654166
902903,7217978,7217978,14435956,18622.538051843643,0.0005546697193494765
903904,7225986,7225986,14451972,18634.13712000847,0.0005546684060391271
904905,7233994,7233994,14467988,18646.05605697632,0.0005546670945477672
905906,7242000,7242000,14484000,18657.641555070877,0.0005546411630348302
906907,7250008,7250008,14500016,18669.035091161728,0.0005546398515434703
907908,7258016,7258016,14516032,18680.448533058167,0.0005546385382331209
908909,7266022,7266022,14532044,18691.748095035553,0.0005546292431972688
909910,7274030,7274030,14548060,18703.10394001007,0.0005546279317059088
910911,7282036,7282036,14564072,18714.562381267548,0.0005546231150219683
911912,7290044,7290044,14580088,18726.00936102867,0.0005546218035306083
912913,7298050,7298050,14596100,18737.408664226532,0.0005544441937672673
913914,7306058,7306058,14612116,18748.710274219513,0.0005544428822759073
914915,7314066,7314066,14628132,18760.027292966843,0.0005544415707845474
915916,7322072,7322072,14644144,18771.66737794876,0.0005544312261918094
916917,7330080,7330080,14660160,18783.23081088066,0.00055442991288146
917918,7338086,7338086,14676172,18794.79917407036,0.0005544277337321546
918919,7346094,7346094,14692188,18806.101351976395,0.000554426424059784
919920,7354100,7354100,14708200,18817.567160844803,0.0005544114756048657
920921,7362108,7362108,14724216,18829.009583950043,0.0005544101622945163
921922,7370112,7370112,14740224,18840.58359003067,0.0005542009512282675
922923,7378120,7378120,14756240,18852.132174253464,0.0005541996397369076
923924,7386128,7386128,14772256,18863.53776907921,0.000554198330064537
924925,7394134,7394134,14788268,18875.2746591568,0.0005541949249163736
925926,7402140,7402140,14804280,18886.684490203857,0.0005541668160731206
926927,7410148,7410148,14820296,18897.9823949337,0.0005541655045817606
927928,7418156,7418156,14836312,18909.381816148758,0.0005541641949093901
928929,7426162,7426162,14852324,18920.80085515976,0.0005541529371839715
929930,7434170,7434170,14868340,18932.307261943817,0.0005541516238736222
930931,7442176,7442176,14884352,18944.218766212463,0.0005541435748455115
931932,7450184,7450184,14900368,18956.120840072632,0.0005541422633541515
932933,7458190,7458190,14916380,18968.17236804962,0.0005541366499528522
933934,7466198,7466198,14932396,18980.121285915375,0.0005541353402804816
934935,7474206,7474206,14948412,18992.179656982422,0.0005541340306081111
935936,7482212,7482212,14964424,19004.26588511467,0.0005541155442188028
936937,7490220,7490220,14980440,19015.74630999565,0.0005541142327274429
937938,7498222,7498222,14996444,19027.233483076096,0.0005540417332667857
938939,7506230,7506230,15012460,19039.002902030945,0.0005540404254134046
939940,7514238,7514238,15028476,19050.441384077072,0.0005540391175600234
940941,7522246,7522246,15044492,19062.097890138626,0.0005540378060686635
941942,7530252,7530252,15060504,19074.526039123535,0.0005540302208828507
942943,7538258,7538258,15076516,19086.71080994606,0.0005540284637390869
943944,7546264,7546264,15092528,19098.62997317314,0.0005539775502256816
944945,7554272,7554272,15108544,19111.162976026535,0.0005539762423723005
945946,7562280,7562280,15124560,19123.267846107483,0.0005539749308809405
946947,7570286,7570286,15140572,19135.241762161255,0.0005539562553167343
947948,7578292,7578292,15156584,19147.80711889267,0.0005539556113944855
948949,7586298,7586298,15172596,19159.17620897293,0.0005538589575735386
949950,7594306,7594306,15188612,19170.257687091827,0.0005538576479011681
950951,7602314,7602314,15204628,19181.135100126266,0.0005538563364098081
951952,7610320,7610320,15220640,19191.881246089935,0.0005538536479434697
952953,7618326,7618326,15236652,19202.487357139587,0.00055383562357747
953954,7626334,7626334,15252668,19213.242748975754,0.00055383431208611
954955,7634342,7634342,15268684,19224.154766082764,0.0005538330042327289
955956,7642348,7642348,15284696,19235.64248895645,0.0005538253080885625
956957,7650356,7650356,15300712,19247.65472793579,0.0005538240002351813
957958,7658364,7658364,15316728,19259.135328054428,0.0005538226887438213
958959,7666366,7666366,15332732,19271.047002077103,0.0005537589586310787
959960,7674374,7674374,15348748,19282.187783002853,0.0005537576489587082
960961,7682382,7682382,15364764,19293.46390414238,0.000553756341105327
961962,7690388,7690388,15380776,19304.471920967102,0.0005537532833841396
962963,7698394,7698394,15396788,19315.768384218216,0.000553739821043564
963964,7706402,7706402,15412804,19326.971466064453,0.0005537385150091723
964965,7714410,7714410,15428820,19337.802368164062,0.0005537372035178123
965966,7722416,7722416,15444832,19348.767367124557,0.0005537278066185536
966967,7730424,7730424,15460848,19359.7031519413,0.000553726496946183
967968,7738430,7738430,15476860,19370.833254098892,0.0005535030431929044
968969,7746438,7746438,15492876,19381.881833076477,0.0005535017371585127
969970,7754446,7754446,15508892,19392.897832155228,0.0005535004293051315
970971,7762450,7762450,15524900,19403.873665094376,0.0005534965166589245
971972,7770458,7770458,15540916,19414.557794094086,0.0005534952088055434
972973,7778464,7778464,15556928,19425.282449007034,0.0005534352349059191
973974,7786470,7786470,15572940,19435.834894180298,0.0005534363826882327
974975,7794478,7794478,15588956,19446.47182917595,0.0005534350748348515
975976,7802486,7802486,15604972,19457.105219125748,0.0005534337669814704
976977,7810492,7810492,15620984,19467.71969103813,0.000553239964574459
977978,7818498,7818498,15636996,19478.3276822567,0.0005532365321414545
978979,7826506,7826506,15653012,19489.123991250992,0.0005532352261070628
979980,7834514,7834514,15669028,19499.799411058426,0.0005532339182536816
980981,7842520,7842520,15685040,19510.621809005737,0.0005532312861760147
981982,7850528,7850528,15701056,19521.590136051178,0.0005532299801416229
982983,7858534,7858534,15717068,19532.174680233,0.0005532146587938769
983984,7866542,7866542,15733084,19543.643908023834,0.0005532133527594851
984985,7874550,7874550,15749100,19554.463207006454,0.000553212044906104
985986,7882556,7882556,15765112,19565.257491111755,0.0005531844963115873
986987,7890564,7890564,15781128,19576.205094099045,0.0005531831902771955
987988,7898572,7898572,15797144,19587.152179002762,0.0005531818842428038
988989,7906578,7906578,15813156,19598.38582611084,0.000553135818336159
989990,7914586,7914586,15829172,19609.08522415161,0.0005531345123017672
990991,7922592,7922592,15845184,19619.979506969452,0.0005531311562663177
991992,7930600,7930600,15861200,19631.12739419937,0.000553129850231926
992993,7938606,7938606,15877212,19641.927596092224,0.0005531251881620847
993994,7946612,7946612,15893224,19653.068011045456,0.0005531082206289284
994995,7954620,7954620,15909240,19663.896962165833,0.000553106916413526
995996,7962628,7962628,15925256,19675.12880706787,0.0005531056085601449
996997,7970634,7970634,15941268,19686.151942014694,0.0005531026472453959
997998,7978640,7978640,15957280,19697.09569501877,0.00055309757226496
998999,7986646,7986646,15973292,19707.815543174744,0.0005530855705728754
1000000,7994654,7994654,15989308,19718.463359117508,0.0005530842627194943


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.03370094299316406,12064.709122577777
1001,3744,3744,7488,24.570235013961792,0.1510504415291507
2002,7736,7736,15472,49.48080587387085,0.013294467175001046
3003,11916,11916,23832,75.53520393371582,0.004405298595884233
4004,15908,15908,31816,101.01627397537231,0.0007309857865038794
5005,20050,20050,40100,126.56784105300903,0.0005847362608619733
6006,24640,24640,49280,154.9280309677124,0.000517089221830247
7007,29176,29176,58352,182.63866996765137,0.0005145269660715712
8008,33434,33434,66868,208.81292486190796,0.000395150447729975
9009,38974,38974,77948,241.5090959072113,0.0003945950302295387
10010,46578,46578,93156,284.647038936615,0.00039447286690119654
11011,53052,53052,106104,322.9363238811493,0.000389044846087927
12012,59502,59502,119004,362.36348605155945,0.000388112119253492
13013,64786,64786,129572,395.8347849845886,0.0003517358400131343
14014,70386,70386,140772,429.0076129436493,0.00035001113792532124
15015,78042,78042,156084,472.1558930873871,0.0003497763882478466
16016,85172,85172,170344,511.93689489364624,0.00034545769267424475
17017,91700,91700,183400,547.4451830387115,0.00034386813240416814
18018,99454,99454,198908,588.505609035492,0.00034371587753412314
19019,107258,107258,214516,631.1718430519104,0.0003436467195570003
20020,114154,114154,228308,670.3175601959229,0.00033932807309611235
21021,121984,121984,243968,712.5952031612396,0.00033928822267625947
22022,129354,129354,258708,751.2601149082184,0.00033439869548601564
23023,134600,134600,269200,781.5855128765106,0.0003256054205849068
24024,142500,142500,285000,824.2899069786072,0.0003255189149058424
25025,150388,150388,300776,865.334371805191,0.00032547817136219237
26026,157174,157174,314348,902.3457779884338,0.0003108118053205544
27027,164622,164622,329244,942.4063968658447,0.00031069875512912404
28028,172290,172290,344580,982.5411729812622,0.0003105367886746535
29029,177950,177950,355900,1016.2306320667267,0.00023654973847442307
30030,183888,183888,367776,1051.3777160644531,0.00023641393272555433
31031,191862,191862,383724,1093.8815088272095,0.0002364025785936974
32032,199852,199852,399704,1132.814083814621,0.00023639086430193856
33033,207844,207844,415688,1170.989816904068,0.00023638605125597678
34034,215842,215842,431684,1209.6943891048431,0.00023638254060642794
35035,223298,223298,446596,1246.281741142273,0.0002329058279428864
36036,231164,231164,462328,1285.2384457588196,0.0002328642876818776
37037,239160,239160,478320,1327.4551508426666,0.0002328611990378704
38038,247158,247158,494316,1372.9769008159637,0.00023285733186639845
39039,255144,255144,510288,1416.3611640930176,0.00023283911286853254
40040,263146,263146,526292,1458.8248829841614,0.00023283669361262582
41041,271146,271146,542292,1505.4257040023804,0.00023283476912183687
42042,279144,279144,558288,1548.9402058124542,0.00023283105838345364
43043,287142,287142,574284,1589.1929709911346,0.00023282845540961716
44044,295134,295134,590268,1625.5218119621277,0.00023282286019821186
45045,303130,303130,606260,1658.487459897995,0.0002328199643670814
46046,310462,310462,620924,1687.56454205513,0.0002294297555636149
47047,318432,318432,636864,1720.8271689414978,0.00022942101350054145
48048,326424,326424,652848,1755.4392981529236,0.00022941479801374953
49049,334424,334424,668848,1793.0070128440857,0.0002294119585712906
50050,342420,342420,684840,1827.5726201534271,0.00022940793678571936
51051,350410,350410,700820,1862.482922077179,0.00022940135204407852
52052,358406,358406,716812,1899.3222908973694,0.00022939711197977886
53053,366404,366404,732808,1934.7543618679047,0.0002293895886396058
54054,374400,374400,748800,1966.746001958847,0.00022938516303838696
55055,382392,382392,764784,2003.0047628879547,0.00022938034453545697
56056,390392,390392,780784,2042.3198509216309,0.00022937747780815698
57057,398390,398390,796780,2083.792552947998,0.00022937446738069411
58058,406186,406186,812372,2116.5271739959717,0.00022752280528948177
59059,413654,413654,827308,2148.911017894745,0.00022740377426089253
60060,421608,421608,843216,2184.2568259239197,0.0002273705122206593
61061,429594,429594,859188,2222.064164876938,0.00022736206483386923
62062,437580,437580,875160,2257.978492975235,0.00022735560742148664
63063,445578,445578,891156,2294.018215894699,0.00022735144193575252
64064,453568,453568,907136,2339.6987159252167,0.0002273464106110623
65065,461568,461568,923136,2380.095151901245,0.00022734387493983377
66066,469554,469554,939108,2420.5389120578766,0.00022732974139216822
67067,477548,477548,955096,2455.735311985016,0.00022732636716682464
68068,485540,485540,971080,2489.6733119487762,0.0002273211630381411
69069,493536,493536,987072,2519.494947910309,0.0002273172194691142
70070,501538,501538,1003076,2544.7791318893433,0.00022731373792339582
71071,509534,509534,1019068,2570.4060339927673,0.00022731130047759507
72072,517496,517496,1034992,2595.2097527980804,0.00022700486442772672
73073,525478,525478,1050956,2620.546282052994,0.00022699927831126843
74074,533374,533374,1066748,2645.2544469833374,0.00022683046699967235
75075,541356,541356,1082712,2671.7022149562836,0.00022682297276332974
76076,549346,549346,1098692,2697.5187599658966,0.00022681942027702462
77077,557338,557338,1114676,2722.9032320976257,0.00022681451628159266
78078,565336,565336,1130672,2751.0731978416443,0.000226808126171818
79079,573332,573332,1146664,2776.5863728523254,0.00022680457004753407
80080,581316,581316,1162632,2801.134136915207,0.00022679908761347178
81081,589120,589120,1178240,2825.9595239162445,0.00022651914332527667
82082,597108,597108,1194216,2851.0717639923096,0.00022651173640042543
83083,605034,605034,1210068,2877.315779209137,0.00022641810755885672
84084,613020,613020,1226040,2904.294902086258,0.0002264099439344136
85085,621014,621014,1242028,2930.4323511123657,0.0002264047652715817
86086,628992,628992,1257984,2955.569155931473,0.00022637344591203146
87087,636982,636982,1273964,2983.0813360214233,0.0002263388978462899
88088,644982,644982,1289964,3009.477791070938,0.00022633708613284398
89089,652980,652980,1305960,3035.3698630332947,0.00022633497428614646
90090,659988,659988,1319976,3061.910552740097,0.00021260894754959736
91091,666550,666550,1333100,3082.974928855896,0.00021252491205814295
92092,674422,674422,1348844,3106.5318768024445,0.00021248089979053475
93093,682414,682414,1364828,3132.529401779175,0.00021247828954074066
94094,690406,690406,1380812,3156.875715970993,0.00021247541735647246
95095,698382,698382,1396764,3180.883882045746,0.00021246663345664274
96096,706380,706380,1412760,3203.3221859931946,0.0002124616366927512
97097,714222,714222,1428444,3225.229383945465,0.00021225445561867673
98098,722198,722198,1444396,3247.148458003998,0.000212247727176873
99099,730180,730180,1460360,3268.9125208854675,0.0002122202695318265
100100,738176,738176,1476352,3291.2116339206696,0.00021221728457021527
101101,746172,746172,1492344,3314.845472097397,0.000212212631595321
102102,754168,754168,1508336,3339.2325451374054,0.00021220853705017362
103103,762162,762162,1524324,3361.511691093445,0.000212204729905352
104104,770160,770160,1540320,3383.2873480319977,0.00021220034250291064
105105,778158,778158,1556316,3405.085837125778,0.00021219773225311656
106106,786148,786148,1572296,3427.2405047416687,0.00021219387235760223
107107,794144,794144,1588288,3449.23069190979,0.00021218976144155022
108108,802142,802142,1604284,3470.649158000946,0.00021218616348051
109109,810146,810146,1620292,3492.6417520046234,0.0002121838078892324
110110,818132,818132,1636264,3516.1608798503876,0.00021214416301518213
111111,826124,826124,1652248,3535.0470700263977,0.00021213692889432423
112112,834118,834118,1668236,3546.9941897392273,0.00021213425679889042
113113,842114,842114,1684228,3558.896024942398,0.0002121300985891139
114114,850118,850118,1700236,3570.377990961075,0.00021212718456808943
115115,858114,858114,1716228,3581.8843977451324,0.00021212387036939617
116116,866110,866110,1732220,3593.4034729003906,0.00021211938110354822
117117,874108,874108,1748216,3604.8283970355988,0.00021211616694927216
118118,882098,882098,1764196,3616.2749099731445,0.0002121120851370506
119119,887784,887784,1775568,3625.1378738880157,0.00012878716916020494
120120,895692,895692,1791384,3636.7137200832367,0.00012876090477220714
121121,903646,903646,1807292,3648.867218017578,0.00012873057676188182
122122,911632,911632,1823264,3660.2262370586395,0.00012872759907622822
123123,919622,919622,1839244,3671.6866149902344,0.00012872150909970514
124124,927616,927616,1855232,3685.695802927017,0.00012871750732301734
125125,935616,935616,1871232,3700.687515974045,0.0001287147151742829
126126,943616,943616,1887232,3717.2433109283447,0.00012871183207607828
127127,951614,951614,1903228,3733.0330379009247,0.00012870947102783248
128128,959616,959616,1919232,3747.420691013336,0.0001287082504859427
129129,967618,967618,1935236,3762.912610054016,0.0001287063532799948
130130,975618,975618,1951236,3781.1386399269104,0.00012870479076809715
131131,983618,983618,1967236,3795.9526600837708,0.0001287015365960542
132132,991620,991620,1983240,3810.3910558223724,0.00012869987767771818
133133,999622,999622,1999244,3823.1089940071106,0.0001286979913857067
134134,1007620,1007620,2015240,3834.569680929184,0.00012869426973338705
135135,1015622,1015622,2031244,3846.331226825714,0.00012869211423094384
136136,1023620,1023620,2047240,3857.901059150696,0.00012868945304944646
137137,1031616,1031616,2063232,3869.54248714447,0.00012868628618889488
138138,1039616,1039616,2079232,3880.936819076538,0.00012868367048213258
139139,1047618,1047618,2095236,3892.4136798381805,0.00012868180419900455
140140,1055608,1055608,2111216,3903.828374147415,0.0001286555616388796
141141,1063610,1063610,2127220,3915.238378047943,0.00012865052667621057
142142,1071612,1071612,2143224,3926.7469000816345,0.00012864957716374192
143143,1079614,1079614,2159228,3938.0702180862427,0.00012864775453635957
144144,1087614,1087614,2175228,3949.3470029830933,0.00012864447853644378
145145,1095610,1095610,2191220,3960.817620038986,0.00012863859956269152
146146,1103610,1103610,2207220,3972.1446809768677,0.00012863606571045239
147147,1111612,1111612,2223224,3983.5570800304413,0.0001286321257794043
148148,1119604,1119604,2239208,3994.8636429309845,0.00012856915600423235
149149,1126932,1126932,2253864,4005.4253561496735,0.00012851599240093492
150150,1134922,1134922,2269844,4016.926246881485,0.00012851386418333277
151151,1142914,1142914,2285828,4028.1593108177185,0.00012851139763370156
152152,1150914,1150914,2301828,4039.8310449123383,0.0001285092112084385
153153,1158910,1158910,2317820,4051.3211929798126,0.00012850600433012005
154154,1166912,1166912,2333824,4062.580992937088,0.00012850409075326752
155155,1174912,1174912,2349824,4074.086574792862,0.00012850273196818307
156156,1182912,1182912,2365824,4085.668756008148,0.00012850061102653854
157157,1190910,1190910,2381820,4098.488373994827,0.0001284989557461813
158158,1198910,1198910,2397820,4110.498142004013,0.0001284961344936164
159159,1206912,1206912,2413824,4122.488536119461,0.00012849414451920893
160160,1214914,1214914,2429828,4134.26748085022,0.0001284931058762595
161161,1222916,1222916,2445832,4146.327313899994,0.00012849149788962677
162162,1230916,1230916,2461832,4158.29457783699,0.00012848852566094138
163163,1238918,1238918,2477836,4170.734170913696,0.00012848769983975217
164164,1246916,1246916,2493832,4182.645689964294,0.00012848285768995993
165165,1254920,1254920,2509840,4195.120733976364,0.00012848159531131387
166166,1262922,1262922,2525844,4207.078237056732,0.00012847992729803082
167167,1270920,1270920,2541840,4219.505419969559,0.00012847747711930424
168168,1278922,1278922,2557844,4232.2941699028015,0.00012847541256633122
169169,1286926,1286926,2573852,4244.087624073029,0.00012847403195337392
170170,1294926,1294926,2589852,4255.841005086899,0.00012846994832216296
171171,1302928,1302928,2605856,4268.012058973312,0.00012846823301515542
172172,1310928,1310928,2621856,4280.049883842468,0.00012846276331401896
173173,1318932,1318932,2637864,4291.755327939987,0.00012846141362388153
174174,1326936,1326936,2653872,4303.303432941437,0.00012846064964833204
175175,1334936,1334936,2669872,4317.851277112961,0.00012845788660342805
176176,1342938,1342938,2685876,4333.194609880447,0.00012845625133195426
177177,1350940,1350940,2701880,4346.961420059204,0.00012845458513766062
178178,1358940,1358940,2717880,4360.093638896942,0.00012845305172959343
179179,1366942,1366942,2733884,4372.969460964203,0.00012845122910221107
180180,1374944,1374944,2749888,4384.588947057724,0.00012844900811614934
181181,1382948,1382948,2765896,4396.164185762405,0.00012844756383856293
182182,1390950,1390950,2781900,4407.838757991791,0.00012844561933889054
183183,1398952,1398952,2797904,4419.305959939957,0.0001284433928958606
184184,1406956,1406956,2813912,4430.8508207798,0.00012844218690588605
185185,1414958,1414958,2829916,4442.5232310295105,0.00012844003867940046
186186,1422962,1422962,2845924,4454.0750641822815,0.00012843849071941804
187187,1430964,1430964,2861928,4465.65437912941,0.00012843712829635479
188188,1438966,1438966,2877932,4477.528153896332,0.00012843505282944534
189189,1446964,1446964,2893928,4489.243874073029,0.00012842859905504156
190190,1454966,1454966,2909932,4500.71951007843,0.0001284265108552063
191191,1462968,1462968,2925936,4512.281453847885,0.0001284246191062266
192192,1470970,1470970,2941940,4523.6219210624695,0.0001284231293539051
193193,1478970,1478970,2957940,4539.338864803314,0.0001284201534872409
194194,1486970,1486970,2973940,4554.9510180950165,0.00012841774696426
195195,1494970,1494970,2989940,4567.416013002396,0.0001284138907067245
196196,1502970,1502970,3005940,4578.896003007889,0.00012841254647355527
197197,1510968,1510968,3021936,4590.3297238349915,0.00012840982526540756
198198,1518970,1518970,3037940,4601.934168100357,0.00012840795534430072
199199,1526972,1526972,3053944,4613.60711979866,0.0001284047721128445
200200,1534974,1534974,3069948,4625.188829898834,0.00012840047202189453
201201,1542978,1542978,3085956,4637.025455951691,0.000128399897221243
202202,1550982,1550982,3101964,4648.79921579361,0.0001283980927837547
203203,1558982,1558982,3117964,4660.691928863525,0.00012839336886827368
204204,1566986,1566986,3133972,4672.444634914398,0.00012839252121921163
205205,1574988,1574988,3149976,4684.362588882446,0.00012838898328482173
206206,1582994,1582994,3165988,4696.561088085175,0.00012838817747251596
207207,1590996,1590996,3181992,4708.355170726776,0.00012838451220886782
208208,1598996,1598996,3197992,4720.089191913605,0.00012838324073527474
209209,1607000,1607000,3214000,4731.900423049927,0.00012838048860430717
210210,1615004,1615004,3230008,4743.635693788528,0.000128379275338375
211211,1623008,1623008,3246016,4755.384136915207,0.00012837714530178346
212212,1631012,1631012,3262024,4767.552789926529,0.0001283759829675546
213213,1639014,1639014,3278028,4780.019968032837,0.00012837325994041748
214214,1647018,1647018,3294036,4792.289016962051,0.0001283719320781529
215215,1655020,1655020,3310040,4804.5820479393005,0.00012837007852795068
216216,1663024,1663024,3326048,4816.9277057647705,0.00012836889436584897
217217,1671024,1671024,3342048,4829.313600063324,0.00012836713358410634
218218,1679020,1679020,3358040,4841.686496973038,0.00012836178575525992
219219,1687022,1687022,3374044,4853.968790054321,0.00012835995585191995
220220,1695026,1695026,3390052,4866.220376968384,0.000128357927678735
221221,1703028,1703028,3406056,4878.467287063599,0.000128355673950864
222222,1711032,1711032,3422064,4890.719105005264,0.0001283539259020472
223223,1719034,1719034,3438068,4903.061386108398,0.0001283519268326927
224224,1727036,1727036,3454072,4915.44403886795,0.0001283484434679849
225225,1735040,1735040,3470080,4927.763195991516,0.0001283471610804554
226226,1743038,1743038,3486076,4940.134296178818,0.00012834499284508638
227227,1751042,1751042,3502084,4952.420919179916,0.00012834359222324565
228228,1759042,1759042,3518084,4964.739177942276,0.00012834104381909128
229229,1767046,1767046,3534092,4977.020128965378,0.0001283391520701116
230230,1775048,1775048,3550096,4989.585595846176,0.00012833759319619276
231231,1783052,1783052,3566104,5002.128290176392,0.00012833604341722094
232232,1791054,1791054,3582108,5014.485070943832,0.0001283334058825858
233233,1799056,1799056,3598112,5026.758986949921,0.00012833218715968542
234234,1807056,1807056,3614112,5039.004461050034,0.0001283289948332822
235235,1815058,1815058,3630116,5051.275520086288,0.0001283269502891926
236236,1823060,1823060,3646120,5063.5558989048,0.00012832567517762072
237237,1831060,1831060,3662120,5076.000226736069,0.00012832257198169827
238238,1839062,1839062,3678124,5088.358386039734,0.00012832138236262836
239239,1847064,1847064,3694128,5100.754555940628,0.0001283196579606738
240240,1855066,1855066,3710132,5113.060527801514,0.00012831715685024392
241241,1863068,1863068,3726136,5125.411423921585,0.00012831531785195693
242242,1871066,1871066,3742132,5137.749664068222,0.0001283121218875749
243243,1879072,1879072,3758144,5150.103564977646,0.00012831120693590492
244244,1887072,1887072,3774144,5162.317451953888,0.00012830872219637968
245245,1895074,1895074,3790148,5174.580306053162,0.00012830659397877753
246246,1903076,1903076,3806152,5186.827437162399,0.00012830340710934252
247247,1911078,1911078,3822156,5199.2992651462555,0.0001283025831071427
248248,1919076,1919076,3838152,5211.683309793472,0.0001282990433537634
249249,1927078,1927078,3854156,5223.939905166626,0.00012829779552703258
250250,1935080,1935080,3870160,5236.198469877243,0.00012829625302401837
251251,1943080,1943080,3886160,5248.506452083588,0.0001282945777347777
252252,1951084,1951084,3902168,5260.841114997864,0.00012829168190364726
253253,1959086,1959086,3918172,5273.230198144913,0.00012828745457227342
254254,1967086,1967086,3934172,5285.477291107178,0.00012828490071115084
255255,1975088,1975088,3950176,5298.250988006592,0.00012828230137529317
256256,1983092,1983092,3966184,5313.202978134155,0.00012827981299778912
257257,1991096,1991096,3982192,5324.8506371974945,0.00012827758473576978
258258,1998802,1998802,3997604,5337.541549921036,0.0001252429519809084
259259,2006802,2006802,4013604,5349.650938987732,0.00012524130215751939
260260,2014802,2014802,4029604,5362.020940065384,0.00012523893201432656
261261,2022804,2022804,4045608,5374.491523981094,0.00012523654731921852
262262,2030806,2030806,4061612,5386.9840540885925,0.00012523523582785856
263263,2038812,2038812,4077624,5399.540489912033,0.0001252342826774111
264264,2046814,2046814,4093628,5412.232903003693,0.00012523234181571752
265265,2054814,2054814,4109628,5426.435230016708,0.00012522936594905332
266266,2062812,2062812,4125624,5437.735954999924,0.00012522668112069368
267267,2070814,2070814,4141628,5448.926114082336,0.00012522395445557777
268268,2078818,2078818,4157636,5460.291704893112,0.00012522278120741248
269269,2086822,2086822,4173644,5471.503994941711,0.00012522153883764986
270270,2094824,2094824,4189648,5483.1088671684265,0.00012521970165835228
271271,2102828,2102828,4205656,5495.996042966843,0.0001252185356861446
272272,2110828,2110828,4221656,5507.194375991821,0.00012521582721092273
273273,2118830,2118830,4237660,5518.6162350177765,0.00012521346434368752
274274,2126670,2126670,4253340,5530.4660930633545,0.00012521127609943505
275275,2134188,2134188,4268376,5541.6887810230255,0.0001252032943739323
276276,2142184,2142184,4284368,5554.421329975128,0.0001252005204150919
277277,2150186,2150186,4300372,5568.799757003784,0.00012519931442511734
278278,2158184,2158184,4316368,5584.357756853104,0.00012519720985437743
279279,2166184,2166184,4332368,5603.60191488266,0.00012519377196440473
280280,2174188,2174188,4348376,5621.260301113129,0.00012519061419880018
281281,2182190,2182190,4364380,5637.624014854431,0.00012518890071078204
282282,2190194,2190194,4380388,5653.164602994919,0.00012518808580352925
283283,2198192,2198192,4396384,5668.542858123779,0.0001251835928997025
284284,2206194,2206194,4412388,5683.79052400589,0.00012518140101747122
285285,2214198,2214198,4428396,5699.943472862244,0.00012517889263108373
286286,2222200,2222200,4444400,5715.262746810913,0.00012517765753727872
287287,2230204,2230204,4460408,5729.080220937729,0.00012517541290435474
288288,2238208,2238208,4476416,5740.52348279953,0.00012517447430582251
289289,2246210,2246210,4492420,5751.92795085907,0.00012517197683337145
290290,2254212,2254212,4508424,5765.444638967514,0.00012517027244030032
291291,2262214,2262214,4524428,5778.417139053345,0.00012516890274127945
292292,2270218,2270218,4540436,5791.729398012161,0.00012516760580183472
293293,2278220,2278220,4556440,5804.88260102272,0.0001251647754543228
294294,2286222,2286222,4572444,5817.881295919418,0.00012516312199295498
295295,2294224,2294224,4588448,5831.8684849739075,0.00012516165770648513
296296,2302222,2302222,4604444,5845.4414529800415,0.00012515865455497988
297297,2310224,2310224,4620448,5858.954015016556,0.0001251567136932863
298298,2318224,2318224,4636448,5872.146395921707,0.0001251538942597108
299299,2326224,2326224,4652448,5883.985730171204,0.00012515260459622368
300300,2334226,2334226,4668452,5896.1515510082245,0.00012514955415099394
301301,2342230,2342230,4684460,5908.569751024246,0.00012514847730926704
302302,2350230,2350230,4700460,5920.020653963089,0.00012514657828432973
303303,2358232,2358232,4716464,5931.856449127197,0.0001251429675903637
304304,2366236,2366236,4732472,5943.795552015305,0.00012514151785580907
305305,2374234,2374234,4748468,5955.154008865356,0.00012513777801359538
306306,2382238,2382238,4764476,5966.435963869095,0.00012513661567936651
307307,2390240,2390240,4780480,5977.806407928467,0.00012513549154391512
308308,2398240,2398240,4796480,5989.247911930084,0.0001251337926078122
309309,2406238,2406238,4812476,6000.830489873886,0.00012513072942965664
310310,2414242,2414242,4828484,6013.073851823807,0.00012512945613707416
311311,2422242,2422242,4844484,6030.538470983505,0.00012512736066128127
312312,2430246,2430246,4860492,6043.975510120392,0.0001251259836863028
313313,2438246,2438246,4876492,6056.071017980576,0.00012512305693235248
314314,2446248,2446248,4892496,6068.395761966705,0.00012512084322224837
315315,2454250,2454250,4908500,6080.677345991135,0.00012511885142885149
316316,2462252,2462252,4924504,6092.623369932175,0.00012511621753219515
317317,2470256,2470256,4940512,6104.379503965378,0.00012511513887147885
318318,2478256,2478256,4956512,6116.763386964798,0.00012511242312029935
319319,2486258,2486258,4972516,6128.660869836807,0.00012511019849625882
320320,2494260,2494260,4988520,6140.503742933273,0.00012510738451965153
321321,2502262,2502262,5004524,6152.5683851242065,0.00012510546184785198
322322,2510264,2510264,5020528,6164.5177528858185,0.00012510292617662344
323323,2518266,2518266,5036532,6176.655643939972,0.00012510113083408214
324324,2526268,2526268,5052536,6194.67565703392,0.00012509242696978617
325325,2534274,2534274,5068548,6207.944283008575,0.00012509158113971353
326326,2542278,2542278,5084556,6219.951514959335,0.00012509097177826334
327327,2550282,2550282,5100564,6231.6118631362915,0.00012508974032243714
328328,2558286,2558286,5116572,6244.47140789032,0.00012508814324974082
329329,2566290,2566290,5132580,6255.6332359313965,0.00012508656072895974
330330,2574286,2574286,5148572,6267.773761987686,0.00012508307736425195
331331,2582290,2582290,5164580,6279.043306112289,0.0001250823352165753
332332,2590294,2590294,5180588,6292.3280119895935,0.00012508080362749752
333333,2598298,2598298,5196596,6305.864173173904,0.00012507923929661047
334334,2606300,2606300,5212600,6317.9916639328,0.00012507663268479519
335335,2614304,2614304,5228608,6330.468508005142,0.0001250747955054976
336336,2622306,2622306,5244612,6342.582706928253,0.00012507328210631385
337337,2630312,2630312,5260624,6355.472275018692,0.00012507225619629025
338338,2638312,2638312,5276624,6367.330697059631,0.00012506887469498906
339339,2646314,2646314,5292628,6382.596949100494,0.0001250673994945828
340340,2654318,2654318,5308636,6398.684818029404,0.00012506577877502423
341341,2662324,2662324,5324648,6411.5422258377075,0.00012506522398325615
342342,2670328,2670328,5340656,6423.605112075806,0.00012506255006883293
343343,2678328,2678328,5356656,6435.580946922302,0.00012506103666964918
344344,2686330,2686330,5372660,6447.407645940781,0.00012505865197454114
345345,2694330,2694330,5388660,6459.097005844116,0.00012505477752711158
346346,2702334,2702334,5404668,6470.741888046265,0.00012505394806794357
347347,2710334,2710334,5420668,6482.883458137512,0.00012505177983257454
348348,2718336,2718336,5436672,6494.868124008179,0.00012504988626460545
349349,2726340,2726340,5452680,6506.836760759354,0.00012504829282988794
350350,2734342,2734342,5468684,6519.70134305954,0.00012504597725637723
351351,2742346,2742346,5484692,6530.873027086258,0.0001250444784091087
352352,2750348,2750348,5500696,6542.14056801796,0.00012504372716648504
353353,2758348,2758348,5516696,6554.865004062653,0.00012504122059908696
354354,2766352,2766352,5532704,6567.168065071106,0.00012503982725320384
355355,2774354,2774354,5548708,6580.040006875992,0.0001250366240128642
356356,2782358,2782358,5564716,6592.5682418346405,0.00012503475954872556
357357,2790358,2790358,5580716,6605.594779968262,0.00012503294783527963
358358,2798362,2798362,5596724,6618.735512018204,0.00012503089419624303
359359,2806362,2806362,5612724,6630.167984962463,0.00012502897516242228
360360,2814366,2814366,5628732,6641.644560813904,0.00012502756180765573
361361,2822368,2822368,5644736,6653.638688087463,0.00012502642857725732
362362,2830372,2830372,5660744,6665.934872150421,0.00012502485878940206
363363,2838372,2838372,5676744,6679.76530790329,0.00012502073514042422
364364,2846372,2846372,5692744,6692.8518679142,0.0001250192926818272
365365,2854372,2854372,5708744,6706.292948007584,0.00012501627315941732
366366,2862374,2862374,5724748,6719.344580888748,0.00012501433957368135
367367,2870376,2870376,5740752,6732.678937911987,0.00012501197124947794
368368,2878378,2878378,5756756,6744.900636911392,0.0001250085697392933
369369,2886382,2886382,5772764,6758.11622095108,0.0001250066125066951
370370,2894386,2894386,5788772,6770.7238709926605,0.00012500578304752707
371371,2902388,2902388,5804776,6783.242136955261,0.000125003285575076
372372,2910390,2910390,5820780,6795.534957885742,0.0001250017903657863
373373,2918392,2918392,5836784,6807.97528886795,0.00012499962031142786
374374,2926392,2926392,5852784,6819.581696033478,0.00012499638614826836
375375,2934392,2934392,5868784,6832.616817951202,0.00012499453077907674
376376,2942396,2942396,5884792,6846.03028512001,0.00012499241893237922
377377,2950400,2950400,5900800,6858.176805973053,0.00012499095646489877
378378,2958402,2958402,5916804,6870.874392747879,0.00012498800970206503
379379,2966404,2966404,5932808,6883.1028008461,0.00012498657451942563
380380,2974400,2974400,5948800,6895.187607049942,0.00012497580974013545
381381,2982406,2982406,5964812,6907.423002958298,0.0001249746019311715
382382,2990406,2990406,5980812,6920.233165740967,0.0001249716242455179
383383,2998408,2998408,5996816,6932.956657886505,0.00012497041097958572
384384,3006410,3006410,6012820,6945.411376953125,0.00012496884301071987
385385,3014410,3014410,6028820,6958.144511938095,0.00012496544695750345
386386,3022410,3022410,6044820,6970.164781808853,0.00012496349336288404
387387,3030414,3030414,6060828,6982.766247034073,0.0001249617362191202
388388,3038418,3038418,6076836,6995.960958957672,0.00012496058661781717
389389,3046418,3046418,6092836,7008.350476026535,0.00012495902956288774
390390,3054420,3054420,6108840,7020.360216140747,0.00012495722330641001
391391,3062422,3062422,6124844,7032.614036083221,0.0001249549131898675
392392,3070424,3070424,6140848,7045.47666478157,0.00012495267765189055
393393,3078428,3078428,6156856,7057.614020824432,0.00012495148075686302
394394,3086432,3086432,6172864,7070.628415107727,0.00012494985821831506
395395,3094430,3094430,6188860,7082.365241765976,0.00012494742804847192
396396,3102432,3102432,6204864,7093.864673137665,0.00012494619477365632
397397,3110436,3110436,6220872,7105.319988965988,0.00012494389011408202
398398,3118438,3118438,6236876,7116.599404096603,0.00012494318434619345
399399,3126440,3126440,6252880,7127.848965883255,0.00012494145812524948
400400,3134444,3134444,6268888,7139.223310947418,0.00012494045950006694
401401,3142444,3142444,6284888,7150.870596885681,0.00012493719441408757
402402,3150446,3150446,6300892,7162.381810903549,0.0001249357155757025
403403,3158014,3158014,6316028,7174.680063962936,0.00010959440623992123
404404,3165892,3165892,6331784,7187.240710020065,0.00010959029532386921
405405,3173892,3173892,6347784,7199.995045900345,0.00010958868369925767
406406,3181894,3181894,6363788,7212.686920881271,0.00010958656275761314
407407,3189898,3189898,6379796,7225.7264268398285,0.00010958576785924379
408408,3197900,3197900,6395800,7238.345395088196,0.0001095834668376483
409409,3205902,3205902,6411804,7251.639906167984,0.0001095811567211058
410410,3213904,3213904,6427808,7263.866077899933,0.00010957959057122935
411411,3221908,3221908,6443816,7276.611510038376,0.00010957802442135289
412412,3229912,3229912,6459824,7289.589246034622,0.00010957631820929237
413413,3237912,3237912,6475824,7301.855880975723,0.00010957275662804022
414414,3245916,3245916,6491832,7314.181037902832,0.00010957144331769086
415415,3253918,3253918,6507836,7326.046238899231,0.00010956824735330883
416416,3261920,3261920,6523840,7338.6136248111725,0.0001095664320018841
417417,3269924,3269924,6539848,7351.382882118225,0.00010956491496472154
418418,3277928,3277928,6555856,7364.3281490802765,0.00010956393271044362
419419,3285932,3285932,6571864,7376.870957136154,0.00010956302685372066
420420,3293934,3293934,6587868,7389.599715948105,0.00010956184632959776
421421,3301936,3301936,6603872,7402.2928919792175,0.00010955993820971344
422422,3309936,3309936,6619872,7415.195160865784,0.00010955756988551002
423423,3317938,3317938,6635876,7426.832075119019,0.00010955580728477798
424424,3325940,3325940,6651880,7439.722184896469,0.00010955433754133992
425425,3333942,3333942,6667884,7452.085119962692,0.00010955214202112984
426426,3341946,3341946,6683892,7465.505810022354,0.00010955067227769177
427427,3349950,3349950,6699900,7479.051707983017,0.00010954901517834514
428428,3357952,3357952,6715904,7490.9896059036255,0.0001095470433938317
429429,3365956,3365956,6731912,7503.865708112717,0.00010954557183140423
430430,3373960,3373960,6747920,7516.778349876404,0.00010954450226563495
431431,3381964,3381964,6763928,7529.343622922897,0.0001095436546165729
432432,3389968,3389968,6779936,7542.358554840088,0.00010954241588478908
433433,3397964,3397964,6795928,7554.412557125092,0.0001095399657060625
434434,3405968,3405968,6811936,7566.601452112198,0.00010953826676995959
435435,3413966,3413966,6827932,7579.318102121353,0.00010953491255349945
436436,3421968,3421968,6843936,7592.3171210289,0.00010953338824037928
437437,3429970,3429970,6859940,7604.620557069778,0.0001095318602892803
438438,3437972,3437972,6875944,7616.636275053024,0.00010953029959637206
439439,3445976,3445976,6891952,7628.108855009079,0.00010952836055366788
440440,3453976,3453976,6907952,7641.320461034775,0.00010952650336548686
441441,3461982,3461982,6923964,7654.079284906387,0.0001095262668968644
442442,3469966,3469966,6939932,7665.964652061462,0.00010952610136882868
443443,3477802,3477802,6955604,7678.510760068893,0.00010952576849376783
444444,3484800,3484800,6969600,7689.956108093262,9.331427827419247e-05
445445,3492780,3492780,6985560,7702.12292098999,9.33101346163312e-05
446446,3500766,3500766,7001532,7715.421035051346,9.330525426776148e-05
447447,3508758,3508758,7017516,7727.2190709114075,9.329622844234109e-05
448448,3516758,3516758,7033516,7739.302773952484,9.329357999376953e-05
449449,3524142,3524142,7048284,7751.205189943314,9.32848433876643e-05
450450,3531926,3531926,7063852,7763.112648010254,9.327789848612156e-05
451451,3539908,3539908,7079816,7776.368840932846,9.327565021521877e-05
452452,3547898,3547898,7095796,7788.299333810806,9.326638246420771e-05
453453,3555896,3555896,7111792,7800.243298768997,9.326481267635245e-05
454454,3563896,3563896,7127792,7812.622358083725,9.32636085053673e-05
455455,3571894,3571894,7143788,7824.803128004074,9.326185136160348e-05
456456,3579894,3579894,7159788,7838.015746116638,9.325787141278852e-05
457457,3587890,3587890,7175780,7851.329700946808,9.325564133177977e-05
458458,3595890,3595890,7191780,7864.760426998138,9.325376413471531e-05
459459,3603892,3603892,7207784,7877.570760011673,9.32511902647093e-05
460460,3611890,3611890,7223780,7889.782081127167,9.324963684775867e-05
461461,3619892,3619892,7239784,7902.575755119324,9.324804705101997e-05
462462,3627896,3627896,7255792,7915.021718978882,9.32469865801977e-05
463463,3635898,3635898,7271796,7927.207176923752,9.324567508883774e-05
464464,3643898,3643898,7287796,7939.758256912231,9.324465463578235e-05
465465,3651900,3651900,7303800,7953.7641248703,9.324337588623166e-05
466466,3659904,3659904,7319808,7965.389960050583,9.324146776634734e-05
467467,3667906,3667906,7335812,7976.912811040878,9.323909216618631e-05
468468,3675910,3675910,7351820,7988.763071060181,9.323812810180243e-05
469469,3683914,3683914,7367828,8000.462677001953,9.323732410848606e-05
470470,3691916,3691916,7383832,8012.727912902832,9.323614722234197e-05
471471,3699920,3699920,7399840,8024.564216852188,9.32351886149263e-05
472472,3707922,3707922,7415844,8036.464766025543,9.323424819740467e-05
473473,3715926,3715926,7431852,8048.344675779343,9.32328257476911e-05
474474,3723928,3723928,7447856,8060.349511861801,9.323191443399992e-05
475475,3731932,3731932,7463864,8072.104546070099,9.323110498371534e-05
476476,3739936,3739936,7479872,8083.538738965988,9.322996265836991e-05
477477,3747936,3747936,7495872,8095.040255069733,9.322870755568147e-05
478478,3755936,3755936,7511872,8106.432404994965,9.322444202553015e-05
479479,3763940,3763940,7527880,8118.080888748169,9.322333426098339e-05
480480,3771946,3771946,7543892,8129.671411991119,9.322275764134247e-05
481481,3779948,3779948,7559896,8141.188038825989,9.322082951257471e-05
482482,3787952,3787952,7575904,8152.7881190776825,9.321957440988626e-05
483483,3795956,3795956,7591912,8164.237859964371,9.321847028331831e-05
484484,3803958,3803958,7607916,8175.593590974808,9.321612560597714e-05
485485,3811962,3811962,7623924,8187.124344110489,9.321563265984878e-05
486486,3819966,3819966,7639932,8200.554944992065,9.321493234892841e-05
487487,3827970,3827970,7655940,8213.730453968048,9.321399011241738e-05
488488,3835954,3835954,7671908,8227.371016979218,9.310379755333997e-05
489489,3843956,3843956,7687912,8239.517596960068,9.310275527241174e-05
490490,3851960,3851960,7703920,8251.235055923462,9.310152199759614e-05
491491,3859962,3859962,7719924,8262.69276189804,9.309989945904817e-05
492492,3867964,3867964,7735928,8275.806792974472,9.309884080721531e-05
493493,3875966,3875966,7751932,8288.074819803238,9.309794404543936e-05
494494,3883970,3883970,7767940,8300.369486808777,9.309297638537828e-05
495495,3891974,3891974,7783948,8312.145826101303,9.309220513387118e-05
496496,3899974,3899974,7799948,8326.291639089584,9.309015695180278e-05
497497,3907980,3907980,7815960,8338.73748087883,9.308921653428115e-05
498498,3915982,3915982,7831964,8350.725409030914,9.308669541496783e-05
499499,3923988,3923988,7847976,8362.926189899445,9.308609696745407e-05
500501,3931996,3931996,7863992,8375.878509759903,9.30839050852228e-05
501502,3939998,3939998,7879996,8389.091576099396,9.308329936175141e-05
502503,3948000,3948000,7896000,8401.820761919022,9.308116386819165e-05
503504,3956002,3956002,7912004,8414.116397857666,9.307700020144694e-05
504505,3964006,3964006,7928012,8426.638839006424,9.307589425588958e-05
505506,3972008,3972008,7944016,8438.018276929855,9.307480468123686e-05
506507,3980014,3980014,7960028,8449.595999956131,9.307383334089536e-05
507508,3988018,3988018,7976036,8461.069015979767,9.307281834480818e-05
508509,3996018,3996018,7992036,8472.493729114532,9.307177606387995e-05
509510,4004022,4004022,8008044,8484.18180513382,9.306993160862476e-05
510511,4012024,4012024,8024048,8495.849211931229,9.306932588515338e-05
511512,4020026,4020026,8040052,8507.608264923096,9.306861284130719e-05
512513,4028028,4028028,8056056,8520.143522024155,9.306618812843226e-05
513514,4036034,4036034,8072068,8531.95577287674,9.306608444603626e-05
514515,4044038,4044038,8088076,8544.568274021149,9.306440006184857e-05
515516,4052042,4052042,8104084,8556.474166154861,9.30635433178395e-05
516517,4060046,4060046,8120092,8568.518056869507,9.306250649387948e-05
517518,4068046,4068046,8136092,8580.012729883194,9.305941784987226e-05
518519,4076048,4076048,8152096,8592.345742940903,9.305717321694829e-05
519520,4084048,4084048,8168096,8604.35098695755,9.305583444074728e-05
520521,4092052,4092052,8184104,8617.085340976715,9.305496314482298e-05
521522,4100058,4100058,8200116,8628.92749118805,9.305354979005642e-05
522523,4108062,4108062,8216124,8640.487235069275,9.305300045525655e-05
523524,4116064,4116064,8232128,8652.296590805054,9.305216553912032e-05
524525,4124070,4124070,8248140,8664.14608001709,9.305135063186754e-05
525526,4132072,4132072,8264144,8676.16763496399,9.304971354140434e-05
526527,4140076,4140076,8280152,8690.493170976639,9.30482037801994e-05
527528,4148078,4148078,8296156,8702.46970295906,9.304621016781311e-05
528529,4156084,4156084,8312168,8715.192216157913,9.304567902290728e-05
529530,4164086,4164086,8328172,8727.687076807022,9.304438754043076e-05
530531,4172088,4172088,8344176,8738.781017780304,9.304236846219283e-05
531532,4180092,4180092,8360184,8750.087146043777,9.303996193921193e-05
532533,4188094,4188094,8376188,8761.90893793106,9.303955812356435e-05
533534,4196094,4196094,8392188,8773.515941858292,9.303741353505757e-05
534535,4204096,4204096,8408192,8785.30028295517,9.303617844125256e-05
535536,4212100,4212100,8424200,8797.418647050858,9.303465230914298e-05
536537,4220102,4220102,8440204,8809.02745294571,9.303359183832072e-05
537538,4228106,4228106,8456212,8820.906100034714,9.303246770286933e-05
538539,4236106,4236106,8472212,8832.24810910225,9.303154911322054e-05
539540,4244108,4244108,8488216,8844.100095033646,9.303028491558507e-05
540541,4252110,4252110,8504220,8855.823643922806,9.30292753764661e-05
541542,4260114,4260114,8520228,8867.317800998688,9.302834041591268e-05
542543,4268118,4268118,8536236,8879.337297916412,9.302734542870894e-05
543544,4276118,4276118,8552236,8892.006641864777,9.302567195845768e-05
544545,4284122,4284122,8568244,8903.657879114151,9.302274156652857e-05
545546,4292126,4292126,8584252,8915.200784921646,9.302154285251163e-05
546547,4300128,4300128,8600256,8927.12379693985,9.302033868152648e-05
547548,4308134,4308134,8616268,8939.898137807846,9.30199385038577e-05
548549,4316138,4316138,8632276,8952.366358995438,9.301948921347503e-05
549550,4324140,4324140,8648280,8964.040583848953,9.301753743784502e-05
550551,4332144,4332144,8664288,8975.338287830353,9.301594946009573e-05
551552,4340146,4340146,8680292,8986.493261814117,9.301428508479148e-05
552553,4348150,4348150,8696300,8997.917036056519,9.301300269726198e-05
553554,4356150,4356150,8712300,9009.360985994339,9.301067984779365e-05
554555,4364154,4364154,8728308,9021.158399105072,9.300997589889448e-05
555556,4372156,4372156,8744312,9032.728719949722,9.300760575570166e-05
556557,4380158,4380158,8760316,9044.252444982529,9.300633792008739e-05
557558,4388162,4388162,8776324,9055.62809920311,9.300486635765992e-05
558559,4396164,4396164,8792328,9069.715762853622,9.300371857534628e-05
559560,4404168,4404168,8808336,9083.132019996643,9.299959492636845e-05
560561,4412172,4412172,8824344,9097.204033136368,9.299864359491039e-05
561562,4420176,4420176,8840352,9108.964668989182,9.299753401137423e-05
562563,4428178,4428178,8856356,9120.870739936829,9.2996802777634e-05
563564,4436178,4436178,8872356,9132.944772958755,9.299369776272215e-05
564565,4444180,4444180,8888360,9147.402414798737,9.299247722083237e-05
565566,4452184,4452184,8904368,9159.865628004074,9.299191151512787e-05
566567,4460184,4460184,8920368,9172.669539928436,9.297786527895369e-05
567568,4468184,4468184,8936368,9184.846221923828,9.297553879150655e-05
568569,4476188,4476188,8952376,9197.15489578247,9.297444012190681e-05
569570,4484194,4484194,8968388,9209.215960741043,9.297396718466189e-05
570571,4492196,4492196,8984392,9222.009803056717,9.297277574660257e-05
571572,4500202,4500202,9000404,9233.969883918762,9.29715133679565e-05
572573,4507662,4507662,9015324,9245.714777946472,4.8176270865951665e-05
573574,4515622,4515622,9031244,9257.929999828339,4.817403714696411e-05
574575,4523616,4523616,9047232,9270.128941059113,4.8172505557886325e-05
575576,4531614,4531614,9063228,9282.448985815048,4.817110311705619e-05
576577,4539616,4539616,9079232,9294.967912912369,4.816964974452276e-05
577578,4547620,4547620,9095240,9307.761698007584,4.8168838475248776e-05
578579,4555622,4555622,9111244,9319.646728038788,4.816767614101991e-05
579580,4563626,4563626,9127252,9332.970612049103,4.816683940589428e-05
580581,4571628,4571628,9143256,9345.460038900375,4.816522778128274e-05
581582,4579628,4579628,9159256,9358.031720876694,4.8164056352106854e-05
582583,4587630,4587630,9175260,9371.18741106987,4.816251566808205e-05
583584,4595636,4595636,9191272,9383.659312009811,4.816140790353529e-05
584585,4603638,4603638,9207276,9396.575572013855,4.815865213458892e-05
585586,4611642,4611642,9223284,9407.89815402031,4.8157737182918936e-05
586587,4619648,4619648,9239296,9419.292406082153,4.8157342462218367e-05
587588,4627654,4627654,9255308,9430.898927927017,4.8155725380638614e-05
588589,4635656,4635656,9271312,9442.289084911346,4.815300417249091e-05
589590,4643660,4643660,9287320,9454.825087070465,4.8152247472899035e-05
590591,4651662,4651662,9303324,9466.337843894958,4.815159445570316e-05
591592,4659664,4659664,9319328,9478.207419872284,4.815058127860539e-05
592593,4667666,4667666,9335332,9490.523386955261,4.814886415260844e-05
593594,4675672,4675672,9351344,9502.565751075745,4.814832027477678e-05
594595,4683676,4683676,9367352,9514.53267788887,4.814743260794785e-05
595596,4691682,4691682,9383364,9526.580249786377,4.814589919988066e-05
596597,4699686,4699686,9399372,9538.920305013657,4.8144234824576415e-05
597598,4707694,4707694,9415388,9551.408746957779,4.8144111133296974e-05
598599,4715698,4715698,9431396,9564.133141040802,4.814279418496881e-05
599600,4723704,4723704,9447408,9577.139149188995,4.814233579963911e-05
600601,4731710,4731710,9463420,9589.55125784874,4.814201020053588e-05
601602,4739712,4739712,9479424,9602.02046585083,4.813949271920137e-05
602603,4747718,4747718,9495436,9615.50515294075,4.813863961317111e-05
603604,4755720,4755720,9511440,9628.117332935333,4.813809209736064e-05
604605,4763724,4763724,9527448,9641.702644109726,4.813597479369491e-05
605606,4771730,4771730,9543460,9654.045153141022,4.813275700144004e-05
606607,4779736,4779736,9559472,9666.422271966934,4.813237137568649e-05
607608,4787742,4787742,9575484,9678.515363931656,4.8131882067536935e-05
608609,4795748,4795748,9591496,9691.074465990067,4.813087980437558e-05
609610,4803750,4803750,9607500,9703.952887058258,4.812935549125541e-05
610611,4811756,4811756,9623512,9716.62767291069,4.8128655180335045e-05
611612,4819760,4819760,9639520,9728.967235088348,4.812797124031931e-05
612613,4827762,4827762,9655524,9742.684159994125,4.812401130038779e-05
613614,4835768,4835768,9671536,9754.84210896492,4.812340921489522e-05
614615,4843774,4843774,9687548,9766.688544988632,4.811994222109206e-05
615616,4851780,4851780,9703560,9779.015278816223,4.811945836991072e-05
616617,4859782,4859782,9719564,9791.074779987335,4.8117841288330965e-05
617618,4867786,4867786,9735572,9804.311798095703,4.8113819502759725e-05
618619,4875792,4875792,9751584,9815.737643957138,4.811343751498498e-05
619620,4883792,4883792,9767584,9827.515342950821,4.8111623982549645e-05
620621,4891796,4891796,9783592,9840.064710855484,4.811002690985333e-05
621622,4899800,4899800,9799600,9853.050737857819,4.8109664930962026e-05
622623,4907804,4907804,9815608,9867.77434706688,4.8107935072039254e-05
623624,4915808,4915808,9831616,9880.79858994484,4.810676728084218e-05
624625,4923812,4923812,9847624,9894.015525817871,4.810495192941744e-05
625626,4931816,4931816,9863632,9908.20220899582,4.8103775043273345e-05
626627,4939820,4939820,9879640,9921.329432964325,4.8100841013365425e-05
627628,4947824,4947824,9895648,9933.83042883873,4.810060818272177e-05
628629,4955826,4955826,9911652,9947.765688180923,4.809844176634215e-05
629630,4963832,4963832,9927664,9959.724628925323,4.809497477253899e-05
630631,4971838,4971838,9943676,9971.735690116882,4.809445090359077e-05
631632,4979842,4979842,9959684,9984.18023610115,4.809403617400676e-05
632633,4987846,4987846,9975692,9997.60100197792,4.809228266822174e-05
633634,4995854,4995854,9991708,10010.004081010818,4.809216261492111e-05
634635,5003856,5003856,10007712,10022.337241888046,4.809085112356115e-05
635636,5011860,5011860,10023720,10034.962509155273,4.809022539120633e-05
636637,5019862,5019862,10039724,10049.69403386116,4.808710036741104e-05
637638,5027868,5027868,10055736,10062.690940856934,4.8084830268635415e-05
638639,5035870,5035870,10071740,10076.460229873657,4.80836442875443e-05
639640,5043874,5043874,10087748,10090.313735961914,4.808209814655129e-05
640641,5051880,5051880,10103760,10103.056557178497,4.808185622096062e-05
641642,5059884,5059884,10119768,10114.799787044525,4.808013000001665e-05
642643,5067884,5067884,10135768,10127.604351043701,4.80788221466355e-05
643644,5075890,5075890,10151780,10139.585155963898,4.80761009384878e-05
644645,5083894,5083894,10167788,10151.546803951263,4.807567711395677e-05
645646,5091896,5091896,10183792,10165.186940908432,4.807386903848965e-05
646647,5099902,5099902,10199804,10177.915655851364,4.807206641999073e-05
647648,5107906,5107906,10215812,10190.212120056152,4.807131517736707e-05
648649,5115908,5115908,10231816,10202.41528391838,4.8069732656585984e-05
649650,5123914,5123914,10247828,10213.978256940842,4.806924880540464e-05
650651,5131916,5131916,10263832,10225.440024852753,4.8067071475088596e-05
651652,5139920,5139920,10279840,10237.002223968506,4.8066367526189424e-05
652653,5147926,5147926,10295852,10248.948096036911,4.8065865485114045e-05
653654,5155930,5155930,10311860,10260.54241681099,4.806418473890517e-05
654655,5163932,5163932,10327864,10272.007558822632,4.8060643166536465e-05
655656,5171938,5171938,10343876,10283.404302835464,4.8057723688543774e-05
656657,5179946,5179946,10359892,10295.13494515419,4.805759817827493e-05
657658,5187948,5187948,10375896,10306.85745382309,4.805463686352596e-05
658659,5195954,5195954,10391908,10318.169606924057,4.8054133003461175e-05
659660,5203960,5203960,10407920,10329.642491817474,4.8050973418867216e-05
660661,5211964,5211964,10423928,10342.053047180176,4.805018215847667e-05
661662,5219970,5219970,10439940,10355.102109909058,4.804994932783302e-05
662663,5227972,5227972,10455944,10368.625874042511,4.8049361794255674e-05
663664,5235242,5235242,10470484,10380.006292104721,4.785737291967962e-05
664665,5243236,5243236,10486472,10392.492612838745,4.785667078976985e-05
665666,5251238,5251238,10502476,10405.086639881134,4.785606142831966e-05
666667,5259236,5259236,10518472,10416.587924957275,4.785514647664968e-05
667668,5267240,5267240,10534480,10428.32358288765,4.785450983035844e-05
668669,5275240,5275240,10550480,10440.38830280304,4.785342389368452e-05
669670,5283246,5283246,10566492,10453.45567893982,4.785311466548592e-05
670671,5291250,5291250,10582500,10466.931813955307,4.7851886847638525e-05
671672,5299254,5299254,10598508,10479.614068984985,4.78517195006134e-05
672673,5307258,5307258,10614516,10491.78339099884,4.785102646565065e-05
673674,5315260,5315260,10630520,10504.245143175125,4.784829434356652e-05
674675,5323262,5323262,10646524,10516.511357069016,4.784764860232826e-05
675676,5331266,5331266,10662532,10528.734397888184,4.784660632140003e-05
676677,5339268,5339268,10678536,10541.593277931213,4.784544580616057e-05
677678,5347274,5347274,10694548,10554.355508089066,4.784531301993411e-05
678679,5355278,5355278,10710556,10566.836457967758,4.784456905326806e-05
679680,5363284,5363284,10726568,10579.287019968033,4.78439233120298e-05
680681,5371290,5371290,10742580,10592.574565887451,4.784359589393716e-05
681682,5379296,5379296,10758592,10605.007993936539,4.7842228013905697e-05
682683,5387302,5387302,10774604,10618.326171875,4.7841929699643515e-05
683684,5395304,5395304,10790608,10630.940546989441,4.784082921105437e-05
684685,5403310,5403310,10806620,10644.06333398819,4.784042903338559e-05
685686,5411312,5411312,10822624,10656.065248012543,4.783993608725723e-05
686687,5419316,5419316,10838632,10668.493372917175,4.7838564569246955e-05
687688,5427320,5427320,10854640,10680.878556013107,4.7837775127845816e-05
688689,5435322,5435322,10870644,10693.317858934402,4.7837056627031416e-05
689690,5443324,5443324,10886648,10705.729650974274,4.783639087690972e-05
690691,5451326,5451326,10902652,10719.116044044495,4.783586518897209e-05
691692,5459330,5459330,10918660,10732.285477876663,4.7835399527684785e-05
692693,5467332,5467332,10934664,10744.91076207161,4.7833829739829525e-05
693694,5475336,5475336,10950672,10757.913442850113,4.783312397194095e-05
694695,5483342,5483342,10966684,10769.572745084763,4.7832767450017855e-05
695696,5491348,5491348,10982696,10781.531282901764,4.783236545335967e-05
696697,5499352,5499352,10998704,10793.63192820549,4.78317124361638e-05
697698,5507356,5507356,11014712,10806.358540058136,4.783075019076932e-05
698699,5515362,5515362,11030724,10818.911438941956,4.78303281852277e-05
699700,5523364,5523364,11046728,10832.092458963394,4.782959513249807e-05
700701,5531368,5531368,11062736,10845.898658752441,4.782903124578297e-05
701702,5539372,5539372,11078744,10860.12159705162,4.782723954122048e-05
702703,5547374,5547374,11094748,10872.064903974533,4.782674295711331e-05
703704,5555380,5555380,11110760,10884.715074062347,4.782627001986839e-05
704705,5563384,5563384,11126768,10896.848695993423,4.782577889272943e-05
705706,5571390,5571390,11142780,10909.136403083801,4.782431096828077e-05
706707,5579396,5579396,11158792,10921.555417776108,4.782402720593382e-05
707708,5587402,5587402,11174804,10934.279505968094,4.7822759370319545e-05
708709,5595408,5595408,11190816,10946.919122934341,4.782264295499772e-05
709710,5603410,5603410,11206820,10958.833219051361,4.78205292893108e-05
710711,5611412,5611412,11222824,10971.079831123352,4.781991992786061e-05
711712,5619412,5619412,11238824,10983.755379915237,4.781688221555669e-05
712713,5627416,5627416,11254832,10996.278589010239,4.781659117725212e-05
713714,5635420,5635420,11270840,11008.594157934189,4.781525240105111e-05
714715,5643428,5643428,11286856,11021.198805093765,4.781517600349616e-05
715716,5651424,5651424,11302848,11033.865684986115,4.780938797921408e-05
716717,5659430,5659430,11318860,11046.696181058884,4.78089878015453e-05
717718,5667432,5667432,11334864,11061.011116981506,4.780832750839181e-05
718719,5675436,5675436,11350872,11073.200289964676,4.780658855452202e-05
719720,5683440,5683440,11366880,11085.766306877136,4.7806410293560475e-05
720721,5691446,5691446,11382892,11098.257323026657,4.780597191711422e-05
721722,5699450,5699450,11398900,11110.888752937317,4.780500603374094e-05
722723,5707454,5707454,11414908,11122.976371049881,4.78040637972299e-05
723724,5715460,5715460,11430920,11135.825340032578,4.7803589040995575e-05
724725,5723462,5723462,11446924,11148.2471139431,4.780275048688054e-05
725726,5731468,5731468,11462936,11160.279664993286,4.780213021149393e-05
726727,5739470,5739470,11478940,11173.962476015091,4.780132439918816e-05
727728,5747474,5747474,11494948,11189.050549983978,4.77993435197277e-05
728729,5755480,5755480,11510960,11202.177257061005,4.779927621711977e-05
729730,5763484,5763484,11526968,11214.847149133682,4.779697883350309e-05
730731,5771490,5771490,11542980,11227.723116159439,4.779663686349522e-05
731732,5779498,5779498,11558996,11238.93217587471,4.7796560465940274e-05
732733,5787498,5787498,11574996,11250.166974067688,4.7795309001230635e-05
733734,5795506,5795506,11591012,11262.054144144058,4.779523442266509e-05
734735,5803510,5803510,11607020,11273.665156841278,4.7794816055102274e-05
735736,5811516,5811516,11623032,11285.241919994354,4.7794032070669346e-05
736737,5819520,5819520,11639040,11296.802202939987,4.779391747433692e-05
737738,5827524,5827524,11655048,11308.57255101204,4.779110167874023e-05
738739,5835528,5835528,11671056,11321.52963399887,4.7790723328944296e-05
739740,5843534,5843534,11687068,11333.626747846603,4.7790148528292775e-05
740741,5851540,5851540,11703080,11347.607811927795,4.778982111020014e-05
741742,5859544,5859544,11719088,11360.292216062546,4.778920265380293e-05
742743,5867550,5867550,11735100,11373.597379207611,4.7788460506126285e-05
743744,5875552,5875552,11751104,11386.352909088135,4.7787871153559536e-05
744745,5883558,5883558,11767116,11399.350744962692,4.778678703587502e-05
745746,5891562,5891562,11783124,11411.982241153717,4.778640141012147e-05
746747,5899564,5899564,11799128,11424.559586763382,4.778568836627528e-05
747748,5907566,5907566,11815132,11438.705055952072,4.778476977662649e-05
748749,5915572,5915572,11831144,11452.11277604103,4.778365655511152e-05
749750,5923576,5923576,11847152,11465.306929826736,4.7783049012650736e-05
750751,5931578,5931578,11863156,11477.798770904541,4.778214679390658e-05
751752,5939582,5939582,11879164,11489.69396519661,4.7781535613466986e-05
752753,5947586,5947586,11895172,11501.652084112167,4.778132824867498e-05
753754,5955588,5955588,11911176,11513.816824913025,4.7780627937754616e-05
754755,5963592,5963592,11927184,11527.826241016388,4.7778898078831844e-05
755756,5971596,5971596,11943192,11539.723148107529,4.777869617100805e-05
756757,5979600,5979600,11959200,11552.129284858704,4.777796311827842e-05
757758,5987602,5987602,11975204,11563.963531017303,4.777680442202836e-05
758759,5995606,5995606,11991212,11577.24056816101,4.777631693286821e-05
759760,6003612,6003612,12007224,11590.163790941238,4.777578214998357e-05
760761,6011614,6011614,12023228,11603.050202846527,4.7774661652510986e-05
761762,6019620,6019620,12039240,11615.134126901627,4.7773881306056865e-05
762763,6027626,6027626,12055252,11627.955046892166,4.777308458869811e-05
763764,6035630,6035630,12071260,11640.224630117416,4.7772629841347225e-05
764765,6043636,6043636,12087272,11652.376775979996,4.777260073751677e-05
765766,6051642,6051642,12103284,11664.545330047607,4.777257527166512e-05
766767,6059646,6059646,12119292,11678.037868022919,4.777057620231062e-05
767768,6067650,6067650,12135300,11690.42997097969,4.7769988668733276e-05
768769,6075652,6075652,12151304,11702.850441932678,4.776951391249895e-05
769770,6083656,6083656,12167312,11716.030636072159,4.776684545504395e-05
770771,6091660,6091660,12183320,11728.68485403061,4.776650166604668e-05
771772,6099664,6099664,12199328,11742.335248947144,4.776566493092105e-05
772773,6107668,6107668,12215336,11754.792183160782,4.776495916303247e-05
773774,6115674,6115674,12231348,11768.23114991188,4.776475361722987e-05
774775,6123678,6123678,12247356,11781.476903915405,4.776332752953749e-05
775776,6131684,6131684,12263368,11793.535983800888,4.776309469889384e-05
776777,6139690,6139690,12279380,11805.85387301445,4.7762328904354945e-05
777778,6147696,6147696,12295392,11818.382637023926,4.776198147737887e-05
778779,6155700,6155700,12311400,11831.308364152908,4.776138666784391e-05
779780,6163702,6163702,12327404,11842.950328826904,4.776079731527716e-05
780781,6171708,6171708,12343416,11854.945634126663,4.7760040615685284e-05
781782,6179712,6179712,12359424,11866.953306913376,4.775966044689994e-05
782783,6187712,6187712,12375424,11879.385663986206,4.7758732762304135e-05
783784,6195720,6195720,12391440,11891.862858057022,4.7758656364749186e-05
784785,6203446,6203446,12406892,11904.108717918396,4.3524112697923556e-05
785786,6211450,6211450,12422900,11917.143632888794,4.3523634303710423e-05
786787,6219454,6219454,12438908,11929.784616947174,4.3522968553588726e-05
787788,6227460,6227460,12454920,11941.910083055496,4.352061478130054e-05
788789,6235466,6235466,12470932,11954.158799886703,4.352051837486215e-05
789790,6243470,6243470,12486940,11966.320015907288,4.352004179963842e-05
790791,6251476,6251476,12502952,11978.297960996628,4.3518259190022945e-05
791792,6259480,6259480,12518960,11992.404437065125,4.3517802623682655e-05
792793,6267484,6267484,12534968,12004.691654920578,4.3515765355550684e-05
793794,6275490,6275490,12550980,12016.869148015976,4.35155689046951e-05
794795,6283494,6283494,12566988,12028.902195930481,4.351429015514441e-05
795796,6291498,6291498,12582996,12040.913276910782,4.351368988864124e-05
796797,6299504,6299504,12599008,12052.899644851685,4.351353163656313e-05
797798,6307506,6307506,12615012,12064.247332811356,4.351075040176511e-05
798799,6315508,6315508,12631016,12076.0521941185,4.3510020987014286e-05
799800,6323512,6323512,12647024,12088.375960826874,4.350902418082114e-05
800801,6331518,6331518,12663036,12101.415224075317,4.350853669166099e-05
801802,6339524,6339524,12679048,12114.004008054733,4.3505639041541144e-05
802803,6347526,6347526,12695052,12126.874216079712,4.350494600657839e-05
803804,6355532,6355532,12711064,12140.80870294571,4.350473318481818e-05
804805,6363534,6363534,12727068,12154.307427883148,4.3503525375854224e-05
805806,6371538,6371538,12743076,12168.269876003265,4.3502879634615965e-05
806807,6379542,6379542,12759084,12181.800481081009,4.350252856966108e-05
807808,6387548,6387548,12775096,12195.031320095062,4.3501560867298394e-05
808809,6395552,6395552,12791104,12208.1079890728,4.3500258470885456e-05
809810,6403554,6403554,12807108,12221.078359127045,4.3499057937879115e-05
810811,6411560,6411560,12823120,12233.868082046509,4.349834671302233e-05
811812,6419564,6419564,12839128,12246.700219869614,4.3498021113919094e-05
812813,6427564,6427564,12855128,12259.243822813034,4.3494286728673615e-05
813814,6435570,6435570,12871140,12272.015914916992,4.3493953853612766e-05
814815,6443572,6443572,12887144,12285.48195695877,4.349326809460763e-05
815816,6451580,6451580,12903160,12298.2425699234,4.349319169705268e-05
816817,6459582,6459582,12919164,12310.46561908722,4.3492496843100525e-05
817818,6467588,6467588,12935176,12322.87373805046,4.349172559159342e-05
818819,6475592,6475592,12951184,12335.196906089783,4.3491158066899516e-05
819820,6483596,6483596,12967192,12348.866146802902,4.3490701500559226e-05
820821,6491602,6491602,12983204,12362.335932016373,4.349042137619108e-05
821822,6499606,6499606,12999212,12374.57818698883,4.3489941162988544e-05
822823,6507610,6507610,13015220,12386.952405929565,4.348959919298068e-05
823824,6515618,6515618,13031236,12398.722290039062,4.348952279542573e-05
824825,6523620,6523620,13047240,12411.196585893631,4.348830225353595e-05
825826,6531624,6531624,13063248,12423.392183065414,4.348687616584357e-05
826827,6539628,6539628,13079256,12435.598186016083,4.3486377762747e-05
827828,6547634,6547634,13095268,12449.042984962463,4.3486119466251694e-05
828829,6555634,6555634,13111268,12461.746957063675,4.3484258640091866e-05
829830,6563640,6563640,13127280,12474.119660139084,4.348403490439523e-05
830831,6571642,6571642,13143284,12487.06882095337,4.348327456682455e-05
831832,6579648,6579648,13159296,12500.166156053543,4.348292532085907e-05
832833,6587652,6587652,13175304,12512.510522842407,4.348144830146339e-05
833834,6595658,6595658,13191316,12525.820997953415,4.348007860244252e-05
834835,6603662,6603662,13207324,12538.977834939957,4.3479436499183066e-05
835836,6611670,6611670,13223340,12550.928814888,4.347936010162812e-05
836837,6619676,6619676,13239352,12562.88616490364,4.3478876250446774e-05
837838,6627680,6627680,13255360,12575.34111905098,4.347888352640439e-05
838839,6635682,6635682,13271364,12589.308527946472,4.347871981735807e-05
839840,6643688,6643688,13287376,12602.417680978775,4.3478697989485227e-05
840841,6651692,6651692,13303384,12615.108706951141,4.3478743464220315e-05
841842,6659696,6659696,13319392,12628.59992980957,4.347606409282889e-05
842843,6667700,6667700,13335400,12641.096162080765,4.347471440269146e-05
843844,6675706,6675706,13351412,12653.823755025864,4.3474423364386894e-05
844845,6683712,6683712,13367424,12665.706953048706,4.3473957703099586e-05
845846,6691716,6691716,13383432,12677.312358856201,4.347335379861761e-05
846847,6699718,6699718,13399436,12689.356693029404,4.3472458855831064e-05
847848,6707722,6707722,13415444,12701.132019042969,4.3471731260069646e-05
848849,6715728,6715728,13431456,12714.162924051285,4.3471514800330624e-05
849850,6723732,6723732,13447464,12725.623893022537,4.34701178164687e-05
850851,6731738,6731738,13463476,12737.190071105957,4.346972309576813e-05
851852,6739744,6739744,13479488,12748.949939966202,4.346933747001458e-05
852853,6747746,6747746,13495492,12760.993965148926,4.346847163105849e-05
853854,6755750,6755750,13511500,12772.81253695488,4.346780224295799e-05
854855,6763754,6763754,13527508,12784.358081102371,4.346716741565615e-05
855856,6771758,6771758,13543516,12797.334072828293,4.346615787653718e-05
856857,6779764,6779764,13559528,12811.377378940582,4.3465801354614086e-05
857858,6787768,6787768,13575536,12824.06705212593,4.346559762780089e-05
858859,6795770,6795770,13591540,12837.458355903625,4.346461719251238e-05
859860,6803776,6803776,13607552,12849.781985998154,4.346211972006131e-05
860861,6811776,6811776,13623552,12862.22312092781,4.346189780335408e-05
861862,6819778,6819778,13639556,12874.413198947906,4.3459787775645964e-05
862863,6827782,6827782,13655564,12887.127958059311,4.34596004197374e-05
863864,6835788,6835788,13671576,12899.912195205688,4.345890920376405e-05
864865,6843792,6843792,13687584,12912.574253797531,4.345832348917611e-05
865866,6851796,6851796,13703592,12926.434584140778,4.345684283180162e-05
866867,6859800,6859800,13719600,12939.212681055069,4.3456551793497056e-05
867868,6867804,6867804,13735608,12951.740791082382,4.345454726717435e-05
868869,6875806,6875806,13751612,12964.312457084656,4.345342131273355e-05
869870,6883808,6883808,13767616,12977.069447040558,4.345296474639326e-05
870871,6891812,6891812,13783624,12989.222445964813,4.3452073441585526e-05
871872,6899812,6899812,13799624,13001.835490942001,4.3449590521049686e-05
872873,6907818,6907818,13815636,13014.25734090805,4.344926310295705e-05
873874,6915826,6915826,13831652,13026.708012104034,4.34491867054021e-05
874875,6923832,6923832,13847664,13039.280030965805,4.344746230344754e-05
875876,6931836,6931836,13863672,13051.748080015182,4.344695480540395e-05
876877,6939844,6939844,13879688,13064.317367076874,4.3446882045827806e-05
877878,6947844,6947844,13895688,13077.26681303978,4.3444486436783336e-05
878879,6955846,6955846,13911692,13091.039024829865,4.344324588601012e-05
879880,6963850,6963850,13927700,13104.440226078033,4.344277112977579e-05
880881,6971856,6971856,13943712,13117.640795946121,4.344244734966196e-05
881882,6979860,6979860,13959720,13129.946136951447,4.3441797970444895e-05
882883,6987868,6987868,13975736,13142.037905931473,4.344172339187935e-05
883884,6995872,6995872,13991744,13154.97809100151,4.344040098658297e-05
884885,7003876,7003876,14007752,13167.525307893753,4.344029366620816e-05
885886,7011878,7011878,14023756,13180.471816062927,4.3439238652354106e-05
886887,7019884,7019884,14039768,13194.218608856201,4.343909859017003e-05
887888,7027884,7027884,14055768,13206.680840015411,4.3432810343801975e-05
888889,7035884,7035884,14071768,13219.063599824905,4.3431091398815624e-05
889890,7043890,7043890,14087780,13231.363952875137,4.343075488577597e-05
890891,7051892,7051892,14103784,13244.174374818802,4.3429747165646404e-05
891892,7059898,7059898,14119796,13256.614900112152,4.342919601185713e-05
892893,7067904,7067904,14135808,13268.954445838928,4.342886131780688e-05
893894,7075910,7075910,14151820,13280.849478960037,4.3428224671515636e-05
894895,7083914,7083914,14167828,13292.840643167496,4.34278463217197e-05
895896,7091918,7091918,14183836,13306.400995969772,4.342745342000853e-05
896897,7099922,7099922,14199844,13318.250848054886,4.342642750998493e-05
897898,7107924,7107924,14215848,13331.432574987411,4.34256908192765e-05
898899,7115930,7115930,14231860,13344.23004078865,4.3425387048046105e-05
899900,7123932,7123932,14247864,13355.893873929977,4.342313150118571e-05
900901,7131934,7131934,14263868,13368.544867753983,4.3422196540632285e-05
901902,7139938,7139938,14279876,13380.904015779495,4.342147076386027e-05
902903,7147944,7147944,14295888,13392.054584741592,4.342104512033984e-05
903904,7155948,7155948,14311896,13403.773056983948,4.342050124250818e-05
904905,7163952,7163952,14327904,13415.876689910889,4.3419411667855456e-05
905906,7171954,7171954,14343908,13428.41902589798,4.3417498091002926e-05
906907,7179960,7179960,14359920,13441.07817697525,4.341720159573015e-05
907908,7187964,7187964,14375928,13453.278559923172,4.341647945693694e-05
908909,7195968,7195968,14391936,13466.205044984818,4.341570820542984e-05
909910,7203974,7203974,14407948,13479.697678804398,4.341542626207229e-05
910911,7211982,7211982,14423964,13491.603130817413,4.341534622653853e-05
911912,7219984,7219984,14439968,13504.393987894058,4.341442581790034e-05
912913,7227992,7227992,14455984,13519.857613801956,4.341434942034539e-05
913914,7235392,7235392,14470784,13531.592653751373,4.341268868301995e-05
914915,7243386,7243386,14486772,13544.37918996811,4.341220483183861e-05
915916,7251384,7251384,14502768,13555.975635051727,4.341181193012744e-05
916917,7259386,7259386,14518772,13567.494168758392,4.3411388105596416e-05
917918,7267390,7267390,14534780,13580.286394834518,4.3410227590356953e-05
918919,7275394,7275394,14550788,13592.625545024872,4.340974737715442e-05
919920,7283392,7283392,14566784,13604.369197845459,4.340895429777447e-05
920921,7291398,7291398,14582796,13615.99936580658,4.3408719648141414e-05
921922,7299402,7299402,14598804,13628.24512887001,4.340808118286077e-05
922923,7307408,7307408,14614816,13641.845431089401,4.3407853809185326e-05
923924,7315414,7315414,14630828,13655.43402504921,4.340761915955227e-05
924925,7323418,7323418,14646836,13668.406026124954,4.340759005572181e-05
925926,7331420,7331420,14662840,13679.977890729904,4.340715895523317e-05
926927,7339420,7339420,14678840,13692.455008983612,4.340629493526649e-05
927928,7347420,7347420,14694840,13704.591820001602,4.340558734838851e-05
928929,7355420,7355420,14710840,13716.922101020813,4.34049670730019e-05
929930,7363422,7363422,14726844,13728.77842593193,4.340454870543908e-05
930931,7371426,7371426,14742852,13740.805862903595,4.3404328607721254e-05
931932,7379428,7379428,14758856,13752.169239997864,4.3403651943663135e-05
932933,7387432,7387432,14774864,13763.51307797432,4.34034282079665e-05
933934,7395434,7395434,14790868,13776.763675928116,4.340294799476396e-05
934935,7403440,7403440,14806880,13789.88859295845,4.340272607805673e-05
935936,7411440,7411440,14822880,13803.600567102432,4.340180930739734e-05
936937,7419444,7419444,14838888,13816.309986829758,4.3401430957601406e-05
937938,7427446,7427446,14854892,13828.083345890045,4.3401219954830594e-05
938939,7435452,7435452,14870904,13839.338204860687,4.34010162280174e-05
939940,7443456,7443456,14886912,13851.715706825256,4.3400748836575076e-05
940941,7451460,7451460,14902920,13863.348667860031,4.340025952842552e-05
941942,7459466,7459466,14918932,13876.380854129791,4.339964289101772e-05
942943,7467470,7467470,14934940,13889.137466907501,4.3399297283031046e-05
943944,7475474,7475474,14950948,13901.654238939285,4.339815677667502e-05
944945,7483476,7483476,14966952,13914.627781867981,4.3397758417995647e-05
945946,7491480,7491480,14982960,13927.069828987122,4.3397218178142793e-05
946947,7499482,7499482,14998964,13940.782978057861,4.3396561522968113e-05
947948,7507488,7507488,15014976,13952.792669057846,4.339647421147674e-05
948949,7515490,7515490,15030980,13965.299055814743,4.339569204603322e-05
949950,7523498,7523498,15046996,13978.885556936264,4.339564293331932e-05
950951,7531494,7531494,15062988,13994.516617059708,4.3393658415880054e-05
951952,7539496,7539496,15078992,14006.626850128174,4.339333463576622e-05
952953,7547504,7547504,15095008,14018.874220132828,4.339328734204173e-05
953954,7555504,7555504,15111008,14031.349503040314,4.339151564636268e-05
954955,7563506,7563506,15127012,14044.78676199913,4.3389492930145934e-05
955956,7571510,7571510,15143020,14056.324828863144,4.338900907896459e-05
956957,7579516,7579516,15159032,14067.857383012772,4.338887447374873e-05
957958,7587520,7587520,15175040,14080.759607076645,4.3388616177253425e-05
958959,7595524,7595524,15191048,14092.575716972351,4.338777580414899e-05
959960,7603530,7603530,15207060,14105.393985033035,4.338774306233972e-05
960961,7611534,7611534,15223068,14118.302013874054,4.338723010732792e-05
961962,7619538,7619538,15239076,14130.832818984985,4.338685539551079e-05
962963,7627540,7627540,15255080,14143.54448390007,4.3386435208958574e-05
963964,7635544,7635544,15271088,14155.870110034943,4.338620783528313e-05
964965,7643548,7643548,15287096,14167.52370095253,4.338529106462374e-05
965966,7651552,7651552,15303104,14180.279592037201,4.3385118260630406e-05
966967,7659558,7659558,15319116,14193.734405994415,4.338457256380934e-05
967968,7667560,7667560,15335120,14205.359507083893,4.338372127676848e-05
968969,7675564,7675564,15351128,14217.451033830643,4.338369035394862e-05
969970,7683570,7683570,15367140,14229.88090801239,4.3383455704315566e-05
970971,7691570,7691570,15383140,14242.750043869019,4.338202779763378e-05
971972,7699572,7699572,15399144,14256.297116041183,4.3380192437325604e-05
972973,7707576,7707576,15415152,14269.222537994385,4.338005601312034e-05
973974,7715578,7715578,15431156,14282.917984008789,4.337889913585968e-05
974975,7723582,7723582,15447164,14294.878370761871,4.337825521361083e-05
975976,7731586,7731586,15463172,14308.45861005783,4.3378058762755245e-05
976977,7739588,7739588,15479176,14320.889060974121,4.337755854066927e-05
977978,7747590,7747590,15495180,14333.10948586464,4.337716927693691e-05
978979,7755592,7755592,15511184,14345.908413887024,4.3376658140914515e-05
979980,7763304,7763304,15526608,14359.862401008606,3.829822162515484e-05
980981,7771302,7771302,15542604,14373.060348033905,3.829777233477216e-05
981982,7779304,7779304,15558608,14386.333557128906,3.829737761407159e-05
982983,7787306,7787306,15574612,14398.906306028366,3.829709748970345e-05
983984,7795308,7795308,15590616,14411.830615997314,3.8296573620755225e-05
984985,7803312,7803312,15606624,14423.778312921524,3.829605338978581e-05
985986,7811316,7811316,15622632,14436.628542900085,3.829554952972103e-05
986987,7819320,7819320,15638640,14449.16763806343,3.8295285776257515e-05
987988,7827324,7827324,15654648,14461.559640169144,3.829488377959933e-05
988989,7835328,7835328,15670656,14474.140588998795,3.8293726902338676e-05
989990,7843332,7843332,15686664,14486.581846952438,3.829323759418912e-05
990991,7851338,7851338,15702676,14499.4039208889,3.829315937764477e-05
991992,7859334,7859334,15718668,14511.509483098984,3.8290150769171305e-05
992993,7867338,7867338,15734676,14523.539192914963,3.828949593298603e-05
993994,7875344,7875344,15750688,14535.310198068619,3.828935950878076e-05
994995,7883344,7883344,15766688,14547.280365943909,3.828837907349225e-05
995996,7891352,7891352,15782704,14559.146865844727,3.828833359875716e-05
996997,7899356,7899356,15798712,14571.26872086525,3.8287493225652725e-05
997998,7907362,7907362,15814724,14583.39840888977,3.828737135336269e-05
998999,7915352,7915352,15830704,14596.655728816986,3.827371801889967e-05
1000000,7923356,7923356,15846712,14609.249511003494,3.827304135484155e-05


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.0007541179656982422,848.1427353403399
28,58,29,87,0.027872085571289062,62.9785207281368
55,112,56,168,0.0475161075592041,54.08712962900722
83,168,84,252,0.0693511962890625,50.44031887741676
111,224,112,336,0.08897113800048828,47.81801451262527
139,280,140,420,0.10674524307250977,45.73767180609639
166,334,167,501,0.125413179397583,43.01569059937947
194,390,195,585,0.14530301094055176,41.32841072373549
222,446,223,669,0.16881918907165527,39.63842301050522
249,500,250,750,0.19244003295898438,37.43437196943228
277,556,278,834,0.21297812461853027,36.02296302893592
305,612,306,918,0.23708319664001465,34.663163670765925
332,666,333,999,0.2603950500488281,33.35483586732539
360,722,361,1083,0.2879030704498291,32.112270620477375
388,778,389,1167,0.31032228469848633,31.14301324740495
416,834,417,1251,0.3396260738372803,29.9049479763205
443,888,444,1332,0.3611431121826172,29.110408485795915
471,944,472,1416,0.387911319732666,28.168331680457413
499,1000,500,1500,0.41123104095458984,27.293755769228483
526,1054,527,1581,0.4339640140533447,26.56888695102839
554,1110,555,1665,0.45282816886901855,25.81195523052247
582,1166,583,1749,0.4752650260925293,25.01229219333368
610,1222,611,1833,0.4978921413421631,24.278415489758117
637,1276,638,1914,0.517747163772583,23.710236182238532
665,1332,666,1998,0.5412211418151855,22.869710564221123
693,1388,694,2082,0.562333345413208,22.296544512702212
720,1442,721,2163,0.5876290798187256,21.741147679447977
748,1498,749,2247,0.6129472255706787,21.125168196835602
776,1554,777,2331,0.6397240161895752,20.58861788311674
803,1608,804,2412,0.6614241600036621,20.1106513522991
831,1664,832,2496,0.691115140914917,19.478609929034747
859,1720,860,2580,0.7135300636291504,19.086483057199075
887,1776,888,2664,0.7416760921478271,18.59882410197565
914,1830,915,2745,0.7599589824676514,18.09824517795232
942,1886,943,2829,0.7899692058563232,17.656307852144664
970,1942,971,2913,0.8138501644134521,17.21000513088393
997,1996,998,2994,0.8396971225738525,16.830750287960882
1025,2052,1026,3078,0.8605010509490967,16.370067496020056
1053,2108,1054,3162,0.8853302001953125,15.914391900723672
1080,2162,1081,3243,0.9048969745635986,15.586359335893121
1108,2218,1109,3327,0.9290130138397217,15.123075582424804
1136,2274,1137,3411,0.9534091949462891,14.759768984733682
1164,2330,1165,3495,0.9793891906738281,14.391866584223067
1191,2384,1192,3576,1.0035440921783447,14.055229421168406
1219,2440,1220,3660,1.0293681621551514,13.666414132949285
1247,2496,1248,3744,1.05134916305542,13.338787395585655
1274,2550,1275,3825,1.072033166885376,12.97936002973779
1302,2606,1303,3909,1.096764326095581,12.69275364453415
1330,2662,1331,3993,1.118096113204956,12.39773409934537
1358,2718,1359,4077,1.1422131061553955,12.100561865667942
1385,2772,1386,4158,1.161945104598999,11.763971178456472
1413,2828,1414,4242,1.1851892471313477,11.493092600531327
1441,2884,1442,4326,1.2156710624694824,11.18170053347069
1468,2938,1469,4407,1.241936206817627,10.938399802216736
1496,2994,1497,4491,1.2624702453613281,10.690158432390035
1524,3050,1525,4575,1.28999924659729,10.406784462091537
1551,3104,1552,4656,1.3100993633270264,10.16194930722395
1579,3160,1580,4740,1.3384771347045898,9.922262942234738
1607,3216,1608,4824,1.3609051704406738,9.671782730840278
1635,3272,1636,4908,1.3822941780090332,9.489333558555245
1662,3326,1663,4989,1.4068472385406494,9.26062684169608
1690,3382,1691,5073,1.4354681968688965,9.046359510964976
1718,3438,1719,5157,1.4568822383880615,8.795828827192963
1745,3492,1746,5238,1.4759411811828613,8.587777290410486
1773,3548,1774,5322,1.4987640380859375,8.365397199631957
1801,3604,1802,5406,1.5181550979614258,8.171766451319854
1829,3660,1830,5490,1.5394291877746582,7.961504883600128
1856,3714,1857,5571,1.557967185974121,7.772093108553008
1884,3770,1885,5655,1.5758731365203857,7.604615363180187
1912,3826,1913,5739,1.5979411602020264,7.451451584378333
1939,3880,1940,5820,1.6171209812164307,7.27314990262812
1967,3936,1968,5904,1.6408910751342773,7.083838351395798
1995,3992,1996,5988,1.6602232456207275,6.940368190290997
2022,4046,2023,6069,1.679152250289917,6.7936718899459265
2050,4102,2051,6153,1.7029411792755127,6.642920606674579
2078,4158,2079,6237,1.7283201217651367,6.489029000869209
2106,4214,2107,6321,1.7579162120819092,6.360667965209359
2133,4268,2134,6402,1.7862040996551514,6.216809083711951
2161,4324,2162,6486,1.8117141723632812,6.043094573864096
2189,4380,2190,6570,1.8402869701385498,5.916810670858922
2216,4434,2217,6651,1.8651020526885986,5.768203951020723
2244,4490,2245,6735,1.889336109161377,5.648015565805849
2272,4546,2273,6819,1.912363052368164,5.51768675875303
2299,4600,2300,6900,1.9360101222991943,5.388995710716131
2327,4656,2328,6984,1.9595072269439697,5.27248492617332
2355,4712,2356,7068,1.9828600883483887,5.161338424568612
2383,4768,2384,7152,2.003826141357422,5.036150162889953
2410,4822,2411,7233,2.0267152786254883,4.928494558631428
2438,4878,2439,7317,2.0496041774749756,4.821204667270763
2466,4934,2467,7401,2.069819211959839,4.714834846503322
2493,4988,2494,7482,2.0919251441955566,4.604259396444718
2521,5044,2522,7566,2.1168551445007324,4.505424804495988
2549,5100,2550,7650,2.143430233001709,4.374935722466262
2577,5156,2578,7734,2.165928363800049,4.278392448825571
2604,5210,2605,7815,2.1917293071746826,4.19288551206273
2632,5266,2633,7899,2.2177860736846924,4.103881519381503
2660,5322,2661,7983,2.242631196975708,4.005607600030771
2687,5376,2688,8064,2.259593963623047,3.925759419023734
2715,5432,2716,8148,2.2858030796051025,3.843844862392416
2743,5488,2744,8232,2.3113882541656494,3.74975078780642
2770,5542,2771,8313,2.3364832401275635,3.6724037756241614
2798,5598,2799,8397,2.35707426071167,3.5987788214595184
2826,5654,2827,8481,2.3781871795654297,3.5154606424553094
2854,5710,2855,8565,2.4029953479766846,3.4500955670428084
2881,5764,2882,8646,2.426405191421509,3.36528787235045
2909,5820,2910,8730,2.452336072921753,3.279679178230367
2937,5876,2938,8814,2.473421096801758,3.191057992460742
2964,5930,2965,8895,2.494589328765869,3.124343806610682
2992,5986,2993,8979,2.5171780586242676,3.046801280378645
3020,6042,3021,9063,2.54404616355896,2.9785401346276785
3048,6098,3049,9147,2.5676021575927734,2.918059458103812
3075,6152,3076,9228,2.5958609580993652,2.852750058508377
3103,6208,3104,9312,2.6198971271514893,2.796880845954547
3131,6264,3132,9396,2.646818161010742,2.731537533055757
3158,6318,3159,9477,2.667677164077759,2.6757269538330775
3186,6374,3187,9561,2.6947813034057617,2.6149809638875467
3214,6430,3215,9645,2.7159311771392822,2.5604816274740188
3241,6484,3242,9726,2.7406063079833984,2.496592492695754
3269,6540,3270,9810,2.7714290618896484,2.4400812695192826
3297,6596,3298,9894,2.795133352279663,2.38986884892347
3325,6652,3326,9978,2.818082094192505,2.340611723425468
3352,6706,3353,10059,2.843513250350952,2.293429170645254
3380,6762,3381,10143,2.865770101547241,2.2476892737659
3408,6818,3409,10227,2.8919801712036133,2.2013732748529264
3435,6872,3436,10308,2.914130210876465,2.161049728314879
3463,6928,3464,10392,2.937425136566162,2.112691846804182
3491,6984,3492,10476,2.9662342071533203,2.0670714791787077
3518,7038,3519,10557,2.9923250675201416,2.01704351806427
3546,7094,3547,10641,3.016613245010376,1.9799226080664312
3574,7150,3575,10725,3.04260516166687,1.931849975170394
3602,7206,3603,10809,3.066373109817505,1.8995391219154953
3629,7260,3630,10890,3.0908942222595215,1.861644925508699
3657,7316,3658,10974,3.1124751567840576,1.8175810471751674
3685,7372,3686,11058,3.138500213623047,1.781051397787337
3712,7426,3713,11139,3.161234140396118,1.7481321899771274
3740,7482,3741,11223,3.18624210357666,1.714150949594
3768,7538,3769,11307,3.207332134246826,1.6771094496625665
3796,7594,3797,11391,3.2335453033447266,1.6430176179939053
3823,7648,3824,11472,3.2517030239105225,1.6122366601410931
3851,7704,3852,11556,3.273480176925659,1.5657950181331444
3879,7760,3880,11640,3.295208215713501,1.5344477636540432
3906,7814,3907,11721,3.316620111465454,1.4926852773064638
3934,7870,3935,11805,3.340567111968994,1.4633175988759604
3962,7926,3963,11889,3.362133026123047,1.4331852166893668
3989,7980,3990,11970,3.3862762451171875,1.4037953376362111
4017,8036,4018,12054,3.41154408454895,1.3819495653198146
4045,8092,4046,12138,3.43974232673645,1.3511405421105565
4073,8148,4074,12222,3.4674339294433594,1.3191313449184463
4100,8202,4101,12303,3.4952480792999268,1.2931968569864694
4128,8258,4129,12387,3.5296173095703125,1.2695835780074276
4156,8314,4157,12471,3.5610973834991455,1.233425365253197
4183,8368,4184,12552,3.5961501598358154,1.2089709635509962
4211,8424,4212,12636,3.6360931396484375,1.1838466426237346
4239,8480,4240,12720,3.6751911640167236,1.15748345786983
4267,8536,4268,12804,3.7121100425720215,1.1380132238612077
4294,8590,4295,12885,3.749972343444824,1.110501750980461
4322,8646,4323,12969,3.7891101837158203,1.085870126916916
4350,8702,4351,13053,3.8266661167144775,1.0619125173186603
4377,8756,4378,13134,3.868129014968872,1.039679957549538
4405,8812,4406,13218,3.9334051609039307,1.018579682026484
4433,8868,4434,13302,3.997619152069092,0.9979220562618139
4460,8922,4461,13383,4.0366621017456055,0.9758771161091317
4488,8978,4489,13467,4.066941261291504,0.9565635480043966
4516,9034,4517,13551,4.099197149276733,0.9366270217748252
4544,9090,4545,13635,4.141613006591797,0.9153423845207271
4571,9144,4572,13716,4.172988176345825,0.8986206988797676
4599,9200,4600,13800,4.208719253540039,0.8800657217118442
4627,9256,4628,13884,4.240479946136475,0.8618623049831058
4654,9310,4655,13965,4.269463062286377,0.8461200866669287
4682,9366,4683,14049,4.300256967544556,0.8266359372789793
4710,9422,4711,14133,4.331299066543579,0.810359869730064
4738,9478,4739,14217,4.38027811050415,0.792284592380156
4765,9532,4766,14298,4.4127891063690186,0.7786977914543058
4793,9588,4794,14382,4.444561243057251,0.7604912154821477
4821,9644,4822,14466,4.477039098739624,0.7447394254977553
4848,9698,4849,14547,4.508830308914185,0.7308812422052142
4876,9754,4877,14631,4.542116165161133,0.7152780298853259
4904,9810,4905,14715,4.57656717300415,0.7018370061218775
4931,9864,4932,14796,4.606893062591553,0.690227642382979
4959,9920,4960,14880,4.640318155288696,0.6759268617292946
4987,9976,4988,14964,4.671295404434204,0.6618985247292812
5015,10032,5016,15048,4.70070219039917,0.6496330033709228
5042,10086,5043,15129,4.724452257156372,0.6364550819042734
5070,10142,5071,15213,4.748804092407227,0.6240414297269581
5098,10198,5099,15297,4.7733540534973145,0.6101240118297255
5125,10252,5126,15378,4.799408197402954,0.5989210909486928
5153,10308,5154,15462,4.825534343719482,0.5850987584852874
5181,10364,5182,15546,4.850808143615723,0.5733277946044382
5208,10418,5209,15627,4.877289295196533,0.5590503633524122
5236,10474,5237,15711,4.904937267303467,0.5479305739246456
5264,10530,5265,15795,4.928648233413696,0.536087058150656
5292,10586,5293,15879,4.954827070236206,0.525386760375909
5319,10640,5320,15960,4.985384225845337,0.5148848336472156
5347,10696,5348,16044,5.014208078384399,0.5036473356539091
5375,10752,5376,16128,5.041919946670532,0.4946276680042274
5402,10806,5403,16209,5.067045211791992,0.48440321439943546
5430,10862,5431,16293,5.098858118057251,0.47387671302351464
5458,10918,5459,16377,5.130134105682373,0.4651176334843967
5486,10974,5487,16461,5.156344175338745,0.45564570950944017
5513,11028,5514,16542,5.1850481033325195,0.44844240394741064
5541,11084,5542,16626,5.217642068862915,0.4387525107675856
5569,11140,5570,16710,5.249446153640747,0.43051012389344123
5596,11194,5597,16791,5.2780983448028564,0.4211646141760639
5624,11250,5625,16875,5.308264255523682,0.41306499670702124
5652,11306,5653,16959,5.3343541622161865,0.4056583221963592
5679,11360,5680,17040,5.358744144439697,0.3981244934186634
5707,11416,5708,17124,5.387263298034668,0.38943822054693555
5735,11472,5736,17208,5.410082101821899,0.3816753974523408
5763,11528,5764,17292,5.438868999481201,0.37309997066711276
5790,11582,5791,17373,5.467315196990967,0.36701250745102243
5818,11638,5819,17457,5.49651312828064,0.3593452125899148
5846,11694,5847,17541,5.526661157608032,0.3522645034369134
5873,11748,5874,17622,5.553770065307617,0.3449312239298479
5901,11804,5902,17706,5.584686040878296,0.33876234077433764
5929,11860,5930,17790,5.608465194702148,0.33210397992741036
5957,11916,5958,17874,5.632411241531372,0.3243177599701994
5984,11970,5985,17955,5.658111333847046,0.3181306990752546
6012,12026,6013,18039,5.687489986419678,0.3114557632957258
6040,12082,6041,18123,5.716582298278809,0.3079543799773319
6067,12136,6068,18204,5.74631404876709,0.2994189916317964
6095,12192,6096,18288,5.773771047592163,0.29377831832175616
6123,12248,6124,18372,5.802634954452515,0.28807808652436506
6150,12302,6151,18453,5.823675155639648,0.28248756085395144
6178,12358,6179,18537,5.851465225219727,0.2765581061329385
6206,12414,6207,18621,5.877790927886963,0.27078235426631636
6234,12470,6235,18705,5.903419256210327,0.2656082016322898
6261,12524,6262,18786,5.932351350784302,0.2601573828879964
6289,12580,6290,18870,5.958473205566406,0.2552990384087934
6317,12636,6318,18954,5.989652395248413,0.2508066023339097
6344,12690,6345,19035,6.01829719543457,0.24572889525632036
6372,12746,6373,19119,6.049241065979004,0.24154529231157085
6400,12802,6401,19203,6.080609083175659,0.23635272679314312
6427,12856,6428,19284,6.109547138214111,0.23208876855778726
6455,12912,6456,19368,6.140810966491699,0.22746106789509213
6483,12968,6484,19452,6.183608055114746,0.22340052596246096
6511,13024,6512,19536,6.2145020961761475,0.21942967463053265
6538,13078,6539,19617,6.239042043685913,0.21515663927038986
6566,13134,6567,19701,6.2668352127075195,0.21120681794150187
6594,13190,6595,19785,6.2920050621032715,0.20740848820025803
6621,13244,6622,19866,6.319305181503296,0.20395381664422985
6649,13300,6650,19950,6.346409320831299,0.1997843792007643
6677,13356,6678,20034,6.373592138290405,0.19594407864497043
6705,13412,6706,20118,6.409592151641846,0.19109108514135187
6732,13466,6733,20199,6.43633508682251,0.18735237862426857
6760,13522,6761,20283,6.46246337890625,0.18369031109784828
6788,13578,6789,20367,6.49076509475708,0.1798549543173067
6815,13632,6816,20448,6.515305995941162,0.17683639075130486
6843,13688,6844,20532,6.542750358581543,0.17300320881338394
6871,13744,6872,20616,6.57021427154541,0.1698205252663456
6898,13798,6899,20697,6.596320152282715,0.16690578694488067
6926,13854,6927,20781,6.624206066131592,0.16373416980025013
6954,13910,6955,20865,6.651098251342773,0.1605137436519044
6982,13966,6983,20949,6.681046009063721,0.1570411992083791
7009,14020,7010,21030,6.706024169921875,0.15434707572637762
7037,14076,7038,21114,6.734183311462402,0.151199855663549
7065,14132,7066,21198,6.7605881690979,0.14852957772518494
7092,14186,7093,21279,6.7877702713012695,0.14569002082691895
7120,14242,7121,21363,6.815388202667236,0.1426262043544284
7148,14298,7149,21447,6.842389106750488,0.13997194191074414
7176,14354,7177,21531,6.87074613571167,0.1372196775273551
7203,14408,7204,21612,6.89624810218811,0.13493119195470626
7231,14464,7232,21696,6.924584150314331,0.13199867928722142
7259,14520,7260,21780,6.952178239822388,0.1295167494653242
7286,14574,7287,21861,6.981628179550171,0.1270616236965907
7314,14630,7315,21945,7.008795261383057,0.12466572475000248
7342,14686,7343,22029,7.037944078445435,0.12239162012338056
7369,14740,7370,22110,7.065275192260742,0.11980869808485295
7397,14796,7398,22194,7.09419322013855,0.11800736456962113
7425,14852,7426,22278,7.1249840259552,0.11566989816708428
7453,14908,7454,22362,7.149729013442993,0.11305555183014349
7480,14962,7481,22443,7.177881240844727,0.1110453024537037
7508,15018,7509,22527,7.204951047897339,0.10905818604680917
7536,15074,7537,22611,7.237300395965576,0.10699033915545897
7563,15128,7564,22692,7.264734268188477,0.10544569393596248
7591,15184,7592,22776,7.290753126144409,0.10321443973941768
7619,15240,7620,22860,7.31657600402832,0.10104472410307608
7646,15294,7647,22941,7.339034080505371,0.09935963413727222
7674,15350,7675,23025,7.365571022033691,0.0971814264224804
7702,15406,7703,23109,7.39338231086731,0.09527506298240951
7730,15462,7731,23193,7.417602062225342,0.09346428158391973
7757,15516,7758,23274,7.444220304489136,0.09178086915312633
7785,15572,7786,23358,7.473144054412842,0.090005409327091
7813,15628,7814,23442,7.4991700649261475,0.08800690269231382
7840,15682,7841,23523,7.5270631313323975,0.08646001056069963
7868,15738,7869,23607,7.555288076400757,0.08496733832669179
7896,15794,7897,23691,7.582757234573364,0.08331016120826007
7924,15850,7925,23775,7.610968112945557,0.08158628218313879
7951,15904,7952,23856,7.638467073440552,0.08006013939586865
7979,15960,7980,23940,7.667974233627319,0.07851072892935917
8007,16016,8008,24024,7.698706150054932,0.07687027742667851
8034,16070,8035,24105,7.728804111480713,0.07564242095895679
8062,16126,8063,24189,7.7567222118377686,0.07423216284291811
8090,16182,8091,24273,7.784558057785034,0.07276935545792185
8117,16236,8118,24354,7.812218189239502,0.0714859897855149
8145,16292,8146,24438,7.841609954833984,0.07009680877320079
8173,16348,8174,24522,7.868368148803711,0.06864930902963806
8201,16404,8202,24606,7.900987148284912,0.06734459178346697
8228,16458,8229,24687,7.940467357635498,0.06617213769527552
8256,16514,8257,24771,7.966590166091919,0.06489445725424048
8284,16570,8285,24855,7.996625185012817,0.06383517718336407
8311,16624,8312,24936,8.024496078491211,0.06259848684692315
8339,16680,8340,25020,8.051894187927246,0.06141564735889915
8367,16736,8368,25104,8.080941200256348,0.060269989042126326
8395,16792,8396,25188,8.107566118240356,0.05909873027201229
8422,16846,8423,25269,8.143607139587402,0.057873103584825
8450,16902,8451,25353,8.171893119812012,0.0568134611099822
8478,16958,8479,25437,8.200618028640747,0.0557904156830773
8505,17012,8506,25518,8.229648113250732,0.054704573688013625
8533,17068,8534,25602,8.258805990219116,0.05368323502318617
8561,17124,8562,25686,8.287060260772705,0.05270092253351777
8588,17178,8589,25767,8.315822124481201,0.05180789837561406
8616,17234,8617,25851,8.345954179763794,0.05081672515404989
8644,17290,8645,25935,8.373959302902222,0.05026483001518045
8672,17346,8673,26019,8.40185022354126,0.0489143769424345
8699,17400,8700,26100,8.431100130081177,0.047978939613017246
8727,17456,8728,26184,8.458436250686646,0.04711416331474538
8755,17512,8756,26268,8.485572099685669,0.04625088183524895
8782,17566,8783,26349,8.514223098754883,0.04547922164579177
8810,17622,8811,26433,8.540209293365479,0.04460048487851509
8838,17678,8839,26517,8.56876516342163,0.04377063290667138
8866,17734,8867,26601,8.593563079833984,0.042953574163561825
8893,17788,8894,26682,8.618652105331421,0.042175552225785395
8921,17844,8922,26766,8.645879030227661,0.041457580181827325
8949,17900,8950,26850,8.673803091049194,0.04064700420781264
8976,17954,8977,26931,8.700744152069092,0.03983878457790979
9004,18010,9005,27015,8.730082035064697,0.039097795582279105
9032,18066,9033,27099,8.758937120437622,0.03841230515854477
9059,18120,9060,27180,8.780961990356445,0.037656009157103654
9087,18176,9088,27264,8.809125185012817,0.03691393659460118
9115,18232,9116,27348,8.8353111743927,0.03624804182152275
9143,18288,9144,27432,8.861115217208862,0.03550422795160557
9170,18342,9171,27513,8.887612104415894,0.03489837335007451
9198,18398,9199,27597,8.914819240570068,0.03421070959461758
9226,18454,9227,27681,8.941171169281006,0.03354449749929245
9253,18508,9254,27762,8.964392185211182,0.03292670596408698
9281,18564,9282,27846,8.99210810661316,0.03232874685511433
9309,18620,9310,27930,9.020501136779785,0.03177889001551648
9336,18674,9337,28011,9.048687219619751,0.0311238437755037
9364,18730,9365,28095,9.078456163406372,0.030493538557720967
9392,18786,9393,28179,9.107745170593262,0.029905441075356975
9420,18842,9421,28263,9.135643243789673,0.029218273140600104
9447,18896,9448,28344,9.16053819656372,0.028668189959716983
9475,18952,9476,28428,9.188784122467041,0.028141415776303802
9503,19008,9504,28512,9.213098049163818,0.02762516075745225
9530,19062,9531,28593,9.23681926727295,0.0271185895534245
9558,19118,9559,28677,9.265273094177246,0.02667414999416451
9586,19174,9587,28761,9.289067029953003,0.026147805754703768
9614,19230,9615,28845,9.315514087677002,0.025659909137402792
9641,19284,9642,28926,9.341468334197998,0.025251208634472277
9669,19340,9670,29010,9.366173267364502,0.02476047120342173
9697,19396,9698,29094,9.394100189208984,0.02442449007310188
9724,19450,9725,29175,9.422119140625,0.02389037826446838
9752,19506,9753,29259,9.450075149536133,0.023387890877870632
9780,19562,9781,29343,9.478881120681763,0.02292294312951526
9807,19616,9808,29424,9.503732204437256,0.022549758771674533
9835,19672,9836,29508,9.53240418434143,0.022138989673408105
9863,19728,9864,29592,9.559676170349121,0.021688310679564893
9891,19784,9892,29676,9.588720083236694,0.02132692581540141
9918,19838,9919,29757,9.61478328704834,0.02090360022691584
9946,19894,9947,29841,9.651864051818848,0.020544179296962284
9974,19950,9975,29925,9.679033041000366,0.020107732270730594
10001,20004,10002,30006,9.703642129898071,0.019755908447109505
10029,20060,10030,30090,9.731635332107544,0.019413764479168094
10057,20116,10058,30174,9.758392095565796,0.019093379691526025
10085,20172,10086,30258,9.786338090896606,0.01875741010701404
10112,20226,10113,30339,9.811901330947876,0.018421848884713654
10140,20282,10141,30423,9.845861196517944,0.018070071138595267
10168,20338,10169,30507,9.871158123016357,0.017703016593259235
10195,20392,10196,30588,9.897144079208374,0.017374468407183485
10223,20448,10224,30672,9.92430830001831,0.01701516574280504
10251,20504,10252,30756,9.94895625114441,0.016716161219733294
10278,20558,10279,30837,9.973603248596191,0.01641897920330848
10306,20614,10307,30921,9.99888825416565,0.016114547697043236
10334,20670,10335,31005,10.025790214538574,0.015795907587857982
10362,20726,10363,31089,10.048740148544312,0.015525675678418338
10389,20780,10390,31170,10.075391292572021,0.015267412898992916
10417,20836,10418,31254,10.102866172790527,0.014985340917064605
10445,20892,10446,31338,10.12938904762268,0.01467682628856437
10472,20946,10473,31419,10.152947187423706,0.014445921836113484
10500,21002,10501,31503,10.178368091583252,0.014165557303613241
10528,21058,10529,31587,10.200932264328003,0.013877459398941028
10555,21112,10556,31668,10.224419116973877,0.013642928307717739
10583,21168,10584,31752,10.247849941253662,0.013388561149895395
10611,21224,10612,31836,10.273009300231934,0.013209073472808086
10639,21280,10640,31920,10.296837091445923,0.01287383510998552
10666,21334,10667,32001,10.320914268493652,0.012653237335598533
10694,21390,10695,32085,10.348509311676025,0.012355745248100902
10722,21446,10723,32169,10.378191232681274,0.0121398840016127
10749,21500,10750,32250,10.403655290603638,0.01188898523230364
10777,21556,10778,32334,10.431331157684326,0.011685010835890353
10805,21612,10806,32418,10.456984043121338,0.011438412213465199
10833,21668,10834,32502,10.484262228012085,0.011233861897267161
10860,21722,10861,32583,10.506540060043335,0.011058411448971128
10888,21778,10889,32667,10.532646179199219,0.01081197981011428
10916,21834,10917,32751,10.556749105453491,0.010623916814097356
10943,21888,10944,32832,10.578893184661865,0.010443653739002912
10971,21944,10972,32916,10.604942083358765,0.010244831408272148
10999,22000,11000,33000,10.629993200302124,0.010011277839453214
11026,22054,11027,33081,10.652830362319946,0.009855904899268353
11054,22110,11055,33165,10.681917190551758,0.009678328848281126
11082,22166,11083,33249,10.709084272384644,0.009473877031723532
11110,22222,11111,33333,10.736906051635742,0.009283286975460214
11137,22276,11138,33414,10.763917207717896,0.00910568989274907
11165,22332,11166,33498,10.789997100830078,0.00893972595190462
11193,22388,11194,33582,10.814517974853516,0.0087984648374686
11220,22442,11221,33663,10.83947229385376,0.00862347187432988
11248,22498,11249,33747,10.865342378616333,0.008497609230971648
11276,22554,11277,33831,10.893601179122925,0.008283114295977612
11304,22610,11305,33915,10.918837070465088,0.008132351279073191
11331,22664,11332,33996,10.941429138183594,0.007971428318569451
11359,22720,11360,34080,10.966848134994507,0.007812770838768301
11387,22776,11388,34164,10.99337911605835,0.007674038366417335
11414,22830,11415,34245,11.019044160842896,0.00754855530635723
11442,22886,11443,34329,11.043788194656372,0.007413091637772595
11470,22942,11471,34413,11.067917108535767,0.00727898224602086
11497,22996,11498,34494,11.092756986618042,0.007160927448808252
11525,23052,11526,34578,11.117375373840332,0.007032522906229133
11553,23108,11554,34662,11.142545223236084,0.006904779421802232
11581,23164,11582,34746,11.168327331542969,0.006775902129561473
11608,23218,11609,34827,11.194935083389282,0.0066569392217843415
11636,23274,11637,34911,11.221460342407227,0.0065467100157547975
11664,23330,11665,34995,11.248265266418457,0.0064196003361303156
11691,23384,11692,35076,11.276602268218994,0.006297978671341298
11719,23440,11720,35160,11.310823202133179,0.006191364328287818
11747,23496,11748,35244,11.33568525314331,0.0060705555248432574
11774,23550,11775,35325,11.35779619216919,0.005960226465390406
11802,23606,11803,35409,11.384268045425415,0.0058568297181409434
11830,23662,11831,35493,11.408149003982544,0.005758636874588774
11858,23718,11859,35577,11.430946111679077,0.005654514479942918
11885,23772,11886,35658,11.451589107513428,0.005563314650089524
11913,23828,11914,35742,11.47514820098877,0.0054494514615726075
11941,23884,11942,35826,11.507597208023071,0.005348808073335931
11968,23938,11969,35907,11.535240173339844,0.005251911181403557
11996,23994,11997,35991,11.558746099472046,0.005163814566117253
12024,24050,12025,36075,11.584134101867676,0.005069562366543323
12052,24106,12053,36159,11.607579231262207,0.004967620350271318
12079,24160,12080,36240,11.631842136383057,0.004882100674649337
12107,24216,12108,36324,11.654685258865356,0.004789003208884424
12135,24272,12136,36408,11.679461240768433,0.004698945644804553
12162,24326,12163,36489,11.705031156539917,0.004616364123535277
12190,24382,12191,36573,11.72990894317627,0.0045332488632539025
12218,24438,12219,36657,11.756989240646362,0.004443347414735399
12245,24492,12246,36738,11.779288053512573,0.004366560649373241
12273,24548,12274,36822,11.802694082260132,0.0042939918532738375
12301,24604,12302,36906,11.825706958770752,0.004212064109424318
12329,24660,12330,36990,11.850353240966797,0.004132697908630689
12356,24714,12357,37071,11.87250018119812,0.004036077957039197
12384,24770,12385,37155,11.895758152008057,0.003958004649007307
12412,24826,12413,37239,11.923527240753174,0.0038876010769399727
12439,24880,12440,37320,11.947973251342773,0.003825655805144379
12467,24936,12468,37404,11.971924304962158,0.0037558427980002307
12495,24992,12496,37488,11.994056224822998,0.0036709502185203746
12523,25048,12524,37572,12.018509149551392,0.0036105520399587476
12550,25102,12551,37653,12.041122198104858,0.0035393836483308405
12578,25158,12579,37737,12.06562614440918,0.0034676026832585194
12606,25214,12607,37821,12.090470314025879,0.00339601040332127
12633,25268,12634,37902,12.114280223846436,0.0033338178875510494
12661,25324,12662,37986,12.13633108139038,0.003276454419960828
12689,25380,12690,38070,12.162108182907104,0.003214816239051288
12716,25434,12717,38151,12.185348272323608,0.0031567245235919472
12744,25490,12745,38235,12.210783004760742,0.0030997021721077544
12772,25546,12773,38319,12.23725414276123,0.0030490006378158796
12800,25602,12801,38403,12.264141082763672,0.0029917293669541323
12827,25656,12828,38484,12.290761947631836,0.0029304064084954007
12855,25712,12856,38568,12.31675124168396,0.002874927488960566
12883,25768,12884,38652,12.343955278396606,0.0028258496824946633
12910,25822,12911,38733,12.369264125823975,0.0027694442304664335
12938,25878,12939,38817,12.393898010253906,0.002723388045978936
12966,25934,12967,38901,12.420905351638794,0.002668742191531237
12994,25990,12995,38985,12.44691514968872,0.0026186688728557783
13021,26044,13022,39066,12.472209215164185,0.002574014473339048
13049,26100,13050,39150,12.499651193618774,0.002526244023442814
13077,26156,13078,39234,12.530351161956787,0.0024774910524456573
13104,26210,13105,39315,12.5553719997406,0.0024304486629489475
13132,26266,13133,39399,12.582417249679565,0.002393707117107624
13160,26322,13161,39483,12.610626220703125,0.0023459241484715676
13187,26376,13188,39564,12.635544061660767,0.0023036644219018854
13215,26432,13216,39648,12.66070818901062,0.0022639191830648997
13243,26488,13244,39732,12.686697244644165,0.002219672678961615
13271,26544,13272,39816,12.710216283798218,0.00217924358230448
13298,26598,13299,39897,12.734861135482788,0.0021449375406064064
13326,26654,13327,39981,12.76098108291626,0.002106374964114366
13354,26710,13355,40065,12.787257194519043,0.00206645669095451
13381,26764,13382,40146,12.811132192611694,0.002027527276368346
13409,26820,13410,40230,12.835801124572754,0.0019944218361160893
13437,26876,13438,40314,12.861021280288696,0.0019532263021346807
13464,26930,13465,40395,12.885723114013672,0.0019104986214415476
13492,26986,13493,40479,12.912604331970215,0.0018767463180893174
13520,27042,13521,40563,12.940264225006104,0.0018402836817585921
13548,27098,13549,40647,12.966398239135742,0.0018067761798192805
13575,27152,13576,40728,12.991663217544556,0.0017780421857196416
13603,27208,13604,40812,13.01641321182251,0.0017485735629634291
13631,27264,13632,40896,13.042967081069946,0.0017152663759816278
13658,27318,13659,40977,13.066840171813965,0.0016851465219360762
13686,27374,13687,41061,13.092332124710083,0.001657230416526545
13714,27430,13715,41145,13.11628532409668,0.0016266376159137508
13742,27486,13743,41229,13.143638134002686,0.0015964460636723743
13769,27540,13770,41310,13.174851179122925,0.0015678414488320414
13797,27596,13798,41394,13.20388126373291,0.0015416983395653006
13825,27652,13826,41478,13.226733207702637,0.0015116369460201895
13852,27706,13853,41559,13.250425100326538,0.0014851728416260812
13880,27762,13881,41643,13.274453163146973,0.0014594762537853967
13908,27818,13909,41727,13.295915126800537,0.0014351020624872035
13935,27872,13936,41808,13.317694187164307,0.0014096987363245717
13963,27928,13964,41892,13.33971619606018,0.0013755214714592512
13991,27984,13992,41976,13.36734414100647,0.0013512886259832158
14019,28040,14020,42060,13.39046335220337,0.0013168687778488675
14046,28094,14047,42141,13.411140203475952,0.001294988670906605
14074,28150,14075,42225,13.433037042617798,0.0012716812769895114
14102,28206,14103,42309,13.455631256103516,0.0012486190275922127
14129,28260,14130,42390,13.478150129318237,0.0012286917807386999
14157,28316,14158,42474,13.499829053878784,0.0012070105300381329
14185,28372,14186,42558,13.522906064987183,0.0011843878164654598
14213,28428,14214,42642,13.549633026123047,0.0011613923302320472
14240,28482,14241,42723,13.574531078338623,0.0011435828200774267
14268,28538,14269,42807,13.595169067382812,0.0011227528149220234
14296,28594,14297,42891,13.619397163391113,0.0011004806584651305
14323,28648,14324,42972,13.640095949172974,0.0010817919135206466
14351,28704,14352,43056,13.66241717338562,0.001060374639564543
14379,28760,14380,43140,13.685225248336792,0.0010410932975446485
14406,28814,14407,43221,13.704789161682129,0.0010235986590032553
14434,28870,14435,43305,13.726202249526978,0.0010051432640239
14462,28926,14463,43389,13.746289253234863,0.0009855017866584603
14490,28982,14491,43473,13.7680082321167,0.0009672105151139476
14517,29036,14518,43554,13.790014266967773,0.0009511109362847492
14545,29092,14546,43638,13.81280517578125,0.0009338924860458064
14573,29148,14574,43722,13.833069086074829,0.000916850794851598
14600,29202,14601,43803,13.851853132247925,0.0009016335189926394
14628,29258,14629,43887,13.877360105514526,0.0008815848635777002
14656,29314,14657,43971,13.897704362869263,0.0008648051273212332
14683,29368,14684,44052,13.92150616645813,0.0008494681767388101
14711,29424,14712,44136,13.943263053894043,0.000826369348260414
14739,29480,14740,44220,13.965784072875977,0.0008135907077075899
14767,29536,14768,44304,13.9880952835083,0.0007996155671889937
14794,29590,14795,44385,14.009329319000244,0.0007826018423884307
14822,29646,14823,44469,14.033300399780273,0.0007665089603960951
14850,29702,14851,44553,14.05745816230774,0.0007537257497460814
14877,29756,14878,44634,14.077330350875854,0.0007398570594432385
14905,29812,14906,44718,14.106863260269165,0.0007287284091717083
14933,29868,14934,44802,14.128763198852539,0.0007141684625366906
14961,29924,14962,44886,14.148128986358643,0.0007015723402901131
14988,29978,14989,44967,14.171683073043823,0.0006881973185954848
15016,30034,15017,45051,14.192183017730713,0.000675962314858225
15044,30090,15045,45135,14.215455055236816,0.0006613414670937345
15071,30144,15072,45216,14.234999179840088,0.0006492997870282124
15099,30200,15100,45300,14.263405084609985,0.000636319382124384
15127,30256,15128,45384,14.290868997573853,0.0006243787599942152
15154,30310,15155,45465,14.31221604347229,0.0006124074163835758
15182,30366,15183,45549,14.336841344833374,0.0006014546444248481
15210,30422,15211,45633,14.36016321182251,0.0005914830447864006
15238,30478,15239,45717,14.380365133285522,0.0005784404133919452
15265,30532,15266,45798,14.40210509300232,0.0005678405314029078
15293,30588,15294,45882,14.423915147781372,0.0005591269418800948
15321,30644,15322,45966,14.445572137832642,0.0005482029148424772
15348,30698,15349,46047,14.466154098510742,0.0005395258012867998
15376,30754,15377,46131,14.489819288253784,0.0005279487626239643
15404,30810,15405,46215,14.513472080230713,0.0005189078412968229
15432,30866,15433,46299,14.537757158279419,0.0005086703595225117
15459,30920,15460,46380,14.558234214782715,0.0005007111896020433
15487,30976,15488,46464,14.584810018539429,0.0004910240469371274
15515,31032,15516,46548,14.609713315963745,0.00048190439099471405
15542,31086,15543,46629,14.631912231445312,0.0004727724016220236
15570,31142,15571,46713,14.655231952667236,0.0004643354735662797
15598,31198,15599,46797,14.68007516860962,0.00045566651465378527
15625,31252,15626,46878,14.702394247055054,0.0004485513120471296
15653,31308,15654,46962,14.728318214416504,0.00044041345392997755
15681,31364,15682,47046,14.752803087234497,0.0004314531396403254
15709,31420,15710,47130,14.78127408027649,0.00042542648736798583
15736,31474,15737,47211,14.806275129318237,0.00041734906596957444
15764,31530,15765,47295,14.834227323532104,0.0004095927257594667
15792,31586,15793,47379,14.858636140823364,0.0004018921235910966
15819,31640,15820,47460,14.881899118423462,0.000395204226720125
15847,31696,15848,47544,14.903694152832031,0.0003884546925974064
15875,31752,15876,47628,14.92784833908081,0.00038072075085437973
15903,31808,15904,47712,14.9531409740448,0.0003730760987536996
15930,31862,15931,47793,14.973373174667358,0.0003655193271470125
15958,31918,15959,47877,14.998674154281616,0.00035898505677778303
15986,31974,15987,47961,15.021287202835083,0.000352443790234247
16013,32028,16014,48042,15.043866157531738,0.0003468781342235161
16041,32084,16042,48126,15.064213991165161,0.0003404867391054722
16069,32140,16070,48210,15.088024139404297,0.0003333976424073626
16096,32194,16097,48291,15.109080076217651,0.0003280582847082769
16124,32250,16125,48375,15.128584146499634,0.00032111427287873084
16152,32306,16153,48459,15.154659032821655,0.00031515538876192295
16180,32362,16181,48543,15.17943811416626,0.00030843103468214395
16207,32416,16208,48624,15.204667091369629,0.00030305202869840286
16235,32472,16236,48708,15.233350276947021,0.00029672105699773965
16263,32528,16264,48792,15.26200819015503,0.00029047666089354607
16290,32582,16291,48873,15.291398286819458,0.0002848388630809495
16318,32638,16319,48957,15.317901134490967,0.00027859000556418323
16346,32694,16347,49041,15.3475501537323,0.00027371309113277675
16373,32748,16374,49122,15.37631106376648,0.00026901523540345806
16401,32804,16402,49206,15.41103720664978,0.0002640534275997197
16429,32860,16430,49290,15.450969219207764,0.0002595150784827638
16457,32916,16458,49374,15.493372201919556,0.00025526081947191415
16484,32970,16485,49455,15.531009197235107,0.00025128252536887885
16512,33026,16513,49539,15.56016206741333,0.0002457615137245739
16540,33082,16541,49623,15.583781242370605,0.0002414439941276214
16567,33136,16568,49704,15.607931137084961,0.0002367552314126442
16595,33192,16596,49788,15.635333061218262,0.00023238732023855846
16623,33248,16624,49872,15.662265062332153,0.00022821400011707738
16651,33304,16652,49956,15.68855619430542,0.00022434989625708113
16678,33358,16679,50037,15.712406158447266,0.00021991537880694523
16706,33414,16707,50121,15.737910032272339,0.00021626551313147502
16734,33470,16735,50205,15.761220216751099,0.00021199039247221663
16761,33524,16762,50286,15.785994052886963,0.00020773199764789751
16789,33580,16790,50370,15.809305191040039,0.00020421541364612494
16817,33636,16818,50454,15.836794137954712,0.00020097410936159577
16844,33690,16845,50535,15.85940408706665,0.0001971231002926288
16872,33746,16873,50619,15.885891199111938,0.00019312454878672725
16900,33802,16901,50703,15.911293268203735,0.00018991466583884176
16928,33858,16929,50787,15.940332174301147,0.00018626984376624023
16955,33912,16956,50868,15.969178199768066,0.00018287112334292033
16983,33968,16984,50952,15.999344110488892,0.00017977028267068818
17011,34024,17012,51036,16.02697491645813,0.00017654048110671283
17038,34078,17039,51117,16.05499815940857,0.0001729915060195708
17066,34134,17067,51201,16.09232997894287,0.00017010790213589644
17094,34190,17095,51285,16.122716188430786,0.0001671110563847833
17122,34246,17123,51369,16.155351161956787,0.00016437946965197625
17149,34300,17150,51450,16.18497109413147,0.00016117055042741413
17177,34356,17178,51534,16.206690073013306,0.00015824710862943903
17205,34412,17206,51618,16.22945213317871,0.0001551849175029929
17232,34466,17233,51699,16.250972270965576,0.00015276999374691513
17260,34522,17261,51783,16.270840167999268,0.000150019786019584
17288,34578,17289,51867,16.2953200340271,0.00014680797528399125
17315,34632,17316,51948,16.31498122215271,0.00014449199670707458
17343,34688,17344,52032,16.337212324142456,0.0001418210860038016
17371,34744,17372,52116,16.358834266662598,0.00013939280461272574
17399,34800,17400,52200,16.38262128829956,0.0001363943305250359
17426,34854,17427,52281,16.403253078460693,0.00013421365406429686
17454,34910,17455,52365,16.42362332344055,0.00013217691957834177
17482,34966,17483,52449,16.448291063308716,0.00012918421646190836
17509,35020,17510,52530,16.467221975326538,0.0001267870975425467
17537,35076,17538,52614,16.49146318435669,0.00012485064155498549
17565,35132,17566,52698,16.513527154922485,0.0001219681331576794
17592,35186,17593,52779,16.534902095794678,0.00011988882715741056
17620,35242,17621,52863,16.55510711669922,0.00011753482533549686
17648,35298,17649,52947,16.576682090759277,0.000115515549509837
17676,35354,17677,53031,16.599945306777954,0.00011306521321330365
17703,35408,17704,53112,16.619155168533325,0.00011120169824607729
17731,35464,17732,53196,16.64199924468994,0.00010918967984707706
17759,35520,17760,53280,16.664066076278687,0.00010714316181292816
17786,35574,17787,53361,16.686105251312256,0.00010536588797549484
17814,35630,17815,53445,16.707059144973755,0.00010358388908571214
17842,35686,17843,53529,16.72948122024536,0.00010145428825580893
17870,35742,17871,53613,16.752455234527588,9.939313235918235e-05
17897,35796,17898,53694,16.7773859500885,9.764440937942709e-05
17925,35852,17926,53778,16.806846380233765,9.585132158917986e-05
17953,35908,17954,53862,16.83027195930481,9.41474797855335e-05
17980,35962,17981,53943,16.85122513771057,9.259061982902494e-05
18008,36018,18009,54027,16.877024173736572,9.083993347758224e-05
18036,36074,18037,54111,16.89958119392395,8.91626165184789e-05
18063,36128,18064,54192,16.92099094390869,8.771070895363664e-05
18091,36184,18092,54276,16.944321155548096,8.609217798039026e-05
18119,36240,18120,54360,17.03759527206421,8.446861602351419e-05
18147,36296,18148,54444,17.059890270233154,8.270004582300317e-05
18174,36350,18175,54525,17.07925295829773,8.144528896991687e-05
18202,36406,18203,54609,17.100958347320557,7.999300453320757e-05
18230,36462,18231,54693,17.119803190231323,7.844937908885186e-05
18257,36516,18258,54774,17.13989233970642,7.71947121620542e-05
18285,36572,18286,54858,17.160617351531982,7.555681827398075e-05
18313,36628,18314,54942,17.1807701587677,7.390646067051421e-05
18341,36684,18342,55026,17.200085163116455,7.254420506797032e-05
18368,36738,18369,55107,17.218356370925903,7.125431704935181e-05
18396,36794,18397,55191,17.24160099029541,7.033172789761011e-05
18424,36850,18425,55275,17.260990381240845,6.874086079733388e-05
18451,36904,18452,55356,17.283583402633667,6.745865630364278e-05
18479,36960,18480,55440,17.305256366729736,6.616018117711064e-05
18507,37016,18508,55524,17.327458143234253,6.481920740952773e-05
18534,37070,18535,55605,17.348226070404053,6.353203616527026e-05
18562,37126,18563,55689,17.36776113510132,6.2375406969295e-05
18590,37182,18591,55773,17.391239166259766,6.129492396667047e-05
18618,37238,18619,55857,17.412877082824707,6.021782030529721e-05
18645,37292,18646,55938,17.43406915664673,5.9017326179855445e-05
18673,37348,18674,56022,17.45603108406067,5.7675523180478194e-05
18701,37404,18702,56106,17.477459192276,5.671579492627643e-05
18728,37458,18729,56187,17.49916124343872,5.561318448599195e-05
18756,37514,18757,56271,17.520507097244263,5.441081736989872e-05
18784,37570,18785,56355,17.544991970062256,5.336737581274065e-05
18811,37624,18812,56436,17.565855979919434,5.2403360768948914e-05
18839,37680,18840,56520,17.59119415283203,5.143566374954389e-05
18867,37736,18868,56604,17.610488176345825,5.050450101862225e-05
18895,37792,18896,56688,17.633098125457764,4.951173866629688e-05
18922,37846,18923,56769,17.652668237686157,4.873654302173236e-05
18950,37902,18951,56853,17.67254614830017,4.781592497238307e-05
18978,37958,18979,56937,17.695624351501465,4.686658280661504e-05
19005,38012,19006,57018,17.714227199554443,4.614131489688589e-05
19033,38068,19034,57102,17.734788179397583,4.5351707399277075e-05
19061,38124,19062,57186,17.753865242004395,4.4553717316375696e-05
19089,38180,19090,57270,17.772517204284668,4.373292529180617e-05
19116,38234,19117,57351,17.794178009033203,4.2998175672437355e-05
19144,38290,19145,57435,17.814305067062378,4.224437645916623e-05
19172,38346,19173,57519,17.835864067077637,4.1320122363686096e-05
19199,38400,19200,57600,17.857025146484375,4.063301844325906e-05
19227,38456,19228,57684,17.878644943237305,3.956099862989504e-05
19255,38512,19256,57768,17.899935007095337,3.8906461554688576e-05
19282,38566,19283,57849,17.918339014053345,3.816365165221214e-05
19310,38622,19311,57933,17.93884515762329,3.7512362951019895e-05
19338,38678,19339,58017,17.958896160125732,3.643594732238853e-05
19366,38734,19367,58101,17.981353282928467,3.580665338631661e-05
19393,38788,19394,58182,18.00074601173401,3.518697235449508e-05
19421,38844,19422,58266,18.022192239761353,3.454984573636466e-05
19449,38900,19450,58350,18.044355154037476,3.399990578145662e-05
19476,38954,19477,58431,18.06330418586731,3.342804859585158e-05
19504,39010,19505,58515,18.084084272384644,3.2799817859086033e-05
19532,39066,19533,58599,18.103824138641357,3.21748198075511e-05
19560,39122,19561,58683,18.123342037200928,3.157387868668593e-05
19587,39176,19588,58764,18.145576238632202,3.106290159848868e-05
19615,39232,19616,58848,18.167498111724854,3.046230801828642e-05
19643,39288,19644,58932,18.19278621673584,2.9915203640484833e-05
19670,39342,19671,59013,18.2138192653656,2.9444276947288017e-05
19698,39398,19699,59097,18.23986506462097,2.892571274060174e-05
19726,39454,19727,59181,18.261413097381592,2.839296507772815e-05
19753,39508,19754,59262,18.285269021987915,2.78912730209413e-05
19781,39564,19782,59346,18.306682109832764,2.7345707735548785e-05
19809,39620,19810,59430,18.329870223999023,2.6917774448520504e-05
19837,39676,19838,59514,18.354345321655273,2.6356369744462427e-05
19864,39730,19865,59595,18.376697063446045,2.587898734418559e-05
19892,39786,19893,59679,18.400330066680908,2.5460000301791297e-05
19920,39842,19921,59763,18.424073219299316,2.4971999664558098e-05
19947,39896,19948,59844,18.446746110916138,2.4516197754564928e-05
19975,39952,19976,59928,18.46800923347473,2.4061977796918654e-05
20003,40008,20004,60012,18.49190616607666,2.366276839893544e-05
20031,40064,20032,60096,18.51272439956665,2.3268588847713545e-05
20058,40118,20059,60177,18.535322189331055,2.280571561641409e-05
20086,40174,20087,60261,18.55672597885132,2.2372660055225424e-05
20114,40230,20115,60345,18.579366207122803,2.18888919789606e-05
20141,40284,20142,60426,18.60024118423462,2.151325270460802e-05
20169,40340,20170,60510,18.623353242874146,2.116476446190063e-05
20197,40396,20198,60594,18.645437240600586,2.076949795082328e-05
20224,40450,20225,60675,18.668039321899414,2.038305729001877e-05
20252,40506,20253,60759,18.693255186080933,2.0001176494588435e-05
20280,40562,20281,60843,18.71615719795227,1.958947927960253e-05
20308,40618,20309,60927,18.738429307937622,1.9168227481713984e-05
20335,40672,20336,61008,18.76139211654663,1.8838174128177343e-05
20363,40728,20364,61092,18.784212350845337,1.8424779341330577e-05
20391,40784,20392,61176,18.804254293441772,1.8094327401740884e-05
20418,40838,20419,61257,18.823647022247314,1.782031017683039e-05
20446,40894,20447,61341,18.844423294067383,1.7443009483031346e-05
20474,40950,20475,61425,18.866457223892212,1.7136960195784923e-05
20501,41004,20502,61506,18.887078285217285,1.6852812677825568e-05
20529,41060,20530,61590,18.911709308624268,1.651885622777627e-05
20557,41116,20558,61674,18.936569213867188,1.6207103158194514e-05
20585,41172,20586,61758,18.959107160568237,1.5894245962044806e-05
20612,41226,20613,61839,19.03662109375,1.5586390645694337e-05
20640,41282,20641,61923,19.071868181228638,1.532786529878649e-05
20668,41338,20669,62007,19.095790147781372,1.5055243693495868e-05
20695,41392,20696,62088,19.11725425720215,1.490363843004161e-05
20723,41448,20724,62172,19.138249158859253,1.4451106267188152e-05
20751,41504,20752,62256,19.158860206604004,1.4175433648233593e-05
20779,41560,20780,62340,19.179696083068848,1.3900928706789273e-05
20806,41614,20807,62421,19.1996111869812,1.3678119671567401e-05
20834,41670,20835,62505,19.220736980438232,1.3411400459517608e-05
20862,41726,20863,62589,19.244043111801147,1.3140315104465117e-05
20889,41780,20890,62670,19.263323307037354,1.293959519443888e-05
20917,41836,20918,62754,19.285704135894775,1.268692858502618e-05
20945,41892,20946,62838,19.306133031845093,1.2467431020013464e-05
20972,41946,20973,62919,19.326436042785645,1.2257028856765828e-05
21000,42002,21001,63003,19.3478901386261,1.2025349064970214e-05
21028,42058,21029,63087,19.36734414100647,1.1804127325376612e-05
21056,42114,21057,63171,19.39073920249939,1.1576594715734245e-05
21083,42168,21084,63252,19.40908718109131,1.1314332709844166e-05
21111,42224,21112,63336,19.430596113204956,1.1117403914795432e-05
21139,42280,21140,63420,19.451919078826904,1.0933238058896677e-05
21166,42334,21167,63501,19.470147132873535,1.0753521792139509e-05
21194,42390,21195,63585,19.490941286087036,1.0542645895839087e-05
21222,42446,21223,63669,19.510687112808228,1.0351013656872965e-05
21250,42502,21251,63753,19.53142499923706,1.017925546875631e-05
21277,42556,21278,63834,19.549975156784058,9.995575283028302e-06
21305,42612,21306,63918,19.569111108779907,9.803191687751678e-06
21333,42668,21334,64002,19.59092617034912,9.595087703928584e-06
21360,42722,21361,64083,19.609430074691772,9.434793696527777e-06
21388,42778,21389,64167,19.630467176437378,9.250071002497862e-06
21416,42834,21417,64251,19.660685062408447,9.089655804928043e-06
21443,42888,21444,64332,19.684868097305298,8.923213272282737e-06
21471,42944,21472,64416,19.70859122276306,8.771624266046274e-06
21499,43000,21500,64500,19.731942176818848,8.596329962529126e-06
21527,43056,21528,64584,19.755104064941406,8.439138127869228e-06
21554,43110,21555,64665,19.776244163513184,8.300383910864184e-06
21582,43166,21583,64749,19.796136140823364,8.140651971189072e-06
21610,43222,21611,64833,19.815309047698975,7.986729087861022e-06
21637,43276,21638,64914,19.840618133544922,7.833631912035344e-06
21665,43332,21666,64998,19.869929313659668,7.684920092287939e-06
21693,43388,21694,65082,19.90418815612793,7.538177555943548e-06
21720,43442,21721,65163,19.93033719062805,7.3998558036691975e-06
21748,43498,21749,65247,19.953477144241333,7.2706512810327695e-06
21776,43554,21777,65331,19.979318141937256,7.14130510459654e-06
21804,43610,21805,65415,20.0085871219635,7.0173973654164e-06
21831,43664,21832,65496,20.037707090377808,6.8922679474781035e-06
21859,43720,21860,65580,20.065237998962402,6.747534598616767e-06
21887,43776,21888,65664,20.092122077941895,6.6342644231554004e-06
21914,43830,21915,65745,20.114522218704224,6.503494773824059e-06
21942,43886,21943,65829,20.13832116127014,6.385905408023973e-06
21970,43942,21971,65913,20.1588191986084,6.266907234930841e-06
21998,43998,21999,65997,20.180113315582275,6.129268854238035e-06
22025,44052,22026,66078,20.20172119140625,6.032995997884427e-06
22053,44108,22054,66162,20.222175121307373,5.909618380428583e-06
22081,44164,22082,66246,20.247762203216553,5.811124879073759e-06
22108,44218,22109,66327,20.26716637611389,5.6954286264954135e-06
22136,44274,22137,66411,20.290878295898438,5.586522206613154e-06
22164,44330,22165,66495,20.311838150024414,5.491110300681612e-06
22191,44384,22192,66576,20.333884239196777,5.383754114518524e-06
22219,44440,22220,66660,20.35724902153015,5.287417366162117e-06
22247,44496,22248,66744,20.378576278686523,5.197323957872868e-06
22275,44552,22276,66828,20.402085065841675,5.090239142191422e-06
22302,44606,22303,66909,20.42308521270752,4.996816528546333e-06
22330,44662,22331,66993,20.44649910926819,4.90639149575145e-06
22358,44718,22359,67077,20.466233253479004,4.815032298211008e-06
22385,44772,22386,67158,20.48797106742859,4.719687240140047e-06
22413,44828,22414,67242,20.507166147232056,4.6395874733207165e-06
22441,44884,22442,67326,20.52649426460266,4.528533509073895e-06
22469,44940,22470,67410,20.55652618408203,4.460878699319437e-06
22496,44994,22497,67491,20.58320713043213,4.377905838737206e-06
22524,45050,22525,67575,20.602959156036377,4.287634396860085e-06
22552,45106,22553,67659,20.625761032104492,4.209962526147137e-06
22579,45160,22580,67740,20.646667003631592,4.133726747568289e-06
22607,45216,22608,67824,20.665995121002197,4.052953954669647e-06
22635,45272,22636,67908,20.68818712234497,3.982810198976949e-06
22662,45326,22663,67989,20.708990335464478,3.900672822965134e-06
22690,45382,22691,68073,20.73417019844055,3.822268354269909e-06
22718,45438,22719,68157,20.75531315803528,3.748897711375321e-06
22746,45494,22747,68241,20.788517236709595,3.679128553812916e-06
22773,45548,22774,68322,20.808711290359497,3.622400186031882e-06
22801,45604,22802,68406,20.836037158966064,3.5445102639641846e-06
22829,45660,22830,68490,20.8565571308136,3.490911240078276e-06
22856,45714,22857,68571,20.878221035003662,3.413610329516814e-06
22884,45770,22885,68655,20.900418043136597,3.3514880897200783e-06
22912,45826,22913,68739,20.92010521888733,3.290509880571335e-06
22939,45880,22940,68820,20.94679617881775,3.2253407198368222e-06
22967,45936,22968,68904,20.969382286071777,3.1635827326681465e-06
22995,45992,22996,68988,21.00130033493042,3.1025379030324984e-06
23023,46048,23024,69072,21.021065950393677,3.0475114272121573e-06
23050,46102,23051,69153,21.04791808128357,2.9965548264954123e-06
23078,46158,23079,69237,21.07033109664917,2.936366058747808e-06
23106,46214,23107,69321,21.100560188293457,2.8853811500084703e-06
23133,46268,23134,69402,21.12225914001465,2.829694039974129e-06
23161,46324,23162,69486,21.14666223526001,2.778377961476508e-06
23189,46380,23190,69570,21.16882610321045,2.7243669364906964e-06
23217,46436,23218,69654,21.198824167251587,2.672836785677646e-06
23244,46490,23245,69735,21.217530250549316,2.6136460746783996e-06
23272,46546,23273,69819,21.24640417098999,2.5664184022389236e-06
23300,46602,23301,69903,21.267471075057983,2.517653797440289e-06
23327,46656,23328,69984,21.28837013244629,2.472761593708128e-06
23355,46712,23356,70068,21.307223081588745,2.418976578155707e-06
23383,46768,23384,70152,21.333214282989502,2.3749340698486776e-06
23410,46822,23411,70233,21.355006217956543,2.3342446411334095e-06
23438,46878,23439,70317,21.378380060195923,2.2840954443381634e-06
23466,46934,23467,70401,21.40373134613037,2.2400678290068754e-06
23494,46990,23495,70485,21.423359394073486,2.1994309236106346e-06
23521,47044,23522,70566,21.451011180877686,2.155086235688941e-06
23549,47100,23550,70650,21.470518112182617,2.1073957441331004e-06
23577,47156,23578,70734,21.494027137756348,2.068896151286026e-06
23604,47210,23605,70815,21.513630151748657,2.030544692388503e-06
23632,47266,23633,70899,21.536607027053833,1.9908954982383875e-06
23660,47322,23661,70983,21.557760000228882,1.957468043656263e-06
23688,47378,23689,71067,21.578994274139404,1.9142058818033547e-06
23715,47432,23716,71148,21.59985113143921,1.876380679277645e-06
23743,47488,23744,71232,21.619001150131226,1.83714462309581e-06
23771,47544,23772,71316,21.65002703666687,1.8028047179541318e-06
23798,47598,23799,71397,21.668360233306885,1.7617506955502904e-06
23826,47654,23827,71481,21.70004916191101,1.7320246570307063e-06
23854,47710,23855,71565,21.72639012336731,1.696181925581186e-06
23881,47764,23882,71646,21.747079133987427,1.66506083587592e-06
23909,47820,23910,71730,21.76650905609131,1.6287967810058035e-06
23937,47876,23938,71814,21.78846311569214,1.5976602298906073e-06
23965,47932,23966,71898,21.808138132095337,1.560801479172369e-06
23992,47986,23993,71979,21.838760137557983,1.5343898667197209e-06
24020,48042,24021,72063,21.859254121780396,1.4988157772677368e-06
24048,48098,24049,72147,21.890302181243896,1.4670516748083173e-06
24075,48152,24076,72228,21.91069531440735,1.4390788010132383e-06
24103,48208,24104,72312,21.937729120254517,1.4069631788515835e-06
24131,48264,24132,72396,21.95745301246643,1.379764398734551e-06
24159,48320,24160,72480,21.977827072143555,1.351008563688083e-06
24186,48374,24187,72561,22.00026535987854,1.3263465916679706e-06
24214,48430,24215,72645,22.0195951461792,1.2989352171643986e-06
24242,48486,24243,72729,22.044079065322876,1.2731193237414118e-06
24269,48540,24270,72810,22.06304931640625,1.2508345434980583e-06
24297,48596,24298,72894,22.096562147140503,1.2245232028362807e-06
24325,48652,24326,72978,22.115764379501343,1.1988752248726087e-06
24352,48706,24353,73059,22.138880014419556,1.177443209599005e-06
24380,48762,24381,73143,22.158903121948242,1.1532148391779629e-06
24408,48818,24409,73227,22.179235219955444,1.1272898063907633e-06
24436,48874,24437,73311,22.203140258789062,1.104793000195059e-06
24463,48928,24464,73392,22.223124980926514,1.0849369118659524e-06
24491,48984,24492,73476,22.246652126312256,1.063354943653394e-06
24519,49040,24520,73560,22.268081188201904,1.0420319540571654e-06
24546,49094,24547,73641,22.300719261169434,1.0212714869339834e-06
24574,49150,24575,73725,22.320056200027466,9.982962865251466e-07
24602,49206,24603,73809,22.347124338150024,9.714804036775604e-07
24629,49260,24630,73890,22.366733074188232,9.535970093565993e-07
24657,49316,24658,73974,22.386763095855713,9.309056849815533e-07
24685,49372,24686,74058,22.405622005462646,9.131551905738888e-07
24713,49428,24714,74142,22.424840211868286,8.935774076235248e-07
24740,49482,24741,74223,22.442711114883423,8.779844620221411e-07
24768,49538,24769,74307,22.46216917037964,8.555845170121756e-07
24796,49594,24797,74391,22.483342170715332,8.39458607515553e-07
24823,49648,24824,74472,22.502527952194214,8.211877684516367e-07
24851,49704,24852,74556,22.521119117736816,8.068566330621252e-07
24879,49760,24880,74640,22.54176115989685,7.876420795582817e-07
24907,49816,24908,74724,22.56036615371704,7.692217423027614e-07
24934,49870,24935,74805,22.581789255142212,7.547147333752946e-07
24962,49926,24963,74889,22.60028910636902,7.372403842964559e-07
24990,49982,24991,74973,22.62061905860901,7.19064928489388e-07
25017,50036,25018,75054,22.638657093048096,7.026999355730368e-07
25045,50092,25046,75138,22.657097339630127,6.873002575957798e-07
25073,50148,25074,75222,22.675401210784912,6.719066050209221e-07
25100,50202,25101,75303,22.693665027618408,6.598195341211976e-07
25128,50258,25129,75387,22.71160912513733,6.428946335290675e-07
25156,50314,25157,75471,22.73012614250183,6.284421942837071e-07
25184,50370,25185,75555,22.748688220977783,6.135030616860604e-07
25211,50424,25212,75636,22.766526222229004,6.019149623170961e-07
25239,50480,25240,75720,22.788652181625366,5.884105576114962e-07
25267,50536,25268,75804,22.807037353515625,5.771768201157101e-07
25294,50590,25295,75885,22.828202962875366,5.630882924378966e-07
25322,50646,25323,75969,22.850134134292603,5.492082664204645e-07
25350,50702,25351,76053,22.869577169418335,5.341120186130865e-07
25378,50758,25379,76137,22.893025159835815,5.220271077632788e-07
25405,50812,25406,76218,22.912606239318848,5.058610668129404e-07
25433,50868,25434,76302,22.932220220565796,4.912858457828406e-07
25461,50924,25462,76386,22.952024221420288,4.812744691662374e-07
25488,50978,25489,76467,22.971140146255493,4.6726472646696493e-07
25516,51034,25517,76551,22.992119073867798,4.5633487388840877e-07
25544,51090,25545,76635,23.0102322101593,4.456192073121201e-07
25571,51144,25572,76716,23.02943205833435,4.3300678953528404e-07
25599,51200,25600,76800,23.048673152923584,4.238079327478772e-07
25627,51256,25628,76884,23.06871509552002,4.1130931549560046e-07
25655,51312,25656,76968,23.08830428123474,4.016386583316489e-07
25682,51366,25683,77049,23.10685896873474,3.9256212858163053e-07
25710,51422,25711,77133,23.12608003616333,3.825081194008817e-07
25738,51478,25739,77217,23.14479899406433,3.7295956190064317e-07
25765,51532,25766,77298,23.16411805152893,3.6412745885172626e-07
25793,51588,25794,77382,23.18424916267395,3.540733359841397e-07
25821,51644,25822,77466,23.206477165222168,3.4470178889023373e-07
25848,51698,25849,77547,23.227795362472534,3.370844297023723e-07
25876,51754,25877,77631,23.248380184173584,3.2892103263293393e-07
25904,51810,25905,77715,23.270203113555908,3.1959564239514293e-07
25932,51866,25933,77799,23.29250717163086,3.111078967776848e-07
25959,51920,25960,77880,23.31305432319641,3.0354260616149986e-07
25987,51976,25988,77964,23.331570148468018,2.954379851871636e-07
26015,52032,26016,78048,23.349744081497192,2.872377535823034e-07
26042,52086,26043,78129,23.36848521232605,2.8089766601624433e-07
26070,52142,26071,78213,23.391951084136963,2.7139140001963824e-07
26098,52198,26099,78297,23.41035532951355,2.6442012313054875e-07
26126,52254,26127,78381,23.4289231300354,2.568542640801752e-07
26153,52308,26154,78462,23.449515104293823,2.4909127205319237e-07
26181,52364,26182,78546,23.468569040298462,2.430972472211579e-07
26209,52420,26210,78630,23.49342632293701,2.3573375074192882e-07
26236,52474,26237,78711,23.512142181396484,2.2941230781725608e-07
26264,52530,26265,78795,23.530887126922607,2.2131439436634537e-07
26292,52586,26293,78879,23.550523281097412,2.151747366951895e-07
26319,52640,26320,78960,23.570176124572754,2.0812228740396677e-07
26347,52696,26348,79044,23.594755172729492,2.0041863990627462e-07
26375,52752,26376,79128,23.613352298736572,1.948430963238934e-07
26403,52808,26404,79212,23.635149002075195,1.8890386854764074e-07
26430,52862,26431,79293,23.65655517578125,1.8350272057432448e-07
26458,52918,26459,79377,23.676483154296875,1.7683885289443424e-07
26486,52974,26487,79461,23.698671102523804,1.7130059859482571e-07
26513,53028,26514,79542,23.71691918373108,1.6483738818351412e-07
26541,53084,26542,79626,23.73634934425354,1.5944965525704902e-07
26569,53140,26570,79710,23.75484323501587,1.5368084405054105e-07
26597,53196,26598,79794,23.77335023880005,1.4803890735493042e-07
26624,53250,26625,79875,23.793626070022583,1.4355327948578633e-07
26652,53306,26653,79959,23.81164312362671,1.384504457746516e-07
26680,53362,26681,80043,23.831847190856934,1.3337501059140777e-07
26707,53416,26708,80124,23.851325273513794,1.2908367352792993e-07
26735,53472,26736,80208,23.86991834640503,1.2422924555721693e-07
26763,53528,26764,80292,23.889081239700317,1.197071242131642e-07
26790,53582,26791,80373,23.90705108642578,1.1509837349876761e-07
26818,53638,26819,80457,23.92680335044861,1.1063161764468532e-07
26846,53694,26847,80541,23.945966243743896,1.06514448816597e-07
26874,53750,26875,80625,23.964279174804688,1.0119697435584385e-07
26901,53804,26902,80706,23.984554052352905,9.871507700154325e-08
26929,53860,26930,80790,24.002838134765625,9.255427357857116e-08
26957,53916,26958,80874,24.021290063858032,8.82423591974657e-08
26984,53970,26985,80955,24.039764165878296,8.43772340886062e-08
27012,54026,27013,81039,24.059559106826782,7.987227945704944e-08
27040,54082,27041,81123,24.08005404472351,7.610992724949028e-08
27067,54136,27068,81204,24.099643230438232,7.19066974852467e-08
27095,54192,27096,81288,24.11896324157715,6.788070550101111e-08
27123,54248,27124,81372,24.14459800720215,6.379400474543218e-08
27151,54304,27152,81456,24.16301417350769,5.991171292407671e-08
27178,54358,27179,81537,24.18171215057373,5.627305199595867e-08
27206,54414,27207,81621,24.201255321502686,5.284073267830536e-08
27234,54470,27235,81705,24.219962120056152,4.88716977997683e-08
27261,54524,27262,81786,24.240989208221436,4.5746446630801074e-08
27289,54580,27290,81870,24.262890100479126,4.2601982386258896e-08
27317,54636,27318,81954,24.29202103614807,3.9315182220889255e-08
27345,54692,27346,82038,24.31822633743286,3.584307251003338e-08
27372,54746,27373,82119,24.343953132629395,3.309992280264851e-08
27400,54802,27401,82203,24.37060523033142,2.9627244657604024e-08
27428,54858,27429,82287,24.398126125335693,2.585966285550967e-08
27455,54912,27456,82368,24.417197227478027,2.3124016479414422e-08
27483,54968,27484,82452,24.439725160598755,1.9924755179090425e-08
27511,55024,27512,82536,24.458341121673584,1.6909666555875447e-08
27538,55078,27539,82617,24.47724223136902,1.4345232557388954e-08
27566,55134,27567,82701,24.497626066207886,1.1582187653402798e-08
27594,55190,27595,82785,24.516467332839966,8.494907888234593e-09
27622,55246,27623,82869,24.53535509109497,5.682295523001812e-09
27649,55300,27650,82950,24.55495810508728,2.7974920158158056e-09
27677,55356,27678,83034,24.57558298110962,3.7971403799019754e-11


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012929439544677734,2181.4194943796983
1001,2003,2002,4005,2.083881139755249,35.469008324394736
2002,4005,4004,8009,3.7600128650665283,34.40807984936259
3003,6007,6006,12013,5.381834030151367,33.40915906251007
4004,8009,8008,16017,6.823575973510742,32.46649241354112
5005,10011,10010,20021,8.367573022842407,31.574817185092343
6006,12013,12012,24025,10.655004978179932,30.729356494634658
7007,14015,14014,28029,13.033334016799927,29.925806080461598
8008,16017,16016,32033,14.922853946685791,29.160312226378892
9009,18019,18018,36037,17.020570993423462,28.429442473491918
10010,20021,20020,40041,18.604860067367554,27.730151575056198
11011,22023,22022,44045,20.18110489845276,27.05974513210731
12012,24025,24024,48049,21.71625304222107,26.415842942091558
13013,26027,26026,52053,23.18020987510681,25.796343564906238
14014,28029,28028,56057,24.672911882400513,25.199391102974914
15015,30031,30030,60061,26.131555795669556,24.62334476796559
16016,32033,32032,64065,27.623703956604004,24.066751484178212
17017,34035,34034,68069,29.105128049850464,23.528321551468252
18018,36037,36036,72073,30.58879804611206,23.00690724257811
19019,38039,38038,76077,32.114301919937134,22.501484122476768
20020,40041,40040,80081,33.72951793670654,22.011134833710912
21021,42043,42042,84085,35.22915315628052,21.53503507780397
22022,44045,44044,88089,36.72470784187317,21.07244152781209
23023,46047,46046,92093,38.18768119812012,20.622681423360746
24024,48049,48048,96097,39.694260120391846,20.18514362154656
25025,50051,50050,100101,41.20482683181763,19.759270901450236
26026,52053,52052,104105,42.723315954208374,19.344553344373935
27027,54055,54054,108109,44.233383893966675,18.94052263505432
28028,56057,56056,112113,45.79564189910889,18.546747150268857
29029,58059,58058,116117,47.311460971832275,18.16283425082861
30030,60061,60060,120121,48.81859302520752,17.788409349263247
31031,62063,62062,124125,50.32033395767212,17.42312502340951
32032,64065,64064,128129,51.78358197212219,17.066659395597753
33033,66067,66066,132133,53.26893186569214,16.718711055442327
34034,68069,68068,136137,54.753591775894165,16.378996975641485
35035,70071,70070,140141,56.22053575515747,16.047250692088596
36036,72073,72072,144145,57.750038146972656,15.723220711224826
37037,74075,74074,148149,59.27613091468811,15.406669113086082
38038,76077,76076,152153,60.7823760509491,15.097370323150471
39039,78079,78078,156157,62.327457904815674,14.795110030047113
40040,80081,80080,160161,63.81347990036011,14.499684229522131
41041,82083,82082,164165,65.2956600189209,14.210898377900776
42042,84085,84084,168169,66.79907393455505,13.928566640679605
43043,86087,86086,172173,68.30095076560974,13.652511223918623
44044,88089,88088,176177,69.80014085769653,13.382561777846263
45045,90091,90090,180181,71.35210800170898,13.118554863542954
46046,92093,92092,184185,72.86093282699585,12.860333474838967
47047,94095,94094,188189,74.35861301422119,12.607746608625234
48048,96097,96096,192193,75.85052704811096,12.360648877686799
49049,98099,98098,196197,77.35159087181091,12.118900160955377
50050,100101,100100,200201,78.83917713165283,11.882365286744289
51051,102103,102102,204205,80.308434009552,11.65091374510655
52052,104105,104104,208209,81.79112887382507,11.424419425951896
53053,106107,106106,212213,83.31579494476318,11.202760379985875
54054,108109,108108,216217,84.82643795013428,10.985818599903496
55055,110111,110110,220221,86.52674698829651,10.773479819588829
56056,112113,112112,224225,88.25576210021973,10.565633329353773
57057,114115,114114,228229,89.87662601470947,10.362171805483285
58058,116117,116116,232233,91.5476450920105,10.162991152574818
59059,118119,118118,236237,93.23581385612488,9.96799035733693
60060,120121,120120,240241,94.82266616821289,9.777071352677467
61061,122123,122122,244245,96.33524990081787,9.59013889105222
62062,124125,124124,248249,97.79210710525513,9.407100426173315
63063,126127,126126,252253,99.27154111862183,9.227866002281985
64064,128129,128128,256257,100.75854897499084,9.052348150292346
65065,130131,130130,260261,102.22938990592957,8.880461790195795
66066,132133,132132,264265,103.87586688995361,8.71212413919261
67067,134135,134134,268269,105.56757998466492,8.547254625079518
68068,136137,136136,272273,107.23592495918274,8.385774804486573
69069,138139,138138,276277,108.9399528503418,8.227608285596375
70070,140141,140140,280281,111.11850094795227,8.072680655033082
71071,142143,142142,284285,113.05877208709717,7.920919408630425
72072,144145,144144,288289,114.5725519657135,7.772253885831674
73073,146147,146146,292293,116.02846002578735,7.626615207490545
74074,148149,148148,296297,117.48810982704163,7.483936216864095
75075,150151,150150,300301,118.9675281047821,7.344151423606263
76076,152153,152152,304305,120.4232349395752,7.207196950584375
77077,154155,154154,308309,121.91765594482422,7.07301048334466
78078,156157,156156,312313,123.36713409423828,6.941531222071831
79079,158159,158158,316317,124.82455205917358,6.812699835883905
80080,160161,160160,320321,126.3263030052185,6.686458419317773
81081,162163,162162,324325,127.78291320800781,6.562750450860449
82082,164165,164164,328329,129.29141211509705,6.441520753393206
83083,166167,166166,332333,130.75920796394348,6.322715456413903
84084,168169,168168,336337,132.22711086273193,6.206281959916623
85085,170171,170170,340341,133.69375705718994,6.092168899808144
86086,172173,172172,344345,135.20442390441895,5.980326114754462
87087,174175,174174,348349,136.66602206230164,5.870704614348256
88088,176177,176176,352353,138.15738987922668,5.763256548507343
89089,178179,178178,356357,139.6510307788849,5.65793517801319
90090,180181,180180,360361,141.17385601997375,5.554694846107395
91091,182183,182182,364365,142.70920515060425,5.453490951075423
92092,184185,184184,368369,144.49027681350708,5.354279919749274
93093,186187,186186,372373,146.2180609703064,5.257019181869168
94094,188189,188188,376377,147.8789598941803,5.161667145250817
95095,190191,190190,380381,149.55553603172302,5.0681831717073464
96096,192193,192192,384385,151.38532400131226,4.976527553688356
97097,194195,194194,388389,152.936940908432,4.886661491588143
98098,196197,196196,392393,154.8321931362152,4.798547071696703
99099,198199,198198,396397,156.51292991638184,4.712147244757261
100100,200201,200200,400401,158.12949681282043,4.627425805103599
101101,202203,202202,404405,159.7592761516571,4.544347370351716
102102,204205,204204,408409,161.38389587402344,4.462877361623441
103103,206207,206206,412413,162.9303059577942,4.382981984279695
104104,208209,208208,416417,164.49662899971008,4.304628209147609
105105,210211,210210,420421,166.30677890777588,4.227783754217853
106106,212213,212212,424425,168.0950129032135,4.152417066806038
107107,214215,214214,428429,169.67587113380432,4.078497306154077
108108,216217,216216,432433,171.26953601837158,4.005994326462201
109109,218219,218218,436437,172.9979898929596,3.9348786603396775
110110,220221,220220,440441,174.49671292304993,3.8651215026609407
111111,222223,222222,444445,176.18326210975647,3.7966946948155282
112112,224225,224224,448449,177.72758507728577,3.729570709342397
113113,226227,226226,452453,179.26203083992004,3.6637226349374714
114114,228229,228228,456457,180.74593901634216,3.599124161827376
115115,230231,230230,460461,182.2393307685852,3.535749567495145
116116,232233,232232,464465,183.91442394256592,3.4735737027557434
117117,234235,234234,468469,185.79115295410156,3.4125719781663975
118118,236237,236236,472473,187.85199284553528,3.3527203507696868
119119,238239,238238,476477,189.4576530456543,3.293995311154731
120120,240241,240240,480481,191.7632598876953,3.2363738708371557
121121,242243,242242,484485,194.07678604125977,3.1798335499411223
122122,244245,244244,488489,196.22145700454712,3.1243523651841087
123123,246247,246246,492493,198.05195093154907,3.069908818152385
124124,248249,248248,496497,199.80928707122803,3.01648188386298
125125,250251,250250,500501,201.94151210784912,2.964050999602705
126126,252253,252252,504505,203.71742391586304,2.912596054041387
127127,254255,254254,508509,205.3281009197235,2.862097376609313
128128,256257,256256,512513,206.99701404571533,2.8125357271352414
129129,258259,258258,516517,208.6107521057129,2.7638922857354373
130130,260261,260260,520521,211.1240200996399,2.7161486429528168
131131,262263,262262,524525,214.37007808685303,2.6692867901351747
132132,264265,264264,528529,216.9112949371338,2.623289110049768
133133,266267,266266,532533,219.82853198051453,2.578138367727661
134134,268269,268268,536537,222.14451098442078,2.53381770153203
135135,270271,270270,540541,223.9102349281311,2.490310614445548
136136,272273,272272,544545,225.42290687561035,2.4476009655709277
137137,274275,274274,548549,226.90721011161804,2.4056729618411055
138138,276277,276276,552553,228.39407086372375,2.3645111499299674
139139,278279,278278,556557,229.8681070804596,2.3241004083648704
140140,280281,280280,560561,231.41905808448792,2.2844259398290205
141141,282283,282282,564565,232.87300419807434,2.245473263654958
142142,284285,284284,568569,234.48126602172852,2.2072282085010784
143143,286287,286286,572573,236.04758310317993,2.169676905206984
144144,288289,288288,576577,237.60983514785767,2.1328057798257305
145145,290291,290290,580581,239.11916613578796,2.096601546823649
146146,292293,292292,584585,240.60955595970154,2.061051202449221
147147,294295,294294,588589,242.11716103553772,2.026142018263158
148148,296297,296296,592593,243.6458351612091,1.9918615348259436
149149,298299,298298,596597,245.10939192771912,1.9581975555402096
150150,300301,300300,600601,246.59456181526184,1.9251381406446626
151151,302303,302302,604605,248.13989305496216,1.8926716013512532
152152,304305,304304,608609,249.82379388809204,1.8607864941290018
153153,306307,306306,612613,251.38520002365112,1.8294716151234525
154154,308309,308308,616617,253.03842902183533,1.7987159947157352
155155,310311,310310,620621,254.65541005134583,1.7685088922096384
156156,312313,312312,624625,256.1574580669403,1.7388397906520368
157157,314315,314314,628629,257.8459348678589,1.7096983917748503
158158,316317,316316,632633,259.8594970703125,1.6810746110627406
159159,318319,318318,636637,262.4168908596039,1.6529585729392693
160160,320321,320320,640641,264.20900106430054,1.6253406060684483
161161,322323,322322,644645,265.8316287994385,1.5982112387703182
162162,324325,324324,648649,267.3621199131012,1.5715611945486216
163163,326327,326326,652653,268.9387140274048,1.5453813877238645
164164,328329,328328,656657,270.51087284088135,1.5196629191732427
165165,330331,330330,660661,272.05711698532104,1.4943970721715232
166166,332333,332332,664665,273.59478998184204,1.469575308333674
167167,334335,334334,668669,275.25572299957275,1.4451892636521961
168168,336337,336336,672673,276.768404006958,1.421230744632112
169169,338339,338338,676677,278.3619258403778,1.3976917245158802
170170,340341,340340,680681,279.9427740573883,1.3745643396001697
171171,342343,342342,684685,281.5807189941406,1.35184088563949
172172,344345,344344,688689,283.1321179866791,1.3295138143355416
173173,346347,346346,692693,284.67947816848755,1.307575729910809
174174,348349,348348,696697,286.19439601898193,1.286019385761847
175175,350351,350350,700701,287.8056569099426,1.2648376811933986
176176,352353,352352,704705,289.3196039199829,1.2440236582299349
177177,354355,354354,708709,290.8781158924103,1.223570498499953
178178,356357,356356,712713,292.39645290374756,1.203471520197354
179179,358359,358358,716717,293.94718194007874,1.1837201751116027
180180,360361,360360,720721,295.5593099594116,1.1643100457295077
181181,362363,362362,724725,297.2651951313019,1.1452348424038519
182182,364365,364364,728729,298.9030411243439,1.1264884005884142
183183,366367,366366,732733,300.4367370605469,1.1080646781384758
184184,368369,368368,736737,301.9581341743469,1.0899577526743087
185185,370371,370370,740741,303.6370198726654,1.0721618190052595
186186,372373,372372,744745,305.2214081287384,1.0546711866140868
187187,374375,374374,748749,306.9389970302582,1.0374802772009843
188188,376377,376376,752753,308.9530141353607,1.0205836222824018
189189,378379,378378,756757,310.5337691307068,1.0039758608479588
190190,380381,380380,760761,312.1881408691406,0.9876517370696547
191191,382383,382382,764765,313.7639980316162,0.9716060980638304
192192,384385,384384,768769,315.88754200935364,0.9558338917067886
193193,386387,386386,772773,317.484158039093,0.9403301644989597
194194,388389,388388,776777,319.1244819164276,0.9250900594778386
195195,390391,390390,780781,320.65000796318054,0.9101088141801483
196196,392393,392392,784785,322.64821887016296,0.8953817586490231
197197,394395,394394,788789,324.6876459121704,0.8809043134890544
198198,396397,396396,792793,326.2199378013611,0.8666719879626044
199199,398399,398398,796797,327.6965398788452,0.8526803781318222
200200,400401,400400,800801,329.62812089920044,0.8389251650427241
201201,402403,402402,804805,331.33516907691956,0.8254021129483817
202202,404405,404404,808809,332.8357560634613,0.8121070675754254
203203,406407,406406,812813,334.3291931152344,0.7990359544268131
204204,408409,408408,816817,335.8507647514343,0.7861847771252997
205205,410411,410410,820821,337.3313009738922,0.7735496157919215
206206,412413,412412,824825,338.82484579086304,0.761126625463362
207207,414415,414414,828829,340.3615849018097,0.7489120345429683
208208,416417,416416,832833,341.8581988811493,0.7369021432870113
209209,418419,418418,836837,343.3538899421692,0.7250933223252787
210210,420421,420420,840841,344.8160619735718,0.713482011213614
211211,422423,422422,844845,346.3023750782013,0.7020647170203347
212212,424425,424424,848849,348.04337215423584,0.6908380129425495
213213,426427,426426,852853,349.99447894096375,0.6797985369532853
214214,428429,428428,856857,351.9109888076782,0.6689429904805593
215215,430431,430430,860861,353.71790075302124,0.6582681371128274
216216,432433,432432,864865,356.5361649990082,0.6477708013349002
217217,434435,434434,868869,358.2806899547577,0.6374478672912574
218218,436437,436436,872873,360.2280559539795,0.6272962775761926
219219,438439,438438,876877,362.0223979949951,0.6173130320518112
220220,440441,440440,880881,363.74486088752747,0.607495186689448
221221,442443,442442,884885,365.25109100341797,0.5978398524393924
222222,444445,444444,888889,366.710923910141,0.5883441941230103
223223,446447,446446,892893,368.2026119232178,0.5790054293506728
224224,448449,448448,896897,370.1302638053894,0.569820827461399
225225,450451,450450,900901,371.91219902038574,0.5607877084875099
226226,452453,452452,904905,373.77894401550293,0.5519034421406559
227227,454455,454454,908909,375.4575660228729,0.5431654468193301
228228,456457,456456,912913,377.06607389450073,0.5345711886394611
229229,458459,458458,916917,378.7015690803528,0.5261181804845592
230230,460461,460460,920921,380.2967960834503,0.5178039810754171
231231,462463,462462,924925,381.84259581565857,0.5096261940634577
232232,464465,464464,928929,383.364688873291,0.5015824671393148
233233,466467,466466,932933,384.86215686798096,0.4936704911626748
234234,468469,468468,936937,386.41525888442993,0.4858879993108758
235235,470471,470470,940941,388.03363490104675,0.4782327662450143
236236,472473,472472,944945,389.6580581665039,0.47070260729321944
237237,474475,474474,948949,391.2225959300995,0.4632953776534805
238238,476477,476476,952953,392.8113408088684,0.4560089716103448
239239,478479,478478,956957,394.3230941295624,0.4488413217715106
240240,480481,480480,960961,395.95538902282715,0.44179039831760747
241241,482483,482482,964965,397.5481140613556,0.43485420826868904
242242,484485,484484,968969,399.0875668525696,0.42803079476937
243243,486487,486486,972973,400.70999789237976,0.42131823638351307
244244,488489,488488,976977,402.2746651172638,0.4147146464074467
245245,490491,490490,980981,403.83442282676697,0.4082181721961433
246246,492493,492492,984985,405.37931990623474,0.4018269945048587
247247,494495,494494,988989,406.9428598880768,0.3955393268425951
248248,496497,496496,992993,408.57129979133606,0.38935341484113906
249249,498499,498498,996997,410.0449938774109,0.38326753563535476
250250,500501,500500,1001001,411.6105990409851,0.377279997257574
251251,502503,502502,1005005,413.19141578674316,0.3713891380440373
252252,504505,504504,1009009,415.08250999450684,0.3655933260541815
253253,506507,506506,1013013,416.6780707836151,0.3598909585007277
254254,508509,508508,1017017,418.58472204208374,0.354280461193639
255255,510511,510510,1021021,421.5215120315552,0.3487602879926044
256256,512513,512512,1025025,424.4566390514374,0.3433289202733931
257257,514515,514514,1029029,426.69137501716614,0.3379848664050087
258258,516517,516516,1033033,428.72213411331177,0.33272666123446015
259259,518519,518518,1037037,430.313688993454,0.3275528655871085
260260,520521,520520,1041041,431.8591899871826,0.3224620657719015
261261,522523,522522,1045045,433.4155170917511,0.317452873101729
262262,524525,524524,1049049,435.04981899261475,0.31252392341923496
263263,526527,526526,1053053,436.6104609966278,0.30767387663502177
264264,528529,528528,1057057,438.4976189136505,0.3029014162742669
265265,530531,530530,1061061,440.9537398815155,0.2982052490330034
266266,532533,532532,1065065,443.45016598701477,0.29358410434213056
267267,534535,534534,1069069,446.4544520378113,0.2890367339416571
268268,536537,536536,1073073,449.74092292785645,0.28456191146301535
269269,538539,538538,1077077,451.83477210998535,0.28015843201978896
270270,540541,540540,1081081,453.4889061450958,0.2758251118067392
271271,542543,542542,1085085,455.7225890159607,0.2715607877058801
272272,544545,544544,1089089,457.82564997673035,0.2673643169026718
273273,546547,546546,1093093,459.91726183891296,0.263234576507557
274274,548549,548548,1097097,461.8300449848175,0.2591704631865923
275275,550551,550550,1101101,463.48366808891296,0.25517089279890115
276276,552553,552552,1105105,465.9145748615265,0.25123480004083376
277277,554555,554554,1109109,467.5399158000946,0.24736113809854032
278278,556557,556556,1113113,469.0089180469513,0.24354887830588723
279279,558559,558558,1117117,470.5237190723419,0.2397970098102178
280280,560561,560560,1121121,472.0708839893341,0.23610453924470676
281281,562563,562562,1125125,473.55119585990906,0.23247049040617185
282282,564565,564564,1129129,475.07728481292725,0.228893903940957
283283,566567,566566,1133133,476.5823268890381,0.22537383703445357
284284,568569,568568,1137137,478.12467789649963,0.2219093631100577
285285,570571,570570,1141141,479.92449283599854,0.2184995715307423
286286,572573,572572,1145145,481.5176680088043,0.21514356730881445
287287,574575,574574,1149149,483.3350429534912,0.21184047082056168
288288,576577,576576,1153153,485.599986076355,0.20858941752567262
289289,578579,578578,1157157,487.2259101867676,0.20538955769404765
290290,580581,580580,1161161,488.81172585487366,0.20224005613511054
291291,582583,582582,1165165,490.5898859500885,0.1991400919357602
292292,584585,584584,1169169,492.1198990345001,0.19608885820093747
293293,586587,586586,1173173,493.63612508773804,0.1930855617998759
294294,588589,588588,1177177,495.3560960292816,0.19012942311724146
295295,590591,590590,1181181,496.8751058578491,0.18721967580995624
296296,592593,592592,1185185,498.4121811389923,0.1843555665667509
297297,594595,594594,1189189,499.9608430862427,0.18153635487510655
298298,596597,596596,1193193,501.57096004486084,0.17876131278967478
299299,598599,598598,1197197,503.14889788627625,0.17602972470774603
300300,600601,600600,1201201,504.7812650203705,0.17334088714687823
301301,602603,602602,1205205,506.4297261238098,0.1706941085286644
302302,604605,604604,1209209,508.0949478149414,0.16808870896534245
303303,606607,606606,1213213,509.6425061225891,0.16552402005106615
304304,608609,608608,1217217,511.1891348361969,0.16299938465726882
305305,610611,610610,1221221,512.8450100421906,0.16051415673064184
306306,612613,612612,1225225,514.4998970031738,0.15806770109702484
307307,614615,614614,1229229,516.3061451911926,0.15565939326802436
308308,616617,616616,1233233,518.0048940181732,0.15328861925036108
309309,618619,618618,1237237,519.5243759155273,0.1509547753599918
310310,620621,620620,1241241,521.0237319469452,0.1486572680403242
311311,622623,622622,1245245,522.5365388393402,0.1463955136820232
312312,624625,624624,1249249,524.0075490474701,0.14416893844759215
313313,626627,626626,1253253,525.6239619255066,0.14197697809879628
314314,628629,628628,1257257,527.2467138767242,0.1398190778273829
315315,630631,630630,1261261,528.7908849716187,0.137694692088985
316316,632633,632632,1265265,530.2969009876251,0.13560328444066272
317317,634635,634634,1269269,531.8795638084412,0.13354432737992283
318318,636637,636636,1273273,533.373025894165,0.13151730218851299
319319,638639,638638,1277277,534.9211468696594,0.1295216987787171
320320,640641,640640,1281281,536.562490940094,0.12755701554124244
321321,642643,642642,1285285,538.1881458759308,0.12562275919799504
322322,644645,644644,1289289,539.8302171230316,0.12371844465587856
323323,646647,646646,1293293,541.3767008781433,0.12184359486400353
324324,648649,648648,1297297,542.8505659103394,0.11999774067339786
325325,650651,650650,1301301,544.5142171382904,0.11818042070001411
326326,652653,652652,1305305,546.2323958873749,0.11639118118921488
327327,654655,654654,1309309,548.1695868968964,0.11462957588253175
328328,656657,656656,1313313,549.9125699996948,0.11289516588919923
329329,658659,658658,1317317,552.0765039920807,0.11118751955677908
330330,660661,660660,1321321,554.0630779266357,0.10950621234724167
331331,662663,662662,1325325,556.079626083374,0.10785082671236523
332332,664665,664664,1329329,558.4239959716797,0.10622095197425097
333333,666667,666666,1333333,560.658059835434,0.10461618420583818
334334,668669,668668,1337337,563.3796119689941,0.10303612611539847
335335,670671,670670,1341341,566.2039530277252,0.10148038693137096
336336,672673,672672,1345345,568.0788481235504,0.0999485822906081
337337,674675,674674,1349349,570.6535220146179,0.09844033412775843
338338,676677,676676,1353353,573.0854439735413,0.09695527056794617
339339,678679,678678,1357357,574.6968479156494,0.09549302581979191
340340,680681,680680,1361361,579.6232509613037,0.09405324007127547
341341,682683,682682,1365365,582.2939369678497,0.09263555938821355
342342,684685,684684,1369369,585.5080149173737,0.09123963561239634
343343,686687,686686,1373373,587.3019030094147,0.08986512626404419
344344,688689,688688,1377377,590.3649439811707,0.08851169444415063
345345,690691,690690,1381381,593.5418682098389,0.08717900873978124
346346,692693,692692,1385385,595.8186140060425,0.08586674313039566
347347,694695,694694,1389389,597.7735619544983,0.08457457689621606
348348,696697,696696,1393393,599.3062291145325,0.08330219452761867
349349,698699,698698,1397397,601.1020638942719,0.0820492856380497
350350,700701,700700,1401401,603.4389388561249,0.0808155448752359
351351,702703,702702,1405405,606.8552379608154,0.07960067183717001
352352,704705,704704,1409409,609.7155301570892,0.07840437098786879
353353,706707,706706,1413413,612.4791588783264,0.07722635157472268
354354,708709,708708,1417417,615.2498669624329,0.07606632754857401
355355,710711,710710,1421421,617.4275019168854,0.07492401748299926
356356,712713,712712,1425425,619.0401768684387,0.07379914449768421
357357,714715,714714,1429429,620.838241815567,0.07269143618088947
358358,716717,716716,1433433,622.3816299438477,0.07160062451453086
359359,718719,718718,1437437,623.7922661304474,0.07052644579994194
360360,720721,720720,1441441,625.8118290901184,0.06946864058602387
361361,722723,722722,1445445,627.6198899745941,0.06842695359739537
362362,724725,724724,1449449,629.5348088741302,0.06740113366390688
363363,726727,726726,1453453,631.3125720024109,0.06639093365288318
364364,728729,728728,1457457,633.2668948173523,0.065396110401025
365365,730731,730730,1461461,634.9822328090668,0.06441642464744746
366366,732733,732732,1465465,636.7290461063385,0.06345164096933331
367367,734735,734734,1469469,638.830276966095,0.06250152771713147
368368,736737,736736,1473473,640.5057799816132,0.061565856952483955
369369,738739,738738,1477477,642.1734538078308,0.06064440438535712
370370,740741,740740,1481481,644.1469750404358,0.05973694931390128
371371,742743,742742,1485485,645.8243868350983,0.05884327456453775
372372,744745,744744,1489489,647.2769720554352,0.057963166432955404
373373,746747,746746,1493493,648.9276819229126,0.05709641462772197
374374,748749,748748,1497497,650.8939108848572,0.05624281221162164
375375,750751,750750,1501501,652.9153180122375,0.055402155548222254
376376,752753,752752,1505505,654.4899549484253,0.05457424424537294
377377,754755,754754,1509509,655.9602048397064,0.053758881102453415
378378,756757,756756,1513513,657.474662065506,0.05295587205750962
379379,758759,758758,1517517,659.0079698562622,0.052165026134844084
380380,760761,760760,1521521,660.5581789016724,0.05138615539510738
381381,762763,762762,1525525,662.0801811218262,0.050619074884025395
382382,764765,764764,1529529,663.6221551895142,0.049863602583513966
383383,766767,766766,1533533,665.2602179050446,0.049119559364157794
384384,768769,768768,1537537,666.8516569137573,0.048386768936097724
385385,770771,770770,1541541,668.4445359706879,0.04766505780355601
386386,772773,772772,1545545,670.2754330635071,0.046954255219361585
387387,774775,774774,1549549,672.1788399219513,0.04625419313765633
388388,776777,776776,1553553,673.7409899234772,0.04556470617171726
389389,778779,778778,1557557,675.3825340270996,0.04488563154939129
390390,780781,780780,1561561,676.9084801673889,0.04421680907080372
391391,782783,782782,1565565,678.462819814682,0.04355808106504355
392392,784785,784784,1569569,680.061821937561,0.04290929235105523
393393,786787,786786,1573573,681.6637001037598,0.0422702901937555
394394,788789,788788,1577577,684.1441879272461,0.0416409242671989
395395,790791,790790,1581581,685.8457140922546,0.04102104661365047
396396,792793,792792,1585585,688.4269239902496,0.04041051160470488
397397,794795,794794,1589589,690.9165678024292,0.039809175904565564
398398,796797,796796,1593593,692.7332179546356,0.039216898431618574
399399,798799,798798,1597597,694.3697049617767,0.038633540322393856
400400,800801,800800,1601601,696.0239808559418,0.03805896489495808
401401,802803,802802,1605605,697.5905921459198,0.03749303761412648
402402,804805,804804,1609609,699.180716753006,0.03693562605610623
403403,806807,806806,1613613,700.8056309223175,0.03638659987439041
404404,808809,808808,1617617,702.3442749977112,0.03584583076622039
405405,810811,810810,1621621,703.8180329799652,0.03531319243916187
406406,812813,812812,1625625,705.4626219272614,0.03478856057881785
407407,814815,814814,1629629,707.0664420127869,0.03427181281733738
408408,816817,816816,1633633,708.7188141345978,0.033762828700105274
409409,818819,818818,1637637,710.2664699554443,0.03326148965754783
410410,820821,820820,1641641,711.7947678565979,0.032767678972163594
411411,822823,822822,1645645,713.373703956604,0.03228128175044276
412412,824825,824824,1649649,714.8350191116333,0.031802184892740115
413413,826827,826826,1653653,716.4481670856476,0.031330277063716494
414414,828829,828828,1657657,718.087563753128,0.03086544866573604
415415,830831,830830,1661661,719.5986020565033,0.03040759180908026
416416,832833,832832,1665665,721.0676691532135,0.029956600285345303
417417,834835,834834,1669669,722.5775728225708,0.029512369540384498
418418,836837,836836,1673673,724.3216478824615,0.029074796647819312
419419,838839,838838,1677677,726.0019710063934,0.02864378028266401
420420,840841,840840,1681681,727.6663110256195,0.028219220695518743
421421,842843,842842,1685685,729.7207469940186,0.027801019688240558
422422,844845,844844,1689689,731.2978367805481,0.027389080587681747
423423,846847,846846,1693693,733.4269268512726,0.0269833082227251
424424,848849,848848,1697697,736.7841098308563,0.026583608899272804
425425,850851,850850,1701701,739.3764219284058,0.02618989037694064
426426,852853,852852,1705705,741.6490890979767,0.025802061845752178
427427,854855,854854,1709709,744.1863691806793,0.025420033903856165
428428,856857,856856,1713713,746.2378540039062,0.02504371853410703
429429,858859,858858,1717717,747.9747169017792,0.02467302908291913
430430,860861,860860,1721721,749.6189799308777,0.02430788023787045
431431,862863,862862,1725725,751.1734759807587,0.023948188007011595
432432,864865,864864,1729729,752.7681059837341,0.023593869696696856
433433,866867,866866,1733733,754.2743828296661,0.02324484389259851
434434,868869,868868,1737737,755.7419819831848,0.022901030438106318
435435,870871,870870,1741741,757.239599943161,0.022562350414659704
436436,872873,872872,1745745,759.0637068748474,0.022228726121966247
437437,874875,874874,1749749,760.9606280326843,0.021900081059357035
438438,876877,876876,1753753,762.6018781661987,0.02157633990634622
439439,878879,878878,1757757,764.5117998123169,0.021257428502849507
440440,880881,880880,1761761,766.5312139987946,0.02094327383304062
441441,882883,882882,1765765,768.3320798873901,0.0206338040055698
442442,884885,884884,1769769,769.8804459571838,0.02032894823605602
443443,886887,886886,1773773,771.3542490005493,0.02002863683014766
444444,888889,888888,1777777,772.9983351230621,0.019732801165673663
445445,890891,890890,1781781,774.5590941905975,0.01944137367604526
446446,892893,892892,1785785,776.1016359329224,0.01915428783331663
447447,894895,894894,1789789,777.5996849536896,0.018871478132496122
448448,896897,896896,1793793,779.0565729141235,0.018592880074493223
449449,898899,898898,1797797,780.6422238349915,0.018318430150884524
450450,900901,900900,1801801,782.1979489326477,0.01804806582811125
451451,902903,902902,1805805,783.8035228252411,0.01778172553213153
452452,904905,904904,1809809,785.3429498672485,0.017519348633527443
453453,906907,906906,1813813,786.8189399242401,0.017260875432384637
454454,908909,908908,1817817,788.304477930069,0.017006247143513065
455455,910911,910910,1821821,789.8129739761353,0.0167554058832593
456456,912913,912912,1825825,791.343444108963,0.016508294653135636
457457,914915,914914,1829829,792.9946839809418,0.016264857328565085
458458,916917,916916,1833833,794.5882499217987,0.01602503864285154
459459,918919,918918,1837837,796.2825980186462,0.015788784175242654
460460,920921,920920,1841841,798.0063519477844,0.015556040337855848
461461,922923,922922,1845845,800.505469083786,0.015326754360444284
462462,924925,924924,1849849,802.2385580539703,0.015100874280392418
463463,926927,926926,1853853,804.3967199325562,0.01487834892839146
464464,928929,928928,1857857,805.987212896347,0.01465912791672963
465465,930931,930930,1861861,807.6101651191711,0.014443161626559231
466466,932933,932932,1865865,809.3756580352783,0.014230401196073217
467467,934935,934934,1869869,811.1825728416443,0.014020798509363885
468468,936937,936936,1873873,812.7694659233093,0.013814306183576264
469469,938939,938938,1877877,814.3181698322296,0.013610877558562606
470470,940941,940940,1881881,815.892914056778,0.013410466684945277
471471,942943,942942,1885885,817.6385819911957,0.013213028313202813
472472,944945,944944,1889889,819.5301997661591,0.013018517883097047
473473,946947,946946,1893893,821.7420098781586,0.012826891512759175
474474,948949,948948,1897897,824.0959408283234,0.012638105987775816
475475,950951,950950,1901901,826.1199538707733,0.012452118750957197
476476,952953,952952,1905905,827.9618000984192,0.012268887892901148
477477,954955,954954,1909909,829.7815268039703,0.012088372140738102
478478,956957,956956,1913913,832.0713858604431,0.011910530849263523
479479,958959,958958,1917917,833.9903299808502,0.011735323990478719
480480,960961,960960,1921921,837.0897009372711,0.011562712143927456
481481,962963,962962,1925925,839.1562850475311,0.01139265648851051
482482,964965,964964,1929929,841.0239889621735,0.011225118792140165
483483,966967,966966,1933933,843.1007080078125,0.01106006140196314
484484,968969,968968,1937937,845.1555318832397,0.010897447236970947
485485,970971,970970,1941941,847.4159939289093,0.010737239778450203
486486,972973,972972,1945945,849.4353170394897,0.010579403061001358
487487,974975,974974,1949949,851.4134228229523,0.010423901664353252
488488,976977,976976,1953953,853.3664228916168,0.010270700704609226
489489,978979,978978,1957957,855.2427349090576,0.010119765826516414
490490,980981,980980,1961961,857.2877569198608,0.009971063194484486
491491,982983,982982,1965965,859.3593330383301,0.009824559485423379
492492,984985,984984,1969969,861.252995967865,0.009680221880444151
493493,986987,986986,1973973,863.0996398925781,0.00953801805690091
494494,988989,988988,1977977,864.794037103653,0.009397916180660104
495495,990991,990990,1981981,867.1613368988037,0.009259884899961435
496496,992993,992992,1985985,869.2286639213562,0.009123893335072353
497497,994995,994994,1989989,871.4325180053711,0.008989911074650081
498498,996997,996996,1993993,873.0712480545044,0.008857908165282424
499499,998999,998998,1997997,874.6091821193695,0.008727855106940297
500501,1001003,1001002,2002005,876.9717299938202,0.00859959579054248
501502,1003005,1003004,2006009,878.5755898952484,0.008473357582261087
502503,1005007,1005006,2010013,880.2785937786102,0.008348983339942606
503504,1007009,1007008,2014017,882.4516260623932,0.008226445303876062
504505,1009011,1009010,2018021,884.4257628917694,0.008105716133513852
505506,1011013,1011012,2022025,886.3976330757141,0.00798676889996841
506507,1013015,1013014,2026029,888.3215570449829,0.007869577080214185
507508,1015017,1015016,2030033,891.1111009120941,0.007754114551175917
508509,1017019,1017018,2034037,893.396087884903,0.007640355583134806
509510,1019021,1019020,2038041,895.3021910190582,0.007528274833589421
510511,1021023,1021022,2042045,897.3537061214447,0.0074178473416850466
511512,1023025,1023024,2046049,899.8741579055786,0.007309048522643025
512513,1025027,1025026,2050053,902.4229238033295,0.00720185416082586
513514,1027029,1027028,2054057,904.3198537826538,0.007096240405644494
514515,1029031,1029030,2058061,906.84565782547,0.006992183764850779
515516,1031033,1031032,2062065,908.5179579257965,0.006889661099080513
516517,1033035,1033034,2066069,910.1490440368652,0.006788649617419651
517518,1035037,1035036,2070073,912.3793859481812,0.0066891268711515295
518519,1037039,1037038,2074077,914.4166448116302,0.006591070748640959
519520,1039041,1039040,2078081,916.6821398735046,0.006494459470559377
520521,1041043,1041042,2082085,918.3181049823761,0.0063992715848826265
521522,1043045,1043044,2086089,920.5580580234528,0.006305485961206614
522523,1045047,1045046,2090093,922.4653630256653,0.006213081786540897
523524,1047049,1047048,2094097,924.6560459136963,0.00612203855973803
524525,1049051,1049050,2098101,926.5708329677582,0.006032336087855583
525526,1051053,1051052,2102105,928.8300700187683,0.005943954480585489
526527,1053055,1053054,2106109,930.5555238723755,0.005856874145592883
527528,1055057,1055056,2110113,932.2247791290283,0.005771075784991808
528529,1057059,1057058,2114117,933.9365799427032,0.005686540388865069
529530,1059061,1059060,2118121,935.6209769248962,0.005603249233217866
530531,1061063,1061062,2122125,937.5695340633392,0.00552118387452083
531532,1063065,1063064,2126129,939.382443189621,0.00544032614459411
532533,1065067,1065066,2130133,941.1519770622253,0.005360658148447328
533534,1067069,1067068,2134137,942.9054238796234,0.005282162258026801
534535,1069071,1069070,2138141,945.208655834198,0.0052048211096007435
535536,1071073,1071072,2142145,947.0988628864288,0.005128617599552854
536537,1073075,1073074,2146149,949.147971868515,0.005053534879380095
537538,1075077,1075076,2150153,950.88294506073,0.004979556353191583
538539,1077079,1077078,2154157,952.6901121139526,0.004906665672933741
539540,1079081,1079080,2158161,954.5809559822083,0.004834846735207066
540541,1081083,1081082,2162165,956.5117309093475,0.00476408367728709
541542,1083085,1083084,2166169,958.1338467597961,0.004694360873259029
542543,1085087,1085086,2170173,960.5444979667664,0.004625662930948238
543544,1087089,1087088,2174177,962.6839168071747,0.0045579746880548555
544545,1089091,1089090,2178181,964.8709740638733,0.004491281208629516
545546,1091093,1091092,2182185,966.7732150554657,0.004425567780003803
546547,1093095,1093094,2186189,968.9131798744202,0.004360819908697522
547548,1095097,1095096,2190193,970.8889639377594,0.004297023317917592
548549,1097099,1097098,2194197,972.931834936142,0.004234163943806379
549550,1099101,1099100,2198201,974.9159018993378,0.004172227932485839
550551,1101103,1101102,2202205,976.7013189792633,0.00411120163630585
551552,1103105,1103104,2206209,978.6761898994446,0.004051071611684165
552553,1105107,1105106,2210213,981.1528720855713,0.003991824615127371
553554,1107109,1107108,2214217,983.2041611671448,0.003933447600616091
554555,1109111,1109110,2218221,985.0454449653625,0.003875927716762817
555556,1111113,1111112,2222225,986.8987939357758,0.003819252303628673
556557,1113115,1113114,2226229,988.7714738845825,0.003763408889653874
557558,1115117,1115116,2230233,990.6970720291138,0.003708385189497676
558559,1117119,1117118,2234237,993.1144127845764,0.003654169100400395
559560,1119121,1119120,2238241,995.26713514328,0.0036007486999096727
560561,1121123,1121122,2242245,997.9448490142822,0.0035481122433793644
561562,1123125,1123124,2246249,999.8556339740753,0.0034962481604452478
562563,1125127,1125126,2250253,1001.9260160923004,0.003445145053547094
563564,1127129,1127128,2254257,1003.772962808609,0.003394791693949628
564565,1129131,1129130,2258261,1005.371297121048,0.0033451770207193476
565566,1131133,1131132,2262265,1007.2165961265564,0.0032962901374276043
566567,1133135,1133134,2266269,1009.1328480243683,0.003248120308739999
567568,1135137,1135136,2270273,1011.0434677600861,0.003200656959961634
568569,1137139,1137138,2274277,1012.6643040180206,0.0031538896731717614
569570,1139141,1139140,2278281,1014.333172082901,0.0031078081859732265
570571,1141143,1141142,2282285,1015.9527750015259,0.003062402386717622
571572,1143145,1143144,2286289,1017.7954609394073,0.003017662316096903
572573,1145147,1145146,2290293,1020.7842938899994,0.002973578161459045
573574,1147149,1147148,2294297,1022.477698802948,0.002930140256580671
574575,1149151,1149150,2298301,1024.1235001087189,0.002887339078029072
575576,1151153,1151152,2302305,1026.1263377666473,0.002845165244366399
576577,1153155,1153154,2306309,1027.66081905365,0.002803609513648553
577578,1155157,1155156,2310313,1029.2135691642761,0.0027626627802419534
578579,1157159,1157158,2314317,1031.6785538196564,0.002722316074596165
579580,1159161,1159160,2318321,1033.9846711158752,0.0026825605596059177
580581,1161163,1161162,2322325,1035.5047571659088,0.002643387529587926
581582,1163165,1163164,2326329,1036.9898898601532,0.0026047884078934658
582583,1165167,1165166,2330333,1038.4939589500427,0.0025667547449756967
583584,1167169,1167168,2334337,1039.967668056488,0.0025292782169117345
584585,1169171,1169170,2338341,1041.6126170158386,0.0024923506227878534
585586,1171173,1171172,2342345,1043.1584689617157,0.0024559638834489306
586587,1173175,1173174,2346349,1044.6671209335327,0.0024201100396794573
587588,1175177,1175176,2350353,1046.163341999054,0.0023847812500434884
588589,1177179,1177178,2354357,1047.6545929908752,0.0023499697889519666
589590,1179181,1179180,2358361,1049.1608378887177,0.002315668046207975
590591,1181183,1181182,2362365,1050.6289110183716,0.0022818685231413838
591592,1183185,1183184,2366369,1052.1176459789276,0.0022485638329499125
592593,1185187,1185186,2370373,1053.60014295578,0.002215746698084331
593594,1187189,1187188,2374377,1055.084142923355,0.0021834099487705316
594595,1189191,1189190,2378381,1056.5601181983948,0.0021515465210768525
595596,1191193,1191192,2382385,1058.040647983551,0.002120149455890896
596597,1193195,1193194,2386389,1059.5090000629425,0.0020892118969868534
597598,1195197,1195196,2390393,1060.9876430034637,0.0020587270898886345
598599,1197199,1197198,2394397,1062.471673965454,0.002028688379596133
599600,1199201,1199200,2398401,1063.960350036621,0.0019990892099031043
600601,1201203,1201202,2402405,1065.4211149215698,0.001969923121123429
601602,1203205,1203204,2406409,1066.9044160842896,0.0019411837497500528
602603,1205207,1205206,2410413,1068.3845839500427,0.0019128648261812486
603604,1207209,1207208,2414417,1069.8677451610565,0.0018849601733563759
604605,1209211,1209210,2418421,1071.3730299472809,0.0018574637050505771
605606,1211213,1211212,2422425,1072.8705749511719,0.001830369425988465
606607,1213215,1213214,2426429,1074.383271932602,0.0018036714290019518
607608,1215217,1215216,2430433,1075.850989818573,0.0017773638942344405
608609,1217219,1217218,2434437,1077.3372559547424,0.0017514410874355235
609610,1219221,1219220,2438441,1078.777979850769,0.0017258973599609817
610611,1221223,1221222,2442445,1080.077645778656,0.001700727145930614
611612,1223225,1223224,2446449,1081.3844170570374,0.0016759249615461158
612613,1225227,1225226,2450453,1082.6279110908508,0.0016514854047500194
613614,1227229,1227228,2454457,1084.3220229148865,0.0016274031526108956
614615,1229231,1229230,2458461,1086.0358619689941,0.0016036729606412337
615616,1231233,1231232,2462465,1087.6390800476074,0.00158028966245638
616617,1233235,1233234,2466469,1089.2484109401703,0.0015572481673871152
617618,1235237,1235236,2470473,1090.8872079849243,0.0015345434600249064
618619,1237239,1237238,2474477,1092.4597730636597,0.0015121705989713519
619620,1239241,1239240,2478481,1094.8574759960175,0.0014901247160423736
620621,1241243,1241242,2482485,1096.791396856308,0.0014684010139944803
621622,1243245,1243244,2486489,1098.4171109199524,0.001446994767434262
622623,1245247,1245246,2490493,1100.1244518756866,0.00142590132031728
623624,1247249,1247248,2494497,1101.8116188049316,0.0014051160846975108
624625,1249251,1249250,2498501,1103.3087661266327,0.0013846345407273475
625626,1251253,1251252,2502505,1104.780993938446,0.0013644522352933564
626627,1253255,1253254,2506509,1106.317270040512,0.0013445647808794092
627628,1255257,1255256,2510513,1107.7915210723877,0.001324967854429815
628629,1257259,1257258,2514517,1109.3613109588623,0.0013056571966671981
629630,1259261,1259260,2518521,1110.9052579402924,0.0012866286112966918
630631,1261263,1261262,2522525,1112.4609949588776,0.0012678779638690685
631632,1263265,1263264,2526529,1113.932373046875,0.0012494011803028116
632633,1265267,1265266,2530533,1115.4272768497467,0.0012311942472251758
633634,1267269,1267268,2534537,1116.9079189300537,0.001213253210039511
634635,1269271,1269270,2538541,1118.3680970668793,0.0011955741720157675
635636,1271273,1271272,2542545,1119.904606103897,0.001178153294972617
636637,1273275,1273274,2546549,1121.3769309520721,0.001160986796094221
637638,1275277,1275276,2550553,1122.8546059131622,0.0011440709483849787
638639,1277279,1277278,2554557,1124.3504309654236,0.0011274020805558393
639640,1279281,1279280,2558561,1125.8294730186462,0.0011109765745231925
640641,1281283,1281282,2562565,1127.3055770397186,0.0010947908657499283
641642,1283285,1283284,2566569,1128.8044650554657,0.0010788414422222559
642643,1285287,1285286,2570573,1130.2579538822174,0.0010631248436538954
643644,1287289,1287288,2574577,1131.7844140529633,0.0010476376598944626
644645,1289291,1289290,2578581,1133.2597961425781,0.0010323765325210843
645646,1291293,1291292,2582585,1134.7624979019165,0.0010173381512004198
646647,1293295,1293294,2586589,1136.231286764145,0.001002519254825529
647648,1295297,1295296,2590593,1137.7213609218597,0.0009879166298105702
648649,1297299,1297298,2594597,1139.1755480766296,0.0009735271106592336
649650,1299301,1299300,2598601,1140.6670908927917,0.0009593475776910054
650651,1301303,1301302,2602605,1142.148628950119,0.000945374957268541
651652,1303305,1303304,2606609,1143.6043128967285,0.000931606221115544
652653,1305307,1305306,2610613,1145.0676350593567,0.0009180383852935847
653654,1307309,1307308,2614617,1146.5252950191498,0.0009046685099747265
654655,1309311,1309310,2618621,1147.9916639328003,0.0008914936981909705
655656,1311313,1311312,2622625,1149.4833180904388,0.0008785110958342557
656657,1313315,1313314,2626629,1150.9694731235504,0.0008657178906332774
657658,1315317,1315316,2630633,1152.4259819984436,0.0008531113114713662
658659,1317319,1317318,2634637,1153.9009108543396,0.0008406886283864878
659660,1319321,1319320,2638641,1155.4164538383484,0.0008284471512070013
660661,1321323,1321322,2642645,1156.9141600131989,0.0008163842288695378
661662,1323325,1323324,2646649,1158.369174003601,0.0008044972502148084
662663,1325327,1325326,2650653,1159.8423500061035,0.0007927836417138678
663664,1327329,1327328,2654657,1161.3172209262848,0.0007812408679228611
664665,1329331,1329330,2658661,1162.8587930202484,0.0007698664305735292
665666,1331333,1331332,2662665,1164.353096961975,0.0007586578680047751
666667,1333335,1333334,2666669,1165.8622069358826,0.0007476127547079159
667668,1335337,1335336,2670673,1167.29869389534,0.000736728700758249
668669,1337339,1337338,2674677,1168.7741258144379,0.0007260033514739916
669670,1339341,1339340,2678681,1170.2696499824524,0.0007154343868478463
670671,1341343,1341342,2682685,1171.7576739788055,0.0007050195201827592
671672,1343345,1343344,2686689,1173.2124750614166,0.0006947564993424749
672673,1345347,1345346,2690693,1174.6972448825836,0.0006846431045914869
673674,1347349,1347348,2694697,1176.1436760425568,0.0006746771488224113
674675,1349351,1349350,2698701,1177.6081931591034,0.0006648564775559862
675676,1351353,1351352,2702705,1179.1008431911469,0.0006551789667810226
676677,1353355,1353354,2706709,1180.5615129470825,0.0006456425251144537
677678,1355357,1355356,2710713,1182.0388538837433,0.0006362450906181039
678679,1357359,1357358,2714717,1183.5355851650238,0.0006269846320492434
679680,1359361,1359360,2718721,1185.030529975891,0.0006178591481784679
680681,1361363,1361362,2722725,1186.483638048172,0.0006088666668802034
681682,1363365,1363364,2726729,1187.9643337726593,0.0006000052451327065
682683,1365367,1365366,2730733,1189.4364838600159,0.0005912729679948825
683684,1367369,1367368,2734737,1190.9025061130524,0.0005826679490610331
684685,1369371,1369370,2738741,1192.405996799469,0.000574188329323988
685686,1371373,1371372,2742745,1194.081160068512,0.0005658322767203572
686687,1373375,1373374,2746749,1195.9119699001312,0.0005575979870400261
687688,1375377,1375376,2750753,1198.0495479106903,0.0005494836814250448
688689,1377379,1377378,2754757,1199.7810430526733,0.0005414876078475572
689690,1379381,1379380,2758761,1201.4741787910461,0.0005336080395181853
690691,1381383,1381382,2762765,1203.3126118183136,0.0005258432749997155
691692,1383385,1383384,2766769,1205.2339000701904,0.0005181916379797258
692693,1385387,1385386,2770773,1207.1239268779755,0.000510651476588464
693694,1387389,1387388,2774777,1208.818778038025,0.0005032211631714745
694695,1389391,1389390,2778781,1210.8859779834747,0.0004958990938348506
695696,1391393,1391392,2782785,1212.629059791565,0.0004886836883315482
696697,1393395,1393394,2786789,1214.7946310043335,0.00048157338937926397
697698,1395397,1395396,2790793,1216.9837248325348,0.00047456666277412296
698699,1397399,1397398,2794797,1219.1485919952393,0.0004676619963674966
699700,1399401,1399400,2798801,1221.7541148662567,0.00046085790074812394
700701,1401403,1401402,2802805,1224.3597960472107,0.00045415290765049576
701702,1403405,1403404,2806809,1226.1448090076447,0.00044754557063697575
702703,1405407,1405406,2810813,1228.007661819458,0.0004410344647567399
703704,1407409,1407408,2814817,1230.1437249183655,0.0004346181851815345
704705,1409411,1409410,2818821,1232.020499944687,0.0004282953484562313
705706,1411413,1411412,2822825,1234.4600939750671,0.00042206459045246447
706707,1413415,1413414,2826829,1236.2216238975525,0.00041592456818762
707708,1415417,1415416,2830833,1238.0804388523102,0.0004098739569826648
708709,1417419,1417418,2834837,1239.7527210712433,0.00040391145296325703
709710,1419421,1419420,2838841,1241.5778200626373,0.00039803577010388835
710711,1421423,1421422,2842845,1243.5030410289764,0.00039224564193318656
711712,1423425,1423424,2846849,1245.3506209850311,0.00038653982005598664
712713,1425427,1425426,2850853,1247.0711069107056,0.0003809170749491386
713714,1427429,1427428,2854857,1248.8661918640137,0.00037537619448357873
714715,1429431,1429430,2858861,1250.6152169704437,0.00036991598449276353
715716,1431433,1431432,2862865,1252.3947370052338,0.00036453526820423576
716717,1433435,1433434,2866869,1254.1048710346222,0.0003592328863533112
717718,1435437,1435436,2870873,1255.7681379318237,0.000354007696159897
718719,1437439,1437438,2874877,1257.6842529773712,0.0003488585717832393
719720,1439441,1439440,2878881,1259.401687860489,0.0003437844042082361
720721,1441443,1441442,2882885,1261.1539878845215,0.0003387840999948821
721722,1443445,1443444,2886889,1263.241196155548,0.00033385658207407687
722723,1445447,1445446,2890893,1264.8056960105896,0.00032900078883812967
723724,1447449,1447448,2894897,1266.3042788505554,0.00032421567459550715
724725,1449451,1449450,2898901,1267.8601460456848,0.0003195002088887122
725726,1451453,1451452,2902905,1269.3553721904755,0.00031485337603953667
726727,1453455,1453454,2906909,1270.8700859546661,0.00031027417526274803
727728,1455457,1455456,2910913,1272.4684660434723,0.00030576162089346326
728729,1457459,1457458,2914917,1273.9979348182678,0.00030131474090921984
729730,1459461,1459460,2918921,1275.4946780204773,0.00029693257783947047
730731,1461463,1461462,2922925,1276.983680009842,0.0002926141887655831
731732,1463465,1463464,2926929,1278.6192059516907,0.00028835864316079096
732733,1465467,1465466,2930933,1280.2253148555756,0.0002841650260734241
733734,1467469,1467468,2934937,1281.7300369739532,0.0002800324336931226
734735,1469471,1469470,2938941,1283.217406988144,0.00027595997721618915
735736,1471473,1471472,2942945,1284.7103779315948,0.00027194677988973126
736737,1473475,1473474,2946949,1286.1972959041595,0.0002679919781485296
737738,1475477,1475476,2950953,1287.9405121803284,0.00026409472093291697
738739,1477479,1477478,2954957,1289.525321006775,0.00026025416934771783
739740,1479481,1479480,2958961,1291.0595290660858,0.0002564694973443693
740741,1481483,1481482,2962965,1292.5289280414581,0.0002527398905840528
741742,1483485,1483484,2966969,1294.0035500526428,0.0002490645463240071
742743,1485487,1485486,2970973,1295.614806175232,0.00024544267421333643
743744,1487489,1487488,2974977,1297.308376789093,0.00024187349481508136
744745,1489491,1489490,2978981,1299.35098195076,0.00023835624062940042
745746,1491493,1491492,2982985,1300.9177868366241,0.0002348901548430149
746747,1493495,1493494,2986989,1302.589998960495,0.0002314744921250167
747748,1495497,1495496,2990993,1304.1508538722992,0.00022810851783106045
748749,1497499,1497498,2994997,1305.730689048767,0.00022479150788967672
749750,1499501,1499500,2999001,1307.5523359775543,0.0002215227492570193
750751,1501503,1501502,3003005,1309.305125951767,0.00021830153877999692
751752,1503505,1503504,3007009,1310.8703918457031,0.00021512718365102046
752753,1505507,1505506,3011013,1312.700756072998,0.00021199900186275045
753754,1507509,1507508,3015017,1314.3228991031647,0.00020891632038910757
754755,1509511,1509510,3019021,1315.9773478507996,0.00020587847677688842
755756,1511513,1511512,3023025,1317.4515228271484,0.00020288481755414978
756757,1513515,1513514,3027029,1318.9692900180817,0.00019993469959445065
757758,1515517,1515516,3031033,1320.5043759346008,0.0001970274884115497
758759,1517519,1517518,3035037,1321.9696309566498,0.00019416255929627368
759760,1519521,1519520,3039041,1323.4395008087158,0.00019133929640702263
760761,1521523,1521522,3043045,1324.9675879478455,0.0001885570928834568
761762,1523525,1523524,3047049,1327.054015159607,0.00018581535084649659
762763,1525527,1525526,3051053,1328.58455991745,0.0001831134810572621
763764,1527529,1527528,3055057,1330.0781960487366,0.0001804509029170731
764765,1529531,1529530,3059061,1331.5608370304108,0.00017782704424007534
765766,1531533,1531532,3063065,1333.1238911151886,0.0001752413411395537
766767,1533535,1533534,3067069,1334.6973600387573,0.00017269323825530591
767768,1535537,1535536,3071073,1336.2416388988495,0.00017018218807152152
768769,1537539,1537538,3075077,1337.9591670036316,0.0001677076510304687
769770,1539541,1539540,3079081,1339.7335150241852,0.00016526909530512057
770771,1541543,1541542,3083085,1341.6031160354614,0.00016286599748127628
771772,1543545,1543544,3087089,1343.2406568527222,0.00016049784107963205
772773,1545547,1545546,3091093,1344.7744960784912,0.00015816411735158908
773774,1547549,1547548,3095097,1346.2995069026947,0.00015586432527925353
774775,1549551,1549550,3099101,1347.7879610061646,0.00015359797066594183
775776,1551553,1551552,3103105,1349.3402349948883,0.00015136456670461484
776777,1553555,1553554,3107109,1350.8788800239563,0.00014916363420525158
777778,1555557,1555556,3111113,1352.3724389076233,0.00014699470000323345
778779,1557559,1557558,3115117,1353.8494579792023,0.00014485729855095997
779780,1559561,1559560,3119121,1355.3235857486725,0.00014275097078098042
780781,1561563,1561562,3123125,1356.8142659664154,0.00014067526444705436
781782,1563565,1563564,3127129,1358.2862060070038,0.00013862973401046474
782783,1565567,1565566,3131133,1359.7849490642548,0.00013661394007158378
783784,1567569,1567568,3135137,1361.2767519950867,0.0001346274499383071
784785,1569571,1569570,3139141,1362.7690551280975,0.0001326698370576196
785786,1571573,1571572,3143145,1364.2494418621063,0.000130740681242969
786787,1573575,1573574,3147149,1365.765552997589,0.0001288395682195187
787788,1575577,1575576,3151153,1367.2521770000458,0.00012696609019258176
788789,1577579,1577578,3155157,1368.7487120628357,0.00012511984448337898
789790,1579581,1579580,3159161,1370.2330009937286,0.00012330043568908877
790791,1581583,1581582,3163165,1371.7150721549988,0.00012150747215855517
791792,1583585,1583584,3167169,1373.2070689201355,0.00011974057031238772
792793,1585587,1585586,3171173,1374.7159719467163,0.00011799934986811422
793794,1587589,1587588,3175177,1376.255264043808,0.00011628343759184645
794795,1589591,1589590,3179181,1377.7171819210052,0.00011459246536560386
795796,1591593,1591592,3183185,1379.2202739715576,0.0001129260701873136
796797,1593595,1593594,3187189,1380.7130959033966,0.00011128389451187104
797798,1595597,1595596,3191193,1382.213355064392,0.0001096655857963924
798799,1597599,1597598,3195197,1383.710401058197,0.00010807079695496213
799800,1599601,1599600,3199201,1385.1981270313263,0.00010649918567651184
800801,1601603,1601602,3203205,1386.6637499332428,0.00010495041499325453
801802,1603605,1603604,3207209,1388.1383697986603,0.00010342415259856352
802803,1605607,1605606,3211213,1389.6362178325653,0.0001019200710743462
803804,1607609,1607608,3215217,1391.1277358531952,0.0001004378472089229
804805,1609611,1609610,3219221,1392.461769104004,9.89771638160164e-05
805806,1611613,1611612,3223225,1393.83758187294,9.753770711995458e-05
806807,1613615,1613614,3227229,1395.1213698387146,9.611916834728618e-05
807808,1615617,1615616,3231233,1396.4075741767883,9.47212433857203e-05
808809,1617619,1617618,3235237,1397.673283815384,9.334363244306587e-05
809810,1619621,1619620,3239241,1398.9189131259918,9.198603970617114e-05
810811,1621623,1621622,3243245,1400.2110919952393,9.064817447779205e-05
811812,1623625,1623624,3247249,1401.9012858867645,8.932974958497653e-05
812813,1625627,1625626,3251253,1403.4575598239899,8.803048206118547e-05
813814,1627629,1627628,3255257,1404.974997997284,8.675009382841381e-05
814815,1629631,1629630,3259261,1406.488399028778,8.548830965082743e-05
815816,1631633,1631632,3263265,1408.0382328033447,8.424485952218674e-05
816817,1633635,1633634,3267269,1409.6905591487885,8.301947650579677e-05
817818,1635637,1635636,3271273,1411.312332868576,8.181189775768871e-05
818819,1637639,1637638,3275277,1412.8594398498535,8.062186464030674e-05
819820,1639641,1639640,3279281,1414.4943478107452,7.944912215407385e-05
820821,1641643,1641642,3283285,1416.2201948165894,7.829341825527081e-05
821822,1643645,1643644,3287289,1417.916630744934,7.715450556133874e-05
822823,1645647,1645646,3291293,1419.5568799972534,7.603214010032389e-05
823824,1647649,1647648,3295297,1421.9481489658356,7.492608062875661e-05
824825,1649651,1649650,3299301,1424.9580838680267,7.38360905643276e-05
825826,1651653,1651652,3303305,1427.4926180839539,7.276193605321168e-05
826827,1653655,1653654,3307309,1431.4553129673004,7.17033869932493e-05
827828,1655657,1655656,3311313,1434.4900560379028,7.066021623813867e-05
828829,1657659,1657658,3315317,1437.1507759094238,6.963220039324369e-05
829830,1659661,1659660,3319321,1439.3630888462067,6.861911890609917e-05
830831,1661663,1661662,3323325,1441.3990769386292,6.762075497590558e-05
831832,1663665,1663664,3327329,1442.957545042038,6.663689430297381e-05
832833,1665667,1665666,3331333,1444.9156019687653,6.566732622559357e-05
833834,1667669,1667668,3335337,1447.1766159534454,6.471184281053866e-05
834835,1669671,1669670,3339341,1449.433270931244,6.377023930781434e-05
835836,1671673,1671672,3343345,1451.7362129688263,6.284231403697049e-05
836837,1673675,1673674,3347349,1453.6466779708862,6.192786804604111e-05
837838,1675677,1675676,3351353,1455.6601338386536,6.10267054526048e-05
838839,1677679,1677678,3355357,1457.4025838375092,6.013863298903743e-05
839840,1679681,1679680,3359361,1459.399132013321,5.926346034357266e-05
840841,1681683,1681682,3363365,1460.9141509532928,5.840100050136243e-05
841842,1683685,1683684,3367369,1462.4378628730774,5.7551068039174424e-05
842843,1685687,1685686,3371373,1464.0003778934479,5.671348117175512e-05
843844,1687689,1687688,3375377,1465.949858903885,5.5888060501274595e-05
844845,1689691,1689690,3379381,1467.9850549697876,5.507462878995284e-05
845846,1691693,1691692,3383385,1469.7522897720337,5.427301221061498e-05
846847,1693695,1693694,3387389,1471.8649649620056,5.348303886876238e-05
847848,1695697,1695696,3391393,1473.4828927516937,5.2704539598380507e-05
848849,1697699,1697698,3395397,1475.8232789039612,5.193734739350475e-05
849850,1699701,1699700,3399401,1477.946534872055,5.118129809034144e-05
850851,1701703,1701702,3403405,1480.182512998581,5.043622968514683e-05
851852,1703705,1703704,3407409,1482.3532729148865,4.9701982561600744e-05
852853,1705707,1705706,3411413,1484.322496175766,4.897839960449346e-05
853854,1707709,1707708,3415417,1486.23433303833,4.826532551760465e-05
854855,1709711,1709710,3419421,1488.2088038921356,4.756260784688493e-05
855856,1711713,1711712,3423425,1490.0609829425812,4.687009584358748e-05
856857,1713715,1713714,3427429,1491.9202148914337,4.618764148744958e-05
857858,1715717,1715716,3431433,1493.7153811454773,4.5515098463511094e-05
858859,1717719,1717718,3435437,1495.5194280147552,4.4852322616861784e-05
859860,1719721,1719720,3439441,1497.2207729816437,4.419917218001501e-05
860861,1721723,1721722,3443445,1498.889818906784,4.3555507090786705e-05
861862,1723725,1723724,3447449,1500.71089220047,4.292118978810322e-05
862863,1725727,1725726,3451453,1502.4309980869293,4.229608384775929e-05
863864,1727729,1727728,3455457,1504.1096861362457,4.168005614246795e-05
864865,1729731,1729730,3459461,1505.8451888561249,4.107297445443692e-05
865866,1731733,1731732,3463465,1507.8136332035065,4.047470861223701e-05
866867,1733735,1733734,3467469,1510.0362861156464,3.9885130831862625e-05
867868,1735737,1735736,3471473,1512.0821089744568,3.930411446617654e-05
868869,1737739,1737738,3475477,1514.055408000946,3.8731535710212484e-05
869870,1739741,1739740,3479481,1516.0485620498657,3.816727121375152e-05
870871,1741743,1741742,3483485,1518.4001939296722,3.76112005824325e-05
871872,1743745,1743744,3487489,1520.4131951332092,3.706320489982318e-05
872873,1745747,1745746,3491493,1522.45693898201,3.65231665000465e-05
873874,1747749,1747748,3495497,1524.5003941059113,3.599097010464902e-05
874875,1749751,1749750,3499501,1526.508798122406,3.546650168573251e-05
875876,1751753,1751752,3503505,1528.6743409633636,3.494964857964078e-05
876877,1753755,1753754,3507509,1530.8451590538025,3.444030051014124e-05
877878,1755757,1755756,3511513,1532.9218399524689,3.39383486789302e-05
878879,1757759,1757758,3515517,1534.5282011032104,3.344368496982497e-05
879880,1759761,1759760,3519521,1536.0749080181122,3.295620388144016e-05
880881,1761763,1761762,3523525,1537.6527349948883,3.2475801049258735e-05
881882,1763765,1763764,3527529,1539.2162990570068,3.2002373700379394e-05
882883,1765767,1765766,3531533,1540.7616519927979,3.153582042614289e-05
883884,1767769,1767768,3535537,1542.2781729698181,3.107604118213203e-05
884885,1769771,1769770,3539541,1543.7680039405823,3.062293774291902e-05
885886,1771773,1771772,3543545,1545.2808630466461,3.0176413247318123e-05
886887,1773775,1773774,3547549,1546.7944300174713,2.9736371971011977e-05
887888,1775777,1775776,3551553,1548.713536977768,2.930271955392527e-05
888889,1777779,1777778,3555557,1550.956955909729,2.8875363341285265e-05
889890,1779781,1779780,3559561,1552.588143825531,2.8454212156248104e-05
890891,1781783,1781782,3563565,1554.23175573349,2.8039175276717287e-05
891892,1783785,1783784,3567569,1555.8303561210632,2.7630164481706743e-05
892893,1785787,1785786,3571573,1557.4215638637543,2.722709189129091e-05
893894,1787789,1787788,3575577,1559.0495371818542,2.6829871217159962e-05
894895,1789791,1789790,3579581,1560.5685079097748,2.6438417535246117e-05
895896,1791793,1791792,3583585,1562.0602388381958,2.605264739941049e-05
896897,1793795,1793794,3587589,1563.5916140079498,2.5672477590887866e-05
897898,1795797,1795796,3591593,1565.5371007919312,2.5297827278336626e-05
898899,1797799,1797798,3595597,1567.2068359851837,2.4928615971475665e-05
899900,1799801,1799800,3599601,1569.040277004242,2.456476488532644e-05
900901,1801803,1801802,3603605,1570.5874419212341,2.4206196144405112e-05
901902,1803805,1803804,3607609,1572.7006359100342,2.385283289640938e-05
902903,1805807,1805806,3611613,1574.3484728336334,2.3504599880652677e-05
903904,1807809,1807808,3615617,1575.9580459594727,2.31614220638221e-05
904905,1809811,1809810,3619621,1577.4998998641968,2.2823226458967838e-05
905906,1811813,1811812,3623625,1579.318463087082,2.2489940306513745e-05
906907,1813815,1813814,3627629,1581.0266258716583,2.2161492665873084e-05
907908,1815817,1815816,3631633,1583.3741540908813,2.183781293751963e-05
908909,1817819,1817818,3635637,1584.885351896286,2.1518832113542885e-05
909910,1819821,1819820,3639641,1586.3469741344452,2.1204482095527055e-05
910911,1821823,1821822,3643645,1587.8667171001434,2.0894695126116858e-05
911912,1823825,1823824,3647649,1589.328775882721,2.058940549432009e-05
912913,1825827,1825826,3651653,1591.0559067726135,2.0288547602831386e-05
913914,1827829,1827828,3655657,1592.7813138961792,1.999205687752692e-05
914915,1829831,1829830,3659661,1594.3326921463013,1.9699870222211757e-05
915916,1831833,1831832,3663665,1595.8432919979095,1.9411924995438312e-05
916917,1833835,1833834,3667669,1597.3114178180695,1.9128159806314216e-05
917918,1835837,1835836,3671673,1598.9234960079193,1.8848513491320773e-05
918919,1837839,1837838,3675677,1600.384677886963,1.8572926705928694e-05
919920,1839841,1839840,3679681,1601.8462080955505,1.8301340332982363e-05
920921,1841843,1841842,3683685,1603.3594880104065,1.8033696164820867e-05
921922,1843845,1843844,3687689,1604.9359550476074,1.776993713065167e-05
922923,1845847,1845846,3691693,1607.0012230873108,1.7510006614429585e-05
923924,1847849,1847848,3695697,1608.4964399337769,1.7253849136977806e-05
924925,1849851,1849850,3699701,1609.9689939022064,1.7001410128614225e-05
925926,1851853,1851852,3703705,1612.1955008506775,1.6752635133343574e-05
926927,1853855,1853854,3707709,1614.1737768650055,1.6507471173099475e-05
927928,1855857,1855856,3711713,1615.5876460075378,1.6265865838249738e-05
928929,1857859,1857858,3715717,1616.8650479316711,1.6027767514970037e-05
929930,1859861,1859860,3719721,1619.315311908722,1.5793125157870236e-05
930931,1861863,1861862,3723725,1620.9788229465485,1.5561888403681223e-05
931932,1863865,1863864,3727729,1622.6626379489899,1.533400825337594e-05
932933,1865867,1865866,3731733,1626.1250689029694,1.510943582161417e-05
933934,1867869,1867868,3735737,1627.811075925827,1.4888122791489877e-05
934935,1869871,1869870,3739741,1629.485948085785,1.4670022096652247e-05
935936,1871873,1871872,3743745,1631.3667759895325,1.4455087011810974e-05
936937,1873875,1873874,3747749,1633.2183909416199,1.4243271721170458e-05
937938,1875877,1875876,3751753,1634.9651079177856,1.4034530636308773e-05
938939,1877879,1877878,3755757,1637.5993139743805,1.382881919198553e-05
939940,1879881,1879880,3759761,1639.7569789886475,1.3626093846141885e-05
940941,1881883,1881882,3763765,1641.572278022766,1.3426310601971636e-05
941942,1883885,1883884,3767769,1643.250303030014,1.3229427054284315e-05
942943,1885887,1885886,3771773,1644.8329319953918,1.3035401025263127e-05
943944,1887889,1887888,3775777,1646.373820066452,1.2844191132899141e-05
944945,1889891,1889890,3779781,1647.886962890625,1.2655756449930777e-05
945946,1891893,1891892,3783785,1649.5157661437988,1.2470056617530645e-05
946947,1893895,1893894,3787789,1651.0491700172424,1.2287052072679217e-05
947948,1895897,1895896,3791793,1652.5844161510468,1.2106703366043803e-05
948949,1897899,1897898,3795797,1654.073117017746,1.192897229884693e-05
949950,1899901,1899900,3799801,1655.6435749530792,1.1753820672311122e-05
950951,1901903,1901902,3803805,1657.0885059833527,1.1581211197153607e-05
951952,1903905,1903904,3807809,1658.5575828552246,1.1411106925152126e-05
952953,1905907,1905906,3811813,1660.0255570411682,1.1243471249144932e-05
953954,1907909,1907908,3815817,1661.4697279930115,1.107826847146498e-05
954955,1909911,1909910,3819821,1663.0807089805603,1.091546323550574e-05
955956,1911913,1911912,3823825,1664.622614145279,1.0755020866781706e-05
956957,1913915,1913914,3827829,1666.2312641143799,1.0596907145554724e-05
957958,1915917,1915916,3831833,1667.7876827716827,1.0441087965773477e-05
958959,1917919,1917918,3835837,1669.6672129631042,1.0287530244568188e-05
959960,1919921,1919920,3839841,1671.1684329509735,1.0136200899069081e-05
960961,1921923,1921922,3843845,1672.624459028244,9.987067983274756e-06
961962,1923925,1923924,3847849,1674.2891669273376,9.840099096436461e-06
962963,1925927,1925926,3851853,1675.7717578411102,9.695263543108013e-06
963964,1927929,1927928,3855857,1677.271973848343,9.55252937728801e-06
964965,1929931,1929930,3859861,1679.755931854248,9.41186692671181e-06
965966,1931933,1931932,3863865,1681.7612388134003,9.273245609620062e-06
966967,1933935,1933934,3867869,1683.2586650848389,9.136636322182312e-06
967968,1935937,1935936,3871873,1684.7193858623505,9.002009505820752e-06
968969,1937939,1937938,3875877,1686.1767120361328,8.869336056704924e-06
969970,1939941,1939940,3879881,1687.6339769363403,8.738588348933263e-06
970971,1941943,1941942,3883885,1690.0143508911133,8.6097378471095e-06
971972,1943945,1943944,3887889,1691.876741886139,8.48275738007942e-06
972973,1945947,1945946,3891893,1693.9625718593597,8.357619435628294e-06
973974,1947949,1947948,3895897,1695.7516210079193,8.234297524722933e-06
974975,1949951,1949950,3899901,1697.6294569969177,8.112765385703824e-06
975976,1951953,1951952,3903905,1699.9072489738464,7.99299687059829e-06
976977,1953955,1953954,3907909,1701.574786901474,7.874966172494169e-06
977978,1955957,1955956,3911913,1703.2171568870544,7.758648393974e-06
978979,1957959,1957958,3915917,1704.7270810604095,7.64401863762032e-06
979980,1959961,1959960,3919921,1706.6277949810028,7.531052233389346e-06
980981,1961963,1961962,3923925,1708.228462934494,7.41972507967148e-06
981982,1963965,1963964,3927929,1710.057797908783,7.310013756978151e-06
982983,1965967,1965966,3931933,1712.4082930088043,7.2018942773866e-06
983984,1967969,1967968,3935937,1714.6061577796936,7.095343676155608e-06
984985,1969971,1969970,3939941,1716.0885798931122,6.990339329604467e-06
985986,1971973,1971972,3943945,1718.0037610530853,6.886858614052471e-06
986987,1973975,1973974,3947949,1719.6641418933868,6.784879815313616e-06
987988,1975977,1975976,3951953,1721.338320016861,6.684380423394032e-06
988989,1977979,1977978,3955957,1722.928689956665,6.585339633602416e-06
989990,1979981,1979980,3959961,1724.5073020458221,6.487735959126439e-06
990991,1981983,1981982,3963965,1726.0778620243073,6.391548481587961e-06
991992,1983985,1983984,3967969,1727.799901008606,6.296756964729866e-06
992993,1985987,1985986,3971973,1729.3629240989685,6.2033407175476896e-06
993994,1987989,1987988,3975977,1730.9545149803162,6.111280185905343e-06
994995,1989991,1989990,3979981,1732.6308498382568,6.020555474606226e-06
995996,1991993,1991992,3983985,1734.2629129886627,5.931147370574763e-06
996997,1993995,1993994,3987989,1735.896164894104,5.843036319674866e-06
997998,1995997,1995996,3991993,1737.560971736908,5.756203904638824e-06
998999,1997999,1997998,3995997,1739.0456221103668,5.67063148082525e-06
1000000,2000001,2000000,4000001,1740.5057470798492,5.58630085834011e-06


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0010797977447509766,2181.4194943796983
1001,2003,2002,4005,1.7322759628295898,60.32343774180572
2002,4005,4004,8009,3.436156988143921,53.8499366883982
3003,6007,6006,12013,5.12670111656189,50.99186825038555
4004,8009,8008,16017,6.967211008071899,48.752759392813005
5005,10011,10010,20021,8.713039875030518,46.758201211835285
6006,12013,12012,24025,10.542521953582764,44.93193088011094
7007,14015,14014,28029,12.3138587474823,43.244418145702184
8008,16017,16016,32033,14.05112886428833,41.67791649327205
9009,18019,18018,36037,15.774017095565796,40.219524300277726
10010,20021,20020,40041,17.488980054855347,38.85890210790262
11011,22023,22022,44045,19.48236083984375,37.58720739053888
12012,24025,24024,48049,21.045321941375732,36.39654519750411
13013,26027,26026,52053,22.687103986740112,35.27969401642213
14014,28029,28028,56057,24.253175020217896,34.229983159542144
15015,30031,30030,60061,25.87743592262268,33.24124787055848
16016,32033,32032,64065,27.68208909034729,32.30781785900831
17017,34035,34034,68069,29.286262035369873,31.424514341854547
18018,36037,36036,72073,30.84328293800354,30.586643297693854
19019,38039,38038,76077,32.451483964920044,29.789980392475854
20020,40041,40040,80081,34.00261688232422,29.030747349822832
21021,42043,42042,84085,35.51441311836243,28.30558157639757
22022,44045,44044,88089,37.08456778526306,27.61150150678054
23023,46047,46046,92093,38.65678906440735,26.945870036554425
24024,48049,48048,96097,40.437087059020996,26.306357978694678
25025,50051,50050,100101,41.981207847595215,25.69090895068757
26026,52053,52052,104105,43.678956031799316,25.09770660584445
27027,54055,54054,108109,45.30334115028381,24.52514471664108
28028,56057,56056,112113,46.770617961883545,23.971800313401673
29029,58059,58058,116117,48.33151698112488,23.436409869876798
30030,60061,60060,120121,49.86950993537903,22.917848391327652
31031,62063,62062,124125,51.71391797065735,22.415111182313467
32032,64065,64064,128129,53.72916889190674,21.92729803387965
33033,66067,66066,132133,55.447169065475464,21.45359955994786
34034,68069,68068,136137,57.34312987327576,20.993285420167922
35035,70071,70070,140141,59.047394037246704,20.545694184102103
36036,72073,72072,144145,60.51428985595703,20.110224614280924
37037,74075,74074,148149,61.963146924972534,19.686328170149636
38038,76077,76076,152153,63.38620400428772,19.27350255917554
39039,78079,78078,156157,64.84578204154968,18.871286184204337
40040,80081,80080,160161,66.27766680717468,18.479253356940035
41041,82083,82082,164165,67.70236396789551,18.097018269415912
42042,84085,84084,168169,69.13035297393799,17.724207800410795
43043,86087,86086,172173,70.611496925354,17.36048033181214
44044,88089,88088,176177,72.0864610671997,17.005517709993683
45045,90091,90090,180181,73.59081101417542,16.659021865107206
46046,92093,92092,184185,75.19619107246399,16.320712775821903
47047,94095,94094,188189,76.85569596290588,15.990326691478117
48048,96097,96096,192193,78.4301528930664,15.667614575622565
49049,98099,98098,196197,79.9661009311676,15.35234074024629
50050,100101,100100,200201,81.73948812484741,15.04428164456101
51051,102103,102102,204205,83.44010305404663,14.743224836003606
52052,104105,104104,208209,84.96208906173706,14.448968014390289
53053,106107,106106,212213,86.52702283859253,14.161318202901498
54054,108109,108108,216217,88.09581589698792,13.880091011916534
55055,110111,110110,220221,89.69855284690857,13.605109983691818
56056,112113,112112,224225,91.22568202018738,13.336206007555916
57057,114115,114114,228229,92.76970386505127,13.073216796736347
58058,116117,116116,232233,94.44235801696777,12.815986419143883
59059,118119,118118,236237,96.17238688468933,12.564364875481033
60060,120121,120120,240241,97.62502408027649,12.318207718933081
61061,122123,122122,244245,99.17944002151489,12.07737571146265
62062,124125,124124,248249,100.89015889167786,11.841734512372796
63063,126127,126126,252253,102.48617196083069,11.611154395377412
64064,128129,128128,256257,104.11504697799683,11.38550999088909
65065,130131,130130,260261,105.81780791282654,11.164680050656784
66066,132133,132132,264265,107.56823301315308,10.948547232246938
67067,134135,134134,268269,109.26113891601562,10.736997901167115
68068,136137,136136,272273,110.99563598632812,10.529921948711717
69069,138139,138138,276277,112.70289206504822,10.327212623838022
70070,140141,140140,280281,114.56143379211426,10.128766377590182
71071,142143,142142,284285,115.99800491333008,9.93448271876639
72072,144145,144144,288289,117.48617815971375,9.744264079690652
73073,146147,146146,292293,119.2016749382019,9.558015691076093
74074,148149,148148,296297,120.78351497650146,9.375645465104412
75075,150151,150150,300301,122.33246397972107,9.197063885941361
76076,152153,152152,304305,123.70971083641052,9.022183907010799
77077,154155,154154,308309,125.13052487373352,8.850920854432843
78078,156157,156156,312313,126.47548484802246,8.683192336101342
79079,158159,158158,316317,127.83176875114441,8.518918155943197
80080,160161,160160,320321,129.17073011398315,8.358020232960826
81081,162163,162162,324325,130.49153995513916,8.200422524697615
82082,164165,164164,328329,131.99801301956177,8.046050954820885
83083,166167,166166,332333,133.59094619750977,7.894833344540302
84084,168169,168168,336337,135.0182249546051,7.746699347615731
85085,170171,170170,340341,136.77029514312744,7.601580388726575
86086,172173,172172,344345,138.58396077156067,7.459409605000246
87087,174175,174174,348349,140.23649287223816,7.320121790511962
88088,176177,176176,352353,141.78791308403015,7.183653343569858
89089,178179,178178,356357,143.33162808418274,7.0499422166299155
90090,180181,180180,360361,145.12626194953918,6.918927868669698
91091,182183,182182,364365,147.12427806854248,6.790551219876079
92092,184185,184184,368369,148.90420579910278,6.664754608496992
93093,186187,186186,372373,150.76070404052734,6.54148174971499
94094,188189,188188,376377,152.99188089370728,6.420677696409257
95095,190191,190190,380381,154.6596338748932,6.302288801675672
96096,192193,192192,384385,156.37361311912537,6.186262682982374
97097,194195,194194,388389,158.0727949142456,6.072548187842131
98098,196197,196196,392393,159.73547291755676,5.961095360895797
99099,198199,198198,396397,161.3861608505249,5.851855412302029
100100,200201,200200,400401,162.9097499847412,5.744780687337993
101101,202203,202202,404405,164.58627891540527,5.639824637129436
102102,204205,204204,408409,166.17558979988098,5.5369417904232705
103103,206207,206206,412413,167.80450582504272,5.436087726335927
104104,208209,208208,416417,169.47753190994263,5.337219048009047
105105,210211,210210,420421,171.2418909072876,5.240293357116116
106106,212213,212212,424425,172.97698092460632,5.145269229163546
107107,214215,214214,428429,174.4481749534607,5.052106189540837
108108,216217,216216,432433,175.86870789527893,4.960764690277983
109109,218219,218218,436437,177.31137800216675,4.871206087469091
110110,220221,220220,440441,178.80704593658447,4.783392619330357
111111,222223,222222,444445,180.22077012062073,4.69728738486026
112112,224225,224224,448449,181.71382308006287,4.612854323075112
113113,226227,226226,452453,183.16911005973816,4.53005819279565
114114,228229,228228,456457,184.7056269645691,4.4488645529600035
115115,230231,230230,460461,186.13558197021484,4.3692397434441546
116116,232233,232232,464465,187.60770106315613,4.291150866371822
117117,234235,234234,468469,189.01887106895447,4.21456576789592
118118,236237,236236,472473,190.56363201141357,4.139453020433166
119119,238239,238238,476477,192.0859830379486,4.065781905345943
120120,240241,240240,480481,193.64076280593872,3.9935223960445683
121121,242243,242242,484485,195.3561737537384,3.9226451415119072
122122,244245,244244,488489,197.02102398872375,3.853121450227036
123123,246247,246246,492493,198.68611788749695,3.784923274483276
124124,248249,248248,496497,200.40835213661194,3.7180231950885627
125125,250251,250250,500501,201.93067383766174,3.6523944064375655
126126,252253,252252,504505,203.46500396728516,3.5880107019460183
127127,254255,254254,508509,204.95498299598694,3.524846459839523
128128,256257,256256,512513,206.463800907135,3.4628766292865976
129129,258259,258258,516517,208.0123360157013,3.4020767168683506
130130,260261,260260,520521,209.43351292610168,3.342422773377166
131131,262263,262262,524525,210.88280296325684,3.283891380934051
132132,264265,264264,528529,212.32262992858887,3.22645964042124
133133,266267,266266,532533,213.7566740512848,3.1701051592176555
134134,268269,268268,536537,215.1654908657074,3.1148060392353045
135135,270271,270270,540541,216.59967279434204,3.0605408652443202
136136,272273,272272,544545,218.12200498580933,3.007288693483474
137137,274275,274274,548549,219.5482850074768,2.955029040548652
138138,276277,276276,552553,220.99099707603455,2.90374187255145
139139,278279,278278,556557,222.43630695343018,2.853407594542432
140140,280281,280280,560561,223.89934992790222,2.804007040193028
141141,282283,282282,564565,225.34400010108948,2.7555214617298134
142142,284285,284284,568569,226.80340886116028,2.7079325201143547
143143,286287,286286,572573,228.28753113746643,2.6612222754635013
144144,288289,288288,576577,229.72203397750854,2.6153731777041003
145145,290291,290290,580581,231.2172770500183,2.5703680574572445
146146,292293,292292,584585,232.7512469291687,2.5261901171438694
147147,294295,294294,588589,234.2582437992096,2.4828229223113567
148148,296297,296296,592593,235.76648497581482,2.440250393169663
149149,298299,298298,596597,237.32105612754822,2.3984567963369727
150150,300301,300300,600601,238.811350107193,2.357426736786465
151151,302303,302302,604605,240.25778484344482,2.317145149990779
152152,304305,304304,608609,241.70306205749512,2.2775972942599765
153153,306307,306306,612613,243.16847705841064,2.2387687432658367
154154,308309,308308,616617,244.66359090805054,2.2006453787498685
155155,310311,310310,620621,246.16386008262634,2.1632133834108345
156156,312313,312312,624625,247.6495499610901,2.126459233964624
157157,314315,314314,628629,249.3806929588318,2.0903696943755676
158158,316317,316316,632633,250.90651607513428,2.0549318092529347
159159,318319,318318,636637,252.366632938385,2.020132897408189
160160,320321,320320,640641,253.81283688545227,1.9859605455708333
161161,322323,322322,644645,255.2459421157837,1.952402602256825
162162,324325,324324,648649,256.6880919933319,1.9194471717870556
163163,326327,326326,652653,258.12754106521606,1.8870826084518058
164164,328329,328328,656657,259.6324019432068,1.855297510817195
165165,330331,330330,660661,261.1683750152588,1.8240807161696466
166166,332333,332332,664665,262.75125193595886,1.793421295097005
167167,334335,334334,668669,264.4774489402771,1.7633085462001645
168168,336337,336336,672673,266.2025330066681,1.7337319909333928
169169,338339,338338,676677,267.8260519504547,1.7046813685698226
170170,340341,340340,680681,269.4344849586487,1.6761466312890434
171171,342343,342342,684685,271.05233001708984,1.6481179393834964
172172,344345,344344,688689,272.4718699455261,1.6205856565803742
173173,346347,346346,692693,273.92745995521545,1.5935403454776633
174174,348349,348348,696697,275.3689799308777,1.5669727630886428
175175,350351,350350,700701,276.8403158187866,1.5408738564954092
176176,352353,352352,704705,278.2819619178772,1.515234758605743
177177,354355,354354,708709,279.69067907333374,1.4900467840113834
178178,356357,356356,712713,281.1738669872284,1.4653014249485068
179179,358359,358358,716717,282.7337670326233,1.4409903473512031
180180,360361,360360,720721,284.28206396102905,1.4171053870035166
181181,362363,362362,724725,285.9685320854187,1.3936385457786855
182182,364365,364364,728729,287.4524779319763,1.370581987972514
183183,366367,366366,732733,288.9851019382477,1.347928036722351
184184,368369,368368,736737,290.4384949207306,1.325669170509741
185185,370371,370370,740741,291.84865498542786,1.3037980197493653
186186,372373,372372,744745,293.33456897735596,1.2823073634563116
187187,374375,374374,748749,294.76203179359436,1.261190125993835
188188,376377,376376,752753,296.2577769756317,1.2404393738961517
189189,378379,378378,756757,297.7465190887451,1.2200483127692223
190190,380381,380380,760761,299.23288893699646,1.200010284261566
191191,382383,382382,764765,300.7024619579315,1.1803187631088576
192192,384385,384384,768769,302.14919686317444,1.1609673542459404
193193,386387,386386,772773,303.6593849658966,1.1419497899877342
194194,388389,388388,776777,305.13542199134827,1.1232599272769903
195195,390391,390390,780781,306.689838886261,1.1048917449935516
196196,392393,392392,784785,308.15411400794983,1.0868393413301192
197197,394395,394394,788789,309.5803861618042,1.069096931226909
198198,396397,396396,792793,311.0343277454376,1.051658843865539
199199,398399,398398,796797,312.49370098114014,1.0345195202236255
200200,400401,400400,800801,313.945405960083,1.017673510683153
201201,402403,402402,804805,315.41670083999634,1.0011154726970517
202202,404405,404404,808809,316.8891599178314,0.9848401685069348
203203,406407,406406,812813,318.341383934021,0.9688424629160863
204204,408409,408408,816817,319.77430987358093,0.9531173211120176
205205,410411,410410,820821,321.21938490867615,0.9376598065392727
206206,412413,412412,824825,322.6912567615509,0.9224650788221425
207207,414415,414414,828829,324.12787890434265,0.9075283917339902
208208,416417,416416,832833,325.5614469051361,0.8928450912128483
209209,418419,418418,836837,327.03112983703613,0.878410613423739
210210,420421,420420,840841,328.51766085624695,0.8642204828635158
211211,422423,422422,844845,330.005872964859,0.8502703105094724
212212,424425,424424,848849,331.43304991722107,0.8365557920106994
213213,426427,426426,852853,332.8832359313965,0.8230727059193441
214214,428429,428428,856857,334.31148076057434,0.8098169119622298
215215,430431,430430,860861,335.74777603149414,0.7967843493526061
216216,432433,432432,864865,337.23565793037415,0.7839710351377107
217217,434435,434434,868869,339.89169216156006,0.7713730625855533
218218,436437,436436,872873,341.644366979599,0.7589865996083063
219219,438439,438438,876877,343.31804299354553,0.7468078872178694
220220,440441,440440,880881,345.0448188781738,0.734833238020542
221221,442443,442442,884885,346.804456949234,0.7230590347403449
222222,444445,444444,888889,348.3226659297943,0.7114817287806545
223223,446447,446446,892893,349.80082297325134,0.70009783881369
224224,448449,448448,896897,351.28832387924194,0.6889039494025155
225225,450451,450450,900901,352.7531988620758,0.6778967096552151
226226,452453,452452,904905,354.2611541748047,0.6670728319063528
227227,454455,454454,908909,355.7190499305725,0.6564290904298105
228228,456457,456456,912913,357.24599504470825,0.6459623201781142
229229,458459,458458,916917,358.847247838974,0.635669415551547
230230,460461,460460,920921,360.50407886505127,0.6255473291923863
231231,462463,462462,924925,362.07214283943176,0.6155930708072219
232232,464465,464464,928929,363.76761388778687,0.605803706013603
233233,466467,466466,932933,365.3004820346832,0.5961763552134016
234234,468469,468468,936937,366.7652518749237,0.5867081924897093
235235,470471,470470,940941,368.2267589569092,0.5773964445279489
236236,472473,472472,944945,369.66329407691956,0.5682383895614294
237237,474475,474474,948949,371.135812997818,0.5592313563379321
238238,476477,476476,952953,372.6351261138916,0.5503727231103994
239239,478479,478478,956957,374.08500480651855,0.5416599166485412
240240,480481,480480,960961,375.56579208374023,0.5330904112734061
241241,482483,482482,964965,377.03762006759644,0.5246617279086649
242242,484485,484484,968969,378.5284900665283,0.5163714331580422
243243,486487,486486,972973,380.033714056015,0.5082171383980949
244244,488489,488488,976977,381.529226064682,0.5001964988923646
245245,490491,490490,980981,382.97447776794434,0.4923072129238335
246246,492493,492492,984985,384.45708179473877,0.48454702094670665
247247,494495,494494,988989,385.8790400028229,0.4769137047555887
248248,496497,496496,992993,387.3605749607086,0.4694050866728503
249249,498499,498498,996997,388.83515977859497,0.4620190287519108
250250,500501,500500,1001001,390.2911560535431,0.4547534320003024
251251,502503,502502,1005005,391.7824649810791,0.447606235615126
252252,504505,504504,1009009,393.25491309165955,0.44057541623965335
253253,506507,506506,1013013,394.7461578845978,0.4336589872299328
254254,508509,508508,1017017,396.2552800178528,0.4268549979428826
255255,510511,510510,1021021,397.7375659942627,0.4201615330347295
256256,512513,512512,1025025,399.1716060638428,0.4135767117747946
257257,514515,514514,1029029,400.67915391921997,0.40709868737701527
258258,516517,516516,1033033,402.17130398750305,0.40072564634090213
259259,518519,518518,1037037,403.6134867668152,0.3944558078093223
260260,520521,520520,1041041,405.09507417678833,0.3882874229391291
261261,522523,522522,1045045,406.5473837852478,0.38221877428429707
262262,524525,524524,1049049,408.0195851325989,0.3762481751917903
263263,526527,526526,1053053,409.5424358844757,0.37037396921073196
264264,528529,528528,1057057,411.02641201019287,0.3645945295132833
265265,530531,530530,1061061,412.51233291625977,0.358908258327574
266266,532533,532532,1065065,413.9544668197632,0.3533135863821144
267267,534535,534534,1069069,415.4346499443054,0.3478089723625999
268268,536537,536536,1073073,416.9812397956848,0.34239290237871955
269269,538539,538538,1077077,418.4554901123047,0.33706388944222
270270,540541,540540,1081081,419.916512966156,0.33182047295645134
271271,542543,542542,1085085,421.4290599822998,0.326661218214781
272272,544545,544544,1089089,423.05970001220703,0.32158471591139914
273273,546547,546546,1093093,424.7674341201782,0.31658958166065077
274274,548549,548548,1097097,426.3863959312439,0.3116744555255764
275275,550551,550550,1101101,428.09225702285767,0.3068380015574803
276276,552553,552552,1105105,429.7419879436493,0.30207890734493503
277277,554555,554554,1109109,431.21353697776794,0.2973958835701751
278278,556557,556556,1113113,432.7625768184662,0.29278766357583663
279279,558559,558558,1117117,434.280394077301,0.2882530029409054
280280,560561,560560,1121121,435.7316617965698,0.2837906790635998
281281,562563,562562,1125125,437.23168110847473,0.2793994907533488
282282,564565,564564,1129129,438.7042498588562,0.275078257832547
283283,566567,566566,1133133,440.22297406196594,0.27082582074319816
284284,568569,568568,1137137,441.7988369464874,0.26664104016435886
285285,570571,570570,1141141,443.3304579257965,0.2625227966349257
286286,572573,572572,1145145,444.8818829059601,0.2584699901865406
287287,574575,574574,1149149,446.32426500320435,0.2544815399805884
288288,576577,576576,1153153,447.8227159976959,0.250556383955427
289289,578579,578578,1157157,449.3005998134613,0.24669347847896006
290290,580581,580580,1161161,450.8010540008545,0.24289179800825877
291291,582583,582582,1165165,452.37873005867004,0.23915033475645942
292292,584585,584584,1169169,453.9415509700775,0.2354680983654589
293293,586587,586586,1173173,455.44157791137695,0.23184411558656848
294294,588589,588588,1177177,456.92967891693115,0.22827742996514644
295295,590591,590590,1181181,458.4190630912781,0.22476710153387103
296296,592593,592592,1185185,459.8805019855499,0.22131220651010608
297297,594595,594594,1189189,461.33191299438477,0.2179118370006563
298298,596597,596596,1193193,462.85971212387085,0.2145651007114111
299299,598599,598598,1197197,464.34163308143616,0.21127112066255904
300300,600601,600600,1201201,465.84709310531616,0.20802903491016878
301301,602603,602602,1205205,467.30771112442017,0.2048379962729996
302302,604605,604604,1209209,468.83738708496094,0.20169717206340465
303303,606607,606606,1213213,470.32841300964355,0.1986057438257376
304304,608609,608608,1217217,471.8052570819855,0.19556290707782864
305305,610611,610610,1221221,473.3081250190735,0.19256787105769035
306306,612613,612612,1225225,474.7487139701843,0.18961985847715823
307307,614615,614614,1229229,476.1932260990143,0.18671810527735033
308308,616617,616616,1233233,477.7047109603882,0.18386186039026597
309309,618619,618618,1237237,479.17032980918884,0.18105038550640984
310310,620621,620620,1241241,480.65046310424805,0.17828295484412138
311311,622623,622622,1245245,482.1480348110199,0.1755588549250433
312312,624625,624624,1249249,483.6084408760071,0.17287738435334177
313313,626627,626626,1253253,485.9599859714508,0.1702378535999287
314314,628629,628628,1257257,488.04223895072937,0.16763958478964014
315315,630631,630630,1261261,490.30247616767883,0.16508191149330287
316316,632633,632632,1265265,492.00120997428894,0.16256417852355298
317317,634635,634634,1269269,493.6886570453644,0.1600857417338375
318318,636637,636636,1273273,495.20043897628784,0.15764596782310036
319319,638639,638638,1277277,496.6652569770813,0.15524423414240118
320320,640641,640640,1281281,498.15423583984375,0.1528799285055129
321321,642643,642642,1285285,499.63140892982483,0.15055244900327125
322322,644645,644644,1289289,501.106892824173,0.1482612038228126
323323,646647,646646,1293293,502.5863161087036,0.14600561106726673
324324,648649,648648,1297297,504.0683741569519,0.1437850985815885
325325,650651,650650,1301301,505.6792447566986,0.14159910378020868
326326,652653,652652,1305305,507.25518703460693,0.1394470734786637
327327,654655,654654,1309309,508.78602600097656,0.13732846372772656
328328,656657,656656,1313313,510.1982400417328,0.13524273965106204
329329,658659,658658,1317317,511.60401487350464,0.1331893752862925
330330,660661,660660,1321321,513.0901520252228,0.1311678534272005
331331,662663,662662,1325325,514.5436398983002,0.12917766547218434
332332,664665,664664,1329329,516.0252590179443,0.127218311272145
333333,666667,666666,1333333,517.5166819095612,0.1252892989832617
334334,668669,668668,1337337,519.0003719329834,0.12339014492147271
335335,670671,670670,1341341,520.4618229866028,0.12152037342150379
336336,672673,672672,1345345,521.915543794632,0.11967951669475951
337337,674675,674674,1349349,523.4082100391388,0.11786711469414968
338338,676677,676676,1353353,524.8848600387573,0.11608271497880196
339339,678679,678678,1357357,526.3465888500214,0.11432587258150306
340340,680681,680680,1361361,527.8110649585724,0.11259614988000521
341341,682683,682682,1365365,529.3258938789368,0.11089311646821898
342342,684685,684684,1369369,530.7794749736786,0.1092163490332041
343343,686687,686686,1373373,532.2405819892883,0.10756543123102347
344344,688689,688688,1377377,533.712397813797,0.10593995356623509
345345,690691,690690,1381381,535.1796629428864,0.10433951327536306
346346,692693,692692,1385385,536.6775329113007,0.10276371420843589
347347,694695,694694,1389389,538.1994519233704,0.10121216671711863
348348,696697,696696,1393393,539.7711389064789,0.09968448754170822
349349,698699,698698,1397397,541.3140339851379,0.09818029970210773
350350,700701,700700,1401401,542.89031291008,0.09669923238857336
351351,702703,702702,1405405,544.4553301334381,0.0952409208583731
352352,704705,704704,1409409,546.0297379493713,0.09380500632926214
353353,706707,706706,1413413,547.549712896347,0.09239113587864267
354354,708709,708708,1417417,549.0540778636932,0.09099896234386051
355355,710711,710710,1421421,550.5440468788147,0.08962814422284282
356356,712713,712712,1425425,552.1855938434601,0.08827834557780534
357357,714715,714714,1429429,553.8580429553986,0.08694923594055126
358358,716717,716716,1433433,555.4758768081665,0.08564049021970277
359359,718719,718718,1437437,557.1337821483612,0.08435178860804626
360360,720721,720720,1441441,558.8825299739838,0.08308281649419769
361361,722723,722722,1445445,560.4138140678406,0.08183326437278993
362362,724725,724724,1449449,562.0019431114197,0.08060282775966243
363363,726727,726726,1453453,563.4827699661255,0.0793912071047771
364364,728729,728728,1457457,564.9641218185425,0.07819810771093216
365365,730731,730730,1461461,566.4269378185272,0.07702323964929292
366366,732733,732732,1465465,567.8761098384857,0.07586631768037932
367367,734735,734734,1469469,569.3799619674683,0.07472706117493999
368368,736737,736736,1473473,570.945271730423,0.07360519403493981
369369,738739,738738,1477477,572.5459339618683,0.07250044461875405
370370,740741,740740,1481481,574.0724430084229,0.07141254566511179
371371,742743,742742,1485485,575.5712070465088,0.07034123421942695
372372,744745,744744,1489489,577.0665819644928,0.06928625156228918
373373,746747,746746,1493493,578.5458879470825,0.06824734313750014
374374,748749,748748,1497497,580.0982868671417,0.06722425848215607
375375,750751,750750,1501501,581.6805589199066,0.06621675115945891
376376,752753,752752,1505505,583.233628988266,0.06522457868925358
377377,754755,754754,1509509,584.8020029067993,0.06424750248322653
378378,756757,756756,1513513,586.335037946701,0.06328528777999054
379379,758759,758758,1517517,587.8197247982025,0.06233770358005586
380380,760761,760760,1521521,589.2855889797211,0.061404522583984544
381381,762763,762762,1525525,590.7487728595734,0.06048552113043115
382382,764765,764764,1529529,592.2732779979706,0.05958047913543396
383383,766767,766766,1533533,593.7790191173553,0.058689180033752564
384384,768769,768768,1537537,595.2876617908478,0.0578114107189549
385385,770771,770770,1541541,596.7942979335785,0.05694696148680123
386386,772773,772772,1545545,598.2710690498352,0.05609562597851436
387387,774775,774774,1549549,599.7713627815247,0.05525720112586896
388388,776777,776776,1553553,601.2876689434052,0.05443148709628076
389389,778779,778778,1557557,602.8011977672577,0.05361828723857798
390390,780781,780780,1561561,604.2381660938263,0.05281740803161483
391391,782783,782782,1565565,605.7485239505768,0.05202865903163456
392392,784785,784784,1569569,607.2071650028229,0.0512518528222472
393393,786787,786786,1573573,608.6321380138397,0.050486804963270515
394394,788789,788788,1577577,610.1330718994141,0.04973333394298152
395395,790791,790790,1581581,611.7045459747314,0.04899126112911745
396396,792793,792792,1585585,613.2296578884125,0.04826041072158205
397397,794795,794794,1589589,614.7116639614105,0.047540609705947645
398398,796797,796796,1593593,616.2493598461151,0.046831687807980416
399399,798799,798798,1597597,617.8353769779205,0.046133477448279336
400400,800801,800800,1601601,619.3808720111847,0.04544581369759726
401401,802803,802802,1605605,620.8971540927887,0.04476853423466309
402402,804805,804804,1609609,622.3888440132141,0.044101479302298685
403403,806807,806806,1613613,623.8628528118134,0.043444491666264184
404404,808809,808808,1617617,625.2984688282013,0.04279741657308023
405405,810811,810810,1621621,626.7712068557739,0.0421601017105786
406406,812813,812812,1625625,628.2984998226166,0.041532397167088675
407407,814815,814814,1629629,629.845116853714,0.040914155393238616
408408,816817,816816,1633633,631.3794040679932,0.04030523116193763
409409,818819,818818,1637637,632.8831548690796,0.03970548153256459
410410,820821,820820,1641641,634.4005830287933,0.0391147658118598
411411,822823,822822,1645645,635.8793301582336,0.03853294551822728
412412,824825,824824,1649649,637.3277997970581,0.0379598843463782
413413,826827,826826,1653653,638.8237929344177,0.037395448130496334
414414,828829,828828,1657657,640.3080861568451,0.03683950481092779
415415,830831,830830,1661661,641.7435998916626,0.03629192439882445
416416,832833,832832,1665665,643.2663550376892,0.03575257894362949
417417,834835,834834,1669669,644.8045120239258,0.03522134249953979
418418,836837,836836,1673673,646.3415579795837,0.034698091093218864
419419,838839,838838,1677677,647.8439049720764,0.034182702691396116
420420,840841,840840,1681681,649.454393863678,0.03367505717028507
421421,842843,842842,1685685,651.1244060993195,0.03317503628443319
422422,844845,844844,1689689,652.8183870315552,0.03268252363579904
423423,846847,846846,1693693,654.7130579948425,0.03219740464498955
424424,848849,848848,1697697,656.4030609130859,0.03171956652147401
425425,850851,850850,1701701,658.0776147842407,0.031248898234480293
426426,852853,852852,1705705,659.755735874176,0.030785290485368932
427427,854855,854854,1709709,661.4606919288635,0.03032863567852928
428428,856857,856856,1713713,663.0412800312042,0.02987882789602736
429429,858859,858858,1717717,664.5531878471375,0.02943576286827465
430430,860861,860860,1721721,666.4320797920227,0.028999337949471737
431431,862863,862862,1725725,668.4071130752563,0.028569452090664527
432432,864865,864864,1729729,670.383584022522,0.028146005814278396
433433,866867,866866,1733733,672.0726108551025,0.02772890118910709
434434,868869,868868,1737737,673.7473969459534,0.027318041805074245
435435,870871,870870,1741741,675.4432330131531,0.02691333274981389
436436,872873,872872,1745745,677.2095067501068,0.026514680583659356
437437,874875,874874,1749749,678.8389718532562,0.0261219933169059
438438,876877,876876,1753753,680.4062080383301,0.02573518038639122
439439,878879,878878,1757757,682.0567481517792,0.025354152632417026
440440,880881,880880,1761761,683.7107689380646,0.024978822276921164
441441,882883,882882,1765765,685.532408952713,0.024609102901081314
442442,884885,884884,1769769,687.267865896225,0.024244909423941863
443443,886887,886886,1773773,689.097158908844,0.02388615808047234
444444,888889,888888,1777777,690.962338924408,0.02353276640178592
445445,890891,890890,1781781,692.8013670444489,0.023184653193197846
446446,892893,892892,1785785,694.5102317333221,0.02284173851523974
447447,894895,894894,1789789,696.3210351467133,0.022503943662286474
448448,896897,896896,1793793,698.2095670700073,0.022171191144707336
449449,898899,898898,1797797,699.916296005249,0.0218434046684024
450450,900901,900900,1801801,701.7748739719391,0.02152050911581682
451451,902903,902902,1805805,703.4400231838226,0.021202430527523575
452452,904905,904904,1809809,705.2298419475555,0.02088909608482936
453453,906907,906906,1813813,706.9768998622894,0.020580434089652044
454454,908909,908908,1817817,708.8334670066833,0.020276373949059234
455455,910911,910910,1821821,710.6101140975952,0.01997684615628259
456456,912913,912912,1825825,712.3135240077972,0.01968178227377848
457457,914915,914914,1829829,714.1039538383484,0.019391114917311825
458458,916917,916916,1833833,715.8606789112091,0.019104777737652512
459459,918919,918918,1837837,717.3649401664734,0.01882270540625086
460460,920921,920920,1841841,719.0159969329834,0.018544833597502475
461461,922923,922922,1845845,720.5794818401337,0.018271098973286826
462462,924925,924924,1849849,722.246376991272,0.018001439168756406
463463,926927,926926,1853853,723.8177070617676,0.017735792775056325
464464,928929,928928,1857857,725.457878112793,0.017474099325227144
465465,930931,930930,1861861,727.0818729400635,0.017216299279766645
466466,932933,932932,1865865,728.6424770355225,0.016962334011509483
467467,934935,934934,1869869,730.1618609428406,0.01671214579153002
468468,936937,936936,1873873,731.7685859203339,0.016465677774590404
469469,938939,938938,1877877,733.4346377849579,0.016222873986066588
470470,940941,940940,1881881,735.1072220802307,0.015983679308078536
471471,942943,942942,1885885,736.9537401199341,0.015748039465165675
472472,944945,944944,1889889,738.5482559204102,0.015515901012349786
473473,946947,946946,1893893,740.1973130702972,0.015287211321606264
474474,948949,948948,1897897,741.7431490421295,0.015061918568790134
475475,950951,950950,1901901,743.2382380962372,0.01483997172135787
476476,952953,952952,1905905,744.7396008968353,0.014621320526543968
477477,954955,954954,1909909,746.2202010154724,0.014405915497832211
478478,956957,956956,1913913,747.747918844223,0.014193707904269104
479479,958959,958958,1917917,749.2732839584351,0.013984649757958323
480480,960961,960960,1921921,750.7625830173492,0.013778693803033093
481481,962963,962962,1925925,752.2312951087952,0.013575793503378009
482482,964965,964964,1929929,753.7182538509369,0.013375903032624592
483483,966967,966966,1933933,755.3131878376007,0.013178977261532054
484484,968969,968968,1937937,757.0639309883118,0.012984971749119723
485485,970971,970970,1941941,758.7160258293152,0.012793842729820426
486486,972973,972972,1945945,760.2002239227295,0.012605547104612924
487487,974975,974974,1949949,761.678297996521,0.012420042429994282
488488,976977,976976,1953953,763.1602110862732,0.01223728690763437
489489,978979,978978,1957957,764.6522459983826,0.01205723937471248
490490,980981,980980,1961961,766.1437468528748,0.011879859294253947
491491,982983,982982,1965965,767.803328037262,0.01170510674421621
492492,984985,984984,1969969,769.4421379566193,0.011532942409871794
493493,986987,986986,1973973,771.1369931697845,0.011363327572325943
494494,988989,988988,1977977,773.0053551197052,0.01119622410124066
495495,990991,990990,1981981,774.4782328605652,0.011031594444489201
496496,992993,992992,1985985,776.4361329078674,0.010869401618833763
497497,994995,994994,1989989,778.109983921051,0.01070960920287689
498498,996997,996996,1993993,779.5952739715576,0.010552181326261234
499499,998999,998998,1997997,781.0977988243103,0.010397082662734647
500501,1001003,1001002,2002005,782.5744640827179,0.010244126905263329
501502,1003005,1003004,2006009,784.046854019165,0.010093585062236343
502503,1005007,1005006,2010013,785.5575790405273,0.009945269597551487
503504,1007009,1007008,2014017,787.0387651920319,0.009799147277021802
504505,1009011,1009010,2018021,788.4889831542969,0.00965518536872878
505506,1011013,1011012,2022025,789.9944620132446,0.009513351636655898
506507,1013015,1013014,2026029,791.462954044342,0.009373614331138924
507508,1015017,1015016,2030033,793.0488448143005,0.009235942183636325
508509,1017019,1017018,2034037,794.5511958599091,0.00910030439717957
509510,1019021,1019020,2038041,796.0280809402466,0.00896667064068879
510511,1021023,1021022,2042045,797.5344920158386,0.008835011040901009
511512,1023025,1023024,2046049,799.2263128757477,0.008705296175776311
512513,1025027,1025026,2050053,800.8709619045258,0.008577497067108197
513514,1027029,1027028,2054057,802.9871439933777,0.008451585174157117
514515,1029031,1029030,2058061,805.3350610733032,0.008327532387170322
515516,1031033,1031032,2062065,806.9185070991516,0.008205311019651162
516517,1033035,1033034,2066069,808.5448060035706,0.00808489380312949
517518,1035037,1035036,2070073,810.2785699367523,0.007966253879772012
518519,1037039,1037038,2074077,811.8565320968628,0.007849364796811642
519520,1039041,1039040,2078081,813.4349269866943,0.007734200499612598
520521,1041043,1041042,2082085,814.9993648529053,0.007620735326554495
521522,1043045,1043044,2086089,816.4991519451141,0.007508944002097451
522523,1045047,1045046,2090093,817.9761028289795,0.00739880163109774
523524,1047049,1047048,2094097,819.4275860786438,0.007290283693237143
524525,1049051,1049050,2098101,821.0453441143036,0.007183366037111227
525526,1051053,1051052,2102105,822.6748390197754,0.007078024874431321
526527,1053055,1053054,2106109,824.3424100875854,0.006974236775135978
527528,1055057,1055056,2110113,826.2070019245148,0.006871978660910827
528529,1057059,1057058,2114117,828.1467900276184,0.006771227800527413
529530,1059061,1059060,2118121,830.0747127532959,0.006671961804158855
530531,1061063,1061062,2122125,831.5190920829773,0.006574158618604997
531532,1063065,1063064,2126129,832.9437928199768,0.006477796521949131
532533,1065067,1065066,2130133,834.2630391120911,0.006382854118328396
533534,1067069,1067068,2134137,835.8341541290283,0.00628931033270419
534535,1069071,1069070,2138141,837.86381483078,0.006197144406996813
535536,1071073,1071072,2142145,839.2682979106903,0.006106335893832693
536537,1073075,1073074,2146149,841.0829849243164,0.006016864653588527
537538,1075077,1075076,2150153,842.7000329494476,0.005928710847570073
538539,1077079,1077078,2154157,844.2881460189819,0.005841854935624724
539540,1079081,1079080,2158161,846.1957819461823,0.005756277669547671
540541,1081083,1081082,2162165,848.0591077804565,0.005671960090239736
541542,1083085,1083084,2166169,849.9270570278168,0.005588883522364085
542543,1085087,1085086,2170173,851.7650408744812,0.005507029570821942
543544,1087089,1087088,2174177,853.6063580513,0.005426380115181928
544545,1089091,1089090,2178181,855.4732229709625,0.005346917307065269
545546,1091093,1091092,2182185,857.9143707752228,0.00526862356480251
546547,1093095,1093094,2186189,860.0232651233673,0.005191481570250289
547548,1095097,1095096,2190193,861.6965479850769,0.005115474264130171
548549,1097099,1097098,2194197,863.5933787822723,0.005040584842845419
549550,1099101,1099100,2198201,865.1754109859467,0.004966796753251401
550551,1101103,1101102,2202205,866.7000961303711,0.004894093690609225
551552,1103105,1103104,2206209,868.4977300167084,0.004822459593242456
552553,1105107,1105106,2210213,870.0587389469147,0.004751878640149698
553554,1107109,1107108,2214217,871.6329071521759,0.004682335246229741
554555,1109111,1109110,2218221,873.3363621234894,0.0046138140595530786
555556,1111113,1111112,2222225,875.943363904953,0.004546299957610245
556557,1113115,1113114,2226229,877.7469170093536,0.0044797780434464585
557558,1115117,1115116,2230233,879.4946990013123,0.0044142336424783934
558559,1117119,1117118,2234237,881.2018330097198,0.004349652299652007
559560,1119121,1119120,2238241,882.6666588783264,0.0042860197751224405
560561,1121123,1121122,2242245,884.3041749000549,0.004223322041980282
561562,1123125,1123124,2246249,885.7905209064484,0.004161545282386214
562563,1125127,1125126,2250253,887.5806488990784,0.0041006758842740965
563564,1127129,1127128,2254257,889.2402718067169,0.004040700439304601
564565,1129131,1129130,2258261,890.9704530239105,0.003981605738545113
565566,1131133,1131132,2262265,892.5709478855133,0.003923378770082309
566567,1133135,1133134,2266269,894.297111749649,0.003866006715838921
567568,1135137,1135136,2270273,896.0486319065094,0.0038094769489589453
568569,1137139,1137138,2274277,897.5153558254242,0.0037537770305107188
569570,1139141,1139140,2278281,899.2181899547577,0.003698894707213185
570571,1141143,1141142,2282285,900.8570377826691,0.003644817907570541
571572,1143145,1143144,2286289,902.4495370388031,0.0035915347405079956
572573,1145147,1145146,2290293,904.1365718841553,0.003539033492188537
573574,1147149,1147148,2294297,905.963082075119,0.0034873026218065206
574575,1149151,1149150,2298301,907.6398739814758,0.003436330761815043
575576,1151153,1151152,2302305,909.7453498840332,0.003386106712810033
576577,1153155,1153154,2306309,911.6182370185852,0.0033366194425070717
577578,1155157,1155156,2310313,913.1316568851471,0.003287858082785533
578579,1157159,1157158,2314317,914.6124799251556,0.0032398119265053538
579580,1159161,1159160,2318321,916.3030619621277,0.0031924704262564774
580581,1161163,1161162,2322325,917.8790040016174,0.0031458231916303703
581582,1163165,1163164,2326329,919.7460589408875,0.003099859986150477
582583,1165167,1165166,2330333,921.4826231002808,0.003054570725225858
583584,1167169,1167168,2334337,923.1619420051575,0.0030099454751280064
584585,1169171,1169170,2338341,924.6416320800781,0.0029659744487844364
585586,1171173,1171172,2342345,926.1776449680328,0.002922648004982875
586587,1173175,1173174,2346349,927.7181389331818,0.002879956645074344
587588,1175177,1175176,2350353,929.2710249423981,0.002837891012632099
588589,1177179,1177178,2354357,930.9037389755249,0.002796441888449408
589590,1179181,1179180,2358361,932.4396188259125,0.0027556001919037953
590591,1181183,1181182,2362365,934.1366589069366,0.0027153569758411322
591592,1183185,1183184,2366369,935.8880920410156,0.0026757034264619506
592593,1185187,1185186,2370373,937.7557578086853,0.002636630860479272
593594,1187189,1187188,2374377,939.3010330200195,0.002598130723754366
594595,1189191,1189190,2378381,940.8032341003418,0.0025601945885682653
595596,1191193,1191192,2382385,942.4042398929596,0.0025228141528259584
596597,1193195,1193194,2386389,944.2511160373688,0.002485981236304724
597598,1195197,1195196,2390393,945.9084610939026,0.0024496877815636253
598599,1197199,1197198,2394397,947.392040014267,0.0024139258495097238
599600,1199201,1199200,2398401,948.8999161720276,0.002378687619284392
600601,1201203,1201202,2402405,950.7193479537964,0.002343965385193769
601602,1203205,1203204,2406409,952.6626598834991,0.0023097515565950744
602603,1205207,1205206,2410413,954.2807040214539,0.0022760386549407485
603604,1207209,1207208,2414417,956.69824385643,0.0022428193118457784
604605,1209211,1209210,2418421,958.3663277626038,0.0022100862692013834
605606,1211213,1211212,2422425,959.9464011192322,0.002177832375309663
606607,1213215,1213214,2426429,961.7352290153503,0.0021460505847699096
607608,1215217,1215216,2430433,964.0117909908295,0.00211473395665962
608609,1217219,1217218,2434437,966.1336989402771,0.002083875652374445
609610,1219221,1219220,2438441,968.4321579933167,0.002053468934718694
610611,1221223,1221222,2442445,969.992527961731,0.0020235071662000337
611612,1223225,1223224,2446449,971.6475117206573,0.001993983807551558
612613,1225227,1225226,2450453,973.3309121131897,0.0019648924157991132
613614,1227229,1227228,2454457,974.8359789848328,0.0019362266441476095
614615,1229231,1229230,2458461,976.2766809463501,0.0019079802386841038
615616,1231233,1231232,2462465,977.7100870609283,0.0018801470383777996
616617,1233235,1233234,2466469,979.1681208610535,0.001852720973374744
617618,1235237,1235236,2470473,980.5889270305634,0.0018256960635198993
618619,1237239,1237238,2474477,982.0731310844421,0.0017990664168792136
619620,1239241,1239240,2478481,984.168536901474,0.0017728262284890661
620621,1241243,1241242,2482485,985.773185968399,0.0017469697795604588
621622,1243245,1243244,2486489,987.3502731323242,0.0017214914354326538
622623,1245247,1245246,2490493,988.9595017433167,0.0016963856446636782
623624,1247249,1247248,2494497,990.5476899147034,0.0016716469381208299
624625,1249251,1249250,2498501,992.0244839191437,0.0016472699272753744
625626,1251253,1251252,2502505,993.4502620697021,0.00162324930295199
626627,1253255,1253254,2506509,995.1702148914337,0.0015995798344192735
627628,1255257,1255256,2510513,997.043613910675,0.0015762563684802444
628629,1257259,1257258,2514517,998.5925760269165,0.0015532738277670433
629630,1259261,1259260,2518521,1000.5119171142578,0.0015306272097177498
630631,1261263,1261262,2522525,1002.4872369766235,0.001508311585894262
631632,1263265,1263264,2526529,1004.0923368930817,0.0014863221001633065
632633,1265267,1265266,2530533,1005.5577340126038,0.0014646539682416915
633634,1267269,1267268,2534537,1006.9987337589264,0.001443302476786812
634635,1269271,1269270,2538541,1008.4286789894104,0.0014222629813502863
635636,1271273,1271272,2542545,1010.1057560443878,0.0014015309063779569
636637,1273275,1273274,2546549,1012.0740239620209,0.0013811017438456474
637638,1275277,1275276,2550553,1013.5565891265869,0.0013609710513264872
638639,1277279,1277278,2554557,1014.9991140365601,0.0013411344533551528
639640,1279281,1279280,2558561,1016.4421629905701,0.0013215876375625157
640641,1281283,1281282,2562565,1017.892077922821,0.0013023263561535714
641642,1283285,1283284,2566569,1019.3163850307465,0.001283346423065268
642643,1285287,1285286,2570573,1020.7520678043365,0.0012646437147623146
643644,1287289,1287288,2574577,1022.1861929893494,0.0012462141679634442
644645,1289291,1289290,2578581,1023.6366090774536,0.0012280537793003532
645646,1291293,1291292,2582585,1025.241261959076,0.0012101586044082069
646647,1293295,1293294,2586589,1027.3831679821014,0.0011925247569024577
647648,1295297,1295296,2590593,1029.571171760559,0.001175148408037785
648649,1297299,1297298,2594597,1031.4095890522003,0.0011580257847754183
649650,1299301,1299300,2598601,1033.346519947052,0.001141153170351572
650651,1301303,1301302,2602605,1035.5646359920502,0.001124526902344769
651652,1303305,1303304,2606609,1037.245770931244,0.0011081433718800326
652653,1305307,1305306,2610613,1039.1778330802917,0.001091999024197321
653654,1307309,1307308,2614617,1041.272570848465,0.001076090355809356
654655,1309311,1309310,2618621,1042.9917469024658,0.001060413915524805
655656,1311313,1311312,2622625,1045.5265259742737,0.001044966302629291
656657,1313315,1313314,2626629,1048.2789950370789,0.001029744165862212
657658,1315317,1315316,2630633,1050.3971688747406,0.001014744204667295
658659,1317319,1317318,2634637,1052.6813640594482,0.000999963165668305
659660,1319321,1319320,2638641,1054.5118107795715,0.0009853978441469735
660661,1321323,1321322,2642645,1056.7115659713745,0.0009710450823376959
661662,1323325,1323324,2646649,1058.6534888744354,0.0009569017686317238
662663,1325327,1325326,2650653,1060.462984085083,0.0009429648373497912
663664,1327329,1327328,2654657,1062.1243209838867,0.0009292312679463066
664665,1329331,1329330,2658661,1063.5991480350494,0.000915698084440919
665666,1331333,1331332,2662665,1065.3962440490723,0.0009023623542816495
666667,1333335,1333334,2666669,1067.1662590503693,0.0008892211878901435
667668,1335337,1335336,2670673,1068.7050340175629,0.0008762717386616714
668669,1337339,1337338,2674677,1071.1616761684418,0.0008635112014871993
669670,1339341,1339340,2678681,1073.4426908493042,0.0008509368126397021
670671,1341343,1341342,2682685,1075.5292029380798,0.0008385458487509823
671672,1343345,1343344,2686689,1077.5852711200714,0.0008263356266979827
672673,1345347,1345346,2690693,1079.1722569465637,0.0008143035025796053
673674,1347349,1347348,2694697,1081.691181898117,0.0008024468716030242
674675,1349351,1349350,2698701,1083.7391498088837,0.0007907631669468174
675676,1351353,1351352,2702705,1085.5600938796997,0.0007792498596472797
676677,1353355,1353354,2706709,1087.017364025116,0.0007679044579163019
677678,1355357,1355356,2710713,1088.4610459804535,0.0007567245064592498
678679,1357359,1357358,2714717,1089.8849878311157,0.0007457075855654693
679680,1359361,1359360,2718721,1091.356279850006,0.0007348513125862155
680681,1361363,1361362,2722725,1092.8142569065094,0.0007241533373871789
681682,1363365,1363364,2726729,1094.6545639038086,0.0007136113467822724
682683,1365367,1365366,2730733,1096.5398950576782,0.0007032230599861578
683684,1367369,1367368,2734737,1098.0755751132965,0.0006929862304332346
684685,1369371,1369370,2738741,1099.623454093933,0.0006828986441860252
685686,1371373,1371372,2742745,1101.1473181247711,0.0006729581197078005
686687,1373375,1373374,2746749,1102.6718690395355,0.0006631625076352066
687688,1375377,1375376,2750753,1104.3801510334015,0.000653509690437204
688689,1377379,1377378,2754757,1106.0763850212097,0.0006439975811645127
689690,1379381,1379380,2758761,1107.6301510334015,0.0006346241234496119
690691,1381383,1381382,2762765,1109.0525670051575,0.0006253872916204273
691692,1383385,1383384,2766769,1110.4306559562683,0.0006162850889950278
692693,1385387,1385386,2770773,1111.927206993103,0.0006073155491321813
693694,1387389,1387388,2774777,1113.424516916275,0.0005984767331028706
694695,1389391,1389390,2778781,1114.9093000888824,0.0005897667318777167
695696,1391393,1391392,2782785,1116.3957509994507,0.0005811836633711209
696697,1393395,1393394,2786789,1117.7999801635742,0.0005727256732370734
697698,1395397,1395396,2790793,1119.5309598445892,0.0005643909346417786
698699,1397399,1397398,2794797,1121.0053000450134,0.0005561776474678481
699700,1399401,1399400,2798801,1122.8722059726715,0.0005480840375184926
700701,1401403,1401402,2802805,1124.49413895607,0.000540108357427016
701702,1403405,1403404,2806809,1125.9315819740295,0.0005322488847241402
702703,1405407,1405406,2810813,1127.3644020557404,0.0005245039226338122
703704,1407409,1407408,2814817,1128.7881071567535,0.0005168717984815885
704705,1409411,1409410,2818821,1130.2519299983978,0.0005093508653999379
705706,1411413,1411412,2822825,1131.7044439315796,0.0005019394993723836
706707,1413415,1413414,2826829,1133.1309299468994,0.0004946361009388056
707708,1415417,1415416,2830833,1134.5472478866577,0.0004874390936038253
708709,1417419,1417418,2834837,1135.9643149375916,0.00048034692429155257
709710,1419421,1419420,2838841,1137.3681480884552,0.0004733580626634648
710711,1421423,1421422,2842845,1138.8042500019073,0.00046647100066365965
711712,1423425,1423424,2846849,1140.2450950145721,0.0004596842521777944
712713,1425427,1425426,2850853,1141.6861598491669,0.0004529963531467729
713714,1427429,1427428,2854857,1143.1551780700684,0.0004464058607709376
714715,1429431,1429430,2858861,1144.871325969696,0.00043991135339638276
715716,1431433,1431432,2862865,1147.2256870269775,0.0004335114302875809
716717,1433435,1433434,2866869,1149.66739487648,0.00042720471151369566
717718,1435437,1435436,2870873,1151.5468270778656,0.0004209898360159059
718719,1437439,1437438,2874877,1153.3593699932098,0.0004148654644495764
719720,1439441,1439440,2878881,1154.913264989853,0.00040883027611471334
720721,1441443,1441442,2882885,1157.3571968078613,0.00040288296941071167
721722,1443445,1443444,2886889,1158.8832530975342,0.00039702226217741554
722723,1445447,1445446,2890893,1160.3093769550323,0.00039124689124037104
723724,1447449,1447448,2894897,1161.7526700496674,0.00038555561150133144
724725,1449451,1449450,2898901,1163.190724849701,0.00037994719605194405
725726,1451453,1451452,2902905,1164.6314477920532,0.00037442043628743704
726727,1453455,1453454,2906909,1166.235605955124,0.0003689741411108116
727728,1455457,1455456,2910913,1168.1514067649841,0.00036360713659178145
728729,1457459,1457458,2914917,1169.950807094574,0.0003583182664215201
729730,1459461,1459460,2918921,1171.7484760284424,0.00035310639111685305
730731,1461463,1461462,2922925,1174.130187034607,0.0003479703874518236
731732,1463465,1463464,2926929,1176.795361995697,0.0003429091490261271
732733,1465467,1465466,2930933,1179.9477808475494,0.0003379215853556161
733734,1467469,1467468,2934937,1181.9571678638458,0.0003330066223270478
734735,1469471,1469470,2938941,1183.8940110206604,0.0003281632009475288
735736,1471473,1471472,2942945,1185.5775508880615,0.0003233902782540099
736737,1473475,1473474,2946949,1187.1736969947815,0.0003186868261764175
737738,1475477,1475476,2950953,1188.6410839557648,0.0003140518317650276
738739,1477479,1477478,2954957,1190.4225940704346,0.0003094842970767786
739740,1479481,1479480,2958961,1192.0803139209747,0.00030498323849315057
740741,1481483,1481482,2962965,1193.79185795784,0.0003005476864927914
741742,1483485,1483484,2966969,1195.4364948272705,0.00029617668667469843
742743,1485487,1485486,2970973,1197.1051001548767,0.0002918692977118553
743744,1487489,1487488,2974977,1198.6495769023895,0.0002876245923744136
744745,1489491,1489490,2978981,1200.085685968399,0.0002834416568475717
745746,1491493,1491492,2982985,1201.5461828708649,0.00027931959073157486
746747,1493495,1493494,2986989,1203.0169160366058,0.000275257507155402
747748,1495497,1495496,2990993,1204.6615591049194,0.0002712545316398973
748749,1497499,1497498,2994997,1207.5599009990692,0.0002673098025525178
749750,1499501,1499500,2999001,1209.9944639205933,0.00026342247110733297
750751,1501503,1501502,3003005,1211.637521982193,0.0002595917009102777
751752,1503505,1503504,3007009,1213.1824069023132,0.00025581666761809174
752753,1505507,1505506,3011013,1214.6191487312317,0.0002520965589383195
753754,1507509,1507508,3015017,1216.0929391384125,0.0002484305746293103
754755,1509511,1509510,3019021,1218.7580659389496,0.000244817925931784
755756,1511513,1511512,3023025,1220.4812240600586,0.00024125783556883107
756757,1513515,1513514,3027029,1222.384771823883,0.00023774953797328635
757758,1515517,1515516,3031033,1223.8714129924774,0.00023429227826454735
758759,1517519,1517518,3035037,1225.3699159622192,0.00023088531315806904
759760,1519521,1519520,3039041,1226.8446128368378,0.00022752790948743495
760761,1521523,1521522,3043045,1228.3347840309143,0.00022421934556859924
761762,1523525,1523524,3047049,1229.961847782135,0.00022095890994933143
762763,1525527,1525526,3051053,1232.1049118041992,0.0002177459009544691
763764,1527529,1527528,3055057,1233.5631098747253,0.0002145796281638468
764765,1529531,1529530,3059061,1235.0505318641663,0.0002114594108206802
765766,1531533,1531532,3063065,1236.5525550842285,0.00020838457783156628
766767,1533535,1533534,3067069,1237.9998090267181,0.00020535446810754365
767768,1535537,1535536,3071073,1239.4516711235046,0.0002023684305640927
768769,1537539,1537538,3075077,1240.9308009147644,0.00019942582298426714
769770,1539541,1539540,3079081,1242.371710062027,0.00019652601292818872
770771,1541543,1541542,3083085,1243.821130990982,0.00019366837693723937
771772,1543545,1543544,3087089,1245.3101079463959,0.00019085230121618224
772773,1545547,1545546,3091093,1246.849191904068,0.00018807718004154594
773774,1547549,1547548,3095097,1248.7584431171417,0.00018534241723955347
774775,1549551,1549550,3099101,1250.661152124405,0.00018264742516294064
775776,1551553,1551552,3103105,1253.6561510562897,0.00017999162457726925
776777,1553555,1553554,3107109,1255.8487408161163,0.00017737444454724027
777778,1555557,1555556,3111113,1257.867651939392,0.00017479532311881485
778779,1557559,1557558,3115117,1259.9674389362335,0.0001722537058412854
779780,1559561,1559560,3119121,1262.216343164444,0.00016974904690414405
780781,1561563,1561562,3123125,1263.7680430412292,0.000167280808113901
781782,1563565,1563564,3127129,1265.4487318992615,0.00016484845900777145
782783,1565567,1565566,3131133,1266.9740197658539,0.00016245147742210975
783784,1567569,1567568,3135137,1268.4492769241333,0.00016008934812816733
784785,1569571,1569570,3139141,1269.933261871338,0.00015776156374158745
785786,1571573,1571572,3143145,1271.7954769134521,0.00015546762472240516
786787,1573575,1573574,3147149,1273.4597570896149,0.00015320703766974475
787788,1575577,1575576,3151153,1275.460753917694,0.00015097931770924333
788789,1577579,1577578,3155157,1276.9854378700256,0.00014878398610562726
789790,1579581,1579580,3159161,1278.9876370429993,0.0001466205713995805
790791,1581583,1581582,3163165,1280.8545730113983,0.00014448860906668415
791792,1583585,1583584,3167169,1282.9901950359344,0.0001423876414037295
792793,1585587,1585586,3171173,1284.7167041301727,0.00014031721696028399
793794,1587589,1587588,3175177,1286.4948060512543,0.00013827689156187262
794795,1589591,1589590,3179181,1288.0851910114288,0.00013626622694573598
795796,1591593,1591592,3183185,1289.6382880210876,0.0001342847913292644
796797,1593595,1593594,3187189,1291.2355918884277,0.00013233215952368482
797798,1595597,1595596,3191193,1292.8392269611359,0.00013040791247931338
798799,1597599,1597598,3195197,1294.2799067497253,0.00012851163683080813
799800,1599601,1599600,3199201,1296.082939863205,0.00012664292546560318
800801,1601603,1601602,3203205,1297.8041207790375,0.0001248013774102219
801802,1603605,1603604,3207209,1299.490285873413,0.00012298659748921636
802803,1605607,1605606,3211213,1300.843894958496,0.00012119819587042002
803804,1607609,1607608,3215217,1302.1300508975983,0.0001194357889744424
804805,1609611,1609610,3219221,1303.41064286232,0.00011769899867886124
805806,1611613,1611612,3223225,1304.6834330558777,0.00011598745209084882
806807,1613615,1613614,3227229,1306.010528087616,0.00011430078166085877
807808,1615617,1615616,3231233,1307.2360100746155,0.00011263862586474715
808809,1617619,1617618,3235237,1308.5837798118591,0.00011100062783953035
809810,1619621,1619620,3239241,1310.2418110370636,0.0001093864359518193
810811,1621623,1621622,3243245,1311.7654631137848,0.00010779570413887996
811812,1623625,1623624,3247249,1313.4040100574493,0.0001062280911128255
812813,1625627,1625626,3251253,1314.8889181613922,0.00010468326024692942
813814,1627629,1627628,3255257,1316.6662259101868,0.00010316088025774661
814815,1629631,1629630,3259261,1318.5431439876556,0.0001016606245229923
815816,1631633,1631632,3263265,1320.3697528839111,0.00010018217130891571
816817,1633635,1633634,3267269,1321.9765288829803,9.872520320186595e-05
817818,1635637,1635636,3271273,1324.105045080185,9.728940790409979e-05
818819,1637639,1637638,3275277,1326.5505819320679,9.587447766534751e-05
819820,1639641,1639640,3279281,1328.4951119422913,9.448010848700505e-05
820821,1641643,1641642,3283285,1330.0965898036957,9.31060013726892e-05
821822,1643645,1643644,3287289,1331.6584918498993,9.175186187349027e-05
822823,1645647,1645646,3291293,1333.7076649665833,9.041739940585103e-05
823824,1647649,1647648,3295297,1335.306442975998,8.91023277063141e-05
824825,1649651,1649650,3299301,1336.9385941028595,8.78063647178351e-05
825826,1651653,1651652,3303305,1338.3825738430023,8.652923304452997e-05
826827,1653655,1653654,3307309,1339.825660943985,8.52706580189988e-05
827828,1655657,1655656,3311313,1341.2753601074219,8.403037043080985e-05
828829,1657659,1657658,3315317,1342.7804398536682,8.280810379801551e-05
829830,1659661,1659660,3319321,1344.2090899944305,8.160359641351533e-05
830831,1661663,1661662,3323325,1345.669333934784,8.041658975344035e-05
831832,1663665,1663664,3327329,1347.172306060791,7.924682950033457e-05
832833,1665667,1665666,3331333,1348.6322371959686,7.809406486103398e-05
833834,1667669,1667668,3335337,1350.060935974121,7.695804856666655e-05
834835,1669671,1669670,3339341,1351.5069661140442,7.583853732739954e-05
835836,1671673,1671672,3343345,1352.9432640075684,7.473529058188433e-05
836837,1673675,1673674,3347349,1354.3863549232483,7.364807242993265e-05
837838,1675677,1675676,3351353,1355.8538451194763,7.257664947246667e-05
838839,1677679,1677678,3355357,1357.34526014328,7.152079217576102e-05
839840,1679681,1679680,3359361,1358.9298470020294,7.048027418932179e-05
840841,1681683,1681682,3363365,1361.345006942749,6.945487234588654e-05
841842,1683685,1683684,3367369,1362.777794122696,6.844436734354531e-05
842843,1685687,1685686,3371373,1364.1905720233917,6.744854181306437e-05
843844,1687689,1687688,3375377,1365.6363110542297,6.64671829326835e-05
844845,1689691,1689690,3379381,1367.0761020183563,6.550008015437925e-05
845846,1691693,1691692,3383385,1368.5285849571228,6.454702611335961e-05
846847,1693695,1693694,3387389,1369.9638719558716,6.36078168554377e-05
847848,1695697,1695696,3391393,1371.4037969112396,6.268225115491077e-05
848849,1697699,1697698,3395397,1372.8603358268738,6.177013017349964e-05
849850,1699701,1699700,3399401,1374.265380859375,6.087125882459077e-05
850851,1701703,1701702,3403405,1375.707107782364,5.9985444408994226e-05
851852,1703705,1703704,3407409,1377.1429278850555,5.911249706969102e-05
852853,1705707,1705706,3411413,1378.6206600666046,5.8252229905519926e-05
853854,1707709,1707708,3415417,1380.7583701610565,5.740445840274333e-05
854855,1709711,1709710,3419421,1382.2608878612518,5.656900100348139e-05
855856,1711713,1711712,3423425,1384.1217198371887,5.574567887833837e-05
856857,1713715,1713714,3427429,1385.5966160297394,5.493431558534212e-05
857858,1715717,1715716,3431433,1387.1120147705078,5.413473695625726e-05
858859,1717719,1717718,3435437,1388.578127861023,5.334677177870617e-05
859860,1719721,1719720,3439441,1389.986188173294,5.257025179616903e-05
860861,1721723,1721722,3443445,1391.3913369178772,5.180500988899439e-05
861862,1723725,1723724,3447449,1392.827898979187,5.105088268919644e-05
862863,1725727,1725726,3451453,1394.2103779315948,5.0307708534091944e-05
863864,1727729,1727728,3455457,1395.6028280258179,4.957532814842125e-05
864865,1729731,1729730,3459461,1397.0287408828735,4.885358441697463e-05
865866,1731733,1731732,3463465,1398.4267678260803,4.8142323294086964e-05
866867,1733735,1733734,3467469,1399.8315689563751,4.744139198464836e-05
867868,1735737,1735736,3471473,1401.216532945633,4.675064030834619e-05
868869,1737739,1737738,3475477,1402.6124629974365,4.6069920927038766e-05
869870,1739741,1739740,3479481,1404.0305919647217,4.539908763945277e-05
870871,1741743,1741742,3483485,1405.465735912323,4.473799651805166e-05
871872,1743745,1743744,3487489,1406.8583891391754,4.4086506363782973e-05
872873,1745747,1745746,3491493,1408.7082979679108,4.3444477455523156e-05
873874,1747749,1747748,3495497,1410.3694729804993,4.281177245957224e-05
874875,1749751,1749750,3499501,1412.0073580741882,4.218825574753282e-05
875876,1751753,1751752,3503505,1414.3403890132904,4.157379385105742e-05
876877,1753755,1753754,3507509,1415.8155500888824,4.096825523447478e-05
877878,1755757,1755756,3511513,1417.347289800644,4.0371510181103076e-05
878879,1757759,1757758,3515517,1418.9426469802856,3.978343102062354e-05
879880,1759761,1759760,3519521,1420.4990510940552,3.9203891674333136e-05
880881,1761763,1761762,3523525,1422.0538659095764,3.863276788251824e-05
881882,1763765,1763764,3527529,1423.5880270004272,3.806993765920197e-05
882883,1765767,1765766,3531533,1425.1315319538116,3.751528072371002e-05
883884,1767769,1767768,3535537,1426.594822883606,3.6968677704862785e-05
884885,1769771,1769770,3539541,1428.0607380867004,3.6430012073651596e-05
885886,1771773,1771772,3543545,1429.6865649223328,3.589916843793617e-05
886887,1773775,1773774,3547549,1431.139524936676,3.537603265613143e-05
887888,1775777,1775776,3551553,1433.4550170898438,3.4860493542510085e-05
888889,1777779,1777778,3555557,1435.6456699371338,3.435244013871852e-05
889890,1779781,1779780,3559561,1437.1976449489594,3.385176387382671e-05
890891,1781783,1781782,3563565,1438.6784269809723,3.335835742745985e-05
891892,1783785,1783784,3567569,1440.1013638973236,3.287211529823253e-05
892893,1785787,1785786,3571573,1441.5928950309753,3.2392933462688234e-05
893894,1787789,1787788,3575577,1443.1632578372955,3.192070937529934e-05
894895,1789791,1789790,3579581,1444.5966439247131,3.1455341741093434e-05
895896,1791793,1791792,3583585,1446.1437258720398,3.0996730970400677e-05
896897,1793795,1793794,3587589,1447.5688889026642,3.0544779292540625e-05
897898,1795797,1795796,3591593,1448.9882318973541,3.009938927789335e-05
898899,1797799,1797798,3595597,1450.5030081272125,2.966046645269671e-05
899900,1799801,1799800,3599601,1452.0898530483246,2.9227916229501716e-05
900901,1801803,1801802,3603605,1453.5944588184357,2.88016461809093e-05
901902,1803805,1803804,3607609,1455.035588979721,2.8381565130075614e-05
902903,1805807,1805806,3611613,1456.5041527748108,2.7967583150712017e-05
903904,1807809,1807808,3615617,1457.9271039962769,2.7559611567085085e-05
904905,1809811,1809810,3619621,1459.3696138858795,2.7157563295077125e-05
905906,1811813,1811812,3623625,1460.8158888816833,2.6761352160065144e-05
906907,1813815,1813814,3627629,1462.2652847766876,2.637089346535504e-05
907908,1815817,1815816,3631633,1463.711175918579,2.598610331006057e-05
908909,1817819,1817818,3635637,1465.1557960510254,2.5606899725971743e-05
909910,1819821,1819820,3639641,1466.5611209869385,2.5233201313312748e-05
910911,1821823,1821822,3643645,1468.0094101428986,2.486492837761034e-05
911912,1823825,1823824,3647649,1469.4035799503326,2.450200213388598e-05
912913,1825827,1825826,3651653,1470.8023040294647,2.4144344479282154e-05
913914,1827829,1827828,3655657,1472.1884939670563,2.379187901624391e-05
914915,1829831,1829830,3659661,1473.6023218631744,2.3444530825145193e-05
915916,1831833,1831832,3663665,1475.0183029174805,2.310222510004678e-05
916917,1833835,1833834,3667669,1476.4033198356628,2.2764888853998855e-05
917918,1835837,1835836,3671673,1477.8114278316498,2.2432449668485788e-05
918919,1837839,1837838,3675677,1479.2414989471436,2.210483660292084e-05
919920,1839841,1839840,3679681,1480.6794929504395,2.178197951252514e-05
920921,1841843,1841842,3683685,1482.0884218215942,2.1463809162014513e-05
921922,1843845,1843844,3687689,1483.5384199619293,2.1150257794033678e-05
922923,1845847,1845846,3691693,1484.95734500885,2.084125821966154e-05
923924,1847849,1847848,3695697,1486.3815550804138,2.053674415947171e-05
924925,1849851,1849850,3699701,1488.2281138896942,2.0236650357219332e-05
925926,1851853,1851852,3703705,1489.690724849701,1.994091337564896e-05
926927,1853855,1853854,3707709,1491.090471982956,1.9649468981697282e-05
927928,1855857,1855856,3711713,1492.3949179649353,1.936225555709825e-05
928929,1857859,1857858,3715717,1493.6897749900818,1.9079211256212147e-05
929930,1859861,1859860,3719721,1495.0089528560638,1.8800275597641303e-05
930931,1861863,1861862,3723725,1496.8992431163788,1.852538900948275e-05
931932,1863865,1863864,3727729,1498.9405510425568,1.8254492601954553e-05
932933,1865867,1865866,3731733,1500.9283239841461,1.798752839476947e-05
933934,1867869,1867868,3735737,1502.78240275383,1.772443954450864e-05
934935,1869871,1869870,3739741,1505.236014842987,1.746516943512688e-05
935936,1871873,1871872,3743745,1509.102061033249,1.720966281482106e-05
936937,1873875,1873874,3747749,1511.9758749008179,1.6957865113909065e-05
937938,1875877,1875876,3751753,1514.3516409397125,1.6709722217456147e-05
938939,1877879,1877878,3755757,1516.035474061966,1.6465181261082762e-05
939940,1879881,1879880,3759761,1517.5780098438263,1.6224189721469884e-05
940941,1881883,1881882,3763765,1519.1111340522766,1.5986696212166862e-05
941942,1883885,1883884,3767769,1521.0358669757843,1.5752650028844073e-05
942943,1885887,1885886,3771773,1522.976313829422,1.552200103560608e-05
943944,1887889,1887888,3775777,1524.777498960495,1.5294699778678478e-05
944945,1889891,1889890,3779781,1526.5182268619537,1.5070697713781556e-05
945946,1891893,1891892,3783785,1528.284462928772,1.4849947092443472e-05
946947,1893895,1893894,3787789,1529.9761190414429,1.4632400393566058e-05
947948,1895897,1895896,3791793,1531.7075290679932,1.4418011346606363e-05
948949,1897899,1897898,3795797,1533.5085229873657,1.4206734249455621e-05
949950,1899901,1899900,3799801,1535.9629938602448,1.3998523513691907e-05
950951,1901903,1901902,3803805,1537.7166409492493,1.3793334801448509e-05
951952,1903905,1903904,3807809,1539.5263550281525,1.3591124343292904e-05
952953,1905907,1905906,3811813,1541.2057979106903,1.3391848597166245e-05
953954,1907909,1907908,3815817,1542.9289529323578,1.3195465157878061e-05
954955,1909911,1909910,3819821,1544.4528048038483,1.3001932188672072e-05
955956,1911913,1911912,3823825,1546.0394780635834,1.281120808016567e-05
956957,1913915,1913914,3827829,1547.5620911121368,1.2623252018784115e-05
957958,1915917,1915916,3831833,1549.1743078231812,1.2438023986760527e-05
958959,1917919,1917918,3835837,1550.9116070270538,1.2255484307388542e-05
959960,1919921,1919920,3839841,1552.3922340869904,1.2075593872395984e-05
960961,1921923,1921922,3843845,1554.1627299785614,1.1898314369318541e-05
961962,1923925,1923924,3847849,1556.019613981247,1.1723607713065576e-05
962963,1925927,1925926,3851853,1557.9082930088043,1.1551436728041153e-05
963964,1927929,1927928,3855857,1559.764002084732,1.1381764352336177e-05
964965,1929931,1929930,3859861,1561.4870820045471,1.1214554547223088e-05
965966,1931933,1931932,3863865,1563.1352100372314,1.1049771501348005e-05
966967,1933935,1933934,3867869,1564.7423770427704,1.0887379858104396e-05
967968,1935937,1935936,3871873,1566.3812589645386,1.0727345170380431e-05
968969,1937939,1937938,3875877,1568.0906569957733,1.0569632991064282e-05
969970,1939941,1939940,3879881,1569.6975438594818,1.0414209555165144e-05
970971,1941943,1941942,3883885,1571.3745849132538,1.0261041893500078e-05
971972,1943945,1943944,3887889,1573.0231239795685,1.011009726425982e-05
972973,1945947,1945946,3891893,1574.5717010498047,9.961342925635108e-06
973974,1947949,1947948,3895897,1576.1535251140594,9.814747613745567e-06
974975,1949951,1949950,3899901,1577.8078479766846,9.670279609963472e-06
975976,1951953,1951952,3903905,1579.4008059501648,9.527908332529478e-06
976977,1953955,1953954,3907909,1580.9208879470825,9.387603085997398e-06
977978,1955957,1955956,3911913,1582.6012680530548,9.24933408441575e-06
978979,1957959,1957958,3915917,1584.1288588047028,9.113071541833051e-06
979980,1959961,1959960,3919921,1585.6806101799011,8.978786695479357e-06
980981,1961963,1961962,3923925,1587.19633102417,8.846450441524212e-06
981982,1963965,1963964,3927929,1588.6943061351776,8.71603458563186e-06
982983,1965967,1965966,3931933,1590.2179729938507,8.587511388213898e-06
983984,1967969,1967968,3935937,1591.8512148857117,8.460853450742434e-06
984985,1969971,1969970,3939941,1593.7313389778137,8.336033488376415e-06
985986,1971973,1971972,3943945,1595.4004549980164,8.213024898395815e-06
986987,1973975,1973974,3947949,1597.0232520103455,8.091801305454283e-06
987988,1975977,1975976,3951953,1598.54838681221,7.972337016326492e-06
988989,1977979,1977978,3955957,1600.2609839439392,7.85460622410028e-06
989990,1979981,1979980,3959961,1601.7771809101105,7.738584031358187e-06
990991,1981983,1981982,3963965,1603.2682361602783,7.624245313309075e-06
991992,1983985,1983984,3967969,1604.7794539928436,7.51156585465651e-06
992993,1985987,1985986,3971973,1606.2584137916565,7.400521667477733e-06
993994,1987989,1987988,3975977,1607.764769077301,7.291088763849984e-06
994995,1989991,1989990,3979981,1609.2649910449982,7.183243951658369e-06
995996,1991993,1991992,3983985,1610.845862865448,7.076964038787992e-06
996997,1993995,1993994,3987989,1612.3757519721985,6.972226401558146e-06
997998,1995997,1995996,3991993,1613.9875819683075,6.8690086436618e-06
998999,1997999,1997998,3995997,1615.5079889297485,6.767288482478762e-06
1000000,2000001,2000000,4000001,1617.0725541114807,6.667044658570376e-06


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0005440711975097656,2181.4194943796983
6,13,6,19,0.007731914520263672,475.341262047961
11,23,11,34,0.010568857192993164,269.2215147773172
17,35,17,52,0.01370382308959961,172.6347767136524
23,47,23,70,0.016872882843017578,128.11197162982648
28,57,28,85,0.020776987075805664,106.89745497453373
34,69,34,103,0.024498939514160156,90.89703659674024
40,81,40,121,0.02764582633972168,80.92403487595084
45,91,45,136,0.03040170669555664,75.4055646350912
51,103,51,154,0.03370189666748047,70.59612599936463
57,115,57,172,0.03753185272216797,66.93782025427026
62,125,62,187,0.041838884353637695,64.47695869392714
68,137,68,205,0.04690384864807129,61.961100934910974
74,149,74,223,0.0506739616394043,59.79211566003187
79,159,79,238,0.05553102493286133,58.27456052332968
85,171,85,256,0.06010603904724121,56.817651051392886
91,183,91,274,0.06392383575439453,55.698538093732395
96,193,96,289,0.06809878349304199,54.97578033758964
102,205,102,307,0.07251882553100586,54.3028992537229
108,217,108,325,0.07663893699645996,53.771986065378314
113,227,113,340,0.08077287673950195,53.38235354402559
119,239,119,358,0.08438587188720703,52.91742223202027
125,251,125,376,0.08962273597717285,52.420336897666175
130,261,130,391,0.09491896629333496,51.976409549316486
136,273,136,409,0.10164189338684082,51.4138911828868
142,285,142,427,0.10776972770690918,50.82463187679514
147,295,147,442,0.11311078071594238,50.313647586099705
153,307,153,460,0.11950087547302246,49.67584367919994
159,319,159,478,0.12598586082458496,49.013822643435105
164,329,164,493,0.13228487968444824,48.448419797262886
170,341,170,511,0.13894081115722656,47.76069773511426
176,353,176,529,0.1454300880432129,47.071279177080896
181,363,181,544,0.15088987350463867,46.501659813889546
187,375,187,562,0.15744686126708984,45.82923394258728
193,387,193,580,0.16385388374328613,45.17017766097433
198,397,198,595,0.1692488193511963,44.62920787606731
204,409,204,613,0.17518281936645508,43.986387521197
210,421,210,631,0.18125486373901367,43.34752713411194
215,431,215,646,0.18689370155334473,42.81677530070351
221,443,221,664,0.1933457851409912,42.18067175063857
227,455,227,682,0.19996285438537598,41.544299002584694
232,465,232,697,0.2057507038116455,41.01296983235011
238,477,238,715,0.21248984336853027,40.373331254076675
244,489,244,733,0.21991872787475586,39.73091391887783
249,499,249,748,0.22577166557312012,39.19349236949347
255,511,255,766,0.2325887680053711,38.54700590607035
261,523,261,784,0.24370789527893066,37.90074619447046
266,533,266,799,0.250180721282959,37.364304631269306
272,545,272,817,0.2567780017852783,36.72540542416391
278,557,278,835,0.263136625289917,36.09364836150303
283,567,283,850,0.26839494705200195,35.573402046420824
289,579,289,868,0.2745048999786377,34.9567192049567
295,591,295,886,0.27955198287963867,34.347982827107444
300,601,300,901,0.28418469429016113,33.84638733393899
306,613,306,919,0.2910647392272949,33.25098235494329
312,625,312,937,0.2984657287597656,32.66263774734762
317,635,317,952,0.3040149211883545,32.17784895510931
323,647,323,970,0.31056785583496094,31.60276804819955
329,659,329,988,0.3167150020599365,31.03477969934579
334,669,334,1003,0.32224488258361816,30.566562423337018
340,681,340,1021,0.3292880058288574,30.01039981665076
346,693,346,1039,0.3351738452911377,29.46014041681792
351,703,351,1054,0.34009289741516113,29.00606429400159
357,715,357,1072,0.34528493881225586,28.466746744174543
363,727,363,1090,0.35013365745544434,27.933892811922988
368,737,368,1105,0.3542928695678711,27.49507989429958
374,749,374,1123,0.3592708110809326,26.975013326032013
380,761,380,1141,0.3634927272796631,26.462100865233197
385,771,385,1156,0.3676338195800781,26.040056772065782
391,783,391,1174,0.372891902923584,25.539889789674362
397,795,397,1192,0.3770596981048584,25.046390408381512
402,805,402,1207,0.38036298751831055,24.640110517797666
408,817,408,1225,0.3843200206756592,24.15839965899181
414,829,414,1243,0.3895597457885742,23.682868847367445
419,839,419,1258,0.39310169219970703,23.291151371228807
425,851,425,1276,0.3969838619232178,22.826339244835253
431,863,431,1294,0.4013667106628418,22.36701887484537
436,873,436,1309,0.40535569190979004,21.988300915081936
442,885,442,1327,0.408998966217041,21.538585978154288
448,897,448,1345,0.41275787353515625,21.093995066514026
453,907,453,1360,0.41579484939575195,20.72741019113687
459,919,459,1378,0.42005467414855957,20.292208956889226
465,931,465,1396,0.4249238967895508,19.86215245143694
470,941,470,1411,0.4287757873535156,19.507716659674543
476,953,476,1429,0.43329477310180664,19.087157602947855
481,963,481,1444,0.4374568462371826,18.740689152243704
487,975,487,1462,0.4411137104034424,18.329768891379672
493,987,493,1480,0.44492173194885254,17.924171738842688
498,997,498,1495,0.4485907554626465,17.590249950868838
504,1009,504,1513,0.4525127410888672,17.1944061482086
510,1021,510,1531,0.45656490325927734,16.80379327116043
515,1031,515,1546,0.45957088470458984,16.482204696050303
521,1043,521,1564,0.46330976486206055,16.100918961261186
527,1055,527,1582,0.46698975563049316,15.724605862734165
532,1065,532,1597,0.4704866409301758,15.414783296224186
538,1077,538,1615,0.47431492805480957,15.047514537390043
544,1089,544,1633,0.4781978130340576,14.68517580920934
549,1099,549,1648,0.48145580291748047,14.386988987590826
555,1111,555,1666,0.48535776138305664,14.033663733000708
561,1123,561,1684,0.48972177505493164,13.685224530902701
566,1133,566,1699,0.49289870262145996,13.398581526181943
572,1145,572,1717,0.49721503257751465,13.059088023725508
578,1157,578,1735,0.5022919178009033,12.724519621129161
583,1167,583,1750,0.5061948299407959,12.44952057377327
589,1179,589,1768,0.510887861251831,12.124150586568817
595,1191,595,1786,0.5147106647491455,11.80388221502335
600,1201,600,1801,0.517838716506958,11.540910947418297
606,1213,606,1819,0.5228378772735596,11.230049713581252
612,1225,612,1837,0.5278947353363037,10.924298972420047
617,1235,617,1852,0.5320818424224854,10.67338263016677
623,1247,623,1870,0.537545919418335,10.376892522634193
629,1259,629,1888,0.5428659915924072,10.085381824844944
634,1269,634,1903,0.5468659400939941,9.846222424750636
640,1281,640,1921,0.5514466762542725,9.563709244205029
646,1293,646,1939,0.5564818382263184,9.286045545250659
651,1303,651,1954,0.5604188442230225,9.058346946772986
657,1315,657,1972,0.5653576850891113,8.78953022904443
663,1327,663,1990,0.5694777965545654,8.525549732458103
668,1337,668,2005,0.5727348327636719,8.309278538963213
674,1349,674,2023,0.5764029026031494,8.054233742906149
680,1361,680,2041,0.5802018642425537,7.804101062697555
685,1371,685,2056,0.5833728313446045,7.599421422482351
691,1383,691,2074,0.5872838497161865,7.3583273740800905
697,1395,697,2092,0.5912008285522461,7.122160295334993
702,1405,702,2107,0.5953218936920166,6.929106981734662
708,1417,708,2125,0.6001129150390625,6.701924687167548
714,1429,714,2143,0.6053357124328613,6.479598803353042
719,1439,719,2158,0.6090118885040283,6.2980049166205845
725,1451,725,2176,0.6128168106079102,6.084458962200529
731,1463,731,2194,0.616506814956665,5.875620319128075
736,1473,736,2209,0.6205887794494629,5.705140189091139
742,1485,742,2227,0.6245718002319336,5.504777573497904
748,1497,748,2245,0.6281819343566895,5.308965880839878
753,1507,753,2260,0.6312687397003174,5.149237685339131
759,1519,759,2278,0.6352968215942383,4.9616754885820455
765,1531,765,2296,0.63997483253479,4.7785757988169735
770,1541,770,2311,0.6443099975585938,4.629385879071378
776,1553,776,2329,0.6494338512420654,4.4544102802829
782,1565,782,2347,0.6545238494873047,4.283830655161751
787,1575,787,2362,0.6580088138580322,4.145016092211449
793,1587,793,2380,0.6627316474914551,3.982407066873975
799,1599,799,2398,0.6679549217224121,3.82408343004613
804,1609,804,2413,0.6722538471221924,3.69538260176364
810,1621,810,2431,0.6765038967132568,3.544774672094036
816,1633,816,2449,0.6801390647888184,3.398292497876014
821,1643,821,2464,0.6835830211639404,3.2793335991316326
827,1655,827,2482,0.6877167224884033,3.140266180550725
833,1667,833,2500,0.6926147937774658,3.0051670831868478
838,1677,838,2515,0.6967990398406982,2.8955793576420774
844,1689,844,2533,0.7015879154205322,2.7676247078436518
850,1701,850,2551,0.7056987285614014,2.6434954373243045
855,1711,855,2566,0.7097606658935547,2.542938441501633
861,1723,861,2584,0.7140789031982422,2.4256830560151457
867,1735,867,2602,0.7193608283996582,2.312096565554384
872,1745,872,2617,0.7246789932250977,2.2202010318935663
878,1757,878,2635,0.7303988933563232,2.1131860523051955
884,1769,884,2653,0.7353019714355469,2.0096699361462242
889,1779,889,2668,0.7407538890838623,1.9260359985871673
895,1791,895,2686,0.745589017868042,1.828779811967138
901,1803,901,2704,0.750450849533081,1.7348563830371404
906,1813,906,2719,0.7539608478546143,1.6590924118647763
912,1825,912,2737,0.7584378719329834,1.5711345173907603
918,1837,918,2755,0.7628350257873535,1.4863518506724631
923,1847,923,2770,0.7659709453582764,1.418083716848514
929,1859,929,2788,0.7710559368133545,1.3389707350016806
935,1871,935,2806,0.7760787010192871,1.2628619244673018
940,1881,940,2821,0.77927565574646,1.2016848340036859
946,1893,946,2839,0.7830069065093994,1.1309090599932006
952,1905,952,2857,0.7879040241241455,1.0629436315472276
957,1915,957,2872,0.7912540435791016,1.0084022270319792
963,1927,963,2890,0.7949337959289551,0.9454093353905364
969,1939,969,2908,0.7986979484558105,0.8850352092281355
974,1949,974,2923,0.8019378185272217,0.8366798778869224
980,1961,980,2941,0.805635929107666,0.7809524359079205
986,1973,986,2959,0.8091819286346436,0.7276838573562827
991,1983,991,2974,0.8120729923248291,0.6851364191112452
997,1995,997,2992,0.8156406879425049,0.6362501446617443
1003,2007,1003,3010,0.820462703704834,0.5896866142137469
1008,2017,1008,3025,0.8248238563537598,0.5526218643780112
1014,2029,1014,3043,0.8293278217315674,0.5101837473280284
1020,2041,1020,3061,0.8346817493438721,0.4699168103146576
1025,2051,1025,3076,0.838864803314209,0.437976414298646
1031,2063,1031,3094,0.8427069187164307,0.4015330653944602
1037,2075,1037,3112,0.8479747772216797,0.36708770415407344
1042,2085,1042,3127,0.852092981338501,0.3398654149243612
1048,2097,1048,3145,0.8568768501281738,0.30892596724277155
1054,2109,1054,3163,0.8619101047515869,0.2798168999183872
1059,2119,1059,3178,0.8658719062805176,0.2569176800502646
1065,2131,1065,3196,0.8709368705749512,0.23102189993198863
1071,2143,1071,3214,0.8762288093566895,0.20680280875762946
1076,2153,1076,3229,0.8799617290496826,0.18786230104217339
1082,2165,1082,3247,0.8836917877197266,0.16657733202760028
1088,2177,1088,3265,0.8886868953704834,0.14681613265611304
1093,2187,1093,3280,0.8918569087982178,0.1314740567128183
1099,2199,1099,3298,0.896636962890625,0.11437005606308048
1105,2211,1105,3316,0.9017088413238525,0.09864617512778295
1110,2221,1110,3331,0.9053938388824463,0.08656536141086235
1116,2233,1116,3349,0.9103586673736572,0.0732602155587756
1122,2245,1122,3367,0.9152719974517822,0.061219436036935804
1127,2255,1127,3382,0.9188597202301025,0.052124674606034205
1133,2267,1133,3400,0.9233818054199219,0.042305593202740965
1139,2279,1139,3418,0.9285078048706055,0.03364339379618286
1144,2289,1144,3433,0.9318568706512451,0.027278246529590433
1150,2301,1150,3451,0.9368588924407959,0.02062519452726974
1156,2313,1156,3469,0.9417927265167236,0.015002335992335247
1161,2323,1161,3484,0.9484298229217529,0.011068859713645907
1167,2335,1167,3502,0.9561569690704346,0.007209945105614679
1173,2347,1173,3520,0.9596529006958008,0.004246828049531359
1178,2357,1178,3535,0.9640567302703857,0.0024300832934613936
1184,2369,1184,3553,0.9676029682159424,0.000997285498669953
1190,2381,1190,3571,0.9719419479370117,0.00034322595229241415
1195,2391,1195,3586,0.9748988151550293,0.00036662368302131654
1201,2403,1201,3604,0.9784839153289795,0.0010463694802638202
1207,2415,1207,3622,0.9830238819122314,0.0024045645272963156
1212,2425,1212,3637,0.9866230487823486,0.004030210173709747
1218,2437,1218,3655,0.990257978439331,0.006544712336221892
1224,2449,1224,3673,0.9936697483062744,0.009643552251873189
1229,2459,1229,3688,0.9964509010314941,0.012649790377508907
1235,2471,1235,3706,0.9998879432678223,0.016740331918413176
1241,2483,1241,3724,1.0043740272521973,0.02133148617497227
1246,2493,1246,3739,1.0078368186950684,0.02552064030578549
1252,2505,1252,3757,1.0128929615020752,0.0309610062114416
1258,2517,1258,3775,1.0167179107666016,0.036827797099704185
1263,2527,1263,3790,1.0210368633270264,0.04202331250712632
1269,2539,1269,3808,1.0255277156829834,0.04860178540855031
1275,2551,1275,3826,1.029686689376831,0.05552824007338586
1280,2561,1280,3841,1.032829999923706,0.061544928005218935
1286,2573,1286,3859,1.03653883934021,0.06903309992958384
1292,2585,1292,3877,1.040024757385254,0.07678674774444971
1297,2595,1297,3892,1.042815923690796,0.08343117715241988
1303,2607,1303,3910,1.0464558601379395,0.0916019416878271
1309,2619,1309,3928,1.0507347583770752,0.09996551352878669
1314,2629,1314,3943,1.0538609027862549,0.1070662321525333
1320,2641,1320,3961,1.0583808422088623,0.11572593531707298
1326,2653,1326,3979,1.0628418922424316,0.12451772208135026
1331,2663,1331,3994,1.0661499500274658,0.13193071234468334
1337,2675,1337,4012,1.070112705230713,0.14091334880879458
1343,2687,1343,4030,1.0748538970947266,0.14997342698188731
1348,2697,1348,4045,1.0786628723144531,0.15756999850066222
1354,2709,1354,4063,1.0823979377746582,0.166727590408982
1360,2721,1360,4081,1.0862059593200684,0.175916464622901
1365,2731,1365,4096,1.089829921722412,0.18358758291890354
1371,2743,1371,4114,1.0945789813995361,0.1927976747450657
1377,2755,1377,4132,1.0988380908966064,0.2020002188048693
1382,2765,1382,4147,1.102529764175415,0.20965327004364553
1388,2777,1388,4165,1.1065196990966797,0.21880558841314723
1394,2789,1394,4183,1.1118638515472412,0.22790960893405554
1399,2799,1399,4198,1.116379976272583,0.23544842610749583
1405,2811,1405,4216,1.1211740970611572,0.24442449664365995
1411,2823,1411,4234,1.130378007888794,0.253309911456995
1416,2833,1416,4249,1.134917974472046,0.2606353044284333
1422,2845,1422,4267,1.1392309665679932,0.26931994930134806
1427,2855,1427,4282,1.1433937549591064,0.2764611726322528
1433,2867,1433,4300,1.1484129428863525,0.284906390634319
1439,2879,1439,4318,1.1524627208709717,0.29320696937236335
1444,2889,1444,4333,1.1555976867675781,0.3000071325926683
1450,2901,1450,4351,1.1593496799468994,0.30801958085987735
1456,2913,1456,4369,1.1639199256896973,0.3158632185133001
1461,2923,1461,4384,1.1678197383880615,0.3222651017172211
1467,2935,1467,4402,1.1722118854522705,0.32977977424116034
1473,2947,1473,4420,1.175710916519165,0.3371053673233746
1478,2957,1478,4435,1.1786696910858154,0.3430611987856764
1484,2969,1484,4453,1.1821858882904053,0.35002476714009845
1490,2981,1490,4471,1.1859078407287598,0.3567833283063919
1495,2991,1495,4486,1.189194917678833,0.3622552924636011
1501,3003,1501,4504,1.194443702697754,0.36862528292465413
1507,3015,1507,4522,1.199828863143921,0.37477657701163025
1512,3025,1512,4537,1.2041599750518799,0.37973222035998333
1518,3037,1518,4555,1.2082078456878662,0.38547053065099135
1524,3049,1524,4573,1.2122178077697754,0.3909773454995502
1529,3059,1529,4588,1.2150869369506836,0.39538662589552587
1535,3071,1535,4606,1.2187058925628662,0.4004589457858856
1541,3083,1541,4624,1.2222228050231934,0.4052895161538572
1546,3093,1546,4639,1.225172996520996,0.40912826097542165
1552,3105,1552,4657,1.229360818862915,0.4135084936272051
1558,3117,1558,4675,1.234252691268921,0.41763979133304474
1563,3127,1563,4690,1.2372608184814453,0.42089097512723583
1569,3139,1569,4708,1.2418959140777588,0.4245611218764225
1575,3151,1575,4726,1.246783971786499,0.427977836910145
1580,3161,1580,4741,1.2509467601776123,0.4306309819875196
1586,3173,1586,4759,1.254300832748413,0.43358166098403217
1592,3185,1592,4777,1.259023904800415,0.4362784002086073
1597,3195,1597,4792,1.2627599239349365,0.43833229304198085
1603,3207,1603,4810,1.2671058177947998,0.4405659122724046
1609,3219,1609,4828,1.271101951599121,0.4425487737360072
1614,3229,1614,4843,1.2742557525634766,0.4440106479522683
1620,3241,1620,4861,1.277923822402954,0.44553751675391595
1626,3253,1626,4879,1.2817208766937256,0.44681762898062516
1631,3263,1631,4894,1.284836769104004,0.44769686224333327
1637,3275,1637,4912,1.289078712463379,0.4485280938940832
1643,3287,1643,4930,1.2945926189422607,0.44911651120139595
1648,3297,1648,4945,1.2990920543670654,0.44942254139846227
1654,3309,1654,4963,1.303602933883667,0.4495701660190434
1660,3321,1660,4981,1.3074288368225098,0.4494801325458866
1665,3331,1665,4996,1.3105196952819824,0.44922518278497137
1671,3343,1671,5014,1.3141648769378662,0.448705490384782
1677,3355,1677,5032,1.317884922027588,0.4479552075176798
1682,3365,1682,5047,1.320863962173462,0.4471560073557157
1688,3377,1688,5065,1.3258037567138672,0.44599110310844026
1694,3389,1694,5083,1.330934762954712,0.44460509263490167
1699,3399,1699,5098,1.3339908123016357,0.44328405832141016
1705,3411,1705,5116,1.3381667137145996,0.44150327190197913
1711,3423,1711,5134,1.3416857719421387,0.43951335852079865
1716,3433,1716,5149,1.3455078601837158,0.43769860819418227
1722,3445,1722,5167,1.3500618934631348,0.43533701652950185
1728,3457,1728,5185,1.3548898696899414,0.4327789755636786
1733,3467,1733,5200,1.3583228588104248,0.43050030024551234
1739,3479,1739,5218,1.3625867366790771,0.42759313923886566
1745,3491,1745,5236,1.367527961730957,0.42450143365022086
1750,3501,1750,5251,1.3705778121948242,0.4217870603794154
1756,3513,1756,5269,1.374189853668213,0.41836800829855747
1762,3525,1762,5287,1.3775157928466797,0.4147767079901996
1767,3535,1767,5302,1.3811709880828857,0.411655794559465
1773,3547,1773,5320,1.3856678009033203,0.40776119196539184
1779,3559,1779,5338,1.3905177116394043,0.403708345338714
1784,3569,1784,5353,1.3940708637237549,0.4002138953311487
1790,3581,1790,5371,1.3988637924194336,0.3958847067347051
1796,3593,1796,5389,1.4027929306030273,0.39141244534062025
1801,3603,1801,5404,1.4063596725463867,0.3875802176938805
1807,3615,1807,5422,1.410017728805542,0.3828599107185937
1813,3627,1813,5440,1.4138257503509521,0.37801216824107087
1818,3637,1818,5455,1.4170408248901367,0.37387907836045997
1824,3649,1824,5473,1.4223120212554932,0.3688122727917289
1830,3661,1830,5491,1.4264919757843018,0.3636339317737338
1835,3671,1835,5506,1.429844856262207,0.35923746110870525
1841,3683,1841,5524,1.4338576793670654,0.35386902264269793
1847,3695,1847,5542,1.4393069744110107,0.34840458228052285
1852,3705,1852,5557,1.4445037841796875,0.34378138475119613
1858,3717,1858,5575,1.4492697715759277,0.33815471246794004
1864,3729,1864,5593,1.4534318447113037,0.33244700867328447
1869,3739,1869,5608,1.456618070602417,0.32763251302651497
1875,3751,1875,5626,1.4603238105773926,0.32179007652450764
1881,3763,1881,5644,1.4643938541412354,0.3158818374429302
1886,3773,1886,5659,1.4684388637542725,0.31091202788252303
1892,3785,1892,5677,1.4735949039459229,0.30489755668941143
1898,3797,1898,5695,1.4774746894836426,0.29883306833664847
1903,3807,1903,5710,1.4811408519744873,0.2937451574141505
1909,3819,1909,5728,1.4852197170257568,0.28760348180105666
1915,3831,1915,5746,1.488846778869629,0.2814275665000423
1920,3841,1920,5761,1.49208402633667,0.27625879503625583
1926,3853,1926,5779,1.4967317581176758,0.2700344211857555
1932,3865,1932,5797,1.5021939277648926,0.26379139633309023
1937,3875,1937,5812,1.5060639381408691,0.258578572209899
1943,3887,1943,5830,1.5096838474273682,0.2523155106827062
1949,3899,1949,5848,1.5132768154144287,0.24604911612368596
1954,3909,1954,5863,1.5161778926849365,0.24082833478371413
1960,3921,1960,5881,1.519709825515747,0.23456922592708906
1966,3933,1966,5899,1.523310899734497,0.2283210718818509
1971,3943,1971,5914,1.5261309146881104,0.22312602967190287
1977,3955,1977,5932,1.5306098461151123,0.21691000328007704
1983,3967,1983,5950,1.5350987911224365,0.2107177992504603
1988,3977,1988,5965,1.5382459163665771,0.2055789484717252
1994,3989,1994,5983,1.5419847965240479,0.19944162272258836
2000,4001,2000,6001,1.545644760131836,0.19334029930109864
2005,4011,2005,6016,1.5486578941345215,0.1882864623776186
2011,4023,2011,6034,1.5525016784667969,0.18226230799098175
2017,4035,2017,6052,1.5564789772033691,0.17628635874746124
2022,4045,2022,6067,1.5604338645935059,0.17134633577006753
2028,4057,2028,6085,1.5651500225067139,0.1654699446532959
2034,4069,2034,6103,1.5694808959960938,0.15965390004714664
2039,4079,2039,6118,1.5731489658355713,0.15485632357206214
2045,4091,2045,6136,1.577807903289795,0.14916175549444688
2051,4103,2051,6154,1.581355094909668,0.1435391977169047
2056,4113,2056,6169,1.585007905960083,0.13891155800570232
2062,4125,2062,6187,1.5906996726989746,0.13343102298108533
2068,4137,2068,6205,1.5948598384857178,0.12803307778244744
2073,4147,2073,6220,1.5993778705596924,0.12360028887974295
2079,4159,2079,6238,1.6041288375854492,0.11836222552392428
2085,4171,2085,6256,1.6093077659606934,0.11321553733898782
2090,4181,2090,6271,1.6135568618774414,0.1089983405233852
2096,4193,2096,6289,1.6178698539733887,0.10402587943303843
2102,4205,2102,6307,1.6216089725494385,0.09915178015296533
2107,4215,2107,6322,1.6246058940887451,0.09516674916972079
2113,4227,2113,6340,1.6281678676605225,0.09047860659836715
2119,4239,2119,6358,1.6317768096923828,0.08589485052505097
2124,4249,2124,6373,1.6347310543060303,0.08215626738012816
2130,4261,2130,6391,1.639375925064087,0.07776917138983208
2136,4273,2136,6409,1.644331693649292,0.07349217725845847
2141,4283,2141,6424,1.6483206748962402,0.07001353104283226
2147,4295,2147,6442,1.6531789302825928,0.06594342417270127
2153,4307,2153,6460,1.6582117080688477,0.06198880736587853
2158,4317,2158,6475,1.6621358394622803,0.05878279550051957
2164,4329,2164,6493,1.6670947074890137,0.05504444463372238
2170,4341,2170,6511,1.6718809604644775,0.05142634698722759
2175,4351,2175,6526,1.675527811050415,0.048504177454560704
2181,4363,2181,6544,1.679926872253418,0.04511019619974377
2187,4375,2187,6562,1.6840567588806152,0.041840133214009256
2192,4385,2192,6577,1.687356948852539,0.03921040552222621
2198,4397,2198,6595,1.69144868850708,0.03616972611689562
2204,4409,2204,6613,1.6950819492340088,0.033254936146363434
2209,4419,2209,6628,1.697948932647705,0.030922293237154008
2215,4431,2215,6646,1.701962947845459,0.028238783010237967
2221,4443,2221,6664,1.7060978412628174,0.025681329893586735
2226,4453,2226,6679,1.7091188430786133,0.023646224027174867
2232,4465,2232,6697,1.7134289741516113,0.021319103555924812
2238,4477,2238,6715,1.717862844467163,0.01911702429720208
2243,4487,2243,6730,1.7209968566894531,0.017377118653030266
2249,4499,2249,6748,1.725822925567627,0.015402964736949798
2255,4511,2255,6766,1.7307178974151611,0.013552356158811563
2260,4521,2260,6781,1.7348217964172363,0.012104137211167654
2266,4533,2266,6799,1.739583969116211,0.010478490181185407
2272,4545,2272,6817,1.744743824005127,0.008974643672559068
2277,4555,2277,6832,1.7483856678009033,0.007813971022983424
2283,4567,2283,6850,1.7537908554077148,0.006531527414608718
2289,4579,2289,6868,1.7582688331604004,0.005368650859509216
2294,4589,2294,6883,1.7621729373931885,0.004490205376896483
2300,4601,2300,6901,1.7677688598632812,0.0035438267567542425
2306,4613,2306,6919,1.772655725479126,0.00271377039825893
2311,4623,2311,6934,1.7771847248077393,0.0021098546393432116
2317,4635,2317,6952,1.7830207347869873,0.001489090122390735
2323,4647,2323,6970,1.7883226871490479,0.0009799993745218671
2328,4657,2328,6985,1.792536735534668,0.0006396558499091043
2334,4669,2334,7003,1.7973499298095703,0.00033012678090926784
2340,4681,2340,7021,1.8028678894042969,0.00012642321905786957
2345,4691,2345,7036,1.8069970607757568,3.589972232020955e-05
2351,4703,2351,7054,1.8116238117218018,2.037836975432583e-05
2357,4715,2357,7072,1.8151679039001465,0.00010425693722027063
2362,4725,2362,7087,1.8192389011383057,0.00024841752338033984
2368,4737,2368,7105,1.8244118690490723,0.0005085125500272625
2373,4747,2373,7120,1.8281407356262207,0.0007962580372122829
2379,4759,2379,7138,1.8334169387817383,0.001224716594038
2385,4771,2385,7156,1.8385059833526611,0.0017416561430536603
2390,4781,2390,7171,1.8432199954986572,0.0022382925137662824
2396,4793,2396,7189,1.8478548526763916,0.0029111602113971458
2402,4805,2402,7207,1.8542699813842773,0.003665560910462773
2407,4815,2407,7222,1.8587899208068848,0.004354662892296801
2413,4827,2413,7240,1.8631079196929932,0.005251828917948842
2419,4839,2419,7258,1.8685297966003418,0.006223066541906519
2424,4849,2424,7273,1.8731939792633057,0.007087004847676326
2430,4861,2430,7291,1.8783879280090332,0.008186741156919197
2436,4873,2436,7309,1.8826618194580078,0.009352445627200723
2441,4883,2441,7324,1.8864319324493408,0.010372100473318824
2447,4895,2447,7342,1.8913118839263916,0.011650937863805666
2453,4907,2453,7360,1.896528959274292,0.012987151618744974
2458,4917,2458,7375,1.9006948471069336,0.014142267165539124
2464,4929,2464,7393,1.9053997993469238,0.015575657566614609
2470,4941,2470,7411,1.9105148315429688,0.017057685773238518
2475,4951,2475,7426,1.9142930507659912,0.018327650542005358
2481,4963,2481,7444,1.919205904006958,0.019890899489041658
2487,4975,2487,7462,1.9244239330291748,0.021494154980132407
2492,4985,2492,7477,1.9289138317108154,0.02285859667040313
2498,4997,2498,7495,1.932804822921753,0.024527425117639723
2504,5009,2504,7513,1.937195062637329,0.02622782869434559
2509,5019,2509,7528,1.9411919116973877,0.027666838571690278
2515,5031,2515,7546,1.9462947845458984,0.029417539673886495
2521,5043,2521,7564,1.9507789611816406,0.0311915665321294
2526,5053,2526,7579,1.9540948867797852,0.03268565596999906
2532,5065,2532,7597,1.9578378200531006,0.03449494269000297
2538,5077,2538,7615,1.9614858627319336,0.03631936458793916
2543,5087,2543,7630,1.9644370079040527,0.03784918434951123
2549,5099,2549,7648,1.968371868133545,0.03969381133720162
2555,5111,2555,7666,1.9727427959442139,0.0415453353242583
2560,5121,2560,7681,1.9758408069610596,0.04309144328783532
2566,5133,2566,7699,1.9808228015899658,0.04494807584717364
2572,5145,2572,7717,1.9856319427490234,0.04680342777703572
2577,5155,2577,7732,1.9888968467712402,0.04834654175340347
2583,5167,2583,7750,1.9927308559417725,0.05019227046705055
2589,5179,2589,7768,1.9973487854003906,0.052028898094704346
2594,5189,2594,7783,2.001643657684326,0.053550575835060954
2600,5201,2600,7801,2.0069339275360107,0.055363773809176564
2606,5213,2606,7819,2.011302947998047,0.05716066985894486
2611,5223,2611,7834,2.0148868560791016,0.058643914364211014
2617,5235,2617,7852,2.019150733947754,0.06040481437287326
2623,5247,2623,7870,2.0233378410339355,0.062142890567884024
2628,5257,2628,7885,2.0280656814575195,0.06357228914157531
2634,5269,2634,7903,2.0332558155059814,0.06526293988872567
2640,5281,2640,7921,2.0386297702789307,0.06692477006708941
2645,5291,2645,7936,2.043071985244751,0.06828614564426516
2651,5303,2651,7954,2.04724383354187,0.06988988466343926
2657,5315,2657,7972,2.051076889038086,0.07145913371698498
2662,5325,2662,7987,2.0554356575012207,0.07273909945922696
2668,5337,2668,8005,2.0606307983398438,0.07424013108823146
2674,5349,2674,8023,2.0657737255096436,0.07570132448745426
2679,5359,2679,8038,2.069429636001587,0.07688727206243584
2685,5371,2685,8056,2.074436902999878,0.07827088013095818
2691,5383,2691,8074,2.0785698890686035,0.07960983980399305
2696,5393,2696,8089,2.081829786300659,0.0806904318199031
2702,5405,2702,8107,2.0857737064361572,0.08194365617555377
2708,5417,2708,8125,2.089550733566284,0.08314818609483154
2713,5427,2713,8140,2.093369722366333,0.08411387313276464
2719,5439,2719,8158,2.098228931427002,0.08522600536673508
2725,5451,2725,8176,2.10257887840271,0.08628620847514412
2730,5461,2730,8191,2.106235980987549,0.08712934207107992
2736,5473,2736,8209,2.110140800476074,0.08809188391012412
2742,5485,2742,8227,2.1138477325439453,0.08899995151318763
2747,5495,2747,8242,2.118285894393921,0.0897145088989646
2753,5507,2753,8260,2.123807907104492,0.09052076614284488
2759,5519,2759,8278,2.128626823425293,0.09127054141697499
2764,5529,2764,8293,2.1324098110198975,0.09185177802180533
2770,5541,2770,8311,2.1369497776031494,0.09249650564993317
2776,5553,2776,8329,2.1405649185180664,0.09308323319896772
2781,5563,2781,8344,2.1434340476989746,0.0935275717862396
2787,5575,2787,8362,2.1468379497528076,0.09400696501529637
2793,5587,2793,8380,2.1501970291137695,0.09442740741963007
2798,5597,2798,8395,2.153775930404663,0.0947326120830212
2804,5609,2804,8413,2.1586058139801025,0.09504457384139187
2810,5621,2810,8431,2.1633107662200928,0.0952973006250204
2815,5631,2815,8446,2.1662516593933105,0.09546270194437056
2821,5643,2821,8464,2.1705589294433594,0.09560706172771916
2827,5655,2827,8482,2.175520658493042,0.0956925876527066
2832,5665,2832,8497,2.178727865219116,0.09571912704780061
2838,5677,2838,8515,2.1842780113220215,0.09569760927990956
2844,5689,2844,8533,2.1895999908447266,0.09561828032622088
2849,5699,2849,8548,2.1936798095703125,0.09550836467440149
2855,5711,2855,8566,2.1987369060516357,0.09532437154814488
2861,5723,2861,8584,2.2052717208862305,0.09508412036927893
2866,5733,2866,8599,2.209697723388672,0.09484141042344163
2872,5745,2872,8617,2.2137038707733154,0.0944997716879925
2878,5757,2878,8635,2.2178759574890137,0.0941038826156273
2883,5767,2883,8650,2.2215628623962402,0.09373311540298346
2889,5779,2889,8668,2.226670742034912,0.09323990293057705
2895,5791,2895,8686,2.232050895690918,0.09269486094490276
2900,5801,2900,8701,2.2357540130615234,0.09220175172470135
2906,5813,2906,8719,2.239763021469116,0.09156419468740751
2912,5825,2912,8737,2.2438149452209473,0.09087763287755024
2917,5835,2917,8752,2.247361660003662,0.09026885112746186
2923,5847,2923,8770,2.2513248920440674,0.08949532256747261
2929,5859,2929,8788,2.2559847831726074,0.08867601448014284
2934,5869,2934,8803,2.2600629329681396,0.08795917296197331
2940,5881,2940,8821,2.2648227214813232,0.0870591609781286
2946,5893,2946,8839,2.268847942352295,0.08611696553737147
2951,5903,2951,8854,2.2724149227142334,0.08530054964683131
2957,5915,2957,8872,2.2759907245635986,0.08428454082820735
2963,5927,2963,8890,2.279719829559326,0.08323025287563723
2968,5937,2968,8905,2.282801866531372,0.08232347501154891
2974,5949,2974,8923,2.2871549129486084,0.08120276184286013
2980,5961,2980,8941,2.292247772216797,0.08004790986603894
2985,5971,2985,8956,2.2959706783294678,0.0790605412333889
2991,5983,2991,8974,2.299452781677246,0.07784702928120169
2997,5995,2997,8992,2.3029699325561523,0.07660370000280636
3002,6005,3002,9007,2.306337833404541,0.07554594167959294
3008,6017,3008,9025,2.3102898597717285,0.07425201755700073
3014,6029,3014,9043,2.3144309520721436,0.07293274760615986
3019,6039,3019,9058,2.318459987640381,0.07181515518027481
3025,6051,3025,9076,2.323943853378296,0.07045360737731698
3031,6063,3031,9094,2.3289709091186523,0.06907130667661932
3036,6073,3036,9109,2.3332178592681885,0.06790471983219959
3042,6085,3042,9127,2.3383827209472656,0.06648863605028055
3048,6097,3048,9145,2.343411922454834,0.06505645594381804
3053,6107,3053,9160,2.3477530479431152,0.06385186182399138
3059,6119,3059,9178,2.3535947799682617,0.06239443254366961
3065,6131,3065,9196,2.357408046722412,0.060925539865706924
3070,6141,3070,9211,2.360585927963257,0.05969387129050574
3076,6153,3076,9229,2.3644628524780273,0.05820814662752127
3082,6165,3082,9247,2.3686039447784424,0.056715498254447994
3087,6175,3087,9262,2.371896743774414,0.05546747304208566
3093,6187,3093,9280,2.376110792160034,0.053966215243690385
3099,6199,3099,9298,2.3865418434143066,0.052462467173768346
3104,6209,3104,9313,2.3911118507385254,0.051208555219886875
3110,6221,3110,9331,2.395443916320801,0.04970424288876529
3116,6233,3116,9349,2.400852918624878,0.04820178741260861
3121,6243,3121,9364,2.404021739959717,0.0469522526819901
3127,6255,3127,9382,2.407867908477783,0.04545712640231159
3133,6267,3133,9400,2.411773920059204,0.0439681145898021
3138,6277,3138,9415,2.4156908988952637,0.042733005200375374
3144,6289,3144,9433,2.420224666595459,0.04125901262523257
3150,6301,3150,9451,2.4237759113311768,0.039795248448399434
3155,6311,3155,9466,2.4267988204956055,0.03858427019042665
3161,6323,3161,9484,2.430764675140381,0.03714287335174049
3167,6335,3167,9502,2.4356019496917725,0.03571558560156518
3172,6345,3172,9517,2.439866781234741,0.03453789409445562
3178,6357,3178,9535,2.443643808364868,0.033139811831802035
3184,6369,3184,9553,2.4477996826171875,0.03175940331186666
3189,6379,3189,9568,2.451427698135376,0.03062341230815946
3195,6391,3195,9586,2.457300901412964,0.029278424622702914
3201,6403,3201,9604,2.4616546630859375,0.02795432641653406
3206,6413,3206,9619,2.465686798095703,0.026867631184359198
3212,6425,3212,9637,2.4700658321380615,0.025584544682942578
3218,6437,3218,9655,2.474616765975952,0.024325242632585287
3223,6447,3223,9670,2.4783918857574463,0.023294683415088002
3229,6459,3229,9688,2.4827957153320312,0.022081446269908156
3235,6471,3235,9706,2.4866509437561035,0.02089462247931806
3240,6481,3240,9721,2.489694833755493,0.019926408733681455
3246,6493,3246,9739,2.4938907623291016,0.018790249685935123
3252,6505,3252,9757,2.4975688457489014,0.017682891954223123
3257,6515,3257,9772,2.5011839866638184,0.016782658498755154
3263,6527,3263,9790,2.505558729171753,0.015730100823702742
3269,6539,3269,9808,2.5094406604766846,0.014708451320075255
3274,6549,3274,9823,2.512807846069336,0.01388116502948833
3280,6561,3280,9841,2.5166878700256348,0.012917859578919888
3286,6573,3286,9859,2.5206117630004883,0.01198720099671391
3291,6583,3291,9874,2.523859977722168,0.011236961207941931
3297,6595,3297,9892,2.527784824371338,0.010367442523602222
3302,6605,3302,9907,2.531038999557495,0.009668762398405306
3308,6617,3308,9925,2.53562593460083,0.008861760592822066
3314,6629,3314,9943,2.540776014328003,0.00808932326856393
3319,6639,3319,9958,2.5448808670043945,0.007472222641808912
3325,6651,3325,9976,2.5497989654541016,0.006763815356066516
3331,6663,3331,9994,2.5549299716949463,0.006090620847089667
3336,6673,3336,10009,2.5589959621429443,0.005556638531288627
3342,6685,3342,10027,2.5630080699920654,0.004948386595287957
3348,6697,3348,10045,2.5722408294677734,0.004375713050080776
3353,6707,3353,10060,2.57696270942688,0.003925716409867164
3359,6719,3359,10078,2.581561803817749,0.003418438169092042
3365,6731,3365,10096,2.5857458114624023,0.002946868369463118
3370,6741,3370,10111,2.589148998260498,0.0025811617073259185
3376,6753,3376,10129,2.5932717323303223,0.002174994949768916
3382,6765,3382,10147,2.597637891769409,0.0018044007805428919
3387,6775,3387,10162,2.6014928817749023,0.0015226569905735232
3393,6787,3393,10180,2.6063339710235596,0.0012169222235343113
3399,6799,3399,10198,2.6112818717956543,0.0009462876288353073
3404,6809,3404,10213,2.6146318912506104,0.000747387859405535
3410,6821,3410,10231,2.618853807449341,0.0005404037165135378
3416,6833,3416,10249,2.6231889724731445,0.0003676726254298046
3421,6843,3421,10264,2.626617908477783,0.0002496197829486846
3427,6855,3427,10282,2.6304218769073486,0.00013866028530173935
3433,6867,3433,10300,2.6346168518066406,6.0766838828385517e-05
3438,6877,3438,10315,2.63875675201416,2.0765610997841577e-05
3444,6889,3444,10333,2.643904685974121,2.2143251499073813e-06
3450,6901,3450,10351,2.649513006210327,1.5286457824004174e-05
3455,6911,3455,10366,2.653184652328491,4.9937377411879424e-05
3461,6923,3461,10384,2.6569418907165527,0.00011953221849125839
3467,6935,3467,10402,2.660738706588745,0.00021913105717885628
3472,6945,3472,10417,2.663595676422119,0.00032461336081723857
3478,6957,3478,10435,2.667147636413574,0.00047763398038114246
3484,6969,3484,10453,2.6705617904663086,0.0006588970068150957
3489,6979,3489,10468,2.674393892288208,0.0008310501272035253
3495,6991,3495,10486,2.678931951522827,0.0010623693798379463
3501,7003,3501,10504,2.6827309131622314,0.0013200143965832467
3506,7013,3506,10519,2.685945749282837,0.0015543100410013722
3512,7025,3512,10537,2.6906518936157227,0.0018583320462539632
3518,7037,3518,10555,2.694788932800293,0.0021865765295387973
3523,7047,3523,10570,2.6979968547821045,0.002478047658655669
3529,7059,3529,10588,2.7023048400878906,0.002848630814924036
3535,7071,3535,10606,2.7066256999969482,0.003241136880319573
3540,7081,3540,10621,2.709696054458618,0.0035843568956579475
3546,7093,3546,10639,2.713873863220215,0.004014826004436145
3552,7105,3552,10657,2.71765398979187,0.004464756905122158
3557,7115,3557,10672,2.7208006381988525,0.004853920711866522
3563,7127,3563,10690,2.7245707511901855,0.005337201686984372
3569,7139,3569,10708,2.728085994720459,0.005837390448846236
3574,7149,3574,10723,2.731001853942871,0.0062664737433806295
3580,7161,3580,10741,2.7345447540283203,0.006795297001986
3586,7173,3586,10759,2.738496780395508,0.007338450993529477
3591,7183,3591,10774,2.7422468662261963,0.007801372194421674
3597,7195,3597,10792,2.746882677078247,0.008368446006556951
3603,7207,3603,10810,2.7516119480133057,0.008947287318051167
3608,7217,3608,10825,2.754859685897827,0.009437993507617648
3614,7229,3614,10843,2.758737802505493,0.010036065988742848
3620,7241,3620,10861,2.7625060081481934,0.010643348474786762
3625,7251,3625,10876,2.7662978172302246,0.011155798521485849
3631,7263,3631,10894,2.7715189456939697,0.011777608051147581
3637,7275,3637,10912,2.775796890258789,0.01240604816450741
3642,7285,3642,10927,2.7789628505706787,0.01293415142606591
3648,7297,3648,10945,2.782700777053833,0.013572363030220913
3654,7309,3654,10963,2.787834882736206,0.014214601608841804
3659,7319,3659,10978,2.7912588119506836,0.014752214536201791
3665,7331,3665,10996,2.7962608337402344,0.015399456877617013
3671,7343,3671,11014,2.800881862640381,0.016048143282546334
3676,7353,3676,11029,2.805027723312378,0.016589173371244215
3682,7365,3682,11047,2.8086798191070557,0.01723819687776995
3688,7377,3688,11065,2.813509941101074,0.01788617168233486
3693,7387,3693,11080,2.817206859588623,0.018424737513555556
3699,7399,3699,11098,2.821347713470459,0.01906860173039604
3705,7411,3705,11116,2.825002908706665,0.01970906431381536
3710,7421,3710,11131,2.828089714050293,0.020239610553289822
3716,7433,3716,11149,2.8317530155181885,0.020871784210044098
3722,7445,3722,11167,2.8358919620513916,0.021498346674434288
3727,7455,3727,11182,2.8391387462615967,0.022015653585981454
3733,7467,3733,11200,2.8438258171081543,0.02262998764592794
3739,7479,3739,11218,2.848256826400757,0.023236614730990368
3744,7489,3744,11233,2.851942777633667,0.023735731846727504
3750,7501,3750,11251,2.8563358783721924,0.02432637308845642
3756,7513,3756,11269,2.860527753829956,0.024907302589554092
3761,7523,3761,11284,2.863489866256714,0.025383497709299263
3767,7535,3767,11302,2.8667778968811035,0.0259448557134192
3773,7547,3773,11320,2.8703670501708984,0.02649460326335884
3778,7557,3778,11335,2.8733277320861816,0.02694339754179964
3784,7569,3784,11353,2.8767240047454834,0.02747022271057631
3790,7581,3790,11371,2.8801119327545166,0.02798369334095696
3795,7591,3795,11386,2.8829777240753174,0.028400973144698582
3801,7603,3801,11404,2.887425661087036,0.028888503444363778
3807,7615,3807,11422,2.891528844833374,0.02936113989687783
3812,7625,3812,11437,2.894526958465576,0.0297432725053568
3818,7637,3818,11455,2.8981807231903076,0.030187353096948755
3824,7649,3824,11473,2.9020938873291016,0.030615226047189026
3829,7659,3829,11488,2.906111001968384,0.03095910796514545
3835,7671,3835,11506,2.9110107421875,0.03135621452315718
3841,7683,3841,11524,2.9155118465423584,0.03173600871502913
3846,7693,3846,11539,2.9185478687286377,0.032039028445296935
3852,7705,3852,11557,2.922144651412964,0.032386197446157894
3858,7717,3858,11575,2.925794839859009,0.03271512306616842
3863,7727,3863,11590,2.928741931915283,0.032975080232859
3869,7739,3869,11608,2.9322450160980225,0.03326981286852515
3875,7751,3875,11626,2.9360337257385254,0.03354552037274061
3880,7761,3880,11641,2.9401397705078125,0.03376056969500496
3886,7773,3886,11659,2.9440059661865234,0.03400078869663048
3892,7785,3892,11677,2.9474518299102783,0.03422135596724729
3897,7795,3897,11692,2.9504168033599854,0.034390020734576865
3903,7807,3903,11710,2.9540839195251465,0.034574114044517046
3909,7819,3909,11728,2.957509756088257,0.03473811564026619
3914,7829,3914,11743,2.961482048034668,0.034859359866345585
3920,7841,3920,11761,2.966207981109619,0.03498627685144129
3926,7853,3926,11779,2.9701788425445557,0.03509288136081068
3931,7863,3931,11794,2.9732208251953125,0.03516618452363218
3937,7875,3937,11812,2.976801872253418,0.035235509915992225
3943,7887,3943,11830,2.9809489250183105,0.03528452938758164
3948,7897,3948,11845,2.9839558601379395,0.035309904862856456
3954,7909,3954,11863,2.9880318641662598,0.0353218511305613
3960,7921,3960,11881,2.992910861968994,0.03531370121152122
3965,7931,3965,11896,2.9964659214019775,0.03529164070278057
3971,7943,3971,11914,3.0000157356262207,0.03524695964847524
3977,7955,3977,11932,3.0036377906799316,0.03518255510232393
3982,7965,3982,11947,3.006647825241089,0.035113936056973216
3988,7977,3988,11965,3.010326862335205,0.03501380961961331
3994,7989,3994,11983,3.013953685760498,0.03489446600224255
3999,7999,3999,11998,3.017443895339966,0.03478048371891873
4005,8011,4005,12016,3.0219669342041016,0.03462646437606054
4011,8023,4011,12034,3.0259227752685547,0.03445386524492733
4016,8033,4016,12049,3.0290067195892334,0.03429602627159056
4022,8045,4022,12067,3.0326600074768066,0.03409005180787972
4028,8057,4028,12085,3.0363218784332275,0.03386628349073817
4033,8067,4033,12100,3.0401060581207275,0.033666444883238
4039,8079,4039,12118,3.0447397232055664,0.033410890755249056
4045,8091,4045,12136,3.048365831375122,0.03313849230437427
4050,8101,4050,12151,3.0513370037078857,0.03289889545385449
4056,8113,4056,12169,3.054921865463257,0.032596599865883036
4062,8125,4062,12187,3.0594067573547363,0.03227856620219427
4067,8135,4067,12202,3.0626020431518555,0.03200182045213751
4073,8147,4073,12220,3.0662498474121094,0.03165604137529954
4079,8159,4079,12238,3.071013927459717,0.031295756672420794
4084,8169,4084,12253,3.0747668743133545,0.030984768704229282
4090,8181,4090,12271,3.0782899856567383,0.03059908611908213
4096,8193,4096,12289,3.0819168090820312,0.030200218525806122
4101,8203,4101,12304,3.0855507850646973,0.029858104290269694
4107,8215,4107,12322,3.0898618698120117,0.02943632037113275
4113,8227,4113,12340,3.094564914703369,0.02900273451234625
4118,8237,4118,12355,3.0983498096466064,0.02863275921811237
4124,8249,4124,12373,3.1020009517669678,0.028178844359899813
4130,8261,4130,12391,3.106370687484741,0.02771456788877913
4135,8271,4135,12406,3.1095588207244873,0.02732013301988445
4141,8283,4141,12424,3.1134417057037354,0.026838225558321938
4147,8295,4147,12442,3.1175248622894287,0.02634746129524501
4152,8305,4152,12457,3.1205198764801025,0.025932120186666907
4158,8317,4158,12475,3.1242527961730957,0.025426546285416407
4164,8329,4164,12493,3.1278889179229736,0.02491368754181167
4169,8339,4169,12508,3.1310060024261475,0.02448115053971378
4175,8351,4175,12526,3.135075807571411,0.02395641718760544
4181,8363,4181,12544,3.139512777328491,0.02342602331600574
4186,8373,4186,12559,3.1427078247070312,0.022980122953640603
4192,8385,4192,12577,3.147185802459717,0.0224408591448082
4198,8397,4198,12595,3.1521248817443848,0.021897580243944503
4203,8407,4203,12610,3.1555399894714355,0.021442198675117652
4209,8419,4209,12628,3.1596360206604004,0.02089306098775978
4215,8431,4215,12646,3.1634130477905273,0.020341541073889857
4220,8441,4220,12661,3.1667206287384033,0.019880531969874937
4226,8453,4226,12679,3.1704137325286865,0.019326118930393932
4232,8465,4232,12697,3.1739587783813477,0.018770923649867655
4237,8475,4237,12712,3.176950693130493,0.01830806462885448
4243,8487,4243,12730,3.181818962097168,0.01775287628345268
4248,8497,4248,12745,3.1853268146514893,0.01729079389644994
4254,8509,4254,12763,3.1893489360809326,0.016737456575469878
4260,8521,4260,12781,3.1930649280548096,0.01618589821362093
4265,8531,4265,12796,3.196337938308716,0.01572801380848432
4271,8543,4271,12814,3.2013509273529053,0.015181112789491635
4277,8555,4277,12832,3.205812931060791,0.014637506120834587
4282,8565,4282,12847,3.2098758220672607,0.014187396623015047
4288,8577,4288,12865,3.2136118412017822,0.013651190827090431
4294,8589,4294,12883,3.2172658443450928,0.013119752114334915
4299,8599,4299,12898,3.221101760864258,0.012680892551429679
4305,8611,4305,12916,3.225944757461548,0.012159497591142099
4311,8623,4311,12934,3.230376958847046,0.0116442735649116
4316,8633,4316,12949,3.2344930171966553,0.011219976364372997
4322,8645,4322,12967,3.238710641860962,0.01071728726924448
4328,8657,4328,12985,3.2435479164123535,0.01022207823973531
4333,8667,4333,13000,3.247519016265869,0.00981543337900348
4339,8679,4339,13018,3.252466917037964,0.009335061983279047
4345,8691,4345,13036,3.2563509941101074,0.008863372671839898
4350,8701,4350,13051,3.260329008102417,0.008477218513121443
4356,8713,4356,13069,3.2653257846832275,0.008022472999414276
4362,8725,4362,13087,3.270509719848633,0.007577506752227237
4367,8735,4367,13102,3.274622917175293,0.007214434482989418
4373,8747,4373,13120,3.2789759635925293,0.006788332490827997
4379,8759,4379,13138,3.2829158306121826,0.006373008588980156
4384,8769,4384,13153,3.2868738174438477,0.006035376451109187
4390,8781,4390,13171,3.292343854904175,0.005640658098741369
4396,8793,4396,13189,3.2966928482055664,0.005257616901644724
4401,8803,4401,13204,3.3003528118133545,0.004947546575635897
4407,8815,4407,13222,3.3047149181365967,0.004586659499864254
4413,8827,4413,13240,3.308605909347534,0.004238235963725856
4418,8837,4418,13255,3.3126018047332764,0.003957582650059521
4424,8849,4424,13273,3.317612886428833,0.003632638797967047
4430,8861,4430,13291,3.3227200508117676,0.0033208143811407353
4435,8871,4435,13306,3.326955795288086,0.0030711256808899634
4441,8883,4441,13324,3.3323488235473633,0.0027838540509037557
4447,8895,4447,13342,3.3372249603271484,0.002510215134293503
4452,8905,4452,13357,3.340566635131836,0.0022927029532411325
4458,8917,4458,13375,3.3442089557647705,0.0020444257113467756
4464,8929,4464,13393,3.347660779953003,0.0018101516646993332
4469,8939,4469,13408,3.3505258560180664,0.0016256916135262145
4475,8951,4475,13426,3.354966640472412,0.001417333948893429
4481,8963,4481,13444,3.3583178520202637,0.0012232169453909592
4486,8973,4486,13459,3.3614258766174316,0.0010723707215447575
4492,8985,4492,13477,3.365504741668701,0.0009044921824852281
4498,8997,4498,13495,3.369243860244751,0.0007509703523282951
4503,9007,4503,13510,3.3722777366638184,0.0006340123932204733
4509,9019,4509,13528,3.3759360313415527,0.0005068350915280462
4515,9031,4515,13546,3.3795058727264404,0.0003940142172496053
4520,9041,4520,13561,3.3825669288635254,0.0003109434870793848
4526,9053,4526,13579,3.387018918991089,0.0002243578343268382
4532,9065,4532,13597,3.392305850982666,0.00015200788618585648
4537,9075,4537,13612,3.3956658840179443,0.00010253858306441543
4543,9087,4543,13630,3.3996009826660156,5.608597587070108e-05
4549,9099,4549,13648,3.4035398960113525,2.3619416765541246e-05
4554,9109,4554,13663,3.4072399139404297,7.1617057528783334e-06
4560,9121,4560,13681,3.411757707595825,1.2792838788300287e-08
4566,9133,4566,13699,3.4170868396759033,6.467403295573604e-06
4571,9143,4571,13714,3.4207608699798584,2.2118684228189522e-05
4577,9155,4577,13732,3.4253509044647217,5.307158517098287e-05
4583,9167,4583,13750,3.428985834121704,9.711956613500661e-05
4588,9177,4588,13765,3.431896686553955,0.00014368075733273145
4594,9189,4594,13783,3.4360718727111816,0.00021119059829288744
4600,9201,4600,13801,3.4407260417938232,0.0002911775748088985
4605,9211,4605,13816,3.4448108673095703,0.00036719115917094314
4611,9223,4611,13834,3.4488818645477295,0.00046941980087922275
4617,9235,4617,13852,3.4526238441467285,0.0005834158771449438
4622,9245,4622,13867,3.4556517601013184,0.000687207087025854
4628,9257,4628,13885,3.460399866104126,0.0008220683614581503
4634,9269,4634,13903,3.4654018878936768,0.0009679066148464699
4639,9279,4639,13918,3.4692628383636475,0.0010976092947885263
4645,9291,4645,13936,3.473435878753662,0.0012627921606735981
4651,9303,4651,13954,3.477186679840088,0.0014380836996679136
4656,9313,4656,13969,3.480353832244873,0.001591647684108466
4662,9325,4662,13987,3.484280824661255,0.0017846207373395373
4668,9337,4668,14005,3.488302707672119,0.0019867569494635973
4673,9347,4673,14020,3.4927470684051514,0.002161950225399778
4679,9359,4679,14038,3.4983737468719482,0.002379966947160028
4685,9371,4685,14056,3.503335952758789,0.002606129768992105
4690,9381,4690,14071,3.507678985595703,0.0028005520493934455
4696,9393,4696,14089,3.5126919746398926,0.003040673856730791
4702,9405,4702,14107,3.517544984817505,0.003287866212986046
4707,9415,4707,14122,3.521829843521118,0.0034989794130524388
4713,9427,4713,14140,3.5257248878479004,0.00375811712660834
4719,9439,4719,14158,3.529228687286377,0.00402320796206368
4724,9449,4724,14173,3.5321168899536133,0.004248374918461195
4730,9461,4730,14191,3.535653829574585,0.004523334854525274
4736,9473,4736,14209,3.5393826961517334,0.004803103081030713
4741,9483,4741,14224,3.542491912841797,0.005039621527203053
4747,9495,4747,14242,3.5463168621063232,0.005327142361238657
4753,9507,4753,14260,3.550618886947632,0.005618309261080867
4758,9517,4758,14275,3.5544447898864746,0.005863435673290951
4764,9529,4764,14293,3.5585858821868896,0.0061602140037848585
4770,9541,4770,14311,3.563408851623535,0.006459466595515551
4775,9551,4775,14326,3.5669188499450684,0.006710434970727874
4781,9563,4781,14344,3.5709009170532227,0.0070131481987800726
4787,9575,4787,14362,3.575065851211548,0.007317163611332944
4792,9585,4792,14377,3.5791707038879395,0.007571207561227311
4798,9597,4798,14395,3.5842769145965576,0.007876542966300804
4804,9609,4804,14413,3.588216781616211,0.008182020363506126
4809,9619,4809,14428,3.5918469429016113,0.008436401643052704
4815,9631,4815,14446,3.597054958343506,0.008741092310629028
4821,9643,4821,14464,3.6013519763946533,0.009044789741324166
4826,9653,4826,14479,3.604412794113159,0.00929682885987404
4832,9665,4832,14497,3.6080589294433594,0.009597689325460124
4838,9677,4838,14515,3.6118390560150146,0.009896457240074596
4843,9687,4843,14530,3.6149868965148926,0.010143559207904218
4849,9699,4849,14548,3.6194097995758057,0.010437513342935745
4855,9711,4855,14566,3.6237120628356934,0.010728319118129548
4860,9721,4860,14581,3.627912998199463,0.010967991520487885
4866,9733,4866,14599,3.632593870162964,0.011252091923893204
4872,9745,4872,14617,3.6371519565582275,0.01153203758883592
4877,9755,4877,14632,3.641366720199585,0.011761904840795978
4883,9767,4883,14650,3.6452159881591797,0.012033350270712617
4889,9779,4889,14668,3.6489927768707275,0.0122996912484723
4894,9789,4894,14683,3.654110908508301,0.012517511801206638
4900,9801,4900,14701,3.6587977409362793,0.012773670178489738
4906,9813,4906,14719,3.662522792816162,0.013023840999267122
4911,9823,4911,14734,3.665560722351074,0.013227530672452303
4917,9835,4917,14752,3.669839859008789,0.0134659688277452
4923,9847,4923,14770,3.6739447116851807,0.013697613884914972
4928,9857,4928,14785,3.678175926208496,0.013885271412391376
4934,9869,4934,14803,3.681964874267578,0.01410378450339067
4940,9881,4940,14821,3.686004877090454,0.014314784891553245
4945,9891,4945,14836,3.689506769180298,0.014484711479326506
4951,9903,4951,14854,3.693849802017212,0.014681342332778513
4957,9915,4957,14872,3.6984798908233643,0.014869830221073244
4962,9925,4962,14887,3.702256917953491,0.015020537687291835
4968,9937,4968,14905,3.706721782684326,0.015193582314395826
4974,9949,4974,14923,3.710463047027588,0.015357942627474586
4979,9959,4979,14938,3.7139737606048584,0.015488152734974392
4985,9971,4985,14956,3.7188286781311035,0.015636158295137648
4991,9983,4991,14974,3.723594903945923,0.01577502676821041
4996,9993,4996,14989,3.7273528575897217,0.0158836707272485
5002,10005,5002,15007,3.731639862060547,0.016005437345938844
5008,10017,5008,15025,3.7353549003601074,0.016117705795863912
5013,10027,5013,15040,3.739396810531616,0.01620393160033018
5019,10039,5019,15058,3.743673801422119,0.016298524622015975
5025,10051,5025,15076,3.7473318576812744,0.01638335639268007
5030,10061,5030,15091,3.7505197525024414,0.016446543369966093
5036,10073,5036,15109,3.7554688453674316,0.016513311614289705
5042,10085,5042,15127,3.759190082550049,0.016570159155207875
5047,10095,5047,15142,3.7622170448303223,0.016609930880349566
5053,10107,5053,15160,3.7658748626708984,0.01664851868383721
5059,10119,5059,15178,3.7697160243988037,0.01667713058850495
5064,10129,5064,15193,3.7728519439697266,0.016693356262180714
5070,10141,5070,15211,3.776319980621338,0.01670369938847216
5076,10153,5076,15229,3.779855728149414,0.01670411016198159
5081,10163,5081,15244,3.782853841781616,0.016696891864967256
5087,10175,5087,15262,3.7869210243225098,0.01667919813030494
5093,10187,5093,15280,3.7921578884124756,0.016651705800541095
5098,10197,5098,15295,3.7966208457946777,0.016621358786096607
5104,10209,5104,15313,3.802114725112915,0.01657608472339689
5110,10221,5110,15331,3.80721378326416,0.016521229450972896
5115,10231,5115,15346,3.8111648559570312,0.016468266856008995
5121,10243,5121,15364,3.8155438899993896,0.01639610331324093
5127,10255,5127,15382,3.8207647800445557,0.016314657812017686
5132,10265,5132,15397,3.8243799209594727,0.01623978636416723
5138,10277,5138,15415,3.828091859817505,0.01614165731336925
5144,10289,5144,15433,3.8332359790802,0.01603462898935959
5149,10299,5149,15448,3.8402607440948486,0.015938752296278835
5155,10311,5155,15466,3.845564842224121,0.015815819105114315
5161,10323,5161,15484,3.851515769958496,0.015684452957543726
5166,10333,5166,15499,3.8555798530578613,0.015568671602068207
5172,10345,5172,15517,3.859318733215332,0.015422329025227555
5178,10357,5178,15535,3.863086700439453,0.01526809803613105
5183,10367,5183,15550,3.866826057434082,0.015133696782527295
5189,10379,5189,15568,3.8721227645874023,0.01496555173730485
5194,10389,5194,15583,3.876710891723633,0.014819862368312897
5200,10401,5200,15601,3.882380723953247,0.014638550861718613
5206,10413,5206,15619,3.8882148265838623,0.014450387070155557
5211,10423,5211,15634,3.8937389850616455,0.014288522437368556
5217,10435,5217,15652,3.8986849784851074,0.014088422990653271
5223,10447,5223,15670,3.903984785079956,0.013882164416031628
5228,10457,5228,15685,3.9141178131103516,0.013705760561265379
5234,10469,5234,15703,3.920747756958008,0.013488873554706515
5240,10481,5240,15721,3.9265449047088623,0.013266559350881835
5245,10491,5245,15736,3.9306087493896484,0.013077344254725176
5251,10503,5251,15754,3.934400796890259,0.012845776930134889
5257,10515,5257,15772,3.939410924911499,0.012609550449724338
5262,10525,5262,15787,3.9428718090057373,0.012409337364488238
5268,10537,5268,15805,3.9474239349365234,0.012165297456590451
5274,10549,5274,15823,3.9527578353881836,0.011917400009906487
5279,10559,5279,15838,3.956540822982788,0.01170808109304744
5285,10571,5285,15856,3.960723876953125,0.011453866424858461
5291,10583,5291,15874,3.964874029159546,0.011196622688316893
5296,10593,5296,15889,3.96828293800354,0.010980153068544496
5302,10605,5302,15907,3.9731216430664062,0.010718127673726485
5308,10617,5308,15925,3.97705078125,0.010453916898654825
5313,10627,5313,15940,3.9814348220825195,0.010232287497615289
5319,10639,5319,15958,3.9870259761810303,0.009964846236130143
5325,10651,5325,15976,3.991255760192871,0.009696065270190957
5330,10661,5330,15991,3.9943089485168457,0.009471271948655158
5336,10673,5336,16009,3.9982337951660156,0.009200804825695741
5342,10685,5342,16027,4.00248384475708,0.008929835215553794
5347,10695,5347,16042,4.006337881088257,0.0087038542665141
5353,10707,5353,16060,4.010167837142944,0.008432721064764337
5359,10719,5359,16078,4.013608932495117,0.00816190824491514
5364,10729,5364,16093,4.016513824462891,0.007936682302556619
5370,10741,5370,16111,4.020924806594849,0.007667198932949759
5376,10753,5376,16129,4.025547742843628,0.007398841106464715
5381,10763,5381,16144,4.028719902038574,0.007176270887839564
5387,10775,5387,16162,4.032788991928101,0.0069106995107404146
5393,10787,5393,16180,4.037771701812744,0.006647036604022105
5398,10797,5398,16195,4.041881799697876,0.006428970039905835
5404,10809,5404,16213,4.045869827270508,0.006169503375303975
5410,10821,5410,16231,4.050508737564087,0.005912698113661463
5415,10831,5415,16246,4.054194927215576,0.005700912128645541
5421,10843,5421,16264,4.05922794342041,0.005449649025763392
5427,10855,5427,16282,4.064428806304932,0.0052017604316461075
5432,10865,5432,16297,4.067728757858276,0.004997938012706982
5438,10877,5438,16315,4.0727598667144775,0.00475685592039099
5444,10889,5444,16333,4.077784776687622,0.004519812894614006
5449,10899,5449,16348,4.082028865814209,0.0043255227143390584
5455,10911,5455,16366,4.086347818374634,0.004096455980175051
5461,10923,5461,16384,4.090022802352905,0.0038720391876267968
5466,10933,5466,16399,4.0937769412994385,0.003688723469508659
5472,10945,5472,16417,4.098735809326172,0.003473352283094755
5478,10957,5478,16435,4.10838770866394,0.003263186553908781
5483,10967,5483,16450,4.113448858261108,0.003092156895490916
5489,10979,5489,16468,4.118034839630127,0.00289200409224577
5495,10991,5495,16486,4.121826887130737,0.002697556233897558
5500,11001,5500,16501,4.124915838241577,0.002539991790854401
5506,11013,5506,16519,4.128843069076538,0.002356419821808231
5512,11025,5512,16537,4.13310170173645,0.002178993881216229
5517,11035,5517,16552,4.136580944061279,0.002035935684261858
5523,11047,5523,16570,4.141037702560425,0.0018701374527836379
5529,11059,5529,16588,4.146277904510498,0.001710863016114672
5534,11069,5534,16603,4.1504967212677,0.0015832025208055711
5540,11081,5540,16621,4.154892683029175,0.0014361861414045052
5546,11093,5546,16639,4.158456802368164,0.0012960022625065903
5551,11103,5551,16654,4.161316871643066,0.0011844680415151743
5557,11115,5557,16672,4.164738893508911,0.0010570418891120426
5563,11127,5563,16690,4.168421745300293,0.0009366842078861737
5568,11137,5568,16705,4.172483921051025,0.00084183343631139
5574,11149,5574,16723,4.176301717758179,0.0007345991617739855
5580,11161,5580,16741,4.180548906326294,0.0006345967956349341
5585,11171,5585,16756,4.184522867202759,0.0005568156583422024
5591,11183,5591,16774,4.188246726989746,0.00047017203496579896
5597,11195,5597,16792,4.191778898239136,0.0003908545322701684
5602,11205,5602,16807,4.194828748703003,0.00033036579372947017
5608,11217,5608,16825,4.198507785797119,0.0002645190594421365
5614,11229,5614,16843,4.202810764312744,0.0002060270926449448
5619,11239,5619,16858,4.2058937549591064,0.00016289851646433817
5625,11251,5625,16876,4.210831880569458,0.00011787108962835191
5631,11263,5631,16894,4.215737819671631,8.016300455437886e-05
5636,11273,5636,16909,4.219132900238037,5.4310857080963615e-05
5642,11285,5642,16927,4.222700834274292,2.9943128538434394e-05
5648,11297,5648,16945,4.22621488571167,1.2794346389455313e-05
5653,11307,5653,16960,4.229109048843384,3.981476197623124e-06
5659,11319,5659,16978,4.2325828075408936,7.15007217877428e-09


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.001032114028930664,2181.4194943796983
2002,2003,2002,4005,2.966780185699463,59.063444236102214
4004,4005,4004,8009,5.555600166320801,53.10730164883603
6006,6007,6006,12013,7.849394083023071,50.21336123158744
8008,8009,8008,16017,10.164947032928467,47.8494876308398
10010,10011,10010,20021,12.66627812385559,45.73338437039615
12012,12013,12012,24025,15.117233276367188,43.80213242083164
14014,14015,14014,28029,17.606956005096436,42.02663547953284
16016,16017,16016,32033,20.53499126434326,40.38770314813041
18018,18019,18018,36037,22.705068111419678,38.870672513610316
20020,20021,20020,40041,25.33299708366394,37.46332494316175
22022,22023,22022,44045,27.550679206848145,36.15490131437582
24024,24025,24024,48049,29.69358801841736,34.935646044907344
26026,26027,26026,52053,31.895568132400513,33.79662211954178
28028,28029,28028,56057,34.087729930877686,32.72965306120659
30030,30031,30030,60061,36.28276205062866,31.727311024429582
32032,32033,32032,64065,38.48111319541931,30.78290970167336
34034,34035,34034,68069,40.65879702568054,29.890484826944885
36036,36037,36036,72073,42.76422309875488,29.044758501028582
38038,38039,38038,76077,45.023120164871216,28.24108999942746
40040,40041,40040,80081,47.22663712501526,27.475417962206166
42042,42043,42042,84085,49.494938135147095,26.74419888149555
44044,44045,44044,88089,51.70404624938965,26.044345854958692
46046,46047,46046,92093,53.87692904472351,25.373170376284634
48048,48049,48048,96097,56.020230293273926,24.728328837686604
50050,50051,50050,100101,58.1987841129303,24.10777455747234
52052,52053,52052,104105,60.37129497528076,23.50971553548061
54054,54055,54054,108109,62.64399790763855,22.932577745933713
56056,56057,56056,112113,64.84451627731323,22.374973550532786
58058,58059,58058,116117,67.07564330101013,21.83567470537514
60060,60061,60060,120121,69.24432325363159,21.313589403281412
62062,62063,62062,124125,71.40091109275818,20.807742808159674
64064,64065,64064,128129,73.55668306350708,20.317260579029607
66066,66067,66066,132133,75.66166615486145,19.841354934348146
68068,68069,68068,136137,77.8868260383606,19.379312863610267
70070,70071,70070,140141,80.0694031715393,18.930486147815373
72072,72073,72072,144145,82.2739908695221,18.49428290057699
74074,74075,74074,148149,84.44458293914795,18.070169126264545
76076,76077,76076,152153,86.5980532169342,17.657637363636468
78078,78079,78078,156157,88.7101981639862,17.25622437570769
80080,80081,80080,160161,90.87451219558716,16.865501709786486
82082,82083,82082,164165,93.01063013076782,16.485070475632256
84084,84085,84084,168169,95.23677802085876,16.114558070234352
86086,86087,86086,172173,97.42873501777649,15.75361535636614
88088,88089,88088,176177,99.59606504440308,15.401914225278233
90090,90091,90090,180181,101.73148012161255,15.059145485233444
92092,92093,92092,184185,103.86776494979858,14.72501702701561
94094,94095,94094,188189,106.0079140663147,14.399252225397959
96096,96097,96096,192193,108.18506026268005,14.081588542074883
98098,98099,98098,196197,110.60195827484131,13.771776300995953
100100,100101,100100,200201,113.03631591796875,13.469577611585123
102102,102103,102102,204205,115.44395399093628,13.17476541907979
104104,104105,104104,208209,117.67642903327942,12.88712266440541
106106,106107,106106,212213,119.83737111091614,12.606441538636886
108108,108109,108108,216217,121.98102307319641,12.332522819321525
110110,110111,110110,220221,124.1361391544342,12.06517527780477
112112,112113,112112,224225,126.59023904800415,11.804215148270714
114114,114115,114114,228229,128.91676497459412,11.54946565053956
116116,116117,116116,232233,131.60820198059082,11.300756559786805
118118,118119,118118,236237,133.79722905158997,11.057923817308279
120120,120121,120120,240241,136.0001220703125,10.820809177260571
122122,122123,122122,244245,138.7726891040802,10.589259885006186
124124,124125,124124,248249,141.38688015937805,10.363128383281264
126126,126127,126126,252253,143.83098602294922,10.14227204291933
128128,128129,128128,256257,146.89123106002808,9.926552915296725
130130,130131,130130,260261,149.60768508911133,9.715837504048181
132132,132133,132132,264265,152.0485360622406,9.509996553932865
134134,134135,134134,268269,154.80645608901978,9.308904855007881
136136,136137,136136,272273,157.39810729026794,9.112441060522656
138138,138139,138138,276277,160.0643870830536,8.920487517157426
140140,140141,140140,280281,162.4995629787445,8.732930106419076
142142,142143,142142,284285,165.007404088974,8.54965809616749
144144,144145,144144,288289,167.21952509880066,8.37056400138431
146146,146147,146146,292293,169.60943698883057,8.195543453415553
148148,148149,148148,296297,172.25153994560242,8.024495077019651
150150,150151,150150,300301,175.16075491905212,7.857320374633105
152152,152153,152152,304305,177.3848729133606,7.693923617337191
154154,154155,154154,308309,179.61347723007202,7.534211742061757
156156,156157,156156,312313,181.94244003295898,7.378094254606026
158158,158159,158158,316317,184.35407900810242,7.225483138091022
160160,160161,160160,320321,186.59959197044373,7.076292766483675
162162,162163,162162,324325,189.09044194221497,6.930439822854623
164164,164165,164164,328329,192.03437328338623,6.78784322204433
166166,166167,166166,332333,194.2692151069641,6.648424037434552
168168,168169,168168,336337,196.50883889198303,6.512105431524105
170170,170171,170170,340341,198.75022530555725,6.378812590034045
172172,172173,172172,344345,202.32450795173645,6.248472659269169
174174,174175,174174,348349,204.89441013336182,6.121014686484273
176176,176177,176176,352353,208.41334295272827,5.996369563019698
178178,178179,178178,356357,210.52745509147644,5.874469969982442
180180,180181,180180,360361,212.75950813293457,5.755250326269106
182182,182183,182182,364365,215.12861609458923,5.638646738749344
184184,184185,184184,368369,217.24889492988586,5.524596954430876
186186,186187,186186,372373,219.44216012954712,5.413040314465661
188188,188189,188188,376377,221.654620885849,5.30391770984977
190190,190191,190190,380381,224.8390121459961,5.197171538702719
192192,192193,192192,384385,227.77209901809692,5.092745665014263
194194,194195,194194,388389,230.26854014396667,4.990585378763285
196196,196197,196196,392393,232.76904821395874,4.890637357326
198198,198199,198198,396397,235.11821699142456,4.7928496280947
200200,200201,200200,400401,237.4797420501709,4.697171532244624
202202,202203,202202,404405,239.7732961177826,4.603553689585397
204204,204205,204204,408409,242.01655101776123,4.511947964449178
206206,206207,206206,412413,244.24516201019287,4.422307432564139
208208,208209,208208,416417,246.48767518997192,4.3345863488736995
210210,210211,210210,420421,248.69043517112732,4.24874011626207
212212,212213,212212,424425,250.94519209861755,4.16472525515303
214214,214215,214214,428429,253.33358216285706,4.082499373947712
216216,216217,216216,432433,255.5663559436798,4.002021140275247
218218,218219,218218,436437,258.05944204330444,3.9232502530285274
220220,220221,220220,440441,260.4791522026062,3.846147415157816
222222,222223,222222,444445,262.77548122406006,3.7706743072042173
224224,224225,224224,448449,265.01763820648193,3.6967935615456327
226226,226227,226226,452453,267.1816201210022,3.624468737338475
228228,228229,228228,456457,269.40205001831055,3.5536642961332063
230230,230231,230230,460461,271.57134318351746,3.484345578146417
232232,232233,232232,464465,273.80611419677734,3.416478779171598
234234,234235,234234,468469,276.0877401828766,3.3500309281097316
236236,236237,236236,472473,278.25258016586304,3.284969865105836
238238,238239,238238,476477,280.52464413642883,3.221264220272815
240240,240241,240240,480481,282.8376500606537,3.158883392989651
242242,242243,242242,484485,285.02022314071655,3.0977975317556457
244244,244245,244244,488489,287.16080808639526,3.037977514591148
246246,246247,246246,492493,289.50498509407043,2.9793949299631777
248248,248249,248248,496497,291.9288709163666,2.9220220582307093
250250,250251,250250,500501,294.11228919029236,2.865831853589043
252252,252253,252252,504505,296.36933398246765,2.8107979265035965
254254,254255,254254,508509,298.60532999038696,2.7568945266195897
256256,256257,256256,512513,300.79305601119995,2.704096526134549
258258,258259,258258,516517,302.974246263504,2.6523794036222625
260260,260261,260260,520521,305.16347908973694,2.6017192282943142
262262,262263,262262,524525,307.31700921058655,2.552092644690674
264264,264265,264264,528529,309.5170922279358,2.50347685778479
266266,266267,266266,532533,313.76140117645264,2.455849618493744
268268,268269,268268,536537,317.36070919036865,2.4091892095813137
270270,270271,270270,540541,320.5915882587433,2.3634744319451784
272272,272273,272272,544545,323.517117023468,2.31868459127611
274274,274275,274274,548549,326.5876512527466,2.274799485079825
276276,276277,276276,552553,329.4556291103363,2.2317993900502415
278278,278279,278278,556557,331.85805106163025,2.1896650497884593
280280,280281,280280,560561,334.7219588756561,2.14837766285234
282282,282283,282282,564565,337.25730991363525,2.10791887113146
284284,284285,284284,568569,339.8537690639496,2.0682707485382252
286286,286287,286286,572573,342.5423891544342,2.029415790004464
288288,288289,288288,576577,344.88647508621216,1.9913369007770143
290290,290291,290290,580581,347.1361060142517,1.9540173860015102
292292,292293,292292,584585,349.54904413223267,1.9174409405923143
294294,294295,294294,588589,351.8588001728058,1.8815916393691623
296296,296297,296296,592593,354.25594902038574,1.846453927468474
298298,298299,298298,596597,356.78024196624756,1.8120126110067076
300300,300301,300300,600601,359.0993900299072,1.7782528479995108
302302,302303,302302,604605,362.50561809539795,1.7451601395231364
304304,304305,304304,608609,365.50804829597473,1.7127203211159667
306306,306307,306306,612613,368.8825442790985,1.6809195544086606
308308,308309,308308,616617,371.7179400920868,1.649744318980197
310310,310311,310310,620621,374.2357749938965,1.6191814044321973
312312,312313,312312,624625,376.7801320552826,1.589217902676296
314314,314315,314314,628629,379.1017951965332,1.5598412004251259
316316,316317,316316,632633,381.4930970668793,1.5310389718870283
318318,318319,318318,636637,383.7626540660858,1.5027991716531233
320320,320321,320320,640641,385.8909361362457,1.4751100277748037
322322,322323,322322,644645,388.1316111087799,1.4479600350260853
324324,324325,324324,648649,390.23581409454346,1.421337948342284
326326,326327,326326,652653,392.3359749317169,1.3952327764362735
328328,328329,328328,656657,394.387332201004,1.3696337755795867
330330,330331,330330,660661,396.56231927871704,1.3445304435513208
332332,332333,332332,664665,399.5133922100067,1.3199125137450665
334334,334335,334334,668669,401.75457406044006,1.295769949431019
336336,336337,336336,672673,404.1871690750122,1.2720929381697488
338338,338339,338338,676677,406.8348820209503,1.2488718863706936
340340,340341,340340,680681,409.29335927963257,1.226097413996854
342342,342343,342342,684685,411.64442706108093,1.203760349403865
344344,344345,344344,688689,413.97056698799133,1.1818517243169708
346346,346347,346346,692693,416.10920119285583,1.1603627689365794
348348,348349,348348,696697,418.27911710739136,1.1392849071742148
350350,350351,350350,700701,420.4157431125641,1.1186097520084104
352352,352353,352352,704705,422.46865725517273,1.0983291009639515
354354,354355,354354,708709,424.5550420284271,1.0784349317071928
356356,356357,356356,712713,426.6414852142334,1.0589193977549485
358358,358359,358358,716717,429.53977131843567,1.039774824293545
360360,360361,360360,720721,432.0335569381714,1.0209937041072408
362362,362363,362362,724725,434.79177713394165,1.0025686936089642
364364,364365,364364,728729,437.32297921180725,0.9844926089753017
366366,366367,366366,732733,439.71326518058777,0.966758422377552
368368,368369,368368,736737,441.91686511039734,0.9493592583115742
370370,370371,370370,740741,444.1623430252075,0.9322883900197212
372372,372373,372372,744745,446.28526520729065,0.9155392360046335
374374,374375,374374,748749,448.57410526275635,0.8991053566307983
376376,376377,376376,752753,451.5341761112213,0.8829804508133066
378378,378379,378378,756757,454.25962805747986,0.8671583527881239
380380,380381,380380,760761,456.40905117988586,0.8516330289678535
382382,382383,382382,764765,458.76431703567505,0.8363985748720779
384384,384385,384384,768769,461.1304440498352,0.8214492121387593
386386,386387,386386,772773,463.4117000102997,0.8067792856083997
388388,388389,388388,776777,465.77326226234436,0.7923832604818699
390390,390391,390390,780781,467.96668910980225,0.7782557195492927
392392,392393,392392,784785,470.1970839500427,0.7643913604886166
394394,394395,394394,788789,472.3408451080322,0.7507849932305817
396396,396397,396396,792793,474.4171509742737,0.7374315373888294
398398,398399,398398,796797,477.0116720199585,0.7243260197553809
400400,400401,400400,800801,479.5989282131195,0.711463571857621
402402,402403,402402,804805,481.9451861381531,0.698839427573148
404404,404405,404404,808809,484.015013217926,0.6864489208076066
406406,406407,406406,812813,486.096009016037,0.6742874832262942
408408,408409,408408,816817,488.66506695747375,0.6623506420430658
410410,410411,410410,820821,491.86006808280945,0.6506340178628989
412412,412413,412412,824825,494.0011692047119,0.6391333225776634
414414,414415,414414,828829,496.2203571796417,0.6278443573118011
416416,416417,416416,832833,498.839182138443,0.6167630104214368
418418,418419,418418,836837,500.94674825668335,0.6058852555371459
420420,420421,420420,840841,503.62285113334656,0.5952071496592453
422422,422423,422422,844845,506.3993110656738,0.5847248312956026
424424,424425,424424,848849,508.78658723831177,0.5744345186463988
426426,426427,426426,852853,511.61372208595276,0.5643325078312955
428428,428429,428428,856857,514.0317921638489,0.5544151711605991
430430,430431,430430,860861,516.6100301742554,0.5446789554475799
432432,432433,432432,864865,519.3004331588745,0.5351203803604676
434434,434435,434434,868869,522.1640419960022,0.5257360368148056
436436,436437,436436,872873,525.1935660839081,0.5165225854032087
438438,438439,438438,876877,527.81982421875,0.5074767548641148
440440,440441,440440,880881,530.2431533336639,0.4985953405853252
442442,442443,442442,884885,532.6692931652069,0.4898752031440381
444444,444445,444444,888889,535.0900390148163,0.4813132668813296
446446,446447,446446,892893,538.1379721164703,0.47290651850994436
448448,448449,448448,896897,540.496856212616,0.46465200575494237
450450,450451,450450,900901,542.7915141582489,0.45654683602754176
452452,452453,452452,904905,545.2565350532532,0.44858817512783844
454454,454455,454454,908909,547.6703312397003,0.44077324598094947
456456,456457,456456,912913,550.0684130191803,0.43309932739941814
458458,458459,458458,916917,552.6427421569824,0.4255637528784746
460460,460461,460460,920921,554.847540140152,0.4181639094148295
462462,462463,462462,924925,557.2431969642639,0.41089723635650444
464464,464465,464464,928929,559.6153690814972,0.40376122427846894
466466,466467,466466,932933,561.9007701873779,0.3967534138831752
468468,468469,468468,936937,564.1356780529022,0.3898713949286048
470470,470471,470470,940941,566.3571252822876,0.3831128051790529
472472,472473,472472,944945,568.5638320446014,0.37647532938092354
474474,474475,474474,948949,570.7859442234039,0.3699566982629676
476476,476477,476476,952953,573.0472812652588,0.3635546875578939
478478,478479,478478,956957,575.5159711837769,0.3572671170476269
480480,480481,480480,960961,577.9671061038971,0.3510918496294835
482482,482483,482482,964965,580.2509713172913,0.3450267904050861
484484,484485,484484,968969,583.2527549266815,0.3390698857879215
486486,486487,486486,972973,585.6153380870819,0.3332191226335226
488488,488489,488488,976977,588.2054400444031,0.3274725273877266
490490,490491,490490,980981,590.6776719093323,0.3218281652547148
492492,492493,492492,984985,593.2686469554901,0.3162841393842655
494494,494495,494494,988989,595.7541880607605,0.310838590076969
496496,496497,496496,992993,598.1670432090759,0.30548969400774695
498498,498499,498498,996997,600.2722702026367,0.3002356634659691
500501,500502,500501,1001003,602.4144051074982,0.29507219071115287
502503,502504,502503,1005007,604.568253993988,0.29000271208440154
504505,504506,504505,1009011,606.7222011089325,0.2850229413691068
506507,506508,506507,1013015,608.8292701244354,0.2801312260719442
508509,508510,508509,1017019,610.9498591423035,0.2753259457655304
510511,510512,510511,1021023,613.08837723732,0.27060551142528766
512513,512514,512513,1025027,615.2021141052246,0.26596836478120167
514515,514516,514515,1029031,617.5813410282135,0.2614129776837899
516517,516518,516517,1033035,620.1208620071411,0.2569378514847358
518519,518520,518519,1037039,622.9683611392975,0.2525415164303695
520521,520522,520521,1041043,625.6705989837646,0.24822253106935932
522523,522524,522523,1045047,628.2865490913391,0.24397948167222694
524525,524526,524525,1049051,630.8839681148529,0.23981098166598258
526527,526528,526527,1053055,633.6639602184296,0.23571567107740066
528529,528530,528529,1057059,636.2872068881989,0.23169221599289358
530531,530532,530531,1061063,638.8301079273224,0.2277393080261163
532533,532534,532533,1065067,641.1171400547028,0.22385566380046384
534535,534536,534535,1069071,643.8871450424194,0.2200400244408911
536537,536538,536537,1073075,646.5402691364288,0.2162911550769877
538539,538540,538539,1077079,649.180822134018,0.21260784435798996
540541,540542,540541,1081083,651.5867280960083,0.20898890397711511
542543,542544,542543,1085087,653.8452880382538,0.20543316820624113
544545,544546,544545,1089091,656.3239450454712,0.2019394934416141
546547,546548,546547,1093095,658.9532012939453,0.1985067577584232
548549,548550,548549,1097099,661.4691121578217,0.19513386047560743
550551,550552,550551,1101103,664.1425778865814,0.19181972172827955
552553,552554,552553,1105107,666.8064570426941,0.18856328205367845
554555,554556,554555,1109111,669.3785312175751,0.1853635019797366
556557,556558,556557,1113115,671.9685711860657,0.18221936162785823
558559,558560,558559,1117119,674.4244260787964,0.17912986032138178
560561,560562,560561,1121123,677.02783203125,0.17609401620313747
562563,562564,562563,1125127,679.674751996994,0.1731108658610765
564565,564566,564565,1129131,682.1251521110535,0.17017946396197203
566567,566568,566567,1133135,684.7328860759735,0.16729888289319206
568569,568570,568569,1137139,687.8198232650757,0.1644682124101564
570571,570572,570571,1141143,690.5205190181732,0.1616865592945942
572573,572574,572573,1145147,693.7662301063538,0.1589530470172349
574575,574576,574575,1149151,696.3028430938721,0.1562668154089124
576577,576578,576577,1153155,698.3969120979309,0.153627020337467
578579,578580,578579,1157159,701.1206951141357,0.1510328333929465
580581,580582,580581,1161163,703.1323680877686,0.14848344157883275
582583,582584,582583,1165167,705.1990909576416,0.14597804700827055
584585,584586,584585,1169171,707.2402591705322,0.14351586660961857
586587,586588,586587,1173175,709.2788002490997,0.1410961318357522
588589,588590,588589,1177179,711.4976511001587,0.13871808837905064
590591,590592,590591,1181183,713.8107891082764,0.13638099589547892
592593,592594,592593,1185187,716.1574981212616,0.13408412773117107
594595,594596,594595,1189191,718.6747169494629,0.13182677065503867
596597,596598,596597,1193195,721.1525082588196,0.1296082245995649
598599,598600,598599,1197199,723.9155530929565,0.12742780240364482
600601,600602,600601,1201203,726.1070892810822,0.12528482956338394
602603,602604,602603,1205207,728.2534899711609,0.12317864398551137
604605,604606,604605,1209211,730.4537391662598,0.12110859574852384
606607,606608,606607,1213215,732.6578271389008,0.1190740468664444
608609,608610,608609,1217219,734.8751220703125,0.11707437105951612
610611,610612,610611,1221223,737.2151391506195,0.115108953526601
612613,612614,612613,1225227,739.4285209178925,0.11317719072712862
614615,614616,614615,1229231,741.552402973175,0.11127849016156688
616617,616618,616617,1233235,743.8576619625092,0.10941227016076027
618619,618620,618619,1237239,746.3246359825134,0.10757795967845141
620621,620622,620621,1241243,748.6019721031189,0.10577499808687207
622623,622624,622623,1245247,751.0790269374847,0.10400283497756391
624625,624626,624625,1249251,753.2712881565094,0.10226092996595071
626627,626628,626627,1253255,755.4270551204681,0.10054875250079931
628629,628630,628629,1257259,757.788407087326,0.09886578167493099
630631,630632,630631,1261263,760.0445330142975,0.0972115060434362
632633,632634,632633,1265267,762.2954759597778,0.09558542344188936
634635,634636,634635,1269271,764.518590927124,0.09398704081081632
636637,636638,636637,1273275,766.7221939563751,0.09241587402289042
638639,638640,638639,1277279,768.9942591190338,0.09087144771331168
640641,640642,640641,1281283,771.2260801792145,0.08935329511405143
642643,642644,642643,1285287,773.3898251056671,0.08786095789014325
644645,644646,644645,1289291,775.5959720611572,0.08639398598188563
646647,646648,646647,1293295,777.776976108551,0.0849519374474994
648649,648650,648649,1297299,779.9323709011078,0.08353437831055999
650651,650652,650651,1301303,782.1461429595947,0.08214088240924866
652653,652654,652653,1305307,784.327455997467,0.08077103124969653
654655,654656,654655,1309311,786.6046900749207,0.07942441386273913
656657,656658,656657,1313315,788.7806122303009,0.07810062666055728
658659,658660,658659,1317319,790.9917030334473,0.07679927330048031
660661,660662,660661,1321323,793.1728811264038,0.07551996454719756
662663,662664,662663,1325327,795.3470332622528,0.07426231814110906
664665,664666,664665,1329331,797.5549912452698,0.0730259586672446
666667,666668,666667,1333335,799.7429940700531,0.07181051742782074
668669,668670,668669,1337339,801.9985952377319,0.07061563231673063
670671,670672,670671,1341343,804.3244171142578,0.06944094769573894
672673,672674,672673,1345347,806.8258621692657,0.06828611427590658
674675,674676,674675,1349351,809.315446138382,0.06715078899776472
676677,676678,676677,1353355,811.6431400775909,0.06603463491660477
678679,678680,678679,1357359,813.9129521846771,0.06493732108799577
680681,680682,680681,1361363,816.2440309524536,0.06385852245773549
682683,682684,682683,1365367,818.4847590923309,0.06279791975134685
684685,684686,684685,1369371,820.7031071186066,0.061755199368121794
686687,686688,686687,1373375,823.0979270935059,0.06073005327596093
688689,688690,688689,1377379,825.4712841510773,0.05972217890791853
690691,690692,690691,1381383,827.7605950832367,0.05873127906215814
692693,692694,692693,1385387,830.1328990459442,0.05775706180236284
694695,694696,694695,1389391,832.234708070755,0.056799240361328884
696697,696698,696697,1393395,834.3588349819183,0.05585753304501395
698699,698700,698699,1397399,836.5266120433807,0.05493166314010978
700701,700702,700701,1401403,838.6907730102539,0.05402135882229686
702703,702704,702703,1405407,840.9185132980347,0.05312635306597713
704705,704706,704705,1409411,843.2238771915436,0.05224638355684874
706707,706708,706707,1413415,845.5249762535095,0.05138119260584517
708709,708710,708709,1417419,847.5926380157471,0.05053052706375638
710711,710712,710711,1421423,849.6791019439697,0.04969413823857849
712713,712714,712713,1425427,851.8270599842072,0.048871781814114
714715,714716,714715,1429431,853.9907221794128,0.04806321777004996
716717,716718,716717,1433435,856.6775801181793,0.047268210303855085
718719,718720,718719,1437439,858.7679522037506,0.046486527753245355
720721,720722,720721,1441443,860.8425831794739,0.04571794252160544
722723,722724,722723,1445447,862.8837549686432,0.044962231003751185
724725,724726,724725,1449451,864.9471220970154,0.04421917351328375
726727,726728,726727,1453455,867.0846221446991,0.0434885542115353
728729,728730,728729,1457459,869.2284271717072,0.042770161037537946
730731,730732,730731,1461463,871.2465662956238,0.042063785640038986
732733,732734,732733,1465467,873.3330292701721,0.041369223310084635
734735,734736,734735,1469471,875.4164271354675,0.04068627291496796
736737,736738,736737,1473475,877.5082471370697,0.04001473683342738
738739,738740,738739,1477479,879.5951859951019,0.03935442089289154
740741,740742,740741,1481483,881.6303060054779,0.03870513430661049
742743,742744,742743,1485487,883.7168691158295,0.03806668961271953
744745,744746,744745,1489491,885.775876045227,0.037438902614781
746747,746748,746747,1493495,887.9950411319733,0.03682159232198501
748749,748750,748749,1497499,890.612909078598,0.036214580892647064
750751,750752,750751,1501503,893.141948223114,0.03561769357679623
752753,752754,752753,1505507,895.727203130722,0.035030758661150685
754755,754756,754755,1509511,898.098776102066,0.03445360741409331
756757,756758,756757,1513515,900.2966148853302,0.033886074032693614
758759,758760,758759,1517519,902.5962901115417,0.03332799558984334
760761,760762,760761,1521523,905.2670841217041,0.03277921198287004
762763,762764,762763,1525527,907.5089871883392,0.03223956588351484
764765,764766,764765,1529531,909.860472202301,0.03170890268734183
766767,766768,766767,1533535,912.618674993515,0.031187070465989564
768769,768770,768769,1537539,914.8732950687408,0.03067391991896784
770771,770772,770771,1541543,916.9125740528107,0.03016930432670506
772773,772774,772773,1545547,919.0380811691284,0.029673079504732414
774775,774776,774775,1549551,921.8588643074036,0.029185103758777586
776777,776778,776777,1553555,924.4153161048889,0.028705237839858455
778779,778780,778779,1557559,927.3115820884705,0.028233344901195778
780781,780782,780781,1561563,929.8621001243591,0.027769290455125883
782783,782784,782783,1565567,932.0543532371521,0.027312942332628154
784785,784786,784785,1569571,934.2613971233368,0.026864170639328222
786787,786788,786787,1573575,936.4692580699921,0.026422847718208686
788789,788790,788789,1577579,938.6023008823395,0.025988848108113416
790791,790792,790791,1581583,941.0866980552673,0.02556204850566246
792793,792794,792793,1585587,944.0780611038208,0.02514232772671221
794795,794796,794795,1589591,946.26806807518,0.024729566668838743
796797,796798,796797,1593595,948.3858041763306,0.024323648274503284
798799,798800,798799,1597599,950.5385799407959,0.023924457495695606
800801,800802,800801,1601603,952.6523950099945,0.023531881257554232
802803,802804,802803,1605607,954.7293410301208,0.023145808423805647
804805,804806,804805,1609611,956.9053182601929,0.022766129762885612
806807,806808,806807,1613615,959.1583271026611,0.022392737914174177
808809,808810,808809,1617619,961.3118810653687,0.022025527355367558
810811,810812,810811,1621623,963.4311311244965,0.021664394369167894
812813,812814,812813,1625627,965.5568602085114,0.02130923701292886
814815,814816,814815,1629631,967.7257039546967,0.020959955086823356
816817,816818,816817,1633635,969.8346750736237,0.020616450102806994
818819,818820,818819,1637639,971.9858272075653,0.020278625255627958
820821,820822,820821,1641643,974.0967121124268,0.01994638539213156
822823,822824,822823,1645647,976.1666638851166,0.019619636983406963
824825,824826,824825,1649651,978.2901451587677,0.01929828809556966
826827,826828,826827,1653655,980.3721480369568,0.018982248362362952
828829,828830,828829,1657659,982.4853398799896,0.01867142895730467
830831,830832,830831,1661663,984.5959103107452,0.018365742567084453
832833,832834,832833,1665667,986.6680619716644,0.018065103365302093
834835,834836,834835,1669671,989.3436269760132,0.017769426986092185
836837,836838,836837,1673675,991.9849779605865,0.017478630498430903
838839,838840,838839,1677679,994.5866351127625,0.017192632381920703
840841,840842,840841,1681683,997.1054179668427,0.01691135250212028
842843,842844,842843,1685687,999.6857581138611,0.016634712085192405
844845,844846,844845,1689691,1002.609503030777,0.01636263369596236
846847,846848,846847,1693695,1005.2246861457825,0.01609504121313421
848849,848850,848849,1697699,1008.1062841415405,0.015831859807803994
850851,850852,850851,1701703,1010.4697751998901,0.0155730159194718
852853,852854,852853,1705707,1012.6467342376709,0.015318437235691817
854855,854856,854855,1709711,1014.7478630542755,0.015068052669107601
856857,856858,856857,1713715,1017.048201084137,0.014821792336761064
858859,858860,858859,1717719,1019.8612680435181,0.014579587538833039
860861,860862,860861,1721723,1022.4068241119385,0.014341370739316517
862863,862864,862863,1725727,1024.963278055191,0.014107075544075087
864865,864866,864865,1729731,1027.6632270812988,0.013876636682539356
866867,866868,866867,1733735,1030.1756439208984,0.013649989987357003
868869,868870,868869,1737739,1032.759693145752,0.0134270723760892
870871,870872,870871,1741743,1035.3606631755829,0.013207821831883848
872873,872874,872873,1745747,1038.0130739212036,0.012992177385171999
874875,874876,874875,1749751,1040.3194539546967,0.012780079095932706
876877,876878,876877,1753755,1042.6850340366364,0.012571468035730504
878879,878880,878879,1757759,1044.961207151413,0.012366286269866578
880881,880882,880881,1761763,1047.1586701869965,0.01216447684078048
882883,882884,882883,1765767,1049.973295211792,0.011965983751338172
884885,884886,884885,1769771,1052.3949902057648,0.011770751948006364
886887,886888,886887,1773775,1054.671019077301,0.011578727304140557
888889,888890,888889,1777779,1057.156939983368,0.01138985660486469
890891,890892,890891,1781783,1059.5092091560364,0.01120408753126867
892893,892894,892893,1785787,1061.933737039566,0.011021368644833274
894895,894896,894895,1789791,1064.3290202617645,0.010841649371513995
896897,896898,896897,1793795,1066.5822882652283,0.0106648799891218
898899,898900,898899,1797799,1068.6624991893768,0.010491011610042733
900901,900902,900901,1801803,1071.4331421852112,0.010319996168391299
902903,902904,902903,1805807,1073.4621441364288,0.010151786406481733
904905,904906,904905,1809811,1075.6359889507294,0.00998633585936659
906907,906908,906907,1813815,1077.9658529758453,0.009823598842672254
908909,908910,908909,1817819,1080.3561401367188,0.009663530438274393
910911,910912,910911,1821823,1082.4761989116669,0.009506086481678722
912913,912914,912913,1825827,1085.3722989559174,0.009351223549288079
914915,914916,914915,1829831,1087.3967821598053,0.009198898945442124
916917,916918,916917,1833835,1089.4103980064392,0.009049070689911787
918919,918920,918919,1837839,1091.630527973175,0.008901697505962147
920921,920922,920921,1841843,1093.6706221103668,0.0087567388077332
922923,922924,922923,1845847,1095.7313861846924,0.008614154689894349
924925,924926,924925,1849851,1097.8299350738525,0.008473905914115676
926927,926928,926927,1853855,1099.9027903079987,0.008335953899404558
928929,928930,928929,1857859,1102.2150809764862,0.008200260709372742
930931,930932,930931,1861863,1104.4630799293518,0.008066789042914024
932933,932934,932933,1865867,1106.6975700855255,0.007935502221812385
934935,934936,934935,1869871,1109.0215220451355,0.00780636418130598
936937,936938,936937,1873875,1111.5220999717712,0.00767933945905952
938939,938940,938939,1877879,1113.8647191524506,0.0075543931851598245
940941,940942,940941,1881883,1116.0137732028961,0.007431491071770324
942943,942944,942943,1885887,1118.8539080619812,0.00731059940335399
944945,944946,944945,1889891,1121.2118940353394,0.007191685027692074
946947,946948,946947,1893895,1123.3735501766205,0.007074715344742799
948949,948950,948949,1897899,1126.5753030776978,0.006959658298910654
950951,950952,950951,1901903,1128.6262440681458,0.00684648236870089
952953,952954,952953,1905907,1130.6459510326385,0.006735156558647759
954955,954956,954955,1909911,1132.7285141944885,0.006625650388741633
956957,956958,956957,1913915,1134.7637960910797,0.006517933887948857
958959,958960,958959,1917919,1136.8002281188965,0.0064119775837525594
960961,960962,960961,1921923,1138.848158121109,0.006307752494763008
962963,962964,962963,1925927,1140.8907310962677,0.006205230121736349
964965,964966,964965,1929931,1143.015242099762,0.006104382439616529
966967,966968,966967,1933935,1145.1637082099915,0.00600518189014565
968969,968970,968969,1937939,1147.2032051086426,0.005907601372996396
970971,970972,970971,1941943,1149.9513700008392,0.00581161423872345
972973,972974,972973,1945947,1152.768984079361,0.0057171942808054155
974975,974976,974975,1949951,1155.0117061138153,0.005624315728368856
976977,976978,976977,1953955,1157.2159821987152,0.005532953238684968
978979,978980,978979,1957959,1159.4809970855713,0.005443081890120993
980981,980982,980981,1961963,1161.7263522148132,0.005354677174750577
982983,982984,982983,1965967,1164.0095889568329,0.005267714991873618
984985,984986,984985,1969971,1166.1841390132904,0.0051821716406266205
986987,986988,986987,1973975,1168.3558061122894,0.005098023813388863
988989,988990,988989,1977979,1170.5532901287079,0.005015248589643306
990991,990992,990991,1981983,1172.9630541801453,0.004933823428473261
992993,992994,992993,1985987,1175.1814489364624,0.004853726163332794
994995,994996,994995,1989991,1177.3744111061096,0.004774934995111835
996997,996998,996997,1993995,1179.6609971523285,0.004697428485314958
998999,999000,998999,1997999,1181.6047801971436,0.004621185551741291
1001001,1001002,1001001,2002003,1183.5157392024994,0.004546185460981178
1003003,1003004,1003003,2006007,1185.340496301651,0.0044724078228455255
1005005,1005006,1005005,2010011,1187.2339231967926,0.0043998325852498965
1007007,1007008,1007007,2014015,1189.1552951335907,0.0043284400276206725
1009009,1009010,1009009,2018019,1191.2916412353516,0.004258210756574954
1011011,1011012,1011011,2022023,1193.3903329372406,0.0041891256985309155
1013013,1013014,1013013,2026027,1195.2974500656128,0.004121166096751949
1015015,1015016,1015015,2030031,1197.7315571308136,0.004054313503615958
1017017,1017018,1017017,2034035,1200.1696121692657,0.00398854977731844
1019019,1019020,1019019,2038039,1202.6566331386566,0.003923857075960768
1021021,1021022,1021021,2042043,1205.022227048874,0.0038602178519795416
1023023,1023024,1023023,2046047,1207.3571710586548,0.003797614848849662
1025025,1025026,1025025,2050051,1209.8896052837372,0.003736031094035752
1027027,1027028,1027027,2054055,1212.6847710609436,0.0036754498963773585
1029029,1029030,1029029,2058059,1215.0187120437622,0.0036158548399498613
1031031,1031032,1031031,2062063,1217.3819670677185,0.0035572297796306884
1033033,1033034,1033033,2066067,1219.8088471889496,0.0034995588374613362
1035035,1035036,1035035,2070071,1222.4615380764008,0.003442826396849341
1037037,1037038,1037037,2074075,1225.1922051906586,0.0033870170997261084
1039039,1039040,1039039,2078079,1227.6991019248962,0.0033321158408625706
1041041,1041042,1041041,2082083,1230.6856219768524,0.003278107764572269
1043043,1043044,1043043,2086087,1233.4131741523743,0.0032249782598228194
1045045,1045046,1045045,2090091,1235.9054369926453,0.003172712956711621
1047047,1047048,1047047,2094095,1238.5850670337677,0.003121297722259442
1049049,1049050,1049049,2098099,1241.214122056961,0.0030707186563176947
1051051,1051052,1051051,2102103,1243.3861062526703,0.003020962088271517
1053053,1053054,1053053,2106107,1245.5323462486267,0.0029720145716964907
1055055,1055056,1055055,2110111,1247.7214159965515,0.002923862883108086
1057057,1057058,1057057,2114115,1249.7591590881348,0.002876494015595199
1059059,1059060,1059059,2118119,1252.5128371715546,0.00282989517745591
1061061,1061062,1061061,2122123,1255.5332350730896,0.002784053786626828
1063063,1063064,1063063,2126127,1258.1603379249573,0.0027389574689777874
1065065,1065066,1065065,2130131,1260.5847690105438,0.002694594053309629
1067067,1067068,1067067,2134135,1263.3566489219666,0.0026509515695352093
1069069,1069070,1069069,2138139,1265.791412115097,0.0026080182436771793
1071071,1071072,1071071,2142143,1267.9555730819702,0.002565782496048996
1073073,1073074,1073073,2146147,1269.9847249984741,0.0025242329371621963
1075075,1075076,1075075,2150151,1271.866698026657,0.0024833583651115987
1077077,1077078,1077077,2154155,1273.7627351284027,0.0024431477613688912
1079079,1079080,1079079,2158159,1275.6432461738586,0.002403590289645763
1081081,1081082,1081081,2162163,1277.4503211975098,0.0023646752906643087
1083083,1083084,1083083,2166167,1279.265370130539,0.002326392281133849
1085085,1085086,1085085,2170171,1281.0787541866302,0.002288730949771889
1087087,1087088,1087087,2174175,1282.9125530719757,0.002251681154234575
1089089,1089090,1089089,2178179,1284.7311480045319,0.0022152329194113918
1091091,1091092,1091091,2182183,1286.6131739616394,0.002179376433446123
1093093,1093094,1093093,2186187,1288.4539949893951,0.002144102046372609
1095095,1095096,1095095,2190191,1290.3001770973206,0.0021094002656809607
1097097,1097098,1097097,2194195,1292.0672430992126,0.0020752617551806907
1099099,1099100,1099099,2198199,1293.8752300739288,0.002041677331817482
1101101,1101102,1101101,2202203,1295.730278968811,0.002008637963626825
1103103,1103104,1103103,2206207,1298.1344242095947,0.0019761347659823514
1105105,1105106,1105105,2210211,1300.4348340034485,0.0019441590003452802
1107107,1107108,1107107,2214215,1302.2194011211395,0.0019127020719906795
1109109,1109110,1109109,2218219,1303.9917130470276,0.0018817555265968622
1111111,1111112,1111111,2222223,1305.9912042617798,0.001851311048540083
1113113,1113114,1113113,2226227,1307.9268670082092,0.0018213604582797416
1115115,1115116,1115115,2230231,1310.1452841758728,0.001791895711221514
1117117,1117118,1117117,2234235,1313.171308040619,0.001762908893738313
1119119,1119120,1119119,2238239,1315.751795053482,0.0017343922221471075
1121121,1121122,1121121,2242243,1317.8700122833252,0.0017063380403214978
1123123,1123124,1123123,2246247,1319.918004989624,0.0016787388176453533
1125125,1125126,1125125,2250251,1321.9880390167236,0.0016515871465117016
1127127,1127128,1127127,2254255,1324.0240271091461,0.0016248757409584869
1129129,1129130,1129129,2258259,1326.0927131175995,0.0015985974345085197
1131131,1131132,1131131,2262263,1328.169809103012,0.0015727451770999323
1133133,1133134,1133133,2266267,1330.2834491729736,0.0015473120353135528
1135135,1135136,1135135,2270271,1332.8699781894684,0.0015222911881664913
1137137,1137138,1137137,2274275,1335.5171530246735,0.0014976759268847673
1139139,1139140,1139139,2278279,1338.0107090473175,0.0014734596522885113
1141141,1141142,1141141,2282283,1340.1270589828491,0.0014496358734277237
1143143,1143144,1143143,2286287,1342.7565121650696,0.001426198204967477
1145145,1145146,1145145,2290291,1345.3038930892944,0.001403140366505795
1147147,1147148,1147147,2294295,1347.3820350170135,0.0013804561800725423
1149149,1149150,1149149,2298299,1349.4589531421661,0.0013581395691062426
1151151,1151152,1151151,2302303,1351.4581639766693,0.0013361845556119079
1153153,1153154,1153153,2306307,1353.5106310844421,0.0013145852605020991
1155155,1155156,1155155,2310311,1355.5326342582703,0.0012933358997315736
1157157,1157158,1157157,2314315,1357.540560245514,0.001272430784183598
1159159,1159160,1159159,2318319,1359.520622253418,0.0012518643175098987
1161161,1161162,1161161,2322323,1361.4573891162872,0.0012316309954485405
1163163,1163164,1163163,2326327,1363.323430299759,0.001211725402868069
1165165,1165166,1165165,2330331,1365.7264111042023,0.0011921422135401372
1167167,1167168,1167167,2334335,1368.0269210338593,0.0011728761882068284
1169169,1169170,1169169,2338339,1370.4897379875183,0.0011539221728753546
1171171,1171172,1171171,2342343,1372.653668165207,0.001135275098135935
1173173,1173174,1173173,2346347,1374.886393070221,0.0011169299771154328
1175175,1175176,1175175,2350351,1377.100203037262,0.0010988819043404874
1177177,1177178,1177177,2354355,1379.562586069107,0.0010811260543732715
1179179,1179180,1179179,2358359,1381.5869960784912,0.0010636576804472497
1181181,1181182,1181181,2362363,1383.5565462112427,0.0010464721140124311
1183183,1183184,1183183,2366367,1385.9393322467804,0.0010295647616658243
1185185,1185186,1185185,2370371,1387.9052081108093,0.0010129311053788115
1187187,1187188,1187187,2374375,1390.4403421878815,0.0009965667013602797
1189189,1189190,1189189,2378379,1392.6259450912476,0.0009804671771007634
1191191,1191192,1191191,2382383,1394.4861340522766,0.0009646282325093125
1193193,1193194,1193193,2386387,1396.5204501152039,0.0009490456371850087
1195195,1195196,1195195,2390391,1398.6646091938019,0.0009337152297348439
1197197,1197198,1197197,2394395,1400.7015731334686,0.0009186329165231655
1199199,1199200,1199199,2398399,1402.6781430244446,0.000903794670989555
1201201,1201202,1201201,2402403,1404.6853721141815,0.0008891965314887784
1203203,1203204,1203203,2406407,1407.1318790912628,0.0008748346023139675
1205205,1205206,1205205,2410411,1409.740956068039,0.0008607050494902069
1207207,1207208,1207207,2414415,1412.1557381153107,0.0008468041031619578
1209209,1209210,1209209,2418419,1414.4761452674866,0.0008331280537277053
1211211,1211212,1211211,2422423,1417.4806442260742,0.0008196732524083927
1213213,1213214,1213213,2426427,1419.9104719161987,0.0008064361101105533
1215215,1215216,1215215,2430431,1422.1335980892181,0.0007934130959483809
1217217,1217218,1217217,2434435,1424.153109073639,0.0007806007367889833
1219219,1219220,1219219,2438439,1426.132805109024,0.0007679956154333922
1221221,1221222,1221221,2442443,1428.6929259300232,0.0007555943712986846
1223223,1223224,1223223,2446447,1431.076425075531,0.000743393697916872
1225225,1225226,1225225,2450451,1433.488251209259,0.0007313903423664669
1227227,1227228,1227227,2454455,1435.740462064743,0.0007195811056135426
1229229,1229230,1229229,2458459,1437.798131942749,0.0007079628397832494
1231231,1231232,1231231,2462463,1439.955194234848,0.0006965324486145619
1233233,1233234,1233233,2466467,1442.4599533081055,0.0006852868864370976
1235235,1235236,1235235,2470471,1445.0056929588318,0.0006742231569205615
1237237,1237238,1237237,2474475,1447.1464450359344,0.0006633383122789382
1239239,1239240,1239239,2478479,1449.317491054535,0.000652629453497866
1241241,1241242,1241241,2482483,1451.6800022125244,0.0006420937273787786
1243243,1243244,1243243,2486487,1454.2637162208557,0.0006317283283578945
1245245,1245246,1245245,2490491,1457.1297662258148,0.0006215304958914203
1247247,1247248,1247247,2494495,1460.5593321323395,0.0006114975149102975
1249249,1249250,1249249,2498499,1463.4443171024323,0.0006016267138875264
1251251,1251252,1251251,2502503,1465.9618821144104,0.0005919154646107927
1253253,1253254,1253253,2506507,1468.5548601150513,0.0005823611825235275
1255255,1255256,1255255,2510511,1470.9908080101013,0.0005729613238827369
1257257,1257258,1257257,2514515,1473.650547027588,0.0005637133876916778
1259259,1259260,1259259,2518519,1476.2907168865204,0.0005546149124029398
1261261,1261262,1261261,2522523,1479.096692085266,0.0005456634769416269
1263263,1263264,1263263,2526527,1481.6561350822449,0.0005368566996821755
1265265,1265266,1265265,2530531,1484.8823070526123,0.0005281922375388604
1267267,1267268,1267267,2534535,1488.736060142517,0.000519667785852107
1269269,1269270,1269269,2538539,1492.231593132019,0.0005112810767968767
1271271,1271272,1271271,2542543,1496.312870979309,0.0005030298797237265
1273273,1273274,1273273,2546547,1499.941209077835,0.0004949120005903751
1275275,1275276,1275275,2550551,1503.53977394104,0.0004869252803700874
1277277,1277278,1277277,2554555,1507.130790233612,0.00047906759527904796
1279279,1279280,1279279,2558559,1510.557501077652,0.00047133685643530043
1281281,1281282,1281281,2562563,1512.94762301445,0.0004637310083808188
1283283,1283284,1283283,2566567,1514.7950241565704,0.0004562480293088811
1285285,1285286,1285285,2570571,1516.8727922439575,0.00044888593038194813
1287287,1287288,1287287,2574575,1519.2123410701752,0.00044164275448110857
1289289,1289290,1289289,2578579,1521.3456063270569,0.00043451657677451294
1291291,1291292,1291291,2582583,1523.487514257431,0.0004275055035805053
1293293,1293294,1293293,2586587,1526.6383502483368,0.00042060767225393647
1295295,1295296,1295295,2590591,1528.9351201057434,0.0004138212492534876
1297297,1297298,1297297,2594595,1531.3333220481873,0.00040714443252909405
1299299,1299300,1299299,2598599,1533.3683211803436,0.00040057544788396626
1301301,1301302,1301301,2602603,1535.2226121425629,0.0003941125504525189
1303303,1303304,1303303,2606607,1537.1441452503204,0.0003877540235635024
1305305,1305306,1305305,2610611,1539.1349470615387,0.0003814981783989424
1307307,1307308,1307307,2614615,1541.4024152755737,0.00037534335399413976
1309309,1309310,1309309,2618619,1543.1655659675598,0.00036928791575974174
1311311,1311312,1311311,2622623,1545.0904519557953,0.0003633302554817419
1313313,1313314,1313313,2626627,1547.074443101883,0.00035746879200360127
1315315,1315316,1315315,2630631,1549.0447742938995,0.0003517019687251377
1317317,1317318,1317317,2634635,1550.9635801315308,0.00034602825473939447
1319319,1319320,1319319,2638639,1552.968299150467,0.0003404461443778928
1321321,1321322,1321321,2642643,1554.9546301364899,0.00033495415584638977
1323323,1323324,1323323,2646647,1556.8416271209717,0.00032955083133856533
1325325,1325326,1325325,2650651,1558.7157802581787,0.00032423473680864845
1327327,1327328,1327327,2654655,1560.5555310249329,0.000319004462085104
1329329,1329330,1329329,2658659,1562.416393995285,0.00031385861893795663
1331331,1331332,1331331,2662663,1564.299203157425,0.00030879584232934576
1333333,1333334,1333333,2666667,1566.170662164688,0.00030381478848084953
1335335,1335336,1335335,2670671,1568.0013031959534,0.0002989141363514136
1337337,1337338,1337337,2674675,1569.883073091507,0.0002940925860457355
1339339,1339340,1339339,2678679,1571.8309881687164,0.00028934885858689086
1341341,1341342,1341341,2682683,1573.80921292305,0.0002846816953478992
1343343,1343344,1343343,2686687,1575.7740380764008,0.0002800898591885925
1345345,1345346,1345345,2690691,1577.6954560279846,0.0002755721319545046
1347347,1347348,1347347,2694695,1579.5538539886475,0.0002711273156137395
1349349,1349350,1349349,2698699,1581.3833620548248,0.00026675423180222424
1351351,1351352,1351351,2702703,1583.2195510864258,0.0002624517209142141
1353353,1353354,1353353,2706707,1585.134080171585,0.0002582186421022925
1355355,1355356,1355355,2710711,1587.0947360992432,0.0002540538730499975
1357357,1357358,1357357,2714715,1589.0346670150757,0.00024995631008550845
1359359,1359360,1359359,2718719,1590.9991512298584,0.0002459248668174041
1361361,1361362,1361361,2722723,1592.944435119629,0.00024195847481678356
1363363,1363364,1363363,2726727,1594.824098110199,0.00023805608259408473
1365365,1365366,1365365,2730731,1596.6850440502167,0.00023421665594014485
1367367,1367368,1367367,2734735,1598.5709431171417,0.00023043917747145315
1369369,1369370,1369369,2738739,1600.43705701828,0.00022672264640277717
1371371,1371372,1371371,2742743,1602.334319114685,0.00022306607741029438
1373373,1373374,1373373,2746747,1604.2360870838165,0.00021946850210952107
1375375,1375376,1375375,2750751,1606.2062451839447,0.00021592896700894926
1377377,1377378,1377377,2754755,1608.1424100399017,0.0002124465346469151
1379379,1379380,1379379,2758759,1610.0925822257996,0.00020902028234104364
1381381,1381382,1381381,2762763,1611.9563891887665,0.00020564930252930935
1383383,1383384,1383383,2766767,1613.869649887085,0.00020233270220160193
1385385,1385386,1385385,2770771,1615.7416172027588,0.00019906960312709998
1387387,1387388,1387387,2774775,1617.5641112327576,0.0001958591406037158
1389389,1389390,1389389,2778779,1619.4010319709778,0.00019270046504971106
1391391,1391392,1391391,2782783,1621.2066750526428,0.00018959273950258648
1393393,1393394,1393393,2786787,1623.1523940563202,0.00018653514109701064
1395395,1395396,1395395,2790791,1624.9776961803436,0.0001835268602690121
1397397,1397398,1397397,2794795,1626.7848770618439,0.0001805671005286058
1399399,1399400,1399399,2798799,1628.5825831890106,0.0001776550781187325
1401401,1401402,1401401,2802803,1630.4095571041107,0.00017479002212894557
1403403,1403404,1403403,2806807,1632.297255039215,0.00017197117426803743
1405405,1405406,1405405,2810811,1634.1866040229797,0.00016919778795454476
1407407,1407408,1407407,2814815,1636.0602900981903,0.00016646912922624324
1409409,1409410,1409409,2818819,1637.9185512065887,0.00016378447605802648
1411411,1411412,1411411,2822823,1639.8131351470947,0.00016114311756609823
1413413,1413414,1413413,2826827,1641.6922161579132,0.000158544354917467
1415415,1415416,1415415,2830831,1643.5560100078583,0.00015598750007939088
1417417,1417418,1417417,2834835,1645.3810820579529,0.00015347187650149863
1419419,1419420,1419419,2838839,1647.3131079673767,0.00015099681854735536
1421421,1421422,1421421,2842843,1649.6598629951477,0.00014856167126708897
1423423,1423424,1423423,2846847,1652.0357172489166,0.00014616579051107692
1425425,1425426,1425425,2850851,1654.6069450378418,0.00014380854190676473
1427427,1427428,1427427,2854855,1656.9496068954468,0.000141489302222908
1429429,1429430,1429429,2858859,1659.1131241321564,0.00013920745777795673
1431431,1431432,1431431,2862863,1661.1856272220612,0.0001369624048948026
1433433,1433434,1433433,2866867,1663.3521621227264,0.00013475354944603168
1435435,1435436,1435435,2870871,1665.267344236374,0.00013258030764973228
1437437,1437438,1437437,2874875,1667.2851440906525,0.00013044210402313183
1439439,1439440,1439439,2878879,1669.2208790779114,0.00012833837354264688
1441441,1441442,1441441,2882883,1671.0847821235657,0.00012626855937014625
1443443,1443444,1443443,2886887,1672.9313452243805,0.00012423211455825367
1445445,1445446,1445445,2890891,1675.135411977768,0.00012222850034504518
1447447,1447448,1447447,2894895,1677.0224840641022,0.00012025718683617015
1449449,1449450,1449449,2898899,1678.9199900627136,0.00011831765255010396
1451451,1451452,1451451,2902903,1680.8232100009918,0.00011640938498658215
1453453,1453454,1453453,2906907,1682.6538219451904,0.00011453187937604525
1455455,1455456,1455455,2910911,1684.4577751159668,0.00011268463936175976
1457457,1457458,1457457,2914915,1686.7152781486511,0.00011086717654507083
1459459,1459460,1459459,2918919,1689.408224105835,0.00010907901037171541
1461461,1461462,1461461,2922923,1691.4993040561676,0.00010731966813182225
1463463,1463464,1463463,2926927,1693.7255229949951,0.00010558868495991192
1465465,1465466,1465465,2930931,1695.792729139328,0.00010388560281171522
1467467,1467468,1467467,2934935,1697.9294950962067,0.00010220997194210213
1469469,1469470,1469469,2938939,1700.1132690906525,0.00010056134919977922
1471471,1471472,1471471,2942943,1702.2895741462708,9.893929893678433e-05
1473473,1473474,1473473,2946947,1704.5258991718292,9.734339221267874e-05
1475475,1475476,1475475,2950951,1706.5620801448822,9.577320759035501e-05
1477477,1477478,1477477,2954955,1708.3390681743622,9.42283298854818e-05
1479479,1479480,1479479,2958959,1710.267864227295,9.2708350734938e-05
1481481,1481482,1481481,2962963,1712.363652229309,9.121286882418644e-05
1483483,1483484,1483483,2966967,1714.3536930084229,8.974148852303188e-05
1485485,1485486,1485485,2970971,1716.29203414917,8.82938213635498e-05
1487487,1487488,1487487,2974975,1718.2264409065247,8.686948478953127e-05
1489489,1489490,1489489,2978979,1720.1347572803497,8.54681023838566e-05
1491491,1491492,1491491,2982983,1722.128007888794,8.408930386849534e-05
1493493,1493494,1493493,2986987,1723.9576289653778,8.27327249908194e-05
1495495,1495496,1495495,2990991,1725.8029201030731,8.139800752360316e-05
1497497,1497498,1497497,2994995,1727.6315081119537,8.00847985829023e-05
1499499,1499500,1499499,2998999,1729.4859070777893,7.879275131017494e-05
1501502,1501503,1501502,3003005,1731.3466711044312,7.75208947061401e-05
1503504,1503505,1503504,3007009,1733.230901002884,7.627016259448283e-05
1505506,1505507,1505506,3011013,1735.1465611457825,7.503958477173e-05
1507508,1507509,1507508,3015017,1737.055741071701,7.382883575246524e-05
1509510,1509511,1509510,3019021,1739.0073459148407,7.26375963040482e-05
1511512,1511513,1511512,3023025,1740.9127700328827,7.146555105919106e-05
1513514,1513515,1513514,3027029,1742.7490320205688,7.031239135812939e-05
1515516,1515517,1515516,3031033,1744.6073200702667,6.917781195170392e-05
1517518,1517519,1517518,3035037,1746.6158781051636,6.806151361615775e-05
1519520,1519521,1519520,3039041,1748.454534292221,6.696320110677334e-05
1521522,1521523,1521522,3043045,1750.2806012630463,6.588258509054867e-05
1523524,1523525,1523524,3047049,1752.0678470134735,6.481937964508688e-05
1525526,1525527,1525526,3051053,1753.8262810707092,6.377330407758564e-05
1527528,1527529,1527528,3055057,1755.6373000144958,6.274408258377662e-05
1529530,1529531,1529530,3059061,1757.4572591781616,6.173144288368348e-05
1531532,1531533,1531532,3063065,1759.2958941459656,6.073511804061127e-05
1533534,1533535,1533534,3067069,1761.0507640838623,5.9754844755843806e-05
1535536,1535537,1535536,3071073,1762.8137900829315,5.879036427813844e-05
1537538,1537539,1537538,3075077,1764.5597620010376,5.7841422062665515e-05
1539540,1539541,1539540,3079081,1766.2850601673126,5.690776765732153e-05
1541542,1541543,1541542,3083085,1767.9826109409332,5.598915402060811e-05
1543544,1543545,1543544,3087089,1769.676743030548,5.5085339567995106e-05
1545546,1545547,1545546,3091093,1771.3953459262848,5.419608487500227e-05
1547548,1547549,1547548,3095097,1773.14306807518,5.3321155860430736e-05
1549550,1549551,1549550,3099101,1774.913027048111,5.246032117156574e-05
1551552,1551553,1551552,3103105,1776.6656761169434,5.161335411685286e-05
1553554,1553555,1553554,3107109,1778.4031801223755,5.078003039216128e-05
1555556,1555557,1555556,3111113,1780.102133989334,4.996013069558103e-05
1557558,1557559,1557558,3115117,1781.7964470386505,4.9153438112625736e-05
1559560,1559561,1559560,3119121,1783.5907320976257,4.83597401625957e-05
1561562,1561563,1561562,3123125,1785.493222951889,4.757882720696216e-05
1563564,1563565,1563564,3127129,1787.4214479923248,4.681049313148833e-05
1565566,1565567,1565566,3131133,1789.334801197052,4.6054535459916224e-05
1567568,1567569,1567568,3135137,1791.1408400535583,4.531075421709829e-05
1569570,1569571,1569570,3139141,1792.793632030487,4.457895352061314e-05
1571572,1571573,1571572,3143145,1794.567548274994,4.38589399891498e-05
1573574,1573575,1573574,3147149,1796.3512959480286,4.315052399306296e-05
1575576,1575577,1575576,3151153,1798.1909050941467,4.2453518403817725e-05
1577578,1577579,1577578,3155157,1800.0123262405396,4.17677393897975e-05
1579580,1579581,1579580,3159161,1801.7844061851501,4.109300584786979e-05
1581582,1581583,1581582,3163165,1803.5241532325745,4.042913974444673e-05
1583584,1583585,1583584,3167169,1805.23423910141,3.977596611548506e-05
1585586,1585587,1585586,3171173,1806.914008140564,3.91333126117388e-05
1587588,1587589,1587588,3175177,1808.6122949123383,3.850100961244607e-05
1589590,1589591,1589590,3179181,1810.3421189785004,3.787889045270276e-05
1591592,1591593,1591592,3183185,1812.0812029838562,3.726679074134154e-05
1593594,1593595,1593594,3187189,1813.8287312984467,3.666454938411334e-05
1595596,1595597,1595596,3191193,1815.6049921512604,3.607200721944537e-05
1597598,1597599,1597598,3195197,1817.3472571372986,3.5489007927935745e-05
1599600,1599601,1599600,3199201,1819.0345001220703,3.491539791866671e-05
1601602,1601603,1601602,3203205,1820.7425711154938,3.4351025760770426e-05
1603604,1603605,1603604,3207209,1822.4176692962646,3.3795742751863145e-05
1605606,1605607,1605606,3211213,1824.1272552013397,3.3249402349611046e-05
1607608,1607609,1607608,3215217,1825.8535470962524,3.271186028541706e-05
1609610,1609611,1609610,3219221,1827.6474959850311,3.2182975019168225e-05
1611612,1611613,1611612,3223225,1829.404410123825,3.166260694342782e-05
1613614,1613615,1613614,3227229,1831.1017112731934,3.115061872449587e-05
1615616,1615617,1615616,3231233,1832.792890071869,3.0646875643469684e-05
1617618,1617619,1617618,3235237,1834.4942321777344,3.0151244686749124e-05
1619620,1619621,1619620,3239241,1836.1857540607452,2.966359500078397e-05
1621622,1621623,1621622,3243245,1837.874029159546,2.918379823313444e-05
1623624,1623625,1623624,3247249,1839.5972542762756,2.8711727736663306e-05
1625626,1625627,1625626,3251253,1841.3152530193329,2.824725879690959e-05
1627628,1627629,1627628,3255257,1843.0491580963135,2.779026942789642e-05
1629630,1629631,1629630,3259261,1844.7992839813232,2.7340638780515292e-05
1631632,1631633,1631632,3263265,1846.5282020568848,2.6898248393081303e-05
1633634,1633635,1633634,3267269,1848.2147750854492,2.6462981509212113e-05
1635636,1635637,1635636,3271273,1849.9000430107117,2.6034723646262137e-05
1637638,1637639,1637638,3275277,1851.556617975235,2.561336168582784e-05
1639640,1639641,1639640,3279281,1853.269368171692,2.5198784442181932e-05
1641642,1641643,1641642,3283285,1855.0564670562744,2.47908827759602e-05
1643644,1643645,1643644,3287289,1856.803015947342,2.4389549139414157e-05
1645646,1645647,1645646,3291293,1858.5488300323486,2.3994677690097888e-05
1647648,1647649,1647648,3295297,1860.2362110614777,2.3606164290868037e-05
1649650,1649651,1649650,3299301,1861.9211020469666,2.3223906509883818e-05
1651652,1651653,1651652,3303305,1863.6131551265717,2.284780362060701e-05
1653654,1653655,1653654,3307309,1865.326042175293,2.247775637442828e-05
1655656,1655657,1655656,3311313,1867.0220029354095,2.211366756910138e-05
1657658,1657659,1657658,3315317,1868.743940114975,2.1755440684501082e-05
1659660,1659661,1659660,3319321,1870.4870150089264,2.140298158792575e-05
1661662,1661663,1661662,3323325,1872.2034821510315,2.105619751091581e-05
1663664,1663665,1663664,3327329,1873.9001641273499,2.071499682188005e-05
1665666,1665667,1665666,3331333,1875.6092751026154,2.0379289480843e-05
1667668,1667669,1667668,3335337,1877.3090119361877,2.0048987380505423e-05
1669670,1669671,1669670,3339341,1879.0019690990448,1.9724003095689113e-05
1671672,1671673,1671672,3343345,1880.6930932998657,1.940425124757894e-05
1673674,1673675,1673674,3347349,1882.3705191612244,1.908964736685448e-05
1675676,1675677,1675676,3351353,1884.0783760547638,1.878010846212419e-05
1677678,1677679,1677678,3355357,1885.7469861507416,1.847555336098594e-05
1679680,1679681,1679680,3359361,1887.5016250610352,1.8175901118411275e-05
1681682,1681683,1681682,3363365,1889.249655008316,1.788107351785584e-05
1683684,1683685,1683684,3367369,1890.9518358707428,1.7590992456462118e-05
1685686,1685687,1685686,3371373,1892.636875152588,1.7305581422988325e-05
1687688,1687689,1687688,3375377,1894.3198790550232,1.7024765270434727e-05
1689690,1689691,1689690,3379381,1896.002748966217,1.6748470102356805e-05
1691692,1691693,1691692,3383385,1897.7161102294922,1.647662293180474e-05
1693694,1693695,1693694,3387389,1899.41011095047,1.620915213607077e-05
1695696,1695697,1695696,3391393,1901.101585149765,1.594598757037602e-05
1697698,1697699,1697698,3395397,1902.823055267334,1.5687059431002126e-05
1699700,1699701,1699700,3399401,1904.5100951194763,1.543229984690697e-05
1701702,1701703,1701702,3403405,1906.2021670341492,1.5181641515482625e-05
1703704,1703705,1703704,3407409,1907.9070799350739,1.4935018043615855e-05
1705706,1705707,1705706,3411413,1909.7510251998901,1.4692365084556513e-05
1707708,1707709,1707708,3415417,1911.7060952186584,1.4453618405241286e-05
1709710,1709711,1709710,3419421,1913.5638799667358,1.4218715023162076e-05
1711712,1711713,1711712,3423425,1915.4454991817474,1.3987593433739676e-05
1713714,1713715,1713714,3427429,1917.2445030212402,1.376019201870804e-05
1715716,1715717,1715716,3431433,1918.9384372234344,1.3536451547224715e-05
1717718,1717719,1717718,3435437,1920.6666922569275,1.3316312561073573e-05
1719720,1719721,1719720,3439441,1922.3649642467499,1.3099717307341052e-05
1721722,1721723,1721722,3443445,1923.9156880378723,1.288660894260829e-05
1723724,1723725,1723724,3447449,1925.5111560821533,1.2676930850830104e-05
1725726,1725727,1725726,3451453,1927.052983045578,1.247062823495071e-05
1727728,1727729,1727728,3455457,1928.63183426857,1.2267646525288e-05
1729730,1729731,1729730,3459461,1930.2177731990814,1.2067932175341411e-05
1731732,1731733,1731732,3463465,1931.746865272522,1.1871432434418239e-05
1733734,1733735,1733734,3467469,1933.3133072853088,1.1678096143441508e-05
1735736,1735737,1735736,3471473,1934.8658530712128,1.1487871688586893e-05
1737738,1737739,1737738,3475477,1936.4007360935211,1.130070938870631e-05
1739740,1739741,1739740,3479481,1938.0282711982727,1.1116559790025349e-05
1741742,1741743,1741742,3483485,1939.5831460952759,1.0935374234577466e-05
1743744,1743745,1743744,3487489,1941.4293291568756,1.0757105314951332e-05
1745746,1745747,1745746,3491493,1943.1087260246277,1.0581705737422453e-05
1747748,1747749,1747748,3495497,1944.7847859859467,1.0409129572508391e-05
1749750,1749751,1749750,3499501,1946.5242931842804,1.0239331345474056e-05
1751752,1751753,1751752,3503505,1948.3348460197449,1.0072265922644874e-05
1753754,1753755,1753754,3507509,1950.3266413211823,9.907889761961997e-06
1755756,1755757,1755756,3511513,1952.278911113739,9.746159435053414e-06
1757758,1757759,1757758,3515517,1953.9673871994019,9.587032423041819e-06
1759760,1759761,1759760,3519521,1955.65731716156,9.430466548110417e-06
1761762,1761763,1761762,3523525,1957.3401200771332,9.276420882997627e-06
1763764,1763765,1763764,3527529,1959.0521800518036,9.124854614128708e-06
1765766,1765767,1765766,3531533,1960.7854690551758,8.975727723736782e-06
1767768,1767769,1767768,3535537,1962.54261302948,8.829001444610185e-06
1769770,1769771,1769770,3539541,1964.368819952011,8.684636441103066e-06
1771772,1771773,1771772,3543545,1966.1872911453247,8.542595310245815e-06
1773774,1773775,1773774,3547549,1967.9393780231476,8.402840308008308e-06
1775776,1775777,1775776,3551553,1969.6801249980927,8.265334827228799e-06
1777778,1777779,1777778,3555557,1971.399343252182,8.130042488119216e-06
1779780,1779781,1779780,3559561,1973.1371490955353,7.996927479325677e-06
1781782,1781783,1781782,3563565,1975.085372209549,7.865955126362678e-06
1783784,1783785,1783784,3567569,1976.9234380722046,7.737090868431551e-06
1785786,1785787,1785786,3571573,1978.6699361801147,7.610300372107304e-06
1787788,1787789,1787788,3575577,1980.2973420619965,7.485550895580673e-06
1789790,1789791,1789790,3579581,1981.9010429382324,7.362809014921368e-06
1791792,1791793,1791792,3583585,1983.5347311496735,7.242042670441151e-06
1793794,1793795,1793794,3587589,1985.345558166504,7.123220029825461e-06
1795796,1795797,1795796,3591593,1987.0462222099304,7.006309715507086e-06
1797798,1797799,1797798,3595597,1988.9636631011963,6.89128114572668e-06
1799800,1799801,1799800,3599601,1990.9319820404053,6.778103625038057e-06
1801802,1801803,1801802,3603605,1992.834834098816,6.666747935923922e-06
1803804,1803805,1803804,3607609,1994.64133310318,6.557184406119632e-06
1805806,1805807,1805806,3611613,1996.4504640102386,6.449383931794728e-06
1807808,1807809,1807808,3615617,1998.1544930934906,6.343318659673969e-06
1809810,1809811,1809810,3619621,1999.8049499988556,6.2389603954216e-06
1811812,1811813,1811812,3623625,2001.3793451786041,6.1362816268228926e-06
1813814,1813815,1813814,3627629,2002.8955101966858,6.035255523784144e-06
1815816,1815817,1815816,3631633,2004.4107971191406,5.93585491515114e-06
1817818,1817819,1817818,3635637,2005.9221260547638,5.838054448759067e-06
1819820,1819821,1819820,3639641,2007.5356140136719,5.741827862948412e-06
1821822,1821823,1821822,3643645,2009.120796918869,5.647149805554363e-06
1823824,1823825,1823824,3647649,2010.7496840953827,5.553995606533135e-06
1825826,1825827,1825826,3651653,2012.3402812480927,5.462340482154104e-06
1827828,1827829,1827828,3655657,2013.9522140026093,5.372160330807674e-06
1829830,1829831,1829830,3659661,2015.521371126175,5.283431619318435e-06
1831832,1831833,1831832,3663665,2017.1281189918518,5.19613081451098e-06
1833834,1833835,1833834,3667669,2018.6850531101227,5.11023483795725e-06
1835836,1835837,1835836,3671673,2020.261836051941,5.025721293350216e-06
1837838,1837839,1837838,3675677,2021.8524222373962,4.942567898069683e-06
1839840,1839841,1839840,3679681,2023.44389295578,4.860752824242809e-06
1841842,1841843,1841842,3683685,2025.145387172699,4.780254357683589e-06
1843844,1843845,1843844,3687689,2026.8694820404053,4.701051238953369e-06
1845846,1845847,1845846,3691693,2028.4387941360474,4.6231227770476835e-06
1847848,1847849,1847848,3695697,2030.0026559829712,4.546448394648905e-06
1849850,1849851,1849850,3699701,2031.5526101589203,4.471008082873595e-06
1851852,1851853,1851852,3703705,2033.130112171173,4.396781605464639e-06
1853854,1853855,1853854,3707709,2034.701523065567,4.323749635659624e-06
1855856,1855857,1855856,3711713,2036.2653810977936,4.251892960382975e-06
1857858,1857859,1857858,3715717,2037.8988432884216,4.18119270761963e-06
1859860,1859861,1859860,3719721,2039.585594177246,4.111630232728203e-06
1861862,1861863,1861862,3723725,2041.223974943161,4.043187118440983e-06
1863864,1863865,1863864,3727729,2042.7847411632538,3.975845515924448e-06
1865866,1865867,1865866,3731733,2044.3540170192719,3.909587576345075e-06
1867868,1867869,1867868,3735737,2045.9130601882935,3.8443957919298555e-06
1869870,1869871,1869870,3739741,2047.4742331504822,3.780253223339969e-06
1871872,1871873,1871872,3743745,2049.041595220566,3.717142703862919e-06
1873874,1873875,1873874,3747749,2050.6147241592407,3.655047976280912e-06
1875876,1875877,1875876,3751753,2052.11971616745,3.593952328628802e-06
1877878,1877879,1877878,3755757,2053.6467850208282,3.533839844749309e-06
1879880,1879881,1879880,3759761,2055.2140889167786,3.474694835858827e-06
1881882,1881883,1881882,3763765,2056.7668731212616,3.416501272113237e-06
1883884,1883885,1883884,3767769,2058.3022091388702,3.3592443742236355e-06
1885886,1885887,1885886,3771773,2059.8407130241394,3.3029089081537677e-06
1887888,1887889,1887888,3775777,2061.3731651306152,3.247479980927892e-06
1889890,1889891,1889890,3779781,2062.848610162735,3.1929429269439424e-06
1891892,1891893,1891892,3783785,2064.322375059128,3.1392835353472037e-06
1893894,1893895,1893894,3787789,2065.8313541412354,3.0864875952829607e-06
1895896,1895897,1895896,3791793,2067.0076870918274,3.0345411232701736e-06
1897898,1897899,1897898,3795797,2068.156907081604,2.9834305905751535e-06
1899900,1899901,1899900,3799801,2069.3307390213013,2.9331425821510493e-06
1901902,1901903,1901902,3803805,2070.44411110878,2.8836637966378476e-06
1903904,1903905,1903904,3807809,2071.5464050769806,2.8349811600492103e-06
1905906,1905907,1905906,3811813,2072.6082060337067,2.787081825772475e-06
1907908,1907909,1907908,3815817,2073.6773750782013,2.73995340194233e-06
1909910,1909911,1909910,3819821,2074.726521253586,2.6935831556329504e-06
1911912,1911913,1911912,3823825,2075.783523082733,2.647959263413213e-06
1913914,1913915,1913914,3827829,2076.8744311332703,2.6030694471046445e-06
1915916,1915917,1915916,3831833,2078.1220610141754,2.558901996962959e-06
1917918,1917919,1917918,3835837,2079.645839214325,2.5154450895570335e-06
1919920,1919921,1919920,3839841,2081.208747148514,2.472687697263609e-06
1921922,1921923,1921922,3843845,2082.8361310958862,2.4306182240252383e-06
1923924,1923925,1923924,3847849,2084.442432165146,2.389225642218662e-06
1925926,1925927,1925926,3851853,2086.036999940872,2.348499037907459e-06
1927928,1927929,1927928,3855857,2087.6058270931244,2.308427838215721e-06
1929930,1929931,1929930,3859861,2089.1367700099945,2.26900147026754e-06
1931932,1931933,1931932,3863865,2090.660045146942,2.2302094748738455e-06
1933934,1933935,1933934,3867869,2092.212503194809,2.1920417339060805e-06
1935936,1935937,1935936,3871873,2093.7899510860443,2.15448801554885e-06
1937938,1937939,1937938,3875877,2095.419631242752,2.117538883794623e-06
1939940,1939941,1939940,3879881,2097.2959492206573,2.081183879454329e-06
1941942,1941943,1941942,3883885,2098.9404590129852,2.045414134954626e-06
1943944,1943945,1943944,3887889,2100.4371662139893,2.0102196458537946e-06
1945946,1945947,1945946,3891893,2101.916139125824,1.9755917719521676e-06
1947948,1947949,1947948,3895897,2103.4321250915527,1.941520849868539e-06
1949950,1949951,1949950,3899901,2104.9783141613007,1.907998353090079e-06
1951952,1951953,1951952,3903905,2106.5621631145477,1.8750149592960952e-06
1953954,1953955,1953954,3907909,2108.2790122032166,1.8425627104079467e-06
1955956,1955957,1955956,3911913,2110.070247888565,1.8106323977917782e-06
1957958,1957959,1957958,3915917,2111.641347169876,1.7792156086215982e-06
1959960,1959961,1959960,3919921,2113.223520040512,1.7483047258792794e-06
1961962,1961963,1961962,3923925,2115.1428632736206,1.7178909956783173e-06
1963964,1963965,1963964,3927929,2116.8896420001984,1.6879668010005844e-06
1965966,1965967,1965966,3931933,2118.4526829719543,1.658523842706927e-06
1967968,1967969,1967968,3935937,2119.8803782463074,1.629554958526569e-06
1969970,1969971,1969970,3939941,2121.397181034088,1.601051963007194e-06
1971972,1971973,1971972,3943945,2122.812366247177,1.573007580191188e-06
1973974,1973975,1973974,3947949,2124.5056982040405,1.5454144204340992e-06
1975976,1975977,1975976,3951953,2126.112965106964,1.518265321465151e-06
1977978,1977979,1977978,3955957,2127.463401079178,1.4915528936398914e-06
1979980,1979981,1979980,3959961,2128.877253293991,1.4652705431217328e-06
1981982,1981983,1981982,3963965,2130.407905101776,1.4394109939530608e-06
1983984,1983985,1983984,3967969,2131.7334191799164,1.41396753861045e-06
1985986,1985987,1985986,3971973,2133.2756972312927,1.388933355883637e-06
1987988,1987989,1987988,3975977,2134.526848077774,1.364301851936034e-06
1989990,1989991,1989990,3979981,2135.7392740249634,1.3400668876784039e-06
1991992,1991993,1991992,3983985,2136.889461040497,1.316221869274159e-06
1993994,1993995,1993994,3987989,2137.967408180237,1.2927604302603868e-06
1995996,1995997,1995996,3991993,2138.9909381866455,1.269676545234688e-06
1997998,1997999,1997998,3995997,2140.039754152298,1.2469638477341505e-06
2000000,2000001,2000000,4000001,2141.0965712070465,1.2246168807905633e-06


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0008759498596191406,2181.4194943796983
1,4,4,8,0.0025529861450195312,1651.0810025948942
2,6,6,12,0.004111766815185547,787.0138414872515
3,8,8,16,0.005583047866821289,443.6895532228107
4,12,12,24,0.007873058319091797,300.66016246667004
5,20,20,40,0.01164388656616211,289.49557450497423
6,24,24,48,0.01399993896484375,223.78623088754762
7,32,32,64,0.018385887145996094,220.81261182620847
8,36,36,72,0.02080988883972168,183.77908068817942
9,44,44,88,0.02485203742980957,182.1170983560105
10,50,50,100,0.027957916259765625,181.27504299099633
11,56,56,112,0.031132936477661133,170.13408406175336
12,60,60,120,0.03370094299316406,148.65325821818533
13,64,64,128,0.03749895095825195,133.7311705141201
14,70,70,140,0.042738914489746094,109.91007130056119
15,72,72,144,0.04452991485595703,82.23078898851077
16,76,76,152,0.04692888259887695,80.91936398800976
17,80,80,160,0.04934287071228027,79.04529536254631
18,88,88,176,0.05314517021179199,78.85624657588028
19,92,92,184,0.05566596984863281,75.58327398235679
20,96,96,192,0.05786395072937012,73.92414756257904
21,102,102,204,0.06100893020629883,73.46183075002295
22,106,106,212,0.06332206726074219,70.76717652738853
23,110,110,220,0.06579780578613281,69.26330237974526
24,116,116,232,0.06909489631652832,68.49817273290205
25,124,124,248,0.07320284843444824,68.44794841411067
26,128,128,256,0.07548117637634277,65.47411002685817
27,134,134,268,0.07845497131347656,65.00800772888533
28,138,138,276,0.08075594902038574,63.04930993963785
29,146,146,292,0.08486819267272949,63.01626689073737
30,150,150,300,0.0878760814666748,60.585296799987645
31,158,158,316,0.09429192543029785,60.558948448604724
32,162,162,324,0.09705090522766113,58.35275952431084
33,168,168,336,0.10044288635253906,57.9806696844048
34,172,172,344,0.10273575782775879,56.84317694752394
35,180,180,360,0.10667181015014648,56.83095757162528
36,184,184,368,0.10909700393676758,55.80233445900785
37,188,188,376,0.11155414581298828,55.26741500557728
38,196,196,392,0.11548495292663574,55.260526121163366
39,200,200,400,0.1177821159362793,54.71731502524608
40,208,208,416,0.12210202217102051,54.71238647379096
41,212,212,424,0.12491393089294434,54.182335491579806
42,220,220,440,0.12903404235839844,54.178004291141406
43,226,226,452,0.1326918601989746,53.95350490107603
44,234,234,468,0.1372988224029541,53.949722585297195
45,240,240,480,0.14156794548034668,53.58659410904352
46,248,248,496,0.14683103561401367,53.58308064107223
47,254,254,508,0.15015101432800293,53.02376492425742
48,262,262,524,0.15372896194458008,53.020486627652645
49,268,268,536,0.15672707557678223,52.363445531572324
50,276,276,552,0.16040396690368652,52.36040531387562
51,282,282,564,0.16334795951843262,51.534811430448826
52,290,290,580,0.1678609848022461,51.53184572684222
53,298,298,596,0.17274999618530273,51.52889704564018
54,306,306,612,0.17676281929016113,51.52596401722826
55,314,314,628,0.18097996711730957,51.523045408566986
56,320,320,640,0.18393397331237793,49.70963317137989
57,328,328,656,0.1880970001220703,49.70675919202199
58,336,336,672,0.19238495826721191,49.70392743917978
59,344,344,688,0.19648408889770508,49.70113320769474
60,350,350,700,0.19957399368286133,47.28948443135232
61,358,358,716,0.2033989429473877,47.28695536312193
62,366,366,732,0.20725607872009277,47.284457457507415
63,374,374,748,0.21102380752563477,47.28198773234476
64,380,380,760,0.21399974822998047,44.50139544548506
65,388,388,776,0.21788787841796875,44.49901055163082
66,396,396,792,0.22166895866394043,44.49666438437498
67,402,402,804,0.22466206550598145,41.628758446245456
68,410,410,820,0.22832894325256348,41.62652138665749
69,418,418,836,0.23200488090515137,41.62432679554627
70,426,426,852,0.23574495315551758,41.62216970167037
71,432,432,864,0.2389380931854248,38.47845638222566
72,440,440,880,0.24344491958618164,38.4764978048629
73,446,446,892,0.24777603149414062,35.605241254758994
74,454,454,908,0.251964807510376,35.603498638495694
75,460,460,920,0.2549409866333008,32.79745501433467
76,468,468,936,0.2587740421295166,32.79595320932981
77,474,474,948,0.2617659568786621,30.281377828350514
78,482,482,964,0.2657759189605713,30.280015378572898
79,488,488,976,0.2702641487121582,27.96866530868556
80,496,496,992,0.2741730213165283,27.967421028228046
81,502,502,1004,0.2773277759552002,25.31751598934352
82,510,510,1020,0.2813849449157715,25.316356268892605
83,516,516,1032,0.28475499153137207,22.79057474097681
84,524,524,1048,0.2895689010620117,22.789515262186114
85,530,530,1060,0.2928040027618408,20.195509882466013
86,538,538,1076,0.29683995246887207,20.1945174394441
87,546,546,1092,0.30082201957702637,20.193532850744305
88,552,552,1104,0.30373501777648926,18.196492665958885
89,560,560,1120,0.3074958324432373,18.19557843901748
90,568,568,1136,0.31119203567504883,18.194674315126576
91,576,576,1152,0.31499695777893066,18.19377921116984
92,582,582,1164,0.3179929256439209,15.855835403595961
93,590,590,1180,0.321727991104126,15.854996069153913
94,596,596,1192,0.3247079849243164,13.63403399250251
95,604,604,1208,0.3285040855407715,13.633220217886446
96,610,610,1220,0.3314077854156494,11.559610759062593
97,618,618,1236,0.3350369930267334,11.558905750267627
98,624,624,1248,0.3383979797363281,9.875058336087818
99,632,632,1264,0.342897891998291,9.874432987100136
100,638,638,1276,0.3462231159210205,8.450791633237714
101,646,646,1292,0.35015201568603516,8.450220112861643
102,654,654,1308,0.3537750244140625,8.449653610203882
103,660,660,1320,0.3567831516265869,7.287453598091474
104,668,668,1336,0.36051297187805176,7.2869027186224
105,676,676,1352,0.36424899101257324,7.28635734374177
106,684,684,1368,0.36819887161254883,7.285817055112943
107,692,692,1384,0.37193894386291504,7.285281478272395
108,700,700,1400,0.375715970993042,7.284750277743683
109,708,708,1416,0.37961602210998535,7.284223152710297
110,712,712,1424,0.38193583488464355,7.112176431706416
111,720,720,1440,0.3856377601623535,7.11169473953953
112,724,724,1448,0.38825082778930664,6.996298979986932
113,732,732,1464,0.3926379680633545,6.9958610614829695
114,736,736,1472,0.3952169418334961,6.895541195452211
115,744,744,1488,0.3997528553009033,6.895200796451377
116,750,750,1500,0.40306997299194336,6.8524637146970235
117,758,758,1516,0.40709710121154785,6.8521624695990795
118,764,764,1528,0.4103727340698242,6.78937145325699
119,772,772,1544,0.41417813301086426,6.78909277828086
120,778,778,1556,0.41724586486816406,6.70426366562765
121,786,786,1572,0.42114996910095215,6.704004095999835
122,792,792,1584,0.4247889518737793,6.619096416169782
123,800,800,1600,0.4285738468170166,6.618859003474313
124,806,806,1612,0.43161702156066895,6.531396723279158
125,812,812,1624,0.4346790313720703,6.444216556788206
126,820,820,1640,0.43909287452697754,6.444001119788936
127,828,828,1656,0.4441089630126953,6.443787795403637
128,834,834,1668,0.44785308837890625,6.341279464076251
129,842,842,1684,0.4521169662475586,6.341071465569371
130,848,848,1696,0.4554009437561035,6.226331071003756
131,856,856,1712,0.45934319496154785,6.226126738472544
132,862,862,1724,0.4623119831085205,6.106090354097773
133,870,870,1740,0.46617603302001953,6.105892757609013
134,878,878,1756,0.4700300693511963,6.1056966709778635
135,886,886,1772,0.4739818572998047,6.10550197386317
136,894,894,1788,0.4779369831085205,6.105308558801539
137,902,902,1804,0.48174309730529785,6.10511632970713
138,910,910,1820,0.4858839511871338,6.10492520055675
139,918,918,1836,0.4902048110961914,6.104735094229909
140,926,926,1852,0.49434399604797363,6.104545941489732
141,932,932,1864,0.4979689121246338,6.050129058606558
142,940,940,1880,0.5021259784698486,6.04994914112217
143,946,946,1892,0.5053088665008545,5.977639815893326
144,954,954,1908,0.5090360641479492,5.977468607945525
145,960,960,1920,0.5126168727874756,5.906851342289201
146,966,966,1932,0.515949010848999,5.831078057195782
147,974,974,1948,0.520359992980957,5.830926949525406
148,982,982,1964,0.5242187976837158,5.830776880698295
149,990,990,1980,0.5278909206390381,5.830627787165099
150,998,998,1996,0.5315699577331543,5.830479611450755
151,1006,1006,2012,0.5353059768676758,5.830332301483736
152,1014,1014,2028,0.5400240421295166,5.830185810001922
153,1022,1022,2044,0.5500359535217285,5.830040094029528
154,1030,1030,2060,0.553900957107544,5.829895114411897
155,1038,1038,2076,0.5576009750366211,5.829750835405321
156,1046,1046,2092,0.5613808631896973,5.829607224313804
157,1054,1054,2108,0.5651628971099854,5.829464251165518
158,1062,1062,2124,0.5689640045166016,5.829321888429149
159,1070,1070,2140,0.5725619792938232,5.829180110758784
160,1078,1078,2156,0.5763630867004395,5.829038894770406
161,1086,1086,2172,0.5802288055419922,5.828898218842028
162,1094,1094,2188,0.5839369297027588,5.828758062936913
163,1102,1102,2204,0.5878851413726807,5.828618408445095
164,1110,1110,2220,0.5925719738006592,5.828479238044679
165,1118,1118,2236,0.5988919734954834,5.828340535576444
166,1126,1126,2252,0.6035089492797852,5.828202285932889
167,1134,1134,2268,0.6076958179473877,5.828064474958978
168,1142,1142,2284,0.6130139827728271,5.827927089364721
169,1150,1150,2300,0.6172580718994141,5.827790116645815
170,1158,1158,2316,0.6215219497680664,5.827653545013277
171,1166,1166,2332,0.6263108253479004,5.827517363330458
172,1174,1174,2348,0.6328141689300537,5.827381561057109
173,1180,1180,2360,0.6361939907073975,5.795390582761115
174,1188,1188,2376,0.6406688690185547,5.795260712016898
175,1196,1196,2392,0.6489050388336182,5.795131316634638
176,1204,1204,2408,0.6528158187866211,5.795002367832012
177,1212,1212,2424,0.6566300392150879,5.794873840011064
178,1220,1220,2440,0.6614358425140381,5.794745710334382
179,1228,1228,2456,0.6665210723876953,5.794617958359254
180,1236,1236,2472,0.6708638668060303,5.794490565725255
181,1244,1244,2488,0.6756839752197266,5.794363515883219
182,1252,1252,2504,0.6794209480285645,5.79423679386332
183,1260,1260,2520,0.6830499172210693,5.7941103860741805
184,1268,1268,2536,0.6874518394470215,5.79398428013053
185,1276,1276,2552,0.6922769546508789,5.793858464704158
186,1282,1282,2564,0.6957497596740723,5.757370221176188
187,1290,1290,2580,0.6994428634643555,5.757248045425172
188,1298,1298,2596,0.703434944152832,5.757126287913479
189,1306,1306,2612,0.7072157859802246,5.757004921382418
190,1314,1314,2628,0.7111649513244629,5.756883921255167
191,1322,1322,2644,0.7148599624633789,5.756763265335621
192,1330,1330,2660,0.7186880111694336,5.756642933541798
193,1338,1338,2676,0.7227258682250977,5.7565229076702735
194,1344,1344,2688,0.7259159088134766,5.734999213158403
195,1352,1352,2704,0.7296760082244873,5.7348820557074305
196,1360,1360,2720,0.7334861755371094,5.734765199734511
197,1368,1368,2736,0.738274097442627,5.734648625522027
198,1376,1376,2752,0.743211030960083,5.7345323153745085
199,1384,1384,2768,0.7478699684143066,5.734416253374093
200,1392,1392,2784,0.7518389225006104,5.734300425164861
201,1400,1400,2800,0.7559189796447754,5.734184817765822
202,1406,1406,2812,0.7590231895446777,5.6933271837418715
203,1414,1414,2828,0.7627241611480713,5.693213156221759
204,1422,1422,2844,0.7665069103240967,5.693099426483968
205,1430,1430,2860,0.7703428268432617,5.6929859734493675
206,1438,1438,2876,0.7741508483886719,5.692872778115429
207,1446,1446,2892,0.7779510021209717,5.692759823323058
208,1454,1454,2908,0.7816798686981201,5.692647093551614
209,1462,1462,2924,0.785679817199707,5.6925345747368965
210,1470,1470,2940,0.789849042892456,5.692422254111534
211,1478,1478,2956,0.794701099395752,5.692310120064576
212,1486,1486,2972,0.7995009422302246,5.692198162014279
213,1494,1494,2988,0.8038830757141113,5.692086370299194
214,1502,1502,3004,0.8078210353851318,5.69197473608051
215,1510,1510,3020,0.8120989799499512,5.691863251253835
216,1518,1518,3036,0.8164310455322266,5.691751908374954
217,1526,1526,3052,0.8227200508117676,5.691640700589346
218,1534,1534,3068,0.8288140296936035,5.691529621573977
219,1542,1542,3084,0.832988977432251,5.691418665482729
220,1550,1550,3100,0.8387918472290039,5.691307826899106
221,1558,1558,3116,0.8446259498596191,5.691197100794739
222,1562,1562,3124,0.8473730087280273,5.641108237551293
223,1570,1570,3140,0.8512489795684814,5.6409997384630515
224,1578,1578,3156,0.8551139831542969,5.640891420515345
225,1586,1586,3172,0.858922004699707,5.640783267834308
226,1594,1594,3188,0.8628840446472168,5.640675266372114
227,1602,1602,3204,0.8668410778045654,5.640567403673117
228,1610,1610,3220,0.8706738948822021,5.640459668671383
229,1618,1618,3236,0.874413013458252,5.640352051516061
230,1626,1626,3252,0.8781261444091797,5.640244543418703
231,1632,1632,3264,0.8812868595123291,5.488862212086701
232,1640,1640,3280,0.8849730491638184,5.488756904219258
233,1648,1648,3296,0.8901598453521729,5.488651790106928
234,1654,1654,3308,0.8936169147491455,4.897993398479002
235,1662,1662,3324,0.8976671695709229,4.897891023196848
236,1670,1670,3340,0.9015250205993652,4.897789446025172
237,1678,1678,3356,0.9052858352661133,4.8976885814823845
238,1686,1686,3372,0.9090008735656738,4.897588353914671
239,1694,1694,3388,0.9126651287078857,4.89748869633172
240,1702,1702,3404,0.9163100719451904,4.897389549384002
241,1710,1710,3420,0.9201018810272217,4.897290860461453
242,1718,1718,3436,0.9240379333496094,4.897192582902903
243,1726,1726,3452,0.9277739524841309,4.897094675298149
244,1732,1732,3464,0.9306769371032715,4.800094329690182
245,1740,1740,3480,0.9345238208770752,4.799998451898318
246,1748,1748,3496,0.9385101795196533,4.799903085759183
247,1756,1756,3512,0.9421718120574951,4.799808188153747
248,1764,1764,3528,0.9459898471832275,4.799713720221575
249,1772,1772,3544,0.949836015701294,4.7996196468981225
250,1780,1780,3560,0.9537520408630371,4.7995259365037555
251,1788,1788,3576,0.9575281143188477,4.799432560379728
252,1796,1796,3592,0.9615108966827393,4.799339492568265
253,1804,1804,3608,0.9653539657592773,4.799246709526187
254,1812,1812,3624,0.969092845916748,4.799154189872411
255,1820,1820,3640,0.9730329513549805,4.799061914164781
256,1828,1828,3656,0.9767968654632568,4.7989698647005525
257,1836,1836,3672,0.9805259704589844,4.798878025339263
258,1844,1844,3688,0.9842729568481445,4.798786381344939
259,1852,1852,3704,0.988523006439209,4.798694919247623
260,1860,1860,3720,0.9925839900970459,4.798603626717181
261,1868,1868,3736,0.9966180324554443,4.79851249245246
262,1876,1876,3752,1.0002028942108154,4.798421506082491
263,1884,1884,3768,1.0039830207824707,4.798330658076679
264,1892,1892,3784,1.0077481269836426,4.798239939666814
265,1900,1900,3800,1.0115368366241455,4.798149342774536
266,1906,1906,3812,1.0146009922027588,4.711683660194353
267,1914,1914,3828,1.0183501243591309,4.711593663658618
268,1922,1922,3844,1.0221529006958008,4.711503872069102
269,1930,1930,3860,1.0261640548706055,4.7114142727996295
270,1938,1938,3876,1.0298569202423096,4.7113248541694475
271,1946,1946,3892,1.0337328910827637,4.7112356053603435
272,1954,1954,3908,1.037672996520996,4.7111465163415005
273,1962,1962,3924,1.0413718223571777,4.711057577803331
274,1970,1970,3940,1.0452289581298828,4.710968781094834
275,1978,1978,3956,1.049185037612915,4.710880118169598
276,1986,1986,3972,1.0529170036315918,4.7107915815358865
277,1994,1994,3988,1.0566110610961914,4.710703164211395
278,2002,2002,4004,1.060256004333496,4.710614859682551
279,2010,2010,4020,1.0640549659729004,4.710526661866879
280,2018,2018,4036,1.0678200721740723,4.710438565080267
281,2026,2026,4052,1.0716969966888428,4.710350564004784
282,2028,2028,4056,1.0730280876159668,4.710262653662539
283,2036,2036,4072,1.0767669677734375,4.710174829388734
284,2044,2044,4088,1.0804119110107422,4.710087086808585
285,2052,2052,4104,1.0841789245605469,4.709999421817429
286,2060,2060,4120,1.0879099369049072,4.709911830559008
287,2068,2068,4136,1.0918028354644775,4.7098243094101235
288,2076,2076,4152,1.0957129001617432,4.709736854961534
289,2084,2084,4168,1.0997178554534912,4.70964946400602
290,2092,2092,4184,1.1034679412841797,4.70956213352224
291,2100,2100,4200,1.1072289943695068,4.709474860662908
292,2108,2108,4216,1.1109728813171387,4.709387642742854
293,2116,2116,4232,1.1147761344909668,4.709300477228908
294,2124,2124,4248,1.1184790134429932,4.709213361729439
295,2132,2132,4264,1.122297763824463,4.709126293985037
296,2140,2140,4280,1.1263999938964844,4.7090392718604335
297,2146,2146,4292,1.1294457912445068,4.675862713420884
298,2154,2154,4308,1.13326096534729,4.675776550498199
299,2162,2162,4324,1.1372449398040771,4.675690435673573
300,2170,2170,4340,1.1439049243927002,4.675604366564812
301,2178,2178,4356,1.1491940021514893,4.6755183409405845
302,2186,2186,4372,1.153012990951538,4.675432356708143
303,2192,2192,4384,1.1562178134918213,4.527601693628867
304,2200,2200,4400,1.16025710105896,4.5275177741079915
305,2206,2206,4412,1.1632771492004395,3.882447474365449
306,2214,2214,4428,1.167382001876831,3.882371247395554
307,2220,2220,4440,1.1712419986724854,3.3491916022717305
308,2228,2228,4456,1.175199031829834,3.349117732645709
309,2236,2236,4472,1.17976975440979,3.3490444067174394
310,2244,2244,4488,1.183473825454712,3.3489715612086
311,2252,2252,4504,1.1878700256347656,3.348899141685365
312,2260,2260,4520,1.192141056060791,3.3488271012596442
313,2268,2268,4536,1.1963510513305664,3.3487553994849577
314,2276,2276,4552,1.200251817703247,3.3486840014147674
315,2284,2284,4568,1.204190969467163,3.348612876803145
316,2292,2292,4584,1.2079689502716064,3.3485419994226504
317,2300,2300,4600,1.211899995803833,3.3484713464831657
318,2308,2308,4616,1.2158048152923584,3.348400898138493
319,2316,2316,4632,1.219757080078125,3.3483306370646915
320,2324,2324,4648,1.2238819599151611,3.348260548100029
321,2332,2332,4664,1.2280199527740479,3.3481906179405314
322,2340,2340,4680,1.2317240238189697,3.3481208348783866
323,2346,2346,4692,1.2348270416259766,3.3055820497268087
324,2354,2354,4708,1.2393641471862793,3.3055140823302054
325,2362,2362,4724,1.2439429759979248,3.3054463679944774
326,2370,2370,4740,1.2481269836425781,3.3053788908223396
327,2378,2378,4756,1.2519888877868652,3.3053116363471418
328,2386,2386,4772,1.256108045578003,3.3052445913743895
329,2394,2394,4788,1.2600760459899902,3.3051777438450927
330,2402,2402,4804,1.2638120651245117,3.305111082712756
331,2410,2410,4820,1.267807960510254,3.305044597835945
332,2414,2414,4828,1.2702860832214355,3.232720765495287
333,2422,2422,4844,1.2741179466247559,3.2326584950266124
334,2430,2430,4860,1.278235912322998,3.2325964086380736
335,2438,2438,4876,1.282020092010498,3.2325344925438912
336,2446,2446,4892,1.2860119342803955,3.2324727344467874
337,2454,2454,4908,1.2906429767608643,3.2324111233428994
338,2462,2462,4924,1.295365810394287,3.2323496493545463
339,2470,2470,4940,1.2994911670684814,3.2322883035870973
340,2478,2478,4956,1.3035809993743896,3.23222707800403
341,2486,2486,4972,1.307508945465088,3.2321659653219967
342,2494,2494,4988,1.3116600513458252,3.2321049589190807
343,2502,2502,5004,1.3155567646026611,3.232044052754759
344,2510,2510,5020,1.3195829391479492,3.231983241302828
345,2518,2518,5036,1.3239097595214844,3.2319225194918317
346,2526,2526,5052,1.327974796295166,3.231861882655153
347,2534,2534,5068,1.3316638469696045,3.231801326484856
348,2542,2542,5084,1.3354339599609375,3.2317408469943985
349,2550,2550,5100,1.3398430347442627,3.231680440485775
350,2554,2554,5108,1.3421919345855713,3.1801732424349893
351,2562,2562,5124,1.3460590839385986,3.1801140483861445
352,2570,2570,5140,1.34993314743042,3.180054949414398
353,2578,2578,5156,1.3539340496063232,3.1799959404460196
354,2586,2586,5172,1.3578288555145264,3.1799370167918823
355,2594,2594,5188,1.3620390892028809,3.1798781741056246
356,2602,2602,5204,1.3659420013427734,3.1798194083532962
357,2610,2610,5220,1.3698759078979492,3.1797607157822085
358,2618,2618,5236,1.3737537860870361,3.1797020928950133
359,2626,2626,5252,1.3779568672180176,3.179643536427079
360,2634,2634,5268,1.3818371295928955,3.1795850433248916
361,2642,2642,5284,1.3856770992279053,3.179526610728317
362,2650,2650,5300,1.3901660442352295,3.1794682359540047
363,2658,2658,5316,1.3947398662567139,3.1794099164804948
364,2666,2666,5332,1.3991401195526123,3.179351649934688
365,2674,2674,5348,1.402918815612793,3.1792934340817283
366,2682,2682,5364,1.4067468643188477,3.1792352668118156
367,2690,2690,5380,1.4107341766357422,3.1791771461330427
368,2698,2698,5396,1.4145910739898682,3.1791190701607093
369,2706,2706,5412,1.41914701461792,3.1790610371116372
370,2714,2714,5428,1.4236679077148438,3.1790030452949622
371,2722,2722,5444,1.427968978881836,3.178945093107245
372,2730,2730,5460,1.4319407939910889,3.178887179025878
373,2738,2738,5476,1.436100959777832,3.1788293016040825
374,2746,2746,5492,1.4408760070800781,3.178771459465679
375,2754,2754,5508,1.4453179836273193,3.178713651301223
376,2762,2762,5524,1.4495389461517334,3.178655875862887
377,2770,2770,5540,1.4534988403320312,3.178598131962076
378,2778,2778,5556,1.4572811126708984,3.178540418464763
379,2786,2786,5572,1.461426019668579,3.178482734288764
380,2794,2794,5588,1.4651970863342285,3.178425078401574
381,2800,2800,5600,1.4697940349578857,3.166429272537016
382,2808,2808,5616,1.4740631580352783,3.166371896210194
383,2816,2816,5632,1.4784231185913086,3.1663145671587927
384,2824,2824,5648,1.4823291301727295,3.166257281689923
385,2832,2832,5664,1.4869718551635742,3.1662000365274707
386,2840,2840,5680,1.4912750720977783,3.1661428287588933
387,2848,2848,5696,1.4957098960876465,3.1660856557878105
388,2856,2856,5712,1.499722957611084,3.166028515292851
389,2864,2864,5728,1.5040669441223145,3.165971405194
390,2872,2872,5744,1.5077917575836182,3.1659143236209957
391,2880,2880,5760,1.5117249488830566,3.165857268888658
392,2888,2888,5776,1.515528917312622,3.16580023947256
393,2894,2894,5788,1.518707036972046,3.113935064784414
394,2902,2902,5804,1.5233888626098633,3.1138787139341275
395,2910,2910,5820,1.5298559665679932,3.1138224269103603
396,2918,2918,5836,1.5349807739257812,3.113766199331394
397,2926,2926,5852,1.5404038429260254,3.1137100272004545
398,2934,2934,5868,1.5465238094329834,3.113653906867853
399,2942,2942,5884,1.5505390167236328,3.113597834996426
400,2950,2950,5900,1.5543479919433594,3.113541808531295
401,2958,2958,5916,1.5581440925598145,3.1134858246726935
402,2966,2966,5932,1.5621769428253174,3.1134298808508447
403,2974,2974,5948,1.5661430358886719,3.113373974704473
404,2982,2982,5964,1.570105791091919,3.1133181040606814
405,2990,2990,5980,1.5739829540252686,3.1132622669179
406,2998,2998,5996,1.5779430866241455,3.113206461429172
407,3006,3006,6012,1.581852912902832,3.1131506858888542
408,3008,3008,6016,1.5832159519195557,3.113094938718632
409,3016,3016,6032,1.587697982788086,3.1130392184569473
410,3024,3024,6048,1.5918688774108887,3.1129835237477437
411,3032,3032,6064,1.5962340831756592,3.1129278533322804
412,3040,3040,6080,1.600496768951416,3.112872206039242
413,3046,3046,6092,1.6036529541015625,3.074804226109336
414,3054,3054,6108,1.607522964477539,3.0747487386947796
415,3062,3062,6124,1.6117382049560547,3.0746933529158014
416,3070,3070,6140,1.6157989501953125,3.07463805789007
417,3078,3078,6156,1.6197729110717773,3.0745828441081358
418,3086,3086,6172,1.6236400604248047,3.0745277032492595
419,3094,3094,6188,1.6277339458465576,3.074472628023045
420,3102,3102,6204,1.6317839622497559,3.074417612032903
421,3110,3110,6220,1.6359727382659912,3.074362649657246
422,3116,3116,6232,1.6393249034881592,2.978436393499919
423,3124,3124,6248,1.6439170837402344,2.9783822745130237
424,3132,3132,6264,1.6480379104614258,2.9783282441412666
425,3140,3140,6280,1.6518568992614746,2.9782742956309676
426,3148,3148,6296,1.655815839767456,2.978220422944787
427,3154,3154,6308,1.659193754196167,2.5448435682088757
428,3162,3162,6324,1.6631689071655273,2.5447940644098708
429,3168,3168,6336,1.6661708354949951,2.184483480129188
430,3176,3176,6352,1.670255184173584,2.1844399969406822
431,3184,3184,6368,1.6740880012512207,2.1843966594497033
432,3192,3192,6384,1.678375005722046,2.184353455793371
433,3200,3200,6400,1.682286024093628,2.184310375268524
434,3208,3208,6416,1.6863460540771484,2.184267408206324
435,3216,3216,6432,1.690551996231079,2.184224545861184
436,3224,3224,6448,1.694648027420044,2.1841817803152708
437,3232,3232,6464,1.6986029148101807,2.1841391043893736
438,3240,3240,6480,1.7025988101959229,2.1840965115671906
439,3248,3248,6496,1.7067310810089111,2.184053995925865
440,3256,3256,6512,1.7110750675201416,2.1840115520761856
441,3264,3264,6528,1.7149569988250732,2.1839691751067676
442,3272,3272,6544,1.7189090251922607,2.1839268605378948
443,3276,3276,6552,1.7213099002838135,2.174849106264901
444,3284,3284,6568,1.7253599166870117,2.1748071879737836
445,3292,3292,6584,1.7293498516082764,2.174765393677035
446,3300,3300,6600,1.7332520484924316,2.1747237096078607
447,3308,3308,6616,1.7373580932617188,2.1746821237686618
448,3316,3316,6632,1.7417619228363037,2.1746406256921773
449,3324,3324,6648,1.745988130569458,2.1745992062350297
450,3332,3332,6664,1.7499058246612549,2.1745578573987814
451,3340,3340,6680,1.7538628578186035,2.174516572177822
452,3348,3348,6696,1.757962942123413,2.174475344426355
453,3356,3356,6712,1.7621140480041504,2.174434168744824
454,3364,3364,6728,1.7660329341888428,2.1743930403820286
455,3372,3372,6744,1.769974946975708,2.1743519551491772
456,3380,3380,6760,1.7738280296325684,2.174310909347696
457,3388,3388,6776,1.7780940532684326,2.1742698997051093
458,3396,3396,6792,1.781933069229126,2.174228923320584
459,3398,3398,6796,1.7833280563354492,2.1112894876903283
460,3406,3406,6812,1.7876977920532227,2.1112498494900365
461,3414,3414,6828,1.7918028831481934,2.11121029632352
462,3422,3422,6844,1.7963268756866455,2.111170822235408
463,3430,3430,6860,1.8004770278930664,2.11113142188492
464,3438,3438,6876,1.8050360679626465,2.111092090473562
465,3446,3446,6892,1.8093299865722656,2.111052823681348
466,3454,3454,6908,1.8134520053863525,2.111013617612116
467,3462,3462,6924,1.817375898361206,2.1109744687446437
468,3470,3470,6940,1.821775197982788,2.1109353738899017
469,3474,3474,6948,1.824397087097168,2.0963996713381903
470,3482,3482,6964,1.828446865081787,2.096361783427824
471,3490,3490,6980,1.8324148654937744,2.0963239551522292
472,3498,3498,6996,1.8363828659057617,2.0962861824713173
473,3506,3506,7012,1.841252088546753,2.096248461727214
474,3514,3514,7028,1.8452370166778564,2.096210789603788
475,3522,3522,7044,1.8494231700897217,2.0961731630881104
476,3530,3530,7060,1.853430986404419,2.0961355794383962
477,3538,3538,7076,1.8573970794677734,2.096098036155581
478,3546,3546,7092,1.8615858554840088,2.0960605309569473
479,3552,3552,7104,1.8647239208221436,2.0899037671180167
480,3560,3560,7120,1.8691258430480957,2.0898666740324643
481,3568,3568,7136,1.8734550476074219,2.089829616348993
482,3576,3576,7152,1.8787100315093994,2.089792591733385
483,3584,3584,7168,1.8830101490020752,2.0897555980794777
484,3592,3592,7184,1.89090895652771,2.0897186334808566
485,3600,3600,7200,1.8963508605957031,2.08968169621005
486,3608,3608,7216,1.9004950523376465,2.0896447846961337
487,3614,3614,7228,1.9038798809051514,2.0703473468723814
488,3622,3622,7244,1.907667875289917,2.070310947635221
489,3630,3630,7260,1.9119648933410645,2.0702745815672188
490,3638,3638,7276,1.916287899017334,2.0702382465680103
491,3646,3646,7292,1.9210739135742188,2.0702019407178796
492,3654,3654,7308,1.9257118701934814,2.070165662259342
493,3662,3662,7324,1.9305038452148438,2.0701294095794083
494,3670,3670,7340,1.9345951080322266,2.0700931811956025
495,3676,3676,7352,1.9388439655303955,2.039311624333777
496,3684,3684,7368,1.9446449279785156,2.039275715802887
497,3690,3690,7380,1.948564052581787,1.7835434920621083
498,3698,3698,7396,1.9526710510253906,1.7835082414787848
499,3704,3704,7408,1.9561238288879395,1.5789441239281814
500,3712,3712,7424,1.9600918292999268,1.5789103737700998
501,3720,3720,7440,1.96400785446167,1.5788766799233827
502,3728,3728,7456,1.9681169986724854,1.5788430403407574
503,3736,3736,7472,1.9728519916534424,1.5788094530989838
504,3744,3744,7488,1.977543830871582,1.5787759163885084
505,3752,3752,7504,1.9816739559173584,1.5787424285040288
506,3760,3760,7520,1.9862210750579834,1.5787089878360803
507,3768,3768,7536,1.9907970428466797,1.578675592863533
508,3776,3776,7552,1.995445966720581,1.5786422421477937
509,3784,3784,7568,1.9995930194854736,1.5786089343255298
510,3792,3792,7584,2.0035579204559326,1.5785756681036673
511,3798,3798,7596,2.0067219734191895,1.571874385888691
512,3806,3806,7612,2.0104639530181885,1.571842090012069
513,3814,3814,7628,2.0142641067504883,1.5718098630030681
514,3820,3820,7640,2.0174551010131836,1.5246449807913223
515,3828,3828,7656,2.0216310024261475,1.5246138101326778
516,3834,3834,7668,2.024852991104126,1.4831982288235395
517,3842,3842,7684,2.028873920440674,1.483167675652453
518,3850,3850,7700,2.0328400135040283,1.483137284508075
519,3858,3858,7716,2.0368540287017822,1.4831070447789898
520,3866,3866,7732,2.040958881378174,1.4830769469620009
521,3874,3874,7748,2.0448389053344727,1.483046982524229
522,3882,3882,7764,2.048875093460083,1.4830171437852187
523,3890,3890,7780,2.0528159141540527,1.482987423812915
524,3898,3898,7796,2.0568881034851074,1.4829578163329415
525,3906,3906,7812,2.060642957687378,1.4829283156525435
526,3914,3914,7828,2.064656972885132,1.4828989165904432
527,3922,3922,7844,2.06850004196167,1.4828696144193145
528,3930,3930,7860,2.0723907947540283,1.4828404048134871
529,3938,3938,7876,2.0764269828796387,1.4828112838043808
530,3946,3946,7892,2.08062481880188,1.4827822477400332
531,3954,3954,7908,2.0848608016967773,1.4827532932523582
532,3962,3962,7924,2.088939905166626,1.4827244172257679
533,3970,3970,7940,2.093045949935913,1.482695616770343
534,3976,3976,7952,2.096118927001953,1.4842243044622592
535,3984,3984,7968,2.100098133087158,1.4841958248538276
536,3992,3992,7984,2.103945016860962,1.4841674357721786
537,4000,4000,8000,2.107631206512451,1.4841391320326238
538,4008,4008,8016,2.1115729808807373,1.4841109089151132
539,4016,4016,8032,2.115300178527832,1.4840827621139852
540,4024,4024,8048,2.1192891597747803,1.4840546876921508
541,4032,4032,8064,2.123185873031616,1.4840266820419856
542,4040,4040,8080,2.1270320415496826,1.4839987418505416
543,4048,4048,8096,2.1309239864349365,1.483970864068624
544,4056,4056,8112,2.1347639560699463,1.4839430458846437
545,4064,4064,8128,2.1387388706207275,1.4839152846996058
546,4072,4072,8144,2.142573118209839,1.4838875781072147
547,4080,4080,8160,2.1466000080108643,1.483859923875002
548,4088,4088,8176,2.150580883026123,1.4838323199273873
549,4096,4096,8192,2.154489755630493,1.4838047643314667
550,4104,4104,8208,2.1583759784698486,1.4837772552835986
551,4112,4112,8224,2.162341833114624,1.483749791098262
552,4120,4120,8240,2.1662089824676514,1.4837223701970288
553,4128,4128,8256,2.1700520515441895,1.4836949910999238
554,4136,4136,8272,2.173845052719116,1.4836676524167842
555,4144,4144,8288,2.1776628494262695,1.4836403528391884
556,4152,4152,8304,2.181691884994507,1.4836130911352257
557,4160,4160,8320,2.185534954071045,1.4835858661416523
558,4168,4168,8336,2.1896021366119385,1.4835586767601399
559,4174,4174,8348,2.192857027053833,1.4722450910305724
560,4182,4182,8364,2.197115898132324,1.4722184157868696
561,4190,4190,8380,2.2010769844055176,1.4721918023575427
562,4198,4198,8396,2.204986810684204,1.4721652472857159
563,4206,4206,8412,2.2088451385498047,1.4721387474219227
564,4214,4214,8428,2.2128689289093018,1.4721122998910232
565,4222,4222,8444,2.2167208194732666,1.4720859020625312
566,4230,4230,8460,2.2205958366394043,1.4720595515238983
567,4238,4238,8476,2.22448992729187,1.4720332460584586
568,4246,4246,8492,2.22837495803833,1.4720069836236007
569,4254,4254,8508,2.2321391105651855,1.4719807623343968
570,4262,4262,8524,2.2361669540405273,1.4719545804456402
571,4270,4270,8540,2.2401280403137207,1.4719284363395673
572,4278,4278,8556,2.2441327571868896,1.4719023285124422
573,4286,4286,8572,2.2481698989868164,1.4718762555630747
574,4294,4294,8588,2.2520289421081543,1.471850216183043
575,4302,4302,8604,2.255880832672119,1.4718242091490765
576,4310,4310,8620,2.2597548961639404,1.4717982333133932
577,4318,4318,8636,2.2635908126831055,1.4717722875983554
578,4326,4326,8652,2.2675881385803223,1.471746370988967
579,4334,4334,8668,2.2714791297912598,1.471720482527985
580,4342,4342,8684,2.275416135787964,1.4716946213117126
581,4348,4348,8696,2.2785470485687256,1.4602378381679273
582,4356,4356,8712,2.2822468280792236,1.4602120626759643
583,4364,4364,8728,2.2860841751098633,1.4601863507401731
584,4372,4372,8744,2.290191173553467,1.4601606976659696
585,4380,4380,8760,2.2940621376037598,1.460135099230797
586,4388,4388,8776,2.298082113265991,1.4601095516283067
587,4396,4396,8792,2.3022239208221436,1.46008405142004
588,4404,4404,8808,2.306360960006714,1.4600585954938197
589,4412,4412,8824,2.3102290630340576,1.4600331810262333
590,4420,4420,8840,2.314257860183716,1.4600078054513688
591,4428,4428,8856,2.31830096244812,1.459982466430688
592,4436,4436,8872,2.322673797607422,1.4599571618299478
593,4444,4444,8888,2.326586961746216,1.4599318896971454
594,4446,4446,8892,2.327997922897339,1.459906648241713
595,4454,4454,8908,2.331822156906128,1.459881435819625
596,4462,4462,8924,2.335783004760742,1.4598562509169142
597,4470,4470,8940,2.3402087688446045,1.459831092137506
598,4478,4478,8956,2.3439769744873047,1.4598059581906
599,4486,4486,8972,2.3480660915374756,1.4597808478816887
600,4494,4494,8988,2.352146863937378,1.4597557601015296
601,4502,4502,9004,2.3558878898620605,1.4597306938195516
602,4508,4508,9016,2.3590359687805176,1.4545977700599906
603,4516,4516,9032,2.3631279468536377,1.4545728384761105
604,4524,4524,9048,2.3670480251312256,1.4545479341312557
605,4532,4532,9064,2.3709628582000732,1.45452305513777
606,4540,4540,9080,2.3748910427093506,1.4544981997946707
607,4548,4548,9096,2.3787992000579834,1.4544733665654803
608,4554,4554,9108,2.3818750381469727,1.4364713888861615
609,4562,4562,9124,2.385650873184204,1.4364467315895126
610,4570,4570,9140,2.389538049697876,1.4364221138307585
611,4578,4578,9156,2.3945138454437256,1.4363975325039746
612,4586,4586,9172,2.398697853088379,1.4363729848014373
613,4594,4594,9188,2.402662992477417,1.4363484681808814
614,4602,4602,9204,2.4065558910369873,1.4363239803378747
615,4610,4610,9220,2.410433053970337,1.4362995191822847
616,4618,4618,9236,2.414318084716797,1.4362750828146318
617,4626,4626,9252,2.418116807937622,1.4362506695078991
618,4634,4634,9268,2.422122001647949,1.4362262776885473
619,4642,4642,9284,2.425989866256714,1.4362019059225304
620,4650,4650,9300,2.42996883392334,1.4361775528996077
621,4656,4656,9312,2.4330220222473145,1.4171495382875037
622,4664,4664,9328,2.4368820190429688,1.4171254353237828
623,4672,4672,9344,2.4409079551696777,1.4171013570972946
624,4678,4678,9356,2.4442391395568848,1.1890238143164424
625,4686,4686,9372,2.448815107345581,1.1890012344119896
626,4692,4692,9384,2.452026844024658,0.9977350904274545
627,4698,4698,9396,2.455118179321289,0.8365107641935765
628,4706,4706,9412,2.4589481353759766,0.8364922607819381
629,4710,4710,9420,2.461195945739746,0.43763535231778405
630,4718,4718,9436,2.4651551246643066,0.4376183455743785
631,4724,4724,9448,2.4681758880615234,0.3671899368976028
632,4732,4732,9464,2.471879005432129,0.36717510184746516
633,4738,4738,9476,2.4749979972839355,0.30653764755231805
634,4746,4746,9492,2.4789559841156006,0.3065240748676388
635,4752,4752,9504,2.4820311069488525,0.2562917124166688
636,4758,4758,9516,2.485083818435669,0.21365881537110454
637,4766,4766,9532,2.489886999130249,0.21364769382796567
638,4770,4770,9540,2.4931390285491943,0.11018171739283389
639,4776,4776,9552,2.4966888427734375,0.09265626177682407
640,4782,4782,9564,2.4997730255126953,0.07267670700059625
641,4788,4788,9576,2.502908945083618,0.06037062448240249
642,4794,4794,9588,2.5059797763824463,0.0508112176605664
643,4800,4800,9600,2.509174108505249,0.04311152230150128
644,4808,4808,9616,2.5131289958953857,0.043105276225105627
645,4812,4812,9624,2.515428066253662,0.023532723595849347
646,4820,4820,9640,2.5192859172821045,0.023528284134044952
647,4824,4824,9648,2.521665096282959,0.01296340566489107
648,4832,4832,9664,2.525930881500244,0.01295975675157024
649,4838,4838,9676,2.5291168689727783,0.011123589837779946
650,4844,4844,9688,2.532418966293335,0.009593391951625563
651,4852,4852,9704,2.5363829135894775,0.009590317314064123
652,4856,4856,9712,2.5386929512023926,0.005422181105359414
653,4864,4864,9728,2.542746067047119,0.005419527534286317
654,4868,4868,9736,2.5454840660095215,0.003123863559608253
655,4876,4876,9752,2.5500738620758057,0.0031217839089094923
656,4880,4880,9760,2.552438974380493,0.0018710307707578977
657,4884,4884,9768,2.5549428462982178,0.0012102509300575548
658,4892,4892,9784,2.559061050415039,0.0012091206184550174
659,4896,4896,9792,2.5614709854125977,0.0008252528043612983
660,4904,4904,9808,2.5657711029052734,0.000824426313783988
661,4908,4908,9816,2.568753957748413,0.0005876671955320489
662,4916,4916,9832,2.573817014694214,0.0005869586824474027
663,4920,4920,9840,2.576528787612915,0.00042886974608791206
664,4928,4928,9856,2.5817079544067383,0.00042832090935007727
665,4932,4932,9864,2.5846099853515625,0.0003171531765246982
666,4936,4936,9872,2.587815999984741,0.0002492295660658783
667,4944,4944,9888,2.5930328369140625,0.00024881111039576354
668,4948,4948,9896,2.5957419872283936,0.00019086109864474565
669,4954,4954,9908,2.599421977996826,0.00017982852466502663
670,4962,4962,9924,2.6035521030426025,0.00017953416954696877
671,4966,4966,9932,2.6063270568847656,0.00013753296832419437
672,4974,4974,9948,2.610403060913086,0.00013732904540120217
673,4978,4978,9956,2.6128180027008057,0.00010768005472527875
674,4986,4986,9972,2.617086887359619,0.00010753105300409516
675,4990,4990,9980,2.619792938232422,8.69035918640293e-05
676,4998,4998,9996,2.623887062072754,8.679715642756491e-05
677,5004,5004,10008,2.627142906188965,8.107928078970872e-05
678,5010,5010,10020,2.630445957183838,7.558949300801032e-05
679,5016,5016,10032,2.6337029933929443,7.079197905568435e-05
680,5024,5024,10048,2.637809991836548,7.070447566093208e-05
681,5028,5028,10056,2.640316963195801,5.304549461015995e-05
682,5036,5036,10072,2.6444480419158936,5.297910809076711e-05
683,5040,5040,10080,2.64711594581604,4.0218869798991363e-05
684,5048,5048,10096,2.6512019634246826,4.0170136799133616e-05
685,5052,5052,10104,2.6535229682922363,3.135934207421087e-05
686,5060,5060,10120,2.6575019359588623,3.1319979825639166e-05
687,5064,5064,10128,2.6598620414733887,2.4009507569644484e-05
688,5072,5072,10144,2.6638598442077637,2.3974464511411497e-05
689,5076,5076,10152,2.6662800312042236,1.752195453263994e-05
690,5084,5084,10168,2.6703829765319824,1.7497752537565248e-05
691,5088,5088,10176,2.6729750633239746,1.2511766271927627e-05
692,5096,5096,10192,2.677109956741333,1.2491399616010312e-05
693,5100,5100,10200,2.679450035095215,8.90570345291053e-06
694,5108,5108,10216,2.6839969158172607,8.890541039363598e-06
695,5112,5112,10224,2.686990976333618,6.352883815452515e-06
696,5118,5118,10236,2.6917219161987305,5.918186047892959e-06
697,5122,5122,10244,2.6949269771575928,4.37242135831184e-06
698,5130,5130,10260,2.698970079421997,4.364135179457662e-06
699,5134,5134,10268,2.70121693611145,3.1005122309579747e-06
700,5140,5140,10280,2.7042739391326904,2.8815994710384985e-06
701,5144,5144,10288,2.7065658569335938,2.145240273421223e-06
702,5152,5152,10304,2.7105488777160645,2.140489527846512e-06
703,5156,5156,10312,2.7128188610076904,1.5130729025258915e-06
704,5162,5162,10324,2.7158939838409424,1.4051680636839592e-06
705,5166,5166,10332,2.7182159423828125,1.0610763183649397e-06
706,5172,5172,10344,2.721359968185425,1.000877091428265e-06
707,5176,5176,10352,2.723615884780884,7.703553137616836e-07
708,5182,5182,10364,2.72672700881958,7.301526920855395e-07
709,5186,5186,10372,2.7291109561920166,5.743983138017938e-07
710,5194,5194,10388,2.7330498695373535,5.732119916501688e-07
711,5198,5198,10396,2.7353458404541016,4.5602348563988926e-07
712,5206,5206,10412,2.7394609451293945,4.551878873826354e-07
713,5210,5210,10420,2.7430739402770996,3.5632297112897504e-07
714,5218,5218,10436,2.7486979961395264,3.5571349599194946e-07
715,5222,5222,10444,2.7509818077087402,2.659055553522194e-07
716,5230,5230,10460,2.755126953125,2.654522859302233e-07
717,5234,5234,10468,2.7575418949127197,1.9895367131539388e-07
718,5240,5240,10480,2.761183023452759,1.8749449282040587e-07
719,5246,5246,10492,2.7645139694213867,1.7561990262038307e-07
720,5252,5252,10504,2.7677690982818604,1.6517890344402986e-07
721,5256,5256,10512,2.770352840423584,1.298193410548265e-07
722,5264,5264,10528,2.7744901180267334,1.2958355455339188e-07
723,5268,5268,10536,2.7769179344177246,9.678626611275831e-08
724,5276,5276,10552,2.780996799468994,9.662028332968475e-08
725,5280,5280,10560,2.783247947692871,7.09484311300912e-08
726,5284,5284,10568,2.785487174987793,4.861499292019289e-08
727,5292,5292,10584,2.790328025817871,4.84919837617781e-08
728,5296,5296,10592,2.792768955230713,2.924150521721458e-08
729,5302,5302,10604,2.7962570190429688,2.5634790290496312e-08
730,5308,5308,10616,2.7995588779449463,2.245201358164195e-08
731,5312,5312,10624,2.802121877670288,1.2066720955772325e-08
732,5316,5316,10632,2.8047239780426025,4.67684913019184e-09
733,5324,5324,10648,2.8091189861297607,4.629555405699648e-09
734,5328,5328,10656,2.8116071224212646,1.8530954548623413e-09


==> extragradient/plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0011909008026123047,2181.4194943796983
1,4,4,8,0.005404949188232422,1651.0810025948942
2,6,6,12,0.006912946701049805,811.3696513540854
3,8,8,16,0.008089780807495117,540.5334161789265
4,10,10,20,0.009407997131347656,340.5664798776347
5,12,12,24,0.010545015335083008,246.140754933793
6,14,14,28,0.011706829071044922,179.24733065039914
7,18,18,36,0.013952970504760742,176.1873394977806
8,22,22,44,0.016134023666381836,179.58271494054793
9,24,24,48,0.017527103424072266,132.35720100719527
10,26,26,52,0.01906895637512207,127.5058312975259
11,28,28,56,0.020360946655273438,131.4658535876756
12,32,32,64,0.022569894790649414,126.9273311629006
13,34,34,68,0.0243380069732666,106.38123453026947
14,36,36,72,0.026174068450927734,102.97302140781767
15,40,40,80,0.028110027313232422,102.56973292267685
16,44,44,88,0.030094146728515625,101.90902027413154
17,46,46,92,0.03180122375488281,97.10644598258204
18,50,50,100,0.03448200225830078,93.96666929492062
19,52,52,104,0.03574800491333008,80.51470788221422
20,54,54,108,0.03700089454650879,81.38939433846622
21,56,56,112,0.03817915916442871,82.00616609540543
22,58,58,116,0.039652109146118164,81.40809900282443
23,60,60,120,0.04092001914978027,77.27750404624817
24,62,62,124,0.04237484931945801,77.41682296761519
25,64,64,128,0.043810129165649414,77.29127669344939
26,66,66,132,0.04514884948730469,75.38269629840511
27,68,68,136,0.04643106460571289,74.57344655132124
28,70,70,140,0.047791242599487305,74.45491375690153
29,72,72,144,0.050438880920410156,72.89565423677095
30,76,76,152,0.05244016647338867,72.83600996361133
31,78,78,156,0.05365395545959473,70.95660971649431
32,82,82,164,0.05543875694274902,70.8559514329113
33,84,84,168,0.05681419372558594,66.7040948524666
34,88,88,176,0.05882596969604492,66.70628838848688
35,90,90,180,0.0600588321685791,64.6110555713069
36,94,94,188,0.06197619438171387,64.62213936484864
37,96,96,192,0.06398582458496094,61.35867357934194
38,98,98,196,0.06548690795898438,61.38600898506115
39,100,100,200,0.06685209274291992,59.51669595146177
40,102,102,204,0.06798291206359863,58.8749888722914
41,104,104,208,0.0691530704498291,58.44336644526447
42,108,108,216,0.07172894477844238,58.4360573106178
43,110,110,220,0.07315516471862793,56.43453445098294
44,112,112,224,0.07435393333435059,56.551864421448954
45,114,114,228,0.07572102546691895,56.620124460127045
46,118,118,236,0.07779097557067871,56.49773390423138
47,120,120,240,0.07900810241699219,56.26668731028121
48,124,124,248,0.0812528133392334,56.26031895604524
49,126,126,252,0.08301591873168945,55.34762315016383
50,128,128,256,0.08427119255065918,55.35964365627274
51,130,130,260,0.08552908897399902,55.135816007733865
52,134,134,268,0.08737993240356445,55.11996700146119
53,136,136,272,0.08849215507507324,54.47187253877382
54,140,140,280,0.09038805961608887,54.460106571777715
55,142,142,284,0.09173989295959473,53.995674247524676
56,146,146,292,0.09503316879272461,53.98969323174424
57,148,148,296,0.09651780128479004,53.54799543413492
58,152,152,304,0.1009979248046875,53.547729439598015
59,154,154,308,0.10247206687927246,53.297972867992485
60,158,158,316,0.10521912574768066,53.28910465196236
61,160,160,320,0.1068730354309082,52.98907781832577
62,164,164,328,0.11747503280639648,52.97954489768176
63,168,168,336,0.12012004852294922,52.90770113835151
64,172,172,344,0.12801408767700195,52.83963764705277
65,176,176,352,0.1328749656677246,52.78713789992162
66,178,178,356,0.14022493362426758,52.25327558316644
67,182,182,364,0.14376187324523926,52.248644915350724
68,184,184,368,0.1462268829345703,51.77790444441848
69,188,188,376,0.15604496002197266,51.7729651594334
70,190,190,380,0.15787506103515625,51.1308652608252
71,194,194,388,0.16051411628723145,51.144042207439725
72,198,198,396,0.16318106651306152,51.14235790919838
73,200,200,400,0.16576099395751953,50.19738391472356
74,204,204,408,0.17054104804992676,50.18790358401748
75,206,206,412,0.17378783226013184,49.01987311435073
76,210,210,420,0.1770789623260498,49.0151181990102
77,214,214,428,0.18018412590026855,48.813888695023934
78,218,218,436,0.186323881149292,48.45078280481425
79,222,222,444,0.18867802619934082,48.25445844813794
80,226,226,452,0.19124412536621094,48.12914163925393
81,228,228,456,0.1943039894104004,47.78043202340723
82,232,232,464,0.20229887962341309,47.803659177300005
83,236,236,472,0.20585203170776367,47.74127696793107
84,238,238,476,0.20785093307495117,46.6917099609675
85,242,242,484,0.21006202697753906,46.68986907280987
86,246,246,492,0.21241188049316406,46.5350640111194
87,250,250,500,0.2186739444732666,46.43962633016986
88,254,254,508,0.22170495986938477,46.36275224338169
89,256,256,512,0.2232041358947754,44.603278747423474
90,260,260,520,0.2252979278564453,44.61722790112458
91,264,264,528,0.22761797904968262,44.55255070294106
92,266,266,532,0.22904491424560547,44.202186014393874
93,270,270,540,0.231428861618042,44.16553095498216
94,274,274,548,0.23483610153198242,43.956234997552656
95,276,276,552,0.23643708229064941,41.3888165030487
96,280,280,560,0.2387678623199463,41.412520489006056
97,282,282,564,0.24010396003723145,38.53731514314245
98,288,288,576,0.2429518699645996,38.52108653706773
99,292,292,584,0.24497103691101074,38.32462242309771
100,294,294,588,0.24639487266540527,36.3725934846027
101,298,298,596,0.25074195861816406,35.45290479418327
102,302,302,604,0.25292110443115234,35.145798198275315
103,304,304,608,0.25431084632873535,34.43120198338033
104,306,306,612,0.255810022354126,33.8112297347966
105,310,310,620,0.25812697410583496,33.82724564697105
106,312,312,624,0.25946998596191406,33.55399990068668
107,316,316,632,0.2614309787750244,33.11477046947175
108,318,318,636,0.2647511959075928,30.245051758503678
109,322,322,644,0.2672121524810791,30.405262184572166
110,326,326,652,0.26905298233032227,30.561979020608305
111,328,328,656,0.27028799057006836,29.94582935692324
112,332,332,664,0.27252197265625,29.9901192699499
113,336,336,672,0.2747070789337158,30.01721787064048
114,340,340,680,0.27681493759155273,29.85000213716512
115,344,344,688,0.27961301803588867,29.571844819323132
116,348,348,696,0.28217196464538574,29.05370405994654
117,352,352,704,0.28421878814697266,28.50284601506405
118,356,356,712,0.286578893661499,27.94759427352824
119,360,360,720,0.28884100914001465,27.48897837057939
120,362,362,724,0.29035401344299316,25.13154886062148
121,366,366,732,0.292496919631958,24.935208757318378
122,370,370,740,0.2957329750061035,24.73677631097712
123,372,372,744,0.2974419593811035,22.762698919210834
124,376,376,752,0.30011796951293945,22.799630572042815
125,380,380,760,0.30266404151916504,22.959608318923983
126,382,382,764,0.30402302742004395,23.85094554175248
127,386,386,772,0.30598878860473633,23.869656402449436
128,388,388,776,0.30730199813842773,23.124501286195255
129,392,392,784,0.3099820613861084,23.149328377794518
130,396,396,792,0.3151359558105469,23.215561523934184
131,398,398,796,0.3172469139099121,22.85033307290678
132,400,400,800,0.320904016494751,22.734638782003458
133,402,402,804,0.3227870464324951,22.034492601362444
134,406,406,812,0.32555198669433594,22.03470805771167
135,408,408,816,0.3272829055786133,20.267372641775182
136,412,412,824,0.33960914611816406,20.246939110776793
137,414,414,828,0.34471702575683594,18.621050064706424
138,420,420,840,0.34987401962280273,18.62050186296915
139,424,424,848,0.35263991355895996,18.604731339084537
140,426,426,852,0.35439205169677734,18.28569076951044
141,430,430,860,0.3566930294036865,18.25929530312601
142,432,432,864,0.3581809997558594,16.073354066111847
143,436,436,872,0.3607628345489502,16.054788212609992
144,440,440,880,0.3644380569458008,16.000858459471374
145,444,444,888,0.36811184883117676,15.940291716132265
146,446,446,892,0.3699531555175781,15.121231866329708
147,450,450,900,0.3729829788208008,15.143674407780168
148,452,452,904,0.37450098991394043,13.586876436336752
149,456,456,912,0.3766050338745117,13.677500722518971
150,458,458,916,0.37886810302734375,13.36653466168832
151,462,462,924,0.3895859718322754,13.329561554868746
152,466,466,932,0.39307284355163574,13.356639302294184
153,468,468,936,0.3955409526824951,12.929975249683594
154,472,472,944,0.39837217330932617,12.953606236539827
155,476,476,952,0.40097689628601074,12.9863600374822
156,480,480,960,0.40569186210632324,13.012764427370143
157,484,484,968,0.40807199478149414,12.968375152335739
158,488,488,976,0.4102029800415039,12.944639389041527
159,490,490,980,0.41189098358154297,11.18712633352493
160,494,494,988,0.41433191299438477,11.228704895451074
161,498,498,996,0.41758108139038086,10.857200179936626
162,502,502,1004,0.42369699478149414,10.65782094159033
163,510,510,1020,0.4278299808502197,10.657483168600834
164,512,512,1024,0.4290812015533447,9.245447615018406
165,520,520,1040,0.4330408573150635,9.245136022170414
166,522,522,1044,0.43439793586730957,8.429720695927472
167,526,526,1052,0.43653297424316406,8.507294381690713
168,528,528,1056,0.4380300045013428,8.531101657455224
169,532,532,1064,0.4404029846191406,8.560325653437303
170,534,534,1068,0.44237208366394043,7.589703500604628
171,536,536,1072,0.4436819553375244,7.953682581923545
172,540,540,1080,0.44567298889160156,7.616555722885778
173,544,544,1088,0.44800305366516113,7.574580517953905
174,548,548,1096,0.45029616355895996,7.566321619887049
175,550,550,1100,0.4515509605407715,7.243394234190646
176,554,554,1108,0.4535679817199707,7.268056553781435
177,558,558,1116,0.45540308952331543,7.298242213413232
178,560,560,1120,0.4564979076385498,7.187162948870196
179,564,564,1128,0.45810985565185547,7.1205426126261955
180,568,568,1136,0.45970702171325684,7.074956299939231
181,570,570,1140,0.46080589294433594,7.087459260031892
182,574,574,1148,0.4627799987792969,7.071548680202682
183,576,576,1152,0.46448588371276855,6.821196601189399
184,580,580,1160,0.4669339656829834,6.796033939556196
185,582,582,1164,0.46891117095947266,6.228855834697129
186,588,588,1176,0.47176194190979004,6.236601937179216
187,592,592,1184,0.4733920097351074,6.293919745173412
188,596,596,1192,0.47500181198120117,6.359442289687877
189,598,598,1196,0.47607922554016113,6.521003829996403
190,602,602,1204,0.4776730537414551,6.512558077328322
191,604,604,1208,0.478740930557251,5.847446609088593
192,608,608,1216,0.4807591438293457,5.859913015601478
193,610,610,1220,0.4831380844116211,5.659978771089527
194,614,614,1228,0.48526597023010254,5.670019739357372
195,616,616,1232,0.4866499900817871,5.64224090566438
196,620,620,1240,0.48880887031555176,5.63404288730635
197,624,624,1248,0.4906949996948242,5.602492974419761
198,628,628,1256,0.4923529624938965,5.580511403290075
199,632,632,1264,0.49403810501098633,5.56938012108867
200,634,634,1268,0.49517297744750977,5.435562679775217
201,638,638,1276,0.497204065322876,5.434873864739302
202,640,640,1280,0.498582124710083,4.837847624007281
203,644,644,1288,0.5004730224609375,4.840673819508538
204,646,646,1292,0.5016047954559326,4.6435275391570485
205,650,650,1300,0.5033071041107178,4.640981651519041
206,652,652,1304,0.5044758319854736,4.5142310480180186
207,656,656,1312,0.5067300796508789,4.538011176606119
208,660,660,1320,0.508734941482544,4.560935305809608
209,662,662,1324,0.5100281238555908,4.723550369520581
210,666,666,1332,0.5123240947723389,4.730616050704498
211,668,668,1336,0.5136079788208008,4.556358233995866
212,672,672,1344,0.5158898830413818,4.552716025382665
213,674,674,1348,0.5176410675048828,4.466320291599004
214,678,678,1356,0.5200231075286865,4.465891799332553
215,680,680,1360,0.5214018821716309,4.373901208883922
216,684,684,1368,0.5231490135192871,4.36580800993238
217,688,688,1376,0.5248351097106934,4.3559591903201635
218,692,692,1384,0.5264871120452881,4.358085663279894
219,696,696,1392,0.5281460285186768,4.359842055745048
220,700,700,1400,0.5303390026092529,4.36682935590909
221,704,704,1408,0.5323441028594971,4.374100823418985
222,708,708,1416,0.5342929363250732,4.348138084984157
223,712,712,1424,0.536067008972168,4.326429468286619
224,714,714,1428,0.5372779369354248,4.266774030251781
225,718,718,1436,0.5390090942382812,4.265184141984264
226,722,722,1444,0.5408360958099365,4.253302605378963
227,726,726,1452,0.5426030158996582,4.220596798062843
228,730,730,1460,0.5445849895477295,4.188952159157338
229,734,734,1468,0.5464498996734619,4.1584766482944815
230,738,738,1476,0.5487618446350098,4.112089669454235
231,740,740,1480,0.5501160621643066,3.713281204803934
232,744,744,1488,0.5518798828125,3.7107961217249112
233,748,748,1496,0.5537769794464111,3.676816040407175
234,752,752,1504,0.5554838180541992,3.6187146551633305
235,754,754,1508,0.5565829277038574,3.366097906214236
236,758,758,1516,0.5582818984985352,3.3627573009764546
237,760,760,1520,0.5593969821929932,3.011416037967706
238,764,764,1528,0.5611240863800049,3.0254132918505547
239,768,768,1536,0.5630500316619873,3.046265884426248
240,770,770,1540,0.5647039413452148,2.97333372435844
241,774,774,1548,0.5667760372161865,2.963158100698706
242,776,776,1552,0.5678179264068604,2.422341959974915
243,780,780,1560,0.5695140361785889,2.4165503498222733
244,782,782,1564,0.5706570148468018,2.171991077868256
245,786,786,1572,0.5723409652709961,2.1787124557118887
246,790,790,1580,0.5739881992340088,2.1902494847363414
247,794,794,1588,0.5755839347839355,2.18428848031499
248,798,798,1596,0.5772249698638916,2.170407507663981
249,802,802,1604,0.5789289474487305,2.137938621803869
250,806,806,1612,0.5810308456420898,2.072429053774272
251,810,810,1620,0.5828959941864014,2.0129492395110447
252,812,812,1624,0.5840280055999756,1.677308643836227
253,816,816,1632,0.5857200622558594,1.6788453760448192
254,818,818,1636,0.5869178771972656,1.6505786667931943
255,822,822,1644,0.5885748863220215,1.6396601297292364
256,824,824,1648,0.5896730422973633,1.5488360872138855
257,828,828,1656,0.5913238525390625,1.5434853379498463
258,830,830,1660,0.5923640727996826,1.2276104195492508
259,834,834,1668,0.593925952911377,1.2249832041452464
260,836,836,1672,0.5950069427490234,1.0827841567438554
261,840,840,1680,0.5970518589019775,1.0996045005945234
262,842,842,1684,0.5983932018280029,1.1144954862855911
263,844,844,1688,0.599513053894043,1.0900817375234055
264,848,848,1696,0.6012380123138428,1.0722291506041302
265,850,850,1700,0.6023070812225342,0.99418177011853
266,854,854,1708,0.603909969329834,0.976142243436243
267,858,858,1716,0.605522871017456,0.9476558397360577
268,860,860,1720,0.6065590381622314,0.8263356761838168
269,864,864,1728,0.6083030700683594,0.8079683856437896
270,866,866,1732,0.6093780994415283,0.7607931042946348
271,868,868,1736,0.6104462146759033,0.7045481816105621
272,870,870,1740,0.6116108894348145,0.7676323867150359
273,872,872,1744,0.6129648685455322,0.625838136807829
274,876,876,1752,0.6151230335235596,0.61745450774049
275,878,878,1756,0.6162729263305664,0.5900308022642093
276,882,882,1764,0.6179399490356445,0.5814758852825435
277,886,886,1772,0.6195950508117676,0.5714492992512987
278,888,888,1776,0.6207160949707031,0.5121740816555302
279,892,892,1784,0.6223509311676025,0.5061323176248607
280,894,894,1788,0.62335205078125,0.4765180821003696
281,898,898,1796,0.6249768733978271,0.4783328322671423
282,902,902,1804,0.6267180442810059,0.4803574623863369
283,904,904,1808,0.6278390884399414,0.50668309455898
284,906,906,1812,0.6288940906524658,0.50447473107522
285,908,908,1816,0.6301259994506836,0.5066514735162855
286,912,912,1824,0.6333670616149902,0.5035911119769025
287,914,914,1828,0.6346859931945801,0.45878260016809236
288,918,918,1836,0.636660099029541,0.4581787625598963
289,920,920,1840,0.6380019187927246,0.42717602566710866
290,924,924,1848,0.6404399871826172,0.4284628797956884
291,926,926,1852,0.6419680118560791,0.3554739890212204
292,930,930,1860,0.6438388824462891,0.35553685513548317
293,932,932,1864,0.6448891162872314,0.2735203277270557
294,936,936,1872,0.646895170211792,0.2768641062310735
295,938,938,1876,0.648252010345459,0.23847275312130023
296,942,942,1884,0.6503801345825195,0.23460966792379168
297,944,944,1888,0.6517481803894043,0.14435280310271992
298,948,948,1896,0.6538088321685791,0.14328032700018412
299,950,950,1900,0.6557040214538574,0.10942330235332065
300,956,956,1912,0.659555196762085,0.10897390629600068
301,958,958,1916,0.6608471870422363,0.09676745776368989
302,962,962,1924,0.6630358695983887,0.09838578806363785
303,964,964,1928,0.6645801067352295,0.0918062154682957
304,968,968,1936,0.6668510437011719,0.09128369003144599
305,970,970,1940,0.6681890487670898,0.08183384591143295
306,974,974,1948,0.6701979637145996,0.08201369090261323
307,976,976,1952,0.671489953994751,0.0950657021276129
308,980,980,1960,0.673353910446167,0.09546193218864119
309,982,982,1964,0.6746060848236084,0.09421461155989164
310,986,986,1972,0.6766080856323242,0.0933677534853814
311,990,990,1980,0.678455114364624,0.09274384950822423
312,992,992,1984,0.6798160076141357,0.09158487132481241
313,996,996,1992,0.6825339794158936,0.09163068108841799
314,998,998,1996,0.683908224105835,0.08409951380826897
315,1002,1002,2004,0.6859021186828613,0.08377055567984826
316,1004,1004,2008,0.6871590614318848,0.06372367439109894
317,1008,1008,2016,0.6891510486602783,0.06319521949183127
318,1010,1010,2020,0.690446138381958,0.05119802426645492
319,1014,1014,2028,0.6925630569458008,0.05119415893841506
320,1016,1016,2032,0.6936681270599365,0.0478339415640221
321,1020,1020,2040,0.6954779624938965,0.04780319042481551
322,1022,1022,2044,0.6968650817871094,0.0441973877698274
323,1026,1026,2052,0.6991591453552246,0.04489069923340594
324,1030,1030,2060,0.7011258602142334,0.0456954275445014
325,1032,1032,2064,0.702570915222168,0.03758258398192993
326,1036,1036,2072,0.7047469615936279,0.037391458993738524
327,1038,1038,2076,0.7058498859405518,0.030924722081408618
328,1042,1042,2084,0.7075049877166748,0.030542568484634103
329,1044,1044,2088,0.7086961269378662,0.02568381401033548
330,1048,1048,2096,0.7106540203094482,0.025620221678195776
331,1050,1050,2100,0.7119858264923096,0.01917237687666784
332,1054,1054,2108,0.7140820026397705,0.019686785330804923
333,1056,1056,2112,0.7154591083526611,0.020558709244255624
334,1060,1060,2120,0.7172729969024658,0.02031906664296912
335,1062,1062,2124,0.7186229228973389,0.017501860238667177
336,1066,1066,2132,0.7203230857849121,0.0175582601559654
337,1068,1068,2136,0.721444845199585,0.01601047412373191
338,1072,1072,2144,0.723228931427002,0.01600514837218725
339,1074,1074,2148,0.7243578433990479,0.016048765076789095
340,1078,1078,2156,0.7260470390319824,0.016033443105015976
341,1082,1082,2164,0.7277250289916992,0.015720385292411265
342,1084,1084,2168,0.7289071083068848,0.012734328836700115
343,1088,1088,2176,0.7313930988311768,0.012814544578645837
344,1090,1090,2180,0.7326569557189941,0.01309871109458527
345,1094,1094,2188,0.7342679500579834,0.013056761511620607
346,1096,1096,2192,0.7353060245513916,0.010825750192225314
347,1100,1100,2200,0.7369489669799805,0.010743819134404475
348,1102,1102,2204,0.7380399703979492,0.005123215733988218
349,1104,1104,2208,0.7390918731689453,0.005297060616726412
350,1106,1106,2212,0.7402172088623047,0.006753163238386151
351,1108,1108,2216,0.7413508892059326,0.005406084588457816
352,1110,1110,2220,0.7424759864807129,0.005402350168765224
353,1112,1112,2224,0.7436020374298096,0.0044947352013196
354,1116,1116,2232,0.7452480792999268,0.004399154975203601
355,1118,1118,2236,0.7464351654052734,0.004133567514600145
356,1120,1120,2240,0.7479250431060791,0.003955842519417274
357,1122,1122,2244,0.74959397315979,0.003510233288238851
358,1126,1126,2252,0.7515981197357178,0.003495331839872051
359,1128,1128,2256,0.7531259059906006,0.003068597704213971
360,1132,1132,2264,0.7553191184997559,0.0030402714103274775
361,1134,1134,2268,0.7566540241241455,0.002170877033904617
362,1138,1138,2276,0.7585489749908447,0.0021628295966138467
363,1140,1140,2280,0.7596521377563477,0.001617727236293831
364,1144,1144,2288,0.7614390850067139,0.0015950655538290448
365,1146,1146,2292,0.7626690864562988,0.001230847769193133
366,1150,1150,2300,0.7651729583740234,0.001217942083599155
367,1152,1152,2304,0.7666089534759521,0.0007826954067695624
368,1156,1156,2312,0.7684259414672852,0.0007627611745419927
369,1158,1158,2316,0.769665002822876,0.0006341938913010381
370,1160,1160,2320,0.7708280086517334,0.0005550962341658305
371,1164,1164,2328,0.7728838920593262,0.0005526757203142552
372,1166,1166,2332,0.7742750644683838,0.0005202491499858297
373,1168,1168,2336,0.7754471302032471,0.00029142001176296617
374,1172,1172,2344,0.7773098945617676,0.0002874642310644049
375,1174,1174,2348,0.7786810398101807,0.00020180802493996453
376,1178,1178,2356,0.7807409763336182,0.00019240123754116212
377,1180,1180,2360,0.7823030948638916,0.00013825711596382462
378,1184,1184,2368,0.7840659618377686,0.00013772645536391792
379,1186,1186,2372,0.7852039337158203,0.00013240588020835276
380,1190,1190,2380,0.7869389057159424,0.00013480029815582384
381,1192,1192,2384,0.7879409790039062,0.00014746661690878682
382,1196,1196,2392,0.7896928787231445,0.0001468657636678472
383,1198,1198,2396,0.7908527851104736,0.00010960520580738375
384,1200,1200,2400,0.7918908596038818,0.00013297390216848726
385,1204,1204,2408,0.7935450077056885,0.0001338348527042399
386,1206,1206,2412,0.7946078777313232,5.7178381211997475e-05
387,1210,1210,2420,0.7966568470001221,5.45742254871584e-05
388,1212,1212,2424,0.7981979846954346,3.300166235931101e-05
389,1216,1216,2432,0.8001930713653564,3.298585681932309e-05
390,1218,1218,2436,0.8012599945068359,2.5327511821160442e-05
391,1222,1222,2444,0.8029289245605469,2.517205723506777e-05
392,1224,1224,2448,0.8040928840637207,2.1975171875965316e-05
393,1228,1228,2456,0.8060758113861084,2.134618978288927e-05
394,1230,1230,2460,0.8071050643920898,1.9876769783877535e-05
395,1234,1234,2468,0.808945894241333,1.9999223354716378e-05
396,1236,1236,2472,0.8100669384002686,1.8451926393936446e-05
397,1240,1240,2480,0.8118879795074463,1.8110386918124277e-05
398,1242,1242,2484,0.8131568431854248,1.3605173080577515e-05
399,1244,1244,2488,0.8146061897277832,1.2448575034795795e-05
400,1248,1248,2496,0.81675124168396,1.2452739952095726e-05
401,1250,1250,2500,0.8180418014526367,1.982117464649491e-05
402,1252,1252,2504,0.8192918300628662,2.1884840180064202e-05
403,1254,1254,2508,0.8204360008239746,1.9758361645472178e-05
404,1258,1258,2516,0.8222699165344238,1.9769432242355833e-05
405,1260,1260,2520,0.8237020969390869,2.5000072014336183e-05
406,1264,1264,2528,0.8257720470428467,2.4924918875512958e-05
407,1266,1266,2532,0.8269808292388916,2.4043991970756906e-05
408,1270,1270,2540,0.829010009765625,2.436320335164055e-05
409,1272,1272,2544,0.8315021991729736,2.6029244963865494e-05
410,1276,1276,2552,0.8337719440460205,2.6009704811258416e-05
411,1278,1278,2556,0.8352019786834717,2.5176859026032616e-05
412,1280,1280,2560,0.8366029262542725,2.3615653844899498e-05
413,1284,1284,2568,0.8385531902313232,2.341657761917304e-05
414,1286,1286,2572,0.8396549224853516,1.8670598024073115e-05
415,1290,1290,2580,0.8415579795837402,1.8595581423141994e-05
416,1292,1292,2584,0.8427920341491699,1.6297840488732618e-05
417,1296,1296,2592,0.8445398807525635,1.6314718664034444e-05
418,1298,1298,2596,0.8457939624786377,1.5316657140829193e-05
419,1302,1302,2604,0.8479681015014648,1.512813912540878e-05
420,1304,1304,2608,0.8493180274963379,1.4231123032004689e-05
421,1308,1308,2616,0.8511600494384766,1.4111672498984262e-05
422,1310,1310,2620,0.8532638549804688,1.3261920457807719e-05
423,1312,1312,2624,0.8544361591339111,1.2610547400981886e-05
424,1316,1316,2632,0.8561100959777832,1.260642113720678e-05
425,1318,1318,2636,0.8572020530700684,1.2034275755468116e-05
426,1322,1322,2644,0.8590221405029297,1.2013871128147002e-05
427,1324,1324,2648,0.8603899478912354,1.1890473160747206e-05
428,1328,1328,2656,0.8622331619262695,1.1883923889399739e-05
429,1330,1330,2660,0.8634939193725586,1.1481146771075146e-05
430,1332,1332,2664,0.8656589984893799,1.0954465437862382e-05
431,1336,1336,2672,0.8674030303955078,1.094808305879269e-05
432,1338,1338,2676,0.8685188293457031,1.0447021622894681e-05
433,1342,1342,2684,0.8701679706573486,1.0448139164509485e-05
434,1346,1346,2692,0.8718400001525879,1.0448844022903359e-05
435,1350,1350,2700,0.8734688758850098,1.0431756663820124e-05
436,1352,1352,2704,0.8745169639587402,9.911056849887245e-06
437,1356,1356,2712,0.8762218952178955,9.90433136394131e-06
438,1358,1358,2716,0.877331018447876,9.243488193533267e-06
439,1362,1362,2724,0.8790898323059082,9.218531204169267e-06
440,1364,1364,2728,0.8803520202636719,8.988491003947274e-06
441,1368,1368,2736,0.882472038269043,8.989656976154947e-06
442,1370,1370,2740,0.8836081027984619,8.44459486870619e-06
443,1374,1374,2748,0.8854410648345947,8.435916356575035e-06
444,1376,1376,2752,0.8865799903869629,7.982856004673522e-06
445,1380,1380,2760,0.8883659839630127,7.973290394147625e-06
446,1382,1382,2764,0.8895390033721924,7.880529892645427e-06
447,1386,1386,2772,0.8914060592651367,7.884352726250654e-06
448,1388,1388,2776,0.8925471305847168,7.84526878305769e-06
449,1392,1392,2784,0.894158124923706,7.797284979460528e-06
450,1396,1396,2792,0.8959228992462158,7.737118266959442e-06
451,1400,1400,2800,0.8981518745422363,7.66444736655103e-06
452,1404,1404,2808,0.899946928024292,7.602708137710579e-06
453,1406,1406,2812,0.9010140895843506,7.489072800126451e-06
454,1410,1410,2820,0.9031198024749756,7.498381592085934e-06
455,1414,1414,2828,0.9048409461975098,7.506919814659341e-06
456,1418,1418,2836,0.9065289497375488,7.457811307176598e-06
457,1422,1422,2844,0.9082350730895996,7.4281680326748756e-06
458,1426,1426,2852,0.9099111557006836,7.410294301735121e-06
459,1430,1430,2860,0.9115819931030273,7.4020729243784444e-06
460,1434,1434,2868,0.9138779640197754,7.3928442816395545e-06
461,1438,1438,2876,0.9162280559539795,7.3751491527218604e-06
462,1440,1440,2880,0.917396068572998,6.929242999831331e-06
463,1444,1444,2888,0.9191110134124756,6.926831133569067e-06
464,1446,1446,2892,0.9201788902282715,6.692016654596955e-06
465,1450,1450,2900,0.9218349456787109,6.6896168391394895e-06
466,1452,1452,2904,0.9230170249938965,6.525480898744718e-06
467,1456,1456,2912,0.9247369766235352,6.51730647405202e-06
468,1460,1460,2920,0.9263401031494141,6.489570978374104e-06
469,1464,1464,2928,0.9280431270599365,6.391764145519119e-06
470,1468,1468,2936,0.9299421310424805,6.321135970210889e-06
471,1472,1472,2944,0.9322569370269775,6.219894316927821e-06
472,1476,1476,2952,0.9339351654052734,6.143801329017151e-06
473,1480,1480,2960,0.9355881214141846,6.079730269448191e-06
474,1484,1484,2968,0.9371850490570068,6.0174381815158995e-06
475,1488,1488,2976,0.9387750625610352,5.973606562292844e-06
476,1490,1490,2980,0.9398400783538818,5.859031716681784e-06
477,1494,1494,2988,0.9414529800415039,5.863496426172787e-06
478,1498,1498,2996,0.9431369304656982,5.872451879440632e-06
479,1502,1502,3004,0.9446988105773926,5.867059940101171e-06
480,1506,1506,3012,0.9468848705291748,5.86030682825367e-06
481,1510,1510,3020,0.9489119052886963,5.858115969203936e-06
482,1512,1512,3024,0.9499950408935547,5.8957964483852265e-06
483,1516,1516,3032,0.9516549110412598,5.8951590062861214e-06
484,1518,1518,3036,0.9527370929718018,5.72976364310307e-06
485,1522,1522,3044,0.9543848037719727,5.728558221562707e-06
486,1526,1526,3052,0.9559919834136963,5.702584985556314e-06
487,1528,1528,3056,0.9570209980010986,5.5485326129200985e-06
488,1532,1532,3064,0.9587130546569824,5.546452484850306e-06
489,1536,1536,3072,0.9603400230407715,5.4966028528724564e-06
490,1540,1540,3080,0.9618968963623047,5.452190976029669e-06
491,1542,1542,3084,0.9631638526916504,5.067843858341803e-06
492,1546,1546,3092,0.9652318954467773,5.043633450441121e-06
493,1550,1550,3100,0.9669549465179443,4.98698727824376e-06
494,1552,1552,3104,0.9680368900299072,4.733235186904494e-06
495,1556,1556,3112,0.9695339202880859,4.6918680709495675e-06
496,1560,1560,3120,0.9711089134216309,4.611756253325439e-06
497,1562,1562,3124,0.9721858501434326,4.146200126342592e-06
498,1566,1566,3132,0.9738020896911621,4.117093112654402e-06
499,1568,1568,3136,0.974761962890625,3.5987890214528306e-06
500,1572,1572,3144,0.9766170978546143,3.5856343174600624e-06
501,1574,1574,3148,0.9777657985687256,3.5802620459435275e-06
502,1578,1578,3156,0.9795620441436768,3.5837737186739105e-06
503,1580,1580,3160,0.9809510707855225,3.1865929486230016e-06
504,1584,1584,3168,0.9827671051025391,3.1754062774780323e-06
505,1586,1586,3172,0.9839270114898682,2.8346939870971255e-06
506,1590,1590,3180,0.985572099685669,2.8257300073164515e-06
507,1592,1592,3184,0.9866609573364258,2.036787122960959e-06
508,1596,1596,3192,0.9882349967956543,2.0317785356382956e-06
509,1598,1598,3196,0.9892690181732178,1.7320904817097471e-06
510,1602,1602,3204,0.9909839630126953,1.7211274325745762e-06
511,1604,1604,3208,0.9920687675476074,1.1732245184248313e-06
512,1608,1608,3216,0.9937009811401367,1.171197027360904e-06
513,1610,1610,3220,0.9949660301208496,1.016456394609122e-06
514,1614,1614,3228,0.9972469806671143,9.841462542681256e-07
515,1616,1616,3232,0.9987211227416992,6.118057171988767e-07
516,1620,1620,3240,1.0005629062652588,6.121798605818185e-07
517,1622,1622,3244,1.001749038696289,3.861464392684866e-07
518,1626,1626,3252,1.0038468837738037,3.821398877335014e-07
519,1628,1628,3256,1.0050098896026611,2.5592157726350706e-07
520,1632,1632,3264,1.006875991821289,2.536371539463289e-07
521,1634,1634,3268,1.0082809925079346,1.1618408279900905e-07
522,1638,1638,3276,1.0103991031646729,1.2089321899111383e-07
523,1640,1640,3280,1.0116548538208008,1.424417632733821e-07
524,1644,1644,3288,1.014059066772461,1.3934629805589793e-07
525,1646,1646,3292,1.015429973602295,1.3984288216306595e-07
526,1650,1650,3300,1.0174601078033447,1.404511067448766e-07
527,1652,1652,3304,1.0187220573425293,1.1906502095371252e-07
528,1656,1656,3312,1.0206248760223389,1.1417637324484531e-07
529,1658,1658,3316,1.0218369960784912,5.6224394029413816e-08
530,1662,1662,3324,1.0238609313964844,5.542824510484934e-08
531,1664,1664,3328,1.0250828266143799,6.547566044901032e-08
532,1668,1668,3336,1.0269849300384521,6.871277946629561e-08
533,1670,1670,3340,1.0281879901885986,1.0020244189945515e-07
534,1674,1674,3348,1.0310349464416504,1.0007477158069378e-07
535,1676,1676,3352,1.0326159000396729,6.496418336610077e-08
536,1680,1680,3360,1.034553050994873,6.200218649610179e-08
537,1682,1682,3364,1.0357909202575684,3.257468961237464e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha0/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,8.392333984375e-05,4.387061074692293
200,201,200,401,0.00596308708190918,0.1842133593717011
400,401,400,801,0.013149023056030273,0.08950090778682597
601,602,601,1203,0.019085168838500977,0.0640727904903761
801,802,801,1603,0.026002883911132812,0.05368010844351703
1001,1002,1001,2003,0.03272700309753418,0.04784400270691025
1201,1202,1201,2403,0.038706064224243164,0.043962346568317545
1401,1402,1401,2803,0.04642510414123535,0.040170424392327105
1602,1603,1602,3205,0.05220603942871094,0.0378297155531487
1802,1803,1802,3605,0.05798912048339844,0.03500764031340371
2002,2003,2002,4005,0.06401896476745605,0.033218977387609094
2202,2203,2202,4405,0.07025623321533203,0.031712977453885745
2402,2403,2402,4805,0.07633113861083984,0.030488556797115297
2603,2604,2603,5207,0.08235502243041992,0.029160518425359824
2803,2804,2803,5607,0.08842611312866211,0.02808380132600252
3003,3004,3003,6007,0.09497809410095215,0.027439038899275816
3203,3204,3203,6407,0.10264921188354492,0.02695027946362406
3403,3404,3403,6807,0.11031413078308105,0.026584533343648
3604,3605,3604,7209,0.11766409873962402,0.02608917186135332
3804,3805,3804,7609,0.12536191940307617,0.029376093689549996
4004,4005,4004,8009,0.13289308547973633,0.025416334225533774
4204,4205,4204,8409,0.14143109321594238,0.024972310198149255
4404,4405,4404,8809,0.14855098724365234,0.024715147719762857
4605,4606,4605,9211,0.15561914443969727,0.024591685184676682
4805,4806,4805,9611,0.16398906707763672,0.02880578201952542
5005,5006,5005,10011,0.1708831787109375,0.02474827063384724
5205,5206,5205,10411,0.17736601829528809,0.02527854875902983
5405,5406,5405,10811,0.18422198295593262,0.027694679864959045
5606,5607,5606,11213,0.19057607650756836,0.02795125230114081
5806,5807,5806,11613,0.19726204872131348,0.023608594264080074
6006,6007,6006,12013,0.20487403869628906,0.023527162933789102
6206,6207,6206,12413,0.21230220794677734,0.023341135626410606
6406,6407,6406,12813,0.21848511695861816,0.02310628117723416
6607,6608,6607,13215,0.22456598281860352,0.023122723586407712
6807,6808,6807,13615,0.23079395294189453,0.02377070920682427
7007,7008,7007,14015,0.2368299961090088,0.022869241994367823
7207,7208,7207,14415,0.24302101135253906,0.022819616348137704
7407,7408,7407,14815,0.2491300106048584,0.022491314432376227
7608,7609,7608,15217,0.25562500953674316,0.02251223999144792
7808,7809,7808,15617,0.26163411140441895,0.022361100974653488
8008,8009,8008,16017,0.2675960063934326,0.022206739994266353
8208,8209,8208,16417,0.2734389305114746,0.022090115079058198
8408,8409,8408,16817,0.27960801124572754,0.02201226857961251
8609,8610,8609,17219,0.28551197052001953,0.02206761219570357
8809,8810,8809,17619,0.291409969329834,0.02532542037528179
9009,9010,9009,18019,0.2972989082336426,0.02170092808990991
9209,9210,9209,18419,0.3033599853515625,0.021560398210116696
9409,9410,9409,18819,0.3095860481262207,0.021370971442305983
9610,9611,9610,19221,0.3158071041107178,0.023018260673251138
9810,9811,9810,19621,0.32196617126464844,0.022092837094809345
10010,10011,10010,20021,0.32786989212036133,0.021082136954524492
10210,10211,10210,20421,0.3337540626525879,0.02105114947261687
10410,10411,10410,20821,0.3396790027618408,0.02104825035317345
10611,10612,10611,21223,0.34578514099121094,0.020883696401520716
10811,10812,10811,21623,0.35199689865112305,0.02103615413548143
11011,11012,11011,22023,0.3580470085144043,0.020849232031725236
11211,11212,11211,22423,0.3639209270477295,0.020621427912150585
11411,11412,11411,22823,0.36974406242370605,0.020507565956851187
11612,11613,11612,23225,0.37547898292541504,0.020163599691971262
11812,11813,11812,23625,0.38126325607299805,0.020357944259584922
12012,12013,12012,24025,0.3872079849243164,0.02329837724243542
12212,12213,12212,24425,0.39293909072875977,0.02006217064033194
12412,12413,12412,24825,0.3987252712249756,0.019968714368819664
12613,12614,12613,25227,0.4045541286468506,0.019621998615492634
12813,12814,12813,25627,0.4103271961212158,0.019899776004216118
13013,13014,13013,26027,0.4161970615386963,0.01993662452670902
13213,13214,13213,26427,0.42197394371032715,0.019652571174822473
13413,13414,13413,26827,0.4277491569519043,0.022252880702721165
13614,13615,13614,27229,0.4342200756072998,0.01925047727339765
13814,13815,13814,27629,0.4399750232696533,0.019169855049710513
14014,14015,14014,28029,0.44704198837280273,0.0236484376452837
14214,14215,14214,28429,0.45429515838623047,0.019161913414835825
14414,14415,14414,28829,0.4602701663970947,0.020047409941289892
14615,14616,14615,29231,0.46623706817626953,0.018652850296161528
14815,14816,14815,29631,0.472365140914917,0.020111290038272937
15015,15016,15015,30031,0.4783952236175537,0.018503485751028174
15215,15216,15215,30431,0.4847140312194824,0.022785686975259425
15415,15416,15415,30831,0.4907369613647461,0.022488827658294897
15616,15617,15616,31233,0.49677324295043945,0.022505017714190806
15816,15817,15816,31633,0.5029451847076416,0.01821839774626749
16016,16017,16016,32033,0.5090959072113037,0.01805512329677396
16216,16217,16216,32433,0.5150740146636963,0.02059380622184377
16416,16417,16416,32833,0.5211362838745117,0.017892965512531923
16617,16618,16617,33235,0.5271739959716797,0.017968702738862623
16817,16818,16817,33635,0.5330660343170166,0.017881281551843195
17017,17018,17017,34035,0.5392539501190186,0.017607733741237874
17217,17218,17217,34435,0.5454950332641602,0.01844185460455576
17417,17418,17417,34835,0.5514712333679199,0.020809148761590388
17618,17619,17618,35237,0.5574369430541992,0.017501993938133356
17818,17819,17818,35637,0.5638132095336914,0.017329461393972474
18018,18019,18018,36037,0.5704550743103027,0.017220536921859684
18218,18219,18218,36437,0.5777370929718018,0.017163429339517384
18418,18419,18418,36837,0.5841779708862305,0.017427318626169475
18619,18620,18619,37239,0.5908281803131104,0.020523368668403007
18819,18820,18819,37639,0.5973050594329834,0.01685197121953309
19019,19020,19019,38039,0.6035699844360352,0.021856660079918353
19219,19220,19219,38439,0.6097431182861328,0.016747392759050222
19419,19420,19419,38839,0.6163280010223389,0.016581568709277673
19620,19621,19620,39241,0.6232771873474121,0.016589931914777367
19820,19821,19820,39641,0.6302900314331055,0.016499111602322994
20020,20021,20020,40041,0.6365640163421631,0.02035303289088751
20220,20221,20220,40441,0.6427550315856934,0.017184700367162003
20420,20421,20420,40841,0.64906907081604,0.01626664845034462
20621,20622,20621,41243,0.6552200317382812,0.018844066069117336
20821,20822,20821,41643,0.66121506690979,0.015877683449230566
21021,21022,21021,42043,0.6673181056976318,0.016889381576759756
21221,21222,21221,42443,0.673382043838501,0.018468896118016307
21421,21422,21421,42843,0.679440975189209,0.015771494062805747
21622,21623,21622,43245,0.6859970092773438,0.01583270682596724
21822,21823,21822,43645,0.6922240257263184,0.015595182074509889
22022,22023,22022,44045,0.698371171951294,0.0155996405448533
22222,22223,22222,44445,0.7045419216156006,0.015460291942131082
22422,22423,22422,44845,0.7106409072875977,0.015551359833280098
22623,22624,22623,45247,0.7167580127716064,0.015364964758678212
22823,22824,22823,45647,0.722999095916748,0.015259065297969962
23023,23024,23023,46047,0.7290802001953125,0.0151621643664495
23223,23224,23223,46447,0.7351911067962646,0.015133444717631216
23423,23424,23423,46847,0.7414772510528564,0.015979810705922953
23624,23625,23624,47249,0.7476301193237305,0.01722911183769795
23824,23825,23824,47649,0.7537322044372559,0.014810854232805483
24024,24025,24024,48049,0.7597920894622803,0.015275523085091556
24224,24225,24224,48449,0.765869140625,0.014709586575179127
24424,24425,24424,48849,0.772284984588623,0.01681523933371397
24625,24626,24625,49251,0.7784140110015869,0.015242620309582471
24825,24826,24825,49651,0.7844760417938232,0.014505814625316516
25025,25026,25025,50051,0.790524959564209,0.014420089579536171
25225,25226,25225,50451,0.7966358661651611,0.014477080655222387
25425,25426,25425,50851,0.8027269840240479,0.014348836205393123
25626,25627,25626,51253,0.8088440895080566,0.014235110793421385
25826,25827,25826,51653,0.8148989677429199,0.014241671170314437
26026,26027,26026,52053,0.8209578990936279,0.013992561867390996
26226,26227,26226,52453,0.8270111083984375,0.01398753211140654
26426,26427,26426,52853,0.8330380916595459,0.014147185056737423
26627,26628,26627,53255,0.8391051292419434,0.015957573560474694
26827,26828,26827,53655,0.845142126083374,0.013737339576572749
27027,27028,27027,54055,0.8511919975280762,0.013618643265642823
27227,27228,27227,54455,0.85725998878479,0.015659829778024274
27427,27428,27427,54855,0.8637239933013916,0.013505103169415852
27628,27629,27628,55257,0.8697431087493896,0.01349951621601422
27828,27829,27828,55657,0.875669002532959,0.01342429139348619
28028,28029,28028,56057,0.8817222118377686,0.014339094300417046
28228,28229,28228,56457,0.8878011703491211,0.013366143462820135
28428,28429,28428,56857,0.8939299583435059,0.014336431517761884
28629,28630,28629,57259,0.9001600742340088,0.013252705114974263
28829,28830,28829,57659,0.9063811302185059,0.013181256507363083
29029,29030,29029,58059,0.9125480651855469,0.013063788847197983
29229,29230,29229,58459,0.9187159538269043,0.015745701304893764
29429,29430,29429,58859,0.9248089790344238,0.014587684914652909
29630,29631,29630,59261,0.9310240745544434,0.013654264398053444
29830,29831,29830,59661,0.9372920989990234,0.012745491950715875
30030,30031,30030,60061,0.9433979988098145,0.013995564545420065
30230,30231,30230,60461,0.9497780799865723,0.012629157072454248
30430,30431,30430,60861,0.9561190605163574,0.012609507220559986
30631,30632,30631,61263,0.9625170230865479,0.012486798200242248
30831,30832,30831,61663,0.9694032669067383,0.012429828369275824
31031,31032,31031,62063,0.9757640361785889,0.01233793456389007
31231,31232,31231,62463,0.9817290306091309,0.012273760072572065
31431,31432,31431,62863,0.9877619743347168,0.013390922066411737
31632,31633,31632,63265,0.9939792156219482,0.014677482178872719
31832,31833,31832,63665,0.9999749660491943,0.012135463319280044
32032,32033,32032,64065,1.0069389343261719,0.01538484873071717
32232,32233,32232,64465,1.0131299495697021,0.014984331008584479
32432,32433,32432,64865,1.0202341079711914,0.011938306999697378
32633,32634,32633,65267,1.026522159576416,0.01210897758471628
32833,32834,32833,65667,1.0324649810791016,0.012529778225425831
33033,33034,33033,66067,1.0384151935577393,0.011662466355523291
33233,33234,33233,66467,1.044335126876831,0.015335092939516353
33433,33434,33433,66867,1.0502829551696777,0.011658389270715408
33634,33635,33634,67269,1.0562701225280762,0.011550851084817532
33834,33835,33834,67669,1.0625770092010498,0.011442153251707577
34034,34035,34034,68069,1.0685770511627197,0.011533268032610506
34234,34235,34234,68469,1.074627161026001,0.011402700849156738
34434,34435,34434,68869,1.0809710025787354,0.011323583234960395
34635,34636,34635,69271,1.087151050567627,0.011367177427921291
34835,34836,34835,69671,1.0939030647277832,0.011344341238345696
35035,35036,35035,70071,1.10001802444458,0.011161932342710287
35235,35236,35235,70471,1.1061089038848877,0.01355887504151913
35435,35436,35435,70871,1.1121799945831299,0.013314579110700196
35636,35637,35636,71273,1.1182451248168945,0.01294219570337818
35836,35837,35836,71673,1.1242640018463135,0.01097024139430618
36036,36037,36036,72073,1.1303081512451172,0.010965834461048063
36236,36237,36236,72473,1.136348009109497,0.011888154741444171
36436,36437,36436,72873,1.142388105392456,0.010759902989858027
36637,36638,36637,73275,1.148463249206543,0.010689466699165125
36837,36838,36837,73675,1.154466152191162,0.010703263173325608
37037,37038,37037,74075,1.1604831218719482,0.010691816212449455
37237,37238,37237,74475,1.1664690971374512,0.011457087115894497
37437,37438,37437,74875,1.1723041534423828,0.01057078430266816
37638,37639,37638,75277,1.1780641078948975,0.011290875105509196
37838,37839,37838,75677,1.183912992477417,0.010352720637895257
38038,38039,38038,76077,1.1897921562194824,0.011165393564655403
38238,38239,38238,76477,1.1956291198730469,0.010250936751035156
38438,38439,38438,76877,1.2014999389648438,0.010291781271826337
38639,38640,38639,77279,1.2076449394226074,0.010090867243373346
38839,38840,38839,77679,1.2135770320892334,0.01016562891382518
39039,39040,39039,78079,1.2226932048797607,0.011701398280788219
39239,39240,39239,78479,1.2294721603393555,0.010245664140523265
39439,39440,39439,78879,1.2353920936584473,0.00996534469500198
39640,39641,39640,79281,1.2437961101531982,0.009948367557898762
39840,39841,39840,79681,1.2500810623168945,0.009903463810679662
40040,40041,40040,80081,1.2582800388336182,0.00980710031279822
40240,40241,40240,80481,1.2649180889129639,0.01203257202896133
40440,40441,40440,80881,1.2708699703216553,0.009729798017285693
40641,40642,40641,81283,1.2779450416564941,0.009982092153465481
40841,40842,40841,81683,1.2844059467315674,0.009637874136854494
41041,41042,41041,82083,1.29062819480896,0.009570404293112096
41241,41242,41241,82483,1.2967901229858398,0.011148533065216506
41441,41442,41441,82883,1.3029050827026367,0.009481025770236252
41642,41643,41642,83285,1.309061050415039,0.009456963085172672
41842,41843,41842,83685,1.315237045288086,0.009382659323967259
42042,42043,42042,84085,1.3218450546264648,0.011448509340062174
42242,42243,42242,84485,1.3279650211334229,0.009345144855758401
42442,42443,42442,84885,1.3344430923461914,0.009217754436636354
42643,42644,42643,85287,1.3404102325439453,0.009161943486176372
42843,42844,42843,85687,1.3468642234802246,0.009142820677727653
43043,43044,43043,86087,1.3528120517730713,0.010143596241899824
43243,43244,43243,86487,1.3587861061096191,0.008994178343671163
43443,43444,43443,86887,1.3646860122680664,0.009304369683762009
43644,43645,43644,87289,1.3706350326538086,0.008937245085437973
43844,43845,43844,87689,1.3765439987182617,0.009320026988471586
44044,44045,44044,88089,1.3830931186676025,0.008890415276702616
44244,44245,44244,88489,1.3890140056610107,0.008850883211299286
44444,44445,44444,88889,1.3949570655822754,0.009008247036694872
44645,44646,44645,89291,1.4009530544281006,0.008828107987199702
44845,44846,44845,89691,1.4069430828094482,0.010151020588288909
45045,45046,45045,90091,1.4128341674804688,0.008798780492575323
45245,45246,45245,90491,1.4187588691711426,0.008542407031617629
45445,45446,45445,90891,1.4246909618377686,0.008587599773307487
45646,45647,45646,91293,1.430643081665039,0.008585586616359712
45846,45847,45846,91693,1.4365298748016357,0.00856437548795065
46046,46047,46046,92093,1.4426629543304443,0.00847780016859289
46246,46247,46246,92493,1.4487922191619873,0.008436203431380664
46446,46447,46446,92893,1.454787015914917,0.008400786679596282
46647,46648,46647,93295,1.460726022720337,0.009022651241716079
46847,46848,46847,93695,1.4666450023651123,0.00828299455687527
47047,47048,47047,94095,1.472594976425171,0.008653361338931865
47247,47248,47247,94495,1.4783082008361816,0.008244454831417556
47447,47448,47447,94895,1.4840140342712402,0.008443839618910955
47648,47649,47648,95297,1.4897000789642334,0.008097907247944947
47848,47849,47848,95697,1.4957571029663086,0.008118665054317456
48048,48049,48048,96097,1.5032310485839844,0.00818648728571346
48248,48249,48248,96497,1.5106351375579834,0.00829676985019953
48448,48449,48448,96897,1.517035961151123,0.0081780990262309
48649,48650,48649,97299,1.5230610370635986,0.007949077293283629
48849,48850,48849,97699,1.5288410186767578,0.007814239057312032
49049,49050,49049,98099,1.5346181392669678,0.0077974849276984965
49249,49250,49249,98499,1.5407471656799316,0.007809645299363575
49449,49450,49449,98899,1.547408103942871,0.007773459803747118
49650,49651,49650,99301,1.5532801151275635,0.00783703922826673
49850,49851,49850,99701,1.5591180324554443,0.0076902340014995
50050,50051,50050,100101,1.564958095550537,0.007579996032670245
50250,50251,50250,100501,1.5708842277526855,0.00930518785887562
50450,50451,50450,100901,1.5768399238586426,0.0077449079115948635
50651,50652,50651,101303,1.5828521251678467,0.007485673990440684
50851,50852,50851,101703,1.5888011455535889,0.007436660587515145
51051,51052,51051,102103,1.594763994216919,0.007484348524433028
51251,51252,51251,102503,1.6007380485534668,0.007416223104808162
51451,51452,51451,102903,1.6066820621490479,0.007329371516299548
51652,51653,51652,103305,1.6126511096954346,0.007593209689607612
51852,51853,51852,103705,1.618588924407959,0.007262764164795382
52052,52053,52052,104105,1.6245100498199463,0.007295176720471927
52252,52253,52252,104505,1.6304352283477783,0.007174263478162078
52452,52453,52452,104905,1.6363589763641357,0.0071672415049468296
52653,52654,52653,105307,1.6423921585083008,0.007147963595512411
52853,52854,52853,105707,1.6483421325683594,0.007123158366932032
53053,53054,53053,106107,1.6544718742370605,0.007760234507233116
53253,53254,53253,106507,1.6604039669036865,0.007040737099156903
53453,53454,53453,106907,1.6663439273834229,0.006941576805611954
53654,53655,53654,107309,1.67215895652771,0.00855396703792472
53854,53855,53854,107709,1.6778161525726318,0.006918943363875176
54054,54055,54054,108109,1.683495044708252,0.006907321159691736
54254,54255,54254,108509,1.689338207244873,0.006919407245725566
54454,54455,54454,108909,1.695418119430542,0.006905896520878805
54655,54656,54655,109311,1.701267957687378,0.006774720413557326
54855,54856,54855,109711,1.7071502208709717,0.006966943424937531
55055,55056,55055,110111,1.7129158973693848,0.008284943342452038
55255,55256,55255,110511,1.7186739444732666,0.006675640675454933
55455,55456,55455,110911,1.7244360446929932,0.006887294746810684
55656,55657,55656,111313,1.730757236480713,0.006665509007886521
55856,55857,55856,111713,1.7365729808807373,0.006671097530787778
56056,56057,56056,112113,1.742692232131958,0.0065286326538250145
56256,56257,56256,112513,1.7490081787109375,0.006512178681099781
56456,56457,56456,112913,1.7550148963928223,0.007170814998733508
56657,56658,56657,113315,1.7607841491699219,0.007036975323387839
56857,56858,56857,113715,1.7665510177612305,0.006628510898732772
57057,57058,57057,114115,1.7722859382629395,0.006411856692851152
57257,57258,57257,114515,1.7780930995941162,0.006427970010303372
57457,57458,57457,114915,1.783865213394165,0.006296796937530491
57658,57659,57658,115317,1.7897169589996338,0.0065113234634079685
57858,57859,57858,115717,1.7956559658050537,0.006223892145659718
58058,58059,58058,116117,1.8014731407165527,0.006238527342008057
58258,58259,58258,116517,1.8072659969329834,0.006934188763934251
58458,58459,58458,116917,1.8131258487701416,0.006191489784595947
58659,58660,58659,117319,1.819025993347168,0.006129301607581325
58859,58860,58859,117719,1.8248131275177002,0.006128510236352602
59059,59060,59059,118119,1.8306171894073486,0.006012974400067028
59259,59260,59259,118519,1.8365230560302734,0.006503450496967767
59459,59460,59459,118919,1.842345952987671,0.006969063310439132
59660,59661,59660,119321,1.848282814025879,0.005955188446155179
59860,59861,59860,119721,1.8541979789733887,0.005944758400561272
60060,60061,60060,120121,1.8600919246673584,0.005954715249174598
60260,60261,60260,120521,1.8658618927001953,0.005929704913928896
60460,60461,60460,120921,1.8716650009155273,0.005874443116280285
60661,60662,60661,121323,1.878913164138794,0.006368864791791769
60861,60862,60861,121723,1.8869860172271729,0.005843942343254285
61061,61062,61061,122123,1.8939540386199951,0.00573028977690027
61261,61262,61261,122523,1.9010372161865234,0.005761455181750258
61461,61462,61461,122923,1.9074602127075195,0.0056893122943081405
61662,61663,61662,123325,1.9132869243621826,0.005716393864227136
61862,61863,61862,123725,1.9191172122955322,0.005763568976174787
62062,62063,62062,124125,1.924957036972046,0.006830292075994993
62262,62263,62262,124525,1.930811882019043,0.005639443525685054
62462,62463,62462,124925,1.936629056930542,0.006354217891780564
62663,62664,62663,125327,1.9428942203521729,0.005649345742346727
62863,62864,62863,125727,1.949002981185913,0.005922099622513662
63063,63064,63063,126127,1.9551770687103271,0.00549446712282669
63263,63264,63263,126527,1.960773229598999,0.005404755339666591
63463,63464,63463,126927,1.966426134109497,0.005448619248934733
63664,63665,63664,127329,1.9722869396209717,0.00539733937481982
63864,63865,63864,127729,1.9781520366668701,0.006329431523668227
64064,64065,64064,128129,1.9840080738067627,0.006071161406448663
64264,64265,64264,128529,1.9898529052734375,0.005378177169698621
64464,64465,64464,128929,1.9957730770111084,0.006297521759131589
64665,64666,64665,129331,2.001701831817627,0.005499432729780842
64865,64866,64865,129731,2.0076041221618652,0.005206590121344269
65065,65066,65065,130131,2.013468027114868,0.005165210976184468
65265,65266,65265,130531,2.019310235977173,0.005186362543535456
65465,65466,65465,130931,2.0251970291137695,0.0051491589271982436
65666,65667,65666,131333,2.0310862064361572,0.005094684891638816
65866,65867,65866,131733,2.0369300842285156,0.005089414485359224
66066,66067,66066,132133,2.042809247970581,0.005084373667053362
66266,66267,66266,132533,2.0486888885498047,0.005019498584227978
66466,66467,66466,132933,2.054676055908203,0.0057519883578847535
66667,66668,66667,133335,2.060727119445801,0.0059973431784928494
66867,66868,66867,133735,2.066754102706909,0.005198702771323449
67067,67068,67067,134135,2.072866201400757,0.00495725920870504
67267,67268,67267,134535,2.078994035720825,0.004967827608209544
67467,67468,67467,134935,2.085029125213623,0.004912304888524369
67668,67669,67668,135337,2.0911848545074463,0.004907585766098389
67868,67869,67868,135737,2.0972900390625,0.004821251958755352
68068,68069,68068,136137,2.1034791469573975,0.004916036586098999
68268,68269,68268,136537,2.1096949577331543,0.004777763562331958
68468,68469,68468,136937,2.115812063217163,0.0056909401098151815
68669,68670,68669,137339,2.122056007385254,0.004751102848833676
68869,68870,68869,137739,2.1282291412353516,0.004708817096448989
69069,69070,69069,138139,2.1342568397521973,0.004740308783840497
69269,69270,69269,138539,2.1404459476470947,0.00471294447544304
69469,69470,69469,138939,2.146618127822876,0.0046557639966246945
69670,69671,69670,139341,2.1528570652008057,0.005438587423022217
69870,69871,69870,139741,2.159011125564575,0.004620582415964322
70070,70071,70070,140141,2.1652369499206543,0.00467691717402689
70270,70271,70270,140541,2.1713950634002686,0.004633310967836424
70470,70471,70470,140941,2.178497076034546,0.005135959582836533
70671,70672,70671,141343,2.184680938720703,0.004818497442031835
70871,70872,70871,141743,2.190891981124878,0.004537664851487004
71071,71072,71071,142143,2.1971330642700195,0.004478370570521063
71271,71272,71271,142543,2.203507900238037,0.0044380542917019416
71471,71472,71471,142943,2.2098512649536133,0.00550553512503129
71672,71673,71672,143345,2.2163431644439697,0.004418308941482875
71872,71873,71872,143745,2.2228901386260986,0.0044010790322850345
72072,72073,72072,144145,2.2295732498168945,0.004550585163954764
72272,72273,72272,144545,2.2354471683502197,0.004336360023473361
72472,72473,72472,144945,2.2421350479125977,0.004386385452943663
72673,72674,72673,145347,2.2483861446380615,0.004266148950698774
72873,72874,72873,145747,2.2545549869537354,0.004306013271173263
73073,73074,73073,146147,2.260401964187622,0.004368505208174496
73273,73274,73273,146547,2.2671220302581787,0.004220452475308665
73473,73474,73473,146947,2.2731690406799316,0.004232532645310114
73674,73675,73674,147349,2.27935528755188,0.00420454142805173
73874,73875,73874,147749,2.2855072021484375,0.0041778686714670525
74074,74075,74074,148149,2.29158091545105,0.0041492419813747
74274,74275,74274,148549,2.297776937484741,0.0049413642641980594
74474,74475,74474,148949,2.3039159774780273,0.004094237889205395
74675,74676,74675,149351,2.3100149631500244,0.004347989379374318
74875,74876,74875,149751,2.3160719871520996,0.004352237742207087
75075,75076,75075,150151,2.3221099376678467,0.004111572405706692
75275,75276,75275,150551,2.328226089477539,0.004016017647812896
75475,75476,75475,150951,2.3343141078948975,0.003967689654041947
75676,75677,75676,151353,2.340445041656494,0.0039585771005068125
75876,75877,75876,151753,2.3465962409973145,0.004016242266465073
76076,76077,76076,152153,2.3527119159698486,0.003922439245840739
76276,76277,76276,152553,2.3587920665740967,0.0039232251695556376
76476,76477,76476,152953,2.365058183670044,0.003927968373853759
76677,76678,76677,153355,2.37115216255188,0.0039155854501979346
76877,76878,76877,153755,2.377155065536499,0.0038379269602644914
77077,77078,77077,154155,2.3830771446228027,0.004017083666070026
77277,77278,77277,154555,2.388982057571411,0.00380998928413208
77477,77478,77477,154955,2.394925117492676,0.004253593401453428
77678,77679,77678,155357,2.4008991718292236,0.004505435811539767
77878,77879,77878,155757,2.4071109294891357,0.003796784374044313
78078,78079,78078,156157,2.4129929542541504,0.003761760084559125
78278,78279,78278,156557,2.418830156326294,0.003752619746253092
78478,78479,78478,156957,2.4246721267700195,0.004442957393857844
78679,78680,78679,157359,2.4305460453033447,0.0037194109519679826
78879,78880,78879,157759,2.4364190101623535,0.004289927016560843
79079,79080,79079,158159,2.442671060562134,0.0036335026142721603
79279,79280,79279,158559,2.4497642517089844,0.0036619962806652235
79479,79480,79479,158959,2.455785036087036,0.003637455317627421
79680,79681,79680,159361,2.4616808891296387,0.0036215236095768003
79880,79881,79880,159761,2.467574119567871,0.0035811287507339614
80080,80081,80080,160161,2.473362922668457,0.003549600837316861
80280,80281,80280,160561,2.4792211055755615,0.003525268798222221
80480,80481,80480,160961,2.484923839569092,0.003530853858326753
80681,80682,80681,161363,2.4906370639801025,0.0035012477240758816
80881,80882,80881,161763,2.496381998062134,0.0035396966291925324
81081,81082,81081,162163,2.502146005630493,0.0034937515058734423
81281,81282,81281,162563,2.5079381465911865,0.0034794799775795236
81481,81482,81481,162963,2.5136141777038574,0.0034531336162571284
81682,81683,81682,163365,2.51933217048645,0.0035234022151713327
81882,81883,81882,163765,2.525048017501831,0.003391207761783828
82082,82083,82082,164165,2.530730962753296,0.00342141062564471
82282,82283,82282,164565,2.536450147628784,0.0033739122836171555
82482,82483,82482,164965,2.542114019393921,0.003362924229011136
82683,82684,82683,165367,2.547842025756836,0.003337813068802138
82883,82884,82883,165767,2.5535471439361572,0.00333957901680127
83083,83084,83083,166167,2.559235095977783,0.003308847359710524
83283,83284,83283,166567,2.5649170875549316,0.0032614769889697487
83483,83484,83483,166967,2.57066011428833,0.0032901329092645953
83684,83685,83684,167369,2.5762760639190674,0.0032522562928965267
83884,83885,83884,167769,2.5819830894470215,0.003430670210142134
84084,84085,84084,168169,2.587728977203369,0.0032498172627532704
84284,84285,84284,168569,2.5934841632843018,0.0032878764332279478
84484,84485,84484,168969,2.5991880893707275,0.003178506228619986
84685,84686,84685,169371,2.605015993118286,0.0031827645694890837
84885,84886,84885,169771,2.6107521057128906,0.003153012815661423
85085,85086,85085,170171,2.6165740489959717,0.003131743231737187
85285,85286,85285,170571,2.6222851276397705,0.0038548792050088483
85485,85486,85485,170971,2.6281180381774902,0.0031241580021964623
85686,85687,85686,171373,2.6347761154174805,0.00309213250228823
85886,85887,85886,171773,2.640895128250122,0.003653988181409942
86086,86087,86086,172173,2.6471450328826904,0.0030565048907959962
86286,86287,86286,172573,2.6534039974212646,0.0030133734220454582
86486,86487,86486,172973,2.6596450805664062,0.003035299043922183
86687,86688,86687,173375,2.6660962104797363,0.0034117501226775294
86887,86888,86887,173775,2.672119140625,0.0029837631199694696
87087,87088,87087,174175,2.6783318519592285,0.0029793056537222285
87287,87288,87287,174575,2.6846542358398438,0.003472783261981378
87487,87488,87487,174975,2.6917810440063477,0.0034719139830723294
87688,87689,87688,175377,2.6986539363861084,0.0029383688664977115
87888,87889,87888,175777,2.7064080238342285,0.0029286020786804426
88088,88089,88088,176177,2.7125189304351807,0.002890123528292857
88288,88289,88288,176577,2.7185258865356445,0.003254860081970538
88488,88489,88488,176977,2.7245709896087646,0.0028831670632926687
88689,88690,88689,177379,2.730557918548584,0.0028617709267257417
88889,88890,88889,177779,2.736582040786743,0.0028787458454369707
89089,89090,89089,178179,2.7438299655914307,0.002854293197406956
89289,89290,89289,178579,2.7501399517059326,0.0028335521645838557
89489,89490,89489,178979,2.756319046020508,0.0027986226215475658
89690,89691,89690,179381,2.7623910903930664,0.002797017562184415
89890,89891,89890,179781,2.768386125564575,0.0028771675413115853
90090,90091,90090,180181,2.774447202682495,0.0027601793921146586
90290,90291,90290,180581,2.780560255050659,0.0027510336896191382
90490,90491,90490,180981,2.7874722480773926,0.0027328906662145115
90691,90692,90691,181383,2.7946600914001465,0.002765741384548856
90891,90892,90891,181783,2.8012499809265137,0.0027078023550482838
91091,91092,91091,182183,2.808372974395752,0.0026857046355221828
91291,91292,91291,182583,2.8166069984436035,0.0027055606298255503
91491,91492,91491,182983,2.824234962463379,0.0029223895109068325
91692,91693,91692,183385,2.8326730728149414,0.0030508969340298
91892,91893,91892,183785,2.8407440185546875,0.002642757492388949
92092,92093,92092,184185,2.848912239074707,0.002747672159544797
92292,92293,92292,184585,2.8567261695861816,0.002632957874924081
92492,92493,92492,184985,2.8642420768737793,0.002662579054659466
92693,92694,92693,185387,2.8719630241394043,0.002595387658751011
92893,92894,92893,185787,2.8790111541748047,0.002602040684684526
93093,93094,93093,186187,2.8853180408477783,0.002546957466465552
93293,93294,93293,186587,2.891637086868286,0.0025601583943741673
93493,93494,93493,186987,2.898045063018799,0.0025336463686294664
93694,93695,93694,187389,2.904486894607544,0.0025248093091717414
93894,93895,93894,187789,2.9108500480651855,0.0025017686748316716
94094,94095,94094,188189,2.9174411296844482,0.002482368142545164
94294,94295,94294,188589,2.923586130142212,0.002484588387495414
94494,94495,94494,188989,2.9296951293945312,0.002484490234709274
94695,94696,94695,189391,2.9358069896698,0.0024628206096987603
94895,94896,94895,189791,2.9423019886016846,0.002445507890017871
95095,95096,95095,190191,2.949517011642456,0.002421010781207876
95295,95296,95295,190591,2.9557950496673584,0.002797926268710221
95495,95496,95495,190991,2.9620649814605713,0.0024683017547263387
95696,95697,95696,191393,2.968714952468872,0.002819048677648437
95896,95897,95896,191793,2.9756102561950684,0.0023796505504858297
96096,96097,96096,192193,2.982501983642578,0.002366768593489598
96296,96297,96296,192593,2.989962100982666,0.00234162770136808
96496,96497,96496,192993,2.997338056564331,0.0023410311782760284
96697,96698,96697,193395,3.0042402744293213,0.0023317232604085276
96897,96898,96897,193795,3.010906934738159,0.002315832830699188
97097,97098,97097,194195,3.016913890838623,0.0023151788170183716
97297,97298,97297,194595,3.023452043533325,0.002327021936142518
97497,97498,97497,194995,3.0296928882598877,0.002345124183046016
97698,97699,97698,195397,3.0362401008605957,0.002273092235491242
97898,97899,97898,195797,3.0429370403289795,0.0022919999418918166
98098,98099,98098,196197,3.0491230487823486,0.002267009526085826
98298,98299,98298,196597,3.0556600093841553,0.002257641773356471
98498,98499,98498,196997,3.0620250701904297,0.0022360462938346252
98699,98700,98699,197399,3.068444013595581,0.002236744638619309
98899,98900,98899,197799,3.0745880603790283,0.0022276731004945796
99099,99100,99099,198199,3.080963134765625,0.002186273404782907
99299,99300,99299,198599,3.0873401165008545,0.002199848622595925
99499,99500,99499,198999,3.093677043914795,0.002172153627115488
99700,99701,99700,199401,3.0999109745025635,0.0021663422529639357
99900,99901,99900,199801,3.106419086456299,0.0021586298501468882
100100,100101,100100,200201,3.112997055053711,0.0021607337677454173
100300,100301,100300,200601,3.121328830718994,0.0021265191688241984
100501,100502,100501,201003,3.1273579597473145,0.002477897831871667
100701,100702,100701,201403,3.1336541175842285,0.0021588591862794523
100901,100902,100901,201803,3.139907121658325,0.002097600059635112
101101,101102,101101,202203,3.146394968032837,0.0020934499449136437
101301,101302,101301,202603,3.1525208950042725,0.002078212015683252
101502,101503,101502,203005,3.1586930751800537,0.002135682411642782
101702,101703,101702,203405,3.1647841930389404,0.0020467714399281024
101902,101903,101902,203805,3.1708521842956543,0.0020564319544325205
102102,102103,102102,204205,3.176826238632202,0.0020544327762940595
102302,102303,102302,204605,3.1827900409698486,0.002025394241734383
102503,102504,102503,205007,3.188847064971924,0.002013846267478056
102703,102704,102703,205407,3.194821834564209,0.0019795264523525453
102903,102904,102903,205807,3.2008020877838135,0.0020271959647076006
103103,103104,103103,206207,3.2068421840667725,0.0020624523265620727
103303,103304,103303,206607,3.2129290103912354,0.002365685617369958
103504,103505,103504,207009,3.2192740440368652,0.0019512594178104565
103704,103705,103704,207409,3.225306272506714,0.001959356593229385
103904,103905,103904,207809,3.2313220500946045,0.0019266817791848475
104104,104105,104104,208209,3.237375020980835,0.0023203157803093175
104304,104305,104304,208609,3.2437450885772705,0.0024666992166183788
104505,104506,104505,209011,3.249797821044922,0.0019104162862166017
104705,104706,104705,209411,3.2557880878448486,0.0019150513659901653
104905,104906,104905,209811,3.2617599964141846,0.0019035008963317218
105105,105106,105105,210211,3.267735004425049,0.001878819774269109
105305,105306,105305,210611,3.27384090423584,0.0018628549165607459
105506,105507,105506,211013,3.279711961746216,0.0018434927025985327
105706,105707,105706,211413,3.2856481075286865,0.00186391662555715
105906,105907,105906,211813,3.2915608882904053,0.0018314255923566186
106106,106107,106106,212213,3.2972910404205322,0.0018231154342759294
106306,106307,106306,212613,3.3029990196228027,0.0018303941707185757
106507,106508,106507,213015,3.3087520599365234,0.0019020799693027308
106707,106708,106707,213415,3.3144619464874268,0.0018242506477508273
106907,106908,106907,213815,3.3201658725738525,0.0018116413887355855
107107,107108,107107,214215,3.325888156890869,0.001794353317253482
107307,107308,107307,214615,3.331618070602417,0.001770503820076475
107508,107509,107508,215017,3.3373360633850098,0.0017688444047526436
107708,107709,107708,215417,3.3431789875030518,0.0017633297263442487
107908,107909,107908,215817,3.348910093307495,0.00175689116111394
108108,108109,108108,216217,3.354748010635376,0.0017505104472458285
108308,108309,108308,216617,3.360464096069336,0.0017336300323418958
108509,108510,108509,217019,3.3662359714508057,0.0017570439491589017
108709,108710,108709,217419,3.3719420433044434,0.001771568470308674
108909,108910,108909,217819,3.3774871826171875,0.0017184764659409298
109109,109110,109109,218219,3.3831369876861572,0.001690736181115698
109309,109310,109309,218619,3.388843059539795,0.001685560043985458
109510,109511,109510,219021,3.394631862640381,0.0020503060785849563
109710,109711,109710,219421,3.401560068130493,0.0017933072858361137
109910,109911,109910,219821,3.407201051712036,0.0016670729948234423
110110,110111,110110,220221,3.413037061691284,0.0016720652008267666
110310,110311,110310,220621,3.41866397857666,0.0016681153537302523
110511,110512,110511,221023,3.424373149871826,0.0017043666700417043
110711,110712,110711,221423,3.4300100803375244,0.001630730147572345
110911,110912,110911,221823,3.435783863067627,0.0016462189922318785
111111,111112,111111,222223,3.441925048828125,0.0016272382822902238
111311,111312,111311,222623,3.447645902633667,0.001630860545235837
111512,111513,111512,223025,3.453498125076294,0.001973421864346481
111712,111713,111712,223425,3.4594061374664307,0.0016497760140332248
111912,111913,111912,223825,3.465385913848877,0.0016509893443243599
112112,112113,112112,224225,3.471330165863037,0.0015922264368267536
112312,112313,112312,224625,3.4773151874542236,0.001866095632571293
112513,112514,112513,225027,3.483408212661743,0.0015679692610233965
112713,112714,112713,225427,3.49135422706604,0.0015570706777178992
112913,112914,112913,225827,3.497330904006958,0.0017688504923033003
113113,113114,113113,226227,3.503391981124878,0.0015306489640070085
113313,113314,113313,226627,3.509456157684326,0.0018244976674517558
113514,113515,113514,227029,3.5155200958251953,0.0015950948368420189
113714,113715,113714,227429,3.521696090698242,0.001514327481886504
113914,113915,113914,227829,3.527379035949707,0.0015037345010464015
114114,114115,114114,228229,3.5330350399017334,0.0014906765327306873
114314,114315,114314,228629,3.5387442111968994,0.001492603407971611
114515,114516,114515,229031,3.5449442863464355,0.001572575354195766
114715,114716,114715,229431,3.5506060123443604,0.0016918182829638556
114915,114916,114915,229831,3.55627703666687,0.0015894605538221043
115115,115116,115115,230231,3.5619959831237793,0.0014511839250585102
115315,115316,115315,230631,3.5677571296691895,0.0014447147318500412
115516,115517,115516,231033,3.5734710693359375,0.0014290836295854491
115716,115717,115716,231433,3.579155921936035,0.0014220382512299898
115916,115917,115916,231833,3.584869146347046,0.0015123753057512438
116116,116117,116116,232233,3.5907561779022217,0.0014527219363455234
116316,116317,116316,232633,3.5965209007263184,0.0014317939071454746
116517,116518,116517,233035,3.6023061275482178,0.001397616744222485
116717,116718,116717,233435,3.6081840991973877,0.001729923687399927
116917,116918,116917,233835,3.61393404006958,0.0014060680161308318
117117,117118,117117,234235,3.6196930408477783,0.0013829640546094008
117317,117318,117317,234635,3.6254470348358154,0.0013658441305125168
117518,117519,117518,235037,3.63128399848938,0.0013741863874188968
117718,117719,117718,235437,3.6370790004730225,0.0013616081073660167
117918,117919,117918,235837,3.642910957336426,0.0013478107742836423
118118,118119,118118,236237,3.6486852169036865,0.0013481359131859551
118318,118319,118318,236637,3.654442071914673,0.001333985521968418
118519,118520,118519,237039,3.6602728366851807,0.001351580207503543
118719,118720,118719,237439,3.6660261154174805,0.0013623949920032797
118919,118920,118919,237839,3.6717939376831055,0.0016236333137807136
119119,119120,119119,238239,3.677556037902832,0.0013440041576175774
119319,119320,119319,238639,3.683351993560791,0.0013031999390708008
119520,119521,119520,239041,3.689303159713745,0.001299802838990786
119720,119721,119720,239441,3.6947929859161377,0.0012936138090681559
119920,119921,119920,239841,3.700490951538086,0.001280803175899679
120120,120121,120120,240241,3.7061381340026855,0.0012915421528494654
120320,120321,120320,240641,3.711609125137329,0.0015741380128025107
120521,120522,120521,241043,3.7179951667785645,0.0012574759024699162
120721,120722,120721,241443,3.723543167114258,0.0012584205682553118
120921,120922,120921,241843,3.7291011810302734,0.0012628521176559918
121121,121122,121121,242243,3.734652042388916,0.0012605110390395647
121321,121322,121321,242643,3.740784168243408,0.0012520548309660488
121522,121523,121522,243045,3.746443033218384,0.0012370507540522637
121722,121723,121722,243445,3.75209903717041,0.001233221417735528
121922,121923,121922,243845,3.757869005203247,0.0012620581211772945
122122,122123,122122,244245,3.763512134552002,0.001396477825447388
122322,122323,122322,244645,3.769150972366333,0.0012068895063344009
122523,122524,122523,245047,3.7749099731445312,0.0012076667823499904
122723,122724,122723,245447,3.780634880065918,0.0012093911294735976
122923,122924,122923,245847,3.7863521575927734,0.001193351806952085
123123,123124,123123,246247,3.792379856109619,0.0013862279925165386
123323,123324,123323,246647,3.79809308052063,0.001192049627098032
123524,123525,123524,247049,3.8038480281829834,0.0011871920101064234
123724,123725,123724,247449,3.8095500469207764,0.001171623254379103
123924,123925,123924,247849,3.815338134765625,0.0011733665565287024
124124,124125,124124,248249,3.8210980892181396,0.0011496159962049329
124324,124325,124324,248649,3.826862096786499,0.0011759479773421648
124525,124526,124525,249051,3.832611083984375,0.0011452044261821117
124725,124726,124725,249451,3.8383100032806396,0.0011360195480188888
124925,124926,124925,249851,3.8440871238708496,0.0011979675754439376
125125,125126,125125,250251,3.849799871444702,0.0011257432005647137
125325,125326,125325,250651,3.855563163757324,0.0014572170404162624
125526,125527,125526,251053,3.861307144165039,0.0011143353716482124
125726,125727,125726,251453,3.8670551776885986,0.001344827512584897
125926,125927,125926,251853,3.8728342056274414,0.0011916298614509518
126126,126127,126126,252253,3.878615140914917,0.001334492990883916
126326,126327,126326,252653,3.8843789100646973,0.0010970876455032254
126527,126528,126527,253055,3.8901638984680176,0.001087715043927725
126727,126728,126727,253455,3.898062229156494,0.0010786454520220771
126927,126928,126927,253855,3.9039130210876465,0.0010753172322552566
127127,127128,127127,254255,3.909770965576172,0.001080036759620222
127327,127328,127327,254655,3.9154438972473145,0.0010720323463715993
127528,127529,127528,255057,3.921091079711914,0.0010617718705357366
127728,127729,127728,255457,3.926607131958008,0.001064745852923373
127928,127929,127928,255857,3.932122230529785,0.0011163869088877953
128128,128129,128128,256257,3.9377641677856445,0.0011684356160127569
128328,128329,128328,256657,3.9432928562164307,0.0011079505507777484
128529,128530,128529,257059,3.9488840103149414,0.001036137601422121
128729,128730,128729,257459,3.9546561241149902,0.001029208300109196
128929,128930,128929,257859,3.960767984390259,0.0010151670591419212
129129,129130,129129,258259,3.9664809703826904,0.001160114270210304
129329,129330,129329,258659,3.972261905670166,0.0010118230418512438
129530,129531,129530,259061,3.977795124053955,0.0010108026739660723
129730,129731,129730,259461,3.9833080768585205,0.0010040421387750834
129930,129931,129930,259861,3.988878011703491,0.0009964625398363467
130130,130131,130130,260261,3.99446702003479,0.000995443159684135
130330,130331,130330,260661,4.000014066696167,0.0011963462071715252
130531,130532,130531,261063,4.0056610107421875,0.0009893129355422823
130731,130732,130731,261463,4.011348009109497,0.0009740912169129199
130931,130932,130931,261863,4.016903877258301,0.0009832487700799225
131131,131132,131131,262263,4.024167060852051,0.0009675248846267337
131331,131332,131331,262663,4.029836177825928,0.0012085797639784857
131532,131533,131532,263065,4.035996913909912,0.0009561088254208913
131732,131733,131732,263465,4.04387092590332,0.0011324472505581471
131932,131933,131932,263865,4.050867080688477,0.0009488652833244813
132132,132133,132132,264265,4.058872222900391,0.0009416677131564679
132332,132333,132332,264665,4.0671820640563965,0.0010474106550642805
132533,132534,132533,265067,4.074672222137451,0.0009391527990270324
132733,132734,132733,265467,4.081303119659424,0.0009346015618101989
132933,132934,132933,265867,4.087646007537842,0.0009252652448546309
133133,133134,133133,266267,4.094093084335327,0.0009282484550835479
133333,133334,133333,266667,4.100348949432373,0.0009107167911038078
133534,133535,133534,267069,4.1074910163879395,0.0009229251679655787
133734,133735,133734,267469,4.113518238067627,0.0009053848049808773
133934,133935,133934,267869,4.1195409297943115,0.0009046697339533317
134134,134135,134134,268269,4.125558137893677,0.0011015384923384905
134334,134335,134334,268669,4.131557941436768,0.000892351678143847
134535,134536,134535,269071,4.137609004974365,0.0008835631272666769
134735,134736,134735,269471,4.143641233444214,0.0008824844498494463
134935,134936,134935,269871,4.149658203125,0.0008814480288405924
135135,135136,135135,270271,4.15588903427124,0.0008664775752209806
135335,135336,135335,270671,4.162125110626221,0.0011121516441556652
135536,135537,135536,271073,4.168336868286133,0.0008716514274627282
135736,135737,135736,271473,4.174356937408447,0.0008718763087799703
135936,135937,135936,271873,4.1803882122039795,0.0008701320144015297
136136,136137,136136,272273,4.186373233795166,0.0008633270653788447
136336,136337,136336,272673,4.192474126815796,0.0008428195950073837
136537,136538,136537,273075,4.198529005050659,0.0009622815812748764
136737,136738,136737,273475,4.204576015472412,0.0008453180415168806
136937,136938,136937,273875,4.210543155670166,0.0008691796185143435
137137,137138,137137,274275,4.216644048690796,0.0008621890132352567
137337,137338,137337,274675,4.222623109817505,0.0009724587126406361
137538,137539,137538,275077,4.228631019592285,0.0008225407993310344
137738,137739,137738,275477,4.234624147415161,0.0008178716715195934
137938,137939,137938,275877,4.2406580448150635,0.0008719273092150432
138138,138139,138138,276277,4.2466700077056885,0.0008076750692895464
138338,138339,138338,276677,4.252785921096802,0.0008072514943052438
138539,138540,138539,277079,4.259169101715088,0.0008037699328223744
138739,138740,138739,277479,4.265147924423218,0.0007962183868394575
138939,138940,138939,277879,4.2710959911346436,0.0008370568078086618
139139,139140,139139,278279,4.276912212371826,0.000798955002818312
139339,139340,139339,278679,4.2827630043029785,0.0008179378083061257
139540,139541,139540,279081,4.28889012336731,0.0007808744853122916
139740,139741,139740,279481,4.295107126235962,0.0007715505045615191
139940,139941,139940,279881,4.301197052001953,0.0007701095901389206
140140,140141,140140,280281,4.307244062423706,0.0008829414118405274
140340,140341,140340,280681,4.313421010971069,0.0007681930363129683
140541,140542,140541,281083,4.320026874542236,0.0007602449461354242
140741,140742,140741,281483,4.325862884521484,0.0007524530035653965
140941,140942,140941,281883,4.334167003631592,0.0007591521167983261
141141,141142,141141,282283,4.340939044952393,0.0007489894230189703
141341,141342,141341,282683,4.347537040710449,0.0007513495897013959
141542,141543,141542,283085,4.355116128921509,0.0007486385834564896
141742,141743,141742,283485,4.362594127655029,0.0009191136660090752
141942,141943,141942,283885,4.369481086730957,0.0007363847392440774
142142,142143,142142,284285,4.37546706199646,0.0007266661033785641
142342,142343,142342,284685,4.381401062011719,0.0007287518830309675
142543,142544,142543,285087,4.387360095977783,0.000721231495867403
142743,142744,142743,285487,4.39601993560791,0.0007272428029268289
142943,142944,142943,285887,4.4020280838012695,0.0007196440344845118
143143,143144,143143,286287,4.40802788734436,0.0007177238235414018
143343,143344,143343,286687,4.413977146148682,0.0007090762179392175
143544,143545,143544,287089,4.419948101043701,0.0007504219890605997
143744,143745,143744,287489,4.426149845123291,0.0007511017002516375
143944,143945,143944,287889,4.43210506439209,0.0006953815426757991
144144,144145,144144,288289,4.438138246536255,0.0007866793868530316
144344,144345,144344,288689,4.4446611404418945,0.0006941051463635806
144545,144546,144545,289091,4.451077938079834,0.0006886556749827547
144745,144746,144745,289491,4.45818018913269,0.0006930992297283054
144945,144946,144945,289891,4.4647932052612305,0.0007290451122745437
145145,145146,145145,290291,4.47192907333374,0.0006757342744131555
145345,145346,145345,290691,4.478311061859131,0.0006800463279515547
145546,145547,145546,291093,4.484546184539795,0.0006726292077813969
145746,145747,145746,291493,4.490753173828125,0.0006735967903033116
145946,145947,145946,291893,4.496976852416992,0.0006696160115679304
146146,146147,146146,292293,4.503147125244141,0.0006550809927905331
146346,146347,146346,292693,4.509557008743286,0.0006579191183080772
146547,146548,146547,293095,4.515882968902588,0.0007588485683847496
146747,146748,146747,293495,4.522067070007324,0.000654859091435867
146947,146948,146947,293895,4.52822208404541,0.0007626097930480924
147147,147148,147147,294295,4.534364938735962,0.0006539400142594591
147347,147348,147347,294695,4.5405189990997314,0.0006398937594515995
147548,147549,147548,295097,4.546767234802246,0.0006309352394024798
147748,147749,147748,295497,4.552958965301514,0.0006301908264619116
147948,147949,147948,295897,4.559099912643433,0.0006341250734221485
148148,148149,148148,296297,4.565240144729614,0.0007294904541625422
148348,148349,148348,296697,4.571562051773071,0.0006199280915566175
148549,148550,148549,297099,4.577552080154419,0.0006215067286359311
148749,148750,148749,297499,4.583526849746704,0.0006234459301208046
148949,148950,148949,297899,4.589659929275513,0.0006187376467107481
149149,149150,149149,298299,4.59571099281311,0.0007240656962584647
149349,149350,149349,298699,4.601701259613037,0.00063522301640395
149550,149551,149550,299101,4.607801198959351,0.0006084015211351991
149750,149751,149750,299501,4.613699197769165,0.0006300910072013121
149950,149951,149950,299901,4.619568824768066,0.0006000672268320527
150150,150151,150150,300301,4.62552809715271,0.0006053260583021621
150350,150351,150350,300701,4.631399869918823,0.0005989790327182159
150551,150552,150551,301103,4.637290000915527,0.0005889145124479104
150751,150752,150751,301503,4.643148183822632,0.0005919802959962046
150951,150952,150951,301903,4.649040937423706,0.000583767641232543
151151,151152,151151,302303,4.655080080032349,0.0006896638590626267
151351,151352,151351,302703,4.661136865615845,0.0005898321416545478
151552,151553,151552,303105,4.667191028594971,0.0005738304089787259
151752,151753,151752,303505,4.673123121261597,0.0006553232276423368
151952,151953,151952,303905,4.678899049758911,0.0005689630868226012
152152,152153,152152,304305,4.68464994430542,0.000616742827320846
152352,152353,152352,304705,4.690564155578613,0.0005695178016930882
152553,152554,152553,305107,4.697937965393066,0.0005579720652972241
152753,152754,152753,305507,4.704041004180908,0.0005609425282615424
152953,152954,152953,305907,4.710277080535889,0.000556402154053537
153153,153154,153153,306307,4.716645240783691,0.0005649123186464199
153353,153354,153353,306707,4.72368597984314,0.0005497716367166829
153554,153555,153554,307109,4.730372190475464,0.0005478378911291875
153754,153755,153754,307509,4.736592054367065,0.0006257059473216982
153954,153955,153954,307909,4.742831230163574,0.0006138146603546427
154154,154155,154154,308309,4.750833988189697,0.0005549644384654061
154354,154355,154354,308709,4.75726318359375,0.0005435916514393337
154555,154556,154555,309111,4.763485908508301,0.0005348504324938715
154755,154756,154755,309511,4.770111083984375,0.0005411296592752773
154955,154956,154955,309911,4.776684045791626,0.0005279530502752121
155155,155156,155155,310311,4.784116983413696,0.000523160911245305
155355,155356,155355,310711,4.791898965835571,0.0005206017490215979
155556,155557,155556,311113,4.799359083175659,0.0005175400273136614
155756,155757,155756,311513,4.805708169937134,0.0005187604407791742
155956,155957,155956,311913,4.811750888824463,0.0005205375817327428
156156,156157,156156,312313,4.818008184432983,0.0005434485371678235
156356,156357,156356,312713,4.82404899597168,0.000514362858967838
156557,156558,156557,313115,4.83056902885437,0.000531503515378153
156757,156758,156757,313515,4.836606025695801,0.00057676372530731
156957,156958,156957,313915,4.843160152435303,0.0005039868974430141
157157,157158,157157,314315,4.849131107330322,0.0005012883830006463
157357,157358,157357,314715,4.85510516166687,0.0005928086847497647
157558,157559,157558,315117,4.861465215682983,0.0004978901243677881
157758,157759,157758,315517,4.867424011230469,0.0004908455438178869
157958,157959,157958,315917,4.873827219009399,0.0004901962280133639
158158,158159,158158,316317,4.879883050918579,0.0004846508601206442
158358,158359,158358,316717,4.885889053344727,0.0004855767662551454
158559,158560,158559,317119,4.892207145690918,0.00048366702073812933
158759,158760,158759,317519,4.898288249969482,0.0004794584849106455
158959,158960,158959,317919,4.904277086257935,0.0004761610829343989
159159,159160,159159,318319,4.910499095916748,0.0004748427246493994
159359,159360,159359,318719,4.916738033294678,0.0004718117556958178
159560,159561,159560,319121,4.922813892364502,0.000464894777586666
159760,159761,159760,319521,4.9287049770355225,0.0004678210733110973
159960,159961,159960,319921,4.934571981430054,0.0004809036131793822
160160,160161,160160,320321,4.940781116485596,0.00047188082456982056
160360,160361,160360,320721,4.946885108947754,0.00046582920277660504
160561,160562,160561,321123,4.956192970275879,0.00045901124193607046
160761,160762,160761,321523,4.962559938430786,0.00045460726639254745
160961,160962,160961,321923,4.96855616569519,0.00045444083074762414
161161,161162,161161,322323,4.974496126174927,0.00045391411570882493
161361,161362,161361,322723,4.980443954467773,0.00045258913913899995
161562,161563,161562,323125,4.986407995223999,0.0004442577053349836
161762,161763,161762,323525,4.99234414100647,0.00044226038666085864
161962,161963,161962,323925,4.9983720779418945,0.00048539236280799883
162162,162163,162162,324325,5.004338026046753,0.000545605697776332
162362,162363,162362,324725,5.010426044464111,0.00044052363286115845
162563,162564,162563,325127,5.016526222229004,0.0005304419123240473
162763,162764,162763,325527,5.022649049758911,0.0005014111847095812
162963,162964,162963,325927,5.02888298034668,0.00043146831832868883
163163,163164,163163,326327,5.035049915313721,0.00042593209832637305
163363,163364,163363,326727,5.041283130645752,0.0004243638517011122
163564,163565,163564,327129,5.047581911087036,0.0004248246144064964
163764,163765,163764,327529,5.054059028625488,0.00042310731021801484
163964,163965,163964,327929,5.060664176940918,0.0004188423977482823
164164,164165,164164,328329,5.066979169845581,0.0004191934786234894
164364,164365,164364,328729,5.073336124420166,0.000416931293971408
164565,164566,164565,329131,5.079945087432861,0.0004134096319817943
164765,164766,164765,329531,5.086087942123413,0.0004072371329818886
164965,164966,164965,329931,5.092339992523193,0.00040694825483742874
165165,165166,165165,330331,5.098221063613892,0.00040675735506080606
165365,165366,165365,330731,5.104362964630127,0.000434841169707032
165566,165567,165566,331133,5.110666036605835,0.0004005913771831611
165766,165767,165766,331533,5.116876125335693,0.0004018425750016604
165966,165967,165966,331933,5.1231749057769775,0.0004274617659233051
166166,166167,166166,332333,5.129440069198608,0.0003960376922236419
166366,166367,166366,332733,5.1357262134552,0.00039738053076470673
166567,166568,166567,333135,5.141992092132568,0.0003953172411127106
166767,166768,166767,333535,5.147974014282227,0.00038838694427199095
166967,166968,166967,333935,5.15397310256958,0.00039058822737542066
167167,167168,167167,334335,5.159934043884277,0.0003845160311542035
167367,167368,167367,334735,5.165893077850342,0.0003943911909553938
167568,167569,167568,335137,5.17189621925354,0.00043361647743507
167768,167769,167768,335537,5.177868127822876,0.0004854314432980932
167968,167969,167968,335937,5.183833122253418,0.0003792898388876672
168168,168169,168168,336337,5.189929008483887,0.000388295054301492
168368,168369,168368,336737,5.196310997009277,0.00046268618192321545
168569,168570,168569,337139,5.20226788520813,0.00036954529346390914
168769,168770,168769,337539,5.208165884017944,0.00037281932380677223
168969,168970,168969,337939,5.214069128036499,0.0003714898094938882
169169,169170,169169,338339,5.219969987869263,0.0003673734146756985
169369,169370,169369,338739,5.2260191440582275,0.0003695138056925279
169570,169571,169570,339141,5.231956958770752,0.00036386070551619904
169770,169771,169770,339541,5.238887071609497,0.0003597263154288514
169970,169971,169970,339941,5.2451090812683105,0.0003637617085146127
170170,170171,170170,340341,5.251421928405762,0.00035672227513760613
170370,170371,170370,340741,5.257649898529053,0.0003549410851476745
170571,170572,170571,341143,5.264033079147339,0.0003557734288630801
170771,170772,170771,341543,5.270365953445435,0.00036003794816088917
170971,170972,170971,341943,5.276633024215698,0.00036259572969769973
171171,171172,171171,342343,5.282819032669067,0.00043387044140503496
171371,171372,171371,342743,5.2891130447387695,0.0003526685205801025
171572,171573,171572,343145,5.295519113540649,0.0003542319320621289
171772,171773,171772,343545,5.3015429973602295,0.0003477255963992194
171972,171973,171972,343945,5.3077099323272705,0.0003639883817650026
172172,172173,172172,344345,5.3138439655303955,0.0003903290118092034
172372,172373,172372,344745,5.319900035858154,0.000338185814128999
172573,172574,172573,345147,5.325945138931274,0.00035036308243509707
172773,172774,172773,345547,5.332123041152954,0.0003352636019525433
172973,172974,172973,345947,5.337990045547485,0.0003353930970071596
173173,173174,173173,346347,5.3438720703125,0.00039730535750351245
173373,173374,173373,346747,5.349778890609741,0.0003336561320582976
173574,173575,173574,347149,5.355725049972534,0.0003953041197756024
173774,173775,173774,347549,5.361598014831543,0.00032699604239713856
173974,173975,173974,347949,5.367469072341919,0.00032448678119324
174174,174175,174174,348349,5.373390197753906,0.00032240336553091947
174374,174375,174374,348749,5.37935996055603,0.0003218876315850002
174575,174576,174575,349151,5.385490894317627,0.00031892126444114043
174775,174776,174775,349551,5.391595125198364,0.00031780933279829007
174975,174976,174975,349951,5.397444248199463,0.00031767658614543034
175175,175176,175175,350351,5.403226137161255,0.0003170290253647121
175375,175376,175375,350751,5.409119129180908,0.00031574794127072945
175576,175577,175576,351153,5.414889097213745,0.000313341181104001
175776,175777,175776,351553,5.420750141143799,0.0003112425959706701
175976,175977,175976,351953,5.426484107971191,0.0003089204095466061
176176,176177,176176,352353,5.432289123535156,0.0003602665614480855
176376,176377,176376,352753,5.438261032104492,0.0003847424523713432
176577,176578,176577,353155,5.444620132446289,0.0003026051251339166
176777,176778,176777,353555,5.450724124908447,0.00030218129240591095
176977,176978,176977,353955,5.456570148468018,0.0003868828761804963
177177,177178,177177,354355,5.462739944458008,0.0003286602758874009
177377,177378,177377,354755,5.4686689376831055,0.00029683848061824513
177578,177579,177578,355157,5.474549055099487,0.0003381156672813502
177778,177779,177778,355557,5.480371952056885,0.00029485843449589375
177978,177979,177978,355957,5.486234188079834,0.0002959516010246236
178178,178179,178178,356357,5.4921650886535645,0.00029379591406455735
178378,178379,178378,356757,5.498064279556274,0.00033033504433212956
178579,178580,178579,357159,5.504678964614868,0.0002940531678635279
178779,178780,178779,357559,5.510596036911011,0.0002883188176822511
178979,178980,178979,357959,5.516426086425781,0.0003401817459499014
179179,179180,179179,358359,5.523452997207642,0.00028767645134080956
179379,179380,179379,358759,5.529356002807617,0.0002841154628224168
179580,179581,179580,359161,5.535557985305786,0.00028273230785779666
179780,179781,179780,359561,5.541690111160278,0.0002813915890793804
179980,179981,179980,359961,5.547508001327515,0.000292933446136171
180180,180181,180180,360361,5.553593158721924,0.000279122320265064
180380,180381,180380,360761,5.5601890087127686,0.00029625684403312454
180581,180582,180581,361163,5.568521022796631,0.00027568675540764185
180781,180782,180781,361563,5.5745580196380615,0.00027311049069369956
180981,180982,180981,361963,5.580512046813965,0.0002724797902356959
181181,181182,181181,362363,5.586742162704468,0.0003110329297033935
181381,181382,181381,362763,5.592849969863892,0.00026923465257679374
181582,181583,181582,363165,5.598818063735962,0.0002875842521175985
181782,181783,181782,363565,5.604816913604736,0.00030832610270207193
181982,181983,181982,363965,5.61084508895874,0.0003021819723720803
182182,182183,182182,364365,5.616818904876709,0.00027387796156166277
182382,182383,182382,364765,5.622966051101685,0.00027520710625293817
182583,182584,182583,365167,5.629870176315308,0.0002585944338142107
182783,182784,182783,365567,5.63630485534668,0.00026409072355995986
182983,182984,182983,365967,5.642567873001099,0.0002593932311743648
183183,183184,183183,366367,5.648600101470947,0.00030421101746746306
183383,183384,183383,366767,5.654539108276367,0.0002548493891848503
183584,183585,183584,367169,5.660656929016113,0.0002557005498134259
183784,183785,183784,367569,5.6666481494903564,0.0002661511832057892
183984,183985,183984,367969,5.6726861000061035,0.00025127229110594683
184184,184185,184184,368369,5.678584098815918,0.00025066394799333307
184384,184385,184384,368769,5.684732913970947,0.0002482721286143449
184585,184586,184585,369171,5.690938234329224,0.0002480101237386213
184785,184786,184785,369571,5.697250127792358,0.00024531213783366015
184985,184986,184985,369971,5.7031848430633545,0.00024512924252334046
185185,185186,185185,370371,5.7093939781188965,0.00024357394991545757
185385,185386,185385,370771,5.715309143066406,0.00024182026139709983
185586,185587,185586,371173,5.721649885177612,0.00025008617682130885
185786,185787,185786,371573,5.7278220653533936,0.00029011158199657183
185986,185987,185986,371973,5.734095096588135,0.00027486539654629667
186186,186187,186186,372373,5.740170001983643,0.0002384808034714095
186386,186387,186386,372773,5.7470619678497314,0.00023471671119783806
186587,186588,186587,373175,5.753270149230957,0.0002745534899662632
186787,186788,186787,373575,5.75948691368103,0.0002335043870584064
186987,186988,186987,373975,5.765733957290649,0.0002672833787622686
187187,187188,187187,374375,5.77222204208374,0.0002729668310545426
187387,187388,187387,374775,5.7784881591796875,0.00023221335571923073
187588,187589,187588,375177,5.784893989562988,0.00023113189685331054
187788,187789,187788,375577,5.7915730476379395,0.00022854059922586156
187988,187989,187988,375977,5.797904968261719,0.00022714517783529927
188188,188189,188188,376377,5.804168939590454,0.00027250520513978226
188388,188389,188388,376777,5.8103320598602295,0.00022363630717678538
188589,188590,188589,377179,5.817324161529541,0.0002262462250111337
188789,188790,188789,377579,5.82368803024292,0.00022363248477573375
188989,188990,188989,377979,5.830142021179199,0.00022172403201245187
189189,189190,189189,378379,5.8369081020355225,0.00021977923851245195
189389,189390,189389,378779,5.843222141265869,0.00025900164191725033
189590,189591,189590,379181,5.849500894546509,0.000228038030296149
189790,189791,189790,379581,5.855754137039185,0.0002167964599494826
189990,189991,189990,379981,5.861678123474121,0.00021501620074210377
190190,190191,190190,380381,5.867967128753662,0.00021694122131495864
190390,190391,190390,380781,5.874185085296631,0.0002120389590269198
190591,190592,190591,381183,5.8803629875183105,0.00029827212924373115
190791,190792,190791,381583,5.886468172073364,0.00021094661318686933
190991,190992,190991,381983,5.892568111419678,0.00021161005061647844
191191,191192,191191,382383,5.898640155792236,0.00021767600259413612
191391,191392,191391,382783,5.9046831130981445,0.00020912774266787623
191592,191593,191592,383185,5.910820245742798,0.00020745164122263843
191792,191793,191792,383585,5.916913986206055,0.00025870781041512607
191992,191993,191992,383985,5.922997951507568,0.0002040953535588511
192192,192193,192192,384385,5.929072856903076,0.0002062000658832997
192392,192393,192392,384785,5.935148000717163,0.00020395440604012034
192593,192594,192593,385187,5.941354036331177,0.00020086218581682626
192793,192794,192793,385587,5.947381973266602,0.00020051696255671272
192993,192994,192993,385987,5.953437089920044,0.00023976091373831225
193193,193194,193193,386387,5.95947003364563,0.00019963382807135316
193393,193394,193393,386787,5.965485095977783,0.00020119134891362798
193594,193595,193594,387189,5.971453905105591,0.00022944715013016178
193794,193795,193794,387589,5.977291107177734,0.00020197763413767192
193994,193995,193994,387989,5.983159065246582,0.0001944407344532303
194194,194195,194194,388389,5.988994121551514,0.00019336009155058683
194394,194395,194394,388789,5.99533486366272,0.00019279448643281675
194595,194596,194595,389191,6.001224994659424,0.00019022000634029974
194795,194796,194795,389591,6.007076025009155,0.00019256913859278893
194995,194996,194995,389991,6.012937068939209,0.00018934059880832842
195195,195196,195195,390391,6.019092082977295,0.0001884795232287495
195395,195396,195395,390791,6.025193929672241,0.00018597517864970165
195596,195597,195596,391193,6.031227111816406,0.00021023132681399247
195796,195797,195796,391593,6.037191867828369,0.00018585019699536958
195996,195997,195996,391993,6.043178081512451,0.00018461738845802867
196196,196197,196196,392393,6.049242258071899,0.0001827993903157307
196396,196397,196396,392793,6.055253982543945,0.00018326277535487675
196597,196598,196597,393195,6.061342000961304,0.00018275301994597515
196797,196798,196797,393595,6.068274974822998,0.00018143382325329667
196997,196998,196997,393995,6.075947999954224,0.00018059143169079893
197197,197198,197197,394395,6.084223031997681,0.000181073413260446
197397,197398,197397,394795,6.092506170272827,0.00017729309811006128
197598,197599,197598,395197,6.100609064102173,0.0001757924055001007
197798,197799,197798,395597,6.108780145645142,0.00021093220848104804
197998,197999,197998,395997,6.1170759201049805,0.00017556605811814644
198198,198199,198198,396397,6.125242233276367,0.00017340960413312844
198398,198399,198398,396797,6.1336400508880615,0.00017251911235031944
198599,198600,198599,397199,6.142135143280029,0.00017324527596625252
198799,198800,198799,397599,6.15003228187561,0.00017514524245488788
198999,199000,198999,397999,6.157486200332642,0.00020136233979246203
199199,199200,199199,398399,6.164865016937256,0.00017015670715026703
199399,199400,199399,398799,6.1718809604644775,0.0001708085984260323
199600,199601,199600,399201,6.177896976470947,0.00016842327097694456
199800,199801,199800,399601,6.183763027191162,0.00016932244511551553
200000,200001,200000,400001,6.189651966094971,0.00020154354922429128


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha0/eag-c.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,8.20159912109375e-05,4.387061074692293
100,201,0,201,0.0046558380126953125,1.0673545918633924
200,401,0,401,0.010454177856445312,0.4049021910637366
300,601,0,601,0.015111923217773438,0.3042707958389895
400,801,0,801,0.01993393898010254,0.21271367149175655
501,1003,0,1003,0.024610042572021484,0.1717728895974256
601,1203,0,1203,0.030383825302124023,0.14972243764114768
701,1403,0,1403,0.03548598289489746,0.1217329166933894
801,1603,0,1603,0.04034686088562012,0.10203790309631597
901,1803,0,1803,0.04562997817993164,0.08933779537451116
1001,2003,0,2003,0.050582170486450195,0.08265066885959595
1101,2203,0,2203,0.05531191825866699,0.08230505365279778
1201,2403,0,2403,0.0604090690612793,0.06176758946000925
1301,2603,0,2603,0.06524300575256348,0.0695209338266348
1401,2803,0,2803,0.06975412368774414,0.0589485050023372
1502,3005,0,3005,0.0746009349822998,0.0627481296261858
1602,3205,0,3205,0.07983589172363281,0.05293675918341365
1702,3405,0,3405,0.0847630500793457,0.04722635532851449
1802,3605,0,3605,0.09051108360290527,0.05093361305164786
1902,3805,0,3805,0.09790396690368652,0.04504451194371095
2002,4005,0,4005,0.1035451889038086,0.04177796728718847
2102,4205,0,4205,0.10905718803405762,0.04067682130710717
2202,4405,0,4405,0.11379504203796387,0.03842459003575901
2302,4605,0,4605,0.11889314651489258,0.04007450093735216
2402,4805,0,4805,0.12466907501220703,0.03627332959248263
2503,5007,0,5007,0.12936615943908691,0.034346849076908
2603,5207,0,5207,0.13394403457641602,0.03365380370352932
2703,5407,0,5407,0.1384119987487793,0.03299723751354892
2803,5607,0,5607,0.1430220603942871,0.03135474476718378
2903,5807,0,5807,0.14801788330078125,0.026535319435883005
3003,6007,0,6007,0.15320706367492676,0.029390797885835523
3103,6207,0,6207,0.15788006782531738,0.02612188985375729
3203,6407,0,6407,0.1625521183013916,0.02748500625159133
3303,6607,0,6607,0.16750383377075195,0.02424581732098491
3403,6807,0,6807,0.17211008071899414,0.024008143925917536
3504,7009,0,7009,0.17679119110107422,0.025162460325511227
3604,7209,0,7209,0.18116092681884766,0.022578718206167147
3704,7409,0,7409,0.18564891815185547,0.021494259299025112
3804,7609,0,7609,0.190155029296875,0.02043875890666776
3904,7809,0,7809,0.19461607933044434,0.01987993616688908
4004,8009,0,8009,0.19915127754211426,0.02015308122435684
4104,8209,0,8209,0.2035839557647705,0.017455340496693332
4204,8409,0,8409,0.20844221115112305,0.018193517796546033
4304,8609,0,8609,0.21246004104614258,0.017525793056724182
4404,8809,0,8809,0.21614694595336914,0.018550087622006765
4505,9011,0,9011,0.21981215476989746,0.016164363810323944
4605,9211,0,9211,0.22364401817321777,0.01611030940457769
4705,9411,0,9411,0.22757816314697266,0.01611548503031052
4805,9611,0,9611,0.2311859130859375,0.01538845563391613
4905,9811,0,9811,0.2348320484161377,0.014905501717866506
5005,10011,0,10011,0.2384331226348877,0.01366056757129582
5105,10211,0,10211,0.24202609062194824,0.014068546361759207
5205,10411,0,10411,0.24564719200134277,0.014925184532832122
5305,10611,0,10611,0.24953413009643555,0.013640662268505044
5405,10811,0,10811,0.2531242370605469,0.01386276237210343
5506,11013,0,11013,0.2567439079284668,0.013639937871897831
5606,11213,0,11213,0.26033592224121094,0.014041214092744102
5706,11413,0,11413,0.2639482021331787,0.013441807764246163
5806,11613,0,11613,0.26752686500549316,0.012562686014286216
5906,11813,0,11813,0.27134013175964355,0.012706676435404613
6006,12013,0,12013,0.2749161720275879,0.012894773898899512
6106,12213,0,12213,0.2784910202026367,0.012936444587394073
6206,12413,0,12413,0.2820770740509033,0.012225834205619113
6306,12613,0,12613,0.28563785552978516,0.012636036977946803
6406,12813,0,12813,0.28920912742614746,0.013037047529582194
6507,13015,0,13015,0.29280900955200195,0.012716971695537092
6607,13215,0,13215,0.2963690757751465,0.012510088247604023
6707,13415,0,13415,0.3000919818878174,0.01191296661983371
6807,13615,0,13615,0.3036532402038574,0.01228381496683447
6907,13815,0,13815,0.30721521377563477,0.012154934084562058
7007,14015,0,14015,0.3107719421386719,0.01143366202513963
7107,14215,0,14215,0.31433606147766113,0.011593119488544449
7207,14415,0,14415,0.31784605979919434,0.0116494057725054
7307,14615,0,14615,0.3213231563568115,0.011910279317454647
7407,14815,0,14815,0.3248021602630615,0.011463874642140671
7508,15017,0,15017,0.3284599781036377,0.011237794855793343
7608,15217,0,15217,0.33194494247436523,0.011236355233733394
7708,15417,0,15417,0.3354299068450928,0.011160862470629666
7808,15617,0,15617,0.3388960361480713,0.010678561032865207
7908,15817,0,15817,0.34237003326416016,0.01012244253562772
8008,16017,0,16017,0.34584712982177734,0.010267321945978992
8108,16217,0,16217,0.3493199348449707,0.010258392149599074
8208,16417,0,16417,0.3528120517730713,0.009970428254309695
8308,16617,0,16617,0.3562769889831543,0.009805773793440862
8408,16817,0,16817,0.35987210273742676,0.009612290022200577
8509,17019,0,17019,0.36338114738464355,0.009843928341412143
8609,17219,0,17219,0.36684703826904297,0.009394042355870174
8709,17419,0,17419,0.37032413482666016,0.00887133103669788
8809,17619,0,17619,0.37380099296569824,0.008724093024721866
8909,17819,0,17819,0.37726712226867676,0.008641432623350877
9009,18019,0,18019,0.38073301315307617,0.008447788572745304
9109,18219,0,18219,0.3843100070953369,0.00807796240372097
9209,18419,0,18419,0.3878591060638428,0.00802890122705077
9309,18619,0,18619,0.3914680480957031,0.008202690218464951
9409,18819,0,18819,0.39497923851013184,0.008147570997580322
9510,19021,0,19021,0.3985931873321533,0.007813795330105162
9610,19221,0,19221,0.40212416648864746,0.0075448511345763206
9710,19421,0,19421,0.4056510925292969,0.007657580682796772
9810,19621,0,19621,0.40918612480163574,0.007423646563510711
9910,19821,0,19821,0.41271209716796875,0.007125141438191955
10010,20021,0,20021,0.4161369800567627,0.006979110647953697
10110,20221,0,20221,0.41951704025268555,0.007072047529712677
10210,20421,0,20421,0.42281508445739746,0.007306044548107694
10310,20621,0,20621,0.4261031150817871,0.007122484668401108
10410,20821,0,20821,0.43041110038757324,0.007054476557523793
10511,21023,0,21023,0.43421101570129395,0.007197522422412029
10611,21223,0,21223,0.43970799446105957,0.007217110692236581
10711,21423,0,21423,0.44394803047180176,0.007034724766388607
10811,21623,0,21623,0.44763708114624023,0.006801956835663474
10911,21823,0,21823,0.452099084854126,0.006853774568441507
11011,22023,0,22023,0.4561789035797119,0.0069720348285935785
11111,22223,0,22223,0.4595949649810791,0.006963776379840413
11211,22423,0,22423,0.46294617652893066,0.00688826026740812
11311,22623,0,22623,0.4663100242614746,0.00701225189075417
11411,22823,0,22823,0.46984410285949707,0.007227540837921803
11512,23025,0,23025,0.4733011722564697,0.0071371224056349675
11612,23225,0,23225,0.4767942428588867,0.007007994851043972
11712,23425,0,23425,0.48030710220336914,0.006932453786308687
11812,23625,0,23625,0.4838709831237793,0.006963093971099112
11912,23825,0,23825,0.4876730442047119,0.006931159863468218
12012,24025,0,24025,0.4912550449371338,0.006748001210483645
12112,24225,0,24225,0.4946420192718506,0.0067614090825382014
12212,24425,0,24425,0.4989020824432373,0.0069063461046462655
12312,24625,0,24625,0.5027320384979248,0.006933862111952244
12412,24825,0,24825,0.506472110748291,0.006831744835719266
12513,25027,0,25027,0.5100760459899902,0.006736872446141184
12613,25227,0,25227,0.5136499404907227,0.006740973300526169
12713,25427,0,25427,0.5182862281799316,0.006652254223970815
12813,25627,0,25627,0.5219011306762695,0.006446150083099497
12913,25827,0,25827,0.5254449844360352,0.006256808269584062
13013,26027,0,26027,0.5289821624755859,0.006266652863865043
13113,26227,0,26227,0.5325100421905518,0.006284665353945361
13213,26427,0,26427,0.5363509654998779,0.006161205162714325
13313,26627,0,26627,0.5398960113525391,0.006084193536884966
13413,26827,0,26827,0.5434141159057617,0.006070544577842459
13514,27029,0,27029,0.5471451282501221,0.006049756629090452
13614,27229,0,27229,0.5507619380950928,0.005883855083628956
13714,27429,0,27429,0.5542910099029541,0.005630819649733052
13814,27629,0,27629,0.5578229427337646,0.005534136269399937
13914,27829,0,27829,0.561378002166748,0.005484136694319016
14014,28029,0,28029,0.5649011135101318,0.005359328750633811
14114,28229,0,28229,0.568479061126709,0.005226611260802524
14214,28429,0,28429,0.572045087814331,0.005221411119496696
14314,28629,0,28629,0.575645923614502,0.005284486990020055
14414,28829,0,28829,0.5791559219360352,0.005238478021754753
14515,29031,0,29031,0.5826930999755859,0.005094542465507088
14615,29231,0,29231,0.5862460136413574,0.004986087068140045
14715,29431,0,29431,0.5897510051727295,0.004970757367798045
14815,29631,0,29631,0.5932741165161133,0.0048753573432271475
14915,29831,0,29831,0.5969328880310059,0.0047153357472845365
15015,30031,0,30031,0.6004810333251953,0.004681158358388621
15115,30231,0,30231,0.6039800643920898,0.004753516654410479
15215,30431,0,30431,0.607867956161499,0.004824672478728818
15315,30631,0,30631,0.6113669872283936,0.004803612360299999
15415,30831,0,30831,0.6151151657104492,0.004785380106719047
15516,31033,0,31033,0.6187341213226318,0.004852157638110348
15616,31233,0,31233,0.6221351623535156,0.004856474899261709
15716,31433,0,31433,0.6255390644073486,0.004759914324156903
15816,31633,0,31633,0.6289422512054443,0.00467911114166003
15916,31833,0,31833,0.6323671340942383,0.004710220906360681
16016,32033,0,32033,0.6371688842773438,0.004771719012250733
16116,32233,0,32233,0.6427431106567383,0.004783929100922037
16216,32433,0,32433,0.6463611125946045,0.00479909611065722
16316,32633,0,32633,0.6498630046844482,0.00488299111987913
16416,32833,0,32833,0.6537039279937744,0.0049767506537911725
16517,33035,0,33035,0.6573150157928467,0.0049572996567738255
16617,33235,0,33235,0.6608982086181641,0.004886877152238715
16717,33435,0,33435,0.6643378734588623,0.004869768005565191
16817,33635,0,33635,0.6678421497344971,0.004871100810860564
16917,33835,0,33835,0.672476053237915,0.004841582355329571
17017,34035,0,34035,0.6767139434814453,0.004788829128157551
17117,34235,0,34235,0.681481122970581,0.004806423949449826
17217,34435,0,34435,0.6853160858154297,0.004882998782845022
17317,34635,0,34635,0.6897449493408203,0.004901780150849659
17417,34835,0,34835,0.6946251392364502,0.004855225454750469
17518,35037,0,35037,0.6992430686950684,0.004816319531499973
17618,35237,0,35237,0.7039849758148193,0.004797525307041281
17718,35437,0,35437,0.7088472843170166,0.004730441596576756
17818,35637,0,35637,0.713468074798584,0.004613402370356125
17918,35837,0,35837,0.7179470062255859,0.004527855825744497
18018,36037,0,36037,0.7225990295410156,0.004516580614556767
18118,36237,0,36237,0.7273080348968506,0.0045147033825063965
18218,36437,0,36437,0.7318761348724365,0.004461157724276734
18318,36637,0,36637,0.7363431453704834,0.0044181650949096886
18418,36837,0,36837,0.7409069538116455,0.004410184870183538
18519,37039,0,37039,0.745373010635376,0.004368532686871857
18619,37239,0,37239,0.7493700981140137,0.0042590714074018056
18719,37439,0,37439,0.7533791065216064,0.004126576417163519
18819,37639,0,37639,0.7572841644287109,0.004049446008025196
18919,37839,0,37839,0.7610828876495361,0.004002818432140154
19019,38039,0,38039,0.764815092086792,0.003928673885354569
19119,38239,0,38239,0.7684831619262695,0.00386619047830315
19219,38439,0,38439,0.7726211547851562,0.00386803342265996
19319,38639,0,38639,0.7762649059295654,0.003889534286485661
19419,38839,0,38839,0.779853105545044,0.003854552340424131
19520,39041,0,39041,0.7835211753845215,0.003775596866220422
19620,39241,0,39241,0.7871758937835693,0.0037153477204209524
19720,39441,0,39441,0.7907800674438477,0.003678904356854645
19820,39641,0,39641,0.7943990230560303,0.003616669886075913
19920,39841,0,39841,0.7979919910430908,0.0035381985450971707
20020,40041,0,40041,0.8015921115875244,0.003526437686351484
20120,40241,0,40241,0.8051819801330566,0.003575674516521372
20220,40441,0,40441,0.8088772296905518,0.0036133678409468843
20320,40641,0,40641,0.8125109672546387,0.0036186268317476857
20420,40841,0,40841,0.8161280155181885,0.003627340671491457
20521,41043,0,41043,0.8197300434112549,0.003656158071737758
20621,41243,0,41243,0.8235070705413818,0.003653164365296124
20721,41443,0,41443,0.8278841972351074,0.003602992153220731
20821,41643,0,41643,0.8314781188964844,0.003569686309565726
20921,41843,0,41843,0.8351991176605225,0.0035921667269177902
21021,42043,0,42043,0.8388440608978271,0.003631074678563314
21121,42243,0,42243,0.84328293800354,0.0036535544170685896
21221,42443,0,42443,0.8468780517578125,0.003686664727612707
21321,42643,0,42643,0.850776195526123,0.0037470837426399127
21421,42843,0,42843,0.8544168472290039,0.0037963152073887817
21522,43045,0,43045,0.8595478534698486,0.00379166801913963
21622,43245,0,43245,0.8637840747833252,0.0037589148665859804
21722,43445,0,43445,0.8679649829864502,0.0037478345902089353
21822,43645,0,43645,0.8723700046539307,0.003745491355419233
21922,43845,0,43845,0.8776042461395264,0.003726830686026307
22022,44045,0,44045,0.8819730281829834,0.0037120395408280107
22122,44245,0,44245,0.8863308429718018,0.003733454809577551
22222,44445,0,44445,0.8907780647277832,0.0037757134425443414
22322,44645,0,44645,0.8952891826629639,0.0037885982486271655
22422,44845,0,44845,0.8994729518890381,0.003766394419145786
22523,45047,0,45047,0.9033010005950928,0.0037422645456167036
22623,45247,0,45247,0.9070920944213867,0.0037181432689013046
22723,45447,0,45447,0.9110012054443359,0.003665817263423618
22823,45647,0,45647,0.9146749973297119,0.0035931714449502408
22923,45847,0,45847,0.9183430671691895,0.0035439321086579508
23023,46047,0,46047,0.9224488735198975,0.00353070734188824
23123,46247,0,46247,0.9265532493591309,0.0035213418232610933
23223,46447,0,46447,0.9308590888977051,0.0034937777095578573
23323,46647,0,46647,0.9349651336669922,0.003468387443767022
23423,46847,0,46847,0.9393291473388672,0.00345312519873274
23524,47049,0,47049,0.9433281421661377,0.0034126824227102186
23624,47249,0,47249,0.947066068649292,0.0033339798472745608
23724,47449,0,47449,0.9506881237030029,0.0032494506430725766
23824,47649,0,47649,0.9543271064758301,0.003190818179037223
23924,47849,0,47849,0.9579782485961914,0.00314816800225836
24024,48049,0,48049,0.9617102146148682,0.003101494128553399
24124,48249,0,48249,0.9653260707855225,0.0030686659149796983
24224,48449,0,48449,0.9689531326293945,0.0030686960000341702
24324,48649,0,48649,0.972559928894043,0.003073462535060667
24424,48849,0,48849,0.9766771793365479,0.0030464672044980138
24525,49051,0,49051,0.980463981628418,0.0029965700214453542
24625,49251,0,49251,0.9840729236602783,0.0029544012890565475
24725,49451,0,49451,0.9876821041107178,0.002918925108141795
24825,49651,0,49651,0.9920220375061035,0.0028742019167119453
24925,49851,0,49851,0.9958631992340088,0.0028337408024300937
25025,50051,0,50051,0.9994900226593018,0.002832319380721873
25125,50251,0,50251,1.0031192302703857,0.0028648651626167034
25225,50451,0,50451,1.0071282386779785,0.00289237084146579
25325,50651,0,50651,1.011199951171875,0.0029046182394376102
25425,50851,0,50851,1.0148711204528809,0.002918167177645575
25526,51053,0,51053,1.0184969902038574,0.002932861464379709
25626,51253,0,51253,1.0225720405578613,0.0029270260384629786
25726,51453,0,51453,1.0283551216125488,0.002900882643863504
25826,51653,0,51653,1.032628059387207,0.0028876571036222935
25926,51853,0,51853,1.038682222366333,0.002905310701126534
26026,52053,0,52053,1.04355788230896,0.0029345608700795
26126,52253,0,52253,1.0484910011291504,0.0029607131939564076
26226,52453,0,52453,1.0530781745910645,0.0029950039188995333
26326,52653,0,52653,1.0579121112823486,0.003039302832940597
26426,52853,0,52853,1.0627760887145996,0.00306967821135482
26527,53055,0,53055,1.0672650337219238,0.003069426646637729
26627,53255,0,53255,1.0717320442199707,0.0030538434962603376
26727,53455,0,53455,1.0761878490447998,0.003045823841038101
26827,53655,0,53655,1.0806221961975098,0.0030421477618152817
26927,53855,0,53855,1.0850801467895508,0.003033339287844165
27027,54055,0,54055,1.0895402431488037,0.003032260331735814
27127,54255,0,54255,1.09425687789917,0.0030519622958326384
27227,54455,0,54455,1.098656177520752,0.0030783286808199815
27327,54655,0,54655,1.1027462482452393,0.003086780736451006
27427,54855,0,54855,1.1067121028900146,0.003074839446928304
27528,55057,0,55057,1.1103579998016357,0.0030563605640995
27628,55257,0,55257,1.1139678955078125,0.003031795773763916
27728,55457,0,55457,1.117522954940796,0.0029907482973340824
27828,55657,0,55657,1.1210429668426514,0.002942111915777855
27928,55857,0,55857,1.1246089935302734,0.0029094092781719663
28028,56057,0,56057,1.1281201839447021,0.0028967349611878856
28128,56257,0,56257,1.131636142730713,0.0028865494460537625
28228,56457,0,56457,1.1352698802947998,0.002869306967611539
28328,56657,0,56657,1.1391749382019043,0.0028516527401632073
28428,56857,0,56857,1.1428852081298828,0.0028328620082355973
28529,57059,0,57059,1.1467058658599854,0.0027957228795076634
28629,57259,0,57259,1.1503009796142578,0.002736760860113118
28729,57459,0,57459,1.1539888381958008,0.002675925385800521
28829,57659,0,57659,1.1575109958648682,0.0026297566770034017
28929,57859,0,57859,1.161041021347046,0.0025938837059872786
29029,58059,0,58059,1.1645541191101074,0.002562142342374719
29129,58259,0,58259,1.1680688858032227,0.0025430374654775065
29229,58459,0,58459,1.1716029644012451,0.0025409813493694903
29329,58659,0,58659,1.1751110553741455,0.0025383157864291646
29429,58859,0,58859,1.1786088943481445,0.0025167910720348056
29530,59061,0,59061,1.1821389198303223,0.002481681851320229
29630,59261,0,59261,1.1856489181518555,0.002448782228785596
29730,59461,0,59461,1.1893320083618164,0.0024182065431847906
29830,59661,0,59661,1.1929900646209717,0.0023861388914979487
29930,59861,0,59861,1.196531057357788,0.002364104747120316
30030,60061,0,60061,1.2000770568847656,0.002367698564722654
30130,60261,0,60261,1.2035839557647705,0.0023909315353088955
30230,60461,0,60461,1.207103967666626,0.0024129709734338383
30330,60661,0,60661,1.2105998992919922,0.0024270664134750757
30430,60861,0,60861,1.2140958309173584,0.0024395367695122525
30531,61063,0,61063,1.217829942703247,0.0024478946063307074
30631,61263,0,61263,1.2213060855865479,0.002442747059705675
30731,61463,0,61463,1.2248010635375977,0.0024290991694118982
30831,61663,0,61663,1.2286128997802734,0.0024256606886608996
30931,61863,0,61863,1.2321019172668457,0.0024409120402841857
31031,62063,0,62063,1.2355949878692627,0.0024653568860609257
31131,62263,0,62263,1.2399611473083496,0.002491638587731647
31231,62463,0,62463,1.2435331344604492,0.0025228999495527805
31331,62663,0,62663,1.2473008632659912,0.002556152224293601
31431,62863,0,62863,1.2510159015655518,0.0025770961227783084
31532,63065,0,63065,1.25474214553833,0.002578710047573433
31632,63265,0,63265,1.2583510875701904,0.0025708250686072823
31732,63465,0,63465,1.26192307472229,0.002565260237147976
31832,63665,0,63665,1.2654900550842285,0.002562116239532298
31932,63865,0,63865,1.269050121307373,0.0025593424183206273
32032,64065,0,64065,1.272723913192749,0.002564000987120601
32132,64265,0,64265,1.2762250900268555,0.0025805201565868947
32232,64465,0,64465,1.2797009944915771,0.002598429086823534
32332,64665,0,64665,1.2831859588623047,0.002604072588794919
32432,64865,0,64865,1.286729097366333,0.0025961199015487597
32533,65067,0,65067,1.2902662754058838,0.002580434899538899
32633,65267,0,65267,1.2937862873077393,0.002557471529815911
32733,65467,0,65467,1.2973110675811768,0.0025247817938927066
32833,65667,0,65667,1.3008430004119873,0.0024901144690407944
32933,65867,0,65867,1.3043429851531982,0.002466397793160908
33033,66067,0,66067,1.3078391551971436,0.002454819228397141
33133,66267,0,66267,1.311337947845459,0.0024454603410924477
33233,66467,0,66467,1.3148281574249268,0.002432846910746171
33333,66667,0,66667,1.3183350563049316,0.0024182556688892467
33433,66867,0,66867,1.321835994720459,0.0023985743866934794
33534,67069,0,67069,1.325364112854004,0.0023651400529902753
33634,67269,0,67269,1.328861951828003,0.002318907170465284
33734,67469,0,67469,1.3326680660247803,0.0022721500895469464
33834,67669,0,67669,1.3362791538238525,0.0022346662565864697
33934,67869,0,67869,1.3408279418945312,0.0022053767897853935
34034,68069,0,68069,1.3447020053863525,0.0021825933955287717
34134,68269,0,68269,1.348315954208374,0.0021700126169286126
34234,68469,0,68469,1.3518390655517578,0.0021665415103854974
34334,68669,0,68669,1.3553731441497803,0.0021606134371208647
34434,68869,0,68869,1.3588778972625732,0.0021427101809933643
34535,69071,0,69071,1.362403154373169,0.0021159631283091864
34635,69271,0,69271,1.3659000396728516,0.0020891404026423706
34735,69471,0,69471,1.3699140548706055,0.002063793360179333
34835,69671,0,69671,1.3734431266784668,0.002040907189189321
34935,69871,0,69871,1.3769550323486328,0.002028770954314745
35035,70071,0,70071,1.3804481029510498,0.002034549152724416
35135,70271,0,70271,1.3839600086212158,0.002052669323688617
35235,70471,0,70471,1.3877341747283936,0.0020709974722026158
35335,70671,0,70671,1.391254186630249,0.0020846801539058457
35435,70871,0,70871,1.3947761058807373,0.0020951716392265227
35536,71073,0,71073,1.398324966430664,0.002100399054862868
35636,71273,0,71273,1.4018280506134033,0.002096974938302714
35736,71473,0,71473,1.4053308963775635,0.0020904186106610804
35836,71673,0,71673,1.4088411331176758,0.002092034359565157
35936,71873,0,71873,1.4125499725341797,0.0021061480100324262
36036,72073,0,72073,1.4160749912261963,0.002127761501764157
36136,72273,0,72273,1.4195771217346191,0.002152533196306687
36236,72473,0,72473,1.4230751991271973,0.0021798869320937574
36336,72673,0,72673,1.4265830516815186,0.002205586639121379
36436,72873,0,72873,1.430105209350586,0.002221102722655808
36537,73075,0,73075,1.4336450099945068,0.002223570722706126
36637,73275,0,73275,1.4371531009674072,0.0022194318393253683
36737,73475,0,73475,1.4406630992889404,0.0022157487507988042
36837,73675,0,73675,1.4442508220672607,0.0022139257771392118
36937,73875,0,73875,1.4478249549865723,0.002214604506085151
37037,74075,0,74075,1.4514482021331787,0.0022215017775233836
37137,74275,0,74275,1.454962968826294,0.002235081247068343
37237,74475,0,74475,1.4584519863128662,0.002247825420073512
37337,74675,0,74675,1.4619290828704834,0.002251518604418499
37437,74875,0,74875,1.465433120727539,0.002245042937601857
37538,75077,0,75077,1.4689691066741943,0.002231014346963123
37638,75277,0,75277,1.4724669456481934,0.0022103529675977047
37738,75477,0,75477,1.4759650230407715,0.0021838873123087507
37838,75677,0,75677,1.4794659614562988,0.0021578568792885956
37938,75877,0,75877,1.4829812049865723,0.0021396246368093025
38038,76077,0,76077,1.486480951309204,0.002129259708038191
38138,76277,0,76277,1.4899981021881104,0.00212081880499033
38238,76477,0,76477,1.4934980869293213,0.0021104087864917166
38338,76677,0,76677,1.4971141815185547,0.002097047679753491
38438,76877,0,76877,1.5006420612335205,0.0020776336726437273
38539,77079,0,77079,1.5041768550872803,0.002047804554149655
38639,77279,0,77279,1.5076720714569092,0.002010141474435998
38739,77479,0,77479,1.5111701488494873,0.001972672241692261
38839,77679,0,77679,1.5146830081939697,0.0019417435881117022
38939,77879,0,77879,1.518315076828003,0.00191788715728436
39039,78079,0,78079,1.5221729278564453,0.0019008010596479048
39139,78279,0,78279,1.5255250930786133,0.001891489312936453
39239,78479,0,78479,1.5288619995117188,0.0018871085664988573
39339,78679,0,78679,1.53218412399292,0.0018798460438502528
39439,78879,0,78879,1.5355899333953857,0.001864446560580227
39540,79081,0,79081,1.539039134979248,0.0018428981672343637
39640,79281,0,79281,1.542375087738037,0.0018206565068441588
39740,79481,0,79481,1.545835018157959,0.0018000411650954675
39840,79681,0,79681,1.549149990081787,0.001783742000643617
39940,79881,0,79881,1.5526468753814697,0.001777376958453249
40040,80081,0,80081,1.5559659004211426,0.0017840396158051786
40140,80281,0,80281,1.5592799186706543,0.0017990672649556576
40240,80481,0,80481,1.5625998973846436,0.0018146615456116344
40340,80681,0,80681,1.5659940242767334,0.0018270402166984331
40440,80881,0,80881,1.5693728923797607,0.001835746855021983
40541,81083,0,81083,1.572732925415039,0.0018394784187885458
40641,81283,0,81283,1.576186180114746,0.0018377815219774848
40741,81483,0,81483,1.5795142650604248,0.00183555560134167
40841,81683,0,81683,1.5828440189361572,0.0018399645519211777
40941,81883,0,81883,1.5862071514129639,0.00185344131589539
41041,82083,0,82083,1.5895459651947021,0.00187306880101494
41141,82283,0,82283,1.5929689407348633,0.0018957201759200815
41241,82483,0,82483,1.596365213394165,0.0019193069247216187
41341,82683,0,82683,1.5997068881988525,0.0019397285607861035
41441,82883,0,82883,1.6030750274658203,0.0019518075881724579
41542,83085,0,83085,1.6064488887786865,0.0019546000724135013
41642,83285,0,83285,1.609762191772461,0.0019525026496811885
41742,83485,0,83485,1.613145112991333,0.0019502839928196548
41842,83685,0,83685,1.616481065750122,0.0019498322230946388
41942,83885,0,83885,1.619854211807251,0.0019524621463306805
42042,84085,0,84085,1.6232750415802002,0.0019599428528215656
42142,84285,0,84285,1.6266450881958008,0.0019710879937284175
42242,84485,0,84485,1.63002610206604,0.0019803854505259792
42342,84685,0,84685,1.6334199905395508,0.00198255989837258
42442,84885,0,84885,1.6370229721069336,0.0019765870262380405
42543,85087,0,85087,1.6404950618743896,0.001963759587821181
42643,85287,0,85287,1.6438210010528564,0.0019454469354159318
42743,85487,0,85487,1.6471660137176514,0.0019236817275325418
42843,85687,0,85687,1.6506929397583008,0.001903304448633611
42943,85887,0,85887,1.6540250778198242,0.001888684005523003
43043,86087,0,86087,1.6582798957824707,0.0018794421717620684
43143,86287,0,86287,1.6615900993347168,0.0018716928282145036
43243,86487,0,86487,1.6649038791656494,0.0018623299520830734
43343,86687,0,86687,1.668360948562622,0.0018495533259617865
43443,86887,0,86887,1.6716768741607666,0.0018308946169432092
43544,87089,0,87089,1.675034999847412,0.001804305349139528
43644,87289,0,87289,1.6783461570739746,0.00177275944832017
43744,87489,0,87489,1.6816561222076416,0.001741861222188358
43844,87689,0,87689,1.685028076171875,0.001716075882038835
43944,87889,0,87889,1.689070224761963,0.0016965063759835366
44044,88089,0,88089,1.6925499439239502,0.0016831551437075628
44144,88289,0,88289,1.6958909034729004,0.0016755953064798953
44244,88489,0,88489,1.6992390155792236,0.0016706572997871952
44344,88689,0,88689,1.702639102935791,0.001662943041747961
44444,88889,0,88889,1.7059688568115234,0.0016493942336650478
44545,89091,0,89091,1.709522008895874,0.001631404133151033
44645,89291,0,89291,1.7128551006317139,0.0016128391603971583
44745,89491,0,89491,1.7162270545959473,0.001596276118128307
44845,89691,0,89691,1.7197661399841309,0.0015847302278729437
44945,89891,0,89891,1.7231628894805908,0.0015819193136072374
45045,90091,0,90091,1.7265658378601074,0.0015888856592116217
45145,90291,0,90291,1.7299671173095703,0.0016018155797608274
45245,90491,0,90491,1.73335599899292,0.0016152686111808672
45345,90691,0,90691,1.7367520332336426,0.0016261502889058426
45445,90891,0,90891,1.7401630878448486,0.0016334445515196866
45546,91093,0,91093,1.7435970306396484,0.0016365424923272182
45646,91293,0,91293,1.7470111846923828,0.0016363215071425394
45746,91493,0,91493,1.750411033630371,0.0016368719445404487
45846,91693,0,91693,1.7539000511169434,0.001642922858312116
45946,91893,0,91893,1.7573041915893555,0.0016559245946463973
46046,92093,0,92093,1.7606990337371826,0.001673934619050464
46146,92293,0,92293,1.7641081809997559,0.0016943532655905075
46246,92493,0,92493,1.7675058841705322,0.0017146210662758554
46346,92693,0,92693,1.7708978652954102,0.0017312309762592898
46446,92893,0,92893,1.7744920253753662,0.00174098146307194
46547,93095,0,93095,1.777940034866333,0.0017438341999876249
46647,93295,0,93295,1.7814340591430664,0.0017429755020846177
46747,93495,0,93495,1.784877061843872,0.001741921796825721
46847,93695,0,93695,1.7883782386779785,0.001742610907538379
46947,93895,0,93895,1.7919402122497559,0.001746297346197491
47047,94095,0,94095,1.795409917831421,0.0017535961114787015
47147,94295,0,94295,1.7988171577453613,0.0017627427130379565
47247,94495,0,94495,1.8022501468658447,0.0017695842377897883
47347,94695,0,94695,1.8056461811065674,0.0017705243217322978
47447,94895,0,94895,1.8090450763702393,0.0017646910755345162
47548,95097,0,95097,1.8124611377716064,0.001752873039526044
47648,95297,0,95297,1.8158762454986572,0.001736709332267942
47748,95497,0,95497,1.8192791938781738,0.0017185381453621042
47848,95697,0,95697,1.8226020336151123,0.0017020556367588222
47948,95897,0,95897,1.825937032699585,0.0016899421372710982
48048,96097,0,96097,1.8294620513916016,0.0016816394361211457
48148,96297,0,96297,1.832787036895752,0.0016743529732910726
48248,96497,0,96497,1.836143970489502,0.001665476250721223
48348,96697,0,96697,1.8396549224853516,0.0016530795894744753
48448,96897,0,96897,1.842972993850708,0.0016353771220881086
48549,97099,0,97099,1.846325159072876,0.001611599123157771
48649,97299,0,97299,1.8496901988983154,0.0015846500058269701
48749,97499,0,97499,1.8530702590942383,0.0015586584171250505
48849,97699,0,97699,1.8564071655273438,0.0015369674553322628
48949,97899,0,97899,1.859910011291504,0.0015207396250883228
49049,98099,0,98099,1.8632361888885498,0.0015099043845301888
49149,98299,0,98299,1.866569995880127,0.001503347659574665
49249,98499,0,98499,1.8699510097503662,0.0014980979783085903
49349,98699,0,98699,1.8733620643615723,0.001490344674723202
49449,98899,0,98899,1.8772571086883545,0.0014782526788620924
49550,99101,0,99101,1.8806910514831543,0.0014629201228826235
49650,99301,0,99301,1.884155035018921,0.0014473930755653677
49750,99501,0,99501,1.887679100036621,0.0014342099814929612
49850,99701,0,99701,1.8911731243133545,0.001426143531259742
49950,99901,0,99901,1.8946659564971924,0.0014256056501998754
50050,100101,0,100101,1.8982181549072266,0.0014325955599946872
50150,100301,0,100301,1.9017689228057861,0.001443964823865616
50250,100501,0,100501,1.9053690433502197,0.00145567188038496
50350,100701,0,100701,1.908884048461914,0.00146515598749627
50450,100901,0,100901,1.9125089645385742,0.001471392692476386
50551,101103,0,101103,1.916067123413086,0.0014743001787036042
50651,101303,0,101303,1.9196979999542236,0.0014752831662834588
50751,101503,0,101503,1.9232730865478516,0.0014776801378005996
50851,101703,0,101703,1.9268090724945068,0.0014847256112442478
50951,101903,0,101903,1.930413007736206,0.0014972804382558545
51051,102103,0,102103,1.9339990615844727,0.0015138549507893954
51151,102303,0,102303,1.9375932216644287,0.0015321431250083664
51251,102503,0,102503,1.9411580562591553,0.0015495912978981258
51351,102703,0,102703,1.94482421875,0.001563358806754074
51451,102903,0,102903,1.9484329223632812,0.0015714482131111915
51552,103105,0,103105,1.952120065689087,0.0015742496757250536
51652,103305,0,103305,1.955714225769043,0.0015742132430969882
51752,103505,0,103505,1.9593260288238525,0.0015740859340015211
51852,103705,0,103705,1.9628591537475586,0.0015756322334849514
51952,103905,0,103905,1.9664452075958252,0.0015798242092214393
52052,104105,0,104105,1.9700119495391846,0.00158660307348652
52152,104305,0,104305,1.9736452102661133,0.001594092872228056
52252,104505,0,104505,1.9772560596466064,0.0015990904973808282
52352,104705,0,104705,1.980794906616211,0.0015990256360576252
52452,104905,0,104905,1.9844181537628174,0.001593220942615384
52553,105107,0,105107,1.9880499839782715,0.0015823085725213055
52653,105307,0,105307,1.9917278289794922,0.0015680283698008043
52753,105507,0,105507,1.995365858078003,0.0015526400410521425
52853,105707,0,105707,1.9989981651306152,0.0015389546135519798
52953,105907,0,105907,2.0031850337982178,0.0015286469364750711
53053,106107,0,106107,2.0068180561065674,0.0015210830926291688
53153,106307,0,106307,2.0109829902648926,0.001514087654483631
53253,106507,0,106507,2.014400005340576,0.0015054371893267224
53353,106707,0,106707,2.0181918144226074,0.0014933736354768282
53453,106907,0,106907,2.021656036376953,0.0014766919303561717
53554,107109,0,107109,2.0251641273498535,0.0014553321310045483
53654,107309,0,107309,2.0286290645599365,0.001431978129637149
53754,107509,0,107509,2.0320918560028076,0.0014098005328303052
53854,107709,0,107709,2.0356149673461914,0.0013913938383567056
53954,107909,0,107909,2.0404410362243652,0.0013777651422495036
54054,108109,0,108109,2.0439019203186035,0.001368674712736372
54154,108309,0,108309,2.0474109649658203,0.0013627332153544128
54254,108509,0,108509,2.050922155380249,0.0013573385267385061
54354,108709,0,108709,2.054392099380493,0.0013497499870769975
54454,108909,0,108909,2.0578551292419434,0.0013388685261992274
54555,109111,0,109111,2.061483144760132,0.0013256575137909697
54655,109311,0,109311,2.065088987350464,0.0013126796004695681
54755,109511,0,109511,2.0685372352600098,0.0013022792481171162
54855,109711,0,109711,2.072007894515991,0.001296798391623782
54955,109911,0,109911,2.0756711959838867,0.0012977533953724629
55055,110111,0,110111,2.079303026199341,0.0013046169334038893
55155,110311,0,110311,2.083024024963379,0.001314747113687327
55255,110511,0,110511,2.08660888671875,0.0013250041709871683
55355,110711,0,110711,2.0900821685791016,0.0013332857111948589
55455,110911,0,110911,2.0935401916503906,0.001338756528243636
55556,111113,0,111113,2.0980610847473145,0.0013416946855590904
55656,111313,0,111313,2.101519823074341,0.0013436433226989945
55756,111513,0,111513,2.104964256286621,0.0013473029313144638
55856,111713,0,111713,2.108415126800537,0.0013549428453512148
55956,111913,0,111913,2.111846923828125,0.0013670299464661575
56056,112113,0,112113,2.1153111457824707,0.0013822859606987328
56156,112313,0,112313,2.118833065032959,0.0013986276495806529
56256,112513,0,112513,2.122354030609131,0.0014137135899817091
56356,112713,0,112713,2.125887155532837,0.0014253041260339978
56456,112913,0,112913,2.129401206970215,0.0014321617427647832
56557,113115,0,113115,2.132951021194458,0.001434877803544759
56657,113315,0,113315,2.136521100997925,0.0014354256210066564
56757,113515,0,113515,2.1401240825653076,0.0014360229291114713
56857,113715,0,113715,2.1436550617218018,0.0014381689783241978
56957,113915,0,113915,2.1472229957580566,0.0014425229720969805
57057,114115,0,114115,2.150745153427124,0.0014486468343088718
57157,114315,0,114315,2.1542890071868896,0.0014547473271161297
57257,114515,0,114515,2.1578140258789062,0.0014583069703305832
57357,114715,0,114715,2.1613481044769287,0.0014574324940890948
57457,114915,0,114915,2.164865016937256,0.0014516483723575394
57558,115117,0,115117,2.168416976928711,0.0014415642444502198
57658,115317,0,115317,2.171950101852417,0.0014289046131346177
57758,115517,0,115517,2.1755049228668213,0.001415699521821569
57858,115717,0,115717,2.179046869277954,0.0014040874652643553
57958,115917,0,115917,2.1826581954956055,0.0013951133704164019
58058,116117,0,116117,2.1868669986724854,0.0013881101410605037
58158,116317,0,116317,2.190425157546997,0.0013812903671307703
58258,116517,0,116517,2.1943271160125732,0.0013727584629237572
58358,116717,0,116717,2.197892904281616,0.001361034835554449
58458,116917,0,116917,2.2017669677734375,0.0013453705796312573
58559,117119,0,117119,2.2054340839385986,0.001326097236770188
58659,117319,0,117319,2.2089879512786865,0.0013056419979946352
58759,117519,0,117519,2.2125749588012695,0.0012865137995573131
58859,117719,0,117719,2.2161669731140137,0.0012707579701460867
58959,117919,0,117919,2.2197110652923584,0.0012591564610793036
59059,118119,0,118119,2.2232539653778076,0.0012513118157479498
59159,118319,0,118319,2.226792097091675,0.0012457782827354135
59259,118519,0,118519,2.2305381298065186,0.0012403512366213174
59359,118719,0,118719,2.234490156173706,0.0012330350489255998
59459,118919,0,118919,2.238278865814209,0.001223204105869211
59560,119121,0,119121,2.2423551082611084,0.0012117644303724217
59660,119321,0,119321,2.24596905708313,0.0012009442503621134
59760,119521,0,119521,2.24949312210083,0.0011928230134014698
59860,119721,0,119721,2.2531981468200684,0.001189288274385339
59960,119921,0,119921,2.2567949295043945,0.001191239292838619
60060,120121,0,120121,2.2603650093078613,0.0011978910627687836
60160,120321,0,120321,2.2639801502227783,0.0012069953109918629
60260,120521,0,120521,2.267529010772705,0.0012160416406080858
60360,120721,0,120721,2.271031141281128,0.0012233289727530394
60460,120921,0,120921,2.2746970653533936,0.0012282581349603644
60561,121123,0,121123,2.2782840728759766,0.0012313321069720839
60661,121323,0,121323,2.28183913230896,0.0012340492612210427
60761,121523,0,121523,2.2853949069976807,0.0012385862275623662
60861,121723,0,121723,2.2889840602874756,0.0012465550501840653
60961,121923,0,121923,2.2925660610198975,0.0012581417940070547
61061,122123,0,122123,2.2961370944976807,0.0012721759013534003
61161,122323,0,122323,2.2997052669525146,0.0012867770811281246
61261,122523,0,122523,2.303274154663086,0.0012998905564955393
61361,122723,0,122723,2.306823968887329,0.0013097779899204935
61461,122923,0,122923,2.3103859424591064,0.0013156965635649413
61562,123125,0,123125,2.3139760494232178,0.0013183268886036094
61662,123325,0,123325,2.317549228668213,0.0013193081901889466
61762,123525,0,123525,2.321101188659668,0.0013204583064103268
61862,123725,0,123725,2.3246610164642334,0.0013229926965235045
61962,123925,0,123925,2.3282251358032227,0.001327294607374821
62062,124125,0,124125,2.331808090209961,0.0013327255067515278
62162,124325,0,124325,2.335353136062622,0.0013376491374219816
62262,124525,0,124525,2.3389031887054443,0.0013400594333804524
62362,124725,0,124725,2.342466115951538,0.0013385416414368352
62462,124925,0,124925,2.3460280895233154,0.0013328070640767876
62563,125127,0,125127,2.350684881210327,0.001323481762663548
62663,125327,0,125327,2.354182004928589,0.0013122055010089079
62763,125527,0,125527,2.357678174972534,0.001300734676191776
62863,125727,0,125727,2.3611881732940674,0.0012906962131568177
62963,125927,0,125927,2.364698886871338,0.0012827227509193122
63063,126127,0,126127,2.3682188987731934,0.0012761361411390132
63163,126327,0,126327,2.3717150688171387,0.0012694212515995242
63263,126527,0,126527,2.37520694732666,0.0012609750828942302
63363,126727,0,126727,2.3787100315093994,0.0012496128339744
63463,126927,0,126927,2.382205009460449,0.001234930306391453
63564,127129,0,127129,2.385767936706543,0.001217469957805779
63664,127329,0,127329,2.3893609046936035,0.0011994065953910115
63764,127529,0,127529,2.392911911010742,0.0011827644365060613
63864,127729,0,127729,2.3964061737060547,0.0011691608259753834
63964,127929,0,127929,2.39990496635437,0.0011591500512954734
64064,128129,0,128129,2.4035580158233643,0.0011522205255517085
64164,128329,0,128329,2.407111883163452,0.001146982188772943
64264,128529,0,128529,2.410668134689331,0.0011416009200992106
64364,128729,0,128729,2.414216995239258,0.0011346175558625768
64464,128929,0,128929,2.417710065841675,0.0011257272052057057
64565,129131,0,129131,2.4211652278900146,0.001115808639143752
64665,129331,0,129331,2.424527883529663,0.0011068243116640866
64765,129531,0,129531,2.427888870239258,0.001100567830344454
64865,129731,0,129731,2.4312479496002197,0.00109851252859559
64965,129931,0,129931,2.4346508979797363,0.001101130304909402
65065,130131,0,130131,2.438149929046631,0.0011075219812861166
65165,130331,0,130331,2.4415621757507324,0.001115755643891863
65265,130531,0,130531,2.4449520111083984,0.0011237911960981048
65365,130731,0,130731,2.449080228805542,0.001130274921076301
65465,130931,0,130931,2.4525229930877686,0.001134828826836185
65566,131133,0,131133,2.4559781551361084,0.0011380825563218396
65666,131333,0,131333,2.459439277648926,0.0011414079735422653
65766,131533,0,131533,2.4628028869628906,0.0011465554335009156
65866,131733,0,131733,2.466235876083374,0.0011546681539989963
65966,131933,0,131933,2.4696269035339355,0.001165726350479626
66066,132133,0,132133,2.4729971885681152,0.0011786288192106341
66166,132333,0,132333,2.4763588905334473,0.001191690770077236
66266,132533,0,132533,2.4797089099884033,0.0012031546966401784
66366,132733,0,132733,2.4830620288848877,0.0012116872205620423
66466,132933,0,132933,2.4864580631256104,0.0012168758669294545
66567,133135,0,133135,2.4898860454559326,0.0012194317193560643
66667,133335,0,133335,2.4932281970977783,0.0012207407797331406
66767,133535,0,133535,2.4965720176696777,0.0012222991794524135
66867,133735,0,133735,2.499958038330078,0.0012250560419659654
66967,133935,0,133935,2.5033512115478516,0.0012291736107488877
67067,134135,0,134135,2.5066990852355957,0.0012339206869557088
67167,134335,0,134335,2.5102789402008057,0.0012378394893487123
67267,134535,0,134535,2.5136289596557617,0.0012393177079660135
67367,134735,0,134735,2.5170440673828125,0.001237296667797865
67467,134935,0,134935,2.5207512378692627,0.0012316485220151459
67568,135137,0,135137,2.52414608001709,0.001223016155154614
67668,135337,0,135337,2.527517080307007,0.0012129176072889238
67768,135537,0,135537,2.530879020690918,0.0012028394107488792
67868,135737,0,135737,2.535799026489258,0.0011940161635542708
67968,135937,0,135937,2.5394740104675293,0.0011868012363774071
68068,136137,0,136137,2.5428380966186523,0.0011805212034008876
68168,136337,0,136337,2.5462231636047363,0.0011738724413281761
68268,136537,0,136537,2.550309896469116,0.001165514426206311
68368,136737,0,136737,2.5537970066070557,0.0011545350063868374
68468,136937,0,136937,2.557539224624634,0.0011407845371504465
68569,137139,0,137139,2.560987949371338,0.0011249117431240384
68669,137339,0,137339,2.5651650428771973,0.0011088563688309893
68769,137539,0,137539,2.568681001663208,0.0010942690903759655
68869,137739,0,137739,2.5720388889312744,0.001082422994812133
68969,137939,0,137939,2.575618028640747,0.0010736708217486185
69069,138139,0,138139,2.5796051025390625,0.0010674326315821324
69169,138339,0,138339,2.5830330848693848,0.001062427913293851
69269,138539,0,138539,2.5864830017089844,0.001057148788560264
69369,138739,0,138739,2.5903899669647217,0.0010505338237381976
69469,138939,0,138939,2.595863103866577,0.0010425026912944588
69570,139141,0,139141,2.599390983581543,0.0010339126606182904
69670,139341,0,139341,2.6028249263763428,0.001026495450055356
69770,139541,0,139541,2.606271982192993,0.0010217661391864405
69870,139741,0,139741,2.611877202987671,0.001020843501182434
69970,139941,0,139941,2.6156911849975586,0.00102390269709295
70070,140141,0,140141,2.6199162006378174,0.0010300095649300647
70170,140341,0,140341,2.6240949630737305,0.0010374949610785222
70270,140541,0,140541,2.628316879272461,0.0010446884701483068
70370,140741,0,140741,2.634481906890869,0.0010505317433506447
70470,140941,0,140941,2.639354944229126,0.0010548314352339418
70571,141143,0,141143,2.643930196762085,0.0010582760176608638
70671,141343,0,141343,2.648426055908203,0.001062079422990922
70771,141543,0,141543,2.6531269550323486,0.001067644585432602
70871,141743,0,141743,2.657792091369629,0.0010757683914840797
70971,141943,0,141943,2.662247896194458,0.001086280161536596
71071,142143,0,142143,2.666651964187622,0.001098138340525941
71171,142343,0,142343,2.67108416557312,0.0011098464311664297
71271,142543,0,142543,2.675725221633911,0.0011199259105610653
71371,142743,0,142743,2.6803150177001953,0.0011273660513241653
71471,142943,0,142943,2.6847779750823975,0.001131979012644588
71572,143145,0,143145,2.6895790100097656,0.0011344729888931018
71672,143345,0,143345,2.6940760612487793,0.0011360291941346357
71772,143545,0,143545,2.6985931396484375,0.0011378759739134109
71872,143745,0,143745,2.70304799079895,0.0011407285274978249
71972,143945,0,143945,2.7076261043548584,0.001144581882564306
72072,144145,0,144145,2.712111234664917,0.0011486769909599388
72172,144345,0,144345,2.7166459560394287,0.0011517331373246031
72272,144545,0,144545,2.7208681106567383,0.0011524496331047787
72372,144745,0,144745,2.7247021198272705,0.0011500418924641545
72472,144945,0,144945,2.7283971309661865,0.0011445132817639889
72573,145147,0,145147,2.732077121734619,0.0011365109185042838
72673,145347,0,145347,2.735759973526001,0.001127414905486295
72773,145547,0,145547,2.7395730018615723,0.001118465039975015
72873,145747,0,145747,2.7432940006256104,0.0011105922646403718
72973,145947,0,145947,2.747101068496704,0.0011039565284082827
73073,146147,0,146147,2.7506871223449707,0.0010979021646176223
73173,146347,0,146347,2.7544500827789307,0.0010913023810353642
73273,146547,0,146547,2.7581520080566406,0.0010830501191108903
73373,146747,0,146747,2.7620890140533447,0.0010724700576519703
73473,146947,0,146947,2.7656900882720947,0.0010595972327050896
73574,147149,0,147149,2.769379138946533,0.0010451243864532133
73674,147349,0,147349,2.773400068283081,0.0010307764571610273
73774,147549,0,147549,2.7770261764526367,0.0010179050433600494
73874,147749,0,147749,2.7806320190429688,0.0010075025947601035
73974,147949,0,147949,2.784230947494507,0.000999755940570069
74074,148149,0,148149,2.7878479957580566,0.0009940549924147145
74174,148349,0,148349,2.791781187057495,0.0009892509704428464
74274,148549,0,148549,2.7954869270324707,0.0009841161546772458
74374,148749,0,148749,2.7991838455200195,0.0009778906604127285
74474,148949,0,148949,2.8028790950775146,0.0009706534699824129
74575,149151,0,149151,2.8067851066589355,0.000963235322718374
74675,149351,0,149351,2.8104560375213623,0.0009571588910445978
74775,149551,0,149551,2.8141701221466064,0.0009536822883274291
74875,149751,0,149751,2.817946195602417,0.0009536305562602861
74975,149951,0,149951,2.822200059890747,0.0009569733320912373
75075,150151,0,150151,2.825923204421997,0.0009627865947572978
75175,150351,0,150351,2.829524040222168,0.0009696252805129255
75275,150551,0,150551,2.833138942718506,0.0009761192061184185
75375,150751,0,150751,2.8372390270233154,0.0009814569153328478
75475,150951,0,150951,2.841132164001465,0.000985589195091962
75576,151153,0,151153,2.8447301387786865,0.0009892179249460424
75676,151353,0,151353,2.848677158355713,0.000993392577900434
75776,151553,0,151553,2.853555917739868,0.0009992315010242854
75876,151753,0,151753,2.85771107673645,0.0010072697187388814
75976,151953,0,151953,2.8614389896392822,0.0010172283249528437
76076,152153,0,152153,2.8650949001312256,0.001028126651325982
76176,152353,0,152353,2.868774890899658,0.001038646622963756
76276,152553,0,152553,2.8726680278778076,0.0010475591321412114
76376,152753,0,152753,2.8764820098876953,0.0010541089416690136
76476,152953,0,152953,2.8800342082977295,0.0010582622461742708
76577,153155,0,153155,2.8836240768432617,0.0010607040932872844
76677,153355,0,153355,2.887326955795288,0.0010624423897540266
76777,153555,0,153555,2.8910861015319824,0.0010644792284496484
76877,153755,0,153755,2.895432949066162,0.0010673323349624038
76977,153955,0,153955,2.898948907852173,0.0010708756407884438
77077,154155,0,154155,2.9024908542633057,0.0010743610897160404
77177,154355,0,154355,2.9062180519104004,0.0010766741907691337
77277,154555,0,154555,2.9107091426849365,0.001076766172798292
77377,154755,0,154755,2.9143290519714355,0.0010740675802313
77477,154955,0,154955,2.9179630279541016,0.0010686840101889498
77578,155157,0,155157,2.9216930866241455,0.0010612520454229123
77678,155357,0,155357,2.9260900020599365,0.0010530103474834815
77778,155557,0,155557,2.929650068283081,0.0010449812440112172
77878,155757,0,155757,2.933237075805664,0.0010378588910046292
77978,155957,0,155957,2.936803102493286,0.0010316681549368664
78078,156157,0,156157,2.94096302986145,0.0010257819239320035
78178,156357,0,156357,2.944582939147949,0.0010192278131191368
78278,156557,0,156557,2.948184013366699,0.0010111040246629243
78378,156757,0,156757,2.9517860412597656,0.0010009338801809779
78478,156957,0,156957,2.9559099674224854,0.000988883896991085
78579,157159,0,157159,2.959567070007324,0.0009756528945409037
78679,157359,0,157359,2.9631760120391846,0.000962770786885982
78779,157559,0,157559,2.966797113418579,0.0009513435271498311
78879,157759,0,157759,2.9705841541290283,0.000942134118170347
78979,157959,0,157959,2.9742720127105713,0.0009351994843797639
79079,158159,0,158159,2.977879047393799,0.0009299282455535872
79179,158359,0,158359,2.9831809997558594,0.0009253084871290601
79279,158559,0,158559,2.9869260787963867,0.0009203502965556831
79379,158759,0,158759,2.9907588958740234,0.0009145258799706488
79479,158959,0,158959,2.9943530559539795,0.0009080264991396564
79580,159161,0,159161,2.9980008602142334,0.0009016478581305168
79680,159361,0,159361,3.0015950202941895,0.000896720479762326
79780,159561,0,159561,3.005255937576294,0.0008942730757924846
79880,159761,0,159761,3.008970022201538,0.000894892054526377
79980,159961,0,159961,3.012559175491333,0.000898406278121127
80080,160161,0,160161,3.0161211490631104,0.0009039281050257195
80180,160361,0,160361,3.0196261405944824,0.0009102070487694014
80280,160561,0,160561,3.023428201675415,0.0009161213339080752
80380,160761,0,160761,3.0269949436187744,0.0009210627257674832
80480,160961,0,160961,3.0305700302124023,0.0009250889085619462
80581,161163,0,161163,3.0341591835021973,0.0009288855001947785
80681,161363,0,161363,3.037943124771118,0.0009333430672882763
80781,161563,0,161563,3.041501998901367,0.0009393457209627499
80881,161763,0,161763,3.0449979305267334,0.000947227954407332
80981,161963,0,161963,3.0485000610351562,0.0009566364992142678
81081,162163,0,162163,3.0519859790802,0.0009666556808162054
81181,162363,0,162363,3.0557498931884766,0.0009761334800950727
81281,162563,0,162563,3.0593390464782715,0.000984057923238766
81381,162763,0,162763,3.062840223312378,0.0009898753841833911
81481,162963,0,162963,3.0663528442382812,0.0009936572447954426
81582,163165,0,163165,3.0699379444122314,0.000996052643186995
81682,163365,0,163365,3.0736582279205322,0.0009979188030616651
81782,163565,0,163565,3.0772180557250977,0.00100006586852164
81882,163765,0,163765,3.08076810836792,0.0010028493010776991
81982,163965,0,163965,3.0843241214752197,0.0010060591730787088
82082,164165,0,164165,3.0881130695343018,0.0010089813913014317
82182,164365,0,164365,3.0916481018066406,0.0010106534682368252
82282,164565,0,164565,3.095255136489868,0.0010102333151440046
82382,164765,0,164765,3.0987861156463623,0.001007321848753464
82482,164965,0,164965,3.1024110317230225,0.0010021007930145808
82583,165167,0,165167,3.1062259674072266,0.0009951833618913296
82683,165367,0,165367,3.1097640991210938,0.0009876707091756424
82783,165567,0,165567,3.113284111022949,0.0009803972486307473
82883,165767,0,165767,3.1167800426483154,0.0009738716515537823
82983,165967,0,165967,3.12054705619812,0.0009680251008316155
83083,166167,0,166167,3.1241350173950195,0.0009622674978916743
83183,166367,0,166367,3.127635955810547,0.0009557641521839236
83283,166567,0,166567,3.1311402320861816,0.0009477917322843659
83383,166767,0,166767,3.134683847427368,0.0009380364695932248
83483,166967,0,166967,3.138427972793579,0.0009267560803420624
83584,167169,0,167169,3.1423659324645996,0.0009146319587977128
83684,167369,0,167369,3.146127223968506,0.0009030174031439471
83784,167569,0,167569,3.1496479511260986,0.0008928135405595049
83884,167769,0,167769,3.153323173522949,0.000884596317954252
83984,167969,0,167969,3.15708589553833,0.0008783251616144327
84084,168169,0,168169,3.160644054412842,0.000873407874743729
84184,168369,0,168369,3.164292097091675,0.0008689655711052333
84284,168569,0,168569,3.1679091453552246,0.0008642089964452994
84384,168769,0,168769,3.171663999557495,0.0008587904249607236
84484,168969,0,168969,3.1751749515533447,0.000852978107370054
84585,169171,0,169171,3.1790311336517334,0.00084752432169788
84685,169371,0,169371,3.1825249195098877,0.0008435828867218076
84785,169571,0,169571,3.1860039234161377,0.0008419820779379084
84885,169771,0,169771,3.1911139488220215,0.000843117064672766
84985,169971,0,169971,3.194791078567505,0.0008467226248128713
85085,170171,0,170171,3.198374032974243,0.0008519626875088011
85185,170371,0,170371,3.202700138092041,0.0008577575277262221
85285,170571,0,170571,3.2079219818115234,0.0008631927728393921
85385,170771,0,170771,3.2114319801330566,0.0008678251250297845
85485,170971,0,170971,3.2149388790130615,0.0008717876261863695
85586,171173,0,171173,3.218487024307251,0.0008757308410332178
85686,171373,0,171373,3.2222111225128174,0.0008803975726308011
85786,171573,0,171573,3.226487159729004,0.0008864785712112553
85886,171773,0,171773,3.2299678325653076,0.0008941541631040388
85986,171973,0,171973,3.2334530353546143,0.0009030236132339664
86086,172173,0,172173,3.237173080444336,0.0009122398475144123
86186,172373,0,172373,3.2423360347747803,0.0009208029937222869
86286,172573,0,172573,3.245877981185913,0.0009278871317429346
86386,172773,0,172773,3.249380111694336,0.0009330972104073045
86486,172973,0,172973,3.2528951168060303,0.0009365749854052516
86587,173175,0,173175,3.2572450637817383,0.0009389256965602678
86687,173375,0,173375,3.2608048915863037,0.0009408738110536373
86787,173575,0,173575,3.2643678188323975,0.0009430668705487247
86887,173775,0,173775,3.268019914627075,0.0009457297563372018
86987,173975,0,173975,3.272245168685913,0.0009485978005525292
87087,174175,0,174175,3.2761752605438232,0.0009510039896589251
87187,174375,0,174375,3.279932975769043,0.0009521228972955541
87287,174575,0,174575,3.283474922180176,0.0009512835600976517
87387,174775,0,174775,3.287317991256714,0.0009482220234699681
87487,174975,0,174975,3.2915141582489014,0.0009431738001132771
87588,175177,0,175177,3.295168161392212,0.0009367190248346826
87688,175377,0,175377,3.2989261150360107,0.0009298293871590868
87788,175577,0,175577,3.3026230335235596,0.0009231788541380415
87888,175777,0,175777,3.306917190551758,0.0009171306367946925
87988,175977,0,175977,3.3104441165924072,0.0009115525521134318
88088,176177,0,176177,3.314249038696289,0.0009058976204110063
88188,176377,0,176377,3.3180339336395264,0.000899454848901086
88288,176577,0,176577,3.3483850955963135,0.0008916545532991943
88388,176777,0,176777,3.3699910640716553,0.0008823143472637314
88488,176977,0,176977,3.3758552074432373,0.0008717526528191332
88589,177179,0,177179,3.3809049129486084,0.0008606188648109262
88689,177379,0,177379,3.3858072757720947,0.0008501066459656683
88789,177579,0,177579,3.3908050060272217,0.0008409450479955734
88889,177779,0,177779,3.39578914642334,0.0008335584689124669
88989,177979,0,177979,3.4024641513824463,0.000827836304251596
89089,178179,0,178179,3.407876968383789,0.0008232192833545158
89189,178379,0,178379,3.4231371879577637,0.0008189531924501059
89289,178579,0,178579,3.4282398223876953,0.0008144174185373537
89389,178779,0,178779,3.4337339401245117,0.000809404162514606
89489,178979,0,178979,3.438847064971924,0.0008042315951174141
89590,179181,0,179181,3.4442861080169678,0.0007996018393932136
89690,179381,0,179381,3.4491569995880127,0.0007965070918047374
89790,179581,0,179581,3.4542860984802246,0.0007956031503644702
89890,179781,0,179781,3.459423065185547,0.0007971336884171355
89990,179981,0,179981,3.4643101692199707,0.0008007734895635716
90090,180181,0,180181,3.4691169261932373,0.0008057464206869393
90190,180381,0,180381,3.4743869304656982,0.0008111233436595108
90290,180581,0,180581,3.4792661666870117,0.000816163577950558
90390,180781,0,180781,3.4840471744537354,0.0008205558831743719
90490,180981,0,180981,3.488896131515503,0.0008244831050824066
90591,181183,0,181183,3.4939231872558594,0.0008285494418414911
90691,181383,0,181383,3.4987399578094482,0.0008333633743347014
90791,181583,0,181583,3.5032429695129395,0.0008394559346877494
90891,181783,0,181783,3.5082719326019287,0.0008468893408817444
90991,181983,0,181983,3.513010025024414,0.0008552365358413432
91091,182183,0,182183,3.5174720287323,0.0008637209964976449
91191,182383,0,182383,3.5218911170959473,0.0008714804862890933
91291,182583,0,182583,3.5272090435028076,0.0008778468552083648
91391,182783,0,182783,3.5316529273986816,0.0008825492118494932
91491,182983,0,182983,3.5360829830169678,0.0008857743363477003
91592,183185,0,183185,3.5413761138916016,0.000888078899176781
91692,183385,0,183385,3.5457961559295654,0.0008900699096325926
91792,183585,0,183585,3.55013108253479,0.0008922577659147486
91892,183785,0,183785,3.5546162128448486,0.0008947641844294143
91992,183985,0,183985,3.5591139793395996,0.0008972920815997399
92092,184185,0,184185,3.563408851623535,0.0008992284103945579
92192,184385,0,184385,3.5672829151153564,0.0008998702672839234
92292,184585,0,184585,3.5713300704956055,0.0008986890341270558
92392,184785,0,184785,3.574937105178833,0.0008955275128232423
92492,184985,0,184985,3.5785129070281982,0.0008906565533221694
92593,185187,0,185187,3.5821280479431152,0.0008846166159663174
92693,185387,0,185387,3.585875988006592,0.000878260034818713
92793,185587,0,185587,3.5897490978240967,0.0008721249110783372
92893,185787,0,185787,3.593717098236084,0.0008664606690127524
92993,185987,0,185987,3.5973682403564453,0.0008610943982780624
93093,186187,0,186187,3.601130962371826,0.0008555261481078117
93193,186387,0,186387,3.6049420833587646,0.0008491560470077379
93293,186587,0,186587,3.6086480617523193,0.0008415455333584331
93393,186787,0,186787,3.6123032569885254,0.0008326166216676273
93493,186987,0,186987,3.616245985031128,0.0008227253420393627
93594,187189,0,187189,3.6200110912323,0.0008124802718371369
93694,187389,0,187389,3.623756170272827,0.000802931143436931
93794,187589,0,187589,3.627552032470703,0.000794662113098775
93894,187789,0,187789,3.6315081119537354,0.0007879758349172392
93994,187989,0,187989,3.6352031230926514,0.0007827141134753449
94094,188189,0,188189,3.638916254043579,0.0007783592113028995
94194,188389,0,188389,3.6430931091308594,0.0007742711600968495
94294,188589,0,188589,3.64690899848938,0.0007699705472040792
94394,188789,0,188789,3.6505138874053955,0.0007653578326524802
94494,188989,0,188989,3.654366970062256,0.0007607801791359441
94595,189191,0,189191,3.6581919193267822,0.0007568849673641497
94695,189391,0,189391,3.6620049476623535,0.0007545176678981245
94795,189591,0,189591,3.665663957595825,0.0007541874035616835
94895,189791,0,189791,3.669290065765381,0.0007560192327353153
94995,189991,0,189991,3.6730690002441406,0.0007596530200392278
95095,190191,0,190191,3.677060842514038,0.0007643765134928485
95195,190391,0,190391,3.6806721687316895,0.0007693934798117416
95295,190591,0,190591,3.6843130588531494,0.0007741085895051778
95395,190791,0,190791,3.6880509853363037,0.0007783148567584336
95495,190991,0,190991,3.692629098892212,0.0007822248145111499
95596,191193,0,191193,3.696319103240967,0.0007863901271057027
95696,191393,0,191393,3.699997901916504,0.0007912990200015061
95796,191593,0,191593,3.70408296585083,0.0007973508190031904
95896,191793,0,191793,3.7078709602355957,0.0008045181797518771
95996,191993,0,191993,3.7116639614105225,0.0008123640812578168
96096,192193,0,192193,3.71527099609375,0.0008201826783622205
96196,192393,0,192393,3.719097137451172,0.0008272349627148337
96296,192593,0,192593,3.722944974899292,0.0008329855468372971
96396,192793,0,192793,3.726785182952881,0.0008372600970994839
96496,192993,0,192993,3.730323076248169,0.0008402717264357288
96597,193195,0,193195,3.7341508865356445,0.0008425262976018672
96697,193395,0,193395,3.738075017929077,0.0008445270207044877
96797,193595,0,193595,3.741772174835205,0.0008466693057664391
96897,193795,0,193795,3.74531626701355,0.0008489948638913945
96997,193995,0,193995,3.7488510608673096,0.0008511910529386722
97097,194195,0,194195,3.7524330615997314,0.0008527016737781329
97197,194395,0,194395,3.7562949657440186,0.0008529326600357097
97297,194595,0,194595,3.7603719234466553,0.0008514739423800917
97397,194795,0,194795,3.7638840675354004,0.0008482519684506491
97497,194995,0,194995,3.767380952835083,0.0008435580921917654
97598,195197,0,195197,3.771170139312744,0.0008378891808847192
97698,195397,0,195397,3.774707078933716,0.0008319891550956358
97798,195597,0,195597,3.778409957885742,0.0008262818387742534
97898,195797,0,195797,3.782233238220215,0.0008209282039933645
97998,195997,0,195997,3.785723924636841,0.0008157316669440638
98098,196197,0,196197,3.7894668579101562,0.0008102412984337118
98198,196397,0,196397,3.7933170795440674,0.0008039566797691744
98298,196597,0,196597,3.7972350120544434,0.0007965502411254371
98398,196797,0,196797,3.8007209300994873,0.0007880257015586181
98498,196997,0,196997,3.804518938064575,0.0007787592225022795
98599,197199,0,197199,3.8080739974975586,0.0007693136027286702
98699,197399,0,197399,3.811836004257202,0.0007606092228967299
98799,197599,0,197599,3.815371036529541,0.0007531083759723326
98899,197799,0,197799,3.8189902305603027,0.0007470169310039487
98999,197999,0,197999,3.822650194168091,0.0007421469632506081
99099,198199,0,198199,3.826956033706665,0.0007380270677818757
99199,198399,0,198399,3.830493927001953,0.0007341203675572351
99299,198599,0,198599,3.834023952484131,0.0007300651489868317
99399,198799,0,198799,3.8377699851989746,0.0007258447735270744
99499,198999,0,198999,3.8417880535125732,0.000721819252360302
99600,199201,0,199201,3.8455049991607666,0.000718578735194168
99700,199401,0,199401,3.849048137664795,0.0007168365414369836
99800,199601,0,199601,3.8526060581207275,0.0007169783094077633
99900,199801,0,199801,3.8568131923675537,0.0007190374731894531
100000,200001,0,200001,3.8604700565338135,0.0007226374491856396


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha0/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.224082946777344e-05,4.387061074692293
100,201,200,401,0.0042340755462646484,0.24400872360835765
200,401,400,801,0.008651971817016602,0.11396482179674887
300,601,600,1201,0.013067007064819336,0.07772603596230616
400,801,800,1601,0.01716923713684082,0.06190660644187962
501,1003,1002,2005,0.021404266357421875,0.05363210938132448
601,1203,1202,2405,0.025474071502685547,0.04854289708923014
701,1403,1402,2805,0.029764175415039062,0.044811894255043366
801,1603,1602,3205,0.03382611274719238,0.04179654400397964
901,1803,1802,3605,0.037937164306640625,0.03924971924554778
1001,2003,2002,4005,0.04191422462463379,0.03706348955839846
1101,2203,2202,4405,0.045882225036621094,0.035178785925197326
1201,2403,2402,4805,0.049880027770996094,0.03355453267398762
1301,2603,2602,5205,0.05383610725402832,0.03215726348792642
1401,2803,2802,5605,0.05793619155883789,0.03095767199648659
1502,3005,3004,6009,0.06195712089538574,0.02991998323202208
1602,3205,3204,6409,0.06588602066040039,0.029040939320774044
1702,3405,3404,6809,0.06990790367126465,0.02828835829650628
1802,3605,3604,7209,0.0738520622253418,0.027643543602227788
1902,3805,3804,7609,0.0777430534362793,0.027090075263709473
2002,4005,4004,8009,0.08164715766906738,0.02661366298608146
2102,4205,4204,8409,0.0855553150177002,0.026201975227758096
2202,4405,4404,8809,0.08989405632019043,0.0258444527270099
2302,4605,4604,9209,0.09481215476989746,0.02553211595577548
2402,4805,4804,9609,0.09883308410644531,0.02525737490279822
2503,5007,5006,10013,0.1029660701751709,0.025011551173271675
2603,5207,5206,10413,0.10695910453796387,0.02479413074736284
2703,5407,5406,10813,0.11099910736083984,0.024598087482034042
2803,5607,5606,11213,0.1149911880493164,0.02441972624861084
2903,5807,5806,11613,0.11914205551147461,0.024255984393149754
3003,6007,6006,12013,0.12314605712890625,0.02410432926149394
3103,6207,6206,12413,0.12713122367858887,0.023962670451067175
3203,6407,6406,12813,0.13113808631896973,0.02382928529238106
3303,6607,6606,13213,0.1352701187133789,0.023702755993531773
3403,6807,6806,13613,0.13924026489257812,0.023581916916485614
3504,7009,7008,14017,0.1432480812072754,0.023464670603200708
3604,7209,7208,14417,0.1472160816192627,0.023352546952781245
3704,7409,7408,14817,0.1515500545501709,0.02324371933040331
3804,7609,7608,15217,0.1555020809173584,0.02313765993724719
3904,7809,7808,15617,0.15942597389221191,0.023033936061227892
4004,8009,8008,16017,0.16335606575012207,0.02293219301852367
4104,8209,8208,16417,0.1672811508178711,0.022832140115381733
4204,8409,8408,16817,0.1717979907989502,0.02273353910866042
4304,8609,8608,17217,0.1758420467376709,0.022636194729250055
4404,8809,8808,17617,0.17992901802062988,0.02253994690559794
4505,9011,9010,18021,0.18398308753967285,0.022443716054252546
4605,9211,9210,18421,0.18813323974609375,0.022349299282451357
4705,9411,9410,18821,0.19263100624084473,0.022255651010420593
4805,9611,9610,19221,0.19651508331298828,0.022162698835552937
4905,9811,9810,19621,0.20040297508239746,0.022070383260160423
5005,10011,10010,20021,0.20429611206054688,0.02197865534524145
5105,10211,10210,20421,0.20817303657531738,0.02188747479025684
5205,10411,10410,20821,0.21209001541137695,0.021796808361813313
5305,10611,10610,21221,0.21645903587341309,0.021706628608024154
5405,10811,10810,21621,0.22035717964172363,0.021616912806721164
5506,11013,11012,22025,0.2243189811706543,0.02152675159037204
5606,11213,11212,22425,0.22822308540344238,0.02143791452511929
5706,11413,11412,22825,0.23304009437561035,0.021349493655195773
5806,11613,11612,23225,0.23719120025634766,0.021261478021364178
5906,11813,11812,23625,0.24240899085998535,0.021173858394926075
6006,12013,12012,24025,0.2477099895477295,0.0210866269634385
6106,12213,12212,24425,0.2525019645690918,0.02099977707368877
6206,12413,12412,24825,0.2570030689239502,0.020913303021499314
6306,12613,12612,25225,0.2615621089935303,0.020827199879831903
6406,12813,12812,25625,0.26665401458740234,0.02074146335821519
6507,13015,13014,26029,0.2707061767578125,0.020655237771859597
6607,13215,13214,26429,0.2746002674102783,0.020570227190828582
6707,13415,13414,26829,0.2787151336669922,0.020485573100828172
6807,13615,13614,27229,0.2826039791107178,0.02040127280177237
6907,13815,13814,27629,0.28647398948669434,0.020317323829549257
7007,14015,14014,28029,0.29040002822875977,0.020233723914058508
7107,14215,14214,28429,0.29442501068115234,0.020150470944893955
7207,14415,14414,28829,0.29851794242858887,0.020067562943277894
7307,14615,14614,29229,0.30258917808532715,0.019984998039106475
7407,14815,14814,29629,0.30667591094970703,0.019902774452176045
7508,15017,15016,30033,0.31112122535705566,0.019820073346504125
7608,15217,15216,30433,0.31519103050231934,0.019738530710620945
7708,15417,15416,30833,0.3192932605743408,0.019657324434985902
7808,15617,15616,31233,0.3233621120452881,0.019576452971328227
7908,15817,15816,31633,0.32742905616760254,0.0194959148077385
8008,16017,16016,32033,0.33158206939697266,0.01941570846305175
8108,16217,16216,32433,0.3356630802154541,0.019335832482250178
8208,16417,16416,32833,0.33975815773010254,0.01925628543269952
8308,16617,16616,33233,0.3438279628753662,0.019177065901067873
8408,16817,16816,33633,0.3481781482696533,0.019098172490801885
8509,17019,17018,34037,0.3522531986236572,0.01901881976864435
8609,17219,17218,34437,0.35626697540283203,0.018940577695431893
8709,17419,17418,34837,0.3607921600341797,0.0188626576221969
8809,17619,17618,35237,0.3652820587158203,0.018785058202323093
8909,17819,17818,35637,0.36936402320861816,0.018707778098734175
9009,18019,18018,36037,0.3736100196838379,0.018630815983125406
9109,18219,18218,36437,0.3777179718017578,0.01855417053533105
9209,18419,18418,36837,0.3817882537841797,0.018477840442803484
9309,18619,18618,37237,0.3858602046966553,0.018401824400183057
9409,18819,18818,37637,0.3899199962615967,0.018326121108942536
9510,19021,19020,38041,0.39412927627563477,0.01824997692728853
9610,19221,19220,38441,0.3981759548187256,0.01817489836439712
9710,19421,19420,38841,0.40213823318481445,0.018100128682825716
9810,19621,19620,39241,0.40610504150390625,0.018025666608942708
9910,19821,19820,39641,0.41005802154541016,0.01795151087488961
10010,20021,20020,40041,0.41402316093444824,0.017877660218460007
10110,20221,20220,40441,0.4181392192840576,0.017804113382996836
10210,20421,20420,40841,0.4221010208129883,0.01773086911730443
10310,20621,20620,41241,0.4261600971221924,0.017657926175572894
10410,20821,20820,41641,0.4301149845123291,0.01758528331731253
10511,21023,21022,42045,0.4341120719909668,0.017512217372213767
10611,21223,21222,42445,0.43808507919311523,0.01744017395041506
10711,21423,21422,42845,0.44231510162353516,0.017368426909774835
10811,21623,21622,43245,0.4463019371032715,0.01729697503062207
10911,21823,21822,43645,0.4502692222595215,0.0172258170983744
11011,22023,22022,44045,0.45433712005615234,0.01715495190350446
11111,22223,22222,44445,0.4583280086517334,0.017084378241508134
11211,22423,22422,44845,0.4622809886932373,0.017014094912875637
11311,22623,22622,45245,0.46623730659484863,0.016944100723063484
11411,22823,22822,45645,0.47032904624938965,0.01687439448246843
11512,23025,23024,46049,0.4743030071258545,0.016804282255806782
11612,23225,23224,46449,0.4782378673553467,0.016735151214378838
11712,23425,23424,46849,0.4823112487792969,0.016666304571029123
11812,23625,23624,47249,0.4862809181213379,0.01659774115572194
11912,23825,23824,47649,0.49027514457702637,0.01652945980324449
12012,24025,24024,48049,0.4945690631866455,0.016461459353185378
12112,24225,24224,48449,0.4983370304107666,0.016393738649913198
12212,24425,24424,48849,0.5020861625671387,0.016326296542556084
12312,24625,24624,49249,0.5058190822601318,0.016259131884980845
12412,24825,24824,49649,0.5095071792602539,0.016192243535772873
12513,25027,25026,50053,0.513343095779419,0.016124965612223152
12613,25227,25226,50453,0.5171399116516113,0.016058629208975092
12713,25427,25426,50853,0.5208921432495117,0.015992565706711873
12813,25627,25626,51253,0.5246310234069824,0.015926773982740765
12913,25827,25826,51653,0.5284171104431152,0.015861252918988957
13013,26027,26026,52053,0.5322270393371582,0.01579600140198428
13113,26227,26226,52453,0.5359642505645752,0.015731018322836098
13213,26427,26426,52853,0.5398991107940674,0.01566630257721642
13313,26627,26626,53253,0.5440230369567871,0.015601853065340806
13413,26827,26826,53653,0.5489370822906494,0.015537668691949714
13514,27029,27028,54057,0.5541501045227051,0.015473110492795109
13614,27229,27228,54457,0.5587470531463623,0.015409455752744657
13714,27429,27428,54857,0.5633211135864258,0.015346062881567299
13814,27629,27628,55257,0.568317174911499,0.015282930801961206
13914,27829,27828,55657,0.572749137878418,0.015220058441056731
14014,28029,28028,56057,0.5778090953826904,0.015157444730397951
14114,28229,28228,56457,0.5818061828613281,0.015095088605924645
14214,28429,28428,56857,0.5859382152557373,0.015032989007954085
14314,28629,28628,57257,0.5903000831604004,0.014971144881162992
14414,28829,28828,57657,0.5946240425109863,0.014909555174569671
14515,29031,29030,58061,0.5987870693206787,0.014847606754191575
14615,29231,29230,58461,0.602849006652832,0.014786525270388241
14715,29431,29430,58861,0.6068291664123535,0.014725695069349514
14815,29631,29630,59261,0.6108050346374512,0.014665115117324604
14915,29831,29830,59661,0.6151680946350098,0.014604784384815403
15015,30031,30030,60061,0.6191501617431641,0.014544701846559078
15115,30231,30230,60461,0.6232509613037109,0.01448486648151075
15215,30431,30430,60861,0.6275300979614258,0.014425277272825825
15315,30631,30630,61261,0.6314842700958252,0.014365933207843056
15415,30831,30830,61661,0.6356039047241211,0.014306833278067182
15516,31033,31032,62065,0.6396870613098145,0.01424738913558572
15616,31233,31232,62465,0.6436700820922852,0.01418877688358528
15716,31433,31432,62865,0.648705005645752,0.014130405756190456
15816,31633,31632,63265,0.6532611846923828,0.014072274761440025
15916,31833,31832,63665,0.6572730541229248,0.014014382911453726
16016,32033,32032,64065,0.6614441871643066,0.0139567292224153
16116,32233,32232,64465,0.665600061416626,0.013899312714555747
16216,32433,32432,64865,0.6696760654449463,0.013842132412136788
16316,32633,32632,65265,0.6737301349639893,0.013785187343434193
16416,32833,32832,65665,0.677731990814209,0.013728476540721377
16517,33035,33034,66069,0.6817142963409424,0.013671435440173726
16617,33235,33234,66469,0.6857509613037109,0.013615192600759746
16717,33435,33434,66869,0.6897521018981934,0.013559181138438509
16817,33635,33634,67269,0.6936790943145752,0.01350340010134909
16917,33835,33834,67669,0.6976170539855957,0.013447848541546467
17017,34035,34034,68069,0.7015552520751953,0.013392525514985343
17117,34235,34234,68469,0.7056329250335693,0.013337430081504184
17217,34435,34434,68869,0.7095701694488525,0.013282561304809058
17317,34635,34634,69269,0.7135601043701172,0.013227918252457985
17417,34835,34834,69669,0.7174949645996094,0.01317349999584482
17518,35037,35036,70073,0.7214810848236084,0.013118764793756114
17618,35237,35236,70473,0.7254080772399902,0.013064795582927223
17718,35437,35436,70873,0.7296030521392822,0.01301104839572354
17818,35637,35636,71273,0.7335391044616699,0.012957522318763317
17918,35837,35836,71673,0.73750901222229,0.012904216442422432
18018,36037,36036,72073,0.7415122985839844,0.012851129860818794
18118,36237,36236,72473,0.7454450130462646,0.01279826167179707
18218,36437,36436,72873,0.7493631839752197,0.012745610976913279
18318,36637,36636,73273,0.7532899379730225,0.012693176881419535
18418,36837,36836,73673,0.7572453022003174,0.012640958494248851
18519,37039,37038,74077,0.7613260746002197,0.012588435974189925
18619,37239,37238,74477,0.7652568817138672,0.012536648480033455
18719,37439,37438,74877,0.769366979598999,0.012485074034150523
18819,37639,37638,75277,0.773292064666748,0.012433711760083094
18919,37839,37838,75677,0.7772190570831299,0.012382560784978723
19019,38039,38038,76077,0.7811520099639893,0.012331620239575868
19119,38239,38238,76477,0.7850711345672607,0.01228088925818896
19219,38439,38438,76877,0.7892191410064697,0.012230366978693818
19319,38639,38638,77277,0.793126106262207,0.012180052542512906
19419,38839,38838,77677,0.7969589233398438,0.012129945094600848
19520,39041,39040,78081,0.8008460998535156,0.012079545808436398
19620,39241,39240,78481,0.8046901226043701,0.01202985183459805
19720,39441,39440,78881,0.8085460662841797,0.011980362296512089
19820,39641,39640,79281,0.8124451637268066,0.011931076353151427
19920,39841,39840,79681,0.8164150714874268,0.011881993166948941
20020,40041,40040,80081,0.8202581405639648,0.01183311190378311
20120,40241,40240,80481,0.8241310119628906,0.011784431732963906
20220,40441,40440,80881,0.8279950618743896,0.011735951827218701
20320,40641,40640,81281,0.8320162296295166,0.011687671362678157
20420,40841,40840,81681,0.8359780311584473,0.011639589518862252
20521,41043,41042,82085,0.8400139808654785,0.011591227634416544
20621,41243,41242,82485,0.8439500331878662,0.011543542549898145
20721,41443,41442,82885,0.8480823040008545,0.011496053636773956
20821,41643,41642,83285,0.8520209789276123,0.011448760088015549
20921,41843,41842,83685,0.8559520244598389,0.011401661099914676
21021,42043,42042,84085,0.8598682880401611,0.011354755872069319
21121,42243,42242,84485,0.8639211654663086,0.011308043607370302
21221,42443,42442,84885,0.8678140640258789,0.011261523511987627
21321,42643,42642,85285,0.871757984161377,0.0112151947953571
21421,42843,42842,85685,0.8756351470947266,0.011169056670166717
21522,43045,43044,86089,0.879734992980957,0.01112264982504777
21622,43245,43244,86489,0.8839521408081055,0.011076892420077013
21722,43445,43444,86889,0.8878650665283203,0.011031323256230713
21822,43645,43644,87289,0.8918561935424805,0.010985941559104768
21922,43845,43844,87689,0.8956599235534668,0.010940746557480913
22022,44045,44044,88089,0.8994722366333008,0.010895737483313583
22122,44245,44244,88489,0.9032208919525146,0.010850913571716898
22222,44445,44444,88889,0.9069671630859375,0.010806274060951618
22322,44645,44644,89289,0.9107160568237305,0.010761818192412247
22422,44845,44844,89689,0.9145369529724121,0.010717545210614084
22523,45047,45046,90093,0.9183211326599121,0.010673014371946841
22623,45247,45246,90493,0.9220809936523438,0.010629106719673554
22723,45447,45446,90893,0.9258322715759277,0.010585379698837745
22823,45647,45646,91293,0.9296250343322754,0.010541832566340786
22923,45847,45846,91693,0.9333739280700684,0.010498464582141067
23023,46047,46046,92093,0.937265157699585,0.010455275009241429
23123,46247,46246,92493,0.9410390853881836,0.010412263113676686
23223,46447,46446,92893,0.9453420639038086,0.010369428164501055
23323,46647,46646,93293,0.949099063873291,0.010326769433775803
23423,46847,46846,93693,0.9528682231903076,0.010284286196556858
23524,47049,47048,94097,0.9566593170166016,0.010241555526386868
23624,47249,47248,94497,0.9607012271881104,0.010199422850170116
23724,47449,47448,94897,0.9647140502929688,0.010157463503327056
23824,47649,47648,95297,0.9686059951782227,0.010115676772798968
23924,47849,47848,95697,0.9726309776306152,0.010074061948460666
24024,48049,48048,96097,0.9764940738677979,0.010032618323108216
24124,48249,48248,96497,0.9807159900665283,0.009991345192447064
24224,48449,48448,96897,0.984647274017334,0.00995024185508015
24324,48649,48648,97297,0.988490104675293,0.009909307612495753
24424,48849,48848,97697,0.9929032325744629,0.009868541769055873
24525,49051,49050,98101,0.9975769519805908,0.009827538495193936
24625,49251,49250,98501,1.0013749599456787,0.009787109041254165
24725,49451,49450,98901,1.0055480003356934,0.009746845909811806
24825,49651,49650,99301,1.0096821784973145,0.009706748416633661
24925,49851,49850,99701,1.0153982639312744,0.009666815880301487
25025,50051,50050,100101,1.0196411609649658,0.009627047622200218
25125,50251,50250,100501,1.0234911441802979,0.009587442966506592
25225,50451,50450,100901,1.0276331901550293,0.009548001240177635
25325,50651,50650,101301,1.0314500331878662,0.009508721772939172
25425,50851,50850,101701,1.0354349613189697,0.009469603897274465
25526,51053,51052,102105,1.0395619869232178,0.009430258189362294
25626,51253,51252,102505,1.0438709259033203,0.009391463104581561
25726,51453,51452,102905,1.0482978820800781,0.009352827618676379
25826,51653,51652,103305,1.0532422065734863,0.009314351075073826
25926,51853,51852,103705,1.0578601360321045,0.009276032819902103
26026,52053,52052,104105,1.062164068222046,0.00923787220197936
26126,52253,52252,104505,1.066918134689331,0.009199868572802628
26226,52453,52452,104905,1.071547031402588,0.009162021286536771
26326,52653,52652,105305,1.0760669708251953,0.009124329700003632
26426,52853,52852,105705,1.0801610946655273,0.009086793172670976
26527,53055,53054,106109,1.0842421054840088,0.009049038023257273
26627,53255,53254,106509,1.0890002250671387,0.009011811237919354
26727,53455,53454,106909,1.0932800769805908,0.008974737599638951
26827,53655,53654,107309,1.0972881317138672,0.008937816478385275
26927,53855,53854,107709,1.101464033126831,0.008901047246719404
27027,54055,54054,108109,1.1054801940917969,0.008864429279783642
27127,54255,54254,108509,1.1096251010894775,0.008827961955290868
27227,54455,54454,108909,1.1138370037078857,0.008791644653514006
27327,54655,54654,109309,1.1180031299591064,0.008755476757275497
27427,54855,54854,109709,1.1226401329040527,0.008719457651936706
27528,55057,55056,110113,1.126812219619751,0.008683228762360428
27628,55257,55256,110513,1.1310851573944092,0.008647506877631283
27728,55457,55456,110913,1.1350481510162354,0.00861193194895774
27828,55657,55656,111313,1.1389849185943604,0.008576503371778088
27928,55857,55856,111713,1.143226146697998,0.008541220544017788
28028,56057,56056,112113,1.1476221084594727,0.00850608286607914
28128,56257,56256,112513,1.1526870727539062,0.008471089740831111
28228,56457,56456,112913,1.157310962677002,0.008436240573599233
28328,56657,56656,113313,1.1618170738220215,0.008401534772155474
28428,56857,56856,113713,1.1664760112762451,0.008366971746708104
28529,57059,57058,114117,1.1721351146697998,0.008332207417595033
28629,57259,57258,114517,1.1775360107421875,0.008297929597551771
28729,57459,57458,114917,1.1830260753631592,0.008263792792834741
28829,57659,57658,115317,1.1884031295776367,0.008229796423321747
28929,57859,57858,115717,1.1939740180969238,0.008195939911277242
29029,58059,58058,116117,1.1993741989135742,0.008162222681342373
29129,58259,58258,116517,1.2045209407806396,0.008128644160525297
29229,58459,58458,116917,1.209618091583252,0.008095203778191359
29329,58659,58658,117317,1.214677095413208,0.00806190096605345
29429,58859,58858,117717,1.2195031642913818,0.008028735158162345
29530,59061,59060,118121,1.2237060070037842,0.007995376184348438
29630,59261,59260,118521,1.227769136428833,0.007962484052373132
29730,59461,59460,118921,1.23183012008667,0.007929727235149852
29830,59661,59660,119321,1.2358620166778564,0.007897105176008062
29930,59861,59860,119721,1.2398719787597656,0.007864617320567235
30030,60061,60060,120121,1.2440011501312256,0.007832263116727552
30130,60261,60260,120521,1.248466968536377,0.007800042014660447
30230,60461,60460,120921,1.2526161670684814,0.007767953466799313
30330,60661,60660,121321,1.256519079208374,0.007735996927830199
30430,60861,60860,121721,1.2606582641601562,0.007704171854682442
30531,61063,61062,122125,1.2650041580200195,0.007672161424384856
30631,61263,61262,122525,1.2694041728973389,0.0076405989637465845
30731,61463,61462,122925,1.273772954940796,0.007609166347733111
30831,61663,61662,123325,1.2784199714660645,0.0075778630421773656
30931,61863,61862,123725,1.2823750972747803,0.0075466885151098265
31031,62063,62062,124125,1.2866101264953613,0.007515642236749418
31131,62263,62262,124525,1.2905709743499756,0.007484723679494517
31231,62463,62462,124925,1.2947142124176025,0.007453932317913985
31331,62663,62662,125325,1.298706293106079,0.007423267628738286
31431,62863,62862,125725,1.3027739524841309,0.007392729090850528
31532,63065,63064,126129,1.3072528839111328,0.007362012688914633
31632,63265,63264,126529,1.3116331100463867,0.007331726147370554
31732,63465,63464,126929,1.3157880306243896,0.007301564201455097
31832,63665,63664,127329,1.320909023284912,0.007271526338594972
31932,63865,63864,127729,1.3253450393676758,0.007241612048325651
32032,64065,64064,128129,1.3304932117462158,0.007211820822282571
32132,64265,64264,128529,1.335482120513916,0.007182152154192482
32232,64465,64464,128929,1.3404242992401123,0.007152605539864971
32332,64665,64664,129329,1.345487117767334,0.007123180477183726
32432,64865,64864,129729,1.350135087966919,0.007093876466098154
32533,65067,65066,130133,1.3543200492858887,0.007064401781155894
32633,65267,65266,130533,1.35843825340271,0.007035339579408933
32733,65467,65466,130933,1.3631842136383057,0.007006396936486132
32833,65667,65666,131333,1.3674860000610352,0.0069775733605351295
32933,65867,65866,131733,1.3714392185211182,0.006948868361727015
33033,66067,66066,132133,1.3754560947418213,0.006920281452247954
33133,66267,66266,132533,1.3797800540924072,0.006891812146290943
33233,66467,66466,132933,1.3843541145324707,0.006863459960047532
33333,66667,66666,133333,1.388416051864624,0.006835224411699583
33433,66867,66866,133733,1.3926060199737549,0.006807105021411168
33534,67069,67068,134137,1.397078037261963,0.006778821856792532
33634,67269,67268,134537,1.401266098022461,0.006750934500649469
33734,67469,67468,134937,1.405649185180664,0.00672316187014001
33834,67669,67668,135337,1.4102470874786377,0.006695503493295036
33934,67869,67868,135737,1.4148521423339844,0.006667958900087056
34034,68069,68068,136137,1.4191012382507324,0.006640527622422218
34134,68269,68268,136537,1.4235708713531494,0.006613209194132384
34234,68469,68468,136937,1.427860975265503,0.006586003150967135
34334,68669,68668,137337,1.4323320388793945,0.006558909030585957
34434,68869,68868,137737,1.4367852210998535,0.00653192637255039
34535,69071,69070,138141,1.4409420490264893,0.006504786560796256
34635,69271,69270,138541,1.4451451301574707,0.006478026556877027
34735,69471,69470,138941,1.4503579139709473,0.006451376640783591
34835,69671,69670,139341,1.454531192779541,0.006424836359626273
34935,69871,69870,139741,1.4586851596832275,0.0063984052623785575
35035,70071,70070,140141,1.4633700847625732,0.0063720828998694015
35135,70271,70270,140541,1.4675321578979492,0.0063458688247755345
35235,70471,70470,140941,1.4717559814453125,0.006319762591614038
35335,70671,70670,141341,1.4758851528167725,0.006293763756734599
35435,70871,70870,141741,1.4801380634307861,0.006267871878312006
35536,71073,71072,142145,1.484264850616455,0.006241829199142931
35636,71273,71272,142545,1.4884510040283203,0.006216150973997304
35736,71473,71472,142945,1.492661952972412,0.006190578386354045
35836,71673,71672,143345,1.4967260360717773,0.006165111001631597
35936,71873,71872,143745,1.5008361339569092,0.006139748387036292
36036,72073,72072,144145,1.504967212677002,0.006114490111554905
36136,72273,72272,144545,1.5090980529785156,0.0060893357459473624
36236,72473,72472,144945,1.5131499767303467,0.006064284862739422
36336,72673,72672,145345,1.517212152481079,0.0060393370362154435
36436,72873,72872,145745,1.5212771892547607,0.006014491842411115
36537,73075,73074,146149,1.525362253189087,0.005989501944012134
36637,73275,73274,146549,1.5295469760894775,0.005964861766506236
36737,73475,73474,146949,1.5337352752685547,0.005940322956084465
36837,73675,73674,147349,1.5377681255340576,0.005915885095733384
36937,73875,73874,147749,1.5418212413787842,0.0058915477701550695
37037,74075,74074,148149,1.545882225036621,0.005867310565760089
37137,74275,74274,148549,1.55000901222229,0.0058431730706605236
37237,74475,74474,148949,1.5542190074920654,0.005819134874662815
37337,74675,74674,149349,1.5583479404449463,0.005795195569261004
37437,74875,74874,149749,1.562596082687378,0.005771354747629617
37538,75077,75076,150153,1.5668652057647705,0.0057473750711171815
37638,75277,75276,150553,1.5710961818695068,0.005723730977957329
37738,75477,75476,150953,1.575301170349121,0.005700184154095967
37838,75677,75676,151353,1.5795261859893799,0.005676734199377498
37938,75877,75876,151753,1.5837931632995605,0.005653380715292511
38038,76077,76076,152153,1.5879302024841309,0.005630123304971026
38138,76277,76276,152553,1.5922322273254395,0.005606961573175729
38238,76477,76476,152953,1.5964231491088867,0.005583895126295303
38338,76677,76676,153353,1.6006519794464111,0.005560923572337659
38438,76877,76876,153753,1.6048979759216309,0.005538046520923362
38539,77079,77078,154157,1.6090753078460693,0.005515036227865703
38639,77279,77278,154557,1.6133301258087158,0.005492347952133196
38739,77479,77478,154957,1.6174850463867188,0.005469753013567384
38839,77679,77678,155357,1.621725082397461,0.005447251028189034
38939,77879,77878,155757,1.6259970664978027,0.0054248416135985736
39039,78079,78078,156157,1.630958080291748,0.005402524388969544
39139,78279,78278,156557,1.635099172592163,0.005380298975042232
39239,78479,78478,156957,1.6393489837646484,0.005358164994117084
39339,78679,78678,157357,1.6435890197753906,0.0053361220700484215
39439,78879,78878,157757,1.6478462219238281,0.005314169828237971
39540,79081,79080,158161,1.65214204788208,0.005292089731105537
39640,79281,79280,158561,1.6563019752502441,0.005270318633680339
39740,79481,79480,158961,1.6604421138763428,0.0052486371002472615
39840,79681,79680,159361,1.6646831035614014,0.005227044762349522
39940,79881,79880,159761,1.6689331531524658,0.005205541253046146
40040,80081,80080,160161,1.6730711460113525,0.005184126206905686
40140,80281,80280,160561,1.6772222518920898,0.005162799260000051
40240,80481,80480,160961,1.681467056274414,0.005141560049898295
40340,80681,80680,161361,1.6856372356414795,0.005120408215660488
40440,80881,80880,161761,1.6897892951965332,0.005099343397831577
40541,81083,81082,162165,1.6940820217132568,0.0050781558932589165
40641,81283,81282,162565,1.698256254196167,0.005057264897015461
40741,81483,81482,162965,1.7024362087249756,0.00503645984412097
40841,81683,81682,163365,1.7067761421203613,0.005015740381013602
40941,81883,81882,163765,1.7110099792480469,0.0049951061555860285
41041,82083,82082,164165,1.7152140140533447,0.004974556817179435
41141,82283,82282,164565,1.719468116760254,0.004954092016577594
41241,82483,82482,164965,1.723667860031128,0.004933711406000938
41341,82683,82682,165365,1.7278079986572266,0.004913414639100601
41441,82883,82882,165765,1.7320561408996582,0.004893201370952563
41542,83085,83084,166169,1.7363619804382324,0.004872870375698116
41642,83285,83284,166569,1.7405319213867188,0.004852823902361474
41742,83485,83484,166969,1.7446610927581787,0.004832859898095875
41842,83685,83684,167369,1.7488722801208496,0.004812978023632288
41942,83885,83884,167769,1.7531170845031738,0.004793177941097396
42042,84085,84084,168169,1.7573418617248535,0.004773459314007856
42142,84285,84284,168569,1.7614710330963135,0.004753821807264584
42242,84485,84484,168969,1.765606164932251,0.0047342650871470575
42342,84685,84684,169369,1.7697980403900146,0.004714788821307638
42442,84885,84884,169769,1.7740490436553955,0.004695392678765937
42543,85087,85086,170173,1.7784221172332764,0.004675883568260828
42643,85287,85286,170573,1.7826790809631348,0.004656647477815262
42743,85487,85486,170973,1.7869250774383545,0.004637490522611249
42843,85687,85686,171373,1.7911641597747803,0.004618412377094773
42943,85887,85886,171773,1.7953600883483887,0.004599412717051115
43043,86087,86086,172173,1.799626111984253,0.004580491219599321
43143,86287,86286,172573,1.8038020133972168,0.004561647563186797
43243,86487,86486,172973,1.8079442977905273,0.004542881427583712
43343,86687,86686,173373,1.8121490478515625,0.004524192493877646
43443,86887,86886,173773,1.8163912296295166,0.004505580444468188
43544,87089,87088,174177,1.8205952644348145,0.004486859993848942
43644,87289,87288,174577,1.8247590065002441,0.004468401526396055
43744,87489,87488,174977,1.8291351795196533,0.004450018995125976
43844,87689,87688,175377,1.8333990573883057,0.004431712087645273
43944,87889,87888,175777,1.8381991386413574,0.004413480492845678
44044,88089,88088,176177,1.8424110412597656,0.004395323900898777
44144,88289,88288,176577,1.8466742038726807,0.0043772420032507885
44244,88489,88488,176977,1.8504791259765625,0.004359234492617242
44344,88689,88688,177377,1.854259967803955,0.004341301062977856
44444,88889,88888,177777,1.858546257019043,0.004323441409571246
44545,89091,89090,178181,1.8623402118682861,0.004305477737096482
44645,89291,89290,178581,1.8678321838378906,0.004287765457063616
44745,89491,89490,178981,1.8718981742858887,0.004270126043477431
44845,89691,89690,179381,1.875899076461792,0.00425255919657306
44945,89891,89890,179781,1.8798582553863525,0.00423506461781887
45045,90091,90090,180181,1.8836300373077393,0.00421764200991132
45145,90291,90290,180581,1.8874211311340332,0.004200291076769972
45245,90491,90490,180981,1.8913002014160156,0.004183011523532391
45345,90691,90690,181381,1.895211935043335,0.004165803056549231
45445,90891,90890,181781,1.8990600109100342,0.004148665383379156
45546,91093,91092,182185,1.9031410217285156,0.0041314278961336074
45646,91293,91292,182585,1.9073431491851807,0.004114431638737725
45746,91493,91492,182985,1.9114181995391846,0.004097505302147127
45846,91693,91692,183385,1.916445255279541,0.004080648598715015
45946,91893,91892,183785,1.921093225479126,0.0040638612419779405
46046,92093,92092,184185,1.9253759384155273,0.0040471429466509235
46146,92293,92292,184585,1.9297599792480469,0.004030493428622653
46246,92493,92492,184985,1.933933973312378,0.0040139124049505676
46346,92693,92692,185385,1.93784499168396,0.003997399593856141
46446,92893,92892,185785,1.9418540000915527,0.003980954714720053
46547,93095,93094,186189,1.9458322525024414,0.003964414056513435
46647,93295,93294,186589,1.9497380256652832,0.003948104876389191
46747,93495,93494,186989,1.9538002014160156,0.00393186279050701
46847,93695,93694,187389,1.9580039978027344,0.003915687522848269
46947,93895,93894,187789,1.962663173675537,0.003899578798529858
47047,94095,94094,188189,1.967353105545044,0.003883536343799519
47147,94295,94294,188589,1.9725430011749268,0.003867559886031196
47247,94495,94494,188989,1.9767701625823975,0.0038516491537203333
47347,94695,94694,189389,1.9814090728759766,0.003835803876479375
47447,94895,94894,189789,1.9858360290527344,0.0038200237850330694
47548,95097,95096,190193,1.9898622035980225,0.0038041517864052616
47648,95297,95296,190593,1.9938008785247803,0.0037885019083097856
47748,95497,95496,190993,1.9977970123291016,0.0037729164121575445
47848,95697,95696,191393,2.001753091812134,0.0037573950330880546
47948,95897,95896,191793,2.005697011947632,0.003741937507330403
48048,96097,96096,192193,2.0096471309661865,0.003726543572198825
48148,96297,96296,192593,2.0136210918426514,0.0037112129660882044
48248,96497,96496,192993,2.018357038497925,0.0036959454284696516
48348,96697,96696,193393,2.0224449634552,0.0036807406998860446
48448,96897,96896,193793,2.026492118835449,0.0036655985219476842
48549,97099,97098,194197,2.0305590629577637,0.0036503681521949135
48649,97299,97298,194597,2.0346779823303223,0.0036353509237053447
48749,97499,97498,194997,2.038794994354248,0.003620395474505458
48849,97699,97698,195397,2.042757034301758,0.003605501550441781
48949,97899,97898,195797,2.0467541217803955,0.003590668898406413
49049,98099,98098,196197,2.050711154937744,0.0035758972663327026
49149,98299,98298,196597,2.054669141769409,0.0035611864031910023
49249,98499,98498,196997,2.058642864227295,0.0035465360589843316
49349,98699,98698,197397,2.0625970363616943,0.0035319459847442335
49449,98899,98898,197797,2.067305088043213,0.0035174159325263876
49550,99101,99100,198201,2.0714008808135986,0.003502801253666727
49650,99301,99300,198601,2.0754711627960205,0.003488391099789987
49750,99501,99500,199001,2.0795161724090576,0.003474040227762176
49850,99701,99700,199401,2.08347487449646,0.00345974839370404
49950,99901,99900,199801,2.087563991546631,0.003445515354739607
50050,100101,100100,200201,2.091517925262451,0.003431340868992097
50150,100301,100300,200601,2.0954182147979736,0.0034172246955797496
50250,100501,100500,201001,2.0992770195007324,0.003403166594611812
50350,100701,100700,201401,2.103113889694214,0.0033891663271843615
50450,100901,100900,201801,2.10695219039917,0.003375223655376346
50551,101103,101102,202205,2.110896110534668,0.003361199777976271
50651,101303,101302,202605,2.114927053451538,0.00334737215759376
50751,101503,101502,203005,2.1188101768493652,0.00333360142257898
50851,101703,101702,203405,2.1227121353149414,0.0033198873389115777
50951,101903,101902,203805,2.1266181468963623,0.003306229673533883
51051,102103,102102,204205,2.1305010318756104,0.003292628194347024
51151,102303,102302,204605,2.134335994720459,0.0032790826702069516
51251,102503,102502,205005,2.138216257095337,0.0032655928709205283
51351,102703,102702,205405,2.1420531272888184,0.0032521585672415864
51451,102903,102902,205805,2.145983934402466,0.003238779530867077
51552,103105,103104,206209,2.1498641967773438,0.0032253225716536013
51652,103305,103304,206609,2.153797149658203,0.003212053935726564
51752,103505,103504,207009,2.1580002307891846,0.0031988398855643464
51852,103705,103704,207409,2.1624629497528076,0.003185680196606894
51952,103905,103904,207809,2.166996955871582,0.003172574645217944
52052,104105,104104,208209,2.170894145965576,0.0031595230086812944
52152,104305,104304,208609,2.174776077270508,0.003146525065196907
52252,104505,104504,209009,2.178746223449707,0.0031335805938772707
52352,104705,104704,209409,2.1825919151306152,0.003120689374743531
52452,104905,104904,209809,2.1865899562835693,0.0031078511887218507
52553,105107,105106,210213,2.1904749870300293,0.0030949382299083083
52653,105307,105306,210613,2.19441294670105,0.003082205981372849
52753,105507,105506,211013,2.19850492477417,0.0030695261119612276
52853,105707,105706,211413,2.202594041824341,0.003056898406191248
52953,105907,105906,211813,2.2067770957946777,0.003044322649467209
53053,106107,106106,212213,2.210813283920288,0.003031798628076219
53153,106307,106306,212613,2.215015172958374,0.0030193261291846262
53253,106507,106506,213013,2.2189621925354004,0.0030069049408342867
53353,106707,106706,213413,2.222851037979126,0.0029945348519390645
53453,106907,106906,213813,2.226912021636963,0.0029822156522812003
53554,107109,107108,214217,2.230988025665283,0.002969824702537307
53654,107309,107308,214617,2.23488712310791,0.002957607157820564
53754,107509,107508,215017,2.238758087158203,0.002945439874790568
53854,107709,107708,215417,2.2426531314849854,0.002933322646676077
53954,107909,107908,215817,2.24652099609375,0.0029212552675564546
54054,108109,108108,216217,2.250386953353882,0.002909237532358191
54154,108309,108308,216617,2.2543039321899414,0.002897269236851446
54254,108509,108508,217017,2.2581632137298584,0.0028853501776465677
54354,108709,108708,217417,2.262083053588867,0.0028734801521906176
54454,108909,108908,217817,2.2659902572631836,0.0028616589587639393
54555,109111,109110,218221,2.2698869705200195,0.0028497689157634975
54655,109311,109310,218621,2.2737619876861572,0.0028380452678556027
54755,109511,109510,219021,2.277714967727661,0.002826369849795231
54855,109711,109710,219421,2.2816290855407715,0.002814742463169884
54955,109911,109910,219821,2.285494089126587,0.002803162910383327
55055,110111,110110,220221,2.2893600463867188,0.0027916309946521838
55155,110311,110310,220621,2.2932002544403076,0.0027801465200026636
55255,110511,110510,221021,2.297118902206421,0.002768709291267182
55355,110711,110710,221421,2.300899028778076,0.002757319114081033
55455,110911,110910,221821,2.304965019226074,0.0027459757948791255
55556,111113,111112,222225,2.3094210624694824,0.00273456640936194
55656,111313,111312,222625,2.313225030899048,0.0027233166923807577
55756,111513,111512,223025,2.317125082015991,0.0027121132555454016
55856,111713,111712,223425,2.3209149837493896,0.002700955908464218
55956,111913,111912,223825,2.3246772289276123,0.0026898444615288527
56056,112113,112112,224225,2.328550100326538,0.002678778725910949
56156,112313,112312,224625,2.3323190212249756,0.0026677585135589927
56256,112513,112512,225025,2.3361918926239014,0.002656783637195071
56356,112713,112712,225425,2.3400800228118896,0.0026458539103117354
56456,112913,112912,225825,2.3440821170806885,0.002634969147168808
56557,113115,113114,226229,2.348036050796509,0.0026240209884552273
56657,113315,113314,226629,2.3518362045288086,0.0026132260436435933
56757,113515,113514,227029,2.355675220489502,0.0026024755080931777
56857,113715,113714,227429,2.359462261199951,0.002591769199108963
56957,113915,113914,227829,2.3634631633758545,0.0025811069347475447
57057,114115,114114,228229,2.3676280975341797,0.002570488533813974
57157,114315,114314,228629,2.3718321323394775,0.002559913815858767
57257,114515,114514,229029,2.375697135925293,0.002549382601174776
57357,114715,114714,229429,2.3795711994171143,0.0025388947107941365
57457,114915,114914,229829,2.3834311962127686,0.0025284499664852606
57558,115117,115116,230233,2.3873112201690674,0.002517944389384992
57658,115317,115316,230633,2.391184091567993,0.002507585832482533
57758,115517,115516,231033,2.394991159439087,0.002497269889587577
57858,115717,115716,231433,2.3988568782806396,0.002486996385390603
57958,115917,115916,231833,2.4027771949768066,0.002476765145303307
58058,116117,116116,232233,2.4065699577331543,0.0024665759954555846
58158,116317,116316,232633,2.410529136657715,0.002456428762692665
58258,116517,116516,233033,2.414454936981201,0.002446323274572094
58358,116717,116716,233433,2.4183762073516846,0.0024362593593608246
58458,116917,116916,233833,2.4222850799560547,0.00242623684603231
58559,117119,117118,234237,2.4262380599975586,0.0024161559590907575
58659,117319,117318,234637,2.430109977722168,0.0024062161490246686
58759,117519,117518,235037,2.434115171432495,0.0023963172302858896
58859,117719,117718,235437,2.437952995300293,0.0023864590346518114
58959,117919,117918,235837,2.4417781829833984,0.0023766413945919148
59059,118119,118118,236237,2.445823907852173,0.0023668641432648277
59159,118319,118318,236637,2.4496071338653564,0.0023571271145156024
59259,118519,118518,237037,2.453782081604004,0.0023474301428727863
59359,118719,118718,237437,2.4576821327209473,0.002337773063545691
59459,118919,118918,237837,2.461740016937256,0.0023281557124215464
59560,119121,119120,238241,2.465588092803955,0.0023184823474499345
59660,119321,119320,238641,2.469618082046509,0.002308944356291497
59760,119521,119520,239041,2.4734740257263184,0.0022994456034198755
59860,119721,119720,239441,2.477555990219116,0.002289985927412913
59960,119921,119920,239841,2.481586217880249,0.0022805651675125134
60060,120121,120120,240241,2.4854190349578857,0.0022711831636219463
60160,120321,120320,240641,2.4894251823425293,0.0022618397563030795
60260,120521,120520,241041,2.4934372901916504,0.0022525347867736975
60360,120721,120720,241441,2.4985709190368652,0.0022432680969048063
60460,120921,120920,241841,2.5028669834136963,0.0022340395292179192
60561,121123,121122,242245,2.5074622631073,0.002224757212055106
60661,121323,121322,242645,2.512153148651123,0.0022156047961906537
60761,121523,121522,243045,2.516890048980713,0.0022064900323970297
60861,121723,121722,243445,2.522747039794922,0.0021974127657776177
60961,121923,121922,243845,2.527501106262207,0.002188372842073003
61061,122123,122122,244245,2.5315771102905273,0.002179370107658379
61161,122323,122322,244645,2.5355210304260254,0.0021704044095409553
61261,122523,122522,245045,2.5393800735473633,0.002161475595357307
61361,122723,122722,245445,2.5432300567626953,0.002152583513370839
61461,122923,122922,245845,2.5470991134643555,0.002143728012469163
61562,123125,123124,246249,2.5509960651397705,0.002134820934925411
61662,123325,123324,246649,2.555021047592163,0.002126038507392765
61762,123525,123524,247049,2.5590810775756836,0.002117292209838103
61862,123725,123724,247449,2.563133955001831,0.002108581893626524
61962,123925,123924,247849,2.5672309398651123,0.0020999074107345707
62062,124125,124124,248249,2.571460008621216,0.0020912686137477534
62162,124325,124324,248649,2.575634241104126,0.0020826653558580453
62262,124525,124524,249049,2.579768180847168,0.0020740974908613615
62362,124725,124724,249449,2.583954095840454,0.0020655648731550767
62462,124925,124924,249849,2.588083267211914,0.002057067357735554
62563,125127,125126,250253,2.592586040496826,0.002048520350670511
62663,125327,125326,250653,2.596724033355713,0.002040092954613752
62763,125527,125526,251053,2.600939989089966,0.0020317002279730155
62863,125727,125726,251453,2.6050732135772705,0.002023342028122002
62963,125927,125926,251853,2.6092379093170166,0.002015018213021156
63063,126127,126126,252253,2.613415241241455,0.0020067286412152655
63163,126327,126326,252653,2.6175670623779297,0.0019984731718310084
63263,126527,126526,253053,2.621795177459717,0.001990251664574641
63363,126727,126726,253453,2.626000165939331,0.0019820639797295697
63463,126927,126926,253853,2.6300289630889893,0.001973909978153963
63564,127129,127128,254257,2.6340630054473877,0.0019657084856429846
63664,127329,127328,254657,2.6381640434265137,0.0019576217688401843
63764,127529,127528,255057,2.6421329975128174,0.0019495683199349915
63864,127729,127728,255457,2.6462361812591553,0.001941548002066804
63964,127929,127928,255857,2.6502010822296143,0.001933560678938055
64064,128129,128128,256257,2.6541781425476074,0.0019256062148118587
64164,128329,128328,256657,2.6581192016601562,0.0019176844745097572
64264,128529,128528,257057,2.662067174911499,0.001909795323409397
64364,128729,128728,257457,2.666079044342041,0.0019019386274422444
64464,128929,128928,257857,2.670044183731079,0.0018941142530913338
64565,129131,129130,258261,2.6740641593933105,0.0018862443076360902
64665,129331,129330,258661,2.6780130863189697,0.0018784844980569133
64765,129531,129530,259061,2.6819770336151123,0.0018707566115136087
64865,129731,129730,259461,2.6859281063079834,0.0018630605166781858
64965,129931,129930,259861,2.6899912357330322,0.001855396082762924
65065,130131,130130,260261,2.6941370964050293,0.00184776317951815
65165,130331,130330,260661,2.697991132736206,0.0018401616772300232
65265,130531,130530,261061,2.701833963394165,0.001832591446718308
65365,130731,130730,261461,2.705677032470703,0.0018250523593342407
65465,130931,130930,261861,2.7095091342926025,0.0018175442869582783
65566,131133,131132,262265,2.713608980178833,0.001809992485699441
65666,131333,131332,262665,2.717433214187622,0.0018025463680507784
65766,131533,131532,263065,2.7212741374969482,0.001795130882942572
65866,131733,131732,263465,2.7250969409942627,0.0017877459043557924
65966,131933,131932,263865,2.7289059162139893,0.0017803913067898248
66066,132133,132132,264265,2.732745885848999,0.0017730669652603658
66166,132333,132332,264665,2.7365639209747314,0.0017657727552972784
66266,132533,132532,265065,2.7403719425201416,0.0017585085529425069
66366,132733,132732,265465,2.7442259788513184,0.0017512742347479118
66466,132933,132932,265865,2.7480759620666504,0.0017440696777732204
66567,133135,133134,266269,2.751953125,0.001736823159664914
66667,133335,133334,266669,2.755751132965088,0.0017296780528846538
66767,133535,133534,267069,2.759554147720337,0.0017225623403179775
66867,133735,133734,267469,2.7634270191192627,0.0017154759010401923
66967,133935,133934,267869,2.7672481536865234,0.0017084186146240808
67067,134135,134134,268269,2.771076202392578,0.0017013903611378695
67167,134335,134334,268669,2.7749061584472656,0.001694391021143133
67267,134535,134534,269069,2.778722047805786,0.0016874204756928367
67367,134735,134734,269469,2.7825331687927246,0.0016804786063292691
67467,134935,134934,269869,2.7863340377807617,0.0016735652950820312
67568,135137,135136,270273,2.790178060531616,0.001666611718988814
67668,135337,135336,270673,2.7940380573272705,0.0016597554546494539
67768,135537,135536,271073,2.798145055770874,0.0016529273962564194
67868,135737,135736,271473,2.8029732704162598,0.001646127427773425
67968,135937,135936,271873,2.8073770999908447,0.0016393554336415486
68068,136137,136136,272273,2.8113012313842773,0.001632611298777284
68168,136337,136336,272673,2.815762996673584,0.0016258949085705442
68268,136537,136536,273073,2.81977915763855,0.001619206148882733
68368,136737,136736,273473,2.8243091106414795,0.001612544906044839
68468,136937,136936,273873,2.8283021450042725,0.0016059110668554268
68569,137139,137138,274277,2.8325490951538086,0.0015992385905348953
68669,137339,137338,274677,2.8366241455078125,0.0015926594921201371
68769,137539,137538,275077,2.8404250144958496,0.0015861074594204127
68869,137739,137738,275477,2.8442962169647217,0.0015795823810902084
68969,137939,137938,275877,2.848341941833496,0.0015730841462421178
69069,138139,138138,276277,2.852306842803955,0.0015666126444448963
69169,138339,138338,276677,2.8561041355133057,0.0015601677657215997
69269,138539,138538,277077,2.8598179817199707,0.0015537494005477077
69369,138739,138738,277477,2.8635692596435547,0.0015473574398492983
69469,138939,138938,277877,2.8674070835113525,0.0015409917750011423
69570,139141,139140,278281,2.8713600635528564,0.0015345890349359838
69670,139341,139340,278681,2.875135898590088,0.0015282758979551663
69770,139541,139540,279081,2.8791401386260986,0.001521988732552163
69870,139741,139740,279481,2.883018970489502,0.0015157274318826548
69970,139941,139940,279881,2.886850118637085,0.0015094918895418635
70070,140141,140140,280281,2.8908801078796387,0.0015032819995627511
70170,140341,140340,280681,2.894803047180176,0.0014970976564141962
70270,140541,140540,281081,2.898698091506958,0.001490938754999273
70370,140741,140740,281481,2.903381109237671,0.0014848051906533562
70470,140941,140940,281881,2.907392978668213,0.0014786968591424235
70571,141143,141142,282285,2.911487102508545,0.0014725529511879349
70671,141343,141342,282685,2.9155020713806152,0.0014664950240942938
70771,141543,141542,283085,2.9197349548339844,0.0014604620186719783
70871,141743,141742,283485,2.923704147338867,0.001454453832395876
70971,141943,141942,283885,2.927739143371582,0.00144847036316264
71071,142143,142142,284285,2.9316470623016357,0.0014425115092889865
71171,142343,142342,284685,2.9355452060699463,0.0014365771695099103
71271,142543,142542,285085,2.939439058303833,0.0014306672429770244
71371,142743,142742,285485,2.9433772563934326,0.0014247816292568235
71471,142943,142942,285885,2.9474339485168457,0.0014189202283289575
71572,143145,143144,286289,2.951399087905884,0.0014130246891427183
71672,143345,143344,286689,2.955310106277466,0.0014072116550229877
71772,143545,143544,287089,2.959230899810791,0.001401422535110811
71872,143745,143744,287489,2.9632692337036133,0.001395657231025652
71972,143945,143944,287889,2.9673142433166504,0.0013899156447917012
72072,144145,144144,288289,2.971369981765747,0.0013841976788362704
72172,144345,144344,288689,2.975304126739502,0.0013785032359880003
72272,144545,144544,289089,2.97920298576355,0.001372832219475324
72372,144745,144744,289489,2.983100175857544,0.001367184532924772
72472,144945,144944,289889,2.986973285675049,0.001361560080359351
72573,145147,145146,290293,2.9908900260925293,0.0013559028695818089
72673,145347,145346,290693,2.994753122329712,0.0013503248285861524
72773,145547,145546,291093,2.9985899925231934,0.0013447697350611769
72873,145747,145746,291493,3.002389907836914,0.001339237494603421
72973,145947,145946,291893,3.006186008453369,0.001333728013197769
73073,146147,146146,292293,3.0100090503692627,0.0013282411972158998
73173,146347,146346,292693,3.0140249729156494,0.0013227769534146663
73273,146547,146546,293093,3.0180561542510986,0.0013173351889344982
73373,146747,146746,293493,3.0222089290618896,0.0013119158112978406
73473,146947,146946,293893,3.026095151901245,0.0013065187284075806
73574,147149,147148,294297,3.030019998550415,0.0013010902115628044
73674,147349,147348,294697,3.0338852405548096,0.0012957376640448696
73774,147549,147548,295097,3.0377700328826904,0.0012904071363412947
73874,147749,147748,295497,3.0417861938476562,0.0012850985378648904
73974,147949,147948,295897,3.045875310897827,0.0012798117784011552
74074,148149,148148,296297,3.049718141555786,0.0012745467681066836
74174,148349,148348,296697,3.0543291568756104,0.001269303417507698
74274,148549,148548,297097,3.0584890842437744,0.0012640816374985138
74374,148749,148748,297497,3.062343120574951,0.0012588813393399842
74474,148949,148948,297897,3.066356897354126,0.0012537024346580565
74575,149151,149150,298301,3.0701942443847656,0.001248493366745823
74675,149351,149350,298701,3.074120283126831,0.0012433571970844517
74775,149551,149550,299101,3.0780138969421387,0.0012382421570818233
74875,149751,149750,299501,3.081794023513794,0.0012331481598127723
74975,149951,149950,299901,3.08559513092041,0.0012280751187097034
75075,150151,150150,300301,3.089437246322632,0.0012230229475611747
75175,150351,150350,300701,3.0932552814483643,0.0012179915605103951
75275,150551,150550,301101,3.0971219539642334,0.001212980872053783
75375,150751,150750,301501,3.1011099815368652,0.0012079907970395229
75475,150951,150950,301901,3.105386972427368,0.0012030212506660963
75576,151153,151152,302305,3.109337091445923,0.0011980227604172593
75676,151353,151352,302705,3.113215923309326,0.0011930942214922022
75776,151553,151552,303105,3.117711067199707,0.0011881859580550004
75876,151753,151752,303505,3.121809244155884,0.001183297886694451
75976,151953,151952,303905,3.1259021759033203,0.001178429924342487
76076,152153,152152,304305,3.1297600269317627,0.0011735819882727528
76176,152353,152352,304705,3.133815050125122,0.0011687539960992717
76276,152553,152552,305105,3.137727975845337,0.0011639458657749313
76376,152753,152752,305505,3.141606092453003,0.0011591575155902255
76476,152953,152952,305905,3.1455280780792236,0.001154388864171719
76577,153155,153154,306309,3.1495091915130615,0.0011495924389400586
76677,153355,153354,306709,3.1533710956573486,0.001144863137235229
76777,153555,153554,307109,3.157231092453003,0.001140153291377413
76877,153755,153754,307509,3.161393165588379,0.0011354628213273007
76977,153955,153954,307909,3.165436267852783,0.0011307916473748854
77077,154155,154154,308309,3.1693811416625977,0.0011261396901380532
77177,154355,154354,308709,3.1732993125915527,0.0011215068705612604
77277,154555,154554,309109,3.1772470474243164,0.0011168931099141952
77377,154755,154754,309509,3.181220054626465,0.0011122983297904595
77477,154955,154954,309909,3.185124158859253,0.0011077224521061743
77578,155157,155156,310313,3.1890621185302734,0.0011031199233709635
77678,155357,155356,310713,3.192978858947754,0.0010985818046799188
77778,155557,155556,311113,3.1969780921936035,0.0010940623553291973
77878,155757,155756,311513,3.2009332180023193,0.0010895614985150842
77978,155957,155956,311913,3.2048420906066895,0.0010850791577498718
78078,156157,156156,312313,3.208735942840576,0.001080615256860472
78178,156357,156356,312713,3.2127292156219482,0.0010761697199872051
78278,156557,156556,313113,3.216768980026245,0.0010717424715824412
78378,156757,156756,313513,3.2207159996032715,0.0010673334364093585
78478,156957,156956,313913,3.224621057510376,0.0010629425395406503
78579,157159,157158,314317,3.22855806350708,0.0010585260689953125
78679,157359,157358,314717,3.2325351238250732,0.001054171404704609
78779,157559,157558,315117,3.2364320755004883,0.0010498346550422174
78879,157759,157758,315517,3.2403481006622314,0.0010455157463092463
78979,157959,157958,315917,3.244263172149658,0.0010412146051100048
79079,158159,158158,316317,3.248152017593384,0.0010369311583507488
79179,158359,158358,316717,3.253278970718384,0.0010326653332384033
79279,158559,158558,317117,3.2571940422058105,0.0010284170572793824
79379,158759,158758,317517,3.26117205619812,0.0010241862582783293
79479,158959,158958,317917,3.265075922012329,0.0010199728643369079
79580,159161,159160,318321,3.2691729068756104,0.0010157349305401128
79680,159361,159360,318721,3.2731881141662598,0.0010115563044671315
79780,159561,159560,319121,3.2770941257476807,0.0010073948688198546
79880,159761,159760,319521,3.2810120582580566,0.0010032505528786693
79980,159961,159960,319921,3.284907102584839,0.000999123286214956
80080,160161,160160,320321,3.288804054260254,0.0009950129986897663
80180,160361,160360,320721,3.292694091796875,0.0009909196204527177
80280,160561,160560,321121,3.2966341972351074,0.0009868430819407832
80380,160761,160760,321521,3.3004138469696045,0.0009827833138771347
80480,160961,160960,321921,3.3043088912963867,0.0009787402472699015
80581,161163,161162,322325,3.308115005493164,0.0009746736328361112
80681,161363,161362,322725,3.311941146850586,0.0009706639285989526
80781,161563,161562,323125,3.3159570693969727,0.0009666707198609293
80881,161763,161762,323525,3.319808006286621,0.0009626939387612899
80981,161963,161962,323925,3.3237900733947754,0.0009587335177184958
81081,162163,162162,324325,3.3278450965881348,0.0009547893894289958
81181,162363,162362,324725,3.3321480751037598,0.0009508614868661091
81281,162563,162562,325125,3.335961103439331,0.0009469497432789391
81381,162763,162762,325525,3.3400120735168457,0.0009430540921911496
81481,162963,162962,325925,3.3438169956207275,0.0009391744673998846
81582,163165,163164,326329,3.347633123397827,0.000935272246707893
81682,163365,163364,326729,3.3514840602874756,0.0009314246356059012
81782,163565,163564,327129,3.3555991649627686,0.0009275928531690238
81882,163765,163764,327529,3.3594858646392822,0.0009237768342798167
81982,163965,163964,327929,3.3632829189300537,0.0009199765140887116
82082,164165,164164,328329,3.3671321868896484,0.0009161918280129229
82182,164365,164364,328729,3.3708841800689697,0.0009124227117353531
82282,164565,164564,329129,3.374678134918213,0.0009086691012035014
82382,164765,164764,329529,3.378476142883301,0.0009049309326283809
82482,164965,164964,329929,3.3822362422943115,0.0009012081424833965
82583,165167,165166,330333,3.386070966720581,0.0008974636698816971
82683,165367,165366,330733,3.3898510932922363,0.0008937715992658582
82783,165567,165566,331133,3.3936691284179688,0.0008900947174380366
82883,165767,165766,331533,3.3974599838256836,0.0008864329619131639
82983,165967,165966,331933,3.4012279510498047,0.000882786270463232
83083,166167,166166,332333,3.4050040245056152,0.0008791545811162163
83183,166367,166366,332733,3.4087889194488525,0.0008755378321550661
83283,166567,166566,333133,3.412574052810669,0.0008719359621165982
83383,166767,166766,333533,3.416714906692505,0.0008683489097905232
83483,166967,166966,333933,3.4206111431121826,0.0008647766142183077
83584,167169,167168,334337,3.424520969390869,0.0008611835127072635
83684,167369,167368,334737,3.4283089637756348,0.000857640694820799
83784,167569,167568,335137,3.4320502281188965,0.0008541124517124077
83884,167769,167768,335537,3.435857057571411,0.0008505987234229927
83984,167969,167968,335937,3.4396331310272217,0.0008470994502401269
84084,168169,168168,336337,3.4434852600097656,0.0008436145726970179
84184,168369,168368,336737,3.4472970962524414,0.0008401440315715475
84284,168569,168568,337137,3.4510631561279297,0.0008366877678851835
84384,168769,168768,337537,3.4548189640045166,0.0008332457229020795
84484,168969,168968,337937,3.4586281776428223,0.0008298178381279802
84585,169171,169170,338341,3.462549924850464,0.0008263699884994855
84685,169371,169370,338741,3.4667229652404785,0.000822970389769486
84785,169571,169570,339141,3.4706239700317383,0.0008195847766291025
84885,169771,169770,339541,3.4745142459869385,0.0008162130915430944
84985,169971,169970,339941,3.4783971309661865,0.0008128552772129153
85085,170171,170170,340341,3.4822280406951904,0.0008095112765757376
85185,170371,170370,340741,3.486030101776123,0.0008061810328035038
85285,170571,170570,341141,3.4898340702056885,0.0008028644893019075
85385,170771,170770,341541,3.4936671257019043,0.0007995615897095013
85485,170971,170970,341941,3.497497081756592,0.0007962722778966719
85586,171173,171172,342345,3.501399040222168,0.0007929638083128772
85686,171373,171372,342745,3.5052971839904785,0.000789701639074892
85786,171573,171572,343145,3.5091309547424316,0.0007864528900561255
85886,171773,171772,343545,3.512953042984009,0.0007832175060472207
85986,171973,171972,343945,3.5167312622070312,0.0007799954320659252
86086,172173,172172,344345,3.5205721855163574,0.0007767866133561951
86186,172373,172372,344745,3.5244300365448,0.0007735909953872531
86286,172573,172572,345145,3.5283620357513428,0.0007704085238526242
86386,172773,172772,345545,3.532210111618042,0.0007672391446693147
86486,172973,172972,345945,3.536079168319702,0.0007640828039767418
86587,173175,173174,346349,3.539933919906616,0.0007609080799701154
86687,173375,173374,346749,3.5438551902770996,0.0007577777846080904
86787,173575,173574,347149,3.547760248184204,0.000754660366950111
86887,173775,173774,347549,3.5516090393066406,0.0007515557740186439
86987,173975,173974,347949,3.5554749965667725,0.0007484639530541494
87087,174175,174174,348349,3.559433937072754,0.0007453848515140839
87187,174375,174374,348749,3.563720941543579,0.0007423184170720906
87287,174575,174574,349149,3.5676732063293457,0.0007392645976170561
87387,174775,174774,349549,3.571605920791626,0.0007362233412522726
87487,174975,174974,349949,3.5754411220550537,0.0007331945962945061
87588,175177,175176,350353,3.579324245452881,0.0007301482111720159
87688,175377,175376,350753,3.5834429264068604,0.0007271444586568655
87788,175577,175576,351153,3.5880539417266846,0.0007241530632618487
87888,175777,175776,351553,3.5920162200927734,0.0007211739741510998
87988,175977,175976,351953,3.5959041118621826,0.0007182071406978532
88088,176177,176176,352353,3.599799156188965,0.0007152525124836574
88188,176377,176376,352753,3.6037650108337402,0.0007123100392974267
88288,176577,176576,353153,3.607771158218384,0.0007093796711346646
88388,176777,176776,353553,3.6116371154785156,0.000706461358196588
88488,176977,176976,353953,3.6154990196228027,0.0007035550508892803
88589,177179,177178,354357,3.6198551654815674,0.0007006318165245928
88689,177379,177378,354757,3.6238150596618652,0.0006977494913351491
88789,177579,177578,355157,3.6277291774749756,0.0006948790237266729
88889,177779,177778,355557,3.6315839290618896,0.0006920203649183336
88989,177979,177978,355957,3.6363582611083984,0.0006891734663299825
89089,178179,178178,356357,3.640247106552124,0.0006863382795813204
89189,178379,178378,356757,3.6442041397094727,0.0006835147564910646
89289,178579,178578,357157,3.6482129096984863,0.0006807028490761866
89389,178779,178778,357557,3.6521410942077637,0.0006779025095509966
89489,178979,178978,357957,3.656219244003296,0.0006751136903264208
89590,179181,179180,358361,3.6601130962371826,0.0006723086283243344
89690,179381,179380,358761,3.663987874984741,0.0006695428217354923
89790,179581,179580,359161,3.667983055114746,0.0006667883933824186
89890,179781,179780,359561,3.671999931335449,0.0006640452964562696
89990,179981,179980,359961,3.6758809089660645,0.000661313484340747
90090,180181,180180,360361,3.6797430515289307,0.0006585929106113304
90190,180381,180380,360761,3.683608055114746,0.0006558835290344818
90290,180581,180580,361161,3.687519073486328,0.0006531852935668883
90390,180781,180780,361561,3.691534996032715,0.0006504981583546004
90490,180981,180980,361961,3.695482015609741,0.0006478220777323728
90591,181183,181182,362365,3.6993792057037354,0.0006451304109503172
90691,181383,181382,362765,3.7032649517059326,0.0006424764126731859
90791,181583,181582,363165,3.707130193710327,0.0006398333326642635
90891,181783,181782,363565,3.7110509872436523,0.000637201126006946
90991,181983,181982,363965,3.7149670124053955,0.0006345797479694101
91091,182183,182182,364365,3.7188479900360107,0.0006319691540038736
91191,182383,182382,364765,3.722745180130005,0.0006293692997457922
91291,182583,182582,365165,3.7266879081726074,0.0006267801410131619
91391,182783,182782,365565,3.7306201457977295,0.0006242016338056925
91491,182983,182982,365965,3.7345762252807617,0.0006216337343041626
91592,183185,183184,366369,3.738535165786743,0.0006190508787165712
91692,183385,183384,366769,3.742434024810791,0.000616504168876702
91792,183585,183584,367169,3.746457099914551,0.0006139679359317464
91892,183785,183784,367569,3.7504281997680664,0.0006114421367808764
91992,183985,183984,367969,3.75433611869812,0.0006089267285005744
92092,184185,184184,368369,3.7582719326019287,0.0006064216683438989
92192,184385,184384,368769,3.76225209236145,0.0006039269137397423
92292,184585,184584,369169,3.7662670612335205,0.0006014424222921702
92392,184785,184784,369569,3.7702388763427734,0.0005989681517796376
92492,184985,184984,369969,3.774260997772217,0.0005965040601543032
92593,185187,185186,370373,3.778351068496704,0.0005940256170458203
92693,185387,185386,370773,3.7823071479797363,0.0005915818584856152
92793,185587,185586,371173,3.7862610816955566,0.0005891481532896432
92893,185787,185786,371573,3.7902321815490723,0.0005867244600994535
92993,185987,185986,371973,3.7942070960998535,0.0005843107377267003
93093,186187,186186,372373,3.7981250286102295,0.0005819069451524923
93193,186387,186386,372773,3.802006959915161,0.0005795130415266957
93293,186587,186586,373173,3.8059849739074707,0.0005771289861672234
93393,186787,186786,373573,3.810091018676758,0.0005747547385593525
93493,186987,186986,373973,3.8140430450439453,0.0005723902583550136
93594,187189,187188,374377,3.818120241165161,0.0005700120068292604
93694,187389,187388,374777,3.822064161300659,0.0005676670377216321
93794,187589,187588,375177,3.8261680603027344,0.0005653317155688939
93894,187789,187788,375577,3.830095052719116,0.0005630060006845002
93994,187989,187988,375977,3.8340320587158203,0.0005606898535451493
94094,188189,188188,376377,3.838024139404297,0.0005583832347901581
94194,188389,188388,376777,3.842036008834839,0.0005560861052207555
94294,188589,188588,377177,3.846261978149414,0.0005537984257994406
94394,188789,188788,377577,3.850346088409424,0.0005515201576493039
94494,188989,188988,377977,3.854344129562378,0.000549251262053377
94595,189191,189190,378381,3.858315944671631,0.0005469691518445876
94695,189391,189390,378781,3.8622519969940186,0.0005447189786051994
94795,189591,189590,379181,3.866274118423462,0.0005424780623405207
94895,189791,189790,379581,3.8702311515808105,0.0005402463649683385
94995,189991,189990,379981,3.8741941452026367,0.0005380238485631097
95095,190191,190190,380381,3.87813401222229,0.0005358104753552924
95195,190391,190390,380781,3.882075071334839,0.0005336062077307536
95295,190591,190590,381181,3.886025905609131,0.0005314110082300831
95395,190791,190790,381581,3.8899550437927246,0.0005292248395479789
95495,190991,190990,381981,3.893908977508545,0.0005270476645326075
95596,191193,191192,382385,3.897879123687744,0.0005248578091078595
95696,191393,191392,382785,3.9018101692199707,0.0005226985995938372
95796,191593,191592,383185,3.905750036239624,0.0005205482728393725
95896,191793,191792,383585,3.909684896469116,0.0005184067923017403
95996,191993,191992,383985,3.9136171340942383,0.0005162741215885456
96096,192193,192192,384385,3.9175710678100586,0.0005141502244571144
96196,192393,192392,384785,3.9215240478515625,0.0005120350648138418
96296,192593,192592,385185,3.9254910945892334,0.0005099286067136191
96396,192793,192792,385585,3.9294891357421875,0.0005078308143592323
96496,192993,192992,385985,3.9334330558776855,0.0005057416521007108
96597,193195,193194,386389,3.9374051094055176,0.0005036403220410416
96697,193395,193394,386789,3.9413859844207764,0.0005015683990246994
96797,193595,193594,387189,3.945505142211914,0.0004995049996805148
96897,193795,193794,387589,3.9494619369506836,0.0004974500889429897
96997,193995,193994,387989,3.9535531997680664,0.0004954036318908944
97097,194195,194194,388389,3.9575071334838867,0.0004933655937466648
97197,194395,194394,388789,3.9615988731384277,0.0004913359398757927
97297,194595,194594,389189,3.965451955795288,0.0004893146357862796
97397,194795,194794,389589,3.969343900680542,0.000487301647128011
97497,194995,194994,389989,3.9731712341308594,0.0004852969396921588
97598,195197,195196,390393,3.9771602153778076,0.00048328055634108214
97698,195397,195396,390793,3.981372117996216,0.00048129239124743264
97798,195597,195596,391193,3.985795021057129,0.00047931240525470335
97898,195797,195796,391593,3.9898180961608887,0.00047734056471492676
97998,195997,195996,391993,3.9946539402008057,0.0004753768361185795
98098,196197,196196,392393,3.998885154724121,0.000473421186093979
98198,196397,196396,392793,4.003031015396118,0.0004714735814067335
98298,196597,196596,393193,4.006967067718506,0.00046953398895918826
98398,196797,196796,393593,4.011446952819824,0.0004676023757898199
98498,196997,196996,393993,4.016211986541748,0.00046567870907273816
98599,197199,197198,394397,4.0201661586761475,0.0004637438384417335
98699,197399,197398,394797,4.024298906326294,0.0004618360453391859
98799,197599,197598,395197,4.028473138809204,0.00045993610069567774
98899,197799,197798,395597,4.032583236694336,0.0004580439722234852
98999,197999,197998,395997,4.0366621017456055,0.0004561596277677057
99099,198199,198198,396397,4.0413312911987305,0.00045428303530572464
99199,198399,198398,396797,4.045583009719849,0.000452414162946645
99299,198599,198598,397197,4.05014705657959,0.000450552978930778
99399,198799,198798,397597,4.0540242195129395,0.0004486994516291035
99499,198999,198998,397997,4.058033227920532,0.0004468535495427096
99600,199201,199200,398401,4.0619330406188965,0.000444996896462976
99700,199401,199400,398801,4.065977096557617,0.00044316622629691983
99800,199601,199600,399201,4.070139169692993,0.00044134308731430094
99900,199801,199800,399601,4.074229955673218,0.00043952744853262976
100000,200001,200000,400001,4.078203201293945,0.00043771927909687125


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha0/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.605552673339844e-05,4.387061074692293
100,201,200,401,0.004263162612915039,0.24400872360835765
200,401,400,801,0.008306264877319336,0.11396482179674887
300,601,600,1201,0.012281179428100586,0.07772603596230616
400,801,800,1601,0.01627802848815918,0.06190660644187962
501,1003,1002,2005,0.020492076873779297,0.05363210938132448
601,1203,1202,2405,0.02526116371154785,0.04854289708923014
701,1403,1402,2805,0.029702186584472656,0.044811894255043366
801,1603,1602,3205,0.033898115158081055,0.04179654400397964
901,1803,1802,3605,0.03812718391418457,0.03924971924554778
1001,2003,2002,4005,0.0424041748046875,0.03706348955839846
1101,2203,2202,4405,0.04651594161987305,0.035178785925197326
1201,2403,2402,4805,0.05059099197387695,0.03355453267398762
1301,2603,2602,5205,0.05438995361328125,0.03215726348792642
1401,2803,2802,5605,0.05789899826049805,0.03095767199648659
1502,3005,3004,6009,0.06125020980834961,0.02991998323202208
1602,3205,3204,6409,0.0645749568939209,0.029040939320774044
1702,3405,3404,6809,0.06790399551391602,0.02828835829650628
1802,3605,3604,7209,0.07123708724975586,0.027643543602227788
1902,3805,3804,7609,0.07462024688720703,0.027090075263709473
2002,4005,4004,8009,0.11212515830993652,0.02661366298608146
2102,4205,4204,8409,0.12381100654602051,0.026201975227758096
2202,4405,4404,8809,0.12827420234680176,0.0258444527270099
2302,4605,4604,9209,0.13292431831359863,0.02553211595577548
2402,4805,4804,9609,0.13739490509033203,0.02525737490279822
2503,5007,5006,10013,0.14232921600341797,0.025011551173271675
2603,5207,5206,10413,0.14678621292114258,0.02479413074736284
2703,5407,5406,10813,0.15110015869140625,0.024598087482034042
2803,5607,5606,11213,0.15563106536865234,0.02441972624861084
2903,5807,5806,11613,0.15998625755310059,0.024255984393149754
3003,6007,6006,12013,0.16427111625671387,0.02410432926149394
3103,6207,6206,12413,0.1685020923614502,0.023962670451067175
3203,6407,6406,12813,0.17255115509033203,0.02382928529238106
3303,6607,6606,13213,0.1769249439239502,0.023702755993531773
3403,6807,6806,13613,0.18070411682128906,0.023581916916485614
3504,7009,7008,14017,0.18414998054504395,0.023464670603200708
3604,7209,7208,14417,0.18747806549072266,0.023352546952781245
3704,7409,7408,14817,0.19103217124938965,0.02324371933040331
3804,7609,7608,15217,0.1943531036376953,0.02313765993724719
3904,7809,7808,15617,0.19768309593200684,0.023033936061227892
4004,8009,8008,16017,0.20102715492248535,0.02293219301852367
4104,8209,8208,16417,0.2043609619140625,0.022832140115381733
4204,8409,8408,16817,0.20786404609680176,0.02273353910866042
4304,8609,8608,17217,0.2112131118774414,0.022636194729250055
4404,8809,8808,17617,0.21453595161437988,0.02253994690559794
4505,9011,9010,18021,0.21788907051086426,0.022443716054252546
4605,9211,9210,18421,0.2212049961090088,0.022349299282451357
4705,9411,9410,18821,0.2248539924621582,0.022255651010420593
4805,9611,9610,19221,0.22821712493896484,0.022162698835552937
4905,9811,9810,19621,0.23160910606384277,0.022070383260160423
5005,10011,10010,20021,0.23498916625976562,0.02197865534524145
5105,10211,10210,20421,0.2382831573486328,0.02188747479025684
5205,10411,10410,20821,0.24213504791259766,0.021796808361813313
5305,10611,10610,21221,0.24554228782653809,0.021706628608024154
5405,10811,10810,21621,0.24889326095581055,0.021616912806721164
5506,11013,11012,22025,0.2523651123046875,0.02152675159037204
5606,11213,11212,22425,0.2556171417236328,0.02143791452511929
5706,11413,11412,22825,0.2591691017150879,0.021349493655195773
5806,11613,11612,23225,0.2623932361602783,0.021261478021364178
5906,11813,11812,23625,0.26566410064697266,0.021173858394926075
6006,12013,12012,24025,0.26892518997192383,0.0210866269634385
6106,12213,12212,24425,0.27220821380615234,0.02099977707368877
6206,12413,12412,24825,0.27573394775390625,0.020913303021499314
6306,12613,12612,25225,0.2790231704711914,0.020827199879831903
6406,12813,12812,25625,0.2823061943054199,0.02074146335821519
6507,13015,13014,26029,0.2856571674346924,0.020655237771859597
6607,13215,13214,26429,0.2891991138458252,0.020570227190828582
6707,13415,13414,26829,0.2930910587310791,0.020485573100828172
6807,13615,13614,27229,0.29640698432922363,0.02040127280177237
6907,13815,13814,27629,0.29978013038635254,0.020317323829549257
7007,14015,14014,28029,0.3030431270599365,0.020233723914058508
7107,14215,14214,28429,0.3071732521057129,0.020150470944893955
7207,14415,14414,28829,0.3110010623931885,0.020067562943277894
7307,14615,14614,29229,0.3144261837005615,0.019984998039106475
7407,14815,14814,29629,0.3178219795227051,0.019902774452176045
7508,15017,15016,30033,0.3214411735534668,0.019820073346504125
7608,15217,15216,30433,0.3250579833984375,0.019738530710620945
7708,15417,15416,30833,0.32834410667419434,0.019657324434985902
7808,15617,15616,31233,0.33159804344177246,0.019576452971328227
7908,15817,15816,31633,0.3348522186279297,0.0194959148077385
8008,16017,16016,32033,0.3380851745605469,0.01941570846305175
8108,16217,16216,32433,0.3417370319366455,0.019335832482250178
8208,16417,16416,32833,0.34501028060913086,0.01925628543269952
8308,16617,16616,33233,0.34827423095703125,0.019177065901067873
8408,16817,16816,33633,0.3517723083496094,0.019098172490801885
8509,17019,17018,34037,0.3550431728363037,0.01901881976864435
8609,17219,17218,34437,0.3586270809173584,0.018940577695431893
8709,17419,17418,34837,0.3618910312652588,0.0188626576221969
8809,17619,17618,35237,0.3651261329650879,0.018785058202323093
8909,17819,17818,35637,0.3683600425720215,0.018707778098734175
9009,18019,18018,36037,0.37159299850463867,0.018630815983125406
9109,18219,18218,36437,0.3750760555267334,0.01855417053533105
9209,18419,18418,36837,0.37830615043640137,0.018477840442803484
9309,18619,18618,37237,0.3815422058105469,0.018401824400183057
9409,18819,18818,37637,0.3847620487213135,0.018326121108942536
9510,19021,19020,38041,0.3881661891937256,0.01824997692728853
9610,19221,19220,38441,0.39229321479797363,0.01817489836439712
9710,19421,19420,38841,0.39588499069213867,0.018100128682825716
9810,19621,19620,39241,0.3991522789001465,0.018025666608942708
9910,19821,19820,39641,0.4024052619934082,0.01795151087488961
10010,20021,20020,40041,0.4063541889190674,0.017877660218460007
10110,20221,20220,40441,0.4104161262512207,0.017804113382996836
10210,20421,20420,40841,0.41390514373779297,0.01773086911730443
10310,20621,20620,41241,0.4175240993499756,0.017657926175572894
10410,20821,20820,41641,0.4208393096923828,0.01758528331731253
10511,21023,21022,42045,0.42496418952941895,0.017512217372213767
10611,21223,21222,42445,0.42899298667907715,0.01744017395041506
10711,21423,21422,42845,0.43228912353515625,0.017368426909774835
10811,21623,21622,43245,0.4360771179199219,0.01729697503062207
10911,21823,21822,43645,0.4401721954345703,0.0172258170983744
11011,22023,22022,44045,0.44382429122924805,0.01715495190350446
11111,22223,22222,44445,0.44739317893981934,0.017084378241508134
11211,22423,22422,44845,0.4509623050689697,0.017014094912875637
11311,22623,22622,45245,0.45455002784729004,0.016944100723063484
11411,22823,22822,45645,0.45807528495788574,0.01687439448246843
11512,23025,23024,46049,0.4616272449493408,0.016804282255806782
11612,23225,23224,46449,0.4649841785430908,0.016735151214378838
11712,23425,23424,46849,0.4683411121368408,0.016666304571029123
11812,23625,23624,47249,0.47170209884643555,0.01659774115572194
11912,23825,23824,47649,0.47530221939086914,0.01652945980324449
12012,24025,24024,48049,0.47863292694091797,0.016461459353185378
12112,24225,24224,48449,0.4819209575653076,0.016393738649913198
12212,24425,24424,48849,0.4852161407470703,0.016326296542556084
12312,24625,24624,49249,0.4885270595550537,0.016259131884980845
12412,24825,24824,49649,0.4926478862762451,0.016192243535772873
12513,25027,25026,50053,0.4960823059082031,0.016124965612223152
12613,25227,25226,50453,0.4994239807128906,0.016058629208975092
12713,25427,25426,50853,0.5027570724487305,0.015992565706711873
12813,25627,25626,51253,0.5068180561065674,0.015926773982740765
12913,25827,25826,51653,0.510181188583374,0.015861252918988957
13013,26027,26026,52053,0.5135371685028076,0.01579600140198428
13113,26227,26226,52453,0.5168631076812744,0.015731018322836098
13213,26427,26426,52853,0.5201821327209473,0.01566630257721642
13313,26627,26626,53253,0.5236811637878418,0.015601853065340806
13413,26827,26826,53653,0.527076244354248,0.015537668691949714
13514,27029,27028,54057,0.5305280685424805,0.015473110492795109
13614,27229,27228,54457,0.5339250564575195,0.015409455752744657
13714,27429,27428,54857,0.5373172760009766,0.015346062881567299
13814,27629,27628,55257,0.5407631397247314,0.015282930801961206
13914,27829,27828,55657,0.5443511009216309,0.015220058441056731
14014,28029,28028,56057,0.5476820468902588,0.015157444730397951
14114,28229,28228,56457,0.5510151386260986,0.015095088605924645
14214,28429,28428,56857,0.5543591976165771,0.015032989007954085
14314,28629,28628,57257,0.5578272342681885,0.014971144881162992
14414,28829,28828,57657,0.5611703395843506,0.014909555174569671
14515,29031,29030,58061,0.5645041465759277,0.014847606754191575
14615,29231,29230,58461,0.5678131580352783,0.014786525270388241
14715,29431,29430,58861,0.5711159706115723,0.014725695069349514
14815,29631,29630,59261,0.5745720863342285,0.014665115117324604
14915,29831,29830,59661,0.5780589580535889,0.014604784384815403
15015,30031,30030,60061,0.5813860893249512,0.014544701846559078
15115,30231,30230,60461,0.5847113132476807,0.01448486648151075
15215,30431,30430,60861,0.5881342887878418,0.014425277272825825
15315,30631,30630,61261,0.591569185256958,0.014365933207843056
15415,30831,30830,61661,0.5948810577392578,0.014306833278067182
15516,31033,31032,62065,0.5982100963592529,0.01424738913558572
15616,31233,31232,62465,0.6015141010284424,0.01418877688358528
15716,31433,31432,62865,0.6048200130462646,0.014130405756190456
15816,31633,31632,63265,0.6083130836486816,0.014072274761440025
15916,31833,31832,63665,0.6116669178009033,0.014014382911453726
16016,32033,32032,64065,0.6149942874908447,0.0139567292224153
16116,32233,32232,64465,0.6183161735534668,0.013899312714555747
16216,32433,32432,64865,0.6216230392456055,0.013842132412136788
16316,32633,32632,65265,0.6254041194915771,0.013785187343434193
16416,32833,32832,65665,0.62888503074646,0.013728476540721377
16517,33035,33034,66069,0.6323990821838379,0.013671435440173726
16617,33235,33234,66469,0.6357481479644775,0.013615192600759746
16717,33435,33434,66869,0.6392760276794434,0.013559181138438509
16817,33635,33634,67269,0.642951250076294,0.01350340010134909
16917,33835,33834,67669,0.6463322639465332,0.013447848541546467
17017,34035,34034,68069,0.649691104888916,0.013392525514985343
17117,34235,34234,68469,0.6531691551208496,0.013337430081504184
17217,34435,34434,68869,0.6566059589385986,0.013282561304809058
17317,34635,34634,69269,0.6598761081695557,0.013227918252457985
17417,34835,34834,69669,0.6631491184234619,0.01317349999584482
17518,35037,35036,70073,0.6664121150970459,0.013118764793756114
17618,35237,35236,70473,0.6696791648864746,0.013064795582927223
17718,35437,35436,70873,0.6730802059173584,0.01301104839572354
17818,35637,35636,71273,0.6766142845153809,0.012957522318763317
17918,35837,35836,71673,0.6798861026763916,0.012904216442422432
18018,36037,36036,72073,0.683131217956543,0.012851129860818794
18118,36237,36236,72473,0.6863648891448975,0.01279826167179707
18218,36437,36436,72873,0.6899609565734863,0.012745610976913279
18318,36637,36636,73273,0.6935510635375977,0.012693176881419535
18418,36837,36836,73673,0.6968340873718262,0.012640958494248851
18519,37039,37038,74077,0.7001900672912598,0.012588435974189925
18619,37239,37238,74477,0.7034852504730225,0.012536648480033455
18719,37439,37438,74877,0.7074329853057861,0.012485074034150523
18819,37639,37638,75277,0.7107691764831543,0.012433711760083094
18919,37839,37838,75677,0.7140452861785889,0.012382560784978723
19019,38039,38038,76077,0.7173402309417725,0.012331620239575868
19119,38239,38238,76477,0.7206110954284668,0.01228088925818896
19219,38439,38438,76877,0.724013090133667,0.012230366978693818
19319,38639,38638,77277,0.7274312973022461,0.012180052542512906
19419,38839,38838,77677,0.7307100296020508,0.012129945094600848
19520,39041,39040,78081,0.7341761589050293,0.012079545808436398
19620,39241,39240,78481,0.7374720573425293,0.01202985183459805
19720,39441,39440,78881,0.7409861087799072,0.011980362296512089
19820,39641,39640,79281,0.7442638874053955,0.011931076353151427
19920,39841,39840,79681,0.7475481033325195,0.011881993166948941
20020,40041,40040,80081,0.7508599758148193,0.01183311190378311
20120,40241,40240,80481,0.7541511058807373,0.011784431732963906
20220,40441,40440,80881,0.7576830387115479,0.011735951827218701
20320,40641,40640,81281,0.7609663009643555,0.011687671362678157
20420,40841,40840,81681,0.7642569541931152,0.011639589518862252
20521,41043,41042,82085,0.7676081657409668,0.011591227634416544
20621,41243,41242,82485,0.7710020542144775,0.011543542549898145
20721,41443,41442,82885,0.7748911380767822,0.011496053636773956
20821,41643,41642,83285,0.7781713008880615,0.011448760088015549
20921,41843,41842,83685,0.7814791202545166,0.011401661099914676
21021,42043,42042,84085,0.7847769260406494,0.011354755872069319
21121,42243,42242,84485,0.7880520820617676,0.011308043607370302
21221,42443,42442,84885,0.7917649745941162,0.011261523511987627
21321,42643,42642,85285,0.795051097869873,0.0112151947953571
21421,42843,42842,85685,0.7983119487762451,0.011169056670166717
21522,43045,43044,86089,0.8016431331634521,0.01112264982504777
21622,43245,43244,86489,0.8049640655517578,0.011076892420077013
21722,43445,43444,86889,0.8089599609375,0.011031323256230713
21822,43645,43644,87289,0.8122670650482178,0.010985941559104768
21922,43845,43844,87689,0.8156599998474121,0.010940746557480913
22022,44045,44044,88089,0.8190860748291016,0.010895737483313583
22122,44245,44244,88489,0.8232932090759277,0.010850913571716898
22222,44445,44444,88889,0.8267161846160889,0.010806274060951618
22322,44645,44644,89289,0.8299791812896729,0.010761818192412247
22422,44845,44844,89689,0.8335270881652832,0.010717545210614084
22523,45047,45046,90093,0.83685302734375,0.010673014371946841
22623,45247,45246,90493,0.8403279781341553,0.010629106719673554
22723,45447,45446,90893,0.8437702655792236,0.010585379698837745
22823,45647,45646,91293,0.8470070362091064,0.010541832566340786
22923,45847,45846,91693,0.8502500057220459,0.010498464582141067
23023,46047,46046,92093,0.8534872531890869,0.010455275009241429
23123,46247,46246,92493,0.8572039604187012,0.010412263113676686
23223,46447,46446,92893,0.8606619834899902,0.010369428164501055
23323,46647,46646,93293,0.8639049530029297,0.010326769433775803
23423,46847,46846,93693,0.8671972751617432,0.010284286196556858
23524,47049,47048,94097,0.8704659938812256,0.010241555526386868
23624,47249,47248,94497,0.8737242221832275,0.010199422850170116
23724,47449,47448,94897,0.8773071765899658,0.010157463503327056
23824,47649,47648,95297,0.8805890083312988,0.010115676772798968
23924,47849,47848,95697,0.8838472366333008,0.010074061948460666
24024,48049,48048,96097,0.8871171474456787,0.010032618323108216
24124,48249,48248,96497,0.8904011249542236,0.009991345192447064
24224,48449,48448,96897,0.8939011096954346,0.00995024185508015
24324,48649,48648,97297,0.8972022533416748,0.009909307612495753
24424,48849,48848,97697,0.9007790088653564,0.009868541769055873
24525,49051,49050,98101,0.9042141437530518,0.009827538495193936
24625,49251,49250,98501,0.9075078964233398,0.009787109041254165
24725,49451,49450,98901,0.9107611179351807,0.009746845909811806
24825,49651,49650,99301,0.9141221046447754,0.009706748416633661
24925,49851,49850,99701,0.9179441928863525,0.009666815880301487
25025,50051,50050,100101,0.9225962162017822,0.009627047622200218
25125,50251,50250,100501,0.9266631603240967,0.009587442966506592
25225,50451,50450,100901,0.930164098739624,0.009548001240177635
25325,50651,50650,101301,0.933969259262085,0.009508721772939172
25425,50851,50850,101701,0.9380879402160645,0.009469603897274465
25526,51053,51052,102105,0.9415731430053711,0.009430258189362294
25626,51253,51252,102505,0.9448461532592773,0.009391463104581561
25726,51453,51452,102905,0.9481470584869385,0.009352827618676379
25826,51653,51652,103305,0.9514749050140381,0.009314351075073826
25926,51853,51852,103705,0.9547860622406006,0.009276032819902103
26026,52053,52052,104105,0.9580972194671631,0.00923787220197936
26126,52253,52252,104505,0.9614551067352295,0.009199868572802628
26226,52453,52452,104905,0.9647622108459473,0.009162021286536771
26326,52653,52652,105305,0.9680671691894531,0.009124329700003632
26426,52853,52852,105705,0.9713761806488037,0.009086793172670976
26527,53055,53054,106109,0.9747161865234375,0.009049038023257273
26627,53255,53254,106509,0.9780302047729492,0.009011811237919354
26727,53455,53454,106909,0.9813282489776611,0.008974737599638951
26827,53655,53654,107309,0.9847631454467773,0.008937816478385275
26927,53855,53854,107709,0.9880781173706055,0.008901047246719404
27027,54055,54054,108109,0.9913783073425293,0.008864429279783642
27127,54255,54254,108509,0.9946801662445068,0.008827961955290868
27227,54455,54454,108909,0.9979982376098633,0.008791644653514006
27327,54655,54654,109309,1.0013060569763184,0.008755476757275497
27427,54855,54854,109709,1.004992961883545,0.008719457651936706
27528,55057,55056,110113,1.0083389282226562,0.008683228762360428
27628,55257,55256,110513,1.0116453170776367,0.008647506877631283
27728,55457,55456,110913,1.0149621963500977,0.00861193194895774
27828,55657,55656,111313,1.018273115158081,0.008576503371778088
27928,55857,55856,111713,1.0215752124786377,0.008541220544017788
28028,56057,56056,112113,1.0248920917510986,0.00850608286607914
28128,56257,56256,112513,1.028196096420288,0.008471089740831111
28228,56457,56456,112913,1.0315170288085938,0.008436240573599233
28328,56657,56656,113313,1.0348231792449951,0.008401534772155474
28428,56857,56856,113713,1.0381231307983398,0.008366971746708104
28529,57059,57058,114117,1.0414509773254395,0.008332207417595033
28629,57259,57258,114517,1.0447502136230469,0.008297929597551771
28729,57459,57458,114917,1.0480539798736572,0.008263792792834741
28829,57659,57658,115317,1.051281213760376,0.008229796423321747
28929,57859,57858,115717,1.0546891689300537,0.008195939911277242
29029,58059,58058,116117,1.057819128036499,0.008162222681342373
29129,58259,58258,116517,1.0609452724456787,0.008128644160525297
29229,58459,58458,116917,1.0640971660614014,0.008095203778191359
29329,58659,58658,117317,1.0672392845153809,0.00806190096605345
29429,58859,58858,117717,1.070406198501587,0.008028735158162345
29530,59061,59060,118121,1.0735690593719482,0.007995376184348438
29630,59261,59260,118521,1.076709270477295,0.007962484052373132
29730,59461,59460,118921,1.0798752307891846,0.007929727235149852
29830,59661,59660,119321,1.0830662250518799,0.007897105176008062
29930,59861,59860,119721,1.0862131118774414,0.007864617320567235
30030,60061,60060,120121,1.0904719829559326,0.007832263116727552
30130,60261,60260,120521,1.0948641300201416,0.007800042014660447
30230,60461,60460,120921,1.099095106124878,0.007767953466799313
30330,60661,60660,121321,1.1027240753173828,0.007735996927830199
30430,60861,60860,121721,1.1061370372772217,0.007704171854682442
30531,61063,61062,122125,1.1096701622009277,0.007672161424384856
30631,61263,61262,122525,1.1133100986480713,0.0076405989637465845
30731,61463,61462,122925,1.1171820163726807,0.007609166347733111
30831,61663,61662,123325,1.1211252212524414,0.0075778630421773656
30931,61863,61862,123725,1.1252861022949219,0.0075466885151098265
31031,62063,62062,124125,1.1290769577026367,0.007515642236749418
31131,62263,62262,124525,1.133155107498169,0.007484723679494517
31231,62463,62462,124925,1.1370460987091064,0.007453932317913985
31331,62663,62662,125325,1.1405901908874512,0.007423267628738286
31431,62863,62862,125725,1.1446471214294434,0.007392729090850528
31532,63065,63064,126129,1.1482820510864258,0.007362012688914633
31632,63265,63264,126529,1.1515991687774658,0.007331726147370554
31732,63465,63464,126929,1.1552770137786865,0.007301564201455097
31832,63665,63664,127329,1.158674955368042,0.007271526338594972
31932,63865,63864,127729,1.1624341011047363,0.007241612048325651
32032,64065,64064,128129,1.166274070739746,0.007211820822282571
32132,64265,64264,128529,1.1697862148284912,0.007182152154192482
32232,64465,64464,128929,1.1733272075653076,0.007152605539864971
32332,64665,64664,129329,1.1766910552978516,0.007123180477183726
32432,64865,64864,129729,1.1800761222839355,0.007093876466098154
32533,65067,65066,130133,1.1834602355957031,0.007064401781155894
32633,65267,65266,130533,1.1868250370025635,0.007035339579408933
32733,65467,65466,130933,1.1901700496673584,0.007006396936486132
32833,65667,65666,131333,1.193526029586792,0.0069775733605351295
32933,65867,65866,131733,1.1968603134155273,0.006948868361727015
33033,66067,66066,132133,1.200242280960083,0.006920281452247954
33133,66267,66266,132533,1.2036030292510986,0.006891812146290943
33233,66467,66466,132933,1.2069621086120605,0.006863459960047532
33333,66667,66666,133333,1.2103612422943115,0.006835224411699583
33433,66867,66866,133733,1.2136969566345215,0.006807105021411168
33534,67069,67068,134137,1.2171361446380615,0.006778821856792532
33634,67269,67268,134537,1.2206902503967285,0.006750934500649469
33734,67469,67468,134937,1.2241201400756836,0.00672316187014001
33834,67669,67668,135337,1.2275891304016113,0.006695503493295036
33934,67869,67868,135737,1.2309739589691162,0.006667958900087056
34034,68069,68068,136137,1.2344810962677002,0.006640527622422218
34134,68269,68268,136537,1.2378230094909668,0.006613209194132384
34234,68469,68468,136937,1.241157054901123,0.006586003150967135
34334,68669,68668,137337,1.2445251941680908,0.006558909030585957
34434,68869,68868,137737,1.2478430271148682,0.00653192637255039
34535,69071,69070,138141,1.2512471675872803,0.006504786560796256
34635,69271,69270,138541,1.2545831203460693,0.006478026556877027
34735,69471,69470,138941,1.258249044418335,0.006451376640783591
34835,69671,69670,139341,1.261620044708252,0.006424836359626273
34935,69871,69870,139741,1.265002965927124,0.0063984052623785575
35035,70071,70070,140141,1.2682969570159912,0.0063720828998694015
35135,70271,70270,140541,1.2715840339660645,0.0063458688247755345
35235,70471,70470,140941,1.2750191688537598,0.006319762591614038
35335,70671,70670,141341,1.2783501148223877,0.006293763756734599
35435,70871,70870,141741,1.2816822528839111,0.006267871878312006
35536,71073,71072,142145,1.2851309776306152,0.006241829199142931
35636,71273,71272,142545,1.2885680198669434,0.006216150973997304
35736,71473,71472,142945,1.2918701171875,0.006190578386354045
35836,71673,71672,143345,1.295177936553955,0.006165111001631597
35936,71873,71872,143745,1.2984881401062012,0.006139748387036292
36036,72073,72072,144145,1.301919937133789,0.006114490111554905
36136,72273,72272,144545,1.3052332401275635,0.0060893357459473624
36236,72473,72472,144945,1.308535099029541,0.006064284862739422
36336,72673,72672,145345,1.3118321895599365,0.0060393370362154435
36436,72873,72872,145745,1.315134048461914,0.006014491842411115
36537,73075,73074,146149,1.3186571598052979,0.005989501944012134
36637,73275,73274,146549,1.3220269680023193,0.005964861766506236
36737,73475,73474,146949,1.3253529071807861,0.005940322956084465
36837,73675,73674,147349,1.3286809921264648,0.005915885095733384
36937,73875,73874,147749,1.3320331573486328,0.0058915477701550695
37037,74075,74074,148149,1.3353610038757324,0.005867310565760089
37137,74275,74274,148549,1.338691234588623,0.0058431730706605236
37237,74475,74474,148949,1.3420040607452393,0.005819134874662815
37337,74675,74674,149349,1.3453280925750732,0.005795195569261004
37437,74875,74874,149749,1.3487141132354736,0.005771354747629617
37538,75077,75076,150153,1.3519511222839355,0.0057473750711171815
37638,75277,75276,150553,1.3551180362701416,0.005723730977957329
37738,75477,75476,150953,1.3582971096038818,0.005700184154095967
37838,75677,75676,151353,1.3614740371704102,0.005676734199377498
37938,75877,75876,151753,1.3646681308746338,0.005653380715292511
38038,76077,76076,152153,1.3680620193481445,0.005630123304971026
38138,76277,76276,152553,1.3712382316589355,0.005606961573175729
38238,76477,76476,152953,1.3744561672210693,0.005583895126295303
38338,76677,76676,153353,1.3776400089263916,0.005560923572337659
38438,76877,76876,153753,1.3810203075408936,0.005538046520923362
38539,77079,77078,154157,1.3846280574798584,0.005515036227865703
38639,77279,77278,154557,1.3885712623596191,0.005492347952133196
38739,77479,77478,154957,1.392137050628662,0.005469753013567384
38839,77679,77678,155357,1.3966059684753418,0.005447251028189034
38939,77879,77878,155757,1.4002571105957031,0.0054248416135985736
39039,78079,78078,156157,1.4042060375213623,0.005402524388969544
39139,78279,78278,156557,1.4077770709991455,0.005380298975042232
39239,78479,78478,156957,1.411161184310913,0.005358164994117084
39339,78679,78678,157357,1.414586067199707,0.0053361220700484215
39439,78879,78878,157757,1.4182310104370117,0.005314169828237971
39540,79081,79080,158161,1.4215459823608398,0.005292089731105537
39640,79281,79280,158561,1.4247190952301025,0.005270318633680339
39740,79481,79480,158961,1.4280610084533691,0.0052486371002472615
39840,79681,79680,159361,1.43123197555542,0.005227044762349522
39940,79881,79880,159761,1.4344761371612549,0.005205541253046146
40040,80081,80080,160161,1.4376540184020996,0.005184126206905686
40140,80281,80280,160561,1.4409122467041016,0.005162799260000051
40240,80481,80480,160961,1.444087028503418,0.005141560049898295
40340,80681,80680,161361,1.4472720623016357,0.005120408215660488
40440,80881,80880,161761,1.4506349563598633,0.005099343397831577
40541,81083,81082,162165,1.4539179801940918,0.0050781558932589165
40641,81283,81282,162565,1.4571552276611328,0.005057264897015461
40741,81483,81482,162965,1.46038818359375,0.00503645984412097
40841,81683,81682,163365,1.4636249542236328,0.005015740381013602
40941,81883,81882,163765,1.4668631553649902,0.0049951061555860285
41041,82083,82082,164165,1.4701659679412842,0.004974556817179435
41141,82283,82282,164565,1.4734022617340088,0.004954092016577594
41241,82483,82482,164965,1.4766321182250977,0.004933711406000938
41341,82683,82682,165365,1.4798781871795654,0.004913414639100601
41441,82883,82882,165765,1.4831910133361816,0.004893201370952563
41542,83085,83084,166169,1.4866302013397217,0.004872870375698116
41642,83285,83284,166569,1.489866018295288,0.004852823902361474
41742,83485,83484,166969,1.4940290451049805,0.004832859898095875
41842,83685,83684,167369,1.4972460269927979,0.004812978023632288
41942,83885,83884,167769,1.5006589889526367,0.004793177941097396
42042,84085,84084,168169,1.504014015197754,0.004773459314007856
42142,84285,84284,168569,1.507349967956543,0.004753821807264584
42242,84485,84484,168969,1.5106632709503174,0.0047342650871470575
42342,84685,84684,169369,1.5139760971069336,0.004714788821307638
42442,84885,84884,169769,1.5173041820526123,0.004695392678765937
42543,85087,85086,170173,1.5208730697631836,0.004675883568260828
42643,85287,85286,170573,1.5241661071777344,0.004656647477815262
42743,85487,85486,170973,1.527440071105957,0.004637490522611249
42843,85687,85686,171373,1.5307278633117676,0.004618412377094773
42943,85887,85886,171773,1.534024953842163,0.004599412717051115
43043,86087,86086,172173,1.5373282432556152,0.004580491219599321
43143,86287,86286,172573,1.5406122207641602,0.004561647563186797
43243,86487,86486,172973,1.54398512840271,0.004542881427583712
43343,86687,86686,173373,1.5474650859832764,0.004524192493877646
43443,86887,86886,173773,1.5507981777191162,0.004505580444468188
43544,87089,87088,174177,1.5541441440582275,0.004486859993848942
43644,87289,87288,174577,1.5574321746826172,0.004468401526396055
43744,87489,87488,174977,1.5607280731201172,0.004450018995125976
43844,87689,87688,175377,1.5640339851379395,0.004431712087645273
43944,87889,87888,175777,1.5681800842285156,0.004413480492845678
44044,88089,88088,176177,1.5715179443359375,0.004395323900898777
44144,88289,88288,176577,1.5748679637908936,0.0043772420032507885
44244,88489,88488,176977,1.578179121017456,0.004359234492617242
44344,88689,88688,177377,1.5814809799194336,0.004341301062977856
44444,88889,88888,177777,1.584873914718628,0.004323441409571246
44545,89091,89090,178181,1.5885560512542725,0.004305477737096482
44645,89291,89290,178581,1.5918331146240234,0.004287765457063616
44745,89491,89490,178981,1.595184087753296,0.004270126043477431
44845,89691,89690,179381,1.598757266998291,0.00425255919657306
44945,89891,89890,179781,1.6022179126739502,0.00423506461781887
45045,90091,90090,180181,1.6055080890655518,0.00421764200991132
45145,90291,90290,180581,1.6092312335968018,0.004200291076769972
45245,90491,90490,180981,1.6130640506744385,0.004183011523532391
45345,90691,90690,181381,1.6163051128387451,0.004165803056549231
45445,90891,90890,181781,1.6196632385253906,0.004148665383379156
45546,91093,91092,182185,1.6229650974273682,0.0041314278961336074
45646,91293,91292,182585,1.6262671947479248,0.004114431638737725
45746,91493,91492,182985,1.6295502185821533,0.004097505302147127
45846,91693,91692,183385,1.6329452991485596,0.004080648598715015
45946,91893,91892,183785,1.6362502574920654,0.0040638612419779405
46046,92093,92092,184185,1.6396021842956543,0.0040471429466509235
46146,92293,92292,184585,1.6430940628051758,0.004030493428622653
46246,92493,92492,184985,1.6464550495147705,0.0040139124049505676
46346,92693,92692,185385,1.6500091552734375,0.003997399593856141
46446,92893,92892,185785,1.6533701419830322,0.003980954714720053
46547,93095,93094,186189,1.657137155532837,0.003964414056513435
46647,93295,93294,186589,1.6603782176971436,0.003948104876389191
46747,93495,93494,186989,1.663661003112793,0.00393186279050701
46847,93695,93694,187389,1.6672420501708984,0.003915687522848269
46947,93895,93894,187789,1.670553207397461,0.003899578798529858
47047,94095,94094,188189,1.6737961769104004,0.003883536343799519
47147,94295,94294,188589,1.6770381927490234,0.003867559886031196
47247,94495,94494,188989,1.6802639961242676,0.0038516491537203333
47347,94695,94694,189389,1.6835331916809082,0.003835803876479375
47447,94895,94894,189789,1.6869261264801025,0.0038200237850330694
47548,95097,95096,190193,1.6902611255645752,0.0038041517864052616
47648,95297,95296,190593,1.6935410499572754,0.0037885019083097856
47748,95497,95496,190993,1.6967942714691162,0.0037729164121575445
47848,95697,95696,191393,1.7000420093536377,0.0037573950330880546
47948,95897,95896,191793,1.7035491466522217,0.003741937507330403
48048,96097,96096,192193,1.7067639827728271,0.003726543572198825
48148,96297,96296,192593,1.7100021839141846,0.0037112129660882044
48248,96497,96496,192993,1.713327169418335,0.0036959454284696516
48348,96697,96696,193393,1.7165660858154297,0.0036807406998860446
48448,96897,96896,193793,1.7200090885162354,0.0036655985219476842
48549,97099,97098,194197,1.723426103591919,0.0036503681521949135
48649,97299,97298,194597,1.7267682552337646,0.0036353509237053447
48749,97499,97498,194997,1.7300441265106201,0.003620395474505458
48849,97699,97698,195397,1.7337872982025146,0.003605501550441781
48949,97899,97898,195797,1.7370612621307373,0.003590668898406413
49049,98099,98098,196197,1.7415440082550049,0.0035758972663327026
49149,98299,98298,196597,1.7449510097503662,0.0035611864031910023
49249,98499,98498,196997,1.7482361793518066,0.0035465360589843316
49349,98699,98698,197397,1.7518901824951172,0.0035319459847442335
49449,98899,98898,197797,1.7574551105499268,0.0035174159325263876
49550,99101,99100,198201,1.7624292373657227,0.003502801253666727
49650,99301,99300,198601,1.7662270069122314,0.003488391099789987
49750,99501,99500,199001,1.7705159187316895,0.003474040227762176
49850,99701,99700,199401,1.7761149406433105,0.00345974839370404
49950,99901,99900,199801,1.7812259197235107,0.003445515354739607
50050,100101,100100,200201,1.785677194595337,0.003431340868992097
50150,100301,100300,200601,1.7898952960968018,0.0034172246955797496
50250,100501,100500,201001,1.7945899963378906,0.003403166594611812
50350,100701,100700,201401,1.7993590831756592,0.0033891663271843615
50450,100901,100900,201801,1.8038651943206787,0.003375223655376346
50551,101103,101102,202205,1.8083691596984863,0.003361199777976271
50651,101303,101302,202605,1.812788963317871,0.00334737215759376
50751,101503,101502,203005,1.817121982574463,0.00333360142257898
50851,101703,101702,203405,1.8215911388397217,0.0033198873389115777
50951,101903,101902,203805,1.825890064239502,0.003306229673533883
51051,102103,102102,204205,1.830143928527832,0.003292628194347024
51151,102303,102302,204605,1.8345370292663574,0.0032790826702069516
51251,102503,102502,205005,1.8387541770935059,0.0032655928709205283
51351,102703,102702,205405,1.842900037765503,0.0032521585672415864
51451,102903,102902,205805,1.8476181030273438,0.003238779530867077
51552,103105,103104,206209,1.8518431186676025,0.0032253225716536013
51652,103305,103304,206609,1.856018304824829,0.003212053935726564
51752,103505,103504,207009,1.8598980903625488,0.0031988398855643464
51852,103705,103704,207409,1.8634212017059326,0.003185680196606894
51952,103905,103904,207809,1.866833209991455,0.003172574645217944
52052,104105,104104,208209,1.870253086090088,0.0031595230086812944
52152,104305,104304,208609,1.8736591339111328,0.003146525065196907
52252,104505,104504,209009,1.8770999908447266,0.0031335805938772707
52352,104705,104704,209409,1.880511999130249,0.003120689374743531
52452,104905,104904,209809,1.8839740753173828,0.0031078511887218507
52553,105107,105106,210213,1.8875839710235596,0.0030949382299083083
52653,105307,105306,210613,1.8910772800445557,0.003082205981372849
52753,105507,105506,211013,1.8946812152862549,0.0030695261119612276
52853,105707,105706,211413,1.8980810642242432,0.003056898406191248
52953,105907,105906,211813,1.9014461040496826,0.003044322649467209
53053,106107,106106,212213,1.9048182964324951,0.003031798628076219
53153,106307,106306,212613,1.908346176147461,0.0030193261291846262
53253,106507,106506,213013,1.9123361110687256,0.0030069049408342867
53353,106707,106706,213413,1.91566801071167,0.0029945348519390645
53453,106907,106906,213813,1.9190089702606201,0.0029822156522812003
53554,107109,107108,214217,1.922386884689331,0.002969824702537307
53654,107309,107308,214617,1.9258952140808105,0.002957607157820564
53754,107509,107508,215017,1.92946195602417,0.002945439874790568
53854,107709,107708,215417,1.9331791400909424,0.002933322646676077
53954,107909,107908,215817,1.9367790222167969,0.0029212552675564546
54054,108109,108108,216217,1.9405491352081299,0.002909237532358191
54154,108309,108308,216617,1.9439001083374023,0.002897269236851446
54254,108509,108508,217017,1.9481201171875,0.0028853501776465677
54354,108709,108708,217417,1.9516632556915283,0.0028734801521906176
54454,108909,108908,217817,1.9552791118621826,0.0028616589587639393
54555,109111,109110,218221,1.959618091583252,0.0028497689157634975
54655,109311,109310,218621,1.9631149768829346,0.0028380452678556027
54755,109511,109510,219021,1.967061996459961,0.002826369849795231
54855,109711,109710,219421,1.9708402156829834,0.002814742463169884
54955,109911,109910,219821,1.9745569229125977,0.002803162910383327
55055,110111,110110,220221,1.9780240058898926,0.0027916309946521838
55155,110311,110310,220621,1.9821200370788574,0.0027801465200026636
55255,110511,110510,221021,1.9857470989227295,0.002768709291267182
55355,110711,110710,221421,1.9899482727050781,0.002757319114081033
55455,110911,110910,221821,1.9941010475158691,0.0027459757948791255
55556,111113,111112,222225,2.0013041496276855,0.00273456640936194
55656,111313,111312,222625,2.005862236022949,0.0027233166923807577
55756,111513,111512,223025,2.0100719928741455,0.0027121132555454016
55856,111713,111712,223425,2.0153143405914307,0.002700955908464218
55956,111913,111912,223825,2.019813060760498,0.0026898444615288527
56056,112113,112112,224225,2.024792194366455,0.002678778725910949
56156,112313,112312,224625,2.029158115386963,0.0026677585135589927
56256,112513,112512,225025,2.0339109897613525,0.002656783637195071
56356,112713,112712,225425,2.0382111072540283,0.0026458539103117354
56456,112913,112912,225825,2.0431690216064453,0.002634969147168808
56557,113115,113114,226229,2.0473852157592773,0.0026240209884552273
56657,113315,113314,226629,2.052417039871216,0.0026132260436435933
56757,113515,113514,227029,2.0580930709838867,0.0026024755080931777
56857,113715,113714,227429,2.06246018409729,0.002591769199108963
56957,113915,113914,227829,2.067472219467163,0.0025811069347475447
57057,114115,114114,228229,2.0722429752349854,0.002570488533813974
57157,114315,114314,228629,2.0774521827697754,0.002559913815858767
57257,114515,114514,229029,2.082533121109009,0.002549382601174776
57357,114715,114714,229429,2.088052988052368,0.0025388947107941365
57457,114915,114914,229829,2.093203067779541,0.0025284499664852606
57558,115117,115116,230233,2.098886251449585,0.002517944389384992
57658,115317,115316,230633,2.103379011154175,0.002507585832482533
57758,115517,115516,231033,2.1084799766540527,0.002497269889587577
57858,115717,115716,231433,2.112950086593628,0.002486996385390603
57958,115917,115916,231833,2.1177260875701904,0.002476765145303307
58058,116117,116116,232233,2.121906280517578,0.0024665759954555846
58158,116317,116316,232633,2.1262261867523193,0.002456428762692665
58258,116517,116516,233033,2.130425214767456,0.002446323274572094
58358,116717,116716,233433,2.1346209049224854,0.0024362593593608246
58458,116917,116916,233833,2.1389319896698,0.00242623684603231
58559,117119,117118,234237,2.143961191177368,0.0024161559590907575
58659,117319,117318,234637,2.148271083831787,0.0024062161490246686
58759,117519,117518,235037,2.152677059173584,0.0023963172302858896
58859,117719,117718,235437,2.1570801734924316,0.0023864590346518114
58959,117919,117918,235837,2.161283016204834,0.0023766413945919148
59059,118119,118118,236237,2.165497064590454,0.0023668641432648277
59159,118319,118318,236637,2.169724225997925,0.0023571271145156024
59259,118519,118518,237037,2.174208164215088,0.0023474301428727863
59359,118719,118718,237437,2.1784660816192627,0.002337773063545691
59459,118919,118918,237837,2.1825451850891113,0.0023281557124215464
59560,119121,119120,238241,2.1863012313842773,0.0023184823474499345
59660,119321,119320,238641,2.1897451877593994,0.002308944356291497
59760,119521,119520,239041,2.1931309700012207,0.0022994456034198755
59860,119721,119720,239441,2.1969032287597656,0.002289985927412913
59960,119921,119920,239841,2.200469970703125,0.0022805651675125134
60060,120121,120120,240241,2.2039191722869873,0.0022711831636219463
60160,120321,120320,240641,2.207259178161621,0.0022618397563030795
60260,120521,120520,241041,2.2105820178985596,0.0022525347867736975
60360,120721,120720,241441,2.2141501903533936,0.0022432680969048063
60460,120921,120920,241841,2.2175660133361816,0.0022340395292179192
60561,121123,121122,242245,2.220975160598755,0.002224757212055106
60661,121323,121322,242645,2.224339008331299,0.0022156047961906537
60761,121523,121522,243045,2.227703094482422,0.0022064900323970297
60861,121723,121722,243445,2.2316291332244873,0.0021974127657776177
60961,121923,121922,243845,2.2350571155548096,0.002188372842073003
61061,122123,122122,244245,2.2385010719299316,0.002179370107658379
61161,122323,122322,244645,2.2418339252471924,0.0021704044095409553
61261,122523,122522,245045,2.2451388835906982,0.002161475595357307
61361,122723,122722,245445,2.2484662532806396,0.002152583513370839
61461,122923,122922,245845,2.2519149780273438,0.002143728012469163
61562,123125,123124,246249,2.2553012371063232,0.002134820934925411
61662,123325,123324,246649,2.2586512565612793,0.002126038507392765
61762,123525,123524,247049,2.262040138244629,0.002117292209838103
61862,123725,123724,247449,2.265519142150879,0.002108581893626524
61962,123925,123924,247849,2.269213914871216,0.0020999074107345707
62062,124125,124124,248249,2.2726690769195557,0.0020912686137477534
62162,124325,124324,248649,2.276052951812744,0.0020826653558580453
62262,124525,124524,249049,2.279412031173706,0.0020740974908613615
62362,124725,124724,249449,2.282963991165161,0.0020655648731550767
62462,124925,124924,249849,2.2864298820495605,0.002057067357735554
62563,125127,125126,250253,2.2908661365509033,0.002048520350670511
62663,125327,125326,250653,2.294239044189453,0.002040092954613752
62763,125527,125526,251053,2.2976021766662598,0.0020317002279730155
62863,125727,125726,251453,2.301054000854492,0.002023342028122002
62963,125927,125926,251853,2.304435968399048,0.002015018213021156
63063,126127,126126,252253,2.3078153133392334,0.0020067286412152655
63163,126327,126326,252653,2.3112142086029053,0.0019984731718310084
63263,126527,126526,253053,2.3145651817321777,0.001990251664574641
63363,126727,126726,253453,2.3179168701171875,0.0019820639797295697
63463,126927,126926,253853,2.321321964263916,0.001973909978153963
63564,127129,127128,254257,2.3248131275177,0.0019657084856429846
63664,127329,127328,254657,2.328119993209839,0.0019576217688401843
63764,127529,127528,255057,2.3314261436462402,0.0019495683199349915
63864,127729,127728,255457,2.334721088409424,0.001941548002066804
63964,127929,127928,255857,2.3380191326141357,0.001933560678938055
64064,128129,128128,256257,2.3413331508636475,0.0019256062148118587
64164,128329,128328,256657,2.3446362018585205,0.0019176844745097572
64264,128529,128528,257057,2.3479490280151367,0.001909795323409397
64364,128729,128728,257457,2.351149082183838,0.0019019386274422444
64464,128929,128928,257857,2.3543570041656494,0.0018941142530913338
64565,129131,129130,258261,2.3576080799102783,0.0018862443076360902
64665,129331,129330,258661,2.360812187194824,0.0018784844980569133
64765,129531,129530,259061,2.3640151023864746,0.0018707566115136087
64865,129731,129730,259461,2.3672173023223877,0.0018630605166781858
64965,129931,129930,259861,2.370413064956665,0.001855396082762924
65065,130131,130130,260261,2.3736250400543213,0.00184776317951815
65165,130331,130330,260661,2.3768341541290283,0.0018401616772300232
65265,130531,130530,261061,2.3805601596832275,0.001832591446718308
65365,130731,130730,261461,2.383810043334961,0.0018250523593342407
65465,130931,130930,261861,2.3870902061462402,0.0018175442869582783
65566,131133,131132,262265,2.3903801441192627,0.001809992485699441
65666,131333,131332,262665,2.3936309814453125,0.0018025463680507784
65766,131533,131532,263065,2.396876096725464,0.001795130882942572
65866,131733,131732,263465,2.4001190662384033,0.0017877459043557924
65966,131933,131932,263865,2.4033751487731934,0.0017803913067898248
66066,132133,132132,264265,2.406642198562622,0.0017730669652603658
66166,132333,132332,264665,2.410228967666626,0.0017657727552972784
66266,132533,132532,265065,2.41359806060791,0.0017585085529425069
66366,132733,132732,265465,2.4168620109558105,0.0017512742347479118
66466,132933,132932,265865,2.4203851222991943,0.0017440696777732204
66567,133135,133134,266269,2.4237101078033447,0.001736823159664914
66667,133335,133334,266669,2.426983118057251,0.0017296780528846538
66767,133535,133534,267069,2.430253028869629,0.0017225623403179775
66867,133735,133734,267469,2.4336190223693848,0.0017154759010401923
66967,133935,133934,267869,2.437106132507324,0.0017084186146240808
67067,134135,134134,268269,2.4403631687164307,0.0017013903611378695
67167,134335,134334,268669,2.443641185760498,0.001694391021143133
67267,134535,134534,269069,2.446883201599121,0.0016874204756928367
67367,134735,134734,269469,2.450119972229004,0.0016804786063292691
67467,134935,134934,269869,2.453352928161621,0.0016735652950820312
67568,135137,135136,270273,2.4566662311553955,0.001666611718988814
67668,135337,135336,270673,2.4599223136901855,0.0016597554546494539
67768,135537,135536,271073,2.4635610580444336,0.0016529273962564194
67868,135737,135736,271473,2.4674952030181885,0.001646127427773425
67968,135937,135936,271873,2.4711360931396484,0.0016393554336415486
68068,136137,136136,272273,2.4750571250915527,0.001632611298777284
68168,136337,136336,272673,2.4790589809417725,0.0016258949085705442
68268,136537,136536,273073,2.482680082321167,0.001619206148882733
68368,136737,136736,273473,2.4865872859954834,0.001612544906044839
68468,136937,136936,273873,2.4904398918151855,0.0016059110668554268
68569,137139,137138,274277,2.4937491416931152,0.0015992385905348953
68669,137339,137338,274677,2.497007131576538,0.0015926594921201371
68769,137539,137538,275077,2.5004310607910156,0.0015861074594204127
68869,137739,137738,275477,2.503737211227417,0.0015795823810902084
68969,137939,137938,275877,2.5070059299468994,0.0015730841462421178
69069,138139,138138,276277,2.510535955429077,0.0015666126444448963
69169,138339,138338,276677,2.5141451358795166,0.0015601677657215997
69269,138539,138538,277077,2.517402172088623,0.0015537494005477077
69369,138739,138738,277477,2.520659923553467,0.0015473574398492983
69469,138939,138938,277877,2.524022102355957,0.0015409917750011423
69570,139141,139140,278281,2.527338981628418,0.0015345890349359838
69670,139341,139340,278681,2.5305771827697754,0.0015282758979551663
69770,139541,139540,279081,2.5338480472564697,0.001521988732552163
69870,139741,139740,279481,2.537118911743164,0.0015157274318826548
69970,139941,139940,279881,2.5403411388397217,0.0015094918895418635
70070,140141,140140,280281,2.543729305267334,0.0015032819995627511
70170,140341,140340,280681,2.5477402210235596,0.0014970976564141962
70270,140541,140540,281081,2.551131248474121,0.001490938754999273
70370,140741,140740,281481,2.5557761192321777,0.0014848051906533562
70470,140941,140940,281881,2.559143304824829,0.0014786968591424235
70571,141143,141142,282285,2.5625059604644775,0.0014725529511879349
70671,141343,141342,282685,2.5659070014953613,0.0014664950240942938
70771,141543,141542,283085,2.569425106048584,0.0014604620186719783
70871,141743,141742,283485,2.5727570056915283,0.001454453832395876
70971,141943,141942,283885,2.576066017150879,0.00144847036316264
71071,142143,142142,284285,2.5793821811676025,0.0014425115092889865
71171,142343,142342,284685,2.58274507522583,0.0014365771695099103
71271,142543,142542,285085,2.586076259613037,0.0014306672429770244
71371,142743,142742,285485,2.589564323425293,0.0014247816292568235
71471,142943,142942,285885,2.593600034713745,0.0014189202283289575
71572,143145,143144,286289,2.597100019454956,0.0014130246891427183
71672,143345,143344,286689,2.6006901264190674,0.0014072116550229877
71772,143545,143544,287089,2.6042091846466064,0.001401422535110811
71872,143745,143744,287489,2.607793092727661,0.001395657231025652
71972,143945,143944,287889,2.6116490364074707,0.0013899156447917012
72072,144145,144144,288289,2.6156511306762695,0.0013841976788362704
72172,144345,144344,288689,2.6201159954071045,0.0013785032359880003
72272,144545,144544,289089,2.624691963195801,0.001372832219475324
72372,144745,144744,289489,2.629149913787842,0.001367184532924772
72472,144945,144944,289889,2.633350133895874,0.001361560080359351
72573,145147,145146,290293,2.637892246246338,0.0013559028695818089
72673,145347,145346,290693,2.6423659324645996,0.0013503248285861524
72773,145547,145546,291093,2.6466989517211914,0.0013447697350611769
72873,145747,145746,291493,2.651041030883789,0.001339237494603421
72973,145947,145946,291893,2.6552491188049316,0.001333728013197769
73073,146147,146146,292293,2.6596250534057617,0.0013282411972158998
73173,146347,146346,292693,2.6637370586395264,0.0013227769534146663
73273,146547,146546,293093,2.667600154876709,0.0013173351889344982
73373,146747,146746,293493,2.6709721088409424,0.0013119158112978406
73473,146947,146946,293893,2.674309253692627,0.0013065187284075806
73574,147149,147148,294297,2.6776750087738037,0.0013010902115628044
73674,147349,147348,294697,2.6810190677642822,0.0012957376640448696
73774,147549,147548,295097,2.684554100036621,0.0012904071363412947
73874,147749,147748,295497,2.687933921813965,0.0012850985378648904
73974,147949,147948,295897,2.691317081451416,0.0012798117784011552
74074,148149,148148,296297,2.694671154022217,0.0012745467681066836
74174,148349,148348,296697,2.6980249881744385,0.001269303417507698
74274,148549,148548,297097,2.70145320892334,0.0012640816374985138
74374,148749,148748,297497,2.704846143722534,0.0012588813393399842
74474,148949,148948,297897,2.708214044570923,0.0012537024346580565
74575,149151,149150,298301,2.7117602825164795,0.001248493366745823
74675,149351,149350,298701,2.715097188949585,0.0012433571970844517
74775,149551,149550,299101,2.718459129333496,0.0012382421570818233
74875,149751,149750,299501,2.7219130992889404,0.0012331481598127723
74975,149951,149950,299901,2.7253172397613525,0.0012280751187097034
75075,150151,150150,300301,2.7287330627441406,0.0012230229475611747
75175,150351,150350,300701,2.732131004333496,0.0012179915605103951
75275,150551,150550,301101,2.735558271408081,0.001212980872053783
75375,150751,150750,301501,2.7389490604400635,0.0012079907970395229
75475,150951,150950,301901,2.742333173751831,0.0012030212506660963
75576,151153,151152,302305,2.745809316635132,0.0011980227604172593
75676,151353,151352,302705,2.749169111251831,0.0011930942214922022
75776,151553,151552,303105,2.7524731159210205,0.0011881859580550004
75876,151753,151752,303505,2.7559030055999756,0.001183297886694451
75976,151953,151952,303905,2.7592849731445312,0.001178429924342487
76076,152153,152152,304305,2.7629730701446533,0.0011735819882727528
76176,152353,152352,304705,2.7662951946258545,0.0011687539960992717
76276,152553,152552,305105,2.7698750495910645,0.0011639458657749313
76376,152753,152752,305505,2.7739388942718506,0.0011591575155902255
76476,152953,152952,305905,2.777735948562622,0.001154388864171719
76577,153155,153154,306309,2.7817232608795166,0.0011495924389400586
76677,153355,153354,306709,2.7859652042388916,0.001144863137235229
76777,153555,153554,307109,2.7902262210845947,0.001140153291377413
76877,153755,153754,307509,2.794365167617798,0.0011354628213273007
76977,153955,153954,307909,2.798495054244995,0.0011307916473748854
77077,154155,154154,308309,2.802588939666748,0.0011261396901380532
77177,154355,154354,308709,2.8071680068969727,0.0011215068705612604
77277,154555,154554,309109,2.811337947845459,0.0011168931099141952
77377,154755,154754,309509,2.815206289291382,0.0011122983297904595
77477,154955,154954,309909,2.818751096725464,0.0011077224521061743
77578,155157,155156,310313,2.8228821754455566,0.0011031199233709635
77678,155357,155356,310713,2.8266103267669678,0.0010985818046799188
77778,155557,155556,311113,2.829935073852539,0.0010940623553291973
77878,155757,155756,311513,2.833252191543579,0.0010895614985150842
77978,155957,155956,311913,2.836679220199585,0.0010850791577498718
78078,156157,156156,312313,2.84074330329895,0.001080615256860472
78178,156357,156356,312713,2.8440821170806885,0.0010761697199872051
78278,156557,156556,313113,2.847403049468994,0.0010717424715824412
78378,156757,156756,313513,2.850788116455078,0.0010673334364093585
78478,156957,156956,313913,2.8543732166290283,0.0010629425395406503
78579,157159,157158,314317,2.8588011264801025,0.0010585260689953125
78679,157359,157358,314717,2.862999200820923,0.001054171404704609
78779,157559,157558,315117,2.866610288619995,0.0010498346550422174
78879,157759,157758,315517,2.8699920177459717,0.0010455157463092463
78979,157959,157958,315917,2.8745391368865967,0.0010412146051100048
79079,158159,158158,316317,2.8778440952301025,0.0010369311583507488
79179,158359,158358,316717,2.8823111057281494,0.0010326653332384033
79279,158559,158558,317117,2.8857672214508057,0.0010284170572793824
79379,158759,158758,317517,2.890029191970825,0.0010241862582783293
79479,158959,158958,317917,2.893334150314331,0.0010199728643369079
79580,159161,159160,318321,2.8966519832611084,0.0010157349305401128
79680,159361,159360,318721,2.900031089782715,0.0010115563044671315
79780,159561,159560,319121,2.9033701419830322,0.0010073948688198546
79880,159761,159760,319521,2.9081809520721436,0.0010032505528786693
79980,159961,159960,319921,2.9125571250915527,0.000999123286214956
80080,160161,160160,320321,2.9164040088653564,0.0009950129986897663
80180,160361,160360,320721,2.9206771850585938,0.0009909196204527177
80280,160561,160560,321121,2.925488233566284,0.0009868430819407832
80380,160761,160760,321521,2.9293131828308105,0.0009827833138771347
80480,160961,160960,321921,2.9334352016448975,0.0009787402472699015
80581,161163,161162,322325,2.938805103302002,0.0009746736328361112
80681,161363,161362,322725,2.9430739879608154,0.0009706639285989526
80781,161563,161562,323125,2.947453260421753,0.0009666707198609293
80881,161763,161762,323525,2.951794147491455,0.0009626939387612899
80981,161963,161962,323925,2.956806182861328,0.0009587335177184958
81081,162163,162162,324325,2.961050271987915,0.0009547893894289958
81181,162363,162362,324725,2.9654541015625,0.0009508614868661091
81281,162563,162562,325125,2.9696240425109863,0.0009469497432789391
81381,162763,162762,325525,2.973743200302124,0.0009430540921911496
81481,162963,162962,325925,2.977874994277954,0.0009391744673998846
81582,163165,163164,326329,2.9822750091552734,0.000935272246707893
81682,163365,163364,326729,2.986279249191284,0.0009314246356059012
81782,163565,163564,327129,2.9905941486358643,0.0009275928531690238
81882,163765,163764,327529,2.994692087173462,0.0009237768342798167
81982,163965,163964,327929,2.998950242996216,0.0009199765140887116
82082,164165,164164,328329,3.002901077270508,0.0009161918280129229
82182,164365,164364,328729,3.006622076034546,0.0009124227117353531
82282,164565,164564,329129,3.0102710723876953,0.0009086691012035014
82382,164765,164764,329529,3.013606071472168,0.0009049309326283809
82482,164965,164964,329929,3.016956090927124,0.0009012081424833965
82583,165167,165166,330333,3.0203630924224854,0.0008974636698816971
82683,165367,165366,330733,3.0237560272216797,0.0008937715992658582
82783,165567,165566,331133,3.0270471572875977,0.0008900947174380366
82883,165767,165766,331533,3.030333995819092,0.0008864329619131639
82983,165967,165966,331933,3.033628225326538,0.000882786270463232
83083,166167,166166,332333,3.0369069576263428,0.0008791545811162163
83183,166367,166366,332733,3.040318012237549,0.0008755378321550661
83283,166567,166566,333133,3.043642044067383,0.0008719359621165982
83383,166767,166766,333533,3.0469470024108887,0.0008683489097905232
83483,166967,166966,333933,3.0502240657806396,0.0008647766142183077
83584,167169,167168,334337,3.0535261631011963,0.0008611835127072635
83684,167369,167368,334737,3.0568270683288574,0.000857640694820799
83784,167569,167568,335137,3.0600380897521973,0.0008541124517124077
83884,167769,167768,335537,3.063260316848755,0.0008505987234229927
83984,167969,167968,335937,3.066486120223999,0.0008470994502401269
84084,168169,168168,336337,3.069788932800293,0.0008436145726970179
84184,168369,168368,336737,3.0729970932006836,0.0008401440315715475
84284,168569,168568,337137,3.076198101043701,0.0008366877678851835
84384,168769,168768,337537,3.079393148422241,0.0008332457229020795
84484,168969,168968,337937,3.0825998783111572,0.0008298178381279802
84585,169171,169170,338341,3.085824966430664,0.0008263699884994855
84685,169371,169370,338741,3.0890181064605713,0.000822970389769486
84785,169571,169570,339141,3.092302083969116,0.0008195847766291025
84885,169771,169770,339541,3.095506191253662,0.0008162130915430944
84985,169971,169970,339941,3.09871506690979,0.0008128552772129153
85085,170171,170170,340341,3.1019420623779297,0.0008095112765757376
85185,170371,170370,340741,3.1051509380340576,0.0008061810328035038
85285,170571,170570,341141,3.1083619594573975,0.0008028644893019075
85385,170771,170770,341541,3.1115729808807373,0.0007995615897095013
85485,170971,170970,341941,3.114995002746582,0.0007962722778966719
85586,171173,171172,342345,3.1184189319610596,0.0007929638083128772
85686,171373,171372,342745,3.1216881275177,0.000789701639074892
85786,171573,171572,343145,3.125298261642456,0.0007864528900561255
85886,171773,171772,343545,3.128618001937866,0.0007832175060472207
85986,171973,171972,343945,3.131859064102173,0.0007799954320659252
86086,172173,172172,344345,3.1351330280303955,0.0007767866133561951
86186,172373,172372,344745,3.1384010314941406,0.0007735909953872531
86286,172573,172572,345145,3.1417040824890137,0.0007704085238526242
86386,172773,172772,345545,3.1453099250793457,0.0007672391446693147
86486,172973,172972,345945,3.1485209465026855,0.0007640828039767418
86587,173175,173174,346349,3.1524200439453125,0.0007609080799701154
86687,173375,173374,346749,3.155625104904175,0.0007577777846080904
86787,173575,173574,347149,3.1588239669799805,0.000754660366950111
86887,173775,173774,347549,3.1622681617736816,0.0007515557740186439
86987,173975,173974,347949,3.1656482219696045,0.0007484639530541494
87087,174175,174174,348349,3.169098138809204,0.0007453848515140839
87187,174375,174374,348749,3.1723880767822266,0.0007423184170720906
87287,174575,174574,349149,3.1756181716918945,0.0007392645976170561
87387,174775,174774,349549,3.179081916809082,0.0007362233412522726
87487,174975,174974,349949,3.1826329231262207,0.0007331945962945061
87588,175177,175176,350353,3.1859240531921387,0.0007301482111720159
87688,175377,175376,350753,3.189359188079834,0.0007271444586568655
87788,175577,175576,351153,3.192589044570923,0.0007241530632618487
87888,175777,175776,351553,3.1958820819854736,0.0007211739741510998
87988,175977,175976,351953,3.1996560096740723,0.0007182071406978532
88088,176177,176176,352353,3.203274965286255,0.0007152525124836574
88188,176377,176376,352753,3.2070131301879883,0.0007123100392974267
88288,176577,176576,353153,3.210604190826416,0.0007093796711346646
88388,176777,176776,353553,3.214548110961914,0.000706461358196588
88488,176977,176976,353953,3.2185442447662354,0.0007035550508892803
88589,177179,177178,354357,3.222343921661377,0.0007006318165245928
88689,177379,177378,354757,3.2264211177825928,0.0006977494913351491
88789,177579,177578,355157,3.230034112930298,0.0006948790237266729
88889,177779,177778,355557,3.2333950996398926,0.0006920203649183336
88989,177979,177978,355957,3.2384262084960938,0.0006891734663299825
89089,178179,178178,356357,3.2419471740722656,0.0006863382795813204
89189,178379,178378,356757,3.2452139854431152,0.0006835147564910646
89289,178579,178578,357157,3.2485060691833496,0.0006807028490761866
89389,178779,178778,357557,3.2518510818481445,0.0006779025095509966
89489,178979,178978,357957,3.255195140838623,0.0006751136903264208
89590,179181,179180,358361,3.2585642337799072,0.0006723086283243344
89690,179381,179380,358761,3.2619199752807617,0.0006695428217354923
89790,179581,179580,359161,3.265263080596924,0.0006667883933824186
89890,179781,179780,359561,3.268609046936035,0.0006640452964562696
89990,179981,179980,359961,3.2719459533691406,0.000661313484340747
90090,180181,180180,360361,3.2752912044525146,0.0006585929106113304
90190,180381,180380,360761,3.278651237487793,0.0006558835290344818
90290,180581,180580,361161,3.2820122241973877,0.0006531852935668883
90390,180781,180780,361561,3.2857160568237305,0.0006504981583546004
90490,180981,180980,361961,3.2890710830688477,0.0006478220777323728
90591,181183,181182,362365,3.2925779819488525,0.0006451304109503172
90691,181383,181382,362765,3.2959790229797363,0.0006424764126731859
90791,181583,181582,363165,3.2993359565734863,0.0006398333326642635
90891,181783,181782,363565,3.3026959896087646,0.000637201126006946
90991,181983,181982,363965,3.306140899658203,0.0006345797479694101
91091,182183,182182,364365,3.30950927734375,0.0006319691540038736
91191,182383,182382,364765,3.312934160232544,0.0006293692997457922
91291,182583,182582,365165,3.3162741661071777,0.0006267801410131619
91391,182783,182782,365565,3.319714069366455,0.0006242016338056925
91491,182983,182982,365965,3.3230340480804443,0.0006216337343041626
91592,183185,183184,366369,3.3263869285583496,0.0006190508787165712
91692,183385,183384,366769,3.3297040462493896,0.000616504168876702
91792,183585,183584,367169,3.3330130577087402,0.0006139679359317464
91892,183785,183784,367569,3.3363242149353027,0.0006114421367808764
91992,183985,183984,367969,3.3396451473236084,0.0006089267285005744
92092,184185,184184,368369,3.342949151992798,0.0006064216683438989
92192,184385,184384,368769,3.3463191986083984,0.0006039269137397423
92292,184585,184584,369169,3.349705934524536,0.0006014424222921702
92392,184785,184784,369569,3.3530590534210205,0.0005989681517796376
92492,184985,184984,369969,3.356401205062866,0.0005965040601543032
92593,185187,185186,370373,3.3600270748138428,0.0005940256170458203
92693,185387,185386,370773,3.3633511066436768,0.0005915818584856152
92793,185587,185586,371173,3.3673882484436035,0.0005891481532896432
92893,185787,185786,371573,3.3707871437072754,0.0005867244600994535
92993,185987,185986,371973,3.3745882511138916,0.0005843107377267003
93093,186187,186186,372373,3.3780171871185303,0.0005819069451524923
93193,186387,186386,372773,3.3814709186553955,0.0005795130415266957
93293,186587,186586,373173,3.3850691318511963,0.0005771289861672234
93393,186787,186786,373573,3.3884570598602295,0.0005747547385593525
93493,186987,186986,373973,3.3916900157928467,0.0005723902583550136
93594,187189,187188,374377,3.3949670791625977,0.0005700120068292604
93694,187389,187388,374777,3.398426055908203,0.0005676670377216321
93794,187589,187588,375177,3.4016671180725098,0.0005653317155688939
93894,187789,187788,375577,3.404902219772339,0.0005630060006845002
93994,187989,187988,375977,3.408151149749756,0.0005606898535451493
94094,188189,188188,376377,3.4113810062408447,0.0005583832347901581
94194,188389,188388,376777,3.4146649837493896,0.0005560861052207555
94294,188589,188588,377177,3.4179301261901855,0.0005537984257994406
94394,188789,188788,377577,3.4211649894714355,0.0005515201576493039
94494,188989,188988,377977,3.424391984939575,0.000549251262053377
94595,189191,189190,378381,3.4276559352874756,0.0005469691518445876
94695,189391,189390,378781,3.4308888912200928,0.0005447189786051994
94795,189591,189590,379181,3.4341330528259277,0.0005424780623405207
94895,189791,189790,379581,3.4373581409454346,0.0005402463649683385
94995,189991,189990,379981,3.4405839443206787,0.0005380238485631097
95095,190191,190190,380381,3.443808078765869,0.0005358104753552924
95195,190391,190390,380781,3.4470269680023193,0.0005336062077307536
95295,190591,190590,381181,3.45039701461792,0.0005314110082300831
95395,190791,190790,381581,3.453606128692627,0.0005292248395479789
95495,190991,190990,381981,3.456818103790283,0.0005270476645326075
95596,191193,191192,382385,3.4600601196289062,0.0005248578091078595
95696,191393,191392,382785,3.4632701873779297,0.0005226985995938372
95796,191593,191592,383185,3.4666340351104736,0.0005205482728393725
95896,191793,191792,383585,3.4700522422790527,0.0005184067923017403
95996,191993,191992,383985,3.473283052444458,0.0005162741215885456
96096,192193,192192,384385,3.4765000343322754,0.0005141502244571144
96196,192393,192392,384785,3.4797260761260986,0.0005120350648138418
96296,192593,192592,385185,3.4829602241516113,0.0005099286067136191
96396,192793,192792,385585,3.486358165740967,0.0005078308143592323
96496,192993,192992,385985,3.4895901679992676,0.0005057416521007108
96597,193195,193194,386389,3.4928929805755615,0.0005036403220410416
96697,193395,193394,386789,3.496135950088501,0.0005015683990246994
96797,193595,193594,387189,3.499389886856079,0.0004995049996805148
96897,193795,193794,387589,3.5027172565460205,0.0004974500889429897
96997,193995,193994,387989,3.506026029586792,0.0004954036318908944
97097,194195,194194,388389,3.5092689990997314,0.0004933655937466648
97197,194395,194394,388789,3.5125460624694824,0.0004913359398757927
97297,194595,194594,389189,3.515791177749634,0.0004893146357862796
97397,194795,194794,389589,3.519026279449463,0.000487301647128011
97497,194995,194994,389989,3.5223889350891113,0.0004852969396921588
97598,195197,195196,390393,3.525656223297119,0.00048328055634108214
97698,195397,195396,390793,3.528907060623169,0.00048129239124743264
97798,195597,195596,391193,3.532165050506592,0.00047931240525470335
97898,195797,195796,391593,3.5354251861572266,0.00047734056471492676
97998,195997,195996,391993,3.5386621952056885,0.0004753768361185795
98098,196197,196196,392393,3.5419399738311768,0.000473421186093979
98198,196397,196396,392793,3.5452489852905273,0.0004714735814067335
98298,196597,196596,393193,3.548583984375,0.00046953398895918826
98398,196797,196796,393593,3.5519039630889893,0.0004676023757898199
98498,196997,196996,393993,3.5551791191101074,0.00046567870907273816
98599,197199,197198,394397,3.558532238006592,0.0004637438384417335
98699,197399,197398,394797,3.5618250370025635,0.0004618360453391859
98799,197599,197598,395197,3.565160036087036,0.00045993610069567774
98899,197799,197798,395597,3.5684821605682373,0.0004580439722234852
98999,197999,197998,395997,3.5718300342559814,0.0004561596277677057
99099,198199,198198,396397,3.5751349925994873,0.00045428303530572464
99199,198399,198398,396797,3.578705310821533,0.000452414162946645
99299,198599,198598,397197,3.5820579528808594,0.000450552978930778
99399,198799,198798,397597,3.585475206375122,0.0004486994516291035
99499,198999,198998,397997,3.5888519287109375,0.0004468535495427096
99600,199201,199200,398401,3.592280149459839,0.000444996896462976
99700,199401,199400,398801,3.5956621170043945,0.00044316622629691983
99800,199601,199600,399201,3.5991601943969727,0.00044134308731430094
99900,199801,199800,399601,3.6024010181427,0.00043952744853262976
100000,200001,200000,400001,3.606074094772339,0.00043771927909687125


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha0/flex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.985664367675781e-05,4.387061074692293
3,11,0,11,0.0006079673767089844,3.4741628962390445
6,24,0,24,0.0011477470397949219,2.033263258797766
8,32,0,32,0.0014929771423339844,1.5522093526709104
11,43,0,43,0.0019519329071044922,0.9650411560238331
14,56,0,56,0.0024890899658203125,0.6482458383208611
17,67,0,67,0.0029799938201904297,0.39693923901169775
20,80,0,80,0.0040760040283203125,0.27680455314284697
23,91,0,91,0.0047149658203125,0.20419425627261448
25,99,0,99,0.0052318572998046875,0.15265852588613407
28,110,0,110,0.006076812744140625,0.0957299899463542
31,124,0,124,0.006824970245361328,0.0894349852981967
34,137,0,137,0.00745081901550293,0.07677925190745234
37,152,0,152,0.0080718994140625,0.0723100619282481
39,161,0,161,0.008491992950439453,0.06988901781410752
42,176,0,176,0.009246826171875,0.06667845344878436
45,191,0,191,0.009894847869873047,0.06472750147395719
48,205,0,205,0.010663747787475586,0.062263640228154726
51,220,0,220,0.011297941207885742,0.06011079359259012
53,230,0,230,0.011838912963867188,0.0591534071850047
56,245,0,245,0.013303995132446289,0.058124715525270716
59,260,0,260,0.014185905456542969,0.05738350575689567
62,274,0,274,0.014801740646362305,0.05606359877987347
65,289,0,289,0.015417814254760742,0.054133236053776436
68,303,0,303,0.01601099967956543,0.052136238317722676
70,312,0,312,0.01639699935913086,0.04865143368456347
73,326,0,326,0.016981840133666992,0.04626360920109495
76,341,0,341,0.017714738845825195,0.044773326928866174
79,356,0,356,0.01866006851196289,0.04379514667363227
82,371,0,371,0.019322872161865234,0.04310283378045328
84,381,0,381,0.019749879837036133,0.04273835653747295
87,396,0,396,0.020467758178710938,0.04228519146178645
90,410,0,410,0.021309852600097656,0.03966934966391387
93,425,0,425,0.022249937057495117,0.038816030745483156
96,439,0,439,0.023055076599121094,0.03599933450388453
99,454,0,454,0.023736953735351562,0.035486005928600885
101,464,0,464,0.024135828018188477,0.035253876471242604
104,478,0,478,0.024715900421142578,0.03426594091783847
107,493,0,493,0.025307893753051758,0.03334683373825475
110,508,0,508,0.025937795639038086,0.03282104627138537
113,523,0,523,0.02652287483215332,0.0324995592738787
115,533,0,533,0.02690601348876953,0.03234898135129565
118,548,0,548,0.02751302719116211,0.03217875120664512
121,563,0,563,0.028342008590698242,0.03204913635210186
124,578,0,578,0.02912306785583496,0.03194368632734536
127,593,0,593,0.02972698211669922,0.03185352886552249
129,602,0,602,0.03012704849243164,0.03135583217504798
132,615,0,615,0.030731916427612305,0.02949416170223632
135,629,0,629,0.03130006790161133,0.028598796880318737
138,644,0,644,0.03194689750671387,0.02769540070249711
141,659,0,659,0.03253293037414551,0.0271178643751746
144,674,0,674,0.03310894966125488,0.02672647502178294
146,684,0,684,0.033490896224975586,0.02652995274857543
149,699,0,699,0.03407406806945801,0.026298164672867236
152,714,0,714,0.034648895263671875,0.026118140915158055
155,729,0,729,0.03522300720214844,0.02597344358746509
158,744,0,744,0.0357968807220459,0.0258540949835161
160,754,0,754,0.03617978096008301,0.02578536994673653
163,769,0,769,0.036766767501831055,0.025695190573519256
166,784,0,784,0.037323951721191406,0.025617604874861144
169,799,0,799,0.037899017333984375,0.025550178350329505
172,814,0,814,0.03871893882751465,0.025491085489001135
175,829,0,829,0.03944277763366699,0.0254389174760374
177,839,0,839,0.0398409366607666,0.02540742712246746
180,854,0,854,0.040428876876831055,0.025364439726939768
183,869,0,869,0.041046857833862305,0.025325870953955235
186,884,0,884,0.04163503646850586,0.02529108241652566
189,899,0,899,0.04220271110534668,0.02525954534023171
191,909,0,909,0.042578935623168945,0.025240105965788188
194,924,0,924,0.043138980865478516,0.025213042563610163
197,939,0,939,0.04374074935913086,0.02518820384732891
200,954,0,954,0.04438185691833496,0.02516530905747868
203,969,0,969,0.04492378234863281,0.02514411911627242
205,979,0,979,0.04527688026428223,0.025130837428951575
208,994,0,994,0.04580092430114746,0.025112049125038345
211,1009,0,1009,0.04630398750305176,0.025094482567631454
214,1024,0,1024,0.04681396484375,0.025078000671437676
217,1039,0,1039,0.04729175567626953,0.02506248470147327
220,1054,0,1054,0.047831058502197266,0.025047831495011625
222,1064,0,1064,0.04819202423095703,0.02503849712182878
225,1079,0,1079,0.04867076873779297,0.02502508773093823
228,1094,0,1094,0.04916977882385254,0.025012325714159102
231,1109,0,1109,0.049626827239990234,0.025000147888817076
234,1124,0,1124,0.05008983612060547,0.024988498615965728
236,1134,0,1134,0.05040097236633301,0.024981001572740483
239,1149,0,1149,0.05086088180541992,0.0249701268596274
242,1164,0,1164,0.05140089988708496,0.024959661833938687
245,1179,0,1179,0.05191969871520996,0.02494957078499455
248,1194,0,1194,0.052391767501831055,0.024939821879930334
251,1209,0,1209,0.052865028381347656,0.02493038667256916
253,1219,0,1219,0.053177833557128906,0.0249242581168589
256,1234,0,1234,0.05364871025085449,0.024915290412866224
259,1249,0,1249,0.05411887168884277,0.024906574083800367
262,1264,0,1264,0.05458879470825195,0.02489808991443535
265,1279,0,1279,0.05506491661071777,0.02488982054909124
267,1289,0,1289,0.05537676811218262,0.024884419154833293
270,1304,0,1304,0.05593085289001465,0.024876473615579844
273,1319,0,1319,0.0563960075378418,0.024868704156350077
276,1334,0,1334,0.056860923767089844,0.02486109861678486
279,1349,0,1349,0.05736494064331055,0.024853645911718306
281,1359,0,1359,0.05793404579162598,0.024848757314232695
284,1374,0,1374,0.05865287780761719,0.024841537267833752
287,1389,0,1389,0.05913686752319336,0.024834444935688718
290,1404,0,1404,0.059593915939331055,0.024827472307222744
293,1419,0,1419,0.0600588321685791,0.024820612024042597
296,1434,0,1434,0.060545921325683594,0.024813857317037228
298,1444,0,1444,0.06086397171020508,0.024809409732708496
301,1459,0,1459,0.06146502494812012,0.024802817369745846
304,1474,0,1474,0.06203794479370117,0.024796315007519106
307,1489,0,1489,0.06258678436279297,0.02478989760439496
310,1504,0,1504,0.06308388710021973,0.024783560494637768
312,1514,0,1514,0.06339788436889648,0.02477937821432344
315,1529,0,1529,0.06386876106262207,0.024773165476567483
318,1544,0,1544,0.0644829273223877,0.024767022187932582
321,1559,0,1559,0.06518077850341797,0.02476094480347465
324,1574,0,1574,0.06585383415222168,0.024754930026306847
327,1589,0,1589,0.0663900375366211,0.02474897478731834
329,1599,0,1599,0.06671404838562012,0.0247450362844543
332,1614,0,1614,0.06735777854919434,0.02473917401667633
335,1629,0,1629,0.06790971755981445,0.024733364081948886
338,1644,0,1644,0.06850886344909668,0.024727604101530513
341,1659,0,1659,0.06901979446411133,0.024721891851965633
343,1669,0,1669,0.06936383247375488,0.02471810917000097
346,1684,0,1684,0.06983184814453125,0.024712471915575854
349,1699,0,1699,0.07029986381530762,0.024706877135234666
352,1714,0,1714,0.07077288627624512,0.024701323081194042
355,1729,0,1729,0.07132887840270996,0.02469580811378722
357,1739,0,1739,0.07188868522644043,0.024692152419549543
360,1754,0,1754,0.07245993614196777,0.02468669922191886
363,1769,0,1769,0.07293200492858887,0.024681281209452247
366,1784,0,1784,0.07346510887145996,0.024675897076540262
369,1799,0,1799,0.07426977157592773,0.024670545594156646
372,1814,0,1814,0.07475090026855469,0.02466522560454406
374,1824,0,1824,0.07506394386291504,0.024661695899235385
377,1839,0,1839,0.07552981376647949,0.02465642600297453
380,1854,0,1854,0.07602572441101074,0.024651184824451968
383,1869,0,1869,0.07649683952331543,0.024645971428046688
386,1884,0,1884,0.07697081565856934,0.024640784929513486
388,1894,0,1894,0.07741999626159668,0.02463734179223725
391,1908,0,1908,0.0779118537902832,0.02425857612550655
394,1921,0,1921,0.07836484909057617,0.021533031711729222
397,1933,0,1933,0.07893586158752441,0.020698134118432476
400,1944,0,1944,0.07949090003967285,0.008007824111302573
403,1956,0,1956,0.07993793487548828,0.004547834043511745
405,1963,0,1963,0.08021688461303711,0.004101530885530421
408,1976,0,1976,0.08076167106628418,0.003702841073098849
411,1989,0,1989,0.08130979537963867,0.0032970324091014433
414,2001,0,2001,0.08182501792907715,0.0025450657237090766
417,2014,0,2014,0.08262276649475098,0.00220973849520187
419,2023,0,2023,0.08308601379394531,0.002073723942848947
422,2037,0,2037,0.0839080810546875,0.0018195650601700558
425,2048,0,2048,0.08455491065979004,0.0015214498210473115
428,2062,0,2062,0.08523893356323242,0.0013508347226733513
431,2077,0,2077,0.08629179000854492,0.001207069572147657
433,2086,0,2086,0.08687472343444824,0.001094651560872261
436,2099,0,2099,0.08754777908325195,0.0009711085179419887
439,2113,0,2113,0.08809804916381836,0.0009015208564362566
442,2126,0,2126,0.08882880210876465,0.0008087831409044648
445,2139,0,2139,0.08974790573120117,0.0007193114120497419
448,2152,0,2152,0.09026288986206055,0.0005630538695601275
450,2162,0,2162,0.09060978889465332,0.0005196780929800157
453,2176,0,2176,0.09106564521789551,0.00044701962085520454
456,2190,0,2190,0.09151792526245117,0.0003921332285953227
459,2205,0,2205,0.09198594093322754,0.0003683139054069744
462,2220,0,2220,0.09244990348815918,0.0003509344481207514
464,2230,0,2230,0.09275698661804199,0.0003417349195812294
467,2244,0,2244,0.09320592880249023,0.0003163611117141438
470,2259,0,2259,0.09367799758911133,0.0003026315136456489
473,2274,0,2274,0.09416604042053223,0.00029285485163113074
476,2288,0,2288,0.09461808204650879,0.00028048113290541363
479,2303,0,2303,0.09508180618286133,0.0002708117098618962
481,2313,0,2313,0.09539294242858887,0.00026580047979549057
484,2327,0,2327,0.09584474563598633,0.00024802594733156624
487,2341,0,2341,0.09629678726196289,0.0002375704954349332
490,2356,0,2356,0.09676575660705566,0.00023003512579139744
493,2370,0,2370,0.09721899032592773,0.00021823060852090652
495,2380,0,2380,0.09753274917602539,0.00021449641183912544
498,2395,0,2395,0.09800076484680176,0.00021048151470706844
501,2408,0,2408,0.09853696823120117,0.0001991828081748395
504,2423,0,2423,0.09923601150512695,0.00019002361184008545
507,2437,0,2437,0.09992194175720215,0.00017853159588839053
509,2447,0,2447,0.10033392906188965,0.00017537599522289416
512,2462,0,2462,0.10082197189331055,0.00017187365361581293
515,2477,0,2477,0.10130882263183594,0.0001692753905596409
518,2492,0,2492,0.10179686546325684,0.00016722076680375774
521,2506,0,2506,0.10230088233947754,0.00015722657261671137
524,2521,0,2521,0.10290098190307617,0.00015364080241469556
526,2531,0,2531,0.10326504707336426,0.00015203404690728063
529,2544,0,2544,0.10389089584350586,0.00014168781018389836
532,2559,0,2559,0.10452699661254883,0.0001351687674395318
535,2574,0,2574,0.10539007186889648,0.0001310270290919476
538,2589,0,2589,0.10609674453735352,0.00012824139523128953
540,2599,0,2599,0.1064918041229248,0.0001268486575808203
543,2614,0,2614,0.10708975791931152,0.00012520604373537895
546,2628,0,2628,0.10760998725891113,0.0001180379145258233
549,2642,0,2642,0.10808396339416504,0.00011115342987551249
552,2657,0,2657,0.10854291915893555,0.00010832397548732163
555,2672,0,2672,0.10901188850402832,0.00010657792598689384
557,2682,0,2682,0.10948705673217773,0.00010576021967873087
560,2696,0,2696,0.11023879051208496,0.00010264351523154555
563,2711,0,2711,0.11073589324951172,0.0001001674594696168
566,2726,0,2726,0.1115577220916748,9.870961917751572e-05
569,2741,0,2741,0.11240601539611816,9.78047198593085e-05
571,2751,0,2751,0.11299300193786621,9.73818264929344e-05
574,2766,0,2766,0.11369085311889648,9.691180391115723e-05
577,2781,0,2781,0.1143949031829834,9.656618028533662e-05
580,2796,0,2796,0.11501789093017578,9.62968596092095e-05
583,2811,0,2811,0.11579680442810059,9.60763743469509e-05
585,2821,0,2821,0.11628174781799316,9.594819392458769e-05
588,2836,0,2836,0.11702394485473633,9.577619943242469e-05
591,2851,0,2851,0.1175689697265625,9.562225972728403e-05
594,2865,0,2865,0.11805987358093262,9.233894708740227e-05
597,2880,0,2880,0.11855292320251465,9.074348250184262e-05
600,2895,0,2895,0.1190330982208252,8.98033451068699e-05
602,2905,0,2905,0.11936402320861816,8.938448390277437e-05
605,2920,0,2920,0.1202390193939209,8.894024604611798e-05
608,2935,0,2935,0.12123274803161621,8.863157896852904e-05
611,2950,0,2950,0.12193775177001953,8.840363147496694e-05
614,2965,0,2965,0.12269902229309082,8.822605488944881e-05
616,2975,0,2975,0.1232140064239502,8.812672739964085e-05
619,2990,0,2990,0.12382102012634277,8.799803275870952e-05
622,3005,0,3005,0.12435603141784668,8.788728924602006e-05
625,3020,0,3020,0.1248319149017334,8.77896732437476e-05
628,3035,0,3035,0.1257648468017578,8.770196816246733e-05
631,3050,0,3050,0.12661385536193848,8.762194495399807e-05
633,3060,0,3060,0.1272268295288086,8.757205531108966e-05
636,3075,0,3075,0.12804484367370605,8.750149341537334e-05
639,3090,0,3090,0.12880587577819824,8.743520810664194e-05
642,3105,0,3105,0.12946391105651855,8.737244436654954e-05
645,3120,0,3120,0.13013696670532227,8.731261013972552e-05
647,3130,0,3130,0.13046598434448242,8.727411138001614e-05
650,3145,0,3145,0.13097596168518066,8.721815835391431e-05
653,3160,0,3160,0.1314549446105957,8.716407070131462e-05
656,3175,0,3175,0.13193798065185547,8.711157767089571e-05
659,3190,0,3190,0.13241887092590332,8.706045611251313e-05
661,3200,0,3200,0.1327347755432129,8.70270443146247e-05
664,3215,0,3215,0.1332089900970459,8.697781298759961e-05
667,3230,0,3230,0.13371801376342773,8.692952567572587e-05
670,3245,0,3245,0.1342940330505371,8.688206778452041e-05
673,3260,0,3260,0.1349937915802002,8.683534295280606e-05
676,3275,0,3275,0.13564682006835938,8.678926992747992e-05
678,3285,0,3285,0.13616466522216797,8.675888232199677e-05
681,3300,0,3300,0.13687586784362793,8.671374826506103e-05
684,3315,0,3315,0.13753390312194824,8.666910531808103e-05
687,3330,0,3330,0.1380629539489746,8.662490913094082e-05
690,3345,0,3345,0.13854289054870605,8.658112192208818e-05
692,3355,0,3355,0.13887476921081543,8.655214153351362e-05
695,3370,0,3370,0.13937783241271973,8.650896662605235e-05
698,3385,0,3385,0.14002585411071777,8.646612470877439e-05
701,3400,0,3400,0.1406557559967041,8.642359443025714e-05
704,3415,0,3415,0.14171481132507324,8.638135742726899e-05
707,3430,0,3430,0.14247488975524902,8.63393978704527e-05
709,3440,0,3440,0.1428358554840088,8.631157213622939e-05
712,3455,0,3455,0.1433117389678955,8.627004550805357e-05
715,3470,0,3470,0.1438288688659668,8.622876377647581e-05
718,3485,0,3485,0.14430785179138184,8.618771755259032e-05
721,3500,0,3500,0.1448078155517578,8.614689863777933e-05
723,3510,0,3510,0.14529204368591309,8.611980872620727e-05
726,3525,0,3525,0.1458759307861328,8.607935313001347e-05
729,3540,0,3540,0.146345853805542,8.603910754978326e-05
732,3555,0,3555,0.14683008193969727,8.599906684234931e-05
735,3570,0,3570,0.14730191230773926,8.595922643557985e-05
737,3580,0,3580,0.14761590957641602,8.593277540835915e-05
740,3595,0,3595,0.14808893203735352,8.589325997278829e-05
743,3610,0,3610,0.14866876602172852,8.585393485315004e-05
746,3625,0,3625,0.14949703216552734,8.581479695827436e-05
749,3640,0,3640,0.15052580833435059,8.577584347731413e-05
752,3655,0,3655,0.15148282051086426,8.573707184096174e-05
754,3665,0,3665,0.15182209014892578,8.571132393462373e-05
757,3680,0,3680,0.15240478515625,8.567285021623055e-05
760,3695,0,3695,0.15304183959960938,8.563455243503083e-05
763,3710,0,3710,0.1535658836364746,8.5596428658544e-05
766,3725,0,3725,0.15405797958374023,8.555847707747548e-05
768,3735,0,3735,0.15438103675842285,8.553327084301889e-05
771,3750,0,3750,0.15485787391662598,8.549560251852483e-05
774,3765,0,3765,0.15547895431518555,8.545810205242587e-05
777,3780,0,3780,0.15604710578918457,8.542076796669812e-05
780,3795,0,3795,0.15656185150146484,8.538359884909064e-05
783,3809,0,3809,0.15703701972961426,8.473435597312562e-05
785,3819,0,3819,0.15735912322998047,8.369876746675917e-05
788,3832,0,3832,0.1578197479248047,8.083098532877663e-05
791,3847,0,3847,0.15830588340759277,7.773591605776785e-05
794,3861,0,3861,0.15877866744995117,7.20388194621843e-05
797,3874,0,3874,0.15922880172729492,6.430678467285645e-05
799,3882,0,3882,0.15961289405822754,5.481306974263296e-05
802,3894,0,3894,0.16024494171142578,4.216985394060329e-05
805,3908,0,3908,0.16080307960510254,3.906693535659981e-05
808,3922,0,3922,0.1612858772277832,3.5846347559104715e-05
811,3936,0,3936,0.1617567539215088,3.314690226320333e-05
813,3946,0,3946,0.16208577156066895,3.144026364469657e-05
816,3961,0,3961,0.16270780563354492,2.9468854605719053e-05
819,3974,0,3974,0.16321873664855957,2.8200070236143918e-05
822,3989,0,3989,0.16393280029296875,2.528968292881505e-05
825,4003,0,4003,0.16464686393737793,2.388522297227764e-05
828,4017,0,4017,0.16559481620788574,2.2163359595651447e-05
830,4027,0,4027,0.16631484031677246,2.0731018463800352e-05
833,4042,0,4042,0.16720890998840332,1.9232854480488476e-05
836,4055,0,4055,0.16805195808410645,1.7702385049621403e-05
839,4070,0,4070,0.1690218448638916,1.6356498608701972e-05
842,4084,0,4084,0.1700117588043213,1.547256757723561e-05
844,4093,0,4093,0.17043089866638184,1.5115075878595152e-05
847,4107,0,4107,0.1709890365600586,1.437964162442583e-05
850,4122,0,4122,0.17157697677612305,1.36901430520209e-05
853,4137,0,4137,0.17234301567077637,1.3227734809238349e-05
856,4152,0,4152,0.17300081253051758,1.289966438856974e-05
859,4167,0,4167,0.17353391647338867,1.2653142796433078e-05
861,4177,0,4177,0.17386174201965332,1.2518633594967207e-05
864,4192,0,4192,0.1743478775024414,1.2347643613453237e-05
867,4207,0,4207,0.17483091354370117,1.2203226882020337e-05
870,4222,0,4222,0.1753098964691162,1.2077982043050281e-05
873,4237,0,4237,0.17593789100646973,1.1967278115135325e-05
875,4247,0,4247,0.17632579803466797,1.1900019058838337e-05
878,4262,0,4262,0.1769850254058838,1.1807336176903783e-05
881,4277,0,4277,0.177825927734375,1.172309189721127e-05
884,4292,0,4292,0.17867588996887207,1.1646083575684098e-05
887,4307,0,4307,0.1791989803314209,1.1575387099841426e-05
889,4317,0,4317,0.1795177459716797,1.1531392716864084e-05
892,4332,0,4332,0.18009591102600098,1.146964319697035e-05
895,4347,0,4347,0.18074989318847656,1.1412510362149718e-05
898,4362,0,4362,0.18126893043518066,1.1359531551012257e-05
901,4377,0,4377,0.1817338466644287,1.1310304875178827e-05
904,4392,0,4392,0.1822209358215332,1.126447720130086e-05
906,4402,0,4402,0.18253087997436523,1.1235657773067644e-05
909,4417,0,4417,0.18299174308776855,1.1194816696832158e-05
912,4432,0,4432,0.18345069885253906,1.115661314084708e-05
915,4447,0,4447,0.18390870094299316,1.1120814464328493e-05
918,4462,0,4462,0.18436694145202637,1.1087211205686159e-05
920,4472,0,4472,0.18467283248901367,1.106593460143653e-05
923,4487,0,4487,0.1851329803466797,1.1035579396534396e-05
926,4502,0,4502,0.18559002876281738,1.1006954933179441e-05
929,4517,0,4517,0.18605375289916992,1.0979916359792147e-05
932,4531,0,4531,0.18650174140930176,1.0780917933850586e-05
935,4546,0,4546,0.18695974349975586,1.0517633952784924e-05
937,4556,0,4556,0.18726587295532227,1.0410789827685753e-05
940,4571,0,4571,0.187727689743042,1.0305912690208607e-05
943,4586,0,4586,0.18827009201049805,1.023795158638631e-05
946,4601,0,4601,0.18883991241455078,1.018956336381165e-05
949,4616,0,4616,0.1893470287322998,1.0152221591257449e-05
951,4626,0,4626,0.18966293334960938,1.0131235249953983e-05
954,4641,0,4641,0.19014286994934082,1.0103771370975127e-05
957,4656,0,4656,0.1906139850616455,1.0079835549198611e-05
960,4671,0,4671,0.19108200073242188,1.005852952156586e-05
963,4686,0,4686,0.19155287742614746,1.003928966140486e-05
965,4696,0,4696,0.1919569969177246,1.0027418684680486e-05
968,4711,0,4711,0.19248199462890625,1.0010834678464665e-05
971,4726,0,4726,0.19297575950622559,9.995523603870158e-06
974,4741,0,4741,0.19345998764038086,9.981311892237406e-06
977,4756,0,4756,0.19404387474060059,9.968060462798886e-06
980,4771,0,4771,0.19477176666259766,9.955655060284528e-06
982,4781,0,4781,0.1952366828918457,9.947806946623828e-06
985,4796,0,4796,0.19585490226745605,9.93660630500167e-06
988,4811,0,4811,0.1963350772857666,9.9260271944874e-06
991,4826,0,4826,0.19681406021118164,9.916006263364884e-06
994,4841,0,4841,0.19728779792785645,9.9064883326067e-06
996,4851,0,4851,0.1976029872894287,9.900398356717726e-06
999,4866,0,4866,0.19815802574157715,9.891614139317713e-06
1002,4881,0,4881,0.19867682456970215,9.883216257540906e-06
1005,4896,0,4896,0.1991569995880127,9.875169831447068e-06
1008,4911,0,4911,0.1996300220489502,9.86744378695498e-06
1011,4926,0,4926,0.20010590553283691,9.860010355060417e-06
1013,4936,0,4936,0.20042181015014648,9.855204900803382e-06
1016,4951,0,4951,0.2009139060974121,9.848205124829809e-06
1019,4966,0,4966,0.2013859748840332,9.841437084196024e-06
1022,4981,0,4981,0.20185494422912598,9.834882001577028e-06
1025,4996,0,4996,0.20232391357421875,9.828522920888324e-06
1027,5006,0,5006,0.20272088050842285,9.824384788681915e-06
1030,5021,0,5021,0.20326495170593262,9.818319014483997e-06
1033,5036,0,5036,0.20375967025756836,9.81241147299784e-06
1036,5051,0,5051,0.20423483848571777,9.806650342677701e-06
1039,5066,0,5066,0.20470976829528809,9.801024875451488e-06
1041,5076,0,5076,0.20502591133117676,9.797345064155639e-06
1044,5091,0,5091,0.20552277565002441,9.791924392360992e-06
1047,5106,0,5106,0.20599699020385742,9.786615178782104e-06
1050,5121,0,5121,0.20650291442871094,9.781409767545147e-06
1053,5136,0,5136,0.20697784423828125,9.77630116236364e-06
1056,5151,0,5151,0.20745396614074707,9.771282963629966e-06
1058,5161,0,5161,0.20776581764221191,9.76798480951047e-06
1061,5176,0,5176,0.20823907852172852,9.763104511693338e-06
1064,5191,0,5191,0.20874905586242676,9.758300062317807e-06
1067,5206,0,5206,0.20944690704345703,9.753566810876437e-06
1070,5221,0,5221,0.21029877662658691,9.748900486351012e-06
1072,5231,0,5231,0.21103405952453613,9.74582483314123e-06
1075,5246,0,5246,0.21199584007263184,9.741261486601564e-06
1078,5261,0,5261,0.2127218246459961,9.73675528439129e-06
1081,5276,0,5276,0.21338272094726562,9.732303079939436e-06
1084,5291,0,5291,0.213972806930542,9.727901973211027e-06
1087,5306,0,5306,0.21451282501220703,9.723549289494574e-06
1089,5316,0,5316,0.21483898162841797,9.720673175003066e-06
1092,5331,0,5331,0.21534204483032227,9.716395804253315e-06
1095,5346,0,5346,0.2158210277557373,9.712160684655322e-06
1098,5361,0,5361,0.21628689765930176,9.707965815924995e-06
1101,5376,0,5376,0.21675586700439453,9.70380934714901e-06
1103,5386,0,5386,0.21706700325012207,9.701058849626607e-06
1106,5401,0,5401,0.2175297737121582,9.696962634738108e-06
1109,5416,0,5416,0.2180027961730957,9.69290052392771e-06
1112,5431,0,5431,0.21846699714660645,9.688871116432851e-06
1115,5446,0,5446,0.2189328670501709,9.684873111873847e-06
1117,5456,0,5456,0.21925592422485352,9.682224621436693e-06
1120,5471,0,5471,0.21972084045410156,9.678276312777542e-06
1123,5486,0,5486,0.2201859951019287,9.674356371026104e-06
1126,5501,0,5501,0.22064781188964844,9.670463800005541e-06
1129,5516,0,5516,0.22110891342163086,9.66659767174215e-06
1132,5531,0,5531,0.2215738296508789,9.662757121196982e-06
1134,5541,0,5541,0.22188186645507812,9.660210563199086e-06
1137,5556,0,5556,0.2223527431488037,9.656410875286065e-06
1140,5571,0,5571,0.22281599044799805,9.652634729784107e-06
1143,5586,0,5586,0.2232809066772461,9.64888145334034e-06
1146,5601,0,5601,0.22374868392944336,9.645150415868398e-06
1148,5610,0,5610,0.2240450382232666,9.54434565710027e-06
1151,5625,0,5625,0.22450566291809082,9.343970830150073e-06
1154,5640,0,5640,0.22521376609802246,9.215348839973716e-06
1157,5655,0,5655,0.2259230613708496,9.130025999475314e-06
1160,5669,0,5669,0.22639203071594238,8.667467459624952e-06
1163,5684,0,5684,0.22686100006103516,8.485604772775578e-06
1165,5693,0,5693,0.2272648811340332,8.271205142103106e-06
1168,5707,0,5707,0.2279069423675537,8.15504650139453e-06
1171,5722,0,5722,0.22850894927978516,7.99493567570226e-06
1174,5737,0,5737,0.22899198532104492,7.881648790359096e-06
1177,5751,0,5751,0.22945189476013184,7.576963851730788e-06
1179,5761,0,5761,0.229766845703125,7.40886370108487e-06
1182,5775,0,5775,0.2302238941192627,7.037796670165057e-06
1185,5789,0,5789,0.23069190979003906,6.794853974180114e-06
1188,5803,0,5803,0.23114895820617676,6.252171919429999e-06
1191,5818,0,5818,0.23161792755126953,6.046848540733421e-06
1193,5828,0,5828,0.23192787170410156,5.948893192085943e-06
1196,5842,0,5842,0.23238396644592285,5.674514613504086e-06
1199,5856,0,5856,0.23284077644348145,5.319581375798123e-06
1202,5871,0,5871,0.2333087921142578,5.162777448579211e-06
1205,5886,0,5886,0.23377680778503418,5.06512378087763e-06
1208,5901,0,5901,0.23424577713012695,4.9997902214123026e-06
1210,5911,0,5911,0.23456478118896484,4.966920232831599e-06
1213,5926,0,5926,0.23503398895263672,4.927582799110493e-06
1216,5941,0,5941,0.23550200462341309,4.8960661352961686e-06
1219,5956,0,5956,0.23597002029418945,4.869633931660045e-06
1222,5971,0,5971,0.23643803596496582,4.846715599320016e-06
1224,5981,0,5981,0.23675107955932617,4.83290759652159e-06
1227,5996,0,5996,0.23721599578857422,4.8139334748251235e-06
1230,6011,0,6011,0.2376880645751953,4.796663021540097e-06
1233,6026,0,6026,0.23815178871154785,4.780791304806196e-06
1236,6041,0,6041,0.23862600326538086,4.766099950877772e-06
1239,6056,0,6056,0.23909783363342285,4.752425696787479e-06
1241,6066,0,6066,0.2394087314605713,4.743810877719791e-06
1244,6081,0,6081,0.23987293243408203,4.73156298012462e-06
1247,6096,0,6096,0.2403428554534912,4.720046669953409e-06
1250,6111,0,6111,0.24080681800842285,4.709187860305923e-06
1253,6126,0,6126,0.24126887321472168,4.698923630233584e-06
1255,6136,0,6136,0.2415788173675537,4.692384052704127e-06
1258,6151,0,6151,0.24204373359680176,4.682993769653421e-06
1261,6166,0,6166,0.24251580238342285,4.674068232531017e-06
1264,6181,0,6181,0.24297690391540527,4.665569024003183e-06
1267,6196,0,6196,0.24344086647033691,4.657461901369535e-06
1269,6206,0,6206,0.24376797676086426,4.6522596895931536e-06
1272,6221,0,6221,0.2442629337310791,4.64473935196866e-06
1275,6236,0,6236,0.24482297897338867,4.637535813993057e-06
1278,6251,0,6251,0.245344877243042,4.630625648117482e-06
1281,6266,0,6266,0.2458176612854004,4.6239875531992655e-06
1284,6281,0,6281,0.24628281593322754,4.6176021103963825e-06
1286,6291,0,6291,0.24659991264343262,4.6134766852006765e-06
1289,6306,0,6306,0.24706506729125977,4.607473646047468e-06
1292,6321,0,6321,0.24753570556640625,4.601679197213094e-06
1295,6336,0,6336,0.2480030059814453,4.5960792622664015e-06
1298,6351,0,6351,0.24846887588500977,4.5906608989084e-06
1300,6361,0,6361,0.24885869026184082,4.587143606496183e-06
1303,6376,0,6376,0.24939274787902832,4.582001849198763e-06
1306,6391,0,6391,0.24988889694213867,4.577011922227536e-06
1309,6406,0,6406,0.2503647804260254,4.572164217359567e-06
1312,6421,0,6421,0.25084686279296875,4.567449855601241e-06
1315,6436,0,6436,0.25132179260253906,4.562860624854962e-06
1317,6446,0,6446,0.25163698196411133,4.559866877636993e-06
1320,6461,0,6461,0.2521090507507324,4.5554695854547025e-06
1323,6476,0,6476,0.2525808811187744,4.5511783762567146e-06
1326,6491,0,6491,0.2530539035797119,4.546987042801007e-06
1329,6506,0,6506,0.2535247802734375,4.542889824956068e-06
1331,6516,0,6516,0.25383973121643066,4.540207975641629e-06
1334,6531,0,6531,0.25431084632873535,4.536255919982673e-06
1337,6545,0,6545,0.2547750473022461,4.4959858113035005e-06
1340,6560,0,6560,0.2552471160888672,4.445723910529185e-06
1343,6575,0,6575,0.2558329105377197,4.4133497244165455e-06
1345,6585,0,6585,0.2564668655395508,4.397710002879452e-06
1348,6600,0,6600,0.25699281692504883,4.379752583817942e-06
1351,6615,0,6615,0.25756001472473145,4.366015613850074e-06
1354,6630,0,6630,0.2581937313079834,4.354900977657653e-06
1357,6645,0,6645,0.2588338851928711,4.345485976457457e-06
1360,6660,0,6660,0.25968289375305176,4.337222988787778e-06
1362,6670,0,6670,0.2601008415222168,4.3321832859222554e-06
1365,6685,0,6685,0.2607448101043701,4.3251599116785e-06
1368,6700,0,6700,0.26142191886901855,4.3186450439425855e-06
1371,6715,0,6715,0.2619650363922119,4.31253346580538e-06
1374,6730,0,6730,0.2624378204345703,4.3067527028001596e-06
1376,6740,0,6740,0.2627599239349365,4.303056532616548e-06
1379,6755,0,6755,0.2633178234100342,4.297719333297836e-06
1382,6770,0,6770,0.2638518810272217,4.2926032735229544e-06
1385,6785,0,6785,0.2643718719482422,4.287683964894399e-06
1388,6800,0,6800,0.2649538516998291,4.282942028669041e-06
1391,6815,0,6815,0.2655611038208008,4.278361700590493e-06
1393,6825,0,6825,0.2658839225769043,4.275391377625988e-06
1396,6840,0,6840,0.2664949893951416,4.271052328459959e-06
1399,6855,0,6855,0.26711177825927734,4.266844250788583e-06
1402,6870,0,6870,0.26772284507751465,4.262758504336945e-06
1405,6885,0,6885,0.26824378967285156,4.258787516531756e-06
1407,6895,0,6895,0.2686300277709961,4.256200603835833e-06
1410,6910,0,6910,0.2692270278930664,4.252406336497507e-06
1413,6925,0,6925,0.2697908878326416,4.248710472838297e-06
1416,6940,0,6940,0.2702939510345459,4.245107960927535e-06
1419,6955,0,6955,0.2707676887512207,4.241594200341387e-06
1421,6965,0,6965,0.2710850238800049,4.239298904769203e-06
1424,6980,0,6980,0.27155590057373047,4.235923868175396e-06
1427,6995,0,6995,0.2720298767089844,4.2326270717306095e-06
1430,7010,0,7010,0.2727029323577881,4.229405105043775e-06
1433,7025,0,7025,0.27324390411376953,4.226254794377718e-06
1436,7040,0,7040,0.2737116813659668,4.223173176270114e-06
1438,7050,0,7050,0.2740299701690674,4.22115554893465e-06
1441,7065,0,7065,0.27449703216552734,4.2181823345391324e-06
1444,7080,0,7080,0.2749598026275635,4.215270778171154e-06
1447,7095,0,7095,0.2754218578338623,4.212418519253865e-06
1450,7110,0,7110,0.27588605880737305,4.209623327220307e-06
1452,7120,0,7120,0.27619194984436035,4.207790522282433e-06
1455,7135,0,7135,0.2767510414123535,4.205085803250886e-06
1458,7149,0,7149,0.277263879776001,4.152078883574742e-06
1461,7164,0,7164,0.277785062789917,4.0642034763299315e-06
1464,7179,0,7179,0.27826786041259766,4.018708847898653e-06
1467,7194,0,7194,0.27874302864074707,3.994508650673759e-06
1469,7204,0,7204,0.27905893325805664,3.984721103310557e-06
1472,7219,0,7219,0.27953290939331055,3.975237666100525e-06
1475,7234,0,7234,0.28000569343566895,3.969247730997641e-06
1478,7249,0,7249,0.28047895431518555,3.96509411358512e-06
1481,7264,0,7264,0.28095197677612305,3.961937723787839e-06
1483,7274,0,7274,0.2812669277191162,3.960164404464964e-06
1486,7289,0,7289,0.2817368507385254,3.957816326937322e-06
1489,7304,0,7304,0.2822120189666748,3.955716883338864e-06
1492,7319,0,7319,0.2826879024505615,3.953783128710263e-06
1495,7334,0,7334,0.2831599712371826,3.951967467207251e-06
1497,7344,0,7344,0.2834749221801758,3.9508080403693986e-06
1500,7359,0,7359,0.28394579887390137,3.949131195046119e-06
1503,7374,0,7374,0.28441905975341797,3.947517480161389e-06
1506,7389,0,7389,0.28488802909851074,3.945957582645496e-06
1509,7404,0,7404,0.28535890579223633,3.944444806867832e-06
1512,7419,0,7419,0.2858269214630127,3.9429741275022745e-06
1514,7429,0,7429,0.28613972663879395,3.94201509400117e-06
1517,7444,0,7444,0.28661608695983887,3.940606265795427e-06
1520,7459,0,7459,0.28708696365356445,3.939230691915703e-06
1523,7474,0,7474,0.28756093978881836,3.937886061411662e-06
1526,7489,0,7489,0.28803086280822754,3.9365704019534984e-06
1528,7499,0,7499,0.2883439064025879,3.93570853691799e-06
1531,7514,0,7514,0.28882670402526855,3.934437464912861e-06
1534,7529,0,7529,0.28929781913757324,3.933191240819024e-06
1537,7544,0,7544,0.28976988792419434,3.931968619927423e-06
1540,7559,0,7559,0.29024481773376465,3.9307684769413155e-06
1543,7574,0,7574,0.29071569442749023,3.929589786353534e-06
1545,7584,0,7584,0.2910289764404297,3.928815442751141e-06
1548,7599,0,7599,0.29149580001831055,3.927670450602858e-06
1551,7613,0,7613,0.29195475578308105,3.8570963186782086e-06
1554,7628,0,7628,0.29244494438171387,3.7583336356450916e-06
1557,7643,0,7643,0.29291582107543945,3.7095491490320506e-06
1559,7653,0,7653,0.2932288646697998,3.6911627234553678e-06
1562,7668,0,7668,0.293712854385376,3.674547697771007e-06
1565,7683,0,7683,0.2941911220550537,3.6649438029970536e-06
1568,7698,0,7698,0.29468202590942383,3.65884552192187e-06
1571,7713,0,7713,0.2951517105102539,3.654585150882366e-06
1573,7723,0,7723,0.29546689987182617,3.652344772103334e-06
1576,7738,0,7738,0.29593801498413086,3.6495485649512218e-06
1579,7753,0,7753,0.29640793800354004,3.6472057072729166e-06
1582,7768,0,7768,0.29687976837158203,3.6451684280419714e-06
1585,7783,0,7783,0.29735279083251953,3.643350070153565e-06
1588,7798,0,7798,0.2978229522705078,3.641696471206535e-06
1590,7808,0,7808,0.29813599586486816,3.6406673632953786e-06
1593,7823,0,7823,0.2986159324645996,3.639214070904899e-06
1596,7838,0,7838,0.2990849018096924,3.637851769097085e-06
1599,7853,0,7853,0.29954981803894043,3.636565410835143e-06
1602,7868,0,7868,0.3000178337097168,3.635343476208962e-06
1604,7878,0,7878,0.30032896995544434,3.634560109944993e-06
1607,7893,0,7893,0.3007967472076416,3.6334264337604504e-06
1610,7908,0,7908,0.30126190185546875,3.6323369687497417e-06
1613,7923,0,7923,0.3017268180847168,3.631286626019028e-06
1616,7938,0,7938,0.30219388008117676,3.6302711989680614e-06
1619,7953,0,7953,0.30266475677490234,3.62928717172017e-06
1621,7963,0,7963,0.3029758930206299,3.628647112920084e-06
1624,7978,0,7978,0.30344295501708984,3.62770904232268e-06
1627,7993,0,7993,0.3039119243621826,3.6267953880390422e-06
1630,8008,0,8008,0.3043808937072754,3.6259041744873273e-06
1633,8023,0,8023,0.30484771728515625,3.6250336804384266e-06
1635,8033,0,8033,0.3051607608795166,3.6244641083410494e-06
1638,8048,0,8048,0.30566978454589844,3.623624877810636e-06
1641,8063,0,8063,0.30614185333251953,3.622802714877514e-06
1644,8078,0,8078,0.30661988258361816,3.621996517988272e-06
1647,8093,0,8093,0.30709075927734375,3.6212052979401776e-06
1649,8103,0,8103,0.3074049949645996,3.6206856938312544e-06
1652,8118,0,8118,0.3078749179840088,3.6199174920375013e-06
1655,8133,0,8133,0.30834388732910156,3.6191620642097487e-06
1658,8148,0,8148,0.3088109493255615,3.6184187145811386e-06
1661,8163,0,8163,0.3092777729034424,3.617686804662481e-06
1664,8178,0,8178,0.30979394912719727,3.6169657463422952e-06
1666,8188,0,8188,0.31010985374450684,3.616490799355358e-06
1669,8203,0,8203,0.310593843460083,3.615786638841968e-06
1672,8218,0,8218,0.31107497215270996,3.61509196626248e-06
1675,8232,0,8232,0.31153297424316406,3.4946140344808295e-06
1678,8246,0,8246,0.31198787689208984,3.24775327766029e-06
1680,8255,0,8255,0.3122878074645996,3.06965095427407e-06
1683,8269,0,8269,0.31278300285339355,2.8366051481229592e-06
1686,8283,0,8283,0.31324195861816406,2.7458737145017493e-06
1689,8298,0,8298,0.31371593475341797,2.653957244783671e-06
1692,8312,0,8312,0.31417393684387207,2.51981753619023e-06
1695,8327,0,8327,0.31475186347961426,2.479516809595056e-06
1697,8336,0,8336,0.3150928020477295,2.4030418020451307e-06
1700,8351,0,8351,0.3155660629272461,2.340838440300571e-06
1703,8366,0,8366,0.3160359859466553,2.3071743892308185e-06
1706,8380,0,8380,0.31649088859558105,2.278288119770602e-06
1709,8394,0,8394,0.31694579124450684,2.140906259896652e-06
1711,8404,0,8404,0.3172588348388672,2.0920558513521657e-06
1714,8419,0,8419,0.3178579807281494,2.045999349270299e-06
1717,8434,0,8434,0.3186607360839844,2.018434869331488e-06
1720,8448,0,8448,0.3192617893218994,1.9725074483073053e-06
1723,8463,0,8463,0.31978392601013184,1.9178156230662533e-06
1725,8473,0,8473,0.32010483741760254,1.8951299737658743e-06
1728,8488,0,8488,0.32062578201293945,1.8725903847944757e-06
1731,8502,0,8502,0.32113099098205566,1.808152236323549e-06
1734,8516,0,8516,0.3217179775238037,1.678003527631557e-06
1737,8530,0,8530,0.3222661018371582,1.5467416838448125e-06
1740,8544,0,8544,0.3228158950805664,1.441546914974886e-06
1742,8553,0,8553,0.3231179714202881,1.3456774512853018e-06
1745,8567,0,8567,0.32358288764953613,1.2646298491235744e-06
1748,8582,0,8582,0.3240549564361572,1.2366322313648642e-06
1751,8597,0,8597,0.3245229721069336,1.2193729002772983e-06
1754,8612,0,8612,0.3249959945678711,1.2079348398224107e-06
1756,8622,0,8622,0.32531285285949707,1.202229486473116e-06
1759,8637,0,8637,0.32578086853027344,1.1954658531649715e-06
1762,8652,0,8652,0.3262519836425781,1.1901174656293516e-06
1765,8667,0,8667,0.3267240524291992,1.1856968534263312e-06
1768,8682,0,8682,0.32719898223876953,1.1819230493116551e-06
1771,8697,0,8697,0.32767677307128906,1.1786260814493233e-06
1773,8707,0,8707,0.3279910087585449,1.1766378796560973e-06
1776,8722,0,8722,0.328463077545166,1.1739132508938875e-06
1779,8737,0,8737,0.3289310932159424,1.1714485389354575e-06
1782,8752,0,8752,0.32939887046813965,1.169202142607201e-06
1785,8767,0,8767,0.33003783226013184,1.1671426014478325e-06
1787,8777,0,8777,0.3304266929626465,1.1658610139859157e-06
1790,8792,0,8792,0.3311159610748291,1.1640606424456483e-06
1793,8807,0,8807,0.33173608779907227,1.1623915253123963e-06
1796,8822,0,8822,0.3323650360107422,1.1608392048561704e-06
1799,8837,0,8837,0.3328697681427002,1.159391438275882e-06
1801,8847,0,8847,0.33318400382995605,1.158479099449652e-06
1804,8862,0,8862,0.3336508274078369,1.1571829547330737e-06
1807,8877,0,8877,0.334122896194458,1.1559663407071445e-06
1810,8892,0,8892,0.33458781242370605,1.1548219533489124e-06
1813,8907,0,8907,0.3350520133972168,1.153743337168737e-06
1816,8922,0,8922,0.3355140686035156,1.1527247574045983e-06
1818,8932,0,8932,0.33582377433776855,1.1520765083774422e-06
1821,8947,0,8947,0.33629274368286133,1.1511468869501839e-06
1824,8962,0,8962,0.33675599098205566,1.1502648133439724e-06
1827,8977,0,8977,0.3372180461883545,1.1494264515305538e-06
1830,8992,0,8992,0.33768486976623535,1.1486283414491954e-06
1832,9002,0,9002,0.3379960060119629,1.1481170730954467e-06
1835,9017,0,9017,0.33846092224121094,1.1473792459196853e-06
1838,9032,0,9032,0.33894801139831543,1.1466739694624335e-06
1841,9047,0,9047,0.3394160270690918,1.1459988330472289e-06
1844,9062,0,9062,0.33987975120544434,1.1453516438292615e-06
1847,9077,0,9077,0.3403468132019043,1.1447304042331746e-06
1849,9087,0,9087,0.34067296981811523,1.1443297544435627e-06
1852,9102,0,9102,0.3411409854888916,1.1437477935212933e-06
1855,9117,0,9117,0.34160470962524414,1.1431872659721497e-06
1858,9132,0,9132,0.3420748710632324,1.142646736595344e-06
1861,9147,0,9147,0.34253787994384766,1.1421248900974248e-06
1863,9157,0,9157,0.3428459167480469,1.1417867716766637e-06
1866,9171,0,9171,0.3432958126068115,1.1233339937626878e-06
1869,9186,0,9186,0.3437938690185547,1.1098288430123701e-06
1872,9201,0,9201,0.3442709445953369,1.102680788014614e-06
1875,9216,0,9216,0.34473586082458496,1.0987636927553564e-06
1877,9226,0,9226,0.3450448513031006,1.0971373012347272e-06
1880,9241,0,9241,0.34551072120666504,1.0955297370913723e-06
1883,9256,0,9256,0.3459758758544922,1.0945014742289326e-06
1886,9271,0,9271,0.3464388847351074,1.093791678331515e-06
1889,9286,0,9286,0.346904993057251,1.0932627041545505e-06
1892,9301,0,9301,0.347369909286499,1.0928402778989915e-06
1894,9311,0,9311,0.3478078842163086,1.0925967236174648e-06
1897,9326,0,9326,0.3483309745788574,1.0922697009202942e-06
1900,9341,0,9341,0.348801851272583,1.0919748743636344e-06
1903,9356,0,9356,0.34926486015319824,1.0917024674060437e-06
1906,9371,0,9371,0.34972286224365234,1.0914464136824493e-06
1908,9381,0,9381,0.35003089904785156,1.0912828084564243e-06
1911,9396,0,9396,0.3504939079284668,1.0910459974202659e-06
1914,9411,0,9411,0.3509528636932373,1.0908177543225284e-06
1917,9426,0,9426,0.3514118194580078,1.0905966350072423e-06
1920,9441,0,9441,0.35187292098999023,1.0903815788629521e-06
1923,9456,0,9456,0.35233569145202637,1.090171782197688e-06
1925,9466,0,9466,0.35264086723327637,1.0900345247123948e-06
1928,9481,0,9481,0.35309886932373047,1.0898321652963394e-06
1931,9496,0,9496,0.353557825088501,1.0896336566882433e-06
1934,9511,0,9511,0.354017972946167,1.089438637167699e-06
1937,9526,0,9526,0.3544750213623047,1.0892468018191574e-06
1939,9536,0,9536,0.354780912399292,1.0891205501690755e-06
1942,9551,0,9551,0.3552398681640625,1.0889334591420538e-06
1945,9566,0,9566,0.35581493377685547,1.0887489296976737e-06
1948,9581,0,9581,0.35634303092956543,1.0885667787803497e-06
1951,9595,0,9595,0.35680484771728516,1.066351139445198e-06
1953,9605,0,9605,0.3571197986602783,1.0506429550223754e-06
1956,9620,0,9620,0.3575899600982666,1.0364346705707832e-06
1959,9635,0,9635,0.35805487632751465,1.0284061917132734e-06
1962,9649,0,9649,0.3585069179534912,9.714040209772587e-07
1965,9663,0,9663,0.35895800590515137,9.30858060445269e-07
1968,9677,0,9677,0.3594088554382324,8.857969771527988e-07
1970,9687,0,9687,0.35971784591674805,8.713906771432708e-07
1973,9700,0,9700,0.36015892028808594,7.720144428553698e-07
1976,9714,0,9714,0.3606538772583008,7.494991372028566e-07
1979,9729,0,9729,0.36112189292907715,7.319502331513122e-07
1982,9743,0,9743,0.3615727424621582,7.165017168656584e-07
1984,9753,0,9753,0.3618810176849365,7.008793278223044e-07
1987,9768,0,9768,0.362346887588501,6.853886205330874e-07
1990,9783,0,9783,0.36281490325927734,6.754277526319672e-07
1993,9797,0,9797,0.3632678985595703,6.503262232067292e-07
1996,9812,0,9812,0.36373400688171387,6.342359041573143e-07
1999,9826,0,9826,0.36418986320495605,6.169253751644511e-07
2001,9834,0,9834,0.3644700050354004,5.507939345656541e-07
2004,9847,0,9847,0.36490583419799805,4.925307247087546e-07
2007,9862,0,9862,0.3653707504272461,4.589143534080287e-07
2010,9877,0,9877,0.3658428192138672,4.362101641560923e-07
2013,9891,0,9891,0.36629700660705566,3.9896957446340153e-07
2015,9900,0,9900,0.3665938377380371,3.818795726761191e-07
2018,9914,0,9914,0.36705994606018066,3.544990152069041e-07
2021,9929,0,9929,0.36752772331237793,3.3779687278303876e-07
2024,9944,0,9944,0.36799001693725586,3.265769754650029e-07
2027,9959,0,9959,0.3684568405151367,3.1843738037908436e-07
2029,9968,0,9968,0.36875391006469727,3.082374271271786e-07
2032,9982,0,9982,0.36920690536499023,2.875113308386601e-07
2035,9996,0,9996,0.369661808013916,2.6006762742524457e-07
2038,10010,0,10010,0.3701167106628418,2.403691803066288e-07
2041,10025,0,10025,0.37059688568115234,2.3362029442830333e-07
2044,10039,0,10039,0.3710489273071289,2.2349396706193594e-07
2046,10049,0,10049,0.371356725692749,2.184961226131644e-07
2049,10064,0,10064,0.37182092666625977,2.1330744786899495e-07
2052,10078,0,10078,0.3722810745239258,2.091664945340977e-07
2055,10093,0,10093,0.37278199195861816,2.0303197368054724e-07
2058,10108,0,10108,0.373248815536499,1.994010150593106e-07
2060,10118,0,10118,0.37355995178222656,1.9776731918073567e-07
2063,10133,0,10133,0.3740239143371582,1.9600184501951104e-07
2066,10148,0,10148,0.37449002265930176,1.9473037789179394e-07
2069,10162,0,10162,0.3749427795410156,1.8681217511754643e-07
2072,10177,0,10177,0.37540507316589355,1.8392067003479502e-07
2075,10192,0,10192,0.3758687973022461,1.8206319304232422e-07
2077,10202,0,10202,0.37617993354797363,1.811671280934889e-07
2080,10217,0,10217,0.37664294242858887,1.8013936205483857e-07
2083,10232,0,10232,0.37711095809936523,1.7935505851935775e-07
2086,10247,0,10247,0.3775777816772461,1.7872383573462034e-07
2089,10262,0,10262,0.3780379295349121,1.7819394007321574e-07
2091,10272,0,10272,0.3783438205718994,1.7788125891019115e-07
2094,10287,0,10287,0.3788027763366699,1.77458057150491e-07
2097,10302,0,10302,0.379260778427124,1.7707782297452296e-07
2100,10317,0,10317,0.37971973419189453,1.7673119356926208e-07
2103,10332,0,10332,0.38018298149108887,1.7641166920251843e-07
2105,10342,0,10342,0.3804898262023926,1.7621133791137764e-07
2108,10356,0,10356,0.3809347152709961,1.7451936073711394e-07
2111,10371,0,10371,0.3813939094543457,1.7340197086981125e-07
2114,10386,0,10386,0.3818528652191162,1.726968974191335e-07
2117,10401,0,10401,0.38231492042541504,1.7220488055015196e-07
2120,10416,0,10416,0.3827848434448242,1.7182862707173617e-07
2122,10426,0,10426,0.38309192657470703,1.7161694575987406e-07
2125,10441,0,10441,0.38354992866516113,1.7133770012044617e-07
2128,10456,0,10456,0.3840138912200928,1.710905043757121e-07
2131,10470,0,10470,0.3844609260559082,1.689688586730036e-07
2134,10485,0,10485,0.3849210739135742,1.6725634458664134e-07
2136,10495,0,10495,0.3852269649505615,1.6652340930993313e-07
2139,10510,0,10510,0.38568902015686035,1.6578742610617398e-07
2142,10525,0,10525,0.38614988327026367,1.6531533381404275e-07
2145,10539,0,10539,0.3865959644317627,1.6191816399705274e-07
2148,10554,0,10554,0.3870539665222168,1.5912226013744034e-07
2151,10569,0,10569,0.38751673698425293,1.5745124988278692e-07
2153,10579,0,10579,0.38782787322998047,1.5670214538014944e-07
2156,10594,0,10594,0.38828587532043457,1.5590787893983557e-07
2159,10609,0,10609,0.3887457847595215,1.5536049686478412e-07
2162,10624,0,10624,0.38921284675598145,1.5496301598682717e-07
2165,10639,0,10639,0.3896749019622803,1.5466090668319326e-07
2167,10649,0,10649,0.3899807929992676,1.5449621491812513e-07
2170,10664,0,10664,0.3904387950897217,1.5428892234774919e-07
2173,10679,0,10679,0.3908977508544922,1.541172974459682e-07
2176,10694,0,10694,0.3913547992706299,1.539721343137459e-07
2179,10709,0,10709,0.3918190002441406,1.5384717809431987e-07
2181,10719,0,10719,0.39212584495544434,1.537728662302743e-07
2184,10734,0,10734,0.39258480072021484,1.5367238887639532e-07
2187,10749,0,10749,0.39307093620300293,1.5358280767989516e-07
2190,10764,0,10764,0.3935418128967285,1.5350210872337497e-07
2193,10779,0,10779,0.39401793479919434,1.5342872973919481e-07
2196,10794,0,10794,0.39449071884155273,1.533614395101836e-07
2198,10804,0,10804,0.3948037624359131,1.5331946824712755e-07
2201,10819,0,10819,0.3952827453613281,1.5326023707016074e-07
2204,10834,0,10834,0.3958888053894043,1.5320487326617983e-07
2207,10849,0,10849,0.3964259624481201,1.531528106127632e-07
2210,10864,0,10864,0.39693689346313477,1.5310358189961073e-07
2212,10874,0,10874,0.3972489833831787,1.5307214275097726e-07
2215,10889,0,10889,0.3977179527282715,1.5302680686605942e-07
2218,10904,0,10904,0.39818477630615234,1.5298340568830895e-07
2221,10919,0,10919,0.3986508846282959,1.529416957939289e-07
2224,10934,0,10934,0.39911484718322754,1.5290147085908608e-07
2227,10949,0,10949,0.3995780944824219,1.5286255519643267e-07
2229,10959,0,10959,0.399965763092041,1.528372636701882e-07
2232,10974,0,10974,0.4005129337310791,1.5280020678522757e-07
2235,10989,0,10989,0.40100693702697754,1.5276410379266562e-07
2238,11004,0,11004,0.40148401260375977,1.527288535989691e-07
2241,11019,0,11019,0.401958703994751,1.526943684632941e-07
2243,11027,0,11027,0.402249813079834,1.4932756880196208e-07
2246,11042,0,11042,0.402724027633667,1.4655871165464555e-07
2249,11057,0,11057,0.4032008647918701,1.4498649208630152e-07
2252,11072,0,11072,0.40368199348449707,1.4404744667811512e-07
2255,11087,0,11087,0.4041929244995117,1.4345176594874085e-07
2257,11097,0,11097,0.40458178520202637,1.4316774586186548e-07
2260,11112,0,11112,0.40530872344970703,1.4284673757794155e-07
2263,11127,0,11127,0.40625977516174316,1.4260743147863405e-07
2266,11142,0,11142,0.40680384635925293,1.424203069266814e-07
2269,11157,0,11157,0.4073038101196289,1.4226822475142808e-07
2272,11172,0,11172,0.4077780246734619,1.4214078499862782e-07
2274,11182,0,11182,0.4080958366394043,1.42066150757525e-07
2277,11197,0,11197,0.40856289863586426,1.419662416450835e-07
2280,11212,0,11212,0.40903687477111816,1.4187785139749322e-07
2283,11227,0,11227,0.40950870513916016,1.417985637288663e-07
2286,11242,0,11242,0.40997767448425293,1.4172661285758624e-07
2288,11252,0,11252,0.41028881072998047,1.4168205355681875e-07
2291,11267,0,11267,0.41075682640075684,1.4161954306963418e-07
2294,11282,0,11282,0.4112229347229004,1.4156147919102157e-07
2297,11297,0,11297,0.4116950035095215,1.415071836261291e-07
2300,11312,0,11312,0.4121589660644531,1.4145611388658148e-07
2303,11327,0,11327,0.4126248359680176,1.414078308416384e-07
2305,11337,0,11337,0.41293787956237793,1.4137701015115599e-07
2308,11352,0,11352,0.413402795791626,1.4133260456027683e-07
2311,11367,0,11367,0.41388678550720215,1.412901596138005e-07
2314,11382,0,11382,0.41435885429382324,1.412494548907215e-07
2317,11397,0,11397,0.41501283645629883,1.4121030395975473e-07
2319,11407,0,11407,0.4154050350189209,1.4118498709474067e-07
2322,11422,0,11422,0.41591978073120117,1.4114808385696967e-07
2325,11437,0,11437,0.41640377044677734,1.4111235837467383e-07
2328,11452,0,11452,0.4168870449066162,1.4107770302189725e-07
2331,11467,0,11467,0.4174199104309082,1.4104402366542377e-07
2333,11477,0,11477,0.4177358150482178,1.410220716728939e-07
2336,11492,0,11492,0.41820693016052246,1.409898397148771e-07
2339,11507,0,11507,0.4186818599700928,1.4095838338736995e-07
2342,11522,0,11522,0.4191579818725586,1.409276422716598e-07
2345,11537,0,11537,0.4196789264678955,1.4089756220254392e-07
2348,11552,0,11552,0.4203648567199707,1.4086809445528708e-07
2350,11562,0,11562,0.4210968017578125,1.4084876756143381e-07
2353,11577,0,11577,0.4217808246612549,1.4082022461214198e-07
2356,11591,0,11591,0.4223368167877197,1.4068028512961337e-07
2359,11606,0,11606,0.42289304733276367,1.3965426845050038e-07
2362,11621,0,11621,0.42360591888427734,1.390537628773132e-07
2364,11631,0,11631,0.4239468574523926,1.387860253922292e-07
2367,11646,0,11646,0.4245269298553467,1.3850003039676964e-07
2370,11661,0,11661,0.42520976066589355,1.3829803674448818e-07
2373,11675,0,11675,0.425872802734375,1.339006857597917e-07
2376,11690,0,11690,0.4264059066772461,1.3067454438403305e-07
2379,11703,0,11703,0.42685484886169434,1.2143827787017815e-07
2381,11713,0,11713,0.42728090286254883,1.1812054094348568e-07
2384,11728,0,11728,0.4278829097747803,1.1483899136847985e-07
2387,11743,0,11743,0.42838382720947266,1.1275939040006616e-07
2390,11758,0,11758,0.42900872230529785,1.1135284077626073e-07
2393,11773,0,11773,0.4294877052307129,1.1033854403570513e-07
2395,11783,0,11783,0.4299278259277344,1.098021052443834e-07
2398,11797,0,11797,0.4306180477142334,1.071862774858893e-07
2401,11812,0,11812,0.4313499927520752,1.0583658269812247e-07
2404,11827,0,11827,0.4321320056915283,1.049765401080674e-07
2407,11841,0,11841,0.43301987648010254,1.0192654559497664e-07
2409,11851,0,11851,0.43355584144592285,9.991520824665187e-08
2412,11866,0,11866,0.434614896774292,9.798213304401845e-08
2415,11881,0,11881,0.4356958866119385,9.67969172653012e-08
2418,11895,0,11895,0.436647891998291,9.297444716257851e-08
2421,11909,0,11909,0.43755173683166504,8.901656291866641e-08
2424,11923,0,11923,0.4384489059448242,8.304853712572549e-08
2426,11932,0,11932,0.43880391120910645,8.120999674631897e-08
2429,11946,0,11946,0.4395129680633545,7.62657671036834e-08
2432,11961,0,11961,0.44026994705200195,7.302065286405779e-08
2435,11975,0,11975,0.4407837390899658,6.827878056263679e-08
2438,11990,0,11990,0.44125795364379883,6.564563391424253e-08
2440,11999,0,11999,0.4415857791900635,6.221922305223164e-08
2443,12014,0,12014,0.44205784797668457,5.9402798195054947e-08
2446,12028,0,12028,0.44251489639282227,5.524175774220139e-08
2449,12043,0,12043,0.44298481941223145,5.279887883075838e-08
2452,12057,0,12057,0.44344091415405273,5.157628517652942e-08
2455,12072,0,12072,0.44391965866088867,4.837058366056095e-08
2457,12081,0,12081,0.44422292709350586,4.454091198634509e-08
2460,12095,0,12095,0.4446897506713867,4.0423351991983995e-08
2463,12109,0,12109,0.445253849029541,3.754075096282243e-08
2466,12122,0,12122,0.4457530975341797,3.3481765340069285e-08
2469,12137,0,12137,0.44623303413391113,3.176816202888542e-08
2471,12147,0,12147,0.4465508460998535,3.1024141113783454e-08
2474,12162,0,12162,0.4470248222351074,3.027480951791328e-08
2477,12177,0,12177,0.4475688934326172,2.9798508423917438e-08
2480,12192,0,12192,0.4481048583984375,2.948270589644058e-08
2483,12207,0,12207,0.448772668838501,2.9263570245401507e-08
2485,12217,0,12217,0.4492669105529785,2.9152384669332276e-08
2488,12232,0,12232,0.4500448703765869,2.902079827615955e-08
2491,12247,0,12247,0.4508237838745117,2.891858264278499e-08
2494,12262,0,12262,0.4513678550720215,2.8836446644299573e-08
2497,12277,0,12277,0.45192384719848633,2.8768527069833554e-08
2500,12292,0,12292,0.4525790214538574,2.871099920425871e-08
2502,12302,0,12302,0.45304083824157715,2.8677110626559696e-08
2505,12317,0,12317,0.4537239074707031,2.863156823815221e-08
2508,12332,0,12332,0.4544041156768799,2.859113539066607e-08
2511,12347,0,12347,0.4550938606262207,2.8554761529048825e-08
2514,12362,0,12362,0.45568394660949707,2.8521659508252908e-08
2516,12372,0,12372,0.4560990333557129,2.8501105894229205e-08
2519,12387,0,12387,0.4568197727203369,2.8472186315956344e-08
2522,12402,0,12402,0.45729780197143555,2.8445211810102548e-08
2525,12417,0,12417,0.45804786682128906,2.8419864229960874e-08
2528,12432,0,12432,0.45860767364501953,2.8395887748479316e-08
2531,12447,0,12447,0.4591097831726074,2.837307488756562e-08
2533,12457,0,12457,0.459453821182251,2.835842778296981e-08
2536,12472,0,12472,0.4600968360900879,2.8337192881757704e-08
2539,12487,0,12487,0.46079301834106445,2.831673374872998e-08
2542,12502,0,12502,0.4613668918609619,2.8296948742421885e-08
2545,12517,0,12517,0.4619467258453369,2.827775318554469e-08
2547,12527,0,12527,0.46227502822875977,2.82652481501863e-08
2550,12542,0,12542,0.46276402473449707,2.824688327953689e-08
2553,12557,0,12557,0.4632587432861328,2.8228943129827823e-08
2556,12571,0,12571,0.4639158248901367,2.7667735500550876e-08
2559,12586,0,12586,0.4644768238067627,2.745758276529151e-08
2561,12595,0,12595,0.46497297286987305,2.6991187442526004e-08
2564,12610,0,12610,0.46581602096557617,2.670885508227408e-08
2567,12625,0,12625,0.4664597511291504,2.6538194314224406e-08
2570,12640,0,12640,0.46697998046875,2.6429145059748153e-08
2573,12655,0,12655,0.46745800971984863,2.6355279272139347e-08
2576,12670,0,12670,0.46793293952941895,2.6302342306556446e-08
2578,12680,0,12680,0.468250036239624,2.627461358122168e-08
2581,12695,0,12695,0.4687318801879883,2.6240725725537048e-08
2584,12710,0,12710,0.4692058563232422,2.621338328037998e-08
2587,12725,0,12725,0.46968984603881836,2.6190635217403035e-08
2590,12740,0,12740,0.47016286849975586,2.6171239839080552e-08
2592,12750,0,12750,0.4704759120941162,2.615975381469525e-08
2595,12765,0,12765,0.4709470272064209,2.614424683034379e-08
2598,12780,0,12780,0.4714198112487793,2.613041588515973e-08
2601,12795,0,12795,0.4718928337097168,2.6117929596678645e-08
2604,12810,0,12810,0.4724619388580322,2.610653824341977e-08
2607,12825,0,12825,0.4730229377746582,2.6096048973238672e-08
2609,12835,0,12835,0.47345685958862305,2.60894809025282e-08
2612,12850,0,12850,0.4739828109741211,2.6080172681809732e-08
2615,12865,0,12865,0.4744608402252197,2.6071424886552254e-08
2618,12880,0,12880,0.47493696212768555,2.6063151169878236e-08
2621,12895,0,12895,0.4754140377044678,2.6055280382627024e-08
2623,12905,0,12905,0.47572875022888184,2.605022746529256e-08
2626,12920,0,12920,0.47620391845703125,2.6042901938024286e-08
2629,12934,0,12934,0.47666287422180176,2.57368836521039e-08
2632,12949,0,12949,0.47719502449035645,2.5307653222783012e-08
2635,12964,0,12964,0.47768187522888184,2.5073464995321157e-08
2637,12974,0,12974,0.47801685333251953,2.4975790031363437e-08
2640,12989,0,12989,0.4786498546600342,2.487826419117487e-08
2643,13004,0,13004,0.4795098304748535,2.4815105296784064e-08
2646,13019,0,13019,0.48058176040649414,2.4771441209478298e-08
2649,13034,0,13034,0.4812448024749756,2.4739502149944557e-08
2652,13049,0,13049,0.48178577423095703,2.471504284340912e-08
2654,13059,0,13059,0.48209691047668457,2.4701639988506566e-08
2657,13074,0,13074,0.4825620651245117,2.4684708639456107e-08
2660,13089,0,13089,0.48302793502807617,2.467064594219388e-08
2663,13104,0,13104,0.4835031032562256,2.4658720550585914e-08
2666,13119,0,13119,0.48396897315979004,2.464842503641043e-08
2668,13129,0,13129,0.48427796363830566,2.464228243734287e-08
2671,13144,0,13144,0.48473691940307617,2.4633941205629575e-08
2674,13159,0,13159,0.485198974609375,2.462645390872799e-08
2677,13174,0,13174,0.48566174507141113,2.4619650280206178e-08
2680,13189,0,13189,0.4861259460449219,2.4613398509079614e-08
2683,13204,0,13204,0.486588716506958,2.4607595431340154e-08
2685,13214,0,13214,0.4868950843811035,2.4603935028769324e-08
2688,13229,0,13229,0.48736095428466797,2.459870713187976e-08
2691,13244,0,13244,0.4878237247467041,2.459374580636285e-08
2694,13259,0,13259,0.48828792572021484,2.4589006146909624e-08
2697,13274,0,13274,0.4887509346008301,2.4584451858072525e-08
2699,13284,0,13284,0.4890599250793457,2.458150384787038e-08
2702,13299,0,13299,0.4895198345184326,2.4577195692006213e-08
2705,13314,0,13314,0.48998188972473145,2.4573005746206148e-08
2708,13329,0,13329,0.49045586585998535,2.4568916657760642e-08
2711,13344,0,13344,0.4909369945526123,2.4564914092412695e-08
2713,13354,0,13354,0.49127793312072754,2.4562287820342205e-08
2716,13369,0,13369,0.49193286895751953,2.4558404005774383e-08
2719,13384,0,13384,0.4924657344818115,2.45545791939352e-08
2722,13399,0,13399,0.4931528568267822,2.4550805993746568e-08
2725,13414,0,13414,0.49381089210510254,2.4547078172882975e-08
2728,13429,0,13429,0.49433088302612305,2.4543390452860132e-08
2730,13438,0,13438,0.49492979049682617,2.397913015427342e-08
2733,13453,0,13453,0.495790958404541,2.3612567587843286e-08
2736,13468,0,13468,0.49648189544677734,2.3401386775532834e-08
2739,13483,0,13483,0.49695777893066406,2.3274276329359807e-08
2742,13498,0,13498,0.4974229335784912,2.3193512906126084e-08
2744,13508,0,13508,0.4977540969848633,2.3155054629603923e-08
2747,13521,0,13521,0.4982168674468994,2.2081451638600125e-08
2750,13535,0,13535,0.49866795539855957,2.0412266315841715e-08
2753,13550,0,13550,0.4991319179534912,1.977551269857693e-08
2756,13565,0,13565,0.49959397315979004,1.9422738986745017e-08
2759,13580,0,13580,0.5000548362731934,1.9215052041393587e-08
2761,13590,0,13590,0.5003697872161865,1.9121128661394468e-08
2764,13605,0,13605,0.5009059906005859,1.9018545680377035e-08
2767,13619,0,13619,0.5013570785522461,1.8502317377245645e-08
2770,13633,0,13633,0.5018069744110107,1.8002281993301368e-08
2773,13648,0,13648,0.5022678375244141,1.7405406396059824e-08
2775,13658,0,13658,0.5025758743286133,1.71521082487451e-08
2778,13673,0,13673,0.5030367374420166,1.6896276125018953e-08
2781,13688,0,13688,0.5034959316253662,1.6728657872771586e-08
2784,13702,0,13702,0.5039448738098145,1.565429137077172e-08
2787,13716,0,13716,0.5043938159942627,1.5382254540500832e-08
2789,13726,0,13726,0.50469970703125,1.4856438323519034e-08
2792,13740,0,13740,0.505155086517334,1.3484472782578e-08
2795,13755,0,13755,0.5056169033050537,1.320970157789651e-08
2798,13770,0,13770,0.506077766418457,1.3048496922056053e-08
2801,13784,0,13784,0.5066177845001221,1.2868992427977004e-08
2804,13799,0,13799,0.5070860385894775,1.2425856805365642e-08
2806,13808,0,13808,0.507408857345581,1.1746813141539921e-08
2809,13821,0,13821,0.5079169273376465,1.0606194629503335e-08
2812,13835,0,13835,0.5083818435668945,9.619894336086575e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha0/flex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,8.392333984375e-05,4.387061074692293
1,3,0,3,0.00016164779663085938,3.972820061310639
2,6,0,6,0.0003960132598876953,3.6277138409371137
3,9,0,9,0.0006167888641357422,2.672136101364927
4,12,0,12,0.0008528232574462891,2.4152473972739528
5,15,0,15,0.0010077953338623047,1.5663018362335526
6,18,0,18,0.0012497901916503906,1.4690513148498217
7,21,0,21,0.0014667510986328125,1.1803222473760537
8,24,0,24,0.0017218589782714844,1.1176538879410174
9,27,0,27,0.00185394287109375,0.8371978569777179
10,30,0,30,0.001997709274291992,0.7923042912566547
11,33,0,33,0.0021457672119140625,0.6058665094919226
12,36,0,36,0.0022728443145751953,0.5619155753702526
13,39,0,39,0.002410888671875,0.42304132221998136
14,42,0,42,0.0025877952575683594,0.4063780691579256
15,45,0,45,0.0027539730072021484,0.3530784860644457
16,48,0,48,0.002948760986328125,0.3360230322768205
17,51,0,51,0.0031309127807617188,0.2504581101398312
18,54,0,54,0.003337860107421875,0.243588797432846
19,57,0,57,0.0035886764526367188,0.1848838016190087
20,60,0,60,0.0038819313049316406,0.1816862164365556
21,63,0,63,0.004097938537597656,0.15751868498138488
22,66,0,66,0.004323720932006836,0.1561227700654445
23,69,0,69,0.004530906677246094,0.1545808138595481
24,72,0,72,0.00470280647277832,0.12988551246667496
25,75,0,75,0.004971027374267578,0.12719138145398504
26,78,0,78,0.005266904830932617,0.10732356344913943
27,81,0,81,0.005555868148803711,0.10617061691644449
28,84,0,84,0.005786895751953125,0.08117114256989279
29,87,0,87,0.006093740463256836,0.08036303435426277
30,90,0,90,0.0063707828521728516,0.06214829126500654
31,93,0,93,0.006742954254150391,0.061970560300437724
32,96,0,96,0.0069828033447265625,0.061717184794829856
33,99,0,99,0.0071828365325927734,0.06121124869048925
34,102,0,102,0.007505893707275391,0.06084672549290585
35,105,0,105,0.0076999664306640625,0.05856674623062609
36,108,0,108,0.007946968078613281,0.05787597277782032
37,111,0,111,0.008145809173583984,0.05625417319294632
38,114,0,114,0.008436918258666992,0.056038793600903504
39,117,0,117,0.008713960647583008,0.0552963573363964
40,120,0,120,0.008965730667114258,0.05497342971114778
41,123,0,123,0.009103775024414062,0.05316345066299052
42,126,0,126,0.009258031845092773,0.05283932785082342
43,129,0,129,0.009516716003417969,0.05118715449481558
44,132,0,132,0.009733915328979492,0.05086263778902649
45,135,0,135,0.009911775588989258,0.04993084800057317
46,138,0,138,0.01013493537902832,0.049738277962689266
47,141,0,141,0.010326862335205078,0.04952828116935226
48,144,0,144,0.010498762130737305,0.048005372968441117
49,147,0,147,0.010706901550292969,0.04760555149484625
50,150,0,150,0.01094675064086914,0.043664061901952135
51,153,0,153,0.011182785034179688,0.043286005626506883
52,156,0,156,0.01145792007446289,0.039757614613435924
53,159,0,159,0.011671781539916992,0.03957738430879081
54,162,0,162,0.011902809143066406,0.03937412146945766
55,165,0,165,0.012059926986694336,0.037014885460300836
56,168,0,168,0.012419700622558594,0.036594462984156376
57,171,0,171,0.012756824493408203,0.03431368514505277
58,174,0,174,0.013080835342407227,0.03385857369385655
59,177,0,177,0.013355016708374023,0.03346623467796146
60,180,0,180,0.013510942459106445,0.03307048987133748
61,183,0,183,0.013677835464477539,0.03197270026849882
62,186,0,186,0.013883829116821289,0.031638530647653415
63,189,0,189,0.014087915420532227,0.031443130478376685
64,192,0,192,0.014212846755981445,0.030615578352381635
65,195,0,195,0.014351844787597656,0.030398460189068274
66,198,0,198,0.014587879180908203,0.029841110165628425
67,201,0,201,0.014878988265991211,0.02964165001727839
68,204,0,204,0.015160799026489258,0.02877362039134286
69,207,0,207,0.015398740768432617,0.02863060017451247
70,210,0,210,0.015640735626220703,0.028518665137688314
71,213,0,213,0.015851974487304688,0.02817448293810678
72,216,0,216,0.016092777252197266,0.028082674582857358
73,219,0,219,0.016315937042236328,0.027172113701312513
74,222,0,222,0.01654505729675293,0.026994127218704488
75,225,0,225,0.01676797866821289,0.026553638320037903
76,228,0,228,0.01694488525390625,0.026506401763615454
77,231,0,231,0.01724076271057129,0.02644589410096779
78,234,0,234,0.017491817474365234,0.026170206717207118
79,237,0,237,0.017786741256713867,0.026141887556560862
80,240,0,240,0.018077850341796875,0.026102187193532606
81,243,0,243,0.01824188232421875,0.025990502864028896
82,246,0,246,0.018431901931762695,0.025919918560145867
83,249,0,249,0.018684864044189453,0.025808776728355028
84,252,0,252,0.019008874893188477,0.025728034798173878
85,255,0,255,0.01925182342529297,0.025630582685850768
86,258,0,258,0.019450902938842773,0.025573739310599596
87,261,0,261,0.0196688175201416,0.025517507999333403
88,264,0,264,0.01985788345336914,0.025432156512018418
89,267,0,267,0.020048856735229492,0.025371557097750196
90,270,0,270,0.02028179168701172,0.025318874109738747
91,273,0,273,0.020569801330566406,0.02528553751787723
92,276,0,276,0.020825862884521484,0.025251846574996174
93,279,0,279,0.021077871322631836,0.02523550837025913
94,282,0,282,0.021281719207763672,0.0252208078643251
95,285,0,285,0.021575927734375,0.025197849034583816
96,288,0,288,0.021768808364868164,0.025182614111498046
97,291,0,291,0.022122859954833984,0.02517346942198901
98,294,0,294,0.022476673126220703,0.025143602698253276
99,297,0,297,0.022729873657226562,0.025127560802870735
100,300,0,300,0.02291083335876465,0.025112110720254113
101,303,0,303,0.02319788932800293,0.025095403831304774
102,306,0,306,0.023480653762817383,0.025083159218674395
103,309,0,309,0.02378702163696289,0.02504628132956202
104,312,0,312,0.024096965789794922,0.025021791284194298
105,315,0,315,0.0243227481842041,0.02499549537126386
106,318,0,318,0.024542808532714844,0.024955766978176957
107,321,0,321,0.02478790283203125,0.024927569223363782
108,324,0,324,0.025052785873413086,0.024873251026084023
109,327,0,327,0.02532792091369629,0.02483117438201841
110,330,0,330,0.02557063102722168,0.024802542681656242
111,333,0,333,0.02580881118774414,0.024762008284843512
112,336,0,336,0.025966882705688477,0.02472768088995884
113,339,0,339,0.026113033294677734,0.02467773567790932
114,342,0,342,0.02629566192626953,0.024643813251676697
115,345,0,345,0.026472806930541992,0.02453568678621926
116,348,0,348,0.02664780616760254,0.0244479614223705
117,351,0,351,0.026793956756591797,0.024395302470059776
118,354,0,354,0.02697277069091797,0.02429422758032637
119,357,0,357,0.027107715606689453,0.024232182118100527
120,360,0,360,0.027310848236083984,0.02414935154256594
121,363,0,363,0.027580976486206055,0.02408134217683946
122,366,0,366,0.027811765670776367,0.023792158203970605
123,369,0,369,0.028010845184326172,0.023743524880489458
124,372,0,372,0.02815389633178711,0.023631701057902157
125,375,0,375,0.02832794189453125,0.02354559180556853
126,378,0,378,0.028461694717407227,0.023480298401048993
127,381,0,381,0.02860283851623535,0.02341560714144463
128,384,0,384,0.028872966766357422,0.023360453467267114
129,387,0,387,0.0290377140045166,0.023288550809439906
130,390,0,390,0.029181957244873047,0.023224436198453064
131,393,0,393,0.029318809509277344,0.02314950180124878
132,396,0,396,0.02948784828186035,0.023051303166809204
133,399,0,399,0.02961897850036621,0.022973566894599378
134,402,0,402,0.029748916625976562,0.022878661811576318
135,405,0,405,0.029878854751586914,0.022784563967565605
136,408,0,408,0.030019760131835938,0.02271956133092542
137,411,0,411,0.030150890350341797,0.02264935160935507
138,414,0,414,0.030282974243164062,0.022570257438016234
139,417,0,417,0.0304110050201416,0.022496087349308084
140,420,0,420,0.03056478500366211,0.022419268835885367
141,423,0,423,0.03069281578063965,0.022329503097322047
142,426,0,426,0.030818700790405273,0.022243094016345673
143,429,0,429,0.0309450626373291,0.02216381450101317
144,432,0,432,0.03106999397277832,0.022062268752559674
145,435,0,435,0.03119492530822754,0.022021834885724144
146,438,0,438,0.03131890296936035,0.022002481088871286
147,441,0,441,0.0315248966217041,0.021970995341113762
148,444,0,444,0.03164982795715332,0.02194510553508341
149,447,0,447,0.03177380561828613,0.02191561996988637
150,450,0,450,0.03189682960510254,0.02186870828014489
151,453,0,453,0.03202080726623535,0.021834491719108208
152,456,0,456,0.03214383125305176,0.021801740734786593
153,459,0,459,0.032266855239868164,0.021703556341402124
154,462,0,462,0.03239083290100098,0.021643364325623075
155,465,0,465,0.032514095306396484,0.021529592633798614
156,468,0,468,0.03263688087463379,0.021473785987925927
157,471,0,471,0.0327608585357666,0.021431829106612094
158,474,0,474,0.03288602828979492,0.02131402417332323
159,477,0,477,0.03301501274108887,0.021217851957133695
160,480,0,480,0.033124685287475586,0.02096710207125097
161,483,0,483,0.033247947692871094,0.02089958024088399
162,486,0,486,0.033386945724487305,0.020748329468738103
163,489,0,489,0.033496856689453125,0.02037272088185245
164,492,0,492,0.03377270698547363,0.02028442092042225
165,495,0,495,0.03392195701599121,0.020031660322192776
166,498,0,498,0.03420376777648926,0.019881224350753082
167,501,0,501,0.03450584411621094,0.019689611615161723
168,504,0,504,0.0346529483795166,0.0193546674431722
169,507,0,507,0.03478503227233887,0.019225821673965297
170,510,0,510,0.0349428653717041,0.018668064250054447
171,513,0,513,0.03511381149291992,0.018554241262523204
172,516,0,516,0.035240888595581055,0.018430936036658317
173,519,0,519,0.035388946533203125,0.01807303069025801
174,522,0,522,0.0355687141418457,0.017990033847900284
175,525,0,525,0.03571200370788574,0.01780320114737578
176,528,0,528,0.03583884239196777,0.017727784445290544
177,531,0,531,0.03595280647277832,0.01748739513415375
178,534,0,534,0.036078691482543945,0.017399471685760268
179,537,0,537,0.03619194030761719,0.016997466152534602
180,540,0,540,0.03632473945617676,0.01677723495704939
181,543,0,543,0.03645181655883789,0.016582765830698766
182,546,0,546,0.036563873291015625,0.01597712497027778
183,549,0,549,0.03673291206359863,0.01583628255694669
184,552,0,552,0.03686189651489258,0.015468644680974634
185,555,0,555,0.03713202476501465,0.015344696378623006
186,558,0,558,0.037282705307006836,0.01490479770649758
187,561,0,561,0.03743267059326172,0.014856893665414532
188,564,0,564,0.03757476806640625,0.014803709398303729
189,567,0,567,0.037735939025878906,0.014531536848877369
190,570,0,570,0.03786587715148926,0.014482457077822
191,573,0,573,0.037987709045410156,0.014103984559127276
192,576,0,576,0.03811788558959961,0.013987340283889534
193,579,0,579,0.03825187683105469,0.013628385313621798
194,582,0,582,0.03840994834899902,0.013540634903027664
195,585,0,585,0.03856468200683594,0.013443480008777086
196,588,0,588,0.03870582580566406,0.012864248654926132
197,591,0,591,0.038829803466796875,0.012767007828161632
198,594,0,594,0.03894186019897461,0.01204096748764811
199,597,0,597,0.03906679153442383,0.011913309810325016
200,600,0,600,0.03917694091796875,0.011708014143305315
201,603,0,603,0.039302825927734375,0.011498114632789096
202,606,0,606,0.0394139289855957,0.010147170594668804
203,609,0,609,0.03958296775817871,0.010060162179875206
204,612,0,612,0.03971672058105469,0.009928296622471241
205,615,0,615,0.039830923080444336,0.009289147232938178
206,618,0,618,0.03995680809020996,0.009037974374775498
207,621,0,621,0.040100812911987305,0.007798818856907483
208,624,0,624,0.040230751037597656,0.007439183102129483
209,627,0,627,0.04041767120361328,0.006771607210422805
210,630,0,630,0.040573835372924805,0.0064380246134818275
211,633,0,633,0.04069781303405762,0.005807684565014071
212,636,0,636,0.04083395004272461,0.005608037516448095
213,639,0,639,0.04096674919128418,0.004848426588293971
214,642,0,642,0.04110884666442871,0.004722885208239441
215,645,0,645,0.041237831115722656,0.004563547862102925
216,648,0,648,0.04134988784790039,0.0038164094715552404
217,651,0,651,0.041475772857666016,0.0036820084435547334
218,654,0,654,0.041589975357055664,0.0029610357650605105
219,657,0,657,0.04171586036682129,0.0029405069232614944
220,660,0,660,0.041841745376586914,0.0029126332474896646
221,663,0,663,0.04195380210876465,0.0025121133007097412
222,666,0,666,0.042079925537109375,0.0024786491016706457
223,669,0,669,0.042192935943603516,0.0024060602926836722
224,672,0,672,0.04232287406921387,0.002389661701162551
225,675,0,675,0.04251289367675781,0.0023739151853355805
226,678,0,678,0.04269075393676758,0.002271935821227873
227,681,0,681,0.04290199279785156,0.002259458642279899
228,684,0,684,0.043103933334350586,0.0022353958969186394
229,687,0,687,0.043260812759399414,0.0021989164383788306
230,690,0,690,0.04355883598327637,0.0021793748642264027
231,693,0,693,0.04378986358642578,0.002155194368267689
232,696,0,696,0.04401683807373047,0.0020791240438363732
233,699,0,699,0.04417991638183594,0.0020577628265549797
234,702,0,702,0.044304847717285156,0.0019950365447417152
235,705,0,705,0.0444798469543457,0.0019769965066787514
236,708,0,708,0.044606924057006836,0.0019353349319477457
237,711,0,711,0.04473090171813965,0.0019191826040866303
238,714,0,714,0.04484200477600098,0.001888856817355782
239,717,0,717,0.044966936111450195,0.0018786599253796886
240,720,0,720,0.04507803916931152,0.001795540515409886
241,723,0,723,0.04519987106323242,0.0017725790255446994
242,726,0,726,0.045323848724365234,0.0017492477819463503
243,729,0,729,0.04543781280517578,0.0016875118149609243
244,732,0,732,0.04556083679199219,0.0016713294859251966
245,735,0,735,0.04567074775695801,0.001581409893831218
246,738,0,738,0.045793771743774414,0.0015538296816191928
247,741,0,741,0.04590272903442383,0.0014396185953860167
248,744,0,744,0.046025991439819336,0.0014157581416735492
249,747,0,747,0.04613685607910156,0.0013106844058561682
250,750,0,750,0.046260833740234375,0.001276968698954737
251,753,0,753,0.04636979103088379,0.0011658765079819557
252,756,0,756,0.04649186134338379,0.001138529096308344
253,759,0,759,0.0466008186340332,0.0011121243291445104
254,762,0,762,0.0467226505279541,0.0010907506895613411
255,765,0,765,0.04683279991149902,0.0010030766399126893
256,768,0,768,0.04695606231689453,0.0009777920832235577
257,771,0,771,0.047064781188964844,0.0009263723615043483
258,774,0,774,0.047186851501464844,0.0009053277420171519
259,777,0,777,0.047297000885009766,0.0008138726642452717
260,780,0,780,0.04741978645324707,0.0008031956633546212
261,783,0,783,0.04754376411437988,0.0007883696252152073
262,786,0,786,0.0476527214050293,0.0007570596692707624
263,789,0,789,0.047775983810424805,0.0007450505446718422
264,792,0,792,0.04788470268249512,0.0006877589601576199
265,795,0,795,0.04800677299499512,0.000679919969369227
266,798,0,798,0.04813075065612793,0.0006686907258497329
267,801,0,801,0.048239707946777344,0.0006468129837028057
268,804,0,804,0.04836392402648926,0.0006383698810960447
269,807,0,807,0.04848480224609375,0.0005856127369623604
270,810,0,810,0.048609018325805664,0.0005777780801530086
271,813,0,813,0.04871773719787598,0.0005641514628013675
272,816,0,816,0.04886984825134277,0.0005547513988151061
273,819,0,819,0.04898571968078613,0.0005133030671912891
274,822,0,822,0.049243927001953125,0.0005036948699008166
275,825,0,825,0.04939889907836914,0.00048801940452449167
276,828,0,828,0.04965090751647949,0.00048069579109244373
277,831,0,831,0.04982185363769531,0.0004617756082297141
278,834,0,834,0.04998970031738281,0.00045338818410491587
279,837,0,837,0.050192832946777344,0.00040742875251356165
280,840,0,840,0.050351858139038086,0.00040334471791691426
281,843,0,843,0.05048489570617676,0.0003985425034542327
282,846,0,846,0.05060100555419922,0.00038447726664953886
283,849,0,849,0.05075669288635254,0.00038167215289157554
284,852,0,852,0.050868988037109375,0.0003745399231633024
285,855,0,855,0.050992727279663086,0.0003728373732318537
286,858,0,858,0.051117658615112305,0.00037027010237503517
287,861,0,861,0.05123782157897949,0.0003653886958208418
288,864,0,864,0.051364898681640625,0.0003646619204055766
289,867,0,867,0.05148887634277344,0.0003636720082223627
290,870,0,870,0.05159783363342285,0.0003580193141365563
291,873,0,873,0.051721811294555664,0.00035754488226648763
292,876,0,876,0.05184483528137207,0.00035604326487280935
293,879,0,879,0.05196690559387207,0.0003552820765292755
294,882,0,882,0.05212283134460449,0.0003546402603055537
295,885,0,885,0.05225086212158203,0.00035366510153071105
296,888,0,888,0.052403926849365234,0.00035242628924004053
297,891,0,891,0.05257296562194824,0.000350389167267697
298,894,0,894,0.052754878997802734,0.00034941900474488386
299,897,0,897,0.05293583869934082,0.00034833502583343117
300,900,0,900,0.053117990493774414,0.0003471539689233926
301,903,0,903,0.05327486991882324,0.0003461069996420504
302,906,0,906,0.053540706634521484,0.00034485623981708236
303,909,0,909,0.053740739822387695,0.0003437307546062037
304,912,0,912,0.05393385887145996,0.0003424991684555577
305,915,0,915,0.054086923599243164,0.0003416071686626504
306,918,0,918,0.05424690246582031,0.0003406744408411139
307,921,0,921,0.05437493324279785,0.0003390407860549198
308,924,0,924,0.05450272560119629,0.0003377393203449173
309,927,0,927,0.05463385581970215,0.0003361503734998821
310,930,0,930,0.05477285385131836,0.00033411700995919204
311,933,0,933,0.05489778518676758,0.0003302813477793745
312,936,0,936,0.05502676963806152,0.00032955788805494866
313,939,0,939,0.05515480041503906,0.0003287122109173515
314,942,0,942,0.05526876449584961,0.000321963335618328
315,945,0,945,0.05539584159851074,0.0003205389017663497
316,948,0,948,0.05558300018310547,0.0003169888704945883
317,951,0,951,0.05578494071960449,0.0003147813820029535
318,954,0,954,0.05593395233154297,0.00031126882785723395
319,957,0,957,0.0561368465423584,0.00030782615814854724
320,960,0,960,0.056302785873413086,0.0003053311217874906
321,963,0,963,0.05647587776184082,0.0002873794577962101
322,966,0,966,0.056619882583618164,0.00028383977945179074
323,969,0,969,0.05675387382507324,0.00028045437987531
324,972,0,972,0.05689692497253418,0.00027305566081222413
325,975,0,975,0.057022809982299805,0.0002706400940107079
326,978,0,978,0.05713367462158203,0.0002496205298900962
327,981,0,981,0.05726003646850586,0.00024735247862187087
328,984,0,984,0.05738496780395508,0.0002450661053468627
329,987,0,987,0.0574948787689209,0.00023755024564943073
330,990,0,990,0.05761981010437012,0.0002342997979185247
331,993,0,993,0.05773282051086426,0.0002156680666401115
332,996,0,996,0.05786275863647461,0.0002137792103492424
333,999,0,999,0.05798983573913574,0.00021093303549978308
334,1002,0,1002,0.05810379981994629,0.0002052857359565925
335,1005,0,1005,0.05822896957397461,0.00020297631481599134
336,1008,0,1008,0.05833768844604492,0.00017944174935594876
337,1011,0,1011,0.058461904525756836,0.00017781928547857615
338,1014,0,1014,0.05858588218688965,0.00017527813320914948
339,1017,0,1017,0.05869579315185547,0.00017086867701915695
340,1020,0,1020,0.058818817138671875,0.00016944172474491512
341,1023,0,1023,0.058928728103637695,0.00016538127617032427
342,1026,0,1026,0.0590519905090332,0.00016453811594551246
343,1029,0,1029,0.059160709381103516,0.0001582069992081658
344,1032,0,1032,0.059282779693603516,0.00015749191708308054
345,1035,0,1035,0.059407711029052734,0.0001562786172554505
346,1038,0,1038,0.059517860412597656,0.00014831375879404026
347,1041,0,1041,0.05964064598083496,0.0001473331948686196
348,1044,0,1044,0.059764862060546875,0.00014612661799732804
349,1047,0,1047,0.059874773025512695,0.00013956994382541594
350,1050,0,1050,0.0599977970123291,0.00013816837122184074
351,1053,0,1053,0.06010794639587402,0.00013587130960121733
352,1056,0,1056,0.06023073196411133,0.00013386704570531822
353,1059,0,1059,0.060353994369506836,0.0001323824864778186
354,1062,0,1062,0.06047797203063965,0.000130500867537565
355,1065,0,1065,0.06058788299560547,0.00012687386910669452
356,1068,0,1068,0.06070971488952637,0.00012584653892880307
357,1071,0,1071,0.06081891059875488,0.000122729940198746
358,1074,0,1074,0.060942888259887695,0.00012163709753396291
359,1077,0,1077,0.06105494499206543,0.00011835505913689887
360,1080,0,1080,0.06117892265319824,0.00011709411385093045
361,1083,0,1083,0.061287879943847656,0.00011260346616330967
362,1086,0,1086,0.06141066551208496,0.00011136128961988742
363,1089,0,1089,0.06153392791748047,0.0001102712720820973
364,1092,0,1092,0.061644792556762695,0.00010740350059308273
365,1095,0,1095,0.061769962310791016,0.00010606170858596582
366,1098,0,1098,0.06187796592712402,9.493861115296948e-05
367,1101,0,1101,0.06200075149536133,9.410932119757338e-05
368,1104,0,1104,0.06211090087890625,9.149949919118264e-05
369,1107,0,1107,0.062233686447143555,9.12326808730798e-05
370,1110,0,1110,0.06235790252685547,9.063651554783372e-05
371,1113,0,1113,0.06246685981750488,8.907695777426199e-05
372,1116,0,1116,0.06258893013000488,8.864333679455222e-05
373,1119,0,1119,0.06269693374633789,8.765705687823727e-05
374,1122,0,1122,0.06281876564025879,8.718416483700463e-05
375,1125,0,1125,0.0629277229309082,8.611842616979282e-05
376,1128,0,1128,0.0630500316619873,8.567817365344254e-05
377,1131,0,1131,0.06315898895263672,8.445428282536194e-05
378,1134,0,1134,0.06339383125305176,8.397378451481702e-05
379,1137,0,1137,0.06359505653381348,8.062995061644358e-05
380,1140,0,1140,0.06378698348999023,8.007154488007144e-05
381,1143,0,1143,0.06398797035217285,7.93954451013272e-05
382,1146,0,1146,0.0642387866973877,7.828910878533084e-05
383,1149,0,1149,0.06439661979675293,7.800838947045971e-05
384,1152,0,1152,0.06460785865783691,7.568351300168425e-05
385,1155,0,1155,0.06475377082824707,7.507102019140092e-05
386,1158,0,1158,0.06488776206970215,7.432101358623298e-05
387,1161,0,1161,0.06502199172973633,7.037097153559025e-05
388,1164,0,1164,0.06516098976135254,6.990106247787673e-05
389,1167,0,1167,0.06527185440063477,6.811014655328312e-05
390,1170,0,1170,0.06539797782897949,6.75449911818466e-05
391,1173,0,1173,0.06551289558410645,6.455426542920744e-05
392,1176,0,1176,0.06563782691955566,6.417545401665236e-05
393,1179,0,1179,0.06574892997741699,6.352052560021441e-05
394,1182,0,1182,0.06587386131286621,6.29200219054163e-05
395,1185,0,1185,0.06598401069641113,5.968958503523085e-05
396,1188,0,1188,0.06610774993896484,5.9206987236248936e-05
397,1191,0,1191,0.06621885299682617,5.857258543205062e-05
398,1194,0,1194,0.06634283065795898,5.804224715006852e-05
399,1197,0,1197,0.06645393371582031,5.741872726790468e-05
400,1200,0,1200,0.06657791137695312,5.689511853590122e-05
401,1203,0,1203,0.06669187545776367,5.4351482534800625e-05
402,1206,0,1206,0.06683492660522461,5.413588863501726e-05
403,1209,0,1209,0.06699180603027344,5.3568641499623935e-05
404,1212,0,1212,0.06710195541381836,5.257948720994101e-05
405,1215,0,1215,0.06722688674926758,5.2302809124432265e-05
406,1218,0,1218,0.0673367977142334,4.991825009319234e-05
407,1221,0,1221,0.06746077537536621,4.95479306668863e-05
408,1224,0,1224,0.06758499145507812,4.892937796985905e-05
409,1227,0,1227,0.06769585609436035,4.8251071027781776e-05
410,1230,0,1230,0.06781888008117676,4.780695322159361e-05
411,1233,0,1233,0.06793761253356934,4.704287567673822e-05
412,1236,0,1236,0.06806302070617676,4.662778494282435e-05
413,1239,0,1239,0.06817364692687988,4.487921423160235e-05
414,1242,0,1242,0.0682978630065918,4.445908513141862e-05
415,1245,0,1245,0.06842279434204102,4.396208100942105e-05
416,1248,0,1248,0.06853294372558594,4.14695795170196e-05
417,1251,0,1251,0.0686798095703125,4.0682847919018555e-05
418,1254,0,1254,0.06882786750793457,3.718703757338697e-05
419,1257,0,1257,0.0689847469329834,3.6617745089356084e-05
420,1260,0,1260,0.06909584999084473,3.59427517403704e-05
421,1263,0,1263,0.06921982765197754,3.53202086245103e-05
422,1266,0,1266,0.06932973861694336,3.3826333083432856e-05
423,1269,0,1269,0.06945276260375977,3.357018294960088e-05
424,1272,0,1272,0.06957793235778809,3.313856717836052e-05
425,1275,0,1275,0.06968879699707031,3.2020948124033164e-05
426,1278,0,1278,0.06981396675109863,3.17855805349324e-05
427,1281,0,1281,0.06992387771606445,3.1098323932660256e-05
428,1284,0,1284,0.07004785537719727,3.09160143624036e-05
429,1287,0,1287,0.07017087936401367,3.0594039807190176e-05
430,1290,0,1290,0.07028079032897949,3.002832395478796e-05
431,1293,0,1293,0.0704047679901123,2.9780895166355625e-05
432,1296,0,1296,0.07051491737365723,2.921318786155365e-05
433,1299,0,1299,0.07063889503479004,2.9087334416863025e-05
434,1302,0,1302,0.07074880599975586,2.8116181537577776e-05
435,1305,0,1305,0.07087278366088867,2.802663835033805e-05
436,1308,0,1308,0.07099580764770508,2.7917382575351983e-05
437,1311,0,1311,0.0711207389831543,2.7715544890866593e-05
438,1314,0,1314,0.07124471664428711,2.7559764347458856e-05
439,1317,0,1317,0.07135486602783203,2.7270496280320738e-05
440,1320,0,1320,0.07147908210754395,2.7173801053796204e-05
441,1323,0,1323,0.07158780097961426,2.66805593335359e-05
442,1326,0,1326,0.07171201705932617,2.6613795486854273e-05
443,1329,0,1329,0.07183575630187988,2.6546507164924464e-05
444,1332,0,1332,0.0719449520111084,2.6249015940880735e-05
445,1335,0,1335,0.07206869125366211,2.6179997372188878e-05
446,1338,0,1338,0.07219290733337402,2.6060515186280085e-05
447,1341,0,1341,0.07230281829833984,2.5638393592713574e-05
448,1344,0,1344,0.07242584228515625,2.555999828446608e-05
449,1347,0,1347,0.07253575325012207,2.4902897275752626e-05
450,1350,0,1350,0.07265996932983398,2.483257427602559e-05
451,1353,0,1353,0.07280087471008301,2.4743848009171588e-05
452,1356,0,1356,0.07294487953186035,2.4064204764034042e-05
453,1359,0,1359,0.07307291030883789,2.395108000187263e-05
454,1362,0,1362,0.07320690155029297,2.3666408146311795e-05
455,1365,0,1365,0.07333564758300781,2.3519575642357525e-05
456,1368,0,1368,0.0735468864440918,2.343053161453993e-05
457,1371,0,1371,0.07370591163635254,2.3009714896874774e-05
458,1374,0,1374,0.07384395599365234,2.2834545596203818e-05
459,1377,0,1377,0.07396292686462402,2.212340847368128e-05
460,1380,0,1380,0.07409477233886719,2.2000233868948915e-05
461,1383,0,1383,0.07425379753112793,2.184097062522706e-05
462,1386,0,1386,0.07436800003051758,2.148222970629813e-05
463,1389,0,1389,0.07449483871459961,2.134992482239976e-05
464,1392,0,1392,0.07460689544677734,2.1028098708323825e-05
465,1395,0,1395,0.07473278045654297,2.0904100665737893e-05
466,1398,0,1398,0.0748589038848877,2.0736446399223094e-05
467,1401,0,1401,0.07496881484985352,2.007041198970582e-05
468,1404,0,1404,0.07509398460388184,1.9894851845491257e-05
469,1407,0,1407,0.07520484924316406,1.851205388335129e-05
470,1410,0,1410,0.07533788681030273,1.83781361144113e-05
471,1413,0,1413,0.07546591758728027,1.809277430826064e-05
472,1416,0,1416,0.07557988166809082,1.7000340768903357e-05
473,1419,0,1419,0.07570886611938477,1.6769251433575103e-05
474,1422,0,1422,0.07582378387451172,1.5188824789919228e-05
475,1425,0,1425,0.07594966888427734,1.5006361415023809e-05
476,1428,0,1428,0.07605981826782227,1.4658094661448506e-05
477,1431,0,1431,0.07618379592895508,1.4403163400369987e-05
478,1434,0,1434,0.0762948989868164,1.332126050764602e-05
479,1437,0,1437,0.07641792297363281,1.3138806584213654e-05
480,1440,0,1440,0.07652783393859863,1.2703713675676636e-05
481,1443,0,1443,0.07665085792541504,1.2497762387627942e-05
482,1446,0,1446,0.07675981521606445,1.1877892404848101e-05
483,1449,0,1449,0.07688498497009277,1.178922401118293e-05
484,1452,0,1452,0.07700991630554199,1.168149788583275e-05
485,1455,0,1455,0.0771188735961914,1.1381100495495428e-05
486,1458,0,1458,0.07724189758300781,1.1313739015389735e-05
487,1461,0,1461,0.07735085487365723,1.1070581898952227e-05
488,1464,0,1464,0.07747364044189453,1.1023952356034623e-05
489,1467,0,1467,0.07759690284729004,1.0974874490689117e-05
490,1470,0,1470,0.07770586013793945,1.079422987168599e-05
491,1473,0,1473,0.07782983779907227,1.0768295395106556e-05
492,1476,0,1476,0.07802796363830566,1.0720401065791806e-05
493,1479,0,1479,0.07817769050598145,1.068013626265946e-05
494,1482,0,1482,0.07831382751464844,1.0653518259913007e-05
495,1485,0,1485,0.07853269577026367,1.0612249949750192e-05
496,1488,0,1488,0.07877683639526367,1.0579985903698328e-05
497,1491,0,1491,0.07893180847167969,1.0561478928089496e-05
498,1494,0,1494,0.07916903495788574,1.0540449649208203e-05
499,1497,0,1497,0.07936477661132812,1.0526670491404508e-05
500,1500,0,1500,0.07953476905822754,1.0514244864894189e-05
501,1503,0,1503,0.07973384857177734,1.0480862552111934e-05
502,1506,0,1506,0.07988095283508301,1.0453614453537054e-05
503,1509,0,1509,0.0800168514251709,1.0432094353314266e-05
504,1512,0,1512,0.0801689624786377,1.0383829410311021e-05
505,1515,0,1515,0.08031368255615234,1.0327183654508196e-05
506,1518,0,1518,0.08044290542602539,1.0281450555197764e-05
507,1521,0,1521,0.08055663108825684,1.0139555167374788e-05
508,1524,0,1524,0.08068466186523438,1.0120858405251394e-05
509,1527,0,1527,0.08081269264221191,1.0074976633375055e-05
510,1530,0,1530,0.08094072341918945,1.003919780069679e-05
511,1533,0,1533,0.08106875419616699,1.000959213675731e-05
512,1536,0,1536,0.08118295669555664,9.906697991286027e-06
513,1539,0,1539,0.08131098747253418,9.871768146755468e-06
514,1542,0,1542,0.08143782615661621,9.814237005724638e-06
515,1545,0,1545,0.08156585693359375,9.741568204947319e-06
516,1548,0,1548,0.08169293403625488,9.68293883659254e-06
517,1551,0,1551,0.08180475234985352,9.48344626895615e-06
518,1554,0,1554,0.08193278312683105,9.427120735607736e-06
519,1557,0,1557,0.08206582069396973,9.339078118413334e-06
520,1560,0,1560,0.08217978477478027,9.129446320633113e-06
521,1563,0,1563,0.08231782913208008,9.066193444449166e-06
522,1566,0,1566,0.08243203163146973,8.542784674912371e-06
523,1569,0,1569,0.08256101608276367,8.461794929541228e-06
524,1572,0,1572,0.0826728343963623,8.319123373705684e-06
525,1575,0,1575,0.08279991149902344,8.189966554596326e-06
526,1578,0,1578,0.08291482925415039,7.938378494323898e-06
527,1581,0,1581,0.08304095268249512,7.85270321106863e-06
528,1584,0,1584,0.08315396308898926,7.615761326995724e-06
529,1587,0,1587,0.08328080177307129,7.566115789702946e-06
530,1590,0,1590,0.08340787887573242,7.473898798137073e-06
531,1593,0,1593,0.08351993560791016,7.121663159005809e-06
532,1596,0,1596,0.08364701271057129,7.0350556662566405e-06
533,1599,0,1599,0.08375883102416992,6.634549970611506e-06
534,1602,0,1602,0.08388471603393555,6.5648079513017055e-06
535,1605,0,1605,0.08401203155517578,6.485456089196467e-06
536,1608,0,1608,0.08412384986877441,6.3112865986146096e-06
537,1611,0,1611,0.08424973487854004,6.244419744555582e-06
538,1614,0,1614,0.08436298370361328,6.057939989149085e-06
539,1617,0,1617,0.08448982238769531,5.978519675984361e-06
540,1620,0,1620,0.08460283279418945,5.747701979783532e-06
541,1623,0,1623,0.08472967147827148,5.6899362161785965e-06
542,1626,0,1626,0.08484292030334473,5.447357407802517e-06
543,1629,0,1629,0.08497095108032227,5.390280292139356e-06
544,1632,0,1632,0.0850827693939209,5.33458692688825e-06
545,1635,0,1635,0.08520770072937012,5.247433828914395e-06
546,1638,0,1638,0.08532571792602539,4.963920187182699e-06
547,1641,0,1641,0.08545279502868652,4.935816527436838e-06
548,1644,0,1644,0.08557581901550293,4.877300384720961e-06
549,1647,0,1647,0.08570289611816406,4.856584697727898e-06
550,1650,0,1650,0.08581399917602539,4.787127106934944e-06
551,1653,0,1653,0.08593988418579102,4.754661478384586e-06
552,1656,0,1656,0.08605074882507324,4.7020723478415535e-06
553,1659,0,1659,0.08617591857910156,4.6576016130149145e-06
554,1662,0,1662,0.0862877368927002,4.5255047154382646e-06
555,1665,0,1665,0.08641386032104492,4.50335176413489e-06
556,1668,0,1668,0.08652591705322266,4.377245211545457e-06
557,1671,0,1671,0.08664870262145996,4.353083861001177e-06
558,1674,0,1674,0.0867609977722168,4.267632519066496e-06
559,1677,0,1677,0.08688592910766602,4.257266447888737e-06
560,1680,0,1680,0.08701086044311523,4.24586610392595e-06
561,1683,0,1683,0.08712291717529297,4.1922442982543435e-06
562,1686,0,1686,0.087249755859375,4.164565216933406e-06
563,1689,0,1689,0.08736276626586914,4.0627544224095145e-06
564,1692,0,1692,0.08748793601989746,4.0308017985726785e-06
565,1695,0,1695,0.0876007080078125,3.9051954457590014e-06
566,1698,0,1698,0.08772683143615723,3.88149284454093e-06
567,1701,0,1701,0.08785271644592285,3.842988626282019e-06
568,1704,0,1704,0.08796477317810059,3.67634802694527e-06
569,1707,0,1707,0.08809089660644531,3.6300423117007654e-06
570,1710,0,1710,0.08820199966430664,3.5659625382267923e-06
571,1713,0,1713,0.08832788467407227,3.522275414359392e-06
572,1716,0,1716,0.08844685554504395,3.1142536410305417e-06
573,1719,0,1719,0.08857274055480957,3.0876324259638025e-06
574,1722,0,1722,0.0886998176574707,3.050781075846206e-06
575,1725,0,1725,0.08881187438964844,2.9370048496497498e-06
576,1728,0,1728,0.08893799781799316,2.8956585755234755e-06
577,1731,0,1731,0.0890507698059082,2.5201013446343947e-06
578,1734,0,1734,0.08917784690856934,2.480856765413722e-06
579,1737,0,1737,0.08930373191833496,2.4377146675028232e-06
580,1740,0,1740,0.0894157886505127,2.3487036856845756e-06
581,1743,0,1743,0.08967781066894531,2.304146731329825e-06
582,1746,0,1746,0.08986878395080566,2.141113010898445e-06
583,1749,0,1749,0.09001684188842773,2.104159097598349e-06
584,1752,0,1752,0.09018802642822266,2.078975692016625e-06
585,1755,0,1755,0.0903177261352539,2.0489789969381862e-06
586,1758,0,1758,0.09043097496032715,1.9308915774687576e-06
587,1761,0,1761,0.09055685997009277,1.8888155204441244e-06
588,1764,0,1764,0.0906679630279541,1.8254026365347645e-06
589,1767,0,1767,0.09079194068908691,1.7809128169520266e-06
590,1770,0,1770,0.09090304374694824,1.6903395538873396e-06
591,1773,0,1773,0.09102797508239746,1.6724855426998167e-06
592,1776,0,1776,0.09113883972167969,1.597893584101788e-06
593,1779,0,1779,0.09126591682434082,1.5778952182164914e-06
594,1782,0,1782,0.09139084815979004,1.553795663214016e-06
595,1785,0,1785,0.09150171279907227,1.5077917185201388e-06
596,1788,0,1788,0.09162592887878418,1.486345535819349e-06
597,1791,0,1791,0.09174084663391113,1.4331034339873865e-06
598,1794,0,1794,0.09186577796936035,1.4178831019553621e-06
599,1797,0,1797,0.09197783470153809,1.334931362682562e-06
600,1800,0,1800,0.0921018123626709,1.3196739032290732e-06
601,1803,0,1803,0.09221196174621582,1.2806929660408013e-06
602,1806,0,1806,0.09233474731445312,1.2678075755247928e-06
603,1809,0,1809,0.09244585037231445,1.2187863212887098e-06
604,1812,0,1812,0.09256696701049805,1.2018853948504827e-06
605,1815,0,1815,0.09267783164978027,1.142981630960781e-06
606,1818,0,1818,0.09280085563659668,1.1309435668483667e-06
607,1821,0,1821,0.0929098129272461,1.1075667523477279e-06
608,1824,0,1824,0.0930318832397461,1.091871054534579e-06
609,1827,0,1827,0.09314203262329102,1.0647897201865661e-06
610,1830,0,1830,0.09326577186584473,1.052769509436384e-06
611,1833,0,1833,0.09337592124938965,1.0246695715877961e-06
612,1836,0,1836,0.09349775314331055,1.0065266590498897e-06
613,1839,0,1839,0.09379100799560547,9.451293214132315e-07
614,1842,0,1842,0.09396195411682129,9.369172979022515e-07
615,1845,0,1845,0.09411096572875977,9.177204694151453e-07
616,1848,0,1848,0.09433865547180176,9.05439941730272e-07
617,1851,0,1851,0.09448695182800293,8.956723182228203e-07
618,1854,0,1854,0.09471797943115234,8.757670101724319e-07
619,1857,0,1857,0.09489083290100098,8.686586157276519e-07
620,1860,0,1860,0.09502577781677246,8.105233258376966e-07
621,1863,0,1863,0.09516072273254395,8.060193815809518e-07
622,1866,0,1866,0.09532475471496582,7.985708169669114e-07
623,1869,0,1869,0.09544587135314941,7.803642111780212e-07
624,1872,0,1872,0.09557676315307617,7.741950025859118e-07
625,1875,0,1875,0.0956888198852539,7.509030204247773e-07
626,1878,0,1878,0.09581494331359863,7.469743305182896e-07
627,1881,0,1881,0.09594082832336426,7.407905387481744e-07
628,1884,0,1884,0.0960688591003418,7.288915961145239e-07
629,1887,0,1887,0.0962066650390625,7.238632782735467e-07
630,1890,0,1890,0.09638285636901855,7.017523018753157e-07
631,1893,0,1893,0.09653186798095703,6.93221074415942e-07
632,1896,0,1896,0.09665679931640625,6.726598601977193e-07
633,1899,0,1899,0.09679269790649414,6.631383050016196e-07
634,1902,0,1902,0.09691286087036133,6.488408200292809e-07
635,1905,0,1905,0.09707069396972656,6.391342064434182e-07
636,1908,0,1908,0.0971839427947998,6.044912244945665e-07
637,1911,0,1911,0.09731101989746094,5.963562342177389e-07
638,1914,0,1914,0.09743881225585938,5.869670456715973e-07
639,1917,0,1917,0.09763383865356445,5.337227197567524e-07
640,1920,0,1920,0.09778571128845215,5.235926006610697e-07
641,1923,0,1923,0.09790897369384766,4.4562566527019504e-07
642,1926,0,1926,0.09804892539978027,4.3643161727454984e-07
643,1929,0,1929,0.09816694259643555,4.2754975899982754e-07
644,1932,0,1932,0.09832501411437988,4.195321654358544e-07
645,1935,0,1935,0.09843778610229492,3.972735254550833e-07
646,1938,0,1938,0.09856486320495605,3.889306508671243e-07
647,1941,0,1941,0.0986790657043457,3.757354132471679e-07
648,1944,0,1944,0.09880971908569336,3.6479953319590616e-07
649,1947,0,1947,0.0989229679107666,3.5397751144153776e-07
650,1950,0,1950,0.09904885292053223,3.4574217712243097e-07
651,1953,0,1953,0.09916281700134277,3.0839232424262145e-07
652,1956,0,1956,0.09929704666137695,3.032714598009238e-07
653,1959,0,1959,0.0994119644165039,2.9655806056125473e-07
654,1962,0,1962,0.09953784942626953,2.9187056950664935e-07
655,1965,0,1965,0.09964895248413086,2.8367136581971097e-07
656,1968,0,1968,0.09977483749389648,2.779191356235396e-07
657,1971,0,1971,0.09988784790039062,2.663606803958667e-07
658,1974,0,1974,0.10001373291015625,2.634969774830356e-07
659,1977,0,1977,0.10012578964233398,2.5985649167913903e-07
660,1980,0,1980,0.1002497673034668,2.5673105788409346e-07
661,1983,0,1983,0.10036087036132812,2.284331687738653e-07
662,1986,0,1986,0.10048675537109375,2.25708243709346e-07
663,1989,0,1989,0.1006007194519043,2.2243745164840175e-07
664,1992,0,1992,0.10072588920593262,2.19045679276488e-07
665,1995,0,1995,0.10083675384521484,1.95535731497816e-07
666,1998,0,1998,0.10096263885498047,1.926756422942705e-07
667,2001,0,2001,0.1010737419128418,1.8686589245890332e-07
668,2004,0,2004,0.10124802589416504,1.8353793517517469e-07
669,2007,0,2007,0.1013638973236084,1.799781275796748e-07
670,2010,0,2010,0.10149097442626953,1.758267463744407e-07
671,2013,0,2013,0.10160183906555176,1.7008543249257794e-07
672,2016,0,2016,0.10172796249389648,1.6806176608833155e-07
673,2019,0,2019,0.10184288024902344,1.6409174052122677e-07
674,2022,0,2022,0.10197567939758301,1.6285678540575782e-07
675,2025,0,2025,0.10210299491882324,1.610971591947247e-07
676,2028,0,2028,0.10221576690673828,1.5454722235538694e-07
677,2031,0,2031,0.1023406982421875,1.5393466404292298e-07
678,2034,0,2034,0.10246777534484863,1.529668617689059e-07
679,2037,0,2037,0.10257983207702637,1.514370817304158e-07
680,2040,0,2040,0.1027059555053711,1.5085637353057984e-07
681,2043,0,2043,0.10281705856323242,1.4836731347497793e-07
682,2046,0,2046,0.10294294357299805,1.4773909736791769e-07
683,2049,0,2049,0.10306882858276367,1.4647017712952023e-07
684,2052,0,2052,0.1031947135925293,1.4560774290159201e-07
685,2055,0,2055,0.10332083702087402,1.450942850812771e-07
686,2058,0,2058,0.10344696044921875,1.4446399420517387e-07
687,2061,0,2061,0.10357093811035156,1.4360467118801698e-07
688,2064,0,2064,0.10369682312011719,1.4286908290639438e-07
689,2067,0,2067,0.10382270812988281,1.4233680034158488e-07
690,2070,0,2070,0.10394883155822754,1.413758568760153e-07
691,2073,0,2073,0.10412287712097168,1.4045055245226862e-07
692,2076,0,2076,0.10425281524658203,1.3965998474510557e-07
693,2079,0,2079,0.10437989234924316,1.3911724248433814e-07
694,2082,0,2082,0.1045067310333252,1.3863673105435355e-07
695,2085,0,2085,0.10461997985839844,1.3708035597302682e-07
696,2088,0,2088,0.10474586486816406,1.3650984560687276e-07
697,2091,0,2091,0.1048738956451416,1.3546347429342624e-07
698,2094,0,2094,0.10500097274780273,1.3455462763656953e-07
699,2097,0,2097,0.1051328182220459,1.3373940486023212e-07
700,2100,0,2100,0.10525989532470703,1.3319082166809274e-07
701,2103,0,2103,0.10538697242736816,1.3273009692631637e-07
702,2106,0,2106,0.1055150032043457,1.3181406317403873e-07
703,2109,0,2109,0.10564184188842773,1.3098139913891017e-07
704,2112,0,2112,0.10576987266540527,1.303364849497118e-07
705,2115,0,2115,0.1058969497680664,1.2969984713875086e-07
706,2118,0,2118,0.10601091384887695,1.2823735354902023e-07
707,2121,0,2121,0.10616779327392578,1.2761002987852615e-07
708,2124,0,2124,0.10630679130554199,1.266224218476283e-07
709,2127,0,2127,0.10642194747924805,1.2467941536173984e-07
710,2130,0,2130,0.10657095909118652,1.243552210400254e-07
711,2133,0,2133,0.10669994354248047,1.2367907144872245e-07
712,2136,0,2136,0.10683965682983398,1.228656216816619e-07
713,2139,0,2139,0.10703372955322266,1.2222904975367416e-07
714,2142,0,2142,0.10717988014221191,1.215372383032879e-07
715,2145,0,2145,0.10730695724487305,1.2106399712617807e-07
716,2148,0,2148,0.10743379592895508,1.2073767591690352e-07
717,2151,0,2151,0.10762190818786621,1.2029656506418743e-07
718,2154,0,2154,0.10786676406860352,1.1982427344673527e-07
719,2157,0,2157,0.10804295539855957,1.1925910095525016e-07
720,2160,0,2160,0.10823607444763184,1.1886896385877293e-07
721,2163,0,2163,0.1084449291229248,1.185449581381336e-07
722,2166,0,2166,0.1085970401763916,1.1819838390535132e-07
723,2169,0,2169,0.10876679420471191,1.1783020065426487e-07
724,2172,0,2172,0.10907483100891113,1.1755334965923587e-07
725,2175,0,2175,0.10932302474975586,1.1728741123109292e-07
726,2178,0,2178,0.10954976081848145,1.1707274227819753e-07
727,2181,0,2181,0.10969686508178711,1.1694346508532198e-07
728,2184,0,2184,0.1099557876586914,1.1672783600288433e-07
729,2187,0,2187,0.1102290153503418,1.1653636074722699e-07
730,2190,0,2190,0.11046671867370605,1.1637864293204894e-07
731,2193,0,2193,0.11070799827575684,1.1619280719893698e-07
732,2196,0,2196,0.11096596717834473,1.1595944030926881e-07
733,2199,0,2199,0.11121082305908203,1.1579848593393269e-07
734,2202,0,2202,0.11138081550598145,1.1538311039044871e-07
735,2205,0,2205,0.11153888702392578,1.1516107105618155e-07
736,2208,0,2208,0.11167478561401367,1.1500594288327428e-07
737,2211,0,2211,0.11184096336364746,1.1489162575016877e-07
738,2214,0,2214,0.11197185516357422,1.1470242831595407e-07
739,2217,0,2217,0.11210179328918457,1.1456825075265739e-07
740,2220,0,2220,0.11224985122680664,1.1434112480735817e-07
741,2223,0,2223,0.11246275901794434,1.1405335137863646e-07
742,2226,0,2226,0.11262679100036621,1.1387175132913637e-07
743,2229,0,2229,0.11287403106689453,1.1364326719466676e-07
744,2232,0,2232,0.11311101913452148,1.1339112889563411e-07
745,2235,0,2235,0.11327099800109863,1.13205914184047e-07
746,2238,0,2238,0.11342287063598633,1.1302353205790597e-07
747,2241,0,2241,0.11358785629272461,1.1291199338341836e-07
748,2244,0,2244,0.11374902725219727,1.1275670904819057e-07
749,2247,0,2247,0.1138768196105957,1.1263474190832698e-07
750,2250,0,2250,0.11401081085205078,1.1252264936929204e-07
751,2253,0,2253,0.1141366958618164,1.124120280929509e-07
752,2256,0,2256,0.11426568031311035,1.1228374743602122e-07
753,2259,0,2259,0.11439275741577148,1.1209367400466696e-07
754,2262,0,2262,0.11452388763427734,1.1198604126097159e-07
755,2265,0,2265,0.11466383934020996,1.1188783737150605e-07
756,2268,0,2268,0.11479973793029785,1.116916972812169e-07
757,2271,0,2271,0.11499476432800293,1.1161050901417693e-07
758,2274,0,2274,0.11514496803283691,1.1148406172445418e-07
759,2277,0,2277,0.1153097152709961,1.1135931716567375e-07
760,2280,0,2280,0.11557579040527344,1.1125825070622822e-07
761,2283,0,2283,0.11580371856689453,1.11141822880033e-07
762,2286,0,2286,0.11605501174926758,1.1105679243799846e-07
763,2289,0,2289,0.11623978614807129,1.1089451885037445e-07
764,2292,0,2292,0.11643385887145996,1.108185816103508e-07
765,2295,0,2295,0.11658787727355957,1.1072957991365507e-07
766,2298,0,2298,0.11677694320678711,1.1065151839986839e-07
767,2301,0,2301,0.11692285537719727,1.105644928498888e-07
768,2304,0,2304,0.11708903312683105,1.1043066136253465e-07
769,2307,0,2307,0.1172788143157959,1.1029746446066406e-07
770,2310,0,2310,0.11752486228942871,1.10186558417691e-07
771,2313,0,2313,0.11768770217895508,1.1007908756969911e-07
772,2316,0,2316,0.11789178848266602,1.099972594249422e-07
773,2319,0,2319,0.1180868148803711,1.0985619178013489e-07
774,2322,0,2322,0.11828184127807617,1.0971756967777958e-07
775,2325,0,2325,0.11843299865722656,1.0945146517091961e-07
776,2328,0,2328,0.11857986450195312,1.0927799334738818e-07
777,2331,0,2331,0.11877775192260742,1.0917868232882466e-07
778,2334,0,2334,0.11895394325256348,1.0891937600721172e-07
779,2337,0,2337,0.11911487579345703,1.0880053610643437e-07
780,2340,0,2340,0.11926078796386719,1.0845298001438423e-07
781,2343,0,2343,0.11943292617797852,1.0826814867304146e-07
782,2346,0,2346,0.11960983276367188,1.0812044475227576e-07
783,2349,0,2349,0.11979985237121582,1.0756479503417276e-07
784,2352,0,2352,0.11999678611755371,1.0723603358739097e-07
785,2355,0,2355,0.12019586563110352,1.0671828575717635e-07
786,2358,0,2358,0.12038969993591309,1.0601172318669491e-07
787,2361,0,2361,0.12056493759155273,1.0532716571291144e-07
788,2364,0,2364,0.12070083618164062,1.0436857762732721e-07
789,2367,0,2367,0.12084388732910156,1.0337700709018464e-07
790,2370,0,2370,0.12096381187438965,9.940285275160027e-08
791,2373,0,2373,0.12112784385681152,9.878066655856854e-08
792,2376,0,2376,0.1212468147277832,9.522578256053632e-08
793,2379,0,2379,0.12137770652770996,9.422447908355689e-08
794,2382,0,2382,0.12150192260742188,9.124521873160945e-08
795,2385,0,2385,0.12163472175598145,9.040497333395632e-08
796,2388,0,2388,0.12175679206848145,8.885535799234629e-08
797,2391,0,2391,0.12188887596130371,8.815155744313008e-08
798,2394,0,2394,0.12200593948364258,8.690219088723792e-08
799,2397,0,2397,0.12213778495788574,8.608444280624898e-08
800,2400,0,2400,0.12227368354797363,8.507573678710082e-08
801,2403,0,2403,0.12240099906921387,8.41084836467191e-08
802,2406,0,2406,0.12253475189208984,8.335878017462488e-08
803,2409,0,2409,0.12265491485595703,7.855351121689727e-08
804,2412,0,2412,0.12295198440551758,7.794994259984992e-08
805,2415,0,2415,0.12311601638793945,7.705990041565605e-08
806,2418,0,2418,0.12330389022827148,7.655139511816382e-08
807,2421,0,2421,0.12346982955932617,7.543785063240088e-08
808,2424,0,2424,0.12380790710449219,7.49315988085428e-08
809,2427,0,2427,0.12410283088684082,7.189370683815979e-08
810,2430,0,2430,0.12439393997192383,7.144146114648057e-08
811,2433,0,2433,0.12464094161987305,7.044287848007801e-08
812,2436,0,2436,0.12479376792907715,7.005511198503651e-08
813,2439,0,2439,0.12497591972351074,6.821770231437642e-08
814,2442,0,2442,0.12514305114746094,6.780065611215362e-08
815,2445,0,2445,0.12530303001403809,6.717194970989286e-08
816,2448,0,2448,0.1255018711090088,6.653866445544166e-08
817,2451,0,2451,0.12565302848815918,6.615326138114294e-08
818,2454,0,2454,0.12579083442687988,6.419064640311191e-08
819,2457,0,2457,0.12592482566833496,6.38560524140242e-08
820,2460,0,2460,0.12607264518737793,6.206316929364648e-08
821,2463,0,2463,0.12619900703430176,6.159740079314065e-08
822,2466,0,2466,0.1263117790222168,6.026491465261812e-08
823,2469,0,2469,0.12643980979919434,5.995453349721593e-08
824,2472,0,2472,0.12656593322753906,5.9484489638917944e-08
825,2475,0,2475,0.1266796588897705,5.7784737509302736e-08
826,2478,0,2478,0.12680387496948242,5.735286715060585e-08
827,2481,0,2481,0.12694096565246582,5.682354484599753e-08
828,2484,0,2484,0.12705206871032715,5.503472558695887e-08
829,2487,0,2487,0.12717890739440918,5.454720162122127e-08
830,2490,0,2490,0.127288818359375,5.228085938794279e-08
831,2493,0,2493,0.12741303443908691,5.181036239337535e-08
832,2496,0,2496,0.12752485275268555,5.1034293150658153e-08
833,2499,0,2499,0.12764978408813477,5.054979563383385e-08
834,2502,0,2502,0.12779593467712402,5.017134220788604e-08
835,2505,0,2505,0.12798786163330078,4.9162004612401964e-08
836,2508,0,2508,0.12815284729003906,4.864440668564729e-08
837,2511,0,2511,0.12827491760253906,4.5443366216758414e-08
838,2514,0,2514,0.12840771675109863,4.47997085998742e-08
839,2517,0,2517,0.1285538673400879,4.410474011601823e-08
840,2520,0,2520,0.12868189811706543,4.2978668482575837e-08
841,2523,0,2523,0.12880778312683105,4.2353856180515946e-08
842,2526,0,2526,0.1289217472076416,4.0334400275081584e-08
843,2529,0,2529,0.12904763221740723,3.984142568260527e-08
844,2532,0,2532,0.12915992736816406,3.752276967785586e-08
845,2535,0,2535,0.1292867660522461,3.722293773793764e-08
846,2538,0,2538,0.12941384315490723,3.676590900648622e-08
847,2541,0,2541,0.12952876091003418,3.219652948086933e-08
848,2544,0,2544,0.12967586517333984,3.166536081519135e-08
849,2547,0,2547,0.12984085083007812,2.955183753500885e-08
850,2550,0,2550,0.13002395629882812,2.9110799731823176e-08
851,2553,0,2553,0.13019490242004395,2.8173120385869044e-08
852,2556,0,2556,0.1304159164428711,2.7659721428986954e-08
853,2559,0,2559,0.13054585456848145,2.7340025931978695e-08
854,2562,0,2562,0.1306748390197754,2.6588682974691806e-08
855,2565,0,2565,0.13078784942626953,2.4666315454563727e-08
856,2568,0,2568,0.13091373443603516,2.4328632936178054e-08
857,2571,0,2571,0.1310257911682129,2.3524044057395207e-08
858,2574,0,2574,0.13115191459655762,2.3200949931870967e-08
859,2577,0,2577,0.13126397132873535,2.1148056881821232e-08
860,2580,0,2580,0.13138985633850098,2.0962216202502134e-08
861,2583,0,2583,0.13150596618652344,2.0583031633554178e-08
862,2586,0,2586,0.13162970542907715,2.0437002683221236e-08
863,2589,0,2589,0.13173985481262207,2.0127909279230953e-08
864,2592,0,2592,0.1318666934967041,1.9988931685216725e-08
865,2595,0,2595,0.13197684288024902,1.9534566951970095e-08
866,2598,0,2598,0.13210177421569824,1.9361896296996944e-08
867,2601,0,2601,0.13222765922546387,1.9153485529798993e-08
868,2604,0,2604,0.13234186172485352,1.863047116499935e-08
869,2607,0,2607,0.13247108459472656,1.844715890267007e-08
870,2610,0,2610,0.1325829029083252,1.8120893023219098e-08
871,2613,0,2613,0.1327066421508789,1.7915168420006514e-08
872,2616,0,2616,0.13281679153442383,1.6992482936117585e-08
873,2619,0,2619,0.13295888900756836,1.6803052244734363e-08
874,2622,0,2622,0.13308286666870117,1.656493782050697e-08
875,2625,0,2625,0.13320708274841309,1.5869242621016928e-08
876,2628,0,2628,0.13336181640625,1.577203996808989e-08
877,2631,0,2631,0.13348889350891113,1.560135861421117e-08
878,2634,0,2634,0.13371801376342773,1.550140149277015e-08
879,2637,0,2637,0.1338958740234375,1.535756762283928e-08
880,2640,0,2640,0.13402700424194336,1.4818842547969332e-08
881,2643,0,2643,0.13416600227355957,1.4755857488285754e-08
882,2646,0,2646,0.13433289527893066,1.4604484981306362e-08
883,2649,0,2649,0.13448286056518555,1.4560699210116375e-08
884,2652,0,2652,0.13467168807983398,1.4311855504153442e-08
885,2655,0,2655,0.1348249912261963,1.4284591856792392e-08
886,2658,0,2658,0.1350116729736328,1.4252609505603528e-08
887,2661,0,2661,0.1351480484008789,1.408046998960134e-08
888,2664,0,2664,0.13541197776794434,1.4047114944722992e-08
889,2667,0,2667,0.13569378852844238,1.4000799768501932e-08
890,2670,0,2670,0.13590288162231445,1.3944577341527596e-08
891,2673,0,2673,0.13608598709106445,1.3916037092592749e-08
892,2676,0,2676,0.13622498512268066,1.3884054395437005e-08
893,2679,0,2679,0.13635993003845215,1.3853971959551709e-08
894,2682,0,2682,0.1365036964416504,1.3825808164645481e-08
895,2685,0,2685,0.13664674758911133,1.378483750748058e-08
896,2688,0,2688,0.13679170608520508,1.3730445087105458e-08
897,2691,0,2691,0.13692903518676758,1.3697478536888085e-08
898,2694,0,2694,0.13707971572875977,1.3653487076401481e-08
899,2697,0,2697,0.13727784156799316,1.3621324891501071e-08
900,2700,0,2700,0.13753795623779297,1.3594085452091778e-08
901,2703,0,2703,0.13780784606933594,1.3555276017574436e-08
902,2706,0,2706,0.1380019187927246,1.3511473047058047e-08
903,2709,0,2709,0.13818597793579102,1.3479904076112757e-08
904,2712,0,2712,0.13832783699035645,1.3452456388073237e-08
905,2715,0,2715,0.13848876953125,1.3434972613236804e-08
906,2718,0,2718,0.13884782791137695,1.3408977294985873e-08
907,2721,0,2721,0.13908982276916504,1.3373969686181691e-08
908,2724,0,2724,0.13931703567504883,1.3341914595237028e-08
909,2727,0,2727,0.1395859718322754,1.33151850181086e-08
910,2730,0,2730,0.1397860050201416,1.3304573014448313e-08
911,2733,0,2733,0.1401059627532959,1.3297507289521347e-08
912,2736,0,2736,0.1403210163116455,1.3272549844152144e-08
913,2739,0,2739,0.1405787467956543,1.3259114401926972e-08
914,2742,0,2742,0.1407468318939209,1.3224397146381262e-08
915,2745,0,2745,0.14089083671569824,1.3204780464829279e-08
916,2748,0,2748,0.141068696975708,1.3192623585874733e-08
917,2751,0,2751,0.1413567066192627,1.3173509410583836e-08
918,2754,0,2754,0.14148974418640137,1.3158788827841802e-08
919,2757,0,2757,0.14161992073059082,1.3148588418937786e-08
920,2760,0,2760,0.14174795150756836,1.3132207513557338e-08
921,2763,0,2763,0.1418769359588623,1.3119121959290133e-08
922,2766,0,2766,0.14200687408447266,1.3101551523537522e-08
923,2769,0,2769,0.14214086532592773,1.3086101530854644e-08
924,2772,0,2772,0.14228582382202148,1.307276767472657e-08
925,2775,0,2775,0.14245986938476562,1.3043199289868581e-08
926,2778,0,2778,0.14258980751037598,1.302649088339269e-08
927,2781,0,2781,0.1427309513092041,1.3011712035762512e-08
928,2784,0,2784,0.14286279678344727,1.2977426837128126e-08
929,2787,0,2787,0.14300894737243652,1.2958387673066225e-08
930,2790,0,2790,0.1431417465209961,1.2944925268966009e-08
931,2793,0,2793,0.14327597618103027,1.2921766059364977e-08
932,2796,0,2796,0.14345479011535645,1.289186786727576e-08
933,2799,0,2799,0.14362287521362305,1.2872053956049065e-08
934,2802,0,2802,0.14375591278076172,1.2837593094414986e-08
935,2805,0,2805,0.14388394355773926,1.2812332715086743e-08
936,2808,0,2808,0.1440119743347168,1.2792123980824749e-08
937,2811,0,2811,0.14414167404174805,1.2754699964307134e-08
938,2814,0,2814,0.14428377151489258,1.2734210597031165e-08
939,2817,0,2817,0.14449691772460938,1.2715689352380163e-08
940,2820,0,2820,0.144744873046875,1.2690323800050462e-08
941,2823,0,2823,0.14498305320739746,1.2656117727942453e-08
942,2826,0,2826,0.14516472816467285,1.2617282648665933e-08
943,2829,0,2829,0.14546585083007812,1.2575072317563294e-08
944,2832,0,2832,0.1457526683807373,1.254015212308174e-08
945,2835,0,2835,0.14591479301452637,1.247519940502383e-08
946,2838,0,2838,0.14605474472045898,1.2424050917233253e-08
947,2841,0,2841,0.14620375633239746,1.2374532109987044e-08
948,2844,0,2844,0.14648771286010742,1.2338004691196645e-08
949,2847,0,2847,0.14672470092773438,1.2309127412374472e-08
950,2850,0,2850,0.14688372611999512,1.2259952702722392e-08
951,2853,0,2853,0.1471269130706787,1.2211666928050682e-08
952,2856,0,2856,0.1473388671875,1.2162538971423525e-08
953,2859,0,2859,0.1474769115447998,1.2099667208327316e-08
954,2862,0,2862,0.14761686325073242,1.2056123388007097e-08
955,2865,0,2865,0.1477670669555664,1.1991734142082604e-08
956,2868,0,2868,0.1480410099029541,1.192370238088028e-08
957,2871,0,2871,0.14824700355529785,1.1871889535334694e-08
958,2874,0,2874,0.14838290214538574,1.18238745952083e-08
959,2877,0,2877,0.14853191375732422,1.1767450536834076e-08
960,2880,0,2880,0.14865899085998535,1.1714332088284656e-08
961,2883,0,2883,0.14883875846862793,1.1678209900760734e-08
962,2886,0,2886,0.14900875091552734,1.1635580259957274e-08
963,2889,0,2889,0.1491398811340332,1.1601427855391458e-08
964,2892,0,2892,0.1492769718170166,1.1562398851274897e-08
965,2895,0,2895,0.14940690994262695,1.1513670286932568e-08
966,2898,0,2898,0.14955592155456543,1.1480364039983852e-08
967,2901,0,2901,0.14970803260803223,1.1439004955126458e-08
968,2904,0,2904,0.14983868598937988,1.1366557313774784e-08
969,2907,0,2907,0.14996886253356934,1.1326478052926536e-08
970,2910,0,2910,0.1500988006591797,1.1281368001756043e-08
971,2913,0,2913,0.15021371841430664,1.1162963393720947e-08
972,2916,0,2916,0.1503438949584961,1.1129581043510185e-08
973,2919,0,2919,0.15047979354858398,1.1042180020883108e-08
974,2922,0,2922,0.15059566497802734,1.0903392922648653e-08
975,2925,0,2925,0.1507258415222168,1.0867221208571982e-08
976,2928,0,2928,0.15084075927734375,1.0741386149658869e-08
977,2931,0,2931,0.1509697437286377,1.0714522816791165e-08
978,2934,0,2934,0.15110087394714355,1.0652558661025218e-08
979,2937,0,2937,0.15128397941589355,1.0510700864490138e-08
980,2940,0,2940,0.1515038013458252,1.0447641489313247e-08
981,2943,0,2943,0.15167689323425293,1.026564415591162e-08
982,2946,0,2946,0.15187883377075195,1.016942090736609e-08
983,2949,0,2949,0.15213489532470703,9.959243559104295e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha0/flex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.915496826171875e-05,4.387061074692293
1,5,0,5,0.0002422332763671875,4.2514878856800244
2,10,0,10,0.0006430149078369141,3.8546852614608893
3,13,0,13,0.0008800029754638672,3.478351662948141
4,16,0,16,0.00121307373046875,3.416497347893481
5,20,0,20,0.0015110969543457031,3.3058207048491934
6,23,0,23,0.0017261505126953125,3.232429156876266
7,26,0,26,0.0019309520721435547,2.9306400110523825
8,29,0,29,0.0021381378173828125,2.661335825805268
9,32,0,32,0.0023279190063476562,2.3690405162990498
10,35,0,35,0.0025331974029541016,1.574705936211792
11,39,0,39,0.002749204635620117,1.520775780452156
12,43,0,43,0.0030100345611572266,1.4873768897048536
13,46,0,46,0.0032129287719726562,1.4321931702806545
14,49,0,49,0.003434896469116211,1.3612867685608938
15,54,0,54,0.003667116165161133,1.2523733032621758
16,58,0,58,0.003892183303833008,1.1634450518701838
17,61,0,61,0.004083156585693359,1.1304493035466832
18,65,0,65,0.004308938980102539,1.0490884784851864
19,69,0,69,0.004530191421508789,1.0333629673351694
20,72,0,72,0.004723072052001953,0.7504593225166305
21,75,0,75,0.004930973052978516,0.7043616145474156
22,79,0,79,0.005155086517333984,0.6721527858502336
23,83,0,83,0.00537419319152832,0.6275684872258744
24,86,0,86,0.0055789947509765625,0.6067458059024816
25,89,0,89,0.005791902542114258,0.5627057844173515
26,92,0,92,0.005978107452392578,0.3774350180712767
27,95,0,95,0.00617218017578125,0.36624348055570943
28,98,0,98,0.006489992141723633,0.27360860973118356
29,102,0,102,0.006749153137207031,0.2672501843219862
30,105,0,105,0.0069580078125,0.25060346337210215
31,108,0,108,0.0071620941162109375,0.24193320293271187
32,113,0,113,0.0074121952056884766,0.236162747467861
33,118,0,118,0.0076410770416259766,0.23093960191936377
34,123,0,123,0.00797891616821289,0.22618174918983044
35,127,0,127,0.008282184600830078,0.22565862413910037
36,130,0,130,0.008477210998535156,0.21025588936424977
37,133,0,133,0.008669137954711914,0.14630154737886447
38,136,0,136,0.008861064910888672,0.13448460965441264
39,139,0,139,0.009048938751220703,0.1324969318487299
40,143,0,143,0.009274005889892578,0.12422791458147336
41,147,0,147,0.00949716567993164,0.12218109049690261
42,151,0,151,0.009721994400024414,0.11550290277889491
43,154,0,154,0.009911060333251953,0.10169286604791537
44,157,0,157,0.01023721694946289,0.0724491427681876
45,160,0,160,0.010596036911010742,0.07151290218313094
46,164,0,164,0.010996103286743164,0.06922170113813034
47,168,0,168,0.01135706901550293,0.06784237637772056
48,173,0,173,0.01164102554321289,0.06711520764923017
49,178,0,178,0.011980056762695312,0.06645289922371621
50,183,0,183,0.012335062026977539,0.06584585521817748
51,188,0,188,0.012578010559082031,0.06528623187724732
52,193,0,193,0.01282501220703125,0.0647675932860838
53,197,0,197,0.013049125671386719,0.06341646587442311
54,200,0,200,0.013257265090942383,0.06318960685012566
55,203,0,203,0.013543128967285156,0.06065199028853831
56,207,0,207,0.013839006423950195,0.057924669126414266
57,210,0,210,0.014050960540771484,0.05207790987086858
58,213,0,213,0.014243125915527344,0.04573889813603081
59,217,0,217,0.014494180679321289,0.04496774438717166
60,220,0,220,0.014723062515258789,0.04433637795343284
61,225,0,225,0.015008926391601562,0.04387010141612501
62,230,0,230,0.01525115966796875,0.04344863098730567
63,235,0,235,0.015558004379272461,0.04306541052356413
64,240,0,240,0.015796899795532227,0.042715010930761334
65,245,0,245,0.016122102737426758,0.04239292657067039
66,250,0,250,0.016482114791870117,0.042095407976506044
67,255,0,255,0.016820907592773438,0.041819324916231256
68,259,0,259,0.017091989517211914,0.041536830458205665
69,263,0,263,0.017318010330200195,0.0411464513186611
70,266,0,266,0.01754903793334961,0.04064789840843676
71,269,0,269,0.01781916618347168,0.04054330062044691
72,273,0,273,0.01812291145324707,0.04023468805155606
73,276,0,276,0.01843094825744629,0.03992256545827922
74,279,0,279,0.01871514320373535,0.03915876546031952
75,284,0,284,0.019083023071289062,0.038462055687000035
76,289,0,289,0.019479036331176758,0.03782709190521317
77,294,0,294,0.01987600326538086,0.037246108109462585
78,299,0,299,0.020263195037841797,0.036712600895155434
79,304,0,304,0.020615100860595703,0.03622109819500934
80,308,0,308,0.020951032638549805,0.03620578007343768
81,313,0,313,0.021255016326904297,0.035734804219420754
82,318,0,318,0.021531105041503906,0.035303952895963844
83,322,0,322,0.021784067153930664,0.03460571219609875
84,327,0,327,0.022021055221557617,0.03427514444416489
85,332,0,332,0.02225518226623535,0.0339652875569984
86,337,0,337,0.022492170333862305,0.033674521525840856
87,342,0,342,0.022739171981811523,0.03340138689234838
88,346,0,346,0.02295708656311035,0.03218630476712578
89,351,0,351,0.023185014724731445,0.03194041536312966
90,356,0,356,0.02341604232788086,0.03171712993774379
91,361,0,361,0.02364206314086914,0.031513558938983444
92,365,0,365,0.023867130279541016,0.030455154274471524
93,370,0,370,0.02410411834716797,0.03027637616599037
94,375,0,375,0.024335145950317383,0.030118926677209747
95,380,0,380,0.024559974670410156,0.029979441759623048
96,385,0,385,0.024790048599243164,0.02985515471259885
97,390,0,390,0.025141000747680664,0.029743785763353545
98,395,0,395,0.025402069091796875,0.02964345183654465
99,400,0,400,0.025648117065429688,0.029552593062537966
100,405,0,405,0.025925159454345703,0.029469913060360436
101,410,0,410,0.026273012161254883,0.0293943304909836
102,415,0,415,0.026607990264892578,0.029324939791094923
103,420,0,420,0.02696704864501953,0.02926097935995855
104,425,0,425,0.027319908142089844,0.02920180578200157
105,430,0,430,0.027593135833740234,0.029146872928709322
106,435,0,435,0.027857065200805664,0.029095715000416765
107,440,0,440,0.02809000015258789,0.029047932747380708
108,445,0,445,0.02833700180053711,0.02900318225581333
109,450,0,450,0.028574228286743164,0.028961165803604257
110,455,0,455,0.02881002426147461,0.028921624386938023
111,460,0,460,0.029159069061279297,0.028884331596948896
112,465,0,465,0.029488086700439453,0.02884908858836638
113,470,0,470,0.029792070388793945,0.02881571993263034
114,475,0,475,0.030144929885864258,0.028784070188554355
115,480,0,480,0.030532121658325195,0.028754001056202995
116,485,0,485,0.030802249908447266,0.0287253890058
117,490,0,490,0.031054973602294922,0.028698123294460455
118,495,0,495,0.031316280364990234,0.02867210430036916
119,500,0,500,0.03154802322387695,0.028647242117530967
120,505,0,505,0.031858205795288086,0.028623455365061844
121,510,0,510,0.03209519386291504,0.02860067017369859
122,515,0,515,0.032424211502075195,0.028578819319208082
123,520,0,520,0.032675981521606445,0.028557841478013556
124,525,0,525,0.032959938049316406,0.02853768058489521
125,530,0,530,0.033385276794433594,0.02851828527628846
126,535,0,535,0.03384113311767578,0.02849960840566005
127,540,0,540,0.03419685363769531,0.02848160661984041
128,545,0,545,0.03447914123535156,0.028464239987131174
129,550,0,550,0.03480219841003418,0.028447471669584223
130,555,0,555,0.03512310981750488,0.028431267633133216
131,560,0,560,0.03538393974304199,0.028415596390305085
132,565,0,565,0.03562307357788086,0.02840042877109712
133,570,0,570,0.03586292266845703,0.028385737718306304
134,575,0,575,0.036115169525146484,0.02837149810417723
135,580,0,580,0.03638601303100586,0.028357686565709094
136,585,0,585,0.03662705421447754,0.028344281356360457
137,590,0,590,0.03686118125915527,0.028331262212213573
138,595,0,595,0.03710007667541504,0.02831861023093791
139,600,0,600,0.03733491897583008,0.028306307762116036
140,605,0,605,0.037574052810668945,0.02829433830769149
141,610,0,610,0.03780817985534668,0.02828268643145681
142,615,0,615,0.038068294525146484,0.028271337676637365
143,620,0,620,0.038323163986206055,0.02826027849074536
144,625,0,625,0.0385892391204834,0.0282494961569738
145,630,0,630,0.03883099555969238,0.028238978731489214
146,635,0,635,0.03907513618469238,0.028228714986053005
147,640,0,640,0.03932785987854004,0.028218694355465826
148,645,0,645,0.039565086364746094,0.028208906889383354
149,650,0,650,0.03979897499084473,0.028199343208101493
150,655,0,655,0.04005908966064453,0.0281899944619495
151,660,0,660,0.0403590202331543,0.028180852293966524
152,665,0,665,0.040635108947753906,0.028171908805571286
153,670,0,670,0.04092001914978027,0.028163156524960337
154,675,0,675,0.041314125061035156,0.028154588377999383
155,680,0,680,0.04169511795043945,0.02814619766139053
156,685,0,685,0.042086124420166016,0.028137978017923768
157,690,0,690,0.042474985122680664,0.028129923413633427
158,695,0,695,0.042877197265625,0.028122028116701427
159,700,0,700,0.04322409629821777,0.028114286677960187
160,705,0,705,0.04347705841064453,0.028106693912863363
161,710,0,710,0.0437932014465332,0.028099244884803053
162,715,0,715,0.044183969497680664,0.02809193488966376
163,720,0,720,0.04462313652038574,0.02808475944151158
164,725,0,725,0.045037031173706055,0.028077714259328024
165,730,0,730,0.04544711112976074,0.028070795254703813
166,735,0,735,0.0458369255065918,0.02806399852041565
167,740,0,740,0.0461878776550293,0.02805732031981657
168,745,0,745,0.046526193618774414,0.02805075707697485
169,750,0,750,0.04679703712463379,0.0280443053675032
170,755,0,755,0.047181129455566406,0.028037961910023536
171,760,0,760,0.0474390983581543,0.02803172355821921
172,765,0,765,0.047782182693481445,0.02802558729342752
173,770,0,770,0.0481572151184082,0.02801955021773304
174,775,0,775,0.048523902893066406,0.028013609547521367
175,780,0,780,0.04892611503601074,0.028007762607460223
176,785,0,785,0.049363136291503906,0.028002006824874585
177,790,0,790,0.049787044525146484,0.027996339724486233
178,795,0,795,0.05020904541015625,0.027990758923491448
179,800,0,800,0.05064105987548828,0.027985262126950683
180,805,0,805,0.051038265228271484,0.02797984712346799
181,810,0,810,0.051316261291503906,0.027974511781139057
182,815,0,815,0.051651954650878906,0.027969254043747793
183,820,0,820,0.05199098587036133,0.027964071927194245
184,825,0,825,0.05233407020568848,0.027958963516136696
185,830,0,830,0.05269503593444824,0.027953926960833275
186,835,0,835,0.05306601524353027,0.027948960474168616
187,840,0,840,0.05340218544006348,0.027944062328852683
188,845,0,845,0.05364513397216797,0.027939230854780547
189,850,0,850,0.053965091705322266,0.027934464436540567
190,855,0,855,0.05422210693359375,0.027929761511062745
191,860,0,860,0.05448603630065918,0.02792512056539575
192,865,0,865,0.05485105514526367,0.027920540134606098
193,870,0,870,0.05524921417236328,0.027916018799789638
194,875,0,875,0.055541038513183594,0.027911555186188857
195,880,0,880,0.05578112602233887,0.02790714796140937
196,885,0,885,0.0560760498046875,0.027902795833727914
197,890,0,890,0.056539058685302734,0.027898497550487764
198,895,0,895,0.056916236877441406,0.027894251896574705
199,899,0,899,0.05739903450012207,0.02788848071578543
200,904,0,904,0.0578310489654541,0.027870284527089565
201,909,0,909,0.05817914009094238,0.027853739548459454
202,914,0,914,0.05844712257385254,0.027838578817278647
203,919,0,919,0.05882096290588379,0.027824587432018707
204,924,0,924,0.05925798416137695,0.027811591664777216
205,929,0,929,0.059712886810302734,0.027799450426497178
206,933,0,933,0.060012102127075195,0.027784738902869224
207,938,0,938,0.06026315689086914,0.027768475995642774
208,943,0,943,0.06051206588745117,0.02775362071771414
209,948,0,948,0.0608060359954834,0.027739928548222294
210,953,0,953,0.06117510795593262,0.027727206657568757
211,958,0,958,0.06151008605957031,0.027715302377698904
212,962,0,962,0.06182289123535156,0.027700752458607276
213,967,0,967,0.06210803985595703,0.027689600601738192
214,972,0,972,0.062406063079833984,0.02767924231662545
215,977,0,977,0.06265807151794434,0.02766954403823698
216,982,0,982,0.06291818618774414,0.02766039965448348
217,987,0,987,0.06330513954162598,0.027651724543227334
218,992,0,992,0.06370091438293457,0.02764345093545567
219,997,0,997,0.06412506103515625,0.027635524305686006
220,1002,0,1002,0.06457710266113281,0.02762790055856326
221,1007,0,1007,0.06487488746643066,0.027620543833043736
222,1012,0,1012,0.06512928009033203,0.027613424786049667
223,1017,0,1017,0.06540989875793457,0.027606519248736274
224,1022,0,1022,0.06579923629760742,0.027599807172645964
225,1027,0,1027,0.06622314453125,0.02759327180166229
226,1032,0,1032,0.06664490699768066,0.02758689902007315
227,1037,0,1037,0.06699109077453613,0.027580676838181165
228,1042,0,1042,0.06739616394042969,0.027574594985504793
229,1047,0,1047,0.06788015365600586,0.027568644588273378
230,1052,0,1052,0.06827402114868164,0.027562817913077242
231,1057,0,1057,0.06871795654296875,0.027557108162531704
232,1062,0,1062,0.06908607482910156,0.027551509311915964
233,1067,0,1067,0.06951403617858887,0.02754601597815571
234,1072,0,1072,0.06987786293029785,0.027540623314393213
235,1077,0,1077,0.07023501396179199,0.027535326924843666
236,1082,0,1082,0.07050585746765137,0.027530122795775477
237,1087,0,1087,0.0708150863647461,0.027525007239337238
238,1092,0,1092,0.0711359977722168,0.02751997684764709
239,1097,0,1097,0.07142496109008789,0.027515028455103844
240,1102,0,1102,0.07168912887573242,0.027510159107302066
241,1107,0,1107,0.0720219612121582,0.027505366035269988
242,1112,0,1112,0.07234406471252441,0.027500646634008946
243,1117,0,1117,0.07261514663696289,0.027495998444522034
244,1122,0,1122,0.07286810874938965,0.027491419138681455
245,1127,0,1127,0.07312202453613281,0.0274869065064144
246,1132,0,1132,0.07348108291625977,0.027482458444789217
247,1137,0,1137,0.07386994361877441,0.027478072948664677
248,1142,0,1142,0.07423806190490723,0.02747374810263092
249,1147,0,1147,0.07455110549926758,0.027469482074020977
250,1152,0,1152,0.07489824295043945,0.027465273106814243
251,1156,0,1156,0.07522392272949219,0.027460782224937225
252,1161,0,1161,0.07552313804626465,0.02744542235388269
253,1166,0,1166,0.07578206062316895,0.027431721687641054
254,1171,0,1171,0.07616519927978516,0.027419379581339724
255,1176,0,1176,0.07654213905334473,0.027408156198618267
256,1181,0,1181,0.07682919502258301,0.027397859678163123
257,1186,0,1186,0.0772562026977539,0.027388336071538538
258,1191,0,1191,0.0776360034942627,0.027379461445914563
259,1196,0,1196,0.07788515090942383,0.027371135678679104
260,1201,0,1201,0.078125,0.027363277575085936
261,1206,0,1206,0.07838296890258789,0.0273558210213212
262,1211,0,1211,0.07866406440734863,0.02734871194865683
263,1215,0,1215,0.07896900177001953,0.027331414555457435
264,1220,0,1220,0.07921409606933594,0.027312082443708287
265,1225,0,1225,0.07947421073913574,0.027295117430990775
266,1230,0,1230,0.07983517646789551,0.027280084499641245
267,1235,0,1235,0.08020496368408203,0.02726663670021801
268,1240,0,1240,0.08047986030578613,0.027254496539415633
269,1245,0,1245,0.08075404167175293,0.02724344139996646
270,1250,0,1250,0.08110713958740234,0.027233292106982176
271,1255,0,1255,0.08135795593261719,0.027223903950325916
272,1260,0,1260,0.0817101001739502,0.027215159625164236
273,1265,0,1265,0.08203697204589844,0.027206963671831442
274,1269,0,1269,0.08228707313537598,0.027206292491413295
275,1274,0,1274,0.08252620697021484,0.027179575747188853
276,1279,0,1279,0.0827639102935791,0.02715671287976976
277,1284,0,1284,0.08300209045410156,0.02713699692971347
278,1289,0,1289,0.08325695991516113,0.027119858535799606
279,1294,0,1294,0.08349990844726562,0.0271048383057096
280,1299,0,1299,0.0837411880493164,0.02709156483438269
281,1304,0,1304,0.08400201797485352,0.027079737208532476
282,1309,0,1309,0.0842752456665039,0.027069111072521437
283,1314,0,1314,0.08451128005981445,0.027059487520891812
284,1319,0,1319,0.08475613594055176,0.027050704234744677
285,1324,0,1324,0.08512616157531738,0.027042628400088174
286,1329,0,1329,0.0854790210723877,0.027035151042280582
287,1334,0,1334,0.08572006225585938,0.027028182486778202
288,1339,0,1339,0.08597302436828613,0.02702164871661298
289,1344,0,1344,0.08631706237792969,0.027015488444645724
290,1349,0,1349,0.08655929565429688,0.027009650756288524
291,1354,0,1354,0.08680105209350586,0.027004093208151763
292,1359,0,1359,0.08704519271850586,0.026998780291605278
293,1364,0,1364,0.0873720645904541,0.026993682188861536
294,1369,0,1369,0.08774709701538086,0.02698877376392693
295,1374,0,1374,0.08799886703491211,0.02698403374244541
296,1379,0,1379,0.08823490142822266,0.02697944404371822
297,1384,0,1384,0.0884709358215332,0.026974989235537677
298,1389,0,1389,0.08871603012084961,0.026970656088314917
299,1394,0,1394,0.08900809288024902,0.026966433209633583
300,1399,0,1399,0.08925509452819824,0.026962310744067724
301,1404,0,1404,0.08948707580566406,0.026958280126060077
302,1409,0,1409,0.08972001075744629,0.026954333876020784
303,1414,0,1414,0.08995389938354492,0.026950465431699874
304,1419,0,1419,0.09019207954406738,0.02694666900840237
305,1424,0,1424,0.09042596817016602,0.026942939482835614
306,1429,0,1429,0.09065699577331543,0.026939272296355652
307,1434,0,1434,0.09089207649230957,0.026935663374170762
308,1439,0,1439,0.09112310409545898,0.026932109057697058
309,1444,0,1444,0.09137201309204102,0.026928606047775448
310,1449,0,1449,0.09161114692687988,0.026925151356876686
311,1454,0,1454,0.09184408187866211,0.02692174226876079
312,1459,0,1459,0.09208106994628906,0.026918376304329184
313,1464,0,1464,0.0923151969909668,0.02691505119263516
314,1469,0,1469,0.09255003929138184,0.026911764846197932
315,1474,0,1474,0.09278202056884766,0.026908515339916606
316,1479,0,1479,0.0930180549621582,0.026905300893000823
317,1484,0,1484,0.09324908256530762,0.026902119853435796
318,1489,0,1489,0.09348392486572266,0.02689897068458152
319,1494,0,1494,0.09373903274536133,0.0268958519535733
320,1499,0,1499,0.09398007392883301,0.02689276232124498
321,1504,0,1504,0.0942230224609375,0.026889700533345464
322,1509,0,1509,0.09446120262145996,0.026886665412853502
323,1514,0,1514,0.09469318389892578,0.026883655853229504
324,1519,0,1519,0.09493017196655273,0.02688067081246739
325,1524,0,1524,0.09516310691833496,0.026877709307833716
326,1529,0,1529,0.09539914131164551,0.02687477041119564
327,1534,0,1534,0.09562993049621582,0.02687185324485849
328,1539,0,1539,0.09586596488952637,0.02686895697784225
329,1544,0,1544,0.0960991382598877,0.02686608082253995
330,1549,0,1549,0.09633517265319824,0.026863224031707583
331,1554,0,1554,0.09663510322570801,0.02686038589574371
332,1559,0,1559,0.09688019752502441,0.02685756574022263
333,1564,0,1564,0.09715819358825684,0.02685476292365027
334,1569,0,1569,0.09740996360778809,0.026851976835416062
335,1574,0,1574,0.09771895408630371,0.02684920689391904
336,1579,0,1579,0.09795904159545898,0.026846452544847396
337,1584,0,1584,0.09820318222045898,0.026843713259594996
338,1589,0,1589,0.0984339714050293,0.026840988533800954
339,1594,0,1594,0.09866213798522949,0.026838277885998147
340,1599,0,1599,0.09889101982116699,0.026835580856360765
341,1604,0,1604,0.09911704063415527,0.026832897005540715
342,1609,0,1609,0.09935808181762695,0.026830225913584017
343,1614,0,1614,0.09957218170166016,0.026827567178920646
344,1619,0,1619,0.09979104995727539,0.026824920417420288
345,1624,0,1624,0.100006103515625,0.026822285261509
346,1629,0,1629,0.10022401809692383,0.026819661359340857
347,1634,0,1634,0.10054802894592285,0.026817048374020706
348,1639,0,1639,0.10088706016540527,0.026814445982873455
349,1644,0,1644,0.1011502742767334,0.026811853876756404
350,1649,0,1649,0.1013641357421875,0.026809271759411422
351,1654,0,1654,0.10157418251037598,0.026806699346853872
352,1659,0,1659,0.10178804397583008,0.02680413636679557
353,1664,0,1664,0.10200309753417969,0.026801582558099758
354,1669,0,1669,0.1022179126739502,0.026799037670264887
355,1674,0,1674,0.10242819786071777,0.02679650146293735
356,1679,0,1679,0.10264205932617188,0.02679397370544826
357,1684,0,1684,0.10285401344299316,0.026791454176375653
358,1689,0,1689,0.10306715965270996,0.02678894266312795
359,1694,0,1694,0.10327792167663574,0.026786438961550318
360,1699,0,1699,0.10350990295410156,0.026783942875548833
361,1704,0,1704,0.10372614860534668,0.02678145421673507
362,1709,0,1709,0.10394406318664551,0.02677897280408707
363,1714,0,1714,0.10415911674499512,0.02677649846362761
364,1719,0,1719,0.1044001579284668,0.026774031028117547
365,1724,0,1724,0.10463094711303711,0.02677157033676432
366,1729,0,1729,0.10486698150634766,0.026769116234944292
367,1734,0,1734,0.10509896278381348,0.026766668573937624
368,1739,0,1739,0.10535216331481934,0.02676422721067691
369,1744,0,1744,0.10559606552124023,0.026761792007506058
370,1749,0,1749,0.10584497451782227,0.02675936283195166
371,1754,0,1754,0.10609102249145508,0.026756939556503934
372,1759,0,1759,0.10636115074157715,0.02675452205840843
373,1764,0,1764,0.10659909248352051,0.02675211021946683
374,1769,0,1769,0.106842041015625,0.02674970392584693
375,1774,0,1774,0.10707902908325195,0.026747303067901226
376,1779,0,1779,0.10733413696289062,0.026744907539993354
377,1784,0,1784,0.1075592041015625,0.026742517240333195
378,1789,0,1789,0.10786700248718262,0.026740132070817862
379,1794,0,1794,0.10808706283569336,0.026737751936881195
380,1799,0,1799,0.10831403732299805,0.02673537674734911
381,1804,0,1804,0.10854125022888184,0.026733006414301232
382,1809,0,1809,0.10875415802001953,0.026730640852939185
383,1814,0,1814,0.1089639663696289,0.026728279981459893
384,1819,0,1819,0.10931921005249023,0.02672592372093514
385,1824,0,1824,0.10969424247741699,0.02672357199519573
386,1829,0,1829,0.11034798622131348,0.02672122473072098
387,1834,0,1834,0.1106569766998291,0.026718881856532883
388,1839,0,1839,0.11102986335754395,0.026716543304094717
389,1844,0,1844,0.11139130592346191,0.026714209007214246
390,1849,0,1849,0.11175894737243652,0.026711878901950672
391,1854,0,1854,0.1120150089263916,0.026709552926525867
392,1859,0,1859,0.11223220825195312,0.02670723102123923
393,1864,0,1864,0.11245012283325195,0.026704913128386062
394,1869,0,1869,0.11266493797302246,0.026702599192179582
395,1874,0,1874,0.11288213729858398,0.026700289158676005
396,1879,0,1879,0.11309623718261719,0.02669798297570287
397,1884,0,1884,0.11335206031799316,0.026695680592790236
398,1889,0,1889,0.11356616020202637,0.026693381961105076
399,1894,0,1894,0.11378192901611328,0.026691087033387895
400,1899,0,1899,0.1139979362487793,0.026688795763892353
401,1904,0,1904,0.11441802978515625,0.02668650810832727
402,1909,0,1909,0.11478495597839355,0.026684224023801006
403,1914,0,1914,0.11517715454101562,0.02668194346876809
404,1919,0,1919,0.11541295051574707,0.026679666402978048
405,1924,0,1924,0.115631103515625,0.026677392787426386
406,1929,0,1929,0.11584806442260742,0.026675122584307685
407,1934,0,1934,0.11606407165527344,0.026672855756970097
408,1939,0,1939,0.11628198623657227,0.026670592269872298
409,1944,0,1944,0.1165311336517334,0.026668332088542003
410,1949,0,1949,0.11678719520568848,0.026666075179535707
411,1954,0,1954,0.11700296401977539,0.026663821510400875
412,1959,0,1959,0.11722016334533691,0.026661571049638816
413,1964,0,1964,0.11743617057800293,0.02665932376666963
414,1969,0,1969,0.11765217781066895,0.02665707963179823
415,1974,0,1974,0.11786699295043945,0.02665483861618202
416,1979,0,1979,0.11808514595031738,0.026652600691799342
417,1984,0,1984,0.11830019950866699,0.026650365831419904
418,1989,0,1989,0.11851692199707031,0.026648134008575665
419,1994,0,1994,0.11873197555541992,0.02664590519753334
420,1999,0,1999,0.11894917488098145,0.026643679373267795
421,2004,0,2004,0.11916303634643555,0.026641456511436585
422,2009,0,2009,0.11938023567199707,0.02663923658835528
423,2014,0,2014,0.11964011192321777,0.026637019580974083
424,2019,0,2019,0.11986303329467773,0.026634805466855104
425,2024,0,2024,0.12007498741149902,0.026632594224150576
426,2029,0,2029,0.12028622627258301,0.02663038583158201
427,2034,0,2034,0.12055325508117676,0.026628180268420076
428,2039,0,2039,0.12091517448425293,0.026625977514465153
429,2044,0,2044,0.12112617492675781,0.026623777550028996
430,2049,0,2049,0.12137603759765625,0.026621580355916594
431,2054,0,2054,0.12158608436584473,0.026619385913409222
432,2059,0,2059,0.1217961311340332,0.02661719420424772
433,2064,0,2064,0.12200593948364258,0.026615005210616813
434,2069,0,2069,0.12221622467041016,0.026612818915129566
435,2074,0,2074,0.12242412567138672,0.026610635300812976
436,2079,0,2079,0.1226348876953125,0.026608454351093554
437,2084,0,2084,0.12284612655639648,0.02660627604978385
438,2089,0,2089,0.12305617332458496,0.02660410038106931
439,2094,0,2094,0.12326598167419434,0.026601927329495713
440,2099,0,2099,0.12347793579101562,0.02659975687995707
441,2104,0,2104,0.1236882209777832,0.026597589017683727
442,2109,0,2109,0.12389898300170898,0.02659542372823148
443,2114,0,2114,0.12410688400268555,0.02659326099747031
444,2119,0,2119,0.12431812286376953,0.026591100811574415
445,2124,0,2124,0.12452816963195801,0.026588943157011907
446,2129,0,2129,0.12473797798156738,0.02658678802053512
447,2134,0,2134,0.12494707107543945,0.02658463538917145
448,2139,0,2139,0.12515807151794434,0.026582485250214217
449,2144,0,2144,0.1253669261932373,0.026580337591214375
450,2149,0,2149,0.1255779266357422,0.02657819239997161
451,2154,0,2154,0.12578701972961426,0.026576049664526882
452,2159,0,2159,0.12599706649780273,0.02657390937315442
453,2164,0,2164,0.1262061595916748,0.026571771514354237
454,2169,0,2169,0.12641620635986328,0.026569636076845225
455,2174,0,2174,0.12662696838378906,0.026567503049557878
456,2179,0,2179,0.12683796882629395,0.026565372421627848
457,2184,0,2184,0.1270902156829834,0.02656324418238961
458,2189,0,2189,0.12737298011779785,0.0265611183213699
459,2194,0,2194,0.12758326530456543,0.026558994828282036
460,2199,0,2199,0.1277930736541748,0.026556873693020195
461,2204,0,2204,0.12800312042236328,0.026554754905653514
462,2209,0,2209,0.12821292877197266,0.026552638456421154
463,2214,0,2214,0.12842202186584473,0.026550524335726793
464,2219,0,2219,0.1286330223083496,0.026548412534133762
465,2224,0,2224,0.12884116172790527,0.02654630304236031
466,2229,0,2229,0.12905216217041016,0.026544195851274734
467,2234,0,2234,0.12926101684570312,0.026542090951891143
468,2239,0,2239,0.129472017288208,0.02653998833536492
469,2244,0,2244,0.12968111038208008,0.026537887992988653
470,2249,0,2249,0.12989521026611328,0.026535789916188175
471,2254,0,2254,0.13010406494140625,0.02653369409651847
472,2259,0,2259,0.13031601905822754,0.026531600525660035
473,2264,0,2264,0.13052606582641602,0.026529509195415277
474,2269,0,2269,0.1307392120361328,0.02652742009770482
475,2274,0,2274,0.1309490203857422,0.026525333224564355
476,2279,0,2279,0.13116002082824707,0.02652324856814133
477,2284,0,2284,0.13136911392211914,0.02652116612069147
478,2289,0,2289,0.1315779685974121,0.02651908587457624
479,2294,0,2294,0.13178801536560059,0.026517007822259353
480,2299,0,2299,0.13199710845947266,0.026514931956304406
481,2304,0,2304,0.13220596313476562,0.026512858269371824
482,2309,0,2309,0.13242316246032715,0.026510786754216094
483,2314,0,2314,0.13263297080993652,0.026508717403683574
484,2319,0,2319,0.1328439712524414,0.02650665021070974
485,2324,0,2324,0.13305306434631348,0.026504585168316677
486,2329,0,2329,0.13326311111450195,0.026502522269611042
487,2334,0,2334,0.13347291946411133,0.026500461507781556
488,2339,0,2339,0.1336841583251953,0.02649840287609694
489,2344,0,2344,0.1338951587677002,0.026496346367903743
490,2349,0,2349,0.13410496711730957,0.02649429197662449
491,2354,0,2354,0.13431501388549805,0.026492239695755385
492,2359,0,2359,0.13452506065368652,0.026490189518864688
493,2364,0,2364,0.13474011421203613,0.02648814143959058
494,2369,0,2369,0.13508820533752441,0.026486095451639723
495,2374,0,2374,0.1352980136871338,0.026484051548785338
496,2379,0,2379,0.13550829887390137,0.026482009724865363
497,2384,0,2384,0.13571715354919434,0.026479969973781162
498,2389,0,2389,0.1359269618988037,0.026477932289495715
499,2394,0,2394,0.13613605499267578,0.026475896666032155
500,2399,0,2399,0.13634610176086426,0.026473863097472308
501,2404,0,2404,0.13655495643615723,0.026471831577955345
502,2409,0,2409,0.1367661952972412,0.02646980210167613
503,2414,0,2414,0.13697504997253418,0.026467774662884264
504,2419,0,2419,0.13718914985656738,0.026465749255882277
505,2424,0,2424,0.13739895820617676,0.026463725875025025
506,2429,0,2429,0.13760805130004883,0.02646170451471787
507,2434,0,2434,0.13782215118408203,0.02645968516941583
508,2439,0,2439,0.13803315162658691,0.026457667833622224
509,2444,0,2444,0.1382429599761963,0.02645565250188785
510,2449,0,2449,0.13845229148864746,0.026453639168809513
511,2454,0,2454,0.13866114616394043,0.026451627829029378
512,2459,0,2459,0.1388709545135498,0.026449618477233653
513,2464,0,2464,0.13908123970031738,0.02644761110815171
514,2469,0,2469,0.13929104804992676,0.026445605716555215
515,2474,0,2474,0.13949894905090332,0.026443602297257018
516,2479,0,2479,0.1397092342376709,0.02644160084511053
517,2484,0,2484,0.1399211883544922,0.026439601355008457
518,2489,0,2489,0.14013099670410156,0.026437603821882278
519,2494,0,2494,0.14033913612365723,0.026435608240701403
520,2499,0,2499,0.1405501365661621,0.026433614606472065
521,2504,0,2504,0.14076519012451172,0.026431622914236935
522,2509,0,2509,0.1409749984741211,0.02642963315907422
523,2514,0,2514,0.14118504524230957,0.02642764533609687
524,2519,0,2519,0.14146208763122559,0.02642565944045179
525,2524,0,2524,0.14166998863220215,0.02642367546731944
526,2529,0,2529,0.14188098907470703,0.02642169341191292
527,2534,0,2534,0.14208984375,0.02641971326947734
528,2539,0,2539,0.14230108261108398,0.02641773503528938
529,2544,0,2544,0.14251112937927246,0.026415758704656466
530,2549,0,2549,0.14278006553649902,0.02641378427291618
531,2554,0,2554,0.142988920211792,0.02641181173543577
532,2559,0,2559,0.14323186874389648,0.026409841087611637
533,2564,0,2564,0.1434769630432129,0.026407872324868638
534,2569,0,2569,0.1438281536102295,0.02640590544265961
535,2574,0,2574,0.14410686492919922,0.026403940436464896
536,2579,0,2579,0.14433813095092773,0.02640197730179176
537,2584,0,2584,0.14499616622924805,0.026400016034173954
538,2589,0,2589,0.14522004127502441,0.026398056629171322
539,2594,0,2594,0.14544105529785156,0.026396099082368975
540,2599,0,2599,0.14573216438293457,0.02639414338937742
541,2604,0,2604,0.14604806900024414,0.02639218954583162
542,2609,0,2609,0.14635014533996582,0.026390237547390748
543,2614,0,2614,0.14668607711791992,0.02638828738973782
544,2619,0,2619,0.14694809913635254,0.026386339068579217
545,2624,0,2624,0.14716100692749023,0.026384392579644343
546,2629,0,2629,0.1473710536956787,0.026382447918685048
547,2634,0,2634,0.1475849151611328,0.02638050508147566
548,2639,0,2639,0.14790701866149902,0.026378564063812213
549,2644,0,2644,0.14816927909851074,0.026376624861512234
550,2649,0,2649,0.14838123321533203,0.026374687470414444
551,2654,0,2654,0.1486530303955078,0.026372751886378474
552,2659,0,2659,0.1488969326019287,0.02637081810528436
553,2664,0,2664,0.14915800094604492,0.026368886123032228
554,2669,0,2669,0.149367094039917,0.026366955935542207
555,2674,0,2674,0.14957904815673828,0.02636502753875395
556,2679,0,2679,0.14978814125061035,0.026363100928626298
557,2684,0,2684,0.14999794960021973,0.026361176101137133
558,2689,0,2689,0.1502079963684082,0.026359253052283014
559,2694,0,2694,0.15056610107421875,0.026357331778078835
560,2699,0,2699,0.15079307556152344,0.02635541227455777
561,2704,0,2704,0.15104413032531738,0.026353494537770694
562,2708,0,2708,0.15129709243774414,0.026347427380368393
563,2713,0,2713,0.15150904655456543,0.026337636669157373
564,2718,0,2718,0.1518571376800537,0.026328405932720293
565,2723,0,2723,0.1521461009979248,0.02631967028935862
566,2728,0,2728,0.15235614776611328,0.026311375238442895
567,2733,0,2733,0.15256690979003906,0.02630347473640374
568,2737,0,2737,0.15276503562927246,0.026262561192579876
569,2742,0,2742,0.15302300453186035,0.026249214341562258
570,2747,0,2747,0.15336203575134277,0.026236442330971135
571,2751,0,2751,0.1535630226135254,0.026181753165309973
572,2756,0,2756,0.15377306938171387,0.02616338857172021
573,2760,0,2760,0.15397214889526367,0.026138300729742204
574,2765,0,2765,0.15418410301208496,0.02611297914228619
575,2770,0,2770,0.1544349193572998,0.026088991341809357
576,2774,0,2774,0.1546332836151123,0.026080198983602015
577,2779,0,2779,0.1548452377319336,0.026054616293865192
578,2784,0,2784,0.15505504608154297,0.02603034626098535
579,2789,0,2789,0.15526700019836426,0.026007245165615804
580,2794,0,2794,0.15547609329223633,0.02598519274514427
581,2799,0,2799,0.15568804740905762,0.025964087719451082
582,2804,0,2804,0.1558980941772461,0.025943844224824285
583,2809,0,2809,0.15610909461975098,0.02592438896548446
584,2814,0,2814,0.1563282012939453,0.02590565893300093
585,2819,0,2819,0.156541109085083,0.025887599575849757
586,2824,0,2824,0.1567521095275879,0.025870163326405963
587,2829,0,2829,0.15696406364440918,0.025853308412287637
588,2834,0,2834,0.1574702262878418,0.025836997894360825
589,2838,0,2838,0.1578669548034668,0.025796197509325866
590,2843,0,2843,0.1582779884338379,0.025775271507501994
591,2848,0,2848,0.15862011909484863,0.02575529858029857
592,2853,0,2853,0.1588430404663086,0.025736163103450487
593,2858,0,2858,0.15914583206176758,0.02571777041168842
594,2863,0,2863,0.15942811965942383,0.02570004244014853
595,2868,0,2868,0.1596510410308838,0.02568291431871739
596,2872,0,2872,0.15985918045043945,0.025673464970027565
597,2877,0,2877,0.16008210182189941,0.025655112115057003
598,2882,0,2882,0.16031098365783691,0.025637406933913406
599,2887,0,2887,0.16053295135498047,0.02562026370119641
600,2892,0,2892,0.16076207160949707,0.025603613722957552
601,2896,0,2896,0.16097307205200195,0.025568078524267915
602,2901,0,2901,0.16119384765625,0.025552020766732464
603,2906,0,2906,0.16141605377197266,0.025536320746343186
604,2911,0,2911,0.1616370677947998,0.025520935108218495
605,2915,0,2915,0.1618499755859375,0.025485104732586004
606,2920,0,2920,0.16207003593444824,0.02546748315811752
607,2925,0,2925,0.1622922420501709,0.025450279795337184
608,2929,0,2929,0.16250014305114746,0.025382237621583415
609,2933,0,2933,0.16271615028381348,0.025329646522416996
610,2937,0,2937,0.16292405128479004,0.025251680355841633
611,2941,0,2941,0.16313505172729492,0.025122592022094856
612,2945,0,2945,0.1633460521697998,0.02493707039139349
613,2948,0,2948,0.16358208656311035,0.024672065382057393
614,2951,0,2951,0.16397714614868164,0.024176865697497628
615,2954,0,2954,0.16416406631469727,0.02286491895023242
616,2957,0,2957,0.16434407234191895,0.01957540994443955
617,2960,0,2960,0.16457605361938477,0.010493902593661298
618,2963,0,2963,0.16475510597229004,0.008630247063474409
619,2966,0,2966,0.1649341583251953,0.0046034716202297595
620,2969,0,2969,0.16511297225952148,0.004170566791281395
621,2974,0,2974,0.16533708572387695,0.00413735094653529
622,2979,0,2979,0.165557861328125,0.00410727088756372
623,2984,0,2984,0.16578197479248047,0.004079864350285105
624,2989,0,2989,0.16600322723388672,0.004054751823078806
625,2994,0,2994,0.16622519493103027,0.004031620635477792
626,2999,0,2999,0.16644597053527832,0.00401021212945842
627,3004,0,3004,0.16666793823242188,0.003990311340269254
628,3009,0,3009,0.1668870449066162,0.003971738708239337
629,3014,0,3014,0.16710901260375977,0.003954343426915169
630,3019,0,3019,0.16733002662658691,0.003937998105173719
631,3024,0,3024,0.16755294799804688,0.003922594481937824
632,3029,0,3029,0.16777420043945312,0.003908039982746265
633,3034,0,3034,0.16799616813659668,0.003894254948971312
634,3039,0,3039,0.16821599006652832,0.003881170404259485
635,3044,0,3044,0.16844415664672852,0.0038687262500601283
636,3049,0,3049,0.16866493225097656,0.0038568698040348506
637,3054,0,3054,0.1690349578857422,0.0038455546126943715
638,3059,0,3059,0.16945719718933105,0.0038347394836178595
639,3064,0,3064,0.16974210739135742,0.0038243876937665883
640,3068,0,3068,0.17001914978027344,0.003815870456744126
641,3071,0,3071,0.17022204399108887,0.003610483827256078
642,3075,0,3075,0.17043304443359375,0.0035991043083502283
643,3080,0,3080,0.17070317268371582,0.0035693970748949403
644,3085,0,3085,0.17092609405517578,0.0035434669381683667
645,3090,0,3090,0.17114686965942383,0.003520688493879274
646,3095,0,3095,0.17136907577514648,0.0035005486267242016
647,3100,0,3100,0.17158794403076172,0.003482625943715218
648,3105,0,3105,0.17180895805358887,0.0034665738599559295
649,3110,0,3110,0.17203187942504883,0.0034521067582702907
650,3115,0,3115,0.17225003242492676,0.0034389887062372727
651,3120,0,3120,0.172468900680542,0.003427024282257028
652,3125,0,3125,0.17269110679626465,0.0034160511291992436
653,3130,0,3130,0.17290902137756348,0.0034059339160054064
654,3135,0,3135,0.17312908172607422,0.0033965594424679203
655,3140,0,3140,0.17335009574890137,0.0033878326697430504
656,3145,0,3145,0.1735689640045166,0.0033796734991947846
657,3150,0,3150,0.17378926277160645,0.003372014155543419
658,3155,0,3155,0.1740100383758545,0.0033647970578122833
659,3160,0,3160,0.17422723770141602,0.003357973084068216
660,3165,0,3165,0.17444610595703125,0.0033515001542396817
661,3170,0,3170,0.17467212677001953,0.0033453420700885073
662,3175,0,3175,0.17489004135131836,0.003339467563337093
663,3180,0,3180,0.1751091480255127,0.0033338495125428045
664,3185,0,3185,0.17532896995544434,0.003328464297011369
665,3190,0,3190,0.17554616928100586,0.003323291262216842
666,3195,0,3195,0.1757650375366211,0.003318312276146884
667,3200,0,3200,0.1761009693145752,0.0033135113599613623
668,3205,0,3205,0.17648100852966309,0.003308874379535521
669,3210,0,3210,0.17676210403442383,0.0033043887870133474
670,3215,0,3215,0.1769871711730957,0.003300043403548551
671,3220,0,3220,0.17730021476745605,0.0032958282360608993
672,3225,0,3225,0.17752313613891602,0.0032917343221640057
673,3230,0,3230,0.1777498722076416,0.0032877535984927294
674,3235,0,3235,0.17796921730041504,0.0032838787885240707
675,3240,0,3240,0.17818903923034668,0.0032801033066860684
676,3245,0,3245,0.17841100692749023,0.0032764211761178875
677,3250,0,3250,0.17863011360168457,0.0032728269579059797
678,3255,0,3255,0.1788499355316162,0.0032693156899973592
679,3260,0,3260,0.1790759563446045,0.0032658828342983547
680,3265,0,3265,0.17929601669311523,0.003262524230718055
681,3270,0,3270,0.17951607704162598,0.003259236057122147
682,3275,0,3275,0.17973899841308594,0.0032560147943319065
683,3280,0,3280,0.17995691299438477,0.0032528571954429154
684,3285,0,3285,0.18017816543579102,0.0032497602588533107
685,3290,0,3290,0.18040013313293457,0.0032467212044870386
686,3295,0,3295,0.18062400817871094,0.0032437374527769978
687,3300,0,3300,0.1808490753173828,0.003240806606038762
688,3305,0,3305,0.18107104301452637,0.0032379264319211303
689,3310,0,3310,0.1812891960144043,0.003235094848665643
690,3315,0,3315,0.18150901794433594,0.0032323099119460565
691,3320,0,3320,0.1817309856414795,0.003229569803091499
692,3325,0,3325,0.18195390701293945,0.0032268728185243264
693,3330,0,3330,0.1821751594543457,0.0032242173602670798
694,3335,0,3335,0.18239712715148926,0.0032216019273928046
695,3340,0,3340,0.18261504173278809,0.0032190251083095167
696,3345,0,3345,0.18283414840698242,0.003216485573784139
697,3350,0,3350,0.18305611610412598,0.003213982070623282
698,3355,0,3355,0.1832730770111084,0.0032115134159389092
699,3360,0,3360,0.18349313735961914,0.0032090784919357024
700,3365,0,3365,0.1837139129638672,0.003206676241164824
701,3370,0,3370,0.18393206596374512,0.003204305662195529
702,3375,0,3375,0.18415212631225586,0.0032019658056615893
703,3380,0,3380,0.1843729019165039,0.0031996557706448067
704,3385,0,3385,0.18459200859069824,0.0031973747013621036
705,3390,0,3390,0.18481087684631348,0.0031951217841264677
706,3395,0,3395,0.18503212928771973,0.003192896244555388
707,3400,0,3400,0.18525004386901855,0.0031906973450032765
708,3405,0,3405,0.1854701042175293,0.0031885243821969645
709,3410,0,3410,0.18569111824035645,0.003186376685055593
710,3415,0,3415,0.18590903282165527,0.003184253612678013
711,3420,0,3420,0.18621206283569336,0.0031821545524828854
712,3425,0,3425,0.18643593788146973,0.003180078918487911
713,3430,0,3430,0.18665528297424316,0.0031780261497159823
714,3435,0,3435,0.1868760585784912,0.0031759957087175166
715,3440,0,3440,0.18709802627563477,0.0031739870801989795
716,3445,0,3445,0.1873161792755127,0.003171999769748819
717,3450,0,3450,0.18753600120544434,0.0031700333026526526
718,3455,0,3455,0.1877579689025879,0.003168087222790484
719,3460,0,3460,0.18797516822814941,0.003166161091609344
720,3465,0,3465,0.18819403648376465,0.003164254487165317
721,3470,0,3470,0.1884150505065918,0.0031623670032295084
722,3475,0,3475,0.18863296508789062,0.003160498248453018
723,3480,0,3480,0.18885302543640137,0.003158647845586296
724,3485,0,3485,0.18907809257507324,0.003156815430748837
725,3490,0,3490,0.18929600715637207,0.0031550006527454335
726,3495,0,3495,0.18951702117919922,0.0031532031724254513
727,3500,0,3500,0.18973803520202637,0.0031514226620820724
728,3505,0,3505,0.1899559497833252,0.0031496588048885153
729,3510,0,3510,0.19017601013183594,0.003147911294368614
730,3515,0,3515,0.19039607048034668,0.0031461798338993955
731,3520,0,3520,0.1906139850616455,0.0031444641362432307
732,3525,0,3525,0.19083619117736816,0.0031427639231076635
733,3530,0,3530,0.19105911254882812,0.00314107892473096
734,3535,0,3535,0.19127607345581055,0.003139408879491531
735,3540,0,3540,0.1914961338043213,0.003137753533539861
736,3545,0,3545,0.19176316261291504,0.0031361126404511725
737,3550,0,3550,0.191986083984375,0.0031344859608976043
738,3555,0,3555,0.19220495223999023,0.003132873262338608
739,3560,0,3560,0.19242596626281738,0.003131274318728381
740,3565,0,3565,0.19264507293701172,0.003129688910239209
741,3570,0,3570,0.19286608695983887,0.0031281168229997714
742,3575,0,3575,0.19308805465698242,0.003126557848847383
743,3580,0,3580,0.19330596923828125,0.0031250117850933927
744,3585,0,3585,0.19352483749389648,0.0031234784343008738
745,3590,0,3590,0.19379496574401855,0.0031219576040738698
746,3595,0,3595,0.19401311874389648,0.003120449106857496
747,3600,0,3600,0.19423294067382812,0.003118952759748227
748,3605,0,3605,0.19445490837097168,0.003117468384313773
749,3610,0,3610,0.1946730613708496,0.003115995806422024
750,3615,0,3615,0.19489192962646484,0.003114534856078466
751,3620,0,3620,0.1951138973236084,0.0031130853672715485
752,3625,0,3625,0.19533205032348633,0.0031116471778257354
753,3630,0,3630,0.19555187225341797,0.003110220129261513
754,3635,0,3635,0.19577312469482422,0.0031088040666622345
755,3640,0,3640,0.19599008560180664,0.0031073988385472125
756,3645,0,3645,0.19621014595031738,0.003106004296750858
757,3650,0,3650,0.19643115997314453,0.0031046202963074293
758,3655,0,3655,0.19665002822875977,0.0031032466953411384
759,3660,0,3660,0.1968691349029541,0.0031018833549613157
760,3665,0,3665,0.19708991050720215,0.0031005301391623494
761,3670,0,3670,0.1973259449005127,0.003099186914728139
762,3675,0,3675,0.19755101203918457,0.003097853551140859
763,3680,0,3680,0.19790887832641602,0.003096529920493722
764,3685,0,3685,0.19820904731750488,0.003095215897407651
765,3690,0,3690,0.198472261428833,0.0030939113589515586
766,3695,0,3695,0.1987171173095703,0.00309261618456611
767,3700,0,3700,0.19903826713562012,0.0030913302559907006
768,3705,0,3705,0.19926023483276367,0.003090053457193632
769,3710,0,3710,0.19948315620422363,0.0030887856743051587
770,3715,0,3715,0.1997051239013672,0.0030875267955534306
771,3720,0,3720,0.19992709159851074,0.0030862767112030177
772,3725,0,3725,0.2001481056213379,0.003085035313495962
773,3730,0,3730,0.20037126541137695,0.003083802496595363
774,3735,0,3735,0.2005929946899414,0.0030825781565311013
775,3739,0,3739,0.20080304145812988,0.003080686868196376
776,3742,0,3742,0.2010350227355957,0.002993455443975934
777,3745,0,3745,0.20135116577148438,0.0029495920513499933
778,3749,0,3749,0.20156097412109375,0.002928679202933928
779,3752,0,3752,0.2017519474029541,0.002792985018095797
780,3755,0,3755,0.20193004608154297,0.002149576690520089
781,3758,0,3758,0.20210909843444824,0.0014142980567273971
782,3761,0,3761,0.202286958694458,0.0008118826837333725
783,3764,0,3764,0.20246315002441406,0.0006727181052367112
784,3767,0,3767,0.20264005661010742,0.000335780949150917
785,3770,0,3770,0.20283007621765137,0.0003316562315361246
786,3773,0,3773,0.20300889015197754,0.00019560898696204803
787,3776,0,3776,0.2031872272491455,0.00012995723925561043
788,3779,0,3779,0.2033698558807373,8.960494796511472e-05
789,3782,0,3782,0.20355010032653809,5.557787719045879e-05
790,3785,0,3785,0.20372819900512695,3.4676539081345926e-05
791,3788,0,3788,0.20390605926513672,2.5360310410476905e-05
792,3791,0,3791,0.20412421226501465,1.2610300794019908e-05
793,3794,0,3794,0.20430207252502441,6.963790802223473e-06
794,3797,0,3797,0.20447993278503418,2.563222749667823e-06
795,3800,0,3800,0.20465707778930664,1.245310197458052e-06
796,3803,0,3803,0.204833984375,5.483962478958642e-07
797,3806,0,3806,0.20501112937927246,2.7148522811413574e-07
798,3809,0,3809,0.20518803596496582,1.1099044556167601e-07
799,3812,0,3812,0.20543622970581055,6.396594287354097e-08
800,3815,0,3815,0.2056722640991211,3.96006303485275e-08
801,3818,0,3818,0.20592308044433594,2.21694481391203e-08
802,3821,0,3821,0.20612025260925293,1.1487308165073367e-08
803,3824,0,3824,0.2062971591949463,2.924367806202416e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha0/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.4849853515625e-05,4.387061074692293
200,201,200,401,0.004639863967895508,0.40381594893679745
400,401,400,801,0.009566068649291992,0.18772146832154463
601,602,601,1203,0.014384984970092773,0.12171316930208559
801,802,801,1603,0.018986940383911133,0.09207570470781463
1001,1002,1001,2003,0.02441692352294922,0.07543468087628187
1201,1202,1201,2403,0.03086090087890625,0.06522583375503957
1401,1402,1401,2803,0.03684592247009277,0.05859653621384203
1602,1603,1602,3205,0.04312491416931152,0.05398535261256449
1802,1803,1802,3605,0.04867196083068848,0.050568720173414815
2002,2003,2002,4005,0.05451202392578125,0.0478422859343471
2202,2203,2202,4405,0.060353994369506836,0.0455476036427356
2402,2403,2402,4805,0.06594514846801758,0.043545396617649314
2603,2604,2603,5207,0.07175898551940918,0.041751034903912645
2803,2804,2803,5607,0.0773019790649414,0.040138971290728194
3003,3004,3003,6007,0.08293914794921875,0.038673603472839595
3203,3204,3203,6407,0.08861207962036133,0.037337563217904775
3403,3404,3403,6807,0.09429693222045898,0.036118120569035975
3604,3605,3604,7209,0.1000511646270752,0.03499974829122583
3804,3805,3804,7609,0.10587000846862793,0.03398476792451849
4004,4005,4004,8009,0.1114962100982666,0.033059488662706915
4204,4205,4204,8409,0.11748409271240234,0.032216669653139886
4404,4405,4404,8809,0.12268805503845215,0.03144956322393217
4605,4606,4605,9211,0.12755298614501953,0.03074852389352344
4805,4806,4805,9611,0.13243889808654785,0.030114575566108637
5005,5006,5005,10011,0.13726305961608887,0.02953851197544041
5205,5206,5205,10411,0.1418750286102295,0.029015147922301927
5405,5406,5405,10811,0.1475832462310791,0.02853965450247292
5606,5607,5606,11213,0.15314912796020508,0.028105491621590647
5806,5807,5806,11613,0.1589951515197754,0.027712818646694996
6006,6007,6006,12013,0.16504597663879395,0.02735555365139795
6206,6207,6206,12413,0.17233920097351074,0.027030191666559268
6406,6407,6406,12813,0.1787738800048828,0.026733525004316607
6607,6608,6607,13215,0.18533611297607422,0.02646133298374186
6807,6808,6807,13615,0.19366908073425293,0.026213651724174072
7007,7008,7007,14015,0.20147013664245605,0.025986651714084007
7207,7208,7207,14415,0.21007704734802246,0.025778149602909813
7407,7408,7407,14815,0.21673107147216797,0.02558617470872729
7608,7609,7608,15217,0.2242898941040039,0.025408100367590745
7808,7809,7808,15617,0.23203015327453613,0.02524409689608381
8008,8009,8008,16017,0.23858404159545898,0.025091812293413254
8208,8209,8208,16417,0.24652314186096191,0.024949965111438623
8408,8409,8408,16817,0.2538609504699707,0.024817409200464654
8609,8610,8609,17219,0.2609739303588867,0.02469251854947162
8809,8810,8809,17619,0.26759910583496094,0.024575618954594473
9009,9010,9009,18019,0.2747502326965332,0.024465255731341735
9209,9210,9209,18419,0.2814829349517822,0.02436070462914114
9409,9410,9409,18819,0.2900969982147217,0.02426132140062413
9610,9611,9610,19221,0.2969820499420166,0.024166070134813377
9810,9811,9810,19621,0.302947998046875,0.024075387996634137
10010,10011,10010,20021,0.30895090103149414,0.023988338824701205
10210,10211,10210,20421,0.3144810199737549,0.023904522278487276
10410,10411,10410,20821,0.3206162452697754,0.023823583347133786
10611,10612,10611,21223,0.3268110752105713,0.023744821428552845
10811,10812,10811,21623,0.3336350917816162,0.023668740318461796
11011,11012,11011,22023,0.33917999267578125,0.02359469518416844
11211,11212,11211,22423,0.34412217140197754,0.02352246746056376
11411,11412,11411,22823,0.34891200065612793,0.023451863654645657
11612,11613,11612,23225,0.3544459342956543,0.023382370138534076
11812,11813,11812,23625,0.35936927795410156,0.023314526250139973
12012,12013,12012,24025,0.3648490905761719,0.023247848743321895
12212,12213,12212,24425,0.3694040775299072,0.023182219061697918
12412,12413,12412,24825,0.3742189407348633,0.02311753233229215
12613,12614,12613,25227,0.37912702560424805,0.023053378605362995
12813,12814,12813,25627,0.3838629722595215,0.02299031386559606
13013,13014,13013,26027,0.38857007026672363,0.022927944371611247
13213,13214,13213,26427,0.39339303970336914,0.022866205989388277
13413,13414,13413,26827,0.3978731632232666,0.02280504199824271
13614,13615,13614,27229,0.4027230739593506,0.022744100274303992
13814,13815,13814,27629,0.4074130058288574,0.022683942661489834
14014,14015,14014,28029,0.4123549461364746,0.02262422547421498
14214,14215,14214,28429,0.41718220710754395,0.022564914016596417
14414,14415,14414,28829,0.421766996383667,0.022505977593175366
14615,14616,14615,29231,0.42669105529785156,0.02244709693370252
14815,14816,14815,29631,0.4316699504852295,0.022388833786727257
15015,15016,15015,30031,0.436845064163208,0.022330873103682564
15215,15216,15215,30431,0.4429008960723877,0.02227319606086596
15415,15416,15415,30831,0.44853806495666504,0.022215785988761734
15616,15617,15616,31233,0.45428013801574707,0.022158342942859316
15816,15817,15816,31633,0.46036195755004883,0.022101425360413096
16016,16017,16016,32033,0.4663050174713135,0.0220447352442792
16216,16217,16216,32433,0.4726550579071045,0.02198826231413797
16416,16417,16416,32833,0.47873806953430176,0.021931997448480497
16617,16618,16617,33235,0.4845390319824219,0.02187565271502125
16817,16818,16817,33635,0.4904959201812744,0.02181978153656305
17017,17018,17017,34035,0.4963371753692627,0.021764096706864775
17217,17218,17217,34435,0.5020089149475098,0.021708592540622386
17417,17418,17417,34835,0.506845235824585,0.0216532639756776
17618,17619,17618,35237,0.5114028453826904,0.021597831135916627
17818,17819,17818,35637,0.5159249305725098,0.021542841550900242
18018,18019,18018,36037,0.5204808712005615,0.021488015417575432
18218,18219,18218,36437,0.5249919891357422,0.021433349521662506
18418,18419,18418,36837,0.5295209884643555,0.021378840984042746
18619,18620,18619,37239,0.5340499877929688,0.021324215837783468
18819,18820,18819,37639,0.5386450290679932,0.021270015286245968
19019,19020,19019,38039,0.5432412624359131,0.02121596508857388
19219,19220,19219,38439,0.5480492115020752,0.02116206335984908
19419,19420,19419,38839,0.5525989532470703,0.021108308395570062
19620,19621,19620,39241,0.5572519302368164,0.02105443096440624
19820,19821,19820,39641,0.5617220401763916,0.021000965750531356
20020,20021,20020,40041,0.5661952495574951,0.02094764306622261
20220,20221,20220,40441,0.5708270072937012,0.020894461742532046
20420,20421,20420,40841,0.5753891468048096,0.020841420707800085
20621,20622,20621,41243,0.580035924911499,0.020788254816175942
20821,20822,20821,41643,0.5844860076904297,0.020735492168325317
21021,21022,21021,42043,0.5889220237731934,0.02068286706790136
21221,21222,21221,42443,0.5933558940887451,0.020630378732431474
21421,21422,21421,42843,0.5977859497070312,0.02057802643208026
21622,21623,21622,43245,0.6025340557098389,0.020525548737833847
21822,21823,21822,43645,0.607025146484375,0.020473467171214583
22022,22023,22022,44045,0.6114659309387207,0.02042151970603057
22222,22223,22222,44445,0.6158959865570068,0.020369705769302023
22422,22423,22422,44845,0.6204588413238525,0.020318024816702637
22623,22624,22623,45247,0.6248950958251953,0.020266218918848774
22823,22824,22823,45647,0.6292939186096191,0.020214803058901585
23023,23024,23023,46047,0.6338410377502441,0.02016351868903903
23223,23224,23223,46447,0.6382660865783691,0.020112365350706877
23423,23424,23423,46847,0.6426711082458496,0.020061342601119834
23624,23625,23624,47249,0.6470749378204346,0.02001019587489068
23824,23825,23824,47649,0.6516032218933105,0.01995943367667865
24024,24025,24024,48049,0.6567468643188477,0.019908800815002316
24224,24225,24224,48449,0.6613161563873291,0.019858296894657453
24424,24425,24424,48849,0.6659281253814697,0.01980792152928542
24625,24626,24625,49251,0.6704521179199219,0.019757423425907274
24825,24826,24825,49651,0.675152063369751,0.019707304680306563
25025,25026,25025,50051,0.6798830032348633,0.01965731337301269
25225,25226,25225,50451,0.6842730045318604,0.01960744914472076
25425,25426,25425,50851,0.6885790824890137,0.019557711641248768
25626,25627,25626,51253,0.6930191516876221,0.01950785277432785
25826,25827,25826,51653,0.6981379985809326,0.019458368305263263
26026,26027,26026,52053,0.702549934387207,0.019409009522747787
26226,26227,26226,52453,0.7074248790740967,0.019359776088611527
26426,26427,26426,52853,0.7119240760803223,0.01931066766780371
26627,26628,26627,53255,0.7167232036590576,0.019261439322129204
26827,26828,26827,53655,0.7210819721221924,0.019212580554907842
27027,27028,27027,54055,0.7253780364990234,0.019163845810381056
27227,27228,27227,54455,0.7297439575195312,0.019115234763562167
27427,27428,27427,54855,0.7341310977935791,0.019066747091503262
27628,27629,27628,55257,0.7389450073242188,0.019018140958691903
27828,27829,27828,55657,0.7444350719451904,0.018969899687618447
28028,28029,28028,56057,0.7496130466461182,0.018921780831721528
28228,28229,28228,56457,0.7545750141143799,0.01887378407490503
28428,28429,28428,56857,0.7593221664428711,0.018825909102526496
28629,28630,28629,57259,0.7643072605133057,0.01877791713848351
28829,28830,28829,57659,0.7695810794830322,0.01873028540149359
29029,29030,29029,58059,0.7746810913085938,0.018682774511433065
29229,29230,29229,58459,0.7791268825531006,0.018635384158768097
29429,29430,29429,58859,0.7836101055145264,0.018588114035100085
29630,29631,29630,59261,0.7880859375,0.01854072838290067
29830,29831,29830,59661,0.7925732135772705,0.018493698393667487
30030,30031,30030,60061,0.7970349788665771,0.018446787713109657
30230,30231,30230,60461,0.8015620708465576,0.018399996036982964
30430,30431,30430,60861,0.8062691688537598,0.018353323062002852
30631,30632,30631,61263,0.8107690811157227,0.018306536009909707
30831,30832,30831,61663,0.8153362274169922,0.018260100120819935
31031,31032,31031,62063,0.819770097732544,0.01821378202705017
31231,31232,31231,62463,0.8242220878601074,0.018167581428940004
31431,31432,31431,62863,0.8288900852203369,0.018121498027690162
31632,31633,31632,63265,0.8334949016571045,0.018075301986046007
31832,31833,31832,63665,0.8379511833190918,0.018029452667758666
32032,32033,32032,64065,0.8423850536346436,0.017983719653487926
32232,32233,32232,64465,0.8468079566955566,0.01793810264775641
32432,32433,32432,64865,0.8512461185455322,0.01789260135589033
32633,32634,32633,65267,0.8557019233703613,0.01784698884415227
32833,32834,32833,65667,0.8601250648498535,0.017801718674069218
33033,33034,33033,66067,0.8645439147949219,0.017756563337113212
33233,33234,33233,66467,0.8689661026000977,0.017711522541752723
33433,33434,33433,66867,0.8733890056610107,0.017666595997224765
33634,33635,33634,67269,0.8780450820922852,0.01762155963645188
33834,33835,33834,67669,0.8824450969696045,0.017576861291980734
34034,34035,34034,68069,0.8868131637573242,0.017532276329172997
34234,34235,34234,68469,0.8911421298980713,0.017487804460294142
34434,34435,34434,68869,0.8954920768737793,0.017443445398355236
34635,34636,34635,69271,0.8998062610626221,0.017398977906631388
34835,34836,34835,69671,0.9048850536346436,0.017354844161028966
35035,35036,35035,70071,0.9092929363250732,0.017310822364414544
35235,35236,35235,70471,0.9136319160461426,0.017266912232749683
35435,35436,35435,70871,0.917992115020752,0.01722311348272494
35636,35637,35636,71273,0.9225950241088867,0.017179207672164687
35836,35837,35836,71673,0.9270989894866943,0.017135631391772068
36036,36037,36036,72073,0.9326870441436768,0.01709216564603267
36236,36237,36236,72473,0.9378170967102051,0.01704881015452894
36436,36437,36436,72873,0.9426250457763672,0.017005564637559117
36637,36638,36637,73275,0.9474530220031738,0.016962213412170267
36837,36838,36837,73675,0.9520621299743652,0.016919187554402863
37037,37038,37037,74075,0.957766056060791,0.01687627083494987
37237,37238,37237,74475,0.9623599052429199,0.016833462976953414
37437,37438,37437,74875,0.9673869609832764,0.01679076370426042
37638,37639,37638,75277,0.9717590808868408,0.016747960058273063
37838,37839,37838,75677,0.9762961864471436,0.01670547767002248
38038,38039,38038,76077,0.981774091720581,0.016663103041455164
38238,38239,38238,76477,0.986260175704956,0.016620835899219973
38438,38439,38438,76877,0.9907019138336182,0.016578675970660334
38639,38640,38639,77279,0.995150089263916,0.016536412987113464
38839,38840,38839,77679,0.9995901584625244,0.016494467203376332
39039,39040,39039,78079,1.0051891803741455,0.016452627818143002
39239,39240,39239,78479,1.0096559524536133,0.016410894561520253
39439,39440,39439,78879,1.0146658420562744,0.016369267164299924
39640,39641,39640,79281,1.019242286682129,0.016327538013772902
39840,39841,39840,79681,1.0237832069396973,0.016286122056409003
40040,40041,40040,80081,1.0286250114440918,0.01624481115358313
40240,40241,40240,80481,1.0332369804382324,0.016203605038813754
40440,40441,40440,80881,1.0390000343322754,0.016162503446295776
40641,40642,40641,81283,1.043808937072754,0.016121301385723173
40841,40842,40841,81683,1.0491528511047363,0.016080408562288893
41041,41042,41041,82083,1.054746150970459,0.01603961946641369
41241,41242,41241,82483,1.0603530406951904,0.01599893383498341
41441,41442,41441,82883,1.06557297706604,0.015958351405551734
41642,41643,41642,83285,1.070216178894043,0.015917669777090578
41842,41843,41842,83685,1.0747220516204834,0.015877293479719213
42042,42043,42042,84085,1.079261064529419,0.015837019599695096
42242,42243,42242,84485,1.083773136138916,0.015796847877228442
42442,42443,42442,84885,1.0882740020751953,0.01575677805318848
42643,42644,42643,85287,1.0928170680999756,0.015716610283118767
42843,42844,42843,85687,1.0973281860351562,0.015676743987432174
43043,43044,43043,86087,1.1019790172576904,0.015636978815433716
43243,43244,43243,86487,1.1065618991851807,0.015597314510615549
43443,43444,43443,86887,1.1110661029815674,0.015557750817120401
43644,43645,43644,87289,1.1156229972839355,0.015518090414770347
43844,43845,43844,87689,1.1202342510223389,0.01547872767881359
44044,44045,44044,88089,1.1258690357208252,0.01543946478922811
44244,44245,44244,88489,1.130647897720337,0.015400301492746243
44444,44445,44444,88889,1.1353390216827393,0.015361237536742746
44645,44646,44645,89291,1.1402668952941895,0.015322078093433228
44845,44846,44845,89691,1.1450350284576416,0.015283212556627904
45045,45046,45045,90091,1.149496078491211,0.015244445605011868
45245,45246,45245,90491,1.1541821956634521,0.015205776988516741
45445,45446,45445,90891,1.1587119102478027,0.015167206457708372
45646,45647,45646,91293,1.1631782054901123,0.015128541645713789
45846,45847,45846,91693,1.167625904083252,0.015090167027826827
46046,46047,46046,92093,1.172051191329956,0.015051889749877964
46246,46247,46246,92493,1.1764910221099854,0.015013709564957529
46446,46447,46446,92893,1.1809141635894775,0.014975626226782036
46647,46648,46647,93295,1.186079978942871,0.014937449798305899
46847,46848,46847,93695,1.1916022300720215,0.01489955989843313
47047,47048,47047,94095,1.196099042892456,0.01486176610897657
47247,47248,47247,94495,1.2005841732025146,0.014824068186145274
47447,47448,47447,94895,1.2050130367279053,0.014786465886766815
47648,47649,47648,95297,1.209428071975708,0.01474877167293099
47848,47849,47848,95697,1.2138121128082275,0.014711360368494216
48048,48049,48048,96097,1.2182419300079346,0.014674043960482231
48248,48249,48248,96497,1.2226450443267822,0.014636822208183553
48448,48449,48448,96897,1.2271180152893066,0.01459969487149727
48649,48650,48649,97299,1.231537103652954,0.014562476781344738
48849,48850,48849,97699,1.235931158065796,0.014525538027101903
49049,49050,49049,98099,1.2403271198272705,0.014488692970626776
49249,49250,49249,98499,1.2447359561920166,0.014451941374248307
49449,49450,49449,98899,1.250218152999878,0.014415283000898296
49650,49651,49650,99301,1.254668951034546,0.014378535020408414
49850,49851,49850,99701,1.259140968322754,0.014342062847476583
50050,50051,50050,100101,1.2635550498962402,0.014305683188795841
50250,50251,50250,100501,1.2679929733276367,0.01426939580969725
50450,50451,50450,100901,1.2724058628082275,0.01423320047610703
50651,50652,50651,101303,1.2768869400024414,0.014196916667223903
50851,50852,50851,101703,1.2813119888305664,0.01416090518211448
51051,51052,51051,102103,1.2857341766357422,0.014124985042688823
51251,51252,51251,102503,1.2903552055358887,0.014089156017242099
51451,51452,51451,102903,1.2948310375213623,0.014053417874657293
51652,51653,51652,103305,1.2993299961090088,0.01401759237432987
51852,51853,51852,103705,1.303814172744751,0.01398203575799627
52052,52053,52052,104105,1.308351993560791,0.013946569333539537
52252,52253,52252,104505,1.3128039836883545,0.01391119287218155
52452,52453,52452,104905,1.317249059677124,0.013875906145724603
52653,52654,52653,105307,1.3217051029205322,0.013840533164959378
52853,52854,52853,105707,1.326153039932251,0.013805425671856716
53053,53054,53053,106107,1.3305730819702148,0.013770407231397955
53253,53254,53253,106507,1.335010051727295,0.013735477617694843
53453,53454,53453,106907,1.3394138813018799,0.013700636605431978
53654,53655,53654,107309,1.3439929485321045,0.013665710428357495
53854,53855,53854,107709,1.348466157913208,0.013631046385514035
54054,54055,54054,108109,1.3529560565948486,0.013596470270471511
54254,54255,54254,108509,1.3574330806732178,0.013561981860194845
54454,54455,54454,108909,1.3619630336761475,0.013527580932214706
54655,54656,54655,109311,1.3664422035217285,0.01349309591515787
54855,54856,54855,109711,1.37089204788208,0.013458869721258501
55055,55056,55055,110111,1.3753490447998047,0.0134247303445252
55255,55256,55255,110511,1.3797919750213623,0.013390677564740074
55455,55456,55455,110911,1.384174108505249,0.013356711162243835
55656,55657,55656,111313,1.3891198635101318,0.013322661732818054
55856,55857,55856,111713,1.393604040145874,0.013288867857299037
56056,56057,56056,112113,1.3978321552276611,0.0132551597023399
56256,56257,56256,112513,1.4021391868591309,0.013221537050504332
56456,56457,56456,112913,1.4064390659332275,0.01318799968490764
56657,56658,56657,113315,1.4106919765472412,0.013154380341112314
56857,56858,56857,113715,1.4149410724639893,0.013121013323267651
57057,57058,57057,114115,1.419166088104248,0.013087730943228121
57257,57258,57257,114515,1.42336106300354,0.013054532986303933
57457,57458,57457,114915,1.427612066268921,0.013021419238349846
57658,57659,57658,115317,1.4318199157714844,0.012988224547681317
57858,57859,57858,115717,1.4360721111297607,0.012955278995780355
58058,58059,58058,116117,1.4402642250061035,0.012922417012606286
58258,58259,58258,116517,1.4444708824157715,0.012889638386181117
58458,58459,58458,116917,1.4486780166625977,0.012856942905064533
58659,58660,58659,117319,1.4530551433563232,0.012824167503638267
58859,58860,58859,117719,1.4593489170074463,0.01279163809405452
59059,59060,59059,118119,1.4650249481201172,0.01275919119762313
59259,59260,59259,118519,1.4694271087646484,0.012726826605043765
59459,59460,59459,118919,1.473663091659546,0.012694544107546796
59660,59661,59660,119321,1.4785881042480469,0.01266218269923065
59860,59861,59860,119721,1.4828600883483887,0.01263006417558137
60060,60061,60060,120121,1.4874699115753174,0.012598027122843218
60260,60261,60260,120521,1.4919159412384033,0.012566071334359498
60460,60461,60460,120921,1.49635910987854,0.012534196603997582
60661,60662,60661,121323,1.500723123550415,0.01250224395955597
60861,60862,60861,121723,1.505167007446289,0.012470531131853028
61061,61062,61061,122123,1.5095462799072266,0.012438898745984694
61261,61262,61261,122523,1.5138940811157227,0.012407346597904542
61461,61462,61461,122923,1.5182502269744873,0.012375874484083775
61662,61663,61662,123325,1.5226280689239502,0.012344325440332713
61862,61863,61862,123725,1.526975154876709,0.012313013184143793
62062,62063,62062,124125,1.5313341617584229,0.012281780353711453
62262,62263,62262,124525,1.5356709957122803,0.012250626747566594
62462,62463,62462,124925,1.5400030612945557,0.012219552164751285
62663,62664,62663,125327,1.545685052871704,0.012188401623724084
62863,62864,62863,125727,1.5500500202178955,0.01215748487934457
63063,63064,63063,126127,1.5544118881225586,0.012126646557477949
63263,63264,63263,126527,1.558772087097168,0.01209588645919991
63463,63464,63463,126927,1.5631248950958252,0.01206520438609078
63664,63665,63664,127329,1.567528247833252,0.012034447314214212
63864,63865,63864,127729,1.5718870162963867,0.012003921085849887
64064,64065,64064,128129,1.5762500762939453,0.011973472289426836
64264,64265,64264,128529,1.580604076385498,0.01194310072853357
64464,64465,64464,128929,1.584834098815918,0.011912806207256604
64665,64666,64665,129331,1.589043140411377,0.011882437634537609
64865,64866,64865,129731,1.5931921005249023,0.011852296989497092
65065,65066,65065,130131,1.5973520278930664,0.011822232798338432
65265,65266,65265,130531,1.6015799045562744,0.011792244867131
65465,65466,65465,130931,1.6061842441558838,0.011762333002436004
65666,65667,65666,131333,1.6103579998016357,0.011732348021658632
65866,65867,65866,131733,1.6144790649414062,0.011702588089556416
66066,66067,66066,132133,1.6186530590057373,0.011672903645630754
66266,66267,66266,132533,1.6227738857269287,0.01164329449840049
66466,66467,66466,132933,1.626889944076538,0.011613760456870287
66667,66668,66667,133335,1.6311299800872803,0.01158415422280255
66867,66868,66867,133735,1.635815143585205,0.011554770194772038
67067,67068,67067,134135,1.6405069828033447,0.011525460701410733
67267,67268,67267,134535,1.6447300910949707,0.011496225553656161
67467,67468,67467,134935,1.648906946182251,0.011467064562925493
67668,67669,67668,135337,1.6538410186767578,0.011437832291536717
67868,67869,67868,135737,1.6589951515197754,0.011408819419453108
68068,68069,68068,136137,1.663304090499878,0.011379880140575388
68268,68269,68268,136537,1.6675770282745361,0.011351014268229114
68468,68469,68468,136937,1.6717760562896729,0.01132222161621349
68669,68670,68669,137339,1.676020860671997,0.011293358583901018
68869,68870,68869,137739,1.6802289485931396,0.011264712179614122
69069,69070,69069,138139,1.6845300197601318,0.011236138438961521
69269,69270,69269,138539,1.6888511180877686,0.011207637177626852
69469,69470,69469,138939,1.6942031383514404,0.011179208211761124
69670,69671,69670,139341,1.698655128479004,0.011150709754587151
69870,69871,69870,139741,1.703038215637207,0.011122425189163782
70070,70071,70070,140141,1.70849609375,0.01109421236954484
70270,70271,70270,140541,1.7140440940856934,0.011066071113742013
70470,70471,70470,140941,1.7197060585021973,0.011038001240228575
70671,70672,70671,141343,1.7246649265289307,0.01100986275316647
70871,70872,70871,141743,1.7292211055755615,0.010981935456142532
71071,71072,71071,142143,1.7337660789489746,0.010954078998686417
71271,71272,71271,142543,1.7386860847473145,0.010926293201108531
71471,71472,71471,142943,1.7439351081848145,0.010898577884175052
71672,71673,71672,143345,1.7487220764160156,0.010870794820365333
71872,71873,71872,143745,1.7543280124664307,0.0108432202790072
72072,72073,72072,144145,1.7614240646362305,0.01081571568242712
72272,72273,72272,144545,1.7672638893127441,0.010788280853205224
72472,72473,72472,144945,1.7727782726287842,0.010760915614371648
72673,72674,72673,145347,1.778320074081421,0.010733483484387142
72873,72874,72873,145747,1.7840921878814697,0.010706257242962484
73073,73074,73073,146147,1.7896850109100342,0.010679100062828434
73273,73274,73273,146547,1.7951562404632568,0.01065201176880613
73473,73474,73473,146947,1.800079107284546,0.010624992186161093
73674,73675,73674,147349,1.8047630786895752,0.010597906557281505
73874,73875,73874,147749,1.8094439506530762,0.01057102421633934
74074,74075,74074,148149,1.8144240379333496,0.010544210064359861
74274,74275,74274,148549,1.8190429210662842,0.010517463928376887
74474,74475,74474,148949,1.8237311840057373,0.010490785635863056
74675,74676,74675,149351,1.8287551403045654,0.010464042131358842
74875,74876,74875,149751,1.8333821296691895,0.010437499347018535
75075,75076,75075,150151,1.837947130203247,0.010411023890331533
75275,75276,75275,150551,1.8426799774169922,0.010384615590516429
75475,75476,75475,150951,1.8472192287445068,0.01035827427722511
75676,75677,75676,151353,1.8517742156982422,0.010331868575649987
75876,75877,75876,151753,1.8564770221710205,0.010305661058899476
76076,76077,76076,152153,1.8613018989562988,0.01027952001937224
76276,76277,76276,152553,1.8660099506378174,0.010253445288444088
76476,76477,76476,152953,1.870615005493164,0.010227436697918604
76677,76678,76677,153355,1.8752970695495605,0.01020136453241153
76877,76878,76877,153755,1.8799800872802734,0.010175488048414078
77077,77078,77077,154155,1.884425163269043,0.010149677201951911
77277,77278,77277,154555,1.8896920680999756,0.010123931826530708
77477,77478,77477,154955,1.8942430019378662,0.01009825175607857
77678,77679,77678,155357,1.8987770080566406,0.010072508913674031
77878,77879,77878,155757,1.9033520221710205,0.010046959281084143
78078,78079,78078,156157,1.9080009460449219,0.010021474456947755
78278,78279,78278,156557,1.9126639366149902,0.00999605427687362
78478,78479,78478,156957,1.9171559810638428,0.009970698576887533
78679,78680,78679,157359,1.9216229915618896,0.009945280897834979
78879,78880,78879,157759,1.9262380599975586,0.00992005398812255
79079,79080,79079,158159,1.9307711124420166,0.009894891068254181
79279,79280,79279,158559,1.9362010955810547,0.009869791975915053
79479,79480,79479,158959,1.9406070709228516,0.009844756549202152
79680,79681,79680,159361,1.945024013519287,0.0098196599262937
79880,79881,79880,159761,1.9494309425354004,0.009794751663076999
80080,80081,80080,160161,1.9538369178771973,0.009769906581434942
80280,80281,80280,160561,1.958456039428711,0.009745124521102926
80480,80481,80480,160961,1.962989091873169,0.009720405322222984
80681,80682,80681,161363,1.9674978256225586,0.009695625700129735
80881,80882,80881,161763,1.9719021320343018,0.009671032058516674
81081,81082,81081,162163,1.9772090911865234,0.009646500800418244
81281,81282,81281,162563,1.9821500778198242,0.009622031767594248
81481,81482,81481,162963,1.9866971969604492,0.00959762480220585
81682,81683,81682,163365,1.9911441802978516,0.009573158176822716
81882,81883,81882,163765,1.995671033859253,0.00954887518276047
82082,82083,82082,164165,2.000185012817383,0.009524653784233334
82282,82283,82282,164565,2.0047049522399902,0.009500493824999873
82482,82483,82482,164965,2.0095322132110596,0.009476395149214984
82683,82684,82683,165367,2.014035224914551,0.009452237567013466
82883,82884,82883,165767,2.0185141563415527,0.00942826129664634
83083,83084,83083,166167,2.0229952335357666,0.009404345843787973
83283,83284,83283,166567,2.027616024017334,0.009380491054170353
83483,83484,83483,166967,2.032104253768921,0.009356696773916966
83684,83685,83684,167369,2.0370590686798096,0.009332844331306532
83884,83885,83884,167769,2.041511058807373,0.009309170910341929
84084,84085,84084,168169,2.0462749004364014,0.009285557538687048
84284,84285,84284,168569,2.0510239601135254,0.00926200406402262
84484,84485,84484,168969,2.055549144744873,0.00923851033441562
84685,84686,84685,169371,2.0600271224975586,0.009214959177112767
84885,84886,84885,169771,2.0646162033081055,0.009191584780195008
85085,85086,85085,170171,2.069549083709717,0.009168269674091326
85285,85286,85285,170571,2.0739681720733643,0.009145013708406362
85485,85486,85485,170971,2.0783820152282715,0.009121816733126262
85686,85687,85686,171373,2.0832738876342773,0.009098563055531797
85886,85887,85886,171773,2.08787202835083,0.009075483905624149
86086,86087,86086,172173,2.092331886291504,0.009052463297615594
86286,86287,86286,172573,2.097454071044922,0.009029501083010509
86486,86487,86486,172973,2.1019480228424072,0.009006597113689825
86687,86688,86687,173375,2.1066689491271973,0.008983637158273886
86887,86888,86887,173775,2.1120030879974365,0.008960849526048196
87087,87088,87087,174175,2.1173322200775146,0.008938119696266369
87287,87288,87287,174575,2.122162103652954,0.008915447522308394
87487,87488,87487,174975,2.1271259784698486,0.008892832857926216
87688,87689,87688,175377,2.1324288845062256,0.008870162914621072
87888,87889,87888,175777,2.1372158527374268,0.008847663117855108
88088,88089,88088,176177,2.142331123352051,0.008825220393417968
88288,88289,88288,176577,2.1470320224761963,0.008802834596541655
88488,88489,88488,176977,2.1516940593719482,0.008780505582825329
88689,88690,88689,177379,2.1576480865478516,0.008758121988425946
88889,88890,88889,177779,2.162445068359375,0.008735906391408432
89089,89090,89089,178179,2.170429229736328,0.00871374714582693
89289,89290,89289,178579,2.1763408184051514,0.008691644108742054
89489,89490,89489,178979,2.181994915008545,0.008669597137576925
89690,89691,89690,179381,2.187751054763794,0.008647496275149014
89890,89891,89890,179781,2.193161964416504,0.008625561288092052
90090,90091,90090,180181,2.1979870796203613,0.008603681940684067
90290,90291,90290,180581,2.202620029449463,0.008581858091791126
90490,90491,90490,180981,2.207059144973755,0.008560089600637352
90691,90692,90691,181383,2.211686134338379,0.00853826789893286
90891,90892,90891,181783,2.2162270545959473,0.008516609977392021
91091,91092,91091,182183,2.220734119415283,0.008495006992703832
91291,91292,91291,182583,2.225343942642212,0.00847345880551707
91491,91492,91491,182983,2.229825019836426,0.008451965276834023
91692,91693,91692,183385,2.2343380451202393,0.008430419209714088
91892,91893,91892,183785,2.2388479709625244,0.008409034854015509
92092,92093,92092,184185,2.243351936340332,0.008387704741250472
92292,92293,92292,184585,2.2479851245880127,0.008366428733827905
92492,92493,92492,184985,2.2525339126586914,0.00834520669450577
92693,92694,92693,185387,2.2571089267730713,0.00832393278037102
92893,92894,92893,185787,2.2617199420928955,0.008302818535046046
93093,93094,93093,186187,2.2664201259613037,0.008281757847500452
93293,93294,93293,186587,2.2709851264953613,0.008260750581881172
93493,93494,93493,186987,2.2755119800567627,0.008239796602679698
93694,93695,93694,187389,2.280048131942749,0.008218791403907525
93894,93895,93894,187789,2.2845520973205566,0.008197943857134187
94094,94095,94094,188189,2.2889561653137207,0.008177149191640472
94294,94295,94294,188589,2.2934298515319824,0.008156407273289274
94494,94495,94494,188989,2.29830002784729,0.008135717968283742
94695,94696,94695,189391,2.3027591705322266,0.008114978090672851
94895,94896,94895,189791,2.3073971271514893,0.008094393873724655
95095,95096,95095,190191,2.311850070953369,0.008073861870101326
95295,95296,95295,190591,2.316822052001953,0.008053381947360104
95495,95496,95495,190991,2.321263074874878,0.008032953973394047
95696,95697,95696,191393,2.325801134109497,0.008012476065616076
95896,95897,95896,191793,2.3302299976348877,0.007992151852317662
96096,96097,96096,192193,2.3348982334136963,0.00797187919282643
96296,96297,96296,192593,2.339334011077881,0.00795165795637253
96496,96497,96496,192993,2.3437511920928955,0.007931488012517734
96697,96698,96697,193395,2.3483200073242188,0.007911268765575635
96897,96898,96897,193795,2.3527660369873047,0.007891201271765257
97097,97098,97097,194195,2.357196092605591,0.00787118468057487
97297,97298,97297,194595,2.3619072437286377,0.007851218862886417
97497,97498,97497,194995,2.36635422706604,0.007831303689909315
97698,97699,97698,195397,2.370897054672241,0.007811339836602728
97898,97899,97898,195797,2.375274181365967,0.007791525819601563
98098,98099,98098,196197,2.3796262741088867,0.007771762062258557
98298,98299,98298,196597,2.384125232696533,0.007752048437086452
98498,98499,98498,196997,2.388500213623047,0.007732384816921514
98699,98700,98699,197399,2.3931009769439697,0.00771267313131878
98899,98900,98899,197799,2.3975861072540283,0.007693109389407008
99099,99100,99099,198199,2.402040958404541,0.007673595272312884
99299,99300,99299,198599,2.4065818786621094,0.007654130654159521
99499,99500,99499,198999,2.410975217819214,0.007634715409389333
99700,99701,99700,199401,2.415682077407837,0.007615252706306204
99900,99901,99900,199801,2.4202122688293457,0.007595936078205624
100100,100101,100100,200201,2.4245541095733643,0.007576668448100985
100300,100301,100300,200601,2.43087100982666,0.007557449691705395
100501,100502,100501,201003,2.4354331493377686,0.007538183957289869
100701,100702,100701,201403,2.4399569034576416,0.007519062819532193
100901,100902,100901,201803,2.4445149898529053,0.007499990183895353
101101,101102,101101,202203,2.448895215988159,0.007480965927350294
101301,101302,101301,202603,2.453577995300293,0.007461989927179993
101502,101503,101502,203005,2.458428144454956,0.007442967542379198
101702,101703,101702,203405,2.4629878997802734,0.007424087927804905
101902,101903,101902,203805,2.467694044113159,0.007405256202710798
102102,102103,102102,204205,2.47290301322937,0.0073864722456217806
102302,102303,102302,204605,2.4774739742279053,0.007367735935370928
102503,102504,102503,205007,2.4820761680603027,0.007348953826383767
102703,102704,102703,205407,2.486721992492676,0.007330312684261829
102903,102904,102903,205807,2.491117000579834,0.007311718826717828
103103,103104,103103,206207,2.4954750537872314,0.00729317213381102
103303,103304,103303,206607,2.5003280639648438,0.0072746724859049225
103504,103505,103504,207009,2.5048270225524902,0.00725612761775619
103704,103705,103704,207409,2.509537935256958,0.007237721935890049
103904,103905,103904,207809,2.514482021331787,0.007219362941340172
104104,104105,104104,208209,2.5191001892089844,0.007201050515680893
104304,104305,104304,208609,2.5236289501190186,0.007182784540786898
104505,104506,104505,209011,2.5281598567962646,0.0071644739168368115
104705,104706,104705,209411,2.532650947570801,0.007146300721077559
104905,104906,104905,209811,2.5370569229125977,0.007128173622917085
105105,105106,105105,210211,2.541674852371216,0.0071100925054255635
105305,105306,105305,210611,2.5462141036987305,0.00709205725196978
105506,105507,105506,211013,2.5506670475006104,0.007073977913429696
105706,105707,105706,211413,2.555239200592041,0.007056034267195547
105906,105907,105906,211813,2.559953212738037,0.00703813613629158
106106,106107,106106,212213,2.568120002746582,0.007020283405264846
106306,106307,106306,212613,2.573618173599243,0.007002475958955426
106507,106508,106507,213015,2.578350067138672,0.006984624984409787
106707,106708,106707,213415,2.583627939224243,0.006966907988211606
106907,106908,106907,213815,2.588456153869629,0.006949235932429703
107107,107108,107107,214215,2.593257188796997,0.006931608703069472
107307,107308,107307,214615,2.598057270050049,0.006914026186425605
107508,107509,107508,215017,2.6026699542999268,0.006896400691360003
107708,107709,107708,215417,2.607964038848877,0.006878907482332652
107908,107909,107908,215817,2.612884998321533,0.006861458646069543
108108,108109,108108,216217,2.6201488971710205,0.006844054070016028
108308,108309,108308,216617,2.6296989917755127,0.006826693641902931
108509,108510,108509,217019,2.635322093963623,0.006809290778237789
108709,108710,108709,217419,2.6412599086761475,0.00679201852967759
108909,108910,108909,217819,2.6479599475860596,0.006774790093399799
109109,109110,109109,218219,2.6549670696258545,0.006757605358271387
109309,109310,109309,218619,2.6624810695648193,0.00674046421344134
109510,109511,109510,219021,2.668572187423706,0.00672328116907173
109710,109711,109710,219421,2.675765037536621,0.006706227089979789
109910,109911,109910,219821,2.6813700199127197,0.006689216269767864
110110,110111,110110,220221,2.6870241165161133,0.006672248598706794
110310,110311,110310,220621,2.6930012702941895,0.006655323967345684
110511,110512,110511,221023,2.6986629962921143,0.0066383579656871085
110711,110712,110711,221423,2.7042269706726074,0.006621519300318119
110911,110912,110911,221823,2.709254026412964,0.00660472334741702
111111,111112,111111,222223,2.7139408588409424,0.0065879699986406
111311,111312,111311,222623,2.718528985977173,0.006571259145920513
111512,111513,111512,223025,2.7232460975646973,0.0065545074454599886
111712,111713,111712,223425,2.728031873703003,0.006537881472877161
111912,111913,111912,223825,2.7329180240631104,0.006521297673251863
112112,112113,112112,224225,2.7375340461730957,0.006504755939609424
112312,112313,112312,224625,2.7422120571136475,0.00648825616524653
112513,112514,112513,225027,2.746751070022583,0.00647171605909978
112713,112714,112713,225427,2.753690004348755,0.006455300092734991
112913,112914,112913,225827,2.7589569091796875,0.006438925766632075
113113,113114,113113,226227,2.764644145965576,0.006422592975167617
113313,113314,113313,226627,2.7728569507598877,0.006406301612986043
113514,113515,113514,227029,2.778931140899658,0.006389970428460015
113714,113715,113714,227429,2.7846460342407227,0.006373761815679773
113914,113915,113914,227829,2.7903661727905273,0.006357594317194347
114114,114115,114114,228229,2.7959132194519043,0.006341467828714488
114314,114315,114314,228629,2.801302909851074,0.006325382246215377
114515,114516,114515,229031,2.8061470985412598,0.006309257344376332
114715,114716,114715,229431,2.8106679916381836,0.006293253466053127
114915,114916,114915,229831,2.8151352405548096,0.0062772901827013025
115115,115116,115115,230231,2.819669008255005,0.006261367391348863
115315,115316,115315,230631,2.8242039680480957,0.006245484989284952
115516,115517,115516,231033,2.828943967819214,0.006229563764532147
115716,115717,115716,231433,2.8334319591522217,0.00621376203462126
115916,115917,115916,231833,2.838203191757202,0.006198000386917952
116116,116117,116116,232233,2.8429200649261475,0.0061822787197509405
116316,116317,116316,232633,2.8475639820098877,0.00616659693170671
116517,116518,116517,233035,2.85209584236145,0.006150876811351268
116717,116718,116717,233435,2.856610059738159,0.006135274676472807
116917,116918,116917,233835,2.86125111579895,0.006119712117515022
117117,117118,117117,234235,2.8657288551330566,0.00610418903409079
117317,117318,117317,234635,2.870225191116333,0.006088705326067621
117518,117519,117518,235037,2.8747270107269287,0.0060731837699168865
117718,117719,117718,235437,2.8796420097351074,0.0060577787089433
117918,117919,117918,235837,2.8842310905456543,0.006042412723998459
118118,118119,118118,236237,2.888791084289551,0.006027085715963259
118318,118319,118318,236637,2.8935799598693848,0.006011797585969998
118519,118520,118519,237039,2.897994041442871,0.005996472085916947
118719,118720,118719,237439,2.902467966079712,0.0059812616095655515
118919,118920,118919,237839,2.907644033432007,0.005966089715665233
119119,119120,119119,238239,2.9121201038360596,0.005950956306348861
119319,119320,119319,238639,2.916670083999634,0.005935861283997545
119520,119521,119520,239041,2.9215641021728516,0.005920729363615683
119720,119721,119720,239441,2.9260220527648926,0.005905711014046461
119920,119921,119920,239841,2.930438995361328,0.005890730759585137
120120,120121,120120,240241,2.9348111152648926,0.005875788503600753
120320,120321,120320,240641,2.9392318725585938,0.005860884149707467
120521,120522,120521,241043,2.9436440467834473,0.005845943363850492
120721,120722,120721,241443,2.9479920864105225,0.0058311147142689635
120921,120922,120921,241843,2.952345132827759,0.005816323678607846
121121,121122,121121,242243,2.9569661617279053,0.0058015701614567644
121321,121322,121321,242643,2.9613301753997803,0.005786854067647373
121522,121523,121522,243045,2.9661879539489746,0.005772102002054286
121722,121723,121722,243445,2.970616102218628,0.005757460656319332
121922,121923,121922,243845,2.975037097930908,0.005742856449395282
122122,122123,122122,244245,2.9794511795043945,0.005728289287076932
122322,122323,122322,244645,2.984351873397827,0.005713759075398043
122523,122524,122523,245047,2.9888739585876465,0.005699193346302701
122723,122724,122723,245447,2.993381977081299,0.005684736938539269
122923,122924,122923,245847,2.998181104660034,0.005670317200478544
123123,123124,123123,246247,3.0026040077209473,0.005655934039105154
123323,123324,123323,246647,3.0071699619293213,0.005641587361639771
123524,123525,123524,247049,3.0119762420654297,0.005627205615386064
123724,123725,123724,247449,3.0163869857788086,0.005612931809603111
123924,123925,123924,247849,3.0208029747009277,0.005598694210339938
124124,124125,124124,248249,3.0262110233306885,0.005584492725756176
124324,124325,124324,248649,3.030644178390503,0.005570327264244377
124525,124526,124525,249051,3.035069227218628,0.005556127176905643
124725,124726,124725,249451,3.0395660400390625,0.00554203366661847
124925,124926,124925,249851,3.0446109771728516,0.005527975905518786
125125,125126,125125,250251,3.049086093902588,0.005513953802926247
125325,125326,125325,250651,3.0535941123962402,0.005499967268390555
125526,125527,125526,251053,3.058664083480835,0.005485946545394132
125726,125727,125726,251453,3.0630991458892822,0.0054720310532517195
125926,125927,125926,251853,3.0675549507141113,0.005458150858741152
126126,126127,126126,252253,3.0722970962524414,0.00544430587232754
126326,126327,126326,252653,3.0767650604248047,0.005430496004702983
126527,126528,126527,253055,3.081233024597168,0.005416652380459474
126727,126728,126727,253455,3.0879158973693848,0.00540291265787657
126927,126928,126927,253855,3.0934791564941406,0.005389207787073566
127127,127128,127127,254255,3.098233938217163,0.005375537679646487
127327,127328,127327,254655,3.103893995285034,0.005361902247415541
127528,127529,127528,255057,3.1098270416259766,0.005348233484952717
127728,127729,127728,255457,3.1144580841064453,0.005334667311746366
127928,127929,127928,255857,3.1198818683624268,0.005321135550099645
128128,128129,128128,256257,3.1251308917999268,0.005307638112725171
128328,128329,128328,256657,3.12985897064209,0.0052941749125570295
128529,128530,128529,257059,3.1359269618988037,0.005280678803158308
128729,128730,128729,257459,3.141576051712036,0.005267283987189191
128929,128930,128929,257859,3.1464109420776367,0.005253923148119931
129129,129130,129129,258259,3.151136875152588,0.005240596199765714
129329,129330,129329,258659,3.1572201251983643,0.005227303056160358
129530,129531,129530,259061,3.162796974182129,0.005213977419007919
129730,129731,129730,259461,3.167579174041748,0.00520075179582609
129930,129931,129930,259861,3.1720900535583496,0.0051875597203746545
130130,130131,130130,260261,3.1775569915771484,0.005174401107557362
130330,130331,130330,260661,3.1819519996643066,0.005161275872493922
130531,130532,130531,261063,3.1864590644836426,0.0051481185543163395
130731,130732,130731,261463,3.190991163253784,0.00513505998681155
130931,130932,130931,261863,3.195528030395508,0.005122034543288542
131131,131132,131131,262263,3.200019121170044,0.005109042139725998
131331,131332,131331,262663,3.20540714263916,0.005096082692315734
131532,131533,131532,263065,3.210055112838745,0.005083091567040063
131732,131733,131732,263465,3.214607000350952,0.005070197945096265
131932,131933,131932,263865,3.219223976135254,0.005057337028738131
132132,132133,132132,264265,3.2241640090942383,0.005044508735005668
132332,132333,132332,264665,3.22868013381958,0.005031712981149237
132533,132534,132533,265067,3.2332651615142822,0.005018885949557319
132733,132734,132733,265467,3.238084077835083,0.0050061551897117975
132933,132934,132933,265867,3.24259614944458,0.004993456722340708
133133,133134,133133,266267,3.247114896774292,0.004980790465531935
133333,133334,133333,266667,3.2516610622406006,0.004968156337581089
133534,133535,133534,267069,3.2561869621276855,0.004955491326970448
133734,133735,133734,267469,3.260715961456299,0.004942921372077208
133934,133935,133934,267869,3.265350103378296,0.004930383301765281
134134,134135,134134,268269,3.2699639797210693,0.004917877035157156
134334,134335,134334,268669,3.274613857269287,0.004905402491580428
134535,134536,134535,269071,3.2791242599487305,0.004892897455429441
134735,134736,134735,269471,3.2837259769439697,0.004880486274326736
134935,134936,134935,269871,3.2880759239196777,0.0048681065750643526
135135,135136,135135,270271,3.2924599647521973,0.004855758277786337
135335,135336,135335,270671,3.2968008518218994,0.004843441302839373
135536,135537,135536,271073,3.3011679649353027,0.004831094220476361
135736,135737,135736,271473,3.3056528568267822,0.004818839807658439
135936,135937,135936,271873,3.3110859394073486,0.004806616479026973
136136,136137,136136,272273,3.3157169818878174,0.004794424155734727
136336,136337,136336,272673,3.320298194885254,0.004782262759134454
136537,136538,136537,273075,3.3253660202026367,0.004770071635411346
136737,136738,136737,273475,3.329951286315918,0.004757972010704472
136937,136938,136937,273875,3.3344669342041016,0.004745903077553035
137137,137138,137137,274275,3.3388898372650146,0.004733864758105729
137337,137338,137337,274675,3.343325138092041,0.004721856974708722
137538,137539,137538,275077,3.3477742671966553,0.0047098198396785425
137738,137739,137738,275477,3.3523099422454834,0.004697873047920935
137938,137939,137938,275877,3.3567872047424316,0.004685956560047129
138138,138139,138138,276277,3.3612220287323,0.004674070299189218
138338,138339,138338,276677,3.365654945373535,0.004662214188674224
138539,138540,138539,277079,3.3701019287109375,0.004650329097272837
138739,138740,138739,277479,3.3745131492614746,0.004638533207998814
138939,138940,138939,277879,3.378941059112549,0.0046267672398337765
139139,139140,139139,278279,3.3838372230529785,0.004615031116880701
139339,139340,139339,278679,3.388705015182495,0.004603324763435134
139540,139541,139540,279081,3.3936879634857178,0.004591589795166921
139740,139741,139740,279481,3.3983170986175537,0.004579942902294908
139940,139941,139940,279881,3.4027931690216064,0.00456832555259194
140140,140141,140140,280281,3.4073169231414795,0.0045567376711197
140340,140341,140340,280681,3.411733865737915,0.004545179183129904
140541,140542,140541,281083,3.416163921356201,0.004533592441757457
140741,140742,140741,281483,3.4205589294433594,0.004522092663282006
140941,140942,140941,281883,3.4249560832977295,0.004510622054809551
141141,141142,141141,282283,3.4293742179870605,0.004499180542348242
141341,141342,141341,282683,3.4338221549987793,0.0044877680520940605
141542,141543,141542,283085,3.438246011734009,0.004476327665331723
141742,141743,141742,283485,3.4426400661468506,0.004464973143019432
141942,141943,141942,283885,3.4470582008361816,0.004453647422257546
142142,142143,142142,284285,3.4514620304107666,0.004442350429988914
142342,142343,142342,284685,3.455867052078247,0.004431082093341641
142543,142544,142543,285087,3.4603209495544434,0.004419786212552994
142743,142744,142743,285487,3.467211961746216,0.004408575111642157
142943,142944,142943,285887,3.4716639518737793,0.0043973924484831915
143143,143144,143143,286287,3.476091146469116,0.004386238150941722
143343,143344,143343,286687,3.4805328845977783,0.004375112147066345
143544,143545,143544,287089,3.4849929809570312,0.00436395894696553
143744,143745,143744,287489,3.489423990249634,0.004352889455869734
143944,143945,143944,287889,3.4938652515411377,0.00434184804332246
144144,144145,144144,288289,3.4983022212982178,0.004330834638100505
144344,144345,144344,288689,3.502737045288086,0.004319849169161288
144545,144546,144545,289091,3.507201910018921,0.00430883684751801
144745,144746,144745,289491,3.511641025543213,0.004297907177533361
144945,144946,144945,289891,3.5161068439483643,0.0042870052314310835
145145,145146,145145,290291,3.520534038543701,0.004276130938887613
145345,145346,145345,290691,3.52496600151062,0.0042652842297577044
145546,145547,145546,291093,3.5294220447540283,0.004254411007105969
145746,145747,145746,291493,3.5338220596313477,0.004243619392122112
145946,145947,145946,291893,3.5382282733917236,0.004232855150834335
146146,146147,146146,292293,3.542628049850464,0.004222118213807327
146346,146347,146346,292693,3.5470340251922607,0.0042114085117819205
146547,146548,146547,293095,3.5515849590301514,0.004200672631132604
146747,146748,146747,293495,3.5560271739959717,0.004190017327347273
146947,146948,146947,293895,3.5606000423431396,0.004179389051495029
147147,147148,147147,294295,3.5650410652160645,0.004168787735017573
147347,147348,147347,294695,3.569599151611328,0.004158213309530556
147548,147549,147548,295097,3.574129104614258,0.004147613036087471
147748,147749,147748,295497,3.5786030292510986,0.004137092321724753
147948,147949,147948,295897,3.5840580463409424,0.004126598293899459
148148,148149,148148,296297,3.5884671211242676,0.00411613088491934
148348,148349,148348,296697,3.5928831100463867,0.004105690027263842
148549,148550,148549,297099,3.598079204559326,0.004095223648143318
148749,148750,148749,297499,3.6027870178222656,0.004084835823175376
148949,148950,148949,297899,3.6076819896698,0.00407447434766153
149149,149150,149149,298299,3.612837076187134,0.004064139154764519
149349,149350,149349,298699,3.6176600456237793,0.004053830177816649
149550,149551,149550,299101,3.622602939605713,0.004043496001770825
149750,149751,149750,299501,3.6272361278533936,0.004033239387643274
149950,149951,149950,299901,3.6314730644226074,0.004023008790144223
150150,150151,150150,300301,3.6357879638671875,0.004012804143280672
150350,150351,150350,300701,3.6404190063476562,0.004002625381226962
150551,150552,150551,301103,3.644974946975708,0.0039924217383705465
150751,150752,150751,301503,3.649306058883667,0.003982294677731186
150951,150952,150951,301903,3.653745174407959,0.003972193305098745
151151,151152,151151,302303,3.6589059829711914,0.003962117555313767
151351,151352,151351,302703,3.6635618209838867,0.003952067363382061
151552,151553,151552,303105,3.66792893409729,0.003941992604922365
151752,151753,151752,303505,3.673567056655884,0.003931993461353369
151952,151953,151952,303905,3.6779088973999023,0.003922019681320576
152152,152153,152152,304305,3.6822640895843506,0.003912071200487557
152352,152353,152352,304705,3.6870720386505127,0.003902147954681117
152553,152554,152553,305107,3.691509962081909,0.003892200452651772
152753,152754,152753,305507,3.6958959102630615,0.0038823276104052538
152953,152954,152953,305907,3.70062518119812,0.0038724798113226686
153153,153154,153153,306307,3.70510196685791,0.0038626569918802553
153353,153354,153353,306707,3.7096481323242188,0.0038528590887154024
153554,153555,153554,307109,3.7141001224517822,0.0038430372357131973
153754,153755,153754,307509,3.7185380458831787,0.003833289099450113
153954,153955,153954,307909,3.722999095916748,0.00382356569002539
154154,154155,154154,308309,3.7283661365509033,0.003813866944717681
154354,154355,154354,308709,3.733494997024536,0.00380419280096468
154555,154556,154555,309111,3.738358974456787,0.0037944950098898144
154755,154756,154755,309511,3.7433021068573,0.003784870004422191
154955,154956,154955,309911,3.747972011566162,0.0037752694134629444
155155,155156,155155,310311,3.7523770332336426,0.0037656931750829664
155355,155356,155355,310711,3.757538080215454,0.0037561412275102057
155556,155557,155556,311113,3.7619640827178955,0.0037465659313099878
155756,155757,155756,311513,3.766451120376587,0.003737062501346391
155956,155957,155956,311913,3.770836114883423,0.0037275831775063118
156156,156157,156156,312313,3.7752392292022705,0.003718127898642853
156356,156357,156356,312713,3.779635190963745,0.0037086966037642288
156557,156558,156557,313115,3.784111976623535,0.003699242255179645
156757,156758,156757,313515,3.788612127304077,0.003689858865073868
156957,156958,156957,313915,3.7932589054107666,0.003680499276602011
157157,157158,157157,314315,3.7978270053863525,0.0036711634293895377
157357,157358,157357,314715,3.8023672103881836,0.0036618512632150438
157558,157559,157558,315117,3.8068931102752686,0.003652516334530871
157758,157759,157758,315517,3.811429977416992,0.0036432514680337824
157958,157959,157958,315917,3.8159191608428955,0.003634010102527092
158158,158159,158158,316317,3.820413112640381,0.0036247921783988278
158358,158359,158358,316717,3.8249130249023438,0.003615597636188298
158559,158560,158559,317119,3.8294520378112793,0.003606380618986234
158759,158760,158759,317519,3.833972930908203,0.0035972327790007672
158959,158960,158959,317919,3.8384859561920166,0.003588108143159671
159159,159160,159159,318319,3.84299898147583,0.00357900665260393
159359,159360,159359,318719,3.8475019931793213,0.003569928248623905
159560,159561,159560,319121,3.8520731925964355,0.003560827653538796
159760,159761,159760,319521,3.8565869331359863,0.0035517953618780505
159960,159961,159960,319921,3.8610970973968506,0.0035427859812651318
160160,160161,160160,320321,3.8657991886138916,0.0035337994535845196
160360,160361,160360,320721,3.870487928390503,0.003524835720868156
160561,160562,160561,321123,3.8782289028167725,0.0035158500773472758
160761,160762,160761,321523,3.882905960083008,0.0035069318744956157
160961,160962,160961,321923,3.887327194213867,0.0034980362932974358
161161,161162,161161,322323,3.8917081356048584,0.003489163276371288
161361,161362,161361,322723,3.8962290287017822,0.003480312766481335
161562,161563,161562,323125,3.900676965713501,0.003471440622546906
161762,161763,161762,323525,3.9051029682159424,0.003462635067424167
161962,161963,161962,323925,3.9096932411193848,0.003453851848215928
162162,162163,162162,324325,3.914144992828369,0.0034450909082656177
162362,162363,162362,324725,3.9185619354248047,0.003436352191060261
162563,162564,162563,325127,3.923245906829834,0.0034275921130747142
162763,162764,162763,325527,3.9278392791748047,0.0034188977828033353
162963,162964,162963,325927,3.932257890701294,0.003410225506316767
163163,163164,163163,326327,3.9366650581359863,0.003401575227674002
163363,163364,163363,326727,3.94154691696167,0.0033929468910759704
163564,163565,163564,327129,3.945966958999634,0.0033842974635103244
163764,163765,163764,327529,3.9503750801086426,0.0033757129531853925
163964,163965,163964,327929,3.954911947250366,0.00336715021807918
164164,164165,164164,328329,3.9594979286193848,0.003358609202957306
164364,164365,164364,328729,3.9638729095458984,0.0033500898527254962
164565,164566,164565,329131,3.9682610034942627,0.003341549677930612
164765,164766,164765,329531,3.97263503074646,0.0033330736003928502
164965,164966,164965,329931,3.977023124694824,0.003324619023026386
165165,165166,165165,330331,3.981421947479248,0.003316185891294523
165365,165366,165365,330731,3.985774040222168,0.003307774150798822
165566,165567,165566,331133,3.9903149604797363,0.0032993418487795648
165766,165767,165766,331533,3.994797945022583,0.0032909728343912706
165966,165967,165966,331933,3.999268054962158,0.003282625048601005
166166,166167,166166,332333,4.006880044937134,0.003274298437560889
166366,166367,166366,332733,4.012535095214844,0.003265992947559694
166567,166568,166567,333135,4.018732070922852,0.0032576671557519505
166767,166768,166767,333535,4.023627042770386,0.0032494038521755724
166967,166968,166967,333935,4.029053211212158,0.003241161509054232
167167,167168,167167,334335,4.036983966827393,0.0032329400732202533
167367,167368,167367,334735,4.046328067779541,0.0032247394916408412
167568,167569,167568,335137,4.052470922470093,0.0032165188646913257
167768,167769,167768,335537,4.058600187301636,0.0032083599366709383
167968,167969,167968,335937,4.065925121307373,0.0032002217043496078
168168,168169,168168,336337,4.072242021560669,0.003192104115231256
168368,168369,168368,336737,4.0799360275268555,0.0031840071169528784
168569,168570,168569,337139,4.087360858917236,0.0031758903265017716
168769,168770,168769,337539,4.096652984619141,0.0031678344556474243
168969,168970,168969,337939,4.102794885635376,0.003159799019080331
169169,169170,169169,338339,4.1094300746917725,0.0031517839649674757
169369,169370,169369,338739,4.115489959716797,0.0031437892416073094
169570,169571,169570,339141,4.1220362186431885,0.0031357749760735796
169770,169771,169770,339541,4.127902269363403,0.0031278208606481373
169970,169971,169970,339941,4.133656024932861,0.0031198869214000883
170170,170171,170170,340341,4.14047908782959,0.0031119731071511014
170370,170371,170370,340741,4.146496057510376,0.0031040793668527487
170571,170572,170571,341143,4.152493953704834,0.0030961663312222025
170771,170772,170771,341543,4.158803224563599,0.003088312685931053
170971,170972,170971,341943,4.165171146392822,0.0030804789619677036
171171,171172,171171,342343,4.170989990234375,0.00307266510880026
171371,171372,171371,342743,4.17682409286499,0.0030648710760250797
171572,171573,171572,343145,4.182631015777588,0.0030570579916411513
171772,171773,171772,343545,4.188448905944824,0.0030493035474245464
171972,171973,171972,343945,4.194558143615723,0.0030415687729051654
172172,172173,172172,344345,4.200323104858398,0.003033853618189424
172372,172373,172372,344745,4.207042932510376,0.0030261580335103197
172573,172574,172573,345147,4.213131904602051,0.0030184436378674433
172773,172774,172773,345547,4.2190210819244385,0.003010787141695362
172973,172974,172973,345947,4.225080966949463,0.0030031500667683534
173173,173174,173173,346347,4.230849981307983,0.0029955323638230598
173373,173374,173373,346747,4.236495018005371,0.002987933983721062
173574,173575,173574,347149,4.242198944091797,0.0029803170302606158
173774,173775,173774,347549,4.247821092605591,0.0029727572449303706
173974,173975,173974,347949,4.253468036651611,0.0029652166355312757
174174,174175,174174,348349,4.260303020477295,0.0029576951534222595
174374,174375,174374,348749,4.266318082809448,0.002950192750085565
174575,174576,174575,349151,4.272324085235596,0.002942672007994456
174775,174776,174775,349551,4.278205156326294,0.002935207711930698
174975,174976,174975,349951,4.283829927444458,0.002927762349582789
175175,175176,175175,350351,4.289273023605347,0.002920335872924058
175375,175376,175375,350751,4.294083118438721,0.002912928234049598
175576,175577,175576,351153,4.298681974411011,0.0029055024880614566
175776,175777,175776,351553,4.303272247314453,0.0028981324751187693
175976,175977,175976,351953,4.307853937149048,0.0028907811567361673
176176,176177,176176,352353,4.3124330043792725,0.0028834484854935324
176376,176377,176376,352753,4.317001104354858,0.0028761344140911024
176577,176578,176577,353155,4.321575164794922,0.00286880246428984
176777,176778,176777,353555,4.326189994812012,0.002861525543557997
176977,176978,176977,353955,4.33063006401062,0.0028542670812512294
177177,177178,177177,354355,4.335105895996094,0.002847027030548416
177377,177378,177377,354755,4.33955717086792,0.00283980534474726
177578,177579,177578,355157,4.344050168991089,0.0028325660063731437
177778,177779,177778,355557,4.348605155944824,0.0028253810019845025
177978,177979,177978,355957,4.35305118560791,0.002818214222868624
178178,178179,178178,356357,4.357568979263306,0.0028110656227957843
178378,178379,178378,356757,4.362022161483765,0.0028039351556535695
178579,178580,178579,357159,4.3665220737457275,0.0027967872589118453
178779,178780,178779,357559,4.3710150718688965,0.0027896930098513886
178979,178980,178979,357959,4.375468015670776,0.0027826167558563718
179179,179180,179179,358359,4.380005121231079,0.0027755584512810113
179379,179380,179379,358759,4.384310960769653,0.0027685180505953692
179580,179581,179580,359161,4.388675928115845,0.0027614604404672034
179780,179781,179780,359561,4.3929221630096436,0.00275445580038499
179980,179981,179980,359961,4.397171258926392,0.0027474689280686704
180180,180181,180180,360361,4.40146017074585,0.002740499778449068
180380,180381,180380,360761,4.405695915222168,0.0027335483065712924
180581,180582,180581,361163,4.413992166519165,0.0027265798426271497
180781,180782,180781,361563,4.418247222900391,0.002719663679652952
180981,180982,180981,361963,4.422490119934082,0.002712765060016202
181181,181182,181181,362363,4.426723957061768,0.0027058839392170007
181381,181382,181381,362763,4.430969953536987,0.0026990202728682925
181582,181583,181582,363165,4.435219049453735,0.0026921398290836373
181782,181783,181782,363565,4.439456939697266,0.0026853110256441957
181982,181983,181982,363965,4.443682909011841,0.002678499543948546
182182,182183,182182,364365,4.447916030883789,0.002671705340058889
182382,182383,182382,364765,4.452163934707642,0.0026649283701488387
182583,182584,182583,365167,4.456423044204712,0.0026581348347221997
182783,182784,182783,365567,4.460663080215454,0.002651392287360521
182983,182984,182983,365967,4.4649200439453125,0.0026446668429479826
183183,183184,183183,366367,4.469156980514526,0.0026379584581017407
183383,183384,183383,366767,4.4734461307525635,0.0026312670895490367
183584,183585,183584,367169,4.47771692276001,0.0026245593647223242
183784,183785,183784,367569,4.48191499710083,0.002617901983919412
183984,183985,183984,367969,4.486170053482056,0.0026112614900346636
184184,184185,184184,368369,4.490373134613037,0.002604637840233177
184384,184385,184384,368769,4.4947121143341064,0.002598030991788761
184585,184586,184585,369171,4.499017238616943,0.002591407993669971
184785,184786,184785,369571,4.503262042999268,0.00258483470366882
184985,184986,184985,369971,4.507582187652588,0.002578278087283528
185185,185186,185185,370371,4.512171983718872,0.002571738102220309
185385,185386,185385,370771,4.516378164291382,0.0025652147062926274
185586,185587,185586,371173,4.520653963088989,0.002558675364680543
185786,185787,185786,371573,4.525377035140991,0.00255218510331225
185986,185987,185986,371973,4.530637979507446,0.0025457113049517865
186186,186187,186186,372373,4.536639213562012,0.002539253927839608
186386,186387,186386,372773,4.5422890186309814,0.00253281293032204
186587,186588,186587,373175,4.546748161315918,0.0025263561885334406
186787,186788,186787,373575,4.551181077957153,0.002519947907045528
186987,186988,186987,373975,4.555535078048706,0.0025135558806177096
187187,187188,187187,374375,4.560405015945435,0.0025071800680178742
187387,187388,187387,374775,4.564992904663086,0.002500820428118482
187588,187589,187588,375177,4.569801092147827,0.002494445242817289
187788,187789,187788,375577,4.574223041534424,0.002488117905704369
187988,187989,187988,375977,4.578836917877197,0.0024818066183304147
188188,188189,188188,376377,4.583453178405762,0.0024755113399840857
188388,188389,188388,376777,4.587907075881958,0.0024692320300573555
188589,188590,188589,377179,4.592449903488159,0.0024629373710861337
188789,188790,188789,377579,4.59685206413269,0.0024566899559225084
188989,188990,188989,377979,4.601490020751953,0.002450458387770133
189189,189190,189189,378379,4.606061935424805,0.002444242626431924
189389,189390,189389,378779,4.610547065734863,0.0024380426318127797
189590,189591,189590,379181,4.614964962005615,0.002431827482026249
189790,189791,189790,379581,4.619652032852173,0.0024256589793006465
189990,189991,189990,379981,4.624585151672363,0.0024195061234192987
190190,190191,190190,380381,4.629069089889526,0.002413368874692881
190390,190391,190390,380781,4.633462905883789,0.002407247193532746
190591,190592,190591,381183,4.638270139694214,0.0024011105486333464
190791,190792,190791,381583,4.642724990844727,0.00239501996158587
190991,190992,190991,381983,4.6473400592803955,0.002388944823744032
191191,191192,191191,382383,4.6520140171051025,0.0023828850959197686
191391,191392,191391,382783,4.656520128250122,0.0023768407390245276
191592,191593,191592,383185,4.66109824180603,0.0023707816074002414
191792,191793,191792,383585,4.665687084197998,0.0023647679518612966
191992,191993,191992,383985,4.670867204666138,0.002358769550385751
192192,192193,192192,384385,4.675429105758667,0.002352786364280576
192392,192393,192392,384785,4.679938077926636,0.00234681835495092
192593,192594,192593,385187,4.685871124267578,0.002340835757514978
192793,192794,192793,385587,4.691040992736816,0.0023348980617462116
192993,192994,192993,385987,4.696424245834351,0.0023289754273635058
193193,193194,193193,386387,4.702118158340454,0.002323067816162557
193393,193394,193393,386787,4.744407892227173,0.002317175190036016
193594,193595,193594,387189,4.759785175323486,0.002311268160068691
193794,193795,193794,387589,4.765887975692749,0.0023054054646059847
193994,193995,193994,387989,4.771918058395386,0.0022995576402857353
194194,194195,194194,388389,4.777663230895996,0.002293724649386227
194394,194395,194394,388789,4.783301115036011,0.002287906454281474
194595,194596,194595,389191,4.788863897323608,0.002282074037273913
194795,194796,194795,389591,4.794321060180664,0.002276285394772344
194995,194996,194995,389991,4.799955129623413,0.0022705114355726507
195195,195196,195195,390391,4.805140256881714,0.0022647521224296095
195395,195396,195395,390791,4.809629201889038,0.0022590074181924507
195596,195597,195596,391193,4.814056158065796,0.0022532486716923756
195796,195797,195796,391593,4.818421840667725,0.0022475331467731283
195996,195997,195996,391993,4.822854042053223,0.0022418321196878443
196196,196197,196196,392393,4.82722020149231,0.002236145553661752
196396,196397,196396,392793,4.831588983535767,0.002230473412013305
196597,196598,196597,393195,4.836055040359497,0.0022247874054727823
196797,196798,196797,393595,4.840457916259766,0.0022191440745720574
196997,196998,196997,393995,4.84543514251709,0.002213515058380037
197197,197198,197197,394395,4.8498921394348145,0.002207900320586445
197397,197398,197397,394795,4.854305982589722,0.0022022998249731293
197598,197599,197598,395197,4.859023094177246,0.0021966856395981573
197798,197799,197798,395597,4.864130020141602,0.0021911135908178176
197998,197999,197998,395997,4.8688600063323975,0.002185555675934069
198198,198199,198198,396397,4.874026298522949,0.0021800118590952437
198398,198399,198398,396797,4.878791093826294,0.0021744821045406922
198599,198600,198599,397199,4.883849143981934,0.0021689388331427354
198799,198800,198799,397599,4.8891191482543945,0.002163437166103118
198999,199000,198999,397999,4.894381046295166,0.002157949454431793
199199,199200,199199,398399,4.900327205657959,0.002152475662729984
199399,199400,199399,398799,4.906171083450317,0.0021470157556886765
199600,199601,199600,399201,4.912016153335571,0.002141542502538169
199800,199801,199800,399601,4.917961120605469,0.002136110328232437
200000,200001,200000,400001,4.924265146255493,0.0021306919330217103


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.508827209472656e-05,4.387072431292609
200,201,200,401,0.008509159088134766,0.18936632320225483
400,401,400,801,0.01695728302001953,0.09223193431015458
601,602,601,1203,0.02475714683532715,0.0656058045305487
801,802,801,1603,0.03294706344604492,0.058322281162373334
1001,1002,1001,2003,0.04091310501098633,0.0469572063819363
1201,1202,1201,2403,0.04848623275756836,0.04918596952880194
1401,1402,1401,2803,0.05623817443847656,0.03888773044947158
1602,1603,1602,3205,0.06370997428894043,0.03525175629247065
1802,1803,1802,3605,0.07074832916259766,0.034352401565386034
2002,2003,2002,4005,0.07820796966552734,0.031016241446923453
2202,2203,2202,4405,0.0861198902130127,0.035049799478285466
2402,2403,2402,4805,0.09404611587524414,0.028056873132843118
2603,2604,2603,5207,0.1020960807800293,0.030061297549765595
2803,2804,2803,5607,0.10983514785766602,0.025832454724797196
3003,3004,3003,6007,0.11786913871765137,0.024880387381991612
3203,3204,3203,6407,0.12548518180847168,0.024193856608383208
3403,3404,3403,6807,0.13296103477478027,0.024058938603714674
3604,3605,3604,7209,0.13966107368469238,0.022938487728528013
3804,3805,3804,7609,0.1464982032775879,0.022289682909653826
4004,4005,4004,8009,0.15436220169067383,0.02197021947981532
4204,4205,4204,8409,0.1637890338897705,0.02135702103118868
4404,4405,4404,8809,0.17178916931152344,0.02100253807346372
4605,4606,4605,9211,0.17949318885803223,0.02086916290451464
4805,4806,4805,9611,0.1868600845336914,0.020532725704852046
5005,5006,5005,10011,0.1934499740600586,0.021631294533434244
5205,5206,5205,10411,0.20018410682678223,0.023962975766511446
5405,5406,5405,10811,0.20939016342163086,0.02022322378491767
5606,5607,5606,11213,0.21814513206481934,0.019468949583072995
5806,5807,5806,11613,0.22635698318481445,0.019200864140216142
6006,6007,6006,12013,0.23558306694030762,0.01909213074102498
6206,6207,6206,12413,0.24349713325500488,0.018628386500526617
6406,6407,6406,12813,0.2520711421966553,0.018451161085895115
6607,6608,6607,13215,0.2598690986633301,0.0180974497030236
6807,6808,6807,13615,0.2691991329193115,0.018447839173058173
7007,7008,7007,14015,0.2773261070251465,0.017884349215526073
7207,7208,7207,14415,0.2900872230529785,0.017941500555366897
7407,7408,7407,14815,0.3037140369415283,0.01740299098682146
7608,7609,7608,15217,0.3131141662597656,0.018055002919716758
7808,7809,7808,15617,0.3235001564025879,0.016823907178130065
8008,8009,8008,16017,0.3314859867095947,0.016859474518199354
8208,8209,8208,16417,0.3393080234527588,0.016441605892395357
8408,8409,8408,16817,0.34732532501220703,0.019960701559353998
8609,8610,8609,17219,0.3550112247467041,0.016093323168860172
8809,8810,8809,17619,0.3629770278930664,0.015874946252434154
9009,9010,9009,18019,0.37096619606018066,0.015602412735053191
9209,9210,9209,18419,0.37881922721862793,0.015601365957870698
9409,9410,9409,18819,0.38684511184692383,0.0153145626693603
9610,9611,9610,19221,0.39486217498779297,0.015076835135817458
9810,9811,9810,19621,0.4026920795440674,0.015181358822380515
10010,10011,10010,20021,0.40994715690612793,0.01477895305301629
10210,10211,10210,20421,0.4165470600128174,0.014726288203231519
10410,10411,10410,20821,0.42304205894470215,0.016382810727969446
10611,10612,10611,21223,0.42925596237182617,0.014629764591720492
10811,10812,10811,21623,0.43610334396362305,0.01396198876920678
11011,11012,11011,22023,0.4423370361328125,0.013829626942600948
11211,11212,11211,22423,0.44876909255981445,0.013624943905131465
11411,11412,11411,22823,0.45528411865234375,0.015117473715436433
11612,11613,11612,23225,0.46155214309692383,0.013298472572415914
11812,11813,11812,23625,0.46808600425720215,0.01320426748339519
12012,12013,12012,24025,0.47472119331359863,0.012885826262499405
12212,12213,12212,24425,0.48104405403137207,0.012994895968908593
12412,12413,12412,24825,0.4871940612792969,0.012672476183744919
12613,12614,12613,25227,0.4934041500091553,0.012641742579447304
12813,12814,12813,25627,0.4996161460876465,0.01238883748889857
13013,13014,13013,26027,0.5058472156524658,0.012178265993356908
13213,13214,13213,26427,0.5120241641998291,0.015094596451200053
13413,13414,13413,26827,0.5181922912597656,0.012030395735244444
13614,13615,13614,27229,0.5246939659118652,0.012126957956764009
13814,13815,13814,27629,0.5308411121368408,0.012002607330754575
14014,14015,14014,28029,0.5370161533355713,0.011539917288380701
14214,14215,14214,28429,0.5432021617889404,0.011329175291189538
14414,14415,14414,28829,0.5494050979614258,0.011161804582309634
14615,14616,14615,29231,0.5556333065032959,0.011318460044441125
14815,14816,14815,29631,0.5618271827697754,0.011000663185771828
15015,15016,15015,30031,0.5681211948394775,0.010807434981269654
15215,15216,15215,30431,0.5748691558837891,0.010764290775629093
15415,15416,15415,30831,0.5812900066375732,0.010650466539483221
15616,15617,15616,31233,0.5877540111541748,0.010448891170656215
15816,15817,15816,31633,0.5943601131439209,0.010264291978760203
16016,16017,16016,32033,0.602161169052124,0.010240915647861112
16216,16217,16216,32433,0.6088321208953857,0.01215317495361385
16416,16417,16416,32833,0.6155731678009033,0.009895740843234989
16617,16618,16617,33235,0.623751163482666,0.0098090809487204
16817,16818,16817,33635,0.6318521499633789,0.009664723317671082
17017,17018,17017,34035,0.6395430564880371,0.00959986527487779
17217,17218,17217,34435,0.6476039886474609,0.009515207769177341
17417,17418,17417,34835,0.6549220085144043,0.009275128961142574
17618,17619,17618,35237,0.6613750457763672,0.009225325310501744
17818,17819,17818,35637,0.667626142501831,0.008986579994002444
18018,18019,18018,36037,0.6739780902862549,0.010708088533237209
18218,18219,18218,36437,0.6803340911865234,0.008814615837177181
18418,18419,18418,36837,0.6865322589874268,0.00879944874303613
18619,18620,18619,37239,0.6928021907806396,0.008652917092832045
18819,18820,18819,37639,0.6990201473236084,0.008712470530932971
19019,19020,19019,38039,0.7053210735321045,0.008504296575971203
19219,19220,19219,38439,0.7119801044464111,0.008387193883851176
19419,19420,19419,38839,0.7181661128997803,0.008220568209398886
19620,19621,19620,39241,0.7243351936340332,0.008117352777286951
19820,19821,19820,39641,0.7304301261901855,0.008009904006628817
20020,20021,20020,40041,0.7366280555725098,0.007940983569068881
20220,20221,20220,40441,0.7431061267852783,0.007889662933258358
20420,20421,20420,40841,0.749812126159668,0.0077723100979238315
20621,20622,20621,41243,0.7564730644226074,0.007810089276610669
20821,20822,20821,41643,0.7631649971008301,0.0075172092443144154
21021,21022,21021,42043,0.7697570323944092,0.008998716612139681
21221,21222,21221,42443,0.7765100002288818,0.007418951378251925
21421,21422,21421,42843,0.783095121383667,0.00725303773588433
21622,21623,21622,43245,0.7899901866912842,0.007269600127948643
21822,21823,21822,43645,0.7968840599060059,0.007021484866976556
22022,22023,22022,44045,0.8038170337677002,0.006979136237117952
22222,22223,22222,44445,0.8106000423431396,0.006904146298492021
22422,22423,22422,44845,0.8174121379852295,0.007300334625210108
22623,22624,22623,45247,0.8242402076721191,0.006683180186684013
22823,22824,22823,45647,0.8310489654541016,0.006626367437470176
23023,23024,23023,46047,0.8378281593322754,0.006620403077963792
23223,23224,23223,46447,0.8447561264038086,0.007553795138001914
23423,23424,23423,46847,0.8515172004699707,0.00639871498362701
23624,23625,23624,47249,0.8585600852966309,0.006663144832643188
23824,23825,23824,47649,0.865645170211792,0.006194223434858175
24024,24025,24024,48049,0.8725950717926025,0.006645302841427511
24224,24225,24224,48449,0.8795111179351807,0.006135576843184301
24424,24425,24424,48849,0.887714147567749,0.006333564171553187
24625,24626,24625,49251,0.895050048828125,0.005946056495598024
24825,24826,24825,49651,0.902778148651123,0.0058509123411267395
25025,25026,25025,50051,0.9104640483856201,0.0058691425915221905
25225,25226,25225,50451,0.9178721904754639,0.0057862559460983305
25425,25426,25425,50851,0.9243481159210205,0.005663728474846472
25626,25627,25626,51253,0.9305260181427002,0.005552027312139043
25826,25827,25826,51653,0.9367029666900635,0.005579929500003388
26026,26027,26026,52053,0.9429092407226562,0.005437261182126389
26226,26227,26226,52453,0.9491031169891357,0.005394347340894282
26426,26427,26426,52853,0.9553370475769043,0.0052778581011025715
26627,26628,26627,53255,0.9620349407196045,0.005415266220562603
26827,26828,26827,53655,0.9681360721588135,0.00518203603924742
27027,27028,27027,54055,0.9746532440185547,0.0050845789484168505
27227,27228,27227,54455,0.9808392524719238,0.005159841247919578
27427,27428,27427,54855,0.9871721267700195,0.005043737832281305
27628,27629,27628,55257,0.9934902191162109,0.004938746064361496
27828,27829,27828,55657,0.9997291564941406,0.004846336994202827
28028,28029,28028,56057,1.0058810710906982,0.005159935308467211
28228,28229,28228,56457,1.0120329856872559,0.004839691231055434
28428,28429,28428,56857,1.0181410312652588,0.004714567034551519
28629,28630,28629,57259,1.0242841243743896,0.004601631472806232
28829,28830,28829,57659,1.0305161476135254,0.004923546115768655
29029,29030,29029,58059,1.0365381240844727,0.004488375769277907
29229,29230,29229,58459,1.0425710678100586,0.004578261145488517
29429,29430,29429,58859,1.048525094985962,0.00437786755848694
29630,29631,29630,59261,1.0557191371917725,0.0043314455539875665
29830,29831,29830,59661,1.0618741512298584,0.004289557788411757
30030,30031,30030,60061,1.0679171085357666,0.005539839666283146
30230,30231,30230,60461,1.073979139328003,0.0042073426893633635
30430,30431,30430,60861,1.0800011157989502,0.004137473006305593
30631,30632,30631,61263,1.0860931873321533,0.0040915970695461195
30831,30832,30831,61663,1.0923819541931152,0.004002592387646612
31031,31032,31031,62063,1.0983989238739014,0.004197112413802173
31231,31232,31231,62463,1.1048400402069092,0.004114854305821307
31431,31432,31431,62863,1.1112651824951172,0.0038855601763930544
31632,31633,31632,63265,1.11753511428833,0.0038649826746741216
31832,31833,31832,63665,1.1236889362335205,0.0038122965186893577
32032,32033,32032,64065,1.1297039985656738,0.0037627668591842826
32232,32233,32232,64465,1.1357390880584717,0.003858035859669507
32432,32433,32432,64865,1.14182710647583,0.004351484784835877
32633,32634,32633,65267,1.1479182243347168,0.0044259842915955775
32833,32834,32833,65667,1.1540501117706299,0.003572830870195248
33033,33034,33033,66067,1.1601221561431885,0.0035281308133604263
33233,33234,33233,66467,1.1662251949310303,0.0034676550734832534
33433,33434,33433,66867,1.1722922325134277,0.003456781886342454
33634,33635,33634,67269,1.178382158279419,0.0033954657588784166
33834,33835,33834,67669,1.184507131576538,0.0033818201240780376
34034,34035,34034,68069,1.1905710697174072,0.0033702232840683017
34234,34235,34234,68469,1.1966681480407715,0.003318529209116326
34434,34435,34434,68869,1.202775001525879,0.0032244343043375183
34635,34636,34635,69271,1.2090041637420654,0.0038585534259573152
34835,34836,34835,69671,1.2155461311340332,0.003175856125217855
35035,35036,35035,70071,1.2218081951141357,0.0031209457823914155
35235,35236,35235,70471,1.2279181480407715,0.0030992611151014404
35435,35436,35435,70871,1.2340221405029297,0.003047244078095222
35636,35637,35636,71273,1.2401471138000488,0.0030464325878349296
35836,35837,35836,71673,1.246225118637085,0.002964719611763382
36036,36037,36036,72073,1.2523820400238037,0.0029147279175290287
36236,36237,36236,72473,1.2585132122039795,0.0034312153404067315
36436,36437,36436,72873,1.264733076095581,0.003308813677753265
36637,36638,36637,73275,1.2709541320800781,0.0027972694383065736
36837,36838,36837,73675,1.2771499156951904,0.0027573223896803986
37037,37038,37037,74075,1.283318042755127,0.002749260636676773
37237,37238,37237,74475,1.2895112037658691,0.002704614543534682
37437,37438,37437,74875,1.2958650588989258,0.002670902749121971
37638,37639,37638,75277,1.3024020195007324,0.0029432606285557028
37838,37839,37838,75677,1.3088350296020508,0.0025904928060624033
38038,38039,38038,76077,1.3152251243591309,0.0031118128257939196
38238,38239,38238,76477,1.3215880393981934,0.002564314367350419
38438,38439,38438,76877,1.3275032043457031,0.002527417164791063
38639,38640,38639,77279,1.3336162567138672,0.0025171501544321508
38839,38840,38839,77679,1.3397769927978516,0.0024600644260109753
39039,39040,39039,78079,1.3463900089263916,0.0025075659242937386
39239,39240,39239,78479,1.3524999618530273,0.0023913299958036784
39439,39440,39439,78879,1.358557939529419,0.002375559295211246
39640,39641,39640,79281,1.3646202087402344,0.0027013897581320088
39840,39841,39840,79681,1.3706512451171875,0.0023139889145285964
40040,40041,40040,80081,1.3766491413116455,0.00234852905752498
40240,40241,40240,80481,1.38279128074646,0.0022798769941750493
40440,40441,40440,80881,1.388733148574829,0.0022401000885318447
40641,40642,40641,81283,1.394714117050171,0.0022033881697113133
40841,40842,40841,81683,1.401036024093628,0.002213888062684831
41041,41042,41041,82083,1.4071311950683594,0.002137040693037244
41241,41242,41241,82483,1.4132881164550781,0.002147630562696853
41441,41442,41441,82883,1.4193570613861084,0.0020929778249970526
41642,41643,41642,83285,1.4254631996154785,0.0020908003253091727
41842,41843,41842,83685,1.4314391613006592,0.0020563636552439583
42042,42043,42042,84085,1.4372951984405518,0.0023306501074101516
42242,42243,42242,84485,1.443145990371704,0.00199142783074224
42442,42443,42442,84885,1.4491610527038574,0.0019507656611844762
42643,42644,42643,85287,1.4552409648895264,0.0019502284494540497
42843,42844,42843,85687,1.4617242813110352,0.002168060817332156
43043,43044,43043,86087,1.4679701328277588,0.0018967517759683119
43243,43244,43243,86487,1.4741010665893555,0.0019295853546895498
43443,43444,43443,86887,1.4802219867706299,0.0018534573876843319
43644,43645,43644,87289,1.4863512516021729,0.0018212919504890387
43844,43845,43844,87689,1.4924559593200684,0.002042161189273212
44044,44045,44044,88089,1.4993832111358643,0.001794196852668956
44244,44245,44244,88489,1.5081470012664795,0.0017833914042765305
44444,44445,44444,88889,1.5142841339111328,0.0017446666519049857
44645,44646,44645,89291,1.5202751159667969,0.001982087316456891
44845,44846,44845,89691,1.5261411666870117,0.001754287650500231
45045,45046,45045,90091,1.5321271419525146,0.0017783027210222571
45245,45246,45245,90491,1.5380780696868896,0.0016788605181189192
45445,45446,45445,90891,1.5440330505371094,0.0016425052969819233
45646,45647,45646,91293,1.5504071712493896,0.00160881532734715
45846,45847,45846,91693,1.556401252746582,0.0015878052664582108
46046,46047,46046,92093,1.5625312328338623,0.0015844995126847478
46246,46247,46246,92493,1.5684940814971924,0.0015491767718694564
46446,46447,46446,92893,1.5744593143463135,0.001536120923365317
46647,46648,46647,93295,1.5804851055145264,0.0017802034600299737
46847,46848,46847,93695,1.5864770412445068,0.0015108316641576614
47047,47048,47047,94095,1.5924551486968994,0.0014934169793777868
47247,47248,47247,94495,1.598464012145996,0.0014762320963331713
47447,47448,47447,94895,1.6044471263885498,0.0014627195144624881
47648,47649,47648,95297,1.6105320453643799,0.0014758449833815444
47848,47849,47848,95697,1.6165142059326172,0.0017235546750329518
48048,48049,48048,96097,1.6224629878997803,0.00169702435989609
48248,48249,48248,96497,1.628387212753296,0.0016389660027173554
48448,48449,48448,96897,1.6341912746429443,0.0013610546849134224
48649,48650,48649,97299,1.6400620937347412,0.0013329508895245327
48849,48850,48849,97699,1.6461372375488281,0.0013342613164774326
49049,49050,49049,98099,1.6520051956176758,0.001308252165271267
49249,49250,49249,98499,1.6578521728515625,0.001291017864819047
49449,49450,49449,98899,1.6640121936798096,0.0012669938266558207
49650,49651,49650,99301,1.669888973236084,0.001259489771561379
49850,49851,49850,99701,1.6757440567016602,0.001257180356093915
50050,50051,50050,100101,1.6817049980163574,0.0012761061152001517
50250,50251,50250,100501,1.6877210140228271,0.001210896332177958
50450,50451,50450,100901,1.6936731338500977,0.0011958834561842824
50651,50652,50651,101303,1.6996469497680664,0.0011802308236679739
50851,50852,50851,101703,1.7056331634521484,0.0011815262425043948
51051,51052,51051,102103,1.7116711139678955,0.0011511631009639778
51251,51252,51251,102503,1.7175979614257812,0.0011430920456135367
51451,51452,51451,102903,1.7235100269317627,0.0011399293616745616
51652,51653,51652,103305,1.729485034942627,0.0011092160775322967
51852,51853,51852,103705,1.7354261875152588,0.0011480099033130354
52052,52053,52052,104105,1.7414031028747559,0.0010822530136601308
52252,52253,52252,104505,1.7474660873413086,0.0010786503584009493
52452,52453,52452,104905,1.753263235092163,0.001059424522184412
52653,52654,52653,105307,1.7589612007141113,0.0011145389309266038
52853,52854,52853,105707,1.7648100852966309,0.0010418424666027366
53053,53054,53053,106107,1.7708642482757568,0.00105051897296275
53253,53254,53253,106507,1.777036190032959,0.0010196371351831586
53453,53454,53453,106907,1.783271312713623,0.000993383461113229
53654,53655,53654,107309,1.7895371913909912,0.001010762369160719
53854,53855,53854,107709,1.795884132385254,0.000978610576887985
54054,54055,54054,108109,1.8022992610931396,0.001007279354977609
54254,54255,54254,108509,1.8088161945343018,0.0009471167685648379
54454,54455,54454,108909,1.815364122390747,0.0009403220256554005
54655,54656,54655,109311,1.8218750953674316,0.0009333010607565112
54855,54856,54855,109711,1.8283300399780273,0.0009089427186434027
55055,55056,55055,110111,1.834902048110962,0.0009038832135878346
55255,55256,55255,110511,1.8414041996002197,0.0008933525857824101
55455,55456,55455,110911,1.8478331565856934,0.0008886519162789888
55656,55657,55656,111313,1.8546881675720215,0.001066405363168276
55856,55857,55856,111713,1.861295223236084,0.0008620896445564649
56056,56057,56056,112113,1.8678452968597412,0.0008557050380351302
56256,56257,56256,112513,1.8744299411773682,0.0008470371416339308
56456,56457,56456,112913,1.8810372352600098,0.0009403818013693754
56657,56658,56657,113315,1.8876652717590332,0.0008183932863532129
56857,56858,56857,113715,1.8942341804504395,0.0010537181469475701
57057,57058,57057,114115,1.9008400440216064,0.0008009848355961437
57257,57258,57257,114515,1.9073331356048584,0.000791428124913332
57457,57458,57457,114915,1.9139032363891602,0.0009724292912953357
57658,57659,57658,115317,1.9205219745635986,0.0008936225177321889
57858,57859,57858,115717,1.9270520210266113,0.0007594032827857095
58058,58059,58058,116117,1.9334940910339355,0.0007729268571477627
58258,58259,58258,116517,1.9401342868804932,0.000743943561101582
58458,58459,58458,116917,1.9467132091522217,0.000750120000451758
58659,58660,58659,117319,1.9532852172851562,0.0007186203428864305
58859,58860,58859,117719,1.9598701000213623,0.0007182899824800161
59059,59060,59059,118119,1.966454029083252,0.0007089889205573614
59259,59260,59259,118519,1.973114252090454,0.0006941616118195918
59459,59460,59459,118919,1.9790520668029785,0.0006842639126734692
59660,59661,59660,119321,1.9850959777832031,0.0006796811886498607
59860,59861,59860,119721,1.9911561012268066,0.000678502152963456
60060,60061,60060,120121,1.997063159942627,0.0006677944842935721
60260,60261,60260,120521,2.0031590461730957,0.0006541835069575465
60460,60461,60460,120921,2.0094830989837646,0.0007457916555517015
60661,60662,60661,121323,2.0161080360412598,0.0006397622019535159
60861,60862,60861,121723,2.02268123626709,0.0006386283395736357
61061,61062,61061,122123,2.0293021202087402,0.0006238764464738079
61261,61262,61261,122523,2.0359532833099365,0.0006141465441017105
61461,61462,61461,122923,2.042532205581665,0.0006065640587473677
61662,61663,61662,123325,2.0491771697998047,0.0005977095537268667
61862,61863,61862,123725,2.0560362339019775,0.000592998107815703
62062,62063,62062,124125,2.0628769397735596,0.0005833639524103019
62262,62263,62262,124525,2.06980299949646,0.0005749242847428038
62462,62463,62462,124925,2.0766501426696777,0.0005764137800943921
62663,62664,62663,125327,2.083549976348877,0.0005726210672522799
62863,62864,62863,125727,2.090280055999756,0.0005568585558126129
63063,63064,63063,126127,2.097039222717285,0.0005550588498016388
63263,63264,63263,126527,2.103759288787842,0.0005434210513721822
63463,63464,63463,126927,2.1106009483337402,0.0005358084999106396
63664,63665,63664,127329,2.117305040359497,0.0006141556844611439
63864,63865,63864,127729,2.1242172718048096,0.0005234754288909909
64064,64065,64064,128129,2.1311440467834473,0.0005195450188445753
64264,64265,64264,128529,2.1380350589752197,0.0005109078123326022
64464,64465,64464,128929,2.144947052001953,0.0005019191403487335
64665,64666,64665,129331,2.15171217918396,0.0004953302279644816
64865,64866,64865,129731,2.158449172973633,0.0004930574809476508
65065,65066,65065,130131,2.165166139602661,0.0004884452477499748
65265,65266,65265,130531,2.1718993186950684,0.0004912597518909316
65465,65466,65465,130931,2.1786081790924072,0.0005928154665372958
65666,65667,65666,131333,2.1853482723236084,0.0004676712476322441
65866,65867,65866,131733,2.1920571327209473,0.00046334895654448466
66066,66067,66066,132133,2.1987130641937256,0.000479662229086581
66266,66267,66266,132533,2.2054340839385986,0.00045484791674220085
66466,66467,66466,132933,2.212263345718384,0.0004458759191980196
66667,66668,66667,133335,2.2191271781921387,0.000569349976193558
66867,66868,66867,133735,2.2258381843566895,0.00043266922214699356
67067,67068,67067,134135,2.232586145401001,0.00042729314507960466
67267,67268,67267,134535,2.2393059730529785,0.0004264498160471299
67467,67468,67467,134935,2.245936155319214,0.00041423575392115244
67668,67669,67668,135337,2.2526261806488037,0.000417030281584983
67868,67869,67868,135737,2.259369134902954,0.0004757344653838603
68068,68069,68068,136137,2.2662532329559326,0.0004029429726365288
68268,68269,68268,136537,2.273076057434082,0.0004004415233222935
68468,68469,68468,136937,2.2797701358795166,0.0004659878621661099
68669,68670,68669,137339,2.286651134490967,0.00038961160374922254
68869,68870,68869,137739,2.2934420108795166,0.0004004739509990538
69069,69070,69069,138139,2.300537109375,0.0003769642752731677
69269,69270,69269,138539,2.307690143585205,0.00037295116118747494
69469,69470,69469,138939,2.314119338989258,0.00036845300639498516
69670,69671,69670,139341,2.320202112197876,0.0003648788631296523
69870,69871,69870,139741,2.3264191150665283,0.0003723101600442952
70070,70071,70070,140141,2.3324952125549316,0.00035891798740044954
70270,70271,70270,140541,2.3386611938476562,0.00036045059473189015
70470,70471,70470,140941,2.345715045928955,0.00034505583240410244
70671,70672,70671,141343,2.3519370555877686,0.00034901430743082627
70871,70872,70871,141743,2.358417272567749,0.00033664982330264194
71071,71072,71071,142143,2.3645150661468506,0.00034238256451853155
71271,71272,71271,142543,2.3709142208099365,0.0003321969058845939
71471,71472,71471,142943,2.377272129058838,0.0003258016854977912
71672,71673,71672,143345,2.3837382793426514,0.0003528283606996271
71872,71873,71872,143745,2.3902792930603027,0.000316786760886895
72072,72073,72072,144145,2.396698236465454,0.0003124144292271852
72272,72273,72272,144545,2.403118133544922,0.00030911521341396917
72472,72473,72472,144945,2.409658193588257,0.0003057506937818344
72673,72674,72673,145347,2.4162721633911133,0.0003023546905691867
72873,72874,72873,145747,2.423577070236206,0.0003021569283136254
73073,73074,73073,146147,2.43023419380188,0.00030122389268549127
73273,73274,73273,146547,2.4363040924072266,0.0003008908572041375
73473,73474,73473,146947,2.44252610206604,0.00028587018927202787
73674,73675,73674,147349,2.4487321376800537,0.00028090202024747896
73874,73875,73874,147749,2.455151081085205,0.00027967051293527703
74074,74075,74074,148149,2.461663007736206,0.0002799580284167689
74274,74275,74274,148549,2.467957019805908,0.0002733212009032821
74474,74475,74474,148949,2.474274158477783,0.00027076669754557775
74675,74676,74675,149351,2.4807381629943848,0.00027021720573033387
74875,74876,74875,149751,2.487229347229004,0.00026259410635216807
75075,75076,75075,150151,2.4933671951293945,0.00026096778856667574
75275,75276,75275,150551,2.4997990131378174,0.00025496050586454056
75475,75476,75475,150951,2.5070672035217285,0.0002562315654034277
75676,75677,75676,151353,2.514064311981201,0.00024854122035586107
75876,75877,75876,151753,2.5203452110290527,0.00024524485667148184
76076,76077,76076,152153,2.5266170501708984,0.00024391282762353266
76276,76277,76276,152553,2.5329442024230957,0.00024076529931652308
76476,76477,76476,152953,2.539116144180298,0.000243776846986331
76677,76678,76677,153355,2.545271158218384,0.00023555531283554298
76877,76878,76877,153755,2.551464080810547,0.00023285761290924953
77077,77078,77077,154155,2.5576672554016113,0.00023390060270605511
77277,77278,77277,154555,2.5638530254364014,0.00028638126038683427
77477,77478,77477,154955,2.5700459480285645,0.00022436889539241323
77678,77679,77678,155357,2.5762290954589844,0.00022077747087294105
77878,77879,77878,155757,2.5824172496795654,0.0002177276347992638
78078,78079,78078,156157,2.5886871814727783,0.00021413661189858567
78278,78279,78278,156557,2.594870090484619,0.0002145656570745633
78478,78479,78478,156957,2.601081132888794,0.00022014639047870525
78679,78680,78679,157359,2.6072680950164795,0.00024527792614346245
78879,78880,78879,157759,2.6134190559387207,0.00023545947797480523
79079,79080,79079,158159,2.6196091175079346,0.0002047673710091494
79279,79280,79279,158559,2.626967191696167,0.00020928586764659926
79479,79480,79479,158959,2.6332879066467285,0.0001979445048319038
79680,79681,79680,159361,2.639653205871582,0.00020456134958535277
79880,79881,79880,159761,2.645848035812378,0.0002523395527971514
80080,80081,80080,160161,2.6521480083465576,0.000227407815957995
80280,80281,80280,160561,2.6584670543670654,0.00019308668083876194
80480,80481,80480,160961,2.6647801399230957,0.00018689639874739367
80681,80682,80681,161363,2.6709771156311035,0.0001819785439901213
80881,80882,80881,161763,2.677140951156616,0.0001806094474548321
81081,81082,81081,162163,2.683345317840576,0.00017849233474237202
81281,81282,81281,162563,2.689311981201172,0.00017659066354242618
81481,81482,81481,162963,2.695272922515869,0.00017467240529319696
81682,81683,81682,163365,2.7012879848480225,0.0001722781260454133
81882,81883,81882,163765,2.7072713375091553,0.00017651048465356338
82082,82083,82082,164165,2.7132601737976074,0.00017515900581428995
82282,82283,82282,164565,2.7192471027374268,0.00016736783214985662
82482,82483,82482,164965,2.7252471446990967,0.0001644645338704823
82683,82684,82683,165367,2.7312099933624268,0.000162618894098003
82883,82884,82883,165767,2.73711895942688,0.00015997542577295438
83083,83084,83083,166167,2.7429702281951904,0.00015745223230779568
83283,83284,83283,166567,2.749068021774292,0.00015564568164004515
83483,83484,83483,166967,2.7551302909851074,0.00015308416032923394
83684,83685,83684,167369,2.761012077331543,0.0001704053405254614
83884,83885,83884,167769,2.7669100761413574,0.00017467562209046958
84084,84085,84084,168169,2.772775173187256,0.00014825236630237797
84284,84285,84284,168569,2.7786171436309814,0.00014596745582512278
84484,84485,84484,168969,2.7844769954681396,0.00014758683585723594
84685,84686,84685,169371,2.7903659343719482,0.00014236409731893838
84885,84886,84885,169771,2.7964160442352295,0.0001418100602602085
85085,85086,85085,170171,2.802692174911499,0.00014074620383331118
85285,85286,85285,170571,2.8090529441833496,0.00013646176077016282
85485,85486,85485,170971,2.8149361610412598,0.0001366447932558617
85686,85687,85686,171373,2.8208162784576416,0.00013308589987016018
85886,85887,85886,171773,2.8266592025756836,0.00014132619374342066
86086,86087,86086,172173,2.8326022624969482,0.00013034075890192893
86286,86287,86286,172573,2.8400371074676514,0.000128326317736356
86486,86487,86486,172973,2.8462681770324707,0.00012756627924542585
86687,86688,86687,173375,2.8525519371032715,0.00015580749647914802
86887,86888,86887,173775,2.8583340644836426,0.00013192667305912892
87087,87088,87087,174175,2.8643200397491455,0.00012332743389390952
87287,87288,87287,174575,2.8701560497283936,0.00012118098456173516
87487,87488,87487,174975,2.876237154006958,0.00012178805643084498
87688,87689,87688,175377,2.882580041885376,0.00011785917224262932
87888,87889,87888,175777,2.8890221118927,0.00011824858180604125
88088,88089,88088,176177,2.8955280780792236,0.00011418557572960618
88288,88289,88288,176577,2.9021639823913574,0.00012093081173768782
88488,88489,88488,176977,2.9088282585144043,0.00011683565804736673
88689,88690,88689,177379,2.9154093265533447,0.00011153684572822592
88889,88890,88889,177779,2.9214820861816406,0.0001112056541500708
89089,89090,89089,178179,2.9299731254577637,0.00010952328586933862
89289,89290,89289,178579,2.936018943786621,0.00010629033255295073
89489,89490,89489,178979,2.9420223236083984,0.00010485829610616229
89690,89691,89690,179381,2.948078155517578,0.00010557627423730322
89890,89891,89890,179781,2.9545421600341797,0.00010316959027482173
90090,90091,90090,180181,2.961099147796631,0.00012325489755441666
90290,90291,90290,180581,2.968156337738037,0.00010032341656503546
90490,90491,90490,180981,2.974247932434082,9.962978385673239e-05
90691,90692,90691,181383,2.9803152084350586,9.899245481955809e-05
90891,90892,90891,181783,2.986298084259033,0.00011069340406822679
91091,91092,91091,182183,2.9923341274261475,9.551250429228721e-05
91291,91292,91291,182583,2.9983620643615723,9.417254692589146e-05
91491,91492,91491,182983,3.004399061203003,9.344081708993713e-05
91692,91693,91692,183385,3.010498046875,9.116765843064488e-05
91892,91893,91892,183785,3.016498327255249,0.00010681115733310933
92092,92093,92092,184185,3.0224692821502686,8.960218543845837e-05
92292,92293,92292,184585,3.0284390449523926,9.025180454623383e-05
92492,92493,92492,184985,3.0343880653381348,8.782977217522352e-05
92693,92694,92693,185387,3.0403802394866943,8.703177011976952e-05
92893,92894,92893,185787,3.046342134475708,0.0001014868780834589
93093,93094,93093,186187,3.0523180961608887,8.420108282531066e-05
93293,93294,93293,186587,3.058298110961914,8.418813476863588e-05
93493,93494,93493,186987,3.064338207244873,8.987289328429977e-05
93694,93695,93694,187389,3.070350170135498,8.225192504751872e-05
93894,93895,93894,187789,3.0763211250305176,8.317907774141632e-05
94094,94095,94094,188189,3.082393169403076,8.473203710771134e-05
94294,94295,94294,188589,3.088454246520996,7.821065708183481e-05
94494,94495,94494,188989,3.0947062969207764,7.709262644769465e-05
94695,94696,94695,189391,3.1008431911468506,7.707042535309829e-05
94895,94896,94895,189791,3.1071832180023193,7.5419136050492e-05
95095,95096,95095,190191,3.113556146621704,7.437435890532373e-05
95295,95296,95295,190591,3.119739294052124,8.292500816823628e-05
95495,95496,95495,190991,3.125904083251953,8.680202168866334e-05
95696,95697,95696,191393,3.132089138031006,8.60488527819318e-05
95896,95897,95896,191793,3.1382851600646973,7.072734195692914e-05
96096,96097,96096,192193,3.144573926925659,7.00088322942223e-05
96296,96297,96296,192593,3.150930166244507,7.175660495109339e-05
96496,96497,96496,192993,3.1573071479797363,6.969973776882796e-05
96697,96698,96697,193395,3.1637439727783203,7.190156668902314e-05
96897,96898,96897,193795,3.169997215270996,6.647556443484934e-05
97097,97098,97097,194195,3.176302194595337,6.535205237323198e-05
97297,97298,97297,194595,3.18271803855896,6.470286714712475e-05
97497,97498,97497,194995,3.189056158065796,6.394866078499578e-05
97698,97699,97698,195397,3.1955173015594482,6.308510441960049e-05
97898,97899,97898,195797,3.201881170272827,6.225594146552387e-05
98098,98099,98098,196197,3.2081589698791504,6.258031710256728e-05
98298,98299,98298,196597,3.2143962383270264,6.078887219511706e-05
98498,98499,98498,196997,3.2206552028656006,7.219631892191601e-05
98699,98700,98699,197399,3.2269272804260254,5.957118753449854e-05
98899,98900,98899,197799,3.233215093612671,5.818650490089061e-05
99099,99100,99099,198199,3.239474296569824,5.772234705375203e-05
99299,99300,99299,198599,3.2458109855651855,5.733891816689826e-05
99499,99500,99499,198999,3.252230167388916,5.679310143579812e-05
99700,99701,99700,199401,3.2585532665252686,5.589199180689728e-05
99900,99901,99900,199801,3.2648260593414307,5.5096813347387144e-05
100100,100101,100100,200201,3.2710251808166504,5.5105111296008415e-05
100300,100301,100300,200601,3.2795610427856445,5.3775951217307354e-05
100501,100502,100501,201003,3.285814046859741,5.3186995594096465e-05
100701,100702,100701,201403,3.292013168334961,5.2409926041677455e-05
100901,100902,100901,201803,3.2982442378997803,5.211240499657924e-05
101101,101102,101101,202203,3.304561138153076,5.5268578510028415e-05
101301,101302,101301,202603,3.310698986053467,5.137427991622855e-05
101502,101503,101502,203005,3.3168561458587646,5.059432072294306e-05
101702,101703,101702,203405,3.3229622840881348,4.957861833512934e-05
101902,101903,101902,203805,3.3289690017700195,4.8562620513266604e-05
102102,102103,102102,204205,3.3352062702178955,4.854316083345967e-05
102302,102303,102302,204605,3.341177225112915,4.785703916139307e-05
102503,102504,102503,205007,3.347104072570801,4.712196574379781e-05
102703,102704,102703,205407,3.3539161682128906,4.665135155718452e-05
102903,102904,102903,205807,3.359771251678467,4.616656785981134e-05
103103,103104,103103,206207,3.365593194961548,4.52280374975071e-05
103303,103304,103303,206607,3.3714041709899902,4.6073519863402534e-05
103504,103505,103504,207009,3.377275228500366,4.403582340013325e-05
103704,103705,103704,207409,3.383070945739746,4.351158994028342e-05
103904,103905,103904,207809,3.388930082321167,4.309094134786419e-05
104104,104105,104104,208209,3.3949902057647705,4.252588963552499e-05
104304,104305,104304,208609,3.4010801315307617,4.177307915906495e-05
104505,104506,104505,209011,3.406954050064087,4.3668813919207046e-05
104705,104706,104705,209411,3.412877082824707,4.148917433418831e-05
104905,104906,104905,209811,3.418684244155884,4.5928592308759736e-05
105105,105106,105105,210211,3.424499034881592,4.000766264082689e-05
105305,105306,105305,210611,3.430953025817871,4.019060407253873e-05
105506,105507,105506,211013,3.4380931854248047,3.8911708274189055e-05
105706,105707,105706,211413,3.445233106613159,3.872882115816259e-05
105906,105907,105906,211813,3.4512581825256348,3.827069540152509e-05
106106,106107,106106,212213,3.457261085510254,3.770132624007468e-05
106306,106307,106306,212613,3.4631459712982178,3.7578655449777765e-05
106507,106508,106507,213015,3.469052314758301,3.705923062485912e-05
106707,106708,106707,213415,3.4749181270599365,3.636644284606308e-05
106907,106908,106907,213815,3.4808361530303955,3.562177507910643e-05
107107,107108,107107,214215,3.4867401123046875,4.3848943151532606e-05
107307,107308,107307,214615,3.4926531314849854,3.47827342380591e-05
107508,107509,107508,215017,3.498617172241211,3.462390382432192e-05
107708,107709,107708,215417,3.5047261714935303,4.28213473909761e-05
107908,107909,107908,215817,3.510730028152466,3.404959035982612e-05
108108,108109,108108,216217,3.5167901515960693,3.3364485604790165e-05
108308,108309,108308,216617,3.5226380825042725,3.3089848135927206e-05
108509,108510,108509,217019,3.5286121368408203,3.2702920526996506e-05
108709,108710,108709,217419,3.5345962047576904,3.202688358113077e-05
108909,108910,108909,217819,3.540553092956543,3.169108456303799e-05
109109,109110,109109,218219,3.5465259552001953,3.106727202455559e-05
109309,109310,109309,218619,3.552489995956421,3.123434240296276e-05
109510,109511,109510,219021,3.5585060119628906,3.0470769327162635e-05
109710,109711,109710,219421,3.5645172595977783,3.056328971259842e-05
109910,109911,109910,219821,3.5704760551452637,3.474455125580427e-05
110110,110111,110110,220221,3.5764710903167725,2.966146983090472e-05
110310,110311,110310,220621,3.5824172496795654,3.0058354929561093e-05
110511,110512,110511,221023,3.5884170532226562,2.9994930553934403e-05
110711,110712,110711,221423,3.5943901538848877,2.850866773231168e-05
110911,110912,110911,221823,3.6003382205963135,2.8966687695429275e-05
111111,111112,111111,222223,3.6064701080322266,2.7753873113852654e-05
111311,111312,111311,222623,3.612459182739258,2.913819180256128e-05
111512,111513,111512,223025,3.618425130844116,2.720032901244792e-05
111712,111713,111712,223425,3.624303102493286,3.527254635160127e-05
111912,111913,111912,223825,3.6301991939544678,2.6573188955485415e-05
112112,112113,112112,224225,3.636188268661499,2.7386693903152526e-05
112312,112313,112312,224625,3.642252206802368,2.692669458841448e-05
112513,112514,112513,225027,3.648280143737793,2.5468334141809556e-05
112713,112714,112713,225427,3.6575632095336914,2.954828118701907e-05
112913,112914,112913,225827,3.663623332977295,2.498792357288694e-05
113113,113114,113113,226227,3.6696691513061523,2.6825328477614437e-05
113313,113314,113313,226627,3.675751209259033,2.4124509843595786e-05
113514,113515,113514,227029,3.6819651126861572,2.424459651637916e-05
113714,113715,113714,227429,3.6880531311035156,2.3399533516611858e-05
113914,113915,113914,227829,3.6941301822662354,2.330232662361915e-05
114114,114115,114114,228229,3.700179100036621,2.295042193018484e-05
114314,114315,114314,228629,3.7063560485839844,2.6908321163074278e-05
114515,114516,114515,229031,3.7125110626220703,2.241655403630026e-05
114715,114716,114715,229431,3.718635082244873,2.2256491350054897e-05
114915,114916,114915,229831,3.724713087081909,2.5344345066696452e-05
115115,115116,115115,230231,3.7307870388031006,2.1508013675113872e-05
115315,115316,115315,230631,3.736887216567993,2.134952274543923e-05
115516,115517,115516,231033,3.743014097213745,2.228620382910377e-05
115716,115717,115716,231433,3.7491400241851807,2.0814184390845635e-05
115916,115917,115916,231833,3.7552552223205566,2.1309382158407383e-05
116116,116117,116116,232233,3.761404275894165,2.0345587945279152e-05
116316,116317,116316,232633,3.767512083053589,2.002633227705324e-05
116517,116518,116517,233035,3.773587942123413,1.9869182414451293e-05
116717,116718,116717,233435,3.779651165008545,1.9413176083698914e-05
116917,116918,116917,233835,3.7857253551483154,2.0462290925340315e-05
117117,117118,117117,234235,3.791776180267334,1.906969198783235e-05
117317,117318,117317,234635,3.7978382110595703,1.8810826179011795e-05
117518,117519,117518,235037,3.804004192352295,1.8695933900566174e-05
117718,117719,117718,235437,3.8101470470428467,1.836449327587319e-05
117918,117919,117918,235837,3.816202163696289,1.808678135474876e-05
118118,118119,118118,236237,3.8220560550689697,2.1611847643001454e-05
118318,118319,118318,236637,3.827883005142212,2.0897739410018463e-05
118519,118520,118519,237039,3.834151268005371,1.7355096755205724e-05
118719,118720,118719,237439,3.842480182647705,1.7384820138524058e-05
118919,118920,118919,237839,3.8509480953216553,2.1026006823525362e-05
119119,119120,119119,238239,3.859036922454834,1.695395693353354e-05
119319,119320,119319,238639,3.865316152572632,1.6731852206706848e-05
119520,119521,119520,239041,3.8714871406555176,1.637029712752614e-05
119720,119721,119720,239441,3.8772571086883545,1.612001197492694e-05
119920,119921,119920,239841,3.883239269256592,1.6010009661206135e-05
120120,120121,120120,240241,3.8890020847320557,1.58445956919048e-05
120320,120321,120320,240641,3.8947551250457764,1.5612302775042657e-05
120521,120522,120521,241043,3.900759220123291,1.5350187566845035e-05
120721,120722,120721,241443,3.9067063331604004,1.517465190706958e-05
120921,120922,120921,241843,3.912750244140625,1.5024878759271466e-05
121121,121122,121121,242243,3.9186482429504395,1.50480287599429e-05
121321,121322,121321,242643,3.9246132373809814,1.4625559609280584e-05
121522,121523,121522,243045,3.9308102130889893,1.657911933826497e-05
121722,121723,121722,243445,3.936967134475708,1.4433596244964465e-05
121922,121923,121922,243845,3.943143129348755,1.4294441349217588e-05
122122,122123,122122,244245,3.9492852687835693,1.6840266045418116e-05
122322,122323,122322,244645,3.955489158630371,1.386687804613045e-05
122523,122524,122523,245047,3.9617180824279785,1.3594014848095107e-05
122723,122724,122723,245447,3.967834234237671,1.3551728317497118e-05
122923,122924,122923,245847,3.973982095718384,1.3675545394091057e-05
123123,123124,123123,246247,3.980159044265747,1.306384251923826e-05
123323,123324,123323,246647,3.9863080978393555,1.28468745301326e-05
123524,123525,123524,247049,3.9924941062927246,1.290271324902128e-05
123724,123725,123724,247449,3.9986531734466553,1.5562843084246013e-05
123924,123925,123924,247849,4.004827260971069,1.2515793326897772e-05
124124,124125,124124,248249,4.011003255844116,1.2390719373172888e-05
124324,124325,124324,248649,4.0171332359313965,1.247873695493349e-05
124525,124526,124525,249051,4.023289203643799,1.2101885616451989e-05
124725,124726,124725,249451,4.029350280761719,1.3521148209225386e-05
124925,124926,124925,249851,4.035176038742065,1.175331646411607e-05
125125,125126,125125,250251,4.041056156158447,1.1600698601489588e-05
125325,125326,125325,250651,4.047062158584595,1.162323479270221e-05
125526,125527,125526,251053,4.053927898406982,1.119264260569039e-05
125726,125727,125726,251453,4.060307025909424,1.1155715348143569e-05
125926,125927,125926,251853,4.066490173339844,1.1049222949602968e-05
126126,126127,126126,252253,4.072695016860962,1.0944826211755985e-05
126326,126327,126326,252653,4.078886270523071,1.0846348237545397e-05
126527,126528,126527,253055,4.085102081298828,1.054502120633906e-05
126727,126728,126727,253455,4.09502100944519,1.0519849149975148e-05
126927,126928,126927,253855,4.101766109466553,1.1942046871093114e-05
127127,127128,127127,254255,4.107816934585571,1.0335252055105219e-05
127327,127328,127327,254655,4.11392617225647,1.0050350536960756e-05
127528,127529,127528,255057,4.120104074478149,9.923345020746319e-06
127728,127729,127728,255457,4.126197099685669,9.875618081208476e-06
127928,127929,127928,255857,4.132596969604492,9.723419365464508e-06
128128,128129,128128,256257,4.138758182525635,1.096515647646657e-05
128328,128329,128328,256657,4.144896030426025,9.517059715686455e-06
128529,128530,128529,257059,4.1511852741241455,9.31962801075557e-06
128729,128730,128729,257459,4.157404899597168,9.18532761173725e-06
128929,128930,128929,257859,4.1637701988220215,1.146658714643614e-05
129129,129130,129129,258259,4.169922113418579,1.0506673231530585e-05
129329,129330,129329,258659,4.1760241985321045,8.922244494345241e-06
129530,129531,129530,259061,4.182181119918823,8.823926217887748e-06
129730,129731,129730,259461,4.188377141952515,1.0319157005358073e-05
129930,129931,129930,259861,4.194831132888794,8.56661989756683e-06
130130,130131,130130,260261,4.201367139816284,8.488683643402174e-06
130330,130331,130330,260661,4.207776069641113,8.473283295257463e-06
130531,130532,130531,261063,4.214083194732666,8.4617440279455e-06
130731,130732,130731,261463,4.220350027084351,8.360511168548996e-06
130931,130932,130931,261863,4.226482152938843,8.05901117691232e-06
131131,131132,131131,262263,4.232638120651245,7.970971311938229e-06
131331,131332,131331,262663,4.238765239715576,7.891508442731263e-06
131532,131533,131532,263065,4.2449259757995605,7.752015173657623e-06
131732,131733,131732,263465,4.2510740756988525,7.704197414257477e-06
131932,131933,131932,263865,4.257220268249512,7.595000315845007e-06
132132,132133,132132,264265,4.26340913772583,7.490861373962019e-06
132332,132333,132332,264665,4.269548177719116,7.328466186137465e-06
132533,132534,132533,265067,4.275717258453369,7.2899212733774555e-06
132733,132734,132733,265467,4.281890153884888,7.5392497369003365e-06
132933,132934,132933,265867,4.287790060043335,7.4199772692693155e-06
133133,133134,133133,266267,4.293699026107788,7.0261546810501935e-06
133333,133334,133333,266667,4.299812078475952,7.955772806194022e-06
133534,133535,133534,267069,4.3059000968933105,6.8509057737080336e-06
133734,133735,133734,267469,4.311847925186157,6.70854441425976e-06
133934,133935,133934,267869,4.31775426864624,8.365562626696814e-06
134134,134135,134134,268269,4.323650121688843,6.584567144068124e-06
134334,134335,134334,268669,4.329766273498535,6.51884302764629e-06
134535,134536,134535,269071,4.33590030670166,6.4202658255237656e-06
134735,134736,134735,269471,4.342056035995483,6.393396225727438e-06
134935,134936,134935,269871,4.348212957382202,6.271155163365352e-06
135135,135136,135135,270271,4.354537010192871,6.254147814229632e-06
135335,135336,135335,270671,4.360960006713867,6.149579909043258e-06
135536,135537,135536,271073,4.3673601150512695,6.138303393905823e-06
135736,135737,135736,271473,4.373855113983154,6.510428564059207e-06
135936,135937,135936,271873,4.380258083343506,5.884439132029822e-06
136136,136137,136136,272273,4.386660099029541,5.8065031798018565e-06
136336,136337,136336,272673,4.393125295639038,5.739152688081443e-06
136537,136538,136537,273075,4.3995561599731445,5.7346005237905015e-06
136737,136738,136737,273475,4.406141996383667,5.593924919731909e-06
136937,136938,136937,273875,4.412703990936279,6.412481238379042e-06
137137,137138,137137,274275,4.41923713684082,5.423667916281992e-06
137337,137338,137337,274675,4.425746917724609,5.473349183677953e-06
137538,137539,137538,275077,4.432325124740601,5.377551891470863e-06
137738,137739,137738,275477,4.438687086105347,5.2434909023115236e-06
137938,137939,137938,275877,4.445166110992432,6.74214092398881e-06
138138,138139,138138,276277,4.451617002487183,5.173359864058756e-06
138338,138339,138338,276677,4.458080053329468,5.055742365243315e-06
138539,138540,138539,277079,4.464656114578247,4.984002108085313e-06
138739,138740,138739,277479,4.471056222915649,5.019733332321473e-06
138939,138940,138939,277879,4.477553129196167,4.971767170451161e-06
139139,139140,139139,278279,4.483901262283325,4.823178154221928e-06
139339,139340,139339,278679,4.49049711227417,4.7895981547007086e-06
139540,139541,139540,279081,4.4968791007995605,4.715265273764784e-06
139740,139741,139740,279481,4.503442287445068,4.655313321042163e-06
139940,139941,139940,279881,4.509963035583496,4.699516933698947e-06
140140,140141,140140,280281,4.516343116760254,4.58924398000537e-06
140340,140341,140340,280681,4.522862195968628,5.068706332521063e-06
140541,140542,140541,281083,4.529538154602051,5.061311297309117e-06
140741,140742,140741,281483,4.535328149795532,4.388482026364389e-06
140941,140942,140941,281883,4.541093111038208,4.3345970408009775e-06
141141,141142,141141,282283,4.547465085983276,4.440333282547334e-06
141341,141342,141341,282683,4.5533833503723145,4.218827422591186e-06
141542,141543,141542,283085,4.5593390464782715,4.190200862463272e-06
141742,141743,141742,283485,4.565205097198486,4.120620571880089e-06
141942,141943,141942,283885,4.572019100189209,4.073015771920886e-06
142142,142143,142142,284285,4.577911138534546,4.013342770070335e-06
142342,142343,142342,284685,4.583944082260132,4.770913384440841e-06
142543,142544,142543,285087,4.59003210067749,3.9008236184263565e-06
142743,142744,142743,285487,4.598098278045654,3.885084015219158e-06
142943,142944,142943,285887,4.604199171066284,3.8445810031004355e-06
143143,143144,143143,286287,4.610411167144775,3.809993652276734e-06
143343,143344,143343,286687,4.616595983505249,3.7391334834528754e-06
143544,143545,143544,287089,4.62282395362854,3.7000508842302033e-06
143744,143745,143744,287489,4.629065036773682,3.632123497121603e-06
143944,143945,143944,287889,4.635249137878418,3.6120553325909824e-06
144144,144145,144144,288289,4.641423225402832,3.551932092419718e-06
144344,144345,144344,288689,4.647565126419067,3.5110613142969814e-06
144545,144546,144545,289091,4.653842210769653,3.848222867860496e-06
144745,144746,144745,289491,4.66016411781311,3.4053739439048227e-06
144945,144946,144945,289891,4.6663031578063965,3.3793475793066097e-06
145145,145146,145145,290291,4.672421216964722,3.352446436964405e-06
145345,145346,145345,290691,4.678701162338257,3.3402537287269003e-06
145546,145547,145546,291093,4.684972047805786,3.2284317991731692e-06
145746,145747,145746,291493,4.691030025482178,3.17424211479885e-06
145946,145947,145946,291893,4.697184085845947,3.197142763114319e-06
146146,146147,146146,292293,4.70408821105957,3.19394941156465e-06
146346,146347,146346,292693,4.710229158401489,3.097795956795957e-06
146547,146548,146547,293095,4.716462135314941,3.039755019363212e-06
146747,146748,146747,293495,4.7242591381073,3.3030844010869067e-06
146947,146948,146947,293895,4.730990171432495,2.961163347373841e-06
147147,147148,147147,294295,4.737912178039551,2.967744033289512e-06
147347,147348,147347,294695,4.745345115661621,2.8899467973009833e-06
147548,147549,147548,295097,4.753355979919434,2.859079692284836e-06
147748,147749,147748,295497,4.760982036590576,2.8976315906809044e-06
147948,147949,147948,295897,4.7681663036346436,3.3605816146949385e-06
148148,148149,148148,296297,4.774352312088013,3.237954533346689e-06
148348,148349,148348,296697,4.780794143676758,3.2482034431127943e-06
148549,148550,148549,297099,4.786880016326904,2.830747079371265e-06
148749,148750,148749,297499,4.792908191680908,2.673700611277856e-06
148949,148950,148949,297899,4.799045085906982,2.615626146911646e-06
149149,149150,149149,298299,4.805889129638672,2.9829516842277067e-06
149349,149350,149349,298699,4.8126232624053955,2.53642219448654e-06
149550,149551,149550,299101,4.818977117538452,2.998802579479081e-06
149750,149751,149750,299501,4.825067043304443,2.494878586832314e-06
149950,149951,149950,299901,4.831374168395996,2.9105847011236554e-06
150150,150151,150150,300301,4.8377039432525635,2.4277686099235643e-06
150350,150351,150350,300701,4.843707084655762,2.8060586132497682e-06
150551,150552,150551,301103,4.849789142608643,2.363427567667155e-06
150751,150752,150751,301503,4.856857061386108,2.6923195540671134e-06
150951,150952,150951,301903,4.863542079925537,2.3283176914638506e-06
151151,151152,151151,302303,4.870505094528198,2.283739549533846e-06
151351,151352,151351,302703,4.877261161804199,2.2484880411304065e-06
151552,151553,151552,303105,4.885561227798462,2.234059714006241e-06
151752,151753,151752,303505,4.893440008163452,2.2022414402834065e-06
151952,151953,151952,303905,4.9014573097229,2.1741615529572465e-06
152152,152153,152152,304305,4.909405946731567,2.1464236162344803e-06
152352,152353,152352,304705,4.9175660610198975,2.1031574710253403e-06
152553,152554,152553,305107,4.925073146820068,2.551874751533831e-06
152753,152754,152753,305507,4.933286190032959,2.0574818868659264e-06
152953,152954,152953,305907,4.9410319328308105,2.346427881541085e-06
153153,153154,153153,306307,4.949027061462402,2.137233236214591e-06
153353,153354,153353,306707,4.956990003585815,1.994963731213789e-06
153554,153555,153554,307109,4.964978933334351,1.968880771602553e-06
153754,153755,153754,307509,4.973129034042358,1.9324281456758936e-06
153954,153955,153954,307909,4.981215000152588,2.3671340526462756e-06
154154,154155,154154,308309,4.990375280380249,2.2610350557841944e-06
154354,154355,154354,308709,4.998662233352661,1.8784118855223107e-06
154555,154556,154555,309111,5.006860017776489,1.8496738024470624e-06
154755,154756,154755,309511,5.014652252197266,1.8151121406234122e-06
154955,154956,154955,309911,5.023101329803467,1.968086791684213e-06
155155,155156,155155,310311,5.030726194381714,1.7737582537384079e-06
155355,155356,155355,310711,5.038386344909668,1.9835721929413127e-06
155556,155557,155556,311113,5.046025991439819,1.7369805801229169e-06
155756,155757,155756,311513,5.053798198699951,1.7885391550510047e-06
155956,155957,155956,311913,5.061748027801514,1.68347554804395e-06
156156,156157,156156,312313,5.0694310665130615,1.6674199242076368e-06
156356,156357,156356,312713,5.076279163360596,1.6466532173931244e-06
156557,156558,156557,313115,5.082428216934204,1.61536966216874e-06
156757,156758,156757,313515,5.088503122329712,1.6021300591682864e-06
156957,156958,156957,313915,5.0945680141448975,1.6893344748700593e-06
157157,157158,157157,314315,5.100626230239868,1.6191117435629707e-06
157357,157358,157357,314715,5.106697082519531,1.562033313571096e-06
157558,157559,157558,315117,5.112784147262573,1.5328476799195055e-06
157758,157759,157758,315517,5.118851184844971,1.5130510981739198e-06
157958,157959,157958,315917,5.124872922897339,1.7290611386089624e-06
158158,158159,158158,316317,5.1309661865234375,1.46501212005396e-06
158358,158359,158358,316717,5.137024164199829,1.4563921570041354e-06
158559,158560,158559,317119,5.143101930618286,1.4542300765195218e-06
158759,158760,158759,317519,5.150060176849365,1.4213859507896502e-06
158959,158960,158959,317919,5.157613039016724,1.4095916280691822e-06
159159,159160,159159,318319,5.16532826423645,1.3954067021797025e-06
159359,159360,159359,318719,5.173116207122803,1.6772137098729567e-06
159560,159561,159560,319121,5.181244134902954,1.3542034694982418e-06
159760,159761,159760,319521,5.1894001960754395,1.4573683692941357e-06
159960,159961,159960,319921,5.1975202560424805,1.331437208276086e-06
160160,160161,160160,320321,5.20563817024231,1.6428597100288522e-06
160360,160361,160360,320721,5.213794231414795,1.2984642158865822e-06
160561,160562,160561,321123,5.225613117218018,1.2669788269047665e-06
160761,160762,160761,321523,5.233213186264038,1.3132955286524731e-06
160961,160962,160961,321923,5.240850210189819,1.2465015709764924e-06
161161,161162,161161,322323,5.2484331130981445,1.3406194964583646e-06
161361,161362,161361,322723,5.256340980529785,1.2053634081761273e-06
161562,161563,161562,323125,5.264438152313232,1.3571751035262797e-06
161762,161763,161762,323525,5.27230429649353,1.248878487083569e-06
161962,161963,161962,323925,5.279918193817139,1.197208976758363e-06
162162,162163,162162,324325,5.287299156188965,1.1458463393167003e-06
162362,162363,162362,324725,5.293652057647705,1.344090913449894e-06
162563,162564,162563,325127,5.299865245819092,1.119110618503614e-06
162763,162764,162763,325527,5.305885076522827,1.1200603813220862e-06
162963,162964,162963,325927,5.311923980712891,1.1262495678177784e-06
163163,163164,163163,326327,5.317935228347778,1.2548785122388447e-06
163363,163364,163363,326727,5.324733257293701,1.292027461340207e-06
163564,163565,163564,327129,5.331108093261719,1.3931481982201172e-06
163764,163765,163764,327529,5.337768077850342,1.0382828333757645e-06
163964,163965,163964,327929,5.3447980880737305,1.0457599169050823e-06
164164,164165,164164,328329,5.351647138595581,1.0243123953904081e-06
164364,164365,164364,328729,5.357709169387817,1.0620999518342926e-06
164565,164566,164565,329131,5.36378026008606,1.0171395196515647e-06
164765,164766,164765,329531,5.369803190231323,9.78434379225609e-07
164965,164966,164965,329931,5.375805139541626,9.759547907064413e-07
165165,165166,165165,330331,5.381813049316406,9.490796058146061e-07
165365,165366,165365,330731,5.387921333312988,9.45279582051734e-07
165566,165567,165566,331133,5.39406418800354,9.345157961627962e-07
165766,165767,165766,331533,5.400205135345459,9.168052212886356e-07
165966,165967,165966,331933,5.4062793254852295,9.278282129484127e-07
166166,166167,166166,332333,5.4124181270599365,1.0460973403195052e-06
166366,166367,166366,332733,5.418597221374512,8.778413981244975e-07
166567,166568,166567,333135,5.424782037734985,8.778898825139203e-07
166767,166768,166767,333535,5.430952072143555,8.808894429789593e-07
166967,166968,166967,333935,5.437195062637329,8.495609618667069e-07
167167,167168,167167,334335,5.443427085876465,1.0094049328793677e-06
167367,167368,167367,334735,5.4497292041778564,8.316559811955034e-07
167568,167569,167568,335137,5.456059217453003,8.218904686485549e-07
167768,167769,167768,335537,5.46242094039917,8.120137382530798e-07
167968,167969,167968,335937,5.46867299079895,7.970908162706626e-07
168168,168169,168168,336337,5.47487211227417,7.953190319185381e-07
168368,168369,168368,336737,5.481028079986572,9.39905743269962e-07
168569,168570,168569,337139,5.487243175506592,7.718475317865905e-07
168769,168770,168769,337539,5.493648290634155,8.91157684551756e-07
168969,168970,168969,337939,5.500146150588989,7.541180676129317e-07
169169,169170,169169,338339,5.506546974182129,7.500848356316353e-07
169369,169370,169369,338739,5.5129311084747314,7.339631641192981e-07
169570,169571,169570,339141,5.519313335418701,7.308450518671074e-07
169770,169771,169770,339541,5.525588035583496,7.178497791147157e-07
169970,169971,169970,339941,5.532067060470581,7.486589759345663e-07
170170,170171,170170,340341,5.53825831413269,6.960131782114839e-07
170370,170371,170370,340741,5.544412136077881,6.86722926116795e-07
170571,170572,170571,341143,5.550616025924683,6.811976381023194e-07
170771,170772,170771,341543,5.556886196136475,6.805455807747027e-07
170971,170972,170971,341943,5.5633580684661865,6.678455032439412e-07
171171,171172,171171,342343,5.569498062133789,6.530564376657056e-07
171371,171372,171371,342743,5.575593948364258,6.485015371476206e-07
171572,171573,171572,343145,5.581716060638428,6.426672148283572e-07
171772,171773,171772,343545,5.587815999984741,6.347377928410968e-07
171972,171973,171972,343945,5.593919038772583,6.27111119403621e-07
172172,172173,172172,344345,5.6000142097473145,6.204442704316087e-07
172372,172373,172372,344745,5.6060991287231445,6.13033643265527e-07
172573,172574,172573,345147,5.612231969833374,5.980237746988858e-07
172773,172774,172773,345547,5.618337154388428,5.930146587211975e-07
172973,172974,172973,345947,5.62444806098938,5.873739226775485e-07
173173,173174,173173,346347,5.630995035171509,5.826534659390437e-07
173373,173374,173373,346747,5.637484073638916,5.794831750739887e-07
173574,173575,173574,347149,5.644047260284424,6.547062833364874e-07
173774,173775,173774,347549,5.650547027587891,6.881114201570369e-07
173974,173975,173974,347949,5.657111167907715,5.521908981494015e-07
174174,174175,174174,348349,5.663625955581665,5.477814374748971e-07
174374,174375,174374,348749,5.6701672077178955,5.344290551061449e-07
174575,174576,174575,349151,5.676798105239868,5.342960747959366e-07
174775,174776,174775,349551,5.68330717086792,5.298027510612111e-07
174975,174976,174975,349951,5.689774036407471,5.184292629104269e-07
175175,175176,175175,350351,5.696272134780884,6.095993248871051e-07
175375,175376,175375,350751,5.702808141708374,5.166601427492001e-07
175576,175577,175576,351153,5.709398031234741,4.98134045355357e-07
175776,175777,175776,351553,5.715980052947998,5.116180425154327e-07
175976,175977,175976,351953,5.722454071044922,4.886084990056159e-07
176176,176177,176176,352353,5.728446960449219,4.808971776330483e-07
176376,176377,176376,352753,5.734360218048096,4.859343476601997e-07
176577,176578,176577,353155,5.740240097045898,6.414223658683409e-07
176777,176778,176777,353555,5.7461230754852295,5.40137746254862e-07
176977,176978,176977,353955,5.7519659996032715,4.955800923109687e-07
177177,177178,177177,354355,5.757861137390137,5.385386015199274e-07
177377,177378,177377,354755,5.7637622356414795,4.4587948199326497e-07
177578,177579,177578,355157,5.769626140594482,4.434486968134825e-07
177778,177779,177778,355557,5.775459051132202,4.3482492581524586e-07
177978,177979,177978,355957,5.781702280044556,4.319369821179904e-07
178178,178179,178178,356357,5.787539005279541,4.242385340512532e-07
178378,178379,178378,356757,5.793363094329834,4.278421962978861e-07
178579,178580,178579,357159,5.799211025238037,4.162362849203681e-07
178779,178780,178779,357559,5.805069208145142,4.1271525490493114e-07
178979,178980,178979,357959,5.81104302406311,4.0296546973945234e-07
179179,179180,179179,358359,5.8168933391571045,3.9628408734877e-07
179379,179380,179379,358759,5.822747230529785,4.2208390915807247e-07
179580,179581,179580,359161,5.828995227813721,3.8689081680679643e-07
179780,179781,179780,359561,5.836150169372559,3.881880200227472e-07
179980,179981,179980,359961,5.842638254165649,4.4542765894237637e-07
180180,180181,180180,360361,5.850030183792114,3.7380654365853925e-07
180380,180381,180380,360761,5.857254266738892,3.704341157529024e-07
180581,180582,180581,361163,5.8675782680511475,3.730772609061645e-07
180781,180782,180781,361563,5.873530149459839,3.579674960644339e-07
180981,180982,180981,361963,5.879508018493652,4.2248612024190485e-07
181181,181182,181181,362363,5.885439157485962,3.535832058701111e-07
181381,181382,181381,362763,5.891407251358032,3.4396941058582573e-07
181582,181583,181582,363165,5.897385120391846,3.4600245311618503e-07
181782,181783,181782,363565,5.903462171554565,3.380894901256528e-07
181982,181983,181982,363965,5.909440994262695,3.36216238015233e-07
182182,182183,182182,364365,5.915408134460449,3.270776820703556e-07
182382,182383,182382,364765,5.921365022659302,3.2487487109541917e-07
182583,182584,182583,365167,5.927370071411133,3.227232376907563e-07
182783,182784,182783,365567,5.9340691566467285,3.164472051039615e-07
182983,182984,182983,365967,5.940091133117676,3.14998162035889e-07
183183,183184,183183,366367,5.946025133132935,3.1032618997181164e-07
183383,183384,183383,366767,5.9525229930877686,3.34378598861427e-07
183584,183585,183584,367169,5.958611011505127,3.0066649403855614e-07
183784,183785,183784,367569,5.964915990829468,3.386459294131175e-07
183984,183985,183984,367969,5.9712841510772705,3.127985014054831e-07
184184,184185,184184,368369,5.977713108062744,2.903378903689313e-07
184384,184385,184384,368769,5.983988046646118,2.8663279251171254e-07
184585,184586,184585,369171,5.990061044692993,2.813705481461798e-07
184785,184786,184785,369571,5.996148109436035,2.81816944899207e-07
184985,184986,184985,369971,6.002306222915649,2.788483366068662e-07
185185,185186,185185,370371,6.008733034133911,2.7147854038216606e-07
185385,185386,185385,370771,6.015594005584717,2.71399080225899e-07
185586,185587,185586,371173,6.021989107131958,2.663955081024296e-07
185786,185787,185786,371573,6.028144121170044,2.6396369554276765e-07
185986,185987,185986,371973,6.034408092498779,2.612937017011231e-07
186186,186187,186186,372373,6.040472030639648,2.572260469374294e-07
186386,186387,186386,372773,6.0468971729278564,2.536160903215391e-07
186587,186588,186587,373175,6.053547143936157,2.521241032429757e-07
186787,186788,186787,373575,6.060148000717163,2.4707117246757094e-07
186987,186988,186987,373975,6.066766262054443,2.4805714759952017e-07
187187,187188,187187,374375,6.0734169483184814,2.3930966323112394e-07
187387,187388,187387,374775,6.080028295516968,2.401936639844254e-07
187588,187589,187588,375177,6.08669900894165,2.345962781146952e-07
187788,187789,187788,375577,6.0932652950286865,2.3726606208443758e-07
187988,187989,187988,375977,6.099858999252319,2.3050344234547178e-07
188188,188189,188188,376377,6.1064441204071045,2.2582922485090693e-07
188388,188389,188388,376777,6.113084316253662,2.222927340122151e-07
188589,188590,188589,377179,6.119699954986572,2.3106134090567354e-07
188789,188790,188789,377579,6.126265048980713,2.1717638417812283e-07
188989,188990,188989,377979,6.1328771114349365,2.1502886576686213e-07
189189,189190,189189,378379,6.139456033706665,2.1506718352039058e-07
189389,189390,189389,378779,6.146022319793701,2.5062477535138634e-07
189590,189591,189590,379181,6.152720212936401,2.0690793751832288e-07
189790,189791,189790,379581,6.1593310832977295,2.0866425024417212e-07
189990,189991,189990,379981,6.1659791469573975,2.157410786036651e-07
190190,190191,190190,380381,6.17253303527832,2.001656954132337e-07
190390,190391,190390,380781,6.179088115692139,2.0230920898347357e-07
190591,190592,190591,381183,6.185680150985718,1.9641112258544531e-07
190791,190792,190791,381583,6.192276954650879,1.936086054896392e-07
190991,190992,190991,381983,6.198849201202393,2.3792766872551678e-07
191191,191192,191191,382383,6.20542311668396,2.2717787603018825e-07
191391,191392,191391,382783,6.212013006210327,1.847849098733806e-07
191592,191593,191592,383185,6.218583106994629,1.83047528401909e-07
191792,191793,191792,383585,6.225100040435791,1.7996793750428577e-07
191992,191993,191992,383985,6.231601238250732,1.8480635534904752e-07
192192,192193,192192,384385,6.238171100616455,2.0583636510478517e-07
192392,192393,192392,384785,6.2447521686553955,1.7426141188622477e-07
192593,192594,192593,385187,6.251334190368652,1.726980655669138e-07
192793,192794,192793,385587,6.257974147796631,1.9894162122399899e-07
192993,192994,192993,385987,6.264592170715332,1.721460141068036e-07
193193,193194,193193,386387,6.2713470458984375,1.6536183881732199e-07
193393,193394,193393,386787,6.277925252914429,1.6359554968959807e-07
193594,193595,193594,387189,6.284540176391602,1.6198052573489364e-07
193794,193795,193794,387589,6.2910919189453125,1.61210544363033e-07
193994,193995,193994,387989,6.297656059265137,1.5978896186107317e-07
194194,194195,194194,388389,6.304479122161865,1.5803353896488735e-07
194394,194395,194394,388789,6.311105012893677,1.651762119422239e-07
194595,194596,194595,389191,6.317719221115112,1.5204052372855503e-07
194795,194796,194795,389591,6.3243491649627686,1.5230291389973712e-07
194995,194996,194995,389991,6.330897331237793,1.4749212025377241e-07
195195,195196,195195,390391,6.337467193603516,1.4646330285967154e-07
195395,195396,195395,390791,6.3440330028533936,1.4493927597843125e-07
195596,195597,195596,391193,6.350476026535034,1.4611117054541662e-07
195796,195797,195796,391593,6.356771230697632,1.4086911669171404e-07
195996,195997,195996,391993,6.362819194793701,1.4039907603303907e-07
196196,196197,196196,392393,6.369241237640381,1.7611143306998492e-07
196396,196397,196396,392793,6.3754072189331055,1.3591732837203612e-07
196597,196598,196597,393195,6.381468296051025,1.3609154087814068e-07
196797,196798,196797,393595,6.387593984603882,1.5129802630800884e-07
196997,196998,196997,393995,6.393568992614746,1.4386110121848454e-07
197197,197198,197197,394395,6.400371074676514,1.2859402023238371e-07
197397,197398,197397,394795,6.406495094299316,1.3366788903621074e-07
197598,197599,197598,395197,6.412689208984375,1.2688246889409319e-07
197798,197799,197798,395597,6.418874263763428,1.4237206487837949e-07
197998,197999,197998,395997,6.4250853061676025,1.2534540830501232e-07
198198,198199,198198,396397,6.431403160095215,1.218021094035284e-07
198398,198399,198398,396797,6.437704086303711,1.2737020783306333e-07
198599,198600,198599,397199,6.443819999694824,1.197261432476724e-07
198799,198800,198799,397599,6.450104236602783,1.2194609640495158e-07
198999,199000,198999,397999,6.456501007080078,1.1453764526183931e-07
199199,199200,199199,398399,6.462824106216431,1.1477509256293478e-07
199399,199400,199399,398799,6.469006061553955,1.1887058164038474e-07
199600,199601,199600,399201,6.475252151489258,1.1234135752323488e-07
199800,199801,199800,399601,6.481571197509766,1.093100178755101e-07
200000,200001,200000,400001,6.487688064575195,1.0866655368965862e-07


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/eag-c.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00020599365234375,4.387072431292609
100,201,0,201,0.006331920623779297,1.0665443360783584
200,401,0,401,0.01179814338684082,0.4043848940096791
300,601,0,601,0.01671910285949707,0.3037256513010002
400,801,0,801,0.02155017852783203,0.21227736203975886
501,1003,0,1003,0.026380062103271484,0.1713519080960906
601,1203,0,1203,0.031150102615356445,0.14928003567712142
701,1403,0,1403,0.03576183319091797,0.12137429974972368
801,1603,0,1603,0.040251970291137695,0.10171803824306211
901,1803,0,1803,0.044178009033203125,0.08906050214503931
1001,2003,0,2003,0.04797005653381348,0.08233857129632127
1101,2203,0,2203,0.05176997184753418,0.08191750433497302
1201,2403,0,2403,0.055808067321777344,0.061593030578000016
1301,2603,0,2603,0.05958890914916992,0.06914220766792943
1401,2803,0,2803,0.06345081329345703,0.0586838214605921
1502,3005,0,3005,0.06720304489135742,0.06233212960539554
1602,3205,0,3205,0.07085704803466797,0.05265842431863991
1702,3405,0,3405,0.07465291023254395,0.046996663053960774
1802,3605,0,3605,0.07829403877258301,0.05056909097153807
1902,3805,0,3805,0.08194208145141602,0.04476072777685633
2002,4005,0,4005,0.08572697639465332,0.041527156932835624
2102,4205,0,4205,0.09007692337036133,0.04040439442284881
2202,4405,0,4405,0.09400296211242676,0.03816373522257505
2302,4605,0,4605,0.09813404083251953,0.03972775316304948
2402,4805,0,4805,0.10270214080810547,0.03598618678174246
2503,5007,0,5007,0.10686302185058594,0.03408181646602452
2603,5207,0,5207,0.11076879501342773,0.03336734604469102
2703,5407,0,5407,0.11461210250854492,0.03269156365903751
2803,5607,0,5607,0.11821389198303223,0.031075952608860105
2903,5807,0,5807,0.12191200256347656,0.026396451665066812
3003,6007,0,6007,0.12561583518981934,0.029108798230438118
3103,6207,0,6207,0.12943315505981445,0.025935621345224893
3203,6407,0,6407,0.13337087631225586,0.027208639669736034
3303,6607,0,6607,0.1373310089111328,0.024079134693056833
3403,6807,0,6807,0.1416001319885254,0.02381717386131816
3504,7009,0,7009,0.14567184448242188,0.02488859104687067
3604,7209,0,7209,0.14948701858520508,0.02239884072798269
3704,7409,0,7409,0.15336203575134277,0.021339136634859323
3804,7609,0,7609,0.15718507766723633,0.020310339504418067
3904,7809,0,7809,0.16113519668579102,0.01975540475030197
4004,8009,0,8009,0.16489195823669434,0.019989282796115032
4104,8209,0,8209,0.16865205764770508,0.01742161430226497
4204,8409,0,8409,0.17271089553833008,0.018091804598004163
4304,8609,0,8609,0.17642712593078613,0.017437357656163884
4404,8809,0,8809,0.1801300048828125,0.018375298536051618
4505,9011,0,9011,0.18388986587524414,0.016121970040532493
4605,9211,0,9211,0.1877450942993164,0.016041963127096742
4705,9411,0,9411,0.19188785552978516,0.01602804982848922
4805,9611,0,9611,0.19617009162902832,0.01532893267477553
4905,9811,0,9811,0.19998788833618164,0.014859385705389836
5005,10011,0,10011,0.20383906364440918,0.013690398322403189
5105,10211,0,10211,0.20784497261047363,0.014041328423962104
5205,10411,0,10411,0.2117629051208496,0.014814579509148792
5305,10611,0,10611,0.21607613563537598,0.013608782861523958
5405,10811,0,10811,0.21987295150756836,0.013792742261871178
5506,11013,0,11013,0.2236170768737793,0.01356600599771525
5606,11213,0,11213,0.227463960647583,0.01391757820023729
5706,11413,0,11413,0.23111701011657715,0.01334828483550954
5806,11613,0,11613,0.2347710132598877,0.012523254102915486
5906,11813,0,11813,0.23870587348937988,0.012638187260244318
6006,12013,0,12013,0.24260306358337402,0.01278900089713829
6106,12213,0,12213,0.24686217308044434,0.012812109991528457
6206,12413,0,12413,0.2506840229034424,0.012145655716269544
6306,12613,0,12613,0.2552671432495117,0.012499084650217753
6406,12813,0,12813,0.25907206535339355,0.012850329986397329
6507,13015,0,13015,0.262829065322876,0.012540191102228926
6607,13215,0,13215,0.26653504371643066,0.012335295680174994
6707,13415,0,13415,0.2706129550933838,0.011776097120117483
6807,13615,0,13615,0.2744021415710449,0.012095884072375579
6907,13815,0,13815,0.27825093269348145,0.01196447816127861
7007,14015,0,14015,0.28200197219848633,0.011295828059595675
7107,14215,0,14215,0.28583407402038574,0.011423637654259524
7207,14415,0,14415,0.2905759811401367,0.01145855019705569
7307,14615,0,14615,0.2946200370788574,0.011680890598844773
7407,14815,0,14815,0.2984440326690674,0.011261977053317994
7508,15017,0,15017,0.30297183990478516,0.011042851984904347
7608,15217,0,15217,0.3069570064544678,0.011027691956134815
7708,15417,0,15417,0.311492919921875,0.010944945605208707
7808,15617,0,15617,0.31609606742858887,0.010500237738669477
7908,15817,0,15817,0.32085514068603516,0.009988836466327282
8008,16017,0,16017,0.32564306259155273,0.01010359663388243
8108,16217,0,16217,0.33031606674194336,0.010084120453508878
8208,16417,0,16417,0.33524203300476074,0.009813928371121798
8308,16617,0,16617,0.3399159908294678,0.009654937242058194
8408,16817,0,16817,0.345304012298584,0.009470216265290928
8509,17019,0,17019,0.3500649929046631,0.009662644185313011
8609,17219,0,17219,0.35465002059936523,0.009253328377386294
8709,17419,0,17419,0.35962796211242676,0.008781181360634363
8809,17619,0,17619,0.36448216438293457,0.00863967708134135
8909,17819,0,17819,0.3693702220916748,0.00855564882190571
9009,18019,0,18019,0.37421202659606934,0.008376388418705475
9109,18219,0,18219,0.3791990280151367,0.008042668608496815
9209,18419,0,18419,0.38396596908569336,0.007988637880765745
9309,18619,0,18619,0.38874292373657227,0.008127833753650802
9409,18819,0,18819,0.3941471576690674,0.00806870102553144
9510,19021,0,19021,0.3992791175842285,0.0077703526949124595
9610,19221,0,19221,0.40404415130615234,0.0075269210373787865
9710,19421,0,19421,0.40952491760253906,0.007612854848940511
9810,19621,0,19621,0.41414594650268555,0.007402934480566772
9910,19821,0,19821,0.4187610149383545,0.007137371588020664
10010,20021,0,20021,0.42337512969970703,0.007002868188865024
10110,20221,0,20221,0.4279799461364746,0.007070565082986567
10210,20421,0,20421,0.4328179359436035,0.007259282933053504
10310,20621,0,20621,0.43740105628967285,0.0070931379165547394
10410,20821,0,20821,0.44208407402038574,0.0070246710372417285
10511,21023,0,21023,0.4466109275817871,0.007135187116885399
10611,21223,0,21223,0.45094990730285645,0.007142362344751027
10711,21423,0,21423,0.4557199478149414,0.006978302090438743
10811,21623,0,21623,0.4602789878845215,0.0067710138596092494
10911,21823,0,21823,0.46456098556518555,0.006804903039138827
11011,22023,0,22023,0.4683840274810791,0.0068949303370660605
11111,22223,0,22223,0.47208094596862793,0.006878272504728402
11211,22423,0,22423,0.47579503059387207,0.006805021875594198
11311,22623,0,22623,0.4797849655151367,0.006898933668830561
11411,22823,0,22823,0.4838850498199463,0.007072103364232585
11512,23025,0,23025,0.4876830577850342,0.006986509657554643
11612,23225,0,23225,0.4915609359741211,0.006867588994009879
11712,23425,0,23425,0.49531102180480957,0.006794629695377734
11812,23625,0,23625,0.49916696548461914,0.006811378879244095
11912,23825,0,23825,0.5029189586639404,0.006775875461716418
12012,24025,0,24025,0.5069580078125,0.006613004642975174
12112,24225,0,24225,0.5107951164245605,0.006614899502687346
12212,24425,0,24425,0.5147030353546143,0.00672756497217622
12312,24625,0,24625,0.5184340476989746,0.006742453412286656
12412,24825,0,24825,0.5221350193023682,0.0066480241698004825
12513,25027,0,25027,0.5260579586029053,0.0065593001805355254
12613,25227,0,25227,0.5297799110412598,0.006554614162620634
12713,25427,0,25427,0.5336110591888428,0.006472341040534518
12813,25627,0,25627,0.5373680591583252,0.0062926941395239884
12913,25827,0,25827,0.5415518283843994,0.0061275500197760895
13013,26027,0,26027,0.54526686668396,0.0061271455076797425
13113,26227,0,26227,0.5489778518676758,0.006134622979855065
13213,26427,0,26427,0.5526840686798096,0.006024894061617505
13313,26627,0,26627,0.5564939975738525,0.005953236452739838
13413,26827,0,26827,0.5602660179138184,0.00593420480897846
13514,27029,0,27029,0.5644569396972656,0.005909614789440949
13614,27229,0,27229,0.5681540966033936,0.005766516899424258
13714,27429,0,27429,0.5718550682067871,0.005553085856832774
13814,27629,0,27629,0.5756030082702637,0.005467213228234064
13914,27829,0,27829,0.5792980194091797,0.005419666878266805
14014,28029,0,28029,0.5831749439239502,0.005312448436598062
14114,28229,0,28229,0.5869150161743164,0.005198705856801084
14214,28429,0,28429,0.5906550884246826,0.005186921295217133
14314,28629,0,28629,0.5943968296051025,0.005230433421113172
14414,28829,0,28829,0.5982930660247803,0.0051866974255970885
14515,29031,0,29031,0.6021051406860352,0.005065163136182162
14615,29231,0,29231,0.6057770252227783,0.004972098121249699
14715,29431,0,29431,0.6096639633178711,0.004952967693699861
14815,29631,0,29631,0.613684892654419,0.004871516834848687
14915,29831,0,29831,0.6180479526519775,0.004739281924386812
15015,30031,0,30031,0.6217830181121826,0.004705354071491604
15115,30231,0,30231,0.6256451606750488,0.004754867436692766
15215,30431,0,30431,0.6297070980072021,0.004803819493196498
15315,30631,0,30631,0.6335539817810059,0.004780552583254227
15415,30831,0,30831,0.6372060775756836,0.004759276388593549
15516,31033,0,31033,0.6412539482116699,0.004804613937714447
15616,31233,0,31233,0.6449310779571533,0.00480160906010214
15716,31433,0,31433,0.6489138603210449,0.004719762963471144
15816,31633,0,31633,0.6525900363922119,0.00464990474195754
15916,31833,0,31833,0.6567990779876709,0.00466732561207649
16016,32033,0,32033,0.660506010055542,0.004708872997249917
16116,32233,0,32233,0.6646349430084229,0.004711773320950185
16216,32433,0,32433,0.6683950424194336,0.004716906262737957
16316,32633,0,32633,0.6725058555603027,0.0047757029273886
16416,32833,0,32833,0.6763269901275635,0.004842870464171625
16517,33035,0,33035,0.6803641319274902,0.004821471405621731
16617,33235,0,33235,0.6844749450683594,0.004759799378513179
16717,33435,0,33435,0.6883730888366699,0.004739996530292616
16817,33635,0,33635,0.6923689842224121,0.004734997678963205
16917,33835,0,33835,0.6964371204376221,0.004705931398490438
17017,34035,0,34035,0.7004668712615967,0.004658571905748072
17117,34235,0,34235,0.7045948505401611,0.004665907532615986
17217,34435,0,34435,0.7085740566253662,0.004719482785742899
17317,34635,0,34635,0.712155818939209,0.00472829744303786
17417,34835,0,34835,0.7161788940429688,0.004686039169487886
17518,35037,0,35037,0.7198519706726074,0.004649545633938963
17618,35237,0,35237,0.7243080139160156,0.004629218708250144
17718,35437,0,35437,0.7279260158538818,0.004571707860271163
17818,35637,0,35637,0.7319061756134033,0.004475630436789604
17918,35837,0,35837,0.7356789112091064,0.004404129163616312
18018,36037,0,36037,0.7396202087402344,0.004389765931005424
18118,36237,0,36237,0.7433888912200928,0.0043828957989951196
18218,36437,0,36437,0.7472879886627197,0.0043365072490303865
18318,36637,0,36637,0.7511820793151855,0.004297993031085548
18418,36837,0,36837,0.7550652027130127,0.004286435521387073
18519,37039,0,37039,0.7589881420135498,0.0042495757352079624
18619,37239,0,37239,0.762714147567749,0.004161544365109822
18719,37439,0,37439,0.7667357921600342,0.004056594586943836
18819,37639,0,37639,0.7704670429229736,0.003993675384305692
18919,37839,0,37839,0.7744059562683105,0.003953887279440949
19019,38039,0,38039,0.7781178951263428,0.003893904654458814
19119,38239,0,38239,0.7820768356323242,0.00384252747039768
19219,38439,0,38439,0.7865641117095947,0.003838514292745753
19319,38639,0,38639,0.791205883026123,0.003849363554465216
19419,38839,0,38839,0.7950100898742676,0.003818720750678488
19520,39041,0,39041,0.7992420196533203,0.00375574023968879
19620,39241,0,39241,0.8034958839416504,0.0037067565424039254
19720,39441,0,39441,0.8078889846801758,0.003675353960046598
19820,39641,0,39641,0.8120582103729248,0.003625559356444488
19920,39841,0,39841,0.8160839080810547,0.00356411894402922
20020,40041,0,40041,0.8201079368591309,0.003550433197617234
20120,40241,0,40241,0.8239810466766357,0.003580706030900932
20220,40441,0,40441,0.8276689052581787,0.0036029431285344595
20320,40641,0,40641,0.8316328525543213,0.0036017159467801717
20420,40841,0,40841,0.8353757858276367,0.003602901079325168
20521,41043,0,41043,0.839155912399292,0.003618723526983722
20621,41243,0,41243,0.8431539535522461,0.0036118279084259887
20721,41443,0,41443,0.8469669818878174,0.0035708964820438034
20821,41643,0,41643,0.8508849143981934,0.0035419596328997295
20921,41843,0,41843,0.854640007019043,0.0035530887763210285
21021,42043,0,42043,0.859065055847168,0.003576275418759701
21121,42243,0,42243,0.8627579212188721,0.0035875671678253364
21221,42443,0,42443,0.8665862083435059,0.0036064166339811734
21321,42643,0,42643,0.8704619407653809,0.003645217858188393
21421,42843,0,42843,0.8743031024932861,0.0036762453972208147
21522,43045,0,43045,0.878087043762207,0.0036681969235645793
21622,43245,0,43245,0.8826601505279541,0.0036396635026805
21722,43445,0,43445,0.886430025100708,0.003626875248367201
21822,43645,0,43645,0.8902640342712402,0.0036206297967762667
21922,43845,0,43845,0.8940348625183105,0.003602588496770977
22022,44045,0,44045,0.8982889652252197,0.0035871845989075015
22122,44245,0,44245,0.9020609855651855,0.0035979149157709766
22222,44445,0,44445,0.9057819843292236,0.0036239238012852884
22322,44645,0,44645,0.9097900390625,0.003628814163858306
22422,44845,0,44845,0.9136099815368652,0.0036082656577017453
22523,45047,0,45047,0.9177210330963135,0.003586287286964641
22623,45247,0,45247,0.9215259552001953,0.003564588707962591
22723,45447,0,45447,0.9253330230712891,0.0035228205211254027
22823,45647,0,45647,0.9297800064086914,0.0034665635222424244
22923,45847,0,45847,0.9338748455047607,0.0034271464125292376
23023,46047,0,46047,0.938452959060669,0.003413500539925737
23123,46247,0,46247,0.9434850215911865,0.00340270640135036
23223,46447,0,46447,0.9483120441436768,0.0033790268191162425
23323,46647,0,46647,0.953139066696167,0.0033568553836871395
23423,46847,0,46847,0.9583349227905273,0.003341985643593583
23524,47049,0,47049,0.9631638526916504,0.0033096143429991844
23624,47249,0,47249,0.9677770137786865,0.003250663893688416
23724,47449,0,47449,0.9723258018493652,0.003187966715326419
23824,47649,0,47649,0.9769868850708008,0.003143567319717368
23924,47849,0,47849,0.9816529750823975,0.003110438239946373
24024,48049,0,48049,0.9862661361694336,0.0030746699901534787
24124,48249,0,48249,0.9907259941101074,0.0030483317510129394
24224,48449,0,48449,0.9947671890258789,0.0030443259184981205
24324,48649,0,48649,0.9992420673370361,0.003043715794161994
24424,48849,0,48849,1.0044159889221191,0.003021665593696061
24525,49051,0,49051,1.0087108612060547,0.002984110524663237
24625,49251,0,49251,1.012557029724121,0.0029519652291317353
24725,49451,0,49451,1.0166740417480469,0.0029245228238957387
24825,49651,0,49651,1.0204448699951172,0.0028910579504520134
24925,49851,0,49851,1.0244548320770264,0.0028604281507752234
25025,50051,0,50051,1.0281810760498047,0.0028554824936915346
25125,50251,0,50251,1.0321941375732422,0.0028730390615702922
25225,50451,0,50451,1.0363969802856445,0.0028874201579118337
25325,50651,0,50651,1.0407838821411133,0.0028916465559343132
25425,50851,0,50851,1.0446348190307617,0.0028967179910624422
25526,51053,0,51053,1.0487518310546875,0.0029026497037709636
25626,51253,0,51253,1.052551031112671,0.0028950544779333697
25726,51453,0,51453,1.056431770324707,0.0028739170734494775
25826,51653,0,51653,1.0602591037750244,0.00286126314355283
25926,51853,0,51853,1.0641610622406006,0.0028690586889458984
26026,52053,0,52053,1.0682439804077148,0.0028846535757463794
26126,52253,0,52253,1.0720329284667969,0.0028981906177031574
26226,52453,0,52453,1.07607102394104,0.0029171326269452603
26326,52653,0,52653,1.0800042152404785,0.0029429582601344204
26426,52853,0,52853,1.0838348865509033,0.0029596675901451854
26527,53055,0,53055,1.087705135345459,0.002955786181355829
26627,53255,0,53255,1.091583013534546,0.0029415910178032215
26727,53455,0,53455,1.0953831672668457,0.0029325020451796357
26827,53655,0,53655,1.0992991924285889,0.002926420148133577
26927,53855,0,53855,1.1031138896942139,0.0029168971936250586
27027,54055,0,54055,1.106816053390503,0.0029124523651783835
27127,54255,0,54255,1.1105079650878906,0.0029219266416132287
27227,54455,0,54455,1.1142170429229736,0.002936016896715295
27327,54655,0,54655,1.1179070472717285,0.0029381679117688234
27427,54855,0,54855,1.1222589015960693,0.002926622083477666
27528,55057,0,55057,1.1259610652923584,0.0029107090599823217
27628,55257,0,55257,1.1296310424804688,0.0028909075809120926
27728,55457,0,55457,1.1332721710205078,0.0028602644694026673
27828,55657,0,55657,1.1368520259857178,0.0028246681067335454
27928,55857,0,55857,1.1405329704284668,0.0027996784645783084
28028,56057,0,56057,1.1441128253936768,0.0027879842904407997
28128,56257,0,56257,1.1476831436157227,0.0027779964454126703
28228,56457,0,56457,1.151353120803833,0.00276338593906699
28328,56657,0,56657,1.1549949645996094,0.002748533266638918
28428,56857,0,56857,1.1586840152740479,0.002733063682126576
28529,57059,0,57059,1.1622898578643799,0.00270580824753568
28629,57259,0,57259,1.1658618450164795,0.002664646793863797
28729,57459,0,57459,1.1694550514221191,0.0026225257646584543
28829,57659,0,57659,1.1730780601501465,0.0025900344335061084
28929,57859,0,57859,1.17665696144104,0.0025642686547482454
29029,58059,0,58059,1.180279016494751,0.0025411764739629076
29129,58259,0,58259,1.1838798522949219,0.0025260126463449283
29229,58459,0,58459,1.1874980926513672,0.002521552844074032
29329,58659,0,58659,1.191161870956421,0.0025168133560171104
29429,58859,0,58859,1.1948249340057373,0.0025003696508405318
29530,59061,0,59061,1.1985769271850586,0.0024754895655524343
29630,59261,0,59261,1.2023448944091797,0.002452126789662086
29730,59461,0,59461,1.2059810161590576,0.0024303504082544046
29830,59661,0,59661,1.2096009254455566,0.0024077379172443444
29930,59861,0,59861,1.2132070064544678,0.0023912094795578765
30030,60061,0,60061,1.2168259620666504,0.002390183037840966
30130,60261,0,60261,1.2204458713531494,0.002401126930704741
30230,60461,0,60461,1.2240850925445557,0.0024114327623809863
30330,60661,0,60661,1.2277429103851318,0.002416895735905329
30430,60861,0,60861,1.2313830852508545,0.002421378641681876
30531,61063,0,61063,1.2349328994750977,0.002423397141596426
30631,61263,0,61263,1.238386869430542,0.0024172137774760745
30731,61463,0,61463,1.2419230937957764,0.0024057795027338474
30831,61663,0,61663,1.2462220191955566,0.00240052422105147
30931,61863,0,61863,1.2498109340667725,0.0024066840016367555
31031,62063,0,62063,1.2533900737762451,0.0024185209563215813
31131,62263,0,62263,1.2570230960845947,0.0024315115949985937
31231,62463,0,62463,1.260603904724121,0.0024476134471870096
31331,62663,0,62663,1.2642099857330322,0.0024650980869235003
31431,62863,0,62863,1.2678091526031494,0.0024750934256310194
31532,63065,0,63065,1.2715198993682861,0.0024730614549414516
31632,63265,0,63265,1.2751259803771973,0.0024651323974305707
31732,63465,0,63465,1.278731107711792,0.002458668857591029
31832,63665,0,63665,1.2824928760528564,0.0024537476565542095
31932,63865,0,63865,1.285999059677124,0.002449042281279254
32032,64065,0,64065,1.2894551753997803,0.002448894993958359
32132,64265,0,64265,1.2928550243377686,0.0024561245034953544
32232,64465,0,64465,1.2962470054626465,0.0024643181630573095
32332,64665,0,64665,1.2996528148651123,0.002464945013251972
32432,64865,0,64865,1.3031129837036133,0.002457127956096754
32533,65067,0,65067,1.3067588806152344,0.002444535642370448
32633,65267,0,65267,1.3102920055389404,0.0024275702256925263
32733,65467,0,65467,1.3138070106506348,0.002404703870977499
32833,65667,0,65667,1.3174920082092285,0.0023806950243071717
32933,65867,0,65867,1.3210608959197998,0.0023634406831830996
33033,66067,0,66067,1.3246448040008545,0.0023536495999074915
33133,66267,0,66267,1.3283560276031494,0.002345257713125191
33233,66467,0,66467,1.3319759368896484,0.002334908157663821
33333,66667,0,66667,1.3356130123138428,0.002323405760873682
33433,66867,0,66867,1.3392541408538818,0.0023089401783089425
33534,67069,0,67069,1.3429489135742188,0.002286328457944004
33634,67269,0,67269,1.3466119766235352,0.0022562635208968965
33734,67469,0,67469,1.3502459526062012,0.0022260872915794306
33834,67669,0,67669,1.3539369106292725,0.002201563040054933
33934,67869,0,67869,1.3575379848480225,0.0021819626540537777
34034,68069,0,68069,1.3612711429595947,0.0021661871089955803
34134,68269,0,68269,1.3649709224700928,0.002156311287251824
34234,68469,0,68469,1.3686180114746094,0.0021517208652154056
34334,68669,0,68669,1.372277021408081,0.002145783233388275
34434,68869,0,68869,1.3759238719940186,0.0021330175346486145
34535,69071,0,69071,1.379612922668457,0.0021152184509339676
34635,69271,0,69271,1.3833260536193848,0.0020974924372559123
34735,69471,0,69471,1.3876399993896484,0.0020807020103184725
34835,69671,0,69671,1.391291856765747,0.002065335905473507
34935,69871,0,69871,1.3949828147888184,0.0020559503899802555
35035,70071,0,70071,1.3985910415649414,0.0020565256415721435
35135,70271,0,70271,1.4023330211639404,0.002064025022165248
35235,70471,0,70471,1.4059689044952393,0.0020716963355108687
35335,70671,0,70671,1.4095239639282227,0.00207678055605356
35435,70871,0,70871,1.4129350185394287,0.002080094927042732
35536,71073,0,71073,1.4167470932006836,0.002080464585469403
35636,71273,0,71273,1.420198917388916,0.00207599345823942
35736,71473,0,71473,1.4236059188842773,0.002069716849181548
35836,71673,0,71673,1.4271581172943115,0.00206799725721463
35936,71873,0,71873,1.4306659698486328,0.0020733152463785925
36036,72073,0,72073,1.434251070022583,0.0020829007135832575
36136,72273,0,72273,1.4378161430358887,0.0020943149921211044
36236,72473,0,72473,1.4414949417114258,0.002107268657553717
36336,72673,0,72673,1.4452481269836426,0.0021193971968109927
36436,72873,0,72873,1.4490430355072021,0.002125781770988691
36537,73075,0,73075,1.4531610012054443,0.002124659594861811
36637,73275,0,73275,1.4580740928649902,0.002119755752606077
36737,73475,0,73475,1.462162971496582,0.002115128541092619
36837,73675,0,73675,1.4662442207336426,0.002111584811220459
36937,73875,0,73875,1.4698669910430908,0.0021094610437798
37037,74075,0,74075,1.473402976989746,0.002110883475118884
37137,74275,0,74275,1.4769349098205566,0.002116171211125743
37237,74475,0,74475,1.480454921722412,0.0021210491780371613
37337,74675,0,74675,1.4842958450317383,0.002120762691538424
37437,74875,0,74875,1.4888169765472412,0.0021146439923422486
37538,75077,0,75077,1.4930140972137451,0.0021042100216869587
37638,75277,0,75277,1.4974830150604248,0.0020900783061744326
37738,75477,0,75477,1.5016989707946777,0.0020727091609449985
37838,75677,0,75677,1.5067059993743896,0.002055645361384762
37938,75877,0,75877,1.5107431411743164,0.0020430379032463923
38038,76077,0,76077,1.5149109363555908,0.0020349092102865634
38138,76277,0,76277,1.518885850906372,0.0020278990536196904
38238,76477,0,76477,1.5228638648986816,0.002019810887831849
38338,76677,0,76677,1.5266098976135254,0.0020101222444848968
38438,76877,0,76877,1.5302300453186035,0.001997153574729158
38539,77079,0,77079,1.5339279174804688,0.0019785087416847695
38639,77279,0,77279,1.5376520156860352,0.0019557132898316266
38739,77479,0,77479,1.5413870811462402,0.0019331855190116388
38839,77679,0,77679,1.5451750755310059,0.0019143493972393645
38939,77879,0,77879,1.5490319728851318,0.0018994130612133495
39039,78079,0,78079,1.5534279346466064,0.0018881300208304225
39139,78279,0,78279,1.5572500228881836,0.0018809923668241363
39239,78479,0,78479,1.5610949993133545,0.001876501623858607
39339,78679,0,78679,1.564866065979004,0.0018705328144519439
39439,78879,0,78879,1.5687291622161865,0.0018603063270764086
39540,79081,0,79081,1.5724811553955078,0.00184687255314482
39640,79281,0,79281,1.576197862625122,0.001833166632657935
39740,79481,0,79481,1.5799198150634766,0.0018203690921582503
39840,79681,0,79681,1.5836291313171387,0.0018098171288269778
39940,79881,0,79881,1.5873548984527588,0.0018043402593742037
40040,80081,0,80081,1.591062068939209,0.0018055225047469248
40140,80281,0,80281,1.594797134399414,0.0018110247329532507
40240,80481,0,80481,1.5985841751098633,0.0018168595580224643
40340,80681,0,80681,1.6023359298706055,0.0018210591784672057
40440,80881,0,80881,1.606208086013794,0.0018233829609901595
40541,81083,0,81083,1.6100749969482422,0.001823130062082156
40641,81283,0,81283,1.6138288974761963,0.0018200793030817444
40741,81483,0,81483,1.6175739765167236,0.0018167217419772046
40841,81683,0,81683,1.6213150024414062,0.0018167740805258745
40941,81883,0,81883,1.6250419616699219,0.001821534420071793
41041,82083,0,82083,1.6287622451782227,0.0018295271038641617
41141,82283,0,82283,1.6324479579925537,0.001839148466390585
41241,82483,0,82483,1.6361069679260254,0.0018493362690764723
41341,82683,0,82683,1.6397271156311035,0.0018579474286627188
41441,82883,0,82883,1.643388032913208,0.0018622031303593422
41542,83085,0,83085,1.6470520496368408,0.0018615204732591404
41642,83285,0,83285,1.650805950164795,0.0018582588216374241
41742,83485,0,83485,1.6545090675354004,0.0018549398807084837
41842,83685,0,83685,1.6583118438720703,0.0018525628838782096
41942,83885,0,83885,1.6624300479888916,0.0018518094174418027
42042,84085,0,84085,1.666903018951416,0.0018536249782104665
42142,84285,0,84285,1.670516014099121,0.001857417631387779
42242,84485,0,84485,1.674138069152832,0.0018602791893855871
42342,84685,0,84685,1.6778030395507812,0.0018593836303518285
42442,84885,0,84885,1.6814148426055908,0.0018541747447988765
42543,85087,0,85087,1.6853599548339844,0.0018453448735626004
42643,85287,0,85287,1.6893692016601562,0.0018336896990333543
42743,85487,0,85487,1.693068027496338,0.0018202718818095891
42843,85687,0,85687,1.697378158569336,0.0018076295460359652
42943,85887,0,85887,1.7010810375213623,0.0017980333556378682
43043,86087,0,86087,1.7048649787902832,0.0017912724582326335
43143,86287,0,86287,1.7085480690002441,0.0017853173791990218
43243,86487,0,86487,1.7121751308441162,0.0017785575963324856
43343,86687,0,86687,1.7157912254333496,0.0017700858944828196
43443,86887,0,86887,1.719451904296875,0.0017586698871172144
43544,87089,0,87089,1.7231171131134033,0.001743284084365561
43644,87289,0,87289,1.7267310619354248,0.0017255228013394412
43744,87489,0,87489,1.730349063873291,0.001708217718870248
43844,87689,0,87689,1.7339608669281006,0.0016935749397162918
43944,87889,0,87889,1.7380809783935547,0.0016820778868647157
44044,88089,0,88089,1.7417058944702148,0.0016736661533953462
44144,88289,0,88289,1.7453489303588867,0.0016681028184714244
44244,88489,0,88489,1.748966932296753,0.001663845973427704
44344,88689,0,88689,1.752612829208374,0.001658273217956796
44444,88889,0,88889,1.7562339305877686,0.0016499013411023916
44545,89091,0,89091,1.75990891456604,0.001639405825868006
44645,89291,0,89291,1.7635350227355957,0.001628703071724025
44745,89491,0,89491,1.767204999923706,0.0016189938981112087
44845,89691,0,89691,1.7707970142364502,0.0016116666330663956
44945,89891,0,89891,1.7744319438934326,0.0016084383630695356
45045,90091,0,90091,1.7780230045318604,0.001609805927195397
45145,90291,0,90291,1.7816319465637207,0.001614009484575527
45245,90491,0,90491,1.7852318286895752,0.0016184936227270224
45345,90691,0,90691,1.7888860702514648,0.001621781044552678
45445,90891,0,90891,1.7926020622253418,0.0016233798161173864
45546,91093,0,91093,1.7962439060211182,0.0016229692793124856
45646,91293,0,91293,1.7999050617218018,0.001620983672444938
45746,91493,0,91493,1.803508996963501,0.0016193408487428724
45846,91693,0,91693,1.8074009418487549,0.0016203044877079538
45946,91893,0,91893,1.8110849857330322,0.0016245977356713723
46046,92093,0,92093,1.8147199153900146,0.0016313259466340423
46146,92293,0,92293,1.818432092666626,0.0016392670384607322
46246,92493,0,92493,1.8220739364624023,0.0016472050724217848
46346,92693,0,92693,1.8256640434265137,0.0016534330982215122
46446,92893,0,92893,1.8294289112091064,0.0016563499101214338
46547,93095,0,93095,1.8331289291381836,0.001655876711064969
46647,93295,0,93295,1.836771011352539,0.0016536002968191067
46747,93495,0,93495,1.8403599262237549,0.0016512305899073992
46847,93695,0,93695,1.843963861465454,0.001649715024426822
46947,93895,0,93895,1.847588062286377,0.0016496630441051622
47047,94095,0,94095,1.851172924041748,0.0016513877697684792
47147,94295,0,94295,1.8547677993774414,0.0016540492440290098
47247,94495,0,94495,1.8584351539611816,0.0016556166026718692
47347,94695,0,94695,1.8622899055480957,0.00165430779202747
47447,94895,0,94895,1.8659851551055908,0.0016496894760770486
47548,95097,0,95097,1.8696818351745605,0.001642149981709537
47648,95297,0,95297,1.8732731342315674,0.0016325481320045713
47748,95497,0,95497,1.8768599033355713,0.0016220147811073506
47848,95697,0,95697,1.8804538249969482,0.0016123385602712548
47948,95897,0,95897,1.884063959121704,0.0016048021624173476
48048,96097,0,96097,1.8877592086791992,0.0015991267195110768
48148,96297,0,96297,1.8914299011230469,0.0015939663768588614
48248,96497,0,96497,1.8950409889221191,0.0015880784558755814
48348,96697,0,96697,1.898643970489502,0.0015805624965131366
48448,96897,0,96897,1.9023020267486572,0.0015706009283711535
48549,97099,0,97099,1.9059898853302002,0.0015578503242424059
48649,97299,0,97299,1.9097537994384766,0.0015437366672655742
48749,97499,0,97499,1.9133620262145996,0.001530171156538347
48849,97699,0,97699,1.9172749519348145,0.0015186649935898988
48949,97899,0,97899,1.9210140705108643,0.0015096976652755351
49049,98099,0,98099,1.9247210025787354,0.0015031924721118752
49149,98299,0,98299,1.928765058517456,0.0014986288856568197
49249,98499,0,98499,1.9324870109558105,0.0014946751725461265
49349,98699,0,98699,1.9361968040466309,0.0014896288646744278
49449,98899,0,98899,1.9405550956726074,0.0014826751168555102
49550,99101,0,99101,1.9442617893218994,0.00147430028866525
49650,99301,0,99301,1.9480319023132324,0.001465891217176323
49750,99501,0,99501,1.9517590999603271,0.0014585307337913198
49850,99701,0,99701,1.955489158630371,0.0014533938427232775
49950,99901,0,99901,1.959195852279663,0.0014515028599327469
50050,100101,0,100101,1.9629628658294678,0.0014528670680083915
50150,100301,0,100301,1.9666879177093506,0.001456150285125152
50250,100501,0,100501,1.9708130359649658,0.0014596079002268572
50350,100701,0,100701,1.9747400283813477,0.0014621158776447682
50450,100901,0,100901,1.9783570766448975,0.0014632152201788688
50551,101103,0,101103,1.982226848602295,0.0014628405287040343
50651,101303,0,101303,1.9864089488983154,0.0014616255954982616
50751,101503,0,101503,1.989988088607788,0.0014610123790097286
50851,101703,0,101703,1.993541955947876,0.0014624311312326991
50951,101903,0,101903,1.9971089363098145,0.0014662870142144843
51051,102103,0,102103,2.0006799697875977,0.0014719538429671893
51151,102303,0,102303,2.0045251846313477,0.0014784335470839857
51251,102503,0,102503,2.0081191062927246,0.0014845988371514464
51351,102703,0,102703,2.011727809906006,0.001489164227415954
51451,102903,0,102903,2.015291929244995,0.0014911970065728732
51552,103105,0,103105,2.0188820362091064,0.0014908280360570322
51652,103305,0,103305,2.0224390029907227,0.0014891893350829622
51752,103505,0,103505,2.0261151790618896,0.0014875093896418632
51852,103705,0,103705,2.0296828746795654,0.0014865858344306206
51952,103905,0,103905,2.0332422256469727,0.0014868593926201496
52052,104105,0,104105,2.036808967590332,0.001488315559944031
52152,104305,0,104305,2.0403671264648438,0.0014901208358318525
52252,104505,0,104505,2.043936014175415,0.0014908245004318528
52352,104705,0,104705,2.047546863555908,0.0014892493313470633
52452,104905,0,104905,2.0511999130249023,0.0014850863629610243
52553,105107,0,105107,2.0548951625823975,0.0014786212784479607
52653,105307,0,105307,2.0584700107574463,0.0014706871814646582
52753,105507,0,105507,2.062150001525879,0.0014622923662275951
52853,105707,0,105707,2.065757989883423,0.0014546915792288848
52953,105907,0,105907,2.069540023803711,0.0014486220644176798
53053,106107,0,106107,2.0731780529022217,0.001443795141312597
53153,106307,0,106307,2.076831102371216,0.0014392459505089114
53253,106507,0,106507,2.080591917037964,0.0014339994067943344
53353,106707,0,106707,2.084401845932007,0.0014272992301729648
53453,106907,0,106907,2.088239908218384,0.0014186429087567197
53554,107109,0,107109,2.092210054397583,0.0014080200608261966
53654,107309,0,107309,2.0962259769439697,0.0013966400472604221
53754,107509,0,107509,2.100896120071411,0.0013858453162019619
53854,107709,0,107709,2.105257987976074,0.0013767083230471695
53954,107909,0,107909,2.1097960472106934,0.001369611351928722
54054,108109,0,108109,2.1140260696411133,0.0013644220144945066
54154,108309,0,108309,2.117974042892456,0.0013605518248431226
54254,108509,0,108509,2.1216540336608887,0.0013569272770124427
54354,108709,0,108709,2.1253299713134766,0.0013524228236435286
54454,108909,0,108909,2.128938913345337,0.0013465921202757826
54555,109111,0,109111,2.1325719356536865,0.001339823827538948
54655,109311,0,109311,2.136169910430908,0.0013331879859197061
54755,109511,0,109511,2.1398420333862305,0.0013275996850738057
54855,109711,0,109711,2.143601894378662,0.0013239710278546326
54955,109911,0,109911,2.1474759578704834,0.0013228925503657272
55055,110111,0,110111,2.151362180709839,0.0013241654495624862
55155,110311,0,110311,2.155147075653076,0.0013267584182937798
55255,110511,0,110511,2.159032106399536,0.0013294249346121913
55355,110711,0,110711,2.162942886352539,0.001331315194888048
55455,110911,0,110911,2.166856050491333,0.0013320819042021775
55556,111113,0,111113,2.1714820861816406,0.001331810683326441
55656,111313,0,111313,2.175353765487671,0.0013311429494452885
55756,111513,0,111513,2.179244041442871,0.0013311527095394358
55856,111713,0,111713,2.1831259727478027,0.0013327683797807125
55956,111913,0,111913,2.1870899200439453,0.001336202565865471
56056,112113,0,112113,2.1909279823303223,0.001340962017779316
56156,112313,0,112313,2.194873809814453,0.0013462140937770635
56256,112513,0,112513,2.198751926422119,0.001350999768418385
56356,112713,0,112713,2.2027242183685303,0.0013543772467118228
56456,112913,0,112913,2.2066359519958496,0.001355805076816239
56557,113115,0,113115,2.210606098175049,0.0013554944060138827
56657,113315,0,113315,2.2145609855651855,0.0013542909778587772
56757,113515,0,113515,2.2184641361236572,0.0013531072170158169
56857,113715,0,113715,2.2223780155181885,0.0013525700991557637
56957,113915,0,113915,2.2262778282165527,0.0013529589692924786
57057,114115,0,114115,2.2301650047302246,0.0013541014050576056
57157,114315,0,114315,2.2340760231018066,0.001355257295520203
57257,114515,0,114515,2.2379400730133057,0.0013553713308112922
57357,114715,0,114715,2.2417900562286377,0.0013536425276679598
57457,114915,0,114915,2.2456588745117188,0.001349871933606939
57558,115117,0,115117,2.2496120929718018,0.0013443127069586425
57658,115317,0,115317,2.2535738945007324,0.001337723609506877
57758,115517,0,115517,2.258148193359375,0.0013309391147085707
57858,115717,0,115717,2.2621262073516846,0.001324839320645578
57958,115917,0,115917,2.2661969661712646,0.0013198468816121155
58058,116117,0,116117,2.270009756088257,0.0013156838413206536
58158,116317,0,116317,2.2740318775177,0.0013116206647561933
58258,116517,0,116517,2.2788639068603516,0.0013068926693654405
58358,116717,0,116717,2.2836270332336426,0.0013009145679796596
58458,116917,0,116917,2.288679838180542,0.0012934050885028562
58559,117119,0,117119,2.2935948371887207,0.0012845084773524169
58659,117319,0,117319,2.2983338832855225,0.0012752290156767337
58759,117519,0,117519,2.3036839962005615,0.001266537052489774
58859,117719,0,117719,2.30873703956604,0.0012592053980336809
58959,117919,0,117919,2.313401937484741,0.001253504096722392
59059,118119,0,118119,2.318265199661255,0.0012492571871808604
59159,118319,0,118319,2.322767972946167,0.0012459047071923292
59259,118519,0,118519,2.3271281719207764,0.0012426097945022773
59359,118719,0,118719,2.3310279846191406,0.0012386192653972975
59459,118919,0,118919,2.3347818851470947,0.001233701050916046
59560,119121,0,119121,2.3389129638671875,0.0012281878695332962
59660,119321,0,119321,2.342956066131592,0.00122293283539052
59760,119521,0,119521,2.346719980239868,0.0012186783697693943
59860,119721,0,119721,2.350497007369995,0.0012160999371078765
59960,119921,0,119921,2.354434013366699,0.0012155199502317728
60060,120121,0,120121,2.3581290245056152,0.0012166623174216734
60160,120321,0,120321,2.3621208667755127,0.0012187194790448054
60260,120521,0,120521,2.365949869155884,0.001220774073314742
60360,120721,0,120721,2.369636058807373,0.0012221922124737875
60460,120921,0,120921,2.373338222503662,0.0012227416255297713
60561,121123,0,121123,2.37713885307312,0.0012225859535593085
60661,121323,0,121323,2.38100004196167,0.0012223006685591498
60761,121523,0,121523,2.3849220275878906,0.0012226827673548582
60861,121723,0,121723,2.3889360427856445,0.0012243436966346238
60961,121923,0,121923,2.3929998874664307,0.0012273735766418648
61061,122123,0,122123,2.3971641063690186,0.001231355625244748
61161,122323,0,122323,2.4013261795043945,0.0012355946766753967
61261,122523,0,122523,2.4057071208953857,0.0012393102536817052
61361,122723,0,122723,2.410037040710449,0.0012418231297598177
61461,122923,0,122923,2.413881778717041,0.0012428266010161833
61562,123125,0,123125,2.4177868366241455,0.0012425542007179964
61662,123325,0,123325,2.421778917312622,0.0012416577061724425
61762,123525,0,123525,2.4264798164367676,0.0012408252971129598
61862,123725,0,123725,2.4306299686431885,0.001240527454760931
61962,123925,0,123925,2.4348080158233643,0.0012409171368314904
62062,124125,0,124125,2.4394960403442383,0.001241756621060979
62162,124325,0,124325,2.4440560340881348,0.001242419831528139
62262,124525,0,124525,2.448763847351074,0.0012421288981733344
62362,124725,0,124725,2.453450918197632,0.0012403312630190884
62462,124925,0,124925,2.45894718170166,0.0012369166854815424
62563,125127,0,125127,2.464885950088501,0.0012321244101146213
62663,125327,0,125327,2.4695229530334473,0.0012266191245696413
62763,125527,0,125527,2.474514961242676,0.0012210652015721226
62863,125727,0,125727,2.4790761470794678,0.0012160797815831434
62963,125927,0,125927,2.4835751056671143,0.0012118976748466703
63063,126127,0,126127,2.4888598918914795,0.0012082599318425065
63163,126327,0,126327,2.493957996368408,0.00120459769003242
63263,126527,0,126527,2.49868106842041,0.0012003163124092928
63363,126727,0,126727,2.503229856491089,0.0011949857968336327
63463,126927,0,126927,2.5081119537353516,0.0011884732611662128
63564,127129,0,127129,2.512755870819092,0.0011809862894665978
63664,127329,0,127329,2.517487049102783,0.0011733513085270203
63764,127529,0,127529,2.5221991539001465,0.001166282644140463
63864,127729,0,127729,2.5268049240112305,0.0011603386315335309
63964,127929,0,127929,2.5310800075531006,0.0011556911564069802
64064,128129,0,128129,2.5350239276885986,0.0011521426419972122
64164,128329,0,128329,2.539297103881836,0.0011491994596888352
64264,128529,0,128529,2.5434019565582275,0.0011462211562759045
64364,128729,0,128729,2.547759771347046,0.001142701648598482
64464,128929,0,128929,2.5522549152374268,0.001138537961479029
64565,129131,0,129131,2.556748151779175,0.0011340239964433986
64665,129331,0,129331,2.5605530738830566,0.0011298491327853466
64765,129531,0,129531,2.564363956451416,0.0011265989399070148
64865,129731,0,129731,2.568125009536743,0.0011247580072782657
64965,129931,0,129931,2.5721118450164795,0.001124482778938924
65065,130131,0,130131,2.5762460231781006,0.001125481170424162
65165,130331,0,130331,2.579946994781494,0.0011271143928382014
65265,130531,0,130531,2.583620071411133,0.0011286957858592074
65365,130731,0,130731,2.587661027908325,0.0011297598731765531
65465,130931,0,130931,2.5914671421051025,0.0011301687237887182
65566,131133,0,131133,2.595366954803467,0.0011301177237282632
65666,131333,0,131333,2.599061965942383,0.0011300947190812367
65766,131533,0,131533,2.6027560234069824,0.0011306897841469575
65866,131733,0,131733,2.6067090034484863,0.0011323060767038677
65966,131933,0,131933,2.610440969467163,0.0011349547693523313
66066,132133,0,132133,2.6142849922180176,0.0011382729635034884
66166,132333,0,132333,2.6180858612060547,0.0011416839897066841
66266,132533,0,132533,2.6217780113220215,0.0011445688993648915
66366,132733,0,132733,2.6255879402160645,0.0011464434170615238
66466,132933,0,132933,2.6293389797210693,0.0011471441637435221
66567,133135,0,133135,2.6331498622894287,0.001146900459096897
66667,133335,0,133335,2.6368980407714844,0.0011462238187286667
66767,133535,0,133535,2.6406540870666504,0.0011456353618359868
66867,133735,0,133735,2.6444170475006104,0.0011454753693114971
66967,133935,0,133935,2.6481668949127197,0.0011458068952820769
67067,134135,0,134135,2.651962995529175,0.0011463761667178858
67167,134335,0,134335,2.655730962753296,0.0011466666459666996
67267,134535,0,134535,2.6594738960266113,0.0011461003474947142
67367,134735,0,134735,2.6632399559020996,0.0011442957842391762
67467,134935,0,134935,2.667125940322876,0.0011412094108021213
67568,135137,0,135137,2.670894145965576,0.001137067405729338
67668,135337,0,135337,2.6746509075164795,0.0011324375541589713
67768,135537,0,135537,2.6783947944641113,0.0011278367412604785
67868,135737,0,135737,2.682138204574585,0.0011236965393762062
67968,135937,0,135937,2.6859030723571777,0.0011201369557607545
68068,136137,0,136137,2.6896369457244873,0.0011169220976706524
68168,136337,0,136337,2.6935129165649414,0.0011136018414512408
68268,136537,0,136537,2.697244882583618,0.001109719167754766
68368,136737,0,136737,2.700972080230713,0.0011049711168708354
68468,136937,0,136937,2.704707145690918,0.0010993207147703295
68569,137139,0,137139,2.708482027053833,0.0010929922937294829
68669,137339,0,137339,2.7122340202331543,0.0010866629247025133
68769,137539,0,137539,2.715970993041992,0.0010808635427060522
68869,137739,0,137739,2.719697952270508,0.0010759954128653647
68969,137939,0,137939,2.72340989112854,0.0010721543000711009
69069,138139,0,138139,2.727112054824829,0.0010691395486156514
69169,138339,0,138339,2.7308249473571777,0.0010665337408767173
69269,138539,0,138539,2.734449863433838,0.0010638525610627803
69369,138739,0,138739,2.7380521297454834,0.0010607576175432302
69469,138939,0,138939,2.7416670322418213,0.0010572247979932106
69570,139141,0,139141,2.7453150749206543,0.0010535154242442976
69670,139341,0,139341,2.7489349842071533,0.0010501882519705393
69770,139541,0,139541,2.752548933029175,0.0010476954289753773
69870,139741,0,139741,2.7561750411987305,0.0010463753921475534
69970,139941,0,139941,2.759812116622925,0.0010462827970036045
70070,140141,0,140141,2.7634592056274414,0.0010471379433144659
70170,140341,0,140341,2.7671260833740234,0.0010484325557060816
70270,140541,0,140541,2.7707340717315674,0.001049648491029378
70370,140741,0,140741,2.7757151126861572,0.00105044966195635
70470,140941,0,140941,2.7793290615081787,0.0010507677261430716
70571,141143,0,141143,2.7829740047454834,0.0010508024443291483
70671,141343,0,141343,2.7866098880767822,0.0010509543518747858
70771,141543,0,141543,2.790226936340332,0.0010516588870526672
70871,141743,0,141743,2.793839931488037,0.001053178419091043
70971,141943,0,141943,2.7974488735198975,0.0010554742041952998
71071,142143,0,142143,2.8010590076446533,0.0010582281038651743
71171,142343,0,142343,2.8047659397125244,0.0010609656934591717
71271,142543,0,142543,2.8083860874176025,0.0010632042048116439
71371,142743,0,142743,2.8125030994415283,0.0010646021469074348
71471,142943,0,142943,2.816215991973877,0.0010650843448377291
71572,143145,0,143145,2.8199729919433594,0.0010648635937145026
71672,143345,0,143345,2.8235881328582764,0.0010643448790118787
71772,143545,0,143545,2.827285051345825,0.0010639216882261714
71872,143745,0,143745,2.830989122390747,0.00106383174166696
71972,143945,0,143945,2.8347620964050293,0.0010640782982930725
72072,144145,0,144145,2.8384902477264404,0.0010644167565945777
72172,144345,0,144345,2.8422200679779053,0.0010644271974064267
72272,144545,0,144545,2.846034049987793,0.0010636787842792672
72372,144745,0,144745,2.849760055541992,0.0010619108678613886
72472,144945,0,144945,2.853476047515869,0.0010591269995805107
72573,145147,0,145147,2.8573708534240723,0.0010555367248304035
72673,145347,0,145347,2.8611772060394287,0.0010516168713079817
72773,145547,0,145547,2.865007162094116,0.0010477632946357175
72873,145747,0,145747,2.8688571453094482,0.0010442758675301403
72973,145947,0,145947,2.8726110458374023,0.001041203816810316
73073,146147,0,146147,2.8764140605926514,0.0010383363154786664
73173,146347,0,146347,2.8803091049194336,0.0010353156549094758
73273,146547,0,146547,2.8842549324035645,0.0010317952156195563
73373,146747,0,146747,2.8878769874572754,0.0010275704218453904
73473,146947,0,146947,2.892030954360962,0.0010226638182729317
73574,147149,0,147149,2.8962459564208984,0.0010172930889581027
73674,147349,0,147349,2.899970054626465,0.0010120114512406852
73774,147549,0,147549,2.9037129878997803,0.0010072146842532584
73874,147749,0,147749,2.9076879024505615,0.001003188086494986
73974,147949,0,147949,2.911350965499878,0.0009999726801396334
74074,148149,0,148149,2.9153800010681152,0.000997377237035575
74174,148349,0,148349,2.9191019535064697,0.00099505777197386
74274,148549,0,148549,2.9230329990386963,0.0009926515478930918
74374,148749,0,148749,2.9266300201416016,0.0009899357360331192
74474,148949,0,148949,2.9303579330444336,0.0009869338253171668
74575,149151,0,149151,2.934303045272827,0.0009838767697040714
74675,149351,0,149351,2.9380741119384766,0.0009812164671481982
74775,149551,0,149551,2.941812038421631,0.00097929595496533
74875,149751,0,149751,2.9455008506774902,0.0009783450193277686
74975,149951,0,149951,2.949453115463257,0.000978357161547767
75075,150151,0,150151,2.953118085861206,0.0009790774893403496
75175,150351,0,150351,2.9567580223083496,0.000980100589609415
75275,150551,0,150551,2.960392951965332,0.000981034602931314
75375,150751,0,150751,2.9654181003570557,0.0009816413244499516
75475,150951,0,150951,2.9697248935699463,0.0009819002227939879
75576,151153,0,151153,2.9742751121520996,0.000982000319323306
75676,151353,0,151353,2.978348970413208,0.0009822636814382027
75776,151553,0,151553,2.982651948928833,0.0009830098496363955
75876,151753,0,151753,2.9872262477874756,0.000984404420740607
75976,151953,0,151953,2.992304801940918,0.0009863787728492824
76076,152153,0,152153,2.996997833251953,0.0009886551260767087
76176,152353,0,152353,3.001579999923706,0.0009908463619869425
76276,152553,0,152553,3.0063071250915527,0.0009925803501111216
76376,152753,0,152753,3.0110011100769043,0.000993619383529523
76476,152953,0,152953,3.015742063522339,0.0009939422958839485
76577,153155,0,153155,3.0206520557403564,0.0009937400033900228
76677,153355,0,153355,3.025573968887329,0.000993333947245347
76777,153555,0,153555,3.0303549766540527,0.0009930191276887174
76877,153755,0,153755,3.035099983215332,0.0009929553249342336
76977,153955,0,153955,3.0396909713745117,0.0009931085575488768
77077,154155,0,154155,3.044239044189453,0.0009932554026247482
77177,154355,0,154355,3.0485680103302,0.0009930579273609704
77277,154555,0,154555,3.052454948425293,0.0009921953177591879
77377,154755,0,154755,3.05656099319458,0.0009904933343706597
77477,154955,0,154955,3.0603787899017334,0.000987986631128149
77578,155157,0,155157,3.064196825027466,0.000984864821685105
77678,155357,0,155357,3.0679821968078613,0.00098152361836514
77778,155557,0,155557,3.0717499256134033,0.000978262400855413
77878,155757,0,155757,3.0755231380462646,0.0009752872288474332
77978,155957,0,155957,3.079241991043091,0.0009726040993864001
78078,156157,0,156157,3.082953929901123,0.0009700278403781985
78178,156357,0,156357,3.086671829223633,0.0009672747355840131
78278,156557,0,156557,3.0905117988586426,0.0009640857132585769
78378,156757,0,156757,3.09452486038208,0.0009603297633460427
78478,156957,0,156957,3.0985729694366455,0.0009560642833016454
78579,157159,0,157159,3.10280704498291,0.0009514891482769838
78679,157359,0,157359,3.106834888458252,0.0009470554020773093
78779,157559,0,157559,3.1105690002441406,0.0009430574321662704
78879,157759,0,157759,3.1143438816070557,0.0009396949600593182
78979,157959,0,157959,3.1186230182647705,0.0009369720116275821
79079,158159,0,158159,3.1224520206451416,0.0009347140098899164
79179,158359,0,158359,3.1272079944610596,0.0009326424888329479
79279,158559,0,158559,3.1313509941101074,0.0009304883439525135
79379,158759,0,158759,3.135787010192871,0.0009281090263503995
79479,158959,0,158959,3.1407811641693115,0.0009255554503174779
79580,159161,0,159161,3.1457059383392334,0.0009230294395768686
79680,159361,0,159361,3.150424003601074,0.0009208947919103661
79780,159561,0,159561,3.1550121307373047,0.0009194075756591737
79880,159761,0,159761,3.159976005554199,0.0009187183951992855
79980,159961,0,159961,3.1646862030029297,0.0009187854986979219
80080,160161,0,160161,3.169408082962036,0.0009193832997417783
80180,160361,0,160361,3.174053907394409,0.0009201884760830486
80280,160561,0,160561,3.1789560317993164,0.0009209051308110858
80380,160761,0,160761,3.1837029457092285,0.0009213680167185524
80480,160961,0,160961,3.188443899154663,0.0009215873917321349
80581,161163,0,161163,3.1931920051574707,0.0009217340119056417
80681,161363,0,161363,3.1979010105133057,0.0009220628390283527
80781,161563,0,161563,3.2024898529052734,0.0009228063409379709
80881,161763,0,161763,3.207273006439209,0.0009240631719373771
80981,161963,0,161963,3.2118918895721436,0.0009257487491280232
81081,162163,0,162163,3.216475009918213,0.000927622517548261
81181,162363,0,162363,3.2210397720336914,0.0009293709788256857
81281,162563,0,162563,3.225713014602661,0.0009307099755542141
81381,162763,0,162763,3.230404853820801,0.0009314768072322573
81481,162963,0,162963,3.2349700927734375,0.0009316826100058701
81582,163165,0,163165,3.239313840866089,0.0009314946914512201
81682,163365,0,163365,3.2431271076202393,0.0009311677916317265
81782,163565,0,163565,3.2470779418945312,0.0009309208069065117
81882,163765,0,163765,3.250877857208252,0.000930855875376851
81982,163965,0,163965,3.254654884338379,0.0009309177892654785
82082,164165,0,164165,3.2588889598846436,0.0009309090794040802
82182,164365,0,164365,3.262892007827759,0.0009305599977330671
82282,164565,0,164565,3.2666139602661133,0.0009296327959692951
82382,164765,0,164765,3.270327091217041,0.0009280151744153849
82482,164965,0,164965,3.274229049682617,0.0009257605978534036
82583,165167,0,165167,3.27828311920166,0.0009230369566347484
82683,165367,0,165367,3.282033920288086,0.0009201698537410303
82783,165567,0,165567,3.2857589721679688,0.0009173830743989654
82883,165767,0,165767,3.2896111011505127,0.0009148158098372631
82983,165967,0,165967,3.293401002883911,0.0009124485342667239
83083,166167,0,166167,3.297312021255493,0.000910121211069249
83183,166367,0,166367,3.3010430335998535,0.0009076100957668707
83283,166567,0,166567,3.3047869205474854,0.0009047247322746157
83383,166767,0,166767,3.308932065963745,0.0009013876631708839
83483,166967,0,166967,3.3128609657287598,0.0008976746998178535
83584,167169,0,167169,3.3166520595550537,0.0008937633025923373
83684,167369,0,167369,3.3203771114349365,0.0008900204562466181
83784,167569,0,167569,3.324122190475464,0.0008866637675201256
83884,167769,0,167769,3.3282151222229004,0.0008838301616397827
83984,167969,0,167969,3.331961154937744,0.0008815002681926106
84084,168169,0,168169,3.335679054260254,0.0008795195447258347
84184,168369,0,168369,3.3392961025238037,0.0008776656237199858
84284,168569,0,168569,3.342897891998291,0.0008757410059643323
84384,168769,0,168769,3.3466949462890625,0.0008736589571555772
84484,168969,0,168969,3.3503639698028564,0.0008714845739135534
84585,169171,0,169171,3.3540899753570557,0.0008693919620829593
84685,169371,0,169371,3.3578319549560547,0.0008676723393720726
84785,169571,0,169571,3.361783027648926,0.0008665136985893719
84885,169771,0,169771,3.3653790950775146,0.0008660098678042812
84985,169971,0,169971,3.368966817855835,0.000866100398655721
85085,170171,0,170171,3.372565984725952,0.0008665895062497029
85185,170371,0,170371,3.3761558532714844,0.0008672198387447541
85285,170571,0,170571,3.3797340393066406,0.0008677688736569731
85385,170771,0,170771,3.383322238922119,0.0008681249606959862
85485,170971,0,170971,3.3869152069091797,0.0008683166737615015
85586,171173,0,171173,3.390558958053589,0.0008684935281884914
85686,171373,0,171373,3.394141912460327,0.0008688546805009033
85786,171573,0,171573,3.397726058959961,0.0008695671429942288
85886,171773,0,171773,3.401348114013672,0.0008706834031409542
85986,171973,0,171973,3.4049739837646484,0.0008721124557149325
86086,172173,0,172173,3.408580780029297,0.0008736479217864585
86186,172373,0,172373,3.41231107711792,0.0008750376661399535
86286,172573,0,172573,3.415919780731201,0.0008760665312859014
86386,172773,0,172773,3.419508934020996,0.0008766256973700005
86486,172973,0,172973,3.423097848892212,0.0008767446218802946
86587,173175,0,173175,3.4267420768737793,0.0008765672592557582
86687,173375,0,173375,3.43033504486084,0.0008762946746439859
86787,173575,0,173575,3.434026002883911,0.0008760871494352047
86887,173775,0,173775,3.437623977661133,0.0008760051932431543
86987,173975,0,173975,3.441316843032837,0.0008759833225121085
87087,174175,0,174175,3.4449169635772705,0.000875850885173712
87187,174375,0,174375,3.448606014251709,0.0008753941671112861
87287,174575,0,174575,3.452207088470459,0.0008744384335426315
87387,174775,0,174775,3.455864191055298,0.0008729155540592252
87487,174975,0,174975,3.459537982940674,0.0008708887952690038
87588,175177,0,175177,3.463247060775757,0.0008685040325875125
87688,175377,0,175377,3.466921091079712,0.0008660275022496727
87788,175577,0,175577,3.4705851078033447,0.0008636244374817609
87888,175777,0,175777,3.474250078201294,0.0008613865064298292
87988,175977,0,175977,3.477914810180664,0.00085928019636098
88088,176177,0,176177,3.481600046157837,0.0008571692576980055
88188,176377,0,176377,3.485274076461792,0.000854878682351542
88288,176577,0,176577,3.4889328479766846,0.000852271182995036
88388,176777,0,176777,3.4925949573516846,0.0008493073375937226
88488,176977,0,176977,3.496264934539795,0.0008460706084560198
88589,177179,0,177179,3.499976873397827,0.0008427149705160478
88689,177379,0,177379,3.5036449432373047,0.0008395384075095698
88789,177579,0,177579,3.5073320865631104,0.00083670018619593
88889,177779,0,177779,3.5110280513763428,0.0008342915682834349
88989,177979,0,177979,3.515974998474121,0.0008322796832178614
89089,178179,0,178179,3.519566059112549,0.0008305308718035362
89189,178379,0,178379,3.5232231616973877,0.000828869610054177
89289,178579,0,178579,3.5269041061401367,0.0008271528407871994
89389,178779,0,178779,3.5306010246276855,0.0008253323885796358
89489,178979,0,178979,3.5343050956726074,0.0008234788525828045
89590,179181,0,179181,3.538043975830078,0.0008217404932841114
89690,179381,0,179381,3.5417490005493164,0.0008203490050212823
89790,179581,0,179581,3.5454530715942383,0.0008194398358134963
89890,179781,0,179781,3.549146890640259,0.0008190667545649459
89990,179981,0,179981,3.552845001220703,0.000819161155235075
90090,180181,0,180181,3.5565550327301025,0.0008195555404714558
90190,180381,0,180381,3.560276985168457,0.0008200457185135016
90290,180581,0,180581,3.5639970302581787,0.0008204653412128683
90390,180781,0,180781,3.5677108764648438,0.0008207415490179744
90490,180981,0,180981,3.5714099407196045,0.0008209124895196915
90591,181183,0,181183,3.575134038925171,0.0008211061019937824
90691,181383,0,181383,3.578839063644409,0.0008214759620807018
90791,181583,0,181583,3.5825448036193848,0.0008221399595659456
90891,181783,0,181783,3.586246967315674,0.0008231191307371879
90991,181983,0,181983,3.589940071105957,0.0008243224039541082
91091,182183,0,182183,3.5936269760131836,0.0008255743427610261
91191,182383,0,182383,3.5973260402679443,0.0008266734507235839
91291,182583,0,182583,3.6010079383850098,0.0008274581678295047
91391,182783,0,182783,3.6046981811523438,0.0008278580779419813
91491,182983,0,182983,3.608398199081421,0.0008279119148059469
91592,183185,0,183185,3.612138032913208,0.0008277416370519857
91692,183385,0,183385,3.6158621311187744,0.0008275050550719453
91792,183585,0,183585,3.619542121887207,0.000827317572768543
91892,183785,0,183785,3.6232330799102783,0.0008272103500172629
91992,183985,0,183985,3.6269309520721436,0.000827114862991511
92092,184185,0,184185,3.630617141723633,0.0008268860851503632
92192,184385,0,184385,3.6343259811401367,0.0008263559706830777
92292,184585,0,184585,3.638104200363159,0.0008253976250002553
92392,184785,0,184785,3.641857147216797,0.0008239740481775639
92492,184985,0,184985,3.6455581188201904,0.0008221519837026714
92593,185187,0,185187,3.6492931842803955,0.0008200561295568657
92693,185387,0,185387,3.6530020236968994,0.0008179031625985509
92793,185587,0,185587,3.656705141067505,0.0008158133732980409
92893,185787,0,185787,3.6604931354522705,0.0008138448883398462
92993,185987,0,185987,3.664271116256714,0.0008119577231530521
93093,186187,0,186187,3.668062925338745,0.0008100375084685403
93193,186387,0,186387,3.6717288494110107,0.0008079487361071991
93293,186587,0,186587,3.675189971923828,0.0008055948568062806
93393,186787,0,186787,3.6786530017852783,0.0008029627484150209
93493,186987,0,186987,3.6821041107177734,0.0008001366470948767
93594,187189,0,187189,3.686462879180908,0.0007972478571888059
93694,187389,0,187389,3.6899120807647705,0.0007945378606313771
93794,187589,0,187589,3.6933839321136475,0.0007921216355275383
93894,187789,0,187789,3.6968750953674316,0.000790057632949688
93994,187989,0,187989,3.7003440856933594,0.0007883063933365945
94094,188189,0,188189,3.7038159370422363,0.0007867544387938208
94194,188389,0,188389,3.7082130908966064,0.0007852647036552051
94294,188589,0,188589,3.711786985397339,0.0007837352734987575
94394,188789,0,188789,3.7152321338653564,0.0007821442378403233
94494,188989,0,188989,3.718729019165039,0.0007805621181205609
94595,189191,0,189191,3.722201108932495,0.0007791136019185556
94695,189391,0,189391,3.7256319522857666,0.000777981860183961
94795,189591,0,189591,3.729098081588745,0.0007772622672379343
94895,189791,0,189791,3.7326409816741943,0.0007769808527342268
94995,189991,0,189991,3.7363200187683105,0.0007770674625305682
95095,190191,0,190191,3.7399749755859375,0.0007773804158384673
95195,190391,0,190391,3.7435781955718994,0.0007777583486906501
95295,190591,0,190591,3.747189998626709,0.0007780778384347758
95395,190791,0,190791,3.750783920288086,0.0007782936444075621
95495,190991,0,190991,3.754379987716675,0.0007784475942381758
95596,191193,0,191193,3.758021831512451,0.0007786471756561169
95696,191393,0,191393,3.7616629600524902,0.000779009221887024
95796,191593,0,191593,3.765273094177246,0.0007796149086672052
95896,191793,0,191793,3.768862009048462,0.0007804643279087903
95996,191993,0,191993,3.772447109222412,0.0007814703907463661
96096,192193,0,192193,3.7760329246520996,0.0007824852398633668
96196,192393,0,192393,3.779616117477417,0.000783348813431286
96296,192593,0,192593,3.7832047939300537,0.0007839408649115961
96396,192793,0,192793,3.7867908477783203,0.0007842180605834987
96496,192993,0,192993,3.7904551029205322,0.0007842226028319198
96597,193195,0,193195,3.7940800189971924,0.0007840563959830368
96697,193395,0,193395,3.797691822052002,0.0007838424795929533
96797,193595,0,193595,3.8013648986816406,0.0007836621620644927
96897,193795,0,193795,3.805060863494873,0.0007835264754578041
96997,193995,0,193995,3.808687210083008,0.0007833684471244575
97097,194195,0,194195,3.8122949600219727,0.0007830664764506844
97197,194395,0,194395,3.8159220218658447,0.0007824894867827737
97297,194595,0,194595,3.819537878036499,0.0007815468176617557
97397,194795,0,194795,3.8231379985809326,0.0007802230093839007
97497,194995,0,194995,3.826741933822632,0.0007785840408823177
97598,195197,0,195197,3.83038592338562,0.0007767349951600943
97698,195397,0,195397,3.8339672088623047,0.0007748516070601287
97798,195597,0,195597,3.8375070095062256,0.0007730199539615395
97898,195797,0,195797,3.841040849685669,0.0007712747588061685
97998,195997,0,195997,3.8446099758148193,0.0007695743899653135
98098,196197,0,196197,3.848155975341797,0.0007678241336359563
98198,196397,0,196397,3.8516759872436523,0.0007659203182002026
98298,196597,0,196597,3.8553810119628906,0.0007637972470008317
98398,196797,0,196797,3.859018087387085,0.0007614593832183158
98498,196997,0,196997,3.8626370429992676,0.0007589875075462111
98599,197199,0,197199,3.8663458824157715,0.0007564920287053173
98699,197399,0,197399,3.870007038116455,0.0007541682908846921
98799,197599,0,197599,3.8735969066619873,0.0007520977847984034
98899,197799,0,197799,3.877207040786743,0.0007503157381845929
98999,197999,0,197999,3.8807990550994873,0.0007487807401688889
99099,198199,0,198199,3.884397029876709,0.0007473979239283026
99199,198399,0,198399,3.887993097305298,0.000746061400009243
99299,198599,0,198599,3.8915960788726807,0.0007447001263067465
99399,198799,0,198799,3.8952109813690186,0.000743309665608991
99499,198999,0,198999,3.8988049030303955,0.0007419570167356046
99600,199201,0,199201,3.902611017227173,0.0007407458020672369
99700,199401,0,199401,3.9062609672546387,0.0007398198908731625
99800,199601,0,199601,3.9097659587860107,0.0007392444402055365
99900,199801,0,199801,3.9133970737457275,0.00073902673139159
100000,200001,0,200001,3.9168179035186768,0.0007390990808655018


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.009506225585938e-05,4.387072431292609
86,173,172,345,0.003930091857910156,0.2868497587704457
172,345,344,689,0.007955074310302734,0.13032929019998057
258,517,516,1033,0.012627124786376953,0.08632160440198876
344,689,688,1377,0.016607999801635742,0.06653322942944
430,861,860,1721,0.02032184600830078,0.05598508680505433
516,1033,1032,2065,0.024190187454223633,0.049585547253792064
602,1205,1204,2409,0.02833390235900879,0.045146781145719156
688,1377,1376,2753,0.03180098533630371,0.041682144259711534
774,1549,1548,3097,0.035269975662231445,0.03880524720209769
859,1719,1718,3437,0.03900790214538574,0.036345075405360576
945,1891,1890,3781,0.04271984100341797,0.034170284662348845
1031,2063,2062,4125,0.04707002639770508,0.03224283000397655
1117,2235,2234,4469,0.05065417289733887,0.03054296362001096
1203,2407,2406,4813,0.05423617362976074,0.029035296497065512
1289,2579,2578,5157,0.0582270622253418,0.027703106104165674
1375,2751,2750,5501,0.06169891357421875,0.02651442001967155
1461,2923,2922,5845,0.06516909599304199,0.02546101013882364
1547,3095,3094,6189,0.06864094734191895,0.024523010892009242
1633,3267,3266,6533,0.07217097282409668,0.023687346846406998
1719,3439,3438,6877,0.07585000991821289,0.022934052511305033
1805,3611,3610,7221,0.07942390441894531,0.022257869853309322
1891,3783,3782,7565,0.08297204971313477,0.021648462171941926
1977,3955,3954,7909,0.08651900291442871,0.021095497758925386
2063,4127,4126,8253,0.09007906913757324,0.020587438174011014
2149,4299,4298,8597,0.09393811225891113,0.020121465143950207
2235,4471,4470,8941,0.09759306907653809,0.019693562108026922
2321,4643,4642,9285,0.10183215141296387,0.019417368101809336
2407,4815,4814,9629,0.1062021255493164,0.019172183674350887
2492,4985,4984,9969,0.110382080078125,0.018921408268011784
2578,5157,5156,10313,0.11466789245605469,0.018657797857788646
2664,5329,5328,10657,0.11889195442199707,0.018402733495413853
2750,5501,5500,11001,0.12312102317810059,0.01814994244276452
2836,5673,5672,11345,0.12734603881835938,0.017887781919273416
2922,5845,5844,11689,0.1315901279449463,0.01763123858693001
3008,6017,6016,12033,0.1358950138092041,0.017362972320279106
3094,6189,6188,12377,0.14022207260131836,0.017101644176899133
3180,6361,6360,12721,0.14444303512573242,0.016838588007872475
3266,6533,6532,13065,0.14866304397583008,0.016577476525197324
3352,6705,6704,13409,0.15288496017456055,0.016308887663902285
3438,6877,6876,13753,0.15709710121154785,0.016048883260889657
3524,7049,7048,14097,0.16128921508789062,0.01578802292883813
3610,7221,7220,14441,0.16549205780029297,0.015527102971734942
3696,7393,7392,14785,0.1699061393737793,0.01527411001660001
3782,7565,7564,15129,0.17411303520202637,0.015041641676480944
3868,7737,7736,15473,0.17849493026733398,0.01481386172826168
3954,7909,7908,15817,0.18279314041137695,0.014587650653174493
4040,8081,8080,16161,0.18729901313781738,0.014368607038927466
4126,8253,8252,16505,0.19205904006958008,0.0141532462235422
4211,8423,8422,16845,0.19628000259399414,0.01394315930989325
4297,8595,8594,17189,0.20074987411499023,0.013733178164384716
4383,8767,8766,17533,0.20523500442504883,0.013529112474474369
4469,8939,8938,17877,0.20960497856140137,0.013328034900586556
4555,9111,9110,18221,0.21406102180480957,0.013128264427076005
4641,9283,9282,18565,0.21834588050842285,0.012932727260469538
4727,9455,9454,18909,0.22298216819763184,0.012741426784731535
4813,9627,9626,19253,0.22726893424987793,0.012552387467496073
4899,9799,9798,19597,0.23152494430541992,0.012364675018864197
4985,9971,9970,19941,0.23579001426696777,0.01218181838159426
5071,10143,10142,20285,0.24007320404052734,0.01200201492049166
5157,10315,10314,20629,0.24436712265014648,0.011823540354613851
5243,10487,10486,20973,0.24918699264526367,0.011647503178281398
5329,10659,10658,21317,0.2534492015838623,0.01147586158459793
5415,10831,10830,21661,0.2577230930328369,0.011306427707025913
5501,11003,11002,22005,0.26198601722717285,0.011137946778624805
5587,11175,11174,22349,0.266247034072876,0.010972971369030343
5673,11347,11346,22693,0.2705068588256836,0.0108114814781856
5759,11519,11518,23037,0.2746610641479492,0.010651404932836506
5844,11689,11688,23377,0.2787590026855469,0.01049458181460958
5930,11861,11860,23721,0.2832369804382324,0.010339778396450401
6016,12033,12032,24065,0.2873971462249756,0.010187543338711493
6102,12205,12204,24409,0.29154181480407715,0.010036187324563626
6188,12377,12376,24753,0.29570817947387695,0.00988711950530088
6274,12549,12548,25097,0.299854040145874,0.009741653602306147
6360,12721,12720,25441,0.3040039539337158,0.009597882629587688
6446,12893,12892,25785,0.30814290046691895,0.009454996966850584
6532,13065,13064,26129,0.3123340606689453,0.009315129508769995
6618,13237,13236,26473,0.3164830207824707,0.0091781738174004
6704,13409,13408,26817,0.32077503204345703,0.009042217853600898
6790,13581,13580,27161,0.324998140335083,0.008907677551006144
6876,13753,13752,27505,0.3291490077972412,0.00877639749663704
6962,13925,13924,27849,0.33329081535339355,0.008647187287500677
7048,14097,14096,28193,0.3374509811401367,0.008518664510319511
7134,14269,14268,28537,0.34158802032470703,0.008392267355285886
7220,14441,14440,28881,0.3458220958709717,0.008268865659837105
7306,14613,14612,29225,0.3503420352935791,0.008146744005682417
7392,14785,14784,29569,0.3548240661621094,0.008025477935800333
7477,14955,14954,29909,0.35919809341430664,0.00790822083262498
7563,15127,15126,30253,0.3633692264556885,0.007791966187910349
7649,15299,15298,30597,0.3675239086151123,0.007676460165076236
7735,15471,15470,30941,0.3717038631439209,0.007562300686922235
7821,15643,15642,31285,0.3763291835784912,0.007450910158378703
7907,15815,15814,31629,0.3805501461029053,0.007341170771810391
7993,15987,15986,31973,0.3847029209136963,0.007232015278268057
8079,16159,16158,32317,0.3889460563659668,0.00712478263038193
8165,16331,16330,32661,0.39311718940734863,0.007020047977364422
8251,16503,16502,33005,0.39734601974487305,0.006916293890489678
8337,16675,16674,33349,0.40151309967041016,0.006813350702344683
8423,16847,16846,33693,0.4058709144592285,0.006712715350760621
8509,17019,17018,34037,0.41003990173339844,0.006614018642986916
8595,17191,17190,34381,0.4142019748687744,0.0065158954292452425
8681,17363,17362,34725,0.41837310791015625,0.006419046402364501
8767,17535,17534,35069,0.4225449562072754,0.0063245519056610005
8853,17707,17706,35413,0.42670702934265137,0.006231341633729837
8939,17879,17878,35757,0.43085789680480957,0.006138651602685907
9025,18051,18050,36101,0.43498897552490234,0.006047704179447483
9110,18221,18220,36441,0.4390869140625,0.0059598451948832225
9196,18393,18392,36785,0.4432239532470703,0.00587169522507658
9282,18565,18564,37129,0.44746899604797363,0.005784309226104578
9368,18737,18736,37473,0.4517951011657715,0.005698931172562657
9454,18909,18908,37817,0.45615291595458984,0.005615117610524657
9540,19081,19080,38161,0.4603290557861328,0.005531762059042106
9626,19253,19252,38505,0.46448612213134766,0.005449581471700116
9712,19425,19424,38849,0.46864914894104004,0.005369394941756801
9798,19597,19596,39193,0.47278714179992676,0.005290212291516575
9884,19769,19768,39537,0.47684288024902344,0.005211500709606557
9970,19941,19940,39881,0.48090100288391113,0.0051343434991668845
10056,20113,20112,40225,0.4849510192871094,0.005058886888022648
10142,20285,20284,40569,0.4890449047088623,0.004983998328052962
10228,20457,20456,40913,0.493319034576416,0.004909838751653631
10314,20629,20628,41257,0.497377872467041,0.004837424706467703
10400,20801,20800,41601,0.5014450550079346,0.004766250328787064
10486,20973,20972,41945,0.5055241584777832,0.004695449196591222
10572,21145,21144,42289,0.5096738338470459,0.004625737164106255
10658,21317,21316,42633,0.5139648914337158,0.004557703650000855
10743,21487,21486,42973,0.5180630683898926,0.004491220208653245
10829,21659,21658,43317,0.5222170352935791,0.004424384140809679
10915,21831,21830,43661,0.5263779163360596,0.0043589271431272334
11001,22003,22002,44005,0.5305378437042236,0.004294864458747394
11087,22175,22174,44349,0.5346920490264893,0.004231240652507796
11173,22347,22346,44693,0.5388588905334473,0.004168297771068796
11259,22519,22518,45037,0.5429520606994629,0.004106859217038733
11345,22691,22690,45381,0.5471220016479492,0.0040464068625680975
11431,22863,22862,45725,0.5512990951538086,0.0039862692959178
11517,23035,23034,46069,0.5554690361022949,0.003927121796689074
11603,23207,23206,46413,0.5596890449523926,0.0038693811495276336
11689,23379,23378,46757,0.56386399269104,0.0038122349065508373
11775,23551,23550,47101,0.5679349899291992,0.0037554968647981702
11861,23723,23722,47445,0.572105884552002,0.0036999830955663053
11947,23895,23894,47789,0.5763108730316162,0.0036455970370553297
12033,24067,24066,48133,0.5805401802062988,0.003591548137706487
12119,24239,24238,48477,0.58473801612854,0.003538142551957953
12205,24411,24410,48821,0.5889120101928711,0.0034860281025527995
12291,24583,24582,49165,0.5930819511413574,0.003434682977136378
12377,24755,24754,49509,0.5985698699951172,0.0033836111993406732
12462,24925,24924,49849,0.6027770042419434,0.0033340194622823068
12548,25097,25096,50193,0.6071100234985352,0.003285010635203608
12634,25269,25268,50537,0.6110739707946777,0.003236460173267882
12720,25441,25440,50881,0.6150569915771484,0.003188290985784137
12806,25613,25612,51225,0.6189858913421631,0.0031411954242293273
12892,25785,25784,51569,0.6235759258270264,0.0030950131709430242
12978,25957,25956,51913,0.6276509761810303,0.003049097206707865
13064,26129,26128,52257,0.6316251754760742,0.0030037762713220444
13150,26301,26300,52601,0.6355249881744385,0.0029595559159279593
13236,26473,26472,52945,0.6396441459655762,0.002915939996902421
13322,26645,26644,53289,0.6438539028167725,0.002872566688701584
13408,26817,26816,53633,0.6480391025543213,0.002830005108068641
13494,26989,26988,53977,0.6524121761322021,0.002788412107710217
13580,27161,27160,54321,0.6565830707550049,0.002747166018918603
13666,27333,27332,54665,0.6607010364532471,0.002706282787315864
13752,27505,27504,55009,0.6647839546203613,0.002666339906545504
13838,27677,27676,55353,0.6689000129699707,0.0026271254139762505
13924,27849,27848,55697,0.6730148792266846,0.0025881233580337683
14010,28021,28020,56041,0.6771280765533447,0.002549676250010603
14095,28191,28190,56381,0.6812000274658203,0.002512593170729847
14181,28363,28362,56725,0.6854848861694336,0.0024755412385839377
14267,28535,28534,57069,0.6895980834960938,0.0024387087350410193
14353,28707,28706,57413,0.6938128471374512,0.0024026009073280477
14439,28879,28878,57757,0.6979260444641113,0.0023672914784470082
14525,29051,29050,58101,0.7025902271270752,0.002332249370139559
14611,29223,29222,58445,0.7073628902435303,0.002297546765900458
14697,29395,29394,58789,0.7115039825439453,0.002263659340200623
14783,29567,29566,59133,0.7156620025634766,0.0022303545836092013
14869,29739,29738,59477,0.719886064529419,0.0021972246457266204
14955,29911,29910,59821,0.7240941524505615,0.0021646021212277703
15041,30083,30082,60165,0.7284641265869141,0.002132765370108523
15127,30255,30254,60509,0.7327210903167725,0.0021012899536920603
15213,30427,30426,60853,0.7373909950256348,0.002070018894887582
15299,30599,30598,61197,0.7417058944702148,0.00203939585741918
15385,30771,30770,61541,0.7461040019989014,0.0020094229147547757
15471,30943,30942,61885,0.7503242492675781,0.0019796532848930758
15557,31115,31114,62229,0.7545859813690186,0.0019502055952506764
15643,31287,31286,62573,0.7588231563568115,0.0019214624765181093
15728,31457,31456,62913,0.7629599571228027,0.0018935059097175263
15814,31629,31628,63257,0.7671389579772949,0.0018653656037302048
15900,31801,31800,63601,0.7713460922241211,0.0018376866622826565
15986,31973,31972,63945,0.7755370140075684,0.0018106666193886943
16072,32145,32144,64289,0.7797238826751709,0.0017839261736516674
16158,32317,32316,64633,0.7839100360870361,0.0017573754472919039
16244,32489,32488,64977,0.7880969047546387,0.0017313963457822378
16330,32661,32660,65321,0.7922680377960205,0.0017059468597698157
16416,32833,32832,65665,0.7965888977050781,0.0016806559921501232
16502,33005,33004,66009,0.8007850646972656,0.0016556643497731148
16588,33177,33176,66353,0.8050401210784912,0.001631276594265418
16674,33349,33348,66697,0.8092231750488281,0.0016072508079231177
16760,33521,33520,67041,0.8133900165557861,0.0015833528726454885
16846,33693,33692,67385,0.8175849914550781,0.0015598763240507014
16932,33865,33864,67729,0.8218059539794922,0.0015369472329154765
17018,34037,34036,68073,0.8260698318481445,0.0015142301493565745
17104,34209,34208,68417,0.8306601047515869,0.0014916933086761327
17190,34381,34380,68761,0.8348419666290283,0.0014696604614666201
17276,34553,34552,69105,0.8390209674835205,0.0014480527166614644
17361,34723,34722,69445,0.8431930541992188,0.001426817455733807
17447,34895,34894,69789,0.8474001884460449,0.001405609075854444
17533,35067,35066,70133,0.8516309261322021,0.0013849156093619593
17619,35239,35238,70477,0.8558170795440674,0.001364506585931345
17705,35411,35410,70821,0.8599982261657715,0.0013442108651718445
17791,35583,35582,71165,0.8641698360443115,0.0013242936069577402
17877,35755,35754,71509,0.8684360980987549,0.0013048301800883857
17963,35927,35926,71853,0.8726928234100342,0.0012855299642334644
18049,36099,36098,72197,0.876690149307251,0.0012663984539297401
18135,36271,36270,72541,0.8806519508361816,0.0012477063538433985
18221,36443,36442,72885,0.8847651481628418,0.0012293564118769091
18307,36615,36614,73229,0.8887760639190674,0.001211106027501486
18393,36787,36786,73573,0.8928799629211426,0.0011931139439951507
18479,36959,36958,73917,0.8970668315887451,0.0011755583876097867
18565,37131,37130,74261,0.9012079238891602,0.0011582218978856964
18651,37303,37302,74605,0.905203104019165,0.0011409889784705976
18737,37475,37474,74949,0.9092891216278076,0.0011240968055880435
18823,37647,37646,75293,0.9134249687194824,0.0011075767381814765
18909,37819,37818,75637,0.9174399375915527,0.0010911803926775853
18994,37989,37988,75977,0.9213931560516357,0.0010751312942456133
19080,38161,38160,76321,0.9260830879211426,0.0010592729781472806
19166,38333,38332,76665,0.9317290782928467,0.0010436885102697215
19252,38505,38504,77009,0.9368801116943359,0.0010281858720452006
19338,38677,38676,77353,0.9418621063232422,0.0010129195017940175
19424,38849,38848,77697,0.9473249912261963,0.0009980211880464475
19510,39021,39020,78041,0.9518561363220215,0.0009832931482255801
19596,39193,39192,78385,0.9569690227508545,0.0009686602787933046
19682,39365,39364,78729,0.9615190029144287,0.0009543297434186621
19768,39537,39536,79073,0.9657180309295654,0.0009403040886179995
19854,39709,39708,79417,0.969688892364502,0.0009263741508055436
19940,39881,39880,79761,0.9741439819335938,0.0009125940071025121
20026,40053,40052,80105,0.978665828704834,0.0008991432442850173
20112,40225,40224,80449,0.9828178882598877,0.000885907696836284
20198,40397,40396,80793,0.9870529174804688,0.0008727410207703236
20284,40569,40568,81137,0.9913160800933838,0.0008597917363941337
20370,40741,40740,81481,0.9957249164581299,0.0008471503120180681
20456,40913,40912,81825,1.0001890659332275,0.0008346384509959169
20542,41085,41084,82169,1.0047409534454346,0.0008222162697720637
20628,41257,41256,82513,1.0093491077423096,0.0008100625224006755
20713,41427,41426,82853,1.0138778686523438,0.000798293379316805
20799,41599,41598,83197,1.018463134765625,0.0007864591076304904
20885,41771,41770,83541,1.0231311321258545,0.0007747640836662422
20971,41943,41942,83885,1.0278050899505615,0.0007633514896509858
21057,42115,42114,84229,1.0324749946594238,0.0007521090316510449
21143,42287,42286,84573,1.037165880203247,0.000740926172232646
21229,42459,42458,84917,1.0419330596923828,0.0007299397421287687
21315,42631,42630,85261,1.0467791557312012,0.000719209972165391
21401,42803,42802,85605,1.0515649318695068,0.0007085801271039753
21487,42975,42974,85949,1.0564088821411133,0.0006980340554833696
21573,43147,43146,86293,1.061187982559204,0.0006877233459234417
21659,43319,43318,86637,1.0662260055541992,0.0006776122684189515
21745,43491,43490,86981,1.0709989070892334,0.0006675594015334395
21831,43663,43662,87325,1.0756940841674805,0.0006576372690157614
21917,43835,43834,87669,1.0804839134216309,0.0006479560431649065
22003,44007,44006,88013,1.0852241516113281,0.0006384066721074695
22089,44179,44178,88357,1.0899250507354736,0.0006289105777541214
22175,44351,44350,88701,1.0945179462432861,0.000619592603102619
22261,44523,44522,89045,1.0990879535675049,0.0006104863978389804
22346,44693,44692,89385,1.103600025177002,0.0006015604751864536
22432,44865,44864,89729,1.1083040237426758,0.0005926079075377935
22518,45037,45036,90073,1.1129930019378662,0.0005838606023143588
22604,45209,45208,90417,1.11759614944458,0.0005752740165147019
22690,45381,45380,90761,1.1221611499786377,0.0005667342254203769
22776,45553,45552,91105,1.1267340183258057,0.0005583147063076032
22862,45725,45724,91449,1.1314799785614014,0.0005500994341510182
22948,45897,45896,91793,1.136225938796997,0.0005419871706661015
23034,46069,46068,92137,1.140820026397705,0.0005339231138922232
23120,46241,46240,92481,1.145495891571045,0.0005260180410559427
23206,46413,46412,92825,1.1501359939575195,0.000518287500825606
23292,46585,46584,93169,1.1547009944915771,0.0005106151920184472
23378,46757,46756,93513,1.159369945526123,0.000503017485719737
23464,46929,46928,93857,1.1639540195465088,0.0004955984338883548
23550,47101,47100,94201,1.1685240268707275,0.0004883066773896462
23636,47273,47272,94545,1.1731081008911133,0.00048105317247861863
23722,47445,47444,94889,1.1777069568634033,0.0004739110727562024
23808,47617,47616,95233,1.1823348999023438,0.00046694094080637665
23894,47789,47788,95577,1.1869020462036133,0.00046004965388862925
23979,47959,47958,95917,1.191478967666626,0.0004532822610455747
24065,48131,48130,96261,1.196146011352539,0.0004465759450851923
24151,48303,48302,96605,1.2007231712341309,0.000440012699951178
24237,48475,48474,96949,1.205265998840332,0.00043349449923602636
24323,48647,48646,97293,1.2098159790039062,0.00042704592661497857
24409,48819,48818,97637,1.2148499488830566,0.00042075138744751214
24495,48991,48990,97981,1.2194249629974365,0.0004145580837440585
24581,49163,49162,98325,1.2240180969238281,0.00040839704694045696
24667,49335,49334,98669,1.228632926940918,0.00040233728258456036
24753,49507,49506,99013,1.2332251071929932,0.00039642167591287834
24839,49679,49678,99357,1.2377760410308838,0.00039056706307268686
24925,49851,49850,99701,1.242387056350708,0.0003847541849403505
25011,50023,50022,100045,1.2465908527374268,0.0003790666234591592
25097,50195,50194,100389,1.2507619857788086,0.0003734947471600937
25183,50367,50366,100733,1.2549059391021729,0.00036795744836016234
25269,50539,50538,101077,1.2590539455413818,0.0003624859099159946
25355,50711,50710,101421,1.263207197189331,0.0003571466428954446
25441,50883,50882,101765,1.2673461437225342,0.0003518863779935303
25527,51055,51054,102109,1.2714810371398926,0.00034665411227627227
25612,51225,51224,102449,1.2754788398742676,0.00034157339593042415
25698,51397,51396,102793,1.2795171737670898,0.0003365523801120308
25784,51569,51568,103137,1.2835619449615479,0.00033157840176962957
25870,51741,51740,103481,1.2875900268554688,0.00032664339028418886
25956,51913,51912,103825,1.2916340827941895,0.00032181830084266065
26042,52085,52084,104169,1.295665979385376,0.00031708691481147435
26128,52257,52256,104513,1.299712896347046,0.0003123828388058109
26214,52429,52428,104857,1.3037941455841064,0.0003077395903101878
26300,52601,52600,105201,1.3078711032867432,0.000303209107780399
26386,52773,52772,105545,1.3119258880615234,0.0002987407012144213
26472,52945,52944,105889,1.316011905670166,0.00029429713554051626
26558,53117,53116,106233,1.3200480937957764,0.00028993661245456316
26644,53289,53288,106577,1.3242111206054688,0.0002856753684455206
26730,53461,53460,106921,1.3284058570861816,0.00028144974645986687
26816,53633,53632,107265,1.332564115524292,0.00027726122435001724
26902,53805,53804,107609,1.3366801738739014,0.0002731689792783883
26988,53977,53976,107953,1.3407959938049316,0.0002691514445633689
27074,54149,54148,108297,1.345024824142456,0.00026515567382098517
27160,54321,54320,108641,1.349259853363037,0.000261216650180326
27245,54491,54490,108981,1.3533329963684082,0.0002574173877440626
27331,54663,54662,109325,1.3575100898742676,0.0002536214604679812
27417,54835,54834,109669,1.3618800640106201,0.0002498479913891673
27503,55007,55006,110013,1.3661110401153564,0.00024614866956180223
27589,55179,55178,110357,1.370300054550171,0.0002425311892532004
27675,55351,55350,110701,1.3745050430297852,0.00023894115358455144
27761,55523,55522,111045,1.3786919116973877,0.0002353858267478034
27847,55695,55694,111389,1.3828890323638916,0.00023191397602624644
27933,55867,55866,111733,1.3870420455932617,0.000228501899861128
28019,56039,56038,112077,1.3913559913635254,0.00022510772408899013
28105,56211,56210,112421,1.3956210613250732,0.0002217654412464072
28191,56383,56382,112765,1.399975061416626,0.00021850370055519374
28277,56555,56554,113109,1.404306173324585,0.00021527907687030146
28363,56727,56726,113453,1.4086549282073975,0.0002120753435403348
28449,56899,56898,113797,1.4129829406738281,0.00020893792835379238
28535,57071,57070,114141,1.4172930717468262,0.0002058671835755237
28621,57243,57242,114485,1.4216029644012451,0.00020281732871140374
28707,57415,57414,114829,1.4259159564971924,0.00019980039006669165
28793,57587,57586,115173,1.4302220344543457,0.00019685559941080217
28879,57759,57758,115517,1.4345719814300537,0.000193957801084495
28964,57929,57928,115857,1.4388010501861572,0.0001911084462638326
29050,58101,58100,116201,1.4430460929870605,0.00018827264695451453
29136,58273,58272,116545,1.447378158569336,0.00018550439469113933
29222,58445,58444,116889,1.4517788887023926,0.00018276486887027475
29308,58617,58616,117233,1.456169843673706,0.00018004473588478022
29394,58789,58788,117577,1.4605181217193604,0.00017738310929967286
29480,58961,58960,117921,1.4648411273956299,0.00017477580071856478
29566,59133,59132,118265,1.469188928604126,0.0001721847850031262
29652,59305,59304,118609,1.4735260009765625,0.00016962436506255817
29738,59477,59476,118953,1.4779679775238037,0.00016712579142907043
29824,59649,59648,119297,1.4823431968688965,0.0001646643540578786
29910,59821,59820,119641,1.486694097518921,0.0001622159980690703
29996,59993,59992,119985,1.4910991191864014,0.00015981075512621327
30082,60165,60164,120329,1.4956729412078857,0.0001574616350230963
30168,60337,60336,120673,1.500175952911377,0.00015513428416482508
30254,60509,60508,121017,1.5047600269317627,0.00015282534617115558
30340,60681,60680,121361,1.509263038635254,0.0001505680103093439
30426,60853,60852,121705,1.5137948989868164,0.00014835429502618424
30512,61025,61024,122049,1.5182392597198486,0.00014615328113752615
30597,61195,61194,122389,1.522507905960083,0.0001440059673038253
30683,61367,61366,122733,1.5268042087554932,0.0001418858818719644
30769,61539,61538,123077,1.5310490131378174,0.000139794982111015
30855,61711,61710,123421,1.535581111907959,0.00013771566800297645
30941,61883,61882,123765,1.5398361682891846,0.00013567508085086328
31027,62055,62054,124109,1.5444068908691406,0.00013368102734691114
31113,62227,62226,124453,1.5490880012512207,0.0001317037348863373
31199,62399,62398,124797,1.553415060043335,0.00012974367820158203
31285,62571,62570,125141,1.5580651760101318,0.0001278286161480512
31371,62743,62742,125485,1.5637600421905518,0.00012594866772470706
31457,62915,62914,125829,1.5680181980133057,0.00012407894008885568
31543,63087,63086,126173,1.5725128650665283,0.00012223562471463126
31629,63259,63258,126517,1.5768139362335205,0.00012043702768977838
31715,63431,63430,126861,1.5817959308624268,0.00011866091680611881
31801,63603,63602,127205,1.5870380401611328,0.00011689540200436957
31887,63775,63774,127549,1.5926849842071533,0.000115164757577621
31973,63947,63946,127893,1.5985801219940186,0.00011347226024054985
32059,64119,64118,128237,1.604067087173462,0.00011179245862063107
32145,64291,64290,128581,1.6096460819244385,0.00011012906250855806
32230,64461,64460,128921,1.6150829792022705,0.0001085234524122863
32316,64633,64632,129265,1.6205217838287354,0.00010692682983038258
32402,64805,64804,129609,1.6258659362792969,0.00010533860387139698
32488,64977,64976,129953,1.6310780048370361,0.00010377454064005074
32574,65149,65148,130297,1.6361849308013916,0.00010224818513428412
32660,65321,65320,130641,1.6406819820404053,0.00010073930746994355
32746,65493,65492,130985,1.6449670791625977,9.924016194913382e-05
32832,65665,65664,131329,1.6497409343719482,9.777196061038674e-05
32918,65837,65836,131673,1.6545050144195557,9.633502061207089e-05
33004,66009,66008,132017,1.6589438915252686,9.490790118193469e-05
33090,66181,66180,132361,1.6634211540222168,9.349608966011154e-05
33176,66353,66352,132705,1.667593240737915,9.21180197373169e-05
33262,66525,66524,133049,1.6718719005584717,9.076204433342098e-05
33348,66697,66696,133393,1.6761610507965088,8.941312507459291e-05
33434,66869,66868,133737,1.680422067642212,8.808643938394933e-05
33520,67041,67040,134081,1.6846938133239746,8.679130621036814e-05
33606,67213,67212,134425,1.6889400482177734,8.550948251911404e-05
33692,67385,67384,134769,1.6933040618896484,8.423683098066127e-05
33778,67557,67556,135113,1.6978578567504883,8.299165358082923e-05
33863,67727,67726,135453,1.7024359703063965,8.178589019555024e-05
33949,67899,67898,135797,1.7071049213409424,8.057347103075928e-05
34035,68071,68070,136141,1.7117640972137451,7.937528378257008e-05
34121,68243,68242,136485,1.716614007949829,7.820603229035305e-05
34207,68415,68414,136829,1.7210149765014648,7.70542507126082e-05
34293,68587,68586,137173,1.725532054901123,7.590857275817595e-05
34379,68759,68758,137517,1.7304019927978516,7.478298734340383e-05
34465,68931,68930,137861,1.735079050064087,7.36837087504785e-05
34551,69103,69102,138205,1.7403271198272705,7.259469475049524e-05
34637,69275,69274,138549,1.746056079864502,7.151424724146544e-05
34723,69447,69446,138893,1.7517759799957275,7.045789237003418e-05
34809,69619,69618,139237,1.7570960521697998,6.942200848288173e-05
34895,69791,69790,139581,1.7626028060913086,6.839209308285446e-05
34981,69963,69962,139925,1.7677550315856934,6.73755448689287e-05
35067,70135,70134,140269,1.772508144378662,6.638368016748637e-05
35153,70307,70306,140613,1.7768738269805908,6.540535157596749e-05
35239,70479,70478,140957,1.7817890644073486,6.443247004108123e-05
35325,70651,70650,141301,1.7859618663787842,6.347781310836264e-05
35411,70823,70822,141645,1.790315866470337,6.254487174899817e-05
35497,70995,70994,141989,1.7948682308197021,6.161969598850463e-05
35582,71165,71164,142329,1.7998790740966797,6.071323911077984e-05
35668,71337,71336,142673,1.8048980236053467,5.981705787083369e-05
35754,71509,71508,143017,1.8096449375152588,5.8937359798336586e-05
35840,71681,71680,143361,1.8146798610687256,5.8062456854623936e-05
35926,71853,71852,143705,1.8193190097808838,5.719985271334703e-05
36012,72025,72024,144049,1.8236970901489258,5.635817953017027e-05
36098,72197,72196,144393,1.8283019065856934,5.552708358351253e-05
36184,72369,72368,144737,1.8327021598815918,5.470091517882833e-05
36270,72541,72540,145081,1.8368799686431885,5.389101557122807e-05
36356,72713,72712,145425,1.841158151626587,5.309901490973782e-05
36442,72885,72884,145769,1.846200942993164,5.231299886233082e-05
36528,73057,73056,146113,1.850682020187378,5.153460931439487e-05
36614,73229,73228,146457,1.8549840450286865,5.077451161246858e-05
36700,73401,73400,146801,1.8594379425048828,5.002747213092712e-05
36786,73573,73572,147145,1.864603042602539,4.9284354007641924e-05
36872,73745,73744,147489,1.8689000606536865,4.855263077511301e-05
36958,73917,73916,147833,1.8731560707092285,4.783852850501658e-05
37044,74089,74088,148177,1.8774409294128418,4.71325185116135e-05
37130,74261,74260,148521,1.882030963897705,4.643110068238969e-05
37215,74431,74430,148861,1.8862318992614746,4.575210262874361e-05
37301,74603,74602,149205,1.8905272483825684,4.507969415669968e-05
37387,74775,74774,149549,1.8950860500335693,4.441191458506197e-05
37473,74947,74946,149893,1.8996069431304932,4.375125353345036e-05
37559,75119,75118,150237,1.9045448303222656,4.310636520279342e-05
37645,75291,75290,150581,1.9091439247131348,4.2471862515674544e-05
37731,75463,75462,150925,1.9134409427642822,4.184066503592703e-05
37817,75635,75634,151269,1.9180450439453125,4.121982734813917e-05
37903,75807,75806,151613,1.9223690032958984,4.061376370211291e-05
37989,75979,75978,151957,1.9266560077667236,4.001396098963343e-05
38075,76151,76150,152301,1.930945873260498,3.941842168310659e-05
38161,76323,76322,152645,1.9352309703826904,3.8835711686335444e-05
38247,76495,76494,152989,1.939518928527832,3.82648704959913e-05
38333,76667,76666,153333,1.9438130855560303,3.7697580494257353e-05
38419,76839,76838,153677,1.9481329917907715,3.7137012173231695e-05
38505,77011,77010,154021,1.9524450302124023,3.658999222928708e-05
38591,77183,77182,154365,1.956800937652588,3.605108204933596e-05
38677,77355,77354,154709,1.9612131118774414,3.5515040707859434e-05
38763,77527,77526,155053,1.965501070022583,3.498846043069788e-05
38848,77697,77696,155393,1.9697189331054688,3.448009819991181e-05
38934,77869,77868,155737,1.973963975906372,3.397051652556742e-05
39020,78041,78040,156081,1.978896141052246,3.346491542640307e-05
39106,78213,78212,156425,1.9830381870269775,3.297056907412223e-05
39192,78385,78384,156769,1.9871830940246582,3.248583782220024e-05
39278,78557,78556,157113,1.9913971424102783,3.200391088966711e-05
39364,78729,78728,157457,1.9956209659576416,3.1528202432385715e-05
39450,78901,78900,157801,1.9998021125793457,3.106404534277506e-05
39536,79073,79072,158145,2.003955125808716,3.060626079247855e-05
39622,79245,79244,158489,2.008092164993286,3.0151019814877983e-05
39708,79417,79416,158833,2.012255907058716,2.970427531377726e-05
39794,79589,79588,159177,2.016361951828003,2.9267706119114812e-05
39880,79761,79760,159521,2.020500898361206,2.8834792763700906e-05
39966,79933,79932,159865,2.0246810913085938,2.840567072761419e-05
40052,80105,80104,160209,2.028964042663574,2.798640792263026e-05
40138,80277,80276,160553,2.0331790447235107,2.757481092565292e-05
40224,80449,80448,160897,2.0373940467834473,2.716544490000795e-05
40310,80621,80620,161241,2.0416100025177,2.6761880770991175e-05
40396,80793,80792,161585,2.045837879180908,2.6368107487178306e-05
40481,80963,80962,161925,2.050105094909668,2.598375456593364e-05
40567,81135,81134,162269,2.0543370246887207,2.5597163309410875e-05
40653,81307,81306,162613,2.0587282180786133,2.5218159503550513e-05
40739,81479,81478,162957,2.0629348754882812,2.4847545100435236e-05
40825,81651,81650,163301,2.067134141921997,2.447974692544335e-05
40911,81823,81822,163645,2.071337938308716,2.411549571699214e-05
40997,81995,81994,163989,2.0755701065063477,2.3759794228839994e-05
41083,82167,82166,164333,2.0798051357269287,2.3410227394899664e-05
41169,82339,82338,164677,2.0840070247650146,2.306249479144541e-05
41255,82511,82510,165021,2.0882091522216797,2.2720068618989254e-05
41341,82683,82682,165365,2.0924201011657715,2.2385897083742326e-05
41427,82855,82854,165709,2.0966389179229736,2.205553862533701e-05
41513,83027,83026,166053,2.1009440422058105,2.1727317206850885e-05
41599,83199,83198,166397,2.105232000350952,2.1405882316652922e-05
41685,83371,83370,166741,2.1095120906829834,2.109128257499854e-05
41771,83543,83542,167085,2.1137351989746094,2.077882736697973e-05
41857,83715,83714,167429,2.117950201034546,2.0469737473461178e-05
41943,83887,83886,167773,2.122215986251831,2.0168036727199977e-05
42029,84059,84058,168117,2.1264538764953613,1.987115736066685e-05
42114,84229,84228,168457,2.130622148513794,1.9579237063370162e-05
42200,84401,84400,168801,2.134882926940918,1.928870178618181e-05
42286,84573,84572,169145,2.1391031742095947,1.90050898543715e-05
42372,84745,84744,169489,2.143404960632324,1.872442923603327e-05
42458,84917,84916,169833,2.1474931240081787,1.8445752036728972e-05
42544,85089,85088,170177,2.1516408920288086,1.8173062732124407e-05
42630,85261,85260,170521,2.155764102935791,1.790594269184106e-05
42716,85433,85432,170865,2.159848213195801,1.7640494560195586e-05
42802,85605,85604,171209,2.1639490127563477,1.73781746330066e-05
42888,85777,85776,171553,2.168199062347412,1.712218988332349e-05
42974,85949,85948,171897,2.172212839126587,1.6870016056123874e-05
43060,86121,86120,172241,2.176248073577881,1.6619180104599506e-05
43146,86293,86292,172585,2.1806671619415283,1.6372754794858026e-05
43232,86465,86464,172929,2.1852450370788574,1.613208385588255e-05
43318,86637,86636,173273,2.18973708152771,1.5893649736778355e-05
43404,86809,86808,173617,2.1939618587493896,1.565709743635867e-05
43490,86981,86980,173961,2.199265956878662,1.5425827527910273e-05
43576,87153,87152,174305,2.203488826751709,1.5199032187722161e-05
43662,87325,87324,174649,2.2075271606445312,1.497354112181679e-05
43748,87497,87496,174993,2.211498975753784,1.4750986384827463e-05
43833,87667,87666,175333,2.2154128551483154,1.4536337388823615e-05
43919,87839,87838,175677,2.219491958618164,1.4322125419051483e-05
44005,88011,88010,176021,2.223539113998413,1.41090978687209e-05
44091,88183,88182,176365,2.2276298999786377,1.390003279461031e-05
44177,88355,88354,176709,2.231806993484497,1.3695739533211e-05
44263,88527,88526,177053,2.2358651161193848,1.3493168718444876e-05
44349,88699,88698,177397,2.240049123764038,1.3292359543028983e-05
44435,88871,88870,177741,2.2443461418151855,1.3096156820662643e-05
44521,89043,89042,178085,2.249082088470459,1.2903556240787107e-05
44607,89215,89214,178429,2.2533271312713623,1.2712004600631175e-05
44693,89387,89386,178773,2.2574870586395264,1.2523154106154338e-05
44779,89559,89558,179117,2.261539936065674,1.23388846424572e-05
44865,89731,89730,179461,2.2656118869781494,1.2156922636009888e-05
44951,89903,89902,179805,2.2696831226348877,1.1976043740501662e-05
45037,90075,90074,180149,2.273822069168091,1.1798733630411028e-05
45123,90247,90246,180493,2.2779769897460938,1.162533551203661e-05
45209,90419,90418,180837,2.282125949859619,1.1453241007342942e-05
45295,90591,90590,181181,2.2862818241119385,1.1282822730287928e-05
45381,90763,90762,181525,2.290432929992676,1.111641312059396e-05
45466,90933,90932,181865,2.294529914855957,1.0954752298251405e-05
45552,91105,91104,182209,2.2988109588623047,1.0792039753610796e-05
45638,91277,91276,182553,2.303016185760498,1.0631798584918207e-05
45724,91449,91448,182897,2.307237148284912,1.0475420872429507e-05
45810,91621,91620,183241,2.311401844024658,1.0320836850421121e-05
45896,91793,91792,183585,2.315553903579712,1.0167247288089995e-05
45982,91965,91964,183929,2.3196990489959717,1.0016825158744112e-05
46068,92137,92136,184273,2.323889970779419,9.869609514834563e-06
46154,92309,92308,184617,2.3280529975891113,9.723402279054328e-06
46240,92481,92480,184961,2.3321990966796875,9.57875936369615e-06
46326,92653,92652,185305,2.33634090423584,9.437572433829018e-06
46412,92825,92824,185649,2.340553045272827,9.298653611509171e-06
46498,92997,92996,185993,2.3448948860168457,9.160458311247848e-06
46584,93169,93168,186337,2.3490779399871826,9.0245370822514e-06
46670,93341,93340,186681,2.35327410697937,8.891848892719538e-06
46756,93513,93512,187025,2.3574230670928955,8.760527020436626e-06
46842,93685,93684,187369,2.361565113067627,8.630142915123343e-06
46928,93857,93856,187713,2.365694046020508,8.502571203198931e-06
47014,94029,94028,188057,2.3698232173919678,8.377592144176374e-06
47099,94199,94198,188397,2.373812198638916,8.254826579662353e-06
47185,94371,94370,188741,2.377774953842163,8.132069944355527e-06
47271,94543,94542,189085,2.3818578720092773,8.012277312468747e-06
47357,94715,94714,189429,2.3858678340911865,7.894278206045482e-06
47443,94887,94886,189773,2.3899519443511963,7.77690457164301e-06
47529,95059,95058,190117,2.393980026245117,7.661586308115583e-06
47615,95231,95230,190461,2.398106098175049,7.548963859734535e-06
47701,95403,95402,190805,2.402268171310425,7.43739507767848e-06
47787,95575,95574,191149,2.4065210819244385,7.326701946926654e-06
47873,95747,95746,191493,2.410706043243408,7.218475461441527e-06
47959,95919,95918,191837,2.414868116378784,7.112348705324352e-06
48045,96091,96090,192181,2.4190540313720703,7.006833883961287e-06
48131,96263,96262,192525,2.423272132873535,6.902685540359725e-06
48217,96435,96434,192869,2.427597999572754,6.801066504615991e-06
48303,96607,96606,193213,2.431820869445801,6.7008376318654204e-06
48389,96779,96778,193557,2.4361209869384766,6.601166210913315e-06
48475,96951,96950,193901,2.440380096435547,6.503359267493789e-06
48561,97123,97122,194245,2.444650888442993,6.407778460119969e-06
48647,97295,97294,194589,2.448927164077759,6.3129954407065025e-06
48732,97465,97464,194929,2.453130006790161,6.2201282068247805e-06
48818,97637,97636,195273,2.457395076751709,6.128311877854209e-06
48904,97809,97808,195617,2.461643934249878,6.038186609350915e-06
48990,97981,97980,195961,2.4658899307250977,5.948552786946322e-06
49076,98153,98152,196305,2.470128059387207,5.860176411402969e-06
49162,98325,98324,196649,2.4743478298187256,5.773945079570285e-06
49248,98497,98496,196993,2.478616952896118,5.688800227824727e-06
49334,98669,98668,197337,2.4828829765319824,5.6041595139826154e-06
49420,98841,98840,197681,2.487558126449585,5.521183401589622e-06
49506,99013,99012,198025,2.4918088912963867,5.440042288316114e-06
49592,99185,99184,198369,2.4960649013519287,5.359515896675196e-06
49678,99357,99356,198713,2.5004031658172607,5.279769261296706e-06
49764,99529,99528,199057,2.5046679973602295,5.201895573646095e-06
49850,99701,99700,199401,2.508923053741455,5.125361293618182e-06
49936,99873,99872,199745,2.5131611824035645,5.049228600671948e-06
50022,100045,100044,200089,2.517396926879883,4.97426134453938e-06
50108,100217,100216,200433,2.5216450691223145,4.901100126825626e-06
50194,100389,100388,200777,2.525897979736328,4.828769928450503e-06
50280,100561,100560,201121,2.530133008956909,4.756908975385398e-06
50365,100731,100730,201461,2.5343000888824463,4.6873445772367265e-06
50451,100903,100902,201805,2.538512945175171,4.618455908886837e-06
50537,101075,101074,202149,2.542729139328003,4.550042579687513e-06
50623,101247,101246,202493,2.5469720363616943,4.482357069200044e-06
50709,101419,101418,202837,2.5512681007385254,4.4162868200935e-06
50795,101591,101590,203181,2.5555031299591064,4.351282017481602e-06
50881,101763,101762,203525,2.5597710609436035,4.2866154738530175e-06
50967,101935,101934,203869,2.564099073410034,4.223008643016652e-06
51053,102107,102106,204213,2.5681891441345215,4.160916321202825e-06
51139,102279,102278,204557,2.5722410678863525,4.099467090716604e-06
51225,102451,102450,204901,2.576375961303711,4.038453499149208e-06
51311,102623,102622,205245,2.5803639888763428,3.978753116800276e-06
51397,102795,102794,205589,2.5844881534576416,3.9202702474791925e-06
51483,102967,102966,205933,2.5884671211242676,3.8621522443345645e-06
51569,103139,103138,206277,2.5924770832061768,3.8047214734283827e-06
51655,103311,103310,206621,2.596503973007202,3.7486782189012983e-06
51741,103483,103482,206965,2.600576877593994,3.6934670653005266e-06
51827,103655,103654,207309,2.604598045349121,3.6385496080667923e-06
51913,103827,103826,207653,2.6086370944976807,3.5846001225805252e-06
51999,103999,103998,207997,2.612607955932617,3.5319089116620433e-06
52084,104169,104168,208337,2.616734027862549,3.4803106272101887e-06
52170,104341,104340,208681,2.6207010746002197,3.4285113028449526e-06
52256,104513,104512,209025,2.6247169971466064,3.3778641371420924e-06
52342,104685,104684,209369,2.628793954849243,3.328203372336626e-06
52428,104857,104856,209713,2.632766008377075,3.27883063749508e-06
52514,105029,105028,210057,2.6368491649627686,3.230093757012239e-06
52600,105201,105200,210401,2.6409378051757812,3.1825400119746503e-06
52686,105373,105372,210745,2.6450138092041016,3.1356401587593768e-06
52772,105545,105544,211089,2.6491990089416504,3.089000521804642e-06
52858,105717,105716,211433,2.653301954269409,3.0432302942328116e-06
52944,105889,105888,211777,2.657464027404785,2.9985032258083603e-06
53030,106061,106060,212121,2.661518096923828,2.9541514441893848e-06
53116,106233,106232,212465,2.6655662059783936,2.9101869845754885e-06
53202,106405,106404,212809,2.669609785079956,2.8672321704505634e-06
53288,106577,106576,213153,2.673712968826294,2.8250641023212075e-06
53374,106749,106748,213497,2.6778249740600586,2.783124988433654e-06
53460,106921,106920,213841,2.681887149810791,2.7417790906966887e-06
53546,107093,107092,214185,2.6859371662139893,2.701436289403037e-06
53632,107265,107264,214529,2.6899828910827637,2.6615972063793135e-06
53717,107435,107434,214869,2.6940488815307617,2.6224535261267124e-06
53803,107607,107606,215213,2.6981279850006104,2.58362343848867e-06
53889,107779,107778,215557,2.702230930328369,2.5456535939790627e-06
53975,107951,107950,215901,2.7063488960266113,2.5079728587197565e-06
54061,108123,108122,216245,2.7104389667510986,2.4706545193564296e-06
54147,108295,108294,216589,2.7145299911499023,2.4342118269328957e-06
54233,108467,108466,216933,2.7186222076416016,2.398398833906253e-06
54319,108639,108638,217277,2.7227671146392822,2.3627740045185593e-06
54405,108811,108810,217621,2.7269129753112793,2.3276918161992426e-06
54491,108983,108982,217965,2.73095703125,2.2934553991351676e-06
54577,109155,109154,218309,2.735053062438965,2.2596104984447542e-06
54663,109327,109326,218653,2.7391340732574463,2.225984207461046e-06
54749,109499,109498,218997,2.743285894393921,2.1930524687022117e-06
54835,109671,109670,219341,2.7484419345855713,2.1608214791370485e-06
54921,109843,109842,219685,2.7542471885681152,2.1288105029579198e-06
55007,110015,110014,220029,2.7585928440093994,2.0971434882026484e-06
55093,110187,110186,220373,2.762874126434326,2.0662333938999476e-06
55179,110359,110358,220717,2.7670021057128906,2.035818191657563e-06
55265,110531,110530,221061,2.771113157272339,2.005561238477005e-06
55350,110701,110700,221401,2.775238037109375,1.976145207706934e-06
55436,110873,110872,221745,2.7795748710632324,1.9470887612750627e-06
55522,111045,111044,222089,2.7837212085723877,1.9183353401968875e-06
55608,111217,111216,222433,2.788939952850342,1.8897847434834728e-06
55694,111389,111388,222777,2.7930941581726074,1.8618470582435151e-06
55780,111561,111560,223121,2.7979140281677246,1.834480440189711e-06
55866,111733,111732,223465,2.802610158920288,1.8072852947843174e-06
55952,111905,111904,223809,2.807018995285034,1.7804099040601701e-06
56038,112077,112076,224153,2.811241865158081,1.7541835705245169e-06
56124,112249,112248,224497,2.8153979778289795,1.7283484990540143e-06
56210,112421,112420,224841,2.8195600509643555,1.7026503594481936e-06
56296,112593,112592,225185,2.823759078979492,1.6774033914383054e-06
56382,112765,112764,225529,2.8280279636383057,1.6527463255472664e-06
56468,112937,112936,225873,2.832213878631592,1.6283191019548684e-06
56554,113109,113108,226217,2.836367130279541,1.604084299845657e-06
56640,113281,113280,226561,2.8405210971832275,1.580390201992924e-06
56726,113453,113452,226905,2.8453450202941895,1.5571549536249867e-06
56812,113625,113624,227249,2.8498270511627197,1.534053499145587e-06
56898,113797,113796,227593,2.854116916656494,1.5112523027506792e-06
56983,113967,113966,227933,2.8583321571350098,1.4892606233577353e-06
57069,114139,114138,228277,2.8625290393829346,1.4673147747759306e-06
57155,114311,114310,228621,2.8666868209838867,1.4454901121254035e-06
57241,114483,114482,228965,2.8708488941192627,1.4240708319346085e-06
57327,114655,114654,229309,2.875101089477539,1.4031407633709019e-06
57413,114827,114826,229653,2.8792691230773926,1.382387679643485e-06
57499,114999,114998,229997,2.883527994155884,1.3618147172162132e-06
57585,115171,115170,230341,2.8876688480377197,1.341713330992676e-06
57671,115343,115342,230685,2.8918581008911133,1.321981366588748e-06
57757,115515,115514,231029,2.896048069000244,1.3023569332348881e-06
57843,115687,115686,231373,2.9002060890197754,1.2830087358902253e-06
57929,115859,115858,231717,2.9044361114501953,1.2641299405709782e-06
58015,116031,116030,232061,2.908890962600708,1.2454880103384884e-06
58101,116203,116202,232405,2.9130940437316895,1.2269567621183997e-06
58187,116375,116374,232749,2.917257785797119,1.2087907355480076e-06
58273,116547,116546,233093,2.921386957168579,1.1910259335712941e-06
58359,116719,116718,233437,2.9255049228668213,1.1733950939784465e-06
58445,116891,116890,233781,2.929638147354126,1.155935577012221e-06
58531,117063,117062,234125,2.933812141418457,1.1388865215202522e-06
58617,117235,117234,234469,2.937933921813965,1.1221301036185177e-06
58702,117405,117404,234809,2.9420180320739746,1.105654694240285e-06
58788,117577,117576,235153,2.94620418548584,1.0892375396255605e-06
58874,117749,117748,235497,2.9503469467163086,1.0732163319345084e-06
58960,117921,117920,235841,2.954512119293213,1.0573792889264695e-06
59046,118093,118092,236185,2.9587271213531494,1.0416438520249457e-06
59132,118265,118264,236529,2.962862014770508,1.02623260472598e-06
59218,118437,118436,236873,2.9669668674468994,1.0111502647755533e-06
59304,118609,118608,237217,2.9710590839385986,9.961715502333563e-07
59390,118781,118780,237561,2.975148916244507,9.813527402619427e-07
59476,118953,118952,237905,2.9793200492858887,9.668878339297394e-07
59562,119125,119124,238249,2.9834091663360596,9.52655655970987e-07
59648,119297,119296,238593,2.9875340461730957,9.384976340728266e-07
59734,119469,119468,238937,2.991711139678955,9.245722346828855e-07
59820,119641,119640,239281,2.9958410263061523,9.109781283863287e-07
59906,119813,119812,239625,3.000063896179199,8.975242486817724e-07
59992,119985,119984,239969,3.004261016845703,8.841661841904508e-07
60078,120157,120156,240313,3.0086581707000732,8.710960426024825e-07
60164,120329,120328,240657,3.0133919715881348,8.582918717024834e-07
60250,120501,120500,241001,3.017348051071167,8.455672160723083e-07
60335,120671,120670,241341,3.0212562084198,8.331380970426433e-07
60421,120843,120842,241685,3.0253989696502686,8.208651022055911e-07
60507,121015,121014,242029,3.0293610095977783,8.087761479029388e-07
60593,121187,121186,242373,3.033332109451294,7.967512511705442e-07
60679,121359,121358,242717,3.0372769832611084,7.849366331964429e-07
60765,121531,121530,243061,3.0412650108337402,7.733983057192711e-07
60851,121703,121702,243405,3.0453920364379883,7.619681224215152e-07
60937,121875,121874,243749,3.0495150089263916,7.506273985784029e-07
61023,122047,122046,244093,3.0536069869995117,7.395392385002747e-07
61109,122219,122218,244437,3.057873010635376,7.286665245561759e-07
61195,122391,122390,244781,3.0618999004364014,7.178566127175872e-07
61281,122563,122562,245125,3.0660741329193115,7.071863867959877e-07
61367,122735,122734,245469,3.0700619220733643,6.967752898216133e-07
61453,122907,122906,245813,3.07423996925354,6.865069409471636e-07
61539,123079,123078,246157,3.0783369541168213,6.762956787257074e-07
61625,123251,123250,246501,3.082412004470825,6.662751683099156e-07
61711,123423,123422,246845,3.086487054824829,6.564828153798816e-07
61797,123595,123594,247189,3.0907199382781982,6.467723569966794e-07
61883,123767,123766,247533,3.095555067062378,6.371470929144194e-07
61968,123937,123936,247873,3.099945068359375,6.278509776847169e-07
62054,124109,124108,248217,3.104980945587158,6.186176453502346e-07
62140,124281,124280,248561,3.109220027923584,6.094347363001117e-07
62226,124453,124452,248905,3.1144070625305176,6.00380388696284e-07
62312,124625,124624,249249,3.118649959564209,5.915458188819669e-07
62398,124797,124796,249593,3.1231160163879395,5.828228202802797e-07
62484,124969,124968,249937,3.127331018447876,5.741514230209364e-07
62570,125141,125140,250281,3.1325740814208984,5.656503520570673e-07
62656,125313,125312,250625,3.1368610858917236,5.573373718267283e-07
62742,125485,125484,250969,3.1412031650543213,5.490874823680843e-07
62828,125657,125656,251313,3.1456010341644287,5.409172945559627e-07
62914,125829,125828,251657,3.1500420570373535,5.329389216633643e-07
63000,126001,126000,252001,3.154555082321167,5.250979814520983e-07
63086,126173,126172,252345,3.159036159515381,5.172981701231166e-07
63172,126345,126344,252689,3.1635820865631104,5.096175390981975e-07
63258,126517,126516,253033,3.1681339740753174,5.02122024610876e-07
63344,126689,126688,253377,3.1725878715515137,4.947118857930312e-07
63430,126861,126860,253721,3.1771109104156494,4.873497338184561e-07
63516,127033,127032,254065,3.1816020011901855,4.801399240558397e-07
63601,127203,127202,254405,3.1860241889953613,4.731650975202931e-07
63687,127375,127374,254749,3.1904830932617188,4.6615617290114694e-07
63773,127547,127546,255093,3.1949729919433594,4.592216428212069e-07
63859,127719,127718,255437,3.199505090713501,4.524525648672708e-07
63945,127891,127890,255781,3.2040820121765137,4.457928344408863e-07
64031,128063,128062,256125,3.2086880207061768,4.391677309779974e-07
64117,128235,128234,256469,3.2132840156555176,4.3265101248936674e-07
64203,128407,128406,256813,3.217841148376465,4.262895460184727e-07
64289,128579,128578,257157,3.2222039699554443,4.1999415778971956e-07
64375,128751,128750,257501,3.2265989780426025,4.137433146343117e-07
64461,128923,128922,257845,3.230802059173584,4.076268733322464e-07
64547,129095,129094,258189,3.23502516746521,4.016352799802651e-07
64633,129267,129266,258533,3.239230155944824,3.956811482996995e-07
64719,129439,129438,258877,3.2435801029205322,3.8979728645510573e-07
64805,129611,129610,259221,3.248483896255493,3.8405553627259566e-07
64891,129783,129782,259565,3.252769947052002,3.7839916026866765e-07
64977,129955,129954,259909,3.257049083709717,3.7277282380567354e-07
65063,130127,130126,260253,3.2612531185150146,3.672455206814949e-07
65149,130299,130298,260597,3.265449047088623,3.61847224820581e-07
65234,130469,130468,260937,3.2695980072021484,3.565610263395574e-07
65320,130641,130640,261281,3.2737770080566406,3.512541796915096e-07
65406,130813,130812,261625,3.2779722213745117,3.460652659809035e-07
65492,130985,130984,261969,3.282155990600586,3.409775079785002e-07
65578,131157,131156,262313,3.28635311126709,3.359193074437309e-07
65664,131329,131328,262657,3.290541887283325,3.3092612798974264e-07
65750,131501,131500,263001,3.294715166091919,3.260541475370384e-07
65836,131673,131672,263345,3.2989118099212646,3.212492674696828e-07
65922,131845,131844,263689,3.3031139373779297,3.164709891107004e-07
66008,132017,132016,264033,3.307555913925171,3.1178167288877783e-07
66094,132189,132188,264377,3.3117642402648926,3.0719932648522636e-07
66180,132361,132360,264721,3.315988063812256,3.02655535438336e-07
66266,132533,132532,265065,3.3201639652252197,2.9815132156914646e-07
66352,132705,132704,265409,3.3244099617004395,2.9375048332562964e-07
66438,132877,132876,265753,3.328585147857666,2.894303713940966e-07
66524,133049,133048,266097,3.3327488899230957,2.8513376460558833e-07
66610,133221,133220,266441,3.3369429111480713,2.808978215202873e-07
66696,133393,133392,266785,3.341125011444092,2.767646330157876e-07
66782,133565,133564,267129,3.3452961444854736,2.726831381197184e-07
66868,133737,133736,267473,3.3494889736175537,2.686259765371107e-07
66953,133907,133906,267813,3.353640079498291,2.646945235396948e-07
67039,134079,134078,268157,3.357818126678467,2.6080447419024194e-07
67125,134251,134250,268501,3.362013101577759,2.5694412953426907e-07
67211,134423,134422,268845,3.366175889968872,2.5312081968880676e-07
67297,134595,134594,269189,3.3703560829162598,2.493871741595942e-07
67383,134767,134766,269533,3.3744280338287354,2.4571814496690573e-07
67469,134939,134938,269877,3.378453016281128,2.420684214488433e-07
67555,135111,135110,270221,3.3824238777160645,2.384741969378808e-07
67641,135283,135282,270565,3.3864009380340576,2.3496662167502715e-07
67727,135455,135454,270909,3.3904879093170166,2.3149922672541307e-07
67813,135627,135626,271253,3.395163059234619,2.2805417829274326e-07
67899,135799,135798,271597,3.4004011154174805,2.2468022208833382e-07
67985,135971,135970,271941,3.4044671058654785,2.2137813038172684e-07
68071,136143,136142,272285,3.408557891845703,2.1809861907073757e-07
68157,136315,136314,272629,3.4132909774780273,2.1485425593115568e-07
68243,136487,136486,272973,3.41749906539917,2.1168742825761202e-07
68329,136659,136658,273317,3.421588182449341,2.085714092423637e-07
68415,136831,136830,273661,3.4257659912109375,2.054716115408443e-07
68501,137003,137002,274005,3.4302608966827393,2.0242287997676806e-07
68586,137173,137172,274345,3.4344980716705322,1.994810429371442e-07
68672,137345,137344,274689,3.438516139984131,1.965352666088048e-07
68758,137517,137516,275033,3.4425740242004395,1.9361021713799434e-07
68844,137689,137688,275377,3.447005033493042,1.907479132291259e-07
68930,137861,137860,275721,3.451004981994629,1.879441868261561e-07
69016,138033,138032,276065,3.455026149749756,1.8515805677365556e-07
69102,138205,138204,276409,3.459096908569336,1.8240460650698365e-07
69188,138377,138376,276753,3.4631881713867188,1.7971764964595907e-07
69274,138549,138548,277097,3.4672491550445557,1.7707086808549525e-07
69360,138721,138720,277441,3.4713470935821533,1.7443811577633863e-07
69446,138893,138892,277785,3.475512981414795,1.7185151400712543e-07
69532,139065,139064,278129,3.4796760082244873,1.6932536748659634e-07
69618,139237,139236,278473,3.4838387966156006,1.6682282237172872e-07
69704,139409,139408,278817,3.4880192279815674,1.643399517262983e-07
69790,139581,139580,279161,3.492224931716919,1.6191243414305528e-07
69876,139753,139752,279505,3.4964420795440674,1.5953197253299859e-07
69962,139925,139924,279849,3.5006179809570312,1.5716522671071071e-07
70048,140097,140096,280193,3.504791021347046,1.5482917795844218e-07
70134,140269,140268,280537,3.5089399814605713,1.5254985792547496e-07
70219,140439,140438,280877,3.51305890083313,1.503277337479583e-07
70305,140611,140610,281221,3.5184731483459473,1.480918134986167e-07
70391,140783,140782,281565,3.5226449966430664,1.4589736602959086e-07
70477,140955,140954,281909,3.52679705619812,1.4375305872750564e-07
70563,141127,141126,282253,3.530963182449341,1.416269231411525e-07
70649,141299,141298,282597,3.5351221561431885,1.3951920100135785e-07
70735,141471,141470,282941,3.5393152236938477,1.37459763513016e-07
70821,141643,141642,283285,3.5434799194335938,1.3543821781324585e-07
70907,141815,141814,283629,3.547657012939453,1.3342769010037797e-07
70993,141987,141986,283973,3.551846981048584,1.314454075134706e-07
71079,142159,142158,284317,3.556020975112915,1.2951123134862306e-07
71165,142331,142330,284661,3.5601840019226074,1.2760138261223998e-07
71251,142503,142502,285005,3.5645339488983154,1.2570285222835523e-07
71337,142675,142674,285349,3.5687332153320312,1.238416924857981e-07
71423,142847,142846,285693,3.572962999343872,1.2202167380590278e-07
71509,143019,143018,286037,3.5769970417022705,1.2021542058625597e-07
71595,143191,143190,286381,3.58096981048584,1.1842668355062717e-07
71681,143363,143362,286725,3.584951877593994,1.1667997233172219e-07
71767,143535,143534,287069,3.5889101028442383,1.1496327711367511e-07
71852,143705,143704,287409,3.5928730964660645,1.1327535683954595e-07
71938,143877,143876,287753,3.5972259044647217,1.1159336664212353e-07
72024,144049,144048,288097,3.6012048721313477,1.0995196040136061e-07
72110,144221,144220,288441,3.6051838397979736,1.0832947311621003e-07
72196,144393,144392,288785,3.6092231273651123,1.067173744734097e-07
72282,144565,144564,289129,3.613248825073242,1.0513845163394736e-07
72368,144737,144736,289473,3.6174089908599854,1.0359325706979166e-07
72454,144909,144908,289817,3.6214098930358887,1.0205870865171373e-07
72540,145081,145080,290161,3.6254730224609375,1.005405093333378e-07
72626,145253,145252,290505,3.629599094390869,9.905855002591735e-08
72712,145425,145424,290849,3.6336731910705566,9.760046426593418e-08
72798,145597,145596,291193,3.637714147567749,9.614997072037842e-08
72884,145769,145768,291537,3.6418230533599854,9.472327332976307e-08
72970,145941,145940,291881,3.646036148071289,9.333053340411697e-08
73056,146113,146112,292225,3.650163173675537,9.195219155165083e-08
73142,146285,146284,292569,3.6547000408172607,9.058363786087751e-08
73228,146457,146456,292913,3.6588048934936523,8.92445587717115e-08
73314,146629,146628,293257,3.662869930267334,8.793276658724153e-08
73400,146801,146800,293601,3.6669270992279053,8.66291436967578e-08
73485,146971,146970,293941,3.670948028564453,8.535577996270512e-08
73571,147143,147142,294285,3.675062894821167,8.409838669406913e-08
73657,147315,147314,294629,3.6791160106658936,8.285987489309883e-08
73743,147487,147486,294973,3.68322491645813,8.162791663480763e-08
73829,147659,147658,295317,3.68727707862854,8.0417471795338e-08
73915,147831,147830,295661,3.6913340091705322,7.92353523638655e-08
74001,148003,148002,296005,3.69585919380188,7.806433845902442e-08
74087,148175,148174,296349,3.7007510662078857,7.690246409230166e-08
74173,148347,148346,296693,3.704897880554199,7.576644743933038e-08
74259,148519,148518,297037,3.7091591358184814,7.465253688125694e-08
74345,148691,148690,297381,3.713470220565796,7.35450768271276e-08
74431,148863,148862,297725,3.717827081680298,7.245189841041025e-08
74517,149035,149034,298069,3.722278118133545,7.138526191195088e-08
74603,149207,149206,298413,3.7264628410339355,7.033327588955933e-08
74689,149379,149378,298757,3.7307140827178955,6.928713321609036e-08
74775,149551,149550,299101,3.7349119186401367,6.82605085532337e-08
74861,149723,149722,299445,3.739022970199585,6.725727025889046e-08
74947,149895,149894,299789,3.743185043334961,6.626243662732193e-08
75033,150067,150066,300133,3.747375965118408,6.527630752609028e-08
75119,150239,150238,300477,3.7514750957489014,6.431283311667064e-08
75204,150409,150408,300817,3.75553297996521,6.337793382735866e-08
75290,150581,150580,301161,3.759688138961792,6.243715707903415e-08
75376,150753,150752,301505,3.7638039588928223,6.150952706264794e-08
75462,150925,150924,301849,3.767888069152832,6.060441015462716e-08
75548,151097,151096,302193,3.772033929824829,5.971074413048224e-08
75634,151269,151268,302537,3.7761268615722656,5.882235667067096e-08
75720,151441,151440,302881,3.7803738117218018,5.7951400066256276e-08
75806,151613,151612,303225,3.7844619750976562,5.709972644651793e-08
75892,151785,151784,303569,3.788547992706299,5.6254527678756155e-08
75978,151957,151956,303913,3.792628049850464,5.541747253660384e-08
76064,152129,152128,304257,3.796802043914795,5.460006358546363e-08
76150,152301,152300,304601,3.8009250164031982,5.379676107887067e-08
76236,152473,152472,304945,3.8050589561462402,5.2997675615252765e-08
76322,152645,152644,305289,3.8092031478881836,5.2210776967026994e-08
76408,152817,152816,305633,3.813383102416992,5.144284841794538e-08
76494,152989,152988,305977,3.81754207611084,5.068368885858578e-08
76580,153161,153160,306321,3.821693181991577,4.9929438585661096e-08
76666,153333,153332,306665,3.8259780406951904,4.9190778665413243e-08
76752,153505,153504,307009,3.830068826675415,4.846782814268902e-08
76837,153675,153674,307349,3.8342130184173584,4.77581356978799e-08
76923,153847,153846,307693,3.83833909034729,4.704767538771315e-08
77009,154019,154018,308037,3.842519998550415,4.635416358050207e-08
77095,154191,154190,308381,3.846748113632202,4.567187757235517e-08
77181,154363,154362,308725,3.8509860038757324,4.499314052266171e-08
77267,154535,154534,309069,3.855187177658081,4.4325488003848056e-08
77353,154707,154706,309413,3.8594419956207275,4.367374631700277e-08
77439,154879,154878,309757,3.8636980056762695,4.302879124064925e-08
77525,155051,155050,310101,3.8679089546203613,4.2388392465621556e-08
77611,155223,155222,310445,3.872182846069336,4.176174980979716e-08
77697,155395,155394,310789,3.8764078617095947,4.1147907703381816e-08
77783,155567,155566,311133,3.880702018737793,4.053790840194118e-08
77869,155739,155738,311477,3.885004997253418,3.993509240991983e-08
77955,155911,155910,311821,3.889248847961426,3.9346835399714774e-08
78041,156083,156082,312165,3.893562078475952,3.8767341526234933e-08
78127,156255,156254,312509,3.897778034210205,3.8190920699675064e-08
78213,156427,156426,312853,3.9020540714263916,3.7624630528658325e-08
78299,156599,156598,313197,3.9063820838928223,3.707156717241821e-08
78385,156771,156770,313541,3.9107069969177246,3.6523649493361455e-08
78470,156941,156940,313881,3.9149248600006104,3.5986321787912915e-08
78556,157113,157112,314225,3.9191219806671143,3.545470571316525e-08
78642,157285,157284,314569,3.9233250617980957,3.4933462636950824e-08
78728,157457,157456,314913,3.927820920944214,3.4415250255675586e-08
78814,157629,157628,315257,3.932180881500244,3.3903685433969223e-08
78900,157801,157800,315601,3.9365410804748535,3.3404539095146743e-08
78986,157973,157972,315945,3.940778970718384,3.291228166707564e-08
79072,158145,158144,316289,3.945157051086426,3.2422744777370836e-08
79158,158317,158316,316633,3.950389862060547,3.194230946426575e-08
79244,158489,158488,316977,3.9546611309051514,3.147284275201123e-08
79330,158661,158660,317321,3.9589109420776367,3.100733827734708e-08
79416,158833,158832,317665,3.9631850719451904,3.054587993907727e-08
79502,159005,159004,318009,3.9675450325012207,3.009500412702808e-08
79588,159177,159176,318353,3.971860885620117,2.965240872874254e-08
79674,159349,159348,318697,3.976269006729126,2.9212224017473558e-08
79760,159521,159520,319041,3.9806461334228516,2.8778243455480032e-08
79846,159693,159692,319385,3.985038995742798,2.8354790341807537e-08
79932,159865,159864,319729,3.9895389080047607,2.793664238163798e-08
80018,160037,160036,320073,3.994025230407715,2.7520981012359246e-08
80103,160207,160206,320413,3.9984538555145264,2.71181890582594e-08
80189,160379,160378,320757,4.002921104431152,2.6719650233015506e-08
80275,160551,160550,321101,4.007401943206787,2.632416374405349e-08
80361,160723,160722,321445,4.011825084686279,2.593246372177552e-08
80447,160895,160894,321789,4.016248941421509,2.5549943965691178e-08
80533,161067,161066,322133,4.020685911178589,2.517405224901704e-08
80619,161239,161238,322477,4.025193929672241,2.480013909586006e-08
80705,161411,161410,322821,4.029519081115723,2.4431902569201193e-08
80791,161583,161582,323165,4.034151077270508,2.4072545218474064e-08
80877,161755,161754,323509,4.038272857666016,2.371731187670055e-08
80963,161927,161926,323853,4.042313098907471,2.3364361690079283e-08
81049,162099,162098,324197,4.046506881713867,2.3018688248539285e-08
81135,162271,162270,324541,4.050540924072266,2.2680386493930097e-08
81221,162443,162442,324885,4.054560899734497,2.23444044792868e-08
81307,162615,162614,325229,4.058653116226196,2.2012014581943905e-08
81393,162787,162786,325573,4.062763929367065,2.1687565356266404e-08
81479,162959,162958,325917,4.066911220550537,2.136833115017347e-08
81565,163131,163130,326261,4.071042060852051,2.1050759729531756e-08
81651,163303,163302,326605,4.075285911560059,2.073841192555546e-08
81736,163473,163472,326945,4.0794432163238525,2.0437014302397936e-08
81822,163645,163644,327289,4.083652973175049,2.0135221091503995e-08
81908,163817,163816,327633,4.087831974029541,1.9835544977185406e-08
81994,163989,163988,327977,4.092078924179077,1.954229222193997e-08
82080,164161,164160,328321,4.096301078796387,1.925504932524029e-08
82166,164333,164332,328665,4.100451946258545,1.8969613842568104e-08
82252,164505,164504,329009,4.104664087295532,1.868751873297093e-08
82338,164677,164676,329353,4.108897924423218,1.8412234338467856e-08
82424,164849,164848,329697,4.1131391525268555,1.8141072962120723e-08
82510,165021,165020,330041,4.1173670291900635,1.7871349590437002e-08
82596,165193,165192,330385,4.12148904800415,1.7606347301981765e-08
82682,165365,165364,330729,4.1257569789886475,1.7347540181050285e-08
82768,165537,165536,331073,4.1299779415130615,1.7091155550534226e-08
82854,165709,165708,331417,4.134202003479004,1.683678154434382e-08
82940,165881,165880,331761,4.138441801071167,1.6588074746911648e-08
83026,166053,166052,332105,4.142636060714722,1.6344195794721403e-08
83112,166225,166224,332449,4.146772861480713,1.6101723206476462e-08
83198,166397,166396,332793,4.15104603767395,1.5862389020196612e-08
83284,166569,166568,333137,4.155231237411499,1.5628867256799218e-08
83370,166741,166740,333481,4.159489870071411,1.5398542563404687e-08
83455,166911,166910,333821,4.163668870925903,1.5172146521846747e-08
83541,167083,167082,334165,4.1679160594940186,1.4947320956847124e-08
83627,167255,167254,334509,4.1721508502960205,1.472763381542647e-08
83713,167427,167426,334853,4.176382780075073,1.4509812139681856e-08
83799,167599,167598,335197,4.180613994598389,1.4293871833918747e-08
83885,167771,167770,335541,4.184873819351196,1.4082875865071445e-08
83971,167943,167942,335885,4.189079999923706,1.3875768235850092e-08
84057,168115,168114,336229,4.1933770179748535,1.3669790434085243e-08
84143,168287,168286,336573,4.197612047195435,1.3466700576045132e-08
84229,168459,168458,336917,4.201833963394165,1.326853984105131e-08
84315,168631,168630,337261,4.206060886383057,1.3072878239648012e-08
84401,168803,168802,337605,4.210274934768677,1.2878374746091215e-08
84487,168975,168974,337949,4.214541912078857,1.2687694771636195e-08
84573,169147,169146,338293,4.218761205673218,1.2501232807544324e-08
84659,169319,169318,338637,4.222969055175781,1.2316183589663706e-08
84745,169491,169490,338981,4.227115869522095,1.2132925158376114e-08
84831,169663,169662,339325,4.231366157531738,1.1953970188593235e-08
84917,169835,169834,339669,4.235591173171997,1.1778094711041407e-08
85003,170007,170006,340013,4.239814043045044,1.1603141480210885e-08
85088,170177,170176,340353,4.2439820766448975,1.1432840752970768e-08
85174,170349,170348,340697,4.248200178146362,1.1264675659140722e-08
85260,170521,170520,341041,4.252366065979004,1.1098453954634873e-08
85346,170693,170692,341385,4.256622076034546,1.0933294830561487e-08
85432,170865,170864,341729,4.260814905166626,1.0771531035995722e-08
85518,171037,171036,342073,4.265049934387207,1.0613224974630694e-08
85604,171209,171208,342417,4.2692461013793945,1.0456011383738711e-08
85690,171381,171380,342761,4.273447036743164,1.0300469471273685e-08
85776,171553,171552,343105,4.277652978897095,1.0148638901119764e-08
85862,171725,171724,343449,4.281844854354858,9.999258193884267e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.295608520507812e-05,4.387072431292609
92,185,184,369,0.003635883331298828,0.265498193466344
184,369,368,737,0.006905794143676758,0.12132799283907403
276,553,552,1105,0.009988069534301758,0.08098588184474649
368,737,736,1473,0.013046026229858398,0.06295546836576064
460,921,920,1841,0.017035961151123047,0.0534342328893946
552,1105,1104,2209,0.020149946212768555,0.04755332813973005
644,1289,1288,2577,0.023462772369384766,0.04336819414898068
736,1473,1472,2945,0.026858806610107422,0.040012134760418344
828,1657,1656,3313,0.030059814453125,0.0372103624585227
920,1841,1840,3681,0.034893035888671875,0.03477038957412199
1012,2025,2024,4049,0.03927969932556152,0.03265139713580958
1104,2209,2208,4417,0.042775869369506836,0.03078428506122928
1196,2393,2392,4785,0.04594087600708008,0.029152698139190723
1288,2577,2576,5153,0.049260854721069336,0.027717571667471172
1380,2761,2760,5521,0.05245089530944824,0.026448938785904454
1472,2945,2944,5889,0.05548095703125,0.0253367111154004
1564,3129,3128,6257,0.0586397647857666,0.024347764291400217
1656,3313,3312,6625,0.06255578994750977,0.023480498091803637
1748,3497,3496,6993,0.06614971160888672,0.022695332155553104
1840,3681,3680,7361,0.0693807601928711,0.022005658133093478
1932,3865,3864,7729,0.07249569892883301,0.021375656372689192
2024,4049,4048,8097,0.07589077949523926,0.02081458748885702
2116,4233,4232,8465,0.08002400398254395,0.020293465291431705
2208,4417,4416,8833,0.08359193801879883,0.01982630351650638
2300,4601,4600,9201,0.08737397193908691,0.019389202351310926
2392,4785,4784,9569,0.09133481979370117,0.018986137742038216
2484,4969,4968,9937,0.0944218635559082,0.0186057407100563
2576,5153,5152,10305,0.09764599800109863,0.018253000036295677
2668,5337,5336,10673,0.10088682174682617,0.017918259599596986
2760,5521,5520,11041,0.10417890548706055,0.017597688703256596
2852,5705,5704,11409,0.10752987861633301,0.017293079687255273
2944,5889,5888,11777,0.11089873313903809,0.01700159297397879
3036,6073,6072,12145,0.11423301696777344,0.01672213100002464
3128,6257,6256,12513,0.11756110191345215,0.016447968805384967
3220,6441,6440,12881,0.12093377113342285,0.01618618498607426
3312,6625,6624,13249,0.12436890602111816,0.015930928736841075
3404,6809,6808,13617,0.1278519630432129,0.01568326839769925
3496,6993,6992,13985,0.13132476806640625,0.015438498485822448
3588,7177,7176,14353,0.13480377197265625,0.015203162815280596
3680,7361,7360,14721,0.13841581344604492,0.014972054702171935
3772,7545,7544,15089,0.14188790321350098,0.014745071898047963
3864,7729,7728,15457,0.14533591270446777,0.014521320003355147
3956,7913,7912,15825,0.14876985549926758,0.014304479567288005
4048,8097,8096,16193,0.1521897315979004,0.014091140079077654
4140,8281,8280,16561,0.15564370155334473,0.013879793206978706
4232,8465,8464,16929,0.1589798927307129,0.01367256573915936
4324,8649,8648,17297,0.1623399257659912,0.013470390757701262
4416,8833,8832,17665,0.1657118797302246,0.01327114009934527
4508,9017,9016,18033,0.16915297508239746,0.013073122123599274
4601,9203,9202,18405,0.1725916862487793,0.012877682915089568
4693,9387,9386,18773,0.17622590065002441,0.012688206839978662
4785,9571,9570,19141,0.1796107292175293,0.012500884529289989
4877,9755,9754,19509,0.18302583694458008,0.012315019266588227
4969,9939,9938,19877,0.18642282485961914,0.012133849222633586
5061,10123,10122,20245,0.18982887268066406,0.011955752953232979
5153,10307,10306,20613,0.19339489936828613,0.011779091563424092
5245,10491,10490,20981,0.19673681259155273,0.011604522757011774
5337,10675,10674,21349,0.1998908519744873,0.011434309629244554
5429,10859,10858,21717,0.20307087898254395,0.011266569106741545
5521,11043,11042,22085,0.20621371269226074,0.011099845691387835
5613,11227,11226,22453,0.2092909812927246,0.010935858909671579
5705,11411,11410,22821,0.21239089965820312,0.010775721807310424
5797,11595,11594,23189,0.2154688835144043,0.010617477516402206
5889,11779,11778,23557,0.22146081924438477,0.010460213504775911
5981,11963,11962,23925,0.2245328426361084,0.010306135028158967
6073,12147,12146,24293,0.227586030960083,0.010155337117681955
6165,12331,12330,24661,0.23073506355285645,0.010005895574154346
6257,12515,12514,25029,0.23378872871398926,0.009857696973449577
6349,12699,12698,25397,0.23683786392211914,0.009712878665989464
6441,12883,12882,25765,0.23990583419799805,0.00957074902621629
6533,13067,13066,26133,0.24295377731323242,0.009429574404370878
6625,13251,13250,26501,0.24596691131591797,0.00929005618981176
6717,13435,13434,26869,0.24932193756103516,0.009153875525080868
6809,13619,13618,27237,0.25235986709594727,0.009019791735681399
6901,13803,13802,27605,0.2553868293762207,0.008886468925474024
6993,13987,13986,27973,0.2585878372192383,0.008755226716821038
7085,14171,14170,28341,0.2618579864501953,0.008627086769837568
7177,14355,14354,28709,0.2649190425872803,0.008500489270144644
7269,14539,14538,29077,0.26796388626098633,0.00837467713830362
7361,14723,14722,29445,0.2710988521575928,0.008251280956738483
7453,14907,14906,29813,0.27414798736572266,0.008130610773395611
7545,15091,15090,30181,0.277385950088501,0.008011019211173021
7637,15275,15274,30549,0.2804548740386963,0.007892411026808802
7729,15459,15458,30917,0.2835378646850586,0.007776408916869355
7821,15643,15642,31285,0.28659892082214355,0.007662668823448273
7913,15827,15826,31653,0.28995680809020996,0.007549684538308152
8005,16011,16010,32021,0.2930889129638672,0.007437980592296946
8097,16195,16194,32389,0.2961258888244629,0.007328906930188439
8189,16379,16378,32757,0.29921388626098633,0.007221599435818479
8281,16563,16562,33125,0.3022639751434326,0.007114893454830598
8373,16747,16746,33493,0.3052957057952881,0.007009784309752824
8465,16931,16930,33861,0.3086838722229004,0.006907170505784996
8557,17115,17114,34229,0.31262993812561035,0.006805852309551604
8649,17299,17298,34597,0.3160109519958496,0.006705145554521056
8741,17483,17482,34965,0.3197460174560547,0.006606303590934758
8833,17667,17666,35333,0.32364583015441895,0.00650969024630128
8925,17851,17850,35701,0.32773876190185547,0.0064139795675601475
9017,18035,18034,36069,0.3319737911224365,0.006319021842213154
9109,18219,18218,36437,0.3357207775115967,0.006226099648483291
9201,18403,18402,36805,0.33985304832458496,0.006135049484536082
9293,18587,18586,37173,0.3430447578430176,0.006044625538653565
9385,18771,18770,37541,0.34622883796691895,0.0059551771313401
9477,18955,18954,37909,0.3494267463684082,0.005867811575235608
9569,19139,19138,38277,0.35242581367492676,0.005781921752533535
9661,19323,19322,38645,0.3554098606109619,0.005696516761600805
9753,19507,19506,39013,0.3586287498474121,0.005612334439899687
9845,19691,19690,39381,0.3623940944671631,0.005530155018102414
9937,19875,19874,39749,0.3659708499908447,0.005449066741729208
10029,20059,20058,40117,0.3704869747161865,0.005368453044231705
10121,20243,20242,40485,0.37455296516418457,0.00528928126884425
10213,20427,20426,40853,0.37767696380615234,0.005211921077343562
10305,20611,20610,41221,0.3814530372619629,0.005135324544175749
10397,20795,20794,41589,0.38475894927978516,0.005059299806089426
10489,20979,20978,41957,0.3879818916320801,0.004984867427219348
10581,21163,21162,42325,0.39171886444091797,0.004911974961012428
10673,21347,21346,42693,0.39523768424987793,0.00483960876664503
10765,21531,21530,43061,0.3985006809234619,0.004767981818709862
10857,21715,21714,43429,0.40193772315979004,0.004698003895727218
10949,21899,21898,43797,0.4049100875854492,0.0046292538531218915
11041,22083,22082,44165,0.40804386138916016,0.004560899297492278
11133,22267,22266,44533,0.41120409965515137,0.004493478459971572
11225,22451,22450,44901,0.4143657684326172,0.0044276622138280305
11317,22635,22634,45269,0.41753172874450684,0.004362763648054383
11409,22819,22818,45637,0.42069077491760254,0.004298235352024753
11501,23003,23002,46005,0.423969030380249,0.00423482047838585
11593,23187,23186,46373,0.4274108409881592,0.004172873922160172
11685,23371,23370,46741,0.43082284927368164,0.00411157455832226
11777,23555,23554,47109,0.43450474739074707,0.004050709233969751
11869,23739,23738,47477,0.4378170967102051,0.003991088064324712
11961,23923,23922,47845,0.44106292724609375,0.003932729638024072
12053,24107,24106,48213,0.44449400901794434,0.0038748159003099284
12145,24291,24290,48581,0.44770193099975586,0.0038174611177217363
12237,24475,24474,48949,0.45090675354003906,0.003761409868641858
12329,24659,24658,49317,0.4541287422180176,0.003706377429123302
12421,24843,24842,49685,0.4573369026184082,0.0036516705003094996
12513,25027,25026,50053,0.4606049060821533,0.003597675030105616
12605,25211,25210,50421,0.46386289596557617,0.003544962541065537
12697,25395,25394,50789,0.4671778678894043,0.0034930203102200123
12789,25579,25578,51157,0.47052574157714844,0.0034413691704112204
12881,25763,25762,51525,0.47386693954467773,0.0033905760558328277
12973,25947,25946,51893,0.4771907329559326,0.003340970364213177
13065,26131,26130,52261,0.4804999828338623,0.003291912884447345
13157,26315,26314,52629,0.48380279541015625,0.00324318564432765
13249,26499,26498,52997,0.48708295822143555,0.0031954286291914686
13341,26683,26682,53365,0.4903128147125244,0.003148704613357249
13433,26867,26866,53733,0.4936649799346924,0.00310235732335986
13525,27051,27050,54101,0.4970998764038086,0.0030564322704418776
13617,27235,27234,54469,0.5002810955047607,0.00301153564648463
13709,27419,27418,54837,0.5034918785095215,0.00296748237017715
13802,27605,27604,55209,0.5067148208618164,0.0029232247688510565
13894,27789,27788,55577,0.5099108219146729,0.0028799920729198313
13986,27973,27972,55945,0.5130999088287354,0.002837784026206393
14078,28157,28156,56313,0.5163047313690186,0.002796213973889506
14170,28341,28340,56681,0.5194900035858154,0.0027548750466811545
14262,28525,28524,57049,0.5226709842681885,0.002714202596238064
14354,28709,28708,57417,0.5258688926696777,0.0026744865444963558
14446,28893,28892,57785,0.5290298461914062,0.0026352279723371595
14538,29077,29076,58153,0.5322878360748291,0.0025962244417923573
14630,29261,29260,58521,0.5354406833648682,0.0025579813143309675
14722,29445,29444,58889,0.5385949611663818,0.002520577389079624
14814,29629,29628,59257,0.5417459011077881,0.002483488401584202
14906,29813,29812,59625,0.5448949337005615,0.00244672290927499
14998,29997,29996,59993,0.548027753829956,0.0024107705414662364
15090,30181,30180,60361,0.5511698722839355,0.0023755093897748145
15182,30365,30364,60729,0.5545547008514404,0.0023404709603444887
15274,30549,30548,61097,0.5576808452606201,0.002305848710759603
15366,30733,30732,61465,0.5608177185058594,0.0022720428407652267
15458,30917,30916,61833,0.5639488697052002,0.0022387704994310115
15550,31101,31100,62201,0.5670619010925293,0.002205682619806687
15642,31285,31284,62569,0.5701696872711182,0.002173106409813063
15734,31469,31468,62937,0.5732789039611816,0.0021413008140338066
15826,31653,31652,63305,0.5763928890228271,0.0021098818350858825
15918,31837,31836,63673,0.5795199871063232,0.0020786583248123595
16010,32021,32020,64041,0.5826709270477295,0.0020480255909237784
16102,32205,32204,64409,0.5857930183410645,0.002018076781699672
16194,32389,32388,64777,0.5889127254486084,0.0019883952653954903
16286,32573,32572,65145,0.5920729637145996,0.0019589581143590697
16378,32757,32756,65513,0.5951838493347168,0.0019301601572216638
16470,32941,32940,65881,0.5983107089996338,0.0019019321590398102
16562,33125,33124,66249,0.6014308929443359,0.0018738907105203847
16654,33309,33308,66617,0.6045360565185547,0.0018461648039101739
16746,33493,33492,66985,0.6076228618621826,0.001819088005142344
16838,33677,33676,67353,0.610703706741333,0.0017924564172433744
16930,33861,33860,67721,0.6137478351593018,0.0017659733598326956
17022,34045,34044,68089,0.6167778968811035,0.0017398822854565077
17114,34229,34228,68457,0.6201398372650146,0.0017144108535773336
17206,34413,34412,68825,0.6231777667999268,0.001689265607238832
17298,34597,34596,69193,0.6262528896331787,0.0016642710156157894
17390,34781,34780,69561,0.6293270587921143,0.001639734414830561
17482,34965,34964,69929,0.6324248313903809,0.0016157540197184303
17574,35149,35148,70297,0.6358540058135986,0.0015920005061322458
17666,35333,35332,70665,0.6391270160675049,0.0015684317413351921
17758,35517,35516,71033,0.6423628330230713,0.0015453643826312292
17850,35701,35700,71401,0.6455600261688232,0.001522765977641887
17942,35885,35884,71769,0.6487798690795898,0.0015003245088605383
18034,36069,36068,72137,0.6519737243652344,0.0014781219391614172
18126,36253,36252,72505,0.6552140712738037,0.0014564344150894497
18218,36437,36436,72873,0.6583957672119141,0.0014351175988114616
18310,36621,36620,73241,0.6615910530090332,0.001413921423991352
18402,36805,36804,73609,0.6647248268127441,0.0013930249139625951
18494,36989,36988,73977,0.6678519248962402,0.00137262562945294
18586,37173,37172,74345,0.671180009841919,0.001352501044359688
18678,37357,37356,74713,0.6743838787078857,0.001332493340138499
18770,37541,37540,75081,0.6774709224700928,0.0013128399116096488
18862,37725,37724,75449,0.6805398464202881,0.001293637875208591
18954,37909,37908,75817,0.683708906173706,0.0012746283456325092
19046,38093,38092,76185,0.6867880821228027,0.0012557587104176009
19138,38277,38276,76553,0.6898539066314697,0.001237281558909184
19230,38461,38460,76921,0.6933338642120361,0.0012191894235165886
19322,38645,38644,77289,0.6963949203491211,0.0012012297624199484
19414,38829,38828,77657,0.6994607448577881,0.0011834507626099651
19506,39013,39012,78025,0.7025477886199951,0.001166079589095695
19598,39197,39196,78393,0.7056057453155518,0.0011490164151580393
19690,39381,39380,78761,0.7086760997772217,0.0011320520411398768
19782,39565,39564,79129,0.7119648456573486,0.0011153162905194155
19874,39749,39748,79497,0.7154159545898438,0.0010989787153577704
19966,39933,39932,79865,0.7187540531158447,0.0010828720329040848
20058,40117,40116,80233,0.7228279113769531,0.001066856705379939
20150,40301,40300,80601,0.726942777633667,0.0010511148266447404
20242,40485,40484,80969,0.7307219505310059,0.0010357385162341611
20334,40669,40668,81337,0.734126091003418,0.001020525418182849
20426,40853,40852,81705,0.73726487159729,0.0010054184997175743
20518,41037,41036,82073,0.7403688430786133,0.0009906181465103403
20610,41221,41220,82441,0.7434568405151367,0.0009761332181771718
20702,41405,41404,82809,0.7467210292816162,0.0009617603962747527
20794,41589,41588,83177,0.7497859001159668,0.0009475240788049958
20886,41773,41772,83545,0.7528460025787354,0.0009336100177832578
20978,41957,41956,83913,0.7559018135070801,0.0009199512966263509
21070,42141,42140,84281,0.7590289115905762,0.0009063741034302827
21162,42325,42324,84649,0.7621009349822998,0.0008929709936284395
21254,42509,42508,85017,0.7651770114898682,0.0008798860869909449
21346,42693,42692,85385,0.7682909965515137,0.0008669948604328904
21438,42877,42876,85753,0.7713756561279297,0.0008541756206451709
21530,43061,43060,86121,0.7745959758758545,0.0008415669829172735
21622,43245,43244,86489,0.7780818939208984,0.0008292537945099272
21714,43429,43428,86857,0.7815968990325928,0.0008170788279694626
21806,43613,43612,87225,0.7846786975860596,0.0008049847126842493
21898,43797,43796,87593,0.7877590656280518,0.0007931295369762583
21990,43981,43980,87961,0.790848970413208,0.0007815322228549886
22082,44165,44164,88329,0.7940027713775635,0.0007700299401709775
22174,44349,44348,88697,0.7970578670501709,0.000758630750222288
22266,44533,44532,89065,0.8001337051391602,0.0007474856695962054
22358,44717,44716,89433,0.803210973739624,0.0007365518101358489
22450,44901,44900,89801,0.806290864944458,0.0007256856812763278
22542,45085,45084,90169,0.8094608783721924,0.0007149518624211961
22634,45269,45268,90537,0.8126089572906494,0.0007044718150145092
22726,45453,45452,90905,0.8157439231872559,0.0006941538943671782
22818,45637,45636,91273,0.8188779354095459,0.000683893189650795
22910,45821,45820,91641,0.8220169544219971,0.000673794332587639
23003,46007,46006,92013,0.8251907825469971,0.0006638275156875606
23095,46191,46190,92381,0.8283498287200928,0.0006540843958168244
23187,46375,46374,92749,0.8315038681030273,0.0006444037721387139
23279,46559,46558,93117,0.8346889019012451,0.0006349103317802198
23371,46743,46742,93485,0.8378348350524902,0.0006256262788221503
23463,46927,46926,93853,0.8410019874572754,0.0006164216886807709
23555,47111,47110,94221,0.8443520069122314,0.0006072960816901616
23647,47295,47294,94589,0.8474926948547363,0.0005983712988320675
23739,47479,47478,94957,0.8506288528442383,0.0005896195521110122
23831,47663,47662,95325,0.8537647724151611,0.000580923766582953
23923,47847,47846,95693,0.8568968772888184,0.0005723297201342388
24015,48031,48030,96061,0.8600308895111084,0.0005639379506725266
24107,48215,48214,96429,0.8631877899169922,0.0005556801922258856
24199,48399,48398,96797,0.8663218021392822,0.0005474682509700201
24291,48583,48582,97165,0.8694577217102051,0.000539381765412518
24383,48767,48766,97533,0.8728597164154053,0.000531486824106155
24475,48951,48950,97901,0.8759899139404297,0.0005236892902346711
24567,49135,49134,98269,0.879119873046875,0.0005159397254236186
24659,49319,49318,98637,0.8823227882385254,0.0005083354993011119
24751,49503,49502,99005,0.8854577541351318,0.000500901815490136
24843,49687,49686,99373,0.8885948657989502,0.0004935355795258883
24935,49871,49870,99741,0.891746997833252,0.00048622901670188615
25027,50055,50054,100109,0.894881010055542,0.00047908022736870926
25119,50239,50238,100477,0.8980269432067871,0.0004720740311030119
25211,50423,50422,100845,0.9011528491973877,0.00046511477020851516
25303,50607,50606,101213,0.9042809009552002,0.0004582326134909939
25395,50791,50790,101581,0.9073758125305176,0.0004515111950246925
25487,50975,50974,101949,0.9106910228729248,0.00044490153562262523
25579,51159,51158,102317,0.9137389659881592,0.0004383288604413829
25671,51343,51342,102685,0.916801929473877,0.0004318522378578795
25763,51527,51526,103053,0.919853925704956,0.0004255295446283941
25855,51711,51710,103421,0.9229109287261963,0.00041928899218877106
25947,51895,51894,103789,0.925976037979126,0.00041308547636242454
26039,52079,52078,104157,0.9290728569030762,0.00040699456290012906
26131,52263,52262,104525,0.9321348667144775,0.00040104226183364027
26223,52447,52446,104893,0.9351837635040283,0.00039514720792077434
26315,52631,52630,105261,0.9382328987121582,0.0003892972853707478
26407,52815,52814,105629,0.941321849822998,0.0003835710517549981
26499,52999,52998,105997,0.944591760635376,0.00037796206989134523
26591,53183,53182,106365,0.9477019309997559,0.00037239261455918125
26683,53367,53366,106733,0.9508059024810791,0.0003668815144255489
26775,53551,53550,107101,0.9539029598236084,0.00036149788041558463
26867,53735,53734,107469,0.956995964050293,0.00035620724609618644
26959,53919,53918,107837,0.9602007865905762,0.00035094672325064637
27051,54103,54102,108205,0.9633567333221436,0.0003457595884217484
27143,54287,54286,108573,0.966378927230835,0.0003406959010429492
27235,54471,54470,108941,0.9693927764892578,0.00033570135203015144
27327,54655,54654,109309,0.9724118709564209,0.0003307355947374074
27419,54839,54838,109677,0.97568678855896,0.00032585688648647046
27511,55023,55022,110045,0.9786880016326904,0.0003210906037826207
27603,55207,55206,110413,0.98183274269104,0.00031637288585020226
27695,55391,55390,110781,0.984893798828125,0.00031168936181863
27787,55575,55574,111149,0.9878969192504883,0.0003071025988933133
27879,55759,55758,111517,0.9909067153930664,0.000302612042510919
27971,55943,55942,111885,0.9941260814666748,0.00029815487818055114
28063,56127,56126,112253,0.9982666969299316,0.0002937418313315232
28155,56311,56310,112621,1.001399040222168,0.00028942965630062833
28247,56495,56494,112989,1.0048577785491943,0.00028519470163822154
28339,56679,56678,113357,1.0083980560302734,0.00028098446157715976
28431,56863,56862,113725,1.011920690536499,0.00027683018008864066
28523,57047,57046,114093,1.0149848461151123,0.00027277469741664645
28615,57231,57230,114461,1.018054723739624,0.0002687772948166795
28707,57415,57414,114829,1.0211758613586426,0.00026480244633387884
28799,57599,57598,115197,1.0242419242858887,0.0002608947454917893
28891,57783,57782,115565,1.0275566577911377,0.0002570780412482184
28983,57967,57966,115933,1.0316798686981201,0.00025330249982605387
29075,58151,58150,116301,1.034728765487671,0.0002495529328162509
29167,58335,58334,116669,1.0377569198608398,0.00024587889910674944
29259,58519,58518,117037,1.0410187244415283,0.00024228363517333687
29351,58703,58702,117405,1.044050931930542,0.00023871664504777088
29443,58887,58886,117773,1.0470869541168213,0.00023518298353735343
29535,59071,59070,118141,1.050157070159912,0.00023172898208133612
29627,59255,59254,118509,1.053210735321045,0.00022833895885264214
29719,59439,59438,118877,1.056609869003296,0.00022496937036989891
29811,59623,59622,119245,1.059809923171997,0.0002216423683720039
29903,59807,59806,119613,1.0631158351898193,0.0002183942760326975
29995,59991,59990,119981,1.0663390159606934,0.0002151948747093324
30087,60175,60174,120349,1.0697758197784424,0.00021201328840393769
30179,60359,60358,120717,1.0729749202728271,0.00020888338543868234
30271,60543,60542,121085,1.0761499404907227,0.00020582698227116528
30363,60727,60726,121453,1.079225778579712,0.00020280542651222096
30455,60911,60910,121821,1.0824098587036133,0.00019980367058495432
30547,61095,61094,122189,1.086050033569336,0.00019686075002575942
30639,61279,61278,122557,1.089277744293213,0.00019398218559046177
30731,61463,61462,122925,1.0923848152160645,0.00019112759684743527
30823,61647,61646,123293,1.0957558155059814,0.00018829817775929206
30915,61831,61830,123661,1.099118947982788,0.00018553153597171862
31007,62015,62014,124029,1.103700876235962,0.0001828177853676784
31099,62199,62198,124397,1.1068549156188965,0.0001801210407460635
31191,62383,62382,124765,1.1100668907165527,0.00017745664739668646
31283,62567,62566,125133,1.1142728328704834,0.00017485514910571561
31375,62751,62750,125501,1.117645025253296,0.00017229438503124346
31467,62935,62934,125869,1.1209919452667236,0.00016974781579166378
31559,63119,63118,126237,1.1244587898254395,0.00016724094100036357
31651,63303,63302,126605,1.1279900074005127,0.0001647933111090359
31743,63487,63486,126973,1.1327037811279297,0.000162375139604619
31835,63671,63670,127341,1.1366667747497559,0.00015997212859610518
31927,63855,63854,127709,1.1406466960906982,0.0001576148470484503
32019,64039,64038,128077,1.1447679996490479,0.00015531003427065153
32111,64223,64222,128445,1.148852825164795,0.000153025568670073
32204,64409,64408,128817,1.1528089046478271,0.0001507357196500002
32296,64593,64592,129185,1.156742811203003,0.00014852023872539947
32388,64777,64776,129553,1.160951852798462,0.00014634806719079647
32480,64961,64960,129921,1.164931058883667,0.00014418996234632852
32572,65145,65144,130289,1.168968915939331,0.0001420567253070615
32664,65329,65328,130657,1.172881841659546,0.0001399735989880551
32756,65513,65512,131025,1.176736831665039,0.00013792412750918937
32848,65697,65696,131393,1.1806750297546387,0.00013588604433923462
32940,65881,65880,131761,1.185161828994751,0.00013387871627611108
33032,66065,66064,132129,1.1892828941345215,0.0001319189907571077
33124,66249,66248,132497,1.1932127475738525,0.00012998380352270502
33216,66433,66432,132865,1.1970558166503906,0.00012806039365602517
33308,66617,66616,133233,1.2009477615356445,0.00012617273282482548
33400,66801,66800,133601,1.2047626972198486,0.00012432759097872806
33492,66985,66984,133969,1.2088978290557861,0.00012249946869993122
33584,67169,67168,134337,1.2128639221191406,0.00012068591954823159
33676,67353,67352,134705,1.2169508934020996,0.00011891130740768575
33768,67537,67536,135073,1.2209358215332031,0.00011717236318006302
33860,67721,67720,135441,1.2248330116271973,0.00011544523164664802
33952,67905,67904,135809,1.2286341190338135,0.00011373693881526312
34044,68089,68088,136177,1.2321498394012451,0.00011206844299597608
34136,68273,68272,136545,1.235454797744751,0.00011042799661757901
34228,68457,68456,136913,1.2385609149932861,0.00010879676566996014
34320,68641,68640,137281,1.2416789531707764,0.00010718906780628268
34412,68825,68824,137649,1.2447757720947266,0.00010561960226923476
34504,69009,69008,138017,1.2478649616241455,0.00010407081855074509
34596,69193,69192,138385,1.2509469985961914,0.00010253114478593481
34688,69377,69376,138753,1.2542707920074463,0.00010101915080247275
34780,69561,69560,139121,1.2573628425598145,9.954169475425544e-05
34872,69745,69744,139489,1.2604737281799316,9.807868283564972e-05
34964,69929,69928,139857,1.2636327743530273,9.662669737533456e-05
35056,70113,70112,140225,1.2667288780212402,9.520521883726337e-05
35148,70297,70296,140593,1.2698547840118408,9.381305152733659e-05
35240,70481,70480,140961,1.272958755493164,9.243084201482174e-05
35332,70665,70664,141329,1.2761058807373047,9.106288551765075e-05
35424,70849,70848,141697,1.2793610095977783,8.97264697848083e-05
35516,71033,71032,142065,1.2829928398132324,8.841338087642378e-05
35608,71217,71216,142433,1.286167860031128,8.710781248189942e-05
35700,71401,71400,142801,1.2893388271331787,8.582021395160321e-05
35792,71585,71584,143169,1.2925159931182861,8.45632590282526e-05
35884,71769,71768,143537,1.2956998348236084,8.332370263331216e-05
35976,71953,71952,143905,1.2988557815551758,8.209124294470154e-05
36068,72137,72136,144273,1.3020069599151611,8.088016834109727e-05
36160,72321,72320,144641,1.3051578998565674,7.969709026092745e-05
36252,72505,72504,145009,1.3083267211914062,7.852626302123973e-05
36344,72689,72688,145377,1.3115320205688477,7.736379540152425e-05
36436,72873,72872,145745,1.3147029876708984,7.622517873721227e-05
36528,73057,73056,146113,1.3178627490997314,7.511059773932183e-05
36620,73241,73240,146481,1.321030855178833,7.40044352094628e-05
36712,73425,73424,146849,1.3242318630218506,7.290904551952945e-05
36804,73609,73608,147217,1.327401876449585,7.183860134388646e-05
36896,73793,73792,147585,1.3305718898773193,7.078751416145565e-05
36988,73977,73976,147953,1.3337268829345703,6.974261291654458e-05
37080,74161,74160,148321,1.336869716644287,6.871140616167696e-05
37172,74345,74344,148689,1.3400428295135498,6.770471023668523e-05
37264,74529,74528,149057,1.3432047367095947,6.67126217279365e-05
37356,74713,74712,149425,1.3463380336761475,6.57261051695689e-05
37448,74897,74896,149793,1.3495237827301025,6.475607441240769e-05
37540,75081,75080,150161,1.3526699542999268,6.3808690626651e-05
37632,75265,75264,150529,1.3558619022369385,6.2871687281339e-05
37724,75449,75448,150897,1.3590219020843506,6.19410397507409e-05
37816,75633,75632,151265,1.3621890544891357,6.102899934618879e-05
37908,75817,75816,151633,1.3653669357299805,6.01366264621373e-05
38000,76001,76000,152001,1.3685307502746582,5.9251385215877865e-05
38092,76185,76184,152369,1.371727705001831,5.837428118606883e-05
38184,76369,76368,152737,1.375020980834961,5.751686541022279e-05
38276,76553,76552,153105,1.3782026767730713,5.667547729530797e-05
38368,76737,76736,153473,1.3813939094543457,5.583921373994054e-05
38460,76921,76920,153841,1.3847479820251465,5.5013366726423775e-05
38552,77105,77104,154209,1.388199806213379,5.4207084934912894e-05
38644,77289,77288,154577,1.39158296585083,5.3413041978584466e-05
38736,77473,77472,154945,1.3948557376861572,5.262341088468392e-05
38828,77657,77656,155313,1.3982629776000977,5.1846461084870695e-05
38920,77841,77840,155681,1.401702880859375,5.1087793041045336e-05
39012,78025,78024,156049,1.4054667949676514,5.033790943860535e-05
39104,78209,78208,156417,1.4087069034576416,4.9592876379506964e-05
39196,78393,78392,156785,1.4119117259979248,4.886232816311029e-05
39288,78577,78576,157153,1.4153509140014648,4.814783899776332e-05
39380,78761,78760,157521,1.4186148643493652,4.743939909359214e-05
39472,78945,78944,157889,1.4221539497375488,4.673710432692097e-05
39564,79129,79128,158257,1.4253718852996826,4.6050315993169464e-05
39656,79313,79312,158625,1.4290800094604492,4.537676966340512e-05
39748,79497,79496,158993,1.4325637817382812,4.4707495123863185e-05
39840,79681,79680,159361,1.43611478805542,4.404612978512394e-05
39932,79865,79864,159729,1.439760684967041,4.340034988785914e-05
40024,80049,80048,160097,1.4430017471313477,4.276480268567078e-05
40116,80233,80232,160465,1.4461658000946045,4.2132779607193874e-05
40208,80417,80416,160833,1.449558973312378,4.1510490252938005e-05
40300,80601,80600,161201,1.452678918838501,4.0902928440187974e-05
40392,80785,80784,161569,1.4557888507843018,4.030278928177927e-05
40484,80969,80968,161937,1.4590749740600586,3.970636946595362e-05
40576,81153,81152,162305,1.462212085723877,3.912120100036371e-05
40668,81337,81336,162673,1.4653937816619873,3.8549117494467944e-05
40760,81521,81520,163041,1.4688518047332764,3.798216832895614e-05
40852,81705,81704,163409,1.4721028804779053,3.741986134984287e-05
40944,81889,81888,163777,1.4752418994903564,3.686974150509078e-05
41036,82073,82072,164145,1.478468656539917,3.6330538365849425e-05
41128,82257,82256,164513,1.48164701461792,3.579491490897561e-05
41220,82441,82440,164881,1.48478364944458,3.5265287205416156e-05
41312,82625,82624,165249,1.487973690032959,3.474804915706128e-05
41405,82811,82810,165621,1.491170883178711,3.423383577801234e-05
41497,82995,82994,165989,1.4943747520446777,3.3728014419914725e-05
41589,83179,83178,166357,1.4976539611816406,3.3229731318770864e-05
41681,83363,83362,166725,1.500878095626831,3.274327645723261e-05
41773,83547,83546,167093,1.5040650367736816,3.226300226113365e-05
41865,83731,83730,167461,1.5074667930603027,3.17856210681262e-05
41957,83915,83914,167829,1.510732889175415,3.131703155466878e-05
42049,84099,84098,168197,1.5141229629516602,3.085904094920132e-05
42141,84283,84282,168565,1.5173537731170654,3.0405344941111286e-05
42233,84467,84466,168933,1.5207369327545166,2.995520827208897e-05
42325,84651,84650,169301,1.5240318775177002,2.9514679264135573e-05
42417,84835,84834,169669,1.527297019958496,2.9083070611518622e-05
42509,85019,85018,170037,1.5306627750396729,2.865443588074632e-05
42601,85203,85202,170405,1.5339078903198242,2.8230403498108074e-05
42693,85387,85386,170773,1.5376529693603516,2.7816222792332867e-05
42785,85571,85570,171141,1.540855884552002,2.740908075221723e-05
42877,85755,85754,171509,1.5440268516540527,2.7004236491061818e-05
42969,85939,85938,171877,1.5472629070281982,2.6605156936054884e-05
43061,86123,86122,172245,1.5507798194885254,2.621557181336792e-05
43153,86307,86306,172613,1.553924798965454,2.583119327747372e-05
43245,86491,86490,172981,1.5570869445800781,2.5449056796196093e-05
43337,86675,86674,173349,1.56026291847229,2.5073723340612524e-05
43429,86859,86858,173717,1.5634608268737793,2.4706994244047708e-05
43521,87043,87042,174085,1.5671920776367188,2.434390939003425e-05
43613,87227,87226,174453,1.5703299045562744,2.398351893846167e-05
43705,87411,87410,174821,1.5736486911773682,2.3630651502917647e-05
43797,87595,87594,175189,1.5769257545471191,2.328511019150104e-05
43889,87779,87778,175557,1.581188678741455,2.2942078093906787e-05
43981,87963,87962,175925,1.5851819515228271,2.260252695875759e-05
44073,88147,88146,176293,1.5892317295074463,2.2270779115250287e-05
44165,88331,88330,176661,1.5932908058166504,2.1944881248121035e-05
44257,88515,88514,177029,1.597242832183838,2.1620862855580365e-05
44349,88699,88698,177397,1.602186918258667,2.1301243883609585e-05
44441,88883,88882,177765,1.6062090396881104,2.098923039231683e-05
44533,89067,89066,178133,1.6103878021240234,2.0681594511522806e-05
44625,89251,89250,178501,1.614853858947754,2.0375708953653403e-05
44717,89435,89434,178869,1.6188938617706299,2.0075076092585686e-05
44809,89619,89618,179237,1.6231749057769775,1.9781413850960533e-05
44901,89803,89802,179605,1.6272900104522705,1.949084173697625e-05
44993,89987,89986,179973,1.6314187049865723,1.9202313818962258e-05
45085,90171,90170,180341,1.6354148387908936,1.8919663992451438e-05
45177,90355,90354,180709,1.6394329071044922,1.864301807003898e-05
45269,90539,90538,181077,1.6434028148651123,1.8368494870961034e-05
45361,90723,90722,181445,1.6473829746246338,1.8096602105638193e-05
45453,90907,90906,181813,1.6514108180999756,1.7830877320151142e-05
45545,91091,91090,182181,1.655332088470459,1.757000394751281e-05
45637,91275,91274,182549,1.659390926361084,1.731067976310692e-05
45729,91459,91458,182917,1.6632299423217773,1.7054706462987048e-05
45821,91643,91642,183285,1.6669859886169434,1.6804813018788805e-05
45913,91827,91826,183653,1.6702418327331543,1.6558592806737146e-05
46005,92011,92010,184021,1.6735877990722656,1.631375006165987e-05
46097,92195,92194,184389,1.6768648624420166,1.607295413774309e-05
46189,92379,92378,184757,1.6799979209899902,1.5837793598333784e-05
46281,92563,92562,185125,1.6831169128417969,1.5605250532703724e-05
46373,92747,92746,185493,1.6862719058990479,1.5374263170426554e-05
46465,92931,92930,185861,1.6895079612731934,1.5147858760384209e-05
46557,93115,93114,186229,1.692713975906372,1.4926364176029328e-05
46649,93299,93298,186597,1.6958699226379395,1.4706668621450579e-05
46741,93483,93482,186965,1.6989870071411133,1.4488959743017292e-05
46833,93667,93666,187333,1.7020957469940186,1.4276116071523892e-05
46925,93851,93850,187701,1.7053358554840088,1.4067286909670315e-05
47017,94035,94034,188069,1.7087829113006592,1.385974350602618e-05
47109,94219,94218,188437,1.7122538089752197,1.3654747601262728e-05
47201,94403,94402,188805,1.7162039279937744,1.3454601993220232e-05
47293,94587,94586,189173,1.7198498249053955,1.3257532186414114e-05
47385,94771,94770,189541,1.7237379550933838,1.3061555737262826e-05
47477,94955,94954,189909,1.7276558876037598,1.2868690301076494e-05
47569,95139,95138,190277,1.731994867324829,1.2680371376939848e-05
47661,95323,95322,190645,1.7362878322601318,1.2494266595672808e-05
47753,95507,95506,191013,1.7402429580688477,1.2309350544013742e-05
47845,95691,95690,191381,1.7444558143615723,1.2127999938791617e-05
47937,95875,95874,191749,1.7487258911132812,1.195065594080364e-05
48029,96059,96058,192117,1.7528009414672852,1.177483829486249e-05
48121,96243,96242,192485,1.7567808628082275,1.1600521012361327e-05
48213,96427,96426,192853,1.7611229419708252,1.1430033284620457e-05
48305,96611,96610,193221,1.7654709815979004,1.126286029179358e-05
48397,96795,96794,193589,1.7694189548492432,1.1096760793572647e-05
48489,96979,96978,193957,1.7733068466186523,1.0932594679385211e-05
48581,97163,97162,194325,1.7772448062896729,1.0772290015615763e-05
48673,97347,97346,194693,1.7816798686981201,1.061455543043811e-05
48765,97531,97530,195061,1.7857089042663574,1.0457696391512224e-05
48857,97715,97714,195429,1.7896790504455566,1.0303223814635578e-05
48949,97899,97898,195797,1.79355788230896,1.0152411720682767e-05
49041,98083,98082,196165,1.7975788116455078,1.0003469666979112e-05
49133,98267,98266,196533,1.8013899326324463,9.855440500072648e-06
49225,98451,98450,196901,1.8052637577056885,9.710179152458424e-06
49317,98635,98634,197269,1.808816909790039,9.568180460220801e-06
49409,98819,98818,197637,1.8130989074707031,9.427477355500529e-06
49501,99003,99002,198005,1.816951036453247,9.287907882171835e-06
49593,99187,99186,198373,1.820734977722168,9.151346415409136e-06
49685,99371,99370,198741,1.8282699584960938,9.017515940989037e-06
49777,99555,99554,199109,1.8331959247589111,8.884586209173781e-06
49869,99739,99738,199477,1.8378417491912842,8.75312151133968e-06
49961,99923,99922,199845,1.8426527976989746,8.624724689292646e-06
50053,100107,100106,200213,1.8473179340362549,8.498470752845257e-06
50145,100291,100290,200581,1.8513987064361572,8.37292415815893e-06
50237,100475,100474,200949,1.8557188510894775,8.249204343181273e-06
50329,100659,100658,201317,1.8603029251098633,8.128425599961472e-06
50421,100843,100842,201685,1.864607810974121,8.009223535187804e-06
50513,101027,101026,202053,1.8685507774353027,7.890726736528382e-06
50606,101213,101212,202425,1.8725159168243408,7.7731255090043e-06
50698,101397,101396,202793,1.8772828578948975,7.659445391578745e-06
50790,101581,101580,203161,1.8839709758758545,7.546848914996893e-06
50882,101765,101764,203529,1.8954589366912842,7.4351218706676315e-06
50974,101949,101948,203897,1.905951976776123,7.325765103288293e-06
51066,102133,102132,204265,1.9154908657073975,7.21863888556665e-06
51158,102317,102316,204633,1.9212448596954346,7.112261583235777e-06
51250,102501,102500,205001,1.9258978366851807,7.0070085388562e-06
51342,102685,102684,205369,1.9331018924713135,6.904193856819248e-06
51434,102869,102868,205737,1.938750982284546,6.803145135460273e-06
51526,103053,103052,206105,1.9498028755187988,6.702669723995047e-06
51618,103237,103236,206473,1.9575488567352295,6.603606215051896e-06
51710,103421,103420,206841,1.966156005859375,6.506900122446223e-06
51802,103605,103604,207209,1.9729828834533691,6.4115045720056315e-06
51894,103789,103788,207577,1.9817798137664795,6.316661136491317e-06
51986,103973,103972,207945,1.990710973739624,6.2234894299689755e-06
52078,104157,104156,208313,1.9952607154846191,6.1324609526712e-06
52170,104341,104340,208681,2.000324010848999,6.042351861241501e-06
52262,104525,104524,209049,2.004584789276123,5.952901284826049e-06
52354,104709,104708,209417,2.0095858573913574,5.86530556996465e-06
52446,104893,104892,209785,2.018254041671753,5.779540652275084e-06
52538,105077,105076,210153,2.0238289833068848,5.694408151173242e-06
52630,105261,105260,210521,2.0306448936462402,5.6101257314999054e-06
52722,105445,105444,210889,2.036489963531494,5.527773552954146e-06
52814,105629,105628,211257,2.0410397052764893,5.446888194809428e-06
52906,105813,105812,211625,2.0459299087524414,5.3664728302174834e-06
52998,105997,105996,211993,2.050286054611206,5.287134372217573e-06
53090,106181,106180,212361,2.0543737411499023,5.209683220904636e-06
53182,106365,106364,212729,2.0590689182281494,5.1333333353355e-06
53274,106549,106548,213097,2.06369686126709,5.057415424333019e-06
53366,106733,106732,213465,2.0679500102996826,4.9827874788590494e-06
53458,106917,106916,213833,2.0718798637390137,4.909894802739924e-06
53550,107101,107100,214201,2.076019763946533,4.8377815077350455e-06
53642,107285,107284,214569,2.080256938934326,4.766168207446825e-06
53734,107469,107468,214937,2.0842888355255127,4.696003320080647e-06
53826,107653,107652,215305,2.0888419151306152,4.6273379016286084e-06
53918,107837,107836,215673,2.093397855758667,4.559207806712362e-06
54010,108021,108020,216041,2.098724842071533,4.491719964782375e-06
54102,108205,108204,216409,2.103649854660034,4.425756952066058e-06
54194,108389,108388,216777,2.1081619262695312,4.361009629479392e-06
54286,108573,108572,217145,2.113292932510376,4.2966504940132375e-06
54378,108757,108756,217513,2.1184029579162598,4.233111159542061e-06
54470,108941,108940,217881,2.1229679584503174,4.171079672974764e-06
54562,109125,109124,218249,2.1272568702697754,4.109971717453928e-06
54654,109309,109308,218617,2.132246971130371,4.049204524590929e-06
54746,109493,109492,218985,2.136502981185913,3.989430545541519e-06
54838,109677,109676,219353,2.140605926513672,3.931058622930314e-06
54930,109861,109860,219721,2.144758939743042,3.873346637110213e-06
55022,110045,110044,220089,2.149423837661743,3.81601556079516e-06
55114,110229,110228,220457,2.1534457206726074,3.7598130751159652e-06
55206,110413,110412,220825,2.157482862472534,3.7048360775952642e-06
55298,110597,110596,221193,2.1614677906036377,3.6503129430104537e-06
55390,110781,110780,221561,2.1659319400787354,3.596274846284648e-06
55482,110965,110964,221929,2.1698007583618164,3.5434388003871635e-06
55574,111149,111148,222297,2.1744418144226074,3.49160810924687e-06
55666,111333,111332,222665,2.178309679031372,3.440100169521357e-06
55758,111517,111516,223033,2.1828088760375977,3.389215167415865e-06
55850,111701,111700,223401,2.1867990493774414,3.339532376368276e-06
55942,111885,111884,223769,2.1907238960266113,3.290622449149744e-06
56034,112069,112068,224137,2.194525957107544,3.241983671444466e-06
56126,112253,112252,224505,2.1988730430603027,3.1941079657915138e-06
56218,112437,112436,224873,2.2027478218078613,3.147362752188188e-06
56310,112621,112620,225241,2.2065017223358154,3.101175549887865e-06
56402,112805,112804,225609,2.210233688354492,3.055279787639796e-06
56494,112989,112988,225977,2.2141668796539307,3.01026150853323e-06
56586,113173,113172,226345,2.2179577350616455,2.9662426785263205e-06
56678,113357,113356,226713,2.2217679023742676,2.9226089918872275e-06
56770,113541,113540,227081,2.22541880607605,2.8793416394585464e-06
56862,113725,113724,227449,2.2289090156555176,2.837019896178758e-06
56954,113909,113908,227817,2.233220100402832,2.79552775269708e-06
57046,114093,114092,228185,2.2370927333831787,2.754305483737775e-06
57138,114277,114276,228553,2.24059796333313,2.713555766992273e-06
57230,114461,114460,228921,2.2438528537750244,2.6737626065491253e-06
57322,114645,114644,229289,2.2477848529815674,2.6346148450054686e-06
57414,114829,114828,229657,2.2511448860168457,2.5956847607595452e-06
57506,115013,115012,230025,2.2548367977142334,2.5573396775331364e-06
57598,115197,115196,230393,2.258612871170044,2.51990424654169e-06
57690,115381,115380,230761,2.262126922607422,2.482939882433658e-06
57782,115565,115564,231129,2.266615867614746,2.4461996870959995e-06
57874,115749,115748,231497,2.270495891571045,2.410140253737719e-06
57966,115933,115932,231865,2.2744288444519043,2.374894207759181e-06
58058,116117,116116,232233,2.2782938480377197,2.339975084804948e-06
58150,116301,116300,232601,2.2828190326690674,2.3053328213474158e-06
58242,116485,116484,232969,2.286733865737915,2.2714328631210565e-06
58334,116669,116668,233337,2.2905867099761963,2.2382159894646906e-06
58426,116853,116852,233705,2.294416904449463,2.2052258385120026e-06
58518,117037,117036,234073,2.298923969268799,2.1725936235905645e-06
58610,117221,117220,234441,2.302806854248047,2.1407209385050955e-06
58702,117405,117404,234809,2.3067398071289062,2.1093860462365374e-06
58794,117589,117588,235177,2.310321807861328,2.078227444137373e-06
58886,117773,117772,235545,2.3144898414611816,2.0475163818937188e-06
58978,117957,117956,235913,2.3183627128601074,2.017535770351453e-06
59070,118141,118140,236281,2.3220467567443848,1.987952122668098e-06
59162,118325,118324,236649,2.3257877826690674,1.958541983114862e-06
59254,118509,118508,237017,2.3301098346710205,1.9296588343813625e-06
59346,118693,118692,237385,2.3337740898132324,1.901436263974041e-06
59438,118877,118876,237753,2.337484836578369,1.8734911344299346e-06
59530,119061,119060,238121,2.3413407802581787,1.8457555177207082e-06
59622,119245,119244,238489,2.3452558517456055,1.8186013746163903e-06
59714,119429,119428,238857,2.349745750427246,1.7920084622515903e-06
59807,119615,119614,239229,2.353698968887329,1.765320539497484e-06
59899,119799,119798,239597,2.357844829559326,1.739194761234816e-06
59991,119983,119982,239965,2.361860752105713,1.7136723959477597e-06
60083,120167,120166,240333,2.366259813308716,1.6885930229792115e-06
60175,120351,120350,240701,2.3701658248901367,1.663656787593153e-06
60267,120535,120534,241069,2.3740367889404297,1.6390663021698213e-06
60359,120719,120718,241437,2.3779077529907227,1.6150610548566654e-06
60451,120903,120902,241805,2.3828608989715576,1.59138563090384e-06
60543,121087,121086,242173,2.3868677616119385,1.5678462492134508e-06
60635,121271,121270,242541,2.390944004058838,1.5447175951763247e-06
60727,121455,121454,242909,2.394775867462158,1.522122702060111e-06
60819,121639,121638,243277,2.3993446826934814,1.4997597403039881e-06
60911,121823,121822,243645,2.40321683883667,1.4775577518582697e-06
61003,122007,122006,244013,2.407130718231201,1.4558130166670544e-06
61095,122191,122190,244381,2.41104793548584,1.4345257192476995e-06
61187,122375,122374,244749,2.4156017303466797,1.4133978450722487e-06
61279,122559,122558,245117,2.419583797454834,1.3924775548315298e-06
61371,122743,122742,245485,2.423480987548828,1.3720346545789081e-06
61463,122927,122926,245853,2.4274449348449707,1.3519594801125564e-06
61555,123111,123110,246221,2.4316799640655518,1.3320019053905342e-06
61647,123295,123294,246589,2.435670852661133,1.3123078990941918e-06
61739,123479,123478,246957,2.439525842666626,1.2930821530613655e-06
61831,123663,123662,247325,2.443380832672119,1.2741334051532646e-06
61923,123847,123846,247693,2.447746992111206,1.2552913371918956e-06
62015,124031,124030,248061,2.451687812805176,1.2367660059257572e-06
62107,124215,124214,248429,2.4556047916412354,1.2186725821550857e-06
62199,124399,124398,248797,2.4592947959899902,1.2007757130707108e-06
62291,124583,124582,249165,2.4627137184143066,1.1830011714853004e-06
62383,124767,124766,249533,2.4663538932800293,1.1655834701370917e-06
62475,124951,124950,249901,2.4696288108825684,1.1485401960480685e-06
62567,125135,125134,250269,2.4743947982788086,1.1316319408194742e-06
62659,125319,125318,250637,2.4779508113861084,1.1148804944713148e-06
62751,125503,125502,251005,2.481820821762085,1.0985059489796587e-06
62843,125687,125686,251373,2.4851748943328857,1.0824359838430798e-06
62935,125871,125870,251741,2.4883267879486084,1.0664633399489234e-06
63027,126055,126054,252109,2.4914920330047607,1.0506912328515274e-06
63119,126239,126238,252477,2.4946188926696777,1.0352930216805616e-06
63211,126423,126422,252845,2.4984917640686035,1.0201269677651834e-06
63303,126607,126606,253213,2.501677989959717,1.0050452712568984e-06
63395,126791,126790,253581,2.5048539638519287,9.90207297721576e-07
63487,126975,126974,253949,2.508335828781128,9.757180916840834e-07
63579,127159,127158,254317,2.5117719173431396,9.61395255057095e-07
63671,127343,127342,254685,2.515596866607666,9.471657150159839e-07
63763,127527,127526,255053,2.5187788009643555,9.332140519383784e-07
63855,127711,127710,255421,2.5219650268554688,9.195682180025032e-07
63947,127895,127894,255789,2.5251410007476807,9.06036893652636e-07
64039,128079,128078,256157,2.528373956680298,8.926239897082545e-07
64131,128263,128262,256525,2.5322988033294678,8.795080277572993e-07
64223,128447,128446,256893,2.5354979038238525,8.66643793357391e-07
64315,128631,128630,257261,2.5386757850646973,8.538606127799567e-07
64407,128815,128814,257629,2.5418388843536377,8.412297381316202e-07
64499,128999,128998,257997,2.5450069904327393,8.288967987743431e-07
64591,129183,129182,258365,2.548513889312744,8.16758025732284e-07
64683,129367,129366,258733,2.5515859127044678,8.046865445727458e-07
64775,129551,129550,259101,2.554785966873169,7.928021984072206e-07
64867,129735,129734,259469,2.5578837394714355,7.811989034627063e-07
64959,129919,129918,259837,2.56095290184021,7.697362211598206e-07
65051,130103,130102,260205,2.5644609928131104,7.583450211601594e-07
65143,130287,130286,260573,2.567713975906372,7.471697388873002e-07
65235,130471,130470,260941,2.5709590911865234,7.362437275856207e-07
65327,130655,130654,261309,2.5741429328918457,7.254149014309173e-07
65419,130839,130838,261677,2.5774667263031006,7.146755253210288e-07
65511,131023,131022,262045,2.5807547569274902,7.041696035285491e-07
65603,131207,131206,262413,2.5839180946350098,6.93871275026785e-07
65695,131391,131390,262781,2.5870649814605713,6.836408178423017e-07
65787,131575,131574,263149,2.590197801589966,6.73525846734932e-07
65879,131759,131758,263517,2.5933308601379395,6.636477942983871e-07
65971,131943,131942,263885,2.5965678691864014,6.539317867154504e-07
66063,132127,132126,264253,2.5996909141540527,6.442699357310241e-07
66155,132311,132310,264621,2.6028027534484863,6.347514637935887e-07
66247,132495,132494,264989,2.6059539318084717,6.254590089788171e-07
66339,132679,132678,265357,2.6091368198394775,6.162852000504347e-07
66431,132863,132862,265725,2.6121788024902344,6.071664655509188e-07
66523,133047,133046,266093,2.6152329444885254,5.982151394545897e-07
66615,133231,133230,266461,2.618295907974243,5.894665588426769e-07
66707,133415,133414,266829,2.621387004852295,5.808004710641922e-07
66799,133599,133598,267197,2.6244308948516846,5.722020059150687e-07
66891,133783,133782,267565,2.6274828910827637,5.637866932018878e-07
66983,133967,133966,267933,2.6305787563323975,5.555422063759707e-07
67075,134151,134150,268301,2.6336419582366943,5.473548040285671e-07
67167,134335,134334,268669,2.636704921722412,5.392548435516664e-07
67259,134519,134518,269037,2.6398699283599854,5.31342892797195e-07
67351,134703,134702,269405,2.642974853515625,5.235658866898261e-07
67443,134887,134886,269773,2.646021842956543,5.158328467751338e-07
67535,135071,135070,270141,2.6491448879241943,5.082094309648405e-07
67627,135255,135254,270509,2.6522018909454346,5.007674017519056e-07
67719,135439,135438,270877,2.6552507877349854,4.934253018651696e-07
67811,135623,135622,271245,2.6583499908447266,4.861259124813136e-07
67903,135807,135806,271613,2.661500930786133,4.78956037153505e-07
67995,135991,135990,271981,2.6647279262542725,4.7195072100357624e-07
68087,136175,136174,272349,2.6680078506469727,4.650154016496582e-07
68179,136359,136358,272717,2.6710798740386963,4.5813128136981737e-07
68271,136543,136542,273085,2.67413592338562,4.51390544389617e-07
68363,136727,136726,273453,2.6774237155914307,4.447900747643303e-07
68455,136911,136910,273821,2.680630922317505,4.3823778350699744e-07
68547,137095,137094,274189,2.6836347579956055,4.317516218307784e-07
68639,137279,137278,274557,2.6867129802703857,4.254143489738181e-07
68731,137463,137462,274925,2.689769983291626,4.191892079478661e-07
68823,137647,137646,275293,2.6928207874298096,4.1300005667157706e-07
68915,137831,137830,275661,2.6958320140838623,4.0689455064130484e-07
69008,138017,138016,276033,2.6988778114318848,4.008701770360746e-07
69100,138201,138200,276401,2.701889991760254,3.9499436239904666e-07
69192,138385,138384,276769,2.7049100399017334,3.891520895720616e-07
69284,138569,138568,277137,2.7079317569732666,3.8341071099210205e-07
69376,138753,138752,277505,2.710941791534424,3.778022409984312e-07
69468,138937,138936,277873,2.713993787765503,3.7225227543877414e-07
69560,139121,139120,278241,2.7170989513397217,3.6674166811410643e-07
69652,139305,139304,278609,2.7201168537139893,3.613437617972865e-07
69744,139489,139488,278977,2.723106861114502,3.560601300913546e-07
69836,139673,139672,279345,2.7261109352111816,3.508166936206776e-07
69928,139857,139856,279713,2.7292089462280273,3.456239448463449e-07
70020,140041,140040,280081,2.732200860977173,3.405492452698748e-07
70112,140225,140224,280449,2.7351889610290527,3.355667169420309e-07
70204,140409,140408,280817,2.7383317947387695,3.3061363094411606e-07
70296,140593,140592,281185,2.7413768768310547,3.257250423791776e-07
70388,140777,140776,281553,2.7459449768066406,3.209526150361991e-07
70480,140961,140960,281921,2.7489819526672363,3.1624984883003106e-07
70572,141145,141144,282289,2.752023935317993,3.115734457695158e-07
70664,141329,141328,282657,2.7550859451293945,3.069748003707734e-07
70756,141513,141512,283025,2.7581207752227783,3.0248363877858703e-07
70848,141697,141696,283393,2.7611560821533203,2.980420420999958e-07
70940,141881,141880,283761,2.764188766479492,2.9363038238656585e-07
71032,142065,142064,284129,2.7672338485717773,2.8930662098144237e-07
71124,142249,142248,284497,2.7702760696411133,2.850763406802825e-07
71216,142433,142432,284865,2.773348808288574,2.8088011848112786e-07
71308,142617,142616,285233,2.7765679359436035,2.7672218098428196e-07
71400,142801,142800,285601,2.779857873916626,2.726573887165271e-07
71492,142985,142984,285969,2.782939910888672,2.686688930643806e-07
71584,143169,143168,286337,2.7861807346343994,2.6470480891752743e-07
71676,143353,143352,286705,2.7893028259277344,2.607897723549909e-07
71768,143537,143536,287073,2.7924447059631348,2.569674343286753e-07
71860,143721,143720,287441,2.795522928237915,2.532034462099721e-07
71952,143905,143904,287809,2.798628807067871,2.494603557670797e-07
72044,144089,144088,288177,2.8016769886016846,2.457770617555563e-07
72136,144273,144272,288545,2.8047258853912354,2.4218051088831766e-07
72228,144457,144456,288913,2.8078126907348633,2.3862589666236426e-07
72320,144641,144640,289281,2.810837984085083,2.3509414200655038e-07
72412,144825,144824,289649,2.813823938369751,2.316307932448817e-07
72504,145009,145008,290017,2.8168368339538574,2.2824375343005503e-07
72596,145193,145192,290385,2.820006847381592,2.248856059999347e-07
72688,145377,145376,290753,2.8230838775634766,2.215563710227698e-07
72780,145561,145560,291121,2.8263838291168213,2.1830047719170854e-07
72872,145745,145744,291489,2.8293817043304443,2.1510760165813658e-07
72964,145929,145928,291857,2.832537889480591,2.1193509026390194e-07
73056,146113,146112,292225,2.835510015487671,2.0879981223084403e-07
73148,146297,146296,292593,2.8385887145996094,2.0573835726373788e-07
73240,146481,146480,292961,2.8419268131256104,2.027256743028505e-07
73332,146665,146664,293329,2.845036029815674,1.9972970315623865e-07
73424,146849,146848,293697,2.8480587005615234,1.967796169962621e-07
73516,147033,147032,294065,2.8511528968811035,1.938993914183223e-07
73608,147217,147216,294433,2.854118824005127,1.910545939592078e-07
73700,147401,147400,294801,2.857132911682129,1.8822733695235854e-07
73792,147585,147584,295169,2.8604609966278076,1.8545320047171757e-07
73884,147769,147768,295537,2.8639578819274902,1.8274122384604483e-07
73976,147953,147952,295905,2.8673038482666016,1.8005377067949832e-07
74068,148137,148136,296273,2.870283842086792,1.7738816048590484e-07
74160,148321,148320,296641,2.8733038902282715,1.7478017635370718e-07
74252,148505,148504,297009,2.876476764678955,1.7222412993434655e-07
74344,148689,148688,297377,2.8800058364868164,1.6968515864046426e-07
74436,148873,148872,297745,2.8834497928619385,1.671744075165066e-07
74528,149057,149056,298113,2.886676788330078,1.647223264559211e-07
74620,149241,149240,298481,2.889785051345825,1.6231092412275653e-07
74712,149425,149424,298849,2.8928399085998535,1.599130049490345e-07
74804,149609,149608,299217,2.8962349891662598,1.5755022094741314e-07
74896,149793,149792,299585,2.8993687629699707,1.5524358520297518e-07
74988,149977,149976,299953,2.9030299186706543,1.529668280475569e-07
75080,150161,150160,300321,2.906719923019409,1.5070360877230715e-07
75172,150345,150344,300689,2.9098358154296875,1.484815502718769e-07
75264,150529,150528,301057,2.91290283203125,1.4631001982490972e-07
75356,150713,150712,301425,2.9159939289093018,1.4415930427632923e-07
75448,150897,150896,301793,2.919081926345825,1.4202510746665474e-07
75540,151081,151080,302161,2.922212839126587,1.3993609304816032e-07
75632,151265,151264,302529,2.925407886505127,1.3788979145292274e-07
75724,151449,151448,302897,2.9284868240356445,1.3585786658454815e-07
75816,151633,151632,303265,2.9324939250946045,1.3384730129323495e-07
75908,151817,151816,303633,2.9363648891448975,1.3188326720085005e-07
76000,152001,152000,304001,2.939687728881836,1.2995308794779066e-07
76092,152185,152184,304369,2.943066120147705,1.2803388096782385e-07
76184,152369,152368,304737,2.9464218616485596,1.261415218568605e-07
76276,152553,152552,305105,2.95033597946167,1.242941975609794e-07
76368,152737,152736,305473,2.9537429809570312,1.2247202502767481e-07
76460,152921,152920,305841,2.9569778442382812,1.2066037223085554e-07
76552,153105,153104,306209,2.96042799949646,1.1888054346201887e-07
76644,153289,153288,306577,2.964569091796875,1.171417018683478e-07
76736,153473,153472,306945,2.9681639671325684,1.1542051898111911e-07
76828,153657,153656,307313,2.971881866455078,1.1371185001345835e-07
76920,153841,153840,307681,2.975665807723999,1.1203853133173611e-07
77012,154025,154024,308049,2.979844808578491,1.1040026341583744e-07
77104,154209,154208,308417,2.98393177986145,1.0877413908066418e-07
77196,154393,154392,308785,2.9879610538482666,1.0716416379385071e-07
77288,154577,154576,309153,2.9919819831848145,1.0559101595069752e-07
77380,154761,154760,309521,2.9958860874176025,1.0404598233060232e-07
77472,154945,154944,309889,2.9996910095214844,1.0250995037428603e-07
77564,155129,155128,310257,3.0030970573425293,1.0099439233830102e-07
77656,155313,155312,310625,3.006398916244507,9.951488135418969e-08
77748,155497,155496,310993,3.009777784347534,9.805650168434392e-08
77840,155681,155680,311361,3.0132648944854736,9.660635889522634e-08
77932,155865,155864,311729,3.0165958404541016,9.518076754130286e-08
78024,156049,156048,312097,3.0199568271636963,9.378835495371751e-08
78116,156233,156232,312465,3.0231449604034424,9.241091054569536e-08
78209,156419,156418,312837,3.026371955871582,9.102822078893593e-08
78301,156603,156602,313205,3.0296969413757324,8.968824640006383e-08
78393,156787,156786,313573,3.0330920219421387,8.837681461361381e-08
78485,156971,156970,313941,3.036357879638672,8.7075518782072e-08
78577,157155,157154,314309,3.039508819580078,8.578659925401548e-08
78669,157339,157338,314677,3.042613983154297,8.45268661223366e-08
78761,157523,157522,315045,3.045722007751465,8.32902318842664e-08
78853,157707,157706,315413,3.0489490032196045,8.206097296289424e-08
78945,157891,157890,315781,3.0520570278167725,8.084749474037858e-08
79037,158075,158074,316149,3.0551679134368896,7.9662827894006e-08
79129,158259,158258,316517,3.0598578453063965,7.849567696529446e-08
79221,158443,158442,316885,3.063015937805176,7.733504541147907e-08
79313,158627,158626,317253,3.0661380290985107,7.619349976517837e-08
79405,158811,158810,317621,3.069291830062866,7.507869797408108e-08
79497,158995,158994,317989,3.0724217891693115,7.397639356748442e-08
79589,159179,159178,318357,3.075958013534546,7.28814178485265e-08
79681,159363,159362,318725,3.0791537761688232,7.180808984885597e-08
79773,159547,159546,319093,3.082660675048828,7.075809680968502e-08
79865,159731,159730,319461,3.0867960453033447,6.97166956299279e-08
79957,159915,159914,319829,3.09023380279541,6.868464150055228e-08
80049,160099,160098,320197,3.0939528942108154,6.767560292863167e-08
80141,160283,160282,320565,3.097822904586792,6.668567315486672e-08
80233,160467,160466,320933,3.1018049716949463,6.570186959185193e-08
80325,160651,160650,321301,3.1056768894195557,6.473006049442525e-08
80417,160835,160834,321669,3.1096229553222656,6.378123000626072e-08
80509,161019,161018,322037,3.1134917736053467,6.284706259293495e-08
80601,161203,161202,322405,3.1173598766326904,6.191807575710435e-08
80693,161387,161386,322773,3.121706962585449,6.100375720049496e-08
80785,161571,161570,323141,3.1256470680236816,6.011100928182985e-08
80877,161755,161754,323509,3.129525899887085,5.9228831026124815e-08
80969,161939,161938,323877,3.1334776878356934,5.8352256013700395e-08
81061,162123,162122,324245,3.1373178958892822,5.7492517778530784e-08
81153,162307,162306,324613,3.1410937309265137,5.665181655878648e-08
81245,162491,162490,324981,3.1448328495025635,5.581840560606386e-08
81337,162675,162674,325349,3.1486289501190186,5.499205386857771e-08
81429,162859,162858,325717,3.152477741241455,5.418381347102394e-08
81521,163043,163042,326085,3.156205892562866,5.3391346558311255e-08
81613,163227,163226,326453,3.1601059436798096,5.2603998074571045e-08
81705,163411,163410,326821,3.164320945739746,5.182575064984955e-08
81797,163595,163594,327189,3.1681110858917236,5.106579228017178e-08
81889,163779,163778,327557,3.172074794769287,5.031808269736157e-08
81981,163963,163962,327925,3.175916910171509,4.957452637227752e-08
82073,164147,164146,328293,3.1796798706054688,4.8842219027038e-08
82165,164331,164330,328661,3.1834709644317627,4.8127274008814985e-08
82257,164515,164514,329029,3.187483787536621,4.7421254084634546e-08
82349,164699,164698,329397,3.1913888454437256,4.6719540263283406e-08
82441,164883,164882,329765,3.1952266693115234,4.603089299139288e-08
82533,165067,165066,330133,3.199022054672241,4.5357743713987685e-08
82625,165251,165250,330501,3.202725887298584,4.469078261931747e-08
82717,165435,165434,330869,3.206209897994995,4.402915582651069e-08
82809,165619,165618,331237,3.209707021713257,4.338175109022284e-08
82901,165803,165802,331605,3.2128360271453857,4.2747338414533697e-08
82993,165987,165986,331973,3.2160139083862305,4.2117222905682836e-08
83085,166171,166170,332341,3.219172716140747,4.1494002535057685e-08
83177,166355,166354,332709,3.222532033920288,4.088530871560136e-08
83269,166539,166538,333077,3.225703716278076,4.028682485475968e-08
83361,166723,166722,333445,3.2288808822631836,3.9691700154134313e-08
83453,166907,166906,333813,3.2322537899017334,3.9105183933511736e-08
83545,167091,167090,334181,3.235460042953491,3.85326140420452e-08
83637,167275,167274,334549,3.238755941390991,3.796756736165274e-08
83729,167459,167458,334917,3.241989850997925,3.7405850246068275e-08
83821,167643,167642,335285,3.245210886001587,3.685425158217719e-08
83913,167827,167826,335653,3.24847412109375,3.63152433833782e-08
84005,168011,168010,336021,3.2517077922821045,3.5781487084579576e-08
84097,168195,168194,336389,3.255018949508667,3.525176649878534e-08
84189,168379,168378,336757,3.2581369876861572,3.473319019394859e-08
84281,168563,168562,337125,3.261561870574951,3.422529183462106e-08
84373,168747,168746,337493,3.2647688388824463,3.3721015188852656e-08
84465,168931,168930,337861,3.2680177688598633,3.322195562391213e-08
84557,169115,169114,338229,3.2711007595062256,3.2734410324584665e-08
84649,169299,169298,338597,3.2741658687591553,3.2255357040557166e-08
84741,169483,169482,338965,3.2772939205169678,3.177904378452188e-08
84833,169667,169666,339333,3.280388832092285,3.1309304740099e-08
84925,169851,169850,339701,3.28357195854187,3.085074514799182e-08
85017,170035,170034,340069,3.286655902862549,3.0398515143257757e-08
85109,170219,170218,340437,3.289731025695801,2.994887776823184e-08
85201,170403,170402,340805,3.2928268909454346,2.9507058785678863e-08
85293,170587,170586,341173,3.2959086894989014,2.907544689237405e-08
85385,170771,170770,341541,3.2989916801452637,2.864828961613214e-08
85477,170955,170954,341909,3.3021297454833984,2.8224191560532956e-08
85569,171139,171138,342277,3.3052239418029785,2.7808807422608526e-08
85661,171323,171322,342645,3.308255910873413,2.7402180464040423e-08
85753,171507,171506,343013,3.311262845993042,2.6998614909001605e-08
85845,171691,171690,343381,3.31430983543396,2.6598992767056036e-08
85937,171875,171874,343749,3.317312002182007,2.6208478318966862e-08
86029,172059,172058,344117,3.3203318119049072,2.5825011588691778e-08
86121,172243,172242,344485,3.3233320713043213,2.5443797665178187e-08
86213,172427,172426,344853,3.3263208866119385,2.5067594377167803e-08
86305,172611,172610,345221,3.329556941986084,2.470033424966439e-08
86397,172795,172794,345589,3.332606792449951,2.433838892618536e-08
86489,172979,172978,345957,3.33563494682312,2.397847821664099e-08
86581,173163,173162,346325,3.338660717010498,2.362459548607034e-08
86673,173347,173346,346693,3.3417978286743164,2.3278970477833487e-08
86765,173531,173530,347061,3.344817876815796,2.2937120229033504e-08
86857,173715,173714,347429,3.3478379249572754,2.259759545660908e-08
86949,173899,173898,347797,3.3508448600769043,2.2264869636916508e-08
87041,174083,174082,348165,3.3538668155670166,2.1939310362843644e-08
87133,174267,174266,348533,3.356872797012329,2.1616344298267012e-08
87225,174451,174450,348901,3.3601298332214355,2.1296356941348804e-08
87317,174635,174634,349269,3.363564968109131,2.0983558715423975e-08
87410,174821,174820,349641,3.3667030334472656,2.067327359298059e-08
87502,175005,175004,350009,3.3699567317962646,2.0368196018325836e-08
87594,175189,175188,350377,3.373121976852417,2.006697897043924e-08
87686,175373,175372,350745,3.376343011856079,1.9772906818574094e-08
87778,175557,175556,351113,3.3795077800750732,1.94832382107426e-08
87870,175741,175740,351481,3.38264799118042,1.919518290026481e-08
87962,175925,175924,351849,3.385802984237671,1.8911811478430222e-08
88054,176109,176108,352217,3.388921022415161,1.8635093306291042e-08
88146,176293,176292,352585,3.391995906829834,1.8361525914273146e-08
88238,176477,176476,352953,3.39505672454834,1.8089753202140643e-08
88330,176661,176660,353321,3.3981218338012695,1.7823310998989424e-08
88422,176845,176844,353689,3.4011898040771484,1.756269272887246e-08
88514,177029,177028,354057,3.4042508602142334,1.7304242111875756e-08
88606,177213,177212,354425,3.4073848724365234,1.7048073522185444e-08
88698,177397,177396,354793,3.41054368019104,1.6797590976859782e-08
88790,177581,177580,355161,3.413719892501831,1.655189347781143e-08
88882,177765,177764,355529,3.416958808898926,1.630773409915037e-08
88974,177949,177948,355897,3.420119047164917,1.6066507536576055e-08
89066,178133,178132,356265,3.424514055252075,1.5830976103925172e-08
89158,178317,178316,356633,3.4276950359344482,1.5599128803978717e-08
89250,178501,178500,357001,3.430968999862671,1.53685666815719e-08
89342,178685,178684,357369,3.434175968170166,1.5141602135220025e-08
89434,178869,178868,357737,3.4373559951782227,1.4920000751622412e-08
89526,179053,179052,358105,3.4405078887939453,1.4701062982374358e-08
89618,179237,179236,358473,3.4436628818511963,1.4483499214967246e-08
89710,179421,179420,358841,3.4468178749084473,1.4270078785839407e-08
89802,179605,179604,359209,3.449881076812744,1.4061406768046876e-08
89894,179789,179788,359577,3.4529640674591064,1.3854574333351559e-08
89986,179973,179972,359945,3.4560697078704834,1.3649465536976666e-08
90078,180157,180156,360313,3.4591619968414307,1.3448828523475536e-08
90170,180341,180340,360681,3.4623148441314697,1.325213892815947e-08
90262,180525,180524,361049,3.4653990268707275,1.3056736323083371e-08
90354,180709,180708,361417,3.468564987182617,1.2863558046802787e-08
90446,180893,180892,361785,3.47165584564209,1.2674909983829342e-08
90538,181077,181076,362153,3.47473406791687,1.2489337589024733e-08
90630,181261,181260,362521,3.477832794189453,1.2304798104666865e-08
90722,181445,181444,362889,3.4809088706970215,1.2123015914104993e-08
90814,181629,181628,363257,3.483977794647217,1.1945548036817609e-08
90906,181813,181812,363625,3.4870529174804688,1.1770328267516486e-08
90998,181997,181996,363993,3.4901177883148193,1.1596166154604667e-08
91090,182181,182180,364361,3.493184804916382,1.1425217577417042e-08
91182,182365,182364,364729,3.4962680339813232,1.1258132378580975e-08
91274,182549,182548,365097,3.499325752258301,1.1092608672422978e-08
91366,182733,182732,365465,3.5023837089538574,1.0928387791836457e-08
91458,182917,182916,365833,3.5054588317871094,1.0767676309563755e-08
91550,183101,183100,366201,3.5086047649383545,1.0610214181081646e-08
91642,183285,183284,366569,3.5117719173431396,1.0453833838215315e-08
91734,183469,183468,366937,3.514997959136963,1.0299138019891906e-08
91826,183653,183652,367305,3.5182137489318848,1.014803835416807e-08
91918,183837,183836,367673,3.521383762359619,9.999500834441716e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/flex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.200241088867188e-05,4.387072431292609
3,11,0,11,0.0006048679351806641,3.473448194683989
6,24,0,24,0.0010082721710205078,2.032332276860507
8,32,0,32,0.001280069351196289,1.5510168039236454
11,43,0,43,0.0016410350799560547,0.9646848713255388
14,56,0,56,0.002061128616333008,0.6476669392193777
17,67,0,67,0.002443075180053711,0.39656488334482437
19,75,0,75,0.002730131149291992,0.2958255937252611
22,86,0,86,0.003159046173095703,0.21735477306796255
25,99,0,99,0.0036122798919677734,0.15244269907523542
28,110,0,110,0.004024028778076172,0.09558859304145342
30,119,0,119,0.004328012466430664,0.0912229100773483
33,132,0,132,0.004773139953613281,0.07866502189815996
36,147,0,147,0.005275249481201172,0.0733650030902074
39,161,0,161,0.005918979644775391,0.06963621796749558
41,171,0,171,0.006307125091552734,0.06731282773701364
44,186,0,186,0.006953001022338867,0.06502672477720547
47,200,0,200,0.007467985153198242,0.06317514225694952
50,215,0,215,0.007976055145263672,0.06053816577577747
52,225,0,225,0.008409261703491211,0.059386332536707866
55,240,0,240,0.008903980255126953,0.05817356562641064
58,255,0,255,0.009519100189208984,0.057321804640327975
61,269,0,269,0.010187149047851562,0.05596096137084261
63,278,0,278,0.010576248168945312,0.05322957639247789
66,293,0,293,0.011087179183959961,0.05116145604114655
69,307,0,307,0.011588096618652344,0.04726611454488083
72,322,0,322,0.01226496696472168,0.0462312507190202
75,336,0,336,0.012782096862792969,0.04444062553927025
77,345,0,345,0.013100147247314453,0.04206182246313801
80,359,0,359,0.013576030731201172,0.03987436697304369
83,374,0,374,0.014084100723266602,0.038375133617586
86,388,0,388,0.014566898345947266,0.03624269783099602
88,398,0,398,0.01488804817199707,0.03558201456610184
91,413,0,413,0.015382051467895508,0.03492006541815994
94,427,0,427,0.015857219696044922,0.03397514683577285
97,441,0,441,0.01633310317993164,0.03199715988995219
99,451,0,451,0.01665806770324707,0.03149444519387161
102,466,0,466,0.017144203186035156,0.030959248797765144
105,481,0,481,0.017642974853515625,0.030583791077994096
108,496,0,496,0.01822805404663086,0.03030314873520102
110,506,0,506,0.018606185913085938,0.030150480611865493
113,521,0,521,0.01911020278930664,0.029957380970677554
116,536,0,536,0.01960611343383789,0.029795631990181905
119,551,0,551,0.02011704444885254,0.02965659504714112
121,561,0,561,0.02045416831970215,0.029573748370816805
124,576,0,576,0.020965099334716797,0.029461344280374828
127,591,0,591,0.021743059158325195,0.02936061131995728
130,605,0,605,0.022971153259277344,0.02895793316269333
132,615,0,615,0.023478984832763672,0.02838686221647244
135,630,0,630,0.024059295654296875,0.02783363050467214
138,645,0,645,0.024730205535888672,0.027494570768971816
141,660,0,660,0.025501012802124023,0.027274311617796785
144,675,0,675,0.02613091468811035,0.027121746303874254
146,685,0,685,0.026528120040893555,0.027043311258121507
149,700,0,700,0.027096033096313477,0.026948228512619094
152,715,0,715,0.027677059173583984,0.026871415464039736
155,730,0,730,0.02828693389892578,0.02680676810983676
157,740,0,740,0.028621196746826172,0.0267686030492869
160,755,0,755,0.029140949249267578,0.026716923391911406
163,770,0,770,0.029624223709106445,0.026670437956765696
166,785,0,785,0.0301210880279541,0.026627948961460396
168,794,0,794,0.030431032180786133,0.0257439928240897
171,809,0,809,0.030985116958618164,0.025373942231900527
174,824,0,824,0.031638145446777344,0.02515471479929574
177,839,0,839,0.03217315673828125,0.025014722648002457
179,849,0,849,0.0325009822845459,0.024946988421648126
182,864,0,864,0.033000946044921875,0.02486850396251165
185,879,0,879,0.03348708152770996,0.02480801240041188
188,894,0,894,0.0340421199798584,0.024759029374874796
190,904,0,904,0.034371137619018555,0.024730844192112248
193,919,0,919,0.03496813774108887,0.024693539901186435
196,934,0,934,0.03555607795715332,0.024660721242445564
199,949,0,949,0.03611016273498535,0.024631204633016737
201,959,0,959,0.0365140438079834,0.024612962818743575
204,974,0,974,0.037065982818603516,0.024587319882431784
207,989,0,989,0.03758597373962402,0.024563389911519
210,1004,0,1004,0.038099050521850586,0.02454087139499733
213,1019,0,1019,0.03868508338928223,0.0245195253881657
215,1029,0,1029,0.03904008865356445,0.024505847321655227
218,1044,0,1044,0.03951692581176758,0.024486034355315583
221,1059,0,1059,0.04000425338745117,0.024466936393217068
224,1074,0,1074,0.04048609733581543,0.024448429515566503
226,1084,0,1084,0.04080510139465332,0.024436373658271112
229,1099,0,1099,0.04128003120422363,0.024418655642380254
232,1114,0,1114,0.04175615310668945,0.024401323372577194
235,1129,0,1129,0.04224801063537598,0.02438432716462068
237,1139,0,1139,0.04256415367126465,0.02437316138330255
240,1154,0,1154,0.04303789138793945,0.02435663150553974
243,1169,0,1169,0.04350996017456055,0.02434032942777805
246,1184,0,1184,0.043984174728393555,0.02432421844645624
248,1194,0,1194,0.04430222511291504,0.02431356787183183
251,1209,0,1209,0.044775962829589844,0.024297707098148023
254,1224,0,1224,0.04525113105773926,0.024281966322152328
257,1239,0,1239,0.04572319984436035,0.024266329787030562
259,1249,0,1249,0.046038150787353516,0.024255957371899797
262,1264,0,1264,0.04651212692260742,0.024240469957238994
265,1279,0,1279,0.04698491096496582,0.024225062753684922
268,1294,0,1294,0.04745912551879883,0.024209732646130962
270,1304,0,1304,0.047775983810424805,0.02419955450993122
273,1319,0,1319,0.0482633113861084,0.02418434864333217
276,1334,0,1334,0.04874014854431152,0.02416921307156319
279,1349,0,1349,0.04922008514404297,0.024154142460242355
281,1359,0,1359,0.049636125564575195,0.024144128437403028
284,1374,0,1374,0.05016493797302246,0.02412915262155988
287,1389,0,1389,0.05074620246887207,0.024114226716803282
290,1404,0,1404,0.05132412910461426,0.02409934657608907
293,1419,0,1419,0.051870107650756836,0.0240845081816001
295,1429,0,1429,0.052201032638549805,0.02407463698896906
298,1444,0,1444,0.05290508270263672,0.024059858627752156
301,1459,0,1459,0.05413508415222168,0.02404511132248224
304,1474,0,1474,0.05529022216796875,0.0240303932564344
306,1484,0,1484,0.05602407455444336,0.02402059750081836
309,1499,0,1499,0.0569150447845459,0.024005929566763364
312,1514,0,1514,0.057967185974121094,0.02399129480022125
315,1529,0,1529,0.0587460994720459,0.023976695932150512
317,1539,0,1539,0.05912208557128906,0.023966984408981973
320,1554,0,1554,0.059806108474731445,0.023952449785655534
323,1569,0,1569,0.060658931732177734,0.023937954994789658
326,1584,0,1584,0.06183815002441406,0.023923500355032035
328,1594,0,1594,0.06260514259338379,0.02391388637980172
331,1609,0,1609,0.06359720230102539,0.023899499486953107
334,1624,0,1624,0.06468987464904785,0.02388515416260165
337,1639,0,1639,0.06586599349975586,0.023870851209930998
339,1649,0,1649,0.06656002998352051,0.0238613397413695
342,1664,0,1664,0.06781411170959473,0.023847108438385688
345,1679,0,1679,0.0690622329711914,0.023832920015442564
348,1694,0,1694,0.07016110420227051,0.0238187739263808
350,1704,0,1704,0.07091307640075684,0.02380936638293199
353,1719,0,1719,0.07205009460449219,0.023795289420548572
356,1734,0,1734,0.07332921028137207,0.023781253480465375
359,1749,0,1749,0.07424426078796387,0.023767258814967687
362,1764,0,1764,0.07483220100402832,0.023753306189184663
364,1774,0,1774,0.07528185844421387,0.02374402833541098
367,1789,0,1789,0.07596111297607422,0.02373014829784763
370,1804,0,1804,0.0765829086303711,0.023716313354983906
373,1819,0,1819,0.07750415802001953,0.023702524434385964
375,1829,0,1829,0.07807207107543945,0.023693357735822488
378,1844,0,1844,0.07890009880065918,0.02367964693863637
381,1859,0,1859,0.07974720001220703,0.02366598354920625
384,1874,0,1874,0.0807030200958252,0.023652367712436506
386,1884,0,1884,0.08124804496765137,0.023643316824587035
389,1899,0,1899,0.08211421966552734,0.023629779514760828
392,1914,0,1914,0.08274722099304199,0.023616287863794574
395,1929,0,1929,0.08324003219604492,0.02360283981180163
397,1939,0,1939,0.08356499671936035,0.023593897306110015
400,1954,0,1954,0.08405208587646484,0.023580515447624604
403,1969,0,1969,0.08453822135925293,0.02356716887195732
406,1984,0,1984,0.08510017395019531,0.023553854438211477
408,1994,0,1994,0.08546304702758789,0.023544994712877184
411,2009,0,2009,0.08599209785461426,0.023531728558469203
414,2024,0,2024,0.08648395538330078,0.023518489483737588
417,2039,0,2039,0.08697295188903809,0.023505276927906618
419,2048,0,2048,0.08728408813476562,0.023151368023947398
422,2061,0,2061,0.08774209022521973,0.020353620186680906
425,2076,0,2076,0.0882420539855957,0.01963851371864139
428,2089,0,2089,0.08868408203125,0.015932748789237828
431,2100,0,2100,0.08910608291625977,0.005740104870530547
433,2108,0,2108,0.089385986328125,0.003054949672172139
436,2118,0,2118,0.08977890014648438,0.00245713375297892
439,2129,0,2129,0.09020709991455078,0.002218790866146663
442,2143,0,2143,0.0906832218170166,0.0019017410112598919
444,2151,0,2151,0.09097504615783691,0.0016548982805513878
447,2164,0,2164,0.09143495559692383,0.0014642722143068103
450,2179,0,2179,0.09192109107971191,0.0013142740438146004
453,2194,0,2194,0.09240913391113281,0.001207276140700529
455,2202,0,2202,0.09270620346069336,0.0010790085239374481
458,2214,0,2214,0.09315896034240723,0.0009247657554080052
461,2228,0,2228,0.09363102912902832,0.0007226864081897073
464,2242,0,2242,0.09410524368286133,0.0006344769674104682
466,2251,0,2251,0.09441614151000977,0.0005897699074583846
469,2265,0,2265,0.09489202499389648,0.0005269852936455267
472,2280,0,2280,0.0953819751739502,0.000492883106802978
475,2295,0,2295,0.09586811065673828,0.00046966712086979535
477,2304,0,2304,0.0961771011352539,0.00045060004551826825
480,2318,0,2318,0.09664726257324219,0.00042706870879101705
483,2333,0,2333,0.0971379280090332,0.0004021262300165856
486,2348,0,2348,0.0976252555847168,0.00038390963508222334
488,2358,0,2358,0.09794831275939941,0.00037414737763066374
491,2373,0,2373,0.09843826293945312,0.0003619043551609022
494,2387,0,2387,0.09891819953918457,0.000333370184141835
497,2401,0,2401,0.09939718246459961,0.0003086461614974442
500,2415,0,2415,0.0998992919921875,0.000295787330336128
502,2425,0,2425,0.10029911994934082,0.00028516580742615814
505,2440,0,2440,0.10110116004943848,0.00027377807601868795
508,2454,0,2454,0.10187506675720215,0.0002519677795825361
511,2467,0,2467,0.10256791114807129,0.0002366090609854904
513,2477,0,2477,0.10317707061767578,0.0002261319637696321
516,2491,0,2491,0.10394501686096191,0.00020841754409729876
519,2504,0,2504,0.10457921028137207,0.00018429762930736567
522,2518,0,2518,0.10513615608215332,0.00016524781483703992
524,2527,0,2527,0.1055440902709961,0.0001613500977418623
527,2541,0,2541,0.10615301132202148,0.0001445922586235725
530,2556,0,2556,0.1066591739654541,0.00013555968720327738
533,2570,0,2570,0.10715508460998535,0.00012340025129315446
535,2580,0,2580,0.10749006271362305,0.00012023923789030847
538,2595,0,2595,0.10798907279968262,0.00011664568441771645
541,2609,0,2609,0.1084752082824707,0.000108392890713559
544,2624,0,2624,0.10925412178039551,0.00010543365941472121
546,2634,0,2634,0.10971903800964355,0.00010388128417663508
549,2649,0,2649,0.11022520065307617,0.00010194724094062588
552,2663,0,2663,0.11073899269104004,9.508629272769048e-05
555,2678,0,2678,0.11126089096069336,9.306158450757446e-05
557,2687,0,2687,0.11159205436706543,8.622534615216891e-05
560,2702,0,2702,0.11211705207824707,8.422166123462786e-05
563,2716,0,2716,0.11262011528015137,7.815481662875244e-05
566,2731,0,2731,0.11313509941101074,7.631755764665034e-05
569,2746,0,2746,0.11365818977355957,7.511903246828514e-05
571,2756,0,2756,0.11399030685424805,7.451653085816061e-05
574,2771,0,2771,0.11449408531188965,7.378450638376001e-05
577,2785,0,2785,0.11498022079467773,7.024298615536032e-05
580,2800,0,2800,0.11547708511352539,6.878452041157285e-05
582,2809,0,2809,0.11582708358764648,6.762898915642345e-05
585,2824,0,2824,0.1164090633392334,6.487003514776463e-05
588,2838,0,2838,0.11692309379577637,5.953946802080807e-05
591,2852,0,2852,0.11757326126098633,5.6957350923230264e-05
593,2861,0,2861,0.11806321144104004,5.600607184373165e-05
596,2876,0,2876,0.11900496482849121,5.3828971695533674e-05
599,2891,0,2891,0.1197209358215332,5.264584781484228e-05
602,2906,0,2906,0.1204061508178711,5.1964409822150824e-05
604,2916,0,2916,0.12079906463623047,5.1660631158418854e-05
607,2931,0,2931,0.12133622169494629,5.133114509840949e-05
610,2946,0,2946,0.12184309959411621,5.108910669544961e-05
613,2960,0,2960,0.12232804298400879,4.806616619920637e-05
615,2969,0,2969,0.12264513969421387,4.542406572306242e-05
618,2983,0,2983,0.12313127517700195,4.377184665495077e-05
621,2998,0,2998,0.1236269474029541,4.2766192854533955e-05
624,3013,0,3013,0.12412428855895996,4.21500246589246e-05
626,3023,0,3023,0.12445592880249023,4.1865516718071644e-05
629,3038,0,3038,0.12495303153991699,4.155304558876743e-05
632,3053,0,3053,0.12544894218444824,4.132616040619909e-05
635,3068,0,3068,0.12595319747924805,4.115158870586088e-05
638,3083,0,3083,0.1264500617980957,4.101070594540892e-05
640,3092,0,3092,0.12676715850830078,4.016748237121521e-05
643,3107,0,3107,0.12726497650146484,3.937645202850983e-05
646,3122,0,3122,0.12777113914489746,3.890117844804813e-05
649,3137,0,3137,0.12827110290527344,3.86021549133981e-05
651,3147,0,3147,0.12860321998596191,3.8461232045399426e-05
654,3162,0,3162,0.12909793853759766,3.830347618859395e-05
657,3177,0,3177,0.12958908081054688,3.818638218945729e-05
660,3192,0,3192,0.13009214401245117,3.8094277787451636e-05
662,3202,0,3202,0.13042902946472168,3.804214003540849e-05
665,3217,0,3217,0.13092613220214844,3.797362043479353e-05
668,3232,0,3232,0.1314239501953125,3.791346961183545e-05
671,3247,0,3247,0.13191819190979004,3.785934136233678e-05
673,3257,0,3257,0.13225126266479492,3.782582798005282e-05
676,3272,0,3272,0.13274598121643066,3.777862459058906e-05
679,3287,0,3287,0.1332411766052246,3.773442679088611e-05
682,3302,0,3302,0.13373494148254395,3.769268980082534e-05
684,3312,0,3312,0.1340651512145996,3.76660550603469e-05
687,3327,0,3327,0.13457894325256348,3.7627692775729934e-05
690,3342,0,3342,0.13506102561950684,3.759102783506214e-05
693,3357,0,3357,0.1355452537536621,3.7555811219241306e-05
695,3367,0,3367,0.1358661651611328,3.753301648707805e-05
698,3382,0,3382,0.13634419441223145,3.749969507015592e-05
701,3397,0,3397,0.13682198524475098,3.7467271758358166e-05
704,3412,0,3412,0.13730096817016602,3.743562565474461e-05
706,3422,0,3422,0.13763999938964844,3.741491685478529e-05
709,3437,0,3437,0.13813090324401855,3.738438425752245e-05
712,3452,0,3452,0.13863015174865723,3.735442852619704e-05
715,3466,0,3466,0.13911104202270508,3.662166870016281e-05
718,3481,0,3481,0.13960504531860352,3.618294446085004e-05
720,3491,0,3491,0.1399390697479248,3.598821559546591e-05
723,3506,0,3506,0.14043331146240234,3.578102096073539e-05
726,3521,0,3521,0.14093804359436035,3.563523123788376e-05
729,3536,0,3536,0.1414201259613037,3.552536977028174e-05
731,3546,0,3546,0.14174103736877441,3.546508718722154e-05
734,3561,0,3561,0.14222121238708496,3.538796193539509e-05
737,3576,0,3576,0.14272308349609375,3.532234851378486e-05
740,3591,0,3591,0.1432352066040039,3.526507350592354e-05
742,3601,0,3601,0.1436159610748291,3.523048668780329e-05
745,3616,0,3616,0.14410710334777832,3.518292190764519e-05
748,3631,0,3631,0.14458799362182617,3.5139587945004657e-05
751,3646,0,3646,0.14506912231445312,3.509968051667399e-05
753,3656,0,3656,0.14539003372192383,3.507466622496105e-05
756,3671,0,3671,0.14589691162109375,3.503915621462254e-05
759,3686,0,3686,0.1463930606842041,3.500570597199787e-05
762,3701,0,3701,0.14691901206970215,3.497401577489603e-05
764,3711,0,3711,0.14724206924438477,3.495375412851226e-05
767,3726,0,3726,0.14772295951843262,3.492451383047227e-05
770,3741,0,3741,0.14820313453674316,3.489650288899591e-05
773,3756,0,3756,0.14870500564575195,3.486957204039705e-05
775,3766,0,3766,0.1490330696105957,3.485215675358962e-05
778,3781,0,3781,0.14952397346496582,3.482676059004007e-05
781,3796,0,3796,0.15002107620239258,3.480214235107868e-05
784,3811,0,3811,0.1505138874053955,3.477820236769614e-05
787,3826,0,3826,0.15100908279418945,3.475485819151611e-05
789,3836,0,3836,0.15134215354919434,3.473959582995489e-05
792,3851,0,3851,0.15183615684509277,3.4717119025858044e-05
795,3866,0,3866,0.1523280143737793,3.46951083653743e-05
798,3881,0,3881,0.15282320976257324,3.467352776484152e-05
800,3891,0,3891,0.1531531810760498,3.465936151155762e-05
803,3906,0,3906,0.15366101264953613,3.463841423279218e-05
806,3921,0,3921,0.1542370319366455,3.46177915437681e-05
809,3936,0,3936,0.15477514266967773,3.459744939412476e-05
811,3946,0,3946,0.15510201454162598,3.4584023721541536e-05
814,3960,0,3960,0.15558409690856934,3.3630517307195454e-05
817,3975,0,3975,0.15607023239135742,3.291485116783064e-05
820,3990,0,3990,0.15655303001403809,3.2523462229576256e-05
822,4000,0,4000,0.1568770408630371,3.236053825381198e-05
825,4015,0,4015,0.15736126899719238,3.219768303764772e-05
828,4030,0,4030,0.15787124633789062,3.209119135931888e-05
831,4045,0,4045,0.15836596488952637,3.201549727689728e-05
833,4055,0,4055,0.15871214866638184,3.1975332220436726e-05
836,4070,0,4070,0.1591951847076416,3.192494104982753e-05
839,4085,0,4085,0.15968012809753418,3.188252673347464e-05
842,4100,0,4100,0.16016316413879395,3.1845382555096804e-05
844,4110,0,4110,0.16048312187194824,3.182275103458251e-05
847,4125,0,4125,0.16098833084106445,3.179126482316003e-05
850,4140,0,4140,0.1614840030670166,3.176212962378212e-05
853,4155,0,4155,0.16198015213012695,3.173483615403656e-05
856,4170,0,4170,0.1624760627746582,3.1709026154166334e-05
858,4180,0,4180,0.16280698776245117,3.169250602210052e-05
861,4195,0,4195,0.16330814361572266,3.1668585179186475e-05
864,4210,0,4210,0.16382312774658203,3.164555125988876e-05
867,4225,0,4225,0.16432619094848633,3.162327967477323e-05
869,4235,0,4235,0.1646571159362793,3.16088101655293e-05
872,4250,0,4250,0.16515207290649414,3.158761775064959e-05
875,4265,0,4265,0.16566109657287598,3.1566989953774204e-05
878,4280,0,4280,0.16614413261413574,3.1546872876230645e-05
880,4290,0,4290,0.16648197174072266,3.153371630311464e-05
883,4305,0,4305,0.1669631004333496,3.1514316023895383e-05
886,4319,0,4319,0.1674330234527588,3.0491400397619093e-05
889,4333,0,4333,0.16792702674865723,2.9792504724614573e-05
891,4343,0,4343,0.16826319694519043,2.941702355941309e-05
894,4358,0,4358,0.1687612533569336,2.900335940665186e-05
897,4373,0,4373,0.16925811767578125,2.870166777762944e-05
900,4388,0,4388,0.16975903511047363,2.8468959901981102e-05
902,4398,0,4398,0.17009997367858887,2.8339883068689083e-05
905,4413,0,4413,0.17060613632202148,2.8174564784248173e-05
908,4428,0,4428,0.17126822471618652,2.80348559513363e-05
911,4443,0,4443,0.1717970371246338,2.7914337987608337e-05
913,4453,0,4453,0.172133207321167,2.7842515448762227e-05
916,4468,0,4468,0.17264413833618164,2.7745144451809678e-05
919,4483,0,4483,0.17314505577087402,2.765803445970082e-05
922,4498,0,4498,0.17364931106567383,2.757935936169885e-05
925,4513,0,4513,0.1741471290588379,2.7507633850844746e-05
927,4523,0,4523,0.1744840145111084,2.74630593380091e-05
930,4538,0,4538,0.17498397827148438,2.740031525377644e-05
933,4553,0,4553,0.17548418045043945,2.734180480173763e-05
936,4568,0,4568,0.17599010467529297,2.7286929173332113e-05
938,4578,0,4578,0.1763153076171875,2.7252142568166453e-05
941,4593,0,4593,0.1768040657043457,2.7202387899973066e-05
944,4608,0,4608,0.1772899627685547,2.7155267051705107e-05
947,4623,0,4623,0.17777299880981445,2.7110499274351432e-05
949,4633,0,4633,0.17809629440307617,2.7081835491030957e-05
952,4648,0,4648,0.17858409881591797,2.7040442848585814e-05
955,4663,0,4663,0.17906713485717773,2.7000792785199084e-05
958,4678,0,4678,0.1795499324798584,2.696270733156184e-05
960,4688,0,4688,0.1798710823059082,2.6938112717637753e-05
963,4703,0,4703,0.18035626411437988,2.6902324163238344e-05
966,4718,0,4718,0.1808481216430664,2.686776691796304e-05
969,4733,0,4733,0.18133807182312012,2.683434587946491e-05
971,4743,0,4743,0.18166303634643555,2.681265282468206e-05
974,4758,0,4758,0.18215012550354004,2.6780934445928223e-05
977,4773,0,4773,0.1826491355895996,2.675013363214447e-05
980,4788,0,4788,0.18315696716308594,2.6720175178710732e-05
982,4798,0,4798,0.183488130569458,2.6700633697654127e-05
985,4813,0,4813,0.18398523330688477,2.6671914528579638e-05
988,4828,0,4828,0.18448305130004883,2.6643852328028098e-05
991,4843,0,4843,0.18497729301452637,2.661640131142021e-05
994,4858,0,4858,0.18548107147216797,2.658953269751347e-05
996,4868,0,4868,0.1858382225036621,2.65719347814311e-05
999,4883,0,4883,0.18634819984436035,2.654599888517732e-05
1002,4898,0,4898,0.18685698509216309,2.6520602862961714e-05
1005,4913,0,4913,0.1873641014099121,2.6495730299416528e-05
1007,4923,0,4923,0.18771719932556152,2.647943078641533e-05
1010,4938,0,4938,0.18828916549682617,2.6455391408869424e-05
1013,4953,0,4953,0.18880510330200195,2.6431827173218387e-05
1016,4968,0,4968,0.18930625915527344,2.6408718495113254e-05
1018,4977,0,4977,0.18963003158569336,2.6066785276559637e-05
1021,4992,0,4992,0.1901252269744873,2.5486742568781167e-05
1024,5007,0,5007,0.19064021110534668,2.5114446897001688e-05
1027,5022,0,5022,0.19113922119140625,2.4868600370874648e-05
1029,5032,0,5032,0.19147014617919922,2.474994341416943e-05
1032,5047,0,5047,0.19196701049804688,2.4616335070861864e-05
1035,5062,0,5062,0.19246530532836914,2.4518291408977313e-05
1038,5077,0,5077,0.19295907020568848,2.4443199716635536e-05
1040,5087,0,5087,0.19328904151916504,2.4401899986155708e-05
1043,5102,0,5102,0.19378900527954102,2.434915802222618e-05
1046,5117,0,5117,0.19428110122680664,2.43044131191147e-05
1049,5132,0,5132,0.1947951316833496,2.4265321420386894e-05
1051,5142,0,5142,0.1951301097869873,2.4241626468112216e-05
1054,5157,0,5157,0.1956491470336914,2.420881001108642e-05
1057,5172,0,5172,0.19613909721374512,2.4178574442405588e-05
1060,5187,0,5187,0.19662690162658691,2.4150351675500547e-05
1063,5202,0,5202,0.19711709022521973,2.4123736279301175e-05
1065,5212,0,5212,0.19744420051574707,2.410674250596266e-05
1068,5227,0,5227,0.19797706604003906,2.408222920511702e-05
1071,5242,0,5242,0.19849109649658203,2.4058762445613934e-05
1074,5257,0,5257,0.19906401634216309,2.4036231432366847e-05
1076,5267,0,5267,0.19939827919006348,2.4021681075540284e-05
1079,5282,0,5282,0.1998898983001709,2.4000485830639635e-05
1082,5297,0,5297,0.20037412643432617,2.397996045778909e-05
1085,5312,0,5312,0.20087814331054688,2.3960018929018486e-05
1087,5322,0,5322,0.20120716094970703,2.3947012093277185e-05
1090,5337,0,5337,0.20172500610351562,2.3927886504489185e-05
1093,5352,0,5352,0.20223212242126465,2.3909174012531328e-05
1096,5367,0,5367,0.20276093482971191,2.3890830762721643e-05
1098,5377,0,5377,0.20309209823608398,2.387879081100678e-05
1101,5392,0,5392,0.20359301567077637,2.3860996395854664e-05
1104,5407,0,5407,0.20409607887268066,2.384350442358929e-05
1107,5422,0,5422,0.20459389686584473,2.3826298713828807e-05
1109,5432,0,5432,0.20500707626342773,2.381497972869216e-05
1112,5447,0,5447,0.20552611351013184,2.3798217741200522e-05
1115,5462,0,5462,0.20603108406066895,2.378170431234835e-05
1118,5477,0,5477,0.20653533935546875,2.3765429186089707e-05
1120,5487,0,5487,0.20688104629516602,2.3754707382727457e-05
1123,5502,0,5502,0.2073831558227539,2.373881179494123e-05
1126,5517,0,5517,0.20789504051208496,2.3723134394221175e-05
1129,5532,0,5532,0.2083892822265625,2.3707667227836657e-05
1132,5547,0,5547,0.2089090347290039,2.3692400312984834e-05
1134,5557,0,5557,0.2092432975769043,2.3682327367234782e-05
1137,5572,0,5572,0.2097470760345459,2.3667364026544635e-05
1140,5586,0,5586,0.21023321151733398,2.360369239974509e-05
1143,5601,0,5601,0.21075201034545898,2.2950696132183255e-05
1145,5611,0,5611,0.21110200881958008,2.2671775713168907e-05
1148,5626,0,5626,0.21163392066955566,2.239000377233715e-05
1151,5640,0,5640,0.21216106414794922,2.091860634085116e-05
1154,5654,0,5654,0.21265411376953125,1.9454532864490458e-05
1156,5663,0,5663,0.2130732536315918,1.8995920043161296e-05
1159,5677,0,5677,0.2136859893798828,1.8446754406922826e-05
1162,5692,0,5692,0.21422529220581055,1.7937356027810035e-05
1165,5707,0,5707,0.21476316452026367,1.7621636584056884e-05
1167,5716,0,5716,0.21511602401733398,1.730157197880377e-05
1170,5731,0,5731,0.21575403213500977,1.6899213931133806e-05
1173,5746,0,5746,0.21636724472045898,1.6646298437831857e-05
1176,5761,0,5761,0.21713519096374512,1.6478828339235485e-05
1178,5771,0,5771,0.2175900936126709,1.639624715208663e-05
1181,5784,0,5784,0.21814513206481934,1.5540830658492847e-05
1184,5799,0,5799,0.2187483310699463,1.4933822385498646e-05
1187,5813,0,5813,0.2194070816040039,1.3682323059907663e-05
1189,5822,0,5822,0.2198331356048584,1.293718575380223e-05
1192,5837,0,5837,0.22040510177612305,1.2418189810934193e-05
1195,5852,0,5852,0.22095108032226562,1.21062898598503e-05
1198,5867,0,5867,0.22147297859191895,1.1906193827505775e-05
1200,5877,0,5877,0.22183918952941895,1.1809079994781039e-05
1203,5892,0,5892,0.2225341796875,1.1696351232025888e-05
1206,5907,0,5907,0.22340822219848633,1.1608922897635961e-05
1209,5921,0,5921,0.2240140438079834,1.0739177313455844e-05
1212,5933,0,5933,0.22465801239013672,9.367819130110531e-06
1214,5943,0,5943,0.2250208854675293,8.87575982742842e-06
1217,5957,0,5957,0.2255561351776123,8.174348257065711e-06
1220,5972,0,5972,0.22610712051391602,7.804618536566721e-06
1223,5987,0,5987,0.2269299030303955,7.562391177558796e-06
1225,5997,0,5997,0.22732806205749512,7.4423727032102495e-06
1228,6010,0,6010,0.22786521911621094,7.227316402314338e-06
1231,6025,0,6025,0.22841286659240723,6.714926670071287e-06
1234,6040,0,6040,0.22902822494506836,6.403745728914133e-06
1236,6049,0,6049,0.22937917709350586,6.065867706925964e-06
1239,6064,0,6064,0.22991704940795898,5.836689583325869e-06
1242,6078,0,6078,0.23043608665466309,5.369815191970872e-06
1245,6093,0,6093,0.23096823692321777,5.207950537039575e-06
1247,6103,0,6103,0.2313690185546875,5.1332999916009725e-06
1250,6118,0,6118,0.23208904266357422,5.050563351641869e-06
1253,6132,0,6132,0.2326960563659668,4.8786037704937195e-06
1256,6147,0,6147,0.23322510719299316,4.74772457536148e-06
1258,6157,0,6157,0.23357486724853516,4.691382281608048e-06
1261,6172,0,6172,0.23409795761108398,4.632510958881319e-06
1264,6186,0,6186,0.2347550392150879,4.541990350225188e-06
1267,6201,0,6201,0.23535704612731934,4.398096132484898e-06
1269,6211,0,6211,0.23572397232055664,4.3375240288753915e-06
1272,6226,0,6226,0.23624920845031738,4.276833954276136e-06
1275,6240,0,6240,0.23690009117126465,4.0565511998391445e-06
1278,6254,0,6254,0.23738908767700195,3.909044504854309e-06
1281,6269,0,6269,0.23798298835754395,3.7863016728727783e-06
1283,6279,0,6279,0.23842811584472656,3.733747293082147e-06
1286,6293,0,6293,0.23896408081054688,3.55788173519187e-06
1289,6308,0,6308,0.2395031452178955,3.4854026368160607e-06
1292,6322,0,6322,0.24008607864379883,3.332764230497222e-06
1294,6332,0,6332,0.2404332160949707,3.2679878603229918e-06
1297,6347,0,6347,0.24094009399414062,3.200046604697835e-06
1300,6361,0,6361,0.24143695831298828,3.084055513832537e-06
1303,6376,0,6376,0.24197721481323242,2.9762121344656536e-06
1305,6386,0,6386,0.24232029914855957,2.9293472196525147e-06
1308,6401,0,6401,0.24284911155700684,2.8810480380263296e-06
1311,6416,0,6416,0.24348115921020508,2.848650677813087e-06
1314,6431,0,6431,0.24405813217163086,2.825515003819563e-06
1316,6441,0,6441,0.24441814422607422,2.8133566206820866e-06
1319,6456,0,6456,0.24495911598205566,2.7983834964888803e-06
1322,6471,0,6471,0.24558806419372559,2.786149766740908e-06
1325,6486,0,6486,0.24625420570373535,2.775832357995845e-06
1327,6496,0,6496,0.24669408798217773,2.7697557384574726e-06
1330,6511,0,6511,0.2472381591796875,2.7615716638608936e-06
1333,6526,0,6526,0.24777817726135254,2.7542694851530705e-06
1336,6541,0,6541,0.2482900619506836,2.7476600806567245e-06
1338,6551,0,6551,0.24863004684448242,2.7435688675360953e-06
1341,6566,0,6566,0.24922800064086914,2.7378268414341918e-06
1344,6581,0,6581,0.24977993965148926,2.7324872839029086e-06
1347,6596,0,6596,0.25030517578125,2.7274862083249876e-06
1350,6611,0,6611,0.25083208084106445,2.722770326237086e-06
1352,6621,0,6621,0.2511758804321289,2.7197635210725546e-06
1355,6636,0,6636,0.2517051696777344,2.7154345896449282e-06
1358,6651,0,6651,0.25221824645996094,2.711301336472653e-06
1361,6666,0,6666,0.2527310848236084,2.7073452616810315e-06
1363,6676,0,6676,0.25307393074035645,2.704799064619757e-06
1366,6691,0,6691,0.25369811058044434,2.7011068543580946e-06
1369,6706,0,6706,0.25426197052001953,2.697555819575744e-06
1372,6721,0,6721,0.2549459934234619,2.6941335198392325e-06
1374,6731,0,6731,0.25542616844177246,2.6919178248855605e-06
1377,6746,0,6746,0.25597596168518066,2.6886852134865787e-06
1380,6761,0,6761,0.25649404525756836,2.6855530031216895e-06
1383,6776,0,6776,0.25701212882995605,2.6825122813111043e-06
1385,6786,0,6786,0.2573549747467041,2.680532026026334e-06
1388,6801,0,6801,0.257871150970459,2.6776267311060135e-06
1391,6816,0,6816,0.2583901882171631,2.674793964879876e-06
1394,6831,0,6831,0.2589089870452881,2.6720283521045454e-06
1396,6841,0,6841,0.25942206382751465,2.6702197185129234e-06
1399,6856,0,6856,0.26016712188720703,2.667556692117271e-06
1402,6871,0,6871,0.2609071731567383,2.6649507534873763e-06
1405,6886,0,6886,0.2614731788635254,2.662399051781628e-06
1407,6896,0,6896,0.26180505752563477,2.660726763053682e-06
1410,6911,0,6911,0.2623002529144287,2.658259859108976e-06
1413,6926,0,6926,0.2628202438354492,2.6558409451789093e-06
1416,6941,0,6941,0.26333117485046387,2.6534682140728577e-06
1419,6956,0,6956,0.26384687423706055,2.6511401071389585e-06
1421,6966,0,6966,0.2641761302947998,2.6496121401442438e-06
1424,6980,0,6980,0.264660120010376,2.5875773480749696e-06
1427,6995,0,6995,0.2651660442352295,2.5541930994306583e-06
1430,7010,0,7010,0.26566505432128906,2.535035950216586e-06
1432,7020,0,7020,0.26599597930908203,2.5266874549896376e-06
1435,7035,0,7035,0.26657795906066895,2.517992542086424e-06
1438,7050,0,7050,0.26709818840026855,2.51197890441103e-06
1441,7065,0,7065,0.26761913299560547,2.5074567159187727e-06
1443,7075,0,7075,0.2679469585418701,2.5049497090150837e-06
1446,7090,0,7090,0.26843905448913574,2.501680603717086e-06
1449,7105,0,7105,0.26892900466918945,2.4988055693463373e-06
1452,7120,0,7120,0.2694251537322998,2.4961945620156454e-06
1454,7130,0,7130,0.26975107192993164,2.494562713700712e-06
1457,7145,0,7145,0.27024316787719727,2.492242542892562e-06
1460,7160,0,7160,0.27074313163757324,2.4900436769134085e-06
1463,7175,0,7175,0.2712230682373047,2.487943137534847e-06
1465,7185,0,7185,0.27153992652893066,2.486590041500796e-06
1468,7200,0,7200,0.27204203605651855,2.484622160256594e-06
1471,7215,0,7215,0.27253198623657227,2.482717870221401e-06
1474,7230,0,7230,0.2730412483215332,2.480868038594415e-06
1476,7240,0,7240,0.27338290214538574,2.479662012332434e-06
1479,7255,0,7255,0.2738771438598633,2.4778902388718413e-06
1482,7270,0,7270,0.274367094039917,2.4761603814386782e-06
1485,7285,0,7285,0.2748579978942871,2.474469714802195e-06
1488,7300,0,7300,0.27543091773986816,2.472815425290708e-06
1490,7310,0,7310,0.27579498291015625,2.471731143657675e-06
1493,7325,0,7325,0.2763810157775879,2.4701299211508768e-06
1496,7340,0,7340,0.276885986328125,2.4685557546912557e-06
1499,7355,0,7355,0.2773780822753906,2.467005112061121e-06
1501,7365,0,7365,0.2777259349822998,2.465982805701526e-06
1504,7380,0,7380,0.27823686599731445,2.4644645667696225e-06
1507,7395,0,7395,0.278764009475708,2.4629629791726736e-06
1510,7410,0,7410,0.2792961597442627,2.461477033108419e-06
1512,7420,0,7420,0.2796480655670166,2.4604948564909733e-06
1515,7435,0,7435,0.28017616271972656,2.4590340447750368e-06
1518,7450,0,7450,0.28070497512817383,2.4575877623670133e-06
1521,7465,0,7465,0.2812340259552002,2.4561552657092195e-06
1523,7474,0,7474,0.2815732955932617,2.365294737299574e-06
1526,7489,0,7489,0.28209996223449707,2.3370566017095867e-06
1529,7503,0,7503,0.2826361656188965,2.301593800199192e-06
1532,7517,0,7517,0.2831540107727051,2.155350315394666e-06
1534,7526,0,7526,0.28348708152770996,2.0217226014655007e-06
1537,7540,0,7540,0.2840290069580078,1.8856186458565675e-06
1540,7554,0,7554,0.2845580577850342,1.7585380570023783e-06
1543,7567,0,7567,0.28506922721862793,1.6088711448180783e-06
1545,7576,0,7576,0.2854180335998535,1.4506853157722665e-06
1548,7591,0,7591,0.28597307205200195,1.3783156199846519e-06
1551,7604,0,7604,0.28647708892822266,1.2677989582658838e-06
1554,7619,0,7619,0.2870190143585205,1.211423523901795e-06
1557,7634,0,7634,0.2875509262084961,1.1748658080994442e-06
1559,7644,0,7644,0.28791308403015137,1.157184881247898e-06
1562,7659,0,7659,0.28844594955444336,1.136952819519226e-06
1565,7673,0,7673,0.28895998001098633,1.0810180266804684e-06
1568,7687,0,7687,0.2894761562347412,1.0387579905495046e-06
1570,7697,0,7697,0.2898261547088623,1.0071745192261407e-06
1573,7711,0,7711,0.29033923149108887,9.365621526162807e-07
1576,7726,0,7726,0.2908651828765869,9.114518863847938e-07
1579,7739,0,7739,0.29137301445007324,8.817974357476358e-07
1581,7749,0,7749,0.29172420501708984,8.451743249190282e-07
1584,7763,0,7763,0.2922370433807373,7.908873005083428e-07
1587,7778,0,7778,0.2927720546722412,7.643083082059342e-07
1590,7790,0,7790,0.2932569980621338,7.241382598194564e-07
1592,7800,0,7800,0.2936272621154785,6.968844915145934e-07
1595,7814,0,7814,0.2941560745239258,6.406349371428517e-07
1598,7829,0,7829,0.29470014572143555,6.069295930738345e-07
1601,7843,0,7843,0.2952260971069336,5.855593056319066e-07
1603,7853,0,7853,0.2955892086029053,5.635845660583538e-07
1606,7868,0,7868,0.2961452007293701,5.406935608633478e-07
1609,7881,0,7881,0.2966599464416504,4.7570021930097125e-07
1612,7895,0,7895,0.29718923568725586,4.466822404465061e-07
1614,7905,0,7905,0.2975490093231201,4.3200051560295126e-07
1617,7920,0,7920,0.2980940341949463,4.1666486009349335e-07
1620,7934,0,7934,0.29863810539245605,3.862115809222853e-07
1623,7949,0,7949,0.29917311668395996,3.749186875921931e-07
1625,7959,0,7959,0.2995278835296631,3.695942851358647e-07
1628,7973,0,7973,0.30004215240478516,3.445740207570767e-07
1631,7988,0,7988,0.30059218406677246,3.368327921620668e-07
1634,8002,0,8002,0.30112314224243164,3.211379937928808e-07
1637,8016,0,8016,0.3016550540924072,3.00444764427055e-07
1639,8026,0,8026,0.3020191192626953,2.9433450563544893e-07
1642,8041,0,8041,0.3025641441345215,2.8761056925697303e-07
1645,8056,0,8056,0.30311012268066406,2.8264890164228236e-07
1648,8071,0,8071,0.30364012718200684,2.787252317626068e-07
1650,8081,0,8081,0.30399417877197266,2.764897973650421e-07
1653,8094,0,8094,0.30449509620666504,2.589048349747493e-07
1656,8109,0,8109,0.3050539493560791,2.472809025186362e-07
1659,8124,0,8124,0.3056020736694336,2.405587119630202e-07
1661,8134,0,8134,0.3059682846069336,2.375439817306853e-07
1664,8149,0,8149,0.3065159320831299,2.3424132006756656e-07
1667,8163,0,8163,0.3070511817932129,2.2658136697854052e-07
1670,8178,0,8178,0.30759716033935547,2.205810962843325e-07
1672,8188,0,8188,0.30796003341674805,2.178916801516139e-07
1675,8203,0,8203,0.30850815773010254,2.150099873239416e-07
1678,8218,0,8218,0.309053897857666,2.1296900057017473e-07
1681,8233,0,8233,0.3096120357513428,2.1142757288396532e-07
1683,8243,0,8243,0.30997610092163086,2.105824799641614e-07
1686,8258,0,8258,0.31052112579345703,2.095042480815516e-07
1689,8273,0,8273,0.3110690116882324,2.0859291121511745e-07
1692,8288,0,8288,0.3116140365600586,2.0780429391436728e-07
1694,8298,0,8298,0.31197690963745117,2.0733246554998602e-07
1697,8313,0,8313,0.31252098083496094,2.066909523170197e-07
1700,8328,0,8328,0.3130650520324707,2.0611576422667097e-07
1703,8343,0,8343,0.31361889839172363,2.05595880812514e-07
1706,8358,0,8358,0.3141360282897949,2.0512246916714944e-07
1708,8368,0,8368,0.31447815895080566,2.0482920917259011e-07
1711,8383,0,8383,0.3150179386138916,2.0441877401233036e-07
1714,8398,0,8398,0.31554317474365234,2.0403970161921647e-07
1717,8413,0,8413,0.3160691261291504,2.036882454320115e-07
1719,8423,0,8423,0.316425085067749,2.0346773195244446e-07
1722,8438,0,8438,0.31695103645324707,2.0315575312684168e-07
1725,8453,0,8453,0.3174741268157959,2.0286438522402698e-07
1728,8468,0,8468,0.31800007820129395,2.025916069627767e-07
1730,8478,0,8478,0.31834912300109863,2.0241913551981162e-07
1733,8493,0,8493,0.31888628005981445,2.0217313619263958e-07
1736,8508,0,8508,0.319411039352417,2.0194086555091704e-07
1739,8523,0,8523,0.3199450969696045,2.0172069965744723e-07
1741,8533,0,8533,0.320296049118042,2.015798980484293e-07
1744,8548,0,8548,0.3208472728729248,2.013766673059753e-07
1747,8563,0,8563,0.32140493392944336,2.011820399390155e-07
1750,8578,0,8578,0.32195115089416504,2.009952446799885e-07
1752,8588,0,8588,0.3223130702972412,2.0087480841937712e-07
1755,8603,0,8603,0.32285594940185547,2.0069999705599796e-07
1758,8618,0,8618,0.32340192794799805,2.0053183359116154e-07
1761,8633,0,8633,0.3239428997039795,2.0036984044734644e-07
1763,8643,0,8643,0.32430601119995117,2.0026500261758062e-07
1766,8658,0,8658,0.32485008239746094,2.0011204420996341e-07
1769,8673,0,8673,0.3253939151763916,1.9996371269170867e-07
1772,8688,0,8688,0.3259410858154297,1.998194383917363e-07
1775,8703,0,8703,0.32645726203918457,1.9967871472938914e-07
1777,8712,0,8712,0.3268101215362549,1.9618488660504944e-07
1780,8727,0,8727,0.32734203338623047,1.940914046497025e-07
1783,8742,0,8742,0.3278791904449463,1.928820289633566e-07
1786,8757,0,8757,0.3284111022949219,1.9210858946857104e-07
1788,8766,0,8766,0.3287510871887207,1.8264502389573785e-07
1791,8780,0,8780,0.32927632331848145,1.7172140541568078e-07
1794,8793,0,8793,0.32976508140563965,1.6281623685250698e-07
1797,8806,0,8806,0.33025622367858887,1.409479343077729e-07
1799,8815,0,8815,0.3305931091308594,1.2597720854392425e-07
1802,8830,0,8830,0.3311161994934082,1.1590473804700262e-07
1805,8844,0,8844,0.33162498474121094,1.0446801016866022e-07
1808,8857,0,8857,0.33213210105895996,9.655110907394189e-08
1810,8866,0,8866,0.33246707916259766,9.025142100903125e-08
1813,8881,0,8881,0.3330521583557129,8.462339598941031e-08
1816,8895,0,8895,0.33361101150512695,8.035582729783978e-08
1819,8909,0,8909,0.3341529369354248,7.587679362721931e-08
1821,8919,0,8919,0.3345170021057129,7.362580020392493e-08
1824,8933,0,8933,0.33504724502563477,6.808799968232382e-08
1827,8947,0,8947,0.3355591297149658,6.427227856540295e-08
1830,8962,0,8962,0.3360869884490967,6.216457154865567e-08
1832,8972,0,8972,0.3364369869232178,6.115572400885286e-08
1835,8987,0,8987,0.3369762897491455,6.000083496571296e-08
1838,9002,0,9002,0.33750295639038086,5.9116329630256266e-08
1841,9017,0,9017,0.3380601406097412,5.839728255582356e-08
1844,9030,0,9030,0.3385632038116455,5.539048887028729e-08
1846,9040,0,9040,0.33890819549560547,5.319163436277037e-08
1849,9054,0,9054,0.33941006660461426,4.930200825222037e-08
1852,9068,0,9068,0.33991122245788574,4.505976433244823e-08
1855,9082,0,9082,0.34041500091552734,4.2842693542097526e-08
1857,9092,0,9092,0.34077906608581543,4.169370395121293e-08
1860,9107,0,9107,0.34131717681884766,4.055209696675106e-08
1863,9122,0,9122,0.3418450355529785,3.9806160781881566e-08
1866,9135,0,9135,0.3423440456390381,3.714154313862991e-08
1868,9144,0,9144,0.3426802158355713,3.586465989394687e-08
1871,9159,0,9159,0.34320807456970215,3.4308025561017155e-08
1874,9174,0,9174,0.3437371253967285,3.330340345494854e-08
1877,9189,0,9189,0.3442649841308594,3.261870203936447e-08
1879,9198,0,9198,0.34460020065307617,3.099179535356986e-08
1882,9213,0,9213,0.3451261520385742,3.0093552206720244e-08
1885,9228,0,9228,0.34566307067871094,2.948290428774711e-08
1888,9243,0,9243,0.3461933135986328,2.9042807899759837e-08
1890,9252,0,9252,0.3465311527252197,2.7260395878054802e-08
1893,9265,0,9265,0.34702515602111816,2.4800864385637803e-08
1896,9280,0,9280,0.3475489616394043,2.297537955170156e-08
1899,9294,0,9294,0.34806299209594727,2.1609841117307712e-08
1901,9304,0,9304,0.34841299057006836,2.097774165468364e-08
1904,9319,0,9319,0.3489420413970947,2.038640390842626e-08
1907,9334,0,9334,0.34946608543395996,2.003616097280622e-08
1910,9349,0,9349,0.3500070571899414,1.9812302021227525e-08
1913,9364,0,9364,0.35054898262023926,1.9656648569126002e-08
1915,9374,0,9374,0.3509082794189453,1.9575561891699236e-08
1918,9389,0,9389,0.3514530658721924,1.9475392055780312e-08
1921,9404,0,9404,0.35199618339538574,1.9392641393045845e-08
1924,9418,0,9418,0.3525052070617676,1.8838112446948954e-08
1926,9428,0,9428,0.3528561592102051,1.852445203902256e-08
1929,9442,0,9442,0.3533670902252197,1.771375487713998e-08
1932,9457,0,9457,0.3538932800292969,1.742708759207402e-08
1935,9472,0,9472,0.35442304611206055,1.7257891959607907e-08
1937,9482,0,9482,0.3548281192779541,1.7181235408881338e-08
1940,9497,0,9497,0.3553750514984131,1.7097883439139627e-08
1943,9512,0,9512,0.35595011711120605,1.70373873436917e-08
1946,9527,0,9527,0.35648012161254883,1.6990384324263504e-08
1948,9537,0,9537,0.35683512687683105,1.6964032421793135e-08
1951,9552,0,9552,0.35747623443603516,1.69296260791417e-08
1954,9567,0,9567,0.3580300807952881,1.6899657624674903e-08
1957,9582,0,9582,0.35858607292175293,1.6872907545530327e-08
1959,9592,0,9592,0.35893917083740234,1.685644636981152e-08
1962,9607,0,9607,0.35947489738464355,1.683342913872355e-08
1965,9622,0,9622,0.3600001335144043,1.6812064132909067e-08
1968,9637,0,9637,0.3605220317840576,1.6792040758593045e-08
1970,9647,0,9647,0.3608710765838623,1.6779322010352414e-08
1973,9662,0,9662,0.36139488220214844,1.676103946500058e-08
1976,9677,0,9677,0.36191701889038086,1.6743572564045907e-08
1979,9692,0,9692,0.3624420166015625,1.6726792108561862e-08
1982,9707,0,9707,0.3629581928253174,1.6710597410348718e-08
1984,9717,0,9717,0.36329126358032227,1.6700085442855786e-08
1987,9732,0,9732,0.3638150691986084,1.6684694474117155e-08
1990,9747,0,9747,0.3643321990966797,1.6669715972159157e-08
1993,9762,0,9762,0.36484193801879883,1.665511657542947e-08
1995,9772,0,9772,0.36518025398254395,1.6645581484989312e-08
1998,9787,0,9787,0.36568713188171387,1.6631553058445875e-08
2001,9802,0,9802,0.3662281036376953,1.6617819664473662e-08
2004,9817,0,9817,0.36673521995544434,1.660433894975015e-08
2006,9827,0,9827,0.3671150207519531,1.659547191801201e-08
2009,9842,0,9842,0.36762213706970215,1.658232744625533e-08
2012,9857,0,9857,0.3681371212005615,1.656934834192298e-08
2015,9872,0,9872,0.36903810501098633,1.655651623242577e-08
2017,9882,0,9882,0.3695220947265625,1.6548036116226342e-08
2020,9897,0,9897,0.3701629638671875,1.6535419171668465e-08
2023,9912,0,9912,0.3709421157836914,1.6522917769190396e-08
2026,9927,0,9927,0.371751070022583,1.6510523871246643e-08
2028,9937,0,9937,0.3722350597381592,1.6502317367021553e-08
2031,9952,0,9952,0.3730580806732178,1.649008649514873e-08
2034,9967,0,9967,0.37410998344421387,1.6477944135283423e-08
2037,9982,0,9982,0.3749251365661621,1.6465884188087242e-08
2039,9991,0,9991,0.3755199909210205,1.6412587381851952e-08
2042,10006,0,10006,0.3763699531555176,1.6290512459858528e-08
2045,10021,0,10021,0.37724804878234863,1.621935130111196e-08
2048,10036,0,10036,0.37809109687805176,1.6174301230293025e-08
2051,10051,0,10051,0.3791213035583496,1.6143089577953214e-08
2053,10061,0,10061,0.37967610359191895,1.612673435696325e-08
2056,10076,0,10076,0.38027119636535645,1.6106192557470387e-08
2059,10091,0,10091,0.3808262348175049,1.608866371793412e-08
2062,10106,0,10106,0.3813660144805908,1.6072951659548715e-08
2064,10116,0,10116,0.3817911148071289,1.6063156761092564e-08
2067,10131,0,10131,0.38237690925598145,1.6049167256570386e-08
2070,10146,0,10146,0.38292813301086426,1.6035797523954656e-08
2073,10161,0,10161,0.3834550380706787,1.6022888676760145e-08
2075,10171,0,10171,0.38381528854370117,1.6014476364851885e-08
2078,10186,0,10186,0.3843240737915039,1.6002103168210092e-08
2081,10201,0,10201,0.3848581314086914,1.5989973334887265e-08
2084,10216,0,10216,0.3853881359100342,1.597804538143473e-08
2086,10226,0,10226,0.38573527336120605,1.5970195370986e-08
2089,10241,0,10241,0.38626718521118164,1.595854737417193e-08
2092,10256,0,10256,0.38680195808410645,1.5947038253339007e-08
2095,10271,0,10271,0.387404203414917,1.593565244629328e-08
2097,10281,0,10281,0.3877832889556885,1.5928125796556165e-08
2100,10296,0,10296,0.388322114944458,1.5916933667910425e-08
2103,10311,0,10311,0.3888521194458008,1.5905858825808854e-08
2106,10326,0,10326,0.3893849849700928,1.589490445833459e-08
2108,10336,0,10336,0.38976001739501953,1.588766792560338e-08
2111,10351,0,10351,0.3903040885925293,1.587691020327668e-08
2114,10366,0,10366,0.3908541202545166,1.5866263762621322e-08
2117,10381,0,10381,0.39139723777770996,1.5855719919750517e-08
2119,10391,0,10391,0.39178013801574707,1.5848742892762832e-08
2122,10406,0,10406,0.39233899116516113,1.583834661373175e-08
2125,10421,0,10421,0.39290404319763184,1.582802307355258e-08
2128,10436,0,10436,0.3934462070465088,1.5817761407191452e-08
2131,10451,0,10451,0.39403319358825684,1.5807552949593554e-08
2133,10461,0,10461,0.39455509185791016,1.580077399051287e-08
2136,10476,0,10476,0.3954041004180908,1.5790642743901783e-08
2139,10491,0,10491,0.39608311653137207,1.578055433398382e-08
2142,10506,0,10506,0.39675211906433105,1.5770507768145438e-08
2144,10516,0,10516,0.3971900939941406,1.576383321035503e-08
2147,10531,0,10531,0.39788317680358887,1.5753856631369505e-08
2150,10546,0,10546,0.39856410026550293,1.5743923565809794e-08
2153,10561,0,10561,0.3995802402496338,1.5734035833557267e-08
2155,10571,0,10571,0.4000132083892822,1.5727470046486426e-08
2158,10586,0,10586,0.4005711078643799,1.571766106552973e-08
2161,10601,0,10601,0.4011352062225342,1.5707899270273356e-08
2164,10616,0,10616,0.4017021656036377,1.5698182362675736e-08
2166,10626,0,10626,0.4020988941192627,1.5691727404032292e-08
2169,10641,0,10641,0.40269899368286133,1.5682075542886043e-08
2172,10656,0,10656,0.40326929092407227,1.5672455281827832e-08
2175,10671,0,10671,0.4039900302886963,1.5662861258870307e-08
2177,10681,0,10681,0.40442490577697754,1.5656477703418387e-08
2180,10696,0,10696,0.4050130844116211,1.5646919093850514e-08
2183,10711,0,10711,0.40569615364074707,1.5637379759416416e-08
2186,10726,0,10726,0.406278133392334,1.5627860360337763e-08
2188,10736,0,10736,0.40667223930358887,1.5621526014126872e-08
2191,10751,0,10751,0.4072442054748535,1.5612043915048417e-08
2194,10766,0,10766,0.40780115127563477,1.5602586702760675e-08
2197,10781,0,10781,0.4084789752960205,1.5593155449022405e-08
2200,10796,0,10796,0.4092390537261963,1.558375032201824e-08
2202,10806,0,10806,0.40961313247680664,1.557749453011569e-08
2205,10821,0,10821,0.41017603874206543,1.5568131757044223e-08
2208,10836,0,10836,0.4107639789581299,1.5558793599921895e-08
2211,10850,0,10850,0.4113149642944336,1.526535353822427e-08
2213,10860,0,10860,0.41167521476745605,1.5162176132422967e-08
2216,10875,0,10875,0.4122319221496582,1.5072208351013462e-08
2219,10890,0,10890,0.41298723220825195,1.5023078877337182e-08
2222,10905,0,10905,0.4136021137237549,1.499357073461855e-08
2224,10915,0,10915,0.41402125358581543,1.497964906281329e-08
2227,10930,0,10930,0.4145650863647461,1.4963356036743708e-08
2230,10944,0,10944,0.4150850772857666,1.464584982614754e-08
2233,10959,0,10959,0.41562318801879883,1.4549957328876965e-08
2235,10969,0,10969,0.41597604751586914,1.4505429590381275e-08
2238,10984,0,10984,0.41651201248168945,1.4456305659635585e-08
2241,10999,0,10999,0.4170980453491211,1.4420142477128335e-08
2244,11014,0,11014,0.41768908500671387,1.4391793134172084e-08
2246,11024,0,11024,0.4181530475616455,1.4375732172359353e-08
2249,11039,0,11039,0.4187352657318115,1.4354445848311717e-08
2252,11054,0,11054,0.4192819595336914,1.4335524401056583e-08
2255,11069,0,11069,0.4200022220611572,1.4318224212048567e-08
2257,11079,0,11079,0.42058706283569336,1.4307380636677065e-08
2260,11094,0,11094,0.4214811325073242,1.429192238354577e-08
2263,11109,0,11109,0.4223520755767822,1.427726747721741e-08
2266,11124,0,11124,0.4230351448059082,1.4263277468422398e-08
2269,11139,0,11139,0.4236581325531006,1.424982833821754e-08
2271,11149,0,11149,0.4241631031036377,1.4241114051779284e-08
2274,11164,0,11164,0.424868106842041,1.4228349784860817e-08
2277,11179,0,11179,0.425584077835083,1.421589344319854e-08
2280,11194,0,11194,0.4261939525604248,1.4203693802857495e-08
2282,11204,0,11204,0.4266800880432129,1.4195683372628304e-08
2285,11219,0,11219,0.4275178909301758,1.4183838302883063e-08
2288,11234,0,11234,0.4282529354095459,1.4172181868734036e-08
2291,11249,0,11249,0.42909693717956543,1.4160699889767743e-08
2293,11259,0,11259,0.4296700954437256,1.4153134840758209e-08
2296,11274,0,11274,0.43049120903015137,1.4141906092640723e-08
2299,11289,0,11289,0.4311821460723877,1.4130801515450517e-08
2302,11304,0,11304,0.43186306953430176,1.4119799128415522e-08
2304,11314,0,11314,0.43224191665649414,1.4112513083899246e-08
2307,11329,0,11329,0.43285107612609863,1.4101651738110806e-08
2310,11344,0,11344,0.433427095413208,1.4090871368385995e-08
2313,11359,0,11359,0.43396520614624023,1.4080175631611373e-08
2315,11369,0,11369,0.43431711196899414,1.407309331304796e-08
2318,11384,0,11384,0.43485212326049805,1.4062541020944171e-08
2321,11399,0,11399,0.4353799819946289,1.4052067800695415e-08
2324,11413,0,11413,0.4358952045440674,1.3738035157306085e-08
2326,11423,0,11423,0.4362492561340332,1.3703284990979096e-08
2329,11438,0,11438,0.43677592277526855,1.3666969307788606e-08
2332,11453,0,11453,0.4373040199279785,1.3641618931341367e-08
2335,11468,0,11468,0.43785715103149414,1.3622358543574311e-08
2338,11483,0,11483,0.43851494789123535,1.3606635044770476e-08
2340,11493,0,11493,0.43889617919921875,1.3597372155124794e-08
2343,11508,0,11508,0.43944597244262695,1.3584708703093371e-08
2346,11523,0,11523,0.4399881362915039,1.3573048170528368e-08
2349,11538,0,11538,0.44057607650756836,1.3562076911759877e-08
2351,11548,0,11548,0.4409310817718506,1.3555058471514826e-08
2354,11563,0,11563,0.4414541721343994,1.3544867496324308e-08
2357,11578,0,11578,0.44197607040405273,1.3535011910133828e-08
2360,11593,0,11593,0.44249916076660156,1.3525423588900518e-08
2362,11603,0,11603,0.44284796714782715,1.3519150225969387e-08
2365,11618,0,11618,0.44336891174316406,1.350989189621738e-08
2368,11633,0,11633,0.44388818740844727,1.3500781710172063e-08
2371,11648,0,11648,0.4444139003753662,1.3491797199139283e-08
2373,11658,0,11658,0.4447810649871826,1.3485869798635184e-08
2376,11673,0,11673,0.4453110694885254,1.3477064933272303e-08
2379,11688,0,11688,0.44585108757019043,1.3468362014213292e-08
2382,11703,0,11703,0.4463770389556885,1.3459758845291985e-08
2384,11713,0,11713,0.44672203063964844,1.3454077965125577e-08
2387,11728,0,11728,0.4472391605377197,1.3445633990177339e-08
2390,11743,0,11743,0.4477660655975342,1.3437274916713406e-08
2393,11758,0,11758,0.4482691287994385,1.3428989916594936e-08
2395,11768,0,11768,0.44863414764404297,1.3423502084758148e-08
2398,11783,0,11783,0.44973111152648926,1.3415317386322823e-08
2401,11798,0,11798,0.4508180618286133,1.3407183630277758e-08
2404,11813,0,11813,0.451876163482666,1.3399097061475172e-08
2407,11828,0,11828,0.45247626304626465,1.3391054989374389e-08
2409,11838,0,11838,0.45296216011047363,1.3385716734789305e-08
2412,11853,0,11853,0.45381712913513184,1.3377741471402824e-08
2415,11867,0,11867,0.4545552730560303,1.3182110387603094e-08
2418,11882,0,11882,0.45547008514404297,1.308192614929276e-08
2420,11892,0,11892,0.456118106842041,1.3039115605003103e-08
2423,11907,0,11907,0.4569740295410156,1.2995308780502687e-08
2426,11922,0,11922,0.4577779769897461,1.296563869474951e-08
2429,11937,0,11937,0.4586312770843506,1.2943719184953953e-08
2431,11947,0,11947,0.45919108390808105,1.2931707817093523e-08
2434,11962,0,11962,0.460064172744751,1.2916117542729132e-08
2437,11977,0,11977,0.4606201648712158,1.2902411473338783e-08
2440,11992,0,11992,0.4611551761627197,1.288992371709451e-08
2442,12002,0,12002,0.4615061283111572,1.2882080942191163e-08
2445,12017,0,12017,0.46204113960266113,1.2870845270237794e-08
2448,12032,0,12032,0.462583065032959,1.2860092820115589e-08
2451,12047,0,12047,0.46312499046325684,1.2849709407316408e-08
2453,12057,0,12057,0.4634859561920166,1.2842953302795337e-08
2456,12072,0,12072,0.46402406692504883,1.2833033368196003e-08
2459,12087,0,12087,0.4646131992340088,1.2823341608757687e-08
2462,12102,0,12102,0.46520018577575684,1.2813862767788537e-08
2464,12112,0,12112,0.4655799865722656,1.2807655565881246e-08
2467,12127,0,12127,0.46611523628234863,1.2798503948107474e-08
2470,12142,0,12142,0.46665406227111816,1.278953026632331e-08
2473,12157,0,12157,0.4675741195678711,1.2780719018068833e-08
2476,12172,0,12172,0.4685981273651123,1.2772053558780151e-08
2478,12182,0,12182,0.46927690505981445,1.2766348999969079e-08
2481,12197,0,12197,0.47034406661987305,1.2757889118146377e-08
2484,12212,0,12212,0.47144007682800293,1.2749533804985142e-08
2487,12227,0,12227,0.4724850654602051,1.2741273629175323e-08
2489,12237,0,12237,0.47303199768066406,1.2735816795624168e-08
2492,12252,0,12252,0.4740889072418213,1.2727703770918187e-08
2495,12267,0,12267,0.47518205642700195,1.2719674783546974e-08
2498,12282,0,12282,0.4759361743927002,1.2711726086609146e-08
2500,12292,0,12292,0.4763169288635254,1.270646928789056e-08
2503,12307,0,12307,0.4768829345703125,1.2698643883929764e-08
2506,12322,0,12322,0.47742319107055664,1.2690886139468926e-08
2509,12337,0,12337,0.47808098793029785,1.2683192177211242e-08
2511,12347,0,12347,0.47844624519348145,1.2678096703245207e-08
2514,12362,0,12362,0.47898006439208984,1.2670502079047005e-08
2517,12377,0,12377,0.47951626777648926,1.2662963018826459e-08
2520,12392,0,12392,0.4800550937652588,1.2655476155941587e-08
2522,12402,0,12402,0.48041820526123047,1.2650512261661011e-08
2525,12417,0,12417,0.48104310035705566,1.264310540946287e-08
2528,12432,0,12432,0.48186230659484863,1.2635743942017217e-08
2531,12447,0,12447,0.4825270175933838,1.2628427467361792e-08
2533,12457,0,12457,0.48289012908935547,1.262357501071453e-08
2536,12472,0,12472,0.4834320545196533,1.2616334424828416e-08
2539,12487,0,12487,0.4839742183685303,1.2609139324436626e-08
2542,12502,0,12502,0.4845161437988281,1.2601988413015328e-08
2544,12512,0,12512,0.48488306999206543,1.2597244556459097e-08
2547,12526,0,12526,0.4854001998901367,1.190076571131842e-08
2550,12541,0,12541,0.48595404624938965,1.1714081577272082e-08
2553,12556,0,12556,0.486497163772583,1.159445350509966e-08
2556,12571,0,12571,0.48703789710998535,1.1512623494480643e-08
2558,12581,0,12581,0.48738718032836914,1.1471055108371804e-08
2561,12596,0,12596,0.4879722595214844,1.1421419981625326e-08
2564,12611,0,12611,0.48853516578674316,1.1382223615730718e-08
2567,12626,0,12626,0.4890601634979248,1.1350084445534434e-08
2569,12636,0,12636,0.4894070625305176,1.1331487380405223e-08
2572,12651,0,12651,0.48993515968322754,1.1306795244119044e-08
2575,12666,0,12666,0.4904608726501465,1.1285096167202815e-08
2578,12681,0,12681,0.4909839630126953,1.1265702728679248e-08
2580,12691,0,12691,0.4913301467895508,1.1253817251480656e-08
2583,12706,0,12706,0.491879940032959,1.1237272204436978e-08
2586,12721,0,12721,0.4924123287200928,1.1222013015443201e-08
2589,12736,0,12736,0.49294590950012207,1.120779888759389e-08
2591,12746,0,12746,0.4933052062988281,1.119879984252299e-08
2594,12761,0,12761,0.493847131729126,1.1185895969130038e-08
2597,12776,0,12776,0.4943842887878418,1.1173600725299974e-08
2600,12791,0,12791,0.49493408203125,1.1161827083833318e-08
2602,12801,0,12801,0.49530506134033203,1.1154236111589346e-08
2605,12816,0,12816,0.49584412574768066,1.1143198196328444e-08
2608,12831,0,12831,0.4963819980621338,1.1132539067374412e-08
2611,12846,0,12846,0.4969191551208496,1.1122216052374899e-08
2613,12856,0,12856,0.49727511405944824,1.1115501113258914e-08
2616,12871,0,12871,0.4978141784667969,1.1105651997091809e-08
2619,12886,0,12886,0.4983501434326172,1.109604078130264e-08
2622,12901,0,12901,0.4988832473754883,1.1086639669868788e-08
2625,12916,0,12916,0.4994041919708252,1.1077430583401763e-08
2627,12926,0,12926,0.4998021125793457,1.107139323954439e-08
2630,12941,0,12941,0.5003483295440674,1.1062487048713991e-08
2633,12956,0,12956,0.500885009765625,1.105375600794403e-08
2636,12971,0,12971,0.5014200210571289,1.104519087652998e-08
2638,12981,0,12981,0.501777172088623,1.1039565765493986e-08
2641,12996,0,12996,0.5023109912872314,1.1031241952816138e-08
2644,13010,0,13010,0.5028290748596191,1.0999897894240138e-08
2647,13025,0,13025,0.5039370059967041,1.0938282112619736e-08
2649,13035,0,13035,0.5043749809265137,1.0911878084319813e-08
2652,13050,0,13050,0.5049259662628174,1.0884523472348469e-08
2655,13065,0,13065,0.5054771900177002,1.0865527495988633e-08
2658,13080,0,13080,0.5061841011047363,1.0851159943762737e-08
2660,13090,0,13090,0.5067341327667236,1.0843126552889593e-08
2663,13105,0,13105,0.5073580741882324,1.0832526641687128e-08
2666,13120,0,13120,0.5079700946807861,1.0823071696995068e-08
2669,13135,0,13135,0.5086252689361572,1.0814384727931001e-08
2671,13145,0,13145,0.5090723037719727,1.0808911743239023e-08
2674,13160,0,13160,0.5097780227661133,1.0801073579843694e-08
2677,13175,0,13175,0.5104250907897949,1.079359844390247e-08
2680,13190,0,13190,0.5110621452331543,1.078640926771569e-08
2682,13200,0,13200,0.5114302635192871,1.0781739552052102e-08
2685,13215,0,13215,0.5119800567626953,1.0774883633914322e-08
2688,13230,0,13230,0.5125088691711426,1.076816424124393e-08
2691,13245,0,13245,0.5130372047424316,1.076155315569606e-08
2694,13260,0,13260,0.51357102394104,1.0755034594845142e-08
2696,13270,0,13270,0.5139250755310059,1.0750735640946734e-08
2699,13285,0,13285,0.5147171020507812,1.0744357313842805e-08
2702,13300,0,13300,0.5154850482940674,1.0738058252854611e-08
2705,13315,0,13315,0.5161871910095215,1.073183113286705e-08
2707,13325,0,13325,0.5165722370147705,1.0727714579982125e-08
2710,13340,0,13340,0.5171880722045898,1.0721582859815896e-08
2713,13355,0,13355,0.5179860591888428,1.071549495450761e-08
2716,13370,0,13370,0.5188751220703125,1.0709444556906212e-08
2718,13380,0,13380,0.5195791721343994,1.0705430686522191e-08
2721,13395,0,13395,0.5204942226409912,1.069943916137414e-08
2724,13410,0,13410,0.5213272571563721,1.0693482201470206e-08
2727,13425,0,13425,0.5220742225646973,1.068755749947882e-08
2729,13435,0,13435,0.5224592685699463,1.0683623232135962e-08
2732,13450,0,13450,0.523169994354248,1.0677740571494143e-08
2735,13465,0,13465,0.5238831043243408,1.0671874542924163e-08
2738,13480,0,13480,0.5244491100311279,1.0666019753172266e-08
2740,13490,0,13490,0.5249121189117432,1.0662121144859335e-08
2743,13505,0,13505,0.525604248046875,1.0656279180503394e-08
2746,13519,0,13519,0.5261900424957275,1.052949158506634e-08
2749,13534,0,13534,0.5267930030822754,1.0497365971310564e-08
2751,13544,0,13544,0.5271632671356201,1.048266974087325e-08
2754,13559,0,13559,0.5277750492095947,1.0466609091959363e-08
2757,13573,0,13573,0.5283730030059814,9.967380256916036e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/flex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.295608520507812e-05,4.387072431292609
1,3,0,3,0.00017189979553222656,3.9719937673698036
2,6,0,6,0.0003688335418701172,3.6265995713934247
3,9,0,9,0.0004899501800537109,2.671453375268637
4,12,0,12,0.0006248950958251953,2.4144090921154513
5,15,0,15,0.0007386207580566406,1.5658221694735213
6,18,0,18,0.0008878707885742188,1.4684861444492576
7,21,0,21,0.0010027885437011719,1.1798911647236028
8,24,0,24,0.0011358261108398438,1.117166644632543
9,27,0,27,0.0012538433074951172,0.8368383001013324
10,30,0,30,0.001390695571899414,0.791899118477761
11,33,0,33,0.0015096664428710938,0.6055985084793335
12,36,0,36,0.0016448497772216797,0.5616175798559058
13,39,0,39,0.0017697811126708984,0.4227903890593488
14,42,0,42,0.0019228458404541016,0.4061053285128045
15,45,0,45,0.002045869827270508,0.3528419133996219
16,48,0,48,0.0021889209747314453,0.3357730534047567
17,51,0,51,0.0023186206817626953,0.2502581592012376
18,54,0,54,0.002530813217163086,0.2433781962784082
19,57,0,57,0.002706766128540039,0.18473321536660026
20,60,0,60,0.002873659133911133,0.18152669283485065
21,63,0,63,0.0030210018157958984,0.15738429407532292
22,66,0,66,0.0031769275665283203,0.15596930064324618
23,69,0,69,0.0033278465270996094,0.15441418844404023
24,72,0,72,0.0034618377685546875,0.12974292240134785
25,75,0,75,0.0036127567291259766,0.12704442339728433
26,78,0,78,0.003744840621948242,0.10719610350380714
27,81,0,81,0.003908634185791016,0.10603854634897296
28,84,0,84,0.0040738582611083984,0.08108624863755504
29,87,0,87,0.004220724105834961,0.08027009439315946
30,90,0,90,0.004349946975708008,0.0638939330914072
31,93,0,93,0.004495859146118164,0.06304197476918527
32,96,0,96,0.004624843597412109,0.061981996497830684
33,99,0,99,0.004789829254150391,0.061714185028897445
34,102,0,102,0.00493168830871582,0.06148540189151549
35,105,0,105,0.0050716400146484375,0.060951022819812
36,108,0,108,0.005211830139160156,0.060635107032990326
37,111,0,111,0.005337715148925781,0.0585350634913127
38,114,0,114,0.005478858947753906,0.05799964749239912
39,117,0,117,0.005604743957519531,0.05614581611090632
40,120,0,120,0.0057446956634521484,0.05580850661355847
41,123,0,123,0.005871772766113281,0.05472935751071315
42,126,0,126,0.006081819534301758,0.05448577024452025
43,129,0,129,0.006413698196411133,0.05356067895920529
44,132,0,132,0.0067157745361328125,0.05324735585084745
45,135,0,135,0.007030963897705078,0.05162480880792435
46,138,0,138,0.007487773895263672,0.05140105031967098
47,141,0,141,0.007878780364990234,0.05116693679634146
48,144,0,144,0.00819087028503418,0.049529404058950365
49,147,0,147,0.008530855178833008,0.0493068791924402
50,150,0,150,0.008862972259521484,0.0460716194361311
51,153,0,153,0.009141921997070312,0.04585995135443143
52,156,0,156,0.009457826614379883,0.04565146880844413
53,159,0,159,0.009685993194580078,0.04217592917915784
54,162,0,162,0.009954690933227539,0.04162859787171804
55,165,0,165,0.01012563705444336,0.03907140204258411
56,168,0,168,0.010291814804077148,0.03818517080019767
57,171,0,171,0.01043081283569336,0.03663163635924788
58,174,0,174,0.010680675506591797,0.035901055481322046
59,177,0,177,0.010938882827758789,0.0338782706500878
60,180,0,180,0.011221885681152344,0.03328126152231233
61,183,0,183,0.011490583419799805,0.03294031572574751
62,186,0,186,0.01172780990600586,0.03242192259213498
63,189,0,189,0.011928796768188477,0.03078552357091988
64,192,0,192,0.012151956558227539,0.030335803786928114
65,195,0,195,0.012445926666259766,0.029450995704127094
66,198,0,198,0.012801885604858398,0.029164376272614086
67,201,0,201,0.013107776641845703,0.02881640212142582
68,204,0,204,0.013415813446044922,0.02827588534210063
69,207,0,207,0.013753652572631836,0.02815550424746922
70,210,0,210,0.014047861099243164,0.027713561324896153
71,213,0,213,0.014380931854248047,0.027582182442197966
72,216,0,216,0.01467275619506836,0.027365460541195104
73,219,0,219,0.015024900436401367,0.026999884329266047
74,222,0,222,0.015323877334594727,0.026875269811637733
75,225,0,225,0.015572786331176758,0.02651685309121984
76,228,0,228,0.01587390899658203,0.026470414185559076
77,231,0,231,0.01612377166748047,0.026360742102943854
78,234,0,234,0.016350746154785156,0.026244187492183445
79,237,0,237,0.01658487319946289,0.026121495829515253
80,240,0,240,0.016846656799316406,0.025994641139469706
81,243,0,243,0.01705479621887207,0.025908517075605056
82,246,0,246,0.01729893684387207,0.02576842755569217
83,249,0,249,0.017566919326782227,0.02568897002911488
84,252,0,252,0.017799854278564453,0.025623729099066735
85,255,0,255,0.018080949783325195,0.02552512846908838
86,258,0,258,0.018329858779907227,0.02547191685520478
87,261,0,261,0.01857471466064453,0.02539583515993751
88,264,0,264,0.0188448429107666,0.025350745998375945
89,267,0,267,0.019109725952148438,0.02531401893787343
90,270,0,270,0.0193789005279541,0.02527071651148829
91,273,0,273,0.019634723663330078,0.02524653702302687
92,276,0,276,0.01989603042602539,0.025199319935038805
93,279,0,279,0.020168781280517578,0.025167956914690322
94,282,0,282,0.020352840423583984,0.025142579981223264
95,285,0,285,0.02053976058959961,0.025109724767337395
96,288,0,288,0.0207517147064209,0.02509339592799098
97,291,0,291,0.02097773551940918,0.02506313274605519
98,294,0,294,0.021202802658081055,0.02504550253989337
99,297,0,297,0.021475791931152344,0.02502619918533511
100,300,0,300,0.021773815155029297,0.025008700904128628
101,303,0,303,0.02205681800842285,0.02499743137542306
102,306,0,306,0.022331714630126953,0.024979830689869767
103,309,0,309,0.022522687911987305,0.024969347318028086
104,312,0,312,0.022687911987304688,0.024960112055285425
105,315,0,315,0.02285003662109375,0.02494485709556043
106,318,0,318,0.023027896881103516,0.024933025736361383
107,321,0,321,0.023183822631835938,0.02489592842932073
108,324,0,324,0.023332834243774414,0.024876833025867216
109,327,0,327,0.023544788360595703,0.024862942514154333
110,330,0,330,0.023741722106933594,0.024833628713941337
111,333,0,333,0.023900747299194336,0.02481918117060225
112,336,0,336,0.024052858352661133,0.024800712003671364
113,339,0,339,0.024202823638916016,0.024778211620546255
114,342,0,342,0.024351835250854492,0.024756598904035657
115,345,0,345,0.024600744247436523,0.024722231069264546
116,348,0,348,0.024831771850585938,0.024694408228548608
117,351,0,351,0.025046825408935547,0.02464485777893637
118,354,0,354,0.025275707244873047,0.02462057959579985
119,357,0,357,0.025587797164916992,0.024598353745055444
120,360,0,360,0.0259246826171875,0.02456564580794844
121,363,0,363,0.026190757751464844,0.02454337772448629
122,366,0,366,0.026451826095581055,0.02448364255675555
123,369,0,369,0.026636838912963867,0.024445545047394594
124,372,0,372,0.026788711547851562,0.02441136755208178
125,375,0,375,0.026993751525878906,0.024379208753718462
126,378,0,378,0.027238845825195312,0.02435155746117089
127,381,0,381,0.027431726455688477,0.024269452386885285
128,384,0,384,0.02761983871459961,0.024225779150827846
129,387,0,387,0.027853727340698242,0.024171448071513762
130,390,0,390,0.028070688247680664,0.02412558360837189
131,393,0,393,0.028354883193969727,0.02403859719677517
132,396,0,396,0.02864670753479004,0.023963481215398104
133,399,0,399,0.028973817825317383,0.02390520584736328
134,402,0,402,0.029249906539916992,0.023855284050183445
135,405,0,405,0.029558897018432617,0.023801333458419206
136,408,0,408,0.029803991317749023,0.023721885410648805
137,411,0,411,0.029996871948242188,0.023626620749677776
138,414,0,414,0.030276775360107422,0.023531549734722816
139,417,0,417,0.030566692352294922,0.023434989654914255
140,420,0,420,0.030813932418823242,0.02319479468863174
141,423,0,423,0.031110763549804688,0.02311401381487881
142,426,0,426,0.031357765197753906,0.022772331366697936
143,429,0,429,0.031645774841308594,0.022712343793783427
144,432,0,432,0.03192877769470215,0.02264476412290477
145,435,0,435,0.03216195106506348,0.022509872742809897
146,438,0,438,0.032326698303222656,0.02244423651454695
147,441,0,441,0.03249192237854004,0.02237723158887883
148,444,0,444,0.03263378143310547,0.022087563671959874
149,447,0,447,0.03280186653137207,0.021983527747741344
150,450,0,450,0.03293490409851074,0.02169094413463855
151,453,0,453,0.03308272361755371,0.021609613276818707
152,456,0,456,0.03323078155517578,0.02146679786748275
153,459,0,459,0.03336286544799805,0.021001490377648882
154,462,0,462,0.03354477882385254,0.020908095045159118
155,465,0,465,0.03406476974487305,0.020528279115133156
156,468,0,468,0.03426480293273926,0.020486130849232554
157,471,0,471,0.03447866439819336,0.02042155090350316
158,474,0,474,0.03467082977294922,0.0201608744464448
159,477,0,477,0.03485369682312012,0.020107818604074654
160,480,0,480,0.035042762756347656,0.019734988743270097
161,483,0,483,0.03533172607421875,0.019709618060724594
162,486,0,486,0.03561973571777344,0.01968511498434759
163,489,0,489,0.03590083122253418,0.01957441584645825
164,492,0,492,0.03618192672729492,0.019512764984753517
165,495,0,495,0.03645586967468262,0.01945170709793743
166,498,0,498,0.03673386573791504,0.01932090760125844
167,501,0,501,0.03703761100769043,0.019231223729360012
168,504,0,504,0.03734588623046875,0.019148704962709658
169,507,0,507,0.03764677047729492,0.019064104096234366
170,510,0,510,0.03795289993286133,0.018947355654419067
171,513,0,513,0.03820490837097168,0.018683782126529595
172,516,0,516,0.03849291801452637,0.018633853255029184
173,519,0,519,0.038786888122558594,0.018500292981500934
174,522,0,522,0.03908991813659668,0.01840956108567459
175,525,0,525,0.039381980895996094,0.01831807749253664
176,528,0,528,0.03960871696472168,0.018120711368278378
177,531,0,531,0.039778709411621094,0.017987288192636085
178,534,0,534,0.03991985321044922,0.01724766163208567
179,537,0,537,0.04007387161254883,0.017178592344132645
180,540,0,540,0.040239810943603516,0.017087653069341385
181,543,0,543,0.04038286209106445,0.01658192453500602
182,546,0,546,0.040535926818847656,0.01642643746603651
183,549,0,549,0.04067182540893555,0.016130489687503684
184,552,0,552,0.04082298278808594,0.015871492900802704
185,555,0,555,0.040956735610961914,0.015260409620693116
186,558,0,558,0.041107892990112305,0.014978415942477823
187,561,0,561,0.041240692138671875,0.01285926622354681
188,564,0,564,0.04138970375061035,0.012615529407217888
189,567,0,567,0.041539669036865234,0.012294080654745737
190,570,0,570,0.0416717529296875,0.00980830159442174
191,573,0,573,0.04181981086730957,0.009470333068544053
192,576,0,576,0.04195404052734375,0.008342492936783567
193,579,0,579,0.04210186004638672,0.008111577302213712
194,582,0,582,0.0422358512878418,0.007820397829934165
195,585,0,585,0.04238581657409668,0.007523126185198077
196,588,0,588,0.042517900466918945,0.006522861607147147
197,591,0,591,0.042665958404541016,0.006393684574255771
198,594,0,594,0.0428159236907959,0.006319819591321938
199,597,0,597,0.04296875,0.006175878860235438
200,600,0,600,0.04310488700866699,0.005810035145260915
201,603,0,603,0.04325985908508301,0.0056846156375646
202,606,0,606,0.0433957576751709,0.005314155762290482
203,609,0,609,0.04366278648376465,0.005227953322667981
204,612,0,612,0.04399585723876953,0.00495737030606787
205,615,0,615,0.04418468475341797,0.004880714609683584
206,618,0,618,0.04433083534240723,0.004825520219477261
207,621,0,621,0.04452085494995117,0.004742028457371389
208,624,0,624,0.04477691650390625,0.004281060315970977
209,627,0,627,0.044945716857910156,0.00421815938036587
210,630,0,630,0.045079946517944336,0.004009137687327003
211,633,0,633,0.04522895812988281,0.00393224068662264
212,636,0,636,0.04535984992980957,0.0037817958709922086
213,639,0,639,0.04550766944885254,0.003718051291400541
214,642,0,642,0.0456387996673584,0.0035175276368477047
215,645,0,645,0.045784711837768555,0.0034920211849089663
216,648,0,648,0.04593181610107422,0.0034459467011754463
217,651,0,651,0.046061038970947266,0.0033129918703984165
218,654,0,654,0.046208858489990234,0.0032937703689059974
219,657,0,657,0.046344757080078125,0.003242142200753039
220,660,0,660,0.046489715576171875,0.003191790085506379
221,663,0,663,0.04661989212036133,0.0030819813320071576
222,666,0,666,0.046765804290771484,0.003017237839360968
223,669,0,669,0.04691576957702637,0.0028331694590725326
224,672,0,672,0.04706573486328125,0.0027878431718039156
225,675,0,675,0.047200918197631836,0.0026824037521068446
226,678,0,678,0.04735088348388672,0.0026499719967156385
227,681,0,681,0.0474848747253418,0.002613880657349491
228,684,0,684,0.04763484001159668,0.0025669930096659465
229,687,0,687,0.04776787757873535,0.002300794238216177
230,690,0,690,0.04792976379394531,0.0022657852553129958
231,693,0,693,0.04805779457092285,0.002213156605471406
232,696,0,696,0.0482029914855957,0.0021659428023344538
233,699,0,699,0.04833674430847168,0.0021151149330364467
234,702,0,702,0.048482656478881836,0.0020727449292533176
235,705,0,705,0.04861283302307129,0.0016814590274075107
236,708,0,708,0.0487668514251709,0.0016535384353447452
237,711,0,711,0.04891800880432129,0.0015946222420259626
238,714,0,714,0.04906892776489258,0.001570064889333774
239,717,0,717,0.04920387268066406,0.001539313266893499
240,720,0,720,0.04935765266418457,0.0015150681175784908
241,723,0,723,0.04949378967285156,0.0014198535880699705
242,726,0,726,0.04965400695800781,0.0014051282160094825
243,729,0,729,0.049791812896728516,0.001386285350269362
244,732,0,732,0.04995989799499512,0.0013714491056596465
245,735,0,735,0.05008983612060547,0.0013176168374794334
246,738,0,738,0.050235748291015625,0.0013094627070355995
247,741,0,741,0.050366878509521484,0.0012874609571619908
248,744,0,744,0.05051279067993164,0.0012720728272780934
249,747,0,747,0.05064868927001953,0.0012059537580773707
250,750,0,750,0.05079984664916992,0.00118909085599715
251,753,0,753,0.05094599723815918,0.0011414651456179723
252,756,0,756,0.05108976364135742,0.0011346488821428174
253,759,0,759,0.05123186111450195,0.001124849053485082
254,762,0,762,0.05136990547180176,0.0011069421434018048
255,765,0,765,0.05151486396789551,0.0011017778810861675
256,768,0,768,0.051642656326293945,0.0010767967166861673
257,771,0,771,0.051785945892333984,0.0010676576533637473
258,774,0,774,0.05191183090209961,0.001031416878232423
259,777,0,777,0.05205392837524414,0.001025947388448
260,780,0,780,0.05219459533691406,0.0010177413566925947
261,783,0,783,0.0523226261138916,0.0009863513539062271
262,786,0,786,0.05246472358703613,0.0009791404637128256
263,789,0,789,0.05259275436401367,0.0009448409635365719
264,792,0,792,0.05273580551147461,0.0009354533369074163
265,795,0,795,0.05287981033325195,0.0009217521698288862
266,798,0,798,0.05302882194519043,0.0009144637934911377
267,801,0,801,0.05315876007080078,0.0008949338690277253
268,804,0,804,0.053305625915527344,0.0008881400721893031
269,807,0,807,0.05343985557556152,0.0008729172471181306
270,810,0,810,0.0535888671875,0.0008677979330836488
271,813,0,813,0.053720712661743164,0.0008499564957630037
272,816,0,816,0.053938865661621094,0.0008435297113801884
273,819,0,819,0.05408978462219238,0.0008331392205732868
274,822,0,822,0.05424189567565918,0.0008274421962959793
275,825,0,825,0.05438590049743652,0.0008209591359751657
276,828,0,828,0.054512739181518555,0.0008070259495097694
277,831,0,831,0.05465984344482422,0.0008033616391460187
278,834,0,834,0.05478692054748535,0.0007589962431943003
279,837,0,837,0.054930925369262695,0.0007518021731039839
280,840,0,840,0.055078744888305664,0.0007432753877792076
281,843,0,843,0.0552058219909668,0.0006995545027015209
282,846,0,846,0.055345773696899414,0.0006915972158924699
283,849,0,849,0.05547285079956055,0.000639285381441614
284,852,0,852,0.05561494827270508,0.0006293464430418033
285,855,0,855,0.0557558536529541,0.0006174534798947742
286,858,0,858,0.05588197708129883,0.0005706714966019413
287,861,0,861,0.056024789810180664,0.0005604109870541887
288,864,0,864,0.0561528205871582,0.0005278714466224235
289,867,0,867,0.05629682540893555,0.0005137870832953194
290,870,0,870,0.05642390251159668,0.00048497243692256363
291,873,0,873,0.05656599998474121,0.00047204431095574295
292,876,0,876,0.056691884994506836,0.0004453064868269661
293,879,0,879,0.05689692497253418,0.00043824566400627144
294,882,0,882,0.05707883834838867,0.00042531439248306904
295,885,0,885,0.0572819709777832,0.00041691303118916685
296,888,0,888,0.05746293067932129,0.00039552737023783855
297,891,0,891,0.05766773223876953,0.0003872284250596954
298,894,0,894,0.05785965919494629,0.0003474667961275712
299,897,0,897,0.05805778503417969,0.0003431253165675477
300,900,0,900,0.0582578182220459,0.0003395700213746098
301,903,0,903,0.05842995643615723,0.0003072792491238808
302,906,0,906,0.058573007583618164,0.000300584107224033
303,909,0,909,0.05869793891906738,0.0002575171009324226
304,912,0,912,0.058853864669799805,0.00025081793008133754
305,915,0,915,0.05899691581726074,0.00024403545813014035
306,918,0,918,0.05912375450134277,0.00022506871387435878
307,921,0,921,0.059265851974487305,0.0002196941056966437
308,924,0,924,0.05939292907714844,0.00020609315455761697
309,927,0,927,0.05954790115356445,0.0002010586246740129
310,930,0,930,0.0596768856048584,0.00019566655187200447
311,933,0,933,0.05983996391296387,0.0001913266732059144
312,936,0,936,0.059970855712890625,0.00016404929996082193
313,939,0,939,0.06011795997619629,0.0001604274714068282
314,942,0,942,0.06024980545043945,0.0001566747498462244
315,945,0,945,0.06039595603942871,0.00015447831283416934
316,948,0,948,0.06052684783935547,0.0001497937435299077
317,951,0,951,0.06067490577697754,0.00014855885645727744
318,954,0,954,0.0608220100402832,0.00014709326087815336
319,957,0,957,0.06104874610900879,0.00014286932819367027
320,960,0,960,0.061310768127441406,0.00014165666827397748
321,963,0,963,0.06147193908691406,0.00013456971661870908
322,966,0,966,0.0616297721862793,0.00013383389983709023
323,969,0,969,0.06180286407470703,0.00013280725097085998
324,972,0,972,0.06194281578063965,0.00012770616218214136
325,975,0,975,0.06209874153137207,0.00012669963138275478
326,978,0,978,0.062236785888671875,0.0001234329697282997
327,981,0,981,0.0623927116394043,0.00012272014242462173
328,984,0,984,0.06254792213439941,0.0001220758328618602
329,987,0,987,0.06279778480529785,0.00012038730497875401
330,990,0,990,0.06304669380187988,0.00011968632572121657
331,993,0,993,0.06321573257446289,0.00011569167799041666
332,996,0,996,0.06337666511535645,0.0001147903447260128
333,999,0,999,0.06351685523986816,0.00011278983393982073
334,1002,0,1002,0.06367087364196777,0.00011185659190516713
335,1005,0,1005,0.06382274627685547,0.0001095928875100623
336,1008,0,1008,0.06396985054016113,0.0001086899884084548
337,1011,0,1011,0.0641179084777832,0.00010759139035194271
338,1014,0,1014,0.06424880027770996,0.0001059486896543179
339,1017,0,1017,0.06439590454101562,0.00010547049265231637
340,1020,0,1020,0.06452679634094238,0.00010160053553013474
341,1023,0,1023,0.06467294692993164,0.00010122886390418326
342,1026,0,1026,0.06483983993530273,0.00010077206785352264
343,1029,0,1029,0.06497788429260254,9.843727255104451e-05
344,1032,0,1032,0.06513285636901855,9.807401137858096e-05
345,1035,0,1035,0.06528782844543457,9.728579529997675e-05
346,1038,0,1038,0.06544375419616699,9.667447886302493e-05
347,1041,0,1041,0.06559896469116211,9.621789321905942e-05
348,1044,0,1044,0.06575274467468262,9.547702170145573e-05
349,1047,0,1047,0.06588983535766602,9.42229748603225e-05
350,1050,0,1050,0.06604385375976562,9.373841731654527e-05
351,1053,0,1053,0.06617975234985352,9.160160183868812e-05
352,1056,0,1056,0.06633782386779785,9.104659699008747e-05
353,1059,0,1059,0.06648087501525879,8.992154767496919e-05
354,1062,0,1062,0.06663703918457031,8.956575902807867e-05
355,1065,0,1065,0.06679296493530273,8.869649603895982e-05
356,1068,0,1068,0.06694293022155762,8.661050952286758e-05
357,1071,0,1071,0.0670928955078125,8.589312651636487e-05
358,1074,0,1074,0.06722784042358398,8.216314752533503e-05
359,1077,0,1077,0.06737875938415527,8.189156419341004e-05
360,1080,0,1080,0.06752991676330566,8.160004581014755e-05
361,1083,0,1083,0.06766581535339355,8.067967271488616e-05
362,1086,0,1086,0.06781578063964844,8.030486675593076e-05
363,1089,0,1089,0.06795167922973633,7.827134643823529e-05
364,1092,0,1092,0.06811690330505371,7.758385039114661e-05
365,1095,0,1095,0.06826901435852051,7.673438579112539e-05
366,1098,0,1098,0.06842374801635742,7.610438313542045e-05
367,1101,0,1101,0.0685577392578125,7.471877385554925e-05
368,1104,0,1104,0.06870770454406738,7.440774880249201e-05
369,1107,0,1107,0.06887698173522949,7.391835054583229e-05
370,1110,0,1110,0.06902766227722168,7.336485119259712e-05
371,1113,0,1113,0.06917977333068848,7.290087879774918e-05
372,1116,0,1116,0.06940889358520508,7.250364478938032e-05
373,1119,0,1119,0.06962394714355469,7.223320339018048e-05
374,1122,0,1122,0.06978392601013184,7.192654564753478e-05
375,1125,0,1125,0.06993484497070312,7.162501346947555e-05
376,1128,0,1128,0.07008576393127441,7.137727897445824e-05
377,1131,0,1131,0.07023882865905762,7.10433770633115e-05
378,1134,0,1134,0.0703887939453125,7.084896589551831e-05
379,1137,0,1137,0.07053780555725098,7.068621940877905e-05
380,1140,0,1140,0.07068896293640137,7.041205251232957e-05
381,1143,0,1143,0.07094383239746094,7.025836155554443e-05
382,1146,0,1146,0.07114291191101074,7.014350990242335e-05
383,1149,0,1149,0.0713038444519043,6.997613849136086e-05
384,1152,0,1152,0.07146072387695312,6.98244301949826e-05
385,1155,0,1155,0.07161498069763184,6.96510799049161e-05
386,1158,0,1158,0.07177972793579102,6.952163983453937e-05
387,1161,0,1161,0.07193803787231445,6.917176295247409e-05
388,1164,0,1164,0.07218790054321289,6.89773112571187e-05
389,1167,0,1167,0.07242488861083984,6.8716126596669e-05
390,1170,0,1170,0.07258892059326172,6.853500623823032e-05
391,1173,0,1173,0.07274174690246582,6.831200726283425e-05
392,1176,0,1176,0.07289695739746094,6.791414585734335e-05
393,1179,0,1179,0.07306289672851562,6.756546980803424e-05
394,1182,0,1182,0.07322072982788086,6.720508571579812e-05
395,1185,0,1185,0.07336783409118652,6.670755323333968e-05
396,1188,0,1188,0.07351279258728027,6.639467991110165e-05
397,1191,0,1191,0.07364392280578613,6.564174237516975e-05
398,1194,0,1194,0.07378888130187988,6.525826026858754e-05
399,1197,0,1197,0.0739748477935791,6.403090988206332e-05
400,1200,0,1200,0.0741739273071289,6.369173561889391e-05
401,1203,0,1203,0.0743257999420166,6.15932256519277e-05
402,1206,0,1206,0.07448291778564453,6.128638890107456e-05
403,1209,0,1209,0.07465291023254395,6.0825253976273925e-05
404,1212,0,1212,0.07484889030456543,5.9292237205794206e-05
405,1215,0,1215,0.07506394386291504,5.874953465191718e-05
406,1218,0,1218,0.07520890235900879,5.567365911909027e-05
407,1221,0,1221,0.07538771629333496,5.4815247984436516e-05
408,1224,0,1224,0.07555294036865234,5.4328898348170876e-05
409,1227,0,1227,0.07568669319152832,5.10470630786342e-05
410,1230,0,1230,0.0758368968963623,5.0347006122406135e-05
411,1233,0,1233,0.07596778869628906,4.6519341418492666e-05
412,1236,0,1236,0.07612061500549316,4.576589186951897e-05
413,1239,0,1239,0.07631468772888184,4.515597122556252e-05
414,1242,0,1242,0.07652401924133301,4.4551677907721705e-05
415,1245,0,1245,0.0767066478729248,4.1410732874215455e-05
416,1248,0,1248,0.0768887996673584,4.112089080302465e-05
417,1251,0,1251,0.07707381248474121,4.068481893771839e-05
418,1254,0,1254,0.07723069190979004,3.840102557031192e-05
419,1257,0,1257,0.07739067077636719,3.790528000882402e-05
420,1260,0,1260,0.07761669158935547,3.723560951666276e-05
421,1263,0,1263,0.0778360366821289,3.56948583631248e-05
422,1266,0,1266,0.07800793647766113,3.515453620709023e-05
423,1269,0,1269,0.07814884185791016,3.4165376865936226e-05
424,1272,0,1272,0.07829976081848145,3.351475654382436e-05
425,1275,0,1275,0.0784299373626709,3.207576079615928e-05
426,1278,0,1278,0.07857894897460938,3.177238010971965e-05
427,1281,0,1281,0.07870888710021973,3.0751937690503556e-05
428,1284,0,1284,0.07887101173400879,3.0397990917855048e-05
429,1287,0,1287,0.07900285720825195,3.004883336510241e-05
430,1290,0,1290,0.07914900779724121,2.972539806361043e-05
431,1293,0,1293,0.07929682731628418,2.9282115628188988e-05
432,1296,0,1296,0.07943868637084961,2.7898117388653248e-05
433,1299,0,1299,0.07958769798278809,2.772868673290928e-05
434,1302,0,1302,0.07971882820129395,2.7208767515462438e-05
435,1305,0,1305,0.07988572120666504,2.7026514273442193e-05
436,1308,0,1308,0.08002185821533203,2.6422463206677017e-05
437,1311,0,1311,0.08018088340759277,2.6147816952832093e-05
438,1314,0,1314,0.08031082153320312,2.5187036333982238e-05
439,1317,0,1317,0.08045482635498047,2.4869526748718166e-05
440,1320,0,1320,0.08058285713195801,2.444014433066966e-05
441,1323,0,1323,0.08072590827941895,2.414346162278769e-05
442,1326,0,1326,0.08086180686950684,2.361624824956185e-05
443,1329,0,1329,0.08100676536560059,2.3373200852901532e-05
444,1332,0,1332,0.08113360404968262,2.2111989178653473e-05
445,1335,0,1335,0.08127784729003906,2.194241779041908e-05
446,1338,0,1338,0.08140897750854492,2.1349072038954448e-05
447,1341,0,1341,0.08155989646911621,2.1233023906106364e-05
448,1344,0,1344,0.08170390129089355,2.1114064937281177e-05
449,1347,0,1347,0.08185076713562012,2.045979789151093e-05
450,1350,0,1350,0.08199763298034668,2.033084358936828e-05
451,1353,0,1353,0.08214378356933594,2.0172564111693555e-05
452,1356,0,1356,0.08227396011352539,1.9517874421358366e-05
453,1359,0,1359,0.08242297172546387,1.930282601477055e-05
454,1362,0,1362,0.08255481719970703,1.8996838341730067e-05
455,1365,0,1365,0.08270382881164551,1.8775255898445286e-05
456,1368,0,1368,0.08289480209350586,1.856166702202269e-05
457,1371,0,1371,0.08304381370544434,1.811083404069008e-05
458,1374,0,1374,0.08319473266601562,1.797927537144892e-05
459,1377,0,1377,0.08338284492492676,1.626853128396518e-05
460,1380,0,1380,0.08355188369750977,1.611850464443155e-05
461,1383,0,1383,0.08371496200561523,1.594413568685526e-05
462,1386,0,1386,0.08386397361755371,1.5569219398316693e-05
463,1389,0,1389,0.08400988578796387,1.5451966708043837e-05
464,1392,0,1392,0.08415579795837402,1.5227199102525813e-05
465,1395,0,1395,0.08428478240966797,1.4393317707574952e-05
466,1398,0,1398,0.08451676368713379,1.4242580301315615e-05
467,1401,0,1401,0.08466672897338867,1.342622589917708e-05
468,1404,0,1404,0.08481669425964355,1.3269658300043366e-05
469,1407,0,1407,0.08496379852294922,1.307382173803208e-05
470,1410,0,1410,0.08509182929992676,1.2675022264788921e-05
471,1413,0,1413,0.0852348804473877,1.2522530248024128e-05
472,1416,0,1416,0.0853879451751709,1.1606619265456335e-05
473,1419,0,1419,0.08561182022094727,1.1367976960625284e-05
474,1422,0,1422,0.08577680587768555,1.0712545629665873e-05
475,1425,0,1425,0.08604073524475098,1.0492904322987856e-05
476,1428,0,1428,0.0863039493560791,1.0186816051987526e-05
477,1431,0,1431,0.08661293983459473,9.14561411518982e-06
478,1434,0,1434,0.08687090873718262,8.931363627100013e-06
479,1437,0,1437,0.0870199203491211,7.834929769162489e-06
480,1440,0,1440,0.08717775344848633,7.651453641774849e-06
481,1443,0,1443,0.08738183975219727,7.554698559339343e-06
482,1446,0,1446,0.08761382102966309,7.36770521536352e-06
483,1449,0,1449,0.08782100677490234,6.524403515171131e-06
484,1452,0,1452,0.08804774284362793,6.181383878148966e-06
485,1455,0,1455,0.08822774887084961,5.739086577947242e-06
486,1458,0,1458,0.08848690986633301,5.402262146507937e-06
487,1461,0,1461,0.08873701095581055,4.6947886720868614e-06
488,1464,0,1464,0.0889887809753418,4.5825993433017375e-06
489,1467,0,1467,0.08921480178833008,4.439623008513073e-06
490,1470,0,1470,0.08942794799804688,3.806168433469163e-06
491,1473,0,1473,0.08958578109741211,3.7284819089939114e-06
492,1476,0,1476,0.08972001075744629,3.159689566021068e-06
493,1479,0,1479,0.08986783027648926,3.069908377396534e-06
494,1482,0,1482,0.09000182151794434,2.917586661096243e-06
495,1485,0,1485,0.0901486873626709,2.802853935387038e-06
496,1488,0,1488,0.09027886390686035,2.5657316280525857e-06
497,1491,0,1491,0.09042477607727051,2.4673972535084205e-06
498,1494,0,1494,0.09055471420288086,2.094585416533554e-06
499,1497,0,1497,0.09071779251098633,2.040368148337467e-06
500,1500,0,1500,0.09086275100708008,1.9284614718828594e-06
501,1503,0,1503,0.09101486206054688,1.8794512430434498e-06
502,1506,0,1506,0.09114289283752441,1.6977439710077461e-06
503,1509,0,1509,0.09128379821777344,1.6583927959933698e-06
504,1512,0,1512,0.09141182899475098,1.5457786920622314e-06
505,1515,0,1515,0.09160804748535156,1.5205137735416043e-06
506,1518,0,1518,0.0917518138885498,1.4503958590752955e-06
507,1521,0,1521,0.09190487861633301,1.4151174311461734e-06
508,1524,0,1524,0.09203672409057617,1.37513262040684e-06
509,1527,0,1527,0.09218192100524902,1.3463273878563129e-06
510,1530,0,1530,0.09230995178222656,1.3299766936121285e-06
511,1533,0,1533,0.09246277809143066,1.2975600745590893e-06
512,1536,0,1536,0.09270977973937988,1.1637499006173614e-06
513,1539,0,1539,0.09302496910095215,1.148188862284089e-06
514,1542,0,1542,0.0932307243347168,1.1053471339642678e-06
515,1545,0,1545,0.09339165687561035,1.0772063860096396e-06
516,1548,0,1548,0.09351682662963867,1.0115135269803897e-06
517,1551,0,1551,0.09365487098693848,9.988694818432688e-07
518,1554,0,1554,0.09379291534423828,9.62959616245612e-07
519,1557,0,1557,0.09393477439880371,9.43366138638627e-07
520,1560,0,1560,0.09406089782714844,9.161775885120763e-07
521,1563,0,1563,0.09421777725219727,8.912388964219993e-07
522,1566,0,1566,0.0943758487701416,7.868098217937459e-07
523,1569,0,1569,0.09454774856567383,7.764028601154955e-07
524,1572,0,1572,0.0946817398071289,7.527224272183519e-07
525,1575,0,1575,0.09483790397644043,7.459199704693513e-07
526,1578,0,1578,0.09497380256652832,7.371183647125435e-07
527,1581,0,1581,0.09509396553039551,7.120126241688933e-07
528,1584,0,1584,0.0952298641204834,7.072802317755289e-07
529,1587,0,1587,0.09535098075866699,6.727409395472214e-07
530,1590,0,1590,0.09548592567443848,6.69354465878351e-07
531,1593,0,1593,0.09562063217163086,6.647110593051294e-07
532,1596,0,1596,0.09574174880981445,6.395087707003424e-07
533,1599,0,1599,0.09587788581848145,6.370976233427261e-07
534,1602,0,1602,0.09601378440856934,6.345217897584548e-07
535,1605,0,1605,0.09616875648498535,6.287189751207414e-07
536,1608,0,1608,0.09634995460510254,6.249494527280013e-07
537,1611,0,1611,0.09655594825744629,6.117564929022549e-07
538,1614,0,1614,0.09673595428466797,6.095671525092233e-07
539,1617,0,1617,0.09688973426818848,6.062881176093586e-07
540,1620,0,1620,0.09701871871948242,5.992419141665362e-07
541,1623,0,1623,0.09715986251831055,5.962333840440355e-07
542,1626,0,1626,0.09728479385375977,5.775718897466629e-07
543,1629,0,1629,0.09742379188537598,5.755468615319765e-07
544,1632,0,1632,0.09756278991699219,5.733927999779027e-07
545,1635,0,1635,0.0976870059967041,5.550973068473121e-07
546,1638,0,1638,0.0978248119354248,5.507753083708254e-07
547,1641,0,1641,0.09794878959655762,5.405583209800216e-07
548,1644,0,1644,0.09816288948059082,5.346336065533684e-07
549,1647,0,1647,0.09835386276245117,5.297617177245401e-07
550,1650,0,1650,0.09848284721374512,5.118559539134085e-07
551,1653,0,1653,0.09862494468688965,5.087226614596659e-07
552,1656,0,1656,0.09874773025512695,4.999938482010047e-07
553,1659,0,1659,0.09888672828674316,4.976331547783683e-07
554,1662,0,1662,0.09902477264404297,4.932193807548246e-07
555,1665,0,1665,0.09914684295654297,4.823914814324542e-07
556,1668,0,1668,0.09928488731384277,4.808318074016248e-07
557,1671,0,1671,0.09942173957824707,4.773642281911023e-07
558,1674,0,1674,0.09954285621643066,4.6881240799704113e-07
559,1677,0,1677,0.09967875480651855,4.6596930069034576e-07
560,1680,0,1680,0.09981274604797363,4.5341056606732077e-07
561,1683,0,1683,0.0999448299407959,4.502073290879528e-07
562,1686,0,1686,0.10006284713745117,4.370663724347469e-07
563,1689,0,1689,0.10020089149475098,4.3551440784249196e-07
564,1692,0,1692,0.10033369064331055,4.3288751274983807e-07
565,1695,0,1695,0.10045075416564941,4.2109274562698557e-07
566,1698,0,1698,0.10058188438415527,4.1901605616280465e-07
567,1701,0,1701,0.10069990158081055,4.10878203481897e-07
568,1704,0,1704,0.10083198547363281,4.080551462272771e-07
569,1707,0,1707,0.10094881057739258,3.998122663564874e-07
570,1710,0,1710,0.10107994079589844,3.985732627700979e-07
571,1713,0,1713,0.10121273994445801,3.9648803673841505e-07
572,1716,0,1716,0.10134482383728027,3.936031519605167e-07
573,1719,0,1719,0.10147976875305176,3.911195518548871e-07
574,1722,0,1722,0.10159897804260254,3.8710145389036424e-07
575,1725,0,1725,0.1017305850982666,3.847195617924348e-07
576,1728,0,1728,0.10184788703918457,3.804196061764433e-07
577,1731,0,1731,0.10197973251342773,3.7870333395595645e-07
578,1734,0,1734,0.1021108627319336,3.7566777329707933e-07
579,1737,0,1737,0.10224199295043945,3.7344851780720145e-07
580,1740,0,1740,0.10237383842468262,3.717511672378546e-07
581,1743,0,1743,0.10250473022460938,3.7053038761563366e-07
582,1746,0,1746,0.10263586044311523,3.691277207811244e-07
583,1749,0,1749,0.10276675224304199,3.680545149030595e-07
584,1752,0,1752,0.10289788246154785,3.6710919170153814e-07
585,1755,0,1755,0.10302877426147461,3.6617085019614855e-07
586,1758,0,1758,0.10315990447998047,3.6535345036881556e-07
587,1761,0,1761,0.10329174995422363,3.6458879307874603e-07
588,1764,0,1764,0.10342884063720703,3.639697924109797e-07
589,1767,0,1767,0.10355973243713379,3.6335529749376873e-07
590,1770,0,1770,0.10369181632995605,3.628338707252441e-07
591,1773,0,1773,0.10384082794189453,3.621974147113112e-07
592,1776,0,1776,0.1039738655090332,3.6168051143107475e-07
593,1779,0,1779,0.10411477088928223,3.6106069567939905e-07
594,1782,0,1782,0.1042487621307373,3.604130930384319e-07
595,1785,0,1785,0.10438394546508789,3.599205135479242e-07
596,1788,0,1788,0.10451984405517578,3.5947221778009344e-07
597,1791,0,1791,0.10465574264526367,3.58852511113013e-07
598,1794,0,1794,0.10479187965393066,3.5806398566110384e-07
599,1797,0,1797,0.10492587089538574,3.575051241126019e-07
600,1800,0,1800,0.10506081581115723,3.5722583798548203e-07
601,1803,0,1803,0.1051948070526123,3.5678501813579996e-07
602,1806,0,1806,0.10532975196838379,3.565353028085719e-07
603,1809,0,1809,0.10546469688415527,3.5617076987708195e-07
604,1812,0,1812,0.10559892654418945,3.5591115346380513e-07
605,1815,0,1815,0.10573387145996094,3.5565719934757034e-07
606,1818,0,1818,0.10587382316589355,3.552912953769603e-07
607,1821,0,1821,0.1060798168182373,3.550112437877619e-07
608,1824,0,1824,0.10631179809570312,3.54309201938633e-07
609,1827,0,1827,0.10646581649780273,3.538620407879445e-07
610,1830,0,1830,0.10661768913269043,3.534956566722419e-07
611,1833,0,1833,0.10675978660583496,3.5314464781925733e-07
612,1836,0,1836,0.10689783096313477,3.528386042168315e-07
613,1839,0,1839,0.10703682899475098,3.5249521393397036e-07
614,1842,0,1842,0.10717988014221191,3.520915693931212e-07
615,1845,0,1845,0.10737371444702148,3.5161664306977637e-07
616,1848,0,1848,0.10757184028625488,3.512677710791511e-07
617,1851,0,1851,0.1077268123626709,3.50736487453488e-07
618,1854,0,1854,0.10786986351013184,3.501989341285289e-07
619,1857,0,1857,0.10801482200622559,3.498175503787707e-07
620,1860,0,1860,0.1081547737121582,3.489562444774406e-07
621,1863,0,1863,0.10829782485961914,3.485949202892878e-07
622,1866,0,1866,0.10843491554260254,3.482758561374849e-07
623,1869,0,1869,0.10858273506164551,3.4739339926608607e-07
624,1872,0,1872,0.10872864723205566,3.468054258550146e-07
625,1875,0,1875,0.1089017391204834,3.4594826264300356e-07
626,1878,0,1878,0.10905981063842773,3.453843051849452e-07
627,1881,0,1881,0.10920071601867676,3.4455232662481837e-07
628,1884,0,1884,0.10935068130493164,3.434469228611645e-07
629,1887,0,1887,0.10949087142944336,3.428467798103976e-07
630,1890,0,1890,0.10963296890258789,3.424012587525449e-07
631,1893,0,1893,0.1097719669342041,3.416050120309271e-07
632,1896,0,1896,0.10995292663574219,3.4079249122010236e-07
633,1899,0,1899,0.11013078689575195,3.395860418398772e-07
634,1902,0,1902,0.11032795906066895,3.3808281663508293e-07
635,1905,0,1905,0.11049485206604004,3.363402987495184e-07
636,1908,0,1908,0.11064481735229492,3.346744716195333e-07
637,1911,0,1911,0.11080598831176758,3.3369796675265046e-07
638,1914,0,1914,0.11095380783081055,3.320856895266527e-07
639,1917,0,1917,0.11110591888427734,3.2993971769444884e-07
640,1920,0,1920,0.1112508773803711,3.278659465307237e-07
641,1923,0,1923,0.11139392852783203,3.259772005102182e-07
642,1926,0,1926,0.11152267456054688,3.1852771007451776e-07
643,1929,0,1929,0.1116647720336914,3.170717265116377e-07
644,1932,0,1932,0.11179280281066895,3.1147138793982474e-07
645,1935,0,1935,0.11193490028381348,3.1014188903363787e-07
646,1938,0,1938,0.11207699775695801,3.06858338663146e-07
647,1941,0,1941,0.11220502853393555,2.998671542570708e-07
648,1944,0,1944,0.11234664916992188,2.9744208365489976e-07
649,1947,0,1947,0.11247467994689941,2.822977740769389e-07
650,1950,0,1950,0.11261677742004395,2.7773377380715184e-07
651,1953,0,1953,0.11274886131286621,2.665078220374557e-07
652,1956,0,1956,0.11289167404174805,2.651994417467385e-07
653,1959,0,1959,0.11303496360778809,2.639003743745568e-07
654,1962,0,1962,0.11316490173339844,2.461755344851478e-07
655,1965,0,1965,0.11339378356933594,2.4441199347036585e-07
656,1968,0,1968,0.11359882354736328,2.4215134016445174e-07
657,1971,0,1971,0.11385273933410645,2.2768804353247158e-07
658,1974,0,1974,0.11413764953613281,2.2521770126313465e-07
659,1977,0,1977,0.1143789291381836,2.0581088087293752e-07
660,1980,0,1980,0.11464881896972656,2.035202900868252e-07
661,1983,0,1983,0.11489295959472656,2.0039925091649163e-07
662,1986,0,1986,0.11516284942626953,1.9729333461249382e-07
663,1989,0,1989,0.1154029369354248,1.933111267422245e-07
664,1992,0,1992,0.11567187309265137,1.9039829344158272e-07
665,1995,0,1995,0.11591863632202148,1.8221537926095094e-07
666,1998,0,1998,0.11618399620056152,1.7991522886351323e-07
667,2001,0,2001,0.11642074584960938,1.6605509373021681e-07
668,2004,0,2004,0.11670970916748047,1.6478759257028604e-07
669,2007,0,2007,0.11700582504272461,1.6337143417746603e-07
670,2010,0,2010,0.11716198921203613,1.523640388709641e-07
671,2013,0,2013,0.11730790138244629,1.5026847584813383e-07
672,2016,0,2016,0.11743283271789551,1.428580913671395e-07
673,2019,0,2019,0.11758279800415039,1.4149474663369464e-07
674,2022,0,2022,0.1177067756652832,1.3503614227065848e-07
675,2025,0,2025,0.11786484718322754,1.3358784308633728e-07
676,2028,0,2028,0.11798977851867676,1.3148952239339154e-07
677,2031,0,2031,0.11814761161804199,1.3007140277137118e-07
678,2034,0,2034,0.11832070350646973,1.2345777202456804e-07
679,2037,0,2037,0.11847686767578125,1.220117482543573e-07
680,2040,0,2040,0.11860299110412598,1.1600674692714107e-07
681,2043,0,2043,0.1187446117401123,1.147765996576606e-07
682,2046,0,2046,0.1189570426940918,1.1359713395512595e-07
683,2049,0,2049,0.11908888816833496,1.0731992732446228e-07
684,2052,0,2052,0.11923384666442871,1.0571605656862714e-07
685,2055,0,2055,0.11936187744140625,9.94106618441621e-08
686,2058,0,2058,0.11957287788391113,9.791719497423925e-08
687,2061,0,2061,0.11978960037231445,9.575626903665146e-08
688,2064,0,2064,0.11993694305419922,8.762831647782296e-08
689,2067,0,2067,0.1200859546661377,8.572412804500914e-08
690,2070,0,2070,0.12022280693054199,7.874845806452541e-08
691,2073,0,2073,0.12041282653808594,7.714518460172219e-08
692,2076,0,2076,0.1205596923828125,7.561007770840277e-08
693,2079,0,2079,0.12068986892700195,7.312721181344534e-08
694,2082,0,2082,0.1208498477935791,7.191709356465061e-08
695,2085,0,2085,0.12098288536071777,6.595121038450772e-08
696,2088,0,2088,0.12121796607971191,6.475916071721377e-08
697,2091,0,2091,0.12143373489379883,6.400502639990662e-08
698,2094,0,2094,0.12164974212646484,6.295565314871677e-08
699,2097,0,2097,0.12184381484985352,5.665528466744856e-08
700,2100,0,2100,0.12211489677429199,5.509556593940298e-08
701,2103,0,2103,0.12226986885070801,5.3957487530400283e-08
702,2106,0,2106,0.12242388725280762,5.182691281303634e-08
703,2109,0,2109,0.12255978584289551,4.512467574306617e-08
704,2112,0,2112,0.12270879745483398,4.415711437073289e-08
705,2115,0,2115,0.12284183502197266,3.4182203812323916e-08
706,2118,0,2118,0.12302374839782715,3.367333295056017e-08
707,2121,0,2121,0.12317681312561035,3.28973178872227e-08
708,2124,0,2124,0.12330961227416992,2.954957457385666e-08
709,2127,0,2127,0.12345695495605469,2.9212518986927172e-08
710,2130,0,2130,0.12359762191772461,2.834973882699673e-08
711,2133,0,2133,0.123748779296875,2.773125908791693e-08
712,2136,0,2136,0.12387871742248535,2.6167029745360934e-08
713,2139,0,2139,0.12402582168579102,2.565801174061523e-08
714,2142,0,2142,0.1241767406463623,2.3717443650515254e-08
715,2145,0,2145,0.1243288516998291,2.31764771383782e-08
716,2148,0,2148,0.12446379661560059,2.240562217821725e-08
717,2151,0,2151,0.12461090087890625,2.204242633436258e-08
718,2154,0,2154,0.12475371360778809,1.937924767140861e-08
719,2157,0,2157,0.12489581108093262,1.8675974756390423e-08
720,2160,0,2160,0.12504172325134277,1.5740205735919886e-08
721,2163,0,2163,0.12526178359985352,1.535814224122831e-08
722,2166,0,2166,0.12546181678771973,1.495106959692597e-08
723,2169,0,2169,0.12559890747070312,1.2623855871938907e-08
724,2172,0,2172,0.12574267387390137,1.2170515745117986e-08
725,2175,0,2175,0.1258690357208252,1.0640144202866676e-08
726,2178,0,2178,0.12601065635681152,1.0240679628359536e-08
727,2181,0,2181,0.12613773345947266,9.137954353095484e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/flex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.818771362304688e-05,4.387072431292609
1,5,0,5,0.0002732276916503906,4.250665939961823
2,10,0,10,0.0007889270782470703,3.8531382361531192
3,13,0,13,0.0011310577392578125,3.47643061415719
5,20,0,20,0.0019021034240722656,3.303295368639145
6,23,0,23,0.002228975296020508,3.229183586814669
7,26,0,26,0.0025479793548583984,2.927464202635655
8,29,0,29,0.002830982208251953,2.6576504050804624
9,32,0,32,0.003061056137084961,2.364109650726281
10,35,0,35,0.003345966339111328,1.5731827434057166
12,43,0,43,0.004054069519042969,1.4851406117614359
13,46,0,46,0.0043070316314697266,1.428959389206125
14,49,0,49,0.004554033279418945,1.3589248416048003
15,54,0,54,0.004807949066162109,1.2499892853674732
16,58,0,58,0.005051136016845703,1.1607886801500642
17,61,0,61,0.005255937576293945,1.1284557623947926
19,69,0,69,0.005774974822998047,1.0301561099391012
20,72,0,72,0.005992889404296875,0.7487005535647958
21,75,0,75,0.00622105598449707,0.7018803739227168
22,79,0,79,0.006585121154785156,0.6697371491413624
23,83,0,83,0.0069730281829833984,0.6252878423563586
24,86,0,86,0.007313251495361328,0.6040251507432601
25,89,0,89,0.007692098617553711,0.5592892115894429
27,95,0,95,0.008296012878417969,0.365015227053497
28,98,0,98,0.008512020111083984,0.27298158946372514
29,102,0,102,0.008755922317504883,0.26656227211663147
30,105,0,105,0.009026050567626953,0.24993191675182944
31,108,0,108,0.009240150451660156,0.24120720947685145
32,113,0,113,0.009492874145507812,0.23541017893173885
34,123,0,123,0.010002851486206055,0.22537494815742176
35,127,0,127,0.010236263275146484,0.22465340135002562
36,130,0,130,0.010438203811645508,0.2091375961535187
37,133,0,133,0.010641098022460938,0.14542651799264927
38,136,0,136,0.010843038558959961,0.13398403246028887
39,139,0,139,0.011039018630981445,0.13241043565502375
41,147,0,147,0.011505126953125,0.1220773126629361
42,151,0,151,0.01174020767211914,0.11559801522273995
43,154,0,154,0.01193690299987793,0.1019014160647584
44,157,0,157,0.012137889862060547,0.07236278696703202
45,160,0,160,0.01234889030456543,0.07143379541046774
46,164,0,164,0.01258397102355957,0.06941271774350248
47,168,0,168,0.012814044952392578,0.06828718231893252
49,178,0,178,0.01330709457397461,0.06677519825094716
50,183,0,183,0.013651847839355469,0.0661129047530508
51,188,0,188,0.014024019241333008,0.0655016460072836
52,193,0,193,0.014380931854248047,0.06493493450102986
53,197,0,197,0.014760971069335938,0.06349321020457878
54,200,0,200,0.015105962753295898,0.062392854417577526
56,206,0,206,0.015709877014160156,0.0557655321048715
57,209,0,209,0.015924930572509766,0.04937189799031506
58,212,0,212,0.01618194580078125,0.04770875610292767
59,216,0,216,0.016434192657470703,0.04753906751117976
60,221,0,221,0.01669025421142578,0.04695533390285294
61,225,0,225,0.016926050186157227,0.046636016804207904
62,230,0,230,0.017184019088745117,0.046210704014629275
64,240,0,240,0.017701148986816406,0.04542971184825339
65,245,0,245,0.017962932586669922,0.04506946037837129
66,250,0,250,0.018208980560302734,0.04472686424337767
67,254,0,254,0.018438100814819336,0.04470650252601006
68,258,0,258,0.01867222785949707,0.04449460159880891
69,261,0,261,0.01888108253479004,0.04408033772652264
71,267,0,267,0.0193021297454834,0.04117708832178915
72,270,0,270,0.01953411102294922,0.04089658842006494
73,275,0,275,0.01978325843811035,0.040289832328292266
74,280,0,280,0.020035982131958008,0.03972420278007966
75,285,0,285,0.020284175872802734,0.03919518381707911
76,290,0,290,0.020551204681396484,0.03869899501335227
78,300,0,300,0.021052122116088867,0.03779271042148884
79,305,0,305,0.021296024322509766,0.03737754047354443
80,310,0,310,0.021543264389038086,0.03698491596460901
81,315,0,315,0.02178502082824707,0.03661307962263415
82,320,0,320,0.02203202247619629,0.03626045812199019
83,325,0,325,0.022274017333984375,0.03592564810276821
84,329,0,329,0.022526025772094727,0.03365705210890599
86,337,0,337,0.02300119400024414,0.03158284254814927
87,342,0,342,0.023250818252563477,0.03140711289388429
88,347,0,347,0.023519039154052734,0.031249232136625883
89,351,0,351,0.023749113082885742,0.031108563700723096
90,356,0,356,0.023996829986572266,0.03097193934655896
91,361,0,361,0.02427220344543457,0.03084599209867091
93,371,0,371,0.024795055389404297,0.03062011301163786
94,376,0,376,0.025041818618774414,0.030517854336800175
95,381,0,381,0.0252840518951416,0.030421490963022442
96,386,0,386,0.02553105354309082,0.030330333207494384
97,391,0,391,0.025784015655517578,0.03024383228820408
98,396,0,396,0.02603912353515625,0.030161525723068718
100,406,0,406,0.026533126831054688,0.030007957271232896
101,411,0,411,0.02678394317626953,0.029936088229964415
102,416,0,416,0.027035236358642578,0.02986717787041467
103,421,0,421,0.02727818489074707,0.02980102277208913
104,426,0,426,0.027551889419555664,0.029737440851220525
105,431,0,431,0.02780890464782715,0.029676272547063415
106,436,0,436,0.02807021141052246,0.02961737705927143
108,446,0,446,0.028603076934814453,0.029505901587797683
109,451,0,451,0.02886819839477539,0.029453097174865103
110,456,0,456,0.02912306785583496,0.02940211498059582
111,461,0,461,0.029373884201049805,0.029352861810133073
112,466,0,466,0.029626131057739258,0.029305249283010548
113,471,0,471,0.029875993728637695,0.02925919705245527
115,481,0,481,0.030379056930541992,0.02917149639750158
116,486,0,486,0.030651092529296875,0.02912972279345215
117,491,0,491,0.030911922454833984,0.029089253290536455
118,496,0,496,0.03117203712463379,0.029050029809728904
119,501,0,501,0.03144693374633789,0.029011998511224046
120,506,0,506,0.03177905082702637,0.02897511009672682
122,516,0,516,0.03234505653381348,0.028904572532985378
123,521,0,521,0.03259015083312988,0.028870829639290545
124,526,0,526,0.032839059829711914,0.028838046323232135
125,531,0,531,0.0330810546875,0.02880618465322838
126,536,0,536,0.03332805633544922,0.0287752086963322
127,541,0,541,0.0335841178894043,0.028745083381145915
128,546,0,546,0.03382396697998047,0.028715775988208878
130,556,0,556,0.034307003021240234,0.02865950097045366
131,561,0,561,0.03454422950744629,0.028632480394039758
132,566,0,566,0.03477907180786133,0.02860616950840076
133,571,0,571,0.03501415252685547,0.02858054303909503
134,576,0,576,0.0352480411529541,0.02855557660918657
135,581,0,581,0.03548693656921387,0.02853124578637207
137,591,0,591,0.035961151123046875,0.028484391606104525
138,596,0,596,0.036195993423461914,0.02846181981392386
139,601,0,601,0.036431074142456055,0.028439787591688876
140,606,0,606,0.0366671085357666,0.02841827317936027
141,611,0,611,0.03690695762634277,0.028397256052029352
142,616,0,616,0.037145137786865234,0.028376717342738913
143,621,0,621,0.03738117218017578,0.028356639910124177
145,631,0,631,0.03785109519958496,0.028317807029574715
146,636,0,636,0.0380861759185791,0.028299023096484625
147,641,0,641,0.03832387924194336,0.028280643064314083
148,646,0,646,0.038583993911743164,0.028262654145410786
149,651,0,651,0.03882598876953125,0.02824504361895586
150,656,0,656,0.03906702995300293,0.028227798659590984
152,666,0,666,0.03954815864562988,0.028194353834574082
153,671,0,671,0.03979325294494629,0.028178128254798915
154,676,0,676,0.040038108825683594,0.02816221690358547
155,681,0,681,0.040281057357788086,0.028146607319005118
156,686,0,686,0.040521860122680664,0.028131287509833524
157,691,0,691,0.04077410697937012,0.028116246071497653
159,701,0,701,0.04126095771789551,0.028086955513063016
160,706,0,706,0.04150509834289551,0.028072686432879777
161,711,0,711,0.04174685478210449,0.02805865589064311
162,716,0,716,0.04198813438415527,0.028044855391187232
163,721,0,721,0.04222893714904785,0.02803127683849535
164,726,0,726,0.04248404502868652,0.028017912480312934
165,731,0,731,0.04273509979248047,0.028004754925156573
167,741,0,741,0.04322314262390137,0.027979032271140458
168,746,0,746,0.043467044830322266,0.027966453789198355
169,751,0,751,0.04370999336242676,0.02795405532213324
170,756,0,756,0.04401826858520508,0.02794183079958178
171,761,0,761,0.04427695274353027,0.027929774430559804
172,766,0,766,0.04454183578491211,0.027917880672325705
174,776,0,776,0.04503202438354492,0.027894560095486524
175,781,0,781,0.045287132263183594,0.027883123567913195
176,786,0,786,0.0455479621887207,0.027871830250679176
177,791,0,791,0.045790910720825195,0.027860676033852165
178,796,0,796,0.04604005813598633,0.02784965710183529
179,801,0,801,0.046285152435302734,0.027838769950725376
181,811,0,811,0.04677605628967285,0.02781737847894494
182,816,0,816,0.04702305793762207,0.027806868545313845
183,821,0,821,0.04731321334838867,0.02779647909043671
184,826,0,826,0.04758024215698242,0.02778620778089133
185,831,0,831,0.04782509803771973,0.027776052385029854
186,836,0,836,0.04807305335998535,0.02776601070291916
187,841,0,841,0.04831504821777344,0.027756080505161932
189,851,0,851,0.048835039138793945,0.027736545250110933
190,856,0,856,0.04909014701843262,0.027726935239007374
191,861,0,861,0.04933905601501465,0.027717426748781148
192,866,0,866,0.049616098403930664,0.027708016906913813
193,871,0,871,0.049871206283569336,0.027698702691956296
194,876,0,876,0.050132036209106445,0.027689480954807152
196,886,0,886,0.050653934478759766,0.0276713018132495
197,891,0,891,0.050916194915771484,0.027662337695034084
198,896,0,896,0.051177978515625,0.02765345269953784
199,901,0,901,0.051434993743896484,0.027644643465558585
200,906,0,906,0.051696062088012695,0.02763590668297691
201,911,0,911,0.05195426940917969,0.027627239118761734
203,921,0,921,0.05246996879577637,0.027610099256413233
204,926,0,926,0.05274486541748047,0.027601621101309582
205,931,0,931,0.05300092697143555,0.02759320048524791
206,936,0,936,0.05326199531555176,0.02758483489382619
207,941,0,941,0.05351710319519043,0.027576522007604062
208,946,0,946,0.05377793312072754,0.02756825971484573
209,951,0,951,0.05403590202331543,0.027560046119906218
211,961,0,961,0.054553985595703125,0.027543758549757436
212,966,0,966,0.05481386184692383,0.02753568189395366
213,971,0,971,0.05507516860961914,0.027527648562799066
214,976,0,976,0.055336952209472656,0.02751965773408677
215,981,0,981,0.05560803413391113,0.027511708761430127
216,986,0,986,0.05586099624633789,0.027503801150138726
218,996,0,996,0.056365013122558594,0.02748810862075423
219,1001,0,1001,0.05661320686340332,0.027480323207808084
220,1006,0,1006,0.05686593055725098,0.027472578104598577
221,1011,0,1011,0.05711507797241211,0.02746487312828562
222,1016,0,1016,0.05737018585205078,0.027457208073883802
223,1021,0,1021,0.05762195587158203,0.02744958269289922
224,1026,0,1026,0.05788016319274902,0.02744199667690138
226,1036,0,1036,0.058381080627441406,0.02742694114573877
227,1041,0,1041,0.05864119529724121,0.02741947064051377
228,1046,0,1046,0.058895111083984375,0.027412037522515507
229,1051,0,1051,0.05915999412536621,0.027404641116928058
230,1056,0,1056,0.059411048889160156,0.02739728069413539
231,1061,0,1061,0.059676170349121094,0.027389955484018316
233,1071,0,1071,0.06018400192260742,0.027375407515529155
234,1076,0,1076,0.060437917709350586,0.027368183161841874
235,1081,0,1081,0.06068921089172363,0.02736099086305885
236,1086,0,1086,0.060945987701416016,0.02735382989038313
237,1091,0,1091,0.06119489669799805,0.027346699565006273
238,1096,0,1096,0.0614471435546875,0.027339599265920146
240,1106,0,1106,0.06194496154785156,0.027325486574257117
241,1111,0,1111,0.062194108963012695,0.02731847325022875
242,1116,0,1116,0.06244611740112305,0.027311488081295538
243,1121,0,1121,0.06269311904907227,0.027304530733331035
244,1126,0,1126,0.06294608116149902,0.02729760090953389
245,1131,0,1131,0.06319403648376465,0.02729069834003918
246,1136,0,1136,0.063446044921875,0.02728382277130068
248,1146,0,1146,0.06396007537841797,0.027270151643643003
249,1151,0,1151,0.06420087814331055,0.027263355573363214
250,1156,0,1156,0.06444692611694336,0.027256585467150304
251,1161,0,1161,0.06468915939331055,0.02724984102558396
252,1166,0,1166,0.06493902206420898,0.027243121924920788
253,1171,0,1171,0.06518006324768066,0.02723642781583484
255,1181,0,1181,0.06566596031188965,0.02722311304923823
256,1186,0,1186,0.06591010093688965,0.02721649157223756
257,1191,0,1191,0.06615114212036133,0.027209893453345898
258,1196,0,1196,0.06641197204589844,0.027203318238549486
259,1201,0,1201,0.06664800643920898,0.02719676546324824
260,1206,0,1206,0.06688714027404785,0.02719023465672303
262,1216,0,1216,0.06736397743225098,0.027177237064022242
263,1221,0,1221,0.06761693954467773,0.02717076934684195
264,1226,0,1226,0.06786394119262695,0.027164321744930525
265,1231,0,1231,0.06810593605041504,0.02715789382326552
266,1236,0,1236,0.06835103034973145,0.027151485165241015
267,1240,0,1240,0.06857895851135254,0.02713864562911509
268,1245,0,1245,0.06882500648498535,0.027128156901796537
270,1255,0,1255,0.06931304931640625,0.027108368272108795
271,1260,0,1260,0.06955504417419434,0.027098966999433278
272,1265,0,1265,0.06979990005493164,0.027089840307477672
273,1270,0,1270,0.07004117965698242,0.027080958733873898
274,1274,0,1274,0.07027292251586914,0.027066689222577517
275,1279,0,1279,0.07051491737365723,0.0270540258536676
277,1289,0,1289,0.07100892066955566,0.027030435793330615
278,1294,0,1294,0.07125496864318848,0.0270193647276227
279,1299,0,1299,0.07149600982666016,0.027008695049277744
280,1304,0,1304,0.07174086570739746,0.02699838359847791
281,1309,0,1309,0.07198309898376465,0.026988396861171788
282,1313,0,1313,0.07221508026123047,0.026972757951651057
284,1323,0,1323,0.07271122932434082,0.026946865796205578
285,1328,0,1328,0.07294702529907227,0.02693510731723154
286,1333,0,1333,0.07318592071533203,0.026923965527402626
287,1338,0,1338,0.07342100143432617,0.026913342330954222
288,1343,0,1343,0.07366013526916504,0.026903163529566135
289,1348,0,1348,0.07389402389526367,0.02689336888412069
290,1353,0,1353,0.07413196563720703,0.02688390461791578
292,1363,0,1363,0.07460713386535645,0.026865786082740664
293,1368,0,1368,0.07484102249145508,0.0268570659341876
294,1373,0,1373,0.07507920265197754,0.026848540904552447
295,1378,0,1378,0.07531309127807617,0.026840191541409382
296,1383,0,1383,0.0755620002746582,0.026832000057246976
297,1388,0,1388,0.07579803466796875,0.026823951589555677
299,1398,0,1398,0.07627201080322266,0.02680823593290346
300,1403,0,1403,0.07651090621948242,0.026800546537612387
301,1408,0,1408,0.07674598693847656,0.026792956187190933
302,1413,0,1413,0.07698607444763184,0.026785457306720356
303,1418,0,1418,0.07722115516662598,0.026778043220258476
304,1423,0,1423,0.07746291160583496,0.02677070673028807
305,1428,0,1428,0.0776970386505127,0.026763440322234145
307,1438,0,1438,0.07817220687866211,0.026749094015454705
308,1443,0,1443,0.07841110229492188,0.02674200599750481
309,1448,0,1448,0.07865214347839355,0.026734969991858728
310,1453,0,1453,0.07889103889465332,0.02672798240690942
311,1458,0,1458,0.07912802696228027,0.026721040249395093
312,1463,0,1463,0.07936716079711914,0.026714141264426908
314,1473,0,1473,0.07984304428100586,0.026700464568095352
315,1478,0,1478,0.080078125,0.026693682695876016
316,1483,0,1483,0.08031797409057617,0.02668693631725861
317,1488,0,1488,0.08055591583251953,0.02668022436364728
318,1493,0,1493,0.08080196380615234,0.026673545803223665
319,1498,0,1498,0.08103799819946289,0.026666899519265073
321,1508,0,1508,0.08151698112487793,0.02665369988157136
322,1513,0,1513,0.0817568302154541,0.026647144856875245
323,1518,0,1518,0.08199286460876465,0.026640618471932172
324,1523,0,1523,0.08223199844360352,0.02663411979684516
325,1528,0,1528,0.08246493339538574,0.026627648112621534
326,1533,0,1533,0.08270406723022461,0.026621202871329346
327,1538,0,1538,0.08293819427490234,0.02661478346745678
329,1548,0,1548,0.08341193199157715,0.02660201900324444
330,1553,0,1553,0.08365011215209961,0.026595672346341595
331,1558,0,1558,0.08388495445251465,0.02658934840273673
332,1563,0,1563,0.08412408828735352,0.0265830462830499
333,1568,0,1568,0.08435821533203125,0.026576764950534012
334,1573,0,1573,0.08462309837341309,0.02657050337454721
336,1583,0,1583,0.08512401580810547,0.02655803591486202
337,1588,0,1588,0.0853722095489502,0.026551828360433738
338,1593,0,1593,0.08562397956848145,0.02654563718719905
339,1598,0,1598,0.08587217330932617,0.026539461749769053
340,1603,0,1603,0.08612394332885742,0.02653330157827453
341,1608,0,1608,0.08637309074401855,0.026527156312246874
343,1618,0,1618,0.08687686920166016,0.026514909342716084
344,1623,0,1623,0.08712196350097656,0.02650880727781811
345,1628,0,1628,0.08736515045166016,0.026502719403918684
346,1633,0,1633,0.08761382102966309,0.02649664568719961
347,1638,0,1638,0.08785510063171387,0.026490586066813555
348,1643,0,1643,0.08810114860534668,0.026484540461561658
349,1648,0,1648,0.08834314346313477,0.02647850877387098
351,1658,0,1658,0.08882808685302734,0.02646648647626488
352,1663,0,1663,0.08907318115234375,0.026460495302195037
353,1668,0,1668,0.08932089805603027,0.02645451694071303
354,1673,0,1673,0.08956599235534668,0.026448550952367998
355,1678,0,1678,0.08980822563171387,0.026442596851698835
356,1683,0,1683,0.09005403518676758,0.026436654109777635
358,1693,0,1693,0.09054112434387207,0.026424800539655437
359,1698,0,1698,0.0907890796661377,0.026418888699252928
360,1703,0,1703,0.09103512763977051,0.026412986215335582
361,1708,0,1708,0.09127593040466309,0.026407092691210898
362,1713,0,1713,0.09152102470397949,0.026401207795266828
363,1718,0,1718,0.09176206588745117,0.02639533127470486
365,1728,0,1728,0.09224796295166016,0.026383602715835515
366,1733,0,1733,0.09249520301818848,0.0263777505080281
367,1738,0,1738,0.09273600578308105,0.02637190632839646
368,1743,0,1743,0.09298205375671387,0.026366070224511564
369,1748,0,1748,0.09322381019592285,0.026360242275481987
370,1753,0,1753,0.09346890449523926,0.026354422574467806
371,1758,0,1758,0.09371018409729004,0.026348611218396063
373,1768,0,1768,0.09420204162597656,0.026337013903434205
374,1773,0,1773,0.09444808959960938,0.02633122807799438
375,1778,0,1778,0.09468889236450195,0.02632545084027596
376,1783,0,1783,0.09493398666381836,0.026319682163995984
377,1788,0,1788,0.09517598152160645,0.026313921978977226
378,1793,0,1793,0.09542083740234375,0.02630817016663895
380,1803,0,1803,0.09590816497802734,0.0262966909214558
381,1808,0,1808,0.09614896774291992,0.02629096299180711
382,1813,0,1813,0.09639406204223633,0.026285242450986412
383,1818,0,1818,0.09664726257324219,0.02627952894474493
384,1823,0,1823,0.09688496589660645,0.02627382208615892
385,1828,0,1828,0.09711885452270508,0.026268121465189562
386,1833,0,1833,0.09735798835754395,0.026262426660318822
388,1843,0,1843,0.09783196449279785,0.02625105281898063
389,1848,0,1848,0.09806704521179199,0.026245372974390023
390,1853,0,1853,0.09830498695373535,0.02623969734978556
391,1858,0,1858,0.09854006767272949,0.026234025617461895
392,1863,0,1863,0.09877800941467285,0.026228357493993607
393,1868,0,1868,0.09901213645935059,0.026222692743820022
395,1878,0,1878,0.09949684143066406,0.026211372672307987
396,1883,0,1883,0.09972405433654785,0.026205717130923453
397,1888,0,1888,0.09994697570800781,0.026200064516527257
398,1893,0,1893,0.10017991065979004,0.026194414826849893
399,1898,0,1898,0.10040283203125,0.026188768091440013
400,1903,0,1903,0.10064315795898438,0.026183124364486002
402,1913,0,1913,0.1010899543762207,0.026171846227572303
403,1918,0,1918,0.10130810737609863,0.026166211976460938
404,1923,0,1923,0.10154485702514648,0.026160581037380965
405,1928,0,1928,0.10176801681518555,0.02615495347298897
406,1933,0,1933,0.10199403762817383,0.026149329330112443
407,1938,0,1938,0.1022179126739502,0.026143708636273914
408,1943,0,1943,0.10244393348693848,0.02613809139776438
410,1953,0,1953,0.10289406776428223,0.02612686720403735
411,1958,0,1958,0.10311698913574219,0.0261212601559398
412,1963,0,1963,0.10334205627441406,0.026115656380785262
413,1968,0,1968,0.10357499122619629,0.026110055789610127
414,1973,0,1973,0.10379695892333984,0.02610445828198514
415,1978,0,1978,0.10401415824890137,0.02609886374945291
417,1988,0,1988,0.10446786880493164,0.026087683155565315
418,1993,0,1993,0.10469388961791992,0.02608209686662183
419,1998,0,1998,0.10491585731506348,0.0260765131034056
420,2003,0,2003,0.10514307022094727,0.026070931763792767
421,2008,0,2008,0.10536599159240723,0.02606535275375664
422,2013,0,2013,0.10559296607971191,0.026059775988559356
424,2023,0,2023,0.1060478687286377,0.026048628904361413
425,2028,0,2028,0.10627102851867676,0.026043058466931744
426,2033,0,2033,0.10649800300598145,0.0260374900368265
427,2038,0,2038,0.106719970703125,0.026031923578658207
428,2043,0,2043,0.10694694519042969,0.026026359065225924
429,2048,0,2048,0.10717105865478516,0.026020796476511104
430,2053,0,2053,0.10739707946777344,0.02601523579859369
432,2063,0,2063,0.10787105560302734,0.0260041201438572
433,2068,0,2068,0.10809898376464844,0.025998565160939492
434,2073,0,2073,0.10833001136779785,0.025993012075148023
435,2078,0,2078,0.10855817794799805,0.02598746088995531
436,2083,0,2083,0.10879111289978027,0.0259819116107896
437,2088,0,2088,0.10902023315429688,0.02597636424504959
439,2098,0,2098,0.10949301719665527,0.025965275294812767
440,2103,0,2103,0.10971903800964355,0.02595973373790315
441,2108,0,2108,0.10994195938110352,0.025954194150957066
442,2113,0,2113,0.1101691722869873,0.02594865655816679
443,2118,0,2118,0.11039113998413086,0.02594312098945891
444,2123,0,2123,0.11061811447143555,0.025937587481385718
446,2133,0,2133,0.11107301712036133,0.025926526831473447
447,2138,0,2138,0.11129498481750488,0.025920999802971807
448,2143,0,2143,0.1115260124206543,0.02591547506278954
449,2148,0,2148,0.11174917221069336,0.0259099526906835
450,2153,0,2153,0.11197590827941895,0.025904432775826103
451,2158,0,2158,0.11219906806945801,0.025898915416558185
452,2163,0,2163,0.1124410629272461,0.02589340071990961
454,2173,0,2173,0.11290216445922852,0.025882379781684683
455,2178,0,2178,0.11312985420227051,0.025876873790485626
456,2183,0,2183,0.11336183547973633,0.0258713709604969
457,2188,0,2188,0.11360621452331543,0.02586587142864114
458,2193,0,2193,0.11383295059204102,0.02586037533432002
459,2198,0,2198,0.11405587196350098,0.025854882818171596
461,2208,0,2208,0.11450505256652832,0.025843909082053577
462,2213,0,2213,0.1147298812866211,0.025838428139238027
463,2218,0,2218,0.11495304107666016,0.025832951327026645
464,2223,0,2223,0.11517786979675293,0.02582747877634974
465,2228,0,2228,0.11540102958679199,0.025822010613911654
466,2233,0,2233,0.11562705039978027,0.02581654696178628
467,2238,0,2238,0.11584782600402832,0.02581108793716711
469,2248,0,2248,0.11629796028137207,0.02580018421433632
470,2253,0,2253,0.11652493476867676,0.025794739725837082
471,2258,0,2258,0.11674690246582031,0.025789300284655925
472,2263,0,2263,0.1169731616973877,0.025783865984434752
473,2268,0,2268,0.11719298362731934,0.025778436914939425
474,2273,0,2273,0.11742305755615234,0.025773013162464983
476,2283,0,2283,0.11787009239196777,0.025762181938889534
477,2288,0,2288,0.11809301376342773,0.025756774626700646
478,2293,0,2293,0.11832022666931152,0.025751372950071235
479,2298,0,2298,0.11854100227355957,0.02574597698372741
480,2303,0,2303,0.11876821517944336,0.025740586800934603
481,2308,0,2308,0.1189889907836914,0.025735202473612113
483,2318,0,2318,0.11943697929382324,0.025724451666363876
484,2323,0,2323,0.11966419219970703,0.025719085323266947
485,2328,0,2328,0.11988615989685059,0.025713725108861284
486,2333,0,2333,0.12011218070983887,0.02570837108675788
487,2338,0,2338,0.12033295631408691,0.02570302331795688
488,2343,0,2343,0.1205589771270752,0.02569768186036289
489,2348,0,2348,0.12078595161437988,0.025692346768258358
491,2358,0,2358,0.12123489379882812,0.025681695876256423
492,2363,0,2363,0.1214609146118164,0.025676380161917606
493,2368,0,2368,0.12168288230895996,0.025671070983184992
494,2373,0,2373,0.12191009521484375,0.025665768368372963
495,2378,0,2378,0.1221320629119873,0.025660472339332337
496,2383,0,2383,0.12235808372497559,0.025655182911212306
498,2393,0,2393,0.12280607223510742,0.02564462388413116
499,2398,0,2398,0.12302899360656738,0.025639354281309742
500,2403,0,2403,0.1232609748840332,0.025634091271972272
501,2408,0,2408,0.12348484992980957,0.025628834837951878
502,2413,0,2413,0.12371087074279785,0.025623584955193044
503,2418,0,2418,0.1239328384399414,0.02561834159421661
505,2428,0,2428,0.12438082695007324,0.025607874295766962
506,2433,0,2433,0.12460684776306152,0.02560265027712795
507,2438,0,2438,0.12483000755310059,0.025597432619115665
508,2443,0,2443,0.12505698204040527,0.025592221273529545
509,2448,0,2448,0.12527894973754883,0.0255870161901085
510,2453,0,2453,0.1255648136138916,0.025581817317000842
511,2458,0,2458,0.12578821182250977,0.02557662460115893
513,2468,0,2468,0.1262362003326416,0.025566257424846354
514,2473,0,2473,0.12646198272705078,0.025561082854564765
515,2478,0,2478,0.12672901153564453,0.025555914222027402
516,2483,0,2483,0.12695598602294922,0.02555075147077095
517,2488,0,2488,0.12717795372009277,0.02554559454343456
518,2493,0,2493,0.12740612030029297,0.025540443381462264
520,2503,0,2503,0.1278550624847412,0.025530158111098208
521,2508,0,2508,0.1280839443206787,0.025525023875956353
522,2513,0,2513,0.128309965133667,0.02551989515169556
523,2518,0,2518,0.12853288650512695,0.02551477186721207
524,2523,0,2523,0.12875914573669434,0.02550965394741034
525,2528,0,2528,0.12898612022399902,0.025504541312740367
527,2538,0,2538,0.12943792343139648,0.025494331555896105
528,2543,0,2543,0.12966489791870117,0.025489234248935188
529,2548,0,2548,0.12988901138305664,0.02548414185705282
530,2553,0,2553,0.13011598587036133,0.025479054273586127
531,2558,0,2558,0.13033795356750488,0.025473971386032458
532,2563,0,2563,0.13056612014770508,0.02546889307611477
533,2568,0,2568,0.13084006309509277,0.02546381921993312
535,2578,0,2578,0.1313788890838623,0.0254536843465455
536,2583,0,2583,0.1316061019897461,0.025448623055907896
537,2588,0,2588,0.13182902336120605,0.025443565672963835
538,2593,0,2593,0.13205599784851074,0.02543851205062695
539,2598,0,2598,0.1322779655456543,0.025433462038583817
540,2603,0,2603,0.13250517845153809,0.025428415483865575
542,2613,0,2613,0.13295698165893555,0.025418332124855083
543,2618,0,2618,0.1331801414489746,0.025413295006809288
544,2623,0,2623,0.13348817825317383,0.02540826071983647
545,2628,0,2628,0.13371491432189941,0.025403229106904384
546,2633,0,2633,0.1339859962463379,0.025398200012037787
547,2638,0,2638,0.13421106338500977,0.025393173280922384
548,2643,0,2643,0.13451910018920898,0.02538814876149088
550,2653,0,2653,0.13528704643249512,0.02537810576400121
551,2658,0,2658,0.13565421104431152,0.02537308699798415
552,2663,0,2663,0.13596892356872559,0.025368069868718333
553,2668,0,2668,0.13619399070739746,0.025363054243260862
554,2673,0,2673,0.13642120361328125,0.025358039993844117
555,2678,0,2678,0.13664507865905762,0.02535302699823428
557,2688,0,2688,0.13718080520629883,0.0253430043089913
558,2693,0,2693,0.1374530792236328,0.02533799440111367
559,2698,0,2698,0.13772320747375488,0.025332985318913363
560,2703,0,2703,0.13794612884521484,0.025327976971450377
561,2708,0,2708,0.13834905624389648,0.025322969274369993
562,2713,0,2713,0.13860607147216797,0.02531796214986562
564,2723,0,2723,0.13904905319213867,0.025307949339421706
565,2728,0,2728,0.1392660140991211,0.025302943529369255
566,2733,0,2733,0.13948893547058105,0.025297938043149726
567,2738,0,2738,0.13970708847045898,0.025292932832914033
568,2743,0,2743,0.13992905616760254,0.02528792785584598
569,2748,0,2748,0.14014792442321777,0.025282923073736585
570,2753,0,2753,0.14036989212036133,0.025277918452531224
572,2763,0,2763,0.1408381462097168,0.025267909574563076
573,2768,0,2768,0.14106106758117676,0.02526290526622582
574,2772,0,2772,0.14127421379089355,0.02525124562688441
575,2777,0,2777,0.14149713516235352,0.02524199500606629
576,2782,0,2782,0.14173007011413574,0.025233180877829657
577,2787,0,2787,0.1419529914855957,0.025224733758052956
579,2795,0,2795,0.1423799991607666,0.025161895554419018
580,2799,0,2799,0.1425950527191162,0.0251464981535766
581,2804,0,2804,0.14281916618347168,0.025129269769810093
582,2809,0,2809,0.14304614067077637,0.025112890133950825
583,2813,0,2813,0.14325714111328125,0.02510127337215882
584,2818,0,2818,0.14348483085632324,0.02508463536435819
586,2827,0,2827,0.1439211368560791,0.025029716885337915
587,2832,0,2832,0.14414405822753906,0.025014915295573294
588,2837,0,2837,0.14437007904052734,0.02500067423644542
589,2842,0,2842,0.1445939540863037,0.024986934764756615
590,2847,0,2847,0.144819974899292,0.024973635199284624
591,2852,0,2852,0.14504194259643555,0.02496071517786864
592,2857,0,2857,0.14526891708374023,0.024948130678928856
594,2867,0,2867,0.14581298828125,0.0249238557892673
595,2872,0,2872,0.14603686332702637,0.02491210839454105
596,2877,0,2877,0.14626407623291016,0.024900584577251375
597,2882,0,2882,0.14648795127868652,0.024889268308271935
598,2886,0,2886,0.14670419692993164,0.024851273593198515
599,2891,0,2891,0.146928071975708,0.024827150817976797
601,2901,0,2901,0.14746499061584473,0.02478461869376803
602,2906,0,2906,0.14769887924194336,0.02476553729697829
603,2911,0,2911,0.14792180061340332,0.024747567097105357
604,2916,0,2916,0.1481480598449707,0.024730512970314027
605,2921,0,2921,0.14837098121643066,0.024714224796253098
606,2926,0,2926,0.14859890937805176,0.0246985824380741
608,2936,0,2936,0.1490480899810791,0.024668842433005045
609,2941,0,2941,0.14927101135253906,0.02465460100559103
610,2946,0,2946,0.14949703216552734,0.024640718271425163
611,2951,0,2951,0.1497211456298828,0.024627159166943212
612,2956,0,2956,0.1499481201171875,0.024613887220904372
613,2961,0,2961,0.15017104148864746,0.024600869910798004
614,2966,0,2966,0.15039682388305664,0.024588084606551184
616,2976,0,2976,0.15085315704345703,0.024563144526873342
617,2981,0,2981,0.15107512474060059,0.024550952806038598
618,2986,0,2986,0.15130114555358887,0.024538923121899148
619,2991,0,2991,0.15152406692504883,0.024527045140852324
620,2996,0,2996,0.15175104141235352,0.02451531187674653
621,3001,0,3001,0.15197420120239258,0.024503714563703892
623,3011,0,3011,0.15242314338684082,0.024480886949455587
624,3016,0,3016,0.15264892578125,0.024469641901110433
625,3021,0,3021,0.15287303924560547,0.024458502131682144
626,3026,0,3026,0.15309786796569824,0.024447461202687034
627,3031,0,3031,0.15332603454589844,0.02443651282378287
628,3036,0,3036,0.15355324745178223,0.0244256525714055
629,3041,0,3041,0.1537761688232422,0.02441487737699572
631,3051,0,3051,0.15422606468200684,0.024393568446063163
632,3056,0,3056,0.15445184707641602,0.024383027685131363
633,3061,0,3061,0.15471792221069336,0.024372559340102618
634,3066,0,3066,0.15494489669799805,0.024362161301880746
635,3071,0,3071,0.1551680564880371,0.024351830972839855
636,3076,0,3076,0.1553950309753418,0.024341565526790787
638,3086,0,3086,0.15584397315979004,0.024321220313518622
639,3091,0,3091,0.1560659408569336,0.0243111370659839
640,3096,0,3096,0.15629315376281738,0.024301110959117835
641,3101,0,3101,0.15651607513427734,0.02429114012780775
642,3106,0,3106,0.15674304962158203,0.024281223075674287
643,3111,0,3111,0.15696501731872559,0.02427135863383264
645,3121,0,3121,0.15741300582885742,0.024251782540922816
646,3126,0,3126,0.1576392650604248,0.02424206806000556
647,3131,0,3131,0.15786099433898926,0.02423240096058427
648,3136,0,3136,0.15808796882629395,0.02422278021890103
649,3141,0,3141,0.158311128616333,0.02421320480752115
650,3146,0,3146,0.1585369110107422,0.024203673697320294
651,3151,0,3151,0.15876102447509766,0.02419418599117609
653,3161,0,3161,0.15921401977539062,0.024175337870932272
654,3166,0,3166,0.15944123268127441,0.02416597599983756
655,3171,0,3171,0.15966510772705078,0.024156654574113572
656,3176,0,3176,0.15989089012145996,0.02414737288163996
657,3181,0,3181,0.16011404991149902,0.02413813022935322
658,3186,0,3186,0.1603410243988037,0.024128925873503227
660,3196,0,3196,0.1607952117919922,0.024110628822908337
661,3201,0,3201,0.16101908683776855,0.024101534490104753
662,3206,0,3206,0.16124582290649414,0.024092475163250866
663,3211,0,3211,0.1614689826965332,0.02408344994125024
664,3216,0,3216,0.1616959571838379,0.02407445789483538
665,3221,0,3221,0.16191887855529785,0.02406549810526228
667,3231,0,3231,0.162369966506958,0.02404767172994408
668,3235,0,3235,0.1625840663909912,0.023978969461699133
669,3240,0,3240,0.16280698776245117,0.02394970923825519
670,3245,0,3245,0.16303420066833496,0.02392436267942075
671,3250,0,3250,0.16325616836547852,0.023902085376789
672,3255,0,3255,0.1634831428527832,0.02388221433675906
673,3260,0,3260,0.1637129783630371,0.023864239615249812
675,3269,0,3269,0.164154052734375,0.02382989085985306
676,3274,0,3274,0.1643810272216797,0.02375229002733949
677,3279,0,3279,0.16460490226745605,0.02368866075403447
678,3284,0,3284,0.16483712196350098,0.02363596136569743
679,3289,0,3289,0.16506218910217285,0.02359182901776294
680,3294,0,3294,0.16528892517089844,0.02355444073033394
682,3304,0,3304,0.1657390594482422,0.023494502544826087
683,3309,0,3309,0.16596293449401855,0.0234699505414532
684,3314,0,3314,0.16618895530700684,0.023448065546558802
685,3319,0,3319,0.1664109230041504,0.023428348216534757
686,3323,0,3323,0.16672992706298828,0.023399874570025167
687,3328,0,3328,0.16698122024536133,0.02318628216321106
689,3338,0,3338,0.1674330234527588,0.02287712319307391
690,3343,0,3343,0.1676640510559082,0.022765590316713394
691,3348,0,3348,0.16787505149841309,0.022674893392423925
692,3353,0,3353,0.16808795928955078,0.022600777340888004
693,3358,0,3358,0.16829895973205566,0.022539869653770125
694,3363,0,3363,0.16851305961608887,0.022489441958843233
695,3368,0,3368,0.16872406005859375,0.022447306352746506
697,3378,0,3378,0.16921496391296387,0.022381461824366438
698,3383,0,3383,0.16949701309204102,0.022355430498444476
699,3388,0,3388,0.16984915733337402,0.02233283691428922
700,3392,0,3392,0.17008614540100098,0.022111416439716453
701,3397,0,3397,0.17029714584350586,0.021996012679391858
702,3401,0,3401,0.17049908638000488,0.021914107817700167
704,3411,0,3411,0.17093801498413086,0.021784631766488916
705,3416,0,3416,0.17114710807800293,0.021733562725095516
706,3421,0,3421,0.17136096954345703,0.02168948520640234
707,3426,0,3426,0.1715710163116455,0.02165113028929833
708,3431,0,3431,0.1717832088470459,0.021617477016586294
709,3436,0,3436,0.17199301719665527,0.021587730155990005
710,3441,0,3441,0.17220497131347656,0.02156124844100331
712,3451,0,3451,0.17262697219848633,0.021515996757891558
713,3456,0,3456,0.1728370189666748,0.021496438296489395
714,3461,0,3461,0.173051118850708,0.02147853212992469
715,3466,0,3466,0.17325997352600098,0.021462034757915964
716,3471,0,3471,0.17347192764282227,0.021446720756794883
717,3476,0,3476,0.17368102073669434,0.0214324098897975
719,3486,0,3486,0.17410516738891602,0.021406326447155073
720,3491,0,3491,0.1743171215057373,0.021394360341220636
721,3496,0,3496,0.17452502250671387,0.021382979293379865
722,3501,0,3501,0.17473793029785156,0.02137210720469461
723,3506,0,3506,0.17494702339172363,0.021361694563079965
724,3511,0,3511,0.17516016960144043,0.021351700480896067
726,3521,0,3521,0.17562103271484375,0.02133278093808614
727,3526,0,3526,0.17582988739013672,0.02132377519381118
728,3531,0,3531,0.1760420799255371,0.021315041382329033
729,3536,0,3536,0.1762559413909912,0.021306561199154018
730,3541,0,3541,0.1764678955078125,0.021298309566420075
731,3546,0,3546,0.1766810417175293,0.021290260759375075
732,3551,0,3551,0.176893949508667,0.02128239748189811
734,3561,0,3561,0.17731499671936035,0.021267183239203274
735,3566,0,3566,0.17752504348754883,0.02125980305407909
736,3571,0,3571,0.1777358055114746,0.021252554006268437
737,3576,0,3576,0.17794513702392578,0.021245427585615997
738,3581,0,3581,0.17815709114074707,0.02123841733729386
739,3586,0,3586,0.17836594581604004,0.0212315136089906
741,3596,0,3596,0.17878508567810059,0.021217981809505918
742,3601,0,3601,0.17903804779052734,0.02121134043225785
743,3606,0,3606,0.1792459487915039,0.021204776680179505
744,3611,0,3611,0.1794581413269043,0.02119828455134666
745,3616,0,3616,0.17966699600219727,0.021191857609454235
746,3621,0,3621,0.17987918853759766,0.02118549203685979
748,3631,0,3631,0.1802990436553955,0.021172939086887076
749,3636,0,3636,0.18050813674926758,0.021166746457794323
750,3641,0,3641,0.18072223663330078,0.021160605070020686
751,3646,0,3646,0.18093109130859375,0.021154513127344638
752,3651,0,3651,0.18114399909973145,0.021148469815254187
753,3656,0,3656,0.18135285377502441,0.021142473516247717
754,3661,0,3661,0.18156909942626953,0.021136521608739255
756,3671,0,3671,0.18198919296264648,0.021124742966829365
757,3676,0,3676,0.18219804763793945,0.021118914094163756
758,3681,0,3681,0.18241000175476074,0.02111312357434157
759,3686,0,3686,0.1826190948486328,0.021107369344304492
760,3691,0,3691,0.1828310489654541,0.021101649764254434
761,3696,0,3696,0.18306303024291992,0.021095963748486872
763,3706,0,3706,0.18349909782409668,0.021084687233180674
764,3711,0,3711,0.1837301254272461,0.021079093380136568
765,3716,0,3716,0.18395495414733887,0.02107352725424467
766,3721,0,3721,0.18417811393737793,0.02106798785013937
767,3726,0,3726,0.1844010353088379,0.021062474022379204
768,3731,0,3731,0.18463897705078125,0.021056984386149415
770,3741,0,3741,0.18507599830627441,0.021046072780123232
771,3746,0,3746,0.18529415130615234,0.021040648954873516
772,3750,0,3750,0.18550491333007812,0.020999560032069473
773,3755,0,3755,0.18572688102722168,0.02099101401763718
774,3759,0,3759,0.18593311309814453,0.020789843213600345
775,3764,0,3764,0.18615007400512695,0.02077347053965485
776,3769,0,3769,0.1863880157470703,0.020758726026587956
778,3779,0,3779,0.18683695793151855,0.02073299150525714
779,3784,0,3784,0.18705987930297852,0.020721576474893755
780,3789,0,3789,0.18729400634765625,0.02071091872028325
781,3794,0,3794,0.18751788139343262,0.02070089625093696
782,3799,0,3799,0.18774080276489258,0.020691404689700963
783,3804,0,3804,0.18796420097351074,0.02068235655001808
785,3814,0,3814,0.18841910362243652,0.02066533683317147
786,3819,0,3819,0.18864107131958008,0.020657275825201726
787,3824,0,3824,0.18886303901672363,0.020649465002592276
788,3829,0,3829,0.18909215927124023,0.02064187168565404
789,3834,0,3834,0.189316987991333,0.020634469686944188
790,3839,0,3839,0.1895589828491211,0.02062723917969535
791,3844,0,3844,0.18978619575500488,0.020620163309240748
793,3854,0,3854,0.19025206565856934,0.020606415140683704
794,3859,0,3859,0.19048118591308594,0.02059971908888768
795,3864,0,3864,0.19070887565612793,0.020593129732715768
796,3869,0,3869,0.1909470558166504,0.02058663924974401
797,3874,0,3874,0.1911768913269043,0.02058024051930164
798,3879,0,3879,0.1914050579071045,0.020573927366277472
800,3889,0,3889,0.19186806678771973,0.020561534721611926
801,3894,0,3894,0.19209814071655273,0.020555444067656956
802,3899,0,3899,0.19232892990112305,0.020549417996498724
803,3904,0,3904,0.19257593154907227,0.020543453475661444
804,3909,0,3909,0.19281816482543945,0.02053754742507177
805,3914,0,3914,0.19305706024169922,0.020531696204177084
807,3924,0,3924,0.19354605674743652,0.020520145010435076
808,3929,0,3929,0.19378209114074707,0.02051444045735736
809,3934,0,3934,0.19401288032531738,0.020508780551696883
810,3939,0,3939,0.1942429542541504,0.020503162849433428
811,3944,0,3944,0.1944730281829834,0.02049758506289177
812,3949,0,3949,0.19470787048339844,0.020492045459560317
813,3954,0,3954,0.19493913650512695,0.020486542545269375
815,3964,0,3964,0.19541001319885254,0.020475639608132416
816,3969,0,3969,0.19568204879760742,0.02047023592068015
817,3974,0,3974,0.1959090232849121,0.020464862161815353
818,3979,0,3979,0.19613313674926758,0.02045951707505203
819,3984,0,3984,0.19635605812072754,0.020454199300588644
820,3989,0,3989,0.19658899307250977,0.020448907543776727
822,3999,0,3999,0.19703912734985352,0.020438398365707895
823,4004,0,4004,0.19726109504699707,0.020433179478591697
824,4009,0,4009,0.19750714302062988,0.020427983404415824
825,4014,0,4014,0.1977379322052002,0.02042280953680913
826,4019,0,4019,0.1979680061340332,0.020417657494203302
827,4024,0,4024,0.1981959342956543,0.020412526988920873
829,4033,0,4033,0.19867324829101562,0.02040305596836204
830,4038,0,4038,0.1989119052886963,0.020394653670245837
831,4043,0,4043,0.19915103912353516,0.02038695642706138
832,4048,0,4048,0.19939303398132324,0.020379825564414866
833,4053,0,4053,0.1996321678161621,0.02037315560662846
834,4058,0,4058,0.19986820220947266,0.020366869691713
835,4063,0,4063,0.2001030445098877,0.020360903323560064
837,4073,0,4073,0.20060014724731445,0.02034969050958927
838,4078,0,4078,0.20083093643188477,0.02034435625072366
839,4083,0,4083,0.20105910301208496,0.020339170147485246
840,4088,0,4088,0.2012951374053955,0.020334112170524346
841,4093,0,4093,0.20152807235717773,0.020329159395795382
842,4098,0,4098,0.20175695419311523,0.020324292233274383
844,4108,0,4108,0.2022230625152588,0.020314774072358013
845,4113,0,4113,0.2024550437927246,0.020310107984279558
846,4118,0,4118,0.2026841640472412,0.020305491015121916
847,4123,0,4123,0.20291399955749512,0.020300915747931685
848,4128,0,4128,0.20314908027648926,0.020296378913555665
849,4133,0,4133,0.20338106155395508,0.020291877945825206
851,4143,0,4143,0.203840970993042,0.02028296578054838
852,4148,0,4148,0.20407700538635254,0.020278548116466257
853,4153,0,4153,0.20430803298950195,0.02027415521728847
854,4158,0,4158,0.20453810691833496,0.020269786025198473
855,4163,0,4163,0.20476794242858887,0.020265438172315912
856,4168,0,4168,0.20500922203063965,0.02026110980255026
857,4173,0,4173,0.20524096488952637,0.020256800425487605
859,4183,0,4183,0.20570015907287598,0.020248236044645943
860,4188,0,4188,0.20593619346618652,0.02024397786335767
861,4193,0,4193,0.20617914199829102,0.020239734350738687
862,4198,0,4198,0.20642709732055664,0.020235505656218126
863,4203,0,4203,0.20667219161987305,0.020231291667539453
864,4208,0,4208,0.20691990852355957,0.02022709156691616
866,4218,0,4218,0.20741820335388184,0.02021873053998898
867,4223,0,4223,0.20765900611877441,0.020214569596465125
868,4228,0,4228,0.20789718627929688,0.02021042145390919
869,4233,0,4233,0.20813417434692383,0.02020628551120236
870,4238,0,4238,0.2083749771118164,0.020202161461758395
871,4243,0,4243,0.20861196517944336,0.02019804946156375
872,4248,0,4248,0.2088470458984375,0.020193949664472483
874,4258,0,4258,0.20932602882385254,0.020185785778765276
875,4263,0,4263,0.20956110954284668,0.020181721312865292
876,4268,0,4268,0.20980191230773926,0.020177668572025687
877,4273,0,4273,0.2100391387939453,0.020173627448075854
878,4278,0,4278,0.21027398109436035,0.020169597549526505
879,4283,0,4283,0.21051502227783203,0.020165578482561203
881,4293,0,4293,0.21098995208740234,0.020157572013261543
882,4298,0,4298,0.21123504638671875,0.020153584038766638
883,4303,0,4303,0.21147394180297852,0.0201496056123232
884,4308,0,4308,0.21170902252197266,0.02014563633089861
885,4313,0,4313,0.21195101737976074,0.020141675916196835
886,4318,0,4318,0.2121899127960205,0.02013772404644483
888,4328,0,4328,0.21266508102416992,0.02012984412537946
889,4333,0,4333,0.2129039764404297,0.02012591525405827
890,4338,0,4338,0.21313881874084473,0.020121993371021572
891,4343,0,4343,0.2133791446685791,0.020118078154496073
892,4348,0,4348,0.21361708641052246,0.02011416925377376
893,4353,0,4353,0.2138521671295166,0.02011026639036867
894,4358,0,4358,0.21409201622009277,0.02010636939700553
896,4367,0,4367,0.2145531177520752,0.02005080732572487
897,4372,0,4372,0.21479511260986328,0.02001746091219067
898,4377,0,4377,0.21503615379333496,0.019987671668554505
899,4382,0,4382,0.2152712345123291,0.01996085026155687
900,4387,0,4387,0.21551203727722168,0.01993652803374587
901,4392,0,4392,0.21575021743774414,0.01991431203067977
903,4402,0,4402,0.21622610092163086,0.019874961833396633
904,4407,0,4407,0.21648001670837402,0.019857372193107545
905,4412,0,4412,0.21672487258911133,0.019840922410663642
906,4417,0,4417,0.21697211265563965,0.019825443009026604
907,4422,0,4422,0.21721696853637695,0.019810801325420197
908,4427,0,4427,0.21746516227722168,0.019796904533170567
910,4437,0,4437,0.21795916557312012,0.019771033303706578
911,4442,0,4442,0.2182011604309082,0.01975890200724154
912,4447,0,4447,0.2184607982635498,0.01974722973156972
913,4452,0,4452,0.21869897842407227,0.019735981048688348
914,4457,0,4457,0.2189328670501709,0.01972511784532327
915,4462,0,4462,0.21917414665222168,0.019714596721332862
916,4467,0,4467,0.21941184997558594,0.019704383559309122
918,4477,0,4477,0.21988606452941895,0.01968480791534498
919,4481,0,4481,0.22011017799377441,0.019640005567586834
920,4486,0,4486,0.22034502029418945,0.019616728077931418
921,4491,0,4491,0.22058486938476562,0.019595983275758903
922,4496,0,4496,0.2208249568939209,0.01957730362153674
923,4501,0,4501,0.22105908393859863,0.019560306140490577
925,4511,0,4511,0.22155499458312988,0.019530167178482317
926,4516,0,4516,0.22179508209228516,0.019516603985542384
927,4521,0,4521,0.22203993797302246,0.01950384509464084
928,4526,0,4526,0.22228407859802246,0.019491760296982297
929,4531,0,4531,0.2225351333618164,0.01948023239618705
930,4536,0,4536,0.22277402877807617,0.019469174993601592
932,4546,0,4546,0.22324514389038086,0.01944825546913113
933,4551,0,4551,0.22348999977111816,0.019438297726650827
934,4556,0,4556,0.22372698783874512,0.019428611508941995
935,4560,0,4560,0.22394704818725586,0.01925816358105504
936,4564,0,4564,0.22417402267456055,0.019133782124090868
937,4569,0,4569,0.2244129180908203,0.01911111180105541
938,4574,0,4574,0.22464799880981445,0.0190903962157881
940,4584,0,4584,0.2251272201538086,0.019053567010480065
941,4589,0,4589,0.22536110877990723,0.019036985083942783
942,4594,0,4594,0.2256009578704834,0.01902138173415262
943,4599,0,4599,0.22583818435668945,0.019006620582989575
944,4604,0,4604,0.22607207298278809,0.018992595399150276
945,4609,0,4609,0.22631287574768066,0.01897921577495025
947,4619,0,4619,0.22678899765014648,0.01895407321730871
948,4624,0,4624,0.22703003883361816,0.0189421891994676
949,4629,0,4629,0.22726798057556152,0.018930711419596923
950,4634,0,4634,0.22750306129455566,0.018919607397900513
951,4639,0,4639,0.22774410247802734,0.018908842059348802
952,4644,0,4644,0.2279820442199707,0.018898382937593706
953,4649,0,4649,0.22821712493896484,0.018888206034934178
955,4659,0,4659,0.22869491577148438,0.018868630001326072
956,4664,0,4664,0.22892999649047852,0.01885919603247041
957,4669,0,4669,0.2291719913482666,0.018849975379690104
958,4674,0,4674,0.2294158935546875,0.018840955343226953
959,4679,0,4679,0.22965097427368164,0.018832125261485894
960,4684,0,4684,0.22989201545715332,0.01882347333020212
962,4694,0,4694,0.23036479949951172,0.018806655370850363
963,4699,0,4699,0.23060393333435059,0.01879847008989779
964,4704,0,4704,0.23084306716918945,0.018790422627765445
965,4708,0,4708,0.231065034866333,0.018249628900590537
966,4713,0,4713,0.2313070297241211,0.01820837865144621
967,4718,0,4718,0.23154497146606445,0.018173512830991737
969,4728,0,4728,0.23201799392700195,0.018118267851611324
970,4733,0,4733,0.2322549819946289,0.018096086696141437
971,4738,0,4738,0.23250722885131836,0.018076618310384096
972,4743,0,4743,0.23275423049926758,0.01805935877700399
973,4748,0,4748,0.2330000400543213,0.01804392115136201
974,4753,0,4753,0.23324322700500488,0.01802999748228412
975,4758,0,4758,0.23350095748901367,0.018017329062638168
977,4768,0,4768,0.23397397994995117,0.01799491452519822
978,4773,0,4773,0.2342090606689453,0.01798484942588115
979,4778,0,4778,0.23444390296936035,0.01797539327860997
980,4783,0,4783,0.2346789836883545,0.01796645670831567
981,4788,0,4788,0.23491597175598145,0.01795796089658547
982,4793,0,4793,0.23515105247497559,0.01794984043900331
984,4803,0,4803,0.23564910888671875,0.01793454056700574
985,4808,0,4808,0.23589301109313965,0.017927289683847995
986,4813,0,4813,0.23613524436950684,0.01792026143385137
987,4818,0,4818,0.23637914657592773,0.017913428352311158
988,4823,0,4823,0.2366321086883545,0.01790676947142521
989,4828,0,4828,0.23686909675598145,0.017900267930029932
991,4838,0,4838,0.23734021186828613,0.01788767494112359
992,4843,0,4843,0.23757219314575195,0.01788155683017909
993,4848,0,4848,0.2378091812133789,0.017875544763222388
994,4853,0,4853,0.23804306983947754,0.017869631481425792
995,4858,0,4858,0.2382798194885254,0.017863810287617278
996,4863,0,4863,0.23851418495178223,0.01785807541586412
997,4868,0,4868,0.23874998092651367,0.017852422489411466
999,4878,0,4878,0.23921990394592285,0.017841347571612588
1000,4883,0,4883,0.23945403099060059,0.01783591735756803
1001,4888,0,4888,0.23969006538391113,0.017830553541075714
1002,4893,0,4893,0.23992300033569336,0.01782525353968312
1003,4898,0,4898,0.2401599884033203,0.01782001531192571
1004,4903,0,4903,0.24039506912231445,0.017814836611711536
1006,4913,0,4913,0.24089598655700684,0.01780464828672365
1007,4918,0,4918,0.24113988876342773,0.01779963453106848
1008,4923,0,4923,0.2413942813873291,0.017794671552379047
1009,4928,0,4928,0.24163103103637695,0.01778975675730329
1010,4933,0,4933,0.24187111854553223,0.017784887538081898
1011,4937,0,4937,0.2420940399169922,0.017774283220188345
1013,4947,0,4947,0.24256420135498047,0.01775997612065628
1014,4952,0,4952,0.2427990436553955,0.017753614777058085
1015,4957,0,4957,0.24303603172302246,0.017747649855528496
1016,4962,0,4962,0.2432701587677002,0.017742005846540662
1017,4967,0,4967,0.24350619316101074,0.017736624822387147
1018,4972,0,4972,0.24374008178710938,0.017731464690962852
1019,4977,0,4977,0.24397587776184082,0.01772649281841097
1021,4987,0,4987,0.2444469928741455,0.017716998752336482
1022,4992,0,4992,0.24468088150024414,0.01771242957468209
1023,4997,0,4997,0.2449181079864502,0.017707957482230717
1024,5002,0,5002,0.24515295028686523,0.017703569723367757
1025,5007,0,5007,0.2453901767730713,0.017699253093630286
1026,5012,0,5012,0.24562406539916992,0.017694995984969274
1028,5022,0,5022,0.2460951805114746,0.017686636411890454
1029,5027,0,5027,0.24633216857910156,0.017682527780871073
1030,5032,0,5032,0.24658823013305664,0.017678460453373828
1031,5037,0,5037,0.24683213233947754,0.017674428879775925
1032,5042,0,5042,0.24707293510437012,0.017670429331603114
1033,5047,0,5047,0.2473158836364746,0.017666459702840785
1034,5052,0,5052,0.24756717681884766,0.017662517768140807
1036,5062,0,5062,0.2480449676513672,0.01765470591709655
1037,5067,0,5067,0.24828314781188965,0.01765083236071139
1038,5072,0,5072,0.2485182285308838,0.01764697933422644
1039,5077,0,5077,0.24875497817993164,0.01764314578338217
1040,5082,0,5082,0.24898886680603027,0.01763933029983189
1041,5087,0,5087,0.24922490119934082,0.0176355318213337
1043,5097,0,5097,0.2496960163116455,0.017627983603072394
1044,5102,0,5102,0.24992895126342773,0.017624232263936536
1045,5107,0,5107,0.2501659393310547,0.01762049471773211
1046,5112,0,5112,0.2504000663757324,0.01761677031042203
1047,5117,0,5117,0.2506380081176758,0.01761305872110932
1048,5122,0,5122,0.25087523460388184,0.0176093595557785
1050,5132,0,5132,0.2513580322265625,0.017601996199921737
1051,5137,0,5137,0.2516012191772461,0.01759833123107165
1052,5142,0,5142,0.25184106826782227,0.0175946771661108
1053,5147,0,5147,0.25208282470703125,0.017591033708462767
1054,5152,0,5152,0.2523231506347656,0.017587400421702794
1055,5157,0,5157,0.2525649070739746,0.017583776935947967
1056,5162,0,5162,0.2528071403503418,0.01758016304155678
1058,5172,0,5172,0.25328898429870605,0.017572963286037312
1059,5177,0,5177,0.25353217124938965,0.01756937688366663
1060,5182,0,5182,0.25377702713012695,0.017565799111879922
1061,5187,0,5187,0.25401997566223145,0.017562229756796992
1062,5192,0,5192,0.2542600631713867,0.017558668559292577
1063,5197,0,5197,0.2545032501220703,0.01755511518163525
1065,5207,0,5207,0.2549870014190674,0.01754803052442205
1066,5212,0,5212,0.25522804260253906,0.01754449867252747
1067,5217,0,5217,0.25546908378601074,0.017540973437582725
1068,5222,0,5222,0.2557098865509033,0.017537454539933633
1069,5227,0,5227,0.2559521198272705,0.01753394174716728
1070,5232,0,5232,0.2561910152435303,0.017530434891778558
1072,5242,0,5242,0.25667905807495117,0.017523438458092202
1073,5247,0,5247,0.25692200660705566,0.017519948639251767
1074,5252,0,5252,0.25716304779052734,0.01751646431750158
1075,5257,0,5257,0.25742101669311523,0.01751298546701686
1076,5262,0,5262,0.25764918327331543,0.017509512069328582
1077,5267,0,5267,0.25788116455078125,0.017506044096742786
1078,5272,0,5272,0.25810813903808594,0.017502581520813815
1080,5282,0,5282,0.258587121963501,0.017495672454839274
1081,5287,0,5287,0.25882387161254883,0.017492225866416345
1082,5292,0,5292,0.25905704498291016,0.01748878445438945
1083,5297,0,5297,0.2592949867248535,0.017485348096746036
1084,5302,0,5302,0.25952887535095215,0.017481916652219032
1085,5307,0,5307,0.2597649097442627,0.01747848995406619
1087,5317,0,5317,0.2602410316467285,0.017471649998401097
1088,5322,0,5322,0.26047515869140625,0.017468236307756974
1089,5327,0,5327,0.2607128620147705,0.017464826515236138
1090,5332,0,5332,0.26094889640808105,0.017461420399863415
1091,5337,0,5337,0.2611870765686035,0.01745801774455788
1092,5342,0,5342,0.26142001152038574,0.01745461834699164
1094,5352,0,5352,0.26189112663269043,0.017447828635666258
1095,5357,0,5357,0.2621290683746338,0.017444438041458482
1096,5362,0,5362,0.2623631954193115,0.01744105014801821
1097,5367,0,5367,0.2625999450683594,0.0174376648924676
1098,5372,0,5372,0.2628340721130371,0.017434282247955946
1099,5377,0,5377,0.26307201385498047,0.017430902220075466
1100,5382,0,5382,0.2633049488067627,0.017427524843139534
1102,5392,0,5392,0.2637920379638672,0.017420778313504637
1103,5396,0,5396,0.26401782035827637,0.01738734890570715
1104,5401,0,5401,0.2642538547515869,0.017375060283439023
1105,5406,0,5406,0.26449108123779297,0.01736377392212545
1106,5411,0,5411,0.264725923538208,0.01735331964629519
1107,5416,0,5416,0.2649650573730469,0.017343550855916396
1109,5426,0,5426,0.2654390335083008,0.017325633762762332
1110,5431,0,5431,0.265671968460083,0.017317341121019087
1111,5436,0,5436,0.26590991020202637,0.01730941630644797
1112,5440,0,5440,0.26613807678222656,0.01729473896525511
1113,5445,0,5445,0.26637697219848633,0.017284185843520046
1114,5450,0,5450,0.2666161060333252,0.017274410299984763
1115,5455,0,5455,0.26685523986816406,0.017265288169285204
1117,5463,0,5463,0.267301082611084,0.017257086956754125
1118,5468,0,5468,0.2675352096557617,0.017243095535011004
1119,5472,0,5472,0.2677581310272217,0.017205183973887195
1120,5476,0,5476,0.2679789066314697,0.01707439716800974
1121,5480,0,5480,0.2682030200958252,0.01683250351038917
1122,5483,0,5483,0.2684028148651123,0.016258213518308983
1124,5489,0,5489,0.2687962055206299,0.014794557689707164
1125,5492,0,5492,0.2689859867095947,0.011182880253704086
1126,5495,0,5495,0.26917290687561035,0.0076302707377840975
1127,5498,0,5498,0.2693629264831543,0.004868987116940013
1128,5501,0,5501,0.2695648670196533,0.003551850782471617
1129,5504,0,5504,0.2697560787200928,0.0023374942699534934
1131,5510,0,5510,0.27013397216796875,0.0013524024415931585
1132,5513,0,5513,0.27033400535583496,0.0013117130463716877
1133,5516,0,5516,0.2705259323120117,0.000999761815581126
1134,5521,0,5521,0.27076196670532227,0.0009829547704617483
1135,5524,0,5524,0.2709670066833496,0.0009702508566402214
1136,5527,0,5527,0.27116894721984863,0.0008862210109272366
1137,5530,0,5530,0.2713639736175537,0.0006400333606527653
1139,5536,0,5536,0.27173900604248047,0.00021689148695494415
1140,5539,0,5539,0.2719249725341797,0.00012169916241697825
1141,5542,0,5542,0.27211427688598633,6.936422758575171e-05
1142,5545,0,5545,0.27230095863342285,3.856406048344592e-05
1143,5548,0,5548,0.2724909782409668,2.4529313802396054e-05
1144,5551,0,5551,0.2726759910583496,1.9931206686165053e-05
1146,5557,0,5557,0.27305006980895996,7.479902760052434e-06
1147,5560,0,5560,0.2732391357421875,7.023951809827678e-06
1148,5563,0,5563,0.2734251022338867,2.7031879686705585e-06
1149,5566,0,5566,0.27361297607421875,1.2686563336056185e-06
1150,5569,0,5569,0.27379918098449707,9.648555064711824e-07
1151,5572,0,5572,0.2739880084991455,3.354222314142178e-07
1153,5578,0,5578,0.27436304092407227,6.72485448216772e-08
1154,5581,0,5581,0.2745652198791504,3.9051705823188195e-08
1155,5584,0,5584,0.27476000785827637,1.5804890709825776e-08
1156,5587,0,5587,0.2749512195587158,6.862875061217013e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.985664367675781e-05,4.387072431292609
187,188,187,375,0.004339933395385742,0.4268561502630121
374,375,374,749,0.008699893951416016,0.19745276258065977
561,562,561,1123,0.013796091079711914,0.12581339699925403
748,749,748,1497,0.018352031707763672,0.0934848928777029
935,936,935,1871,0.023186922073364258,0.07523137209185625
1123,1124,1123,2247,0.02775287628173828,0.06376853690493829
1310,1311,1310,2621,0.0321657657623291,0.056205750750353285
1497,1498,1497,2995,0.03638601303100586,0.05091764264030393
1684,1685,1684,3369,0.040611982345581055,0.04695280207456066
1871,1872,1871,3743,0.044960975646972656,0.0437972404294198
2058,2059,2058,4117,0.04943990707397461,0.04117031359160079
2245,2246,2245,4491,0.054064035415649414,0.038867931179356635
2432,2433,2432,4865,0.05870199203491211,0.03684030277443672
2619,2620,2619,5239,0.06337785720825195,0.034993125101065906
2806,2807,2806,5613,0.06756973266601562,0.03331461063843964
2994,2995,2994,5989,0.07189393043518066,0.03177870754267203
3181,3182,3181,6363,0.07608294486999512,0.030354916945830392
3368,3369,3368,6737,0.08025288581848145,0.029066080496606667
3555,3556,3555,7111,0.08441376686096191,0.02786500136196921
3742,3743,3742,7485,0.0887138843536377,0.0267577835687742
3929,3930,3929,7859,0.09287381172180176,0.025744063208262037
4116,4117,4116,8233,0.09704399108886719,0.024794878822063784
4303,4304,4303,8607,0.10152792930603027,0.02393050656079627
4490,4491,4490,8981,0.10570597648620605,0.023119442976707722
4677,4678,4677,9355,0.11021089553833008,0.02237284101937738
4864,4865,4864,9729,0.11444973945617676,0.02168486245232052
5052,5053,5052,10105,0.11875605583190918,0.02102912963206462
5239,5240,5239,10479,0.12347006797790527,0.02043606541764476
5426,5427,5426,10853,0.12785601615905762,0.01987485982300528
5613,5614,5613,11227,0.13200783729553223,0.01934990754717838
5800,5801,5800,11601,0.13617300987243652,0.01886341533640373
5987,5988,5987,11975,0.1405189037322998,0.018400255484358547
6174,6175,6174,12349,0.14472603797912598,0.017971270740053537
6361,6362,6361,12723,0.14934301376342773,0.017560142448936594
6548,6549,6548,13097,0.15366697311401367,0.0171756492048547
6735,6736,6735,13471,0.15814971923828125,0.016813272787954178
6923,6924,6923,13847,0.1624150276184082,0.016459547202817882
7110,7111,7110,14221,0.16664695739746094,0.016133178815899436
7297,7298,7297,14595,0.17116999626159668,0.015817381999008492
7484,7485,7484,14969,0.17565202713012695,0.015514264913198478
7671,7672,7671,15343,0.1799170970916748,0.01522677549487873
7858,7859,7858,15717,0.1841588020324707,0.014947917601161646
8045,8046,8045,16091,0.1884000301361084,0.014682193545942156
8232,8233,8232,16465,0.19263982772827148,0.014422275110793912
8419,8420,8419,16839,0.1971268653869629,0.014174385269201931
8606,8607,8606,17213,0.2013390064239502,0.013934918586089796
8794,8795,8794,17589,0.2055809497833252,0.01369703818322894
8981,8982,8981,17963,0.20980191230773926,0.013472596708826617
9168,9169,9168,18337,0.2140038013458252,0.013252271747579555
9355,9356,9355,18711,0.2182457447052002,0.013036502041037724
9542,9543,9542,19085,0.22288990020751953,0.012828176861593373
9729,9730,9729,19459,0.22760796546936035,0.012624249932296478
9916,9917,9916,19833,0.23218083381652832,0.012425715384886363
10103,10104,10103,20207,0.2364640235900879,0.012229720233603896
10290,10291,10290,20581,0.24095797538757324,0.012040529824331786
10477,10478,10477,20955,0.24535799026489258,0.011855113113883795
10664,10665,10664,21329,0.24967694282531738,0.011670728932696805
10852,10853,10852,21705,0.25394773483276367,0.011492422069160376
11039,11040,11039,22079,0.2583191394805908,0.011317526455245284
11226,11227,11226,22453,0.262861967086792,0.01114455606127755
11413,11414,11413,22827,0.2673358917236328,0.010976088678887701
11600,11601,11600,23201,0.2717249393463135,0.010810857488491121
11787,11788,11787,23575,0.2759678363800049,0.010648165195958324
11974,11975,11974,23949,0.2801940441131592,0.01048723525225835
12161,12162,12161,24323,0.28456902503967285,0.010331046987734387
12348,12349,12348,24697,0.28880786895751953,0.010177000422903149
12535,12536,12535,25071,0.29303789138793945,0.010023687607376788
12723,12724,12723,25447,0.2972888946533203,0.009874388351661208
12910,12911,12910,25821,0.301541805267334,0.00972788276227271
13097,13098,13097,26195,0.3057839870452881,0.009582407567945228
13284,13285,13284,26569,0.3100137710571289,0.009440210097111403
13471,13472,13471,26943,0.31427884101867676,0.009300807491451043
13658,13659,13658,27317,0.31868481636047363,0.009162805912689139
13845,13846,13845,27691,0.3229219913482666,0.009026351998973232
14032,14033,14032,28065,0.3271489143371582,0.00889361708138467
14219,14220,14219,28439,0.33136796951293945,0.008762362962220048
14406,14407,14406,28813,0.33560800552368164,0.008631818311148658
14593,14594,14593,29187,0.33982396125793457,0.008504935131714412
14781,14782,14781,29563,0.3440549373626709,0.008379168733483884
14968,14969,14968,29937,0.34828901290893555,0.008254754687540009
15155,15156,15155,30311,0.3530550003051758,0.008132971972377896
15342,15343,15342,30685,0.35790395736694336,0.00801367599825493
15529,15530,15529,31059,0.3624858856201172,0.007895271987635863
15716,15717,15716,31433,0.3673441410064697,0.007778287115184196
15903,15904,15903,31807,0.37218403816223145,0.007664377113772949
16090,16091,16090,32181,0.377392053604126,0.007551615131602499
16277,16278,16277,32555,0.3825337886810303,0.007439546237710235
16464,16465,16464,32929,0.38794398307800293,0.0073304387459651715
16652,16653,16652,33305,0.3921971321105957,0.007222358433041664
16839,16840,16839,33679,0.3975968360900879,0.007115366707040971
17026,17027,17026,34053,0.4030458927154541,0.007010580369468733
17213,17214,17213,34427,0.40810108184814453,0.006907993880371653
17400,17401,17400,34801,0.41236305236816406,0.006806040535705541
17587,17588,17587,35175,0.4165329933166504,0.0067053749515346575
17774,17775,17774,35549,0.4206888675689697,0.006607308327007169
17961,17962,17961,35923,0.4248518943786621,0.0065101815597963944
18148,18149,18148,36297,0.42905688285827637,0.006413705463970871
18335,18336,18335,36671,0.4332888126373291,0.006319698938833546
18523,18524,18523,37047,0.43753480911254883,0.0062266161705918435
18710,18711,18710,37421,0.44176197052001953,0.006134441861422461
18897,18898,18897,37795,0.4460420608520508,0.0060441494603811815
19084,19085,19084,38169,0.45035600662231445,0.005955784028959034
19271,19272,19271,38543,0.45494604110717773,0.0058679024691762754
19458,19459,19458,38917,0.4592769145965576,0.005781171255998769
19645,19646,19645,39291,0.46356797218322754,0.005696657794068482
19832,19833,19832,39665,0.46787405014038086,0.00561293261885974
20019,20020,20019,40039,0.4722170829772949,0.005529799295806987
20206,20207,20206,40413,0.4766080379486084,0.005448758396247348
20393,20394,20393,40787,0.48092198371887207,0.005368958669803844
20581,20582,20581,41163,0.48525381088256836,0.005289077870481344
20768,20769,20768,41537,0.4895598888397217,0.0052112411101270205
20955,20956,20955,41911,0.4939420223236084,0.005135079794354078
21142,21143,21142,42285,0.4982597827911377,0.005059305922840368
21329,21330,21329,42659,0.5025949478149414,0.0049845477762051
21516,21517,21516,43033,0.5069470405578613,0.004911690536079844
21703,21704,21703,43407,0.5115277767181396,0.004839501595318327
21890,21891,21890,43781,0.5158247947692871,0.004767840536468726
22077,22078,22077,44155,0.520150899887085,0.004697967371901102
22264,22265,22264,44529,0.5245480537414551,0.0046291720706896355
22452,22453,22452,44905,0.5288779735565186,0.0045603014920862425
22639,22640,22639,45279,0.5331780910491943,0.004493194112088532
22826,22827,22826,45653,0.5374979972839355,0.004427536615819525
23013,23014,23013,46027,0.5417828559875488,0.004362198228660415
23200,23201,23200,46401,0.5460820198059082,0.004297750083835072
23387,23388,23387,46775,0.5510368347167969,0.004234934945489196
23574,23575,23574,47149,0.555340051651001,0.004172689154264585
23761,23762,23761,47523,0.5595269203186035,0.00411090885270882
23948,23949,23948,47897,0.5637450218200684,0.004050663228690511
24135,24136,24135,48271,0.5680630207061768,0.003991348923488977
24322,24323,24322,48645,0.5722298622131348,0.00393228129136683
24510,24511,24510,49021,0.5765790939331055,0.003874108946001379
24697,24698,24697,49395,0.5808308124542236,0.0038175014797594596
24884,24885,24884,49769,0.5850129127502441,0.003761161252805195
25071,25072,25071,50143,0.589202880859375,0.003705597809745314
25258,25259,25258,50517,0.5933849811553955,0.0036514389321942
25445,25446,25445,50891,0.5976259708404541,0.0035977662035426025
25632,25633,25632,51265,0.6018710136413574,0.0035445013102282335
25819,25820,25819,51639,0.6061060428619385,0.0034925570428766804
26006,26007,26006,52013,0.6103348731994629,0.003441415027124166
26193,26194,26193,52387,0.6146938800811768,0.003390485028179218
26381,26382,26381,52763,0.6190729141235352,0.0033403298414400226
26568,26569,26568,53137,0.6233499050140381,0.003291523035579312
26755,26756,26755,53511,0.6275970935821533,0.0032429422112348854
26942,26943,26942,53885,0.6318190097808838,0.0031950373888009276
27129,27130,27129,54259,0.6361961364746094,0.0031483414658316695
27316,27317,27316,54633,0.6404001712799072,0.0031020610958380555
27503,27504,27503,55007,0.6448569297790527,0.0030561367642648585
27690,27691,27690,55381,0.6492919921875,0.003011350433287845
27877,27878,27877,55755,0.6535708904266357,0.002967253926617867
28064,28065,28064,56129,0.6579461097717285,0.0029233402602818867
28252,28253,28252,56505,0.6623468399047852,0.0028800973980050108
28439,28440,28439,56879,0.6667349338531494,0.002838015510286268
28626,28627,28626,57253,0.6711270809173584,0.002796125791613191
28813,28814,28813,57627,0.6757490634918213,0.0027548234633445285
29000,29001,29000,58001,0.6809210777282715,0.0027145620250565348
29187,29188,29187,58375,0.6866569519042969,0.002674655974004104
29374,29375,29374,58749,0.6919107437133789,0.0026350601225066795
29561,29562,29561,59123,0.6971278190612793,0.002596445648366174
29748,29749,29748,59497,0.702254056930542,0.002558423694653346
29935,29936,29935,59871,0.706618070602417,0.002520559737174191
30122,30123,30122,60245,0.710839033126831,0.002483472184735134
30310,30311,30310,60621,0.7151238918304443,0.0024469927113159313
30497,30498,30497,60995,0.7193319797515869,0.002410872741610936
30684,30685,30684,61369,0.7235229015350342,0.002375262707345216
30871,30872,30871,61743,0.7283368110656738,0.0023405490963662196
31058,31059,31058,62117,0.7325530052185059,0.0023061394876422872
31245,31246,31245,62491,0.736914873123169,0.002271999842067275
31432,31433,31432,62865,0.7411839962005615,0.002238706859569761
31619,31620,31619,63239,0.7454190254211426,0.0022059224976698055
31806,31807,31806,63613,0.7497420310974121,0.0021732748319072044
31993,31994,31993,63987,0.7540299892425537,0.0021412987563475
32181,32182,32181,64363,0.7583498954772949,0.0021098452079797614
32368,32369,32368,64737,0.7626669406890869,0.0020787004024013797
32555,32556,32555,65111,0.7671091556549072,0.0020479980568197816
32742,32743,32742,65485,0.7714197635650635,0.0020180678096168004
32929,32930,32929,65859,0.7757418155670166,0.0019883976344864905
33116,33117,33116,66233,0.7800588607788086,0.0019589622606636424
33303,33304,33303,66607,0.7843718528747559,0.0019302574914298778
33490,33491,33490,66981,0.7888240814208984,0.001901989158075218
33677,33678,33677,67355,0.7932629585266113,0.0018738391836372098
33864,33865,33864,67729,0.7976689338684082,0.0018462701365876725
34051,34052,34051,68103,0.80206298828125,0.0018192937315925127
34239,34240,34239,68479,0.8064699172973633,0.0017922951382207787
34426,34427,34426,68853,0.8108940124511719,0.0017658240745215114
34613,34614,34613,69227,0.8152608871459961,0.0017400180670017755
34800,34801,34800,69601,0.8203020095825195,0.001714434556782584
34987,34988,34987,69975,0.824699878692627,0.001689055195338245
35174,35175,35174,70349,0.8290958404541016,0.0016643063617935718
35361,35362,35361,70723,0.8335018157958984,0.0016399319376308346
35548,35549,35548,71097,0.8378880023956299,0.001615660046207436
35735,35736,35735,71471,0.8422651290893555,0.0015918906517416482
35922,35923,35922,71845,0.8466219902038574,0.0015686307948114557
36110,36111,36110,72221,0.8509061336517334,0.0015453510768855252
36297,36298,36297,72595,0.8553719520568848,0.0015225281380791078
36484,36485,36484,72969,0.8607511520385742,0.0015002780683560184
36671,36672,36671,73343,0.8652548789978027,0.0014782183502988246
36858,36859,36858,73717,0.8696420192718506,0.001456336095182676
37045,37046,37045,74091,0.873938798904419,0.0014349980292786078
37232,37233,37232,74465,0.8781847953796387,0.001413981114709229
37419,37420,37419,74839,0.8825719356536865,0.0013930530528216492
37606,37607,37606,75213,0.8868288993835449,0.00137255963699807
37793,37794,37793,75587,0.8911547660827637,0.0013525042760179707
37981,37982,37981,75963,0.8954248428344727,0.0013324312023538511
38168,38169,38168,76337,0.8997170925140381,0.0013127536132524127
38355,38356,38355,76711,0.9040689468383789,0.0012935694876170215
38542,38543,38542,77085,0.90836501121521,0.0012745482103713932
38729,38730,38729,77459,0.9126479625701904,0.001255681180700022
38916,38917,38916,77833,0.9169809818267822,0.0012372838335572769
39103,39104,39103,78207,0.921889066696167,0.0012191619288234614
39290,39291,39290,78581,0.9261391162872314,0.0012011170404342198
39477,39478,39477,78955,0.9304909706115723,0.0011834480996779726
39664,39665,39664,79329,0.934838056564331,0.001166155739990052
39851,39852,39851,79703,0.9391930103302002,0.0011489393784061142
40039,40040,40039,80079,0.9435498714447021,0.0011318819067622492
40226,40227,40226,80453,0.9478771686553955,0.001115341250087019
40413,40414,40413,80827,0.9521589279174805,0.0010989399098950293
40600,40601,40600,81201,0.956671953201294,0.0010826726292907636
40787,40788,40787,81575,0.9609458446502686,0.0010668107259603123
40974,40975,40974,81949,0.9652400016784668,0.0010511850456671186
41161,41162,41161,82323,0.9696087837219238,0.001035626134311969
41348,41349,41348,82697,0.9739618301391602,0.001020392390872701
41535,41536,41535,83071,0.9783947467803955,0.0010054823686612743
41722,41723,41722,83445,0.9826529026031494,0.0009906374725653308
41910,41911,41910,83821,0.9871499538421631,0.0009759307769135151
42097,42098,42097,84195,0.9916439056396484,0.0009616693294407396
42284,42285,42284,84569,0.9959127902984619,0.0009475270645569473
42471,42472,42471,84943,1.0001840591430664,0.0009335013079019953
42658,42659,42658,85317,1.0044739246368408,0.0009198254240801708
42845,42846,42845,85691,1.008699893951416,0.0009063521177229406
43032,43033,43032,86065,1.0129458904266357,0.0008929367048959243
43219,43220,43219,86439,1.017246961593628,0.0008798025317375594
43406,43407,43406,86813,1.0214660167694092,0.0008669466304561599
43593,43594,43593,87187,1.0257017612457275,0.0008541465471275163
43780,43781,43780,87561,1.0299148559570312,0.0008415331736523942
43968,43969,43968,87937,1.0349397659301758,0.0008291703523994013
44155,44156,44155,88311,1.039167881011963,0.0008169760044934848
44342,44343,44342,88685,1.043375015258789,0.0008048829077523744
44529,44530,44529,89059,1.0475149154663086,0.000793091774372572
44716,44717,44716,89433,1.0516247749328613,0.0007814743576725847
44903,44904,44903,89807,1.0557360649108887,0.0007699071451976803
45090,45091,45090,90181,1.0599470138549805,0.0007585831721729655
45277,45278,45277,90555,1.0640668869018555,0.0007474983954136405
45464,45465,45464,90929,1.0683059692382812,0.0007364614649947085
45651,45652,45651,91303,1.072448968887329,0.0007255864060411758
45839,45840,45839,91679,1.076584815979004,0.0007149271073745293
46026,46027,46026,92053,1.0806918144226074,0.0007044123759109395
46213,46214,46213,92427,1.0848140716552734,0.0006939856339931124
46400,46401,46400,92801,1.088925838470459,0.0006838195014384398
46587,46588,46587,93175,1.0930359363555908,0.0006738023309705584
46774,46775,46774,93549,1.0972118377685547,0.0006638287015945783
46961,46962,46961,93923,1.1013298034667969,0.0006540654403931919
47148,47149,47148,94297,1.1054670810699463,0.0006445077811375885
47335,47336,47335,94671,1.1095941066741943,0.000634991139863052
47522,47523,47522,95045,1.113874912261963,0.0006256148309841272
47710,47711,47710,95421,1.1180698871612549,0.0006164243166301563
47897,47898,47897,95795,1.122565746307373,0.0006073578559281502
48084,48085,48084,96169,1.1266980171203613,0.0005983678582094057
48271,48272,48271,96543,1.1313908100128174,0.0005896027745953714
48458,48459,48458,96917,1.1370689868927002,0.0005809654216387414
48645,48646,48645,97291,1.1412248611450195,0.0005723658348876812
48832,48833,48832,97665,1.145467758178711,0.0005639481824898674
49019,49020,49019,98039,1.1495988368988037,0.0005557072511196488
49206,49207,49206,98413,1.153738021850586,0.00054750148777222
49393,49394,49393,98787,1.158566951751709,0.0005394173797783963
49580,49581,49580,99161,1.1626899242401123,0.0005315351028196626
49768,49769,49768,99537,1.1676008701324463,0.0005236755870301071
49955,49956,49955,99911,1.1718828678131104,0.0005159243611168376
50142,50143,50142,100285,1.1761419773101807,0.0005083672389076913
50329,50330,50329,100659,1.1803350448608398,0.0005009196384750907
50516,50517,50516,101033,1.184433937072754,0.0004935047984842004
50703,50704,50703,101407,1.1885440349578857,0.00048624729810919253
50890,50891,50890,101781,1.1926429271697998,0.00047914169069405115
51077,51078,51077,102155,1.196803092956543,0.00047206623892782895
51264,51265,51264,102529,1.200967788696289,0.0004650962478902133
51451,51452,51451,102903,1.2050628662109375,0.00045830009623682203
51639,51640,51639,103279,1.2091748714447021,0.0004515231296594527
51826,51827,51826,103653,1.2133398056030273,0.0004448399819275751
52013,52014,52013,104027,1.2175049781799316,0.00043832434435669043
52200,52201,52200,104401,1.2216618061065674,0.00043190261253372563
52387,52388,52387,104775,1.225836992263794,0.00042550930152875896
52574,52575,52574,105149,1.229996919631958,0.0004192520567086151
52761,52762,52761,105523,1.234245777130127,0.0004131253615005492
52948,52949,52948,105897,1.2385139465332031,0.0004070245267538294
53135,53136,53135,106271,1.2426879405975342,0.0004010151111022545
53322,53323,53322,106645,1.2468829154968262,0.00039515542186104675
53509,53510,53509,107019,1.251145839691162,0.0003893429463778467
53697,53698,53697,107395,1.25534987449646,0.0003835496539140515
53884,53885,53884,107769,1.2595429420471191,0.00037793196757582764
54071,54072,54071,108143,1.2637391090393066,0.0003723947950661484
54258,54259,54258,108517,1.2679190635681152,0.00036688228080929207
54445,54446,54445,108891,1.2720561027526855,0.00036148743258669944
54632,54633,54632,109265,1.2761988639831543,0.0003562047867527212
54819,54820,54819,109639,1.2805171012878418,0.00035094432038163366
55006,55007,55006,110013,1.284703016281128,0.0003457630986484349
55193,55194,55193,110387,1.288827896118164,0.0003407108320316953
55380,55381,55380,110761,1.2930359840393066,0.0003356989514265951
55568,55569,55568,111137,1.2975449562072754,0.0003307039462884722
55755,55756,55755,111511,1.3016860485076904,0.0003258604591436374
55942,55943,55942,111885,1.305898904800415,0.0003210860016249173
56129,56130,56129,112259,1.31003999710083,0.00031633293976432805
56316,56317,56316,112633,1.3142409324645996,0.0003116816294093094
56503,56504,56503,113007,1.3184947967529297,0.00030712675017526936
56690,56691,56690,113381,1.3226900100708008,0.00030259089545296583
56877,56878,56877,113755,1.3268179893493652,0.0002981237301416173
57064,57065,57064,114129,1.3310589790344238,0.0002937676276306348
57251,57252,57251,114503,1.3352789878845215,0.00028944607016275924
57439,57440,57439,114879,1.3394548892974854,0.0002851393537394223
57626,57627,57626,115253,1.3436839580535889,0.0002809633688917523
57813,57814,57813,115627,1.3479058742523193,0.000276846565735961
58000,58001,58000,116001,1.3521897792816162,0.0002727483288849592
58187,58188,58187,116375,1.3563330173492432,0.00026873807921773657
58374,58375,58374,116749,1.3605430126190186,0.00026481070405130763
58561,58562,58561,117123,1.3648297786712646,0.00026089964904732
58748,58749,58748,117497,1.3690390586853027,0.0002570481323825977
58935,58936,58935,117871,1.3732619285583496,0.00025329226649547766
59122,59123,59122,118245,1.378021001815796,0.0002495659489516071
59309,59310,59309,118619,1.3826570510864258,0.0002458722009310102
59497,59498,59497,118995,1.3869149684906006,0.000242252204687684
59684,59685,59684,119369,1.3911631107330322,0.00023870246703198235
59871,59872,59871,119743,1.395353078842163,0.00023516884179414693
60058,60059,60058,120117,1.3995487689971924,0.0002317112994218359
60245,60246,60245,120491,1.4037489891052246,0.00022832497889522426
60432,60433,60432,120865,1.4079179763793945,0.00022495266019544874
60619,60620,60619,121239,1.4121339321136475,0.00022163194636826454
60806,60807,60806,121613,1.4163179397583008,0.00021839360806899595
60993,60994,60993,121987,1.4205899238586426,0.00021518054373622728
61180,61181,61180,122361,1.4248619079589844,0.00021199577871741196
61368,61369,61368,122737,1.4290738105773926,0.00020887466895676683
61555,61556,61555,123111,1.4332630634307861,0.0002058138862443919
61742,61743,61742,123485,1.4374630451202393,0.00020276708749805613
61929,61930,61929,123859,1.441673994064331,0.0001997860762235303
62116,62117,62116,124233,1.4458868503570557,0.0001968662709630241
62303,62304,62303,124607,1.4503059387207031,0.0001939584799075556
62490,62491,62490,124981,1.455348014831543,0.00019109541606215883
62677,62678,62677,125355,1.4603707790374756,0.00018830329328464444
62864,62865,62864,125729,1.4649288654327393,0.00018553278807336893
63051,63052,63051,126103,1.4702248573303223,0.00018278687126873117
63238,63239,63238,126477,1.4745798110961914,0.00018011005080662335
63426,63427,63426,126853,1.478874921798706,0.00017745671489949457
63613,63614,63613,127227,1.4830987453460693,0.0001748296736363167
63800,63801,63800,127601,1.4871888160705566,0.0001722595161527084
63987,63988,63987,127975,1.4914588928222656,0.0001697419559785232
64174,64175,64174,128349,1.4958388805389404,0.00016723470574940287
64361,64362,64361,128723,1.5002799034118652,0.00016476622054296258
64548,64549,64548,129097,1.504655122756958,0.00016235882771367755
64735,64736,64735,129471,1.509063959121704,0.00015996992474213797
64922,64923,64922,129845,1.5136330127716064,0.0001576023853835781
65109,65110,65109,130219,1.5181629657745361,0.00015529446793741982
65297,65298,65297,130595,1.5227818489074707,0.00015300661261933711
65484,65485,65484,130969,1.5273818969726562,0.00015074149965272035
65671,65672,65671,131343,1.5320518016815186,0.00014852557054781485
65858,65859,65858,131717,1.536651849746704,0.00014635483968029696
66045,66046,66045,132091,1.5413219928741455,0.00014419295730973454
66232,66233,66232,132465,1.5459251403808594,0.00014206467154727874
66419,66420,66419,132839,1.5504088401794434,0.0001399889955190116
66606,66607,66606,133213,1.5550358295440674,0.0001379291339367109
66793,66794,66793,133587,1.5596368312835693,0.00013588783366829993
66980,66981,66980,133961,1.5641188621520996,0.00013389797881273058
67167,67168,67167,134335,1.5686378479003906,0.00013193574579950792
67355,67356,67355,134711,1.5733838081359863,0.0001299722140660792
67542,67543,67542,135085,1.5780677795410156,0.00012806169225653484
67729,67730,67729,135459,1.5828311443328857,0.00012619000944248462
67916,67917,67916,135833,1.5875840187072754,0.00012432592176112224
68103,68104,68103,136207,1.5922138690948486,0.00012249095050165837
68290,68291,68290,136581,1.5968308448791504,0.00012070128307671834
68477,68478,68477,136955,1.6014587879180908,0.00011892514161804504
68664,68665,68664,137329,1.6060898303985596,0.00011716512636873013
68851,68852,68851,137703,1.6106958389282227,0.00011544950032027693
69038,69039,69038,138077,1.6153180599212646,0.0001137575522005755
69226,69227,69226,138453,1.6200129985809326,0.00011206453767014268
69413,69414,69413,138827,1.6248259544372559,0.00011041733077986666
69600,69601,69600,139201,1.6293590068817139,0.0001088034974836542
69787,69788,69787,139575,1.6337499618530273,0.00010719618429535866
69974,69975,69974,139949,1.6380369663238525,0.00010561410404233692
70161,70162,70161,140323,1.6422998905181885,0.00010407103537283537
70348,70349,70348,140697,1.6469669342041016,0.00010253953519663282
70535,70536,70535,141071,1.6512689590454102,0.00010102204525180316
70722,70723,70722,141445,1.655526876449585,9.954285523125846e-05
70909,70910,70909,141819,1.6597659587860107,9.808396173392452e-05
71097,71098,71097,142195,1.6641230583190918,9.662419557322136e-05
71284,71285,71284,142569,1.6684401035308838,9.520401255759551e-05
71471,71472,71471,142943,1.6726980209350586,9.381250606206607e-05
71658,71659,71658,143317,1.6769719123840332,9.2426597511268e-05
71845,71846,71845,143691,1.6813280582427979,9.106255573681657e-05
72032,72033,72032,144065,1.6855731010437012,8.973210643316464e-05
72219,72220,72219,144439,1.6898798942565918,8.841155130848753e-05
72406,72407,72406,144813,1.6941397190093994,8.71031677827014e-05
72593,72594,72593,145187,1.698429822921753,8.582782946020835e-05
72780,72781,72780,145561,1.702692985534668,8.456988862220622e-05
72967,72968,72967,145935,1.7069408893585205,8.331787692839103e-05
73155,73156,73155,146311,1.7112419605255127,8.208678799428864e-05
73342,73343,73342,146685,1.7157728672027588,8.088697944669624e-05
73529,73530,73529,147059,1.7201499938964844,7.969197771693438e-05
73716,73717,73716,147433,1.7244799137115479,7.851592510472913e-05
73903,73904,73903,147807,1.7289578914642334,7.736879793838217e-05
74090,74091,74090,148181,1.7332987785339355,7.623013285887106e-05
74277,74278,74277,148555,1.7377588748931885,7.510204177545216e-05
74464,74465,74464,148929,1.7421259880065918,7.400246145689928e-05
74651,74652,74651,149303,1.7464938163757324,7.291779321502103e-05
74838,74839,74838,149677,1.7508888244628906,7.18382729606123e-05
75026,75027,75026,150053,1.7552800178527832,7.077685691626391e-05
75213,75214,75213,150427,1.759645938873291,6.974233710509548e-05
75400,75401,75400,150801,1.763988971710205,6.871194532311312e-05
75587,75588,75587,151175,1.7681231498718262,6.769797381806686e-05
75774,75775,75774,151549,1.7724449634552002,6.670890853821944e-05
75961,75962,75961,151923,1.7765769958496094,6.572708045283697e-05
76148,76149,76148,152297,1.781285047531128,6.475443822548944e-05
76335,76336,76335,152671,1.7856769561767578,6.380639396660755e-05
76522,76523,76522,153045,1.7900640964508057,6.287113105570844e-05
76709,76710,76709,153419,1.7952229976654053,6.19403381817766e-05
76896,76897,76896,153793,1.8000550270080566,6.1030012126714567e-05
77084,77085,77084,154169,1.8050339221954346,6.0133208114522104e-05
77271,77272,77271,154543,1.8108007907867432,5.924475169351271e-05
77458,77459,77458,154917,1.8152050971984863,5.837052377656789e-05
77645,77646,77645,155291,1.8196039199829102,5.7517740831695094e-05
77832,77833,77832,155665,1.823970079421997,5.66711474266643e-05
78019,78020,78019,156039,1.8283770084381104,5.583253377145629e-05
78206,78207,78206,156413,1.8326399326324463,5.5015141785822924e-05
78393,78394,78393,156787,1.8368780612945557,5.420870453937612e-05
78580,78581,78580,157161,1.8413569927215576,5.3406148904075597e-05
78767,78768,78767,157535,1.8457419872283936,5.2621287127714355e-05
78955,78956,78955,157911,1.8501529693603516,5.1848028848533055e-05
79142,79143,79142,158285,1.8556420803070068,5.1081956537370607e-05
79329,79330,79329,158659,1.8599579334259033,5.032821315381988e-05
79516,79517,79516,159033,1.8643889427185059,4.959293406723678e-05
79703,79704,79703,159407,1.868685007095337,4.88629484713675e-05
79890,79891,79890,159781,1.8729829788208008,4.8139894701805306e-05
80077,80078,80077,160155,1.877267837524414,4.743514930706661e-05
80264,80265,80264,160529,1.8815300464630127,4.673979280293506e-05
80451,80452,80451,160903,1.8858098983764648,4.60478071478506e-05
80638,80639,80638,161277,1.8900859355926514,4.5371117702325076e-05
80826,80827,80826,161653,1.8943758010864258,4.470438499575263e-05
81013,81014,81013,162027,1.89864182472229,4.4043838655355135e-05
81200,81201,81200,162401,1.9028759002685547,4.3393974957106844e-05
81387,81388,81387,162775,1.9071249961853027,4.276000879336506e-05
81574,81575,81574,163149,1.9114348888397217,4.2130569748937e-05
81761,81762,81761,163523,1.915815830230713,4.15071520675612e-05
81948,81949,81948,163897,1.9202649593353271,4.089952903545527e-05
82135,82136,82135,164271,1.9247548580169678,4.029995262096377e-05
82322,82323,82322,164645,1.9292950630187988,3.970330367396945e-05
82509,82510,82509,165019,1.9337809085845947,3.911987785349092e-05
82696,82697,82696,165393,1.9383549690246582,3.8548045155331694e-05
82884,82885,82884,165769,1.9429340362548828,3.7975438997331076e-05
83071,83072,83071,166143,1.947551965713501,3.7415138553727336e-05
83258,83259,83258,166517,1.9521708488464355,3.686852536875304e-05
83445,83446,83445,166891,1.9568419456481934,3.632578385126334e-05
83632,83633,83632,167265,1.9614441394805908,3.578827268195361e-05
83819,83820,83819,167639,1.9660170078277588,3.5264387253500066e-05
84006,84007,84006,168013,1.9706017971038818,3.47473978575505e-05
84193,84194,84193,168387,1.9752271175384521,3.423295101139973e-05
84380,84381,84380,168761,1.9798851013183594,3.3729934884656196e-05
84567,84568,84567,169135,1.9845008850097656,3.323687874229609e-05
84755,84756,84755,169511,1.9891250133514404,3.274314891103856e-05
84942,84943,84942,169885,1.9937548637390137,3.226006833030532e-05
85129,85130,85129,170259,1.9983890056610107,3.178877175301586e-05
85316,85317,85316,170633,2.0029828548431396,3.132078626451701e-05
85503,85504,85503,171007,2.0075879096984863,3.0857343903627296e-05
85690,85691,85690,171381,2.0121960639953613,3.0405655935950376e-05
85877,85878,85877,171755,2.0167810916900635,2.995987775869952e-05
86064,86065,86064,172129,2.0214130878448486,2.9516307945188924e-05
86251,86252,86251,172503,2.026047945022583,2.908261915838893e-05
86438,86439,86438,172877,2.0306930541992188,2.8657487050586945e-05
86625,86626,86625,173251,2.0353541374206543,2.8234023021484022e-05
86813,86814,86813,173627,2.0400187969207764,2.781526547945966e-05
87000,87001,87000,174001,2.0445938110351562,2.7408907654411187e-05
87187,87188,87187,174375,2.049191951751709,2.7005381486189263e-05
87374,87375,87374,174749,2.0537641048431396,2.6605801414724863e-05
87561,87562,87561,175123,2.0583698749542236,2.6216361163541413e-05
87748,87749,87748,175497,2.06292986869812,2.583198535564269e-05
87935,87936,87935,175871,2.0675110816955566,2.5449527751036882e-05
88122,88123,88122,176245,2.072122097015381,2.5075611362282623e-05
88309,88310,88309,176619,2.0767059326171875,2.4709045867219785e-05
88496,88497,88496,176993,2.0813066959381104,2.4343913983341793e-05
88684,88685,88684,177369,2.085984945297241,2.3982869103083224e-05
88871,88872,88871,177743,2.0905709266662598,2.3632502157121766e-05
89058,89059,89058,178117,2.096385955810547,2.3284556841200038e-05
89245,89246,89245,178491,2.101010799407959,2.2940038957551036e-05
89432,89433,89432,178865,2.105602979660034,2.2604267895293994e-05
89619,89620,89619,179239,2.110128879547119,2.2272836717731775e-05
89806,89807,89806,179613,2.1146140098571777,2.1943071792321257e-05
89993,89994,89993,179987,2.1192398071289062,2.162068975784501e-05
90180,90181,90180,180361,2.1239097118377686,2.1304622577706515e-05
90367,90368,90367,180735,2.1287119388580322,2.0989787671283153e-05
90555,90556,90555,181111,2.1334378719329834,2.0678501615143676e-05
90742,90743,90742,181485,2.1381239891052246,2.0376410614917033e-05
90929,90930,90929,181859,2.1428170204162598,2.0076390579461483e-05
91116,91117,91116,182233,2.147420883178711,1.977934740339064e-05
91303,91304,91303,182607,2.152007818222046,1.9489849244247373e-05
91490,91491,91490,182981,2.15659499168396,1.9204069959641847e-05
91677,91678,91677,183355,2.161273956298828,1.8919738139852057e-05
91864,91865,91864,183729,2.165937900543213,1.864178781386721e-05
92051,92052,92051,184103,2.170624017715454,1.8369262176542764e-05
92238,92239,92238,184477,2.1755146980285645,1.8097795901634047e-05
92425,92426,92425,184851,2.18044376373291,1.7830818527634836e-05
92613,92614,92613,185227,2.185357093811035,1.7568944066439988e-05
92800,92801,92800,185601,2.19018292427063,1.731024819765097e-05
92987,92988,92987,185975,2.1949408054351807,1.7054137777743343e-05
93174,93175,93174,186349,2.19973087310791,1.680453554661835e-05
93361,93362,93361,186723,2.204525947570801,1.6558119946092687e-05
93548,93549,93548,187097,2.2093417644500732,1.6312961809951906e-05
93735,93736,93735,187471,2.214207887649536,1.607331945990642e-05
93922,93923,93922,187845,2.2190468311309814,1.583833698793168e-05
94109,94110,94109,188219,2.223914861679077,1.5604265360299654e-05
94296,94297,94296,188593,2.228778839111328,1.537408259337598e-05
94484,94485,94484,188969,2.2337751388549805,1.5148290869013636e-05
94671,94672,94671,189343,2.238529920578003,1.4925227273039049e-05
94858,94859,94858,189717,2.2434568405151367,1.4704409118360275e-05
95045,95046,95045,190091,2.2484798431396484,1.448920467445467e-05
95232,95233,95232,190465,2.2533249855041504,1.427673070911412e-05
95419,95420,95419,190839,2.2581801414489746,1.406534919725595e-05
95606,95607,95606,191213,2.2630269527435303,1.3858735086117635e-05
95793,95794,95793,191587,2.2680089473724365,1.3656123762341962e-05
95980,95981,95980,191961,2.2728869915008545,1.3454295699760046e-05
96167,96168,96167,192335,2.277643918991089,1.3255836568926479e-05
96354,96355,96354,192709,2.2823989391326904,1.30621850642697e-05
96542,96543,96542,193085,2.287161111831665,1.286881656946261e-05
96729,96730,96729,193459,2.2918479442596436,1.2678427432734e-05
96916,96917,96916,193833,2.296588897705078,1.2492880352964783e-05
97103,97104,97103,194207,2.3012988567352295,1.2309672825115145e-05
97290,97291,97290,194581,2.306051015853882,1.212741443448513e-05
97477,97478,97477,194955,2.3106539249420166,1.1949276498073185e-05
97664,97665,97664,195329,2.315268039703369,1.1774576821532299e-05
97851,97852,97851,195703,2.319905996322632,1.1600550792092263e-05
98038,98039,98038,196077,2.3245999813079834,1.1429443194230766e-05
98225,98226,98225,196451,2.3294661045074463,1.1262474152521028e-05
98413,98414,98413,196827,2.3341469764709473,1.1095739892655744e-05
98600,98601,98600,197201,2.338757038116455,1.0931586669747066e-05
98787,98788,98787,197575,2.343461036682129,1.077160982410564e-05
98974,98975,98974,197949,2.3477649688720703,1.0613637512732415e-05
99161,99162,99161,198323,2.3520350456237793,1.0456489857724152e-05
99348,99349,99348,198697,2.356292963027954,1.0302903413991403e-05
99535,99536,99535,199071,2.3606667518615723,1.0152270239699417e-05
99722,99723,99722,199445,2.364922046661377,1.000221652378774e-05
99909,99910,99909,199819,2.3695411682128906,9.854690908197945e-06
100096,100097,100096,200193,2.37441086769104,9.710727807113096e-06
100284,100285,100284,200569,2.3807249069213867,9.566959240369153e-06
100471,100472,100471,200943,2.384960889816284,9.425426627462641e-06
100658,100659,100658,201317,2.3892128467559814,9.287496145729321e-06
100845,100846,100845,201691,2.393415927886963,9.151283102412643e-06
101032,101033,101032,202065,2.397825002670288,9.015786588836505e-06
101219,101220,101219,202439,2.40207576751709,8.883367869682578e-06
101406,101407,101406,202813,2.406338930130005,8.753485771720813e-06
101593,101594,101593,203187,2.410590887069702,8.624102186796792e-06
101780,101781,101780,203561,2.414923906326294,8.49690851360755e-06
101967,101968,101967,203935,2.419221878051758,8.372781418570123e-06
102154,102155,102154,204309,2.423419952392578,8.249473638654357e-06
102342,102343,102342,204685,2.4276390075683594,8.126786173950723e-06
102529,102530,102529,205059,2.4319698810577393,8.007863820417279e-06
102716,102717,102716,205433,2.436149835586548,7.890412883788656e-06
102903,102904,102903,205807,2.4403529167175293,7.77358455114003e-06
103090,103091,103090,206181,2.444559097290039,7.659416151621105e-06
103277,103278,103277,206555,2.448909044265747,7.547426446474483e-06
103464,103465,103464,206929,2.453096866607666,7.43586568047614e-06
103651,103652,103651,207303,2.4572908878326416,7.326201823287667e-06
103838,103839,103838,207677,2.461587905883789,7.219177583850997e-06
104025,104026,104025,208051,2.4658169746398926,7.112854009624092e-06
104213,104214,104213,208427,2.470461845397949,7.0070731382570245e-06
104400,104401,104400,208801,2.474655866622925,6.904539384375117e-06
104587,104588,104587,209175,2.4790759086608887,6.803266230271338e-06
104774,104775,104774,209549,2.4832959175109863,6.702534086080709e-06
104961,104962,104961,209923,2.487504005432129,6.604100688455176e-06
105148,105149,105148,210297,2.491933822631836,6.507538511957495e-06
105335,105336,105335,210671,2.4961321353912354,6.411345466304902e-06
105522,105523,105522,211045,2.5004000663757324,6.316795482318134e-06
105709,105710,105709,211419,2.504795789718628,6.2245175469782834e-06
105896,105897,105896,211793,2.5090909004211426,6.132838809970146e-06
106083,106084,106083,212167,2.5133790969848633,6.04211387141789e-06
106271,106272,106271,212543,2.5179738998413086,5.953231116997114e-06
106458,106459,106458,212917,2.5222740173339844,5.865907392650114e-06
106645,106646,106645,213291,2.526664972305298,5.77905379344793e-06
106832,106833,106832,213665,2.5310728549957275,5.694186749834369e-06
107019,107020,107019,214039,2.5353899002075195,5.610926803063698e-06
107206,107207,107206,214413,2.5396950244903564,5.527984566202865e-06
107393,107394,107393,214787,2.5439929962158203,5.44646547336183e-06
107580,107581,107580,215161,2.548314094543457,5.366901997486145e-06
107767,107768,107767,215535,2.5526130199432373,5.2878509480087e-06
107954,107955,107954,215909,2.556920051574707,5.209628134618074e-06
108142,108143,108142,216285,2.5613629817962646,5.132994213249259e-06
108329,108330,108329,216659,2.565703868865967,5.057698504554659e-06
108516,108517,108516,217033,2.570056915283203,4.982811337183524e-06
108703,108704,108703,217407,2.574458122253418,4.90964089049972e-06
108890,108891,108890,217781,2.578878879547119,4.837850659778172e-06
109077,109078,109077,218155,2.5833189487457275,4.7663339228397066e-06
109264,109265,109264,218529,2.5876519680023193,4.6960498122217484e-06
109451,109452,109451,218903,2.591982126235962,4.627448916350649e-06
109638,109639,109638,219277,2.5963470935821533,4.559286242113124e-06
109825,109826,109825,219651,2.6006689071655273,4.49184275074982e-06
110013,110014,110013,220027,2.6050219535827637,4.425769646000788e-06
110200,110201,110200,220401,2.609369993209839,4.360845198767912e-06
110387,110388,110387,220775,2.6137619018554688,4.296275787205467e-06
110574,110575,110574,221149,2.6182310581207275,4.233189876717868e-06
110761,110762,110761,221523,2.622499942779541,4.1712892984581035e-06
110948,110949,110948,221897,2.6274538040161133,4.109624187575069e-06
111135,111136,111135,222271,2.6316709518432617,4.049026659711502e-06
111322,111323,111322,222645,2.6358609199523926,3.989877853042037e-06
111509,111510,111509,223019,2.640145778656006,3.93110381039468e-06
111696,111697,111696,223393,2.6443488597869873,3.872954238580637e-06
111883,111884,111883,223767,2.6485979557037354,3.816286596150296e-06
112071,112072,112071,224143,2.6529409885406494,3.7600048274759726e-06
112258,112259,112258,224517,2.6572060585021973,3.7043316389209912e-06
112445,112446,112445,224891,2.6614980697631836,3.649940383554433e-06
112632,112633,112632,225265,2.665876865386963,3.596567065886293e-06
112819,112820,112819,225639,2.672712802886963,3.5433965075921052e-06
113006,113007,113006,226013,2.677194833755493,3.4911505612866426e-06
113193,113194,113193,226387,2.68174409866333,3.440151480602137e-06
113380,113381,113380,226761,2.685980796813965,3.3894728971254445e-06
113567,113568,113567,227135,2.69018292427063,3.3393365299366484e-06
113754,113755,113754,227509,2.694535970687866,3.2904781629288617e-06
113942,113943,113942,227885,2.6987509727478027,3.2419486631262925e-06
114129,114130,114129,228259,2.7029848098754883,3.1939460142228856e-06
114316,114317,114316,228633,2.707180976867676,3.147051091054929e-06
114503,114504,114503,229007,2.711411952972412,3.101030326676597e-06
114690,114691,114690,229381,2.7156431674957275,3.0551841840397837e-06
114877,114878,114877,229755,2.719953775405884,3.0101388063667154e-06
115064,115065,115064,230129,2.7245497703552246,2.9661665381162595e-06
115251,115252,115251,230503,2.7288928031921387,2.9224683600527273e-06
115438,115439,115438,230877,2.7331130504608154,2.879240964603016e-06
115625,115626,115625,231251,2.7373178005218506,2.8371156775275918e-06
115812,115813,115812,231625,2.741569995880127,2.795493077687302e-06
116000,116001,116000,232001,2.7457950115203857,2.7538817154258452e-06
116187,116188,116187,232375,2.7501261234283447,2.7134499584416734e-06
116374,116375,116374,232749,2.7543418407440186,2.6737688686372147e-06
116561,116562,116561,233123,2.758549928665161,2.6342381910902593e-06
116748,116749,116748,233497,2.7627508640289307,2.595401000450072e-06
116935,116936,116935,233871,2.766939878463745,2.557487354452493e-06
117122,117123,117122,234245,2.7711710929870605,2.519808112964479e-06
117309,117310,117309,234619,2.7754039764404297,2.4825376196038046e-06
117496,117497,117496,234993,2.77962589263916,2.4462175289935667e-06
117683,117684,117683,235367,2.7838330268859863,2.410328030316202e-06
117871,117872,117871,235743,2.788058042526245,2.3744498149535475e-06
118058,118059,118058,236117,2.792595863342285,2.3395904523992656e-06
118245,118246,118245,236491,2.7968029975891113,2.3053756931419308e-06
118432,118433,118432,236865,2.801146984100342,2.2712905132322475e-06
118619,118620,118619,237239,2.805371046066284,2.23780589717731e-06
118806,118807,118806,237613,2.809678077697754,2.205116087407198e-06
118993,118994,118993,237987,2.813865900039673,2.1726267443665452e-06
119180,119181,119180,238361,2.818150758743286,2.1404922788546726e-06
119367,119368,119367,238735,2.8223800659179688,2.10917737385887e-06
119554,119555,119554,239109,2.826676845550537,2.0782312943984545e-06
119742,119743,119742,239485,2.831016778945923,2.047296333414855e-06
119929,119930,119929,239859,2.835218906402588,2.0172413626205756e-06
120116,120117,120116,240233,2.8394081592559814,1.9877399019095828e-06
120303,120304,120303,240607,2.843596935272217,1.958350090568844e-06
120490,120491,120490,240981,2.84771990776062,1.929480356479852e-06
120677,120678,120677,241355,2.851987838745117,1.901294619387699e-06
120864,120865,120864,241729,2.856260061264038,1.873280326547717e-06
121051,121052,121051,242103,2.8605589866638184,1.8455741315079568e-06
121238,121239,121238,242477,2.8647959232330322,1.8185746515947813e-06
121425,121426,121425,242851,2.8691439628601074,1.79189108145171e-06
121612,121613,121612,243225,2.8733949661254883,1.7653588640214491e-06
121800,121801,121800,243601,2.8776707649230957,1.7393055761729427e-06
121987,121988,121987,243975,2.881967067718506,1.7138681196715793e-06
122174,122175,122174,244349,2.8861899375915527,1.6885268786295739e-06
122361,122362,122361,244723,2.8904287815093994,1.663636002211831e-06
122548,122549,122548,245097,2.894728899002075,1.6393337478974113e-06
122735,122736,122735,245471,2.8989810943603516,1.6151781187238822e-06
122922,122923,122922,245845,2.9031779766082764,1.5912899662961534e-06
123109,123110,123109,246219,2.9073619842529297,1.5680112072536522e-06
123296,123297,123296,246593,2.9115538597106934,1.5450030260410855e-06
123483,123484,123483,246967,2.9158599376678467,1.5221263943804544e-06
123671,123672,123671,247343,2.920197010040283,1.4996638215014759e-06
123858,123859,123858,247717,2.924506902694702,1.4777305214578356e-06
124045,124046,124045,248091,2.9287350177764893,1.455880149434388e-06
124232,124233,124232,248465,2.932987928390503,1.4344197629803027e-06
124419,124420,124419,248839,2.9371750354766846,1.4134659102745938e-06
124606,124607,124606,249213,2.9413628578186035,1.392637458113192e-06
124793,124794,124793,249587,2.9455437660217285,1.3720412105127755e-06
124980,124981,124980,249961,2.9498491287231445,1.3519704245977615e-06
125167,125168,125167,250335,2.95413875579834,1.3321313826633946e-06
125354,125355,125354,250709,2.958393096923828,1.3124066805218723e-06
125541,125542,125541,251083,2.962583065032959,1.2931416288618973e-06
125729,125730,125729,251459,2.9667770862579346,1.2741280741637569e-06
125916,125917,125916,251833,2.971031904220581,1.2552876939649742e-06
126103,126104,126103,252207,2.9753201007843018,1.2367850055225978e-06
126290,126291,126290,252581,2.9795780181884766,1.2187181998561315e-06
126477,126478,126477,252955,2.983773946762085,1.2007586439607143e-06
126664,126665,126664,253329,2.9880030155181885,1.1830006658761244e-06
126851,126852,126851,253703,2.994776964187622,1.1656957672508904e-06
127038,127039,127038,254077,2.99908709526062,1.1485893463400676e-06
127225,127226,127225,254451,3.003325939178467,1.1315823088694163e-06
127412,127413,127412,254825,3.0075669288635254,1.1149724032840394e-06
127600,127601,127600,255201,3.011868953704834,1.098578069764594e-06
127787,127788,127787,255575,3.0161259174346924,1.0823330455517874e-06
127974,127975,127974,255949,3.0204269886016846,1.0663804233047136e-06
128161,128162,128161,256323,3.0247089862823486,1.0508028780979598e-06
128348,128349,128348,256697,3.0290307998657227,1.0353170604498794e-06
128535,128536,128535,257071,3.0333690643310547,1.0200062282335457e-06
128722,128723,128722,257445,3.0375900268554688,1.0050860548689547e-06
128909,128910,128909,257819,3.0418028831481934,9.903358632537747e-07
129096,129097,129096,258193,3.0461349487304688,9.756720566452594e-07
129283,129284,129283,258567,3.050410032272339,9.613513583083727e-07
129470,129471,129470,258941,3.054630756378174,9.47290479189078e-07
129658,129659,129658,259317,3.059141159057617,9.332082424235542e-07
129845,129846,129845,259691,3.063509941101074,9.194542343457325e-07
130032,130033,130032,260065,3.067949056625366,9.06022972105764e-07
130219,130220,130219,260439,3.0723209381103516,8.926701630234539e-07
130406,130407,130406,260813,3.0765650272369385,8.794692506169869e-07
130593,130594,130593,261187,3.080641984939575,8.666051683583116e-07
130780,130781,130780,261561,3.0849769115448,8.538866588057278e-07
130967,130968,130967,261935,3.089171886444092,8.412432371426228e-07
131154,131155,131154,262309,3.0933339595794678,8.288962420503812e-07
131341,131342,131341,262683,3.097531795501709,8.167723206030318e-07
131529,131530,131529,263059,3.1015820503234863,8.046299872612863e-07
131716,131717,131716,263433,3.1079139709472656,7.927715784358725e-07
131903,131904,131903,263807,3.1119189262390137,7.811908787780524e-07
132090,132091,132090,264181,3.1165449619293213,7.69677280117116e-07
132277,132278,132277,264555,3.1206777095794678,7.582955319415095e-07
132464,132465,132464,264929,3.124884843826294,7.47204195567279e-07
132651,132652,132651,265303,3.1290407180786133,7.362375242770884e-07
132838,132839,132838,265677,3.1331467628479004,7.253361221494412e-07
133025,133026,133025,266051,3.1372647285461426,7.146908099303408e-07
133212,133213,133212,266425,3.141300916671753,7.042370171965073e-07
133400,133401,133400,266801,3.145404815673828,6.937673583062973e-07
133587,133588,133587,267175,3.1496188640594482,6.835432953716374e-07
133774,133775,133774,267549,3.153864860534668,6.735581836327191e-07
133961,133962,133961,267923,3.1580867767333984,6.636304644856688e-07
134148,134149,134148,268297,3.162320852279663,6.538171917850861e-07
134335,134336,134335,268671,3.1665499210357666,6.442543036594645e-07
134522,134523,134522,269045,3.170761823654175,6.347981726575333e-07
134709,134710,134709,269419,3.174992084503174,6.253987768253924e-07
134896,134897,134896,269793,3.179297924041748,6.162206177136652e-07
135083,135084,135083,270167,3.183521032333374,6.072068827753552e-07
135270,135271,135270,270541,3.1877219676971436,5.982272346425786e-07
135458,135459,135458,270917,3.191939115524292,5.893645163812807e-07
135645,135646,135645,271291,3.196131944656372,5.807551494252696e-07
135832,135833,135832,271665,3.2003538608551025,5.721948722750327e-07
136019,136020,136019,272039,3.2045629024505615,5.637339318953521e-07
136206,136207,136206,272413,3.2087841033935547,5.554888607671313e-07
136393,136394,136393,272787,3.213050127029419,5.473352086048563e-07
136580,136581,136580,273161,3.217249870300293,5.392308740514155e-07
136767,136768,136767,273535,3.22149395942688,5.313176618707041e-07
136954,136955,136954,273909,3.2257609367370605,5.235456078549778e-07
137141,137142,137141,274283,3.2299749851226807,5.158029592503749e-07
137329,137330,137329,274659,3.234251022338867,5.081617162313897e-07
137516,137517,137516,275033,3.23848295211792,5.007385416909947e-07
137703,137704,137703,275407,3.242722988128662,4.93357356254999e-07
137890,137891,137890,275781,3.2469868659973145,4.86062390195687e-07
138077,138078,138077,276155,3.2510199546813965,4.789535317215973e-07
138264,138265,138264,276529,3.255103826522827,4.7192295543679184e-07
138451,138452,138451,276903,3.259168863296509,4.649352494608263e-07
138638,138639,138638,277277,3.263301134109497,4.581126466015908e-07
138825,138826,138825,277651,3.26743483543396,4.5141122464696227e-07
139012,139013,139012,278025,3.2720067501068115,4.447351736329414e-07
139199,139200,139199,278399,3.2762291431427,4.381816094722867e-07
139387,139388,139387,278775,3.2805349826812744,4.317466434791634e-07
139574,139575,139574,279149,3.284637928009033,4.2538214261452717e-07
139761,139762,139761,279523,3.288749933242798,4.1909247364539517e-07
139948,139949,139948,279897,3.2929489612579346,4.1296325005862696e-07
140135,140136,140135,280271,3.2971549034118652,4.069010577082447e-07
140322,140323,140322,280645,3.3013110160827637,4.008761315761181e-07
140509,140510,140509,281019,3.3054099082946777,3.949938281229224e-07
140696,140697,140696,281393,3.309525966644287,3.892155526202006e-07
140883,140884,140883,281767,3.313713788986206,3.83459170499355e-07
141070,141071,141070,282141,3.3178930282592773,3.778088312002454e-07
141258,141259,141258,282517,3.3231868743896484,3.7226046755732563e-07
141445,141446,141445,282891,3.328665018081665,3.6677261380915337e-07
141632,141633,141632,283265,3.332894802093506,3.61349706537982e-07
141819,141820,141819,283639,3.3370108604431152,3.560651178280321e-07
142006,142007,142006,284013,3.34114408493042,3.5083792472940603e-07
142193,142194,142193,284387,3.3453550338745117,3.4564312666207645e-07
142380,142381,142380,284761,3.3496408462524414,3.4057152876186667e-07
142567,142568,142567,285135,3.3563408851623535,3.355892313149198e-07
142754,142755,142754,285509,3.3606679439544678,3.3062582931825516e-07
142941,142942,142941,285883,3.3651559352874756,3.2575423118729027e-07
143129,143130,143129,286259,3.3695499897003174,3.2097031303285606e-07
143316,143317,143316,286633,3.3747549057006836,3.162383575640425e-07
143503,143504,143503,287007,3.3793249130249023,3.1156276731591115e-07
143690,143691,143690,287381,3.3835787773132324,3.0700641752440606e-07
143877,143878,143877,287755,3.3878419399261475,3.024992114149619e-07
144064,144065,144064,288129,3.392096996307373,2.980201661029779e-07
144251,144252,144251,288503,3.3963420391082764,2.9364754085296806e-07
144438,144439,144438,288877,3.4018709659576416,2.893515713745136e-07
144625,144626,144625,289251,3.4067671298980713,2.850719125142022e-07
144812,144813,144812,289625,3.411733865737915,2.80871728298538e-07
144999,145000,144999,289999,3.4160261154174805,2.7676876323734215e-07
145187,145188,145187,290375,3.420341968536377,2.726667556524391e-07
145374,145375,145374,290749,3.4245359897613525,2.686354977295241e-07
145561,145562,145561,291123,3.4287519454956055,2.6470703124672494e-07
145748,145749,145748,291497,3.4329400062561035,2.608206417130705e-07
145935,145936,145935,291871,3.43715500831604,2.569587322848775e-07
146122,146123,146122,292245,3.4414899349212646,2.5318874611171026e-07
146309,146310,146309,292619,3.4458837509155273,2.494845596386039e-07
146496,146497,146496,292993,3.4503448009490967,2.4579445466600897e-07
146683,146684,146683,293367,3.4548768997192383,2.421731490306202e-07
146870,146871,146870,293741,3.459526777267456,2.38635482836412e-07
147058,147059,147058,294117,3.464223861694336,2.3509848766170576e-07
147245,147246,147245,294491,3.4689650535583496,2.3162276910827044e-07
147432,147433,147432,294865,3.4734349250793457,2.282356600443629e-07
147619,147620,147619,295239,3.4778218269348145,2.248845763107955e-07
147806,147807,147806,295613,3.4821810722351074,2.2155477321519806e-07
147993,147994,147993,295987,3.4865567684173584,2.1830436941342144e-07
148180,148181,148180,296361,3.4909067153930664,2.151104450760749e-07
148367,148368,148367,296735,3.495234966278076,2.1192867965992553e-07
148554,148555,148554,297109,3.499569892883301,2.088064705705582e-07
148741,148742,148741,297483,3.5038809776306152,2.0575621626023136e-07
148928,148929,148928,297857,3.5082128047943115,2.0272259413616273e-07
149116,149117,149116,298233,3.512572765350342,1.9970967272078383e-07
149303,149304,149303,298607,3.516890048980713,1.967893190281721e-07
149490,149491,149490,298981,3.521223783493042,1.9389980855876418e-07
149677,149678,149677,299355,3.5255749225616455,1.910287975334697e-07
149864,149865,149864,299729,3.5299198627471924,1.882263665013078e-07
150051,150052,150051,300103,3.5342750549316406,1.8547241347129842e-07
150238,150239,150238,300477,3.538609743118286,1.8272896092451056e-07
150425,150426,150425,300851,3.542937994003296,1.8003706203624282e-07
150612,150613,150612,301225,3.5471527576446533,1.7740706410564331e-07
150799,150800,150799,301599,3.5512819290161133,1.7479129477704622e-07
150987,150988,150987,301975,3.555433988571167,1.721935786827809e-07
151174,151175,151174,302349,3.5596299171447754,1.6967565909745948e-07
151361,151362,151361,302723,3.5638070106506348,1.671841452918875e-07
151548,151549,151548,303097,3.5685079097747803,1.647087132027681e-07
151735,151736,151735,303471,3.572643995285034,1.6229251472821105e-07
151922,151923,151922,303845,3.5768849849700928,1.5991792516151995e-07
152109,152110,152109,304219,3.58111572265625,1.5755240515411496e-07
152296,152297,152296,304593,3.5852599143981934,1.5523151029432017e-07
152483,152484,152483,304967,3.589366912841797,1.5296386603236943e-07
152670,152671,152670,305341,3.593491792678833,1.5070839451582388e-07
152858,152859,152858,305717,3.5977869033813477,1.4846866568253455e-07
153045,153046,153045,306091,3.6019198894500732,1.462977228006504e-07
153232,153233,153232,306465,3.606074094772339,1.4414938602741438e-07
153419,153420,153419,306839,3.6102120876312256,1.4201502931394068e-07
153606,153607,153606,307213,3.6145458221435547,1.399318323150105e-07
153793,153794,153793,307587,3.618750810623169,1.378843474463667e-07
153980,153981,153980,307961,3.622886896133423,1.3584469746278997e-07
154167,154168,154167,308335,3.6270320415496826,1.3384367416094907e-07
154354,154355,154354,308709,3.6311590671539307,1.3188845879856913e-07
154541,154542,154541,309083,3.6352927684783936,1.2994365769627671e-07
154728,154729,154728,309457,3.6394429206848145,1.2802271924379842e-07
154916,154917,154916,309833,3.6436469554901123,1.2614080178324659e-07
155103,155104,155103,310207,3.64789080619812,1.2428837326937385e-07
155290,155291,155290,310581,3.6520819664001465,1.2244809776594425e-07
155477,155478,155477,310955,3.6562888622283936,1.206520075621557e-07
155664,155665,155664,311329,3.6605348587036133,1.188865675419135e-07
155851,155852,155851,311703,3.664747953414917,1.1712789681402072e-07
156038,156039,156038,312077,3.669055938720703,1.1540265972152531e-07
156225,156226,156225,312451,3.6732118129730225,1.1371682712764783e-07
156412,156413,156412,312825,3.677480936050415,1.1203990470649522e-07
156599,156600,156599,313199,3.6817657947540283,1.103836885341955e-07
156787,156788,156787,313575,3.6860358715057373,1.0876110407652269e-07
156974,156975,156974,313949,3.6902668476104736,1.0716382577077655e-07
157161,157162,157161,314323,3.6946921348571777,1.0557711226218684e-07
157348,157349,157348,314697,3.699476957321167,1.0402855949229468e-07
157535,157536,157535,315071,3.7049999237060547,1.0250631168836324e-07
157722,157723,157722,315445,3.7099671363830566,1.0098991339823764e-07
157909,157910,157909,315819,3.7158660888671875,9.95024530256803e-08
158096,158097,158096,316193,3.720012903213501,9.804888808419536e-08
158283,158284,158283,316567,3.7243950366973877,9.660294669638268e-08
158470,158471,158470,316941,3.728700876235962,9.517497211641233e-08
158657,158658,158657,317315,3.732923746109009,9.378335995732566e-08
158845,158846,158845,317691,3.7372357845306396,9.239871135989565e-08
159032,159033,159032,318065,3.7415030002593994,9.103062334189227e-08
159219,159220,159219,318439,3.745774984359741,8.969549218020015e-08
159406,159407,159406,318813,3.750092029571533,8.838293610725361e-08
159593,159594,159593,319187,3.7543139457702637,8.707543547338188e-08
159780,159781,159780,319561,3.758591890335083,8.579298093650123e-08
159967,159968,159967,319935,3.7627949714660645,8.453968219896845e-08
160154,160155,160154,320309,3.76713490486145,8.329290649778859e-08
160341,160342,160341,320683,3.7713749408721924,8.206172007663993e-08
160528,160529,160528,321057,3.7785818576812744,8.086187514250326e-08
160716,160717,160716,321433,3.7828400135040283,7.966794557522773e-08
160903,160904,160903,321807,3.787095069885254,7.848836014787521e-08
161090,161091,161090,322181,3.7913100719451904,7.733723662582084e-08
161277,161278,161277,322555,3.7955310344696045,7.620548665317318e-08
161464,161465,161464,322929,3.799757957458496,7.507810651337581e-08
161651,161652,161651,323303,3.8039610385894775,7.397240343949954e-08
161838,161839,161838,323677,3.8081939220428467,7.289177867035844e-08
162025,162026,162025,324051,3.812412977218628,7.181673547379847e-08
162212,162213,162212,324425,3.816619873046875,7.075521826307321e-08
162399,162400,162399,324799,3.820905923843384,6.972071427283598e-08
162587,162588,162587,325175,3.825148820877075,6.869123435472955e-08
162774,162775,162774,325549,3.8293590545654297,6.767417895524232e-08
162961,162962,162961,325923,3.833570957183838,6.668170301937797e-08
163148,163149,163148,326297,3.8377788066864014,6.570585263802409e-08
163335,163336,163335,326671,3.842000722885132,6.47337799789688e-08
163522,163523,163522,327045,3.8461339473724365,6.378046804035453e-08
163709,163710,163709,327419,3.85025691986084,6.284872662234328e-08
163896,163897,163896,327793,3.854490041732788,6.1921761421995e-08
164083,164084,164083,328167,3.8587429523468018,6.100653165535744e-08
164270,164271,164270,328541,3.863132953643799,6.011458403097023e-08
164457,164458,164457,328915,3.867577075958252,5.92316210916602e-08
164645,164646,164645,329291,3.872565984725952,5.8349983396150944e-08
164832,164833,164832,329665,3.8772029876708984,5.7494290166987614e-08
165019,165020,165019,330039,3.881387948989868,5.665286383907038e-08
165206,165207,165206,330413,3.88598895072937,5.581470385110371e-08
165393,165394,165393,330787,3.8902530670166016,5.499278014364504e-08
165580,165581,165580,331161,3.8945047855377197,5.4189409360927586e-08
165767,165768,165767,331535,3.8987720012664795,5.3390125798275786e-08
165954,165955,165954,331909,3.903061866760254,5.260102383058928e-08
166141,166142,166141,332283,3.9073410034179688,5.183198780965797e-08
166328,166329,166328,332657,3.9117469787597656,5.107064241780847e-08
166516,166517,166516,333033,3.9161620140075684,5.0310482151614676e-08
166703,166704,166703,333407,3.9210128784179688,4.957272012393854e-08
166890,166891,166890,333781,3.925797700881958,4.8847200666627454e-08
167077,167078,167077,334155,3.9304068088531494,4.8124505769294844e-08
167264,167265,167264,334529,3.9345977306365967,4.7415862018589595e-08
167451,167452,167451,334903,3.9388039112091064,4.672317533712637e-08
167638,167639,167638,335277,3.9429988861083984,4.603398647384917e-08
167825,167826,167825,335651,3.947187900543213,4.5353630821405275e-08
168012,168013,168012,336025,3.951395034790039,4.4690568823628534e-08
168199,168200,168199,336399,3.9555981159210205,4.403408958737512e-08
168386,168387,168386,336773,3.959826946258545,4.33821191228846e-08
168574,168575,168574,337149,3.964092969894409,4.2742584957845226e-08
168761,168762,168761,337523,3.96834397315979,4.211700596310732e-08
168948,168949,168948,337897,3.9726078510284424,4.149386987113811e-08
169135,169136,169135,338271,3.9769768714904785,4.08828935471567e-08
169322,169323,169322,338645,3.9812419414520264,4.02856412882215e-08
169509,169510,169509,339019,3.9854729175567627,3.969138255891882e-08
169696,169697,169696,339393,3.989776134490967,3.910478703350767e-08
169883,169884,169883,339767,3.993980884552002,3.853309552589647e-08
170070,170071,170070,340141,3.9982898235321045,3.7967038360972154e-08
170257,170258,170257,340515,4.002586126327515,3.7404900691561146e-08
170445,170446,170445,340891,4.007117986679077,3.685350663719549e-08
170632,170633,170632,341265,4.011339902877808,3.631410114423049e-08
170819,170820,170819,341639,4.015542030334473,3.577680876241162e-08
171006,171007,171006,342013,4.0197460651397705,3.5250039077813566e-08
171193,171194,171193,342387,4.024014949798584,3.473507265881917e-08
171380,171381,171380,342761,4.028218030929565,3.422266833492817e-08
171567,171568,171567,343135,4.032428979873657,3.371691192635145e-08
171754,171755,171754,343509,4.036618947982788,3.322399979926098e-08
171941,171942,171941,343883,4.040819883346558,3.27359101620612e-08
172128,172129,172128,344257,4.045019865036011,3.225122768154495e-08
172316,172317,172316,344633,4.049232721328735,3.177582627024961e-08
172503,172504,172503,345007,4.053420066833496,3.1310723748089536e-08
172690,172691,172690,345381,4.057626724243164,3.0847449343953033e-08
172877,172878,172877,345755,4.061815977096558,3.039328070909963e-08
173064,173065,173064,346129,4.066055774688721,2.994926311814032e-08
173251,173252,173251,346503,4.070373058319092,2.950743845195563e-08
173438,173439,173438,346877,4.074689865112305,2.9071380796351507e-08
173625,173626,173625,347251,4.079113960266113,2.8646392080266367e-08
173812,173813,173812,347625,4.083492040634155,2.822553080352291e-08
173999,174000,173999,347999,4.087789058685303,2.780763135843333e-08
174186,174187,174186,348373,4.092078924179077,2.739990315000214e-08
174374,174375,174374,348749,4.09627890586853,2.6996714442878874e-08
174561,174562,174561,349123,4.100562810897827,2.6597261327436316e-08
174748,174749,174748,349497,4.104828834533691,2.6205687671125303e-08
174935,174936,174935,349871,4.109675884246826,2.5822843862290246e-08
175122,175123,175122,350245,4.114972829818726,2.5441877126996412e-08
175309,175310,175309,350619,4.120633125305176,2.5065913070254497e-08
175496,175497,175496,350993,4.125016927719116,2.4699487770430386e-08
175683,175684,175683,351367,4.129677057266235,2.4336594972370286e-08
175870,175871,175870,351741,4.1339240074157715,2.3976276842904162e-08
176057,176058,176057,352115,4.138312816619873,2.3624741345245e-08
176245,176246,176245,352491,4.142612934112549,2.3277091667657382e-08
176432,176433,176432,352865,4.146868944168091,2.293266785176763e-08
176619,176620,176619,353239,4.151428937911987,2.2595062110497157e-08
176806,176807,176806,353613,4.155822038650513,2.2264963847638645e-08
176993,176994,176993,353987,4.160130023956299,2.193647239557348e-08
177180,177181,177180,354361,4.164432764053345,2.1612320436636115e-08
177367,177368,177367,354735,4.168722867965698,2.1296388445908573e-08
177554,177555,177554,355109,4.173019886016846,2.09834796874281e-08
177741,177742,177741,355483,4.1772301197052,2.067280901019167e-08
177928,177929,177928,355857,4.1814329624176025,2.0369721713173187e-08
178115,178116,178115,356231,4.185612916946411,2.0071553005666696e-08
178303,178304,178303,356607,4.189847946166992,1.9772985227960805e-08
178490,178491,178490,356981,4.194085121154785,1.9481909446176037e-08
178677,178678,178677,357355,4.198282957077026,1.919728974863388e-08
178864,178865,178864,357729,4.2025768756866455,1.8914045574232594e-08
179051,179052,179051,358103,4.206766128540039,1.8634565521932555e-08
179238,179239,179238,358477,4.210981845855713,1.8362168767574318e-08
179425,179426,179425,358851,4.215178966522217,1.8092359319462724e-08
179612,179613,179612,359225,4.219400882720947,1.782449534564476e-08
179799,179800,179799,359599,4.223622798919678,1.7563179143730434e-08
179986,179987,179986,359973,4.227832078933716,1.730608292129827e-08
180174,180175,180174,360349,4.232095003128052,1.7048646434117338e-08
180361,180362,180361,360723,4.236296892166138,1.6797687684575038e-08
180548,180549,180548,361097,4.24226188659668,1.6552280723680838e-08
180735,180736,180735,361471,4.246525764465332,1.6308051373416883e-08
180922,180923,180922,361845,4.250852108001709,1.6067086955769748e-08
181109,181110,181109,362219,4.255124807357788,1.583222623077113e-08
181296,181297,181296,362593,4.259886980056763,1.55995797012799e-08
181483,181484,181483,362967,4.264092922210693,1.536862429553825e-08
181670,181671,181670,363341,4.268419981002808,1.51433223125604e-08
181857,181858,181857,363715,4.272709846496582,1.49216408435406e-08
182045,182046,182045,364091,4.277017116546631,1.469966940506714e-08
182232,182233,182232,364465,4.281280994415283,1.4483298618388156e-08
182419,182420,182419,364839,4.2855260372161865,1.4271701888326597e-08
182606,182607,182606,365213,4.289830923080444,1.4061113374955824e-08
182793,182794,182793,365587,4.294088840484619,1.3853356754240213e-08
182980,182981,182980,365961,4.298375844955444,1.3650859545166066e-08
183167,183168,183167,366335,4.302585124969482,1.3450257208217989e-08
183354,183355,183354,366709,4.306810140609741,1.325112485841904e-08
183541,183542,183541,367083,4.3110339641571045,1.3056873629458694e-08
183728,183729,183728,367457,4.315233945846558,1.2865728498776868e-08
183915,183916,183915,367831,4.31949782371521,1.267534765172913e-08
184103,184104,184103,368207,4.323732852935791,1.2487786591387566e-08
184290,184291,184290,368581,4.327956914901733,1.2305341906557625e-08
184477,184478,184477,368955,4.3321919441223145,1.2123760498745833e-08
184664,184665,184664,369329,4.336405992507935,1.1944635275202735e-08
184851,184852,184851,369703,4.340651988983154,1.1770041876222476e-08
185038,185039,185038,370077,4.344895839691162,1.1597069976201427e-08
185225,185226,185225,370451,4.34919810295105,1.1425375899939534e-08
185412,185413,185412,370825,4.353798866271973,1.1257896029482623e-08
185599,185600,185599,371199,4.358033895492554,1.1093080874053538e-08
185786,185787,185786,371573,4.3623058795928955,1.0928927415642822e-08
185974,185975,185974,371949,4.366631984710693,1.0767216662943253e-08
186161,186162,186161,372323,4.371365070343018,1.0609907672690896e-08
186348,186349,186348,372697,4.3766467571258545,1.0453337886326874e-08
186535,186536,186535,373071,4.38103175163269,1.0298898344439642e-08
186722,186723,186722,373445,4.385202884674072,1.0148363619096395e-08
186909,186910,186909,373819,4.389369010925293,9.99921645559584e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,4.1961669921875e-05,4.387072431292609
7,25,0,25,0.001046895980834961,1.8599119493748546
14,51,0,51,0.0020608901977539062,0.646060385810488
21,73,0,73,0.0030698776245117188,0.26582040601045587
28,95,0,95,0.004040956497192383,0.1833999765905473
36,121,0,121,0.005692720413208008,0.14479233503308572
43,142,0,142,0.006712913513183594,0.12148628045781244
50,165,0,165,0.00770878791809082,0.10970795608886257
57,186,0,186,0.008830785751342773,0.09676374585392662
64,207,0,207,0.00981593132019043,0.08826038441949174
71,228,0,228,0.010734796524047852,0.08112900746473846
78,249,0,249,0.011662721633911133,0.07580406717955492
85,270,0,270,0.012572765350341797,0.07085971198224368
93,294,0,294,0.013725757598876953,0.06697348496771001
100,315,0,315,0.014948844909667969,0.06333451309322462
107,336,0,336,0.015930652618408203,0.06067674552084343
114,357,0,357,0.016878843307495117,0.05871635172520547
121,378,0,378,0.017834901809692383,0.056659790925287744
128,403,0,403,0.019488811492919922,0.05332127980862829
135,425,0,425,0.020483732223510742,0.05204805447367443
142,450,0,450,0.02148294448852539,0.049579404670590604
150,478,0,478,0.022845745086669922,0.04675689435718442
157,504,0,504,0.023865699768066406,0.045083624619016896
164,527,0,527,0.024821996688842773,0.04301350751104416
171,550,0,550,0.0257718563079834,0.04063370343064385
178,573,0,573,0.02672886848449707,0.03910924173736095
185,600,0,600,0.02775883674621582,0.03822803808081074
192,624,0,624,0.028729677200317383,0.03677797991434598
199,648,0,648,0.02969980239868164,0.03492985198045036
207,677,0,677,0.03085470199584961,0.03391879149751803
214,705,0,705,0.032301902770996094,0.033565670266777495
221,731,0,731,0.0334010124206543,0.033005500441061875
228,758,0,758,0.03451895713806152,0.03231949399972589
235,782,0,782,0.03555488586425781,0.03151048754109619
242,808,0,808,0.03657269477844238,0.030645353634218324
249,833,0,833,0.03755378723144531,0.030081184772192463
256,859,0,859,0.03856396675109863,0.029307968603637585
264,886,0,886,0.03966188430786133,0.02814876150516093
271,910,0,910,0.04063081741333008,0.027039792499845502
278,937,0,937,0.041645050048828125,0.02667730059761686
285,962,0,962,0.0426177978515625,0.02612073706533804
292,991,0,991,0.043673038482666016,0.02582150076757371
299,1019,0,1019,0.04476785659790039,0.025691287272492244
306,1047,0,1047,0.04606986045837402,0.025600828415971277
313,1075,0,1075,0.04742288589477539,0.025523709499047014
320,1100,0,1100,0.04843282699584961,0.025130884984063448
328,1130,0,1130,0.049696922302246094,0.024621272256751328
335,1158,0,1158,0.050752878189086914,0.024450777544715384
342,1187,0,1187,0.0519559383392334,0.024350499141507456
349,1216,0,1216,0.053067922592163086,0.024280694937420518
356,1244,0,1244,0.05420184135437012,0.024214741871332945
363,1271,0,1271,0.055365800857543945,0.024144977691097774
370,1297,0,1297,0.05671286582946777,0.023693693146526727
377,1324,0,1324,0.05797767639160156,0.023468386435305688
385,1352,0,1352,0.05975174903869629,0.0230718920440735
392,1379,0,1379,0.06134295463562012,0.02270568072110944
399,1407,0,1407,0.06255674362182617,0.02256274408688902
406,1434,0,1434,0.0637197494506836,0.022383564707340858
413,1462,0,1462,0.06490492820739746,0.022245878211648428
420,1489,0,1489,0.06615376472473145,0.022061472815687252
427,1517,0,1517,0.06744980812072754,0.021952739670894277
434,1546,0,1546,0.06884074211120605,0.021889230200436587
442,1581,0,1581,0.07019901275634766,0.021838309295896932
449,1609,0,1609,0.07133197784423828,0.02179987744820662
456,1639,0,1639,0.07258176803588867,0.021751620709180335
463,1667,0,1667,0.07374191284179688,0.021707045322382802
470,1695,0,1695,0.07486271858215332,0.021663649470072974
477,1723,0,1723,0.07613205909729004,0.021622498269092405
484,1751,0,1751,0.07725882530212402,0.02158139355226702
491,1779,0,1779,0.07835173606872559,0.021540392700689883
499,1811,0,1811,0.07963061332702637,0.02149427952781886
506,1839,0,1839,0.08072376251220703,0.02145399392835971
513,1867,0,1867,0.08191084861755371,0.02141404610143093
520,1895,0,1895,0.0829918384552002,0.021374292289720615
527,1923,0,1923,0.084075927734375,0.021334715166492976
534,1951,0,1951,0.08514189720153809,0.02129555883622578
541,1979,0,1979,0.08621001243591309,0.021256359756954137
548,2004,0,2004,0.08723282814025879,0.020921216963962697
556,2035,0,2035,0.08844280242919922,0.02055729678707214
563,2061,0,2061,0.08952069282531738,0.020267861625056307
570,2084,0,2084,0.09050989151000977,0.019584040008820063
577,2110,0,2110,0.09155869483947754,0.018973091897810115
584,2131,0,2131,0.0924978256225586,0.018305656258254668
591,2154,0,2154,0.09348082542419434,0.017277265498042312
598,2177,0,2177,0.09446382522583008,0.016598915990918922
605,2202,0,2202,0.09549283981323242,0.016238729235499908
613,2232,0,2232,0.09673190116882324,0.015756773248159
620,2258,0,2258,0.0977938175201416,0.015543776093101907
627,2284,0,2284,0.09886693954467773,0.015066994891946838
634,2311,0,2311,0.09995889663696289,0.014725009626560924
641,2338,0,2338,0.1009976863861084,0.014557724354790743
648,2365,0,2365,0.10205984115600586,0.014297515447903772
655,2391,0,2391,0.10312271118164062,0.014010500853507678
662,2416,0,2416,0.10417890548706055,0.013743857719186509
669,2440,0,2440,0.10532188415527344,0.01326398862732894
677,2471,0,2471,0.1065669059753418,0.01301344918648411
684,2498,0,2498,0.10764575004577637,0.012857413538610266
691,2524,0,2524,0.10905694961547852,0.012667823545067701
698,2553,0,2553,0.1102137565612793,0.012577492348836133
705,2581,0,2581,0.11131787300109863,0.012531026077236728
712,2607,0,2607,0.11236977577209473,0.012322151118212537
719,2635,0,2635,0.11348390579223633,0.012257017369904063
726,2663,0,2663,0.11454892158508301,0.012216447829210407
734,2695,0,2695,0.11574292182922363,0.012180930390465253
741,2723,0,2723,0.1170358657836914,0.012152039184658679
748,2750,0,2750,0.1181337833404541,0.012071384522412111
755,2778,0,2778,0.11960077285766602,0.012017374222100616
762,2805,0,2805,0.1213376522064209,0.011914715395052677
769,2832,0,2832,0.12274503707885742,0.011773116298406956
776,2860,0,2860,0.1239469051361084,0.011721443824168138
783,2885,0,2885,0.12560391426086426,0.011487765543719448
791,2914,0,2914,0.1273508071899414,0.011193753191120821
798,2942,0,2942,0.12911486625671387,0.011074155802639995
805,2970,0,2970,0.13102364540100098,0.011031339378686127
812,2999,0,2999,0.13227272033691406,0.010994569345441348
819,3027,0,3027,0.13341093063354492,0.010954059905350966
826,3055,0,3055,0.13451695442199707,0.010892436456724839
833,3083,0,3083,0.13562893867492676,0.010856460356790219
840,3112,0,3112,0.1367490291595459,0.010830082671694573
848,3145,0,3145,0.13803696632385254,0.010809090497539193
855,3174,0,3174,0.13916778564453125,0.010786129562399546
862,3202,0,3202,0.14028096199035645,0.01076617139498067
869,3230,0,3230,0.14139676094055176,0.010745307346032002
876,3258,0,3258,0.14250802993774414,0.010725306716583508
883,3286,0,3286,0.14371609687805176,0.01070546158461828
890,3314,0,3314,0.14496994018554688,0.010685415774201852
897,3342,0,3342,0.14689874649047852,0.010665656962554934
905,3374,0,3374,0.148298978805542,0.010643393985365762
912,3402,0,3402,0.1501307487487793,0.010624008284960252
919,3430,0,3430,0.15222692489624023,0.01060455927727649
926,3458,0,3458,0.15392374992370605,0.01058519666278113
933,3486,0,3486,0.15535378456115723,0.010565805599911873
940,3514,0,3514,0.15657496452331543,0.0105465054438266
947,3540,0,3540,0.15767598152160645,0.010425788303461638
954,3564,0,3564,0.15900492668151855,0.010149604012924317
961,3590,0,3590,0.1602339744567871,0.009896516371788674
969,3620,0,3620,0.1616077423095703,0.009531479781741344
976,3645,0,3645,0.16321396827697754,0.009287876072602922
983,3671,0,3671,0.16498184204101562,0.009072891497764924
990,3698,0,3698,0.16714882850646973,0.008920205477753405
997,3723,0,3723,0.16893482208251953,0.008724984472195217
1004,3748,0,3748,0.17089462280273438,0.008535198324216247
1011,3776,0,3776,0.1725597381591797,0.008447910433565369
1018,3801,0,3801,0.1739037036895752,0.00823215006695327
1026,3828,0,3828,0.17559480667114258,0.007934355456106141
1033,3851,0,3851,0.17702484130859375,0.00750399194861244
1040,3873,0,3873,0.17857098579406738,0.007045170376187258
1047,3899,0,3899,0.18017888069152832,0.006832579516124469
1054,3926,0,3926,0.18136906623840332,0.0067298775469245824
1061,3952,0,3952,0.18253779411315918,0.006603958983619041
1068,3979,0,3979,0.18372678756713867,0.006485425699952731
1075,4000,0,4000,0.18474388122558594,0.0061917177358785805
1083,4026,0,4026,0.1860957145690918,0.0057632627835811755
1090,4050,0,4050,0.18722772598266602,0.005499813256356118
1097,4072,0,4072,0.1888108253479004,0.0052073244663781194
1104,4098,0,4098,0.19040989875793457,0.0050317779481748245
1111,4123,0,4123,0.1915597915649414,0.004923659896253103
1118,4148,0,4148,0.1929619312286377,0.004790007850628172
1125,4175,0,4175,0.1942768096923828,0.004694884684504137
1132,4200,0,4200,0.19561171531677246,0.004558284467892034
1140,4231,0,4231,0.19837570190429688,0.004447783620024228
1147,4255,0,4255,0.20020675659179688,0.004337150817375206
1154,4282,0,4282,0.2024528980255127,0.004227289301657046
1161,4307,0,4307,0.20400786399841309,0.004114286058133364
1168,4332,0,4332,0.20524287223815918,0.003997462193170067
1175,4358,0,4358,0.20665597915649414,0.003893496984532258
1182,4384,0,4384,0.20812368392944336,0.003833511234926511
1189,4410,0,4410,0.20934391021728516,0.003758958667694934
1197,4440,0,4440,0.21101689338684082,0.0036636716824036113
1204,4466,0,4466,0.2127368450164795,0.003587369974763675
1211,4492,0,4492,0.21468782424926758,0.0034883975647162367
1218,4518,0,4518,0.21705174446105957,0.0034040621504421056
1225,4541,0,4541,0.21844196319580078,0.0032974007765146397
1232,4568,0,4568,0.21974802017211914,0.003234742089075144
1239,4596,0,4596,0.2209939956665039,0.0031957896232695316
1246,4623,0,4623,0.22267985343933105,0.0031410489634962056
1253,4650,0,4650,0.22417974472045898,0.0031027270893140514
1261,4682,0,4682,0.22558879852294922,0.0030609763410219346
1268,4709,0,4709,0.22695088386535645,0.003027626685939332
1275,4737,0,4737,0.22828173637390137,0.0030124081808875053
1282,4764,0,4764,0.23019075393676758,0.0029870357802965486
1289,4790,0,4790,0.23218393325805664,0.0029427594337684566
1296,4817,0,4817,0.23418593406677246,0.002907282658936465
1303,4845,0,4845,0.23625493049621582,0.0028926919923717726
1310,4871,0,4871,0.23790693283081055,0.002844309739643444
1318,4900,0,4900,0.2398838996887207,0.0027739498340588428
1325,4925,0,4925,0.24150705337524414,0.0027086940016188446
1332,4950,0,4950,0.24293184280395508,0.002653446230472659
1339,4977,0,4977,0.24410080909729004,0.0025991854590504317
1346,5002,0,5002,0.2456350326538086,0.002534904913719439
1353,5027,0,5027,0.24679088592529297,0.002432652650888027
1360,5050,0,5050,0.24828267097473145,0.002289230087906931
1367,5077,0,5077,0.25000905990600586,0.0022334445861015577
1375,5106,0,5106,0.2521829605102539,0.0021862977998710863
1382,5131,0,5131,0.25461769104003906,0.002105401575099917
1389,5153,0,5153,0.2567777633666992,0.00197749112587925
1396,5176,0,5176,0.2594449520111084,0.0018785874469849592
1403,5198,0,5198,0.2608938217163086,0.0018037544618197208
1410,5224,0,5224,0.26203274726867676,0.0017486434319929902
1417,5251,0,5251,0.26318883895874023,0.0017220326380171032
1424,5279,0,5279,0.26441478729248047,0.0017047069275176812
1432,5311,0,5311,0.26587581634521484,0.0016941982724202837
1439,5339,0,5339,0.2684779167175293,0.0016869058395555198
1446,5368,0,5368,0.2712829113006592,0.001680824582755222
1453,5396,0,5396,0.27312302589416504,0.0016754288147760802
1460,5426,0,5426,0.27443385124206543,0.001670804374503955
1467,5455,0,5455,0.275925874710083,0.001666318140714204
1474,5483,0,5483,0.27745771408081055,0.0016622105987493172
1481,5512,0,5512,0.2787818908691406,0.0016581169580335243
1489,5545,0,5545,0.28017687797546387,0.0016534828831796093
1496,5577,0,5577,0.2814478874206543,0.0016501593923515852
1503,5605,0,5605,0.2826387882232666,0.0016468676565889037
1510,5634,0,5634,0.28415465354919434,0.0016435453561212375
1517,5663,0,5663,0.28569579124450684,0.0016398868221883568
1524,5691,0,5691,0.28685879707336426,0.0016363873185165567
1531,5719,0,5719,0.28801584243774414,0.0016330509998387008
1538,5747,0,5747,0.28928184509277344,0.0016296619088803758
1546,5779,0,5779,0.29064488410949707,0.001625914193883257
1553,5807,0,5807,0.2918367385864258,0.00162267787999297
1560,5835,0,5835,0.293062686920166,0.0016195354569017272
1567,5863,0,5863,0.2942318916320801,0.0016164029870496038
1574,5891,0,5891,0.2956888675689697,0.0016132506531838316
1581,5919,0,5919,0.29702281951904297,0.001610138448489461
1588,5947,0,5947,0.2982969284057617,0.0016070464838323477
1595,5975,0,5975,0.2996389865875244,0.0016039871300266317
1602,6003,0,6003,0.30170178413391113,0.0016009433343424086
1610,6035,0,6035,0.30335092544555664,0.0015974756394640931
1617,6063,0,6063,0.30495572090148926,0.0015944472316451637
1624,6091,0,6091,0.306182861328125,0.0015914332316285707
1631,6119,0,6119,0.30767297744750977,0.0015884167477150234
1638,6147,0,6147,0.3097968101501465,0.0015854111194303956
1645,6175,0,6175,0.3115408420562744,0.0015824134003774445
1652,6203,0,6203,0.31285691261291504,0.0015794188211790859
1659,6230,0,6230,0.31401491165161133,0.0015737802203411653
1667,6258,0,6258,0.31615471839904785,0.0015357642107741312
1674,6285,0,6285,0.31862497329711914,0.0015115177426354345
1681,6313,0,6313,0.32146406173706055,0.0014998542133134514
1688,6342,0,6342,0.3228909969329834,0.0014946917338918369
1695,6373,0,6373,0.324321985244751,0.0014916019608363902
1702,6402,0,6402,0.3255348205566406,0.0014882508213108297
1709,6430,0,6430,0.32667994499206543,0.0014851037649230051
1716,6459,0,6459,0.3279087543487549,0.001482110004011273
1724,6491,0,6491,0.3293788433074951,0.0014786581568873825
1731,6519,0,6519,0.3307318687438965,0.0014760630929886575
1738,6548,0,6548,0.33199000358581543,0.0014732283116578864
1745,6576,0,6576,0.3331739902496338,0.0014703475014238294
1752,6604,0,6604,0.3343627452850342,0.0014675488744771324
1759,6633,0,6633,0.33633875846862793,0.001464978047325871
1766,6661,0,6661,0.3380467891693115,0.0014622415786642604
1773,6688,0,6688,0.33951568603515625,0.0014592016212316467
1781,6718,0,6718,0.3409006595611572,0.0014339267365587453
1788,6745,0,6745,0.34231090545654297,0.0014171027867715617
1795,6770,0,6770,0.3438568115234375,0.0013767505346596865
1802,6795,0,6795,0.3451356887817383,0.0013363975911142895
1809,6819,0,6819,0.34632396697998047,0.00129496383513475
1816,6845,0,6845,0.3474307060241699,0.0012681858423264668
1823,6867,0,6867,0.34867095947265625,0.0012039796372613747
1830,6893,0,6893,0.34996485710144043,0.0011753729653604839
1838,6927,0,6927,0.3514838218688965,0.0011635930661717986
1845,6955,0,6955,0.3526017665863037,0.0011578487685268526
1852,6982,0,6982,0.3538496494293213,0.0011472259681689155
1859,7009,0,7009,0.35504770278930664,0.0011349101848504833
1866,7037,0,7037,0.3562307357788086,0.0011230393380098473
1873,7064,0,7064,0.3573789596557617,0.0011109830310585172
1880,7090,0,7090,0.3585178852081299,0.0010864882170404555
1887,7118,0,7118,0.35976290702819824,0.0010720939654738637
1894,7147,0,7147,0.36104393005371094,0.001064327566694807
1902,7179,0,7179,0.3628249168395996,0.0010594704047239849
1909,7207,0,7207,0.3645789623260498,0.0010559738768292643
1916,7235,0,7235,0.36592888832092285,0.0010534590023657145
1923,7263,0,7263,0.36733484268188477,0.0010514694688987655
1930,7291,0,7291,0.36862683296203613,0.0010492541026368497
1937,7319,0,7319,0.36981773376464844,0.0010472134231093114
1944,7347,0,7347,0.3711516857147217,0.0010452745401414772
1951,7375,0,7375,0.3729588985443115,0.0010433302710703305
1959,7407,0,7407,0.3747696876525879,0.0010411161152015305
1966,7435,0,7435,0.376018762588501,0.0010391952945919365
1973,7463,0,7463,0.3772158622741699,0.001037314947751924
1980,7491,0,7491,0.3784768581390381,0.0010354265268574967
1987,7519,0,7519,0.3801100254058838,0.0010335230269479685
1994,7547,0,7547,0.3820059299468994,0.0010316408865887548
2001,7575,0,7575,0.3834249973297119,0.0010297556702177572
2008,7603,0,7603,0.384807825088501,0.0010278899612265926
2016,7635,0,7635,0.38619494438171387,0.0010257409655891913
2023,7663,0,7663,0.3873918056488037,0.0010238683032704828
2030,7691,0,7691,0.3885979652404785,0.0010219989933770448
2037,7719,0,7719,0.38979196548461914,0.001020133531236304
2044,7747,0,7747,0.3911867141723633,0.0010182652172315374
2051,7775,0,7775,0.3924729824066162,0.001016406555487199
2058,7803,0,7803,0.3937556743621826,0.0010145482011152784
2065,7827,0,7827,0.3951389789581299,0.0009936259350619597
2073,7855,0,7855,0.3970339298248291,0.0009604254844616037
2080,7878,0,7878,0.39837098121643066,0.000907267473594467
2087,7900,0,7900,0.3997368812561035,0.000856387055155897
2094,7922,0,7922,0.40091586112976074,0.000814006697972245
2101,7944,0,7944,0.4021627902984619,0.0007543719444341699
2108,7972,0,7972,0.4036438465118408,0.0007341672790072191
2115,7999,0,7999,0.4053828716278076,0.0007193713822706727
2122,8026,0,8026,0.40705299377441406,0.0007042062926111283
2130,8055,0,8055,0.4085879325866699,0.0006889698926294775
2137,8080,0,8080,0.40978384017944336,0.0006685491655309611
2144,8106,0,8106,0.41144585609436035,0.0006505178006798233
2151,8136,0,8136,0.41304492950439453,0.0006455137142734156
2158,8163,0,8163,0.4142918586730957,0.0006347913744943423
2165,8189,0,8189,0.4161646366119385,0.000626847833790313
2172,8214,0,8214,0.41735386848449707,0.0006072603681767592
2179,8241,0,8241,0.418820858001709,0.0005999904560247477
2186,8268,0,8268,0.4202139377593994,0.0005881345880837664
2194,8299,0,8299,0.4219329357147217,0.0005794411392145813
2201,8327,0,8327,0.4233419895172119,0.00057637693373513
2208,8352,0,8352,0.4244568347930908,0.0005667785285109741
2215,8378,0,8378,0.42558979988098145,0.0005593958393517749
2222,8405,0,8405,0.4268207550048828,0.0005503516282901374
2229,8433,0,8433,0.42801976203918457,0.0005473488244219273
2236,8463,0,8463,0.42927098274230957,0.0005454501972891038
2243,8492,0,8492,0.4304208755493164,0.0005438675321232291
2251,8524,0,8524,0.4317789077758789,0.0005422821497625454
2258,8553,0,8553,0.43320703506469727,0.0005411079402005408
2265,8581,0,8581,0.43454980850219727,0.0005398248354853959
2272,8609,0,8609,0.4357569217681885,0.0005386738612653564
2279,8638,0,8638,0.4373297691345215,0.0005375956012678048
2286,8666,0,8666,0.4391658306121826,0.0005364996392717083
2293,8694,0,8694,0.44086289405822754,0.0005354114956011809
2300,8722,0,8722,0.44210076332092285,0.0005343824818946956
2308,8754,0,8754,0.44350266456604004,0.0005332140252034864
2315,8782,0,8782,0.4446709156036377,0.000532200847741006
2322,8810,0,8810,0.4459078311920166,0.0005312057679033369
2329,8838,0,8838,0.44725704193115234,0.0005302398453906834
2336,8866,0,8866,0.44911980628967285,0.0005292417129866962
2343,8894,0,8894,0.4513988494873047,0.0005282566064484804
2350,8922,0,8922,0.45304393768310547,0.0005272890953904111
2357,8950,0,8950,0.4547266960144043,0.0005263194424776047
2365,8982,0,8982,0.4566776752471924,0.0005252150082995553
2372,9010,0,9010,0.45799875259399414,0.0005242476441753308
2379,9038,0,9038,0.4595918655395508,0.0005232876750110016
2386,9066,0,9066,0.4610919952392578,0.0005223279494047382
2393,9094,0,9094,0.4625058174133301,0.0005213705776551027
2400,9122,0,9122,0.464277982711792,0.0005204145934960146
2407,9150,0,9150,0.4658827781677246,0.0005194603849088586
2414,9177,0,9177,0.468355655670166,0.0005181644987550393
2422,9206,0,9206,0.4697227478027344,0.0005079842940060036
2429,9233,0,9233,0.4713888168334961,0.0005000755207235917
2436,9259,0,9259,0.47274279594421387,0.0004890949492841227
2443,9281,0,9281,0.4741239547729492,0.0004562870255066304
2450,9304,0,9304,0.4761619567871094,0.0004359118003569785
2457,9328,0,9328,0.47831273078918457,0.00042075064433132105
2464,9355,0,9355,0.48011064529418945,0.0004126764240972104
2471,9381,0,9381,0.4819958209991455,0.0004027773017232554
2478,9404,0,9404,0.48342275619506836,0.00039016986947391707
2486,9435,0,9435,0.4855227470397949,0.00038124010875821774
2493,9461,0,9461,0.4873499870300293,0.0003747119931505209
2500,9485,0,9485,0.4890298843383789,0.00036267960001733023
2507,9507,0,9507,0.490628719329834,0.00033748243198082427
2514,9532,0,9532,0.4926457405090332,0.0003243902013993868
2521,9558,0,9558,0.4941868782043457,0.0003169771201940842
2528,9585,0,9585,0.4963366985321045,0.00031381164970842236
2535,9612,0,9612,0.4988858699798584,0.0003090230823500148
2543,9641,0,9641,0.5015988349914551,0.0003019318740055787
2550,9665,0,9665,0.5036966800689697,0.0002916429930015906
2557,9690,0,9690,0.5056056976318359,0.0002813422660498161
2564,9718,0,9718,0.5079138278961182,0.0002778075713860866
2571,9743,0,9743,0.5104148387908936,0.0002718713513967921
2578,9769,0,9769,0.5129988193511963,0.0002651712574948109
2585,9793,0,9793,0.5154149532318115,0.0002569683760267573
2592,9820,0,9820,0.5185427665710449,0.0002516443025827958
2600,9847,0,9847,0.5210616588592529,0.00024224679464243887
2607,9872,0,9872,0.5233588218688965,0.0002360319376009114
2614,9896,0,9896,0.5258097648620605,0.00022791668273398788
2621,9918,0,9918,0.5284626483917236,0.00021429017936389273
2628,9941,0,9941,0.5304467678070068,0.00020206159163057403
2635,9969,0,9969,0.5323898792266846,0.00019963120690189812
2642,9997,0,9997,0.5343799591064453,0.0001982384945660964
2649,10024,0,10024,0.5365757942199707,0.00019611715591093663
2657,10056,0,10056,0.5386416912078857,0.00019450884112120201
2664,10085,0,10085,0.5402557849884033,0.00019368270235019326
2671,10114,0,10114,0.5424308776855469,0.00019296410401531595
2678,10142,0,10142,0.5441436767578125,0.00019232315922669568
2685,10171,0,10171,0.5464439392089844,0.00019174412703679898
2692,10199,0,10199,0.5490627288818359,0.00019117743781398174
2699,10227,0,10227,0.5514168739318848,0.00019069457996515407
2706,10255,0,10255,0.5531759262084961,0.00019018230602695375
2714,10287,0,10287,0.5557057857513428,0.00018963708692257007
2721,10315,0,10315,0.5582289695739746,0.00018917657138942985
2728,10343,0,10343,0.5609877109527588,0.00018874648405121976
2735,10371,0,10371,0.5636069774627686,0.0001883204169225313
2742,10399,0,10399,0.5663928985595703,0.00018790384364260083
2749,10427,0,10427,0.5690767765045166,0.00018749862943543105
2756,10455,0,10455,0.5714809894561768,0.00018710391692570663
2763,10483,0,10483,0.573793888092041,0.00018671010048460274
2771,10515,0,10515,0.5764298439025879,0.00018627008842162697
2778,10543,0,10543,0.5778517723083496,0.00018588896931889356
2785,10571,0,10571,0.5794088840484619,0.00018551960340144208
2792,10599,0,10599,0.5811009407043457,0.0001851471646208133
2799,10627,0,10627,0.5825338363647461,0.0001847804255051591
2806,10655,0,10655,0.584357738494873,0.00018441643816599875
2813,10683,0,10683,0.5856139659881592,0.00018405896175845705
2820,10711,0,10711,0.5878078937530518,0.00018370188331698207
2827,10739,0,10739,0.5897536277770996,0.0001833502370626352
2835,10771,0,10771,0.5912938117980957,0.00018294927036796162
2842,10799,0,10799,0.5928177833557129,0.000182603005217343
2849,10827,0,10827,0.5941369533538818,0.00018225732836301786
2856,10855,0,10855,0.5957558155059814,0.00018191453819931937
2863,10883,0,10883,0.5973818302154541,0.00018157235299819924
2870,10911,0,10911,0.5989439487457275,0.00018123329641507298
2877,10939,0,10939,0.6013138294219971,0.00018089487845586252
2884,10967,0,10967,0.6039068698883057,0.0001805585209805691
2892,10999,0,10999,0.6054718494415283,0.0001801745660789127
2899,11026,0,11026,0.6067440509796143,0.0001798794964183727
2906,11051,0,11051,0.6081557273864746,0.00017681135976585946
2913,11079,0,11079,0.6094686985015869,0.00017444764702980017
2920,11107,0,11107,0.6106669902801514,0.00017344006829722418
2927,11135,0,11135,0.611818790435791,0.00017264611110601755
2934,11164,0,11164,0.6130077838897705,0.00017171006185993636
2941,11192,0,11192,0.6142950057983398,0.00017125900370942046
2949,11224,0,11224,0.615912914276123,0.0001708199885182744
2956,11252,0,11252,0.6172828674316406,0.00017048535556014573
2963,11280,0,11280,0.6189708709716797,0.00017016742282537805
2970,11308,0,11308,0.6207079887390137,0.0001698530501255912
2977,11336,0,11336,0.6224827766418457,0.0001695442691692197
2984,11364,0,11364,0.6242799758911133,0.0001692355002148899
2991,11392,0,11392,0.6260378360748291,0.00016891689348207323
2998,11420,0,11420,0.6280937194824219,0.00016860654007381243
3006,11452,0,11452,0.6295478343963623,0.00016825445035208717
3013,11480,0,11480,0.6307449340820312,0.00016794814132744645
3020,11508,0,11508,0.6319279670715332,0.0001676411788106067
3027,11536,0,11536,0.6331539154052734,0.00016733545799375545
3034,11564,0,11564,0.6345117092132568,0.00016702964469672584
3041,11592,0,11592,0.6359498500823975,0.00016672424256803089
3048,11620,0,11620,0.6371927261352539,0.0001664188912896719
3055,11648,0,11648,0.6383228302001953,0.00016611436346756288
3063,11679,0,11679,0.6396520137786865,0.00016512972430607657
3070,11701,0,11701,0.6410818099975586,0.00016148936844683948
3077,11729,0,11729,0.6426959037780762,0.00015735661929420607
3084,11752,0,11752,0.6440057754516602,0.00014891119742292225
3091,11774,0,11774,0.6455819606781006,0.00014043130419141422
3098,11798,0,11798,0.6473557949066162,0.00013462065548703754
3105,11821,0,11821,0.6490590572357178,0.0001281664899679807
3112,11845,0,11845,0.6506826877593994,0.00012388876994976676
3119,11869,0,11869,0.6521928310394287,0.0001194498523772209
3127,11895,0,11895,0.6535069942474365,0.0001128104824414329
3134,11916,0,11916,0.6546227931976318,0.00010538029774823286
3141,11938,0,11938,0.6557607650756836,0.00010155949671190874
3148,11961,0,11961,0.6570439338684082,9.594305122677648e-05
3155,11983,0,11983,0.6586878299713135,9.001290807942457e-05
3162,12008,0,12008,0.6601107120513916,8.546601230935816e-05
3169,12036,0,12036,0.6620128154754639,8.409059526767545e-05
3176,12064,0,12064,0.663996696472168,8.354022924940024e-05
3184,12093,0,12093,0.6653728485107422,8.214369999921314e-05
3191,12119,0,12119,0.6665928363800049,7.988921595492196e-05
3198,12145,0,12145,0.6680018901824951,7.814208287175728e-05
3205,12169,0,12169,0.6697437763214111,7.561789164008616e-05
3212,12191,0,12191,0.6713988780975342,7.174396098244739e-05
3219,12219,0,12219,0.6732537746429443,7.013285354721268e-05
3226,12246,0,12246,0.674980640411377,6.904635821260319e-05
3233,12273,0,12273,0.6766757965087891,6.747227845142848e-05
3241,12304,0,12304,0.6787056922912598,6.642013111664749e-05
3248,12331,0,12331,0.6805408000946045,6.545853393914696e-05
3255,12358,0,12358,0.6819667816162109,6.43025179404081e-05
3262,12386,0,12386,0.6831557750701904,6.379206759457226e-05
3269,12413,0,12413,0.6847348213195801,6.303273419782432e-05
3276,12440,0,12440,0.686039924621582,6.241720872930543e-05
3283,12466,0,12466,0.6874668598175049,6.132568535532447e-05
3290,12492,0,12492,0.6886730194091797,6.0002512176449865e-05
3298,12524,0,12524,0.6899466514587402,5.9239892973498944e-05
3305,12551,0,12551,0.6910829544067383,5.863851008505307e-05
3312,12577,0,12577,0.6921839714050293,5.7665457771720396e-05
3319,12604,0,12604,0.6933889389038086,5.722993475914855e-05
3326,12631,0,12631,0.6946158409118652,5.6256133405077205e-05
3333,12656,0,12656,0.6957979202270508,5.473822282871096e-05
3340,12684,0,12684,0.696922779083252,5.422949886726851e-05
3347,12711,0,12711,0.6980068683624268,5.359311377301649e-05
3355,12741,0,12741,0.6992459297180176,5.3105223475638243e-05
3362,12767,0,12767,0.7003109455108643,5.2360721441644076e-05
3369,12795,0,12795,0.7017168998718262,5.140829741546763e-05
3376,12823,0,12823,0.7031219005584717,5.1052971721270924e-05
3383,12853,0,12853,0.7049739360809326,5.0827451216872574e-05
3390,12882,0,12882,0.7065739631652832,5.065000746008877e-05
3397,12910,0,12910,0.7078089714050293,5.0490436777905225e-05
3404,12939,0,12939,0.7091948986053467,5.03777889535372e-05
3411,12968,0,12968,0.7104177474975586,5.0252151843181955e-05
3419,13001,0,13001,0.7117419242858887,5.012898292190632e-05
3426,13030,0,13030,0.7128918170928955,5.0033514114045254e-05
3433,13059,0,13059,0.7140517234802246,4.9922613527473604e-05
3440,13086,0,13086,0.7151987552642822,4.9770106494482394e-05
3447,13116,0,13116,0.7164368629455566,4.9398933279993845e-05
3454,13144,0,13144,0.7177059650421143,4.90117977331486e-05
3461,13172,0,13172,0.7189266681671143,4.8523527410772705e-05
3468,13198,0,13198,0.720038890838623,4.786880092378278e-05
3476,13225,0,13225,0.7214667797088623,4.600446732735145e-05
3483,13253,0,13253,0.7226250171661377,4.543017367675816e-05
3490,13278,0,13278,0.7239139080047607,4.439963505313329e-05
3497,13305,0,13305,0.7252278327941895,4.377459145419221e-05
3504,13332,0,13332,0.7264819145202637,4.297251492329189e-05
3511,13357,0,13357,0.727820873260498,4.200703114925181e-05
3518,13383,0,13383,0.7291817665100098,4.1257249109078846e-05
3525,13410,0,13410,0.7304518222808838,4.066844899102014e-05
3533,13441,0,13441,0.7320399284362793,4.006812095027688e-05
3540,13468,0,13468,0.7333707809448242,3.95932869693593e-05
3547,13495,0,13495,0.734595775604248,3.916637430665686e-05
3554,13523,0,13523,0.7358918190002441,3.890148320549529e-05
3561,13551,0,13551,0.7371077537536621,3.8759733350660105e-05
3568,13581,0,13581,0.7382738590240479,3.8658459533970245e-05
3575,13609,0,13609,0.7393567562103271,3.8578937291494095e-05
3582,13639,0,13639,0.740664005279541,3.849062617252951e-05
3590,13671,0,13671,0.7419860363006592,3.840308548983059e-05
3597,13700,0,13700,0.7431027889251709,3.833111991495522e-05
3604,13728,0,13728,0.7441940307617188,3.824808881080018e-05
3611,13756,0,13756,0.7455449104309082,3.817333233852545e-05
3618,13784,0,13784,0.7467508316040039,3.8097068726295737e-05
3625,13812,0,13812,0.7479598522186279,3.8022662388127024e-05
3632,13840,0,13840,0.7496497631072998,3.795170195228008e-05
3639,13868,0,13868,0.7513647079467773,3.788141553354084e-05
3647,13900,0,13900,0.752835750579834,3.780008356068792e-05
3654,13928,0,13928,0.7543280124664307,3.772971411962875e-05
3661,13956,0,13956,0.7560408115386963,3.766074186818022e-05
3668,13984,0,13984,0.7577018737792969,3.759126361663088e-05
3675,14012,0,14012,0.7597799301147461,3.7522515899295374e-05
3682,14040,0,14040,0.761483907699585,3.745389048585642e-05
3689,14068,0,14068,0.7627058029174805,3.738543114756249e-05
3696,14096,0,14096,0.7638938426971436,3.7316960811443136e-05
3704,14128,0,14128,0.7654218673706055,3.723917606201423e-05
3711,14156,0,14156,0.7667698860168457,3.717115560922603e-05
3718,14184,0,14184,0.7681028842926025,3.710340172721881e-05
3725,14212,0,14212,0.7693097591400146,3.7035616925704946e-05
3732,14240,0,14240,0.7704696655273438,3.696794769155812e-05
3739,14268,0,14268,0.7716178894042969,3.69003243295966e-05
3746,14294,0,14294,0.7727198600769043,3.6645277786614185e-05
3753,14319,0,14319,0.7738139629364014,3.567541611540588e-05
3760,14341,0,14341,0.7749438285827637,3.409919844375527e-05
3768,14368,0,14368,0.7761766910552979,3.2272189488065306e-05
3775,14392,0,14392,0.777228832244873,3.1014605514178164e-05
3782,14413,0,14413,0.7782597541809082,2.8789594328077033e-05
3789,14439,0,14439,0.7794098854064941,2.7578824163837168e-05
3796,14466,0,14466,0.7805118560791016,2.711547056234602e-05
3803,14493,0,14493,0.7816119194030762,2.6768951788799676e-05
3810,14518,0,14518,0.782646894454956,2.6092229734068185e-05
3817,14543,0,14543,0.7836787700653076,2.5329711897819128e-05
3825,14573,0,14573,0.7849059104919434,2.4778708982253764e-05
3832,14599,0,14599,0.7859928607940674,2.419422149748075e-05
3839,14626,0,14626,0.7872068881988525,2.370048295428591e-05
3846,14652,0,14652,0.7884316444396973,2.3180371858751885e-05
3853,14680,0,14680,0.7896528244018555,2.303719398821126e-05
3860,14705,0,14705,0.7906920909881592,2.277872898549078e-05
3867,14732,0,14732,0.791827917098999,2.222400095891307e-05
3874,14759,0,14759,0.7928988933563232,2.191812374837019e-05
3882,14790,0,14790,0.7941339015960693,2.1549330199171835e-05
3889,14818,0,14818,0.795292854309082,2.13290897817859e-05
3896,14845,0,14845,0.7965438365936279,2.098360603221086e-05
3903,14873,0,14873,0.797893762588501,2.0853198442615674e-05
3910,14901,0,14901,0.7990448474884033,2.0783208967586173e-05
3917,14929,0,14929,0.8009688854217529,2.0734951925953185e-05
3924,14958,0,14958,0.8022010326385498,2.06867949723269e-05
3931,14986,0,14986,0.8034050464630127,2.0644156311012498e-05
3939,15018,0,15018,0.8047847747802734,2.0594896541968682e-05
3946,15046,0,15046,0.8060238361358643,2.055359158284702e-05
3953,15074,0,15074,0.8073348999023438,2.0514031834196748e-05
3960,15102,0,15102,0.8085267543792725,2.0475297574596366e-05
3967,15130,0,15130,0.8097789287567139,2.0436224050314375e-05
3974,15158,0,15158,0.8111019134521484,2.0397525506742984e-05
3981,15186,0,15186,0.8122909069061279,2.0360207425939565e-05
3988,15214,0,15214,0.8134667873382568,2.032241749640335e-05
3996,15246,0,15246,0.8147628307342529,2.0279662840635823e-05
4003,15274,0,15274,0.8161377906799316,2.0242088127217777e-05
4010,15302,0,15302,0.8174138069152832,2.020482655791986e-05
4017,15330,0,15330,0.818558931350708,2.0167845245744533e-05
4024,15358,0,15358,0.8198409080505371,2.0130747896323958e-05
4031,15386,0,15386,0.8210239410400391,2.009371815200797e-05
4038,15414,0,15414,0.8227477073669434,2.005666672463187e-05
4045,15442,0,15442,0.8241188526153564,2.0019837134613616e-05
4052,15470,0,15470,0.8261017799377441,1.9982869513783582e-05
4060,15502,0,15502,0.8286440372467041,1.9940817700974506e-05
4067,15528,0,15528,0.829871654510498,1.968883182797778e-05
4074,15554,0,15554,0.8309957981109619,1.937331151049915e-05
4081,15581,0,15581,0.8320879936218262,1.9026948529823784e-05
4088,15605,0,15605,0.8331167697906494,1.8335324989881682e-05
4095,15628,0,15628,0.8341388702392578,1.7732727080401893e-05
4102,15655,0,15655,0.8353090286254883,1.7379632803232314e-05
4109,15681,0,15681,0.8363769054412842,1.703773602480818e-05
4117,15712,0,15712,0.8376197814941406,1.6748437951375675e-05
4124,15739,0,15739,0.8387236595153809,1.6572234422836516e-05
4131,15764,0,15764,0.8398258686065674,1.617956922530982e-05
4138,15788,0,15788,0.8409299850463867,1.5712067890001354e-05
4145,15812,0,15812,0.8422188758850098,1.5107844363421414e-05
4152,15835,0,15835,0.8435108661651611,1.4347063082162085e-05
4159,15857,0,15857,0.8445370197296143,1.3429196931259343e-05
4166,15885,0,15885,0.8458700180053711,1.3226699307018858e-05
4174,15917,0,15917,0.8472256660461426,1.2996129249688421e-05
4181,15947,0,15947,0.8483848571777344,1.2916073864672269e-05
4188,15971,0,15971,0.8494219779968262,1.2555500260257313e-05
4195,15996,0,15996,0.8504917621612549,1.211402215564771e-05
4202,16023,0,16023,0.8515896797180176,1.1919164221954576e-05
4209,16049,0,16049,0.8526918888092041,1.1755063059585746e-05
4216,16074,0,16074,0.8538496494293213,1.143351713243476e-05
4223,16102,0,16102,0.8551087379455566,1.1318219179276868e-05
4231,16129,0,16129,0.8564510345458984,1.0930552342392866e-05
4238,16155,0,16155,0.8576338291168213,1.0627902109930844e-05
4245,16179,0,16179,0.858773946762085,1.0335962740304041e-05
4252,16208,0,16208,0.8599469661712646,1.0109208958543549e-05
4259,16234,0,16234,0.86106276512146,9.920692013910312e-06
4266,16262,0,16262,0.8622777462005615,9.85864847775089e-06
4273,16289,0,16289,0.8634107112884521,9.748441300227755e-06
4280,16313,0,16313,0.8645238876342773,9.5368731122376e-06
4288,16343,0,16343,0.8658490180969238,9.293130897888493e-06
4295,16370,0,16370,0.8671379089355469,9.141468173921254e-06
4302,16397,0,16397,0.8684170246124268,9.088756861554277e-06
4309,16424,0,16424,0.8697116374969482,8.97745176981838e-06
4316,16453,0,16453,0.8711237907409668,8.899700667259383e-06
4323,16481,0,16481,0.8724088668823242,8.826530334549867e-06
4330,16508,0,16508,0.8736827373504639,8.736459307087919e-06
4337,16536,0,16536,0.8750009536743164,8.679606927263661e-06
4344,16565,0,16565,0.8761677742004395,8.647951947563968e-06
4352,16598,0,16598,0.8774948120117188,8.623820759809921e-06
4359,16626,0,16626,0.8786239624023438,8.604455704793656e-06
4366,16654,0,16654,0.8797729015350342,8.585886173544612e-06
4373,16682,0,16682,0.8809168338775635,8.567872339480658e-06
4380,16710,0,16710,0.882009744644165,8.5506666213363e-06
4387,16736,0,16736,0.8830587863922119,8.454646565681268e-06
4394,16765,0,16765,0.8841938972473145,8.403403735870667e-06
4401,16793,0,16793,0.8852987289428711,8.375151568356282e-06
4409,16822,0,16822,0.886483907699585,8.237904935696999e-06
4416,16849,0,16849,0.8875529766082764,8.125384577675353e-06
4423,16877,0,16877,0.8886809349060059,8.066818201069684e-06
4430,16904,0,16904,0.8898088932037354,7.98293583830649e-06
4437,16933,0,16933,0.8909597396850586,7.950697524327242e-06
4444,16962,0,16962,0.8920729160308838,7.930865143676378e-06
4451,16990,0,16990,0.8931708335876465,7.912779983280635e-06
4458,17018,0,17018,0.8942608833312988,7.897194740828278e-06
4466,17052,0,17052,0.89556884765625,7.881135983774613e-06
4473,17079,0,17079,0.8966598510742188,7.833155645469218e-06
4480,17105,0,17105,0.8977179527282715,7.711330001397188e-06
4487,17132,0,17132,0.8987917900085449,7.631491509694346e-06
4494,17158,0,17158,0.899965763092041,7.4812922036708895e-06
4501,17186,0,17186,0.9011218547821045,7.444719897514147e-06
4508,17212,0,17212,0.9022047519683838,7.363263194517682e-06
4515,17238,0,17238,0.903282880783081,7.2109003415544e-06
4523,17268,0,17268,0.9044897556304932,7.00094737421988e-06
4530,17293,0,17293,0.9055328369140625,6.786117364686484e-06
4537,17319,0,17319,0.9065768718719482,6.649227633860014e-06
4544,17345,0,17345,0.9076416492462158,6.52133082443982e-06
4551,17374,0,17374,0.9087507724761963,6.4492834948843345e-06
4558,17403,0,17403,0.909949779510498,6.412369438113758e-06
4565,17431,0,17431,0.9111688137054443,6.360861737096741e-06
4572,17456,0,17456,0.9122307300567627,6.239467866819655e-06
4580,17487,0,17487,0.9135339260101318,6.117432828317573e-06
4587,17514,0,17514,0.9146387577056885,6.052148074979043e-06
4594,17542,0,17542,0.9157419204711914,6.015432017695119e-06
4601,17570,0,17570,0.9173128604888916,5.993270405763718e-06
4608,17598,0,17598,0.918449878692627,5.975906904087513e-06
4615,17627,0,17627,0.9197030067443848,5.962974515879388e-06
4622,17655,0,17655,0.9208476543426514,5.947879491740868e-06
4629,17683,0,17683,0.9219996929168701,5.9347412346461154e-06
4637,17715,0,17715,0.9232947826385498,5.894230359413664e-06
4644,17743,0,17743,0.9244039058685303,5.865563049512942e-06
4651,17771,0,17771,0.9255058765411377,5.850235051276248e-06
4658,17797,0,17797,0.9265639781951904,5.776045004267489e-06
4665,17824,0,17824,0.9277377128601074,5.705417781512533e-06
4672,17850,0,17850,0.9288387298583984,5.6132675329743594e-06
4679,17875,0,17875,0.9298858642578125,5.5133260977171535e-06
4686,17901,0,17901,0.9310269355773926,5.424377785631242e-06
4693,17927,0,17927,0.932110071182251,5.306975639160921e-06
4701,17958,0,17958,0.9333889484405518,5.234186642550911e-06
4708,17982,0,17982,0.9344549179077148,5.1253459750734575e-06
4715,18011,0,18011,0.9356117248535156,5.054762060569852e-06
4722,18039,0,18039,0.9368939399719238,5.024106062638304e-06
4729,18064,0,18064,0.9379758834838867,4.922271450422502e-06
4736,18092,0,18092,0.939140796661377,4.8421595622172034e-06
4743,18120,0,18120,0.9402799606323242,4.817441592308211e-06
4750,18146,0,18146,0.9413816928863525,4.739386745088535e-06
4758,18175,0,18175,0.9426379203796387,4.593591371959052e-06
4765,18202,0,18202,0.943922758102417,4.517480762066167e-06
4772,18227,0,18227,0.945084810256958,4.442501856255591e-06
4779,18251,0,18251,0.9461908340454102,4.269514567863426e-06
4786,18275,0,18275,0.9472978115081787,4.1576425464411565e-06
4793,18301,0,18301,0.9484028816223145,4.0628322724842086e-06
4800,18324,0,18324,0.9494309425354004,3.939598969417445e-06
4807,18350,0,18350,0.950516939163208,3.808400035921573e-06
4815,18379,0,18379,0.9518866539001465,3.6891592650294947e-06
4822,18402,0,18402,0.952908992767334,3.578051014307724e-06
4829,18426,0,18426,0.953941822052002,3.374358125032806e-06
4836,18451,0,18451,0.9550168514251709,3.256210841261218e-06
4843,18475,0,18475,0.956049919128418,3.102618103400824e-06
4850,18500,0,18500,0.9572169780731201,2.9909759011387317e-06
4857,18523,0,18523,0.9582226276397705,2.877700256671949e-06
4864,18547,0,18547,0.9592719078063965,2.7573679028558805e-06
4872,18577,0,18577,0.9605166912078857,2.702885664542084e-06
4879,18602,0,18602,0.9615528583526611,2.5977166501669936e-06
4886,18627,0,18627,0.9626078605651855,2.533794039333388e-06
4893,18656,0,18656,0.9637627601623535,2.5158206038185286e-06
4900,18682,0,18682,0.9648559093475342,2.4876524837491206e-06
4907,18706,0,18706,0.9658827781677246,2.4284676665887886e-06
4914,18733,0,18733,0.9669806957244873,2.375193813609605e-06
4921,18761,0,18761,0.9680817127227783,2.3566086371212654e-06
4929,18793,0,18793,0.9693398475646973,2.3280507025467444e-06
4936,18820,0,18820,0.97039794921875,2.3068536200540477e-06
4943,18847,0,18847,0.9714457988739014,2.2747471580720454e-06
4950,18871,0,18871,0.972491979598999,2.2007284801468767e-06
4957,18895,0,18895,0.9735748767852783,2.1258262799367606e-06
4964,18923,0,18923,0.9746899604797363,2.0973174529891647e-06
4971,18949,0,18949,0.975740909576416,2.0720471403672393e-06
4978,18975,0,18975,0.9767918586730957,2.017185519732861e-06
4985,19003,0,19003,0.9778878688812256,1.992931660899429e-06
4993,19033,0,19033,0.9790949821472168,1.949085936642089e-06
5000,19061,0,19061,0.9801967144012451,1.931064753957067e-06
5007,19086,0,19086,0.9812288284301758,1.8967965802329886e-06
5014,19114,0,19114,0.9823269844055176,1.8742815249590714e-06
5021,19142,0,19142,0.983529806137085,1.8641516630888594e-06
5028,19170,0,19170,0.9846358299255371,1.85776979610943e-06
5035,19198,0,19198,0.9857180118560791,1.8521412721419384e-06
5042,19226,0,19226,0.9868090152740479,1.8475122612015278e-06
5050,19258,0,19258,0.9880478382110596,1.8426418066558836e-06
5057,19286,0,19286,0.9891538619995117,1.8386377287714619e-06
5064,19314,0,19314,0.9902687072753906,1.834642341217786e-06
5071,19342,0,19342,0.9913437366485596,1.830833880908308e-06
5078,19370,0,19370,0.9924228191375732,1.8272093369249092e-06
5085,19398,0,19398,0.9935088157653809,1.8235740311842954e-06
5092,19426,0,19426,0.9946408271789551,1.8199878894167726e-06
5099,19454,0,19454,0.9957537651062012,1.8164538093218398e-06
5107,19486,0,19486,0.996978759765625,1.812463414923315e-06
5114,19514,0,19514,0.9980499744415283,1.80902055924182e-06
5121,19542,0,19542,0.9991178512573242,1.805566248440609e-06
5128,19570,0,19570,1.0003130435943604,1.8021341817349568e-06
5135,19598,0,19598,1.0014269351959229,1.7987337633291773e-06
5142,19626,0,19626,1.0025477409362793,1.7953352929193646e-06
5149,19654,0,19654,1.0037438869476318,1.7919531525910234e-06
5156,19682,0,19682,1.0048549175262451,1.7885861800373124e-06
5164,19714,0,19714,1.0061087608337402,1.7847416523032487e-06
5171,19738,0,19738,1.007124900817871,1.7697578544957163e-06
5178,19763,0,19763,1.0082528591156006,1.7186344097747858e-06
5185,19789,0,19789,1.0093088150024414,1.678481981608128e-06
5192,19812,0,19812,1.01031494140625,1.6204310564030227e-06
5199,19838,0,19838,1.0113739967346191,1.5882653969275065e-06
5206,19864,0,19864,1.0126678943634033,1.559843503814501e-06
5213,19892,0,19892,1.0138769149780273,1.5416640446912937e-06
5221,19923,0,19923,1.0151610374450684,1.5154893566718594e-06
5228,19949,0,19949,1.0162327289581299,1.4982131854180366e-06
5235,19976,0,19976,1.0173308849334717,1.472451237640657e-06
5242,20003,0,20003,1.0184249877929688,1.4537190065257862e-06
5249,20031,0,20031,1.0195319652557373,1.445868069439153e-06
5256,20058,0,20058,1.0206897258758545,1.4321474948515283e-06
5263,20086,0,20086,1.0218768119812012,1.425181924094748e-06
5270,20116,0,20116,1.0230367183685303,1.4209312421952117e-06
5277,20144,0,20144,1.0241899490356445,1.4174080237419364e-06
5285,20176,0,20176,1.025493860244751,1.41365693152687e-06
5292,20205,0,20205,1.0266637802124023,1.4106334563810138e-06
5299,20233,0,20233,1.0278027057647705,1.4074605291056993e-06
5306,20261,0,20261,1.0289368629455566,1.404108560386468e-06
5313,20289,0,20289,1.0300710201263428,1.401059820949211e-06
5320,20317,0,20317,1.0312068462371826,1.3979825797770744e-06
5327,20345,0,20345,1.0323357582092285,1.3950305494655155e-06
5334,20373,0,20373,1.0334959030151367,1.3920911165433214e-06
5342,20405,0,20405,1.0348389148712158,1.3888320501514812e-06
5349,20433,0,20433,1.0360028743743896,1.3859928620006938e-06
5356,20461,0,20461,1.0371577739715576,1.383186538734237e-06
5363,20489,0,20489,1.0383307933807373,1.3804088939823479e-06
5370,20517,0,20517,1.0394937992095947,1.377656396167564e-06
5377,20545,0,20545,1.0406489372253418,1.374931271866723e-06
5384,20573,0,20573,1.0418148040771484,1.3722277134224162e-06
5391,20601,0,20601,1.043001651763916,1.3695419823160564e-06
5399,20632,0,20632,1.0443530082702637,1.3581596616382485e-06
5406,20659,0,20659,1.0455007553100586,1.347166644060398e-06
5413,20688,0,20688,1.0467476844787598,1.3403837987992603e-06
5420,20714,0,20714,1.0479059219360352,1.3164725753443858e-06
5427,20740,0,20740,1.049137830734253,1.2994881547845611e-06
5434,20768,0,20768,1.0504539012908936,1.2925082459933033e-06
5441,20795,0,20795,1.0516548156738281,1.2821995949038718e-06
5448,20820,0,20820,1.0527846813201904,1.264280138896828e-06
5456,20848,0,20848,1.0539987087249756,1.2289612471161277e-06
5463,20873,0,20873,1.0550768375396729,1.1942926991668088e-06
5470,20897,0,20897,1.0561509132385254,1.160192410454563e-06
5477,20920,0,20920,1.0571787357330322,1.0984547704216998e-06
5484,20941,0,20941,1.0581817626953125,1.038086456966703e-06
5491,20967,0,20967,1.0592586994171143,9.954071647475085e-07
5498,20991,0,20991,1.0603058338165283,9.635778445681718e-07
5505,21015,0,21015,1.0613276958465576,9.210107288980169e-07
5513,21042,0,21042,1.062485933303833,8.712513165424523e-07
5520,21067,0,21067,1.0635528564453125,8.410736624959489e-07
5527,21091,0,21091,1.0645737648010254,8.216189031140384e-07
5534,21117,0,21117,1.0656607151031494,7.934125031926161e-07
5541,21141,0,21141,1.066868782043457,7.726452264423939e-07
5548,21168,0,21168,1.068070888519287,7.56750092974531e-07
5555,21195,0,21195,1.0692689418792725,7.448205965692736e-07
5562,21223,0,21223,1.0704870223999023,7.385575874058622e-07
5569,21251,0,21251,1.0716867446899414,7.32544074008361e-07
5577,21281,0,21281,1.0729467868804932,7.188907004369247e-07
5584,21309,0,21309,1.074082851409912,7.125491510814963e-07
5591,21335,0,21335,1.0752618312835693,6.997171312130624e-07
5598,21360,0,21360,1.0762968063354492,6.818423226811764e-07
5605,21385,0,21385,1.077544927597046,6.591813465214124e-07
5612,21411,0,21411,1.0786738395690918,6.432833078043371e-07
5619,21437,0,21437,1.0798640251159668,6.294756707631467e-07
5626,21464,0,21464,1.080948829650879,6.20293505374798e-07
5634,21490,0,21490,1.0821118354797363,5.975964949633523e-07
5641,21518,0,21518,1.0832419395446777,5.896208785010172e-07
5648,21545,0,21545,1.0843279361724854,5.837114681549216e-07
5655,21573,0,21573,1.085420846939087,5.799913861455536e-07
5662,21597,0,21597,1.0864698886871338,5.660091967535813e-07
5669,21623,0,21623,1.087547779083252,5.505441066204511e-07
5676,21647,0,21647,1.0885937213897705,5.349683196561116e-07
5683,21672,0,21672,1.0896167755126953,5.181209410350948e-07
5691,21702,0,21702,1.0908088684082031,5.020943059387169e-07
5698,21727,0,21727,1.0918378829956055,4.84928044850314e-07
5705,21752,0,21752,1.09287691116333,4.684481512555906e-07
5712,21781,0,21781,1.0939807891845703,4.62123671617737e-07
5719,21806,0,21806,1.095181941986084,4.539397198121354e-07
5726,21830,0,21830,1.096275806427002,4.3809130478363e-07
5733,21855,0,21855,1.0975968837738037,4.3095700173913065e-07
5740,21879,0,21879,1.0988409519195557,4.1560943580855173e-07
5748,21906,0,21906,1.1000146865844727,4.017649148212277e-07
5755,21933,0,21933,1.1011450290679932,3.954238876834197e-07
5762,21961,0,21961,1.1022958755493164,3.915168090384025e-07
5769,21988,0,21988,1.1034138202667236,3.868378148356825e-07
5776,22015,0,22015,1.1045448780059814,3.8048225437357324e-07
5783,22042,0,22042,1.105654001235962,3.76254498088536e-07
5790,22068,0,22068,1.1068389415740967,3.7020379777817243e-07
5797,22095,0,22095,1.1087048053741455,3.6700079480461726e-07
5805,22125,0,22125,1.1112098693847656,3.610367766666603e-07
5812,22152,0,22152,1.1135847568511963,3.5826574828440987e-07
5819,22180,0,22180,1.1162469387054443,3.5694138975150476e-07
5826,22207,0,22207,1.1181249618530273,3.552653039880038e-07
5833,22236,0,22236,1.1201977729797363,3.5361237877496177e-07
5840,22264,0,22264,1.1220898628234863,3.5256411104808687e-07
5847,22292,0,22292,1.1239008903503418,3.5028933492130584e-07
5854,22320,0,22320,1.1256937980651855,3.4862630076328547e-07
5862,22350,0,22350,1.1271889209747314,3.446158315205192e-07
5869,22377,0,22377,1.1286067962646484,3.41062901763455e-07
5876,22406,0,22406,1.129856824874878,3.3849990867842644e-07
5883,22433,0,22433,1.1310839653015137,3.353952880523819e-07
5890,22459,0,22459,1.1323556900024414,3.3236791272981936e-07
5897,22483,0,22483,1.1335699558258057,3.167740101663338e-07
5904,22510,0,22510,1.1348137855529785,3.119773807207617e-07
5911,22538,0,22538,1.1360077857971191,3.102611316913229e-07
5918,22566,0,22566,1.1371979713439941,3.079567343660073e-07
5926,22595,0,22595,1.1384468078613281,3.018756932111967e-07
5933,22620,0,22620,1.1395347118377686,2.972486416888085e-07
5940,22644,0,22644,1.140617847442627,2.887701786534975e-07
5947,22670,0,22670,1.1418049335479736,2.8059215847672803e-07
5954,22692,0,22692,1.1428589820861816,2.658580468820237e-07
5961,22714,0,22714,1.1439290046691895,2.5229994344404835e-07
5968,22741,0,22741,1.1452698707580566,2.4718638720619736e-07
5975,22768,0,22768,1.1470329761505127,2.4325543872321186e-07
5983,22800,0,22800,1.148484706878662,2.410557947082424e-07
5990,22826,0,22826,1.1496467590332031,2.3746809699079085e-07
5997,22851,0,22851,1.1507837772369385,2.3204470655020929e-07
6004,22879,0,22879,1.1523559093475342,2.2927561416612984e-07
6011,22905,0,22905,1.1543388366699219,2.2495627854734406e-07
6018,22927,0,22927,1.1556198596954346,2.1119130703411246e-07
6025,22949,0,22949,1.1567168235778809,1.9868545488322546e-07
6032,22976,0,22976,1.157923936843872,1.9403947988662943e-07
6040,23007,0,23007,1.1601216793060303,1.9125009072630712e-07
6047,23033,0,23033,1.1618969440460205,1.8912638099946534e-07
6054,23060,0,23060,1.1636247634887695,1.858711415401725e-07
6061,23087,0,23087,1.1648297309875488,1.8371929847093338e-07
6068,23114,0,23114,1.1664838790893555,1.8190436562136438e-07
6075,23141,0,23141,1.1683666706085205,1.7901500607988515e-07
6082,23167,0,23167,1.1700928211212158,1.7643445480375886e-07
6089,23195,0,23195,1.1722428798675537,1.7532637513568309e-07
6097,23225,0,23225,1.174069881439209,1.7185034800781566e-07
6104,23251,0,23251,1.1755356788635254,1.6791994916984303e-07
6111,23278,0,23278,1.1771557331085205,1.656211946937023e-07
6118,23306,0,23306,1.1791768074035645,1.646637883450899e-07
6125,23334,0,23334,1.180506706237793,1.6404777415764635e-07
6132,23361,0,23361,1.181931972503662,1.622420424182464e-07
6139,23389,0,23389,1.1832859516143799,1.617581200511066e-07
6146,23418,0,23418,1.1846997737884521,1.61353383412383e-07
6154,23450,0,23450,1.1863737106323242,1.6089237234744713e-07
6161,23478,0,23478,1.1876866817474365,1.6055994706685064e-07
6168,23505,0,23505,1.1889078617095947,1.5982263299209343e-07
6175,23532,0,23532,1.190220832824707,1.5783085382845765e-07
6182,23559,0,23559,1.191478967666626,1.549554374708023e-07
6189,23585,0,23585,1.1929118633270264,1.5218023377987237e-07
6196,23610,0,23610,1.194133996963501,1.4871168600776222e-07
6203,23637,0,23637,1.1957628726959229,1.4579365456126706e-07
6210,23664,0,23664,1.1977388858795166,1.4397714559393878e-07
6218,23694,0,23694,1.2001068592071533,1.4078790750154024e-07
6225,23716,0,23716,1.202272891998291,1.3406588622257367e-07
6232,23740,0,23740,1.2037708759307861,1.2840005246811214e-07
6239,23764,0,23764,1.2056238651275635,1.2320995761313044e-07
6246,23790,0,23790,1.2077267169952393,1.1969911058371017e-07
6253,23814,0,23814,1.2094767093658447,1.1631395965821431e-07
6260,23837,0,23837,1.2112739086151123,1.109475402182988e-07
6267,23861,0,23861,1.212683916091919,1.0721919750799521e-07
6275,23890,0,23890,1.2144460678100586,1.0415657986266825e-07
6282,23914,0,23914,1.2162506580352783,1.0066299232493574e-07
6289,23937,0,23937,1.2185766696929932,9.552508020751961e-08
6296,23959,0,23959,1.220780849456787,8.941861058580304e-08
6303,23983,0,23983,1.222890853881836,8.504164520361131e-08
6310,24009,0,24009,1.2251908779144287,8.268043863538359e-08
6317,24035,0,24035,1.2269058227539062,8.07681621624949e-08
6324,24059,0,24059,1.2286148071289062,7.799762074773434e-08
6332,24088,0,24088,1.2301807403564453,7.53602591464044e-08
6339,24114,0,24114,1.2315287590026855,7.329828947892965e-08
6346,24139,0,24139,1.233124017715454,7.158356696221928e-08
6353,24165,0,24165,1.2345006465911865,7.001675324756151e-08
6360,24192,0,24192,1.2357537746429443,6.886564224699489e-08
6367,24220,0,24220,1.237149953842163,6.846784033797885e-08
6374,24248,0,24248,1.2384228706359863,6.821367387740686e-08
6381,24278,0,24278,1.2396719455718994,6.804287535361769e-08
6389,24308,0,24308,1.2410669326782227,6.738594318803002e-08
6396,24333,0,24333,1.2422277927398682,6.629616971300999e-08
6403,24360,0,24360,1.24344801902771,6.530762160225094e-08
6410,24388,0,24388,1.2451567649841309,6.482625312694687e-08
6417,24415,0,24415,1.2473647594451904,6.40090698625337e-08
6424,24443,0,24443,1.2493019104003906,6.368593637519847e-08
6431,24471,0,24471,1.2513427734375,6.349123428929812e-08
6438,24500,0,24500,1.2535128593444824,6.334941290269927e-08
6446,24531,0,24531,1.2556958198547363,6.278816351042726e-08
6453,24559,0,24559,1.2571418285369873,6.255933301255271e-08
6460,24587,0,24587,1.2590408325195312,6.202181382238197e-08
6467,24613,0,24613,1.2603929042816162,6.124092096668293e-08
6474,24637,0,24637,1.261551856994629,5.953473004034816e-08
6481,24660,0,24660,1.26320481300354,5.722141716800324e-08
6488,24686,0,24686,1.2646310329437256,5.603668312077355e-08
6495,24712,0,24712,1.266737699508667,5.481798382645805e-08
6502,24738,0,24738,1.2688438892364502,5.3743544170113136e-08
6510,24767,0,24767,1.2707996368408203,5.235508685808024e-08
6517,24790,0,24790,1.2722139358520508,5.017141156987596e-08
6524,24814,0,24814,1.2733278274536133,4.7974064676849904e-08
6531,24840,0,24840,1.2744958400726318,4.679389140060203e-08
6538,24866,0,24866,1.2760980129241943,4.5665111948413035e-08
6545,24890,0,24890,1.2774949073791504,4.407700828288062e-08
6552,24914,0,24914,1.2790958881378174,4.263934528185718e-08
6559,24941,0,24941,1.280493974685669,4.15800010898813e-08
6567,24972,0,24972,1.2824387550354004,4.088466730703086e-08
6574,24998,0,24998,1.2845370769500732,3.995304547378445e-08
6581,25025,0,25025,1.2864477634429932,3.9302179548649204e-08
6588,25052,0,25052,1.2879819869995117,3.889840989338453e-08
6595,25079,0,25079,1.2891676425933838,3.8239501318146574e-08
6602,25105,0,25105,1.2904508113861084,3.7526969035147006e-08
6609,25132,0,25132,1.2917358875274658,3.719940340058367e-08
6616,25159,0,25159,1.2932348251342773,3.670006599348233e-08
6624,25186,0,25186,1.295137882232666,3.5633068247866875e-08
6631,25210,0,25210,1.297070026397705,3.415980399628645e-08
6638,25236,0,25236,1.2983908653259277,3.340261580171718e-08
6645,25262,0,25262,1.2998828887939453,3.278402444038555e-08
6652,25290,0,25290,1.3018558025360107,3.250116332658021e-08
6659,25316,0,25316,1.3031537532806396,3.195037322548931e-08
6666,25342,0,25342,1.3043358325958252,3.134957353039177e-08
6673,25369,0,25369,1.3055589199066162,3.090872546294765e-08
6681,25396,0,25396,1.3069298267364502,3.012329880449105e-08
6688,25420,0,25420,1.3089609146118164,2.890473792294e-08
6695,25446,0,25446,1.3106427192687988,2.8092278823109895e-08
6702,25473,0,25473,1.3127498626708984,2.7472754744714492e-08
6709,25499,0,25499,1.314894676208496,2.6827691378402163e-08
6716,25526,0,25526,1.3167457580566406,2.646944243258327e-08
6723,25554,0,25554,1.3187358379364014,2.633838195293228e-08
6730,25581,0,25581,1.3209667205810547,2.6061284268189556e-08
6738,25613,0,25613,1.323084831237793,2.595442436204398e-08
6745,25640,0,25640,1.324652910232544,2.5735643549487033e-08
6752,25665,0,25665,1.3264949321746826,2.5271271589189814e-08
6759,25691,0,25691,1.328622817993164,2.477755980797033e-08
6766,25718,0,25718,1.3300299644470215,2.446318627902478e-08
6773,25745,0,25745,1.3313498497009277,2.3932733841027068e-08
6780,25768,0,25768,1.3328838348388672,2.335266245651199e-08
6787,25789,0,25789,1.3343846797943115,2.2210743834025936e-08
6795,25816,0,25816,1.3361327648162842,2.0932202311687303e-08
6802,25842,0,25842,1.3378627300262451,2.040440098157445e-08
6809,25868,0,25868,1.339167833328247,2.0096140819927015e-08
6816,25892,0,25892,1.3404889106750488,1.9177135753395474e-08
6823,25915,0,25915,1.341728925704956,1.813233196163259e-08
6830,25939,0,25939,1.3431217670440674,1.7497994307691187e-08
6837,25961,0,25961,1.3446409702301025,1.6488556132170505e-08
6844,25983,0,25983,1.3460469245910645,1.5541888774750502e-08
6851,26007,0,26007,1.3472037315368652,1.5043871848760217e-08
6859,26039,0,26039,1.3487768173217773,1.4884040122489372e-08
6866,26066,0,26066,1.3504607677459717,1.4721687521431587e-08
6873,26093,0,26093,1.3520028591156006,1.4533439393935259e-08
6880,26122,0,26122,1.3532178401947021,1.4445587289163424e-08
6887,26150,0,26150,1.3543989658355713,1.437543241674673e-08
6894,26179,0,26179,1.3557937145233154,1.4323264105039165e-08
6901,26206,0,26206,1.356935739517212,1.4210069510019986e-08
6908,26234,0,26234,1.3582940101623535,1.4153244119117331e-08
6916,26265,0,26265,1.360172986984253,1.4016677987115124e-08
6923,26292,0,26292,1.3613708019256592,1.3914316263596191e-08
6930,26322,0,26322,1.3628008365631104,1.3827452385260206e-08
6937,26350,0,26350,1.364576816558838,1.3780112982257053e-08
6944,26375,0,26375,1.3661978244781494,1.3503196236270455e-08
6951,26402,0,26402,1.3681137561798096,1.3334135039533535e-08
6958,26431,0,26431,1.3701376914978027,1.3264678173552399e-08
6965,26457,0,26457,1.371931791305542,1.3079852267916881e-08
6973,26489,0,26489,1.3738007545471191,1.2922729100255456e-08
6980,26517,0,26517,1.3750598430633545,1.2850715957532644e-08
6987,26546,0,26546,1.3763267993927002,1.2739923409418842e-08
6994,26574,0,26574,1.3779399394989014,1.2685881710418764e-08
7001,26602,0,26602,1.3802008628845215,1.265182947873991e-08
7008,26631,0,26631,1.3818669319152832,1.2623969365917846e-08
7015,26659,0,26659,1.38307785987854,1.2596657139843705e-08
7022,26687,0,26687,1.3853378295898438,1.2569828558874095e-08
7030,26719,0,26719,1.3882238864898682,1.254199941796893e-08
7037,26748,0,26748,1.3908028602600098,1.2517169470982984e-08
7044,26776,0,26776,1.3927710056304932,1.249231440058803e-08
7051,26803,0,26803,1.3940048217773438,1.2397835135615102e-08
7058,26832,0,26832,1.3954269886016846,1.2352355738618232e-08
7065,26862,0,26862,1.3978769779205322,1.2322687793900526e-08
7072,26888,0,26888,1.3997266292572021,1.2116588802743922e-08
7079,26914,0,26914,1.4013350009918213,1.191157221430938e-08
7087,26942,0,26942,1.4034810066223145,1.1540681023622197e-08
7094,26966,0,26966,1.4055218696594238,1.128305730847928e-08
7101,26990,0,26990,1.4067997932434082,1.0696609958148983e-08
7108,27017,0,27017,1.4079537391662598,1.0444120161463193e-08
7115,27039,0,27039,1.4093990325927734,9.967935277830401e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00011301040649414062,4.387072431292609
1,3,0,3,0.00021696090698242188,3.9719937673698036
2,6,0,6,0.0005321502685546875,3.603279457162108
3,8,0,8,0.0007698535919189453,2.5747483139919263
4,11,0,11,0.0010509490966796875,2.3821779761310036
5,13,0,13,0.001280069351196289,1.5284154711849578
6,16,0,16,0.001558065414428711,1.4544037375349537
7,18,0,18,0.0017781257629394531,1.1578500511436216
8,21,0,21,0.0020439624786376953,1.1078200497689445
9,23,0,23,0.0022389888763427734,0.8205300174792192
10,26,0,26,0.0024662017822265625,0.7828090634793574
11,28,0,28,0.0026688575744628906,0.5904335259461263
12,31,0,31,0.0028810501098632812,0.5604305383001765
13,33,0,33,0.003165006637573242,0.4164400016335764
14,36,0,36,0.0034499168395996094,0.4029047476909755
15,38,0,38,0.0036590099334716797,0.34735376671285706
16,41,0,41,0.003976106643676758,0.33434149110626726
17,43,0,43,0.004236936569213867,0.24756978913335823
18,46,0,46,0.0045719146728515625,0.2409097710242463
19,48,0,48,0.004848957061767578,0.1834515429409959
20,51,0,51,0.0053369998931884766,0.18031175088544588
21,53,0,53,0.005614042282104492,0.15618647131006888
22,56,0,56,0.00586700439453125,0.15307297626153776
23,59,0,59,0.006173133850097656,0.15036750884012243
24,61,0,61,0.0064699649810791016,0.12920014138647526
25,64,0,64,0.006768941879272461,0.12662399358928159
26,66,0,66,0.00706791877746582,0.10695245010079718
27,69,0,69,0.00742793083190918,0.10574280743643055
28,71,0,71,0.007742166519165039,0.0809080860106374
29,74,0,74,0.008087873458862305,0.08004463590673186
30,76,0,76,0.008288145065307617,0.06452922396598361
31,79,0,79,0.008507966995239258,0.0638503852946247
32,81,0,81,0.008692026138305664,0.06168907852433439
33,84,0,84,0.008906126022338867,0.06139635380811543
34,86,0,86,0.009103059768676758,0.06127304660417731
35,89,0,89,0.00933694839477539,0.060974523646598514
36,91,0,91,0.009527206420898438,0.0608998066699066
37,94,0,94,0.009745121002197266,0.06056476298718032
38,96,0,96,0.00994110107421875,0.05917650741552297
39,99,0,99,0.010159969329833984,0.058766825732600024
40,101,0,101,0.010350942611694336,0.05644538238148135
41,104,0,104,0.010689020156860352,0.05612953844198272
42,106,0,106,0.010950088500976562,0.054612055556663756
43,109,0,109,0.01129293441772461,0.054439113489907466
44,111,0,111,0.011613130569458008,0.053131353155977314
45,114,0,114,0.011967182159423828,0.052902817062805835
46,116,0,116,0.012221097946166992,0.0500650836771471
47,119,0,119,0.012521982192993164,0.049764449500167965
48,122,0,122,0.012881040573120117,0.0495074205064623
49,124,0,124,0.013196945190429688,0.048209525062440084
50,127,0,127,0.013548851013183594,0.04795411879639343
51,129,0,129,0.013763904571533203,0.044266066724762305
52,132,0,132,0.014003992080688477,0.04370687090977983
53,134,0,134,0.014201879501342773,0.0436517968686343
54,137,0,137,0.014472007751464844,0.04310351934711104
55,139,0,139,0.014689207077026367,0.04031307861543956
56,142,0,142,0.014918088912963867,0.0397557646513919
57,144,0,144,0.015148162841796875,0.037232088003547444
58,147,0,147,0.015578031539916992,0.03681522592621644
59,149,0,149,0.0159609317779541,0.034221877814705745
60,152,0,152,0.017466068267822266,0.03372964428198596
61,154,0,154,0.017802000045776367,0.03202848740227118
62,157,0,157,0.018130064010620117,0.03150612847922555
63,159,0,159,0.018463134765625,0.031113326965804815
64,162,0,162,0.01881885528564453,0.03067794407746471
65,164,0,164,0.019154071807861328,0.02975234068019789
66,167,0,167,0.01950812339782715,0.02944773800323907
67,169,0,169,0.019789934158325195,0.027440228552082363
68,172,0,172,0.020077943801879883,0.027237737006693286
69,174,0,174,0.020300865173339844,0.026758224983282494
70,177,0,177,0.020622968673706055,0.02664691852573306
71,179,0,179,0.02085113525390625,0.026544883667046645
72,182,0,182,0.02120208740234375,0.0264653465563549
73,184,0,184,0.021479129791259766,0.026154654664001787
74,187,0,187,0.021964073181152344,0.02609952591587975
75,189,0,189,0.02230691909790039,0.025907100093064777
76,192,0,192,0.02264094352722168,0.0258586646290572
77,194,0,194,0.022938966751098633,0.025787682299508275
78,197,0,197,0.023257970809936523,0.025748718874631666
79,199,0,199,0.023553133010864258,0.025626850641597393
80,202,0,202,0.023916244506835938,0.025606022163826802
81,204,0,204,0.024219989776611328,0.02546420714535368
82,207,0,207,0.02455902099609375,0.025444108300930184
83,209,0,209,0.024882078170776367,0.025394788985711323
84,212,0,212,0.0252230167388916,0.025374433914411645
85,214,0,214,0.025504112243652344,0.02534302525643383
86,216,0,216,0.025789976119995117,0.025342498206268483
87,219,0,219,0.02617621421813965,0.025327023702289547
88,221,0,221,0.026445865631103516,0.0252956857088296
89,224,0,224,0.026803016662597656,0.025279498752621515
90,226,0,226,0.027018070220947266,0.025249211758632432
91,229,0,229,0.027247905731201172,0.0252358314099076
92,231,0,231,0.027524948120117188,0.025159974680363743
93,234,0,234,0.027781963348388672,0.025149440649797045
94,236,0,236,0.028051137924194336,0.02509783001752685
95,239,0,239,0.02822399139404297,0.025085649293457565
96,241,0,241,0.028361082077026367,0.025057795223862547
97,244,0,244,0.028522014617919922,0.025046714103002937
98,246,0,246,0.028657913208007812,0.02500596984367437
99,249,0,249,0.028815031051635742,0.02499863335724485
100,251,0,251,0.028950214385986328,0.024993959393221098
101,253,0,253,0.0290830135345459,0.024991382343046018
102,255,0,255,0.029215097427368164,0.024989854426610066
103,257,0,257,0.02935004234313965,0.024987107037376857
104,259,0,259,0.029545068740844727,0.02498364327247985
105,261,0,261,0.029733896255493164,0.024982501370369007
106,263,0,263,0.029927968978881836,0.02498137153239303
107,265,0,265,0.030153989791870117,0.024976051869763812
108,267,0,267,0.030360937118530273,0.024974937796555782
109,269,0,269,0.03060317039489746,0.02497320473077321
110,272,0,272,0.030849933624267578,0.0249615320921041
111,274,0,274,0.031045913696289062,0.024886214233830896
112,277,0,277,0.03127884864807129,0.024872036007287244
113,279,0,279,0.03146982192993164,0.02483130442153756
114,282,0,282,0.03170204162597656,0.024815547033058043
115,284,0,284,0.03189897537231445,0.02479792863186847
116,286,0,286,0.03215909004211426,0.024796866996042288
117,288,0,288,0.032404184341430664,0.024790972642931838
118,290,0,290,0.03266596794128418,0.024788740301041515
119,292,0,292,0.032878875732421875,0.024788001662920677
120,294,0,294,0.03307509422302246,0.024785850734190415
121,296,0,296,0.03326606750488281,0.024784016175308194
122,299,0,299,0.03361916542053223,0.024765925155254078
123,301,0,301,0.03394007682800293,0.024576297414966433
124,304,0,304,0.034214019775390625,0.024552995515626952
125,306,0,306,0.03445792198181152,0.024471271071650445
126,309,0,309,0.03476214408874512,0.02443408979126522
127,311,0,311,0.035127878189086914,0.024141797852023975
128,314,0,314,0.0353701114654541,0.02407880534083864
129,316,0,316,0.03552389144897461,0.02402117201753717
130,319,0,319,0.03568911552429199,0.023958535150324586
131,321,0,321,0.03582501411437988,0.023729016216612855
132,324,0,324,0.035984039306640625,0.023607182107820975
133,326,0,326,0.0361180305480957,0.0230078352557911
134,329,0,329,0.03627514839172363,0.022819945872296455
135,331,0,331,0.0364079475402832,0.022032807339049484
136,334,0,334,0.03656506538391113,0.021846831239892492
137,336,0,336,0.03670001029968262,0.021585636393457817
138,339,0,339,0.03691720962524414,0.021417468165791483
139,341,0,341,0.037079811096191406,0.02100380303764967
140,344,0,344,0.03726387023925781,0.020788884250652732
141,346,0,346,0.03740811347961426,0.0204742098725414
142,349,0,349,0.03756999969482422,0.020236094613916046
143,351,0,351,0.03770804405212402,0.019131646143650677
144,354,0,354,0.037869930267333984,0.018792637564216043
145,356,0,356,0.03800797462463379,0.017343749412532968
146,359,0,359,0.03816986083984375,0.01710527758145567
147,361,0,361,0.03830695152282715,0.01641636972280587
148,364,0,364,0.03851819038391113,0.016253488409619318
149,366,0,366,0.038671016693115234,0.01578188720826893
150,369,0,369,0.0388340950012207,0.01562648798947684
151,371,0,371,0.0390019416809082,0.015430063922102732
152,374,0,374,0.03918600082397461,0.015276090539853413
153,376,0,376,0.0393218994140625,0.01411833878954429
154,379,0,379,0.03948187828063965,0.013934999614757014
155,381,0,381,0.03961801528930664,0.013266927227990449
156,384,0,384,0.03977608680725098,0.01311509975729869
157,386,0,386,0.03992605209350586,0.012824218451721728
158,389,0,389,0.04007887840270996,0.01269524527086348
159,391,0,391,0.040209054946899414,0.012190265791544022
160,394,0,394,0.04036116600036621,0.012089135316601753
161,396,0,396,0.04049110412597656,0.011547975854943042
162,399,0,399,0.04064297676086426,0.011411486012810248
163,401,0,401,0.04077291488647461,0.011270140614958431
164,404,0,404,0.040940046310424805,0.011142639607613029
165,406,0,406,0.04106712341308594,0.010597146338311469
166,409,0,409,0.041216135025024414,0.010466316851957598
167,411,0,411,0.041342973709106445,0.010404531975239772
168,414,0,414,0.041491031646728516,0.010280276859588128
169,416,0,416,0.04161691665649414,0.009869283024349824
170,419,0,419,0.041764020919799805,0.009737523863655406
171,421,0,421,0.04189014434814453,0.008773457507487292
172,424,0,424,0.04204988479614258,0.008619009013584622
173,427,0,427,0.04219818115234375,0.008489056440499717
174,429,0,429,0.042320966720581055,0.007900929406002068
175,432,0,432,0.04246401786804199,0.007802461428474801
176,434,0,434,0.04258584976196289,0.007543900175039028
177,437,0,437,0.04272913932800293,0.007463155358667415
178,439,0,439,0.04287123680114746,0.006520011765501445
179,442,0,442,0.04301714897155762,0.006389877450190307
180,444,0,444,0.0431361198425293,0.0062900238111562225
181,447,0,447,0.04327511787414551,0.006137020680160475
182,449,0,449,0.04339599609375,0.005177381695832927
183,452,0,452,0.04354381561279297,0.0050562270361787474
184,454,0,454,0.04366302490234375,0.004876074961915767
185,457,0,457,0.04380393028259277,0.004730040800397637
186,459,0,459,0.04393815994262695,0.004055893409929831
187,462,0,462,0.04409503936767578,0.003960162362777105
188,464,0,464,0.04425311088562012,0.00370362644891699
189,467,0,467,0.04439210891723633,0.0036143987664560115
190,469,0,469,0.04450702667236328,0.0031656085684533004
191,472,0,472,0.04464292526245117,0.0031056538275489112
192,474,0,474,0.04476594924926758,0.0029918523569502234
193,477,0,477,0.0449831485748291,0.00293982405180531
194,479,0,479,0.04515480995178223,0.00253455428491232
195,482,0,482,0.04536008834838867,0.00249898374513087
196,484,0,484,0.04553103446960449,0.002474336427367068
197,487,0,487,0.04573512077331543,0.002433294677734731
198,489,0,489,0.045905113220214844,0.0022439270961719165
199,492,0,492,0.04612898826599121,0.0022050102106286186
200,494,0,494,0.046305179595947266,0.0021689956442589543
201,497,0,497,0.04651498794555664,0.002137744002808717
202,499,0,499,0.04670286178588867,0.0020116149523409497
203,502,0,502,0.04694104194641113,0.0019877599157594435
204,504,0,504,0.04714703559875488,0.0019095381678440563
205,507,0,507,0.04739999771118164,0.0018873453848715289
206,509,0,509,0.047811031341552734,0.0018091411381228862
207,512,0,512,0.048316001892089844,0.0017885529548749125
208,514,0,514,0.04868602752685547,0.0016826610162362576
209,517,0,517,0.049037933349609375,0.0016640432162830924
210,519,0,519,0.049330949783325195,0.0016483526510358301
211,522,0,522,0.04972410202026367,0.0016279030772106946
212,524,0,524,0.05001497268676758,0.0015044515973380444
213,527,0,527,0.0503849983215332,0.001479620966214013
214,529,0,529,0.05099821090698242,0.0013185673275580795
215,532,0,532,0.051319122314453125,0.0012951043338754495
216,534,0,534,0.051579952239990234,0.0012110029287347147
217,537,0,537,0.05181288719177246,0.001192705723050191
218,539,0,539,0.05206012725830078,0.0011819396165242257
219,542,0,542,0.0523679256439209,0.0011661012018266538
220,544,0,544,0.052642822265625,0.0010467948065573092
221,547,0,547,0.05294489860534668,0.0010279736887212224
222,549,0,549,0.053192138671875,0.0009909863748644178
223,551,0,551,0.05345010757446289,0.0009894920451172186
224,554,0,554,0.05374908447265625,0.000963760608805123
225,556,0,556,0.05401611328125,0.0008766083219467356
226,559,0,559,0.05431699752807617,0.0008548523255813485
227,561,0,561,0.054572105407714844,0.0007620566064714051
228,564,0,564,0.054888010025024414,0.0007534762638939558
229,566,0,566,0.05504298210144043,0.0007260146398137649
230,569,0,569,0.055322885513305664,0.0007178767840691969
231,571,0,571,0.05558300018310547,0.0006954834515069214
232,574,0,574,0.055886030197143555,0.0006910703548144164
233,576,0,576,0.05616283416748047,0.0006887804571151704
234,579,0,579,0.05649709701538086,0.0006839450899692996
235,581,0,581,0.05676698684692383,0.0006432233543448019
236,584,0,584,0.05704307556152344,0.000638511480277454
237,586,0,586,0.057244062423706055,0.00060988795707488
238,589,0,589,0.05746912956237793,0.0006069789037122359
239,591,0,591,0.05765199661254883,0.0006060963331889226
240,594,0,594,0.05786705017089844,0.0006036073978859348
241,596,0,596,0.05806398391723633,0.0005933888838318112
242,599,0,599,0.05828404426574707,0.000591552218993424
243,601,0,601,0.05846691131591797,0.0005847079034844904
244,604,0,604,0.05868196487426758,0.0005829447560491637
245,606,0,606,0.0588529109954834,0.0005802944200858546
246,609,0,609,0.059085845947265625,0.0005791446715277945
247,611,0,611,0.05928301811218262,0.0005767298080078308
248,614,0,614,0.059519052505493164,0.0005754504953198641
249,616,0,616,0.05965399742126465,0.0005657650565495023
250,619,0,619,0.05980801582336426,0.0005644642594745028
251,621,0,621,0.05994892120361328,0.0005637232417403873
252,623,0,623,0.060151100158691406,0.0005636444435034568
253,626,0,626,0.06031012535095215,0.0005622719577539522
254,628,0,628,0.06045198440551758,0.0005536826302070262
255,631,0,631,0.06066012382507324,0.0005522368748636804
256,633,0,633,0.06085991859436035,0.0005498372979590759
257,636,0,636,0.06105208396911621,0.0005484538733158137
258,638,0,638,0.06118416786193848,0.0005452853440957309
259,641,0,641,0.06142020225524902,0.0005436786765546807
260,643,0,643,0.061579227447509766,0.0005382002040336667
261,646,0,646,0.061795949935913086,0.0005364176075670393
262,648,0,648,0.06193804740905762,0.0005314111200103819
263,651,0,651,0.06213998794555664,0.0005296618789994999
264,653,0,653,0.0622859001159668,0.0005264300784876542
265,656,0,656,0.06245112419128418,0.0005249949530219674
266,658,0,658,0.0625920295715332,0.0005212800315797323
267,661,0,661,0.06274914741516113,0.0005199097073329166
268,663,0,663,0.06287908554077148,0.0005153765654150362
269,666,0,666,0.06306910514831543,0.0005140877245702443
270,668,0,668,0.06322813034057617,0.0005122886325368135
271,671,0,671,0.06342887878417969,0.000510974055471679
272,673,0,673,0.06365704536437988,0.0005049583418592644
273,676,0,676,0.0639488697052002,0.0005034300907572648
274,678,0,678,0.06416916847229004,0.0005011762572038463
275,681,0,681,0.06445097923278809,0.0004995448455843385
276,683,0,683,0.06470203399658203,0.000496974642442954
277,686,0,686,0.06499791145324707,0.0004951783280730511
278,688,0,688,0.06528592109680176,0.00047732540741248766
279,691,0,691,0.06552600860595703,0.0004741688845189487
280,693,0,693,0.06573200225830078,0.00047168767473510165
281,696,0,696,0.06596803665161133,0.00046917060715243546
282,698,0,698,0.06613302230834961,0.0004549222033980456
283,701,0,701,0.06646203994750977,0.0004528003038105315
284,703,0,703,0.06673598289489746,0.00044840015785050275
285,706,0,706,0.06704401969909668,0.0004468388757815337
286,708,0,708,0.0673379898071289,0.00044320355727656857
287,711,0,711,0.06763982772827148,0.0004419478595868406
288,713,0,713,0.06788301467895508,0.00043703816062178616
289,716,0,716,0.06819486618041992,0.00043513583534072033
290,718,0,718,0.06843996047973633,0.0004191211657486192
291,721,0,721,0.06874823570251465,0.00041740191628130416
292,723,0,723,0.06891822814941406,0.00041624704000501115
293,726,0,726,0.06907296180725098,0.0004147849113722279
294,728,0,728,0.06922602653503418,0.0004080471465126638
295,731,0,731,0.06937885284423828,0.0004063008094412667
296,733,0,733,0.06950688362121582,0.00039551102154432543
297,736,0,736,0.0696558952331543,0.00039454857697394414
298,738,0,738,0.06978321075439453,0.000391855117426603
299,741,0,741,0.0699310302734375,0.0003911133033861798
300,743,0,743,0.07005715370178223,0.00038890515782799936
301,746,0,746,0.07020401954650879,0.0003882364326896722
302,748,0,748,0.07033109664916992,0.0003868646162171148
303,751,0,751,0.07047796249389648,0.000385850007901088
304,753,0,753,0.0706479549407959,0.00038457347405757014
305,756,0,756,0.07086491584777832,0.00038360819766040786
306,758,0,758,0.07104110717773438,0.0003752177168757174
307,761,0,761,0.0711979866027832,0.0003739627569382523
308,763,0,763,0.07132911682128906,0.00036886391954423403
309,766,0,766,0.0714871883392334,0.00036808819915625033
310,768,0,768,0.07161712646484375,0.00036764825487375176
311,771,0,771,0.07176899909973145,0.0003668135060765918
312,773,0,773,0.07202315330505371,0.0003622745666131673
313,776,0,776,0.07223796844482422,0.00036168238665567216
314,778,0,778,0.07242822647094727,0.00035881562980467056
315,781,0,781,0.0725860595703125,0.0003580674288140866
316,783,0,783,0.07271695137023926,0.0003577176225254508
317,786,0,786,0.07288622856140137,0.00035693274500571854
318,788,0,788,0.07301115989685059,0.0003552139639632777
319,791,0,791,0.07315897941589355,0.000354238381361204
320,793,0,793,0.07328391075134277,0.00034993160396381835
321,796,0,796,0.07343125343322754,0.00034917813283925046
322,798,0,798,0.07361006736755371,0.00034697584763186256
323,801,0,801,0.07391023635864258,0.0003460562395217318
324,803,0,803,0.07420921325683594,0.00034419849008489556
325,806,0,806,0.07454395294189453,0.00034318064013698444
326,808,0,808,0.07482600212097168,0.00034022455386258565
327,811,0,811,0.07516813278198242,0.00033872489797023207
328,813,0,813,0.07545995712280273,0.00032774785413820475
329,816,0,816,0.07575607299804688,0.000326564993184197
330,818,0,818,0.0760490894317627,0.00031825751201886065
331,821,0,821,0.07635116577148438,0.0003162388512086076
332,823,0,823,0.07689309120178223,0.0003140544469543526
333,826,0,826,0.07730793952941895,0.0003122895961240771
334,828,0,828,0.07761287689208984,0.0003003932183434371
335,831,0,831,0.0779259204864502,0.00029848936409578557
336,833,0,833,0.07812213897705078,0.00029547095758248525
337,836,0,836,0.07836294174194336,0.0002934910281422496
338,838,0,838,0.07850313186645508,0.0002853873883397469
339,841,0,841,0.07865619659423828,0.0002827330616546176
340,843,0,843,0.07878804206848145,0.00027266295755995414
341,846,0,846,0.07894301414489746,0.0002702773418232661
342,848,0,848,0.0790719985961914,0.0002644157017310618
343,851,0,851,0.07921910285949707,0.0002618870748126798
344,853,0,853,0.0793449878692627,0.00025742842353550807
345,856,0,856,0.07948994636535645,0.0002552199947426567
346,858,0,858,0.07962703704833984,0.00024501689719540166
347,861,0,861,0.07977414131164551,0.00024378783412825144
348,863,0,863,0.07989692687988281,0.0002383733775789626
349,866,0,866,0.0800788402557373,0.0002369709340086945
350,868,0,868,0.08026885986328125,0.00023462673446606507
351,871,0,871,0.08043503761291504,0.00023338524146235832
352,873,0,873,0.0806119441986084,0.00022964927319791965
353,876,0,876,0.08083105087280273,0.00022884944313829016
354,878,0,878,0.08101201057434082,0.00022642822571360775
355,881,0,881,0.08122611045837402,0.00022552735031151403
356,883,0,883,0.08141088485717773,0.00022444287149530343
357,886,0,886,0.08163905143737793,0.00022372155730665603
358,888,0,888,0.08177804946899414,0.0002203615582223416
359,891,0,891,0.08192801475524902,0.00021956171512195434
360,893,0,893,0.08205389976501465,0.000214797150712168
361,896,0,896,0.08220195770263672,0.00021388747397525177
362,898,0,898,0.08232784271240234,0.00020972574033888296
363,901,0,901,0.08247518539428711,0.00020873954453772803
364,903,0,903,0.08272123336791992,0.00020689152777978443
365,906,0,906,0.0830390453338623,0.0002061567775991051
366,908,0,908,0.08329296112060547,0.0002039854427838234
367,911,0,911,0.08358311653137207,0.00020329976981956394
368,913,0,913,0.08381915092468262,0.00020154719915999714
369,916,0,916,0.08398294448852539,0.00020083750919142193
370,918,0,918,0.08411312103271484,0.00019926852422992255
371,921,0,921,0.08426189422607422,0.0001984406213327379
372,923,0,923,0.08438515663146973,0.00019674587767157367
373,926,0,926,0.08453106880187988,0.00019600508477326552
374,928,0,928,0.08465385437011719,0.0001937212907685551
375,931,0,931,0.08479809761047363,0.00019310243652884279
376,933,0,933,0.08493494987487793,0.00019155544776269502
377,936,0,936,0.08509182929992676,0.00019101194784878564
378,938,0,938,0.0852210521697998,0.0001899501514901634
379,941,0,941,0.08537721633911133,0.0001893441353202228
380,943,0,943,0.08550524711608887,0.00018542267788023518
381,946,0,946,0.08565521240234375,0.0001845137440818155
382,948,0,948,0.08578205108642578,0.00018271696582157336
383,951,0,951,0.08593225479125977,0.00018204047932453851
384,953,0,953,0.08609390258789062,0.00017798255186442257
385,956,0,956,0.08635306358337402,0.00017705262822411918
386,958,0,958,0.0865640640258789,0.00017625021070770828
387,961,0,961,0.08672690391540527,0.00017543503517634086
388,963,0,963,0.08686017990112305,0.0001676633514864088
389,966,0,966,0.08701205253601074,0.00016658191448072501
390,969,0,969,0.08716392517089844,0.00016565113872978697
391,971,0,971,0.08729195594787598,0.0001620685879205377
392,974,0,974,0.08744311332702637,0.00016094839994793426
393,976,0,976,0.08757400512695312,0.00015806781566014583
394,979,0,979,0.08772420883178711,0.00015654591786572989
395,981,0,981,0.08785009384155273,0.0001535684553886544
396,984,0,984,0.08801484107971191,0.00015262576961840905
397,986,0,986,0.08814024925231934,0.00014457023952426499
398,989,0,989,0.08828616142272949,0.00014365029364286412
399,991,0,991,0.0884089469909668,0.0001424809604604232
400,994,0,994,0.08855414390563965,0.00014154734228989972
401,996,0,996,0.08868217468261719,0.00013734079000176578
402,999,0,999,0.08882689476013184,0.00013660293788666245
403,1001,0,1001,0.08896398544311523,0.00013251847722251986
404,1004,0,1004,0.08910489082336426,0.00013121173697745907
405,1006,0,1006,0.08922600746154785,0.0001274625395361197
406,1009,0,1009,0.08936715126037598,0.0001261287465087035
407,1011,0,1011,0.08948683738708496,0.00012433653465412827
408,1014,0,1014,0.08962702751159668,0.00012290837675663072
409,1016,0,1016,0.08974599838256836,0.0001148769434841501
410,1019,0,1019,0.0898890495300293,0.00011339350208295875
411,1021,0,1021,0.09000802040100098,0.00010453702448192062
412,1024,0,1024,0.0901479721069336,0.00010297552415078646
413,1026,0,1026,0.09026694297790527,9.042052313465832e-05
414,1029,0,1029,0.09040713310241699,8.879494750226464e-05
415,1032,0,1032,0.0905461311340332,8.736981415042966e-05
416,1034,0,1034,0.09066414833068848,8.269933951465789e-05
417,1037,0,1037,0.0908050537109375,8.111841789272786e-05
418,1039,0,1039,0.09093999862670898,7.621500314492363e-05
419,1042,0,1042,0.09108495712280273,7.49983198493641e-05
420,1044,0,1044,0.09120607376098633,6.588195282040015e-05
421,1047,0,1047,0.09135007858276367,6.523744276065e-05
422,1049,0,1049,0.09147310256958008,6.387867014976528e-05
423,1052,0,1052,0.09161806106567383,6.326461724445657e-05
424,1054,0,1054,0.09173989295959473,6.12177507910992e-05
425,1057,0,1057,0.09188604354858398,6.0734805784862444e-05
426,1059,0,1059,0.09202790260314941,5.4822123148567635e-05
427,1062,0,1062,0.09217691421508789,5.404710506813866e-05
428,1064,0,1064,0.09230399131774902,5.3577745908468054e-05
429,1067,0,1067,0.0924530029296875,5.270157320775314e-05
430,1069,0,1069,0.09257984161376953,4.95068549538471e-05
431,1072,0,1072,0.0927278995513916,4.857943124786631e-05
432,1074,0,1074,0.09287905693054199,4.5446559188426654e-05
433,1077,0,1077,0.09303617477416992,4.440169568636559e-05
434,1079,0,1079,0.09316420555114746,4.1138378842994205e-05
435,1082,0,1082,0.09331321716308594,4.038369170932972e-05
436,1084,0,1084,0.09344005584716797,3.701231335414682e-05
437,1087,0,1087,0.09358811378479004,3.614516447703074e-05
438,1089,0,1089,0.09371495246887207,3.5092948495037376e-05
439,1092,0,1092,0.09386396408081055,3.446530827810914e-05
440,1094,0,1094,0.09400510787963867,2.9389689929199545e-05
441,1097,0,1097,0.09428215026855469,2.883554220258123e-05
442,1099,0,1099,0.09456801414489746,2.8110294710354895e-05
443,1102,0,1102,0.09488105773925781,2.773161643650222e-05
444,1104,0,1104,0.09515500068664551,2.641212506688725e-05
445,1107,0,1107,0.09545302391052246,2.605084142077559e-05
446,1109,0,1109,0.09575414657592773,2.377743078472058e-05
447,1112,0,1112,0.09612917900085449,2.3446995114178253e-05
448,1114,0,1114,0.09644603729248047,2.2920342346875814e-05
449,1117,0,1117,0.09676408767700195,2.2590318398964677e-05
450,1119,0,1119,0.09703397750854492,2.070021924232252e-05
451,1122,0,1122,0.09734797477722168,2.0428716340895525e-05
452,1124,0,1124,0.09761905670166016,1.9316264121496507e-05
453,1127,0,1127,0.09885025024414062,1.9029111624083498e-05
454,1129,0,1129,0.09943103790283203,1.9018867173368354e-05
455,1132,0,1132,0.09986495971679688,1.8704396366345255e-05
456,1134,0,1134,0.10019993782043457,1.7096168261401418e-05
457,1137,0,1137,0.1005258560180664,1.6759791572329233e-05
458,1139,0,1139,0.10078191757202148,1.5049209183100374e-05
459,1142,0,1142,0.10109305381774902,1.4772200274937666e-05
460,1144,0,1144,0.10136198997497559,1.456655607378357e-05
461,1147,0,1147,0.10166406631469727,1.4320559516835536e-05
462,1149,0,1149,0.1019432544708252,1.4115192759272597e-05
463,1152,0,1152,0.10221290588378906,1.3895370849042113e-05
464,1154,0,1154,0.1024179458618164,1.160799908244687e-05
465,1157,0,1157,0.10264396667480469,1.1496695736729792e-05
466,1159,0,1159,0.10284090042114258,1.1417086832705952e-05
467,1162,0,1162,0.1030721664428711,1.1313605704082058e-05
468,1164,0,1164,0.10326313972473145,1.0963240435929785e-05
469,1167,0,1167,0.10349392890930176,1.0872777266937686e-05
470,1170,0,1170,0.10372495651245117,1.079291627294913e-05
471,1172,0,1172,0.10391783714294434,1.029273284421237e-05
472,1175,0,1175,0.10416293144226074,1.0197901512737987e-05
473,1177,0,1177,0.10442996025085449,9.637221858779567e-06
474,1180,0,1180,0.10466599464416504,9.559990636186515e-06
475,1182,0,1182,0.10482120513916016,9.465201064285316e-06
476,1185,0,1185,0.10499215126037598,9.390973031617546e-06
477,1187,0,1187,0.10513806343078613,9.21562510664092e-06
478,1190,0,1190,0.10537409782409668,9.140117346309221e-06
479,1192,0,1192,0.10560178756713867,8.503614302801095e-06
480,1195,0,1195,0.10583686828613281,8.435232972985004e-06
481,1197,0,1197,0.10598111152648926,8.417681801520858e-06
482,1200,0,1200,0.10614681243896484,8.353050215316486e-06
483,1202,0,1202,0.10628414154052734,8.035298199946566e-06
484,1205,0,1205,0.10644412040710449,7.981391467865321e-06
485,1207,0,1207,0.10658907890319824,7.804991701963421e-06
486,1210,0,1210,0.10683703422546387,7.76132874322662e-06
487,1212,0,1212,0.10706591606140137,7.679766771126224e-06
488,1215,0,1215,0.10734796524047852,7.642421676006113e-06
489,1217,0,1217,0.10755109786987305,7.5296603209471354e-06
490,1220,0,1220,0.10777401924133301,7.480657245427223e-06
491,1222,0,1222,0.10795903205871582,7.429750801504634e-06
492,1225,0,1225,0.10817694664001465,7.372231825980338e-06
493,1227,0,1227,0.10835909843444824,7.183200304721797e-06
494,1230,0,1230,0.10857605934143066,7.124343369316845e-06
495,1232,0,1232,0.10876297950744629,6.828475285953329e-06
496,1235,0,1235,0.10900211334228516,6.786209276682111e-06
497,1237,0,1237,0.10918903350830078,6.508089059784384e-06
498,1240,0,1240,0.10940909385681152,6.470104958209587e-06
499,1242,0,1242,0.10959601402282715,6.459220489141117e-06
500,1245,0,1245,0.10980892181396484,6.415088915301154e-06
501,1247,0,1247,0.10996007919311523,5.767499942250243e-06
502,1250,0,1250,0.11011600494384766,5.681995012666865e-06
503,1252,0,1252,0.11024713516235352,5.635283923824104e-06
504,1255,0,1255,0.11040806770324707,5.555960637609182e-06
505,1257,0,1257,0.11059117317199707,5.206801194649771e-06
506,1260,0,1260,0.11075806617736816,5.140742031582461e-06
507,1262,0,1262,0.11089015007019043,4.824835402991116e-06
508,1265,0,1265,0.11104393005371094,4.781188183116045e-06
509,1267,0,1267,0.1111750602722168,4.67930979866105e-06
510,1270,0,1270,0.1113271713256836,4.610407347000589e-06
511,1272,0,1272,0.11146306991577148,4.413448481895368e-06
512,1275,0,1275,0.11165595054626465,4.363245006110899e-06
513,1277,0,1277,0.11184406280517578,4.287457277833019e-06
514,1280,0,1280,0.11207008361816406,4.2480817631348104e-06
515,1282,0,1282,0.1122739315032959,4.156048970321303e-06
516,1285,0,1285,0.11252689361572266,4.110732154228557e-06
517,1287,0,1287,0.11275601387023926,3.968329041685237e-06
518,1290,0,1290,0.11301112174987793,3.936688471539518e-06
519,1292,0,1292,0.11321091651916504,3.831653968580201e-06
520,1295,0,1295,0.11351418495178223,3.794550412686309e-06
521,1297,0,1297,0.11383605003356934,3.6495593903191764e-06
522,1300,0,1300,0.11415505409240723,3.627477177922878e-06
523,1302,0,1302,0.11445212364196777,3.3807763075003555e-06
524,1305,0,1305,0.11479306221008301,3.354252522571791e-06
525,1307,0,1307,0.1150522232055664,3.3183363526408734e-06
526,1310,0,1310,0.11547493934631348,3.29156462492025e-06
527,1312,0,1312,0.11574196815490723,3.277771222987111e-06
528,1315,0,1315,0.11606788635253906,3.2521717227725894e-06
529,1317,0,1317,0.11647391319274902,3.043226963928818e-06
530,1320,0,1320,0.11796402931213379,3.015860700304135e-06
531,1322,0,1322,0.11834597587585449,2.8991929378810733e-06
532,1325,0,1325,0.11868715286254883,2.8596894418134744e-06
533,1327,0,1327,0.11905598640441895,2.8389204217676324e-06
534,1329,0,1329,0.1193540096282959,2.8375612737680786e-06
535,1332,0,1332,0.11968302726745605,2.799612838986582e-06
536,1334,0,1334,0.11995291709899902,2.538971883339705e-06
537,1337,0,1337,0.12026500701904297,2.4755810613254833e-06
538,1339,0,1339,0.1205589771270752,2.3912625979395218e-06
539,1342,0,1342,0.12089204788208008,2.3294491419911636e-06
540,1344,0,1344,0.1211690902709961,2.0215008336655964e-06
541,1347,0,1347,0.1215050220489502,1.997293412105047e-06
542,1349,0,1349,0.12174797058105469,1.919395253296541e-06
543,1352,0,1352,0.12201714515686035,1.8944443923802444e-06
544,1354,0,1354,0.12224006652832031,1.8485568607462421e-06
545,1357,0,1357,0.12250709533691406,1.818122094654074e-06
546,1359,0,1359,0.1227719783782959,1.5861860129572106e-06
547,1362,0,1362,0.12312507629394531,1.574057604718784e-06
548,1365,0,1365,0.12337017059326172,1.5631790810234462e-06
549,1367,0,1367,0.12356686592102051,1.518779600421288e-06
550,1370,0,1370,0.12379288673400879,1.5064133017711964e-06
551,1372,0,1372,0.12398505210876465,1.4934332861540848e-06
552,1375,0,1375,0.12421798706054688,1.4820238554273696e-06
553,1377,0,1377,0.12450003623962402,1.4054410000757548e-06
554,1380,0,1380,0.12482595443725586,1.3940175648318174e-06
555,1382,0,1382,0.12511301040649414,1.3344403143190267e-06
556,1385,0,1385,0.12549591064453125,1.3239326677329289e-06
557,1387,0,1387,0.1257610321044922,1.3205765499182668e-06
558,1390,0,1390,0.12608599662780762,1.3104033421434842e-06
559,1392,0,1392,0.12635087966918945,1.2261881577905354e-06
560,1395,0,1395,0.12664103507995605,1.2170471925184867e-06
561,1397,0,1397,0.12691116333007812,1.2055198843934083e-06
562,1400,0,1400,0.12721896171569824,1.1968708085093869e-06
563,1402,0,1402,0.1274890899658203,1.1759807307705794e-06
564,1405,0,1405,0.12774896621704102,1.1682296073955922e-06
565,1407,0,1407,0.1279439926147461,1.142968068497633e-06
566,1410,0,1410,0.1281900405883789,1.134084976349064e-06
567,1412,0,1412,0.12833499908447266,1.113814547606519e-06
568,1415,0,1415,0.12849688529968262,1.1079983878346925e-06
569,1417,0,1417,0.12867999076843262,1.079425120811968e-06
570,1420,0,1420,0.12894511222839355,1.0695001854125733e-06
571,1422,0,1422,0.12914204597473145,1.0547633350804992e-06
572,1425,0,1425,0.12936902046203613,1.045630769097356e-06
573,1427,0,1427,0.12955904006958008,1.002162123678714e-06
574,1430,0,1430,0.12977910041809082,9.86994147713235e-07
575,1432,0,1432,0.12996220588684082,9.548009605795478e-07
576,1435,0,1435,0.13019084930419922,9.417723642120751e-07
577,1437,0,1437,0.13032793998718262,7.929523325148092e-07
578,1440,0,1440,0.1305990219116211,7.805102026430853e-07
579,1442,0,1442,0.13085007667541504,7.523986388088494e-07
580,1445,0,1445,0.13114094734191895,7.426206263239531e-07
581,1447,0,1447,0.13138914108276367,7.212471399646794e-07
582,1450,0,1450,0.13168001174926758,7.118033594079328e-07
583,1452,0,1452,0.1319279670715332,6.663906440594595e-07
584,1455,0,1455,0.13217592239379883,6.590556323428829e-07
585,1457,0,1457,0.1323850154876709,5.879794323312678e-07
586,1460,0,1460,0.1326150894165039,5.818111516082263e-07
587,1462,0,1462,0.13286113739013672,5.600508566840352e-07
588,1465,0,1465,0.13313603401184082,5.534660575162157e-07
589,1467,0,1467,0.13338398933410645,5.274412266557018e-07
590,1470,0,1470,0.13365507125854492,5.213578840699602e-07
591,1472,0,1472,0.13388991355895996,5.002927105787785e-07
592,1475,0,1475,0.13413310050964355,4.936327004151889e-07
593,1477,0,1477,0.13434505462646484,4.636050421784175e-07
594,1480,0,1480,0.1345810890197754,4.5615801684290073e-07
595,1482,0,1482,0.1347339153289795,4.060611282187766e-07
596,1485,0,1485,0.13490009307861328,3.997113411615038e-07
597,1487,0,1487,0.1350400447845459,3.921967592975495e-07
598,1490,0,1490,0.13520002365112305,3.8797843786212184e-07
599,1492,0,1492,0.13533306121826172,3.6208188220557375e-07
600,1495,0,1495,0.13548994064331055,3.5583921202712114e-07
601,1497,0,1497,0.13562393188476562,3.4225385869734613e-07
602,1500,0,1500,0.13577985763549805,3.371550080198476e-07
603,1502,0,1502,0.1359109878540039,3.0683429785830947e-07
604,1505,0,1505,0.13608002662658691,3.019894599182677e-07
605,1507,0,1507,0.13620901107788086,2.972006030756682e-07
606,1510,0,1510,0.13635993003845215,2.931295680388044e-07
607,1512,0,1512,0.1364879608154297,2.745286645631176e-07
608,1515,0,1515,0.13663816452026367,2.720456668242411e-07
609,1517,0,1517,0.13676714897155762,2.6632121442757374e-07
610,1520,0,1520,0.1369180679321289,2.640228244465936e-07
611,1522,0,1522,0.13704609870910645,2.5390625064275436e-07
612,1525,0,1525,0.13719797134399414,2.5066521339504135e-07
613,1527,0,1527,0.13733506202697754,2.4418215460096256e-07
614,1530,0,1530,0.1374959945678711,2.417825789985812e-07
615,1532,0,1532,0.13762903213500977,2.3124824298157101e-07
616,1535,0,1535,0.13778209686279297,2.2873201891937197e-07
617,1537,0,1537,0.1379101276397705,2.225303377192742e-07
618,1540,0,1540,0.1380608081817627,2.2034925302485412e-07
619,1542,0,1542,0.13818812370300293,2.1568330879013655e-07
620,1545,0,1545,0.13833880424499512,2.1390081920446974e-07
621,1547,0,1547,0.13846611976623535,2.0888988511702286e-07
622,1550,0,1550,0.13861703872680664,2.074213914356843e-07
623,1552,0,1552,0.13874483108520508,2.0297579736125035e-07
624,1555,0,1555,0.13889503479003906,2.020683122994079e-07
625,1557,0,1557,0.13902711868286133,1.9786989514855383e-07
626,1560,0,1560,0.13917803764343262,1.9695437523368433e-07
627,1562,0,1562,0.13930416107177734,1.9609296658452972e-07
628,1565,0,1565,0.13945412635803223,1.9532811112028172e-07
629,1567,0,1567,0.13958311080932617,1.9245937882262533e-07
630,1570,0,1570,0.13973307609558105,1.9152312278692564e-07
631,1572,0,1572,0.1398611068725586,1.8693708285751703e-07
632,1575,0,1575,0.14001202583312988,1.8609342969893066e-07
633,1577,0,1577,0.14013910293579102,1.8462924022719573e-07
634,1580,0,1580,0.14029192924499512,1.8399502273011834e-07
635,1582,0,1582,0.14042401313781738,1.810051451007273e-07
636,1585,0,1585,0.14057612419128418,1.805551456815927e-07
637,1587,0,1587,0.14070510864257812,1.7848935796068045e-07
638,1590,0,1590,0.14085698127746582,1.7806257385343602e-07
639,1592,0,1592,0.1410069465637207,1.779045805049451e-07
640,1594,0,1594,0.14113211631774902,1.778841498025305e-07
641,1596,0,1596,0.14125609397888184,1.7785738828132427e-07
642,1598,0,1598,0.14137983322143555,1.7778751327187154e-07
643,1601,0,1601,0.1415271759033203,1.7739526092763882e-07
644,1603,0,1603,0.14165210723876953,1.7541512452397732e-07
645,1606,0,1606,0.1417999267578125,1.7494261846388963e-07
646,1608,0,1608,0.14192605018615723,1.7312028831124264e-07
647,1611,0,1611,0.1420738697052002,1.7267829134144452e-07
648,1613,0,1613,0.14219903945922852,1.7071489925737407e-07
649,1616,0,1616,0.14234614372253418,1.7021199473275144e-07
650,1618,0,1618,0.1424710750579834,1.6952905711706792e-07
651,1621,0,1621,0.14261794090270996,1.6898155777049971e-07
652,1623,0,1623,0.14274382591247559,1.6519093571587216e-07
653,1626,0,1626,0.14289212226867676,1.6446711154739032e-07
654,1628,0,1628,0.14302921295166016,1.629168540716764e-07
655,1631,0,1631,0.1431729793548584,1.623476926566118e-07
656,1633,0,1633,0.14330005645751953,1.5860447264358823e-07
657,1636,0,1636,0.14344501495361328,1.5781965691525834e-07
658,1638,0,1638,0.14356684684753418,1.5763528758764685e-07
659,1641,0,1641,0.14371013641357422,1.5686448446192974e-07
660,1643,0,1643,0.14388203620910645,1.5389101052167321e-07
661,1646,0,1646,0.14409613609313965,1.5322857369035548e-07
662,1648,0,1648,0.14441609382629395,1.4917743993167482e-07
663,1651,0,1651,0.1447429656982422,1.480633810221551e-07
664,1653,0,1653,0.1450340747833252,1.450870946687687e-07
665,1656,0,1656,0.14533114433288574,1.438412036264245e-07
666,1658,0,1658,0.14557814598083496,1.371928595968352e-07
667,1661,0,1661,0.1458578109741211,1.3606774701815825e-07
668,1663,0,1663,0.14601898193359375,1.3224089320882868e-07
669,1666,0,1666,0.14618206024169922,1.3083748476638483e-07
670,1668,0,1668,0.14631891250610352,1.2178859103339335e-07
671,1671,0,1671,0.14648008346557617,1.200583185346017e-07
672,1673,0,1673,0.14661407470703125,1.1757269514759812e-07
673,1676,0,1676,0.14695501327514648,1.1611421473344387e-07
674,1678,0,1678,0.1472148895263672,1.0697777275327487e-07
675,1681,0,1681,0.14753389358520508,1.055549108150818e-07
676,1683,0,1683,0.147841215133667,9.895056359911035e-08
677,1686,0,1686,0.1482090950012207,9.78323285715369e-08
678,1688,0,1688,0.14851808547973633,9.070577311702179e-08
679,1691,0,1691,0.14884591102600098,8.956292867969454e-08
680,1694,0,1694,0.1490941047668457,8.855126020824265e-08
681,1696,0,1696,0.14932012557983398,8.13626194785863e-08
682,1699,0,1699,0.1495802402496338,8.036353328612543e-08
683,1701,0,1701,0.1497948169708252,7.842395770549923e-08
684,1704,0,1704,0.15005183219909668,7.766449583476945e-08
685,1706,0,1706,0.15035700798034668,7.343032826068544e-08
686,1709,0,1709,0.1507120132446289,7.223277240791524e-08
687,1711,0,1711,0.15101408958435059,7.024125667207271e-08
688,1714,0,1714,0.1512889862060547,6.92421971308087e-08
689,1716,0,1716,0.15144801139831543,6.612517199948632e-08
690,1719,0,1719,0.1516129970550537,6.555548805643118e-08
691,1721,0,1721,0.15182900428771973,6.458022540726504e-08
692,1724,0,1724,0.15207409858703613,6.391964464789463e-08
693,1726,0,1726,0.15227198600769043,6.195841252749546e-08
694,1729,0,1729,0.15250015258789062,6.161661500721421e-08
695,1731,0,1731,0.15269112586975098,6.065638248755814e-08
696,1734,0,1734,0.15291500091552734,6.01589551757732e-08
697,1736,0,1736,0.15311193466186523,5.931018839631262e-08
698,1739,0,1739,0.15332603454589844,5.879402461795209e-08
699,1741,0,1741,0.1535041332244873,5.581059598223322e-08
700,1744,0,1744,0.15372920036315918,5.531951502336182e-08
701,1746,0,1746,0.15392303466796875,5.1474695410801544e-08
702,1749,0,1749,0.1541600227355957,5.084749207908479e-08
703,1751,0,1751,0.15440797805786133,4.9725961539572927e-08
704,1754,0,1754,0.1546928882598877,4.91538501104908e-08
705,1756,0,1756,0.15493202209472656,4.5730537857160135e-08
706,1759,0,1759,0.15523409843444824,4.478451354884494e-08
707,1761,0,1761,0.1554851531982422,4.0364548181640597e-08
708,1764,0,1764,0.1557750701904297,3.971011499501416e-08
709,1766,0,1766,0.15604424476623535,3.91142748016048e-08
710,1769,0,1769,0.15634894371032715,3.8515271047023955e-08
711,1771,0,1771,0.15660595893859863,3.575165587399895e-08
712,1774,0,1774,0.1569061279296875,3.486318146150352e-08
713,1776,0,1776,0.15716910362243652,2.8201353353049965e-08
714,1779,0,1779,0.15745902061462402,2.7764697212636498e-08
715,1781,0,1781,0.1577160358428955,2.7683493411533322e-08
716,1784,0,1784,0.1580209732055664,2.7296384337593946e-08
717,1786,0,1786,0.15825796127319336,2.53461960306916e-08
718,1789,0,1789,0.15852594375610352,2.4958042474497495e-08
719,1791,0,1791,0.15876317024230957,2.4634747687316124e-08
720,1794,0,1794,0.15904593467712402,2.4216845200243603e-08
721,1796,0,1796,0.15928101539611816,2.1868063987713802e-08
722,1799,0,1799,0.15956592559814453,2.150883400500391e-08
723,1801,0,1801,0.159804105758667,2.1018795514225313e-08
724,1804,0,1804,0.16008520126342773,2.0685178721501665e-08
725,1806,0,1806,0.16032195091247559,1.845804243326748e-08
726,1809,0,1809,0.16060400009155273,1.8213326856711394e-08
727,1811,0,1811,0.16083908081054688,1.8207545737969353e-08
728,1814,0,1814,0.16114211082458496,1.794935438501034e-08
729,1816,0,1816,0.16138410568237305,1.58348521604455e-08
730,1819,0,1819,0.16167783737182617,1.561423707243368e-08
731,1821,0,1821,0.16193294525146484,1.500065560985156e-08
732,1824,0,1824,0.16216206550598145,1.4832965230611533e-08
733,1826,0,1826,0.16234707832336426,1.4265813342510977e-08
734,1829,0,1829,0.16256403923034668,1.4136655785552462e-08
735,1831,0,1831,0.16274499893188477,1.3346625189869403e-08
736,1834,0,1834,0.16297411918640137,1.32124393053341e-08
737,1836,0,1836,0.16315698623657227,1.2310525715577536e-08
738,1839,0,1839,0.16340303421020508,1.2194243693592743e-08
739,1841,0,1841,0.1636519432067871,1.2062657468014853e-08
740,1844,0,1844,0.16384387016296387,1.1958705197512337e-08
741,1846,0,1846,0.16401290893554688,1.1540648693760368e-08
742,1849,0,1849,0.1641700267791748,1.1468842546606532e-08
743,1851,0,1851,0.16430401802062988,1.1342357215424276e-08
744,1854,0,1854,0.16448187828063965,1.127684592619382e-08
745,1856,0,1856,0.16466498374938965,1.1194744293280172e-08
746,1859,0,1859,0.16488409042358398,1.1128406757613543e-08
747,1861,0,1861,0.1650850772857666,1.0618194858139142e-08
748,1864,0,1864,0.1655271053314209,1.0507228460887075e-08
749,1866,0,1866,0.16591501235961914,1.0225933506211761e-08
750,1869,0,1869,0.16630101203918457,1.0094031140986934e-08
751,1871,0,1871,0.1665968894958496,9.513732246910624e-09


==> extragradient/plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00010895729064941406,4.387072431292609
2,7,0,7,0.0008800029754638672,3.8559300609188223
4,13,0,13,0.0018200874328613281,3.1805127365100363
7,21,0,21,0.0031538009643554688,2.615570316233742
9,27,0,27,0.004025936126708984,2.191271192448902
11,33,0,33,0.004875898361206055,1.8826796009926408
13,38,0,38,0.00554203987121582,1.5450747111062477
16,46,0,46,0.006451845169067383,1.2951104535495437
18,52,0,52,0.007108926773071289,1.1158175670995938
20,56,0,56,0.007548093795776367,0.7431866161266337
22,62,0,62,0.008030891418457031,0.6516199660515388
24,67,0,67,0.008543968200683594,0.5649756411926242
27,75,0,75,0.009617805480957031,0.45433073002614544
29,81,0,81,0.010355949401855469,0.3871088390019215
31,86,0,86,0.011082887649536133,0.3208279775251849
33,92,0,92,0.011870861053466797,0.2902653527613473
36,101,0,101,0.013031959533691406,0.2552546357138213
38,107,0,107,0.013736963272094727,0.23687583719133645
40,113,0,113,0.014230012893676758,0.22163539267351257
42,117,0,117,0.014692068099975586,0.1676035625280366
44,122,0,122,0.015157938003540039,0.12665917028755536
47,131,0,131,0.015889883041381836,0.1140913424646257
49,137,0,137,0.016371965408325195,0.10820517019885094
51,143,0,143,0.016859054565429688,0.10340568997867958
53,149,0,149,0.017345905303955078,0.09915460262568171
56,159,0,159,0.018095016479492188,0.09569840037841193
58,165,0,165,0.018581867218017578,0.09264126979900225
60,171,0,171,0.019063949584960938,0.08976631271155329
62,177,0,177,0.019551992416381836,0.08712288757616599
64,183,0,183,0.02004098892211914,0.08495728517642527
67,192,0,192,0.02091193199157715,0.08222009826014123
69,198,0,198,0.02172684669494629,0.08060703893336357
71,204,0,204,0.02266097068786621,0.0791255073512142
73,210,0,210,0.02360701560974121,0.07777358802375395
76,219,0,219,0.024927854537963867,0.07634502043921164
78,226,0,226,0.02585291862487793,0.07567029412637268
80,232,0,232,0.026725053787231445,0.07442393602158026
82,238,0,238,0.02763986587524414,0.07304146057554366
84,246,0,246,0.028828859329223633,0.07224563163750264
87,257,0,257,0.030303955078125,0.07125871305496817
89,264,0,264,0.03130316734313965,0.07068488872528286
91,271,0,271,0.032318830490112305,0.07027851854581647
93,279,0,279,0.033255815505981445,0.06976768901557152
96,291,0,291,0.034750938415527344,0.06907298395998851
98,299,0,299,0.03579902648925781,0.06870886340154092
100,306,0,306,0.03681492805480957,0.06719063569697241
102,314,0,314,0.037834882736206055,0.06673418358244398
104,322,0,322,0.03853106498718262,0.06632372019182742
107,332,0,332,0.039407968521118164,0.06602362973826231
109,338,0,338,0.039987802505493164,0.06587926386504214
111,344,0,344,0.04060697555541992,0.06564447479065666
113,350,0,350,0.04111790657043457,0.06545043502837225
116,361,0,361,0.041944026947021484,0.0651556593911532
118,369,0,369,0.04293704032897949,0.0649114535474169
120,377,0,377,0.04395890235900879,0.06466351143612761
122,383,0,383,0.04490995407104492,0.06447667555488906
125,392,0,392,0.04616498947143555,0.064119065234829
127,398,0,398,0.046946048736572266,0.06388373459021203
129,404,0,404,0.047731876373291016,0.06366001823211934
131,410,0,410,0.04842495918273926,0.06343535829850781
133,416,0,416,0.049054861068725586,0.06319900141816029
136,425,0,425,0.04981493949890137,0.06281322227189919
138,431,0,431,0.05032491683959961,0.06252652230101145
140,437,0,437,0.050827980041503906,0.0622117477412763
142,443,0,443,0.051332950592041016,0.061872962522918185
145,452,0,452,0.05208706855773926,0.061334115737910096
147,458,0,458,0.05258989334106445,0.060969575907031025
149,464,0,464,0.05309295654296875,0.06063775500875791
151,470,0,470,0.05359792709350586,0.060484402688794965
153,477,0,477,0.054121971130371094,0.06006632067189576
156,486,0,486,0.05489778518676758,0.05933078297976143
158,492,0,492,0.05540299415588379,0.058455463354690186
160,498,0,498,0.055906057357788086,0.05723633259420055
162,504,0,504,0.056411027908325195,0.05600515889045329
165,513,0,513,0.0572049617767334,0.054248333482093944
167,519,0,519,0.05772209167480469,0.05327974183274877
169,525,0,525,0.0582277774810791,0.05246333317808791
171,531,0,531,0.058740854263305664,0.05178546447548902
173,537,0,537,0.05929112434387207,0.05116051781473578
176,546,0,546,0.06006598472595215,0.0502934540139301
178,552,0,552,0.060575008392333984,0.04979377036454916
180,558,0,558,0.0611119270324707,0.04933007447800771
182,564,0,564,0.061618804931640625,0.048889860661886615
185,573,0,573,0.062374114990234375,0.04822997522597986
187,579,0,579,0.06287789344787598,0.047777032101011085
189,585,0,585,0.06338000297546387,0.04732043341931912
191,591,0,591,0.06388092041015625,0.046875447842948524
193,597,0,597,0.06439590454101562,0.04645611246292111
196,606,0,606,0.06516289710998535,0.04588416782354392
198,612,0,612,0.06583285331726074,0.04553629448636503
200,618,0,618,0.06645393371582031,0.04521093471569802
202,624,0,624,0.06696581840515137,0.04490519508629148
205,633,0,633,0.06773805618286133,0.044478568459481005
207,639,0,639,0.06824278831481934,0.04421384839306528
209,645,0,645,0.06875801086425781,0.04396429125102419
211,651,0,651,0.06924700736999512,0.04373006657212626
213,657,0,657,0.0697319507598877,0.043511437834275274
216,666,0,666,0.07047295570373535,0.043214382561715864
218,672,0,672,0.07100486755371094,0.043040126001650005
220,678,0,678,0.07157397270202637,0.042894145296285956
222,684,0,684,0.07221078872680664,0.042821094895923714
225,695,0,695,0.07305908203125,0.04263548779463991
227,701,0,701,0.0735468864440918,0.04250966506787771
229,709,0,709,0.07414484024047852,0.042417388649961064
231,716,0,716,0.07468795776367188,0.04230931308675669
233,723,0,723,0.07520890235900879,0.042214563532795624
236,735,0,735,0.07603812217712402,0.04208537280144183
238,743,0,743,0.07663607597351074,0.04200507708870703
240,751,0,751,0.07716917991638184,0.04192859398953693
242,759,0,759,0.07770586013793945,0.041855315718832165
245,771,0,771,0.07851386070251465,0.041749357714559336
247,779,0,779,0.0790860652923584,0.041680931553336645
249,787,0,787,0.07961583137512207,0.041614257694008804
251,795,0,795,0.0801551342010498,0.04154944089222986
253,803,0,803,0.08068609237670898,0.041486481590479386
256,815,0,815,0.08150386810302734,0.04139605421772618
258,823,0,823,0.08217215538024902,0.04133970554499109
260,831,0,831,0.08276486396789551,0.041290420834258185
262,840,0,840,0.08352994918823242,0.04124051361546881
265,850,0,850,0.08431005477905273,0.04005523193423162
267,856,0,856,0.08476781845092773,0.0392868659175843
269,862,0,862,0.08519482612609863,0.03873712666934055
271,868,0,868,0.08568906784057617,0.038341561771442885
273,874,0,874,0.08623099327087402,0.038118543709683914
276,883,0,883,0.08693599700927734,0.03785097598498142
278,889,0,889,0.0873568058013916,0.03773035267330131
280,895,0,895,0.08776593208312988,0.037676444303636834
282,902,0,902,0.08830785751342773,0.037637233072617855
285,914,0,914,0.08927607536315918,0.037534479897880196
287,922,0,922,0.0897378921508789,0.03747041768225319
289,930,0,930,0.09019112586975098,0.03740957120854894
291,938,0,938,0.09065794944763184,0.037352145321999236
293,946,0,946,0.0912008285522461,0.03729832313824962
296,958,0,958,0.09188294410705566,0.03723272042965359
298,967,0,967,0.09244990348815918,0.037200309641917964
300,974,0,974,0.09289693832397461,0.03606330327785142
302,982,0,982,0.09358501434326172,0.03567369325370182
305,991,0,991,0.09434390068054199,0.034407239144140775
307,999,0,999,0.09500408172607422,0.03388038448713157
309,1006,0,1006,0.09564208984375,0.03367496834242815
311,1014,0,1014,0.09609484672546387,0.03344163579665906
313,1020,0,1020,0.09650707244873047,0.033282513842686906
316,1031,0,1031,0.09720015525817871,0.032970843270415336
318,1039,0,1039,0.09767389297485352,0.0328324035975801
320,1047,0,1047,0.09829902648925781,0.0327154231367234
322,1055,0,1055,0.09876608848571777,0.032614148104326855
325,1067,0,1067,0.0994410514831543,0.032485549941864686
327,1075,0,1075,0.09989404678344727,0.03241238584572275
329,1083,0,1083,0.1003408432006836,0.03235023631944958
331,1091,0,1091,0.10079598426818848,0.03228607900296913
333,1097,0,1097,0.10120582580566406,0.03225333327353229
336,1107,0,1107,0.10184097290039062,0.03220861136577456
338,1115,0,1115,0.10231280326843262,0.032148688240387545
340,1123,0,1123,0.10277080535888672,0.03209360293008929
342,1131,0,1131,0.10323286056518555,0.03204203082366148
345,1141,0,1141,0.1038661003112793,0.03201323180801919
347,1147,0,1147,0.1042790412902832,0.032006883730057216
349,1153,0,1153,0.10469293594360352,0.032001761818695455
351,1159,0,1159,0.10510778427124023,0.03199914329875191
353,1165,0,1165,0.10550904273986816,0.03199502012808096
356,1174,0,1174,0.10609102249145508,0.031982426826248134
358,1180,0,1180,0.10647296905517578,0.031973584661430236
360,1186,0,1186,0.1068568229675293,0.03196767008844524
362,1192,0,1192,0.10723876953125,0.031965882145057474
365,1204,0,1204,0.10788083076477051,0.03191711318893563
367,1212,0,1212,0.10830903053283691,0.03188541874953381
369,1220,0,1220,0.10873603820800781,0.03185418362965606
371,1227,0,1227,0.1091470718383789,0.03183639280806016
374,1236,0,1236,0.10973310470581055,0.0318149813802028
376,1242,0,1242,0.1101229190826416,0.03179372803564232
378,1248,0,1248,0.11051487922668457,0.03176881903028347
380,1254,0,1254,0.11092090606689453,0.03174067412206088
382,1260,0,1260,0.11133098602294922,0.03170793953230777
385,1269,0,1269,0.11194801330566406,0.03164741923514511
387,1275,0,1275,0.11236190795898438,0.03159921855737255
389,1281,0,1281,0.11277294158935547,0.03154449030425179
391,1287,0,1287,0.1131889820098877,0.03148159028286644
394,1296,0,1296,0.11379194259643555,0.031366663165563205
396,1302,0,1302,0.11419796943664551,0.03127264216721307
398,1308,0,1308,0.11459803581237793,0.031161893770534806
400,1314,0,1314,0.11499214172363281,0.031032132098980435
402,1320,0,1320,0.115386962890625,0.03088123213721216
405,1329,0,1329,0.11599302291870117,0.03061311297948879
407,1335,0,1335,0.11640501022338867,0.030406961940746307
409,1341,0,1341,0.11680984497070312,0.03018085105034826
411,1347,0,1347,0.11721205711364746,0.02993715706981183
414,1356,0,1356,0.11781597137451172,0.0295443208551814
416,1362,0,1362,0.11821794509887695,0.029267744262235
418,1368,0,1368,0.1186208724975586,0.028982125921187825
420,1374,0,1374,0.11903095245361328,0.02868965954207458
422,1380,0,1380,0.11942291259765625,0.028392471263913806
425,1389,0,1389,0.12002992630004883,0.027942297932590156
427,1395,0,1395,0.12043213844299316,0.02764212316128426
429,1401,0,1401,0.1208338737487793,0.027343945278976888
431,1407,0,1407,0.12123799324035645,0.027049133433693192
434,1416,0,1416,0.12185001373291016,0.02661523284334067
436,1422,0,1422,0.12225198745727539,0.026332342967150195
438,1428,0,1428,0.12265491485595703,0.026055049664319516
440,1434,0,1434,0.12305712699890137,0.025783855709356117
442,1440,0,1440,0.1234591007232666,0.025519500141102713
445,1449,0,1449,0.1240849494934082,0.025138254388256998
447,1455,0,1455,0.12450504302978516,0.024896652162793326
449,1461,0,1461,0.1249380111694336,0.02466778633309911
451,1467,0,1467,0.12536191940307617,0.024455011408625077
454,1476,0,1476,0.12596487998962402,0.024177354537159225
456,1482,0,1482,0.12636685371398926,0.0240313738976892
458,1488,0,1488,0.12679791450500488,0.02392657922458249
460,1494,0,1494,0.12744808197021484,0.023852659644086945
462,1500,0,1500,0.12802886962890625,0.023757837386464573
465,1510,0,1510,0.1287858486175537,0.023633886977671093
467,1518,0,1518,0.12936997413635254,0.023584103293992385
469,1526,0,1526,0.13005304336547852,0.02353791642861742
471,1534,0,1534,0.1307229995727539,0.023494614890544538
474,1546,0,1546,0.13179898262023926,0.023434538955814377
476,1554,0,1554,0.13251495361328125,0.023399210177856452
478,1562,0,1562,0.13332200050354004,0.023374401365987618
480,1570,0,1570,0.13395977020263672,0.023344664839009155
482,1577,0,1577,0.13465380668640137,0.02324951972293133
485,1586,0,1586,0.1356348991394043,0.02305558629967229
487,1592,0,1592,0.13621187210083008,0.022905205861186904
489,1598,0,1598,0.13667893409729004,0.022837997983787536
491,1606,0,1606,0.13720011711120605,0.02278159526662363
494,1618,0,1618,0.13811397552490234,0.022708732005388817
496,1626,0,1626,0.13864398002624512,0.022665624745170487
498,1633,0,1633,0.1390688419342041,0.022645178184221047
500,1639,0,1639,0.13947582244873047,0.02258885675777679
502,1645,0,1645,0.1399059295654297,0.02245811292576543
505,1654,0,1654,0.14048981666564941,0.02220521117861091
507,1660,0,1660,0.14088106155395508,0.021995659248492234
509,1666,0,1666,0.1412978172302246,0.0217461538817221
511,1672,0,1672,0.14181900024414062,0.021510243761398866
514,1681,0,1681,0.14260077476501465,0.021175606196762772
516,1687,0,1687,0.14298486709594727,0.020961028054564634
518,1693,0,1693,0.14347195625305176,0.020755271606469214
520,1699,0,1699,0.14400100708007812,0.020555208556321848
522,1705,0,1705,0.14441204071044922,0.020364423105158458
525,1714,0,1714,0.14500093460083008,0.02009382788247886
527,1720,0,1720,0.14541411399841309,0.019916739544159637
529,1726,0,1726,0.1459031105041504,0.019740430834197274
531,1732,0,1732,0.14641880989074707,0.01956622886545284
534,1741,0,1741,0.14708590507507324,0.01931065332812554
536,1747,0,1747,0.14750099182128906,0.019144840178476372
538,1753,0,1753,0.14791584014892578,0.018983514478777934
540,1759,0,1759,0.14835906028747559,0.018827764889293653
542,1765,0,1765,0.14878582954406738,0.018678470153180797
545,1774,0,1774,0.14945292472839355,0.018467900813938936
547,1780,0,1780,0.1498889923095703,0.018336876550441118
549,1786,0,1786,0.15032482147216797,0.018213501619025033
551,1792,0,1792,0.15076088905334473,0.01809786516614195
554,1801,0,1801,0.15144586563110352,0.017939134943592394
556,1807,0,1807,0.15189385414123535,0.01784336279439049
558,1813,0,1813,0.15234088897705078,0.017755728374905397
560,1819,0,1819,0.1528019905090332,0.0176761539048322
562,1825,0,1825,0.15324783325195312,0.01760437640441547
565,1834,0,1834,0.15392088890075684,0.01751066912365386
567,1840,0,1840,0.15437006950378418,0.01745718432988619
569,1846,0,1846,0.15482211112976074,0.017410732034268357
571,1852,0,1852,0.15526604652404785,0.01737112612173743
574,1861,0,1861,0.15593385696411133,0.01732377757040846
576,1867,0,1867,0.15637803077697754,0.017299481638571
578,1873,0,1873,0.15682387351989746,0.017280312213141236
580,1879,0,1879,0.15727686882019043,0.017265749390223205
582,1885,0,1885,0.15770792961120605,0.01725542459675457
585,1894,0,1894,0.15836215019226074,0.017247493500544216
587,1901,0,1901,0.1588149070739746,0.01724172217308104
589,1907,0,1907,0.1592729091644287,0.017236519188457464
591,1914,0,1914,0.15973806381225586,0.01722724668378157
594,1925,0,1925,0.16045093536376953,0.017212231749048942
596,1931,0,1931,0.16089582443237305,0.01720415646143508
598,1938,0,1938,0.1613600254058838,0.017195091378200644
600,1945,0,1945,0.16182494163513184,0.017183594671473422
602,1952,0,1952,0.1622929573059082,0.017178264795127303
605,1962,0,1962,0.16296100616455078,0.0171634226441996
607,1968,0,1968,0.1633930206298828,0.017141503774710472
609,1974,0,1974,0.16382503509521484,0.017126473338202986
611,1981,0,1981,0.16428494453430176,0.017117949252690258
614,1990,0,1990,0.16493511199951172,0.017071369079167176
616,1996,0,1996,0.16536688804626465,0.017030023747389787
618,2002,0,2002,0.16579985618591309,0.016991444532415495
620,2008,0,2008,0.1662299633026123,0.016954891326185068
623,2017,0,2017,0.16687893867492676,0.016900041297922604
625,2023,0,2023,0.16731476783752441,0.016860840243483895
627,2029,0,2029,0.16774797439575195,0.016817864702147602
629,2035,0,2035,0.16817998886108398,0.016769470279277658
631,2041,0,2041,0.16861295700073242,0.016713941683526832
634,2050,0,2050,0.16929197311401367,0.01661248322073767
636,2056,0,2056,0.16974592208862305,0.01652964499222773
638,2062,0,2062,0.17019200325012207,0.016432867573613005
640,2068,0,2068,0.1706390380859375,0.01632185293327401
643,2077,0,2077,0.1713111400604248,0.01612968602413269
645,2083,0,2083,0.17174506187438965,0.01598476146470863
647,2089,0,2089,0.17220497131347656,0.015824799495502837
649,2095,0,2095,0.17264890670776367,0.01564725276226836
651,2101,0,2101,0.1730940341949463,0.015449724522866155
654,2110,0,2110,0.17375898361206055,0.015113824689857072
656,2116,0,2116,0.17420697212219238,0.014864538181000083
658,2122,0,2122,0.17464184761047363,0.014597456666437254
660,2128,0,2128,0.1750929355621338,0.014315841115717105
663,2137,0,2137,0.17576909065246582,0.01387439307152924
665,2143,0,2143,0.17621493339538574,0.013572560518751123
667,2149,0,2149,0.17664790153503418,0.013268616825823172
669,2155,0,2155,0.17708587646484375,0.012966288350903563
671,2161,0,2161,0.1775190830230713,0.01266948224014334
674,2170,0,2170,0.17818593978881836,0.012241955735661074
676,2176,0,2176,0.17862296104431152,0.011972246846885122
678,2182,0,2182,0.17905402183532715,0.011716345952075281
680,2188,0,2188,0.17948579788208008,0.011474890927861123
683,2197,0,2197,0.18015694618225098,0.011140486184184579
685,2203,0,2203,0.1806011199951172,0.010936676465179731
687,2209,0,2209,0.18105792999267578,0.01074864097845244
689,2215,0,2215,0.1814889907836914,0.010576745619572949
691,2221,0,2221,0.18193697929382324,0.010421106614153424
694,2230,0,2230,0.1826038360595703,0.01021808635705773
696,2236,0,2236,0.18305206298828125,0.010102751992033126
698,2242,0,2242,0.18348312377929688,0.010003106990783044
700,2248,0,2248,0.1839148998260498,0.00991876405097425
703,2257,0,2257,0.18456292152404785,0.009819835106221588
705,2263,0,2263,0.18499493598937988,0.009771012373876934
707,2269,0,2269,0.18542695045471191,0.00973419578487535
709,2275,0,2275,0.18585896492004395,0.009707134232744411
711,2281,0,2281,0.18629097938537598,0.009686926667893456
714,2290,0,2290,0.1869518756866455,0.009661999851172921
716,2296,0,2296,0.18738389015197754,0.009643618635849954
718,2302,0,2302,0.18781590461730957,0.009619552198634824
720,2308,0,2308,0.1882469654083252,0.009586592120419738
723,2317,0,2317,0.18889498710632324,0.009521670352793147
725,2324,0,2324,0.1893470287322998,0.009501444783450885
727,2332,0,2332,0.1898200511932373,0.009494594593009283
729,2340,0,2340,0.1902909278869629,0.00948772513854067
731,2348,0,2348,0.1907639503479004,0.009480791131226903
734,2360,0,2360,0.19147300720214844,0.009470141808048645
736,2366,0,2366,0.19190382957458496,0.009460789692679937
738,2372,0,2372,0.19234490394592285,0.009453824449184878
740,2379,0,2379,0.19279980659484863,0.009449184522688002
743,2389,0,2389,0.19347190856933594,0.009442985376104935
745,2395,0,2395,0.1939067840576172,0.00943723777675974
747,2401,0,2401,0.19434285163879395,0.00943329517962556
749,2407,0,2407,0.19478178024291992,0.009429784799956807
751,2413,0,2413,0.19521594047546387,0.009427517609571676
754,2423,0,2423,0.19588804244995117,0.00938793702009624
756,2429,0,2429,0.19632291793823242,0.009310874072072187
758,2435,0,2435,0.19675803184509277,0.009198125673118094
760,2441,0,2441,0.19719696044921875,0.009056610070875744
763,2450,0,2450,0.1978590488433838,0.008834662418596985
765,2456,0,2456,0.19829392433166504,0.008717484473820886
767,2462,0,2462,0.1987299919128418,0.008624269178182806
769,2468,0,2468,0.19916892051696777,0.008559759955910344
771,2474,0,2474,0.19960594177246094,0.008516469269850089
774,2483,0,2483,0.20026111602783203,0.008474105155700712
776,2489,0,2489,0.20069503784179688,0.008454301374486982
778,2495,0,2495,0.20113205909729004,0.00843963817299671
780,2501,0,2501,0.2015669345855713,0.008429841906389663
783,2510,0,2510,0.20221996307373047,0.008422832740165353
785,2517,0,2517,0.20267701148986816,0.0084153753466445
787,2525,0,2525,0.2031569480895996,0.00840212331430054
789,2533,0,2533,0.20363903045654297,0.008389144913693731
791,2541,0,2541,0.2041158676147461,0.008376394300991408
794,2553,0,2553,0.20483183860778809,0.008357634883532939
796,2561,0,2561,0.2053050994873047,0.008345353954490053
798,2569,0,2569,0.20578289031982422,0.008333236418860756
800,2577,0,2577,0.2062549591064453,0.00832126355556309
803,2589,0,2589,0.2069690227508545,0.008303522131044561
805,2597,0,2597,0.2074439525604248,0.008291776305181705
807,2605,0,2605,0.20791912078857422,0.008280023097035051
809,2612,0,2612,0.2083759307861328,0.0082723953881164
811,2620,0,2620,0.2088479995727539,0.008262182353786368
814,2632,0,2632,0.20956802368164062,0.008247669602334943
816,2640,0,2640,0.21004581451416016,0.008238549715134958
818,2648,0,2648,0.21052002906799316,0.00823004739405143
820,2656,0,2656,0.21099376678466797,0.008222608143552659
823,2668,0,2668,0.21170306205749512,0.008216386599000118
825,2677,0,2677,0.21219396591186523,0.00820348375101317
827,2683,0,2683,0.21262693405151367,0.008129272942245748
829,2689,0,2689,0.2130589485168457,0.00805977459716982
831,2695,0,2695,0.21348977088928223,0.008005362932382992
834,2704,0,2704,0.21413588523864746,0.007953640499151057
836,2710,0,2710,0.2145698070526123,0.007933081695925097
838,2716,0,2716,0.21499991416931152,0.007919789131506897
840,2722,0,2722,0.21543598175048828,0.007911064978325104
843,2731,0,2731,0.21608185768127441,0.007901602668961474
845,2737,0,2737,0.21651387214660645,0.00789491219484538
847,2743,0,2743,0.2169489860534668,0.00788677561665995
849,2749,0,2749,0.21738195419311523,0.007877094939546353
851,2755,0,2755,0.21781301498413086,0.0078660010304196
854,2764,0,2764,0.2184591293334961,0.007847448864439634
856,2770,0,2770,0.21889090538024902,0.007834330987212772
858,2776,0,2776,0.21932196617126465,0.007820957817019709
860,2782,0,2782,0.21975088119506836,0.007807293117446986
863,2791,0,2791,0.22042298316955566,0.00778572237602816
865,2797,0,2797,0.22086191177368164,0.007769819304841385
867,2803,0,2803,0.2212998867034912,0.007751930105202423
869,2809,0,2809,0.22174787521362305,0.007731281558108393
872,2818,0,2818,0.2223968505859375,0.007693765005412085
874,2824,0,2824,0.22283005714416504,0.007663587768429263
876,2830,0,2830,0.22326278686523438,0.007628857663588353
878,2836,0,2836,0.22369718551635742,0.0075893453380081076
880,2842,0,2842,0.22412991523742676,0.007544967158843543
883,2851,0,2851,0.22478199005126953,0.0074692892926611415
885,2857,0,2857,0.22521281242370605,0.007412962186868249
887,2863,0,2863,0.22564697265625,0.007352248541688699
889,2869,0,2869,0.22607994079589844,0.00728756747123147
892,2878,0,2878,0.22674298286437988,0.007184248062826256
894,2884,0,2884,0.22718191146850586,0.007112022332423543
896,2890,0,2890,0.22762393951416016,0.007037812176096466
898,2896,0,2896,0.22806000709533691,0.006962189569717763
900,2902,0,2902,0.22849607467651367,0.006885686416688724
903,2911,0,2911,0.22914814949035645,0.006770340798373578
905,2917,0,2917,0.22958087921142578,0.006693688711597784
907,2923,0,2923,0.2300128936767578,0.006617695054705611
909,2929,0,2929,0.23044490814208984,0.006542718108068289
912,2938,0,2938,0.23111486434936523,0.006432866807640996
914,2944,0,2944,0.23155975341796875,0.00636179857105319
916,2950,0,2950,0.2320239543914795,0.006292762818953005
918,2956,0,2956,0.23246002197265625,0.006225982770911932
920,2962,0,2962,0.23289203643798828,0.006161651613909016
923,2971,0,2971,0.23354005813598633,0.00607009992037009
925,2977,0,2977,0.23397397994995117,0.006012557466045806
927,2983,0,2983,0.23441195487976074,0.005957939205527229
929,2989,0,2989,0.234846830368042,0.0059063403648130655
932,2998,0,2998,0.23549985885620117,0.0058347842469731
934,3004,0,3004,0.2359328269958496,0.005791079178734759
936,3010,0,3010,0.23636794090270996,0.005750643354612887
938,3016,0,3016,0.23680400848388672,0.005713523513983479
940,3022,0,3022,0.23726797103881836,0.005679751944912082
943,3031,0,3031,0.23794889450073242,0.005635399061148743
945,3037,0,3037,0.23839616775512695,0.005610015609783736
947,3043,0,3043,0.23885679244995117,0.005587933460453242
949,3049,0,3049,0.2393169403076172,0.005569082454825697
952,3058,0,3058,0.24001407623291016,0.005546644363127666
954,3064,0,3064,0.24045896530151367,0.005535388699401222
956,3070,0,3070,0.2409038543701172,0.005526912316945203
958,3076,0,3076,0.24135112762451172,0.005521033008279043
960,3082,0,3082,0.24179697036743164,0.005517547744714488
963,3092,0,3092,0.24249005317687988,0.005514855806142043
965,3099,0,3099,0.24295997619628906,0.005513348554444378
967,3107,0,3107,0.24345803260803223,0.005510657645045665
969,3115,0,3115,0.24396491050720215,0.0055080151552424645
972,3127,0,3127,0.24467992782592773,0.005504121063687884
974,3135,0,3135,0.24516797065734863,0.005501570307990202
976,3143,0,3143,0.24564099311828613,0.005499059580649151
978,3151,0,3151,0.24611401557922363,0.0054965883532783425
980,3159,0,3159,0.24658608436584473,0.005494154486918324
983,3171,0,3171,0.24744701385498047,0.005490590529470933
985,3179,0,3179,0.2479548454284668,0.005488301282429976
987,3187,0,3187,0.24845409393310547,0.005486131027691802
989,3195,0,3195,0.24895405769348145,0.00548419482860479
992,3208,0,3208,0.24965500831604004,0.005481679094171321
994,3216,0,3216,0.25013089179992676,0.0054737802917180925
996,3224,0,3224,0.2505769729614258,0.00547042740558922
998,3232,0,3232,0.2510209083557129,0.005467486095622619
1000,3240,0,3240,0.2514638900756836,0.005464789060379803
1003,3252,0,3252,0.2521340847015381,0.0054611528968353095
1005,3260,0,3260,0.25258684158325195,0.005459254897488698
1007,3269,0,3269,0.2530488967895508,0.0054575494688336515
1009,3279,0,3279,0.25353002548217773,0.005455199959987869
1012,3291,0,3291,0.2541959285736084,0.005445283222512154
1014,3299,0,3299,0.2546401023864746,0.005438277990413148
1016,3306,0,3306,0.2550630569458008,0.005410648694121824
1018,3313,0,3313,0.25553083419799805,0.005399029139148863
1020,3321,0,3321,0.25597310066223145,0.005393419558045859
1023,3333,0,3333,0.25663089752197266,0.005387008411046106
1025,3342,0,3342,0.25708699226379395,0.005383719900716452
1027,3350,0,3350,0.2575337886810303,0.0053733675611222975
1029,3356,0,3356,0.257936954498291,0.005289857358004484
1032,3365,0,3365,0.25853991508483887,0.00523612001398744
1034,3371,0,3371,0.2589418888092041,0.0052038818019515464
1036,3377,0,3377,0.25934410095214844,0.005170161195981561
1038,3383,0,3383,0.2597517967224121,0.005133284137207123
1040,3389,0,3389,0.26015615463256836,0.005094247008801212
1043,3398,0,3398,0.26076412200927734,0.005031803752550735
1045,3404,0,3404,0.2611730098724365,0.004987227025423146
1047,3410,0,3410,0.26157689094543457,0.0049415131853581
1049,3416,0,3416,0.2619800567626953,0.004894439763868622
1052,3425,0,3425,0.2625861167907715,0.00482224710019077
1054,3431,0,3431,0.26298999786376953,0.0047736523223939386
1056,3437,0,3437,0.2633998394012451,0.00472505037744895
1058,3443,0,3443,0.26380491256713867,0.004676677513229763
1060,3449,0,3449,0.2642080783843994,0.0046287098125719715
1063,3458,0,3458,0.2648189067840576,0.004558059967931355
1065,3464,0,3464,0.2652249336242676,0.004512119762847943
1067,3470,0,3470,0.2656288146972656,0.004467377840247722
1069,3476,0,3476,0.2660388946533203,0.004423916946586237
1072,3485,0,3485,0.26664185523986816,0.004361292425749065
1074,3491,0,3491,0.2670459747314453,0.004321163593873612
1076,3497,0,3497,0.2674558162689209,0.004282193252437626
1078,3503,0,3503,0.26785993576049805,0.004244181670005731
1080,3509,0,3509,0.2682638168334961,0.004206970294836323
1083,3518,0,3518,0.2688717842102051,0.0041522046535798
1085,3524,0,3524,0.2692739963531494,0.004116101003887295
1087,3530,0,3530,0.26967811584472656,0.004080074402092233
1089,3536,0,3536,0.2700810432434082,0.004043983067927375
1092,3545,0,3545,0.27068305015563965,0.003989511965975219
1094,3551,0,3551,0.2710881233215332,0.003952943366515165
1096,3557,0,3557,0.2714967727661133,0.0039162038768555145
1098,3563,0,3563,0.27190089225769043,0.003879382367298886
1100,3569,0,3569,0.27230405807495117,0.003842593967864856
1103,3578,0,3578,0.27291011810302734,0.003787784414103941
1105,3584,0,3584,0.273313045501709,0.0037517159262971645
1107,3590,0,3590,0.2737147808074951,0.003716207208044626
1109,3596,0,3596,0.27411603927612305,0.003681409787469593
1112,3605,0,3605,0.2747230529785156,0.0036308582746367606
1114,3611,0,3611,0.27512383460998535,0.003598437046254979
1116,3617,0,3617,0.2755250930786133,0.0035671617983390248
1118,3623,0,3623,0.275925874710083,0.0035371113092935074
1121,3632,0,3632,0.2765328884124756,0.003494443648273025
1123,3638,0,3638,0.27693676948547363,0.0034676369264427928
1125,3644,0,3644,0.2773427963256836,0.0034421366918626875
1127,3650,0,3650,0.27774500846862793,0.0034179163141127814
1129,3656,0,3656,0.27814602851867676,0.0033949332114838185
1132,3665,0,3665,0.27875185012817383,0.0033626570890498697
1134,3671,0,3671,0.27915382385253906,0.0033425136979775335
1136,3677,0,3677,0.279555082321167,0.0033233933308235175
1138,3683,0,3683,0.2799558639526367,0.0033052325646051465
1141,3692,0,3692,0.28055596351623535,0.0032796633490160283
1143,3698,0,3698,0.2809567451477051,0.0032636572446550017
1145,3704,0,3704,0.2813589572906494,0.003248432422992421
1147,3710,0,3710,0.2817661762237549,0.0032339525904099514
1149,3716,0,3716,0.2821660041809082,0.0032201867202333295
1152,3725,0,3725,0.2827718257904053,0.003200817696585504
1154,3731,0,3731,0.2831740379333496,0.0031887220347743164
1156,3737,0,3737,0.28357601165771484,0.0031772513808955042
1158,3743,0,3743,0.2839798927307129,0.0031663800495556177
1161,3752,0,3752,0.28458380699157715,0.0031511359340277143
1163,3758,0,3758,0.28498387336730957,0.003141637641924333
1165,3764,0,3764,0.2853848934173584,0.0031326327729136135
1167,3770,0,3770,0.28578805923461914,0.003124086299359342
1169,3776,0,3776,0.2861909866333008,0.0031159608523729353
1172,3785,0,3785,0.286801815032959,0.0031044714843631574
1174,3791,0,3791,0.28720784187316895,0.0030972060720640886
1176,3797,0,3797,0.2876100540161133,0.003090179894383124
1178,3803,0,3803,0.2880120277404785,0.003083292732266651
1181,3812,0,3812,0.28865504264831543,0.0030728041215748263
1183,3818,0,3818,0.28905701637268066,0.0030650690842120728
1185,3824,0,3824,0.2894587516784668,0.003055398898505812
1187,3830,0,3830,0.2898590564727783,0.0030407123283156244
1189,3836,0,3836,0.2903869152069092,0.003015233037622289
1192,3845,0,3845,0.2909989356994629,0.0029498683519832212
1194,3851,0,3851,0.29140281677246094,0.002894917895037683
1196,3855,0,3855,0.2917659282684326,0.001682293255992174
1198,3861,0,3861,0.2923009395599365,0.0016282885634946115
1201,3871,0,3871,0.2929229736328125,0.0015282348810834294
1203,3877,0,3877,0.29332709312438965,0.0014775288853000207
1205,3883,0,3883,0.2937288284301758,0.0014422901441305713
1207,3889,0,3889,0.2941319942474365,0.0014105687742588398
1209,3895,0,3895,0.2945380210876465,0.0013885188945920337
1212,3904,0,3904,0.29514384269714355,0.0013649469442903648
1214,3910,0,3910,0.2955460548400879,0.0013511495914430584
1216,3916,0,3916,0.2959930896759033,0.0013352645797054987
1218,3922,0,3922,0.29639601707458496,0.0013197346869653806
1221,3931,0,3931,0.2970008850097656,0.0012761319369287325
1223,3937,0,3937,0.29741692543029785,0.0012508357987249536
1225,3943,0,3943,0.2978217601776123,0.001230825446763804
1227,3949,0,3949,0.29822516441345215,0.0012129774439988332
1229,3955,0,3955,0.2986280918121338,0.001193101869882779
1232,3964,0,3964,0.2992370128631592,0.0011680316556972857
1234,3971,0,3971,0.29965782165527344,0.001162182840230619
1236,3979,0,3979,0.3000979423522949,0.0011519881247054502
1238,3987,0,3987,0.3005390167236328,0.0011421657905699338
1241,3998,0,3998,0.3011770248413086,0.0011317331519201887
1243,4004,0,4004,0.30157995223999023,0.0011274551040557162
1245,4010,0,4010,0.3019881248474121,0.0011208758807557092
1247,4016,0,4016,0.30239200592041016,0.0011133205250341703
1249,4022,0,4022,0.30280113220214844,0.0011044994294762986
1252,4031,0,4031,0.3034098148345947,0.001084290705356171
1254,4039,0,4039,0.3038499355316162,0.0010679256619129795
1256,4045,0,4045,0.30425381660461426,0.001045381141781954
1258,4051,0,4051,0.3046588897705078,0.001010493756221718
1261,4060,0,4060,0.30525994300842285,0.0009568032881818365
1263,4066,0,4066,0.3056609630584717,0.0009232171947273543
1265,4072,0,4072,0.3060619831085205,0.0008918751985328681
1267,4078,0,4078,0.30646300315856934,0.0008626245803153481
1269,4084,0,4084,0.30686211585998535,0.0008347237234567624
1272,4093,0,4093,0.30747008323669434,0.0007943192154938754
1274,4099,0,4099,0.3078761100769043,0.0007686704478157758
1276,4105,0,4105,0.30827784538269043,0.0007442674505537775
1278,4111,0,4111,0.30867815017700195,0.0007213051508195259
1281,4120,0,4120,0.3092789649963379,0.0006900011184074496
1283,4126,0,4126,0.3096799850463867,0.0006736461610314679
1285,4132,0,4132,0.31008100509643555,0.0006580099207600844
1287,4138,0,4138,0.3104839324951172,0.0006375302673503938
1289,4144,0,4144,0.3108839988708496,0.0006177751835485634
1292,4155,0,4155,0.3115229606628418,0.0006063327191526368
1294,4163,0,4163,0.31195998191833496,0.0006035320569105841
1296,4171,0,4171,0.3123970031738281,0.0006008902379058026
1298,4179,0,4179,0.3128340244293213,0.0005983681480269433
1301,4191,0,4191,0.3134949207305908,0.0005948033281511617
1303,4199,0,4199,0.3139340877532959,0.0005925550572862305
1305,4207,0,4207,0.3143730163574219,0.0005904014888760471
1307,4215,0,4215,0.31481289863586426,0.0005883128707486313
1309,4223,0,4223,0.31525182723999023,0.0005862387828814351
1312,4235,0,4235,0.31591010093688965,0.0005827670227231186
1314,4243,0,4243,0.3163480758666992,0.0005795457699541933
1316,4250,0,4250,0.3167688846588135,0.0005675358633840168
1318,4256,0,4256,0.3171730041503906,0.0005636981460224408
1321,4265,0,4265,0.31777405738830566,0.0005595544915547165
1323,4271,0,4271,0.3181748390197754,0.0005582929220974979
1325,4277,0,4277,0.31858181953430176,0.0005576406703237785
1327,4283,0,4283,0.3189830780029297,0.0005570608688338234
1329,4289,0,4289,0.3193960189819336,0.0005559915416550104
1332,4298,0,4298,0.31998586654663086,0.0005522160517413166
1334,4304,0,4304,0.3203771114349365,0.000548008793876116
1336,4310,0,4310,0.3207688331604004,0.0005423235727615523
1338,4316,0,4316,0.32115912437438965,0.0005354962489513944
1341,4325,0,4325,0.3217451572418213,0.0005245290406199872
1343,4331,0,4331,0.32213497161865234,0.0005177374991628867
1345,4337,0,4337,0.3225247859954834,0.0005120695020076857
1347,4343,0,4343,0.32291603088378906,0.0005077337185852515
1349,4349,0,4349,0.3233070373535156,0.0005053224151782522
1352,4359,0,4359,0.32392096519470215,0.0005042042932937179
1354,4365,0,4365,0.3243098258972168,0.000498507821827991
1356,4371,0,4371,0.3247039318084717,0.0004932352041426618
1358,4377,0,4377,0.32509493827819824,0.0004878617738952511
1361,4386,0,4386,0.32567811012268066,0.00047913729904332155
1363,4392,0,4392,0.3260688781738281,0.00047255498585392007
1365,4398,0,4398,0.3264591693878174,0.00046520498389658805
1367,4404,0,4404,0.32684898376464844,0.0004570963627882384
1370,4413,0,4413,0.32744288444519043,0.0004436744783531016
1372,4419,0,4419,0.3278329372406006,0.0004341711902083563
1374,4425,0,4425,0.32822299003601074,0.00042453241986289156
1376,4431,0,4431,0.32862091064453125,0.00041505304056288326
1378,4437,0,4437,0.3290128707885742,0.0004059723207797176
1381,4446,0,4446,0.32959794998168945,0.00039358151550331224
1383,4452,0,4452,0.3299901485443115,0.00038635451842353565
1385,4458,0,4458,0.3303821086883545,0.0003800767750843431
1387,4464,0,4464,0.33077287673950195,0.0003746888445947284
1390,4473,0,4473,0.3313620090484619,0.0003679109238161607
1392,4479,0,4479,0.33175182342529297,0.0003639342621082517
1394,4485,0,4485,0.33214306831359863,0.0003601466201000277
1396,4491,0,4491,0.3325338363647461,0.00035641841923625953
1398,4497,0,4497,0.33292412757873535,0.0003526625448439112
1401,4506,0,4506,0.3335127830505371,0.0003468735136556136
1403,4512,0,4512,0.3339049816131592,0.00034289137505951877
1405,4518,0,4518,0.3343038558959961,0.00033877468037803074
1407,4524,0,4524,0.3346989154815674,0.00033439883715453587
1410,4533,0,4533,0.33528804779052734,0.0003274573840176903
1412,4539,0,4539,0.3356788158416748,0.00032387180637053316
1414,4546,0,4546,0.3360869884490967,0.000322639062033267
1416,4552,0,4552,0.33647608757019043,0.0003189477630859894
1418,4558,0,4558,0.336867094039917,0.00030997701860275504
1421,4567,0,4567,0.33745503425598145,0.00029550708193436525
1423,4573,0,4573,0.3378469944000244,0.00028744677116758835
1425,4579,0,4579,0.3382377624511719,0.00028318300052574904
1427,4586,0,4586,0.3386538028717041,0.00028214117598365286
1430,4595,0,4595,0.33924293518066406,0.0002700696449331984
1432,4601,0,4601,0.3396339416503906,0.00026237044216896875
1434,4607,0,4607,0.3400249481201172,0.000256213601407221
1436,4613,0,4613,0.34041595458984375,0.00025219144769185106
1438,4620,0,4620,0.34082508087158203,0.0002502675900598488
1441,4630,0,4630,0.3414268493652344,0.00022907514750091415
1443,4636,0,4636,0.34181809425354004,0.00022199626470667977
1445,4642,0,4642,0.3422110080718994,0.00021900281804534591
1447,4649,0,4649,0.342620849609375,0.000217810317298603
1450,4659,0,4659,0.343228816986084,0.00021420369081920715
1452,4665,0,4665,0.3436248302459717,0.00021013432529606762
1454,4671,0,4671,0.34401702880859375,0.00020661342689417222
1456,4677,0,4677,0.3444099426269531,0.0002034289436630768
1458,4683,0,4683,0.3448059558868408,0.00020032419784950245
1461,4692,0,4692,0.34539198875427246,0.00019586054702907857
1463,4698,0,4698,0.34578394889831543,0.00019318672611534057
1465,4704,0,4704,0.3461780548095703,0.00019088874176052546
1467,4710,0,4710,0.3465719223022461,0.00018936779089287682
1470,4721,0,4721,0.3472020626068115,0.00018826460623637506
1472,4729,0,4729,0.34763002395629883,0.00018755862166439094
1474,4737,0,4737,0.3480570316314697,0.00018687384876530953
1476,4744,0,4744,0.3484659194946289,0.00018639059860420853
1478,4750,0,4750,0.348862886428833,0.00018341402546618636
1481,4759,0,4759,0.34944987297058105,0.00017864468191509323
1483,4765,0,4765,0.349841833114624,0.00017468873187716412
1485,4771,0,4771,0.3502340316772461,0.00017004925933493826
1487,4777,0,4777,0.35062599182128906,0.00016465996374788946
1490,4786,0,4786,0.35121774673461914,0.00015464262436347387
1492,4792,0,4792,0.3516120910644531,0.00014610517275362613
1494,4798,0,4798,0.3520030975341797,0.00013984654125410613
1496,4804,0,4804,0.35239601135253906,0.00013363928858105097
1498,4810,0,4810,0.35278797149658203,0.0001289020869387585
1501,4819,0,4819,0.35337209701538086,0.00012338080619706486
1503,4825,0,4825,0.35376787185668945,0.00012055026313802429
1505,4831,0,4831,0.35416102409362793,0.00011863383427344868
1507,4838,0,4838,0.35457301139831543,0.00011727434058868447
1510,4850,0,4850,0.3553457260131836,0.00011609716622165331
1512,4858,0,4858,0.355802059173584,0.00011547334016449303
1514,4866,0,4866,0.3562328815460205,0.0001149143781556153
1516,4874,0,4874,0.3566620349884033,0.00011440702784999671
1518,4882,0,4882,0.3570878505706787,0.00011393153173039176
1521,4894,0,4894,0.3577241897583008,0.00011325645439550503
1523,4902,0,4902,0.3581569194793701,0.0001128266992368323
1525,4908,0,4908,0.3585469722747803,0.00011152156462267781
1527,4914,0,4914,0.3589348793029785,0.00010904937892093302
1530,4923,0,4923,0.3595249652862549,0.00010530147420392743
1532,4929,0,4929,0.3599119186401367,0.00010283870481503879
1534,4935,0,4935,0.36029887199401855,0.00010056243902969934
1536,4941,0,4941,0.3606870174407959,9.84035405632141e-05
1538,4947,0,4947,0.36107373237609863,9.638870306512858e-05
1541,4956,0,4956,0.36165499687194824,9.353702176837043e-05
1543,4962,0,4962,0.3620419502258301,9.173783440473856e-05
1545,4968,0,4968,0.36243391036987305,8.999784560460076e-05
1547,4974,0,4974,0.3628220558166504,8.833222992186812e-05
1550,4983,0,4983,0.3634028434753418,8.596214366419784e-05
1552,4989,0,4989,0.36378908157348633,8.451847791304308e-05
1554,4995,0,4995,0.3641808032989502,8.321555787388493e-05
1556,5001,0,5001,0.36457014083862305,8.221441134214455e-05
1558,5007,0,5007,0.3649568557739258,8.158438402443853e-05
1561,5018,0,5018,0.36557698249816895,8.123423175566536e-05
1563,5027,0,5027,0.36601805686950684,8.105396994715917e-05
1565,5033,0,5033,0.3664071559906006,7.694214361419081e-05
1567,5039,0,5039,0.3667948246002197,7.59305616845876e-05
1570,5048,0,5048,0.367372989654541,7.495539009347608e-05
1572,5054,0,5054,0.36775898933410645,7.455525860053734e-05
1574,5060,0,5060,0.3681468963623047,7.426566256726349e-05
1576,5066,0,5066,0.3685338497161865,7.410723704139354e-05
1578,5072,0,5072,0.36892104148864746,7.401723665517313e-05
1581,5081,0,5081,0.3695058822631836,7.377493354783455e-05
1583,5087,0,5087,0.3698921203613281,7.342448655369731e-05
1585,5093,0,5093,0.3702828884124756,7.283106585806163e-05
1587,5099,0,5099,0.3706700801849365,7.200162400000705e-05
1590,5108,0,5108,0.37137889862060547,7.04146445902893e-05
1592,5114,0,5114,0.37184596061706543,6.917754480101096e-05
1594,5120,0,5120,0.37223196029663086,6.78850832187927e-05
1596,5126,0,5126,0.3726167678833008,6.656291121347176e-05
1598,5132,0,5132,0.3730008602142334,6.527749587905652e-05
1601,5141,0,5141,0.3735799789428711,6.347239008292076e-05
1603,5147,0,5147,0.3739650249481201,6.23477118830472e-05
1605,5153,0,5153,0.37435388565063477,6.126975074565049e-05
1607,5159,0,5159,0.3747420310974121,6.020124307468342e-05
1610,5168,0,5168,0.37543296813964844,5.8599273081769883e-05
1612,5174,0,5174,0.3760650157928467,5.7510480112862386e-05
1614,5180,0,5180,0.376953125,5.6394564843929065e-05
1616,5186,0,5186,0.3776397705078125,5.5234534332187356e-05
1619,5195,0,5195,0.37821483612060547,5.336423341342695e-05
1621,5201,0,5201,0.37871694564819336,5.2020298760549205e-05
1623,5207,0,5207,0.379288911819458,5.061192392927605e-05
1625,5213,0,5213,0.37981200218200684,4.917309921093231e-05
1627,5219,0,5219,0.38028693199157715,4.773732959023608e-05
1630,5228,0,5228,0.3810908794403076,4.562053754385058e-05
1632,5234,0,5234,0.38163304328918457,4.423709270807319e-05
1634,5240,0,5240,0.3820767402648926,4.28786898890405e-05
1636,5246,0,5246,0.3826580047607422,4.155828181284062e-05
1639,5255,0,5255,0.3833730220794678,3.969693039998938e-05
1641,5261,0,5261,0.3838157653808594,3.8559772545746845e-05
1643,5267,0,5267,0.38429689407348633,3.750857172290965e-05
1645,5273,0,5273,0.3847160339355469,3.653067881509502e-05
1647,5279,0,5279,0.38513994216918945,3.5607410985805894e-05
1650,5288,0,5288,0.38587307929992676,3.4294008134025816e-05
1652,5294,0,5294,0.3863189220428467,3.346403863921079e-05
1654,5300,0,5300,0.38678503036499023,3.2682840287297686e-05
1656,5306,0,5306,0.3872489929199219,3.196244691637497e-05
1659,5315,0,5315,0.38788509368896484,3.099655959246561e-05
1661,5321,0,5321,0.3884549140930176,3.0417290817349406e-05
1663,5327,0,5327,0.38891100883483887,2.9881557263745126e-05
1665,5333,0,5333,0.389354944229126,2.9390910657909685e-05
1667,5339,0,5339,0.38974499702453613,2.893748386370718e-05
1670,5348,0,5348,0.3904130458831787,2.8271431493918874e-05
1672,5354,0,5354,0.3909170627593994,2.7801473247666146e-05
1674,5360,0,5360,0.3913099765777588,2.730226090706758e-05
1676,5366,0,5366,0.3918571472167969,2.6779973837111576e-05
1679,5375,0,5375,0.39252710342407227,2.5987234500587162e-05
1681,5381,0,5381,0.3929469585418701,2.5495806076192427e-05
1683,5387,0,5387,0.3933570384979248,2.5078866698824033e-05
1685,5393,0,5393,0.39377880096435547,2.4752195510792075e-05
1687,5399,0,5399,0.39419102668762207,2.449364493805834e-05
1690,5408,0,5408,0.3948557376861572,2.4137044675418963e-05
1692,5414,0,5414,0.39527297019958496,2.3868873891872876e-05
1694,5420,0,5420,0.39568614959716797,2.3560747773715007e-05
1696,5426,0,5426,0.39609599113464355,2.3219062154790987e-05
1699,5435,0,5435,0.3967127799987793,2.2673117573772375e-05
1701,5441,0,5441,0.39713406562805176,2.229306668236678e-05
1703,5447,0,5447,0.3976619243621826,2.1895909766339584e-05
1705,5453,0,5453,0.3980751037597656,2.148047071698765e-05
1707,5459,0,5459,0.39861392974853516,2.1053829159289026e-05
1710,5468,0,5468,0.39934301376342773,2.0439469148333726e-05
1712,5474,0,5474,0.3997988700866699,2.0096054391422358e-05
1714,5480,0,5480,0.40044307708740234,1.9833921028866053e-05
1716,5486,0,5486,0.4009988307952881,1.962261123595421e-05
1719,5495,0,5495,0.40176892280578613,1.930108372999335e-05
1721,5501,0,5501,0.40221190452575684,1.9042896923850195e-05
1723,5507,0,5507,0.4027230739593506,1.874912162400951e-05
1725,5514,0,5514,0.40313005447387695,1.8515402151554002e-05
1727,5520,0,5520,0.40352296829223633,1.8079120917774468e-05
1730,5529,0,5529,0.40410494804382324,1.741825502746379e-05
1732,5535,0,5535,0.4045429229736328,1.698955510205731e-05
1734,5541,0,5541,0.4049341678619385,1.6583739888155938e-05
1736,5547,0,5547,0.40532898902893066,1.6330881662416337e-05
1739,5557,0,5557,0.4059278964996338,1.616016212792727e-05
1741,5563,0,5563,0.40631699562072754,1.5921514365770024e-05
1743,5569,0,5569,0.4067051410675049,1.5713289320304876e-05
1745,5575,0,5575,0.4070918560028076,1.5487734837992152e-05
1747,5581,0,5581,0.4074878692626953,1.521691787094063e-05
1750,5590,0,5590,0.40807008743286133,1.4769056524617066e-05
1752,5596,0,5596,0.4085218906402588,1.4497664861342192e-05
1754,5602,0,5602,0.4089200496673584,1.4245379487636543e-05
1756,5608,0,5608,0.40930891036987305,1.3997842824637247e-05
1759,5617,0,5617,0.4098958969116211,1.3677200081424193e-05
1761,5623,0,5623,0.41028499603271484,1.3472636607561133e-05
1763,5629,0,5629,0.41068100929260254,1.3216978596342795e-05
1765,5635,0,5635,0.41107702255249023,1.295766484641629e-05
1767,5641,0,5641,0.4116699695587158,1.2846020014009613e-05
1770,5650,0,5650,0.4122757911682129,1.2761586994081799e-05
1772,5656,0,5656,0.4126718044281006,1.2700919363519428e-05
1774,5662,0,5662,0.4133429527282715,1.2587752965681648e-05
1776,5668,0,5668,0.4137539863586426,1.2425704583223653e-05
1779,5677,0,5677,0.4143409729003906,1.203921275185801e-05
1781,5683,0,5683,0.4147350788116455,1.1643126924919925e-05
1783,5689,0,5689,0.41513586044311523,1.1125578526104903e-05
1785,5695,0,5695,0.4155261516571045,1.0531981033590863e-05
1787,5701,0,5701,0.41591501235961914,1.004107455968091e-05
1790,5710,0,5710,0.41650891304016113,9.680732243048909e-06
1792,5717,0,5717,0.4169158935546875,9.578844501691676e-06
1794,5724,0,5724,0.41732192039489746,9.517134223987538e-06
1796,5730,0,5730,0.4177100658416748,9.409100814100685e-06
1799,5740,0,5740,0.41831016540527344,9.209762048757914e-06
1801,5746,0,5746,0.41869688034057617,9.018233260832844e-06
1803,5752,0,5752,0.4190850257873535,8.875441621985101e-06
1805,5758,0,5758,0.4194929599761963,8.75846160881895e-06
1807,5764,0,5764,0.419888973236084,8.662995436975649e-06
1810,5773,0,5773,0.4204897880554199,8.560559466334149e-06
1812,5779,0,5779,0.4208860397338867,8.527655812081994e-06
1814,5785,0,5785,0.42129087448120117,8.521617591280786e-06
1816,5791,0,5791,0.42179298400878906,8.490627646973958e-06
1819,5800,0,5800,0.4223799705505371,8.350192370370506e-06
1821,5806,0,5806,0.42276811599731445,8.173966328131916e-06
1823,5812,0,5812,0.4231557846069336,7.955925624686251e-06
1825,5818,0,5818,0.42354297637939453,7.718951564284565e-06
1827,5824,0,5824,0.42392897605895996,7.477979053981631e-06
1830,5833,0,5833,0.42450809478759766,7.138142667306327e-06
1832,5839,0,5839,0.4248948097229004,6.927511065218511e-06
1834,5845,0,5845,0.4252889156341553,6.721855041358632e-06
1836,5851,0,5851,0.425678014755249,6.521863655330292e-06
1839,5860,0,5860,0.4262559413909912,6.244190388892446e-06
1841,5866,0,5866,0.426785945892334,6.101490460858484e-06
1843,5872,0,5872,0.42722201347351074,6.002504902149148e-06
1845,5878,0,5878,0.4276280403137207,5.948389091088092e-06
1847,5884,0,5884,0.4281940460205078,5.925089295977574e-06
1850,5894,0,5894,0.42885279655456543,5.748237750679262e-06
1852,5900,0,5900,0.4292619228363037,5.7043422302176085e-06
1854,5906,0,5906,0.42966604232788086,5.682637315531856e-06
1856,5912,0,5912,0.43007397651672363,5.649566276351529e-06
1859,5921,0,5921,0.4306778907775879,5.5640955448617406e-06
1861,5927,0,5927,0.43108701705932617,5.487684995655611e-06
1863,5933,0,5933,0.4314920902252197,5.41273831356324e-06
1865,5939,0,5939,0.43189096450805664,5.346550280679696e-06
1868,5948,0,5948,0.43249082565307617,5.2558708185729845e-06
1870,5954,0,5954,0.4328939914703369,5.17895700673039e-06
1872,5960,0,5960,0.43329286575317383,5.0937474043927874e-06
1874,5966,0,5966,0.43369102478027344,5.015576699897789e-06
1876,5972,0,5972,0.4340949058532715,4.949038522228099e-06
1879,5981,0,5981,0.43469786643981934,4.8692719010574e-06
1881,5987,0,5987,0.43509793281555176,4.824364530884319e-06
1883,5993,0,5993,0.43549489974975586,4.782891298367901e-06
1885,5999,0,5999,0.43590283393859863,4.744319215840162e-06
1888,6008,0,6008,0.43650293350219727,4.691396960023884e-06
1890,6014,0,6014,0.4369027614593506,4.657859714078091e-06
1892,6020,0,6020,0.4372999668121338,4.622527233215063e-06
1894,6026,0,6026,0.43770313262939453,4.582316324670347e-06
1896,6032,0,6032,0.43810391426086426,4.535013568700559e-06
1899,6041,0,6041,0.4387040138244629,4.459408310185962e-06
1901,6047,0,6047,0.4391000270843506,4.4292942984965235e-06
1903,6054,0,6054,0.43951892852783203,4.4158551519488395e-06
1905,6061,0,6061,0.43993592262268066,4.386750071289866e-06
1908,6070,0,6070,0.4405369758605957,4.288471606420333e-06
1910,6076,0,6076,0.4409348964691162,4.21301580986846e-06
1912,6082,0,6082,0.441342830657959,4.13628491655002e-06
1914,6088,0,6088,0.44174695014953613,4.05522021353777e-06
1916,6094,0,6094,0.4421849250793457,3.968261181833069e-06
1919,6103,0,6103,0.44278907775878906,3.8305371895293474e-06
1921,6109,0,6109,0.4431941509246826,3.7389858090446e-06
1923,6115,0,6115,0.44359898567199707,3.654101688758791e-06
1925,6121,0,6121,0.4439988136291504,3.5745515238017193e-06
1928,6130,0,6130,0.44460296630859375,3.4633911248126237e-06
1930,6136,0,6136,0.4450089931488037,3.3927595922862653e-06
1932,6142,0,6142,0.44541192054748535,3.3236642103792565e-06
1934,6148,0,6148,0.44580984115600586,3.255790125275494e-06
1936,6154,0,6154,0.4462308883666992,3.188753048665506e-06
1939,6163,0,6163,0.4468388557434082,3.0942855988742246e-06
1941,6169,0,6169,0.44723987579345703,3.037652267540049e-06
1943,6175,0,6175,0.44763994216918945,2.9839371077441595e-06
1945,6181,0,6181,0.4480459690093994,2.9306777467746685e-06
1948,6190,0,6190,0.44864988327026367,2.849362419593326e-06
1950,6196,0,6196,0.4490528106689453,2.793264520982154e-06
1952,6202,0,6202,0.44945406913757324,2.7357033646313096e-06
1954,6208,0,6208,0.4498610496520996,2.6754275150212552e-06
1956,6214,0,6214,0.45026183128356934,2.6128258326442256e-06
1959,6223,0,6223,0.4508640766143799,2.522605323830659e-06
1961,6229,0,6229,0.4512639045715332,2.4665344795656467e-06
1963,6235,0,6235,0.4516777992248535,2.411294187796453e-06
1965,6241,0,6241,0.45208001136779785,2.3575256039872623e-06
1968,6250,0,6250,0.4526839256286621,2.281438437999771e-06
1970,6256,0,6256,0.4530830383300781,2.234292040149016e-06
1972,6262,0,6262,0.4534881114959717,2.1891283628042634e-06
1974,6268,0,6268,0.4538888931274414,2.145088517337948e-06
1976,6274,0,6274,0.45428895950317383,2.1049012838142355e-06
1979,6283,0,6283,0.454941987991333,2.0522419854299363e-06
1981,6289,0,6289,0.45534586906433105,2.0183081368319804e-06
1983,6295,0,6295,0.4557459354400635,1.9832804438514418e-06
1985,6301,0,6301,0.4561440944671631,1.9479858041170904e-06
1988,6310,0,6310,0.45674800872802734,1.8963459946000772e-06
1990,6316,0,6316,0.4571499824523926,1.8604135714804818e-06
1992,6322,0,6322,0.4575510025024414,1.8211246664850677e-06
1994,6328,0,6328,0.4579489231109619,1.7805076866726734e-06
1996,6334,0,6334,0.45835304260253906,1.7423223202476073e-06
1999,6343,0,6343,0.458953857421875,1.6902831926970196e-06
2001,6349,0,6349,0.45935606956481934,1.6569814884848666e-06
2003,6355,0,6355,0.45975184440612793,1.6254023749674381e-06
2005,6361,0,6361,0.4601559638977051,1.5964927487773213e-06
2008,6370,0,6370,0.46075987815856934,1.5565234433351884e-06
2010,6376,0,6376,0.46116089820861816,1.5305887810640552e-06
2012,6382,0,6382,0.46158695220947266,1.5043193587196617e-06
2014,6388,0,6388,0.4620089530944824,1.4795586681917858e-06
2016,6394,0,6394,0.46240997314453125,1.4569484858481286e-06
2019,6403,0,6403,0.46303296089172363,1.4247953389929131e-06
2021,6409,0,6409,0.4634389877319336,1.4037394715061155e-06
2023,6415,0,6415,0.46384310722351074,1.383200882515953e-06
2025,6421,0,6421,0.4642488956451416,1.3630435387714828e-06
2028,6430,0,6430,0.4648609161376953,1.3300987966746942e-06
2030,6436,0,6436,0.4652700424194336,1.3044090138463078e-06
2032,6442,0,6442,0.46567392349243164,1.2756931832195159e-06
2034,6448,0,6448,0.4660789966583252,1.2461309343459852e-06
2036,6454,0,6454,0.4664878845214844,1.2178652651607452e-06
2039,6463,0,6463,0.4671039581298828,1.1810590215351881e-06
2041,6469,0,6469,0.46750783920288086,1.160817964198903e-06
2043,6475,0,6475,0.4679138660430908,1.142366376892682e-06
2045,6481,0,6481,0.4683208465576172,1.123853991050659e-06
2048,6490,0,6490,0.4689309597015381,1.0943372624798231e-06
2050,6496,0,6496,0.4693338871002197,1.0730677762364225e-06
2052,6502,0,6502,0.4697420597076416,1.051138599909649e-06
2054,6508,0,6508,0.47014904022216797,1.029146399303692e-06
2056,6514,0,6514,0.4705510139465332,1.0084278412557066e-06
2059,6523,0,6523,0.4711599349975586,9.841325531869042e-07
2061,6529,0,6529,0.47156810760498047,9.715112805133928e-07
2063,6535,0,6535,0.47197484970092773,9.599376948482413e-07
2065,6541,0,6541,0.4723827838897705,9.474792491095004e-07
2068,6550,0,6550,0.4729881286621094,9.234415056089584e-07
2070,6556,0,6556,0.47339296340942383,9.02542329863858e-07
2072,6562,0,6562,0.4737989902496338,8.780335157995937e-07
2074,6568,0,6568,0.4742000102996826,8.5127813255361e-07
2076,6574,0,6574,0.47460508346557617,8.271289897036493e-07
2079,6583,0,6583,0.4752161502838135,8.043360141622986e-07
2081,6589,0,6589,0.47562098503112793,7.944774252971988e-07
2083,6595,0,6595,0.4760251045227051,7.852637020033281e-07
2085,6601,0,6601,0.4764289855957031,7.753368342147057e-07
2088,6610,0,6610,0.4770359992980957,7.568577956673808e-07
2090,6616,0,6616,0.4774470329284668,7.417404232224183e-07
2092,6622,0,6622,0.47784900665283203,7.24866274995817e-07
2094,6628,0,6628,0.4782528877258301,7.066342104972851e-07
2096,6634,0,6634,0.47866010665893555,6.899245312368914e-07
2099,6643,0,6643,0.479266881942749,6.745133255984736e-07
2101,6649,0,6649,0.47967004776000977,6.684811292709167e-07
2103,6655,0,6655,0.4800739288330078,6.629273392297042e-07
2105,6661,0,6661,0.4804809093475342,6.564891308354825e-07
2108,6670,0,6670,0.48108696937561035,6.424264638827556e-07
2110,6676,0,6676,0.4814918041229248,6.287856888299277e-07
2112,6682,0,6682,0.48189592361450195,6.126406646356966e-07
2114,6688,0,6688,0.4823019504547119,5.948985792743869e-07
2117,6697,0,6697,0.4829108715057373,5.692538276314373e-07
2119,6703,0,6703,0.48331212997436523,5.57243674294541e-07
2121,6709,0,6709,0.4837150573730469,5.497807543873073e-07
2123,6715,0,6715,0.48412108421325684,5.444018263839964e-07
2125,6721,0,6721,0.48452281951904297,5.386751308735539e-07
2128,6730,0,6730,0.4851360321044922,5.251632111770311e-07
2130,6736,0,6736,0.48554110527038574,5.135729948036206e-07
2132,6742,0,6742,0.4859480857849121,5.022690404946138e-07
2134,6748,0,6748,0.48635005950927734,4.908702636601856e-07
2137,6757,0,6757,0.4869558811187744,4.717290288789441e-07
2139,6763,0,6763,0.4873619079589844,4.6296373596408433e-07
2141,6769,0,6769,0.4877748489379883,4.595552974928987e-07
2143,6775,0,6775,0.4881770610809326,4.579169912486697e-07
2145,6781,0,6781,0.48858213424682617,4.5654114979161346e-07
2148,6792,0,6792,0.489224910736084,4.5379042778055214e-07
2150,6800,0,6800,0.4896690845489502,4.5146103577810145e-07
2152,6806,0,6806,0.49007201194763184,4.4467386348811894e-07
2154,6812,0,6812,0.4904770851135254,4.3514312120271696e-07
2157,6821,0,6821,0.4910850524902344,4.214231888580186e-07
2159,6827,0,6827,0.49149489402770996,4.099210360843654e-07
2161,6833,0,6833,0.4918971061706543,3.9714466600851936e-07
2163,6839,0,6839,0.4923539161682129,3.8550092923572444e-07
2165,6846,0,6846,0.4927799701690674,3.836021822010396e-07
2168,6855,0,6855,0.4933931827545166,3.8056127134495853e-07
2170,6861,0,6861,0.49379801750183105,3.771949168303902e-07
2172,6867,0,6867,0.4942047595977783,3.730846650311065e-07
2174,6873,0,6873,0.4946119785308838,3.6890055110766584e-07
2177,6882,0,6882,0.4952239990234375,3.6501798563296196e-07
2179,6889,0,6889,0.49564695358276367,3.6439489254979305e-07
2181,6895,0,6895,0.49605298042297363,3.617266437388464e-07
2183,6901,0,6901,0.4964599609375,3.536994912360176e-07
2185,6907,0,6907,0.49686384201049805,3.451812832689304e-07
2188,6916,0,6916,0.49747180938720703,3.3296442285415076e-07
2190,6922,0,6922,0.497877836227417,3.256077488236055e-07
2192,6928,0,6928,0.4982919692993164,3.187117297497461e-07
2194,6934,0,6934,0.49869418144226074,3.1227645664948935e-07
2197,6943,0,6943,0.4993021488189697,3.042769669121999e-07
2199,6949,0,6949,0.4997081756591797,3.0014297709376113e-07
2201,6955,0,6955,0.500114917755127,2.966394122606015e-07
2203,6961,0,6961,0.5005171298980713,2.9362088231916977e-07
2205,6967,0,6967,0.5009210109710693,2.921326576985045e-07
2208,6978,0,6978,0.5015678405761719,2.8707000650015454e-07
2210,6985,0,6985,0.5019938945770264,2.860488136437498e-07
2212,6992,0,6992,0.5024161338806152,2.845360745687516e-07
2214,6998,0,6998,0.5028221607208252,2.8053058930582453e-07
2217,7005,0,7005,0.5033960342407227,1.5120112999847873e-07
2219,7009,0,7009,0.5037648677825928,3.457127791943085e-08
2221,7013,0,7013,0.5041310787200928,9.194847961703968e-09


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha0/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.001844167709350586,30.358099469249375
200,201,200,401,0.2851991653442383,1.7006076310549407
400,401,400,801,0.577491044998169,0.9112475403461391
601,602,601,1203,0.8584110736846924,0.6722636706984941
801,802,801,1603,1.160689115524292,0.5549897589038558
1001,1002,1001,2003,1.4554681777954102,0.4774627272054353
1201,1202,1201,2403,1.7318952083587646,0.5020323359805887
1401,1402,1401,2803,2.0084621906280518,0.38067029692333876
1602,1603,1602,3205,2.362065076828003,0.3601892103963759
1802,1803,1802,3605,2.6659011840820312,0.31710086376541813
2002,2003,2002,4005,2.9439010620117188,0.29347919987041415
2202,2203,2202,4405,3.225637197494507,0.27406544712310116
2402,2403,2402,4805,3.5074520111083984,0.2553087833982936
2603,2604,2603,5207,3.7808001041412354,0.28020453691043595
2803,2804,2803,5607,4.054150104522705,0.2712535221053058
3003,3004,3003,6007,4.3579301834106445,0.21318155887917348
3203,3204,3203,6407,4.643322944641113,0.2016132207213287
3403,3404,3403,6807,4.939672231674194,0.19222972981543524
3604,3605,3604,7209,5.267271995544434,0.19720315810070332
3804,3805,3804,7609,5.592290163040161,0.2103584348564755
4004,4005,4004,8009,5.8855061531066895,0.16723134771200343
4204,4205,4204,8409,6.151831150054932,0.16097492421107829
4404,4405,4404,8809,6.322810888290405,0.18559891251431232
4605,4606,4605,9211,6.495526075363159,0.14796662382591377
4805,4806,4805,9611,6.665279150009155,0.14277715729873722
5005,5006,5005,10011,6.83432412147522,0.13693486384378642
5205,5206,5205,10411,7.011662244796753,0.13321751244473776
5405,5406,5405,10811,7.192115068435669,0.12989757235492205
5606,5607,5606,11213,7.396651029586792,0.12372810737229124
5806,5807,5806,11613,7.583511114120483,0.12029605282208732
6006,6007,6006,12013,7.757652044296265,0.11637741263661482
6206,6207,6206,12413,7.934596300125122,0.11304469291731661
6406,6407,6406,12813,8.106170892715454,0.10838983801664176
6607,6608,6607,13215,8.2726469039917,0.10869187317633078
6807,6808,6807,13615,8.456902980804443,0.10290095462612837
7007,7008,7007,14015,8.643841028213501,0.10040248709864004
7207,7208,7207,14415,8.819017171859741,0.09730251506941644
7407,7408,7407,14815,8.987826108932495,0.11108634162819774
7608,7609,7608,15217,9.16200304031372,0.09224893113525348
7808,7809,7808,15617,9.333218097686768,0.08916263693421927
8008,8009,8008,16017,9.512444972991943,0.08742133097297906
8208,8209,8208,16417,9.697824001312256,0.08516906645897578
8408,8409,8408,16817,9.875104188919067,0.0837398182167758
8609,8610,8609,17219,10.070091009140015,0.08038455606222403
8809,8810,8809,17619,10.244209051132202,0.08033410025209158
9009,9010,9009,18019,10.44275712966919,0.07712365252907863
9209,9210,9209,18419,10.710820198059082,0.07546326483973753
9409,9410,9409,18819,10.984771251678467,0.07648345218889664
9610,9611,9610,19221,11.175579071044922,0.07224063238108902
9810,9811,9810,19621,11.43315315246582,0.07113843989150681
10010,10011,10010,20021,11.618467092514038,0.0695586428950319
10210,10211,10210,20421,11.824803113937378,0.08356522464504641
10410,10411,10410,20821,11.981074094772339,0.06712960112109609
10611,10612,10611,21223,12.157926082611084,0.06699359466531633
10811,10812,10811,21623,12.329273223876953,0.06541908874086734
11011,11012,11011,22023,12.506890058517456,0.06382542624128312
11211,11212,11211,22423,12.720428228378296,0.06269648293635686
11411,11412,11411,22823,12.893160104751587,0.0610488090686334
11612,11613,11612,23225,13.046871185302734,0.06338505860176886
11812,11813,11812,23625,13.230136156082153,0.059617103548654356
12012,12013,12012,24025,13.492700099945068,0.05916471716834446
12212,12213,12212,24425,13.692963123321533,0.05832033721416688
12412,12413,12412,24825,13.901644229888916,0.05722802924727787
12613,12614,12613,25227,14.119035959243774,0.05642084573567756
12813,12814,12813,25627,14.306643962860107,0.054970058700584315
13013,13014,13013,26027,14.482401132583618,0.054362710210040736
13213,13214,13213,26427,14.647200107574463,0.0548684809923365
13413,13414,13413,26827,14.816962242126465,0.05329343776503196
13614,13615,13614,27229,14.97458004951477,0.05206264518775205
13814,13815,13814,27629,15.134797096252441,0.053576796645504174
14014,14015,14014,28029,15.307538986206055,0.05143273277248047
14214,14215,14214,28429,15.548218250274658,0.05057808402386697
14414,14415,14414,28829,15.781007289886475,0.05019351604690433
14615,14616,14615,29231,15.967069149017334,0.04907278752747184
14815,14816,14815,29631,16.17525315284729,0.048963949757096954
15015,15016,15015,30031,16.338297128677368,0.048334930520042445
15215,15216,15215,30431,16.545838117599487,0.048956526721502566
15415,15416,15415,30831,16.7501802444458,0.047105109130263494
15616,15617,15616,31233,16.930963039398193,0.04638475401498077
15816,15817,15816,31633,17.100152254104614,0.046620882576732955
16016,16017,16016,32033,17.25538206100464,0.05262818931815664
16216,16217,16216,32433,17.43974995613098,0.04542925345577664
16416,16417,16416,32833,17.680570125579834,0.04522861502190292
16617,16618,16617,33235,17.868226051330566,0.04477520875790979
16817,16818,16817,33635,18.084577083587646,0.04414845185933609
17017,17018,17017,34035,18.289923191070557,0.04366503516601011
17217,17218,17217,34435,18.475831031799316,0.05022539783196252
17417,17418,17417,34835,18.75199604034424,0.04291044853519493
17618,17619,17618,35237,18.93560004234314,0.050873035055087924
17818,17819,17818,35637,19.118653059005737,0.042273969493643954
18018,18019,18018,36037,19.299345016479492,0.05036172028208931
18218,18219,18218,36437,19.47788405418396,0.0415931367633282
18418,18419,18418,36837,19.644554138183594,0.041214840415818035
18619,18620,18619,37239,19.99181318283081,0.04105012665697059
18819,18820,18819,37639,20.18104100227356,0.040860701696957664
19019,19020,19019,38039,20.367293119430542,0.04054281334698695
19219,19220,19219,38439,20.562137126922607,0.039865432952396716
19419,19420,19419,38839,20.87711215019226,0.041147997577064256
19620,19621,19620,39241,21.062576055526733,0.03953747525468505
19820,19821,19820,39641,21.21853494644165,0.03928764681896595
20020,20021,20020,40041,21.394946098327637,0.039082868496820244
20220,20221,20220,40441,21.57203221321106,0.038372768630625304
20420,20421,20420,40841,21.765656232833862,0.037848285778436665
20621,20622,20621,41243,21.937342166900635,0.0417872609059276
20821,20822,20821,41643,22.089575052261353,0.0440074007147347
21021,21022,21021,42043,22.23697805404663,0.03720117020720569
21221,21222,21221,42443,22.4046630859375,0.037688310088188966
21421,21422,21421,42843,22.566400051116943,0.037064899274681075
21622,21623,21622,43245,22.73022699356079,0.037828882228458954
21822,21823,21822,43645,22.931102991104126,0.03677659783669953
22022,22023,22022,44045,23.089967966079712,0.036256182283724556
22222,22223,22222,44445,23.24852204322815,0.03605278245410219
22422,22423,22422,44845,23.404009103775024,0.03598327331237605
22623,22624,22623,45247,23.55874013900757,0.03582717489272665
22823,22824,22823,45647,23.71844792366028,0.043552763093730934
23023,23024,23023,46047,23.880587100982666,0.03500075753036403
23223,23224,23223,46447,24.030436277389526,0.03600642543410127
23423,23424,23423,46847,24.180236101150513,0.03478625972020386
23624,23625,23624,47249,24.332945108413696,0.03488851327720817
23824,23825,23824,47649,24.488089084625244,0.03423711214273072
24024,24025,24024,48049,24.637041091918945,0.03674296420485604
24224,24225,24224,48449,24.799724102020264,0.03412610626459489
24424,24425,24424,48849,24.947165966033936,0.033909140887717654
24625,24626,24625,49251,25.093940019607544,0.03451988308521902
24825,24826,24825,49651,25.251464128494263,0.033948871860907406
25025,25026,25025,50051,25.402979135513306,0.035017848233246836
25225,25226,25225,50451,25.550644159317017,0.03318125025514594
25425,25426,25425,50851,25.69998002052307,0.03308171332205296
25626,25627,25626,51253,25.860636949539185,0.03963620655534278
25826,25827,25826,51653,26.023864269256592,0.03273167493828358
26026,26027,26026,52053,26.183945178985596,0.03273585001029364
26226,26227,26226,52453,26.35003399848938,0.032675332145086236
26426,26427,26426,52853,26.498319149017334,0.032145549115602634
26627,26628,26627,53255,26.651177167892456,0.03203332764990996
26827,26828,26827,53655,26.79727005958557,0.0328141190120363
27027,27028,27027,54055,26.964818954467773,0.03148669957668568
27227,27228,27227,54455,27.11321496963501,0.03821585156448793
27427,27428,27427,54855,27.26255226135254,0.0317038601867372
27628,27629,27628,55257,27.412743091583252,0.03770103610817365
27828,27829,27828,55657,27.558813095092773,0.03107237971700072
28028,28029,28028,56057,27.70581889152527,0.03570891221649926
28228,28229,28228,56457,27.852468013763428,0.031050893488329137
28428,28429,28428,56857,28.00010395050049,0.03099444372477587
28629,28630,28629,57259,28.149030923843384,0.030838816080487313
28829,28830,28829,57659,28.30271005630493,0.03233791651087027
29029,29030,29029,58059,28.467103004455566,0.03542717355646013
29229,29230,29229,58459,28.619551181793213,0.030906676631839124
29429,29430,29429,58859,28.7793390750885,0.030012110790273033
29630,29631,29630,59261,28.95788598060608,0.02983795404344887
29830,29831,29830,59661,29.296247243881226,0.03002670501725421
30030,30031,30030,60061,29.462156057357788,0.029877584039166336
30230,30231,30230,60461,29.63775610923767,0.029568724461103122
30430,30431,30430,60861,29.79379630088806,0.029446427484848898
30631,30632,30631,61263,30.14092707633972,0.02960108497503998
30831,30832,30831,61663,30.308423042297363,0.02905262187562605
31031,31032,31031,62063,30.480440139770508,0.02935833510871864
31231,31232,31231,62463,30.648314952850342,0.0287323953572807
31431,31432,31431,62863,30.822739124298096,0.03100684020902864
31632,31633,31632,63265,30.994270086288452,0.036130863198687704
31832,31833,31832,63665,31.186662912368774,0.03276044561251601
32032,32033,32032,64065,31.36992907524109,0.02941969145489503
32232,32233,32232,64465,31.538377046585083,0.02865252850439644
32432,32433,32432,64865,31.698933124542236,0.02837826018780118
32633,32634,32633,65267,31.86293625831604,0.027867617645529086
32833,32834,32833,65667,32.019264221191406,0.027769006098614483
33033,33034,33033,66067,32.172280073165894,0.027802387375615325
33233,33234,33233,66467,32.33020496368408,0.027692946691787356
33433,33434,33433,66867,32.4995059967041,0.027662822831694623
33634,33635,33634,67269,32.65508413314819,0.029642741706556484
33834,33835,33834,67669,32.813727140426636,0.028898904604688
34034,34035,34034,68069,32.96840190887451,0.0273998198180117
34234,34235,34234,68469,33.16621494293213,0.027348110178125495
34434,34435,34434,68869,33.34608221054077,0.02757111093417047
34635,34636,34635,69271,33.53239297866821,0.02704868541709397
34835,34836,34835,69671,33.710554122924805,0.03455088309289085
35035,35036,35035,70071,33.868221044540405,0.027455113972297614
35235,35236,35235,70471,34.02952718734741,0.02679496865805395
35435,35436,35435,70871,34.20826292037964,0.026701251785294
35636,35637,35636,71273,34.3732750415802,0.026466017926516903
35836,35837,35836,71673,34.53052020072937,0.026475250676945464
36036,36037,36036,72073,34.692973136901855,0.02649334857511161
36236,36237,36236,72473,34.852459192276,0.03260106435085443
36436,36437,36436,72873,35.011834144592285,0.026185302707113816
36637,36638,36637,73275,35.167394161224365,0.03225827264464111
36837,36838,36837,73675,35.335456132888794,0.026713128013641754
37037,37038,37037,74075,35.499940156936646,0.025933681473449245
37237,37238,37237,74475,35.674575328826904,0.026280173564904637
37437,37438,37437,74875,35.834861278533936,0.026168925420021024
37638,37639,37638,75277,35.99336814880371,0.025873610471282373
37838,37839,37838,75677,36.15904712677002,0.025542900344546027
38038,38039,38038,76077,36.31306290626526,0.026901081786780405
38238,38239,38238,76477,36.47179126739502,0.02529367335097412
38438,38439,38438,76877,36.6367130279541,0.027811866616852258
38639,38640,38639,77279,36.79652523994446,0.02527610598335215
38839,38840,38839,77679,36.960472106933594,0.025112990050991022
39039,39040,39039,78079,37.118128061294556,0.025418283680628203
39239,39240,39239,78479,37.28821897506714,0.024842956112366452
39439,39440,39439,78879,37.46559023857117,0.024939275762930098
39640,39641,39640,79281,37.61996817588806,0.024679147976757108
39840,39841,39840,79681,37.78778028488159,0.024681939625606802
40040,40041,40040,80081,37.96039915084839,0.02453795649116443
40240,40241,40240,80481,38.113255977630615,0.024637858555959218
40440,40441,40440,80881,38.26786422729492,0.024564388137275867
40641,40642,40641,81283,38.433757066726685,0.024646483011776986
40841,40842,40841,81683,38.588685274124146,0.024343314299402934
41041,41042,41041,82083,38.74656796455383,0.024251251468409746
41241,41242,41241,82483,38.94645619392395,0.029778130230561847
41441,41442,41441,82883,39.113935232162476,0.02404858714789033
41642,41643,41642,83285,39.27952313423157,0.023936760149282973
41842,41843,41842,83685,39.44606614112854,0.023944416200273703
42042,42043,42042,84085,39.610913038253784,0.023857891869585666
42242,42243,42242,84485,39.76405215263367,0.023874148271617483
42442,42443,42442,84885,39.93184518814087,0.023673734320089707
42643,42644,42643,85287,40.09764623641968,0.023626542539040694
42843,42844,42843,85687,40.252846240997314,0.028651624481657253
43043,43044,43043,86087,40.41276288032532,0.024015123769717952
43243,43244,43243,86487,40.576266050338745,0.02336243383948069
43443,43444,43443,86887,40.73420214653015,0.024508151923644337
43644,43645,43644,87289,40.89054322242737,0.025821325081299265
43844,43845,43844,87689,41.04297614097595,0.023114918596386345
44044,44045,44044,88089,41.20749497413635,0.024528665166417437
44244,44245,44244,88489,41.38906717300415,0.02353646832250001
44444,44445,44444,88889,41.56316113471985,0.02683007715324352
44645,44646,44645,89291,41.72140407562256,0.022905011963139123
44845,44846,44845,89691,41.89132905006409,0.0229479074901674
45045,45046,45045,90091,42.05903506278992,0.022804216155202665
45245,45246,45245,90491,42.23222303390503,0.022675173858634972
45445,45446,45445,90891,42.3913791179657,0.02281835815649117
45646,45647,45646,91293,42.553232192993164,0.02702895904664809
45846,45847,45846,91693,42.70930099487305,0.02256611067697314
46046,46047,46046,92093,42.867419958114624,0.02253197646145024
46246,46247,46246,92493,43.02800798416138,0.0223876499582941
46446,46447,46446,92893,43.19117021560669,0.022171655137270877
46647,46648,46647,93295,43.35110831260681,0.02240833401221567
46847,46848,46847,93695,43.50679111480713,0.022475442667686352
47047,47048,47047,94095,43.6828351020813,0.023773869475390907
47247,47248,47247,94495,43.85932111740112,0.02209162976826666
47447,47448,47447,94895,44.02738308906555,0.022209668720491547
47648,47649,47648,95297,44.20462489128113,0.02250901754905959
47848,47849,47848,95697,44.401094913482666,0.02347167747305269
48048,48049,48048,96097,44.569735050201416,0.021798083184909906
48248,48249,48248,96497,44.73832607269287,0.021860920850733427
48448,48449,48448,96897,44.898242235183716,0.02401069985665101
48649,48650,48649,97299,45.066620111465454,0.02286475559973605
48849,48850,48849,97699,45.26936197280884,0.02233249972215759
49049,49050,49049,98099,45.43558216094971,0.021449405460546286
49249,49250,49249,98499,45.608941078186035,0.022382096814697567
49449,49450,49449,98899,45.76765513420105,0.021516750705197374
49650,49651,49650,99301,45.928842067718506,0.025116030600778924
49850,49851,49850,99701,46.09264016151428,0.021271692750979173
50050,50051,50050,100101,46.26068615913391,0.021209808654068168
50250,50251,50250,100501,46.437785148620605,0.021752525197229484
50450,50451,50450,100901,46.61770009994507,0.02121452811459931
50651,50652,50651,101303,46.80190706253052,0.022474661873852022
50851,50852,50851,101703,46.96491026878357,0.021015955741441588
51051,51052,51051,102103,47.121554136276245,0.023769733002408686
51251,51252,51251,102503,47.286362171173096,0.02291967204938169
51451,51452,51451,102903,47.450494050979614,0.020704511991813297
51652,51653,51652,103305,47.620129108428955,0.02419938209364002
51852,51853,51852,103705,47.789243936538696,0.020749231223402338
52052,52053,52052,104105,47.94547724723816,0.020620607487106726
52252,52253,52252,104505,48.104389905929565,0.020685232419967715
52452,52453,52452,104905,48.262266874313354,0.02036558902563882
52653,52654,52653,105307,48.42462921142578,0.02385088395788482
52853,52854,52853,105707,48.58945417404175,0.020380497047840417
53053,53054,53053,106107,48.756229877471924,0.020337753261422117
53253,53254,53253,106507,48.91973519325256,0.02037664961961324
53453,53454,53453,106907,49.07400703430176,0.020153234964276942
53654,53655,53654,107309,49.25905513763428,0.02647976427329628
53854,53855,53854,107709,49.435271978378296,0.02005722577664801
54054,54055,54054,108109,49.59849190711975,0.020939319830561628
54254,54255,54254,108509,49.78145909309387,0.023854784552125835
54454,54455,54454,108909,49.963935136795044,0.026030499919749883
54655,54656,54655,109311,50.12958121299744,0.020137258994200286
54855,54856,54855,109711,50.39729309082031,0.019906949434133063
55055,55056,55055,110111,50.653836250305176,0.020651124853902584
55255,55256,55255,110511,50.845322132110596,0.019743967917853808
55455,55456,55455,110911,51.005635261535645,0.01962907046913023
55656,55657,55656,111313,51.27200698852539,0.019686220167973903
55856,55857,55856,111713,51.54802417755127,0.019835038598160565
56056,56057,56056,112113,51.72602200508118,0.02232944666929513
56256,56257,56256,112513,51.90032911300659,0.02449304798569066
56456,56457,56456,112913,52.06549906730652,0.019544674350759666
56657,56658,56657,113315,52.2436101436615,0.022574039594402056
56857,56858,56857,113715,52.46863412857056,0.025443530471573023
57057,57058,57057,114115,52.6318621635437,0.019532458163327097
57257,57258,57257,114515,52.79422402381897,0.019342589503502292
57457,57458,57457,114915,52.969149112701416,0.019185174342042918
57658,57659,57658,115317,53.125731229782104,0.019642762255055804
57858,57859,57858,115717,53.342159271240234,0.019079140699214448
58058,58059,58058,116117,53.50138211250305,0.019778510502601005
58258,58259,58258,116517,53.657984018325806,0.01904550931838963
58458,58459,58458,116917,53.81569790840149,0.018888037010169143
58659,58660,58659,117319,53.97003412246704,0.019111321632237926
58859,58860,58859,117719,54.160094022750854,0.018797653314417406
59059,59060,59059,118119,54.31679105758667,0.018843779869422282
59259,59260,59259,118519,54.487590074539185,0.018962402368365158
59459,59460,59459,118919,54.654824018478394,0.01873021573800568
59660,59661,59660,119321,54.82715392112732,0.01871236731439782
59860,59861,59860,119721,55.001466274261475,0.01857267369771664
60060,60061,60060,120121,55.182852268218994,0.01869513943251916
60260,60261,60260,120521,55.34235596656799,0.01865413526086257
60460,60461,60460,120921,55.49633312225342,0.018638327632046432
60661,60662,60661,121323,55.651650190353394,0.02231588678328095
60861,60862,60861,121723,55.804584980010986,0.02104283740568213
61061,61062,61061,122123,55.95757603645325,0.018475950787447168
61261,61262,61261,122523,56.12515211105347,0.018260331725082096
61461,61462,61461,122923,56.29006600379944,0.018424995083053366
61662,61663,61662,123325,56.461634159088135,0.018876204568625387
61862,61863,61862,123725,56.63386607170105,0.01866103394447662
62062,62063,62062,124125,56.80203413963318,0.01833644348252372
62262,62263,62262,124525,56.976911306381226,0.0213161455823791
62462,62463,62462,124925,57.14120602607727,0.02070763618452015
62663,62664,62663,125327,57.3275671005249,0.01801016338788049
62863,62864,62863,125727,57.48940920829773,0.018054005118934183
63063,63064,63063,126127,57.66951513290405,0.01798840849718121
63263,63264,63263,126527,57.84148907661438,0.017820226732605533
63463,63464,63463,126927,58.01320195198059,0.01779550692084509
63664,63665,63664,127329,58.179445028305054,0.017782639732657514
63864,63865,63864,127729,58.350992918014526,0.017795251845324548
64064,64065,64064,128129,58.52941393852234,0.017756334387927248
64264,64265,64264,128529,58.70512795448303,0.017764820182898593
64464,64465,64464,128929,58.91061305999756,0.01767726363769154
64665,64666,64665,129331,59.08381509780884,0.017738505179523894
64865,64866,64865,129731,59.26322913169861,0.01761638975979145
65065,65066,65065,130131,59.45043897628784,0.01797363001266876
65265,65266,65265,130531,59.64099097251892,0.017509799105258204
65465,65466,65465,130931,59.807170152664185,0.017735527388250297
65666,65667,65666,131333,59.98029398918152,0.017379579131193697
65866,65867,65866,131733,60.159669160842896,0.020775241916047654
66066,66067,66066,132133,60.365663051605225,0.021010676567899445
66266,66267,66266,132533,60.55058217048645,0.017334945756246292
66466,66467,66466,132933,60.74827814102173,0.017581446497327086
66667,66668,66667,133335,60.931233167648315,0.02167995598050261
66867,66868,66867,133735,61.166582107543945,0.02122824707557788
67067,67068,67067,134135,61.65830421447754,0.021045458999272938
67267,67268,67267,134535,62.01579189300537,0.017120857847974562
67467,67468,67467,134935,62.27533006668091,0.01688494029381745
67668,67669,67668,135337,62.54130411148071,0.017113718156470465
67868,67869,67868,135737,62.88318920135498,0.016938066044104343
68068,68069,68068,136137,63.16043496131897,0.01708432853341526
68268,68269,68268,136537,63.45049810409546,0.017619598866044493
68468,68469,68468,136937,63.77875995635986,0.017283423762900443
68669,68670,68669,137339,63.97320508956909,0.016643225541608415
68869,68870,68869,137739,64.14732599258423,0.01712715654615588
69069,69070,69069,138139,64.31622409820557,0.01674216501722384
69269,69270,69269,138539,64.54295825958252,0.017426292984704477
69469,69470,69469,138939,64.76776099205017,0.016674579547756394
69670,69671,69670,139341,64.98439311981201,0.019094980375710672
69870,69871,69870,139741,65.23566603660583,0.01658978912873495
70070,70071,70070,140141,65.41444802284241,0.01940435689998246
70270,70271,70270,140541,65.712886095047,0.01665513736190024
70470,70471,70470,140941,65.97577500343323,0.01688376707959082
70671,70672,70671,141343,66.43873620033264,0.016320442559690375
70871,70872,70871,141743,66.68082904815674,0.016399467673715834
71071,71072,71071,142143,66.95831727981567,0.016471362974706832
71271,71272,71271,142543,67.1759901046753,0.016433871311475223
71471,71472,71471,142943,67.43805718421936,0.016304276678523445
71672,71673,71672,143345,67.72649312019348,0.019649387069779405
71872,71873,71872,143745,68.04476714134216,0.016398928867124754
72072,72073,72072,144145,68.36678814888,0.016689615710762603
72272,72273,72272,144545,68.66198921203613,0.01626152835150862
72472,72473,72472,144945,68.9229531288147,0.016314873087065553
72673,72674,72673,145347,69.1053261756897,0.016064256846091165
72873,72874,72873,145747,69.278391122818,0.015983598218756397
73073,73074,73073,146147,69.44797015190125,0.016163364390018354
73273,73274,73273,146547,69.61229801177979,0.01589741843035557
73473,73474,73473,146947,69.77325391769409,0.018704429118366398
73674,73675,73674,147349,69.93091416358948,0.015973272358369855
73874,73875,73874,147749,70.08483004570007,0.015767418260967368
74074,74075,74074,148149,70.23963022232056,0.020060074499005636
74274,74275,74274,148549,70.44899892807007,0.016370083701280475
74474,74475,74474,148949,70.61257100105286,0.015777972849633955
74675,74676,74675,149351,70.76955819129944,0.015673695217123956
74875,74876,74875,149751,70.94456911087036,0.015640090486248235
75075,75076,75075,150151,71.1252920627594,0.015483802438880975
75275,75276,75275,150551,71.29362797737122,0.015875083453601585
75475,75476,75475,150951,71.46879410743713,0.015679891930946724
75676,75677,75676,151353,71.65364098548889,0.015522018411993422
75876,75877,75876,151753,71.88973593711853,0.015515651350156593
76076,76077,76076,152153,72.0450210571289,0.019172175237301647
76276,76277,76276,152553,72.23739814758301,0.01826605117673208
76476,76477,76476,152953,72.41101312637329,0.015489420008557424
76677,76678,76677,153355,72.59922003746033,0.015448653248781079
76877,76878,76877,153755,72.85920214653015,0.015814187188726715
77077,77078,77077,154155,73.02126502990723,0.015253022554040093
77277,77278,77277,154555,73.22256326675415,0.015351540344436334
77477,77478,77477,154955,73.4369249343872,0.0151819946812419
77678,77679,77678,155357,73.60286903381348,0.015317884406705954
77878,77879,77878,155757,73.80817794799805,0.015134925866145022
78078,78079,78078,156157,73.96428513526917,0.017530072381278024
78278,78279,78278,156557,74.1235830783844,0.015477372807974331
78478,78479,78478,156957,74.28442120552063,0.015039927269619837
78679,78680,78679,157359,74.47032809257507,0.015109615762249763
78879,78880,78879,157759,74.64352011680603,0.014961004491263452
79079,79080,79079,158159,74.82810020446777,0.015056746747331054
79279,79280,79279,158559,74.98655009269714,0.014964839789269732
79479,79480,79479,158959,75.14147210121155,0.014861883892788995
79680,79681,79680,159361,75.30649018287659,0.014801881607957345
79880,79881,79880,159761,75.49155521392822,0.014780407867536954
80080,80081,80080,160161,75.65598320960999,0.015277406221414718
80280,80281,80280,160561,75.82381319999695,0.014946267435902291
80480,80481,80480,160961,75.99496507644653,0.014762584548580404
80681,80682,80681,161363,76.16782808303833,0.014737401786930338
80881,80882,80881,161763,76.3424642086029,0.01776307821247424
81081,81082,81081,162163,76.54346299171448,0.014527391654567222
81281,81282,81281,162563,76.71522521972656,0.014727045506573725
81481,81482,81481,162963,76.89745593070984,0.014577351903278255
81682,81683,81682,163365,77.11399817466736,0.014530843011670408
81882,81883,81882,163765,77.28544807434082,0.016861974400582166
82082,82083,82082,164165,77.51314210891724,0.017448226895021526
82282,82283,82282,164565,77.7246081829071,0.014507704448627073
82482,82483,82482,164965,77.88075923919678,0.01451273587397952
82683,82684,82683,165367,78.03357696533203,0.014654598454277627
82883,82884,82883,165767,78.18770003318787,0.0143743086721234
83083,83084,83083,166167,78.34507298469543,0.015190555983361597
83283,83284,83283,166567,78.51148915290833,0.014502384635867269
83483,83484,83483,166967,78.66636800765991,0.014388363138483762
83684,83685,83684,167369,78.82557797431946,0.014360835325272001
83884,83885,83884,167769,79.00286912918091,0.014128426308329552
84084,84085,84084,168169,79.24603605270386,0.014569264888521229
84284,84285,84284,168569,79.42584204673767,0.01616922222725642
84484,84485,84484,168969,79.59760308265686,0.01614332442623157
84685,84686,84685,169371,79.78957390785217,0.014052079513497547
84885,84886,84885,169771,79.95601511001587,0.013962891821019495
85085,85086,85085,170171,80.11181592941284,0.01409555681863181
85285,85286,85285,170571,80.27587795257568,0.013989605992560775
85485,85486,85485,170971,80.46664023399353,0.013975667909497657
85686,85687,85686,171373,80.62461709976196,0.014005264703599885
85886,85887,85886,171773,80.85659408569336,0.01403419892016429
86086,86087,86086,172173,81.05438017845154,0.016684594913685312
86286,86287,86286,172573,81.24004793167114,0.01633826623829239
86486,86487,86486,172973,81.43570303916931,0.016009238985131246
86687,86688,86687,173375,81.61119222640991,0.013898220722144436
86887,86888,86887,173775,81.7781331539154,0.01373810605151921
87087,87088,87087,174175,81.96766400337219,0.013688031395969882
87287,87288,87287,174575,82.19451308250427,0.013800703593006789
87487,87488,87487,174975,82.49215817451477,0.017238578339612683
87688,87689,87688,175377,82.87341809272766,0.013838126249453792
87888,87889,87888,175777,83.19113612174988,0.014610040441163525
88088,88089,88088,176177,83.49578022956848,0.013623594225415748
88288,88289,88288,176577,83.92312407493591,0.013463979960098675
88488,88489,88488,176977,84.36211109161377,0.013666142183179486
88689,88690,88689,177379,84.54315114021301,0.018056632896177982
88889,88890,88889,177779,84.71224093437195,0.013477819521355978
89089,89090,89089,178179,84.89849519729614,0.013565873804621062
89289,89290,89289,178579,85.06662917137146,0.013771769111185793
89489,89490,89489,178979,85.23775601387024,0.01560142996861236
89690,89691,89690,179381,85.5614161491394,0.014902749190971901
89890,89891,89890,179781,85.90626692771912,0.01449821618415836
90090,90091,90090,180181,86.16370797157288,0.013323560697736606
90290,90291,90290,180581,86.34986019134521,0.013287802968408403
90490,90491,90490,180981,86.5174651145935,0.013348869958275358
90691,90692,90691,181383,86.68945121765137,0.013462366228382512
90891,90892,90891,181783,86.8718810081482,0.01317371919729869
91091,91092,91091,182183,87.08196711540222,0.013162862847947645
91291,91292,91291,182583,87.29442310333252,0.013186399768884544
91491,91492,91491,182983,87.58738708496094,0.013356652253427402
91692,91693,91692,183385,87.88721513748169,0.013269390982329522
91892,91893,91892,183785,88.1641161441803,0.01309773135345503
92092,92093,92092,184185,88.34913206100464,0.013040785837659438
92292,92293,92292,184585,88.5307149887085,0.01317509872828938
92492,92493,92492,184985,88.7042281627655,0.012973998902944013
92693,92694,92693,185387,88.87675404548645,0.013066655973427542
92893,92894,92893,185787,89.07757496833801,0.01599176563798967
93093,93094,93093,186187,89.24930810928345,0.01611260530946527
93293,93294,93293,186587,89.444491147995,0.013263634459388551
93493,93494,93493,186987,89.66110610961914,0.012910015218854362
93694,93695,93694,187389,89.88553023338318,0.012892110654134762
93894,93895,93894,187789,90.15001606941223,0.012805016898411934
94094,94095,94094,188189,90.39431500434875,0.01294249037623989
94294,94295,94294,188589,90.60737895965576,0.012853062092041376
94494,94495,94494,188989,90.79513025283813,0.012977144653887284
94695,94696,94695,189391,90.97147011756897,0.013615864220470883
94895,94896,94895,189791,91.14231204986572,0.014648405187975003
95095,95096,95095,190191,91.32156610488892,0.015122422648473263
95295,95296,95295,190591,91.55084919929504,0.012906162741433908
95495,95496,95495,190991,91.74350500106812,0.01253714644483266
95696,95697,95696,191393,91.934396982193,0.012542372764778507
95896,95897,95896,191793,92.11509418487549,0.012746681143910664
96096,96097,96096,192193,92.3457260131836,0.01500593553237307
96296,96297,96296,192593,92.5834641456604,0.015149575036105237
96496,96497,96496,192993,92.75543522834778,0.01253802064752151
96697,96698,96697,193395,92.98802018165588,0.012822815572050164
96897,96898,96897,193795,93.15899014472961,0.012448512944557366
97097,97098,97097,194195,93.45008707046509,0.012404846271103808
97297,97298,97297,194595,93.73636627197266,0.012453320208038618
97497,97498,97497,194995,94.12829399108887,0.012461469044157807
97698,97699,97698,195397,94.48360109329224,0.012464363325068567
97898,97899,97898,195797,94.81160092353821,0.014093359520775573
98098,98099,98098,196197,94.96662926673889,0.01230702634349713
98298,98299,98298,196597,95.13042616844177,0.012269606060666717
98498,98499,98498,196997,95.33817028999329,0.012447858347471684
98699,98700,98699,197399,95.56848120689392,0.012312789878963178
98899,98900,98899,197799,95.72678995132446,0.01484382909505566
99099,99100,99099,198199,95.89674806594849,0.014224649632781425
99299,99300,99299,198599,96.07069802284241,0.012739801233687011
99499,99500,99499,198999,96.23843312263489,0.012134554540379637
99700,99701,99700,199401,96.4112389087677,0.012129207971300047
99900,99901,99900,199801,96.60144114494324,0.012161898810025005
100100,100101,100100,200201,96.79954099655151,0.0121193003684653
100300,100301,100300,200601,96.96107602119446,0.012108584931694666
100501,100502,100501,201003,97.14908719062805,0.01226296230453011
100701,100702,100701,201403,97.31998324394226,0.012026353882558294
100901,100902,100901,201803,97.4936830997467,0.011928954369523594
101101,101102,101101,202203,97.66569805145264,0.012060841542286054
101301,101302,101301,202603,97.83322811126709,0.011942099863048576
101502,101503,101502,203005,98.00671005249023,0.0124207784897671
101702,101703,101702,203405,98.19018602371216,0.011898402978261799
101902,101903,101902,203805,98.3577013015747,0.01217679560229126
102102,102103,102102,204205,98.52115511894226,0.011923691221910093
102302,102303,102302,204605,98.69626712799072,0.011804164298204592
102503,102504,102503,205007,98.88022208213806,0.011864048179084121
102703,102704,102703,205407,99.10545420646667,0.011761085902131778
102903,102904,102903,205807,99.28431010246277,0.011796783610348685
103103,103104,103103,206207,99.44929814338684,0.011872744706361325
103303,103304,103303,206607,99.6044750213623,0.011738274771576523
103504,103505,103504,207009,99.76429390907288,0.011724298227730216
103704,103705,103704,207409,99.93293595314026,0.011783819376983336
103904,103905,103904,207809,100.1128261089325,0.011733144098683129
104104,104105,104104,208209,100.29088997840881,0.01156599305695431
104304,104305,104304,208609,100.44940400123596,0.011605719980288906
104505,104506,104505,209011,100.61313796043396,0.012269477592607674
104705,104706,104705,209411,100.77967429161072,0.011615696522021038
104905,104906,104905,209811,100.96220302581787,0.011553241392740422
105105,105106,105105,210211,101.14305710792542,0.011533835620288787
105305,105306,105305,210611,101.30050611495972,0.01141873101385327
105506,105507,105506,211013,101.45733094215393,0.011544690777160329
105706,105707,105706,211413,101.62643718719482,0.01143594574200608
105906,105907,105906,211813,101.97126412391663,0.011480819638767282
106106,106107,106106,212213,102.16689801216125,0.011534556464425133
106306,106307,106306,212613,102.33386611938477,0.012900737689425424
106507,106508,106507,213015,102.67515707015991,0.011453461218289569
106707,106708,106707,213415,102.94442510604858,0.011410266935850306
106907,106908,106907,213815,103.14092302322388,0.012307663368093405
107107,107108,107107,214215,103.47359418869019,0.011299804614484125
107307,107308,107307,214615,103.67681694030762,0.011241516619958694
107508,107509,107508,215017,103.86155200004578,0.011457745506642247
107708,107709,107708,215417,104.04869818687439,0.012850786765117254
107908,107909,107908,215817,104.31293797492981,0.01318978735044623
108108,108109,108108,216217,104.51949906349182,0.011114226369968885
108308,108309,108308,216617,104.71610307693481,0.011216965687980716
108509,108510,108509,217019,104.88501620292664,0.011136239485539047
108709,108710,108709,217419,105.05681800842285,0.011089214879086234
108909,108910,108909,217819,105.26723408699036,0.0110998353042323
109109,109110,109109,218219,105.44687223434448,0.011202638040689657
109309,109310,109309,218619,105.62309503555298,0.01120224479138858
109510,109511,109510,219021,105.82711625099182,0.014179646918289842
109710,109711,109710,219421,106.09799814224243,0.011059135309609688
109910,109911,109910,219821,106.33467411994934,0.010984270989838773
110110,110111,110110,220221,106.5794460773468,0.01113396497461948
110310,110311,110310,220621,106.84685015678406,0.011301166196161266
110511,110512,110511,221023,107.04477334022522,0.013068348318120359
110711,110712,110711,221423,107.23578190803528,0.0109529549472992
110911,110912,110911,221823,107.46753311157227,0.010954020400936345
111111,111112,111111,222223,107.68378496170044,0.01091904637318369
111311,111312,111311,222623,107.87938117980957,0.011930295123594142
111512,111513,111512,223025,108.07052230834961,0.010991543543120756
111712,111713,111712,223425,108.24532103538513,0.010832119404517261
111912,111913,111912,223825,108.42813229560852,0.010821556301069686
112112,112113,112112,224225,108.61408519744873,0.010733352932146221
112312,112313,112312,224625,108.78882789611816,0.010755916772452233
112513,112514,112513,225027,108.98272609710693,0.01077475462423997
112713,112714,112713,225427,109.18599605560303,0.010726716886486033
112913,112914,112913,225827,109.38346910476685,0.01233583025887605
113113,113114,113113,226227,109.56145906448364,0.012326617809664708
113313,113314,113313,226627,109.77358412742615,0.012900035430581946
113514,113515,113514,227029,110.02549624443054,0.010709826578274056
113714,113715,113714,227429,110.21614694595337,0.010671458032999397
113914,113915,113914,227829,110.53261208534241,0.010859132833548515
114114,114115,114114,228229,110.76699614524841,0.012151001131049659
114314,114315,114314,228629,110.94157814979553,0.010580114384676664
114515,114516,114515,229031,111.1259651184082,0.010613242005584559
114715,114716,114715,229431,111.42464900016785,0.010517361715251293
114915,114916,114915,229831,111.66485714912415,0.010528951674123937
115115,115116,115115,230231,111.86374521255493,0.01051952029493763
115315,115316,115315,230631,112.04085111618042,0.010438443981145344
115516,115517,115516,231033,112.21956729888916,0.010485303445909517
115716,115717,115716,231433,112.40061020851135,0.012250996620992874
115916,115917,115916,231833,112.5551381111145,0.01218725715728835
116116,116117,116116,232233,112.71813106536865,0.010894248462989971
116316,116317,116316,232633,112.8850450515747,0.01044560634174177
116517,116518,116517,233035,113.04864311218262,0.010277112609266937
116717,116718,116717,233435,113.21191310882568,0.010380238942528784
116917,116918,116917,233835,113.37716317176819,0.010343091760791874
117117,117118,117117,234235,113.53854489326477,0.010332286679512087
117317,117318,117317,234635,113.70879316329956,0.010908796523518354
117518,117519,117518,235037,113.88564991950989,0.01027808814539626
117718,117719,117718,235437,114.08132314682007,0.010313122285711475
117918,117919,117918,235837,114.23950815200806,0.010414445175561225
118118,118119,118118,236237,114.40172123908997,0.010142813708327396
118318,118319,118318,236637,114.63504528999329,0.010210946343839369
118519,118520,118519,237039,114.9100329875946,0.010166168063958704
118719,118720,118719,237439,115.16989612579346,0.010158630257559488
118919,118920,118919,237839,115.39216589927673,0.010107553520483875
119119,119120,119119,238239,115.54982113838196,0.010217808098701119
119319,119320,119319,238639,115.70612907409668,0.0100217351108536
119520,119521,119520,239041,115.87060213088989,0.011541666431427686
119720,119721,119720,239441,116.03916597366333,0.010117502632112462
119920,119921,119920,239841,116.20851111412048,0.009997556425028477
120120,120121,120120,240241,116.42821717262268,0.01005956840034649
120320,120321,120320,240641,116.6395161151886,0.010124386396884
120521,120522,120521,241043,116.9223141670227,0.010059213338274
120721,120722,120721,241443,117.1915352344513,0.009928436037329347
120921,120922,120921,241843,117.38760805130005,0.009998451725525236
121121,121122,121121,242243,117.59274125099182,0.009979505084185263
121321,121322,121321,242643,117.8659291267395,0.00996149364456096
121522,121523,121522,243045,118.0432641506195,0.00988967755707389
121722,121723,121722,243445,118.33325505256653,0.010272924040487184
121922,121923,121922,243845,118.5781922340393,0.011234535580851007
122122,122123,122122,244245,118.7420129776001,0.009861471824630735
122322,122323,122322,244645,119.08858823776245,0.009851146241958455
122523,122524,122523,245047,119.26338410377502,0.00995162850168834
122723,122724,122723,245447,119.432687997818,0.009892103426887216
122923,122924,122923,245847,119.62954115867615,0.009949991222945912
123123,123124,123123,246247,119.87240815162659,0.011527609812607423
123323,123324,123323,246647,120.0901460647583,0.009761781264073248
123524,123525,123524,247049,120.291836977005,0.009837274339976672
123724,123725,123724,247449,120.47716307640076,0.010078335224324553
123924,123925,123924,247849,120.65572786331177,0.009725010617936104
124124,124125,124124,248249,120.82745313644409,0.009654695676557136
124324,124325,124324,248649,120.99453210830688,0.009763348826345556
124525,124526,124525,249051,121.16631603240967,0.009630508379325322
124725,124726,124725,249451,121.33256316184998,0.010031573212738662
124925,124926,124925,249851,121.49395728111267,0.010298868374356032
125125,125126,125125,250251,121.66750597953796,0.009559624826556196
125325,125326,125325,250651,121.95039224624634,0.009538026158893853
125526,125527,125526,251053,122.13856220245361,0.009589421010903081
125726,125727,125726,251453,122.31238198280334,0.009678090450041924
125926,125927,125926,251853,122.54311919212341,0.009900632519954693
126126,126127,126126,252253,122.72734212875366,0.009728191795132193
126326,126327,126326,252653,122.93088603019714,0.010108179310892928
126527,126528,126527,253055,123.11342215538025,0.009436023281273288
126727,126728,126727,253455,123.29736089706421,0.009498913462102864
126927,126928,126927,253855,123.49535918235779,0.009452294698635979
127127,127128,127127,254255,123.66302394866943,0.01102878520393662
127327,127328,127327,254655,123.89591932296753,0.009449174077251248
127528,127529,127528,255057,124.15190625190735,0.00947674942285948
127728,127729,127728,255457,124.34173917770386,0.009423879509782651
127928,127929,127928,255857,124.56807208061218,0.009456720156032097
128128,128129,128128,256257,124.82098913192749,0.009417829875795817
128328,128329,128328,256657,125.04939413070679,0.009372796579861977
128529,128530,128529,257059,125.22211623191833,0.00961098785895645
128729,128730,128729,257459,125.39171004295349,0.00925389528871682
128929,128930,128929,257859,125.56152606010437,0.01059893498696668
129129,129130,129129,258259,125.82520508766174,0.0093180754726377
129329,129330,129329,258659,126.02106022834778,0.009304022222332535
129530,129531,129530,259061,126.18066692352295,0.009215106803245483
129730,129731,129730,259461,126.38094115257263,0.009213535628078322
129930,129931,129930,259861,126.55155992507935,0.00931253135001628
130130,130131,130130,260261,126.74574208259583,0.009340083283519086
130330,130331,130330,260661,126.9209291934967,0.009251348471866958
130531,130532,130531,261063,127.14337706565857,0.009242290249366373
130731,130732,130731,261463,127.39124011993408,0.00931353004637865
130931,130932,130931,261863,127.56510400772095,0.009161261458946047
131131,131132,131131,262263,127.76007103919983,0.009335671939552943
131331,131332,131331,262663,127.93418598175049,0.009173141011724669
131532,131533,131532,263065,128.10092902183533,0.009050524137719873
131732,131733,131732,263465,128.28383898735046,0.009113004004221206
131932,131933,131932,263865,128.48217821121216,0.009065373460914836
132132,132133,132132,264265,128.71579813957214,0.009165516539380377
132332,132333,132332,264665,128.92039704322815,0.009063928683591122
132533,132534,132533,265067,129.09946513175964,0.00897545887347874
132733,132734,132733,265467,129.2844259738922,0.010251291997403171
132933,132934,132933,265867,129.45286297798157,0.008971543963634164
133133,133134,133133,266267,129.6189410686493,0.010607985308513881
133333,133334,133333,266667,129.8061592578888,0.009076044816898221
133534,133535,133534,267069,129.9641191959381,0.008943491050210806
133734,133735,133734,267469,130.13363909721375,0.00899229234703203
133934,133935,133934,267869,130.29783987998962,0.009105430727745513
134134,134135,134134,268269,130.48953914642334,0.008854431261487633
134334,134335,134334,268669,130.68420314788818,0.008871215341191386
134535,134536,134535,269071,130.86391401290894,0.008913783722783794
134735,134736,134735,269471,131.04563117027283,0.008869499890056639
134935,134936,134935,269871,131.21175622940063,0.009331767227978722
135135,135136,135135,270271,131.39598608016968,0.008782189408263964
135335,135336,135335,270671,131.5653510093689,0.008758771250236197
135536,135537,135536,271073,131.7448980808258,0.008757699406709911
135736,135737,135736,271473,131.9141390323639,0.008780245605927314
135936,135937,135936,271873,132.07798409461975,0.00878101085470158
136136,136137,136136,272273,132.2607171535492,0.010989781720591155
136336,136337,136336,272673,132.59276604652405,0.008751575469104966
136537,136538,136537,273075,132.77378010749817,0.008772809399974782
136737,136738,136737,273475,132.9396140575409,0.00873624270695012
136937,136938,136937,273875,133.10724902153015,0.00894800842558574
137137,137138,137137,274275,133.47495198249817,0.0087829951074328
137337,137338,137337,274675,133.66870307922363,0.008714111917232979
137538,137539,137538,275077,133.88496017456055,0.01042583758841376
137738,137739,137738,275477,134.08425307273865,0.008774834373895197
137938,137939,137938,275877,134.26160430908203,0.008609071065124744
138138,138139,138138,276277,134.43833923339844,0.008686831116424591
138338,138339,138338,276677,134.61896109580994,0.00924206006899033
138539,138540,138539,277079,134.79979395866394,0.008649698689105083
138739,138740,138739,277479,134.97485494613647,0.00864451472943928
138939,138940,138939,277879,135.14665293693542,0.008525987736081908
139139,139140,139139,278279,135.3116500377655,0.008946204569486263
139339,139340,139339,278679,135.47526502609253,0.008509521011981451
139540,139541,139540,279081,135.63898921012878,0.008588688115487688
139740,139741,139740,279481,135.80885887145996,0.008503458908811757
139940,139941,139940,279881,135.97503900527954,0.009031401962465584
140140,140141,140140,280281,136.14762210845947,0.008465190304366215
140340,140341,140340,280681,136.31745624542236,0.008632334674412882
140541,140542,140541,281083,136.48413610458374,0.008446446126481174
140741,140742,140741,281483,136.64298295974731,0.008436589146717745
140941,140942,140941,281883,136.80612015724182,0.008420219667315633
141141,141142,141141,282283,136.9707682132721,0.008478048542396753
141341,141342,141341,282683,137.14064002037048,0.00839509862325489
141542,141543,141542,283085,137.30417013168335,0.008412266919931646
141742,141743,141742,283485,137.5168342590332,0.008436820500431567
141942,141943,141942,283885,137.6974790096283,0.008353161642363636
142142,142143,142142,284285,137.89439487457275,0.008387687426476878
142342,142343,142342,284685,138.08291101455688,0.00888053140074125
142543,142544,142543,285087,138.28741097450256,0.00835847363634208
142743,142744,142743,285487,138.45022010803223,0.008325230179301363
142943,142944,142943,285887,138.6069691181183,0.008253513999186201
143143,143144,143143,286287,138.76397705078125,0.008269950996072306
143343,143344,143343,286687,138.92216110229492,0.008249171048651084
143544,143545,143544,287089,139.08440399169922,0.0082792658146186
143744,143745,143744,287489,139.24875020980835,0.008275243241087893
143944,143945,143944,287889,139.404314994812,0.008200714539178686
144144,144145,144144,288289,139.55752110481262,0.008121766969706505
144344,144345,144344,288689,139.71018290519714,0.008245778998549632
144545,144546,144545,289091,139.8693652153015,0.008524059794281747
144745,144746,144745,289491,140.04549622535706,0.008177029714609768
144945,144946,144945,289891,140.2011480331421,0.009737302399555033
145145,145146,145145,290291,140.35829830169678,0.008905370623458388
145345,145346,145345,290691,140.51143407821655,0.008124073475947848
145546,145547,145546,291093,140.6761691570282,0.00808116888106706
145746,145747,145746,291493,140.85333728790283,0.008112862918246694
145946,145947,145946,291893,141.02921104431152,0.008095185698134132
146146,146147,146146,292293,141.19852232933044,0.009258644576120287
146346,146347,146346,292693,141.35846996307373,0.00807988420431336
146547,146548,146547,293095,141.5138020515442,0.008096812018507683
146747,146748,146747,293495,141.66849613189697,0.007994822950667587
146947,146948,146947,293895,141.82693815231323,0.007973857188001704
147147,147148,147147,294295,141.98337411880493,0.008031152691236021
147347,147348,147347,294695,142.15061402320862,0.008014149386309366
147548,147549,147548,295097,142.31583499908447,0.00796743333505109
147748,147749,147748,295497,142.46964526176453,0.007914341779779864
147948,147949,147948,295897,142.625018119812,0.007923346518237579
148148,148149,148148,296297,142.78315496444702,0.009454057208496743
148348,148349,148348,296697,142.9380121231079,0.00793589471907791
148549,148550,148549,297099,143.09889221191406,0.00786097599630423
148749,148750,148749,297499,143.25614213943481,0.007881991008647239
148949,148950,148949,297899,143.41129302978516,0.007938148611943627
149149,149150,149149,298299,143.56894898414612,0.007827371511875295
149349,149350,149349,298699,143.72239208221436,0.007906515853022447
149550,149551,149550,299101,143.8817400932312,0.007893637550996343
149750,149751,149750,299501,144.043869972229,0.009155249073513361
149950,149951,149950,299901,144.19972109794617,0.007885306625001124
150150,150151,150150,300301,144.37644720077515,0.007821935693877584
150350,150351,150350,300701,144.53476786613464,0.007800659927461503
150551,150552,150551,301103,144.6893970966339,0.007756089096709396
150751,150752,150751,301503,144.8459711074829,0.007743551452170942
150951,150952,150951,301903,145.00258803367615,0.007805230148917115
151151,151152,151151,302303,145.15796899795532,0.007822679454272697
151351,151352,151351,302703,145.31781315803528,0.007773579658658709
151552,151553,151552,303105,145.47305011749268,0.007786625777609267
151752,151753,151752,303505,145.62621808052063,0.008188088477540606
151952,151953,151952,303905,145.78565621376038,0.007724232013994179
152152,152153,152152,304305,145.939875125885,0.007680748194626401
152352,152353,152352,304705,146.09899926185608,0.007730506354374982
152553,152554,152553,305107,146.25641107559204,0.007706367213526017
152753,152754,152753,305507,146.4165163040161,0.00762715498332955
152953,152954,152953,305907,146.58773612976074,0.00791706489627591
153153,153154,153153,306307,146.74340724945068,0.00763460780652861
153353,153354,153353,306707,146.90388321876526,0.007767040570538845
153554,153555,153554,307109,147.06189513206482,0.007643523845493967
153754,153755,153754,307509,147.21529817581177,0.008772989846751627
153954,153955,153954,307909,147.37680006027222,0.008966614170900118
154154,154155,154154,308309,147.5315752029419,0.007590500179767757
154354,154355,154354,308709,147.68521308898926,0.0076064495755565125
154555,154556,154555,309111,147.84640526771545,0.007501385294664617
154755,154756,154755,309511,148.00435996055603,0.007564479001097998
154955,154956,154955,309911,148.1628930568695,0.007873669962245098
155155,155156,155155,310311,148.32317209243774,0.007565339920360191
155355,155356,155355,310711,148.47743916511536,0.007867875043101585
155556,155557,155556,311113,148.64510011672974,0.007461097036714573
155756,155757,155756,311513,148.8093593120575,0.007500656469029791
155956,155957,155956,311913,148.9647581577301,0.00750294480636719
156156,156157,156156,312313,149.1244831085205,0.007454636396438574
156356,156357,156356,312713,149.28401112556458,0.007391918608558743
156557,156558,156557,313115,149.44246411323547,0.007466534504247478
156757,156758,156757,313515,149.6159701347351,0.008792259862975098
156957,156958,156957,313915,149.77128195762634,0.007352349831027633
157157,157158,157157,314315,149.92721509933472,0.007636624062366665
157357,157358,157357,314715,150.0850031375885,0.007712814862319607
157558,157559,157558,315117,150.2413511276245,0.0073329891806401615
157758,157759,157758,315517,150.40050220489502,0.007322845926917601
157958,157959,157958,315917,150.55524110794067,0.007341118927010941
158158,158159,158158,316317,150.71054434776306,0.008919058511321788
158358,158359,158358,316717,150.8860900402069,0.007704657126456024
158559,158560,158559,317119,151.04381799697876,0.007310468626424947
158759,158760,158759,317519,151.19953608512878,0.007287067545135279
158959,158960,158959,317919,151.35857105255127,0.007347800747026011
159159,159160,159159,318319,151.51284098625183,0.0072693508907606215
159359,159360,159359,318719,151.6679871082306,0.0071948233199174
159560,159561,159560,319121,151.8313500881195,0.00730332955383705
159760,159761,159760,319521,151.9972710609436,0.007222475471885667
159960,159961,159960,319921,152.1707091331482,0.008028507638063906
160160,160161,160160,320321,152.33769702911377,0.0072586390511055
160360,160361,160360,320721,152.50832104682922,0.008699376656412338
160561,160562,160561,321123,152.67820501327515,0.007184173164097839
160761,160762,160761,321523,152.8356339931488,0.007177426609691968
160961,160962,160961,321923,153.06773900985718,0.0072165623601896985
161161,161162,161161,322323,153.25501918792725,0.007279527689931676
161361,161362,161361,322723,153.43290495872498,0.007555670748679247
161562,161563,161562,323125,153.6046290397644,0.007208685451200291
161762,161763,161762,323525,153.75905013084412,0.007109352041474739
161962,161963,161962,323925,154.03298211097717,0.007133319308459207
162162,162163,162162,324325,154.5016052722931,0.007151034511102088
162362,162363,162362,324725,154.91395616531372,0.007415837833856523
162563,162564,162563,325127,155.3045802116394,0.0070354418124986004
162763,162764,162763,325527,155.69009804725647,0.00915390241280144
162963,162964,162963,325927,156.0125172138214,0.0071159804668018386
163163,163164,163163,326327,156.21639823913574,0.00714813505364022
163363,163364,163363,326727,156.40796613693237,0.007147587707735063
163564,163565,163564,327129,156.58833813667297,0.006997457086977219
163764,163765,163764,327529,156.7764801979065,0.007008558036643208
163964,163965,163964,327929,156.9923141002655,0.007004551047061625
164164,164165,164164,328329,157.18797492980957,0.007057053729360782
164364,164365,164364,328729,157.3548390865326,0.006995236933508696
164565,164566,164565,329131,157.53003191947937,0.008715681174227467
164765,164766,164765,329531,157.73478317260742,0.00704238786025648
164965,164966,164965,329931,157.91693019866943,0.007027222218465717
165165,165166,165165,330331,158.08033633232117,0.007273526624039032
165365,165366,165365,330731,158.2382459640503,0.006917692270087891
165566,165567,165566,331133,158.39637517929077,0.0071553487951958395
165766,165767,165766,331533,158.55239605903625,0.0069530513697700965
165966,165967,165966,331933,158.7049241065979,0.006916354580268743
166166,166167,166166,332333,158.86483216285706,0.006890741536764895
166366,166367,166366,332733,159.02222228050232,0.0068774140944735905
166567,166568,166567,333135,159.17742705345154,0.006848700837518759
166767,166768,166767,333535,159.33132028579712,0.0068457376908945605
166967,166968,166967,333935,159.48635029792786,0.00820745202933619
167167,167168,167167,334335,159.6558699607849,0.007101301557516793
167367,167368,167367,334735,159.81241106987,0.006910506932165108
167568,167569,167568,335137,159.96520924568176,0.006844109023073073
167768,167769,167768,335537,160.12548732757568,0.00703566110603919
167968,167969,167968,335937,160.3478500843048,0.006847839856078047
168168,168169,168168,336337,160.52368021011353,0.006902348026370445
168368,168369,168368,336737,160.6905710697174,0.00673786083835732
168569,168570,168569,337139,160.85701894760132,0.007033022338414434
168769,168770,168769,337539,161.03385210037231,0.006783003671104932
168969,168970,168969,337939,161.202054977417,0.0068742895125736905
169169,169170,169169,338339,161.3733992576599,0.006797511961848726
169369,169370,169369,338739,161.53903913497925,0.0067352473323591625
169570,169571,169570,339141,161.70578694343567,0.006735523859930063
169770,169771,169770,339541,161.8975749015808,0.0067261953204085945
169970,169971,169970,339941,162.0712389945984,0.008044465519750906
170170,170171,170170,340341,162.2376091480255,0.0066880302666793645
170370,170371,170370,340741,162.39216208457947,0.007139461514104561
170571,170572,170571,341143,162.54704523086548,0.0066643353769968335
170771,170772,170771,341543,162.70198822021484,0.006692111467564125
170971,170972,170971,341943,162.85624814033508,0.006878438616650221
171171,171172,171171,342343,163.01226019859314,0.006667317994084124
171371,171372,171371,342743,163.16897416114807,0.006713202892431747
171572,171573,171572,343145,163.3215091228485,0.00667475186127107
171772,171773,171772,343545,163.47967219352722,0.0079252238626226
171972,171973,171972,343945,163.76428127288818,0.007032262578603052
172172,172173,172172,344345,164.11213326454163,0.007600198574465188
172372,172373,172372,344745,164.406485080719,0.006602052958166092
172573,172574,172573,345147,164.57944703102112,0.0066336002313243094
172773,172774,172773,345547,164.74891018867493,0.006549669855456327
172973,172974,172973,345947,164.9684660434723,0.006536110604471593
173173,173174,173173,346347,165.16977906227112,0.006509946636779262
173373,173374,173373,346747,165.35704517364502,0.007054299126493971
173574,173575,173574,347149,165.53868913650513,0.006486748411229194
173774,173775,173774,347549,165.69563126564026,0.006500711986352029
173974,173975,173974,347949,165.86422419548035,0.006939852783168362
174174,174175,174174,348349,166.13867902755737,0.006717506179737559
174374,174375,174374,348749,166.3042230606079,0.006481032519986034
174575,174576,174575,349151,166.46356630325317,0.00650337467128419
174775,174776,174775,349551,166.6167721748352,0.006529830275708687
174975,174976,174975,349951,166.77172994613647,0.00766754744698106
175175,175176,175175,350351,166.9896171092987,0.0064405136132717825
175375,175376,175375,350751,167.1790051460266,0.006464089607055333
175576,175577,175576,351153,167.39613819122314,0.006479767604430779
175776,175777,175776,351553,167.56527018547058,0.006431575000341985
175976,175977,175976,351953,167.7673020362854,0.006433068413197165
176176,176177,176176,352353,167.9312620162964,0.0065515364117297555
176376,176377,176376,352753,168.10117506980896,0.006427091946579181
176577,176578,176577,353155,168.2742772102356,0.007583610788692123
176777,176778,176777,353555,168.46595001220703,0.006341176507639105
176977,176978,176977,353955,168.63547015190125,0.006363405897234146
177177,177178,177177,354355,168.8041422367096,0.0063048468935747995
177377,177378,177377,354755,168.97503113746643,0.006357840949663803
177578,177579,177578,355157,169.16733121871948,0.006292928828420557
177778,177779,177778,355557,169.39497208595276,0.006282869209256227
177978,177979,177978,355957,169.5646243095398,0.006310982189794928
178178,178179,178178,356357,169.76467514038086,0.006405452680818838
178378,178379,178378,356757,169.97712588310242,0.007753296757655331
178579,178580,178579,357159,170.2019500732422,0.006329916223735507
178779,178780,178779,357559,170.39128398895264,0.006338468802648996
178979,178980,178979,357959,170.56781697273254,0.006249904512355646
179179,179180,179179,358359,170.73798298835754,0.007480579564437063
179379,179380,179379,358759,170.9151749610901,0.0063122572272611074
179580,179581,179580,359161,171.1033799648285,0.006188527872194101
179780,179781,179780,359561,171.32776618003845,0.006254264602749986
179980,179981,179980,359961,171.5796480178833,0.006215556544600124
180180,180181,180180,360361,171.7715039253235,0.00624531654697829
180380,180381,180380,360761,171.98190116882324,0.00622536509655509
180581,180582,180581,361163,172.1894989013672,0.006209571887635591
180781,180782,180781,361563,172.5296552181244,0.0067603290103265936
180981,180982,180981,361963,172.73101115226746,0.0061479694186351895
181181,181182,181181,362363,173.07157731056213,0.006161536812125701
181381,181382,181381,362763,173.39569211006165,0.006177644940368585
181582,181583,181582,363165,173.6798231601715,0.006113353659113901
181782,181783,181782,363565,173.95360708236694,0.0061682036356954266
181982,181983,181982,363965,174.23387718200684,0.006121840693422839
182182,182183,182182,364365,174.50866222381592,0.006243202242097588
182382,182383,182382,364765,174.88653230667114,0.006134747138029305
182583,182584,182583,365167,175.20333409309387,0.006099577340621476
182783,182784,182783,365567,175.53491616249084,0.006379647022865578
182983,182984,182983,365967,175.7152440547943,0.00639659377947698
183183,183184,183183,366367,175.8970181941986,0.006147094610727292
183383,183384,183383,366767,176.0733151435852,0.00605517422244534
183584,183585,183584,367169,176.24477005004883,0.0061286060185482445
183784,183785,183784,367569,176.40678715705872,0.006002609639392234
183984,183985,183984,367969,176.57780528068542,0.006032450625334812
184184,184185,184184,368369,176.75320601463318,0.006313677937686825
184384,184385,184384,368769,176.92672514915466,0.006043403037192949
184585,184586,184585,369171,177.11764001846313,0.006056962662910708
184785,184786,184785,369571,177.3885042667389,0.006054885261249672
184985,184986,184985,369971,177.59479522705078,0.006058073878730614
185185,185186,185185,370371,177.78032112121582,0.00740973987696174
185385,185386,185385,370771,177.96037101745605,0.006024675498527296
185586,185587,185586,371173,178.1266541481018,0.005984180178193426
185786,185787,185786,371573,178.30271005630493,0.005925951171737144
185986,185987,185986,371973,178.54816317558289,0.005935543058035813
186186,186187,186186,372373,178.768874168396,0.005990615686726449
186386,186387,186386,372773,178.93671107292175,0.006018493547339329
186587,186588,186587,373175,179.1071801185608,0.006012277284874804
186787,186788,186787,373575,179.29962706565857,0.005906337231237099
186987,186988,186987,373975,179.4764120578766,0.005925486164270208
187187,187188,187187,374375,179.6486349105835,0.005903235417230294
187387,187388,187387,374775,179.80592799186707,0.005878703524243212
187588,187589,187588,375177,179.98180627822876,0.005887596127496947
187788,187789,187788,375577,180.14028024673462,0.0059180011340773195
187988,187989,187988,375977,180.2945113182068,0.0059393006735595
188188,188189,188188,376377,180.457417011261,0.006135931182226895
188388,188389,188388,376777,180.61580109596252,0.005853692005958422
188589,188590,188589,377179,180.77295804023743,0.005973391485863774
188789,188790,188789,377579,180.92972707748413,0.0067831598901384816
188989,188990,188989,377979,181.0855040550232,0.006603643895940891
189189,189190,189189,378379,181.24091410636902,0.005799248234351257
189389,189390,189389,378779,181.41825222969055,0.005802333327713945
189590,189591,189590,379181,181.57521605491638,0.0057898230881128976
189790,189791,189790,379581,181.74030423164368,0.005793465360706356
189990,189991,189990,379981,181.90807819366455,0.005789414898781205
190190,190191,190190,380381,182.06684613227844,0.005780591567858376
190390,190391,190390,380781,182.2475781440735,0.005782743635878963
190591,190592,190591,381183,182.4225151538849,0.006977412860854395
190791,190792,190791,381583,182.58565211296082,0.005758826190290514
190991,190992,190991,381983,182.78499722480774,0.005769318108983297
191191,191192,191191,382383,183.02647995948792,0.005790488289332991
191391,191392,191391,382783,183.27716898918152,0.006475180126139326
191592,191593,191592,383185,183.55501914024353,0.005691682214744309
191792,191793,191792,383585,183.86172604560852,0.005949369500595325
191992,191993,191992,383985,184.10692405700684,0.0061715102155348416
192192,192193,192192,384385,184.44330310821533,0.0057347449372095755
192392,192393,192392,384785,184.7663459777832,0.005745203424853079
192593,192594,192593,385187,185.0297770500183,0.005762860027516822
192793,192794,192793,385587,185.3094563484192,0.005682137586648263
192993,192994,192993,385987,185.67203617095947,0.005671018330745232
193193,193194,193193,386387,186.0202922821045,0.0063182659786968935
193393,193394,193393,386787,186.35798621177673,0.006451096022777104
193594,193595,193594,387189,186.69888710975647,0.005676642951078387
193794,193795,193794,387589,186.98595118522644,0.005638826458849299
193994,193995,193994,387989,187.23058795928955,0.006829248203352093
194194,194195,194194,388389,187.4804491996765,0.005662518805251318
194394,194395,194394,388789,187.76417803764343,0.0064715494691431966
194595,194596,194595,389191,188.0267689228058,0.005600368843653895
194795,194796,194795,389591,188.3966453075409,0.00565039732366775
194995,194996,194995,389991,188.68961906433105,0.005597950723103198
195195,195196,195195,390391,189.0507411956787,0.005575669951942582
195395,195396,195395,390791,189.2332649230957,0.006886563409410645
195596,195597,195596,391193,189.41704034805298,0.005584945410830736
195796,195797,195796,391593,189.59671306610107,0.00557124705929816
195996,195997,195996,391993,189.79103112220764,0.005517853055338362
196196,196197,196196,392393,189.97090792655945,0.005618570335416077
196396,196397,196396,392793,190.1597399711609,0.005613990726752969
196597,196598,196597,393195,190.37773489952087,0.005539729397551354
196797,196798,196797,393595,190.58017206192017,0.0055724284858010825
196997,196998,196997,393995,190.7323431968689,0.005502826697989712
197197,197198,197197,394395,190.88750505447388,0.0055304025095857905
197397,197398,197397,394795,191.05578708648682,0.005554831542612902
197598,197599,197598,395197,191.21988201141357,0.005489844418283752
197798,197799,197798,395597,191.38478803634644,0.0066899438090353164
197998,197999,197998,395997,191.55600118637085,0.0058374031437525885
198198,198199,198198,396397,191.8689432144165,0.006416024385678713
198398,198399,198398,396797,192.08561420440674,0.0056518022561128966
198599,198600,198599,397199,192.36643719673157,0.005495770360522918
198799,198800,198799,397599,192.87445306777954,0.005472873238514875
198999,199000,198999,397999,193.45346212387085,0.00546956781320136
199199,199200,199199,398399,193.86799216270447,0.005499488517493203
199399,199400,199399,398799,194.33308601379395,0.005458545254272569
199600,199601,199600,399201,194.82830905914307,0.005437973857626802
199800,199801,199800,399601,195.3700511455536,0.005633167290011079
200000,200001,200000,400001,195.9777889251709,0.005434957686107025


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha0/eag-c.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012149810791015625,30.358099469249375
100,201,0,201,0.14583706855773926,6.497570818090755
200,401,0,401,0.2944481372833252,3.18105807646363
300,601,0,601,0.4670841693878174,2.023030291273728
400,801,0,801,0.635936975479126,1.5000642024628064
501,1003,0,1003,0.7899360656738281,1.2103469417860875
601,1203,0,1203,0.949761152267456,0.9917060130889543
701,1403,0,1403,1.13106107711792,0.8254787271305319
801,1603,0,1603,1.2845561504364014,0.7062811064072342
901,1803,0,1803,1.4317481517791748,0.6543601275560126
1001,2003,0,2003,1.5721988677978516,0.5773048961321726
1101,2203,0,2203,1.7155489921569824,0.5144269762928468
1201,2403,0,2403,1.854905128479004,0.45615330695503536
1301,2603,0,2603,2.0115180015563965,0.4404029996357728
1401,2803,0,2803,2.1761410236358643,0.3975980279547153
1502,3005,0,3005,2.345039129257202,0.36949295128494175
1602,3205,0,3205,2.4993951320648193,0.3453935729189495
1702,3405,0,3405,2.660348892211914,0.3224437473756645
1802,3605,0,3605,2.8231329917907715,0.3003083696808211
1902,3805,0,3805,2.9752602577209473,0.2790046640953164
2002,4005,0,4005,3.124285936355591,0.26758608951506263
2102,4205,0,4205,3.2784199714660645,0.2581574044396648
2202,4405,0,4405,3.4347169399261475,0.25392760853436286
2302,4605,0,4605,3.589181900024414,0.24490737158516468
2402,4805,0,4805,3.736598014831543,0.23075280240887205
2503,5007,0,5007,3.885317087173462,0.2222706985986103
2603,5207,0,5207,4.028550863265991,0.21052433242698215
2703,5407,0,5407,4.180194139480591,0.20151474426108304
2803,5607,0,5607,4.326223134994507,0.19525221603049853
2903,5807,0,5807,4.466821193695068,0.18874538823192655
3003,6007,0,6007,4.627024173736572,0.18043529960724145
3103,6207,0,6207,4.79167914390564,0.1724978037257758
3203,6407,0,6407,4.96924901008606,0.16746846548193717
3303,6607,0,6607,5.122457027435303,0.1634600138497955
3403,6807,0,6807,5.288764953613281,0.15782350719656182
3504,7009,0,7009,5.509546995162964,0.15237471620528026
3604,7209,0,7209,5.705277919769287,0.14989467892912553
3704,7409,0,7409,5.883615016937256,0.1451703990021208
3804,7609,0,7609,6.107993125915527,0.14023450784353794
3904,7809,0,7809,6.271381139755249,0.13736999542970416
4004,8009,0,8009,6.436395168304443,0.1351099220664021
4104,8209,0,8209,6.588837146759033,0.1331033881503364
4204,8409,0,8409,6.738521099090576,0.13152319488662384
4304,8609,0,8609,6.8856000900268555,0.1261771953830402
4404,8809,0,8809,7.046363115310669,0.12212300590662446
4505,9011,0,9011,7.207620143890381,0.11881645204132854
4605,9211,0,9211,7.358686923980713,0.11600223873764948
4705,9411,0,9411,7.504754066467285,0.11238929828935541
4805,9611,0,9611,7.663981199264526,0.1107886084508722
4905,9811,0,9811,7.808404922485352,0.10885204316784926
5005,10011,0,10011,7.957789897918701,0.10629086176646911
5105,10211,0,10211,8.105000972747803,0.10292809789710003
5205,10411,0,10411,8.259253025054932,0.10179722659931073
5305,10611,0,10611,8.407384157180786,0.10050868282250508
5405,10811,0,10811,8.548290014266968,0.099685546227355
5506,11013,0,11013,8.689716100692749,0.0964678127262242
5606,11213,0,11213,8.834662199020386,0.09449470383495231
5706,11413,0,11413,8.977593183517456,0.09494493700747744
5806,11613,0,11613,9.130220174789429,0.09259000418131524
5906,11813,0,11813,9.300217151641846,0.09000840286487526
6006,12013,0,12013,9.44390606880188,0.08932099103487805
6106,12213,0,12213,9.589510917663574,0.08768139282884627
6206,12413,0,12413,9.730094194412231,0.08607332518150468
6306,12613,0,12613,9.87195611000061,0.08352982587031096
6406,12813,0,12813,10.024049997329712,0.0814089279433394
6507,13015,0,13015,10.217818260192871,0.07954965480763306
6607,13215,0,13215,10.367501020431519,0.07843490648794667
6707,13415,0,13415,10.51526403427124,0.07684005998000677
6807,13615,0,13615,10.716358184814453,0.0765324674966933
6907,13815,0,13815,10.859550952911377,0.07652741618012764
7007,14015,0,14015,11.004064083099365,0.07518958956214769
7107,14215,0,14215,11.192026138305664,0.07401083218612478
7207,14415,0,14415,11.357577085494995,0.07415698778432939
7307,14615,0,14615,11.50106406211853,0.07370524568149782
7407,14815,0,14815,11.642937183380127,0.07229548772292166
7508,15017,0,15017,11.785389184951782,0.07053739248907821
7608,15217,0,15217,11.929034948348999,0.06961414134153376
7708,15417,0,15417,12.070999145507812,0.06863808673602492
7808,15617,0,15617,12.229730129241943,0.06791716038317355
7908,15817,0,15817,12.37759804725647,0.06696928014533543
8008,16017,0,16017,12.516961097717285,0.06588325042173358
8108,16217,0,16217,12.66623306274414,0.06521640579231851
8208,16417,0,16417,12.807246208190918,0.06353216538231435
8308,16617,0,16617,12.950984954833984,0.0619337233103036
8408,16817,0,16817,13.108495235443115,0.061551238751332026
8509,17019,0,17019,13.28931999206543,0.06112176638605797
8609,17219,0,17219,13.473052978515625,0.060362107536433965
8709,17419,0,17419,13.660864114761353,0.05962927835119283
8809,17619,0,17619,13.81277322769165,0.05927903453218729
8909,17819,0,17819,13.965537071228027,0.05925507795417719
9009,18019,0,18019,14.127811193466187,0.058501062422898764
9109,18219,0,18219,14.307642221450806,0.057743941901409225
9209,18419,0,18419,14.478209018707275,0.057786603017676394
9309,18619,0,18619,14.638758182525635,0.05747442954460791
9409,18819,0,18819,14.912891149520874,0.056414997407415915
9510,19021,0,19021,15.12336015701294,0.05544709063960474
9610,19221,0,19221,15.326128244400024,0.054828760605241174
9710,19421,0,19421,15.48313021659851,0.05442827870017512
9810,19621,0,19621,15.679784059524536,0.05368941434040843
9910,19821,0,19821,15.855808019638062,0.05309150462705312
10010,20021,0,20021,16.005410194396973,0.05259691805190521
10110,20221,0,20221,16.16487717628479,0.05165413161290116
10210,20421,0,20421,16.3333261013031,0.05062121353460223
10310,20621,0,20621,16.47207808494568,0.04998976431105962
10410,20821,0,20821,16.611127138137817,0.05004660945659487
10511,21023,0,21023,16.76579713821411,0.05002121002999302
10611,21223,0,21223,16.91773009300232,0.04950931341763679
10711,21423,0,21423,17.235530138015747,0.049152421689849846
10811,21623,0,21623,17.409735918045044,0.04898914731937789
10911,21823,0,21823,17.577171087265015,0.048625618325843854
11011,22023,0,22023,17.89622712135315,0.04772417739181262
11111,22223,0,22223,18.091238260269165,0.04695438029453348
11211,22423,0,22423,18.306241989135742,0.04676916665120571
11311,22623,0,22623,18.47876214981079,0.04640352444191618
11411,22823,0,22823,18.68700909614563,0.04538483138154528
11512,23025,0,23025,18.88360595703125,0.044632238828966345
11612,23225,0,23225,19.118389129638672,0.04450915944825903
11712,23425,0,23425,19.40050506591797,0.0440873058419543
11812,23625,0,23625,19.659630060195923,0.04340758855526487
11912,23825,0,23825,19.97952890396118,0.0432488719760236
12012,24025,0,24025,20.363765001296997,0.043407749563252246
12112,24225,0,24225,20.760698080062866,0.04335019559836247
12212,24425,0,24425,20.96196985244751,0.042990962082999976
12312,24625,0,24625,21.163926124572754,0.04275388109482999
12412,24825,0,24825,21.42551302909851,0.04243427748617231
12513,25027,0,25027,21.72847318649292,0.041652132862083184
12613,25227,0,25227,21.90793228149414,0.041017066403614355
12713,25427,0,25427,22.06597924232483,0.04106801677464307
12813,25627,0,25627,22.294294118881226,0.041148731544671135
12913,25827,0,25827,22.595750093460083,0.04074551368596436
13013,26027,0,26027,22.805647134780884,0.04019720042014087
13113,26227,0,26227,22.993518114089966,0.039692474672224407
13213,26427,0,26427,23.17101812362671,0.03915314870425332
13313,26627,0,26627,23.359879970550537,0.03877437987814547
13413,26827,0,26827,23.518441915512085,0.03860817952107695
13514,27029,0,27029,23.70565104484558,0.03829721406596253
13614,27229,0,27229,23.879845142364502,0.03789084925919942
13714,27429,0,27429,24.04662823677063,0.037809088516280745
13814,27629,0,27629,24.21387505531311,0.038039240217240436
13914,27829,0,27829,24.399301052093506,0.03836690575386712
14014,28029,0,28029,24.586053133010864,0.038401421007606226
14114,28229,0,28229,24.76908802986145,0.0379733926422984
14214,28429,0,28429,24.926069021224976,0.03743824067400723
14314,28629,0,28629,25.088829040527344,0.036901513051542253
14414,28829,0,28829,25.569329261779785,0.03629662175375142
14515,29031,0,29031,25.920282125473022,0.035756637644634014
14615,29231,0,29231,26.13672113418579,0.03538888317272155
14715,29431,0,29431,26.304471015930176,0.03523456878359604
14815,29631,0,29631,26.476701974868774,0.03515616978529578
14915,29831,0,29831,26.65602993965149,0.034879516177690285
15015,30031,0,30031,26.816050052642822,0.03448536734146079
15115,30231,0,30231,27.101423263549805,0.03424970520560686
15215,30431,0,30431,27.55671715736389,0.03413788977165118
15315,30631,0,30631,27.81310796737671,0.033982143008598475
15415,30831,0,30831,27.971816062927246,0.033750897970925536
15516,31033,0,31033,28.40077495574951,0.03351612176845904
15616,31233,0,31233,28.760765075683594,0.033310987301973405
15716,31433,0,31433,29.149364948272705,0.03323192877731481
15816,31633,0,31633,29.435465097427368,0.03341173197626887
15916,31833,0,31833,29.597187042236328,0.03362120129994118
16016,32033,0,32033,29.750760078430176,0.03345732291929519
16116,32233,0,32233,29.912723064422607,0.03285815081343183
16216,32433,0,32433,30.059065103530884,0.03218086592959834
16316,32633,0,32633,30.212369918823242,0.03172823435553485
16416,32833,0,32833,30.403232097625732,0.031403064531653854
16517,33035,0,33035,30.573549032211304,0.031038743011142587
16617,33235,0,33235,30.739797115325928,0.03077060747667494
16717,33435,0,33435,30.92891216278076,0.03075550190451851
16817,33635,0,33635,31.08741307258606,0.030798908578795723
16917,33835,0,33835,31.23896288871765,0.030671673122604888
17017,34035,0,34035,31.416900157928467,0.030528277136852692
17117,34235,0,34235,31.576598167419434,0.03059192666022504
17217,34435,0,34435,31.737467288970947,0.030676389257550066
17317,34635,0,34635,31.91404700279236,0.03048265770068797
17417,34835,0,34835,32.09281897544861,0.030111193524697766
17518,35037,0,35037,32.27728009223938,0.029762655465028293
17618,35237,0,35237,32.42514896392822,0.029457723322721677
17718,35437,0,35437,32.57607913017273,0.029207667016899887
17818,35637,0,35637,32.770785093307495,0.029069318564550264
17918,35837,0,35837,33.20151710510254,0.028987998646194328
18018,36037,0,36037,33.49682903289795,0.028754622471627602
18118,36237,0,36237,33.71851110458374,0.028352680225392134
18218,36437,0,36437,34.12039089202881,0.028063798048752392
18318,36637,0,36637,34.718510150909424,0.027954735070929704
18418,36837,0,36837,35.31032919883728,0.027846054165244716
18519,37039,0,37039,35.67848801612854,0.027714318313898558
18619,37239,0,37239,36.30276703834534,0.0276464620901262
18719,37439,0,37439,36.58930420875549,0.027595404030343378
18819,37639,0,37639,36.82678198814392,0.02752070848648731
18919,37839,0,37839,37.00404095649719,0.02748038757635805
19019,38039,0,38039,37.1661639213562,0.027443577174033618
19119,38239,0,38239,37.314332246780396,0.02729219931817483
19219,38439,0,38439,37.549986124038696,0.027010347194604205
19319,38639,0,38639,37.85949110984802,0.02668892568665085
19419,38839,0,38839,38.12392020225525,0.026407814489896486
19520,39041,0,39041,38.34471297264099,0.02617565005284747
19620,39241,0,39241,38.58427023887634,0.02600712537624964
19720,39441,0,39441,38.72247815132141,0.02597071652497352
19820,39641,0,39641,38.86555600166321,0.026034849173947057
19920,39841,0,39841,39.025827169418335,0.02599386069255185
20020,40041,0,40041,39.18114900588989,0.025760449013504987
20120,40241,0,40241,39.32174110412598,0.025508959866733277
20220,40441,0,40441,39.46534705162048,0.02542747375051588
20320,40641,0,40641,39.61157417297363,0.025496766064424543
20420,40841,0,40841,39.766937255859375,0.02556557100236526
20521,41043,0,41043,39.9231219291687,0.025535577563808115
20621,41243,0,41243,40.0694260597229,0.02539664856588189
20721,41443,0,41443,40.20889496803284,0.025166565532885876
20821,41643,0,41643,40.349059104919434,0.02492525364309501
20921,41843,0,41843,40.48798418045044,0.024803135239849016
21021,42043,0,42043,40.62782406806946,0.02478630791517705
21121,42243,0,42243,40.76799011230469,0.02468672157348031
21221,42443,0,42443,40.909953117370605,0.02441362752208856
21321,42643,0,42643,41.04973006248474,0.024122766818374605
21421,42843,0,42843,41.189054012298584,0.023996608574734832
21522,43045,0,43045,41.33164691925049,0.024004181569763822
21622,43245,0,43245,41.47215509414673,0.02402138540707371
21722,43445,0,43445,41.61233615875244,0.024009679198209868
21822,43645,0,43645,41.75184416770935,0.023965775830600826
21922,43845,0,43845,41.90221118927002,0.02385117709501578
22022,44045,0,44045,42.05331301689148,0.02363103468017419
22122,44245,0,44245,42.19299006462097,0.023389617318924666
22222,44445,0,44445,42.33120512962341,0.023301785818496224
22322,44645,0,44645,42.47008419036865,0.023387972371325758
22422,44845,0,44845,42.61061906814575,0.023462034108465472
22523,45047,0,45047,42.752732276916504,0.023387684381331424
22623,45247,0,45247,42.89472699165344,0.023207288172031625
22723,45447,0,45447,43.03316402435303,0.022993623405004132
22823,45647,0,45647,43.17344522476196,0.02276272338568233
22923,45847,0,45847,43.31930708885193,0.022547499551862325
23023,46047,0,46047,43.46453809738159,0.022398049185947524
23123,46247,0,46247,43.60546517372131,0.02226787405332401
23223,46447,0,46447,43.744346141815186,0.022070668505965257
23323,46647,0,46647,43.8832950592041,0.021856559123997667
23423,46847,0,46847,44.02893590927124,0.021768471486244098
23524,47049,0,47049,44.18869924545288,0.021842919983068892
23624,47249,0,47249,44.33228898048401,0.021958606858033698
23724,47449,0,47449,44.47100591659546,0.022000080410013646
23824,47649,0,47649,44.609586000442505,0.021944831394345204
23924,47849,0,47849,44.74910116195679,0.021802858151697475
24024,48049,0,48049,44.89036798477173,0.021612095792515745
24124,48249,0,48249,45.029675006866455,0.021460817274071488
24224,48449,0,48449,45.167815923690796,0.02139638466033242
24324,48649,0,48649,45.31343412399292,0.021361147257037003
24424,48849,0,48849,45.453880071640015,0.021286401970289238
24525,49051,0,49051,45.595492124557495,0.021180462801429323
24625,49251,0,49251,45.73885917663574,0.021079262573999932
24725,49451,0,49451,45.880369901657104,0.020985349095730646
24825,49651,0,49651,46.02093505859375,0.020899380883918146
24925,49851,0,49851,46.16615414619446,0.020809470914720605
25025,50051,0,50051,46.32304906845093,0.020661498724937593
25125,50251,0,50251,46.465835094451904,0.02043151742871085
25225,50451,0,50451,46.612611055374146,0.02021435357845601
25325,50651,0,50651,46.75834107398987,0.020147892675608424
25425,50851,0,50851,46.89830303192139,0.020242890401302557
25526,51053,0,51053,47.04146218299866,0.020371346061538193
25626,51253,0,51253,47.17877411842346,0.020412603751708242
25726,51453,0,51453,47.31961011886597,0.02033943832475628
25826,51653,0,51653,47.460347175598145,0.020173734263635626
25926,51853,0,51853,47.60117197036743,0.01996066471172284
26026,52053,0,52053,47.74102807044983,0.0197563625832987
26126,52253,0,52253,47.88426113128662,0.01960803039736928
26226,52453,0,52453,48.03850293159485,0.01953788957476648
26326,52653,0,52653,48.18619227409363,0.01953295733206041
26426,52853,0,52853,48.328680992126465,0.019560820451539
26527,53055,0,53055,48.518759965896606,0.01958528858456055
26627,53255,0,53255,48.71254920959473,0.019557358963775237
26727,53455,0,53455,48.86417317390442,0.019445105239422056
26827,53655,0,53655,49.006033182144165,0.019282746028292032
26927,53855,0,53855,49.14616513252258,0.019142390769744104
27027,54055,0,54055,49.28472399711609,0.019043495418734374
27127,54255,0,54255,49.42277503013611,0.018953928906568628
27227,54455,0,54455,49.56311511993408,0.01888129073058618
27327,54655,0,54655,49.70645093917847,0.01886469059639454
27427,54855,0,54855,49.8493812084198,0.0188782427952823
27528,55057,0,55057,49.99298095703125,0.018839751056161865
27628,55257,0,55257,50.133131980895996,0.018712613694067202
27728,55457,0,55457,50.2748339176178,0.018527342750287033
27828,55657,0,55657,50.41363501548767,0.01832803994536607
27928,55857,0,55857,50.562516927719116,0.018160704485035876
28028,56057,0,56057,50.7113242149353,0.018083941018111865
28128,56257,0,56257,50.85014009475708,0.01811885679441954
28228,56457,0,56457,50.98836398124695,0.018216511192887773
28328,56657,0,56657,51.125893115997314,0.018313769265381974
28428,56857,0,56857,51.263880014419556,0.018376708617969806
28529,57059,0,57059,51.40371108055115,0.01837708615808386
28629,57259,0,57259,51.543421030044556,0.018285559986872788
28729,57459,0,57459,51.683566093444824,0.018111169242099514
28829,57659,0,57659,51.82315492630005,0.01791647271314816
28929,57859,0,57859,51.96472191810608,0.017769560746001847
29029,58059,0,58059,52.10442614555359,0.017686607375438798
29129,58259,0,58259,52.243226051330566,0.017644811695501
29229,58459,0,58459,52.385149002075195,0.017627732777876527
29329,58659,0,58659,52.525336027145386,0.017617898232168125
29429,58859,0,58859,52.6703622341156,0.01756990663997418
29530,59061,0,59061,52.82514524459839,0.017439505064197548
29630,59261,0,59261,52.964022159576416,0.01724628532322213
29730,59461,0,59461,53.10378408432007,0.017057233385210847
29830,59661,0,59661,53.24269223213196,0.016932406354641362
29930,59861,0,59861,53.38509488105774,0.016901776242951534
30030,60061,0,60061,53.52501821517944,0.016968835602166492
30130,60261,0,60261,53.66336107254028,0.017094077208469755
30230,60461,0,60461,53.8031702041626,0.017206794452329508
30330,60661,0,60661,53.94196820259094,0.01726208936669864
30430,60861,0,60861,54.08150601387024,0.017257346955811506
30531,61063,0,61063,54.2209370136261,0.017195906962887628
30631,61263,0,61263,54.36005926132202,0.01708551879920498
30731,61463,0,61463,54.50392699241638,0.016954606640534647
30831,61663,0,61663,54.66234111785889,0.016830574039153768
30931,61863,0,61863,54.80687618255615,0.016704186058886135
31031,62063,0,62063,54.96155023574829,0.016550320581509233
31131,62263,0,62263,55.10046100616455,0.016374896619064844
31231,62463,0,62463,55.23845314979553,0.016220035409053885
31331,62663,0,62663,55.37863302230835,0.0161251296361851
31431,62863,0,62863,55.51714205741882,0.016093542405230095
31532,63065,0,63065,55.657185077667236,0.0160966317919889
31632,63265,0,63265,55.7992582321167,0.016103484325531322
31732,63465,0,63465,55.94099998474121,0.01610923859250133
31832,63665,0,63665,56.08080315589905,0.016130841199404274
31932,63865,0,63865,56.220020055770874,0.016176988298711652
32032,64065,0,64065,56.361868143081665,0.016232251828354742
32132,64265,0,64265,56.50171494483948,0.016266410752709525
32232,64465,0,64465,56.64208507537842,0.01625265375404626
32332,64665,0,64665,56.78187394142151,0.016184515856696263
32432,64865,0,64865,56.92553901672363,0.016077774893097495
32533,65067,0,65067,57.07921004295349,0.01595553044298982
32633,65267,0,65267,57.222116231918335,0.01584379846074374
32733,65467,0,65467,57.35841202735901,0.015761298626634047
32833,65667,0,65667,57.4971079826355,0.01571436719308903
32933,65867,0,65867,57.63566327095032,0.015684113968030808
33033,66067,0,66067,57.77517008781433,0.01563718628207119
33133,66267,0,66267,57.91653108596802,0.015561430080103095
33233,66467,0,66467,58.05879807472229,0.015488253289237384
33333,66667,0,66667,58.198180198669434,0.015462951018103969
33433,66867,0,66867,58.33907413482666,0.015489346495871357
33534,67069,0,67069,58.4794659614563,0.01552245682061283
33634,67269,0,67269,58.620174169540405,0.015517834758103043
33734,67469,0,67469,58.75796723365784,0.015472652186821128
33834,67669,0,67669,58.90006923675537,0.015409418102235955
33934,67869,0,67869,59.042120933532715,0.015344384012833898
34034,68069,0,68069,59.19281196594238,0.01527794784851376
34134,68269,0,68269,59.34297513961792,0.015199265219672048
34234,68469,0,68469,59.48114514350891,0.01508947506158077
34334,68669,0,68669,59.62051606178284,0.014939526306276768
34434,68869,0,68869,59.76243710517883,0.014775825934942855
34535,69071,0,69071,59.90908908843994,0.014647489877268077
34635,69271,0,69271,60.04636001586914,0.014587607965173083
34735,69471,0,69471,60.18569302558899,0.014589804022144593
34835,69671,0,69671,60.3238799571991,0.014632373822527448
34935,69871,0,69871,60.464760065078735,0.014688287391773719
35035,70071,0,70071,60.60201406478882,0.014729599241684948
35135,70271,0,70271,60.74333119392395,0.014740616450661504
35235,70471,0,70471,60.88303899765015,0.014725003569755538
35335,70671,0,70671,61.02042293548584,0.014694288541799551
35435,70871,0,70871,61.157158851623535,0.01465586360281478
35536,71073,0,71073,61.302310943603516,0.014610209900169662
35636,71273,0,71273,61.45533490180969,0.014550017962549452
35736,71473,0,71473,61.59564018249512,0.014463717806083113
35836,71673,0,71673,61.73346519470215,0.014359620897802967
35936,71873,0,71873,61.87047815322876,0.014267943012794502
36036,72073,0,72073,62.01041316986084,0.014202592977174359
36136,72273,0,72273,62.151121854782104,0.014137619246036265
36236,72473,0,72473,62.2890522480011,0.014044284091892898
36336,72673,0,72673,62.42695903778076,0.013935296262172504
36436,72873,0,72873,62.566468238830566,0.013852339077216174
36537,73075,0,73075,62.7069890499115,0.013825530985620362
36637,73275,0,73275,62.84864115715027,0.013859682257077144
36737,73475,0,73475,62.98637413978577,0.013936462377438149
36837,73675,0,73675,63.1252019405365,0.014017397378569496
36937,73875,0,73875,63.26297187805176,0.014062110896130214
37037,74075,0,74075,63.40336513519287,0.014062010591681353
37137,74275,0,74275,63.55707001686096,0.014041075495928992
37237,74475,0,74475,63.700247049331665,0.014016728621862401
37337,74675,0,74675,63.83834505081177,0.013977594335335545
37437,74875,0,74875,63.97820019721985,0.013903071920659935
37538,75077,0,75077,64.11892819404602,0.013783511178033963
37638,75277,0,75277,64.25683903694153,0.013627208042192342
37738,75477,0,75477,64.39514493942261,0.013454974063232074
37838,75677,0,75677,64.53443884849548,0.013307537678005197
37938,75877,0,75877,64.67640614509583,0.013225433458712235
38038,76077,0,76077,64.81557703018188,0.013215142035751413
38138,76277,0,76277,64.95368194580078,0.013244020639857617
38238,76477,0,76477,65.09136509895325,0.01327506530385277
38338,76677,0,76677,65.22844409942627,0.013297328565262034
38438,76877,0,76877,65.36846899986267,0.013319066659406749
38539,77079,0,77079,65.50663089752197,0.013343588920700122
38639,77279,0,77279,65.65363001823425,0.01336029402186117
38739,77479,0,77479,65.80186223983765,0.013358028375924555
38839,77679,0,77679,65.94392609596252,0.013335559627283874
38939,77879,0,77879,66.08235120773315,0.0133027293595509
39039,78079,0,78079,66.22427701950073,0.013273772774273137
39139,78279,0,78279,66.36777710914612,0.013255730213829196
39239,78479,0,78479,66.5070321559906,0.013238501480488848
39339,78679,0,78679,66.64542412757874,0.013200385365776963
39439,78879,0,78879,66.785325050354,0.013127733246447193
39540,79081,0,79081,66.93263912200928,0.013024919177860115
39640,79281,0,79281,67.17652916908264,0.012911563980715109
39740,79481,0,79481,67.4251389503479,0.012806458175856832
39840,79681,0,79681,67.70243716239929,0.012728732496064377
39940,79881,0,79881,67.93281412124634,0.012692754975207858
40040,80081,0,80081,68.11664509773254,0.012700268423175882
40140,80281,0,80281,68.30796003341675,0.012737914631257466
40240,80481,0,80481,68.48801803588867,0.012784080541779309
40340,80681,0,80681,68.65627694129944,0.012818423149746645
40440,80881,0,80881,68.81160187721252,0.012826821499396273
40541,81083,0,81083,68.95763111114502,0.012801435733162211
40641,81283,0,81283,69.10444712638855,0.012742652291862396
40741,81483,0,81483,69.24606585502625,0.012660988437429419
40841,81683,0,81683,69.38697123527527,0.012579907245720553
40941,81883,0,81883,69.5362958908081,0.012526604825476809
41041,82083,0,82083,69.67928910255432,0.012510698329113678
41141,82283,0,82283,69.82203912734985,0.01251063302229887
41241,82483,0,82483,69.97195506095886,0.012487857864645176
41341,82683,0,82683,70.13462805747986,0.012420150434973628
41441,82883,0,82883,70.29066014289856,0.012323207428942624
41542,83085,0,83085,70.43748211860657,0.012239220431054534
41642,83285,0,83285,70.58119010925293,0.012207380477913964
41742,83485,0,83485,70.74080896377563,0.012234490215297893
41842,83685,0,83685,70.89267420768738,0.012300252157371096
41942,83885,0,83885,71.0392918586731,0.012371385369381871
42042,84085,0,84085,71.31161713600159,0.012416809756613483
42142,84285,0,84285,71.59101915359497,0.012418783475341894
42242,84485,0,84485,71.86282396316528,0.012376067277606621
42342,84685,0,84685,72.03845930099487,0.012297601339261218
42442,84885,0,84885,72.20846009254456,0.012194656045983934
42543,85087,0,85087,72.40397596359253,0.012077897272204034
42643,85287,0,85287,72.58356308937073,0.011963407029654996
42743,85487,0,85487,72.75315523147583,0.011864252928732985
42843,85687,0,85687,72.93398714065552,0.01179295357064305
42943,85887,0,85887,73.09883213043213,0.011758091845178325
43043,86087,0,86087,73.25862407684326,0.011757782339821742
43143,86287,0,86287,73.45214915275574,0.011774297477590442
43243,86487,0,86487,73.62145614624023,0.011783651120177454
43343,86687,0,86687,73.81641292572021,0.011776357852712424
43443,86887,0,86887,73.99177408218384,0.011766461342112728
43544,87089,0,87089,74.25992202758789,0.011777174527791477
43644,87289,0,87289,74.43789792060852,0.011816339292235457
43744,87489,0,87489,74.5992739200592,0.01186796113659586
43844,87689,0,87689,74.75884509086609,0.011904220198060422
43944,87889,0,87889,74.95225024223328,0.011902787024105563
44044,88089,0,88089,75.15810203552246,0.011855651617724497
44144,88289,0,88289,75.32253003120422,0.01176967219173793
44244,88489,0,88489,75.48840022087097,0.011662500697635053
44344,88689,0,88689,75.66220903396606,0.01155419492331616
44444,88889,0,88889,75.88904190063477,0.011458434039250462
44545,89091,0,89091,76.07428097724915,0.011380739199294523
44645,89291,0,89291,76.30490708351135,0.011328151393830461
44745,89491,0,89491,76.51421689987183,0.011308211755799847
44845,89691,0,89691,76.75017213821411,0.01132563582406941
44945,89891,0,89891,76.96222591400146,0.011372041161683093
45045,90091,0,90091,77.14995622634888,0.01142555808082766
45145,90291,0,90291,77.33453798294067,0.011461119215912398
45245,90491,0,90491,77.51585507392883,0.011464065199006678
45345,90691,0,90691,77.72482514381409,0.011438328863609314
45445,90891,0,90891,77.97400498390198,0.011402646613409749
45546,91093,0,91093,78.13556718826294,0.011375255963750212
45646,91293,0,91293,78.2939100265503,0.01135984633320136
45746,91493,0,91493,78.45635724067688,0.011342589272360334
45846,91693,0,91693,78.79091000556946,0.011306161416222045
45946,91893,0,91893,78.99419808387756,0.011242877646983236
46046,92093,0,92093,79.22555494308472,0.011157994082515315
46146,92293,0,92293,79.42173409461975,0.011064107853662623
46246,92493,0,92493,79.69337010383606,0.010974201998277262
46346,92693,0,92693,79.86438822746277,0.010897923728098835
46446,92893,0,92893,80.0498309135437,0.010841124492370196
46547,93095,0,93095,80.22939014434814,0.010806369861447986
46647,93295,0,93295,80.49212312698364,0.010794185282570005
46747,93495,0,93495,80.84655427932739,0.010800816793398539
46847,93695,0,93695,81.09682989120483,0.010820798618606456
46947,93895,0,93895,81.41915798187256,0.010847501831649575
47047,94095,0,94095,81.59665727615356,0.010871896080965988
47147,94295,0,94295,81.75271701812744,0.0108819441686309
47247,94495,0,94495,81.90463900566101,0.010868699765496908
47347,94695,0,94695,82.0954749584198,0.010835407193025965
47447,94895,0,94895,82.26882410049438,0.010796416195112847
47548,95097,0,95097,82.4203588962555,0.01076353217104118
47648,95297,0,95297,82.58019304275513,0.010737019324661885
47748,95497,0,95497,82.74245190620422,0.010707345110592546
47848,95697,0,95697,82.89141511917114,0.01066638270101225
47948,95897,0,95897,83.03838324546814,0.010613234755673967
48048,96097,0,96097,83.19222807884216,0.010556517875377341
48148,96297,0,96297,83.37339401245117,0.010512613064664372
48248,96497,0,96497,83.51478815078735,0.010497428713284317
48348,96697,0,96697,83.6601049900055,0.010516058170096446
48448,96897,0,96897,83.80816698074341,0.010559470569999807
48549,97099,0,97099,83.95699214935303,0.01060986397600848
48649,97299,0,97299,84.10341000556946,0.010645589108546268
48749,97499,0,97499,84.24881625175476,0.010651101774952721
48849,97699,0,97699,84.40064692497253,0.010620718499309085
48949,97899,0,97899,84.5804979801178,0.010560435742633007
49049,98099,0,98099,84.73319101333618,0.010482869130013147
49149,98299,0,98299,84.87895202636719,0.010401054788361272
49249,98499,0,98499,85.02480506896973,0.010325869901391437
49349,98699,0,98699,85.17633104324341,0.010265694908262776
49449,98899,0,98899,85.37422513961792,0.010225602614748109
49550,99101,0,99101,85.53511023521423,0.01020620653417577
49650,99301,0,99301,85.68829011917114,0.010204166888293783
49750,99501,0,99501,85.83882808685303,0.010212448385454754
49850,99701,0,99701,85.99549317359924,0.010223767292644901
49950,99901,0,99901,86.14860701560974,0.01023315134381706
50050,100101,0,100101,86.2969400882721,0.01023965838689479
50150,100301,0,100301,86.4434220790863,0.010245897124337582
50250,100501,0,100501,86.59995913505554,0.0102555662351311
50350,100701,0,100701,86.87744402885437,0.010269959048277951
50450,100901,0,100901,87.1458191871643,0.010284999262658146
50551,101103,0,101103,87.48881506919861,0.010291051589591968
50651,101303,0,101303,87.79291605949402,0.01027659087278254
50751,101503,0,101503,88.0866551399231,0.01023480071332151
50851,101703,0,101703,88.23417615890503,0.010167629691904736
50951,101903,0,101903,88.38058114051819,0.0100860867665856
51051,102103,0,102103,88.56365323066711,0.010005760880145822
51151,102303,0,102303,88.98539113998413,0.009940416899247642
51251,102503,0,102503,89.1446590423584,0.009897968346366796
51351,102703,0,102703,89.30694913864136,0.009880784933201063
51451,102903,0,102903,89.44793128967285,0.009887725324315061
51552,103105,0,103105,89.59834694862366,0.00991455167040193
51652,103305,0,103305,89.76583814620972,0.009951024181346326
51752,103505,0,103505,89.92786717414856,0.009983209989003157
51852,103705,0,103705,90.07943916320801,0.00999760941779912
51952,103905,0,103905,90.24006819725037,0.00998848165511447
52052,104105,0,104105,90.39767289161682,0.009961374294335296
52152,104305,0,104305,90.5492250919342,0.009928890571215319
52252,104505,0,104505,90.6996910572052,0.009901124981513002
52352,104705,0,104705,90.85251092910767,0.009879044978898627
52452,104905,0,104905,91.00477695465088,0.009856324318212761
52553,105107,0,105107,91.14627003669739,0.009825568869789384
52653,105307,0,105307,91.29486322402954,0.00978360800731093
52753,105507,0,105507,91.45438313484192,0.009729440421860842
52853,105707,0,105707,91.67771911621094,0.009664478072257468
52953,105907,0,105907,91.83799719810486,0.009592877024314298
53053,106107,0,106107,91.98370718955994,0.009522148907906907
53153,106307,0,106307,92.12481713294983,0.00946278976011986
53253,106507,0,106507,92.26522612571716,0.009426889822560437
53353,106707,0,106707,92.40559005737305,0.009424827446281966
53453,106907,0,106907,92.55488896369934,0.009459845694395718
53554,107109,0,107109,92.70233702659607,0.009524071734436873
53654,107309,0,107309,92.84269690513611,0.009595575912943214
53754,107509,0,107509,92.98202705383301,0.009648773823382207
53854,107709,0,107709,93.12073016166687,0.00966251742752922
53954,107909,0,107909,93.26300501823425,0.009630419090533386
54054,108109,0,108109,93.4037492275238,0.009563693057695272
54154,108309,0,108309,93.54596614837646,0.009483979155647585
54254,108509,0,108509,93.6908118724823,0.009410635282507882
54354,108709,0,108709,93.83538889884949,0.00935210956849279
54454,108909,0,108909,93.99134111404419,0.009306820460860834
54555,109111,0,109111,94.14050507545471,0.009269354349423395
54655,109311,0,109311,94.28131818771362,0.009236959099700737
54755,109511,0,109511,94.42026710510254,0.009208311950714225
54855,109711,0,109711,94.56079316139221,0.009183786808967925
54955,109911,0,109911,94.72638607025146,0.009164227725637315
55055,110111,0,110111,94.86954808235168,0.009151307714527001
55155,110311,0,110311,95.0194091796875,0.009147877192018383
55255,110511,0,110511,95.16169500350952,0.009156784724165366
55355,110711,0,110711,95.30157709121704,0.009178363207267122
55455,110911,0,110911,95.46712398529053,0.009208301629163853
55556,111113,0,111113,95.61296892166138,0.009237516304892487
55656,111313,0,111313,95.75923705101013,0.009252978045276868
55756,111513,0,111513,95.90106225013733,0.009244426210345798
55856,111713,0,111713,96.04289722442627,0.009209236598211837
55956,111913,0,111913,96.20088911056519,0.009155936879803036
56056,112113,0,112113,96.34087824821472,0.00910036276871182
56156,112313,0,112313,96.49300813674927,0.00905627739051067
56256,112513,0,112513,96.63718819618225,0.009027588012698609
56356,112713,0,112713,96.78135299682617,0.009008467868996254
56456,112913,0,112913,96.95831298828125,0.008990939247917419
56557,113115,0,113115,97.1017861366272,0.00897307191494729
56657,113315,0,113315,97.24572706222534,0.008961567255446655
56757,113515,0,113515,97.38780212402344,0.008964087249593874
56857,113715,0,113715,97.53205704689026,0.008981373214387795
56957,113915,0,113915,97.67836809158325,0.009004982587349008
57057,114115,0,114115,97.82190895080566,0.009023596090446203
57157,114315,0,114315,97.96859216690063,0.009030677997272776
57257,114515,0,114515,98.10745120048523,0.00902606081505389
57357,114715,0,114715,98.25449919700623,0.009011678856836569
57457,114915,0,114915,98.40290403366089,0.008987408243565491
57558,115117,0,115117,98.54612517356873,0.008950698567701785
57658,115317,0,115317,98.6900360584259,0.008901513371717367
57758,115517,0,115517,98.8302800655365,0.008843691868708401
57858,115717,0,115717,98.97291016578674,0.008787300874448893
57958,115917,0,115917,99.11548805236816,0.008745068261557316
58058,116117,0,116117,99.25880026817322,0.00872525576680209
58158,116317,0,116317,99.39929819107056,0.008725586194653063
58258,116517,0,116517,99.54189014434814,0.008734363785181786
58358,116717,0,116717,99.68600821495056,0.008738940966493323
58458,116917,0,116917,99.82930421829224,0.008734441587370752
58559,117119,0,117119,99.97381520271301,0.008725393227144565
58659,117319,0,117319,100.11510825157166,0.008720062531385192
58759,117519,0,117519,100.25537514686584,0.00872157286200503
58859,117719,0,117719,100.40582919120789,0.00872491736932361
58959,117919,0,117919,100.57234716415405,0.008720594293963635
59059,118119,0,118119,100.71954298019409,0.008701867785545634
59159,118319,0,118319,100.86195206642151,0.008669512051335006
59259,118519,0,118519,101.00460505485535,0.00863048508896663
59359,118719,0,118719,101.1545820236206,0.008592301584589195
59459,118919,0,118919,101.33240127563477,0.008558521245335883
59560,119121,0,119121,101.47482490539551,0.008528771966214132
59660,119321,0,119321,101.62335705757141,0.008503384429111407
59760,119521,0,119521,101.78289103507996,0.008484025713812909
59860,119721,0,119721,101.94649600982666,0.008474257189050627
59960,119921,0,119921,102.08744812011719,0.008476758026289328
60060,120121,0,120121,102.23201298713684,0.008490815631207767
60160,120321,0,120321,102.3889889717102,0.008511155376715106
60260,120521,0,120521,102.54405999183655,0.008529374172908834
60360,120721,0,120721,102.7081651687622,0.008537724882208097
60460,120921,0,120921,102.8507981300354,0.00853254399020506
60561,121123,0,121123,102.99373507499695,0.00851433021707082
60661,121323,0,121323,103.13467001914978,0.008486065531925444
60761,121523,0,121523,103.28152704238892,0.008449692949333034
60861,121723,0,121723,103.44727396965027,0.008406956450118639
60961,121923,0,121923,103.58982610702515,0.0083614277628768
61061,122123,0,122123,103.7577211856842,0.008319547845256866
61161,122323,0,122323,103.92042398452759,0.008288408962766681
61261,122523,0,122523,104.06824707984924,0.008271527603507639
61361,122723,0,122723,104.23179221153259,0.00826638416412064
61461,122923,0,122923,104.37338399887085,0.008266331753568884
61562,123125,0,123125,104.51748704910278,0.008265511865901546
61662,123325,0,123325,104.66318893432617,0.008262712286568545
61762,123525,0,123525,104.86228609085083,0.008260756087398315
61862,123725,0,123725,105.03070998191833,0.008262294661417733
61962,123925,0,123925,105.18324995040894,0.008266099637052719
62062,124125,0,124125,105.33392906188965,0.008267272638301964
62162,124325,0,124325,105.47421312332153,0.00826089646099475
62262,124525,0,124525,105.61354613304138,0.008245615116643429
62362,124725,0,124725,105.75525498390198,0.008224278966411829
62462,124925,0,124925,105.89363312721252,0.008201624594823608
62563,125127,0,125127,106.04903721809387,0.008180915031660676
62663,125327,0,125327,106.20800518989563,0.008163058711323997
62763,125527,0,125527,106.34765219688416,0.00814623918410569
62863,125727,0,125727,106.48971605300903,0.00812920947165199
62963,125927,0,125927,106.63437223434448,0.008112874939602594
63063,126127,0,126127,106.77502202987671,0.008099760384747095
63163,126327,0,126327,106.92199611663818,0.008091448412741137
63263,126527,0,126527,107.07033801078796,0.008086365394416376
63363,126727,0,126727,107.21544909477234,0.008080307328251025
63463,126927,0,126927,107.3528220653534,0.008069571872648073
63564,127129,0,127129,107.49187994003296,0.008053758640169696
63664,127329,0,127329,107.63630795478821,0.008036623961967478
63764,127529,0,127529,107.77641916275024,0.008022374792557277
63864,127729,0,127729,107.91569519042969,0.008012990310244416
63964,127929,0,127929,108.06306409835815,0.008006587873010325
64064,128129,0,128129,108.2859902381897,0.007998614467900619
64164,128329,0,128329,108.50383114814758,0.007984986689291288
64264,128529,0,128529,108.7120041847229,0.007965083016907822
64364,128729,0,128729,108.94732308387756,0.007942251210508275
64464,128929,0,128929,109.21158504486084,0.007921319846192933
64565,129131,0,129131,109.46561098098755,0.00790517071069707
64665,129331,0,129331,109.60762906074524,0.007893996470141731
64765,129531,0,129531,109.77391219139099,0.0078855679918898
64865,129731,0,129731,109.92638325691223,0.007877940753567424
64965,129931,0,129931,110.06837105751038,0.007870245200442775
65065,130131,0,130131,110.20969009399414,0.007862136263003496
65165,130331,0,130331,110.36030316352844,0.007852399863565363
65265,130531,0,130531,110.54855513572693,0.007838165750774492
65365,130731,0,130731,110.77166223526001,0.00781596014649091
65465,130931,0,130931,111.00593996047974,0.007784159899085373
65566,131133,0,131133,111.16241908073425,0.007744350593429415
65666,131333,0,131333,111.31581902503967,0.007702494869741139
65766,131533,0,131533,111.46036195755005,0.0076642115634012
65866,131733,0,131733,111.59970903396606,0.007634133292263829
65966,131933,0,131933,111.75437211990356,0.00761464881873025
66066,132133,0,132133,111.89346814155579,0.0076061646821752255
66166,132333,0,132333,112.03252100944519,0.0076075837361616536
66266,132533,0,132533,112.17054796218872,0.007616217898863698
66366,132733,0,132733,112.32135605812073,0.007627396335077593
66466,132933,0,132933,112.47076511383057,0.0076350440915828365
66567,133135,0,133135,112.61216425895691,0.007633977765829463
66667,133335,0,133335,112.79449605941772,0.007623128130622374
66767,133535,0,133535,112.95047092437744,0.007606894023666675
66867,133735,0,133735,113.09694600105286,0.007593205965884688
66967,133935,0,133935,113.24551820755005,0.00758907453480992
67067,134135,0,134135,113.40265226364136,0.0075958917001781295
67167,134335,0,134335,113.56182193756104,0.007607483716554586
67267,134535,0,134535,113.73854422569275,0.00761254319284104
67367,134735,0,134735,113.94308924674988,0.007600361443620601
67467,134935,0,134935,114.12176012992859,0.007566652591332655
67568,135137,0,135137,114.27624607086182,0.007515807541995842
67668,135337,0,135337,114.50277805328369,0.007461601028295551
67768,135537,0,135537,114.7565062046051,0.007418814901836168
67868,135737,0,135737,114.96268105506897,0.007398877673403144
67968,135937,0,135937,115.13690710067749,0.00740513455417546
68068,136137,0,136137,115.27897500991821,0.0074325876775086204
68168,136337,0,136337,115.4219741821289,0.007470847309105479
68268,136537,0,136537,115.57301092147827,0.00750778890636362
68368,136737,0,136737,115.72384119033813,0.007532518788231393
68468,136937,0,136937,115.86351799964905,0.007537989774433869
68569,137139,0,137139,116.00249195098877,0.00752313888246152
68669,137339,0,137339,116.1657202243805,0.007494472214611841
68769,137539,0,137539,116.38540601730347,0.0074626970259235245
68869,137739,0,137739,116.74959421157837,0.0074382113425732
68969,137939,0,137939,116.98537921905518,0.007426332099352638
69069,138139,0,138139,117.23238825798035,0.007425476043649583
69169,138339,0,138339,117.4655601978302,0.007428757128498165
69269,138539,0,138539,117.79416298866272,0.007427495777043327
69369,138739,0,138739,118.04842710494995,0.007414904313323584
69469,138939,0,138939,118.24085402488708,0.00738895568792465
69570,139141,0,139141,118.5178382396698,0.007353324134874132
69670,139341,0,139341,118.74239897727966,0.007317827002583507
69770,139541,0,139541,118.95288920402527,0.007292448049569305
69870,139741,0,139741,119.12213826179504,0.00728388975285166
69970,139941,0,139941,119.27743911743164,0.007291894165148003
70070,140141,0,140141,119.44599294662476,0.007309365579618959
70170,140341,0,140341,119.67044925689697,0.007325867165009194
70270,140541,0,140541,119.91828203201294,0.0073324455463139
70370,140741,0,140741,120.14241218566895,0.007325255432384266
70470,140941,0,140941,120.33767104148865,0.007306403915929946
70571,141143,0,141143,120.57073402404785,0.007281757626730526
70671,141343,0,141343,120.76987385749817,0.007258551240901788
70771,141543,0,141543,120.93386387825012,0.007240710587261453
70871,141743,0,141743,121.09307503700256,0.007228516381931737
70971,141943,0,141943,121.29829406738281,0.007219200857401336
71071,142143,0,142143,121.46290302276611,0.007209207853257677
71171,142343,0,142343,121.64872598648071,0.007196392067677429
71271,142543,0,142543,121.81073307991028,0.007180900905418578
71371,142743,0,142743,122.00678396224976,0.00716463625909981
71471,142943,0,142943,122.27190923690796,0.007150167142516548
71572,143145,0,143145,122.45473790168762,0.007139746825675723
71672,143345,0,143345,122.62981104850769,0.007134875475122783
71772,143545,0,143545,122.76861429214478,0.007134671017617759
71872,143745,0,143745,122.91107296943665,0.007135628063166644
71972,143945,0,143945,123.08014106750488,0.007132077045638832
72072,144145,0,144145,123.27140522003174,0.0071184648046096624
72172,144345,0,144345,123.42334413528442,0.007092230226602446
72272,144545,0,144545,123.56926417350769,0.007055402962332105
72372,144745,0,144745,123.70916104316711,0.0070138702045031255
72472,144945,0,144945,123.86496806144714,0.006974888150241082
72573,145147,0,145147,124.08456802368164,0.006944148022073128
72673,145347,0,145347,124.29730725288391,0.006925292778891284
72773,145547,0,145547,124.48046207427979,0.006917875978146587
72873,145747,0,145747,124.75988912582397,0.006919561963211549
72973,145947,0,145947,125.06754112243652,0.006926965599666051
73073,146147,0,146147,125.38351321220398,0.006936733904770021
73173,146347,0,146347,125.76097798347473,0.006946345144078973
73273,146547,0,146547,125.97258019447327,0.006954547425440428
73373,146747,0,146747,126.16247391700745,0.006961255811001066
73473,146947,0,146947,126.31272196769714,0.00696679508052837
73574,147149,0,147149,126.54048418998718,0.00697077657708188
73674,147349,0,147349,126.7157518863678,0.006971004105582384
73774,147549,0,147549,126.93682718276978,0.006963651394628524
73874,147749,0,147749,127.11744999885559,0.0069442068536887955
73974,147949,0,147949,127.29579019546509,0.006909742711247745
74074,148149,0,148149,127.59825420379639,0.0068613430043831265
74174,148349,0,148349,128.00805616378784,0.006805258170282584
74274,148549,0,148549,128.23109102249146,0.00675162599098296
74374,148749,0,148749,128.37661814689636,0.006711022148998466
74474,148949,0,148949,128.5159511566162,0.00669064787234138
74575,149151,0,149151,128.6654450893402,0.006692343965437919
74675,149351,0,149351,128.81358408927917,0.006712614874554916
74775,149551,0,149551,128.95344424247742,0.0067446851634746655
74875,149751,0,149751,129.0954451560974,0.0067806812984054395
74975,149951,0,149951,129.2683892250061,0.006813073022738576
75075,150151,0,150151,129.44060492515564,0.006835877313430314
75175,150351,0,150351,129.59692907333374,0.006845770609036277
75275,150551,0,150551,129.7460720539093,0.006842793501541607
75375,150751,0,150751,129.88874125480652,0.0068299854795553306
75475,150951,0,150951,130.02975797653198,0.006811728305502138
75576,151153,0,151153,130.1709361076355,0.006791315190474841
75676,151353,0,151353,130.32760310173035,0.006770255221856824
75776,151553,0,151553,130.46893119812012,0.00674718501745225
75876,151753,0,151753,130.60745906829834,0.006720412141146164
75976,151953,0,151953,130.75515389442444,0.006690027402633916
76076,152153,0,152153,130.9137840270996,0.006659366259155786
76176,152353,0,152353,131.05522894859314,0.006634464509510205
76276,152553,0,152553,131.19356322288513,0.006621461699591522
76376,152753,0,152753,131.33073902130127,0.006623375903892735
76476,152953,0,152953,131.47144198417664,0.006638321068541665
76577,153155,0,153155,131.61313796043396,0.00666050710470802
76677,153355,0,153355,131.7515001296997,0.006681896805822162
76777,153555,0,153555,131.8924651145935,0.006696350528726327
76877,153755,0,153755,132.0319311618805,0.0067001831171035675
76977,153955,0,153955,132.17081594467163,0.0066924951361885116
77077,154155,0,154155,132.30967092514038,0.006674730594359985
77177,154355,0,154355,132.45038318634033,0.006650244157891902
77277,154555,0,154555,132.59141302108765,0.0066237300386648235
77377,154755,0,154755,132.730544090271,0.006599995913297083
77477,154955,0,154955,132.87072014808655,0.0065821179626207645
77578,155157,0,155157,133.0448341369629,0.006569880636599748
77678,155357,0,155357,133.21061396598816,0.006560369900230933
77778,155557,0,155557,133.37216114997864,0.006549412963816596
77878,155757,0,155757,133.51990604400635,0.006534898622649607
77978,155957,0,155957,133.6829969882965,0.006518202396201701
78078,156157,0,156157,133.84064626693726,0.006503346344703308
78178,156357,0,156357,133.99485111236572,0.006494244861374653
78278,156557,0,156557,134.1360080242157,0.006491961995770056
78378,156757,0,156757,134.27922320365906,0.006493896391631224
78478,156957,0,156957,134.4324071407318,0.006495311502869715
78579,157159,0,157159,134.5813980102539,0.00649189128732712
78679,157359,0,157359,134.7434229850769,0.006481890426976725
78779,157559,0,157559,134.97652006149292,0.00646621042431409
78879,157759,0,157759,135.256902217865,0.0064472093923532625
78979,157959,0,157959,135.4624011516571,0.006427151118644978
79079,158159,0,158159,135.63749194145203,0.0064076356386270905
79179,158359,0,158359,135.82163619995117,0.006390338561238534
79279,158559,0,158559,135.99434614181519,0.006378026697386923
79379,158759,0,158759,136.15573906898499,0.006374354040562347
79479,158959,0,158959,136.31371021270752,0.006381987764305939
79580,159161,0,159161,136.4780011177063,0.006400499533560202
79680,159361,0,159361,136.64591526985168,0.006424634250228352
79780,159561,0,159561,136.81982016563416,0.006447108938133697
79880,159761,0,159761,137.00808310508728,0.0064611995446432055
79980,159961,0,159961,137.14967107772827,0.006463676570429448
80080,160161,0,160161,137.29407405853271,0.006455402007098146
80180,160361,0,160361,137.46699595451355,0.006439537500525273
80280,160561,0,160561,137.61000299453735,0.0064189038214628544
80380,160761,0,160761,137.7492139339447,0.006394550365080233
80480,160961,0,160961,137.89409518241882,0.006366412110291381
80581,161163,0,161163,138.04481720924377,0.00633476790961611
80681,161363,0,161363,138.18306708335876,0.006302652844544775
80781,161563,0,161563,138.32081723213196,0.006273379416846458
80881,161763,0,161763,138.45838809013367,0.006250110339511776
80981,161963,0,161963,138.6232590675354,0.00623428296851125
81081,162163,0,162163,138.78533005714417,0.006225767921737579
81181,162363,0,162363,138.94178318977356,0.0062241374766599305
81281,162563,0,162563,139.09579396247864,0.006229648012739131
81381,162763,0,162763,139.23503994941711,0.006242775916315337
81481,162963,0,162963,139.3761990070343,0.006262545435833627
81582,163165,0,163165,139.54012489318848,0.006285415471730391
81682,163365,0,163365,139.69847297668457,0.006304797167929721
81782,163565,0,163565,139.84699606895447,0.006314784332886062
81882,163765,0,163765,140.04001808166504,0.006311769696584767
81982,163965,0,163965,140.20177006721497,0.006295885385802326
82082,164165,0,164165,140.37134790420532,0.006270414604406458
82182,164365,0,164365,140.52130722999573,0.0062401539050176945
82282,164565,0,164565,140.67409205436707,0.006209843169198895
82382,164765,0,164765,140.8453402519226,0.006183248415187983
82482,164965,0,164965,141.07239198684692,0.006162774478480729
82583,165167,0,165167,141.23631620407104,0.006149160457764209
82683,165367,0,165367,141.38991689682007,0.006141860684657694
82783,165567,0,165567,141.52978515625,0.0061385579843668825
82883,165767,0,165767,141.7024929523468,0.006136649170444279
82983,165967,0,165967,141.8738832473755,0.006134281681145008
83083,166167,0,166167,142.02905011177063,0.006131269071756184
83183,166367,0,166367,142.21356797218323,0.006129075679639593
83283,166567,0,166567,142.3719961643219,0.006129684572197447
83383,166767,0,166767,142.52038097381592,0.0061338914443654
83483,166967,0,166967,142.67695903778076,0.006140086056369522
83584,167169,0,167169,142.88066506385803,0.0061444197967707405
83684,167369,0,167369,143.07481026649475,0.006142181329987699
83784,167569,0,167569,143.23552417755127,0.006130154332257758
83884,167769,0,167769,143.39515495300293,0.0061077195472763225
83984,167969,0,167969,143.55051708221436,0.006076980668892908
84084,168169,0,168169,143.7028350830078,0.006041784508410828
84184,168369,0,168369,143.86478424072266,0.006006468607677769
84284,168569,0,168569,144.02810287475586,0.005974995922252405
84384,168769,0,168769,144.1792929172516,0.005950567818914391
84484,168969,0,168969,144.33288598060608,0.0059353837950796755
84585,169171,0,169171,144.48845100402832,0.005930319703752788
84685,169371,0,169371,144.69210124015808,0.005934749306204196
84785,169571,0,169571,145.14393019676208,0.005946302601364465
84885,169771,0,169771,145.33721804618835,0.005961595824236312
84985,169971,0,169971,145.60494017601013,0.005976809021279678
85085,170171,0,170171,145.81905794143677,0.005988450289491664
85185,170371,0,170371,146.0904290676117,0.005994009929550721
85285,170571,0,170571,146.26588106155396,0.005992288842454574
85385,170771,0,170771,146.40731120109558,0.005983319956613796
85485,170971,0,170971,146.55114912986755,0.005968047788046652
85586,171173,0,171173,146.72802305221558,0.0059478151662689565
85686,171373,0,171373,146.876718044281,0.0059250600803017655
85786,171573,0,171573,147.02845001220703,0.005901958853229086
85886,171773,0,171773,147.1973090171814,0.005880965149342974
85986,171973,0,171973,147.38454818725586,0.00586427969826137
86086,172173,0,172173,147.54360604286194,0.0058535228034056865
86186,172373,0,172373,147.68598914146423,0.005849545555644804
86286,172573,0,172573,147.84255695343018,0.005852347583971968
86386,172773,0,172773,148.01929807662964,0.005860998555274079
86486,172973,0,172973,148.25293707847595,0.005873583691386906
86587,173175,0,173175,148.49322509765625,0.005887486514964398
86687,173375,0,173375,148.6401720046997,0.005899302629644569
86787,173575,0,173575,148.78002524375916,0.005906398532051152
86887,173775,0,173775,148.96458506584167,0.005906905322535014
86987,173975,0,173975,149.1176860332489,0.005900095205211705
87087,174175,0,174175,149.26267313957214,0.005886322665121651
87187,174375,0,174375,149.40297603607178,0.005866832461069674
87287,174575,0,174575,149.5926010608673,0.005843543259147396
87387,174775,0,174775,149.73688292503357,0.005818807354050644
87487,174975,0,174975,149.8978669643402,0.005795134065922443
87588,175177,0,175177,150.12226819992065,0.005774751563722394
87688,175377,0,175377,150.394033908844,0.0057602003714983105
87788,175577,0,175577,150.58864903450012,0.005752966287897469
87888,175777,0,175777,150.73771023750305,0.005754167029551253
87988,175977,0,175977,150.87875819206238,0.0057640217618467925
88088,176177,0,176177,151.01744103431702,0.0057815269173186225
88188,176377,0,176377,151.17997908592224,0.005804336891111161
88288,176577,0,176577,151.35213017463684,0.005828980776768374
88388,176777,0,176777,151.50598406791687,0.005851350362460072
88488,176977,0,176977,151.78775095939636,0.005867315913916857
88589,177179,0,177179,152.01539611816406,0.005873408181646214
88689,177379,0,177379,152.2049651145935,0.00586740827161925
88789,177579,0,177579,152.4389510154724,0.005849364703384342
88889,177779,0,177779,152.59921312332153,0.005821421115083074
88989,177979,0,177979,152.92333507537842,0.005787459836572886
89089,178179,0,178179,153.20737504959106,0.005752011836838357
89189,178379,0,178379,153.48292112350464,0.005718976874847321
89289,178579,0,178579,153.75070595741272,0.0056907436376041716
89389,178779,0,178779,153.97585201263428,0.005668112818975281
89489,178979,0,178979,154.20731019973755,0.005650983102685955
89590,179181,0,179181,154.36929202079773,0.005639235496334816
89690,179381,0,179381,154.53982710838318,0.005633765057962033
89790,179581,0,179581,154.72615098953247,0.0056355897122020255
89890,179781,0,179781,154.9044361114502,0.005645426708772222
89990,179981,0,179981,155.08114624023438,0.00566236652004075
90090,180181,0,180181,155.26510906219482,0.005683207262295265
90190,180381,0,180381,155.43416118621826,0.005702830823730916
90290,180581,0,180581,155.63620615005493,0.005715545795336341
90390,180781,0,180781,155.8432161808014,0.005716761601732068
90490,180981,0,180981,156.04499316215515,0.0057042531501076375
90591,181183,0,181183,156.23493814468384,0.005678325070470195
90691,181383,0,181383,156.44260001182556,0.005642756741327904
90791,181583,0,181583,156.7292160987854,0.005602528721144498
90891,181783,0,181783,156.92201900482178,0.005563790593965239
90991,181983,0,181983,157.10352993011475,0.005532504653793147
91091,182183,0,182183,157.3036549091339,0.0055131895395466824
91191,182383,0,182383,157.6586492061615,0.005507874513499617
91291,182583,0,182583,157.8646101951599,0.0055156575671707645
91391,182783,0,182783,158.12575912475586,0.005533086733695801
91491,182983,0,182983,158.32921504974365,0.00555522504307542
91592,183185,0,183185,158.48205709457397,0.005577163947456304
91692,183385,0,183385,158.62151718139648,0.00559424406777221
91792,183585,0,183585,158.7595419883728,0.00560399156664209
91892,183785,0,183785,158.92972207069397,0.005605229242751816
91992,183985,0,183985,159.08741402626038,0.0055980204747261425
92092,184185,0,184185,159.25258111953735,0.0055833057392780695
92192,184385,0,184385,159.4234402179718,0.0055626118043588775
92292,184585,0,184585,159.5635120868683,0.005537850435101692
92392,184785,0,184785,159.7730791568756,0.005511150727121902
92492,184985,0,184985,159.91712617874146,0.005484685936412427
92593,185187,0,185187,160.05698609352112,0.0054602780189395425
92693,185387,0,185387,160.19417119026184,0.005440197267207892
92793,185587,0,185587,160.3327281475067,0.0054255769176267945
92893,185787,0,185787,160.49437999725342,0.005417333941815742
92993,185987,0,185987,160.78686809539795,0.005415787020576368
93093,186187,0,186187,160.99368906021118,0.005420460680598427
93193,186387,0,186387,161.13362407684326,0.0054298802582267965
93293,186587,0,186587,161.28353714942932,0.005441541401328151
93393,186787,0,186787,161.4314272403717,0.005452245605063026
93493,186987,0,186987,161.57231998443604,0.0054588226864056835
93594,187189,0,187189,161.7124810218811,0.005458984020522355
93694,187389,0,187389,161.85217308998108,0.00545207683244265
93794,187589,0,187589,162.00004601478577,0.005439266584452467
93894,187789,0,187789,162.1392891407013,0.005422988570335444
93994,187989,0,187989,162.27852606773376,0.005406109251133636
94094,188189,0,188189,162.41775798797607,0.005391042041647015
94194,188389,0,188389,162.59652996063232,0.005379224946806167
94294,188589,0,188589,162.90755414962769,0.005371072419949242
94394,188789,0,188789,163.12249493598938,0.005366241645813789
94494,188989,0,188989,163.36865997314453,0.005363978531556854
94595,189191,0,189191,163.62149930000305,0.0053634302585765774
94695,189391,0,189391,163.82281494140625,0.005363942159532877
94795,189591,0,189591,163.9790711402893,0.005365289784470807
94895,189791,0,189791,164.14393496513367,0.0053677573027863705
94995,189991,0,189991,164.30167412757874,0.005371757729534558
95095,190191,0,190191,164.4682490825653,0.005377068704725491
95195,190391,0,190391,164.63850712776184,0.005382109528850887
95295,190591,0,190591,164.8021628856659,0.00538391401878397
95395,190791,0,190791,164.9569342136383,0.005379133902557709
95495,190991,0,190991,165.11231589317322,0.00536569300449913
95596,191193,0,191193,165.25974416732788,0.005343916411313316
95696,191393,0,191393,165.4378261566162,0.005317724918407336
95796,191593,0,191593,165.58636212348938,0.005292123112114019
95896,191793,0,191793,165.77669310569763,0.005272013856169165
95996,191993,0,191993,165.94322729110718,0.005260215581759211
96096,192193,0,192193,166.11901807785034,0.005256712561439429
96196,192393,0,192393,166.33648800849915,0.005259182730322118
96296,192593,0,192593,166.50023102760315,0.005264330145209936
96396,192793,0,192793,166.65622305870056,0.005269261276951765
96496,192993,0,192993,166.82237911224365,0.005272343481352476
96597,193195,0,193195,167.02314019203186,0.005273385547420351
96697,193395,0,193395,167.34566712379456,0.0052732479417374085
96797,193595,0,193595,167.56524395942688,0.005273179784124477
96897,193795,0,193795,167.7676990032196,0.005273944186596878
96997,193995,0,193995,167.9272301197052,0.00527515241631857
97097,194195,0,194195,168.0821681022644,0.005275011084452454
97197,194395,0,194395,168.23834609985352,0.005270773753736013
97297,194595,0,194595,168.39846920967102,0.005259911846164433
97397,194795,0,194795,168.54546904563904,0.0052415800118470295
97497,194995,0,194995,168.7054169178009,0.00521761165427835
97598,195197,0,195197,168.86825299263,0.005192118958281517
97698,195397,0,195397,169.0228090286255,0.005171088175595341
97798,195597,0,195597,169.1705961227417,0.005158694724669456
97898,195797,0,195797,169.31563711166382,0.0051567222851413505
97998,195997,0,195997,169.45689511299133,0.005163904989248781
98098,196197,0,196197,169.59504890441895,0.005176779088487519
98198,196397,0,196397,169.75076913833618,0.005191127951658085
98298,196597,0,196597,169.8930959701538,0.005203257664675528
98398,196797,0,196797,170.1253740787506,0.00521072285287811
98498,196997,0,196997,170.42989492416382,0.005212539288863898
98599,197199,0,197199,170.62508487701416,0.005209005424576518
98699,197399,0,197399,170.77376890182495,0.005201539048528845
98799,197599,0,197599,170.91800713539124,0.00519184917138891
98899,197799,0,197799,171.05900692939758,0.005181312289746743
98999,197999,0,197999,171.19666624069214,0.00517041114718528
99099,198199,0,198199,171.34251308441162,0.005158709458079069
99199,198399,0,198399,171.50559425354004,0.005145468263441513
99299,198599,0,198599,171.66608119010925,0.00513058545292794
99399,198799,0,198799,171.8084740638733,0.0051152403326529565
99499,198999,0,198999,171.94865798950195,0.005101733863730263
99600,199201,0,199201,172.10014605522156,0.005092447789663876
99700,199401,0,199401,172.2924690246582,0.005088920921608587
99800,199601,0,199601,172.4439182281494,0.0050905507120880406
99900,199801,0,199801,172.5864770412445,0.005095285694376357
100000,200001,0,200001,172.79732203483582,0.005100546728053584


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha0/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0037419795989990234,30.358099469249375
100,201,200,401,0.6152091026306152,1.725251134601807
200,401,400,801,1.028996229171753,1.0331394156994131
300,601,600,1201,1.2279770374298096,0.7736231354158138
400,801,800,1601,1.394481897354126,0.6349280372139878
501,1003,1002,2005,1.8395888805389404,0.5455617951375803
601,1203,1202,2405,2.2045671939849854,0.482543795209007
701,1403,1402,2805,2.436816930770874,0.43443121283005004
801,1603,1602,3205,2.588085174560547,0.396082748791271
901,1803,1802,3605,2.751868963241577,0.3645989873004372
1001,2003,2002,4005,3.0397660732269287,0.33817775845833975
1101,2203,2202,4405,3.3105008602142334,0.31561971894335344
1201,2403,2402,4805,3.6442410945892334,0.29608763453723413
1301,2603,2602,5205,4.038995981216431,0.2789761387097555
1401,2803,2802,5605,4.247813940048218,0.26383524354104326
1502,3005,3004,6009,4.472510099411011,0.25019483089933037
1602,3205,3204,6409,4.753228187561035,0.23805758726442536
1702,3405,3404,6809,5.428587198257446,0.22707177793944233
1802,3605,3604,7209,6.1581199169158936,0.21706993619439596
1902,3805,3804,7609,6.853977918624878,0.20791616240763086
2002,4005,4004,8009,7.264842987060547,0.19949893614020578
2102,4205,4204,8409,7.922374963760376,0.19172585568559014
2202,4405,4404,8809,8.343006134033203,0.18451971692199934
2302,4605,4604,9209,8.539321184158325,0.17781553946480064
2402,4805,4804,9609,8.701730251312256,0.1715582748285912
2503,5007,5006,10013,8.91798210144043,0.16564432077061936
2603,5207,5206,10413,9.178969860076904,0.16015029105088846
2703,5407,5406,10813,9.39064908027649,0.1549811510589118
2803,5607,5606,11213,9.610925197601318,0.15010700224205265
2903,5807,5806,11613,9.802758932113647,0.14550185344186578
3003,6007,6006,12013,9.96560001373291,0.14114300673996125
3103,6207,6206,12413,10.309340953826904,0.13701055044944
3203,6407,6406,12813,10.62016487121582,0.1330869385687235
3303,6607,6606,13213,11.005867004394531,0.12935664054963755
3403,6807,6806,13613,11.699689149856567,0.12580584861601082
3504,7009,7008,14017,11.944730043411255,0.12238920212160206
3604,7209,7208,14417,12.129282236099243,0.11916321177975675
3704,7409,7408,14817,12.29698896408081,0.11608328196435345
3804,7609,7608,15217,12.449980974197388,0.11314041075772609
3904,7809,7808,15617,12.792578220367432,0.11032642169640298
4004,8009,8008,16017,13.281550884246826,0.10763385857735135
4104,8209,8208,16417,13.531161069869995,0.10505589601363031
4204,8409,8408,16817,13.736955881118774,0.1025862632084499
4304,8609,8608,17217,13.935287237167358,0.10021917884265644
4404,8809,8808,17617,14.59101128578186,0.09794929532145866
4505,9011,9010,18021,15.107478141784668,0.09575032438778178
4605,9211,9210,18421,15.363562107086182,0.09366115602452446
4705,9411,9410,18821,15.621525049209595,0.09165526018334968
4805,9611,9610,19221,15.808576107025146,0.08972860996649396
4905,9811,9810,19621,15.959172248840332,0.08787742990858095
5005,10011,10010,20021,16.144999027252197,0.08609817276901403
5105,10211,10210,20421,16.308143138885498,0.08438749926429683
5205,10411,10410,20821,16.453359127044678,0.0827422603099926
5305,10611,10610,21221,16.64315915107727,0.08115948140902517
5405,10811,10810,21621,16.796471118927002,0.07963634887915819
5506,11013,11012,22025,16.942965030670166,0.07815581524163809
5606,11213,11212,22425,17.1023108959198,0.07674465027683981
5706,11413,11412,22825,17.32118511199951,0.07538551682251976
5806,11613,11612,23225,17.46513795852661,0.07407613635346144
5906,11813,11812,23625,17.635382175445557,0.07281434196761298
6006,12013,12012,24025,17.80742621421814,0.07159807137914267
6106,12213,12212,24425,17.979685068130493,0.07042536057263304
6206,12413,12412,24825,18.182366132736206,0.06929433803403764
6306,12613,12612,25225,18.34694814682007,0.06820321948612608
6406,12813,12812,25625,18.50256109237671,0.06715030306641073
6507,13015,13014,26029,18.724119186401367,0.06612398092841468
6607,13215,13214,26429,18.88314199447632,0.06514301371111987
6707,13415,13414,26829,19.038422107696533,0.06419558041511696
6807,13615,13614,27229,19.20353102684021,0.0632802683993876
6907,13815,13814,27629,19.369935989379883,0.062395728307350413
7007,14015,14014,28029,19.5279700756073,0.06154067100873571
7107,14215,14214,28429,19.70085310935974,0.06071386473424732
7207,14415,14414,28829,20.188430070877075,0.05991413238392325
7307,14615,14614,29229,20.510123014450073,0.059140348992611
7407,14815,14814,29629,20.699604034423828,0.05839143933812523
7508,15017,15016,30033,20.86083197593689,0.05765924210431666
7608,15217,15216,30433,21.08720588684082,0.056957265862180737
7708,15417,15416,30833,21.25450086593628,0.056277204937750555
7808,15617,15616,31233,21.448886156082153,0.055618162011791754
7908,15817,15816,31633,21.624284029006958,0.05497927928204562
8008,16017,16016,32033,21.80279302597046,0.05435973671268472
8108,16217,16216,32433,21.985504150390625,0.05375875036499129
8208,16417,16416,32833,22.23034906387329,0.05317557080411595
8308,16617,16616,33233,22.419522047042847,0.05260948157732764
8408,16817,16816,33633,22.624991178512573,0.05205979775965061
8509,17019,17018,34037,22.838798999786377,0.051520602630384243
8609,17219,17218,34437,23.037046194076538,0.05100194225340503
8709,17419,17418,34837,23.212181091308594,0.05049780221954439
8809,17619,17618,35237,23.375786066055298,0.05000761065391924
8909,17819,17818,35637,23.553126096725464,0.04953082081910589
9009,18019,18018,36037,23.73436188697815,0.0490669099988507
9109,18219,18218,36437,23.980046272277832,0.04861537842924969
9209,18419,18418,36837,24.19733715057373,0.04817574827537324
9309,18619,18618,37237,24.432120084762573,0.04774756265143859
9409,18819,18818,37637,24.64034414291382,0.047330384682744496
9510,19021,19020,38041,24.84428596496582,0.046919782839293905
9610,19221,19220,38441,24.995235204696655,0.04652348509582251
9710,19421,19420,38841,25.165574073791504,0.04613699192550532
9810,19621,19620,39241,25.34954810142517,0.045759938057866614
9910,19821,19820,39641,25.5351402759552,0.04539197410606611
10010,20021,20020,40041,25.735128164291382,0.04503276584703184
10110,20221,20220,40441,25.914966106414795,0.04468199353306405
10210,20421,20420,40841,26.103564023971558,0.044339351233674364
10310,20621,20620,41241,26.24663805961609,0.04400454620646485
10410,20821,20820,41641,26.401906967163086,0.04367729829589823
10511,21023,21022,42045,26.557806253433228,0.043354175700984134
10611,21223,21222,42445,26.75298309326172,0.04304131812212202
10711,21423,21422,42845,26.902826070785522,0.042735244693531745
10811,21623,21622,43245,27.04931902885437,0.042435720216392636
10911,21823,21822,43645,27.215392112731934,0.04214251944861459
11011,22023,22022,44045,27.371469259262085,0.04185542664905385
11111,22223,22222,44445,27.51691198348999,0.04157423514255881
11211,22423,22422,44845,27.661495208740234,0.04129874690496824
11311,22623,22622,45245,27.813106060028076,0.04102877216721476
11411,22823,22822,45645,28.008168935775757,0.04076412903771575
11512,23025,23024,46049,28.279133081436157,0.04050207375577833
11612,23225,23224,46449,28.55593705177307,0.04024762697357275
11712,23425,23424,46849,28.81803607940674,0.03999800830159963
11812,23625,23624,47249,29.09761118888855,0.0397530639846592
11912,23825,23824,47649,29.34407091140747,0.0395126465017495
12012,24025,24024,48049,29.562677145004272,0.039276614282708754
12112,24225,24224,48449,29.81929612159729,0.03904483143818287
12212,24425,24424,48849,30.072418212890625,0.03881716750231484
12312,24625,24624,49249,30.265833139419556,0.038593497187575036
12412,24825,24824,49649,30.415390014648438,0.03837370015117433
12513,25027,25026,50053,30.56013298034668,0.03815551897529549
12613,25227,25226,50453,30.703999996185303,0.037943162063118596
12713,25427,25426,50853,30.847543239593506,0.0377343438492354
12813,25627,25626,51253,31.005712032318115,0.03752896168757155
12913,25827,25826,51653,31.184603929519653,0.03732691686285719
13013,26027,26026,52053,31.44921088218689,0.03712811441614046
13113,26227,26226,52453,31.815949201583862,0.03693246297857628
13213,26427,26426,52853,32.107585191726685,0.03673987461309662
13313,26627,26626,53253,32.28674101829529,0.03655026466358583
13413,26827,26826,53653,32.45838022232056,0.036363551611200175
13514,27029,27028,54057,32.650519132614136,0.036177831965269316
13614,27229,27228,54457,32.82671904563904,0.03599670707644524
13714,27429,27428,54857,32.99233913421631,0.035818251299561545
13814,27629,27628,55257,33.160670042037964,0.035642394384972687
13914,27829,27828,55657,33.32263898849487,0.03546906859650301
14014,28029,28028,56057,33.50303792953491,0.035298208604007716
14114,28229,28228,56457,33.66260313987732,0.03512975138098166
14214,28429,28428,56857,33.80476713180542,0.034963636106970473
14314,28629,28628,57257,33.94815492630005,0.03479980407454928
14414,28829,28828,57657,34.091044902801514,0.034638198600647346
14515,29031,29030,58061,34.342962980270386,0.0344771813926357
14615,29231,29230,58461,34.66441607475281,0.03431988759353739
14715,29431,29430,58861,34.87676501274109,0.034164661121646143
14815,29631,29630,59261,35.043591022491455,0.03401145260098112
14915,29831,29830,59661,35.22201204299927,0.03386021429396292
15015,30031,30030,60061,35.485605001449585,0.03371090003473227
15115,30231,30230,60461,35.73064088821411,0.033563465165527585
15215,30431,30430,60861,35.952505111694336,0.03341786647597316
15315,30631,30630,61261,36.15373492240906,0.033274062145135605
15415,30831,30830,61661,36.43344306945801,0.03313201168621398
15516,31033,31032,62065,36.6370792388916,0.03299028106538275
15616,31233,31232,62465,36.8351628780365,0.032851638543969136
15716,31433,31432,62865,37.080663204193115,0.03271463556051868
15816,31633,31632,63265,37.40368914604187,0.03257923647112261
15916,31833,31832,63665,37.75725221633911,0.032445406724262195
16016,32033,32032,64065,38.15865516662598,0.03231311281884127
16116,32233,32232,64465,38.488017082214355,0.03218232226407853
16216,32433,32432,64865,38.85329794883728,0.032053003541169474
16316,32633,32632,65265,39.061028242111206,0.03192512606663327
16416,32833,32832,65665,39.484559059143066,0.031798660157263375
16517,33035,33034,66069,39.90658903121948,0.03167233305252099
16617,33235,33234,66469,40.254624128341675,0.031548618067915195
16717,33435,33434,66869,40.59261918067932,0.03142623040467131
16817,33635,33634,67269,40.807466983795166,0.031305143667268095
16917,33835,33834,67669,41.002110958099365,0.031185332206444923
17017,34035,34034,68069,41.17033100128174,0.031066771092305608
17117,34235,34234,68469,41.34957695007324,0.030949436088563275
17217,34435,34434,68869,41.519410133361816,0.030833303627871574
17317,34635,34634,69269,41.685863971710205,0.03071835078819308
17417,34835,34834,69669,41.932295083999634,0.030604555270155195
17518,35037,35036,70073,42.11677122116089,0.03049077443936755
17618,35237,35236,70473,42.27711009979248,0.030379240089852988
17718,35437,35436,70873,42.438425064086914,0.030268799484460148
17818,35637,35636,71273,42.68152403831482,0.030159432611547094
17918,35837,35836,71673,43.008729219436646,0.030051119982023665
18018,36037,36036,72073,43.257230281829834,0.029943842611752463
18118,36237,36236,72473,43.41159105300903,0.029837582004660062
18218,36437,36436,72873,43.55804491043091,0.029732320136525433
18318,36637,36636,73273,43.7017879486084,0.029628039439415943
18418,36837,36836,73673,43.85853910446167,0.02952472278674026
18519,37039,37038,74077,44.00399589538574,0.029421334514460707
18619,37239,37238,74477,44.16084408760071,0.029319905494727717
18719,37439,37438,74877,44.32167100906372,0.029219391490043062
18819,37639,37638,75277,44.465888023376465,0.02911977700493755
18919,37839,37838,75677,44.69952321052551,0.0290210469187723
19019,38039,38038,76077,44.908053159713745,0.028923186473965537
19119,38239,38238,76477,45.159136056900024,0.028826181264669258
19219,38439,38438,76877,45.319172859191895,0.028730017225875572
19319,38639,38638,77277,45.68703317642212,0.028634680622934186
19419,38839,38838,77677,45.845000982284546,0.02854015804146322
19520,39041,39040,78081,45.9970281124115,0.028445503162067013
19620,39241,39240,78481,46.141364097595215,0.028352577430754568
19720,39441,39440,78881,46.31768202781677,0.028260427180378078
19820,39641,39640,79281,46.72365212440491,0.028169040186821117
19920,39841,39840,79681,47.10638213157654,0.028078404501042573
20020,40041,40040,80081,47.27374505996704,0.02798850844102124
20120,40241,40240,80481,47.4262490272522,0.027899340583990836
20220,40441,40440,80881,47.5725781917572,0.027810889758952812
20320,40641,40640,81281,47.72615194320679,0.0277231450394556
20420,40841,40840,81681,47.894585847854614,0.027636095736629403
20521,41043,41042,82085,48.04158115386963,0.02754887117325509
20621,41243,41242,82485,48.22660207748413,0.02746318825043482
20721,41443,41442,82885,48.47253894805908,0.027378169938052893
20821,41643,41642,83285,48.65586590766907,0.02729380643475468
20921,41843,41842,83685,48.833433866500854,0.027210088145362795
21021,42043,42042,84085,49.08260798454285,0.027127005675241785
21121,42243,42242,84485,49.2607319355011,0.02704454982485341
21221,42443,42442,84885,49.50607490539551,0.026962711584495463
21321,42643,42642,85285,49.858986139297485,0.02688148212921685
21421,42843,42842,85685,50.1140251159668,0.02680085281390182
21522,43045,43044,86089,50.40891408920288,0.026720017751774044
21622,43245,43244,86489,50.6812949180603,0.026640569269127282
21722,43445,43444,86889,50.86413908004761,0.026561695942841326
21822,43645,43644,87289,51.03327012062073,0.026483389802738927
21922,43845,43844,87689,51.202797174453735,0.026405643036174768
22022,44045,44044,88089,51.3668110370636,0.02632844798400672
22122,44245,44244,88489,51.52278113365173,0.026251797136695613
22222,44445,44444,88889,51.688621044158936,0.0261756831305289
22322,44645,44644,89289,51.860565185546875,0.026100098743962265
22422,44845,44844,89689,52.01291513442993,0.026025036894076908
22523,45047,45046,90093,52.159534215927124,0.025949747751090577
22623,45247,45246,90493,52.30336594581604,0.025875715317000777
22723,45447,45446,90893,52.44973802566528,0.025802184902548382
22823,45647,45646,91293,52.67300510406494,0.025729149947264905
22923,45847,45846,91693,52.82845401763916,0.02565660401313399
23023,46047,46046,92093,53.11584806442261,0.025584540781652128
23123,46247,46246,92493,53.38273215293884,0.02551295405097718
23223,46447,46446,92893,53.53171992301941,0.025441837733162487
23323,46647,46646,93293,53.7332329750061,0.025371185851471904
23423,46847,46846,93693,53.93876791000366,0.025300992537774306
23524,47049,47048,94097,54.08831596374512,0.025230556892376153
23624,47249,47248,94497,54.24022316932678,0.025161267975363354
23724,47449,47448,94897,54.40405988693237,0.025092420593584127
23824,47649,47648,95297,54.57792592048645,0.025024009289734053
23924,47849,47848,95697,54.75172805786133,0.02495602870315468
24024,48049,48048,96097,54.917155265808105,0.024888473567647323
24124,48249,48248,96497,55.09845519065857,0.02482133870934882
24224,48449,48448,96897,55.26069092750549,0.02475461904466623
24324,48649,48648,97297,55.41267013549805,0.024688309578270222
24424,48849,48848,97697,55.56258416175842,0.024622405401142206
24525,49051,49050,98101,55.73962926864624,0.024556248657786196
24625,49251,49250,98501,55.897125005722046,0.024491144601499665
24725,49451,49450,98901,56.04494595527649,0.024426431560359774
24825,49651,49650,99301,56.1893310546875,0.02436210495290391
24925,49851,49850,99701,56.333317041397095,0.024298160274975812
25025,50051,50050,100101,56.48233723640442,0.02423459309807016
25125,50251,50250,100501,56.63387203216553,0.024171399067722248
25225,50451,50450,100901,56.802316188812256,0.024108573901939583
25325,50651,50650,101301,56.94934892654419,0.024046113389674717
25425,50851,50850,101701,57.092865228652954,0.023984013389337876
25526,51053,51052,102105,57.250208139419556,0.02392165417812958
25626,51253,51252,102505,57.431265115737915,0.02386026655180488
25726,51453,51452,102905,57.58782505989075,0.023799227375991334
25826,51653,51652,103305,57.751834869384766,0.023738532773443066
25926,51853,51852,103705,57.90252184867859,0.023678178929477357
26026,52053,52052,104105,58.05001091957092,0.023618162090702013
26126,52253,52252,104505,58.19573211669922,0.023558478563774094
26226,52453,52452,104905,58.33688306808472,0.023499124714190127
26326,52653,52652,105305,58.48480701446533,0.02344009696510563
26426,52853,52852,105705,58.62689805030823,0.023381391796184488
26527,53055,53054,106109,58.77273106575012,0.02332242348188586
26627,53255,53254,106509,58.917301177978516,0.023264356272731823
26727,53455,53454,106909,59.063897132873535,0.023206601377380873
26827,53655,53654,107309,59.20615816116333,0.02314915549108807
26927,53855,53854,107709,59.359869956970215,0.023092015360258213
27027,54055,54054,108109,59.51687407493591,0.023035177781452802
27127,54255,54254,108509,59.658894062042236,0.02297863960041945
27227,54455,54454,108909,59.802566051483154,0.0229223977111454
27327,54655,54654,109309,59.951048135757446,0.02286644905493228
27427,54855,54854,109709,60.10778617858887,0.02281079061949307
27528,55057,55056,110113,60.29968214035034,0.022754867166964565
27628,55257,55256,110513,60.4557671546936,0.02269978314617838
27728,55457,55456,110913,60.59699106216431,0.02264498055048805
27828,55657,55656,111313,60.74193811416626,0.02259045654505676
27928,55857,55856,111713,60.88277792930603,0.02253620833723805
28028,56057,56056,112113,61.02861404418945,0.022482233175790744
28128,56257,56256,112513,61.17051291465759,0.02242852835011063
28228,56457,56456,112913,61.31932711601257,0.022375091189480067
28328,56657,56656,113313,61.46492910385132,0.022321919062333745
28428,56857,56856,113713,61.62556290626526,0.022269009375541767
28529,57059,57058,114117,61.768800020217896,0.022215834379556394
28629,57259,57258,114517,61.969677209854126,0.02216344450540145
28729,57459,57458,114917,62.21535396575928,0.022111309491241765
28829,57659,57658,115317,62.424741983413696,0.022059426891176334
28929,57859,57858,115717,62.682064056396484,0.02200779429437483
29029,58059,58058,116117,62.91287708282471,0.021956409324448933
29129,58259,58258,116517,63.0688898563385,0.021905269638837623
29229,58459,58458,116917,63.27750897407532,0.021854372928205596
29329,58659,58658,117317,63.65252614021301,0.021803716915854494
29429,58859,58858,117717,63.851418018341064,0.021753299357146268
29530,59061,59060,118121,64.0942542552948,0.021702617411362677
29630,59261,59260,118521,64.40037894248962,0.02165267248112565
29730,59461,59460,118921,64.74671006202698,0.021602959436031792
29830,59661,59660,119321,65.03890585899353,0.02155347615445676
29930,59861,59860,119721,65.28599500656128,0.021504220544126505
30030,60061,60060,120121,65.58523917198181,0.021455190541609447
30130,60261,60260,120521,65.9805920124054,0.021406384111819585
30230,60461,60460,120921,66.50212907791138,0.021357799247529348
30330,60661,60660,121321,67.05316615104675,0.02130943396889251
30430,60861,60860,121721,67.57220792770386,0.02126128632297706
30531,61063,61062,122125,68.07628107070923,0.021212876146774994
30631,61263,61262,122525,68.29045009613037,0.02116516014142918
30731,61463,61462,122925,68.5170350074768,0.021117656048338717
30831,61663,61662,123325,68.6888370513916,0.02107036201798955
30931,61863,61862,123725,68.84888505935669,0.021023276225578362
31031,62063,62062,124125,69.01636719703674,0.020976396870598997
31131,62263,62262,124525,69.53290295600891,0.020929722176436568
31231,62463,62462,124925,69.74815392494202,0.02088325038997014
31331,62663,62662,125325,69.90891909599304,0.020836979781182922
31431,62863,62862,125725,70.06239008903503,0.020790908642780062
31532,63065,63064,126129,70.20825004577637,0.020744577549456095
31632,63265,63264,126529,70.38369798660278,0.02069890227185976
31732,63465,63464,126929,70.54967617988586,0.020653421459079477
31832,63665,63664,127329,70.73506999015808,0.020608133491244754
31932,63865,63864,127729,70.91125416755676,0.020563036769401223
32032,64065,64064,128129,71.09860301017761,0.020518129715171387
32132,64265,64264,128529,71.24775719642639,0.02047341077042082
32232,64465,64464,128929,71.41112923622131,0.02042887839693129
32332,64665,64664,129329,71.59334421157837,0.020384531076080074
32432,64865,64864,129729,71.7517409324646,0.020340367308525002
32533,65067,65066,130133,71.91094517707825,0.020295946711456982
32633,65267,65266,130533,72.08745098114014,0.0202521474268461
32733,65467,65466,130933,72.23667907714844,0.020208527295788953
32833,65667,65666,131333,72.45071315765381,0.02016508489321509
32933,65867,65866,131733,72.67786812782288,0.020121818811844584
33033,66067,66066,132133,72.91870903968811,0.020078727661907103
33133,66267,66266,132533,73.06122922897339,0.020035810070866345
33233,66467,66466,132933,73.20446109771729,0.019993064683148747
33333,66667,66666,133333,73.34752917289734,0.019950490159878407
33433,66867,66866,133733,73.50932621955872,0.01990808517861562
33534,67069,67068,134137,73.65241503715515,0.01986542691085773
33634,67269,67268,134537,73.79404616355896,0.019823358773752874
33734,67469,67468,134937,73.9540650844574,0.019781456294749658
33834,67669,67668,135337,74.09579014778137,0.01973971821479264
33934,67869,67868,135737,74.23839116096497,0.01969814329002546
34034,68069,68068,136137,74.40338587760925,0.01965673029155704
34134,68269,68268,136537,74.64577317237854,0.019615478005232466
34234,68469,68468,136937,74.83617305755615,0.01957438523140732
34334,68669,68668,137337,75.01430821418762,0.019533450784726052
34434,68869,68868,137737,75.19437599182129,0.01949267349390492
34535,69071,69070,138141,75.3850929737091,0.019451646772505105
34635,69271,69270,138541,75.57234692573547,0.019411181877591423
34735,69471,69470,138941,75.73530602455139,0.019370870695762887
34835,69671,69670,139341,76.0630931854248,0.019330712110055045
34935,69871,69870,139741,76.54358005523682,0.01929070501654202
35035,70071,70070,140141,77.07055306434631,0.019250848324141225
35135,70271,70270,140541,77.53561615943909,0.019211140954421377
35235,70471,70470,140941,78.10362100601196,0.019171581841413602
35335,70671,70670,141341,78.39099025726318,0.019132169931426305
35435,70871,70870,141741,78.88285303115845,0.019092904182862837
35536,71073,71072,142145,79.32910919189453,0.019053393089335718
35636,71273,71272,142545,79.5004460811615,0.019014418022354724
35736,71473,71472,142945,80.09643411636353,0.018975586052796825
35836,71673,71672,143345,80.63446617126465,0.018936896185798812
35936,71873,71872,143745,81.13734817504883,0.018898347437725855
36036,72073,72072,144145,81.65365409851074,0.018859938836007395
36136,72273,72272,144545,82.12487411499023,0.018821669418975857
36236,72473,72472,144945,82.65082812309265,0.018783538235707962
36336,72673,72672,145345,82.85276818275452,0.018745544345868635
36436,72873,72872,145745,83.01058316230774,0.018707686819558044
36537,73075,73074,146149,83.17037296295166,0.018669588197242667
36637,73275,73274,146549,83.37150406837463,0.018632001990064116
36737,73475,73474,146949,83.59158706665039,0.018594549408885233
36837,73675,73674,147349,83.76536703109741,0.01855722956416187
36937,73875,73874,147749,84.1109709739685,0.01852004157605496
37037,74075,74074,148149,84.52816224098206,0.0184829845742918
37137,74275,74274,148549,84.88972616195679,0.018446057698029945
37237,74475,74474,148949,85.03509306907654,0.01840926009572327
37337,74675,74674,149349,85.1806001663208,0.01837259092499031
37437,74875,74874,149749,85.35110998153687,0.018336049352484656
37538,75077,75076,150153,85.50933623313904,0.01829927104322115
37638,75277,75276,150553,85.87705087661743,0.018262983458128306
37738,75477,75476,150953,86.05156302452087,0.018226821016144038
37838,75677,75676,151353,86.20002794265747,0.018190782918893998
37938,75877,75876,151753,86.36766314506531,0.01815486837642129
38038,76077,76076,152153,86.54233002662659,0.018119076607069226
38138,76277,76276,152553,86.75349521636963,0.018083406837366
38238,76477,76476,152953,86.89756393432617,0.018047858301911218
38338,76677,76676,153353,87.05689001083374,0.018012430243264033
38438,76877,76876,153753,87.20026516914368,0.017977121911833673
38539,77079,77078,154157,87.38330292701721,0.017941581270695787
38639,77279,77278,154557,87.64534401893616,0.017906511354616263
38739,77479,77478,154957,87.89432907104492,0.017871558955778594
38839,77679,77678,155357,88.3599910736084,0.017836723355001523
38939,77879,77878,155757,88.67610311508179,0.017802003840429306
39039,78079,78078,156157,88.99925804138184,0.017767399707431936
39139,78279,78278,156557,89.31689190864563,0.017732910258507373
39239,78479,78478,156957,89.59927725791931,0.01769853480318475
39339,78679,78678,157357,89.76380205154419,0.01766427265792939
39439,78879,78878,157757,89.911141872406,0.017630123146049517
39540,79081,79080,158161,90.08273220062256,0.017595745785285163
39640,79281,79280,158561,90.2271192073822,0.017561820646667444
39740,79481,79480,158961,90.38108491897583,0.017528006144959224
39840,79681,79680,159361,90.53634810447693,0.017494301629998436
39940,79881,79880,159761,90.6774001121521,0.017460706458019143
40040,80081,80080,160161,90.81982803344727,0.017427219991566524
40140,80281,80280,160561,90.97404193878174,0.017393841599413325
40240,80481,80480,160961,91.11889219284058,0.017360570656477215
40340,80681,80680,161361,91.26064491271973,0.017327406543740147
40440,80881,80880,161761,91.40309619903564,0.017294348648168065
40541,81083,81082,162165,91.55879211425781,0.017261067371068674
40641,81283,81282,162565,91.70237803459167,0.017228221141340302
40741,81483,81482,162965,91.86002993583679,0.017195479318873882
40841,81683,81682,163365,92.0263090133667,0.017162841313855037
40941,81883,81882,163765,92.17222309112549,0.017130306542071767
41041,82083,82082,164165,92.3143081665039,0.017097874424841997
41141,82283,82282,164565,92.47436809539795,0.017065544388941797
41241,82483,82482,164965,92.63263487815857,0.01703331586653505
41341,82683,82682,165365,92.84792613983154,0.01700118829510394
41441,82883,82882,165765,93.12865424156189,0.01696916111738057
41542,83085,83084,166169,93.31217789649963,0.016936915010264064
41642,83285,83284,166569,93.47365522384644,0.016905087959018444
41742,83485,83484,166969,93.6231460571289,0.016873359655114786
41842,83685,83684,167369,93.76600813865662,0.016841729561671622
41942,83885,83884,167769,93.90808725357056,0.016810197146730238
42042,84085,84084,168169,94.06002116203308,0.016778761883192207
42142,84285,84284,168569,94.20239400863647,0.016747423248758248
42242,84485,84484,168969,94.34679818153381,0.01671618072586743
42342,84685,84684,169369,94.502934217453,0.016685033801637703
42442,84885,84884,169769,94.65139198303223,0.016653981967807166
42543,85087,85086,170173,94.80828022956848,0.016622715624174927
42643,85287,85286,170573,94.9610800743103,0.016591853402918303
42743,85487,85486,170973,95.10688424110413,0.016561084769496595
42843,85687,85686,171373,95.2484061717987,0.016530409233602147
42943,85887,85886,171773,95.38965511322021,0.01649982630926625
43043,86087,86086,172173,95.54370999336243,0.016469335514805256
43143,86287,86286,172573,95.69015002250671,0.016438936372767995
43243,86487,86486,172973,95.83162713050842,0.016408628409883372
43343,86687,86686,173373,95.98566007614136,0.016378411157009207
43443,86887,86886,173773,96.13035011291504,0.0163482841490817
43544,87089,87088,174177,96.27398204803467,0.016317947004684173
43644,87289,87288,174577,96.41754817962646,0.016287999998496797
43744,87489,87488,174977,96.56966996192932,0.016258141861527946
43844,87689,87688,175377,96.71151494979858,0.01622837214457448
43944,87889,87888,175777,96.8697681427002,0.016198690402268984
44044,88089,88088,176177,97.0287561416626,0.01616909619303347
44144,88289,88288,176577,97.17970705032349,0.016139589079034025
44244,88489,88488,176977,97.34281396865845,0.016110168626135502
44344,88689,88688,177377,97.51295113563538,0.016080834403857398
44444,88889,88888,177777,97.65529298782349,0.016051585985330012
44545,89091,89090,178181,97.8078441619873,0.016022131746618748
44645,89291,89290,178581,97.95734214782715,0.015993054516711416
44745,89491,89490,178981,98.10611009597778,0.015964061827038165
44845,89691,89690,179381,98.24909806251526,0.015935153264782634
44945,89891,89890,179781,98.39956212043762,0.015906328420529737
45045,90091,90090,180181,98.55490803718567,0.015877586888225614
45145,90291,90290,180581,98.701003074646,0.015848928265138035
45245,90491,90490,180981,98.84352898597717,0.015820352151817672
45345,90691,90690,181381,99.0050539970398,0.01579185815205944
45445,90891,90890,181781,99.15490412712097,0.015763445872864972
45546,91093,91092,182185,99.3019630908966,0.01573483202432974
45646,91293,91292,182585,99.45688819885254,0.01570658282740587
45746,91493,91492,182985,99.60717296600342,0.015678414187099022
45846,91693,91692,183385,99.74893498420715,0.015650325722899632
45946,91893,91892,183785,99.89362096786499,0.015622317057323056
46046,92093,92092,184185,100.041983127594,0.015594387815874732
46146,92293,92292,184585,100.18849587440491,0.015566537627016092
46246,92493,92492,184985,100.33146715164185,0.015538766122130529
46346,92693,92692,185385,100.50745606422424,0.01551107293549019
46446,92893,92892,185785,100.65173196792603,0.01548345770422327
46547,93095,93094,186189,100.80931806564331,0.01545564508256718
46647,93295,93294,186589,100.95984601974487,0.015428185455279256
46747,93495,93494,186989,101.10566830635071,0.015400802708031612
46847,93695,93694,187389,101.26279616355896,0.015373496489083502
46947,93895,93894,187789,101.41508793830872,0.015346266449392422
47047,94095,94094,188189,101.56841707229614,0.015319112242583413
47147,94295,94294,188589,101.71161198616028,0.015292033524919778
47247,94495,94494,188989,101.85296702384949,0.015265029955273198
47347,94695,94694,189389,102.00884628295898,0.015238101195095102
47447,94895,94894,189789,102.15328407287598,0.015211246908387922
47548,95097,95096,190193,102.317214012146,0.015184199333494748
47648,95297,95296,190593,102.59435606002808,0.015157493732227002
47748,95497,95496,190993,102.86036419868469,0.015130861608190426
47848,95697,95696,191393,103.0884370803833,0.015104302635337465
47948,95897,95896,191793,103.24170923233032,0.015077816490033957
48048,96097,96096,192193,103.4026050567627,0.015051402851032878
48148,96297,96296,192593,103.55156207084656,0.015025061399448316
48248,96497,96496,192993,103.69479823112488,0.014998791818729911
48348,96697,96696,193393,103.84422516822815,0.014972593794637397
48448,96897,96896,193793,104.00021886825562,0.014946467015215766
48549,97099,97098,194197,104.16743516921997,0.014920150969505643
48649,97299,97298,194597,104.32554721832275,0.014894166457308946
48749,97499,97498,194997,104.46856307983398,0.014868252264343478
48849,97699,97698,195397,104.61175417900085,0.014842408087573906
48949,97899,97898,195797,104.76128220558167,0.014816633626129973
49049,98099,98098,196197,104.92377710342407,0.014790928581283582
49149,98299,98298,196597,105.08374619483948,0.014765292656425929
49249,98499,98498,196997,105.23965287208557,0.014739725557045077
49349,98699,98698,197397,105.39168500900269,0.014714226990703978
49449,98899,98898,197797,105.56291007995605,0.014688796667018477
49550,99101,99100,198201,105.71717715263367,0.014663181016140808
49650,99301,99300,198601,105.89237213134766,0.014637886989959022
49750,99501,99500,199001,106.04707527160645,0.014612660344550686
49850,99701,99700,199401,106.20108199119568,0.014587500797550411
49950,99901,99900,199801,106.38625502586365,0.014562408068540787
50050,100101,100100,200201,106.58542013168335,0.01453738187903176
50150,100301,100300,200601,106.77904915809631,0.014512421952441202
50250,100501,100500,201001,106.95468616485596,0.01448752801407491
50350,100701,100700,201401,107.12670016288757,0.014462699791107488
50450,100901,100900,201801,107.27447199821472,0.014437937012562903
50551,101103,101102,202205,107.42329907417297,0.01441299276149233
50651,101303,101302,202605,107.61627197265625,0.014388360713904908
50751,101503,101502,203005,107.81887602806091,0.014363793306075312
50851,101703,101702,203405,107.99001717567444,0.014339290274256703
50951,101903,101902,203805,108.16236710548401,0.014314851356459529
51051,102103,102102,204205,108.33263897895813,0.0142904762924336
51151,102303,102302,204605,108.51706027984619,0.01426616482365087
51251,102503,102502,205005,108.6861560344696,0.014241916693287952
51351,102703,102702,205405,108.8735408782959,0.014217731646209248
51451,102903,102902,205805,109.022625207901,0.014193609428949962
51552,103105,103104,206209,109.16737103462219,0.014169309508478186
51652,103305,103304,206609,109.32016324996948,0.014145312819084519
51752,103505,103504,207009,109.47689604759216,0.014121378206498671
51852,103705,103704,207409,109.62915420532227,0.014097505423791156
51952,103905,103904,207809,109.81001496315002,0.014073694225622347
52052,104105,104104,208209,109.99552607536316,0.01404994436822647
52152,104305,104304,208609,110.16992712020874,0.014026255609396686
52252,104505,104504,209009,110.3243670463562,0.014002627708469512
52352,104705,104704,209409,110.48928117752075,0.013979060426309933
52452,104905,104904,209809,110.65836906433105,0.013955553525296671
52553,105107,105106,210213,110.82561588287354,0.013931872604684651
52653,105307,105306,210613,110.98361396789551,0.013908486357005244
52753,105507,105506,211013,111.1397168636322,0.013885159784220062
52853,105707,105706,211413,111.29452919960022,0.013861892654632132
52953,105907,105906,211813,111.44832420349121,0.013838684737986525
53053,106107,106106,212213,111.59619402885437,0.013815535805456691
53153,106307,106306,212613,111.77924513816833,0.013792445629630744
53253,106507,106506,213013,111.93545413017273,0.013769413984498097
53353,106707,106706,213413,112.11761689186096,0.013746440645436255
53453,106907,106906,213813,112.2702898979187,0.013723525389197551
53554,107109,107108,214217,112.421875,0.013700439711393808
53654,107309,107308,214617,112.5767571926117,0.01367764053178866
53754,107509,107508,215017,112.73654413223267,0.013654898771199535
53854,107709,107708,215417,112.88861227035522,0.013632214211764027
53954,107909,107908,215817,113.04025101661682,0.01360958663693127
54054,108109,108108,216217,113.18748712539673,0.013587015831450056
54154,108309,108308,216617,113.35040807723999,0.013564501581356529
54254,108509,108508,217017,113.56490206718445,0.01354204367396259
54354,108709,108708,217417,113.76403522491455,0.013519641897843921
54454,108909,108908,217817,113.91616415977478,0.013497296042828549
54555,109111,109110,218221,114.08128428459167,0.013474783279199671
54655,109311,109310,218621,114.27163028717041,0.01345254919482705
54755,109511,109510,219021,114.42909693717957,0.01343037040638306
54855,109711,109710,219421,114.57777214050293,0.013408246708603739
54955,109911,109910,219821,114.72149729728699,0.013386177897421475
55055,110111,110110,220221,114.88675904273987,0.013364163769954158
55155,110311,110310,220621,115.07847309112549,0.013342204124494349
55255,110511,110510,221021,115.24696516990662,0.013320298760499127
55355,110711,110710,221421,115.50527501106262,0.013298447478579412
55455,110911,110910,221821,115.78613519668579,0.013276650080489637
55556,111113,111112,222225,115.99187016487122,0.013254689202457986
55656,111313,111312,222625,116.20966625213623,0.013232999515736827
55756,111513,111512,223025,116.40398597717285,0.013211363122926699
55856,111713,111712,223425,116.58046913146973,0.013189779830267258
55956,111913,111912,223825,116.73071217536926,0.013168249445091837
56056,112113,112112,224225,116.88145589828491,0.01314677177581818
56156,112313,112312,224625,117.03979396820068,0.01312534663193894
56256,112513,112512,225025,117.19827318191528,0.013103973824012185
56356,112713,112712,225425,117.34875512123108,0.013082653163652267
56456,112913,112912,225825,117.4949860572815,0.013061384463520571
56557,113115,113114,226229,117.64878797531128,0.013039955628885188
56657,113315,113314,226629,117.79775309562683,0.013018790806291975
56757,113515,113514,227029,118.00857210159302,0.01299767738626663
56857,113715,113714,227429,118.1763710975647,0.012976615185579705
56957,113915,113914,227829,118.3353979587555,0.012955604022004623
57057,114115,114114,228229,118.50096607208252,0.01293464371430911
57157,114315,114314,228629,118.6631350517273,0.012913734082246801
57257,114515,114514,229029,118.81338405609131,0.012892874946548923
57357,114715,114714,229429,118.96398711204529,0.012872066128916037
57457,114915,114914,229829,119.24495220184326,0.012851307452009776
57558,115117,115116,230233,119.50359416007996,0.012830391904044983
57658,115317,115316,230633,119.7720410823822,0.012809733477388006
57758,115517,115516,231033,119.96573209762573,0.012789124663389556
57858,115717,115716,231433,120.11379218101501,0.012768565288485622
57958,115917,115916,231833,120.31945204734802,0.012748055180034057
58058,116117,116116,232233,120.65886807441711,0.012727594166306812
58158,116317,116316,232633,120.96442914009094,0.012707182076482379
58258,116517,116516,233033,121.26995897293091,0.012686818740638432
58358,116717,116716,233433,121.64639329910278,0.012666503989744518
58458,116917,116916,233833,121.95921587944031,0.012646237655654704
58559,117119,117118,234237,122.21729707717896,0.01262581763335122
58659,117319,117318,234637,122.47918105125427,0.012605648111927934
58759,117519,117518,235037,122.64190697669983,0.01258552650645551
58859,117719,117718,235437,122.80093812942505,0.012565452652263543
58959,117919,117918,235837,122.98144006729126,0.01254542638553089
59059,118119,118118,236237,123.15365314483643,0.012525447543278976
59159,118319,118318,236637,123.43775391578674,0.012505515963364805
59259,118519,118518,237037,123.7783100605011,0.012485631484474713
59359,118719,118718,237437,123.95969796180725,0.012465793946117406
59459,118919,118918,237837,124.11163020133972,0.012446003188617685
59560,119121,119120,238241,124.29236698150635,0.012426061846660291
59660,119321,119320,238641,124.6114718914032,0.01240636463892564
59760,119521,119520,239041,124.85502815246582,0.012386713736286269
59860,119721,119720,239441,125.11234307289124,0.01236710898227509
59960,119921,119920,239841,125.26479911804199,0.012347550221209671
60060,120121,120120,240241,125.4175751209259,0.01232803729818582
60160,120321,120320,240641,125.57542109489441,0.012308570059071607
60260,120521,120520,241041,125.72115993499756,0.012289148350501572
60360,120721,120720,241441,125.86584806442261,0.01226977201987071
60460,120921,120920,241841,126.03351998329163,0.012250440915328632
60561,121123,121122,242245,126.18785309791565,0.012230962252597479
60661,121323,121322,242645,126.48192501068115,0.01221172159616075
60761,121523,121522,243045,126.72979211807251,0.012192525713239316
60861,121723,121722,243445,126.9634461402893,0.012173374454951404
60961,121923,121922,243845,127.12130522727966,0.01215426767314145
61061,122123,122122,244245,127.28732490539551,0.012135205220374895
61161,122323,122322,244645,127.44957113265991,0.012116186949932379
61261,122523,122522,245045,127.60030698776245,0.012097212715804754
61361,122723,122722,245445,127.74444603919983,0.012078282372687483
61461,122923,122922,245845,127.8941900730133,0.01205939577597569
61562,123125,123124,246249,128.0493130683899,0.012040364571523868
61662,123325,123324,246649,128.1929440498352,0.0120215654704518
61762,123525,123524,247049,128.33728313446045,0.012002809684693572
61862,123725,123724,247449,128.48845911026,0.011984097072397587
61962,123925,123924,247849,128.63121509552002,0.011965427492386235
62062,124125,124124,248249,128.776141166687,0.011946800804150993
62162,124325,124324,248649,128.91982126235962,0.011928216867847589
62262,124525,124524,249049,129.0771882534027,0.011909675544291117
62362,124725,124724,249449,129.222088098526,0.011891176694951261
62462,124925,124924,249849,129.3884072303772,0.011872720181947644
62563,125127,125126,250253,129.54953908920288,0.011854121937548822
62663,125327,125326,250653,129.69741296768188,0.011835750106090122
62763,125527,125526,251053,129.8459882736206,0.011817420199822857
62863,125727,125726,251453,130.00257325172424,0.011799132083426103
62963,125927,125926,251853,130.15118408203125,0.011780885622206022
63063,126127,126126,252253,130.29499006271362,0.011762680682091079
63163,126327,126326,252653,130.4551088809967,0.011744517129627865
63263,126527,126526,253053,130.60659098625183,0.011726394831976827
63363,126727,126726,253453,130.7664670944214,0.011708313656907696
63463,126927,126926,253853,130.91522312164307,0.011690273472795353
63564,127129,127128,254257,131.0723741054535,0.011672094361274773
63664,127329,127328,254657,131.218111038208,0.011654136173238737
63764,127529,127528,255057,131.36804008483887,0.011636218583577785
63864,127729,127728,255457,131.5419900417328,0.011618341463051452
63964,127929,127928,255857,131.68955087661743,0.011600504683003719
64064,128129,128128,256257,131.8347852230072,0.011582708115358976
64164,128329,128328,256657,132.01572728157043,0.011564951632618016
64264,128529,128528,257057,132.1861870288849,0.011547235107853984
64364,128729,128728,257457,132.3585970401764,0.011529558414708816
64464,128929,128928,257857,132.52499413490295,0.011511921427388995
64565,129131,129130,258261,132.6794571876526,0.011494148246054431
64665,129331,129330,258661,132.83634901046753,0.011476590689176235
64765,129531,129530,259061,133.00986194610596,0.011459072462854887
64865,129731,129730,259461,133.17453408241272,0.011441593443523404
64965,129931,129930,259861,133.32009601593018,0.011424153508160761
65065,130131,130130,260261,133.47564816474915,0.011406752534288241
65165,130331,130330,260661,133.65278911590576,0.011389390399965822
65265,130531,130530,261061,133.8568992614746,0.011372066983788637
65365,130731,130730,261461,134.02431321144104,0.011354782164883313
65465,130931,130930,261861,134.16691899299622,0.011337535822904688
65566,131133,131132,262265,134.3136022090912,0.011320155951482764
65666,131333,131332,262665,134.49438405036926,0.011302986586194321
65766,131533,131532,263065,134.65001606941223,0.011285855338745761
65866,131733,131732,263465,134.80033493041992,0.011268762090875073
65966,131933,131932,263865,134.96050810813904,0.011251706724831254
66066,132133,132132,264265,135.11840105056763,0.011234689123371028
66166,132333,132332,264665,135.26413226127625,0.011217709169755707
66266,132533,132532,265065,135.41616487503052,0.011200766747747691
66366,132733,132732,265465,135.57280898094177,0.011183861741607555
66466,132933,132932,265865,135.72316193580627,0.011166994036090673
66567,133135,133134,266269,135.88150310516357,0.011149995398649155
66667,133335,133334,266669,136.03799510002136,0.01113320232074906
66767,133535,133534,267069,136.1811981201172,0.011116446199540608
66867,133735,133734,267469,136.3254039287567,0.011099726921732184
66967,133935,133934,267869,136.48156595230103,0.011083044374511446
67067,134135,134134,268269,136.62792825698853,0.011066398445542447
67167,134335,134334,268669,136.7719430923462,0.011049789022962631
67267,134535,134534,269069,136.918062210083,0.011033215995379778
67367,134735,134734,269469,137.07875108718872,0.011016679251869298
67467,134935,134934,269869,137.22458291053772,0.0110001786819711
67568,135137,135136,270273,137.3695409297943,0.010983549712374231
67668,135337,135336,270673,137.5224289894104,0.010967121519153593
67768,135537,135536,271073,137.66208410263062,0.010950729169835593
67868,135737,135736,271473,137.80469727516174,0.010934372555794594
67968,135937,135936,271873,137.97744703292847,0.010918051568855542
68068,136137,136136,272273,138.12958312034607,0.010901766101291118
68168,136337,136336,272673,138.27915906906128,0.01088551604581895
68268,136537,136536,273073,138.42954015731812,0.010869301295599118
68368,136737,136736,273473,138.58255815505981,0.010853121744231246
68468,136937,136936,273873,138.7266550064087,0.010836977285752086
68569,137139,137138,274277,138.8749189376831,0.010820706896251716
68669,137339,137338,274677,139.0323941707611,0.010804632655688488
68769,137539,137538,275077,139.17353296279907,0.010788593191675569
68869,137739,137738,275477,139.31937217712402,0.010772588399976161
68969,137939,137938,275877,139.4695701599121,0.010756618176777446
69069,138139,138138,276277,139.61473202705383,0.01074068241868826
69169,138339,138338,276677,139.75825595855713,0.010724781022736616
69269,138539,138538,277077,139.90133094787598,0.010708913886367213
69369,138739,138738,277477,140.06246614456177,0.010693080907438939
69469,138939,138938,277877,140.2162902355194,0.010677281984222546
69570,139141,139140,278281,140.35920906066895,0.0106613595368379
69670,139341,139340,278681,140.51527905464172,0.010645628759519424
69770,139541,139540,279081,140.65612125396729,0.010629931734169071
69870,139741,139740,279481,140.8010129928589,0.010614268360685181
69970,139941,139940,279881,140.95333099365234,0.01059863853936608
70070,140141,140140,280281,141.10060715675354,0.010583042170907768
70170,140341,140340,280681,141.24358987808228,0.010567479156401759
70270,140541,140540,281081,141.38744807243347,0.010551949397332722
70370,140741,140740,281481,141.53786206245422,0.01053645279557633
70470,140941,140940,281881,141.682391166687,0.01052098925339699
70571,141143,141142,282285,141.83826994895935,0.010505404533777012
70671,141343,141342,282685,141.99474120140076,0.010490007147253242
70771,141543,141542,283085,142.14342713356018,0.010474642528446447
70871,141743,141742,283485,142.4555220603943,0.010459310581157993
70971,141943,141942,283885,142.68545794487,0.010444011209567077
71071,142143,142142,284285,142.9405481815338,0.010428744318228945
71171,142343,142342,284685,143.27153205871582,0.01041350981207237
71271,142543,142542,285085,143.48938822746277,0.010398307596397902
71371,142743,142742,285485,143.64665293693542,0.010383137576875551
71471,142943,142942,285885,143.80594325065613,0.010367999659543051
71572,143145,143144,286289,143.98992323875427,0.010352742853043743
71672,143345,143344,286689,144.1526279449463,0.010337669178347931
71772,143545,143544,287089,144.36156010627747,0.010322627325213274
71872,143745,143744,287489,144.53836798667908,0.010307617201131205
71972,143945,143944,287889,144.70294904708862,0.010292638713950824
72072,144145,144144,288289,144.85395097732544,0.01027769177187676
72172,144345,144344,288689,145.04456210136414,0.010262776283467645
72272,144545,144544,289089,145.33063411712646,0.010247892157633672
72372,144745,144744,289489,145.58928894996643,0.010233039303635262
72472,144945,144944,289889,145.87668704986572,0.01021821763108069
72573,145147,145146,290293,146.0500020980835,0.010203279300820748
72673,145347,145346,290693,146.25933003425598,0.010188520030927118
72773,145547,145546,291093,146.4031891822815,0.010173791672480472
72873,145747,145746,291493,146.59773230552673,0.010159094136466484
72973,145947,145946,291893,146.75331211090088,0.010144427334209621
73073,146147,146146,292293,146.899884223938,0.01012979117737153
73173,146347,146346,292693,147.05008506774902,0.010115185577949172
73273,146547,146546,293093,147.1917760372162,0.01010061044827318
73373,146747,146746,293493,147.36380195617676,0.010086065701005903
73473,146947,146946,293893,147.57088208198547,0.010071551249139847
73574,147149,147148,294297,147.72860193252563,0.01005692231582622
73674,147349,147348,294697,147.87789297103882,0.010042468495840836
73774,147549,147548,295097,148.02761721611023,0.010028044711339279
73874,147749,147748,295497,148.20240712165833,0.010013650876620636
73974,147949,147948,295897,148.39412999153137,0.009999286906305714
74074,148149,148148,296297,148.5553171634674,0.00998495271533535
74174,148349,148348,296697,148.73381519317627,0.009970648218968625
74274,148549,148548,297097,148.91385197639465,0.0099563733327815
74374,148749,148748,297497,149.07170796394348,0.009942127972664876
74474,148949,148948,297897,149.22628712654114,0.00992791205482332
74575,149151,149150,298301,149.37991619110107,0.009913583778163
74675,149351,149350,298701,149.53367614746094,0.009899426787068365
74775,149551,149550,299101,149.68820905685425,0.009885298987900538
74875,149751,149750,299501,149.8557960987091,0.009871200298105322
74975,149951,149950,299901,150.0155210494995,0.009857130635434221
75075,150151,150150,300301,150.17052912712097,0.009843089917942964
75175,150351,150350,300701,150.32769012451172,0.00982907806398986
75275,150551,150550,301101,150.48357105255127,0.00981509499223439
75375,150751,150750,301501,150.6338050365448,0.009801140621635535
75475,150951,150950,301901,150.78635811805725,0.009787214871450541
75576,151153,151152,302305,150.9700312614441,0.009773178832986541
75676,151353,151352,302705,151.1271140575409,0.009759310366780592
75776,151553,151552,303105,151.27773022651672,0.009745470279737227
75876,151753,151752,303505,151.44417691230774,0.009731658492294576
75976,151953,151952,303905,151.6123149394989,0.0097178749251816
76076,152153,152152,304305,151.78411412239075,0.009704119499416724
76176,152353,152352,304705,151.95632791519165,0.009690392136306415
76276,152553,152552,305105,152.14277505874634,0.009676692757443756
76376,152753,152752,305505,152.3011589050293,0.00966302128470716
76476,152953,152952,305905,152.45644187927246,0.009649377640258878
76577,153155,153154,306309,152.63556790351868,0.009635625727486065
76677,153355,153354,306709,152.82549214363098,0.009622037783575196
76777,153555,153554,307109,153.00554299354553,0.009608477435360597
76877,153755,153754,307509,153.26513695716858,0.009594944606129162
76977,153955,153954,307909,153.42644786834717,0.009581439219445069
77077,154155,154154,308309,153.58292508125305,0.009567961199148232
77177,154355,154354,308709,153.74885511398315,0.009554510469353053
77277,154555,154554,309109,153.90931797027588,0.009541086954447145
77377,154755,154754,309509,154.08810091018677,0.00952769057909001
77477,154955,154954,309909,154.25027704238892,0.009514321268211777
77578,155157,155156,310313,154.40946006774902,0.009500845659845384
77678,155357,155356,310713,154.57356023788452,0.00948753052256744
77778,155557,155556,311113,154.7304892539978,0.009474242225428524
77878,155757,155756,311513,154.890310049057,0.009460980694431215
77978,155957,155956,311913,155.05088901519775,0.009447745855842505
78078,156157,156156,312313,155.2399299144745,0.009434537636192349
78178,156357,156356,312713,155.40805411338806,0.009421355962272702
78278,156557,156556,313113,155.581768989563,0.00940820076113614
78378,156757,156756,313513,155.75302815437317,0.00939507196009464
78478,156957,156956,313913,155.92951917648315,0.00938196948671854
78579,157159,157158,314317,156.10309314727783,0.009368762639003063
78679,157359,157358,314717,156.26134204864502,0.009355712866169126
78779,157559,157558,315117,156.41201305389404,0.009342689204533832
78879,157759,157758,315517,156.56671500205994,0.009329691582691197
78979,157959,157958,315917,156.72293901443481,0.00931671992948766
79079,158159,158158,316317,156.87489414215088,0.009303774174020951
79179,158359,158358,316717,157.0335350036621,0.009290854245638795
79279,158559,158558,317117,157.20528507232666,0.009277960073937962
79379,158759,158758,317517,157.42616605758667,0.00926509158876296
79479,158959,158958,317917,157.58858919143677,0.009252248720205199
79580,159161,159160,318321,157.7458300590515,0.009239303354162473
79680,159361,159360,318721,157.90259408950806,0.009226511764519909
79780,159561,159560,319121,158.05861520767212,0.009213745582547072
79880,159761,159760,319521,158.2119472026825,0.009201004739313621
79980,159961,159960,319921,158.36032485961914,0.009188289166130226
80080,160161,160160,320321,158.51122999191284,0.009175598794547902
80180,160361,160360,320721,158.65854907035828,0.009162933556356601
80280,160561,160560,321121,158.80921006202698,0.0091502933835844
80380,160761,160760,321521,158.96527910232544,0.009137678208496288
80480,160961,160960,321921,159.15781712532043,0.009125087963593204
80581,161163,161162,322325,159.3828649520874,0.009112397053121802
80681,161363,161362,322725,159.54592108726501,0.00909985671465115
80781,161563,161562,323125,159.7837221622467,0.009087341104606664
80881,161763,161762,323525,159.95104813575745,0.009074850156424858
80981,161963,161962,323925,160.10062503814697,0.00906238380377307
81081,162163,162162,324325,160.30363011360168,0.009049941980548438
81181,162363,162362,324725,160.49111413955688,0.00903752462087687
81281,162563,162562,325125,160.64197516441345,0.00902513165911197
81381,162763,162762,325525,160.87697410583496,0.009012763029834198
81481,162963,162962,325925,161.030091047287,0.009000418667849718
81582,163165,163164,326329,161.18191504478455,0.008987975428595498
81682,163365,163364,326729,161.36017894744873,0.008975679647564273
81782,163565,163564,327129,161.51563119888306,0.008963407938945957
81882,163765,163764,327529,161.72941207885742,0.008951160238442469
81982,163965,163964,327929,161.90333819389343,0.008938936481976746
82082,164165,164164,328329,162.05979299545288,0.008926736605691652
82182,164365,164364,328729,162.21217894554138,0.00891456054594913
82282,164565,164564,329129,162.36691999435425,0.008902408239329317
82382,164765,164764,329529,162.52047324180603,0.008890279622629579
82482,164965,164964,329929,162.67273092269897,0.008878174632863426
82583,165167,165166,330333,162.82637810707092,0.008865972511791073
82683,165367,165366,330733,162.98238706588745,0.008853914822494502
82783,165567,165566,331133,163.13390016555786,0.00884188057183861
82883,165767,165766,331533,163.2909390926361,0.00882986969769517
82983,165967,165966,331933,163.4484622478485,0.008817882138147685
83083,166167,166166,332333,163.60275793075562,0.008805917831490507
83183,166367,166366,332733,163.75610613822937,0.008793976716227883
83283,166567,166566,333133,163.93417501449585,0.008782058731073293
83383,166767,166766,333533,164.09458899497986,0.008770163814948245
83483,166967,166966,333933,164.24871110916138,0.008758291906981772
83584,167169,167168,334337,164.40531301498413,0.008746324572584651
83684,167369,167368,334737,164.565171957016,0.008734498727712887
83784,167569,167568,335137,164.72057604789734,0.008722695709020326
83884,167769,167768,335537,164.87491416931152,0.008710915456458839
83984,167969,167968,335937,165.03441214561462,0.008699157910183178
84084,168169,168168,336337,165.19156217575073,0.008687423010550298
84184,168369,168368,336737,165.34525799751282,0.008675710698118596
84284,168569,168568,337137,165.50127696990967,0.008664020913647038
84384,168769,168768,337537,165.6563651561737,0.008652353598094296
84484,168969,168968,337937,165.8108720779419,0.008640708692617936
84585,169171,169170,338341,165.9781529903412,0.008628970025709922
84685,169371,169370,338741,166.14727807044983,0.008617369987285886
84785,169571,169570,339141,166.30411291122437,0.008605792183014695
84885,169771,169770,339541,166.4706370830536,0.008594236554843345
84985,169971,169970,339941,166.65434193611145,0.008582703044913742
85085,170171,170170,340341,166.80891609191895,0.008571191595561807
85185,170371,170370,340741,166.96645212173462,0.008559702149316813
85285,170571,170570,341141,167.12177205085754,0.008548234648900484
85385,170771,170770,341541,167.2692370414734,0.008536789037226163
85485,170971,170970,341941,167.41848611831665,0.00852536525739832
85586,171173,171172,342345,167.57306599617004,0.008513849342437672
85686,171373,171372,342745,167.7216169834137,0.008502469273277233
85786,171573,171572,343145,167.88717699050903,0.00849111086585197
85886,171773,171772,343545,168.08141207695007,0.008479774064024255
85986,171973,171972,343945,168.2426450252533,0.008468458811843493
86086,172173,172172,344345,168.39245223999023,0.008457165053545518
86186,172373,172372,344745,168.53993916511536,0.00844589273355175
86286,172573,172572,345145,168.68741011619568,0.008434641796468531
86386,172773,172772,345545,168.83306908607483,0.008423412187086277
86486,172973,172972,345945,168.9887990951538,0.008412203850378878
86587,173175,173174,346349,169.13994097709656,0.008400904967279037
86687,173375,173374,346749,169.29013299942017,0.008389739222929127
86787,173575,173574,347149,169.4428551197052,0.008378594586724877
86887,173775,173774,347549,169.58894300460815,0.008367471004368328
86987,173975,173974,347949,169.7364900112152,0.008356368421741254
87087,174175,174174,348349,169.94163012504578,0.008345286784904541
87187,174375,174374,348749,170.11531925201416,0.008334226040097426
87287,174575,174574,349149,170.26015329360962,0.00832318613373682
87387,174775,174774,349549,170.42459201812744,0.008312167012416565
87487,174975,174974,349949,170.57164025306702,0.008301168622906842
87588,175177,175176,350353,170.71737098693848,0.008290081239294492
87688,175377,175376,350753,170.8599500656128,0.008279124360410202
87788,175577,175576,351153,171.00911712646484,0.008268188054171297
87888,175777,175776,351553,171.1566641330719,0.008257272268047962
87988,175977,175976,351953,171.30464506149292,0.008246376949683042
88088,176177,176176,352353,171.45591521263123,0.008235502046891623
88188,176377,176376,352753,171.59975624084473,0.008224647507660221
88288,176577,176576,353153,171.7439420223236,0.008213813280146202
88388,176777,176776,353553,171.88652920722961,0.00820299931267709
88488,176977,176976,353953,172.03851127624512,0.008192205553749962
88589,177179,177178,354357,172.19757294654846,0.008181324317634046
88689,177379,177378,354757,172.35441994667053,0.008170571022759168
88789,177579,177578,355157,172.51506996154785,0.008159837782418624
88889,177779,177778,355557,172.66641998291016,0.008149124545782496
88989,177979,177978,355957,172.8135540485382,0.008138431262187258
89089,178179,178178,356357,172.96719312667847,0.008127757881134784
89189,178379,178378,356757,173.11011505126953,0.00811710435229215
89289,178579,178578,357157,173.25433707237244,0.008106470625490499
89389,178779,178778,357557,173.3990399837494,0.00809585665072483
89489,178979,178978,357957,173.54697108268738,0.008085262378153189
89590,179181,179180,358361,173.69195914268494,0.008074582110972974
89690,179381,179380,358761,173.8388590812683,0.008064027289693009
89790,179581,179580,359161,173.98827505111694,0.008053492021560556
89890,179781,179780,359561,174.13548398017883,0.008042976257381264
89990,179981,179980,359961,174.2803270816803,0.00803247994812076
90090,180181,180180,360361,174.42828106880188,0.008022003044904101
90190,180381,180380,360761,174.5755331516266,0.008011545499014991
90290,180581,180580,361161,174.7397861480713,0.008001107261895308
90390,180781,180780,361561,174.88754606246948,0.007990688285144496
90490,180981,180980,361961,175.03902316093445,0.007980288520518969
90591,181183,181182,362365,175.18570709228516,0.007969804210541661
90691,181383,181382,362765,175.33200597763062,0.007959442916980157
90791,181583,181582,363165,175.48022890090942,0.00794910069127186
90891,181783,181782,363565,175.62655401229858,0.007938777485796538
90991,181983,181982,363965,175.7720341682434,0.007928473253087964
91091,182183,182182,364365,175.92174005508423,0.007918187945833367
91191,182383,182382,364765,176.06903624534607,0.007907921516872833
91291,182583,182582,365165,176.21473217010498,0.007897673919198569
91391,182783,182782,365565,176.35947012901306,0.007887445105954636
91491,182983,182982,365965,176.51067185401917,0.007877235030436138
91592,183185,183184,366369,176.65729117393494,0.007866941826478525
91692,183385,183384,366769,176.81468510627747,0.0078567692731117
91792,183585,183584,367169,176.97467613220215,0.00784661531779491
91892,183785,183784,367569,177.12155604362488,0.007836479914423562
91992,183985,183984,367969,177.2666199207306,0.007826363017041432
92092,184185,184184,368369,177.4150791168213,0.007816264579839964
92192,184385,184384,368769,177.56440806388855,0.007806184557157917
92292,184585,184584,369169,177.71172904968262,0.0077961229034805455
92392,184785,184784,369569,177.8579671382904,0.007786079573439365
92492,184985,184984,369969,178.01034498214722,0.007776054521811322
92593,185187,185186,370373,178.15927004814148,0.0077659477272617955
92693,185387,185386,370773,178.30659794807434,0.007755959279028298
92793,185587,185586,371173,178.45838904380798,0.00774598897395979
92893,185787,185786,371573,178.6047592163086,0.007736036767411587
92993,185987,185986,371973,178.74888610839844,0.007726102614881864
93093,186187,186186,372373,178.9043369293213,0.00771618647201114
93193,186387,186386,372773,179.0715069770813,0.007706288294581779
93293,186587,186586,373173,179.21204113960266,0.007696408038517362
93393,186787,186786,373573,179.35183310508728,0.007686545659882374
93493,186987,186986,373973,179.4958770275116,0.007676701114881473
93594,187189,187188,374377,179.63777709007263,0.007666776182000901
93694,187389,187388,374777,179.77835202217102,0.007656967350685936
93794,187589,187588,375177,179.91814398765564,0.0076471762220223765
93894,187789,187788,375577,180.06331300735474,0.007637402752772151
93994,187989,187988,375977,180.20455408096313,0.007627646899834897
94094,188189,188188,376377,180.34499406814575,0.007617908620247393
94194,188389,188388,376777,180.49297904968262,0.0076081878711831774
94294,188589,188588,377177,180.63466715812683,0.007598484609951875
94394,188789,188788,377577,180.77437496185303,0.007588798793998877
94494,188989,188988,377977,180.91858792304993,0.007579130380904666
94595,189191,189190,378381,181.0667700767517,0.007569382905387485
94695,189391,189390,378781,181.22139310836792,0.007559749344262658
94795,189591,189590,379181,181.36077904701233,0.007550133059124971
94895,189791,189790,379581,181.50528216362,0.0075405340080920945
94995,189991,189990,379981,181.6448142528534,0.007530952149414454
95095,190191,190190,380381,181.78322529792786,0.007521387441474787
95195,190391,190390,380781,181.92550706863403,0.007511839842787465
95295,190591,190590,381181,182.07065415382385,0.0075023093119982445
95395,190791,190790,381581,182.21088409423828,0.007492795807883659
95495,190991,190990,381981,182.3508701324463,0.007483299289350599
95596,191193,191192,382385,182.4966402053833,0.00747372500512869
95696,191393,191392,382785,182.63633012771606,0.007464262503830366
95796,191593,191592,383185,182.775780916214,0.007454816865205057
95896,191793,191792,383585,182.91661024093628,0.007445388048677621
95996,191993,191992,383985,183.06134724617004,0.007435976013800798
96096,192193,192192,384385,183.2016100883484,0.007426580720254902
96196,192393,192392,384785,183.36102104187012,0.00741720212784732
96296,192593,192592,385185,183.5037431716919,0.00740784019651204
96396,192793,192792,385585,183.6436469554901,0.00739849488630915
96496,192993,192992,385985,183.7841260433197,0.007389166157424452
96597,193195,193194,386389,183.92608904838562,0.007379760931697754
96697,193395,193394,386789,184.06936407089233,0.007370465411328744
96797,193595,193594,387189,184.2090141773224,0.007361186353191253
96897,193795,193794,387589,184.35125517845154,0.0073519237179705925
96997,193995,193994,387989,184.49603700637817,0.007342677466475559
97097,194195,194194,388389,184.63534903526306,0.007333447559637854
97197,194395,194394,388789,184.77447986602783,0.007324233958511813
97297,194595,194594,389189,184.9176368713379,0.0073150366242738735
97397,194795,194794,389589,185.06401419639587,0.007305855518222141
97497,194995,194994,389989,185.20578694343567,0.007296690601775942
97598,195197,195196,390393,185.3487730026245,0.007287450430255907
97698,195397,195396,390793,185.51325392723083,0.0072783179386965826
97798,195597,195596,391193,185.65559101104736,0.007269201521342371
97898,195797,195796,391593,185.79662704467773,0.007260101140094465
97998,195997,195996,391993,185.9428551197052,0.007251016756973199
98098,196197,196196,392393,186.0863392353058,0.007241948334117486
98198,196397,196396,392793,186.2250199317932,0.007232895833784522
98298,196597,196596,393193,186.36408710479736,0.007223859218349286
98398,196797,196796,393593,186.51007509231567,0.007214838450304185
98498,196997,196996,393993,186.65111827850342,0.007205833492258538
98599,197199,197198,394397,186.79327487945557,0.007196754494611566
98699,197399,197398,394797,186.9369239807129,0.007187781202027244
98799,197599,197598,395197,187.0820062160492,0.007178823607598379
98899,197799,197798,395597,187.22448706626892,0.0071698816743992365
98999,197999,197998,395997,187.36818099021912,0.007160955365619003
99099,198199,198198,396397,187.51528000831604,0.007152044644561347
99199,198399,198398,396797,187.67605113983154,0.007143149474644061
99299,198599,198598,397197,187.8164141178131,0.007134269819398599
99399,198799,198798,397597,187.96433115005493,0.0071254056424696855
99499,198999,198998,397997,188.1062831878662,0.007116556907614964
99600,199201,199200,398401,188.24982619285583,0.0071076353230935165
99700,199401,199400,398801,188.39081001281738,0.007098817517627355
99800,199601,199600,399201,188.5376341342926,0.007090015045823082
99900,199801,199800,399601,188.67984914779663,0.007081227871886953
100000,200001,200000,400001,188.82434606552124,0.007072455960136204


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha0/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012407302856445312,30.358099469249375
100,201,200,401,0.18846678733825684,1.725251134601807
200,401,400,801,0.35608386993408203,1.0331394156994131
300,601,600,1201,0.5164837837219238,0.7736231354158138
400,801,800,1601,0.674454927444458,0.6349280372139878
501,1003,1002,2005,0.8346707820892334,0.5455617951375803
601,1203,1202,2405,1.0521190166473389,0.482543795209007
701,1403,1402,2805,1.2395477294921875,0.43443121283005004
801,1603,1602,3205,1.4113609790802002,0.396082748791271
901,1803,1802,3605,1.7056248188018799,0.3645989873004372
1001,2003,2002,4005,1.9532716274261475,0.33817775845833975
1101,2203,2202,4405,2.1195788383483887,0.31561971894335344
1201,2403,2402,4805,2.315887689590454,0.29608763453723413
1301,2603,2602,5205,2.5615928173065186,0.2789761387097555
1401,2803,2802,5605,2.7624619007110596,0.26383524354104326
1502,3005,3004,6009,2.9426259994506836,0.25019483089933037
1602,3205,3204,6409,3.1264870166778564,0.23805758726442536
1702,3405,3404,6809,3.3363149166107178,0.22707177793944233
1802,3605,3604,7209,3.501164674758911,0.21706993619439596
1902,3805,3804,7609,3.646152973175049,0.20791616240763086
2002,4005,4004,8009,3.813706874847412,0.19949893614020578
2102,4205,4204,8409,3.9843246936798096,0.19172585568559014
2202,4405,4404,8809,4.146417856216431,0.18451971692199934
2302,4605,4604,9209,4.311557769775391,0.17781553946480064
2402,4805,4804,9609,4.467228889465332,0.1715582748285912
2503,5007,5006,10013,4.646040678024292,0.16564432077061936
2603,5207,5206,10413,4.8161516189575195,0.16015029105088846
2703,5407,5406,10813,5.031245708465576,0.1549811510589118
2803,5607,5606,11213,5.345148801803589,0.15010700224205265
2903,5807,5806,11613,5.586578845977783,0.14550185344186578
3003,6007,6006,12013,5.804050922393799,0.14114300673996125
3103,6207,6206,12413,5.9886908531188965,0.13701055044944
3203,6407,6406,12813,6.169491767883301,0.1330869385687235
3303,6607,6606,13213,6.327349901199341,0.12935664054963755
3403,6807,6806,13613,6.48043966293335,0.12580584861601082
3504,7009,7008,14017,6.7220728397369385,0.12238920212160206
3604,7209,7208,14417,6.935734033584595,0.11916321177975675
3704,7409,7408,14817,7.086650848388672,0.11608328196435345
3804,7609,7608,15217,7.244872808456421,0.11314041075772609
3904,7809,7808,15617,7.410405874252319,0.11032642169640298
4004,8009,8008,16017,7.567966938018799,0.10763385857735135
4104,8209,8208,16417,7.729620933532715,0.10505589601363031
4204,8409,8408,16817,7.889976739883423,0.1025862632084499
4304,8609,8608,17217,8.035264015197754,0.10021917884265644
4404,8809,8808,17617,8.180601835250854,0.09794929532145866
4505,9011,9010,18021,8.323847770690918,0.09575032438778178
4605,9211,9210,18421,8.462627649307251,0.09366115602452446
4705,9411,9410,18821,8.614176988601685,0.09165526018334968
4805,9611,9610,19221,8.754035949707031,0.08972860996649396
4905,9811,9810,19621,8.93245267868042,0.08787742990858095
5005,10011,10010,20021,9.086054801940918,0.08609817276901403
5105,10211,10210,20421,9.240131855010986,0.08438749926429683
5205,10411,10410,20821,9.383841037750244,0.0827422603099926
5305,10611,10610,21221,9.549936771392822,0.08115948140902517
5405,10811,10810,21621,9.859187841415405,0.07963634887915819
5506,11013,11012,22025,10.050968647003174,0.07815581524163809
5606,11213,11212,22425,10.222308874130249,0.07674465027683981
5706,11413,11412,22825,10.43417477607727,0.07538551682251976
5806,11613,11612,23225,10.581081867218018,0.07407613635346144
5906,11813,11812,23625,10.721892833709717,0.07281434196761298
6006,12013,12012,24025,10.869425773620605,0.07159807137914267
6106,12213,12212,24425,11.020484685897827,0.07042536057263304
6206,12413,12412,24825,11.171380996704102,0.06929433803403764
6306,12613,12612,25225,11.309647798538208,0.06820321948612608
6406,12813,12812,25625,11.453434705734253,0.06715030306641073
6507,13015,13014,26029,11.618983745574951,0.06612398092841468
6607,13215,13214,26429,11.75954294204712,0.06514301371111987
6707,13415,13414,26829,11.903349876403809,0.06419558041511696
6807,13615,13614,27229,12.043097734451294,0.0632802683993876
6907,13815,13814,27629,12.181427955627441,0.062395728307350413
7007,14015,14014,28029,12.321580648422241,0.06154067100873571
7107,14215,14214,28429,12.46141004562378,0.06071386473424732
7207,14415,14414,28829,12.61687183380127,0.05991413238392325
7307,14615,14614,29229,12.777913808822632,0.059140348992611
7407,14815,14814,29629,12.932936906814575,0.05839143933812523
7508,15017,15016,30033,13.098574876785278,0.05765924210431666
7608,15217,15216,30433,13.304144859313965,0.056957265862180737
7708,15417,15416,30833,13.459383726119995,0.056277204937750555
7808,15617,15616,31233,13.607781887054443,0.055618162011791754
7908,15817,15816,31633,13.763822793960571,0.05497927928204562
8008,16017,16016,32033,13.923948764801025,0.05435973671268472
8108,16217,16216,32433,14.070174932479858,0.05375875036499129
8208,16417,16416,32833,14.209722757339478,0.05317557080411595
8308,16617,16616,33233,14.377910852432251,0.05260948157732764
8408,16817,16816,33633,14.527161836624146,0.05205979775965061
8509,17019,17018,34037,14.667198896408081,0.051520602630384243
8609,17219,17218,34437,14.805424928665161,0.05100194225340503
8709,17419,17418,34837,14.946286678314209,0.05049780221954439
8809,17619,17618,35237,15.084581851959229,0.05000761065391924
8909,17819,17818,35637,15.242784023284912,0.04953082081910589
9009,18019,18018,36037,15.460799932479858,0.0490669099988507
9109,18219,18218,36437,15.604127883911133,0.04861537842924969
9209,18419,18418,36837,15.74465274810791,0.04817574827537324
9309,18619,18618,37237,15.882848978042603,0.04774756265143859
9409,18819,18818,37637,16.021324634552002,0.047330384682744496
9510,19021,19020,38041,16.160159826278687,0.046919782839293905
9610,19221,19220,38441,16.299185752868652,0.04652348509582251
9710,19421,19420,38841,16.442853689193726,0.04613699192550532
9810,19621,19620,39241,16.590858936309814,0.045759938057866614
9910,19821,19820,39641,16.797423839569092,0.04539197410606611
10010,20021,20020,40041,16.943206787109375,0.04503276584703184
10110,20221,20220,40441,17.084637880325317,0.04468199353306405
10210,20421,20420,40841,17.285278797149658,0.044339351233674364
10310,20621,20620,41241,17.442389965057373,0.04400454620646485
10410,20821,20820,41641,17.603880882263184,0.04367729829589823
10511,21023,21022,42045,17.750391721725464,0.043354175700984134
10611,21223,21222,42445,17.904260873794556,0.04304131812212202
10711,21423,21422,42845,18.059722900390625,0.042735244693531745
10811,21623,21622,43245,18.2131609916687,0.042435720216392636
10911,21823,21822,43645,18.3535258769989,0.04214251944861459
11011,22023,22022,44045,18.494906902313232,0.04185542664905385
11111,22223,22222,44445,18.647389888763428,0.04157423514255881
11211,22423,22422,44845,18.90201497077942,0.04129874690496824
11311,22623,22622,45245,19.060237646102905,0.04102877216721476
11411,22823,22822,45645,19.20056986808777,0.04076412903771575
11512,23025,23024,46049,19.347285985946655,0.04050207375577833
11612,23225,23224,46449,19.486687898635864,0.04024762697357275
11712,23425,23424,46849,19.659742832183838,0.03999800830159963
11812,23625,23624,47249,19.831783771514893,0.0397530639846592
11912,23825,23824,47649,19.984335899353027,0.0395126465017495
12012,24025,24024,48049,20.134594678878784,0.039276614282708754
12112,24225,24224,48449,20.29679584503174,0.03904483143818287
12212,24425,24424,48849,20.456270694732666,0.03881716750231484
12312,24625,24624,49249,20.713943004608154,0.038593497187575036
12412,24825,24824,49649,21.16642475128174,0.03837370015117433
12513,25027,25026,50053,21.46342396736145,0.03815551897529549
12613,25227,25226,50453,21.814056873321533,0.037943162063118596
12713,25427,25426,50853,22.090587854385376,0.0377343438492354
12813,25627,25626,51253,22.246922969818115,0.03752896168757155
12913,25827,25826,51653,22.467447757720947,0.03732691686285719
13013,26027,26026,52053,22.699781894683838,0.03712811441614046
13113,26227,26226,52453,22.897509813308716,0.03693246297857628
13213,26427,26426,52853,23.052035808563232,0.03673987461309662
13313,26627,26626,53253,23.2518208026886,0.03655026466358583
13413,26827,26826,53653,23.421557903289795,0.036363551611200175
13514,27029,27028,54057,23.578909873962402,0.036177831965269316
13614,27229,27228,54457,23.731831789016724,0.03599670707644524
13714,27429,27428,54857,23.925784826278687,0.035818251299561545
13814,27629,27628,55257,24.077009916305542,0.035642394384972687
13914,27829,27828,55657,24.24483299255371,0.03546906859650301
14014,28029,28028,56057,24.426017999649048,0.035298208604007716
14114,28229,28228,56457,24.570894718170166,0.03512975138098166
14214,28429,28428,56857,24.715914964675903,0.034963636106970473
14314,28629,28628,57257,24.868794679641724,0.03479980407454928
14414,28829,28828,57657,25.055131912231445,0.034638198600647346
14515,29031,29030,58061,25.20734477043152,0.0344771813926357
14615,29231,29230,58461,25.3990159034729,0.03431988759353739
14715,29431,29430,58861,25.536054849624634,0.034164661121646143
14815,29631,29630,59261,25.718302965164185,0.03401145260098112
14915,29831,29830,59661,25.872536659240723,0.03386021429396292
15015,30031,30030,60061,26.03413486480713,0.03371090003473227
15115,30231,30230,60461,26.179157972335815,0.033563465165527585
15215,30431,30430,60861,26.346523761749268,0.03341786647597316
15315,30631,30630,61261,26.487440824508667,0.033274062145135605
15415,30831,30830,61661,26.631536722183228,0.03313201168621398
15516,31033,31032,62065,26.812073945999146,0.03299028106538275
15616,31233,31232,62465,27.001683950424194,0.032851638543969136
15716,31433,31432,62865,27.196424961090088,0.03271463556051868
15816,31633,31632,63265,27.376155853271484,0.03257923647112261
15916,31833,31832,63665,27.599483728408813,0.032445406724262195
16016,32033,32032,64065,27.742371797561646,0.03231311281884127
16116,32233,32232,64465,27.913290977478027,0.03218232226407853
16216,32433,32432,64865,28.211784839630127,0.032053003541169474
16316,32633,32632,65265,28.404131650924683,0.03192512606663327
16416,32833,32832,65665,28.559850931167603,0.031798660157263375
16517,33035,33034,66069,28.70042085647583,0.03167233305252099
16617,33235,33234,66469,28.83767604827881,0.031548618067915195
16717,33435,33434,66869,29.009031772613525,0.03142623040467131
16817,33635,33634,67269,29.212663650512695,0.031305143667268095
16917,33835,33834,67669,29.368215799331665,0.031185332206444923
17017,34035,34034,68069,29.507969617843628,0.031066771092305608
17117,34235,34234,68469,29.678935766220093,0.030949436088563275
17217,34435,34434,68869,29.86170792579651,0.030833303627871574
17317,34635,34634,69269,30.009904861450195,0.03071835078819308
17417,34835,34834,69669,30.15048384666443,0.030604555270155195
17518,35037,35036,70073,30.288200855255127,0.03049077443936755
17618,35237,35236,70473,30.424343824386597,0.030379240089852988
17718,35437,35436,70873,30.57048773765564,0.030268799484460148
17818,35637,35636,71273,30.72139072418213,0.030159432611547094
17918,35837,35836,71673,30.877014875411987,0.030051119982023665
18018,36037,36036,72073,31.012609004974365,0.029943842611752463
18118,36237,36236,72473,31.150194883346558,0.029837582004660062
18218,36437,36436,72873,31.29167103767395,0.029732320136525433
18318,36637,36636,73273,31.433238983154297,0.029628039439415943
18418,36837,36836,73673,31.617568016052246,0.02952472278674026
18519,37039,37038,74077,31.826502799987793,0.029421334514460707
18619,37239,37238,74477,31.96522068977356,0.029319905494727717
18719,37439,37438,74877,32.106199741363525,0.029219391490043062
18819,37639,37638,75277,32.26132297515869,0.02911977700493755
18919,37839,37838,75677,32.455671072006226,0.0290210469187723
19019,38039,38038,76077,32.6348557472229,0.028923186473965537
19119,38239,38238,76477,32.826931953430176,0.028826181264669258
19219,38439,38438,76877,32.99612474441528,0.028730017225875572
19319,38639,38638,77277,33.13695573806763,0.028634680622934186
19419,38839,38838,77677,33.28190588951111,0.02854015804146322
19520,39041,39040,78081,33.42279601097107,0.028445503162067013
19620,39241,39240,78481,33.56275200843811,0.028352577430754568
19720,39441,39440,78881,33.707228899002075,0.028260427180378078
19820,39641,39640,79281,33.848108768463135,0.028169040186821117
19920,39841,39840,79681,34.01906991004944,0.028078404501042573
20020,40041,40040,80081,34.19817876815796,0.02798850844102124
20120,40241,40240,80481,34.5095329284668,0.027899340583990836
20220,40441,40440,80881,34.74326777458191,0.027810889758952812
20320,40641,40640,81281,35.125412702560425,0.0277231450394556
20420,40841,40840,81681,35.37105679512024,0.027636095736629403
20521,41043,41042,82085,35.77547788619995,0.02754887117325509
20621,41243,41242,82485,36.02773976325989,0.02746318825043482
20721,41443,41442,82885,36.212889671325684,0.027378169938052893
20821,41643,41642,83285,36.3827338218689,0.02729380643475468
20921,41843,41842,83685,36.630635023117065,0.027210088145362795
21021,42043,42042,84085,36.823121786117554,0.027127005675241785
21121,42243,42242,84485,36.98919486999512,0.02704454982485341
21221,42443,42442,84885,37.25663375854492,0.026962711584495463
21321,42643,42642,85285,37.4508490562439,0.02688148212921685
21421,42843,42842,85685,37.62565302848816,0.02680085281390182
21522,43045,43044,86089,37.77867078781128,0.026720017751774044
21622,43245,43244,86489,37.93336296081543,0.026640569269127282
21722,43445,43444,86889,38.1052508354187,0.026561695942841326
21822,43645,43644,87289,38.28417205810547,0.026483389802738927
21922,43845,43844,87689,38.454025983810425,0.026405643036174768
22022,44045,44044,88089,38.61916494369507,0.02632844798400672
22122,44245,44244,88489,38.77394986152649,0.026251797136695613
22222,44445,44444,88889,38.96636891365051,0.0261756831305289
22322,44645,44644,89289,39.13918900489807,0.026100098743962265
22422,44845,44844,89689,39.35593295097351,0.026025036894076908
22523,45047,45046,90093,39.55876874923706,0.025949747751090577
22623,45247,45246,90493,39.82313799858093,0.025875715317000777
22723,45447,45446,90893,40.024353981018066,0.025802184902548382
22823,45647,45646,91293,40.24172377586365,0.025729149947264905
22923,45847,45846,91693,40.48831272125244,0.02565660401313399
23023,46047,46046,92093,40.69961500167847,0.025584540781652128
23123,46247,46246,92493,40.96152687072754,0.02551295405097718
23223,46447,46446,92893,41.197232723236084,0.025441837733162487
23323,46647,46646,93293,41.3569598197937,0.025371185851471904
23423,46847,46846,93693,41.52293300628662,0.025300992537774306
23524,47049,47048,94097,41.703112840652466,0.025230556892376153
23624,47249,47248,94497,41.85788893699646,0.025161267975363354
23724,47449,47448,94897,42.01358675956726,0.025092420593584127
23824,47649,47648,95297,42.15718078613281,0.025024009289734053
23924,47849,47848,95697,42.29633688926697,0.02495602870315468
24024,48049,48048,96097,42.48435688018799,0.024888473567647323
24124,48249,48248,96497,42.64991474151611,0.02482133870934882
24224,48449,48448,96897,42.79062294960022,0.02475461904466623
24324,48649,48648,97297,42.92878270149231,0.024688309578270222
24424,48849,48848,97697,43.072160959243774,0.024622405401142206
24525,49051,49050,98101,43.211729764938354,0.024556248657786196
24625,49251,49250,98501,43.3509247303009,0.024491144601499665
24725,49451,49450,98901,43.490561723709106,0.024426431560359774
24825,49651,49650,99301,43.6484317779541,0.02436210495290391
24925,49851,49850,99701,43.84451389312744,0.024298160274975812
25025,50051,50050,100101,43.9916558265686,0.02423459309807016
25125,50251,50250,100501,44.14773082733154,0.024171399067722248
25225,50451,50450,100901,44.31429982185364,0.024108573901939583
25325,50651,50650,101301,44.487979888916016,0.024046113389674717
25425,50851,50850,101701,44.67554569244385,0.023984013389337876
25526,51053,51052,102105,44.89056992530823,0.02392165417812958
25626,51253,51252,102505,45.041064977645874,0.02386026655180488
25726,51453,51452,102905,45.18978786468506,0.023799227375991334
25826,51653,51652,103305,45.3525869846344,0.023738532773443066
25926,51853,51852,103705,45.500067710876465,0.023678178929477357
26026,52053,52052,104105,45.65309691429138,0.023618162090702013
26126,52253,52252,104505,45.79879593849182,0.023558478563774094
26226,52453,52452,104905,45.94884777069092,0.023499124714190127
26326,52653,52652,105305,46.08574390411377,0.02344009696510563
26426,52853,52852,105705,46.22511887550354,0.023381391796184488
26527,53055,53054,106109,46.40944480895996,0.02332242348188586
26627,53255,53254,106509,46.56327176094055,0.023264356272731823
26727,53455,53454,106909,46.74500298500061,0.023206601377380873
26827,53655,53654,107309,46.93255972862244,0.02314915549108807
26927,53855,53854,107709,47.089332818984985,0.023092015360258213
27027,54055,54054,108109,47.256129026412964,0.023035177781452802
27127,54255,54254,108509,47.396286964416504,0.02297863960041945
27227,54455,54454,108909,47.58539271354675,0.0229223977111454
27327,54655,54654,109309,47.741039752960205,0.02286644905493228
27427,54855,54854,109709,47.926652908325195,0.02281079061949307
27528,55057,55056,110113,48.08417987823486,0.022754867166964565
27628,55257,55256,110513,48.230151891708374,0.02269978314617838
27728,55457,55456,110913,48.38407278060913,0.02264498055048805
27828,55657,55656,111313,48.5595908164978,0.02259045654505676
27928,55857,55856,111713,48.707963705062866,0.02253620833723805
28028,56057,56056,112113,48.86145377159119,0.022482233175790744
28128,56257,56256,112513,49.02485489845276,0.02242852835011063
28228,56457,56456,112913,49.20037770271301,0.022375091189480067
28328,56657,56656,113313,49.37436485290527,0.022321919062333745
28428,56857,56856,113713,49.5386528968811,0.022269009375541767
28529,57059,57058,114117,49.697630882263184,0.022215834379556394
28629,57259,57258,114517,49.872092962265015,0.02216344450540145
28729,57459,57458,114917,50.023454904556274,0.022111309491241765
28829,57659,57658,115317,50.20407676696777,0.022059426891176334
28929,57859,57858,115717,50.42264175415039,0.02200779429437483
29029,58059,58058,116117,50.60419678688049,0.021956409324448933
29129,58259,58258,116517,50.77872586250305,0.021905269638837623
29229,58459,58458,116917,50.92407488822937,0.021854372928205596
29329,58659,58658,117317,51.0700306892395,0.021803716915854494
29429,58859,58858,117717,51.20922374725342,0.021753299357146268
29530,59061,59060,118121,51.34666681289673,0.021702617411362677
29630,59261,59260,118521,51.50224184989929,0.02165267248112565
29730,59461,59460,118921,51.65288496017456,0.021602959436031792
29830,59661,59660,119321,51.802671909332275,0.02155347615445676
29930,59861,59860,119721,51.94235897064209,0.021504220544126505
30030,60061,60060,120121,52.08350896835327,0.021455190541609447
30130,60261,60260,120521,52.24099779129028,0.021406384111819585
30230,60461,60460,120921,52.411064863204956,0.021357799247529348
30330,60661,60660,121321,52.55040693283081,0.02130943396889251
30430,60861,60860,121721,52.69883179664612,0.02126128632297706
30531,61063,61062,122125,52.837403774261475,0.021212876146774994
30631,61263,61262,122525,52.97602200508118,0.02116516014142918
30731,61463,61462,122925,53.13238883018494,0.021117656048338717
30831,61663,61662,123325,53.284804821014404,0.02107036201798955
30931,61863,61862,123725,53.431501626968384,0.021023276225578362
31031,62063,62062,124125,53.57593393325806,0.020976396870598997
31131,62263,62262,124525,53.712177753448486,0.020929722176436568
31231,62463,62462,124925,53.871914863586426,0.02088325038997014
31331,62663,62662,125325,54.01842379570007,0.020836979781182922
31431,62863,62862,125725,54.17893886566162,0.020790908642780062
31532,63065,63064,126129,54.3364999294281,0.020744577549456095
31632,63265,63264,126529,54.51204872131348,0.02069890227185976
31732,63465,63464,126929,54.66796278953552,0.020653421459079477
31832,63665,63664,127329,54.806551694869995,0.020608133491244754
31932,63865,63864,127729,54.94544792175293,0.020563036769401223
32032,64065,64064,128129,55.08712697029114,0.020518129715171387
32132,64265,64264,128529,55.2261278629303,0.02047341077042082
32232,64465,64464,128929,55.363783836364746,0.02042887839693129
32332,64665,64664,129329,55.50837302207947,0.020384531076080074
32432,64865,64864,129729,55.64882183074951,0.020340367308525002
32533,65067,65066,130133,55.789103746414185,0.020295946711456982
32633,65267,65266,130533,55.931713819503784,0.0202521474268461
32733,65467,65466,130933,56.07023286819458,0.020208527295788953
32833,65667,65666,131333,56.208141803741455,0.02016508489321509
32933,65867,65866,131733,56.35621666908264,0.020121818811844584
33033,66067,66066,132133,56.50940990447998,0.020078727661907103
33133,66267,66266,132533,56.657301902770996,0.020035810070866345
33233,66467,66466,132933,56.80720782279968,0.019993064683148747
33333,66667,66666,133333,56.944931745529175,0.019950490159878407
33433,66867,66866,133733,57.085874795913696,0.01990808517861562
33534,67069,67068,134137,57.22779393196106,0.01986542691085773
33634,67269,67268,134537,57.365620851516724,0.019823358773752874
33734,67469,67468,134937,57.50315070152283,0.019781456294749658
33834,67669,67668,135337,57.64531683921814,0.01973971821479264
33934,67869,67868,135737,57.80676770210266,0.01969814329002546
34034,68069,68068,136137,57.9539840221405,0.01965673029155704
34134,68269,68268,136537,58.09146285057068,0.019615478005232466
34234,68469,68468,136937,58.22878384590149,0.01957438523140732
34334,68669,68668,137337,58.36618375778198,0.019533450784726052
34434,68869,68868,137737,58.50638484954834,0.01949267349390492
34535,69071,69070,138141,58.65211892127991,0.019451646772505105
34635,69271,69270,138541,58.81844401359558,0.019411181877591423
34735,69471,69470,138941,59.03016185760498,0.019370870695762887
34835,69671,69670,139341,59.18880367279053,0.019330712110055045
34935,69871,69870,139741,59.32988476753235,0.01929070501654202
35035,70071,70070,140141,59.481703758239746,0.019250848324141225
35135,70271,70270,140541,59.65912485122681,0.019211140954421377
35235,70471,70470,140941,59.81502079963684,0.019171581841413602
35335,70671,70670,141341,59.968915939331055,0.019132169931426305
35435,70871,70870,141741,60.1289427280426,0.019092904182862837
35536,71073,71072,142145,60.31520986557007,0.019053393089335718
35636,71273,71272,142545,60.45671081542969,0.019014418022354724
35736,71473,71472,142945,60.597020864486694,0.018975586052796825
35836,71673,71672,143345,60.7391459941864,0.018936896185798812
35936,71873,71872,143745,60.87591290473938,0.018898347437725855
36036,72073,72072,144145,61.0247917175293,0.018859938836007395
36136,72273,72272,144545,61.171191692352295,0.018821669418975857
36236,72473,72472,144945,61.30892276763916,0.018783538235707962
36336,72673,72672,145345,61.44645285606384,0.018745544345868635
36436,72873,72872,145745,61.58362293243408,0.018707686819558044
36537,73075,73074,146149,61.72678875923157,0.018669588197242667
36637,73275,73274,146549,61.86574697494507,0.018632001990064116
36737,73475,73474,146949,62.004087686538696,0.018594549408885233
36837,73675,73674,147349,62.141782999038696,0.01855722956416187
36937,73875,73874,147749,62.282848834991455,0.01852004157605496
37037,74075,74074,148149,62.42117667198181,0.0184829845742918
37137,74275,74274,148549,62.55926489830017,0.018446057698029945
37237,74475,74474,148949,62.700498819351196,0.01840926009572327
37337,74675,74674,149349,62.84014177322388,0.01837259092499031
37437,74875,74874,149749,62.97709584236145,0.018336049352484656
37538,75077,75076,150153,63.12242674827576,0.01829927104322115
37638,75277,75276,150553,63.27608275413513,0.018262983458128306
37738,75477,75476,150953,63.4213228225708,0.018226821016144038
37838,75677,75676,151353,63.58037972450256,0.018190782918893998
37938,75877,75876,151753,63.74756979942322,0.01815486837642129
38038,76077,76076,152153,63.911360025405884,0.018119076607069226
38138,76277,76276,152553,64.06628084182739,0.018083406837366
38238,76477,76476,152953,64.20244574546814,0.018047858301911218
38338,76677,76676,153353,64.33897185325623,0.018012430243264033
38438,76877,76876,153753,64.48206281661987,0.017977121911833673
38539,77079,77078,154157,64.62820076942444,0.017941581270695787
38639,77279,77278,154557,64.76527166366577,0.017906511354616263
38739,77479,77478,154957,64.90788578987122,0.017871558955778594
38839,77679,77678,155357,65.04714179039001,0.017836723355001523
38939,77879,77878,155757,65.23844289779663,0.017802003840429306
39039,78079,78078,156157,65.44151782989502,0.017767399707431936
39139,78279,78278,156557,65.62495374679565,0.017732910258507373
39239,78479,78478,156957,65.76462888717651,0.01769853480318475
39339,78679,78678,157357,65.90310382843018,0.01766427265792939
39439,78879,78878,157757,66.04584693908691,0.017630123146049517
39540,79081,79080,158161,66.18773674964905,0.017595745785285163
39640,79281,79280,158561,66.32471585273743,0.017561820646667444
39740,79481,79480,158961,66.46707773208618,0.017528006144959224
39840,79681,79680,159361,66.65527486801147,0.017494301629998436
39940,79881,79880,159761,66.79989504814148,0.017460706458019143
40040,80081,80080,160161,66.97186374664307,0.017427219991566524
40140,80281,80280,160561,67.12818479537964,0.017393841599413325
40240,80481,80480,160961,67.2722659111023,0.017360570656477215
40340,80681,80680,161361,67.42571687698364,0.017327406543740147
40440,80881,80880,161761,67.58071279525757,0.017294348648168065
40541,81083,81082,162165,67.76575994491577,0.017261067371068674
40641,81283,81282,162565,67.95822381973267,0.017228221141340302
40741,81483,81482,162965,68.10752892494202,0.017195479318873882
40841,81683,81682,163365,68.2504346370697,0.017162841313855037
40941,81883,81882,163765,68.3891327381134,0.017130306542071767
41041,82083,82082,164165,68.53026294708252,0.017097874424841997
41141,82283,82282,164565,68.67226982116699,0.017065544388941797
41241,82483,82482,164965,68.85596990585327,0.01703331586653505
41341,82683,82682,165365,69.0464220046997,0.01700118829510394
41441,82883,82882,165765,69.2004599571228,0.01696916111738057
41542,83085,83084,166169,69.35661697387695,0.016936915010264064
41642,83285,83284,166569,69.51279783248901,0.016905087959018444
41742,83485,83484,166969,69.67628288269043,0.016873359655114786
41842,83685,83684,167369,69.82569694519043,0.016841729561671622
41942,83885,83884,167769,69.97501587867737,0.016810197146730238
42042,84085,84084,168169,70.11370086669922,0.016778761883192207
42142,84285,84284,168569,70.2517638206482,0.016747423248758248
42242,84485,84484,168969,70.41540384292603,0.01671618072586743
42342,84685,84684,169369,70.71274375915527,0.016685033801637703
42442,84885,84884,169769,70.88404989242554,0.016653981967807166
42543,85087,85086,170173,71.04432773590088,0.016622715624174927
42643,85287,85286,170573,71.19496870040894,0.016591853402918303
42743,85487,85486,170973,71.3383858203888,0.016561084769496595
42843,85687,85686,171373,71.47724390029907,0.016530409233602147
42943,85887,85886,171773,71.64236283302307,0.01649982630926625
43043,86087,86086,172173,71.80312776565552,0.016469335514805256
43143,86287,86286,172573,71.95533990859985,0.016438936372767995
43243,86487,86486,172973,72.10585761070251,0.016408628409883372
43343,86687,86686,173373,72.28453183174133,0.016378411157009207
43443,86887,86886,173773,72.44390559196472,0.0163482841490817
43544,87089,87088,174177,72.58720898628235,0.016317947004684173
43644,87289,87288,174577,72.73354983329773,0.016287999998496797
43744,87489,87488,174977,72.874107837677,0.016258141861527946
43844,87689,87688,175377,73.0116229057312,0.01622837214457448
43944,87889,87888,175777,73.15029883384705,0.016198690402268984
44044,88089,88088,176177,73.29105877876282,0.01616909619303347
44144,88289,88288,176577,73.42951083183289,0.016139589079034025
44244,88489,88488,176977,73.56735491752625,0.016110168626135502
44344,88689,88688,177377,73.70588684082031,0.016080834403857398
44444,88889,88888,177777,73.84687161445618,0.016051585985330012
44545,89091,89090,178181,74.00267171859741,0.016022131746618748
44645,89291,89290,178581,74.14775776863098,0.015993054516711416
44745,89491,89490,178981,74.2887806892395,0.015964061827038165
44845,89691,89690,179381,74.42463779449463,0.015935153264782634
44945,89891,89890,179781,74.56226181983948,0.015906328420529737
45045,90091,90090,180181,74.69983100891113,0.015877586888225614
45145,90291,90290,180581,74.83955788612366,0.015848928265138035
45245,90491,90490,180981,74.9762818813324,0.015820352151817672
45345,90691,90690,181381,75.11624884605408,0.01579185815205944
45445,90891,90890,181781,75.25440883636475,0.015763445872864972
45546,91093,91092,182185,75.39442992210388,0.01573483202432974
45646,91293,91292,182585,75.53163599967957,0.01570658282740587
45746,91493,91492,182985,75.6684718132019,0.015678414187099022
45846,91693,91692,183385,75.81126093864441,0.015650325722899632
45946,91893,91892,183785,75.94851303100586,0.015622317057323056
46046,92093,92092,184185,76.09194374084473,0.015594387815874732
46146,92293,92292,184585,76.24334478378296,0.015566537627016092
46246,92493,92492,184985,76.38107895851135,0.015538766122130529
46346,92693,92692,185385,76.51947784423828,0.01551107293549019
46446,92893,92892,185785,76.65733289718628,0.01548345770422327
46547,93095,93094,186189,76.80027890205383,0.01545564508256718
46647,93295,93294,186589,76.94225978851318,0.015428185455279256
46747,93495,93494,186989,77.08212995529175,0.015400802708031612
46847,93695,93694,187389,77.22344398498535,0.015373496489083502
46947,93895,93894,187789,77.36382389068604,0.015346266449392422
47047,94095,94094,188189,77.50110173225403,0.015319112242583413
47147,94295,94294,188589,77.64107489585876,0.015292033524919778
47247,94495,94494,188989,77.78159880638123,0.015265029955273198
47347,94695,94694,189389,77.92050099372864,0.015238101195095102
47447,94895,94894,189789,78.05764675140381,0.015211246908387922
47548,95097,95096,190193,78.19446587562561,0.015184199333494748
47648,95297,95296,190593,78.35085272789001,0.015157493732227002
47748,95497,95496,190993,78.490238904953,0.015130861608190426
47848,95697,95696,191393,78.62536764144897,0.015104302635337465
47948,95897,95896,191793,78.7664098739624,0.015077816490033957
48048,96097,96096,192193,78.90308094024658,0.015051402851032878
48148,96297,96296,192593,79.03997373580933,0.015025061399448316
48248,96497,96496,192993,79.177414894104,0.014998791818729911
48348,96697,96696,193393,79.31887173652649,0.014972593794637397
48448,96897,96896,193793,79.45570302009583,0.014946467015215766
48549,97099,97098,194197,79.59435796737671,0.014920150969505643
48649,97299,97298,194597,79.73344278335571,0.014894166457308946
48749,97499,97498,194997,79.87179493904114,0.014868252264343478
48849,97699,97698,195397,80.01256966590881,0.014842408087573906
48949,97899,97898,195797,80.14983081817627,0.014816633626129973
49049,98099,98098,196197,80.29031181335449,0.014790928581283582
49149,98299,98298,196597,80.4366409778595,0.014765292656425929
49249,98499,98498,196997,80.58321571350098,0.014739725557045077
49349,98699,98698,197397,80.72378873825073,0.014714226990703978
49449,98899,98898,197797,80.86993479728699,0.014688796667018477
49550,99101,99100,198201,81.00838279724121,0.014663181016140808
49650,99301,99300,198601,81.14565563201904,0.014637886989959022
49750,99501,99500,199001,81.28639101982117,0.014612660344550686
49850,99701,99700,199401,81.42433786392212,0.014587500797550411
49950,99901,99900,199801,81.56175589561462,0.014562408068540787
50050,100101,100100,200201,81.70142793655396,0.01453738187903176
50150,100301,100300,200601,81.84194684028625,0.014512421952441202
50250,100501,100500,201001,81.98091387748718,0.01448752801407491
50350,100701,100700,201401,82.11768698692322,0.014462699791107488
50450,100901,100900,201801,82.2574577331543,0.014437937012562903
50551,101103,101102,202205,82.39822173118591,0.01441299276149233
50651,101303,101302,202605,82.54064774513245,0.014388360713904908
50751,101503,101502,203005,82.70129990577698,0.014363793306075312
50851,101703,101702,203405,82.84508085250854,0.014339290274256703
50951,101903,101902,203805,82.98545980453491,0.014314851356459529
51051,102103,102102,204205,83.123783826828,0.0142904762924336
51151,102303,102302,204605,83.26370286941528,0.01426616482365087
51251,102503,102502,205005,83.4079339504242,0.014241916693287952
51351,102703,102702,205405,83.5507378578186,0.014217731646209248
51451,102903,102902,205805,83.6874668598175,0.014193609428949962
51552,103105,103104,206209,83.82985806465149,0.014169309508478186
51652,103305,103304,206609,83.96709871292114,0.014145312819084519
51752,103505,103504,207009,84.10930585861206,0.014121378206498671
51852,103705,103704,207409,84.24886298179626,0.014097505423791156
51952,103905,103904,207809,84.38808965682983,0.014073694225622347
52052,104105,104104,208209,84.52569699287415,0.01404994436822647
52152,104305,104304,208609,84.66377973556519,0.014026255609396686
52252,104505,104504,209009,84.82131481170654,0.014002627708469512
52352,104705,104704,209409,84.96163201332092,0.013979060426309933
52452,104905,104904,209809,85.10119986534119,0.013955553525296671
52553,105107,105106,210213,85.24143981933594,0.013931872604684651
52653,105307,105306,210613,85.38179564476013,0.013908486357005244
52753,105507,105506,211013,85.51813578605652,0.013885159784220062
52853,105707,105706,211413,85.65558195114136,0.013861892654632132
52953,105907,105906,211813,85.79571199417114,0.013838684737986525
53053,106107,106106,212213,85.93458676338196,0.013815535805456691
53153,106307,106306,212613,86.07251977920532,0.013792445629630744
53253,106507,106506,213013,86.21053075790405,0.013769413984498097
53353,106707,106706,213413,86.35120368003845,0.013746440645436255
53453,106907,106906,213813,86.4904727935791,0.013723525389197551
53554,107109,107108,214217,86.64728283882141,0.013700439711393808
53654,107309,107308,214617,86.79507875442505,0.01367764053178866
53754,107509,107508,215017,86.94529485702515,0.013654898771199535
53854,107709,107708,215417,87.09095597267151,0.013632214211764027
53954,107909,107908,215817,87.2293848991394,0.01360958663693127
54054,108109,108108,216217,87.3709008693695,0.013587015831450056
54154,108309,108308,216617,87.51129078865051,0.013564501581356529
54254,108509,108508,217017,87.65002393722534,0.01354204367396259
54354,108709,108708,217417,87.79390382766724,0.013519641897843921
54454,108909,108908,217817,87.93157076835632,0.013497296042828549
54555,109111,109110,218221,88.07498598098755,0.013474783279199671
54655,109311,109310,218621,88.21859669685364,0.01345254919482705
54755,109511,109510,219021,88.35911178588867,0.01343037040638306
54855,109711,109710,219421,88.49843668937683,0.013408246708603739
54955,109911,109910,219821,88.63758182525635,0.013386177897421475
55055,110111,110110,220221,88.77845191955566,0.013364163769954158
55155,110311,110310,220621,88.92056775093079,0.013342204124494349
55255,110511,110510,221021,89.0675618648529,0.013320298760499127
55355,110711,110710,221421,89.21735978126526,0.013298447478579412
55455,110911,110910,221821,89.35700678825378,0.013276650080489637
55556,111113,111112,222225,89.49939584732056,0.013254689202457986
55656,111313,111312,222625,89.6375527381897,0.013232999515736827
55756,111513,111512,223025,89.77822470664978,0.013211363122926699
55856,111713,111712,223425,89.91657185554504,0.013189779830267258
55956,111913,111912,223825,90.05492782592773,0.013168249445091837
56056,112113,112112,224225,90.1920657157898,0.01314677177581818
56156,112313,112312,224625,90.33183002471924,0.01312534663193894
56256,112513,112512,225025,90.470529794693,0.013103973824012185
56356,112713,112712,225425,90.60774278640747,0.013082653163652267
56456,112913,112912,225825,90.75121569633484,0.013061384463520571
56557,113115,113114,226229,90.8914487361908,0.013039955628885188
56657,113315,113314,226629,91.03177690505981,0.013018790806291975
56757,113515,113514,227029,91.1712429523468,0.01299767738626663
56857,113715,113714,227429,91.32769203186035,0.012976615185579705
56957,113915,113914,227829,91.46569275856018,0.012955604022004623
57057,114115,114114,228229,91.63544297218323,0.01293464371430911
57157,114315,114314,228629,91.77768874168396,0.012913734082246801
57257,114515,114514,229029,91.94290471076965,0.012892874946548923
57357,114715,114714,229429,92.08070969581604,0.012872066128916037
57457,114915,114914,229829,92.21828985214233,0.012851307452009776
57558,115117,115116,230233,92.35990786552429,0.012830391904044983
57658,115317,115316,230633,92.49860572814941,0.012809733477388006
57758,115517,115516,231033,92.63767886161804,0.012789124663389556
57858,115717,115716,231433,92.77529883384705,0.012768565288485622
57958,115917,115916,231833,92.91642594337463,0.012748055180034057
58058,116117,116116,232233,93.05344891548157,0.012727594166306812
58158,116317,116316,232633,93.19206285476685,0.012707182076482379
58258,116517,116516,233033,93.33506083488464,0.012686818740638432
58358,116717,116716,233433,93.4882140159607,0.012666503989744518
58458,116917,116916,233833,93.62648701667786,0.012646237655654704
58559,117119,117118,234237,93.76618385314941,0.01262581763335122
58659,117319,117318,234637,93.90521192550659,0.012605648111927934
58759,117519,117518,235037,94.04511570930481,0.01258552650645551
58859,117719,117718,235437,94.18263387680054,0.012565452652263543
58959,117919,117918,235837,94.32349276542664,0.01254542638553089
59059,118119,118118,236237,94.46427965164185,0.012525447543278976
59159,118319,118318,236637,94.60693573951721,0.012505515963364805
59259,118519,118518,237037,94.77573490142822,0.012485631484474713
59359,118719,118718,237437,94.9169328212738,0.012465793946117406
59459,118919,118918,237837,95.07843089103699,0.012446003188617685
59560,119121,119120,238241,95.22105765342712,0.012426061846660291
59660,119321,119320,238641,95.35716462135315,0.01240636463892564
59760,119521,119520,239041,95.50209999084473,0.012386713736286269
59860,119721,119720,239441,95.6588728427887,0.01236710898227509
59960,119921,119920,239841,95.79935574531555,0.012347550221209671
60060,120121,120120,240241,95.93604874610901,0.01232803729818582
60160,120321,120320,240641,96.0763750076294,0.012308570059071607
60260,120521,120520,241041,96.21327090263367,0.012289148350501572
60360,120721,120720,241441,96.3504786491394,0.01226977201987071
60460,120921,120920,241841,96.48836398124695,0.012250440915328632
60561,121123,121122,242245,96.62880682945251,0.012230962252597479
60661,121323,121322,242645,96.77012085914612,0.01221172159616075
60761,121523,121522,243045,96.90875482559204,0.012192525713239316
60861,121723,121722,243445,97.05182886123657,0.012173374454951404
60961,121923,121922,243845,97.19072270393372,0.01215426767314145
61061,122123,122122,244245,97.32937288284302,0.012135205220374895
61161,122323,122322,244645,97.46736097335815,0.012116186949932379
61261,122523,122522,245045,97.61078667640686,0.012097212715804754
61361,122723,122722,245445,97.76535177230835,0.012078282372687483
61461,122923,122922,245845,97.94205284118652,0.01205939577597569
61562,123125,123124,246249,98.08090806007385,0.012040364571523868
61662,123325,123324,246649,98.21970582008362,0.0120215654704518
61762,123525,123524,247049,98.35911178588867,0.012002809684693572
61862,123725,123724,247449,98.49649095535278,0.011984097072397587
61962,123925,123924,247849,98.63636684417725,0.011965427492386235
62062,124125,124124,248249,98.77209973335266,0.011946800804150993
62162,124325,124324,248649,98.9133780002594,0.011928216867847589
62262,124525,124524,249049,99.05206990242004,0.011909675544291117
62362,124725,124724,249449,99.18971586227417,0.011891176694951261
62462,124925,124924,249849,99.32772469520569,0.011872720181947644
62563,125127,125126,250253,99.46958065032959,0.011854121937548822
62663,125327,125326,250653,99.64305186271667,0.011835750106090122
62763,125527,125526,251053,99.78349685668945,0.011817420199822857
62863,125727,125726,251453,99.96423196792603,0.011799132083426103
62963,125927,125926,251853,100.10282492637634,0.011780885622206022
63063,126127,126126,252253,100.2392578125,0.011762680682091079
63163,126327,126326,252653,100.3802878856659,0.011744517129627865
63263,126527,126526,253053,100.51718664169312,0.011726394831976827
63363,126727,126726,253453,100.65838885307312,0.011708313656907696
63463,126927,126926,253853,100.81118583679199,0.011690273472795353
63564,127129,127128,254257,100.95366978645325,0.011672094361274773
63664,127329,127328,254657,101.1182427406311,0.011654136173238737
63764,127529,127528,255057,101.26480793952942,0.011636218583577785
63864,127729,127728,255457,101.40157175064087,0.011618341463051452
63964,127929,127928,255857,101.56029987335205,0.011600504683003719
64064,128129,128128,256257,101.71345090866089,0.011582708115358976
64164,128329,128328,256657,101.86260199546814,0.011564951632618016
64264,128529,128528,257057,102.02452182769775,0.011547235107853984
64364,128729,128728,257457,102.1772358417511,0.011529558414708816
64464,128929,128928,257857,102.31560707092285,0.011511921427388995
64565,129131,129130,258261,102.45570778846741,0.011494148246054431
64665,129331,129330,258661,102.59349083900452,0.011476590689176235
64765,129531,129530,259061,102.77000188827515,0.011459072462854887
64865,129731,129730,259461,102.91005802154541,0.011441593443523404
64965,129931,129930,259861,103.04665398597717,0.011424153508160761
65065,130131,130130,260261,103.18808078765869,0.011406752534288241
65165,130331,130330,260661,103.32536482810974,0.011389390399965822
65265,130531,130530,261061,103.46353101730347,0.011372066983788637
65365,130731,130730,261461,103.5998227596283,0.011354782164883313
65465,130931,130930,261861,103.73961091041565,0.011337535822904688
65566,131133,131132,262265,103.87689280509949,0.011320155951482764
65666,131333,131332,262665,104.01487374305725,0.011302986586194321
65766,131533,131532,263065,104.15892386436462,0.011285855338745761
65866,131733,131732,263465,104.30894684791565,0.011268762090875073
65966,131933,131932,263865,104.44644093513489,0.011251706724831254
66066,132133,132132,264265,104.58685493469238,0.011234689123371028
66166,132333,132332,264665,104.72724199295044,0.011217709169755707
66266,132533,132532,265065,104.86812376976013,0.011200766747747691
66366,132733,132732,265465,105.00647974014282,0.011183861741607555
66466,132933,132932,265865,105.14606285095215,0.011166994036090673
66567,133135,133134,266269,105.28568291664124,0.011149995398649155
66667,133335,133334,266669,105.42239093780518,0.01113320232074906
66767,133535,133534,267069,105.55910181999207,0.011116446199540608
66867,133735,133734,267469,105.70390772819519,0.011099726921732184
66967,133935,133934,267869,105.84437680244446,0.011083044374511446
67067,134135,134134,268269,105.98192262649536,0.011066398445542447
67167,134335,134334,268669,106.12137484550476,0.011049789022962631
67267,134535,134534,269069,106.26188278198242,0.011033215995379778
67367,134735,134734,269469,106.41705393791199,0.011016679251869298
67467,134935,134934,269869,106.55633878707886,0.0110001786819711
67568,135137,135136,270273,106.70031690597534,0.010983549712374231
67668,135337,135336,270673,106.83987474441528,0.010967121519153593
67768,135537,135536,271073,106.97951483726501,0.010950729169835593
67868,135737,135736,271473,107.1165509223938,0.010934372555794594
67968,135937,135936,271873,107.2581148147583,0.010918051568855542
68068,136137,136136,272273,107.39563584327698,0.010901766101291118
68168,136337,136336,272673,107.53469061851501,0.01088551604581895
68268,136537,136536,273073,107.67404699325562,0.010869301295599118
68368,136737,136736,273473,107.81630897521973,0.010853121744231246
68468,136937,136936,273873,107.95468592643738,0.010836977285752086
68569,137139,137138,274277,108.09551477432251,0.010820706896251716
68669,137339,137338,274677,108.23859882354736,0.010804632655688488
68769,137539,137538,275077,108.40253067016602,0.010788593191675569
68869,137739,137738,275477,108.58923292160034,0.010772588399976161
68969,137939,137938,275877,108.7675929069519,0.010756618176777446
69069,138139,138138,276277,108.94416189193726,0.01074068241868826
69169,138339,138338,276677,109.09804391860962,0.010724781022736616
69269,138539,138538,277077,109.2518846988678,0.010708913886367213
69369,138739,138738,277477,109.40329074859619,0.010693080907438939
69469,138939,138938,277877,109.5542049407959,0.010677281984222546
69570,139141,139140,278281,109.75689601898193,0.0106613595368379
69670,139341,139340,278681,109.92366886138916,0.010645628759519424
69770,139541,139540,279081,110.06901097297668,0.010629931734169071
69870,139741,139740,279481,110.21507406234741,0.010614268360685181
69970,139941,139940,279881,110.3663239479065,0.01059863853936608
70070,140141,140140,280281,110.52392983436584,0.010583042170907768
70170,140341,140340,280681,110.69974398612976,0.010567479156401759
70270,140541,140540,281081,110.8492968082428,0.010551949397332722
70370,140741,140740,281481,110.99821996688843,0.01053645279557633
70470,140941,140940,281881,111.15212798118591,0.01052098925339699
70571,141143,141142,282285,111.31580591201782,0.010505404533777012
70671,141343,141342,282685,111.5100679397583,0.010490007147253242
70771,141543,141542,283085,111.66594099998474,0.010474642528446447
70871,141743,141742,283485,111.82035779953003,0.010459310581157993
70971,141943,141942,283885,111.95671772956848,0.010444011209567077
71071,142143,142142,284285,112.09353804588318,0.010428744318228945
71171,142343,142342,284685,112.22856783866882,0.01041350981207237
71271,142543,142542,285085,112.36564302444458,0.010398307596397902
71371,142743,142742,285485,112.50172591209412,0.010383137576875551
71471,142943,142942,285885,112.64160895347595,0.010367999659543051
71572,143145,143144,286289,112.79064989089966,0.010352742853043743
71672,143345,143344,286689,112.94397902488708,0.010337669178347931
71772,143545,143544,287089,113.08701586723328,0.010322627325213274
71872,143745,143744,287489,113.25189185142517,0.010307617201131205
71972,143945,143944,287889,113.40697979927063,0.010292638713950824
72072,144145,144144,288289,113.56158065795898,0.01027769177187676
72172,144345,144344,288689,113.70505595207214,0.010262776283467645
72272,144545,144544,289089,113.84617376327515,0.010247892157633672
72372,144745,144744,289489,113.98944282531738,0.010233039303635262
72472,144945,144944,289889,114.13925766944885,0.01021821763108069
72573,145147,145146,290293,114.28895592689514,0.010203279300820748
72673,145347,145346,290693,114.42805075645447,0.010188520030927118
72773,145547,145546,291093,114.57385683059692,0.010173791672480472
72873,145747,145746,291493,114.71752882003784,0.010159094136466484
72973,145947,145946,291893,114.85452270507812,0.010144427334209621
73073,146147,146146,292293,115.00177001953125,0.01012979117737153
73173,146347,146346,292693,115.15779781341553,0.010115185577949172
73273,146547,146546,293093,115.30930376052856,0.01010061044827318
73373,146747,146746,293493,115.47174382209778,0.010086065701005903
73473,146947,146946,293893,115.66998887062073,0.010071551249139847
73574,147149,147148,294297,115.83818078041077,0.01005692231582622
73674,147349,147348,294697,116.00149297714233,0.010042468495840836
73774,147549,147548,295097,116.17995977401733,0.010028044711339279
73874,147749,147748,295497,116.33520674705505,0.010013650876620636
73974,147949,147948,295897,116.49309802055359,0.009999286906305714
74074,148149,148148,296297,116.65278697013855,0.00998495271533535
74174,148349,148348,296697,116.83286094665527,0.009970648218968625
74274,148549,148548,297097,116.99748873710632,0.0099563733327815
74374,148749,148748,297497,117.14688181877136,0.009942127972664876
74474,148949,148948,297897,117.32297492027283,0.00992791205482332
74575,149151,149150,298301,117.47866797447205,0.009913583778163
74675,149351,149350,298701,117.62337279319763,0.009899426787068365
74775,149551,149550,299101,117.77438068389893,0.009885298987900538
74875,149751,149750,299501,117.93020272254944,0.009871200298105322
74975,149951,149950,299901,118.0708179473877,0.009857130635434221
75075,150151,150150,300301,118.22449684143066,0.009843089917942964
75175,150351,150350,300701,118.37483477592468,0.00982907806398986
75275,150551,150550,301101,118.53635573387146,0.00981509499223439
75375,150751,150750,301501,118.6850597858429,0.009801140621635535
75475,150951,150950,301901,118.83643579483032,0.009787214871450541
75576,151153,151152,302305,118.99709677696228,0.009773178832986541
75676,151353,151352,302705,119.15059566497803,0.009759310366780592
75776,151553,151552,303105,119.29952692985535,0.009745470279737227
75876,151753,151752,303505,119.46893787384033,0.009731658492294576
75976,151953,151952,303905,119.63007998466492,0.0097178749251816
76076,152153,152152,304305,119.78420686721802,0.009704119499416724
76176,152353,152352,304705,119.94194793701172,0.009690392136306415
76276,152553,152552,305105,120.11048769950867,0.009676692757443756
76376,152753,152752,305505,120.26459169387817,0.00966302128470716
76476,152953,152952,305905,120.42042088508606,0.009649377640258878
76577,153155,153154,306309,120.57404685020447,0.009635625727486065
76677,153355,153354,306709,120.72712874412537,0.009622037783575196
76777,153555,153554,307109,120.88072776794434,0.009608477435360597
76877,153755,153754,307509,121.07538890838623,0.009594944606129162
76977,153955,153954,307909,121.2291738986969,0.009581439219445069
77077,154155,154154,308309,121.38247489929199,0.009567961199148232
77177,154355,154354,308709,121.55996894836426,0.009554510469353053
77277,154555,154554,309109,121.71825385093689,0.009541086954447145
77377,154755,154754,309509,121.86335182189941,0.00952769057909001
77477,154955,154954,309909,122.00274300575256,0.009514321268211777
77578,155157,155156,310313,122.14138579368591,0.009500845659845384
77678,155357,155356,310713,122.27969884872437,0.00948753052256744
77778,155557,155556,311113,122.41613984107971,0.009474242225428524
77878,155757,155756,311513,122.55758380889893,0.009460980694431215
77978,155957,155956,311913,122.69669771194458,0.009447745855842505
78078,156157,156156,312313,122.83424162864685,0.009434537636192349
78178,156357,156356,312713,122.97447967529297,0.009421355962272702
78278,156557,156556,313113,123.11390280723572,0.00940820076113614
78378,156757,156756,313513,123.25173497200012,0.00939507196009464
78478,156957,156956,313913,123.38852405548096,0.00938196948671854
78579,157159,157158,314317,123.52968692779541,0.009368762639003063
78679,157359,157358,314717,123.68610095977783,0.009355712866169126
78779,157559,157558,315117,123.83247780799866,0.009342689204533832
78879,157759,157758,315517,123.97322487831116,0.009329691582691197
78979,157959,157958,315917,124.11330199241638,0.00931671992948766
79079,158159,158158,316317,124.25182390213013,0.009303774174020951
79179,158359,158358,316717,124.3929808139801,0.009290854245638795
79279,158559,158558,317117,124.53407263755798,0.009277960073937962
79379,158759,158758,317517,124.6854977607727,0.00926509158876296
79479,158959,158958,317917,124.84223365783691,0.009252248720205199
79580,159161,159160,318321,124.98527693748474,0.009239303354162473
79680,159361,159360,318721,125.1247878074646,0.009226511764519909
79780,159561,159560,319121,125.27179288864136,0.009213745582547072
79880,159761,159760,319521,125.4353289604187,0.009201004739313621
79980,159961,159960,319921,125.58103585243225,0.009188289166130226
80080,160161,160160,320321,125.76985883712769,0.009175598794547902
80180,160361,160360,320721,125.92865085601807,0.009162933556356601
80280,160561,160560,321121,126.06532192230225,0.0091502933835844
80380,160761,160760,321521,126.20504093170166,0.009137678208496288
80480,160961,160960,321921,126.37630796432495,0.009125087963593204
80581,161163,161162,322325,126.54357767105103,0.009112397053121802
80681,161363,161362,322725,126.6927638053894,0.00909985671465115
80781,161563,161562,323125,126.85636782646179,0.009087341104606664
80881,161763,161762,323525,127.00050377845764,0.009074850156424858
80981,161963,161962,323925,127.16283392906189,0.00906238380377307
81081,162163,162162,324325,127.30944776535034,0.009049941980548438
81181,162363,162362,324725,127.47383284568787,0.00903752462087687
81281,162563,162562,325125,127.63724899291992,0.00902513165911197
81381,162763,162762,325525,127.77361989021301,0.009012763029834198
81481,162963,162962,325925,127.9265558719635,0.009000418667849718
81582,163165,163164,326329,128.0838499069214,0.008987975428595498
81682,163365,163364,326729,128.248596906662,0.008975679647564273
81782,163565,163564,327129,128.40805673599243,0.008963407938945957
81882,163765,163764,327529,128.5775318145752,0.008951160238442469
81982,163965,163964,327929,128.71837186813354,0.008938936481976746
82082,164165,164164,328329,128.86724972724915,0.008926736605691652
82182,164365,164364,328729,129.00679683685303,0.00891456054594913
82282,164565,164564,329129,129.1476287841797,0.008902408239329317
82382,164765,164764,329529,129.28996300697327,0.008890279622629579
82482,164965,164964,329929,129.44888281822205,0.008878174632863426
82583,165167,165166,330333,129.60233688354492,0.008865972511791073
82683,165367,165366,330733,129.75061082839966,0.008853914822494502
82783,165567,165566,331133,129.92469787597656,0.00884188057183861
82883,165767,165766,331533,130.08220791816711,0.00882986969769517
82983,165967,165966,331933,130.26175999641418,0.008817882138147685
83083,166167,166166,332333,130.41188097000122,0.008805917831490507
83183,166367,166366,332733,130.56286001205444,0.008793976716227883
83283,166567,166566,333133,130.7161328792572,0.008782058731073293
83383,166767,166766,333533,130.86024284362793,0.008770163814948245
83483,166967,166966,333933,131.00860285758972,0.008758291906981772
83584,167169,167168,334337,131.15351176261902,0.008746324572584651
83684,167369,167368,334737,131.2997727394104,0.008734498727712887
83784,167569,167568,335137,131.45223593711853,0.008722695709020326
83884,167769,167768,335537,131.62589287757874,0.008710915456458839
83984,167969,167968,335937,131.79679107666016,0.008699157910183178
84084,168169,168168,336337,131.96790599822998,0.008687423010550298
84184,168369,168368,336737,132.14559173583984,0.008675710698118596
84284,168569,168568,337137,132.31141781806946,0.008664020913647038
84384,168769,168768,337537,132.4697687625885,0.008652353598094296
84484,168969,168968,337937,132.6296796798706,0.008640708692617936
84585,169171,169170,338341,132.77779984474182,0.008628970025709922
84685,169371,169370,338741,132.92731285095215,0.008617369987285886
84785,169571,169570,339141,133.07367181777954,0.008605792183014695
84885,169771,169770,339541,133.2280478477478,0.008594236554843345
84985,169971,169970,339941,133.3905599117279,0.008582703044913742
85085,170171,170170,340341,133.5473599433899,0.008571191595561807
85185,170371,170370,340741,133.7092628479004,0.008559702149316813
85285,170571,170570,341141,133.85274696350098,0.008548234648900484
85385,170771,170770,341541,133.99913382530212,0.008536789037226163
85485,170971,170970,341941,134.13839983940125,0.00852536525739832
85586,171173,171172,342345,134.27999472618103,0.008513849342437672
85686,171373,171372,342745,134.45551776885986,0.008502469273277233
85786,171573,171572,343145,134.6391658782959,0.00849111086585197
85886,171773,171772,343545,134.783344745636,0.008479774064024255
85986,171973,171972,343945,134.94074082374573,0.008468458811843493
86086,172173,172172,344345,135.116516828537,0.008457165053545518
86186,172373,172372,344745,135.27833771705627,0.00844589273355175
86286,172573,172572,345145,135.43167686462402,0.008434641796468531
86386,172773,172772,345545,135.5699577331543,0.008423412187086277
86486,172973,172972,345945,135.71678471565247,0.008412203850378878
86587,173175,173174,346349,135.85392379760742,0.008400904967279037
86687,173375,173374,346749,135.9954957962036,0.008389739222929127
86787,173575,173574,347149,136.13379788398743,0.008378594586724877
86887,173775,173774,347549,136.28429579734802,0.008367471004368328
86987,173975,173974,347949,136.44430685043335,0.008356368421741254
87087,174175,174174,348349,136.59942078590393,0.008345286784904541
87187,174375,174374,348749,136.7954568862915,0.008334226040097426
87287,174575,174574,349149,136.9629566669464,0.00832318613373682
87387,174775,174774,349549,137.13307070732117,0.008312167012416565
87487,174975,174974,349949,137.2737488746643,0.008301168622906842
87588,175177,175176,350353,137.41599583625793,0.008290081239294492
87688,175377,175376,350753,137.56180477142334,0.008279124360410202
87788,175577,175576,351153,137.71506786346436,0.008268188054171297
87888,175777,175776,351553,137.86152982711792,0.008257272268047962
87988,175977,175976,351953,138.01831483840942,0.008246376949683042
88088,176177,176176,352353,138.17918491363525,0.008235502046891623
88188,176377,176376,352753,138.33376169204712,0.008224647507660221
88288,176577,176576,353153,138.50806975364685,0.008213813280146202
88388,176777,176776,353553,138.65686178207397,0.00820299931267709
88488,176977,176976,353953,138.8043828010559,0.008192205553749962
88589,177179,177178,354357,138.9593858718872,0.008181324317634046
88689,177379,177378,354757,139.1055588722229,0.008170571022759168
88789,177579,177578,355157,139.24058389663696,0.008159837782418624
88889,177779,177778,355557,139.37818479537964,0.008149124545782496
88989,177979,177978,355957,139.5398018360138,0.008138431262187258
89089,178179,178178,356357,139.85568475723267,0.008127757881134784
89189,178379,178378,356757,140.03038692474365,0.00811710435229215
89289,178579,178578,357157,140.19322180747986,0.008106470625490499
89389,178779,178778,357557,140.35840678215027,0.00809585665072483
89489,178979,178978,357957,140.5411388874054,0.008085262378153189
89590,179181,179180,358361,140.74852776527405,0.008074582110972974
89690,179381,179380,358761,140.92117977142334,0.008064027289693009
89790,179581,179580,359161,141.14886665344238,0.008053492021560556
89890,179781,179780,359561,141.31525182724,0.008042976257381264
89990,179981,179980,359961,141.476069688797,0.00803247994812076
90090,180181,180180,360361,141.6473789215088,0.008022003044904101
90190,180381,180380,360761,141.8068187236786,0.008011545499014991
90290,180581,180580,361161,141.97564792633057,0.008001107261895308
90390,180781,180780,361561,142.14224791526794,0.007990688285144496
90490,180981,180980,361961,142.30378985404968,0.007980288520518969
90591,181183,181182,362365,142.46888875961304,0.007969804210541661
90691,181383,181382,362765,142.62367177009583,0.007959442916980157
90791,181583,181582,363165,142.79148173332214,0.00794910069127186
90891,181783,181782,363565,142.98132872581482,0.007938777485796538
90991,181983,181982,363965,143.16447162628174,0.007928473253087964
91091,182183,182182,364365,143.34598183631897,0.007918187945833367
91191,182383,182382,364765,143.52281379699707,0.007907921516872833
91291,182583,182582,365165,143.68189001083374,0.007897673919198569
91391,182783,182782,365565,143.85624885559082,0.007887445105954636
91491,182983,182982,365965,144.01464176177979,0.007877235030436138
91592,183185,183184,366369,144.170649766922,0.007866941826478525
91692,183385,183384,366769,144.32359886169434,0.0078567692731117
91792,183585,183584,367169,144.50121188163757,0.00784661531779491
91892,183785,183784,367569,144.67777585983276,0.007836479914423562
91992,183985,183984,367969,144.8327558040619,0.007826363017041432
92092,184185,184184,368369,145.00227880477905,0.007816264579839964
92192,184385,184384,368769,145.18119978904724,0.007806184557157917
92292,184585,184584,369169,145.3630018234253,0.0077961229034805455
92392,184785,184784,369569,145.52877593040466,0.007786079573439365
92492,184985,184984,369969,145.93147373199463,0.007776054521811322
92593,185187,185186,370373,146.18923687934875,0.0077659477272617955
92693,185387,185386,370773,146.42428994178772,0.007755959279028298
92793,185587,185586,371173,146.88805294036865,0.00774598897395979
92893,185787,185786,371573,147.36049103736877,0.007736036767411587
92993,185987,185986,371973,147.71583676338196,0.007726102614881864
93093,186187,186186,372373,147.96683478355408,0.00771618647201114
93193,186387,186386,372773,148.20012068748474,0.007706288294581779
93293,186587,186586,373173,148.3766577243805,0.007696408038517362
93393,186787,186786,373573,148.6666738986969,0.007686545659882374
93493,186987,186986,373973,148.8832356929779,0.007676701114881473
93594,187189,187188,374377,149.0786018371582,0.007666776182000901
93694,187389,187388,374777,149.2723948955536,0.007656967350685936
93794,187589,187588,375177,149.469340801239,0.0076471762220223765
93894,187789,187788,375577,149.66383171081543,0.007637402752772151
93994,187989,187988,375977,149.84480786323547,0.007627646899834897
94094,188189,188188,376377,149.99498963356018,0.007617908620247393
94194,188389,188388,376777,150.15068697929382,0.0076081878711831774
94294,188589,188588,377177,150.30525588989258,0.007598484609951875
94394,188789,188788,377577,150.44918990135193,0.007588798793998877
94494,188989,188988,377977,150.60815000534058,0.007579130380904666
94595,189191,189190,378381,150.7547047138214,0.007569382905387485
94695,189391,189390,378781,150.89684581756592,0.007559749344262658
94795,189591,189590,379181,151.08981776237488,0.007550133059124971
94895,189791,189790,379581,151.2778959274292,0.0075405340080920945
94995,189991,189990,379981,151.46065998077393,0.007530952149414454
95095,190191,190190,380381,151.66411805152893,0.007521387441474787
95195,190391,190390,380781,151.8393428325653,0.007511839842787465
95295,190591,190590,381181,152.03225684165955,0.0075023093119982445
95395,190791,190790,381581,152.18784165382385,0.007492795807883659
95495,190991,190990,381981,152.338223695755,0.007483299289350599
95596,191193,191192,382385,152.50071501731873,0.00747372500512869
95696,191393,191392,382785,152.6608738899231,0.007464262503830366
95796,191593,191592,383185,152.8243477344513,0.007454816865205057
95896,191793,191792,383585,152.98349380493164,0.007445388048677621
95996,191993,191992,383985,153.1467640399933,0.007435976013800798
96096,192193,192192,384385,153.3053708076477,0.007426580720254902
96196,192393,192392,384785,153.4774248600006,0.00741720212784732
96296,192593,192592,385185,153.63528776168823,0.00740784019651204
96396,192793,192792,385585,153.78881001472473,0.00739849488630915
96496,192993,192992,385985,154.19797086715698,0.007389166157424452
96597,193195,193194,386389,154.39213490486145,0.007379760931697754
96697,193395,193394,386789,154.53018188476562,0.007370465411328744
96797,193595,193594,387189,154.67356896400452,0.007361186353191253
96897,193795,193794,387589,154.81192874908447,0.0073519237179705925
96997,193995,193994,387989,155.01846885681152,0.007342677466475559
97097,194195,194194,388389,155.2080478668213,0.007333447559637854
97197,194395,194394,388789,155.36803770065308,0.007324233958511813
97297,194595,194594,389189,155.5416009426117,0.0073150366242738735
97397,194795,194794,389589,155.6977777481079,0.007305855518222141
97497,194995,194994,389989,155.83943486213684,0.007296690601775942
97598,195197,195196,390393,155.97863602638245,0.007287450430255907
97698,195397,195396,390793,156.1172788143158,0.0072783179386965826
97798,195597,195596,391193,156.2650008201599,0.007269201521342371
97898,195797,195796,391593,156.41580963134766,0.007260101140094465
97998,195997,195996,391993,156.55590987205505,0.007251016756973199
98098,196197,196196,392393,156.70049571990967,0.007241948334117486
98198,196397,196396,392793,156.84124064445496,0.007232895833784522
98298,196597,196596,393193,156.9839518070221,0.007223859218349286
98398,196797,196796,393593,157.12638902664185,0.007214838450304185
98498,196997,196996,393993,157.26476073265076,0.007205833492258538
98599,197199,197198,394397,157.40242886543274,0.007196754494611566
98699,197399,197398,394797,157.5398347377777,0.007187781202027244
98799,197599,197598,395197,157.6781439781189,0.007178823607598379
98899,197799,197798,395597,157.81642293930054,0.0071698816743992365
98999,197999,197998,395997,157.9548478126526,0.007160955365619003
99099,198199,198198,396397,158.09150981903076,0.007152044644561347
99199,198399,198398,396797,158.2294316291809,0.007143149474644061
99299,198599,198598,397197,158.36894369125366,0.007134269819398599
99399,198799,198798,397597,158.52389287948608,0.0071254056424696855
99499,198999,198998,397997,158.66252779960632,0.007116556907614964
99600,199201,199200,398401,158.8016209602356,0.0071076353230935165
99700,199401,199400,398801,158.93969583511353,0.007098817517627355
99800,199601,199600,399201,159.07932376861572,0.007090015045823082
99900,199801,199800,399601,159.21761679649353,0.007081227871886953
100000,200001,200000,400001,159.35746574401855,0.007072455960136204


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha0/flex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007658004760742188,30.358099469249375
100,459,0,459,0.7737970352172852,0.4215230331922254
200,946,0,946,1.682675838470459,0.14415849683191745
300,1439,0,1439,2.456393003463745,0.08296605369719261
400,1934,0,1934,3.3106391429901123,0.062152216402440015
501,2439,0,2439,4.015656232833862,0.05516804045776081
601,2936,0,2936,4.708676099777222,0.04367911425214777
701,3436,0,3436,5.647229194641113,0.04257054126154854
801,3934,0,3934,7.0424559116363525,0.03609704005457046
901,4433,0,4433,8.301010847091675,0.03464549120420115
1001,4931,0,4931,9.518473863601685,0.027923755909865604
1101,5431,0,5431,10.941987991333008,0.027367716864216383
1201,5930,0,5930,12.25145697593689,0.02563948412180267
1301,6430,0,6430,13.408919095993042,0.024929295322853623
1401,6925,0,6925,14.608083009719849,0.018852531343604755
1502,7430,0,7430,15.793203115463257,0.017711548583424178
1602,7930,0,7930,16.942715167999268,0.01744872389806109
1702,8430,0,8430,18.04382300376892,0.017277335657916865
1802,8929,0,8929,19.158313035964966,0.01624345545841913
1902,9429,0,9429,20.258270978927612,0.015892218609013832
2002,9925,0,9925,21.372305154800415,0.01252232208241908
2102,10422,0,10422,22.47426700592041,0.009447387251569574
2202,10922,0,10922,23.612605810165405,0.009215036792858521
2302,11422,0,11422,24.72783613204956,0.009092578858768892
2402,11921,0,11921,25.832401037216187,0.008625108105700349
2503,12426,0,12426,26.942195892333984,0.008411289735192114
2603,12926,0,12926,28.046991109848022,0.008330120159723786
2703,13425,0,13425,29.304179906845093,0.007820011044585375
2803,13925,0,13925,30.534913063049316,0.007692774522163792
2903,14425,0,14425,31.59478497505188,0.007636663845164925
3003,14925,0,14925,32.55903100967407,0.007602754988352579
3103,15425,0,15425,33.513426065444946,0.007578790450769863
3203,15919,0,15919,34.520222902297974,0.005293676943958086
3303,16414,0,16414,35.61281204223633,0.0036085656182544283
3403,16914,0,16914,36.73590016365051,0.0034271129373004165
3504,17419,0,17419,37.98022389411926,0.0033262958100213733
3604,17919,0,17919,39.141324043273926,0.0032643605357133565
3704,18419,0,18419,40.24874806404114,0.003222736346880356
3804,18919,0,18919,41.34216809272766,0.003192812212130553
3904,19419,0,19419,42.46130609512329,0.003169946832750147
4004,19917,0,19917,43.614588022232056,0.0029371126523334494
4104,20417,0,20417,44.86804008483887,0.0028292052830992233
4204,20917,0,20917,45.99265718460083,0.002779301627360435
4304,21417,0,21417,47.11980104446411,0.0027491676300833543
4404,21917,0,21917,48.33974504470825,0.0027278821444051094
4505,22422,0,22422,49.453787088394165,0.0027114179130843267
4605,22922,0,22922,50.66906809806824,0.0026983545362234246
4705,23421,0,23421,51.77903890609741,0.0026161719723428495
4805,23921,0,23921,52.90787696838379,0.002541686084152088
4905,24421,0,24421,54.31958508491516,0.0025047428276595615
5005,24921,0,24921,55.53780007362366,0.0024828284896996696
5105,25421,0,25421,56.971012115478516,0.002468301939107873
5205,25921,0,25921,58.198824882507324,0.0024579266179626264
5305,26420,0,26420,59.46351194381714,0.0023760284154975995
5405,26920,0,26920,60.80050992965698,0.002314845987550788
5506,27425,0,27425,61.91122817993164,0.0022859141051942175
5606,27925,0,27925,63.02983808517456,0.0022687141955904625
5706,28425,0,28425,64.13093590736389,0.002257211602285903
5806,28925,0,28925,65.24243307113647,0.002249077473075496
5906,29425,0,29425,66.34016990661621,0.0022430796868371378
6006,29925,0,29925,67.43895101547241,0.00223848457250731
6106,30425,0,30425,68.53821897506714,0.002234830042701346
6206,30924,0,30924,69.63856887817383,0.002132951801704158
6306,31424,0,31424,70.73419904708862,0.0020811789782760872
6406,31924,0,31924,71.8436279296875,0.0020632462997641167
6507,32429,0,32429,73.02259612083435,0.0020544806331060064
6607,32929,0,32929,74.1492190361023,0.002049188344675788
6707,33429,0,33429,75.30297708511353,0.0020454918546595176
6807,33928,0,33928,76.47895693778992,0.001990149044989715
6907,34428,0,34428,77.63214683532715,0.0019476073657675428
7007,34928,0,34928,78.76351714134216,0.0019292345755647455
7107,35428,0,35428,79.86471796035767,0.0019183620866525238
7207,35928,0,35928,80.96234488487244,0.001910902595981127
7307,36428,0,36428,82.0872790813446,0.0019053630377742002
7407,36928,0,36928,83.1859838962555,0.0019010240235913544
7508,37433,0,37433,84.3192241191864,0.0018974510214569372
7608,37933,0,37933,85.45661902427673,0.0018944690699334874
7708,38433,0,38433,86.595468044281,0.0018918839274351677
7808,38933,0,38933,87.70897507667542,0.0018895926298098194
7908,39433,0,39433,88.81377100944519,0.0018875250451852474
8008,39933,0,39933,89.94094109535217,0.001885632277754813
8108,40433,0,40433,91.04318499565125,0.0018838794991216097
8208,40932,0,40932,92.19147205352783,0.001818760712723228
8308,41432,0,41432,93.30373811721802,0.001789968389969063
8408,41932,0,41932,94.39993214607239,0.0017736841118643847
8509,42437,0,42437,95.54891109466553,0.0017630636554577294
8609,42937,0,42937,96.69876503944397,0.0017555361023137363
8709,43437,0,43437,97.79296612739563,0.001749753337854293
8809,43937,0,43937,98.89291596412659,0.001745112907184908
8909,44437,0,44437,100.13803505897522,0.0017412824566138965
9009,44937,0,44937,101.3314118385315,0.0017380585900383778
9109,45437,0,45437,102.56417989730835,0.001735305801026813
9209,45937,0,45937,103.84314012527466,0.00173292789076306
9309,46437,0,46437,105.08283114433289,0.0017308533956030628
9409,46937,0,46937,106.65674686431885,0.0017290274990321652
9510,47442,0,47442,108.02126097679138,0.001727391894159333
9610,47942,0,47942,109.24916100502014,0.0017259443884881584
9710,48442,0,48442,110.58175110816956,0.0017246401418321206
9810,48941,0,48941,111.8296492099762,0.0016566217528740093
9910,49441,0,49441,113.13871502876282,0.0016355190794475785
10010,49941,0,49941,114.36730003356934,0.001623278665956409
10110,50441,0,50441,115.5941870212555,0.0016155208792982
10210,50941,0,50941,116.83213686943054,0.0016102240815659657
10310,51441,0,51441,117.95291590690613,0.001606383580265625
10410,51941,0,51941,119.18492102622986,0.001603461815794071
10511,52446,0,52446,120.35008811950684,0.001601130676987706
10611,52946,0,52946,121.52515602111816,0.0015992491856991766
10711,53446,0,53446,122.84983110427856,0.001597674155605504
10811,53946,0,53946,124.03976202011108,0.0015963280313644876
10911,54446,0,54446,125.2580578327179,0.0015951577712940757
11011,54946,0,54946,126.43523716926575,0.001594125935720596
11111,55446,0,55446,127.77248001098633,0.0015932053251746364
11211,55946,0,55946,128.9714539051056,0.0015923756535023295
11311,56446,0,56446,130.06284999847412,0.001591621427864598
11411,56946,0,56946,131.07624220848083,0.0015909305645563751
11512,57451,0,57451,132.1764190196991,0.0015902873370042285
11612,57951,0,57951,133.4612112045288,0.0015896966775691592
11712,58451,0,58451,134.80274391174316,0.0015891456375254516
11812,58951,0,58951,136.0407190322876,0.0015886289817222728
11912,59451,0,59451,137.31993913650513,0.0015881423354250222
12012,59951,0,59951,138.8134000301361,0.0015876820125445648
12112,60451,0,60451,140.33017897605896,0.0015872448850688084
12212,60951,0,60951,141.69598603248596,0.001586828282093145
12312,61451,0,61451,143.0696530342102,0.001586429910538285
12412,61951,0,61951,144.56727814674377,0.0015860477920604298
12513,62456,0,62456,145.91614890098572,0.0015856766046706992
12613,62956,0,62956,147.10823106765747,0.0015853221954172773
12713,63456,0,63456,148.44882988929749,0.0015849795179945934
12813,63955,0,63955,149.81937408447266,0.0015701138571453039
12913,64455,0,64455,151.1908860206604,0.0015401165917221908
13013,64955,0,64955,152.42096519470215,0.0015256935044077274
13113,65455,0,65455,153.9053831100464,0.0015152047311114206
13213,65955,0,65955,155.0322539806366,0.0015074338869126118
13313,66455,0,66455,156.21609115600586,0.0015015640917532417
13413,66955,0,66955,157.51556086540222,0.0014970422161749725
13514,67460,0,67460,158.77929210662842,0.0014934591259298169
13614,67960,0,67960,160.20272397994995,0.0014906237674928216
13714,68460,0,68460,161.88144302368164,0.0014883154713495991
13814,68960,0,68960,163.5579960346222,0.0014864064375659173
13914,69460,0,69460,165.82221508026123,0.001484805072472107
14014,69960,0,69960,167.52975296974182,0.0014834447352621882
14114,70460,0,70460,169.26739597320557,0.0014822761774845338
14214,70960,0,70960,170.77102994918823,0.001481262423698918
14314,71460,0,71460,172.07248902320862,0.001480375273999726
14414,71960,0,71960,173.35135412216187,0.0014795928907542146
14515,72465,0,72465,174.89433789253235,0.00147889156131945
14615,72965,0,72965,176.10711908340454,0.0014782714062944252
14715,73465,0,73465,177.51745510101318,0.0014777140680310014
14815,73965,0,73965,178.78357815742493,0.0014772105686330535
14915,74465,0,74465,180.2507529258728,0.0014767535052233086
15015,74965,0,74965,182.02218413352966,0.0014763367165983934
15115,75465,0,75465,183.29220604896545,0.001475955032258607
15215,75965,0,75965,184.50288820266724,0.0014756040809814964
15315,76465,0,76465,185.9276750087738,0.001475280142958771
15415,76965,0,76965,187.3540861606598,0.0014749800341990994
15516,77470,0,77470,188.5548870563507,0.0014746983231414155
15616,77970,0,77970,189.78364419937134,0.0014744382018808887
15716,78470,0,78470,190.9731891155243,0.001474194727116462
15816,78970,0,78970,192.25431895256042,0.0014739661098606962
15916,79470,0,79470,193.65815496444702,0.0014737507857434508
16016,79970,0,79970,195.18037700653076,0.0014735473824631503
16116,80470,0,80470,196.6473560333252,0.001473354692677223
16216,80970,0,80970,197.8795518875122,0.0014731716512845997
16316,81470,0,81470,199.42486810684204,0.0014729973162833812
16416,81970,0,81970,200.9453740119934,0.0014728308525596907
16517,82475,0,82475,202.60086917877197,0.0014726699584566392
16617,82975,0,82975,204.0821590423584,0.001472517154151235
16717,83475,0,83475,205.6740870475769,0.001472370223352663
16817,83975,0,83975,206.92817616462708,0.001472228639679986
16917,84475,0,84475,208.15181803703308,0.0014720919316991159
17017,84975,0,84975,209.3706841468811,0.0014719596764349169
17117,85475,0,85475,210.62831711769104,0.0014718314937380694
17217,85975,0,85975,212.07923913002014,0.001471707041381574
17317,86475,0,86475,213.35312509536743,0.001471586010782027
17417,86975,0,86975,214.7158510684967,0.0014714681232576364
17518,87480,0,87480,216.07056403160095,0.0014713519905920223
17618,87980,0,87980,218.05108308792114,0.001471239682327715
17718,88479,0,88479,220.1360239982605,0.001453726355615352
17818,88979,0,88979,221.94627499580383,0.0014398274654221306
17918,89479,0,89479,223.36386919021606,0.001428443320114839
18018,89979,0,89979,224.68647289276123,0.0014190832050994422
18118,90479,0,90479,226.40856909751892,0.0014113554373204476
18218,90979,0,90979,227.89763712882996,0.0014049471186303526
18318,91479,0,91479,229.2643210887909,0.0013996080137561534
18418,91979,0,91979,231.05897116661072,0.001395137718930886
18519,92484,0,92484,232.8597390651703,0.0013913409649710562
18619,92984,0,92984,234.7061550617218,0.0013881627893074368
18719,93484,0,93484,236.57717299461365,0.0013854584796166465
18819,93984,0,93984,237.89364290237427,0.0013831442424122957
18919,94484,0,94484,239.4499580860138,0.0013811522955727328
19019,94984,0,94984,240.78904604911804,0.0013794276768312346
19119,95484,0,95484,242.19161891937256,0.0013779257064189723
19219,95984,0,95984,243.46078515052795,0.001376609966952614
19319,96484,0,96484,244.75834584236145,0.0013754506926929812
19419,96984,0,96984,246.24877405166626,0.0013744234831896884
19520,97489,0,97489,247.79069900512695,0.0013734996292509543
19620,97989,0,97989,248.92548084259033,0.0013726807498526863
19720,98489,0,98489,250.03408312797546,0.0013719434925000403
19820,98989,0,98989,251.22583103179932,0.0013712764946652363
19920,99489,0,99489,252.4295711517334,0.001370670280247951
20020,99989,0,99989,253.58058905601501,0.0013701169149399786
20120,100489,0,100489,254.7513861656189,0.0013696097277896505
20220,100989,0,100989,255.98862886428833,0.0013691430858591969
20320,101489,0,101489,257.20357394218445,0.0013687122115252184
20420,101989,0,101989,258.7736849784851,0.0013683130340783618
20521,102494,0,102494,260.22864985466003,0.0013679384912659868
20621,102994,0,102994,261.43095302581787,0.0013675929799974653
20721,103494,0,103494,262.54585099220276,0.0013672700703054746
20821,103994,0,103994,263.6580410003662,0.0013669675167993843
20921,104494,0,104494,264.87980580329895,0.0013666833607098906
21021,104994,0,104994,266.0875520706177,0.0013664158854195408
21121,105494,0,105494,267.21782183647156,0.0013661635797571222
21221,105994,0,105994,268.5346260070801,0.0013659251076128494
21321,106494,0,106494,269.8905441761017,0.00136569928270858
21421,106994,0,106994,271.1915910243988,0.001365485047580314
21522,107499,0,107499,272.61920714378357,0.0013652794708947091
21622,107999,0,107999,273.84390020370483,0.0013650857671117862
21722,108499,0,108499,275.00320506095886,0.0013649010842918306
21822,108999,0,108999,276.1452510356903,0.001364724731112728
21922,109499,0,109499,277.34990096092224,0.0013645560808691443
22022,109999,0,109999,278.4691791534424,0.001364394563893769
22122,110499,0,110499,279.6695899963379,0.00136423966107005
22222,110999,0,110999,280.85793805122375,0.0013640908982552843
22322,111499,0,111499,282.04875802993774,0.0013639478414652275
22422,111999,0,111999,283.2534370422363,0.0013638100926986756
22523,112504,0,112504,284.4695611000061,0.0013636759820346493
22623,113004,0,113004,285.7271420955658,0.0013635478259691111
22723,113504,0,113504,286.96196699142456,0.0013634239626941452
22823,114004,0,114004,288.0769820213318,0.0013633041062352154
22923,114504,0,114504,289.32564187049866,0.0013631879923299258
23023,115004,0,115004,290.4861249923706,0.0013630753764940782
23123,115504,0,115504,291.59612703323364,0.001362966032298095
23223,116004,0,116004,292.7869770526886,0.0013628597498247291
23323,116504,0,116504,294.072722196579,0.0013627563342855226
23423,117004,0,117004,295.21978425979614,0.0013626556047754011
23524,117509,0,117509,296.32627606391907,0.0013625564232096173
23624,118009,0,118009,297.48679208755493,0.0013624605959271082
23724,118509,0,118509,298.69608902931213,0.0013623669831404747
23824,119009,0,119009,299.8309419155121,0.001362275449346738
23924,119509,0,119509,301.0782949924469,0.0013621858682550186
24024,120009,0,120009,302.3685739040375,0.001362098122090599
24124,120508,0,120508,303.54374384880066,0.0013496038612603265
24224,121008,0,121008,304.76537799835205,0.0013353275625803697
24324,121508,0,121508,306.0356469154358,0.0013234724561885377
24424,122008,0,122008,307.1708950996399,0.0013136215587083737
24525,122513,0,122513,308.3975601196289,0.0013053524753233582
24625,123013,0,123013,309.57282996177673,0.001298537863261558
24725,123513,0,123513,310.75980401039124,0.001292849323433793
24825,124013,0,124013,311.86107110977173,0.0012880896791945952
24925,124513,0,124513,312.9664990901947,0.0012840964428289625
25025,125013,0,125013,314.059739112854,0.0012807359139930705
25125,125513,0,125513,315.16960620880127,0.0012778981926325167
25225,126013,0,126013,316.2655260562897,0.0012754929973965582
25325,126513,0,126513,317.45694303512573,0.0012734461813433053
25425,127013,0,127013,318.5698800086975,0.0012716968431868603
25526,127518,0,127518,319.68397307395935,0.0012701810265898668
25626,128018,0,128018,320.77422404289246,0.0012688872985362634
25726,128518,0,128518,321.874489068985,0.001267765695935465
25826,129018,0,129018,322.97775506973267,0.0012667883749106455
25926,129518,0,129518,324.07425713539124,0.0012659323629714654
26026,130018,0,130018,325.177796125412,0.0012651786765798898
26126,130518,0,130518,326.2821969985962,0.00126451160021098
26226,131018,0,131018,327.3811800479889,0.001263918097595848
26326,131518,0,131518,328.4706599712372,0.0012633873309912703
26426,132018,0,132018,329.57163095474243,0.0012629102686370205
26527,132523,0,132523,330.68808913230896,0.0012624752658956023
26627,133023,0,133023,331.7960319519043,0.0012620845662822129
26727,133523,0,133523,332.9800088405609,0.0012617283391550204
26827,134023,0,134023,334.12314009666443,0.0012614021123656476
26927,134523,0,134523,335.22499203681946,0.0012611021030160413
27027,135023,0,135023,336.33029198646545,0.0012608251000913767
27127,135523,0,135523,337.4251592159271,0.001260568368150225
27227,136023,0,136023,338.5307819843292,0.001260329568193407
27327,136523,0,136523,339.6239960193634,0.0012601066925568751
27427,137023,0,137023,340.73203921318054,0.0012598980112602284
27528,137528,0,137528,341.8365080356598,0.001259700127463341
27628,138028,0,138028,342.94312810897827,0.001259515649879399
27728,138528,0,138528,344.0347559452057,0.001259341426297973
27828,139028,0,139028,345.24867701530457,0.0012591764658930254
27928,139528,0,139528,346.4206681251526,0.0012590198979254626
28028,140028,0,140028,347.6017599105835,0.0012588709542865667
28128,140528,0,140528,348.8383231163025,0.0012587289548988655
28228,141028,0,141028,350.0099160671234,0.0012585932954738512
28328,141528,0,141528,351.1330101490021,0.001258463437216876
28428,142028,0,142028,352.23163414001465,0.0012583388981442822
28529,142533,0,142533,353.3437659740448,0.0012582180725397663
28629,143033,0,143033,354.4567680358887,0.0012581029606474792
28729,143533,0,143533,355.56677508354187,0.001257991991421701
28829,144033,0,144033,356.7377362251282,0.0012578848471878202
28929,144533,0,144533,357.996386051178,0.0012577812397275194
29029,145033,0,145033,359.1471028327942,0.0012576809069366106
29129,145533,0,145533,360.2776219844818,0.0012575836099384269
29229,146033,0,146033,361.38605523109436,0.0012574891305823807
29329,146533,0,146533,362.5019519329071,0.0012573972692680893
29429,147033,0,147033,363.60836601257324,0.0012573078430463108
29530,147538,0,147538,364.7943789958954,0.0012572198232800509
29630,148038,0,148038,365.8967430591583,0.0012571347972722107
29730,148538,0,148538,367.0342161655426,0.0012570517403927865
29830,149038,0,149038,368.1408030986786,0.0012569705216402926
29930,149538,0,149538,369.2565040588379,0.001256891020084921
30030,150038,0,150038,370.37522411346436,0.001256813123967454
30130,150538,0,150538,371.52588415145874,0.0012567367298946196
30230,151038,0,151038,372.72015404701233,0.0012566617421183837
30330,151538,0,151538,373.97816801071167,0.001256588071888809
30430,152038,0,152038,375.16714215278625,0.0012565156368715327
30531,152543,0,152543,376.2782099246979,0.0012564436534663736
30631,153043,0,153043,377.382817029953,0.0012563734754893212
30731,153543,0,153543,378.4848449230194,0.0012563043185648414
30831,154043,0,154043,379.588103055954,0.0012562361212808668
30931,154543,0,154543,380.6855900287628,0.001256168826457197
31031,155043,0,155043,381.781555891037,0.001256102380820952
31131,155543,0,155543,382.883327960968,0.001256036734710361
31231,156043,0,156043,383.9871621131897,0.0012559718418038853
31331,156543,0,156543,385.08619809150696,0.0012559076588721208
31431,157043,0,157043,386.19041991233826,0.0012558441455502534
31532,157548,0,157548,387.29684615135193,0.0012557806383849642
31632,158048,0,158048,388.39893198013306,0.0012557183594161508
31732,158548,0,158548,389.48647594451904,0.0012556566438264164
31832,159048,0,159048,390.59896898269653,0.0012555954608026334
31932,159547,0,159547,391.6956989765167,0.0012464530625578571
32032,160047,0,160047,392.7939021587372,0.0012364923687016626
32132,160547,0,160547,393.96175718307495,0.0012279957206674822
32232,161047,0,161047,395.2146830558777,0.0012207364269669618
32332,161547,0,161547,396.3714668750763,0.0012145258183443894
32432,162047,0,162047,397.61739802360535,0.0012092041617442217
32533,162552,0,162552,398.82832193374634,0.001204593992948788
32633,163052,0,163052,399.93348717689514,0.0012006714165854397
32733,163552,0,163552,401.25598096847534,0.00119729076863617
32833,164052,0,164052,402.4299781322479,0.0011943705502557632
32933,164552,0,164552,403.60028314590454,0.0011918419077725556
33033,165052,0,165052,404.7598559856415,0.001189646660731773
33133,165552,0,165552,405.9167149066925,0.0011877356290642173
33233,166052,0,166052,407.0704171657562,0.0011860672179252261
33333,166552,0,166552,408.2175660133362,0.001184606223108426
33433,167052,0,167052,409.50787806510925,0.0011833228243183223
33534,167557,0,167557,410.70369601249695,0.0011821811206033511
33634,168057,0,168057,411.9112219810486,0.0011811820979201195
33734,168557,0,168557,413.0944170951843,0.001180295524597782
33834,169057,0,169057,414.3856518268585,0.0011795059117805568
33934,169557,0,169557,415.48475098609924,0.0011788000649648007
34034,170057,0,170057,416.5913870334625,0.0011781667289730412
34134,170557,0,170557,417.6896290779114,0.0011775962894242206
34234,171057,0,171057,418.7869381904602,0.0011770805215820601
34334,171557,0,171557,419.90468287467957,0.0011766123789291325
34434,172057,0,172057,421.197252035141,0.0011761858150522101
34535,172562,0,172562,422.3963270187378,0.0011757918996976738
34635,173062,0,173062,423.5483319759369,0.0011754339257815135
34735,173562,0,173562,424.6639370918274,0.001175103967945771
34835,174062,0,174062,425.93229699134827,0.0011747986995168226
34935,174562,0,174562,427.1183490753174,0.0011745152421165279
35035,175062,0,175062,428.16879200935364,0.0011742511008375081
35135,175562,0,175562,429.36598110198975,0.0011740041092469572
35235,176062,0,176062,430.51185512542725,0.0011737723826739416
35335,176562,0,176562,431.63199615478516,0.001173554278485417
35435,177062,0,177062,432.7447819709778,0.0011733483622642549
35536,177567,0,177567,433.8657920360565,0.0011731514805143294
35636,178067,0,178067,434.96127104759216,0.0011729664231411787
35736,178567,0,178567,436.16198801994324,0.0011727902228744255
35836,179067,0,179067,437.30660700798035,0.0011726220300208744
35936,179567,0,179567,438.43443393707275,0.0011724610950725298
36036,180067,0,180067,439.53066420555115,0.0011723067554987347
36136,180567,0,180567,440.6698069572449,0.0011721584244003245
36236,181067,0,181067,441.77562403678894,0.001172015580750487
36336,181567,0,181567,442.88837909698486,0.0011718777609893193
36436,182067,0,182067,444.00212025642395,0.0011717445517747563
36537,182572,0,182572,445.13153886795044,0.0011716143143106316
36637,183072,0,183072,446.2217240333557,0.0011714892941312102
36737,183572,0,183572,447.32184314727783,0.0011713678844774132
36837,184072,0,184072,448.454421043396,0.0011712498184368728
36937,184572,0,184572,449.5621428489685,0.0011711348553267835
37037,185072,0,185072,450.6744728088379,0.00117102277762916
37137,185572,0,185572,451.94183802604675,0.001170913388322258
37237,186072,0,186072,453.1692600250244,0.0011708065085534616
37337,186572,0,186572,454.2804260253906,0.0011707019756068918
37437,187072,0,187072,455.479376077652,0.001170599641126218
37538,187577,0,187577,456.69460797309875,0.001170498376831037
37638,188077,0,188077,457.80696392059326,0.0011704000628555754
37738,188577,0,188577,458.9056921005249,0.001170303572706706
37838,189077,0,189077,460.0026590824127,0.001170208801774726
37938,189577,0,189577,461.1578071117401,0.0011701156536928674
38038,190077,0,190077,462.49005103111267,0.0011700240395172432
38138,190577,0,190577,463.82910990715027,0.001169933877001791
38238,191077,0,191077,465.3217740058899,0.0011698450899560117
38338,191577,0,191577,466.4388451576233,0.0011697576076754176
38438,192077,0,192077,467.6019570827484,0.0011696713644353503
38539,192582,0,192582,469.1100389957428,0.0011695854541382798
38639,193082,0,193082,470.42359495162964,0.0011695015204534608
38739,193582,0,193582,472.0490322113037,0.001169418653732017
38839,194082,0,194082,473.3986930847168,0.0011693368041558246
38939,194582,0,194582,474.62152004241943,0.0011692559250638945
39039,195082,0,195082,475.80223298072815,0.0011691759726944646
39139,195582,0,195582,477.02212023735046,0.0011690969059527294
39239,196082,0,196082,478.3972358703613,0.001169018686201509
39339,196582,0,196582,479.5561351776123,0.0011689412770723535
39439,197082,0,197082,480.9054801464081,0.0011688646442946401
39540,197587,0,197587,482.2337498664856,0.0011687880003058068
39640,198087,0,198087,483.43563413619995,0.0011687128320370323
39740,198587,0,198587,484.8579728603363,0.0011686383481356376
39840,199087,0,199087,486.0132761001587,0.0011685645213240364
39940,199587,0,199587,487.6300220489502,0.0011684913257754208
40040,200087,0,200087,488.95951104164124,0.0011684187370166563
40140,200587,0,200587,490.2770240306854,0.0011683467318394283
40240,201087,0,201087,491.7254910469055,0.0011682752882186305
40340,201587,0,201587,492.84861516952515,0.0011682043852374738
40440,202087,0,202087,494.18026900291443,0.001168134003018333
40541,202592,0,202592,495.5617241859436,0.001168063426328588
40641,203092,0,203092,496.6706430912018,0.0011679940345957784
40741,203592,0,203592,497.7821092605591,0.0011679251094489072
40841,204092,0,204092,498.8820400238037,0.0011678566345860162
40941,204592,0,204592,500.081326007843,0.0011677885944702904
41041,205092,0,205092,501.31694889068604,0.0011677209742869824
41141,205592,0,205592,502.4361729621887,0.0011676537599030407
41241,206092,0,206092,503.5850410461426,0.0011675869378295913
41341,206592,0,206592,504.6983449459076,0.0011675204951870123
41441,207092,0,207092,505.8300368785858,0.0011674544196722853
41542,207597,0,207597,507.17655897140503,0.0011673880440832356
41642,208097,0,208097,508.426322221756,0.0011673226714572036
41742,208597,0,208597,509.66099095344543,0.001167257632109
41842,209097,0,209097,511.1403748989105,0.0011671929157601835
41942,209597,0,209597,512.369117975235,0.0011671285125742393
42042,210097,0,210097,513.5285110473633,0.0011670644131344678
42142,210597,0,210597,514.886293888092,0.0011670006084231151
42242,211097,0,211097,516.1898999214172,0.00116693708980181
42342,211597,0,211597,517.8492851257324,0.0011668738489931654
42442,212097,0,212097,519.2863590717316,0.0011668108780632752
42543,212602,0,212602,520.4765071868896,0.0011667475436183627
42643,213102,0,213102,521.7834041118622,0.0011666850924512927
42743,213602,0,213602,523.0830330848694,0.0011666228891943073
42843,214102,0,214102,524.5062720775604,0.001166560927135047
42943,214602,0,214602,525.9150400161743,0.0011664991998310234
43043,215102,0,215102,527.0491859912872,0.0011664377010970745
43143,215602,0,215602,528.3537662029266,0.0011663764249937763
43243,216102,0,216102,529.8757100105286,0.0011663153658161604
43343,216602,0,216602,531.2435839176178,0.0011662545180831927
43443,217102,0,217102,532.4977991580963,0.001166193876527728
43544,217607,0,217607,533.8453891277313,0.0011661328326815457
43644,218107,0,218107,534.8974871635437,0.001166072590426508
43744,218607,0,218607,535.9173521995544,0.0011660125396919393
43844,219107,0,219107,537.0365629196167,0.0011659526759772415
43944,219607,0,219607,538.3577561378479,0.0011658929949525047
44044,220107,0,220107,539.7520911693573,0.0011658334924510207
44144,220607,0,220607,541.2168428897858,0.0011657741644622817
44244,221107,0,221107,542.5073919296265,0.001165715007125243
44344,221607,0,221607,543.695953130722,0.0011656560167219727
44444,222107,0,222107,545.0843288898468,0.0011655971896715315
44545,222612,0,222612,546.481987953186,0.0011655379366488428
44645,223112,0,223112,547.701208114624,0.0011654794276298422
44745,223612,0,223612,549.0969462394714,0.0011654210719545745
44845,224112,0,224112,550.4801268577576,0.001165362866535833
44945,224612,0,224612,551.9189438819885,0.0011653048083968096
45045,225112,0,225112,553.1148941516876,0.0011652468946665839
45145,225612,0,225612,554.3427498340607,0.001165189122575819
45245,226112,0,226112,555.7498700618744,0.001165131489452384
45345,226612,0,226612,556.9607129096985,0.0011650739927176388
45445,227112,0,227112,558.3731780052185,0.0011650166298823768
45546,227617,0,227617,559.6745629310608,0.0011649588268859367
45646,228117,0,228117,561.0565748214722,0.0011649017260022525
45746,228617,0,228617,562.293879032135,0.001164844752029862
45846,229117,0,229117,563.6021611690521,0.0011647879028034236
45946,229617,0,229617,564.8245379924774,0.0011647311762305128
46046,230117,0,230117,566.1079480648041,0.0011646745702884299
46146,230617,0,230617,567.4345571994781,0.0011646180830216606
46246,231117,0,231117,568.6075391769409,0.0011645617125391023
46346,231617,0,231617,570.0551290512085,0.001164505457011427
46446,232117,0,232117,571.5342650413513,0.0011644493146688146
46547,232622,0,232622,573.1243650913239,0.0011643927240470393
46647,233122,0,233122,574.9363398551941,0.0011643368040809617
46747,233622,0,233622,576.5000722408295,0.0011642809923081553
46847,234122,0,234122,577.7596299648285,0.0011642252871744783
46947,234622,0,234622,579.1096520423889,0.0011641696871744617
47047,235122,0,235122,580.4869010448456,0.001164114190849333
47147,235622,0,235622,581.707267999649,0.0011640587967853687
47247,236122,0,236122,583.2367050647736,0.0011640035036119857
47347,236622,0,236622,584.5325360298157,0.0011639483100002058
47447,237122,0,237122,585.8523499965668,0.0011638932146609718
47548,237627,0,237627,587.5313560962677,0.0011638376668464227
47648,238127,0,238127,589.1273920536041,0.0011637827652896868
47748,238627,0,238627,590.9089782238007,0.0011637279583517344
47848,239127,0,239127,592.3150510787964,0.0011636732448891862
47948,239627,0,239627,593.730663061142,0.0011636186237914715
48048,240127,0,240127,595.2894699573517,0.0011635640939798545
48148,240627,0,240627,596.7445681095123,0.0011635096544060025
48248,241127,0,241127,597.9692499637604,0.0011634553040510772
48348,241627,0,241627,599.2758052349091,0.0011634010419244196
48448,242127,0,242127,600.774934053421,0.0011633468670626756
48549,242632,0,242632,602.2666170597076,0.001163292238076192
48649,243132,0,243132,603.4865279197693,0.001163238235807756
48749,243632,0,243632,604.9298942089081,0.0011631843180589213
48849,244132,0,244132,606.3763098716736,0.0011631304839658364
48949,244632,0,244632,607.9852139949799,0.001163076732687278
49049,245132,0,245132,609.4518389701843,0.0011630230634037248
49149,245632,0,245632,610.9615862369537,0.001162969475316747
49249,246132,0,246132,612.1285791397095,0.0011629159676480045
49349,246632,0,246632,613.29669713974,0.0011628625396387867
49449,247132,0,247132,614.4800050258636,0.0011628091905491556
49550,247637,0,247637,615.8414509296417,0.0011627553873408388
49650,248137,0,248137,616.9054980278015,0.001162702194713821
49750,248637,0,248637,617.9491939544678,0.0011626490788860366
49850,249137,0,249137,619.1326420307159,0.0011625960391864589
49950,249637,0,249637,620.2742509841919,0.0011625430749598506
50050,250137,0,250137,621.4626648426056,0.0011624901855660581
50150,250637,0,250637,622.6167411804199,0.0011624373703795947
50250,251137,0,251137,623.82248711586,0.0011623846287891326
50350,251637,0,251637,625.00364112854,0.0011623319601969618
50450,252137,0,252137,626.3378400802612,0.001162279364018462
50551,252642,0,252642,627.6597239971161,0.0011622263147994475
50651,253142,0,253142,628.855740070343,0.001162173862455327
50751,253642,0,253642,630.0507500171661,0.001162121480840517
50851,254142,0,254142,631.2655851840973,0.001162069169418962
50951,254642,0,254642,632.7342059612274,0.0011620169276656865
51051,255142,0,255142,634.1528401374817,0.0011619647550664839
51151,255642,0,255642,635.4534261226654,0.001161912651117372
51251,256142,0,256142,636.9761221408844,0.0011618606153245474
51351,256642,0,256642,638.2013831138611,0.0011618086472037963
51451,257142,0,257142,639.542845249176,0.0011617567462803248
51552,257647,0,257647,640.8315620422363,0.001161704394081913
51652,258147,0,258147,642.0221679210663,0.001161652626825034
51752,258647,0,258647,643.3485460281372,0.0011616009253898158
51852,259147,0,259147,644.7727379798889,0.001161549289336086
51952,259647,0,259647,645.9163391590118,0.001161497718231684
52052,260147,0,260147,647.143196105957,0.001161446211652078
52152,260647,0,260647,648.3185641765594,0.0011613947691802313
52252,261147,0,261147,649.4882090091705,0.001161343390406321
52352,261647,0,261647,650.6765470504761,0.001161292074927608
52452,262147,0,262147,651.9382410049438,0.0011612408223480304
52553,262652,0,262652,653.3714978694916,0.0011611891206918545
52653,263152,0,263152,654.5300850868225,0.001161137993368067
52753,263652,0,263652,655.8925080299377,0.0011610869277903328
52853,264152,0,264152,657.1314148902893,0.0011610359235879224
52953,264652,0,264652,658.36523604393,0.0011609849803957972
53053,265152,0,265152,659.6284132003784,0.0011609340978546898
53153,265652,0,265652,660.9873280525208,0.0011608832756107002
53253,266152,0,266152,662.1964020729065,0.0011608325133153274
53353,266652,0,266652,663.363254070282,0.0011607818106252087
53453,267152,0,267152,664.6139280796051,0.0011607311672019633
53554,267657,0,267657,665.8527390956879,0.0011606800771637538
53654,268157,0,268157,667.0894808769226,0.0011606295518630794
53754,268657,0,268657,668.6622641086578,0.0011605790848396957
53854,269157,0,269157,669.7262508869171,0.0011605286757739954
53954,269657,0,269657,670.8940751552582,0.0011604783243507378
54054,270157,0,270157,672.1740441322327,0.0011604280302588595
54154,270657,0,270657,673.3631780147552,0.0011603777931914108
54254,271157,0,271157,674.7428379058838,0.0011603276128454554
54354,271657,0,271657,675.9990210533142,0.0011602774889219291
54454,272157,0,272157,677.0983700752258,0.00116022742112559
54555,272662,0,272662,678.2162930965424,0.001160176909326209
54655,273161,0,273161,679.378583908081,0.0011124430619838003
54755,273661,0,273661,680.5047149658203,0.001111420554645428
54855,274161,0,274161,681.6806139945984,0.0011106558237035785
54955,274661,0,274661,682.8106820583344,0.0011099260088512299
55055,275161,0,275161,683.9800939559937,0.0011092203675606813
55155,275661,0,275661,685.1784749031067,0.0011085362346735413
55255,276161,0,276161,686.395092010498,0.0011078722935100324
55355,276661,0,276661,687.5458040237427,0.0011072276147345583
55455,277161,0,277161,688.7286529541016,0.0011066014251988761
55556,277666,0,277666,689.943284034729,0.0011059870364096614
55656,278166,0,278166,691.0634212493896,0.0011053959680213785
55756,278666,0,278666,692.198930978775,0.0011048214452034676
55856,279166,0,279166,693.3259189128876,0.001104262893798323
55956,279666,0,279666,694.6064400672913,0.0011037197652057505
56056,280166,0,280166,695.7239999771118,0.0011031915336896685
56156,280666,0,280666,696.9815149307251,0.001102677694495342
56256,281166,0,281166,698.4169130325317,0.0011021777624309684
56356,281666,0,281666,699.7756369113922,0.0011016912707308571
56456,282166,0,282166,701.0069401264191,0.0011012177700990826
56557,282671,0,282671,702.3950130939484,0.0011007522804499456
56657,283171,0,283171,703.8846929073334,0.0011003035992256409
56757,283671,0,283671,705.4887170791626,0.0010998666541294918
56857,284171,0,284171,707.1264810562134,0.0010994410583110425
56957,284671,0,284671,708.5008821487427,0.0010990264388967403
57057,285171,0,285171,709.8408100605011,0.001098622436433862
57157,285671,0,285671,711.0992512702942,0.0010982287043639976
57257,286171,0,286171,712.4395759105682,0.0010978449085231922
57357,286671,0,286671,713.7068030834198,0.0010974707266652175
57457,287171,0,287171,714.9929032325745,0.0010971058480069118
57558,287676,0,287676,716.2283928394318,0.0010967464585212039
57658,288176,0,288176,717.5901610851288,0.001096399383325513
57758,288676,0,288676,718.8046219348907,0.0010960607407596839
57858,289176,0,289176,720.0929610729218,0.001095730261817897
57958,289676,0,289676,721.263836145401,0.0010954076869527584
58058,290176,0,290176,722.5014090538025,0.0010950927657226717
58158,290676,0,290676,723.8284530639648,0.0010947852564530398
58258,291176,0,291176,725.1628441810608,0.001094484925911081
58358,291676,0,291676,726.4260430335999,0.001094191548992963
58458,292176,0,292176,727.7283198833466,0.0010939049084233616
58559,292681,0,292681,728.9754469394684,0.0010936220255952428
58659,293181,0,293181,730.2781019210815,0.0010933482980195434
58759,293681,0,293681,731.5844888687134,0.0010930806971822973
58859,294181,0,294181,733.1550829410553,0.0010928190344074344
58959,294681,0,294681,734.5173070430756,0.001092563127507021
59059,295181,0,295181,735.9786942005157,0.0010923128005434028
59159,295681,0,295681,737.1589648723602,0.0010920678836008337
59259,296181,0,296181,738.3723628520966,0.001091828212565474
59359,296681,0,296681,739.6891760826111,0.0010915936289139037
59459,297181,0,297181,741.0707249641418,0.0010913639795095773
59560,297686,0,297686,742.3812530040741,0.001091136891459056
59660,298186,0,298186,743.5159091949463,0.0010909167174435513
59760,298686,0,298686,744.6194200515747,0.0010907010473079433
59860,299186,0,299186,745.773766040802,0.0010904897476231674
59960,299686,0,299686,746.8848180770874,0.0010902826894374673
60060,300186,0,300186,747.9872438907623,0.0010900797481148744
60160,300686,0,300686,749.0782001018524,0.0010898808031797969
60260,301186,0,301186,750.222305059433,0.0010896857381674277
60360,301686,0,301686,751.347009897232,0.001089494440479704
60460,302186,0,302186,752.4497120380402,0.0010893068012467612
60561,302691,0,302691,753.5590581893921,0.0010891208919292035
60661,303191,0,303191,754.6740698814392,0.0010889402912578996
60761,303691,0,303691,755.7678399085999,0.001088763042523427
60861,304191,0,304191,756.8666999340057,0.0010885890505153142
60961,304691,0,304691,757.9734709262848,0.001088418223131134
61061,305191,0,305191,759.1388530731201,0.001088250471266347
61161,305691,0,305691,760.3171420097351,0.0010880857087081296
61261,306191,0,306191,761.4961981773376,0.0010879238520331805
61361,306691,0,306691,762.7288310527802,0.0010877648205093189
61461,307191,0,307191,763.9235241413116,0.0010876085360007586
61562,307696,0,307696,765.5158960819244,0.0010874533999864478
61662,308196,0,308196,766.6863548755646,0.0010873024106538276
61762,308696,0,308696,767.869145154953,0.0010871539479145648
61862,309196,0,309196,768.9537761211395,0.0010870079431612935
61962,309696,0,309696,770.1763031482697,0.0010868643299586204
62062,310196,0,310196,771.375864982605,0.0010867230439675197
62162,310696,0,310696,772.6298179626465,0.0010865840228725821
62262,311196,0,311196,773.8038010597229,0.0010864472063119215
62362,311696,0,311696,775.0005149841309,0.001086312535809675
62462,312196,0,312196,776.27002120018,0.0010861799547108187
62563,312701,0,312701,777.318118095398,0.0010860481127456152
62663,313201,0,313201,778.4633920192719,0.0010859195670113364
62763,313701,0,313701,780.0143179893494,0.001085792950518287
62863,314201,0,314201,781.2461738586426,0.0010856682133064861
62963,314701,0,314701,782.599335193634,0.0010855453069451518
63063,315201,0,315201,783.9562270641327,0.0010854241844805335
63163,315701,0,315701,785.0928821563721,0.0010853048003857883
63263,316201,0,316201,786.3158462047577,0.0010851871105127175
63363,316701,0,316701,787.594850063324,0.00108507107204515
63463,317201,0,317201,788.7828369140625,0.001084956643454075
63564,317706,0,317706,789.974053144455,0.0010848426636575243
63664,318206,0,318206,791.3065011501312,0.0010847313502778083
63764,318706,0,318706,792.6789319515228,0.0010846215291119676
63864,319206,0,319206,793.9429621696472,0.0010845131633732536
63964,319706,0,319706,795.3696339130402,0.0010844062173603081
64064,320206,0,320206,796.8654720783234,0.0010843006564212828
64164,320706,0,320706,798.4370110034943,0.001084196446918974
64264,321206,0,321206,799.8587260246277,0.001084093556197409
64364,321706,0,321706,801.0384528636932,0.0010839919525494931
64464,322206,0,322206,802.1421627998352,0.0010838916051859198
64565,322711,0,322711,803.2787570953369,0.0010837914990895032
64665,323211,0,323211,804.5780870914459,0.001083693587277994
64765,323711,0,323711,805.7975289821625,0.0010835968443161416
64865,324211,0,324211,807.2249920368195,0.0010835012428035003
64965,324711,0,324711,808.5293831825256,0.0010834067561171432
65065,325211,0,325211,809.6474649906158,0.0010833133583866112
65165,325711,0,325711,810.7474229335785,0.0010832210244696185
65265,326211,0,326211,811.8418979644775,0.001083129729928735
65365,326711,0,326711,812.9461140632629,0.0010830394510088495
65465,327211,0,327211,814.0306348800659,0.0010829501646153904
65566,327716,0,327716,815.2729640007019,0.0010828609699545725
65666,328216,0,328216,816.5046410560608,0.0010827736112422855
65766,328716,0,328716,817.7767150402069,0.0010826871793201767
65866,329216,0,329216,819.0686681270599,0.0010826016535386946
65966,329716,0,329716,820.5352170467377,0.0010825170138107087
66066,330216,0,330216,822.0522830486298,0.0010824332405938947
66166,330716,0,330716,823.3899819850922,0.0010823503148736462
66266,331216,0,331216,824.5937190055847,0.0010822682181468601
66366,331716,0,331716,825.8589119911194,0.0010821869324057888
66466,332216,0,332216,827.0712850093842,0.0010821064401230767
66567,332721,0,332721,828.3284640312195,0.0010820259309420686
66667,333221,0,333221,829.4628810882568,0.0010819469823566336
66767,333721,0,333721,830.8752839565277,0.0010818687772235827
66867,334221,0,334221,832.1106350421906,0.001081791299797576
66967,334721,0,334721,833.2254371643066,0.0010817145347443464
67067,335221,0,335221,834.6979749202728,0.0010816384671280862
67167,335721,0,335721,835.999941110611,0.0010815630823995512
67267,336221,0,336221,837.2846279144287,0.001081488366384507
67367,336721,0,336721,838.7410538196564,0.001081414305272191
67467,337221,0,337221,839.9496080875397,0.0010813408856048758
67568,337726,0,337726,841.1749789714813,0.0010812673694832024
67668,338226,0,338226,842.8015122413635,0.0010811951997835305
67768,338726,0,338726,844.1938889026642,0.001081123633046015
67868,339226,0,339226,845.5955600738525,0.0010810526571256808
67968,339726,0,339726,847.2136659622192,0.0010809822601811
68068,340226,0,340226,848.5073299407959,0.0010809124306656287
68168,340726,0,340726,849.868588924408,0.0010808431573187283
68268,341226,0,341226,851.1542918682098,0.0010807744291577751
68368,341726,0,341726,852.6634769439697,0.0010807062354699004
68468,342226,0,342226,853.878543138504,0.0010806385658043254
68569,342731,0,342731,855.0401570796967,0.001080570740967388
68669,343231,0,343231,856.4148321151733,0.0010805040939942869
68769,343731,0,343731,857.7037711143494,0.0010804379410936248
68869,344231,0,344231,858.9196960926056,0.0010803722727923228
68969,344731,0,344731,860.2008838653564,0.0010803070798440768
69069,345231,0,345231,861.3555178642273,0.0010802423532229625
69169,345731,0,345731,862.6368548870087,0.0010801780841171742
69269,346230,0,346230,863.8128571510315,0.0010627107461176914
69369,346730,0,346730,865.2313649654388,0.0010611792955333272
69469,347230,0,347230,866.426323890686,0.0010597084212616023
69570,347735,0,347735,867.5721299648285,0.0010582691890635954
69670,348235,0,348235,868.678624868393,0.0010568872370447552
69770,348735,0,348735,869.7909739017487,0.0010555462897183776
69870,349235,0,349235,870.941890001297,0.0010542448072450412
69970,349735,0,349735,872.2951741218567,0.0010529813711810804
70070,350235,0,350235,873.4948351383209,0.001051754641783036
70170,350735,0,350735,874.6322510242462,0.0010505633413833346
70270,351235,0,351235,875.8295950889587,0.001049406246399014
70370,351735,0,351735,877.0185990333557,0.0010482821826549834
70470,352231,0,352231,878.1255860328674,0.0010131479128127807
70571,352736,0,352736,879.2975850105286,0.001012661652461844
70671,353236,0,353236,880.5043818950653,0.0010122015481232353
70771,353736,0,353736,881.7016229629517,0.0010117613286002383
70871,354236,0,354236,883.0782370567322,0.0010113398072038192
70971,354736,0,354736,884.3170599937439,0.001010935915369123
71071,355236,0,355236,885.7851660251617,0.001010548677340959
71171,355736,0,355736,886.9821691513062,0.0010101771934913864
71271,356236,0,356236,888.186222076416,0.0010098206287417165
71371,356736,0,356736,889.6418302059174,0.001009478204150353
71471,357236,0,357236,890.9554190635681,0.0010091491905485804
71572,357741,0,357741,892.5585720539093,0.00100882980273829
71672,358241,0,358241,893.7858741283417,0.001008525716403308
71772,358741,0,358741,894.9171929359436,0.001008233100875547
71872,359241,0,359241,896.271646976471,0.0010079513847400673
71972,359741,0,359741,897.7609939575195,0.0010076800285911116
72072,360241,0,360241,899.13046002388,0.001007418522840397
72172,360741,0,360741,900.3764719963074,0.0010071663857564677
72272,361241,0,361241,901.5416660308838,0.001006923161692335
72372,361741,0,361741,902.7317202091217,0.0010066884194693934
72472,362241,0,362241,903.8736801147461,0.0010064617508943605
72573,362746,0,362746,905.0201561450958,0.001006240617139747
72673,363246,0,363246,906.1762249469757,0.0010060290279042745
72773,363746,0,363746,907.4072208404541,0.0010058244090765443
72873,364246,0,364246,908.5959658622742,0.0010056264318449248
72973,364746,0,364746,909.9544689655304,0.0010054347844323784
73073,365246,0,365246,911.4532120227814,0.0010052491711369422
73173,365746,0,365746,912.7636389732361,0.0010050693114324579
73273,366246,0,366246,914.0386390686035,0.0010048949391251519
73373,366746,0,366746,915.3876130580902,0.0010047258015617613
73473,367246,0,367246,916.522901058197,0.001004561658885512
73574,367751,0,367751,918.3723051548004,0.0010044007129138487
73674,368251,0,368251,920.3712339401245,0.0010042459326238434
73774,368751,0,368751,922.1428751945496,0.0010040954956360413
73874,369251,0,369251,923.975643157959,0.0010039492067845173
73974,369751,0,369751,925.7767460346222,0.0010038068805847096
74074,370251,0,370251,927.6883220672607,0.0010036683407161312
74174,370751,0,370751,929.3277292251587,0.0010035334195345282
74274,371251,0,371251,930.9470808506012,0.0010034019576121102
74374,371751,0,371751,932.7575540542603,0.001003273803303748
74474,372251,0,372251,934.2589612007141,0.0010031488123378033
74575,372756,0,372756,936.1769549846649,0.0010030256426150157
74675,373256,0,373256,937.6854319572449,0.0010029066014194594
74775,373756,0,373756,939.1427550315857,0.001002790330024593
74875,374256,0,374256,940.4350068569183,0.0010026767100593788
74975,374756,0,374756,941.8152539730072,0.0010025656287966152
75075,375256,0,375256,943.2046551704407,0.0010024569788631037
75175,375756,0,375756,944.6051139831543,0.0010023506579657283
75275,376256,0,376256,946.233964920044,0.0010022465686325111
75375,376756,0,376756,947.7768850326538,0.0010021446179680055
75475,377256,0,377256,949.5988550186157,0.0010020447174217998
75576,377761,0,377761,951.5289168357849,0.0010019458128721185
75676,378261,0,378261,953.0126020908356,0.001001849781666429
75776,378761,0,378761,954.6362869739532,0.0010017555581173748
75876,379261,0,379261,955.9703028202057,0.001001663069014874
75976,379761,0,379761,957.3673050403595,0.0010015722445091495
76076,380261,0,380261,958.8503510951996,0.0010014830179447456
76176,380761,0,380761,960.2130448818207,0.0010013953257031669
76276,381261,0,381261,961.5185990333557,0.0010013091070537967
76376,381761,0,381761,962.8100941181183,0.0010012243040128498
76476,382261,0,382261,964.0743000507355,0.0010011408612094893
76577,382766,0,382766,965.3661630153656,0.0010010579108338349
76677,383266,0,383266,966.632285118103,0.00100097704453864
76777,383766,0,383766,967.9122211933136,0.001000897386339385
76877,384266,0,384266,969.1722228527069,0.00100081889013423
76977,384766,0,384766,970.4475922584534,0.0010007415118617024
77077,385266,0,385266,971.7449510097504,0.001000665209403484
77177,385766,0,385766,973.3208739757538,0.0010005899424920359
77277,386266,0,386266,974.9285480976105,0.0010005156726232258
77377,386766,0,386766,976.3028740882874,0.0010004423629729315
77477,387266,0,387266,977.7434411048889,0.0010003699783182796
77578,387771,0,387771,979.2737641334534,0.0010002977744198063
77678,388271,0,388271,980.6194379329681,0.001000227148553861
77778,388771,0,388771,982.4782059192657,0.0010001573505889897
77878,389271,0,389271,983.936402797699,0.0010000883510067086
77978,389771,0,389771,985.7973418235779,0.00100002012154977
78078,390271,0,390271,987.4387891292572,0.0009999526351641653
78178,390771,0,390771,989.5420920848846,0.0009998858659438607
78278,391271,0,391271,991.7075419425964,0.0009998197890782887
78378,391771,0,391771,993.5766279697418,0.0009997543808024057
78478,392271,0,392271,995.0680739879608,0.0009996896183491117
78579,392776,0,392776,996.6663122177124,0.0009996248415994845
78679,393276,0,393276,998.3626420497894,0.0009995613121867822
78779,393776,0,393776,1000.1034018993378,0.0009994983656459924
78879,394276,0,394276,1002.069384098053,0.0009994359827792925
78979,394776,0,394776,1003.6162359714508,0.000999374145181073
79079,395276,0,395276,1005.2721991539001,0.0009993128352026985
79179,395776,0,395776,1007.192461013794,0.0009992520359187996
79279,396276,0,396276,1008.8200640678406,0.0009991917310951985
79379,396776,0,396776,1010.4745950698853,0.000999131905158334
79479,397276,0,397276,1012.4346139431,0.000999072543166189
79580,397781,0,397781,1013.9567821025848,0.0009990130438800252
79680,398281,0,398281,1015.4120831489563,0.000998954571630389
79780,398781,0,398781,1016.8065431118011,0.0009988965218876624
79880,399281,0,399281,1018.2217981815338,0.0009988388819759566
79980,399781,0,399781,1019.6307120323181,0.0009987816397241205
80080,400281,0,400281,1021.0587708950043,0.0009987247834439663
80180,400781,0,400781,1022.4780530929565,0.0009986683019092754
80280,401281,0,401281,1023.8864040374756,0.0009986121843359953
80380,401781,0,401781,1025.4508130550385,0.000998556420363063
80480,402281,0,402281,1027.4131281375885,0.0009985010000344143
80581,402786,0,402786,1029.198026895523,0.000998445364574735
80681,403286,0,403286,1031.0756459236145,0.0009983906064038892
80781,403786,0,403786,1033.6144859790802,0.0009983361641826766
80881,404286,0,404286,1035.4325439929962,0.0009982820294124968
80981,404786,0,404786,1037.1614508628845,0.0009982281939204438
81081,405286,0,405286,1038.769049167633,0.000998174649845404
81181,405786,0,405786,1040.3544821739197,0.0009981213896251234
81281,406286,0,406286,1041.9363749027252,0.0009980684059834892
81381,406786,0,406786,1043.7816832065582,0.000998015691918577
81481,407286,0,407286,1045.4394800662994,0.0009979632406912253
81582,407791,0,407791,1047.0990130901337,0.0009979105251384831
81682,408291,0,408291,1048.7543559074402,0.0009978585828355796
81782,408791,0,408791,1050.567514181137,0.000997806884562805
81882,409291,0,409291,1052.163892030716,0.0009977554245291882
81982,409791,0,409791,1053.7594389915466,0.0009977041971561457
82082,410291,0,410291,1055.3463559150696,0.000997653197068746
82182,410791,0,410791,1056.9474210739136,0.0009976024190874867
82282,411291,0,411291,1058.5352098941803,0.000997551858219994
82382,411791,0,411791,1060.1158549785614,0.0009975015096536078
82482,412291,0,412291,1061.703506231308,0.0009974513687479164
82583,412796,0,412796,1063.3077201843262,0.0009974009326619482
82683,413296,0,413296,1064.906681060791,0.0009973511957781934
82783,413796,0,413796,1066.5089378356934,0.000997301653558031
82883,414296,0,414296,1068.0960409641266,0.0009972523019843645
82983,414796,0,414796,1069.6789209842682,0.0009972031371801025
83083,415296,0,415296,1071.2564420700073,0.0009971541554025208
83183,415796,0,415796,1072.8470141887665,0.0009971053530379143
83283,416296,0,416296,1074.4309208393097,0.0009970567265963207
83383,416796,0,416796,1076.008682012558,0.0009970082727066203
83483,417296,0,417296,1077.5977680683136,0.0009969599881118553
83584,417801,0,417801,1079.2038760185242,0.000996911389308784
83684,418301,0,418301,1080.802225112915,0.0009968634355828642
83784,418801,0,418801,1082.375051021576,0.0009968156419921724
83884,419301,0,419301,1083.9636731147766,0.0009967680056935557
83984,419801,0,419801,1085.566085100174,0.000996720523937052
84084,420301,0,420301,1087.1492249965668,0.0009966731940622016
84184,420801,0,420801,1088.7457950115204,0.0009966260134945905
84284,421301,0,421301,1090.3263640403748,0.000996578979742471
84384,421801,0,421801,1091.9163620471954,0.0009965320903934224
84484,422301,0,422301,1093.4880681037903,0.0009964853431114308
84585,422806,0,422806,1095.0956881046295,0.000996438270257591
84685,423306,0,423306,1096.6889200210571,0.0009963918017575242
84785,423806,0,423806,1098.2736990451813,0.0009963454687244308
84885,424306,0,424306,1099.8768801689148,0.0009962992690997685
84985,424806,0,424806,1101.4876132011414,0.0009962532008876647
85085,425306,0,425306,1103.1068170070648,0.000996207262152484
85185,425806,0,425806,1104.712984085083,0.00099616145101656
85285,426306,0,426306,1106.295737028122,0.000996115765657918
85385,426806,0,426806,1107.8875901699066,0.0009960702043082512
85485,427306,0,427306,1109.5461649894714,0.0009960247652508309
85586,427811,0,427811,1111.2565190792084,0.0009959789942378435
85686,428311,0,428311,1112.9975290298462,0.000995933795993393
85786,428811,0,428811,1114.6998660564423,0.0009958887151658453
85886,429311,0,429311,1116.4390230178833,0.000995843750226554
85986,429811,0,429811,1118.0907709598541,0.0009957988996893911
86086,430311,0,430311,1119.663358926773,0.0009957541621092698
86186,430811,0,430811,1121.2480170726776,0.0009957095360805357
86286,431311,0,431311,1122.833534002304,0.0009956650202355803
86386,431811,0,431811,1124.4476840496063,0.000995620613243358
86486,432311,0,432311,1126.0233631134033,0.0009955763138081643
86587,432816,0,432816,1127.6587150096893,0.0009955316792693825
86687,433316,0,433316,1129.3200340270996,0.0009954875922401562
86787,433816,0,433816,1130.9650650024414,0.000995443609067789
86887,434316,0,434316,1132.6098899841309,0.0009953997285854907
86987,434816,0,434816,1134.2075021266937,0.0009953559496557365
87087,435316,0,435316,1135.826672077179,0.0009953122711692688
87187,435816,0,435816,1137.4092309474945,0.0009952686920440183
87287,436316,0,436316,1139.0059251785278,0.0009952252112241974
87387,436816,0,436816,1140.606411933899,0.0009951818276793163
87487,437316,0,437316,1142.1952650547028,0.0009951385404033456
87588,437821,0,437821,1143.7724730968475,0.000995094916971815
87688,438321,0,438321,1145.3682868480682,0.000995051820247372
87788,438821,0,438821,1146.9478161334991,0.0009950088169025
87888,439321,0,439321,1148.5341639518738,0.0009949659060207326
87988,439821,0,439821,1150.108328819275,0.0009949230867060841
88088,440321,0,440321,1151.6977670192719,0.0009948803580822423
88188,440821,0,440821,1153.29576587677,0.000994837719292042
88288,441321,0,441321,1154.8734331130981,0.0009947951694966159
88388,441821,0,441821,1156.459079027176,0.0009947527078749286
88488,442321,0,442321,1158.056936264038,0.0009947103336231035
88589,442826,0,442826,1159.6635210514069,0.0009946676235117772
88689,443326,0,443326,1161.2265961170197,0.000994625422508149
88789,443826,0,443826,1162.8103229999542,0.000994583306552595
88889,444326,0,444326,1164.4012501239777,0.0009945412749045469
88989,444826,0,444826,1166.0013980865479,0.0009944993268379096
89089,445326,0,445326,1167.5668740272522,0.000994457461640552
89189,445826,0,445826,1169.144688129425,0.0009944156786139049
89289,446326,0,446326,1170.7467260360718,0.0009943739770726142
89389,446826,0,446826,1172.3354361057281,0.000994332356343912
89489,447326,0,447326,1173.8989639282227,0.0009942908157673576
89590,447831,0,447831,1175.538892030716,0.0009942489404830119
89690,448331,0,448331,1177.4305021762848,0.0009942075590621798
89790,448831,0,448831,1179.0191190242767,0.000994166255875874
89890,449331,0,449331,1180.589921951294,0.0009941250303091783
89990,449831,0,449831,1182.1696200370789,0.000994083881757629
90090,450331,0,450331,1183.7645418643951,0.000994042809626897
90190,450831,0,450831,1185.3461220264435,0.0009940018133325133
90290,451331,0,451331,1186.9639730453491,0.0009939608922995354
90390,451831,0,451831,1188.5574970245361,0.0009939200459623087
90490,452331,0,452331,1190.1407470703125,0.000993879273764106
90591,452836,0,452836,1191.730280160904,0.0009938381685406584
90691,453336,0,453336,1193.3202149868011,0.0009937975437127912
90791,453836,0,453836,1194.9115450382233,0.0009937569913997996
90891,454336,0,454336,1196.5064270496368,0.0009937165110784183
90991,454836,0,454836,1198.077075958252,0.000993676102233045
91091,455336,0,455336,1199.6597301959991,0.000993635764355674
91191,455836,0,455836,1201.2489340305328,0.0009935954969455517
91291,456336,0,456336,1202.8347170352936,0.0009935552995090496
91391,456836,0,456836,1204.4133307933807,0.000993515171559389
91491,457336,0,457336,1206.019623041153,0.0009934751126165601
91592,457841,0,457841,1207.6071631908417,0.0009934347226474678
91692,458341,0,458341,1209.1568920612335,0.0009933948009824003
91792,458841,0,458841,1210.7410390377045,0.000993354946917942
91892,459341,0,459341,1212.3323020935059,0.0009933151599991288
91992,459841,0,459841,1213.9237711429596,0.000993275439776908
92092,460341,0,460341,1215.5041861534119,0.0009932357858079288
92192,460841,0,460841,1217.0896360874176,0.0009931961976543408
92292,461341,0,461341,1218.6614079475403,0.0009931566748838056
92392,461841,0,461841,1220.2254619598389,0.0009931172170691345
92492,462341,0,462341,1221.8074889183044,0.0009930778237883576
92593,462846,0,462846,1223.407921075821,0.0009930381016552312
92693,463346,0,463346,1224.994973897934,0.0009929988368311536
92793,463846,0,463846,1226.5622498989105,0.0009929596353005392
92893,464346,0,464346,1228.14391207695,0.000992920496660714
92993,464846,0,464846,1229.7245230674744,0.0009928814205136622
93093,465346,0,465346,1231.3247270584106,0.0009928424064656858
93193,465846,0,465846,1232.8923690319061,0.0009928034541275075
93293,466346,0,466346,1234.4782240390778,0.0009927645631140148
93393,466845,0,466845,1236.0621621608734,0.0009566144773827764
93493,467345,0,467345,1237.6367909908295,0.0009552999840845761
93594,467850,0,467850,1239.2466940879822,0.0009540324558370261
93694,468350,0,468350,1240.836660861969,0.0009528220217901115
93794,468850,0,468850,1242.4292831420898,0.0009516529242226994
93894,469350,0,469350,1243.997458934784,0.0009505233527251142
93994,469850,0,469850,1245.5787391662598,0.0009494317804610445
94094,470350,0,470350,1247.1631710529327,0.000948376798156342
94194,470850,0,470850,1248.7456822395325,0.0009473570696901612
94294,471350,0,471350,1250.3074889183044,0.0009463713164634329
94394,471850,0,471850,1251.8975939750671,0.0009454183103379334
94494,472350,0,472350,1253.4902279376984,0.000944496869651086
94595,472855,0,472855,1255.0683801174164,0.0009435970963039847
94695,473355,0,473355,1256.650209903717,0.0009427357024540015
94795,473855,0,473855,1258.22598195076,0.000941902573360107
94895,474355,0,474355,1259.8383479118347,0.0009410966915345943
94995,474855,0,474855,1261.4190969467163,0.0009403170764220693
95095,475355,0,475355,1263.0051591396332,0.0009395627830543342
95195,475855,0,475855,1264.5943059921265,0.0009388329007734867
95295,476355,0,476355,1266.1753520965576,0.0009381265520108231
95395,476855,0,476855,1267.7434520721436,0.0009374428911137835
95495,477355,0,477355,1269.329400062561,0.0009367811032163659
95596,477860,0,477860,1270.9336659908295,0.0009361341000585821
95696,478360,0,478360,1272.688217163086,0.0009355139308819656
95796,478860,0,478860,1274.3659601211548,0.0009349133569568505
95896,479360,0,479360,1275.966245174408,0.0009343316762882444
95996,479860,0,479860,1277.5606231689453,0.0009337682125641215
96096,480360,0,480360,1279.14186501503,0.0009332223142367763
96196,480860,0,480860,1280.709811925888,0.0009326933536346096
96296,481360,0,481360,1282.2860178947449,0.0009321807261036787
96396,481860,0,481860,1283.8849141597748,0.0009316838491780523
96496,482360,0,482360,1285.4470751285553,0.0009312021617781276
96597,482865,0,482865,1287.0535850524902,0.0009307305252525971
96697,483365,0,483365,1288.6421279907227,0.0009302777540848755
96797,483865,0,483865,1290.2385551929474,0.0009298386049870601
96897,484365,0,484365,1291.802892923355,0.0009294125951201126
96997,484865,0,484865,1293.4338691234589,0.0009289992594080521
97097,485365,0,485365,1295.0364301204681,0.0009285981498877851
97197,485865,0,485865,1296.7013280391693,0.0009282088350819412
97297,486365,0,486365,1298.2774670124054,0.0009278308993933276
97397,486865,0,486865,1299.8802328109741,0.0009274639425209293
97497,487365,0,487365,1301.4888491630554,0.0009271075788963207
97598,487870,0,487870,1303.075101852417,0.0009267580261217038
97698,488370,0,488370,1304.6612470149994,0.0009264218454001378
97798,488870,0,488870,1306.2399332523346,0.0009260951808975818
97898,489370,0,489370,1307.8212690353394,0.0009257777008559627
97998,489870,0,489870,1309.4007630348206,0.0009254690857149768
98098,490370,0,490370,1310.9844698905945,0.0009251690276595051
98198,490870,0,490870,1312.5741090774536,0.0009248772301831271
98298,491370,0,491370,1314.1562111377716,0.0009245934076677388
98398,491870,0,491870,1315.7232098579407,0.0009243172849783144
98498,492370,0,492370,1317.3153629302979,0.0009240485970724168
98599,492875,0,492875,1318.9260499477386,0.0009237845089559853
98699,493375,0,493375,1320.514552116394,0.0009235300021168621
98799,493875,0,493875,1322.1019690036774,0.0009232821894713222
98899,494375,0,494375,1323.684697151184,0.0009230408428063386
98999,494875,0,494875,1325.2765119075775,0.0009228057422507594
99099,495375,0,495375,1326.8513040542603,0.0009225766759633897
99199,495875,0,495875,1328.4406859874725,0.0009223534398329786
99299,496375,0,496375,1330.0236120224,0.000922135837188981
99399,496875,0,496875,1331.612864971161,0.0009219236785233151
99499,497375,0,497375,1333.1818130016327,0.000921716781222369
99600,497880,0,497880,1334.7830669879913,0.0009215129762920005
99700,498380,0,498380,1336.369507074356,0.0009213161284996661
99800,498880,0,498880,1337.9339179992676,0.0009211240314615933
99900,499380,0,499380,1339.5383558273315,0.00092093652771461
100000,499880,0,499880,1341.131443977356,0.0009207534654906799


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha0/flex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0015969276428222656,30.358099469249375
100,300,0,300,1.5694160461425781,0.2558362703474601
200,600,0,600,2.9680771827697754,0.08934174715128616
300,900,0,900,4.286312103271484,0.049966668660965975
400,1200,0,1200,5.708057165145874,0.0398780202880175
501,1503,0,1503,7.092475175857544,0.031023146174764506
601,1803,0,1803,8.427781105041504,0.02740508280333077
701,2103,0,2103,10.170363187789917,0.024792823540412883
801,2403,0,2403,11.865816116333008,0.022930474266950565
901,2703,0,2703,13.542758226394653,0.02066662381302666
1001,3003,0,3003,15.095815896987915,0.019409901675894764
1101,3303,0,3303,16.74511694908142,0.018346287894342544
1201,3603,0,3603,18.314565181732178,0.017428700280383937
1301,3903,0,3903,19.77242612838745,0.01688683574575832
1401,4203,0,4203,21.255264043807983,0.01580968769943279
1502,4506,0,4506,22.689154148101807,0.014860562367812719
1602,4806,0,4806,24.108537197113037,0.014170136818821281
1702,5106,0,5106,25.54394006729126,0.013542236609947626
1802,5406,0,5406,26.951202154159546,0.012716719834548059
1902,5706,0,5706,28.359397172927856,0.012120752412907982
2002,6006,0,6006,29.75666618347168,0.01106241751364803
2102,6306,0,6306,31.185136079788208,0.010520432173213728
2202,6606,0,6606,32.65068221092224,0.010198448836670001
2302,6906,0,6906,34.07006311416626,0.009612793657862223
2402,7206,0,7206,35.42251396179199,0.00894129650469258
2503,7509,0,7509,36.78331398963928,0.008526140473015769
2603,7809,0,7809,38.16009497642517,0.008155833364238745
2703,8109,0,8109,39.52156710624695,0.007773304942162857
2803,8409,0,8409,40.88197708129883,0.0075149241134036164
2903,8709,0,8709,42.25773215293884,0.007148950227893117
3003,9009,0,9009,43.656453132629395,0.006681389289289457
3103,9309,0,9309,45.031299114227295,0.006478944627865752
3203,9609,0,9609,46.399781227111816,0.006326875119112185
3303,9909,0,9909,47.76416015625,0.006028816379464502
3403,10209,0,10209,49.18382215499878,0.0054719963395598575
3504,10512,0,10512,50.629339933395386,0.005227779175794816
3604,10812,0,10812,52.0320930480957,0.0047220832941419835
3704,11112,0,11112,53.40615105628967,0.0044675117660608115
3804,11412,0,11412,54.766002893447876,0.004345113970815105
3904,11712,0,11712,56.148781061172485,0.004235563763521706
4004,12012,0,12012,57.544105052948,0.004142363327059376
4104,12312,0,12312,59.009462118148804,0.00396323733230897
4204,12612,0,12612,60.46846413612366,0.003711737119918045
4304,12912,0,12912,61.87884497642517,0.003607266074338986
4404,13212,0,13212,63.249160051345825,0.0034960592919285093
4505,13515,0,13515,64.68282914161682,0.0033088980902778917
4605,13815,0,13815,66.07096815109253,0.0032198439028488287
4705,14115,0,14115,67.47292590141296,0.003114687304005925
4805,14415,0,14415,68.88489818572998,0.0028966919178996012
4905,14715,0,14715,70.26894211769104,0.0028122775230047395
5005,15015,0,15015,71.68890595436096,0.0027295703794356025
5105,15315,0,15315,73.0758171081543,0.0025972937540775873
5205,15615,0,15615,74.51222610473633,0.0024631905500353984
5305,15915,0,15915,75.92449522018433,0.0024212514694853943
5405,16215,0,16215,77.31047201156616,0.002371449467810702
5506,16518,0,16518,78.70583200454712,0.0023261257472835836
5606,16818,0,16818,80.08439707756042,0.0022749912533666116
5706,17118,0,17118,81.49479293823242,0.0022429914236220655
5806,17418,0,17418,82.88986611366272,0.0022137995710937385
5906,17718,0,17718,84.28218913078308,0.002183990393921515
6006,18018,0,18018,85.65504097938538,0.0021310959063658556
6106,18318,0,18318,87.10112404823303,0.002096316275208014
6206,18618,0,18618,88.5438141822815,0.002053213593059352
6306,18918,0,18918,90.36730599403381,0.0020068434135671
6406,19218,0,19218,91.82156610488892,0.0019819352881957474
6507,19521,0,19521,93.22777915000916,0.0019492732078105854
6607,19821,0,19821,94.6450879573822,0.001923921533106785
6707,20121,0,20121,95.96497106552124,0.0018979154427699056
6807,20421,0,20421,97.31627798080444,0.0018741497301274957
6907,20721,0,20721,98.62140393257141,0.0018335562128723223
7007,21021,0,21021,100.05377316474915,0.0017489235812159728
7107,21321,0,21321,101.36753511428833,0.0017345246459863064
7207,21621,0,21621,102.63075709342957,0.0017128237066868625
7307,21921,0,21921,103.8886251449585,0.0016886356793179888
7407,22221,0,22221,105.13262224197388,0.001675870049511331
7508,22524,0,22524,106.49311304092407,0.0016634591742988047
7608,22824,0,22824,107.80947613716125,0.0016531797803861776
7708,23124,0,23124,109.16131210327148,0.00163707663617967
7808,23424,0,23424,110.4352970123291,0.0016288359103853955
7908,23724,0,23724,111.94999718666077,0.0016177937496011001
8008,24024,0,24024,113.36350202560425,0.0016046359767386395
8108,24324,0,24324,114.68658995628357,0.001583557087554361
8208,24624,0,24624,115.99757814407349,0.001573486183530159
8308,24924,0,24924,117.34181213378906,0.0015682218204635125
8408,25224,0,25224,118.72475290298462,0.0015624137298700408
8509,25527,0,25527,120.08925223350525,0.0015497819417693538
8609,25827,0,25827,121.38509607315063,0.0015282786511432722
8709,26127,0,26127,122.69814610481262,0.0015220383718983147
8809,26427,0,26427,124.07480716705322,0.001512859579084859
8909,26727,0,26727,125.55700516700745,0.0015006782333938451
9009,27027,0,27027,126.9446542263031,0.0014962553365997443
9109,27327,0,27327,128.33493399620056,0.0014911645579553977
9209,27627,0,27627,129.72102308273315,0.0014864907957856022
9309,27927,0,27927,131.09399700164795,0.0014783035177133763
9409,28227,0,28227,132.50326204299927,0.0014606623735140688
9510,28530,0,28530,133.8767511844635,0.0014501532326496656
9610,28830,0,28830,135.31188201904297,0.001446006011782139
9710,29130,0,29130,136.74404406547546,0.0014406175584614836
9810,29430,0,29430,138.16079115867615,0.001434236196280784
9910,29730,0,29730,139.5326521396637,0.0014319336103881216
10010,30030,0,30030,140.79992699623108,0.0014290112593095304
10110,30330,0,30330,142.09016132354736,0.0014250441319356144
10210,30630,0,30630,143.38939595222473,0.0014228873511461758
10310,30930,0,30930,144.67839097976685,0.0014204135096037756
10410,31230,0,31230,145.97482800483704,0.001417568299210541
10511,31533,0,31533,147.2867341041565,0.001414572959186711
10611,31833,0,31833,148.58600497245789,0.0014112818923716383
10711,32133,0,32133,149.8955042362213,0.001405574446687046
10811,32433,0,32433,151.16408514976501,0.0014008713172486422
10911,32733,0,32733,152.45430827140808,0.0013988167794346151
11011,33033,0,33033,153.74529790878296,0.0013976274601485415
11111,33333,0,33333,155.01189613342285,0.0013944267714944508
11211,33633,0,33633,156.284921169281,0.0013817367089062624
11311,33933,0,33933,157.55410504341125,0.0013758678224940223
11411,34233,0,34233,158.83529806137085,0.0013727133104956125
11512,34536,0,34536,160.14355516433716,0.0013705249464476656
11612,34836,0,34836,161.4009358882904,0.0013682075070303975
11712,35136,0,35136,162.6720061302185,0.0013631955166533399
11812,35436,0,35436,163.92781019210815,0.001360984485595176
11912,35736,0,35736,165.1882860660553,0.001358832794136238
12012,36036,0,36036,166.46630907058716,0.0013576474996599922
12112,36336,0,36336,167.72675728797913,0.0013542963012866496
12212,36636,0,36636,168.980486869812,0.0013509068043028795
12312,36936,0,36936,170.24967408180237,0.0013473320656411149
12412,37236,0,37236,171.54247093200684,0.001344224837772137
12513,37539,0,37539,172.83207297325134,0.0013433558619534497
12613,37839,0,37839,174.13171005249023,0.0013411752125357978
12713,38139,0,38139,175.43692111968994,0.0013393772505745861
12813,38439,0,38439,176.70044898986816,0.0013370498173664001
12913,38739,0,38739,178.1264271736145,0.0013342270627008281
13013,39039,0,39039,179.4231722354889,0.001333120817809904
13113,39339,0,39339,180.7413730621338,0.001332049551729179
13213,39639,0,39639,182.05028200149536,0.0013306183461351316
13313,39939,0,39939,183.7640299797058,0.0013291970498147427
13413,40239,0,40239,185.6734049320221,0.0013273655877062795
13514,40542,0,40542,187.06827592849731,0.001326042818516791
13614,40842,0,40842,188.3376920223236,0.0013223803814937153
13714,41142,0,41142,189.60523796081543,0.0013207989779952184
13814,41442,0,41442,190.84255695343018,0.0013192049404253485
13914,41742,0,41742,192.09608912467957,0.0013173567517233255
14014,42042,0,42042,193.3544099330902,0.0013134377299470516
14114,42342,0,42342,194.6783411502838,0.001310072728884646
14214,42642,0,42642,196.05291223526,0.0013082768899863543
14314,42942,0,42942,197.48633408546448,0.001306923211637527
14414,43242,0,43242,198.78944516181946,0.0013053866128682064
14515,43545,0,43545,200.1372790336609,0.0013037819168319998
14615,43845,0,43845,201.47660493850708,0.0013010462448687123
14715,44145,0,44145,202.74161505699158,0.00129825757002798
14815,44445,0,44445,204.00518918037415,0.0012958474844030298
14915,44745,0,44745,205.23338222503662,0.0012947299907995627
15015,45045,0,45045,206.49479818344116,0.0012921293217062419
15115,45345,0,45345,207.7180049419403,0.0012903560298100775
15215,45645,0,45645,208.9744701385498,0.0012882961400547499
15315,45945,0,45945,210.21420907974243,0.0012855284155758198
15415,46245,0,46245,211.45613598823547,0.0012829062707881034
15516,46548,0,46548,212.7536702156067,0.0012756397016340279
15616,46848,0,46848,214.0136260986328,0.0012645033221337267
15716,47148,0,47148,215.26300692558289,0.0012555683953441909
15816,47448,0,47448,216.52209305763245,0.0012501938211999305
15916,47748,0,47748,217.7616400718689,0.0012489939513468913
16016,48048,0,48048,219.08295512199402,0.001247226973879457
16116,48348,0,48348,220.3043611049652,0.0012445684350924308
16216,48648,0,48648,221.5479290485382,0.0012429850380510459
16316,48948,0,48948,222.76180624961853,0.001241099755936911
16416,49248,0,49248,223.99760794639587,0.0012393126369919165
16517,49551,0,49551,225.23018288612366,0.001237581221266661
16617,49851,0,49851,226.48560619354248,0.0012354001604315433
16717,50151,0,50151,227.7475130558014,0.0012338322866639476
16817,50451,0,50451,229.02727818489075,0.0012324222031389281
16917,50751,0,50751,230.31390523910522,0.0012310173003230664
17017,51051,0,51051,231.5667369365692,0.0012285346644902687
17117,51351,0,51351,232.79679894447327,0.0012274328710083565
17217,51651,0,51651,234.04590320587158,0.0012263145218749053
17317,51951,0,51951,235.27164506912231,0.0012238342024227069
17417,52251,0,52251,236.53643703460693,0.0012216112577641746
17518,52554,0,52554,237.76628828048706,0.001220241082545021
17618,52854,0,52854,239.0133090019226,0.0012183853347775071
17718,53154,0,53154,240.23838305473328,0.0012169969823719036
17818,53454,0,53454,241.49704718589783,0.0012149643647868633
17918,53754,0,53754,242.7138650417328,0.0012141074109121128
18018,54054,0,54054,243.92589712142944,0.0012121871220570981
18118,54354,0,54354,245.17532110214233,0.0012108359369192177
18218,54654,0,54654,246.40770411491394,0.0012091431277658615
18318,54954,0,54954,247.67426300048828,0.0012082790090564275
18418,55254,0,55254,248.92826390266418,0.0012071700638810277
18519,55557,0,55557,250.18697309494019,0.001205665404832755
18619,55857,0,55857,251.4319360256195,0.00120419756257901
18719,56157,0,56157,252.66520309448242,0.0012013663299247804
18819,56457,0,56457,253.92733502388,0.001197721873697065
18919,56757,0,56757,255.154314994812,0.0011967313717130622
19019,57057,0,57057,256.3873369693756,0.001194491952860044
19119,57357,0,57357,257.63742423057556,0.0011913341766767826
19219,57657,0,57657,258.8881149291992,0.001189105529927936
19319,57957,0,57957,260.14413499832153,0.0011878832368097184
19419,58257,0,58257,261.34748125076294,0.0011869613654411967
19520,58560,0,58560,262.60861325263977,0.0011861219081959592
19620,58860,0,58860,263.8351800441742,0.0011840736328174784
19720,59160,0,59160,265.0949990749359,0.0011809701342142633
19820,59460,0,59460,266.3303849697113,0.0011795762681907599
19920,59760,0,59760,267.58639001846313,0.0011781804675730374
20020,60060,0,60060,268.8307681083679,0.001175191660263676
20120,60360,0,60360,270.08409309387207,0.0011735573855025186
20220,60660,0,60660,271.35529804229736,0.0011721708347211144
20320,60960,0,60960,272.58766317367554,0.0011709727622967888
20420,61260,0,61260,273.83371901512146,0.0011696954333838745
20521,61563,0,61563,275.0834450721741,0.0011687254715802803
20621,61863,0,61863,276.32500195503235,0.0011675281919757243
20721,62163,0,62163,277.5738801956177,0.0011651024941697309
20821,62463,0,62463,278.818852186203,0.0011627230942854781
20921,62763,0,62763,280.06044006347656,0.0011607014210462878
21021,63063,0,63063,281.26293206214905,0.0011588680697333766
21121,63363,0,63363,282.495726108551,0.0011570776426560504
21221,63663,0,63663,283.7233350276947,0.0011542018562777276
21321,63963,0,63963,284.9812271595001,0.0011519860081981074
21421,64263,0,64263,286.2240540981293,0.0011500335881051854
21522,64566,0,64566,287.4732129573822,0.0011475045841565384
21622,64866,0,64866,288.72698497772217,0.0011418899922247385
21722,65166,0,65166,289.9748511314392,0.0011402733751764316
21822,65466,0,65466,291.2055311203003,0.0011392082999825087
21922,65766,0,65766,292.4308979511261,0.001137221906467666
22022,66066,0,66066,293.6828920841217,0.001133317702732984
22122,66366,0,66366,294.92602014541626,0.0011311187942485736
22222,66666,0,66666,296.14018416404724,0.0011290886661458898
22322,66966,0,66966,297.3732180595398,0.001126332697710338
22422,67266,0,67266,298.6148102283478,0.0011236954582241982
22523,67569,0,67569,299.87996006011963,0.0011224338066998273
22623,67869,0,67869,301.11781096458435,0.0011210565512563826
22723,68169,0,68169,302.3471989631653,0.0011199772450964807
22823,68469,0,68469,303.59064412117004,0.0011165611626388731
22923,68769,0,68769,304.80954122543335,0.0011137227140037868
23023,69069,0,69069,306.06455397605896,0.0011126272174653165
23123,69369,0,69369,307.2867810726166,0.0011109850978361204
23223,69669,0,69669,308.5380861759186,0.0011075967627041832
23323,69969,0,69969,309.7471261024475,0.0011029654586524676
23423,70269,0,70269,310.9844410419464,0.00110198720281138
23524,70572,0,70572,312.2997760772705,0.0011010999679867694
23624,70872,0,70872,313.89983105659485,0.0010988681551477267
23724,71172,0,71172,315.31279706954956,0.0010963683956424098
23824,71472,0,71472,316.5659761428833,0.0010947487012730732
23924,71772,0,71772,317.8002200126648,0.0010934433982869524
24024,72072,0,72072,319.13704919815063,0.0010916564024955949
24124,72372,0,72372,320.7117991447449,0.0010909954158764956
24224,72672,0,72672,322.2054352760315,0.0010898106470108835
24324,72972,0,72972,323.72267508506775,0.001088992810956058
24424,73272,0,73272,325.04703307151794,0.001087229150851696
24525,73575,0,73575,326.4398150444031,0.0010844650877890793
24625,73875,0,73875,327.8295261859894,0.0010785449139202074
24725,74175,0,74175,329.1407370567322,0.0010772225576503962
24825,74475,0,74475,330.39199209213257,0.0010758334475003317
24925,74775,0,74775,331.6338601112366,0.00107476291446671
25025,75075,0,75075,332.8800461292267,0.001073821502103086
25125,75375,0,75375,334.12925601005554,0.0010729084401243517
25225,75675,0,75675,335.36172318458557,0.0010716638054432505
25325,75975,0,75975,336.60751700401306,0.001069648078673986
25425,76275,0,76275,337.8526039123535,0.0010687599149591643
25526,76578,0,76578,339.08982706069946,0.001067665265103101
25626,76878,0,76878,340.64274311065674,0.0010659502585364097
25726,77178,0,77178,342.0128939151764,0.001055176792738626
25826,77478,0,77478,343.43451595306396,0.0010500520417326311
25926,77778,0,77778,344.95423316955566,0.0010488120193617163
26026,78078,0,78078,346.21037220954895,0.0010479146966527306
26126,78378,0,78378,347.5883960723877,0.0010471850642398517
26226,78678,0,78678,348.9197361469269,0.00104624198879052
26326,78978,0,78978,350.229807138443,0.0010455014447005642
26426,79278,0,79278,351.58213210105896,0.0010443354575868336
26527,79581,0,79581,352.8150689601898,0.0010425088718980277
26627,79881,0,79881,354.0677399635315,0.0010400259361896486
26727,80181,0,80181,355.2736802101135,0.00103756220906455
26827,80481,0,80481,356.6804051399231,0.0010367439331607916
26927,80781,0,80781,357.92480206489563,0.0010357784032456532
27027,81081,0,81081,359.2541608810425,0.001034996647003929
27127,81381,0,81381,360.5507252216339,0.0010337245962706355
27227,81681,0,81681,361.9320650100708,0.0010317018359446884
27327,81981,0,81981,363.2376801967621,0.001026612199637923
27427,82281,0,82281,364.50400614738464,0.0010240708877735328
27528,82584,0,82584,365.76367592811584,0.0010229652606323475
27628,82884,0,82884,367.1836030483246,0.001020932625230162
27728,83184,0,83184,368.5045120716095,0.0010189074511659432
27828,83484,0,83484,369.7486379146576,0.0010179436005081231
27928,83784,0,83784,370.9839632511139,0.0010164304809585324
28028,84084,0,84084,372.2045199871063,0.0010149426125149084
28128,84384,0,84384,373.43443298339844,0.0010141109076974787
28228,84684,0,84684,374.6699929237366,0.0010127375122014563
28328,84984,0,84984,375.8980002403259,0.001010998801106065
28428,85284,0,85284,377.1416709423065,0.001007927966664411
28529,85587,0,85587,378.3781991004944,0.0010067351260886494
28629,85887,0,85887,379.66813707351685,0.0010059473082282278
28729,86187,0,86187,380.8970482349396,0.0010051039512799325
28829,86487,0,86487,382.1628460884094,0.0010044338159953623
28929,86787,0,86787,383.40486311912537,0.0010038318649663218
29029,87087,0,87087,384.7445991039276,0.001002838655349658
29129,87387,0,87387,386.08296513557434,0.0010018314839037503
29229,87687,0,87687,387.45009207725525,0.0010006644287503955
29329,87987,0,87987,388.83616518974304,0.0009996994568165303
29429,88287,0,88287,390.0820801258087,0.0009989170483502966
29530,88590,0,88590,391.49170899391174,0.0009979989470967961
29630,88890,0,88890,392.8507490158081,0.0009969161349651443
29730,89190,0,89190,394.12720799446106,0.000996024895611673
29830,89490,0,89490,395.3598699569702,0.0009929890572871823
29930,89790,0,89790,396.5858380794525,0.000990840489829741
30030,90090,0,90090,397.92262291908264,0.000990237948234242
30130,90390,0,90390,399.1714780330658,0.0009895731447058561
30230,90690,0,90690,400.4008300304413,0.0009889563903741434
30330,90990,0,90990,401.6436140537262,0.0009880760514876137
30430,91290,0,91290,402.8750801086426,0.0009860076920814233
30531,91593,0,91593,404.12044405937195,0.0009829239010519229
30631,91893,0,91893,405.30564403533936,0.0009820160466940484
30731,92193,0,92193,406.5220990180969,0.000981219598050536
30831,92493,0,92493,407.7319700717926,0.0009802290086488182
30931,92793,0,92793,408.96454405784607,0.0009776153304173084
31031,93093,0,93093,410.181174993515,0.0009702062725641716
31131,93393,0,93393,411.39081501960754,0.0009660700498601589
31231,93693,0,93693,412.62924218177795,0.0009653853495388265
31331,93993,0,93993,413.8395709991455,0.0009642610571845044
31431,94293,0,94293,415.0666460990906,0.0009608375399531007
31532,94596,0,94596,416.2826511859894,0.0009595135649580971
31632,94896,0,94896,417.5091631412506,0.0009583537017346258
31732,95196,0,95196,418.7291660308838,0.0009564247213903133
31832,95496,0,95496,419.94564723968506,0.0009558543193272055
31932,95796,0,95796,421.17721700668335,0.0009549605630046007
32032,96096,0,96096,422.38077425956726,0.000954379228112735
32132,96396,0,96396,423.6159989833832,0.0009533922144121178
32232,96696,0,96696,424.82818508148193,0.0009515847300693806
32332,96996,0,96996,426.06440806388855,0.0009502919741958354
32432,97296,0,97296,427.27361607551575,0.0009483752513997578
32533,97599,0,97599,428.5167360305786,0.0009472043966983365
32633,97899,0,97899,429.748987197876,0.0009460277097995238
32733,98199,0,98199,430.9790871143341,0.0009437044879418617
32833,98499,0,98499,432.2127842903137,0.000939923060989245
32933,98799,0,98799,433.4258270263672,0.0009368303632945965
33033,99099,0,99099,434.65540409088135,0.0009351119005235398
33133,99399,0,99399,435.865198135376,0.0009336357123907699
33233,99699,0,99699,437.088191986084,0.0009324027768001497
33333,99999,0,99999,438.30022621154785,0.0009306255485093633
33433,100299,0,100299,439.53014612197876,0.0009292189548498899
33534,100602,0,100602,440.757755279541,0.0009278480201448256
33634,100902,0,100902,441.9720530509949,0.0009267720281092097
33734,101202,0,101202,443.20889496803284,0.000926040137566008
33834,101502,0,101502,444.42588114738464,0.0009251699542349449
33934,101802,0,101802,445.6523151397705,0.0009245582660759196
34034,102102,0,102102,446.856733083725,0.000923417847127761
34134,102402,0,102402,448.08529710769653,0.0009228602668796006
34234,102702,0,102702,449.29829716682434,0.0009219950058296013
34334,103002,0,103002,450.50719594955444,0.0009203500519986921
34434,103302,0,103302,451.7210760116577,0.0009193816228026097
34535,103605,0,103605,452.9386579990387,0.0009179665410526352
34635,103905,0,103905,454.178857088089,0.0009164231101394209
34735,104205,0,104205,455.379182100296,0.0009155325139882658
34835,104505,0,104505,456.6069450378418,0.0009138366044695793
34935,104805,0,104805,457.827702999115,0.0009119637904842533
35035,105105,0,105105,459.0925509929657,0.0009098010984321253
35135,105405,0,105405,460.35284304618835,0.0009071015102123827
35235,105705,0,105705,461.6326730251312,0.0009050247993081462
35335,106005,0,106005,462.96211099624634,0.0009041540394820126
35435,106305,0,106305,464.2832701206207,0.0009030773128404266
35536,106608,0,106608,465.68634128570557,0.0009015991287620287
35636,106908,0,106908,467.1455910205841,0.0008994103870773476
35736,107208,0,107208,468.5390999317169,0.0008960840022690119
35836,107508,0,107508,469.78106212615967,0.000894633647849851
35936,107808,0,107808,471.11541724205017,0.0008906145956874567
36036,108108,0,108108,472.4869439601898,0.0008895003752354714
36136,108408,0,108408,473.84032011032104,0.0008886173120793334
36236,108708,0,108708,475.1144902706146,0.0008879448005233853
36336,109008,0,109008,476.4608702659607,0.0008872894996239657
36436,109308,0,109308,477.96062111854553,0.0008866367554571187
36537,109611,0,109611,479.3088541030884,0.0008861426498784016
36637,109911,0,109911,480.5995891094208,0.0008853913358486045
36737,110211,0,110211,481.8702480792999,0.0008847359523240251
36837,110511,0,110511,483.3176620006561,0.0008842243757289713
36937,110811,0,110811,484.55541706085205,0.0008832651437926074
37037,111111,0,111111,485.76682305336,0.0008820021613373829
37137,111411,0,111411,486.9919822216034,0.0008801733384268476
37237,111711,0,111711,488.21957302093506,0.0008777143833189377
37337,112011,0,112011,489.44221901893616,0.0008767292930296168
37437,112311,0,112311,490.6730260848999,0.0008761448296295143
37538,112614,0,112614,491.9037609100342,0.0008748193212632686
37638,112914,0,112914,493.1417751312256,0.0008727923735337776
37738,113214,0,113214,494.36538004875183,0.0008719879738567836
37838,113514,0,113514,495.5904881954193,0.0008711837190499763
37938,113814,0,113814,496.81163024902344,0.0008695644063248293
38038,114114,0,114114,498.0359799861908,0.0008687438241928864
38138,114414,0,114414,499.2672700881958,0.0008648899299744492
38238,114714,0,114714,500.489706993103,0.00085969240292651
38338,115014,0,115014,501.7139639854431,0.0008577549013736174
38438,115314,0,115314,502.9428701400757,0.0008572831017019176
38539,115617,0,115617,504.1942400932312,0.0008563726502165314
38639,115917,0,115917,505.5049510002136,0.0008555725479002678
38739,116217,0,116217,506.91988706588745,0.0008544889979270137
38839,116517,0,116517,508.31813502311707,0.0008533311217068639
38939,116817,0,116817,509.5243682861328,0.0008524786138481396
39039,117117,0,117117,510.73708319664,0.0008517692982830438
39139,117417,0,117417,512.0229871273041,0.0008504550413735417
39239,117717,0,117717,513.4491541385651,0.0008497756585359997
39339,118017,0,118017,514.7585589885712,0.0008489372530253166
39439,118317,0,118317,516.0033342838287,0.0008482525047326497
39540,118620,0,118620,517.2516810894012,0.0008474655744270842
39640,118920,0,118920,518.4912271499634,0.0008468124336527605
39740,119220,0,119220,519.7162082195282,0.0008449799560189141
39840,119520,0,119520,520.9409620761871,0.0008440275514948031
39940,119820,0,119820,522.1587331295013,0.0008429611068873121
40040,120120,0,120120,523.3891499042511,0.000841536496613625
40140,120420,0,120420,524.610758304596,0.0008401715507470532
40240,120720,0,120720,525.8275480270386,0.0008386097913270066
40340,121020,0,121020,527.0438079833984,0.0008373759551088232
40440,121320,0,121320,528.2632701396942,0.0008367487827636548
40541,121623,0,121623,529.4910368919373,0.000835949485029184
40641,121923,0,121923,530.7242529392242,0.0008350252319187682
40741,122223,0,122223,531.9498281478882,0.0008333132101913377
40841,122523,0,122523,533.1663889884949,0.0008303043126705423
40941,122823,0,122823,534.3838069438934,0.0008119140811226807
41041,123123,0,123123,535.6061260700226,0.0007590166832365952
41141,123423,0,123423,536.8244531154633,0.0007487985111082222
41241,123723,0,123723,538.0472500324249,0.0007470430947968511
41341,124023,0,124023,539.2710690498352,0.000745548757977841
41441,124323,0,124323,540.4919991493225,0.0007439000025036214
41542,124626,0,124626,541.7217390537262,0.0007411874641129794
41642,124926,0,124926,542.9377040863037,0.000740311961204941
41742,125226,0,125226,544.1587951183319,0.0007397537447510106
41842,125526,0,125526,545.3816199302673,0.0007383930003967323
41942,125826,0,125826,546.5928530693054,0.0007378595320380245
42042,126126,0,126126,547.8210439682007,0.0007372264300234999
42142,126426,0,126426,549.0428080558777,0.0007367461977622037
42242,126726,0,126726,550.2661399841309,0.000735785826992971
42342,127026,0,127026,551.5043683052063,0.0007343167893560696
42442,127326,0,127326,552.7151770591736,0.0007336047388088667
42543,127629,0,127629,553.9680099487305,0.0007328752686529141
42643,127929,0,127929,555.1962969303131,0.0007323955315045733
42743,128229,0,128229,556.4223830699921,0.000731901421297615
42843,128529,0,128529,557.6452550888062,0.0007312553701311701
42943,128829,0,128829,558.8852250576019,0.0007306142411620908
43043,129129,0,129129,560.1170451641083,0.000729638534647603
43143,129429,0,129429,561.330983877182,0.0007287879947397675
43243,129729,0,129729,562.5588660240173,0.00072828228959458
43343,130029,0,130029,563.7703051567078,0.000727701221827724
43443,130329,0,130329,564.9930801391602,0.0007266882989497586
43544,130632,0,130632,566.2096331119537,0.0007261962582747437
43644,130932,0,130932,567.4349009990692,0.0007256099450452921
43744,131232,0,131232,568.6552813053131,0.0007250928529656784
43844,131532,0,131532,569.883632183075,0.000724507093826673
43944,131832,0,131832,571.1084380149841,0.0007241269439781214
44044,132132,0,132132,572.3270552158356,0.0007234663905146113
44144,132432,0,132432,573.5825481414795,0.0007220397082833272
44244,132732,0,132732,574.8638331890106,0.0007209867072720764
44344,133032,0,133032,576.1847450733185,0.000720436017096445
44444,133332,0,133332,577.5400750637054,0.0007195726834625768
44545,133635,0,133635,578.8453681468964,0.0007177771251470691
44645,133935,0,133935,580.2542111873627,0.000717235544023042
44745,134235,0,134235,581.6388449668884,0.0007167867639739866
44845,134535,0,134535,582.9369232654572,0.0007157385050023212
44945,134835,0,134835,584.169379234314,0.0007152487454922015
45045,135135,0,135135,585.3787660598755,0.0007145734588752367
45145,135435,0,135435,586.6105711460114,0.0007137823424339932
45245,135735,0,135735,587.8287010192871,0.0007123261506942164
45345,136035,0,136035,589.0607490539551,0.0007108672708572434
45445,136335,0,136335,590.2803020477295,0.0007102244750550476
45546,136638,0,136638,591.497955083847,0.0007095909275271812
45646,136938,0,136938,592.702320098877,0.0007081567756591645
45746,137238,0,137238,593.9122622013092,0.0007074597539630707
45846,137538,0,137538,595.226998090744,0.0007068721203844337
45946,137838,0,137838,596.657552242279,0.0007060976121716529
46046,138138,0,138138,597.9949040412903,0.0007054518994480115
46146,138438,0,138438,599.3453462123871,0.0007047942565629794
46246,138738,0,138738,600.6528551578522,0.0007039881164621114
46346,139038,0,139038,601.9522559642792,0.0007032546790122766
46446,139338,0,139338,603.1853060722351,0.0007025878884524528
46547,139641,0,139641,604.464714050293,0.0007016723357656403
46647,139941,0,139941,605.6923110485077,0.0007012425206700386
46747,140241,0,140241,606.9221441745758,0.0007007239349467312
46847,140541,0,140541,608.1836092472076,0.0007000515230333616
46947,140841,0,140841,609.4050571918488,0.0006994433612603057
47047,141141,0,141141,610.6421670913696,0.0006982772927788506
47147,141441,0,141441,611.8637609481812,0.0006973727375403176
47247,141741,0,141741,613.0858361721039,0.000696917017147061
47347,142041,0,142041,614.3551690578461,0.0006959844877530698
47447,142341,0,142341,615.575777053833,0.0006948342166578055
47548,142644,0,142644,616.8963141441345,0.0006864544057144053
47648,142944,0,142944,618.2634408473969,0.0006852113229276288
47748,143244,0,143244,619.6108741760254,0.0006844070407610722
47848,143544,0,143544,620.8368740081787,0.0006827593859874263
47948,143844,0,143844,622.0683121681213,0.0006815144199454441
48048,144144,0,144144,623.3129489421844,0.0006804808975328117
48148,144444,0,144444,624.5993421077728,0.000678942987145915
48248,144744,0,144744,625.8469409942627,0.0006776952543140685
48348,145044,0,145044,627.0991492271423,0.0006770043692948831
48448,145344,0,145344,628.3401942253113,0.00067638028477074
48549,145647,0,145647,629.5828862190247,0.0006758065599945088
48649,145947,0,145947,630.7894999980927,0.0006751556961370021
48749,146247,0,146247,632.0311989784241,0.0006744109781835276
48849,146547,0,146547,633.2358210086823,0.0006738992708169269
48949,146847,0,146847,634.4911119937897,0.0006732451528439657
49049,147147,0,147147,635.6897668838501,0.0006727189795708835
49149,147447,0,147447,636.9060659408569,0.0006700191944843335
49249,147747,0,147747,638.1447460651398,0.0006686761599754407
49349,148047,0,148047,639.3697581291199,0.000667317842151808
49449,148347,0,148347,640.6028780937195,0.0006662611993357956
49550,148650,0,148650,641.8321652412415,0.0006655523811570574
49650,148950,0,148950,643.0769250392914,0.0006647984177003939
49750,149250,0,149250,644.2973189353943,0.0006640611085803307
49850,149550,0,149550,645.5276951789856,0.0006635406523901869
49950,149850,0,149850,646.7368819713593,0.0006628078044517721
50050,150150,0,150150,647.9690170288086,0.0006608911734069305
50150,150450,0,150450,649.1909019947052,0.0006562164335811679
50250,150750,0,150750,650.4004333019257,0.0006544368205241681
50350,151050,0,151050,651.638833284378,0.0006536878375239248
50450,151350,0,151350,652.8553750514984,0.0006530443907935748
50551,151653,0,151653,654.0985569953918,0.0006520902862785296
50651,151953,0,151953,655.3026621341705,0.0006509325063735403
50751,152253,0,152253,656.5384089946747,0.0006503200436920259
50851,152553,0,152553,657.7635791301727,0.000649641206773616
50951,152853,0,152853,659.0028111934662,0.0006491383619415057
51051,153153,0,153153,660.2401180267334,0.0006486193543861046
51151,153453,0,153453,661.4646921157837,0.0006480233225472775
51251,153753,0,153753,662.6930310726166,0.0006474110254226607
51351,154053,0,154053,663.9042510986328,0.0006466904427954644
51451,154353,0,154353,665.1404581069946,0.000645088345250674
51552,154656,0,154656,666.3624069690704,0.0006445218147952175
51652,154956,0,154956,667.5855560302734,0.0006436004279815873
51752,155256,0,155256,668.820405960083,0.0006430177708872788
51852,155556,0,155556,670.0479681491852,0.000642633360288959
51952,155856,0,155856,671.2761981487274,0.0006417063740433708
52052,156156,0,156156,672.5000672340393,0.0006402564242491376
52152,156456,0,156456,673.7222490310669,0.00063807349326587
52252,156756,0,156756,674.9371101856232,0.000637572344085148
52352,157056,0,157056,676.1612710952759,0.0006371480234957903
52452,157356,0,157356,677.3805260658264,0.0006363309096176427
52553,157659,0,157659,678.6029100418091,0.0006331733252719376
52653,157959,0,157959,679.8477811813354,0.0006315959426697869
52753,158259,0,158259,681.1299710273743,0.0006307803525219773
52853,158559,0,158559,682.4489049911499,0.0006301313291565285
52953,158859,0,158859,683.7920892238617,0.0006296154308539065
53053,159159,0,159159,685.0764091014862,0.0006292316352709571
53153,159459,0,159459,686.4276280403137,0.0006288605389822458
53253,159759,0,159759,687.8275241851807,0.0006282301234460855
53353,160059,0,160059,689.0614039897919,0.0006278347307699257
53453,160359,0,160359,690.2691051959991,0.0006274087294359957
53554,160662,0,160662,691.5061190128326,0.0006264337806461785
53654,160962,0,160962,692.7293939590454,0.0006248610367358952
53754,161262,0,161262,693.9509391784668,0.0006244146688379872
53854,161562,0,161562,695.1856400966644,0.0006238257039013878
53954,161862,0,161862,696.3962481021881,0.0006230003201073192
54054,162162,0,162162,697.6152052879333,0.0006220912279851379
54154,162462,0,162462,698.9199471473694,0.0006214936301118038
54254,162762,0,162762,700.1833872795105,0.0006209047999644951
54354,163062,0,163062,701.9442460536957,0.000620255403023788
54454,163362,0,163362,703.2725040912628,0.0006196711802078532
54555,163665,0,163665,705.2190940380096,0.000619036750498362
54655,163965,0,163965,706.5347471237183,0.0006184952308997191
54755,164265,0,164265,708.0725839138031,0.0006176874404313761
54855,164565,0,164565,709.7319722175598,0.0006169454939926869
54955,164865,0,164865,711.2085099220276,0.000616000770849363
55055,165165,0,165165,712.5812659263611,0.0006154948635263304
55155,165465,0,165465,714.1699810028076,0.0006143347267016441
55255,165765,0,165765,715.5163321495056,0.0006133731859060464
55355,166065,0,166065,716.7922630310059,0.000612888596729997
55455,166365,0,166365,718.0101759433746,0.0006124731132866772
55556,166668,0,166668,719.7303411960602,0.0006117183645350648
55656,166968,0,166968,721.9904389381409,0.000610487206527667
55756,167268,0,167268,723.7813980579376,0.0006093784033561696
55856,167568,0,167568,725.0034160614014,0.0006089685738227394
55956,167868,0,167868,726.20942902565,0.0006086798626941223
56056,168168,0,168168,727.4254789352417,0.0006081931171287217
56156,168468,0,168468,728.6548140048981,0.0006075243906265929
56256,168768,0,168768,729.874715089798,0.000606458571810622
56356,169068,0,169068,731.1044390201569,0.0006051050847458595
56456,169368,0,169368,732.3384199142456,0.0006047528964456979
56557,169671,0,169671,733.5940201282501,0.0006040568613076421
56657,169971,0,169971,734.8227939605713,0.0006034897393757673
56757,170271,0,170271,736.0212481021881,0.0006026961113316634
56857,170571,0,170571,737.258373260498,0.0006020155026849796
56957,170871,0,170871,738.4874041080475,0.0006013615186289335
57057,171171,0,171171,739.7215840816498,0.0005996902355359091
57157,171471,0,171471,740.9552371501923,0.0005971181389293232
57257,171771,0,171771,742.2011280059814,0.0005965495577200221
57357,172071,0,172071,743.4441123008728,0.0005961369616345668
57457,172371,0,172371,744.6636111736298,0.0005955298448284727
57558,172674,0,172674,745.93119597435,0.0005948726395337213
57658,172974,0,172974,747.0970942974091,0.0005943580401264034
57758,173274,0,173274,748.3021581172943,0.0005938729367378186
57858,173574,0,173574,749.4788701534271,0.000593239563667743
57958,173874,0,173874,750.6790752410889,0.0005926033466683658
58058,174174,0,174174,752.0660212039948,0.0005922181890898773
58158,174474,0,174474,753.3775329589844,0.0005912305538758527
58258,174774,0,174774,754.6557152271271,0.000590572800410807
58358,175074,0,175074,755.8211042881012,0.0005894691578600356
58458,175374,0,175374,757.1501250267029,0.0005890257071211079
58559,175677,0,175677,758.4196510314941,0.0005881614742855243
58659,175977,0,175977,760.0574991703033,0.0005868217406184607
58759,176277,0,176277,761.3517181873322,0.0005859421863997383
58859,176577,0,176577,762.5510110855103,0.0005844577717837775
58959,176877,0,176877,763.8500111103058,0.0005815446862197296
59059,177177,0,177177,765.124537229538,0.0005801208622523852
59159,177477,0,177477,766.3319702148438,0.0005789864121289067
59259,177777,0,177777,767.6357560157776,0.0005771138648279465
59359,178077,0,178077,768.9127922058105,0.0005766174464682126
59459,178377,0,178377,770.1498839855194,0.000575442152788154
59560,178680,0,178680,771.3668642044067,0.0005747741090570921
59660,178980,0,178980,772.54421210289,0.0005743993091414956
59760,179280,0,179280,773.7525990009308,0.000573806528693677
59860,179580,0,179580,774.9620401859283,0.00057303628080431
59960,179880,0,179880,776.2717771530151,0.000572565903642297
60060,180180,0,180180,777.7211589813232,0.0005721312707595731
60160,180480,0,180480,778.9830729961395,0.0005717689179896899
60260,180780,0,180780,780.2867901325226,0.0005711682167462691
60360,181080,0,181080,781.5978391170502,0.0005707173037757159
60460,181380,0,181380,782.88818526268,0.0005701610254948574
60561,181683,0,181683,784.1372489929199,0.0005694624940560586
60661,181983,0,181983,785.3476741313934,0.0005690612857129664
60761,182283,0,182283,786.591982126236,0.0005685445470392144
60861,182583,0,182583,787.9121179580688,0.0005676979321994044
60961,182883,0,182883,789.521595954895,0.000566956291887927
61061,183183,0,183183,790.7123122215271,0.0005662545416269846
61161,183483,0,183483,791.8912279605865,0.0005657423723739387
61261,183783,0,183783,793.152596950531,0.0005648299753100237
61361,184083,0,184083,794.7179141044617,0.0005639695573972716
61461,184383,0,184383,795.908215045929,0.0005634476386195715
61562,184686,0,184686,797.1836321353912,0.000562754587035744
61662,184986,0,184986,798.3014781475067,0.0005621684732616463
61762,185286,0,185286,799.4205319881439,0.0005617752140069521
61862,185586,0,185586,800.5364952087402,0.000560669579413228
61962,185886,0,185886,801.6321301460266,0.0005581142092160341
62062,186186,0,186186,802.7453792095184,0.0005571935883617886
62162,186486,0,186486,803.8506519794464,0.0005567609041974142
62262,186786,0,186786,804.9670789241791,0.0005562738739972281
62362,187086,0,187086,806.0639569759369,0.0005558627348703859
62462,187386,0,187386,807.173798084259,0.0005552435353033494
62563,187689,0,187689,808.2784271240234,0.0005544952578693931
62663,187989,0,187989,809.3904950618744,0.0005533856606164424
62763,188289,0,188289,810.4954700469971,0.0005528438286388633
62863,188589,0,188589,811.6175980567932,0.0005522224555336209
62963,188889,0,188889,812.7290229797363,0.0005515992960435067
63063,189189,0,189189,813.8234710693359,0.0005511368743598585
63163,189489,0,189489,814.9228720664978,0.0005507479393848278
63263,189789,0,189789,816.0236940383911,0.0005501372745601703
63363,190089,0,190089,817.1325371265411,0.0005498106158902674
63463,190389,0,190389,818.2435519695282,0.0005490574970581004
63564,190692,0,190692,819.3747310638428,0.0005476270428156373
63664,190992,0,190992,820.4751009941101,0.0005446095395582427
63764,191292,0,191292,821.5910320281982,0.0005424007889692499
63864,191592,0,191592,822.6962890625,0.0005416379453507622
63964,191892,0,191892,823.8030490875244,0.0005410688831858528
64064,192192,0,192192,824.903923034668,0.0005407070440719842
64164,192492,0,192492,826.0154249668121,0.0005402984385255615
64264,192792,0,192792,827.1120011806488,0.0005397376379087241
64364,193092,0,193092,828.2192461490631,0.0005391212681581047
64464,193392,0,193392,829.3088021278381,0.0005385712357714674
64565,193695,0,193695,830.4218621253967,0.0005382630198933264
64665,193995,0,193995,831.5202391147614,0.0005378466686390083
64765,194295,0,194295,832.6273851394653,0.0005372771413147472
64865,194595,0,194595,833.7251441478729,0.0005363422865862864
64965,194895,0,194895,834.8265030384064,0.0005353884923918622
65065,195195,0,195195,835.9229040145874,0.0005349399879971648
65165,195495,0,195495,837.0370519161224,0.0005342669435196994
65265,195795,0,195795,838.1325681209564,0.0005338235945966457
65365,196095,0,196095,839.2406551837921,0.0005331810176995092
65465,196395,0,196395,840.3286850452423,0.0005321898075030306
65566,196698,0,196698,841.4483089447021,0.0005316526940853353
65666,196998,0,196998,842.5590310096741,0.0005309665590372361
65766,197298,0,197298,843.6643152236938,0.0005303400198899217
65866,197598,0,197598,844.7610702514648,0.000529961910624051
65966,197898,0,197898,845.8759210109711,0.0005294674951389832
66066,198198,0,198198,846.976674079895,0.0005287847874388455
66166,198498,0,198498,848.103226184845,0.0005273148480771423
66266,198798,0,198798,849.1967470645905,0.0005262471453920353
66366,199098,0,199098,850.2999889850616,0.0005257304375208429
66466,199398,0,199398,851.3972091674805,0.0005244198620124955
66567,199701,0,199701,852.5274062156677,0.000522557094275223
66667,200001,0,200001,853.632404088974,0.0005220566534213724
66767,200301,0,200301,854.7500381469727,0.0005216571240952762
66867,200601,0,200601,855.8574631214142,0.0005209613749127301
66967,200901,0,200901,856.9698979854584,0.0005204568355129876
67067,201201,0,201201,858.132826089859,0.0005196463079730917
67167,201501,0,201501,859.2898831367493,0.0005188437269134972
67267,201801,0,201801,860.4568800926208,0.0005178540722818069
67367,202101,0,202101,861.7431440353394,0.0005170933852292802
67467,202401,0,202401,862.9984781742096,0.0005167490186967363
67568,202704,0,202704,864.3050670623779,0.0005162916875287171
67668,203004,0,203004,865.5311779975891,0.000515580869003265
67768,203304,0,203304,866.654443025589,0.0005148390084276197
67868,203604,0,203604,867.7677590847015,0.0005141907162216273
67968,203904,0,203904,868.8719229698181,0.0005111375859949342
68068,204204,0,204204,869.9903008937836,0.0005101981853689954
68168,204504,0,204504,871.1027159690857,0.0005096760066557091
68268,204804,0,204804,872.2146060466766,0.0005089732938106612
68368,205104,0,205104,873.3406701087952,0.0005082718874911528
68468,205404,0,205404,874.4439611434937,0.0005074038920096846
68569,205707,0,205707,875.5730969905853,0.0005070267492171268
68669,206007,0,206007,876.7158210277557,0.0005060023844627907
68769,206307,0,206307,877.8630900382996,0.000505156616016454
68869,206607,0,206607,879.0017399787903,0.0005048327815682712
68969,206907,0,206907,880.123594045639,0.0005045461938443676
69069,207207,0,207207,881.267664194107,0.0005040347843203674
69169,207507,0,207507,882.3741393089294,0.0005033624915792105
69269,207807,0,207807,883.4902031421661,0.0005028559477344767
69369,208107,0,208107,884.5989890098572,0.0005021103184002664
69469,208407,0,208407,885.6982390880585,0.0005007512522101072
69570,208710,0,208710,886.9205601215363,0.0004984075197913206
69670,209010,0,209010,888.2502992153168,0.0004980172082220609
69770,209310,0,209310,889.4995341300964,0.000497225198149776
69870,209610,0,209610,890.6811480522156,0.0004966792240987585
69970,209910,0,209910,891.7849841117859,0.0004961352959364887
70070,210210,0,210210,892.8879020214081,0.0004956020176086365
70170,210510,0,210510,893.9965372085571,0.0004951255932356604
70270,210810,0,210810,895.1012370586395,0.0004946015961860883
70370,211110,0,211110,896.2047622203827,0.0004940031093638795
70470,211410,0,211410,897.3107631206512,0.0004934403103136281
70571,211713,0,211713,898.4202382564545,0.0004930900225894213
70671,212013,0,212013,899.5374143123627,0.0004927059980740222
70771,212313,0,212313,900.6369531154633,0.0004922583925407336
70871,212613,0,212613,901.7416388988495,0.000491876656397582
70971,212913,0,212913,902.8826420307159,0.0004912457047843515
71071,213213,0,213213,904.1405341625214,0.0004905299596944029
71171,213513,0,213513,905.3562109470367,0.0004899796415272428
71271,213813,0,213813,906.5932130813599,0.0004893326696859011
71371,214113,0,214113,907.6965661048889,0.0004888460948290847
71471,214413,0,214413,908.8113920688629,0.0004883770514314606
71572,214716,0,214716,910.0099079608917,0.00048794652300085785
71672,215016,0,215016,911.2348790168762,0.0004872604887556261
71772,215316,0,215316,912.4262480735779,0.0004865268251114978
71872,215616,0,215616,913.6701571941376,0.0004856029875293046
71972,215916,0,215916,914.9214148521423,0.0004852205427598473
72072,216216,0,216216,916.0292711257935,0.0004847765633196455
72172,216516,0,216516,917.1385090351105,0.0004844751133646553
72272,216816,0,216816,918.2415151596069,0.00048403786932774086
72372,217116,0,217116,919.3458518981934,0.0004836741201958151
72472,217416,0,217416,920.4308910369873,0.0004832313424054268
72573,217719,0,217719,921.5535428524017,0.0004829235948065574
72673,218019,0,218019,922.6551780700684,0.00048257172199848785
72773,218319,0,218319,923.762552022934,0.00048224529176755534
72873,218619,0,218619,924.9161880016327,0.0004810976487404138
72973,218919,0,218919,926.0275819301605,0.00047857269123685673
73073,219219,0,219219,927.1237711906433,0.00047755417577535834
73173,219519,0,219519,928.2290949821472,0.0004769788614952369
73273,219819,0,219819,929.3295521736145,0.00047655249940224584
73373,220119,0,220119,930.4425389766693,0.00047630947929024753
73473,220419,0,220419,931.5495979785919,0.00047577930024776324
73574,220722,0,220722,932.6716091632843,0.0004754492590724056
73674,221022,0,221022,933.7717161178589,0.0004751546654916138
73774,221322,0,221322,934.8876402378082,0.00047490139345277406
73874,221622,0,221622,935.9947619438171,0.0004740945513420383
73974,221922,0,221922,937.1118421554565,0.0004730054114912867
74074,222222,0,222222,938.2265350818634,0.0004726719668715093
74174,222522,0,222522,939.3722941875458,0.00047220275315679953
74274,222822,0,222822,940.6456918716431,0.00047178508421315924
74374,223122,0,223122,941.8419210910797,0.0004709733174584925
74474,223422,0,223422,943.0998950004578,0.0004702665197045311
74575,223725,0,223725,944.3025450706482,0.00046980776820888597
74675,224025,0,224025,945.5947918891907,0.000469355822981002
74775,224325,0,224325,946.6924750804901,0.00046868316978229175
74875,224625,0,224625,947.8044202327728,0.00046661929283167247
74975,224925,0,224925,948.8978481292725,0.00046494847420212187
75075,225225,0,225225,950.0104231834412,0.00046455883550238056
75175,225525,0,225525,951.0993139743805,0.00046382970658304817
75275,225825,0,225825,952.2007710933685,0.00046302207194441673
75375,226125,0,226125,953.2941410541534,0.000461919997087925
75475,226425,0,226425,954.4032802581787,0.0004613342667836558
75576,226728,0,226728,955.5208201408386,0.00046060544834356214
75676,227028,0,227028,956.6273670196533,0.00045995855246999163
75776,227328,0,227328,957.7228710651398,0.00045860626122338366
75876,227628,0,227628,958.829118013382,0.00045798575185682685
75976,227928,0,227928,959.9265310764313,0.0004565894504983974
76076,228228,0,228228,961.0369470119476,0.0004561786465257795
76176,228528,0,228528,962.1314740180969,0.00045576023938751094
76276,228828,0,228828,963.2422270774841,0.00045546406449586296
76376,229128,0,229128,964.3516800403595,0.00045514925515126244
76476,229428,0,229428,965.4620831012726,0.0004548621381002862
76577,229731,0,229731,966.584529876709,0.00045384593283627505
76677,230031,0,230031,967.7962622642517,0.0004491853475986565
76777,230331,0,230331,969.0749661922455,0.00043900999345650074
76877,230631,0,230631,970.2259521484375,0.00042973297367062134
76977,230931,0,230931,971.4221200942993,0.0004196769048801795
77077,231231,0,231231,972.5619411468506,0.00040054739661930745
77177,231531,0,231531,973.7222049236298,0.0003773720401448776
77277,231831,0,231831,974.8984639644623,0.00036790630655279117
77377,232131,0,232131,976.0893449783325,0.00036069038050100884
77477,232431,0,232431,977.3107709884644,0.00035851744035582405
77578,232734,0,232734,978.8712818622589,0.00035796356380773844
77678,233034,0,233034,980.0742740631104,0.0003576692811063946
77778,233334,0,233334,981.1946649551392,0.0003573019715404646
77878,233634,0,233634,982.3800251483917,0.0003566204661239445
77978,233934,0,233934,983.6968531608582,0.00035623092503510675
78078,234234,0,234234,984.8589670658112,0.0003559144610051128
78178,234534,0,234534,985.9630982875824,0.00035536736980298526
78278,234834,0,234834,987.0973470211029,0.0003547461956996096
78378,235134,0,235134,988.2020878791809,0.00035427261262623396
78478,235434,0,235434,989.3539352416992,0.0003539875991934468
78579,235737,0,235737,990.5014090538025,0.0003537871456752606
78679,236037,0,236037,991.6150379180908,0.0003535167452448984
78779,236337,0,236337,992.7444059848785,0.000353127408251749
78879,236637,0,236637,993.8709151744843,0.0003529153703106347
78979,236937,0,236937,995.1454889774323,0.00035209057451026596
79079,237237,0,237237,996.3894562721252,0.00035092392453489943
79179,237537,0,237537,997.6438360214233,0.00035062734370245387
79279,237837,0,237837,998.8848309516907,0.0003503322890290421
79379,238137,0,238137,1000.243411064148,0.0003497658626550906
79479,238437,0,238437,1001.6137919425964,0.0003481132297727646
79580,238740,0,238740,1002.9704160690308,0.0003471649216615669
79680,239040,0,239040,1004.4318861961365,0.00034686187678573165
79780,239340,0,239340,1005.6606621742249,0.0003463829263741389
79880,239640,0,239640,1006.9738161563873,0.0003459257909723785
79980,239940,0,239940,1008.1406750679016,0.0003455695394248755
80080,240240,0,240240,1009.4456970691681,0.0003450417939904828
80180,240540,0,240540,1010.9087340831757,0.00034408495257489324
80280,240840,0,240840,1012.1685791015625,0.00034300936719330286
80380,241140,0,241140,1013.3647191524506,0.0003427004899014929
80480,241440,0,241440,1014.6269490718842,0.0003419820672641981
80581,241743,0,241743,1015.8515660762787,0.0003409098086309755
80681,242043,0,242043,1017.7725791931152,0.00034062183892319344
80781,242343,0,242343,1019.4999680519104,0.0003404302248377472
80881,242643,0,242643,1020.9882230758667,0.0003401514856662899
80981,242943,0,242943,1022.465891122818,0.000339648174753989
81081,243243,0,243243,1023.7569489479065,0.00033941996153949585
81181,243543,0,243543,1025.1506659984589,0.000339086814402488
81281,243843,0,243843,1026.5533361434937,0.0003385779763570661
81381,244143,0,244143,1027.7833001613617,0.00033818281055672024
81481,244443,0,244443,1029.2949771881104,0.00033788533484052684
81582,244746,0,244746,1030.795704126358,0.0003375512395270128
81682,245046,0,245046,1032.1314401626587,0.00033622288819832604
81782,245346,0,245346,1033.3574678897858,0.00033465014652021965
81882,245646,0,245646,1034.591698884964,0.0003343743150409968
81982,245946,0,245946,1035.8603670597076,0.000334176831529614
82082,246246,0,246246,1037.5018792152405,0.00033387562209004926
82182,246546,0,246546,1038.8140170574188,0.00033327583281270965
82282,246846,0,246846,1040.0820128917694,0.0003329978561527485
82382,247146,0,247146,1041.446468114853,0.00033264140550767426
82482,247446,0,247446,1042.646409034729,0.0003322519306883843
82583,247749,0,247749,1044.0785138607025,0.0003318492786837376
82683,248049,0,248049,1045.7478892803192,0.0003315398743705227
82783,248349,0,248349,1046.9688420295715,0.00033128985119582386
82883,248649,0,248649,1048.2204420566559,0.0003307530008846778
82983,248949,0,248949,1049.7379751205444,0.00033037896102199835
83083,249249,0,249249,1051.143478155136,0.0003300735012342284
83183,249549,0,249549,1052.5967061519623,0.0003297931293158224
83283,249849,0,249849,1054.649274110794,0.00032951010493831686
83383,250149,0,250149,1056.098562002182,0.00032917624764774436
83483,250449,0,250449,1057.9252791404724,0.000328755104240709
83584,250752,0,250752,1059.3249552249908,0.00032777607618080906
83684,251052,0,251052,1060.706838130951,0.0003257761047070793
83784,251352,0,251352,1062.1765570640564,0.0003254817811371501
83884,251652,0,251652,1063.4085550308228,0.0003252100780699897
83984,251952,0,251952,1064.5531070232391,0.00032428678026692525
84084,252252,0,252252,1065.7218761444092,0.0003231416831751566
84184,252552,0,252552,1066.927011013031,0.00032290182466849756
84284,252852,0,252852,1068.1650612354279,0.0003226672705189777
84384,253152,0,253152,1069.4361250400543,0.0003223299611254034
84484,253452,0,253452,1070.7192521095276,0.0003219120071608304
84585,253755,0,253755,1072.0217349529266,0.00032115089266205265
84685,254055,0,254055,1074.1585030555725,0.0003209594861430343
84785,254355,0,254355,1076.3663301467896,0.00032053608728901793
84885,254655,0,254655,1077.564227104187,0.00032013940335683545
84985,254955,0,254955,1079.002515077591,0.00031987495238093664
85085,255255,0,255255,1080.3505091667175,0.00031961409605120884
85185,255555,0,255555,1081.5965740680695,0.00031933051400407205
85285,255855,0,255855,1082.8659720420837,0.00031903021371731504
85385,256155,0,256155,1084.0959060192108,0.00031865441431358586
85485,256455,0,256455,1085.278789281845,0.0003184161149761428
85586,256758,0,256758,1086.6199769973755,0.000318139387502692
85686,257058,0,257058,1087.9776740074158,0.00031781585155334476
85786,257358,0,257358,1089.777107000351,0.00031764210284560365
85886,257658,0,257658,1091.0829739570618,0.00031736625287325806
85986,257958,0,257958,1092.4066429138184,0.0003168893110947384
86086,258258,0,258258,1093.601511001587,0.0003158955909572499
86186,258558,0,258558,1094.9216890335083,0.0003153252185612974
86286,258858,0,258858,1096.205999135971,0.00031512773352363897
86386,259158,0,259158,1097.4252190589905,0.0003145567595576184
86486,259458,0,259458,1098.652713060379,0.0003143039295924938
86587,259761,0,259761,1099.8588271141052,0.0003139634192786742
86687,260061,0,260061,1100.9959480762482,0.0003136309144466823
86787,260361,0,260361,1102.2470149993896,0.00031335223246709693
86887,260661,0,260661,1103.5317871570587,0.0003130949545698649
86987,260961,0,260961,1104.7988941669464,0.0003124129102637962
87087,261261,0,261261,1106.015291929245,0.00031109813805775126
87187,261561,0,261561,1107.1420328617096,0.000310438876853793
87287,261861,0,261861,1108.3311650753021,0.0003099699768670068
87387,262161,0,262161,1109.5704340934753,0.00030932894413669736
87487,262461,0,262461,1110.7208971977234,0.0003080360524963414
87588,262764,0,262764,1111.901223897934,0.00030737947078492893
87688,263064,0,263064,1113.1059908866882,0.0003070945209911111
87788,263364,0,263364,1114.2854762077332,0.0003067121576765181
87888,263664,0,263664,1115.4725770950317,0.0003065073967358242
87988,263964,0,263964,1116.64719414711,0.00030601772852751247
88088,264264,0,264264,1117.8803040981293,0.0003056097866603009
88188,264564,0,264564,1119.057433128357,0.000305429562510674
88288,264864,0,264864,1120.205574274063,0.0003052109275263911
88388,265164,0,265164,1121.4052522182465,0.00030476419938246395
88488,265464,0,265464,1122.5595829486847,0.0003043758391850442
88589,265767,0,265767,1123.6852259635925,0.0003040685796488399
88689,266067,0,266067,1125.0057830810547,0.0003032809253853687
88789,266367,0,266367,1126.1730592250824,0.0003024063662564672
88889,266667,0,266667,1127.3286180496216,0.0003021589210895428
88989,266967,0,266967,1128.5882921218872,0.00030193237179398366
89089,267267,0,267267,1129.8247590065002,0.0003010347194880094
89189,267567,0,267567,1130.9648230075836,0.0003000329067674452
89289,267867,0,267867,1132.1738109588623,0.0002988639503051206
89389,268167,0,268167,1133.4813890457153,0.00029757641775162976
89489,268467,0,268467,1134.7474880218506,0.000295975582174794
89590,268770,0,268770,1135.9519202709198,0.00029436548990082454
89690,269070,0,269070,1137.2049720287323,0.0002930954106884687
89790,269370,0,269370,1138.3595910072327,0.0002926109418470654
89890,269670,0,269670,1139.7142641544342,0.0002920593090839834
89990,269970,0,269970,1141.076267004013,0.0002912975205495239
90090,270270,0,270270,1142.5016651153564,0.00029027091426612794
90190,270570,0,270570,1143.8823680877686,0.00028999724976842096
90290,270870,0,270870,1145.1891751289368,0.0002897192139375945
90390,271170,0,271170,1146.5089061260223,0.00028924203424352706
90490,271470,0,271470,1147.8621079921722,0.0002887272827438098
90591,271773,0,271773,1149.6140999794006,0.0002879498023615841
90691,272073,0,272073,1150.9418320655823,0.0002877023018439956
90791,272373,0,272373,1152.178601026535,0.0002873502840199174
90891,272673,0,272673,1153.351718902588,0.00028704411721687615
90991,272973,0,272973,1154.5859310626984,0.00028669915885673274
91091,273273,0,273273,1155.907613992691,0.0002864295782507335
91191,273573,0,273573,1157.053169965744,0.00028598930416887054
91291,273873,0,273873,1159.025318145752,0.000285472817865217
91391,274173,0,274173,1160.443144083023,0.0002851813251819474
91491,274473,0,274473,1161.772931098938,0.0002847282457293065
91592,274776,0,274776,1163.3703980445862,0.0002841431834195013
91692,275076,0,275076,1165.2892701625824,0.0002839330260436813
91792,275376,0,275376,1166.5507571697235,0.0002836994683356116
91892,275676,0,275676,1168.2139892578125,0.00028284003184951757
91992,275976,0,275976,1169.7034690380096,0.0002806318146225018
92092,276276,0,276276,1171.1308181285858,0.00027868171348989707
92192,276576,0,276576,1172.4443361759186,0.00027749845402537317
92292,276876,0,276876,1173.6920709609985,0.00027727501380593383
92392,277176,0,277176,1174.9630160331726,0.0002770610367514565
92492,277476,0,277476,1176.335398197174,0.0002767320739882955
92593,277779,0,277779,1177.7397520542145,0.0002762493917165333
92693,278079,0,278079,1179.031524181366,0.00027605688550258917
92793,278379,0,278379,1180.7677791118622,0.00027580122766529964
92893,278679,0,278679,1182.1475920677185,0.0002754753057292166
92993,278979,0,278979,1183.582150220871,0.00027512587540812677
93093,279279,0,279279,1185.0189189910889,0.0002747577732311563
93193,279579,0,279579,1186.2829520702362,0.0002745551932469773
93293,279879,0,279879,1187.8594481945038,0.00027436173964850134
93393,280179,0,280179,1189.9859981536865,0.0002740084018411443
93493,280479,0,280479,1191.5062851905823,0.0002736865871095069
93594,280782,0,280782,1192.7286050319672,0.0002734861407039395
93694,281082,0,281082,1194.0296819210052,0.00027331886059816005
93794,281382,0,281382,1195.2562580108643,0.0002731502502574717
93894,281682,0,281682,1196.578292131424,0.00027297649734718776
93994,281982,0,281982,1197.9180850982666,0.00027272476268723635
94094,282282,0,282282,1199.059730052948,0.0002722863238900686
94194,282582,0,282582,1200.2792329788208,0.00027175944170888214
94294,282882,0,282882,1201.5448861122131,0.0002714175709044705
94394,283182,0,283182,1202.7905631065369,0.00027119884568146783
94494,283482,0,283482,1203.9337768554688,0.0002709288677969388
94595,283785,0,283785,1205.145478963852,0.0002702022943620325
94695,284085,0,284085,1206.3169662952423,0.0002697030036424473
94795,284385,0,284385,1207.4901161193848,0.00026942285726331595
94895,284685,0,284685,1208.6915700435638,0.0002688729615798026
94995,284985,0,284985,1209.8869190216064,0.0002685451036907283
95095,285285,0,285285,1211.1463060379028,0.0002682681617024928
95195,285585,0,285585,1212.5168042182922,0.00026764917343044515
95295,285885,0,285885,1214.0104739665985,0.0002665456600956138
95395,286185,0,286185,1215.4577569961548,0.00026604631491745575
95495,286485,0,286485,1216.9031450748444,0.0002658289168207139
95596,286788,0,286788,1218.2902002334595,0.0002654188568500362
95696,287088,0,287088,1220.1334400177002,0.00026492891551649
95796,287388,0,287388,1221.5608069896698,0.00026471723321008767
95896,287688,0,287688,1222.8038671016693,0.00026180091970937536
95996,287988,0,287988,1224.09969997406,0.0002597445789562826
96096,288288,0,288288,1225.356994152069,0.0002589341259698407
96196,288588,0,288588,1226.7739081382751,0.00025852640023053114
96296,288888,0,288888,1228.0384030342102,0.0002580564155410985
96396,289188,0,289188,1229.3532531261444,0.0002571232037598842
96496,289488,0,289488,1230.5567581653595,0.00025681164011832306
96597,289791,0,289791,1231.8940780162811,0.0002565629772039285
96697,290091,0,290091,1233.0879430770874,0.0002560155173701239
96797,290391,0,290391,1234.3976180553436,0.0002557180388991759
96897,290691,0,290691,1235.6935200691223,0.00025546044552454455
96997,290991,0,290991,1236.924576997757,0.0002549577395916713
97097,291291,0,291291,1238.1293630599976,0.00025452498914714977
97197,291591,0,291591,1239.2784280776978,0.0002540331767307239
97297,291891,0,291891,1240.432224035263,0.00025379537206609036
97397,292191,0,292191,1241.6381719112396,0.0002535970259417424
97497,292491,0,292491,1243.0206871032715,0.00025296453534016944
97598,292794,0,292794,1244.2035970687866,0.00025272949399594895
97698,293094,0,293094,1245.3505311012268,0.0002525087845061461
97798,293394,0,293394,1246.5448100566864,0.00025237331172359417
97898,293694,0,293694,1247.8006720542908,0.00025220590594731524
97998,293994,0,293994,1249.0164322853088,0.0002518619483135389
98098,294294,0,294294,1250.3026020526886,0.0002515931964728533
98198,294594,0,294594,1251.5402262210846,0.00025139503313426477
98298,294894,0,294894,1252.7948710918427,0.00025123107640206646
98398,295194,0,295194,1254.0257320404053,0.0002506370224762924
98498,295494,0,295494,1255.1903822422028,0.000249491526346033
98599,295797,0,295797,1256.3606390953064,0.0002477186644189012
98699,296097,0,296097,1257.6960220336914,0.0002454797293666816
98799,296397,0,296397,1258.8365659713745,0.00024497832447304687
98899,296697,0,296697,1260.047520160675,0.0002447613227597163
98999,296997,0,296997,1261.2104818820953,0.0002445616949539183
99099,297297,0,297297,1262.4763650894165,0.0002442181961478204
99199,297597,0,297597,1263.5758032798767,0.00024378004627149299
99299,297897,0,297897,1264.7617771625519,0.00024359529896258767
99399,298197,0,298197,1265.9567830562592,0.00024330113640774314
99499,298497,0,298497,1267.1086032390594,0.00024294206740279475
99600,298800,0,298800,1268.443638086319,0.00024264776968781952
99700,299100,0,299100,1269.739690065384,0.00024229777104748664
99800,299400,0,299400,1270.9619920253754,0.00024202806828230674
99900,299700,0,299700,1272.230621099472,0.0002415872942918838
100000,300000,0,300000,1273.4924311637878,0.00024120510503400068


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha0/flex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0020329952239990234,30.358099469249375
100,424,0,424,11.530822992324829,0.7211239886005693
200,904,0,904,22.382174968719482,0.40714633829939134
300,1404,0,1404,34.79979491233826,0.3624245498130248
400,1902,0,1902,48.25783395767212,0.3234305807147064
501,2407,0,2407,61.11792182922363,0.29927923547289564
601,2907,0,2907,85.75802087783813,0.2798141171444672
701,3407,0,3407,98.99608302116394,0.2632947441677823
801,3907,0,3907,112.55429983139038,0.24894925517918357
901,4407,0,4407,126.18071508407593,0.23628795092033392
1001,4907,0,4907,139.6558690071106,0.22497484237422974
1101,5407,0,5407,152.25598907470703,0.21476752442670155
1201,5907,0,5907,165.7279508113861,0.2054846363539787
1301,6407,0,6407,184.41180896759033,0.19698661111494115
1401,6907,0,6907,201.8121268749237,0.18916356405203077
1502,7412,0,7412,221.29149985313416,0.18185766975309853
1602,7912,0,7912,241.743145942688,0.17514117836096976
1702,8412,0,8412,254.947429895401,0.16887965154176085
1802,8912,0,8912,267.55008482933044,0.16302350106398145
1902,9412,0,9412,280.15908002853394,0.1575308461743764
2002,9906,0,9906,292.8066408634186,0.1498909696800842
2102,10406,0,10406,305.7974798679352,0.14511979342703413
2202,10906,0,10906,319.88458704948425,0.1406365536270806
2302,11406,0,11406,334.51855397224426,0.1363983502206184
2402,11906,0,11906,348.7635259628296,0.13238114794475966
2503,12411,0,12411,363.64821791648865,0.12852939777278136
2603,12911,0,12911,379.149533033371,0.12490383158500992
2703,13407,0,13407,392.99544882774353,0.11553399137809793
2803,13907,0,13907,406.1307227611542,0.11231346686490083
2903,14407,0,14407,419.2718060016632,0.10933628292944855
3003,14907,0,14907,434.93468499183655,0.10651303192284882
3103,15407,0,15407,448.0619008541107,0.10382200685747961
3203,15907,0,15907,461.18357396125793,0.10125140448760439
3303,16407,0,16407,479.00568985939026,0.09879265478836109
3403,16907,0,16907,492.33714485168457,0.09643871785544907
3504,17412,0,17412,509.0118637084961,0.09416140847986092
3604,17912,0,17912,521.8378748893738,0.09200032233161215
3704,18412,0,18412,535.0510878562927,0.08992748237389693
3804,18912,0,18912,552.0745508670807,0.08793835459711602
3904,19412,0,19412,568.6648321151733,0.08602875165783933
4004,19912,0,19912,585.7096610069275,0.08419478483088971
4104,20412,0,20412,598.5380339622498,0.0824328268805458
4204,20912,0,20912,613.5069599151611,0.08073948242407632
4304,21412,0,21412,626.9345738887787,0.07911156369042999
4404,21912,0,21912,641.1888289451599,0.07754607031317048
4505,22407,0,22407,659.2055780887604,0.07412162093332915
4605,22907,0,22907,672.944258928299,0.07266764686185315
4705,23407,0,23407,686.1172778606415,0.07129191334254018
4805,23907,0,23907,699.1751177310944,0.06997352237985814
4905,24407,0,24407,712.2094647884369,0.06870656535722068
5005,24907,0,24907,725.0786509513855,0.06748769686123084
5105,25407,0,25407,738.0261557102203,0.06631436994781609
5205,25907,0,25907,750.802943944931,0.06518438528819169
5305,26407,0,26407,763.7665297985077,0.0640957425747773
5405,26907,0,26907,777.0606007575989,0.06304658122831297
5506,27412,0,27412,793.9410650730133,0.06202522276507799
5606,27912,0,27912,810.2395877838135,0.06105022534018896
5706,28412,0,28412,826.6118190288544,0.06010972354705247
5806,28912,0,28912,842.4531509876251,0.05920222813705618
5906,29412,0,29412,859.3099689483643,0.05832632196249025
6006,29912,0,29912,873.7724928855896,0.0574806551447777
6106,30412,0,30412,887.4118149280548,0.056663940917151684
6206,30912,0,30912,901.9954099655151,0.05587495195963205
6306,31412,0,31412,914.8183000087738,0.0551125171130183
6406,31912,0,31912,928.5312740802765,0.05437551839647884
6507,32417,0,32417,942.1256458759308,0.05365588154699887
6607,32917,0,32917,954.4354367256165,0.05296682890984573
6707,33417,0,33417,966.618992805481,0.05230014171908473
6807,33917,0,33917,978.741593837738,0.051654889779197126
6907,34417,0,34417,990.6945848464966,0.05103018423515985
7007,34917,0,34917,1002.7270920276642,0.05042517565306127
7107,35417,0,35417,1015.2092890739441,0.04983905221077293
7207,35917,0,35917,1028.6408529281616,0.04927103798794479
7307,36417,0,36417,1045.7464368343353,0.04872039134625246
7407,36917,0,36917,1060.7387809753418,0.04818640339217861
7508,37422,0,37422,1076.133887052536,0.04766329493547635
7608,37922,0,37922,1093.0635027885437,0.0471607715793348
7708,38422,0,38422,1114.8128159046173,0.04667295638047154
7808,38922,0,38922,1135.1672189235687,0.04619925775612519
7908,39422,0,39422,1149.1382939815521,0.04573911020535582
8008,39922,0,39922,1162.4239869117737,0.04529197315535938
8108,40422,0,40422,1176.490732908249,0.04485732985844246
8208,40922,0,40922,1189.6200489997864,0.044434686336964735
8308,41422,0,41422,1202.6657400131226,0.044023570373814894
8408,41922,0,41922,1215.597286939621,0.04362353054621258
8509,42427,0,42427,1229.867672920227,0.04323029369210993
8609,42927,0,42927,1243.8667237758636,0.042851230758281296
8709,43427,0,43427,1257.5102939605713,0.04248200154872427
8809,43927,0,43927,1271.3605818748474,0.042122229124322834
8909,44427,0,44427,1284.8668088912964,0.04177155308608374
9009,44927,0,44927,1299.300086736679,0.04142962883171067
9109,45427,0,45427,1313.060154914856,0.04109612684404679
9209,45927,0,45927,1326.3377480506897,0.040770732010117626
9309,46427,0,46427,1338.2295548915863,0.04045314296956796
9409,46927,0,46927,1352.7918779850006,0.040143071491339014
9510,47432,0,47432,1367.3644816875458,0.03983724925067063
9610,47932,0,47932,1379.565703868866,0.03954146625473345
9710,48432,0,48432,1391.9209508895874,0.03925240660388256
9810,48932,0,48932,1403.9370110034943,0.03896982898442213
9910,49432,0,49432,1416.0391960144043,0.03869350247681848
10010,49932,0,49932,1428.6557099819183,0.03842320608021646
10110,50432,0,50432,1441.0178439617157,0.0381587282582497
10210,50932,0,50932,1453.5225479602814,0.03789986650528598
10310,51432,0,51432,1465.6704320907593,0.0376464269322772
10410,51932,0,51932,1477.6191189289093,0.03739822387140901
10511,52437,0,52437,1489.7092170715332,0.03715267301898622
10611,52937,0,52937,1501.7192778587341,0.0369144650422313
10711,53437,0,53437,1514.0669329166412,0.036680980616877995
10811,53937,0,53937,1526.2341759204865,0.036452063422408636
10911,54437,0,54437,1538.2167429924011,0.03622756363542651
11011,54937,0,54937,1550.234736919403,0.036007337631807586
11111,55437,0,55437,1562.2655770778656,0.03579124770272562
11211,55937,0,55937,1574.1058077812195,0.03557916178394309
11311,56437,0,56437,1586.0512640476227,0.03537095319778201
11411,56937,0,56937,1597.9737689495087,0.03516650040720988
11512,57442,0,57442,1615.3587369918823,0.03496369664043619
11612,57942,0,57942,1629.4004759788513,0.03476644495400363
11712,58442,0,58442,1642.5760068893433,0.034572611954376276
11812,58942,0,58942,1655.720473766327,0.034382094473384965
11912,59442,0,59442,1670.0420188903809,0.03419479341549434
12012,59942,0,59942,1682.9648687839508,0.034010613573976216
12112,60442,0,60442,1695.883455991745,0.03382946345581324
12212,60942,0,60942,1708.6967058181763,0.033651255114921674
12312,61442,0,61442,1721.6466648578644,0.03347590399330601
12412,61942,0,61942,1734.8478050231934,0.03330332876976875
12513,62447,0,62447,1748.1637229919434,0.03313176580641659
12613,62947,0,62947,1761.2309248447418,0.032964536502534676
12713,63447,0,63447,1777.8363211154938,0.03279985643632003
12813,63947,0,63947,1793.2251427173615,0.032637655886183815
12913,64447,0,64447,1806.698473930359,0.03247786771108069
13013,64947,0,64947,1819.7779068946838,0.03232042723762245
13113,65447,0,65447,1832.9393289089203,0.03216527215255024
13213,65947,0,65947,1846.071567773819,0.03201234240030491
13313,66447,0,66447,1860.9739437103271,0.03186158008544811
13413,66947,0,66947,1877.415676832199,0.031712929379698634
13514,67452,0,67452,1890.791702747345,0.03156488071824445
13614,67952,0,67952,1903.9150910377502,0.031420313377671524
13714,68452,0,68452,1926.4961490631104,0.031277701206731325
13814,68952,0,68952,1942.3393449783325,0.031136995817789413
13914,69452,0,69452,1959.0758409500122,0.030998150486561515
14014,69952,0,69952,1974.363665819168,0.030861120082511715
14114,70452,0,70452,1988.509057044983,0.030725861002498165
14214,70952,0,70952,2001.7513778209686,0.030592331107508468
14314,71452,0,71452,2016.0631008148193,0.030460489662333293
14414,71952,0,71952,2033.0121738910675,0.03033029727803295
14515,72457,0,72457,2051.217803001404,0.03020043805249401
14615,72957,0,72957,2068.4985258579254,0.030073446295327814
14715,73457,0,73457,2081.939071893692,0.029947992622735602
14815,73957,0,73957,2095.5886929035187,0.02982404251793523
14915,74457,0,74457,2109.1607768535614,0.029701562559652565
15015,74957,0,74957,2123.9330780506134,0.029580520378722924
15115,75457,0,75457,2141.0875968933105,0.029460884616658703
15215,75957,0,75957,2158.284019947052,0.02934262488608667
15315,76457,0,76457,2172.0095648765564,0.029225711732965277
15415,76957,0,76957,2186.205173969269,0.02911011660049324
15516,77462,0,77462,2199.3033339977264,0.028994675171147264
15616,77962,0,77962,2215.05273604393,0.028881646329353566
15716,78462,0,78462,2227.8991067409515,0.028769854627310715
15816,78962,0,78962,2240.834687948227,0.028659274774876783
15916,79462,0,79462,2253.863869905472,0.02854988222107437
16016,79962,0,79962,2267.1133980751038,0.028441653126581905
16116,80462,0,80462,2280.759913921356,0.028334564337422295
16216,80962,0,80962,2296.527907848358,0.02822859335979148
16316,81462,0,81462,2313.0370268821716,0.02812371833597236
16416,81962,0,81962,2327.2373938560486,0.02801991802128283
16517,82467,0,82467,2342.548015832901,0.027916149553975544
16617,82967,0,82967,2358.561978816986,0.02781444750641096
16717,83467,0,83467,2374.3455760478973,0.02771375970348491
16817,83967,0,83967,2392.520315885544,0.027614067146357803
16917,84467,0,84467,2407.9821660518646,0.027515351347660956
17017,84967,0,84967,2421.888589859009,0.02741759431370801
17117,85467,0,85467,2435.336438894272,0.02732077852744474
17217,85967,0,85967,2448.6152000427246,0.027224886932101754
17317,86467,0,86467,2463.8463571071625,0.027129902915518755
17417,86967,0,86967,2480.4564638137817,0.027035810295108976
17518,87472,0,87472,2498.2942447662354,0.026941665503121628
17618,87972,0,87972,2515.1728279590607,0.026849317300399776
17718,88472,0,88472,2529.5761048793793,0.026757814234302894
17818,88972,0,88972,2543.8529908657074,0.02666714170567395
17918,89472,0,89472,2559.0662229061127,0.026577285478252936
18018,89972,0,89972,2575.4600887298584,0.02648823166691711
18118,90472,0,90472,2591.9184987545013,0.02639996672638456
18218,90972,0,90972,2608.3714809417725,0.026312477440357824
18318,91472,0,91472,2622.5750579833984,0.026225750911090542
18418,91972,0,91972,2636.3040828704834,0.026139774549356072
18519,92477,0,92477,2649.4175939559937,0.026053687365394207
18619,92977,0,92977,2664.025887966156,0.025969181956384153
18719,93477,0,93477,2678.234997987747,0.025885390587905288
18819,93977,0,93977,2697.1511340141296,0.025802301814638235
18919,94477,0,94477,2715.4963080883026,0.025719904455001306
19019,94977,0,94977,2729.0815908908844,0.02563818758319546
19119,95477,0,95477,2742.195200920105,0.025557140521545334
19219,95977,0,95977,2755.179090976715,0.025476752833121646
19319,96477,0,96477,2768.1082389354706,0.02539701431463412
19419,96977,0,96977,2781.5839698314667,0.025317914989583464
19520,97482,0,97482,2794.8082020282745,0.025238663548976383
19620,97982,0,97982,2808.130770921707,0.025160819707165254
19720,98482,0,98482,2823.2386009693146,0.025083586332892437
19820,98982,0,98982,2838.657737016678,0.025006954295131875
19920,99482,0,99482,2852.1092739105225,0.02493091465886757
20020,99982,0,99982,2865.699343919754,0.02485545867958763
20120,100482,0,100482,2881.40762591362,0.02478057779796985
20220,100982,0,100982,2895.5104768276215,0.024706263634751913
20320,101482,0,101482,2909.3388438224792,0.024632507985778672
20420,101982,0,101982,2923.0371339321136,0.024559302817217885
20521,102487,0,102487,2937.539256811142,0.024485916349359912
20621,102987,0,102987,2951.006284713745,0.024413794009141166
20721,103487,0,103487,2964.9109346866608,0.024342198949622917
20821,103987,0,103987,2979.3916108608246,0.024271123775095913
20921,104487,0,104487,2994.557282924652,0.024200561238531683
21021,104987,0,104987,3009.3928248882294,0.024130504237684668
21121,105487,0,105487,3022.657185792923,0.02406094581132183
21221,105987,0,105987,3035.9876239299774,0.023991879135575656
21321,106487,0,106487,3049.6288447380066,0.023923297520414007
21421,106987,0,106987,3062.98609995842,0.023855194406224477
21522,107492,0,107492,3077.362186908722,0.023786889412548983
21622,107992,0,107992,3091.7328329086304,0.023719728752867975
21722,108492,0,108492,3105.5426609516144,0.023653027604014453
21822,108992,0,108992,3119.379554748535,0.02358677989717937
21922,109492,0,109492,3133.3999869823456,0.023520979678421098
22022,109992,0,109992,3147.999525785446,0.023455621105846466
22122,110492,0,110492,3161.8533248901367,0.023390698446878175
22222,110992,0,110992,3175.673744916916,0.023326206075605784
22322,111492,0,111492,3188.8049507141113,0.02326213847021747
22422,111992,0,111992,3203.571299791336,0.023198490210508734
22523,112497,0,112497,3217.2878918647766,0.02313462570618456
22623,112997,0,112997,3231.0257470607758,0.02307180433358704
22723,113497,0,113497,3244.6159019470215,0.02300938658106969
22823,113997,0,113997,3258.044862985611,0.022947367412315362
22923,114497,0,114497,3271.4005880355835,0.022885741881207046
23023,114997,0,114997,3285.445354938507,0.02282450512974702
23123,115497,0,115497,3298.755598783493,0.022763652386037187
23223,115997,0,115997,3312.2299988269806,0.022703178962316377
23323,116497,0,116497,3325.908143758774,0.022643080253054206
23423,116997,0,116997,3339.0548827648163,0.02258335173309895
23524,117502,0,117502,3352.250956773758,0.02252339716025753
23624,118002,0,118002,3365.502891778946,0.0224643993479438
23724,118502,0,118502,3378.5407979488373,0.022405758571431213
23824,119002,0,119002,3393.227765083313,0.02234747061030448
23924,119502,0,119502,3406.7748880386353,0.022289531315998343
24024,120002,0,120002,3420.1193149089813,0.022231936610233788
24124,120502,0,120502,3433.1112859249115,0.02217468248349646
24224,121002,0,121002,3446.3205959796906,0.022117764993556097
24324,121502,0,121502,3460.9685950279236,0.022061180264026363
24424,122002,0,122002,3480.8348059654236,0.022004924482962318
24525,122507,0,122507,3498.894775867462,0.021948436225412243
24625,123007,0,123007,3514.59432888031,0.021892830353131793
24725,123507,0,123507,3530.4318029880524,0.021837542330694057
24825,124007,0,124007,3547.2124388217926,0.021782568591209733
24925,124507,0,124507,3563.7903077602386,0.02172790562574264
25025,125007,0,125007,3580.576714038849,0.02167354998211346
25125,125507,0,125507,3596.5768909454346,0.02161949826373493
25225,126007,0,126007,3612.113711833954,0.021565747128475997
25325,126507,0,126507,3641.0656049251556,0.021512293287554933
25425,127007,0,127007,3657.1694588661194,0.02145913350446069
25526,127512,0,127512,3672.471748828888,0.021405737363052093
25626,128012,0,128012,3686.926495075226,0.021353159051635536
25726,128512,0,128512,3701.5981509685516,0.02130086536113156
25826,129012,0,129012,3715.98739695549,0.021248853254326214
25926,129512,0,129512,3731.783205986023,0.02119711974126094
26026,130012,0,130012,3763.9249007701874,0.02114566187830369
26126,130512,0,130512,3777.7061519622803,0.021094476767243103
26226,131012,0,131012,3791.025691986084,0.021043561554404063
26326,131512,0,131512,3804.8346440792084,0.020992913429784776
26426,132012,0,132012,3824.6084909439087,0.020942529626214106
26527,132517,0,132517,3844.4832859039307,0.02089190750839625
26627,133017,0,133017,3863.2962958812714,0.020842046788341756
26727,133517,0,133517,3877.8396260738373,0.020792442310443675
26827,134017,0,134017,3891.7798190116882,0.020743091471211724
26927,134517,0,134517,3912.4444386959076,0.020693991706054377
27027,135017,0,135017,3928.9311068058014,0.020645140488547858
27127,135517,0,135517,3942.8960959911346,0.020596535329722145
27227,136017,0,136017,3955.988848924637,0.020548173777362965
27327,136517,0,136517,3969.3295669555664,0.0205000534153299
27427,137017,0,137017,3982.509911775589,0.02045217186288995
27528,137522,0,137522,4002.5028450489044,0.020404051509468234
27628,138022,0,138022,4019.693542957306,0.02035664290235741
27728,138522,0,138522,4035.799248933792,0.02030946614602425
27828,139022,0,139022,4049.135593891144,0.020262518995318703
27928,139522,0,139522,4062.397782802582,0.020215799237376042
28028,140022,0,140022,4076.047504901886,0.020169304691034666
28128,140522,0,140522,4090.8753077983856,0.020123033206266266
28228,141022,0,141022,4105.253634929657,0.02007698266361863
28328,141522,0,141522,4118.593531847,0.02003115097367041
28428,142022,0,142022,4132.012501955032,0.01998553607649742
28529,142527,0,142527,4146.797644853592,0.01993968301754575
28629,143027,0,143027,4159.864371061325,0.019894497759117436
28729,143527,0,143527,4173.096580982208,0.019849523265905597
28829,144027,0,144027,4192.606646060944,0.01980475759113729
28929,144527,0,144527,4208.911221981049,0.01976019881503058
29029,145027,0,145027,4223.244927883148,0.019715845044325317
29129,145527,0,145527,4237.85560297966,0.019671694411823874
29229,146027,0,146027,4252.322020769119,0.019627745075941727
29329,146527,0,146527,4267.300783872604,0.019583995220266548
29429,147027,0,147027,4281.34526181221,0.019540443053127403
29530,147532,0,147532,4295.324011802673,0.019496654228195475
29630,148032,0,148032,4311.269765853882,0.019453494093028642
29730,148532,0,148532,4326.035781860352,0.019410526398567277
29830,149032,0,149032,4339.166349887848,0.01936774944819416
29930,149532,0,149532,4355.426744937897,0.019325161568001153
30030,150032,0,150032,4368.682328939438,0.0192827611064077
30130,150532,0,150532,4383.8657059669495,0.019240546433787326
30230,151032,0,151032,4397.069748878479,0.019198515942101216
30330,151532,0,151532,4410.050049781799,0.01915666804453937
30430,152032,0,152032,4423.111400842667,0.01911500117516862
30531,152537,0,152537,4436.278606891632,0.01907309981593275
30631,153037,0,153037,4456.402772903442,0.019031792158875335
30731,153537,0,153537,4471.444902896881,0.01899066093910085
30831,154037,0,154037,4488.370275735855,0.01894970467099488
30931,154537,0,154537,4504.540289878845,0.01890892188815806
31031,155037,0,155037,4519.899147987366,0.018868311143093695
31131,155537,0,155537,4535.248259782791,0.01882787100690095
31231,156037,0,156037,4550.9323189258575,0.018787600068974442
31331,156537,0,156537,4569.61999797821,0.018747496936709015
31431,157037,0,157037,4584.237385034561,0.018707560235210693
31532,157542,0,157542,4599.297220945358,0.018667391719801824
31632,158042,0,158042,4613.85847401619,0.018627785455204972
31732,158542,0,158542,4628.2091019153595,0.01858834158699828
31832,159042,0,159042,4646.012814760208,0.018549058808511803
31932,159542,0,159542,4662.45658493042,0.0185099358294176
32032,160042,0,160042,4679.039926767349,0.0184709713754715
32132,160542,0,160542,4692.881323099136,0.018432164188259957
32232,161042,0,161042,4706.196378946304,0.01839351302495138
32332,161542,0,161542,4719.370559930801,0.018355016658052243
32432,162042,0,162042,4732.771465063095,0.018316673875167538
32533,162547,0,162547,4746.5471959114075,0.018278102340338775
32633,163047,0,163047,4759.842113018036,0.01824006465363167
32733,163547,0,163547,4777.969171047211,0.018202176990402413
32833,164047,0,164047,4795.4258460998535,0.01816443819648226
32933,164547,0,164547,4814.262102842331,0.018126847131665447
33033,165047,0,165047,4832.705144882202,0.018089402669494978
33133,165547,0,165547,4847.444257736206,0.018052103697051465
33233,166047,0,166047,4860.538408994675,0.018014949114746843
33333,166547,0,166547,4873.884225130081,0.017977937836121154
33433,167047,0,167047,4887.096767902374,0.01794106878764295
33534,167552,0,167552,4900.351341724396,0.017903974339070337
33634,168052,0,168052,4913.354231834412,0.017867387976990452
33734,168552,0,168552,4926.283223867416,0.017830940689796432
33834,169052,0,169052,4940.268539905548,0.017794631453867293
33934,169552,0,169552,4953.855808019638,0.017758459257563333
34034,170052,0,170052,4967.848495960236,0.01772242310104717
34134,170552,0,170552,4982.223167896271,0.017686521996107273
34234,171052,0,171052,4995.872387886047,0.017650754965985373
34334,171552,0,171552,5009.0225076675415,0.017615121045206236
34434,172052,0,172052,5022.987432956696,0.01757961927941072
34535,172557,0,172557,5036.348809957504,0.01754389567910357
34635,173057,0,173057,5051.768779039383,0.01750865670196066
34735,173557,0,173557,5065.557888031006,0.01747354707262698
34835,174057,0,174057,5079.538151025772,0.017438565879698543
34935,174557,0,174557,5092.561466932297,0.017403712222093276
35035,175057,0,175057,5106.118617773056,0.017368985208900296
35135,175557,0,175557,5119.45906996727,0.01733438395923207
35235,176057,0,176057,5132.653561830521,0.01729990760207896
35335,176557,0,176557,5148.04207277298,0.017265555276166467
35435,177057,0,177057,5162.374044895172,0.01723132612981449
35536,177562,0,177562,5177.928067922592,0.017196878867686657
35636,178062,0,178062,5194.768429756165,0.017162894773974095
35736,178562,0,178562,5209.9944977760315,0.01712903135278741
35836,179062,0,179062,5225.215190887451,0.017095287789555744
35936,179562,0,179562,5238.336013793945,0.017061663278633687
36036,180062,0,180062,5251.6657338142395,0.01702815702317388
36136,180562,0,180562,5265.9399428367615,0.016994768235002625
36236,181062,0,181062,5284.2644629478455,0.016961496134496833
36336,181562,0,181562,5299.245818853378,0.016928339950463292
36436,182062,0,182062,5312.542953014374,0.016895298920020185
36537,182567,0,182567,5326.563638687134,0.016862043597346197
36637,183067,0,183067,5339.495131969452,0.016829231750880573
36737,183567,0,183567,5352.5287029743195,0.01679653281072208
36837,184067,0,184067,5366.93318104744,0.016763946046162676
36937,184567,0,184567,5381.473133802414,0.016731470734239515
37037,185067,0,185067,5394.607323884964,0.01669910615962714
37137,185567,0,185567,5407.707150936127,0.016666851614531842
37237,186067,0,186067,5421.348628997803,0.01663470639858739
37337,186567,0,186567,5434.490186929703,0.016602669818753087
37437,187067,0,187067,5447.700494766235,0.016570741189212392
37538,187572,0,187572,5460.95339179039,0.01653860215713823
37638,188072,0,188072,5473.7521867752075,0.016506888461770806
37738,188572,0,188572,5487.338315963745,0.01647528069499903
37838,189072,0,189072,5501.364946842194,0.016443778198997023
37938,189572,0,189572,5514.500148057938,0.016412380322682447
38038,190072,0,190072,5527.543098926544,0.016381086421625245
38138,190572,0,190572,5541.824126005173,0.01634989585795756
38238,191072,0,191072,5555.6445298194885,0.016318808000285154
38338,191572,0,191572,5570.4866898059845,0.016287822223600232
38438,192072,0,192072,5585.365421772003,0.016256937909195864
38539,192577,0,192577,5598.920983791351,0.016225847117169866
38639,193077,0,193077,5613.690835952759,0.01619516489538033
38739,193577,0,193577,5629.315346956253,0.016164582310744288
38839,194077,0,194077,5644.550004959106,0.01613409876898572
38939,194577,0,194577,5660.0046479702,0.01610371368171962
39039,195077,0,195077,5674.547621965408,0.016073426466373834
39139,195577,0,195577,5688.5592448711395,0.01604323654611205
39239,196077,0,196077,5703.5236558914185,0.01601314334975852
39339,196577,0,196577,5717.834055900574,0.015983146311723512
39439,197077,0,197077,5731.921963691711,0.015953244871929933
39540,197582,0,197582,5750.148716688156,0.015923140889886618
39640,198082,0,198082,5770.076623916626,0.01589342993022341
39740,198582,0,198582,5782.537007808685,0.015863812915517462
39840,199082,0,199082,5798.9937908649445,0.015834289307083964
39940,199582,0,199582,5814.733668804169,0.015804858571400248
40040,200082,0,200082,5826.63295006752,0.015775520180039016
40140,200582,0,200582,5837.680618047714,0.015746273609602627
40240,201082,0,201082,5848.406774044037,0.015717118341658398
40340,201582,0,201582,5860.883694887161,0.01568805386267456
40440,202082,0,202082,5871.830550670624,0.015659079663957663
40541,202587,0,202587,5980.4942400455475,0.015629906849044677
40641,203087,0,203087,6015.667729854584,0.015601112594092522
40741,203587,0,203587,6114.309729814529,0.01557240711682054
40841,204087,0,204087,8462.870710134506,0.015543789927324686
40941,204587,0,204587,8478.548333883286,0.015515260540238501
41041,205087,0,205087,8490.662370920181,0.015486818474675602
41141,205587,0,205587,8503.30750989914,0.015458463254173419
41241,206087,0,206087,8514.521641016006,0.015430194406637503
41341,206587,0,206587,8523.777676820755,0.015402011464286505
41441,207087,0,207087,8536.65109205246,0.015373913963598523
41542,207592,0,207592,8547.320729970932,0.015345621747691426
41642,208092,0,208092,8556.726190805435,0.015317694599522324
41742,208592,0,208592,8566.654465675354,0.01528985152298752
41842,209092,0,209092,8576.300031900406,0.01526209207111819
41942,209592,0,209592,8589.799907922745,0.015234415800945773
42042,210092,0,210092,8600.66377401352,0.015206822273453048
42142,210592,0,210592,8611.90098786354,0.01517931105352502
42242,211092,0,211092,8621.686147928238,0.015151881709901453
42342,211592,0,211592,8632.926278829575,0.015124533815129113
42442,212092,0,212092,8643.166986942291,0.015097266945515624
42543,212597,0,212597,8653.303467035294,0.015069809224083524
42643,213097,0,213097,8663.546886920929,0.015042703948323055
42743,213597,0,213597,8673.581441879272,0.015015678444644109
42843,214097,0,214097,8684.581675052643,0.014988732303980259
42943,214597,0,214597,8695.264791727066,0.014961865120802649
43043,215097,0,215097,8706.205473899841,0.014935076493077156
43143,215597,0,215597,8716.964755058289,0.014908366022222253
43243,216097,0,216097,8727.35228395462,0.014881733313067844
43343,216597,0,216597,8737.118810892105,0.014855177973814119
43443,217097,0,217097,8748.437743902206,0.014828699615991578
43544,217602,0,217602,8758.989706993103,0.014802034222321552
43644,218102,0,218102,8768.638134002686,0.014775709435300896
43744,218602,0,218602,8778.854786872864,0.014749460480118768
43844,219102,0,219102,8790.55037689209,0.0147232869812667
43944,219602,0,219602,8802.799507856369,0.014697188566373151
44044,220102,0,220102,8812.342067956924,0.014671164866166667
44144,220602,0,220602,8821.702325105667,0.014645215514439392
44244,221102,0,221102,8831.326150894165,0.014619340148011173
44344,221602,0,221602,8840.806788921356,0.01459353840669427
44444,222102,0,222102,8850.518721103668,0.014567809933258246
44545,222607,0,222607,8860.03893995285,0.014541898184819248
44645,223107,0,223107,8869.607310771942,0.01451631591096859
44745,223607,0,223607,8879.940785884857,0.014490805847239295
44845,224107,0,224107,8890.661899089813,0.01446536764791936
44945,224607,0,224607,8900.345633745193,0.014440000970086792
45045,225107,0,225107,8910.384489059448,0.014414705473577092
45145,225607,0,225607,8920.296431779861,0.014389480820952032
45245,226107,0,226107,8930.53647685051,0.014364326677468316
45345,226607,0,226607,8940.612289905548,0.014339242711046633
45445,227107,0,227107,8951.079374790192,0.014314228592241771
45546,227612,0,227612,8961.427661895752,0.014289034898212531
45646,228112,0,228112,8971.977705001831,0.01426416018702744
45746,228612,0,228612,8982.57979297638,0.014239354347424453
45846,229112,0,229112,8991.973784923553,0.014214617060223608
45946,229612,0,229612,9001.40749502182,0.014189948008732791
46046,230112,0,230112,9010.779054880142,0.014165346878720174
46146,230612,0,230612,9020.4052298069,0.014140813358386344
46246,231112,0,231112,9029.789062976837,0.014116347138337447
46346,231612,0,231612,9038.98078083992,0.014091947911558225
46446,232112,0,232112,9049.335260868073,0.014067615373385564
46547,232617,0,232617,9063.075752973557,0.01404310689419705
46647,233117,0,233117,9076.069846868515,0.014018907487881985
46747,233617,0,233617,9085.790934801102,0.013994773867072288
46847,234117,0,234117,9096.873322963715,0.013970705736278823
46947,234617,0,234617,9107.707082986832,0.013946702802237558
47047,235117,0,235117,9118.63350391388,0.013922764773885177
47147,235617,0,235617,9128.700438022614,0.013898891362334923
47247,236117,0,236117,9139.862745761871,0.013875082280853107
47347,236617,0,236617,9150.109851837158,0.013851337244835636
47447,237117,0,237117,9159.630943059921,0.013827655971784755
47548,237622,0,237622,9169.623924970627,0.013803802323024887
47648,238122,0,238122,9179.314591884613,0.013780248367369756
47748,238622,0,238622,9189.516897678375,0.013756757336847912
47848,239122,0,239122,9199.453819990158,0.01373332895718288
47948,239622,0,239622,9209.531202793121,0.013709962956093497
48048,240122,0,240122,9219.181861877441,0.013686659063272712
48148,240622,0,240622,9228.894155979156,0.013663417010366425
48248,241122,0,241122,9238.673070907593,0.01364023653095287
48348,241622,0,241622,9248.462516069412,0.013617117360522103
48448,242122,0,242122,9259.434008836746,0.013594059236455555
48549,242627,0,242627,9270.479694843292,0.013570832230711864
48649,243127,0,243127,9281.913579702377,0.013547896022951412
48749,243627,0,243627,9293.315866947174,0.013525020082289785
48849,244127,0,244127,9305.835292816162,0.01350220415349594
48949,244627,0,244627,9315.83553481102,0.013479447983133096
49049,245127,0,245127,9327.18855881691,0.013456751319540033
49149,245627,0,245627,9340.198323965073,0.013434113912812476
49249,246127,0,246127,9351.889665842056,0.013411535514785296
49349,246627,0,246627,9363.710286855698,0.013389015879013984
49449,247127,0,247127,9375.097569704056,0.013366554760757455
49550,247632,0,247632,9386.244505882263,0.013343928181989996
49650,248132,0,248132,9397.081467866898,0.013321583950381998
49750,248632,0,248632,9409.173973083496,0.013299297509721149
49850,249132,0,249132,9419.769766807556,0.013277068621922374
49950,249632,0,249632,9430.282648801804,0.013254897050518232
50050,250132,0,250132,9441.471932888031,0.013232782560642654
50150,250632,0,250632,9452.255786895752,0.013210724919014412
50250,251132,0,251132,9463.111022949219,0.013188723893921499
50350,251632,0,251632,9473.654136896133,0.013166779255205102
50450,252132,0,252132,9484.40483379364,0.013144890774244073
50551,252637,0,252637,9495.40102982521,0.013122840180121564
50651,253137,0,253137,9506.44905090332,0.013101063890797796
50751,253637,0,253637,9517.493181943893,0.013079343080205072
50851,254137,0,254137,9527.247332811356,0.013057677525735313
50951,254637,0,254637,9536.703794956207,0.01303606700624295
51051,255137,0,255137,9546.241921901703,0.013014511302030145
51151,255637,0,255637,9555.758731126785,0.0129930101948329
51251,256137,0,256137,9565.529066085815,0.012971563467806608
51351,256637,0,256637,9574.995750904083,0.012950170905512329
51451,257137,0,257137,9584.98644208908,0.012928832293903073
51552,257642,0,257642,9594.834426879883,0.012907334842234943
51652,258142,0,258142,9604.41866183281,0.012886104029558693
51752,258642,0,258642,9614.154953956604,0.012864926531549642
51852,259142,0,259142,9623.658471822739,0.012843802139607324
51952,259642,0,259642,9633.586021900177,0.012822730646456703
52052,260142,0,260142,9645.739177942276,0.012801711846135494
52152,260642,0,260642,9656.986498832703,0.012780745533981574
52252,261142,0,261142,9667.616150856018,0.01275983150662033
52352,261642,0,261642,9678.139098882675,0.012738969561952617
52452,262142,0,262142,9688.14860701561,0.012718159499142416
52553,262647,0,262647,9698.389791965485,0.012697193795122888
52653,263147,0,263147,9708.687941789627,0.012676487412354482
52753,263647,0,263647,9718.845253944397,0.012655832314430389
52853,264147,0,264147,9728.714332818985,0.012635228305461002
52953,264647,0,264647,9740.06717801094,0.012614675190761109
53053,265147,0,265147,9749.807730913162,0.012594172776838702
53153,265647,0,265647,9759.459573030472,0.012573720871383866
53253,266147,0,266147,9769.20603299141,0.012553319283257768
53353,266647,0,266647,9778.770887851715,0.012532967822481577
53453,267147,0,267147,9788.293083906174,0.012512666300225964
53554,267652,0,267652,9798.461561918259,0.0124922122616956
53654,268152,0,268152,9809.273385047913,0.012472010549241996
53754,268652,0,268652,9819.720811128616,0.012451858213762679
53854,269152,0,269152,9829.896369934082,0.012431755070931843
53954,269652,0,269652,9841.372262954712,0.012411700937521041
54054,270152,0,270152,9851.040782928467,0.012391695631389314
54154,270652,0,270652,9861.472233057022,0.012371738971472954
54254,271152,0,271152,9871.528511047363,0.012351830777776155
54354,271652,0,271652,9881.639705896378,0.012331970871361097
54454,272152,0,272152,9891.533362865448,0.012312159074338453
54555,272657,0,272657,9902.298974990845,0.012292197812676754
54655,273157,0,273157,9912.802681922913,0.012272482181600725
54755,273657,0,273657,9922.16532588005,0.012252814130703515
54855,274157,0,274157,9931.523387908936,0.012233193486206616
54955,274657,0,274657,9941.04154586792,0.01221362007533396
55055,275157,0,275157,9950.810774087906,0.012194093726302781
55155,275657,0,275657,9961.264544963837,0.012174614268315105
55255,276157,0,276157,9971.24548983574,0.012155181531548763
55355,276657,0,276657,9981.108448028564,0.012135795347149092
55455,277157,0,277157,9990.698747873306,0.012116455547220285
55556,277662,0,277662,10000.510905742645,0.012096969261828967
55656,278162,0,278162,10010.250191926956,0.012077722190628097
55756,278662,0,278662,10020.198305130005,0.012058521004234522
55856,279162,0,279162,10029.852886676788,0.012039365538514214
55956,279662,0,279662,10040.266149997711,0.012020255630250977
56056,280162,0,280162,10049.796983718872,0.012001191117138554
56156,280662,0,280662,10059.662708997726,0.011982171837772702
56256,281162,0,281162,10069.092726707458,0.011963197631643505
56356,281662,0,281662,10078.742745876312,0.011944268339127729
56456,282162,0,282162,10088.130006790161,0.011925383801481315
56557,282667,0,282667,10097.623077869415,0.011906355686108048
56657,283167,0,283167,10106.969592809677,0.011887560629056925
56757,283667,0,283667,10117.104251861572,0.011868809854285914
56857,284167,0,284167,10128.098474025726,0.011850103206501834
56957,284667,0,284667,10138.67577290535,0.011831440531254036
57057,285167,0,285167,10151.567501783371,0.011812821674927346
57157,285667,0,285667,10162.390696048737,0.011794246484734911
57257,286167,0,286167,10173.01578593254,0.011775714808711491
57357,286667,0,286667,10184.410044908524,0.011757226495706576
57457,287167,0,287167,10194.92893910408,0.011738781395377575
57558,287672,0,287672,10205.336720943451,0.011720195554776075
57658,288172,0,288172,10216.433094978333,0.011701836860364911
57758,288672,0,288672,10226.771605968475,0.011683520930907548
57858,289172,0,289172,10237.523194789886,0.011665247619234901
57958,289672,0,289672,10248.265272855759,0.011647016778953086
58058,290172,0,290172,10257.995198965073,0.011628828264437282
58158,290672,0,290672,10267.64555978775,0.011610681930825262
58258,291172,0,291172,10277.806315660477,0.011592577634011208
58358,291672,0,291672,10289.835191726685,0.011574515230639765
58458,292172,0,292172,10300.367659807205,0.011556494578099982
58559,292677,0,292677,10311.139449834824,0.011538335953730394
58659,293177,0,293177,10320.948433876038,0.011520398791936125
58759,293677,0,293677,10330.873176813126,0.011502502956146488
58859,294177,0,294177,10341.18550491333,0.011484648306675909
58959,294677,0,294677,10351.21304678917,0.011466834704553803
59059,295177,0,295177,10361.330662965775,0.011449062011518962
59159,295677,0,295677,10371.81419301033,0.011431330090014059
59259,296177,0,296177,10382.624109745026,0.011413638803179929
59359,296677,0,296677,10393.03354382515,0.011395988014850231
59459,297177,0,297177,10403.236515760422,0.011378377589545999
59560,297682,0,297682,10414.537937879562,0.011360631893197696
59660,298182,0,298182,10424.552181959152,0.011343102190496137
59760,298682,0,298682,10434.73710489273,0.011325612447122808
59860,299182,0,299182,10444.900592803955,0.01130816253030177
59960,299682,0,299682,10456.019409894943,0.011290752307918168
60060,300182,0,300182,10465.937663078308,0.011273381648513173
60160,300682,0,300682,10475.393593788147,0.011256050421278814
60260,301182,0,301182,10485.239919900894,0.011238758496053363
60360,301682,0,301682,10495.174738883972,0.011221505743315869
60460,302182,0,302182,10505.711631774902,0.011204292034181855
60561,302687,0,302687,10515.210540771484,0.011186945688550458
60661,303187,0,303187,10524.639120817184,0.011169810069725263
60761,303687,0,303687,10534.51963186264,0.011152713110352302
60861,304187,0,304187,10544.810466766357,0.011135654684050271
60961,304687,0,304687,10554.497265815735,0.0111186346650506
61061,305187,0,305187,10564.095353841782,0.011101652928192663
61161,305687,0,305687,10573.61340379715,0.011084709348919355
61261,306187,0,306187,10583.305442810059,0.011067803803272592
61361,306687,0,306687,10593.345868825912,0.011050936167888823
61461,307187,0,307187,10603.586822986603,0.011034106319994894
61562,307692,0,307692,10613.463243961334,0.011017146405375251
61662,308192,0,308192,10623.480993032455,0.011000392141305071
61762,308692,0,308692,10633.266429901123,0.010983675298695589
61862,309192,0,309192,10643.514310836792,0.01096699575709726
61962,309692,0,309692,10657.100888729095,0.01095035339662931
62062,310192,0,310192,10669.566437959671,0.010933748097975846
62162,310692,0,310692,10681.027782917023,0.01091717974238177
62262,311192,0,311192,10691.426622867584,0.010900648211648588
62362,311692,0,311692,10701.616724014282,0.010884153388130622
62462,312192,0,312192,10711.930752038956,0.010867695154730812
62563,312697,0,312697,10722.40866279602,0.010851109361097273
62663,313197,0,313197,10733.002998113632,0.010834724321809909
62763,313697,0,313697,10743.46959900856,0.010818375523451294
62863,314197,0,314197,10753.475327014923,0.010802062851086045
62963,314697,0,314697,10763.40349984169,0.010785786190308306
63063,315197,0,315197,10773.309302091599,0.010769545427238037
63163,315697,0,315697,10783.368887901306,0.010753340448517331
63263,316197,0,316197,10794.259662866592,0.010737171141306746
63363,316697,0,316697,10804.783824920654,0.010721037393281787
63463,317197,0,317197,10816.469074010849,0.010704939092629151
63564,317702,0,317702,10826.451053857803,0.010688715676469408
63664,318202,0,318202,10837.714394807816,0.010672688288844195
63764,318702,0,318702,10848.224430799484,0.010656696015083776
63864,319202,0,319202,10859.21707701683,0.010640738745390092
63964,319702,0,319702,10869.950998783112,0.010624816370458944
64064,320202,0,320202,10880.611844778061,0.010608928781476753
64164,320702,0,320702,10891.909802913666,0.010593075870117026
64264,321202,0,321202,10902.584411859512,0.010577257528537401
64364,321702,0,321702,10912.320845842361,0.010561473649376006
64464,322202,0,322202,10923.036822795868,0.010545724125748446
64565,322707,0,322707,10934.3197119236,0.010529851871098747
64665,323207,0,323207,10945.217736005783,0.010514171080677709
64765,323707,0,323707,10956.440607070923,0.010498524326917459
64865,324207,0,324207,10967.028987884521,0.010482911504816192
64965,324707,0,324707,10976.864063978195,0.01046733250983362
65065,325207,0,325207,10986.665052890778,0.010451787237888107
65165,325707,0,325707,10996.565737009048,0.010436275585353615
65265,326207,0,326207,11006.542742013931,0.010420797449056666
65365,326707,0,326707,11017.005421876907,0.010405352726273402
65465,327207,0,327207,11026.658280849457,0.010389941314726632
65566,327712,0,327712,11036.28273177147,0.010374409497925577
65666,328212,0,328212,11045.669867753983,0.010359064734361963
65766,328712,0,328712,11055.943378925323,0.010343752976846966
65866,329212,0,329212,11066.218785762787,0.010328474124865645
65966,329712,0,329712,11075.997896909714,0.01031322807833529
66066,330212,0,330212,11086.437386989594,0.010298014737602838
66166,330712,0,330712,11096.32517194748,0.010282834003442078
66266,331212,0,331212,11106.033344984055,0.010267685777050832
66366,331712,0,331712,11116.07791185379,0.01025256996004845
66466,332212,0,332212,11126.196492910385,0.010237486454472896
66567,332717,0,332717,11137.560546875,0.010222284812212408
66667,333217,0,333217,11151.138458967209,0.010207265957944597
66767,333717,0,333717,11162.646119832993,0.010192279122738455
66867,334217,0,334217,11172.585657835007,0.010177324210284857
66967,334717,0,334717,11182.68602180481,0.010162401124680144
67067,335217,0,335217,11193.12596487999,0.01014750977042398
67167,335717,0,335717,11205.460018873215,0.010132650052416637
67267,336217,0,336217,11217.020622968674,0.01011782187595667
67367,336717,0,336717,11226.686923980713,0.01010302514673816
67467,337217,0,337217,11237.22343492508,0.010088259770848646
67568,337722,0,337722,11248.542474985123,0.01007337847115224
67668,338222,0,338222,11258.748418807983,0.010058675832941918
67768,338722,0,338722,11269.115036010742,0.010044004267733175
67868,339222,0,339222,11279.634219884872,0.010029363683166441
67968,339722,0,339722,11290.17475104332,0.010014753987263647
68068,340222,0,340222,11301.393749952316,0.010000175088425746
68168,340722,0,340722,11312.228873968124,0.009985626895430482
68268,341222,0,341222,11322.344904899597,0.00997110931743021
68368,341722,0,341722,11332.638699054718,0.009956622263949484
68468,342222,0,342222,11343.332186937332,0.009942165644882985
68569,342727,0,342727,11353.892427921295,0.009927595260687146
68669,343227,0,343227,11364.123274087906,0.009913199543705072
68769,343727,0,343727,11374.355710029602,0.009898833992131227
68869,344227,0,344227,11384.912506818771,0.009884498517322133
68969,344727,0,344727,11396.370728969574,0.009870193030993572
69069,345227,0,345227,11406.558943033218,0.009855917445218387
69169,345727,0,345727,11416.597603797913,0.009841671672424392
69269,346227,0,346227,11426.747312784195,0.009827455625392278
69369,346727,0,346727,11437.085006952286,0.009813269217253612
69469,347227,0,347227,11448.138040781021,0.009799112361488766
69570,347732,0,347732,11458.04262304306,0.00978484384654294
69670,348232,0,348232,11467.934571027756,0.00977074613072348
69770,348732,0,348732,11478.979167938232,0.009756677708938531
69870,349232,0,349232,11488.632525920868,0.009742638496047024
69970,349732,0,349732,11498.18231511116,0.009728628407246753
70070,350232,0,350232,11508.97919178009,0.009714647358072485
70170,350732,0,350732,11520.734184980392,0.009700695264393818
70270,351232,0,351232,11532.754180908203,0.009686772042413642
70370,351732,0,351732,11543.24861907959,0.009672877608665807
70470,352232,0,352232,11555.67118191719,0.009659011880013748
70571,352737,0,352737,11566.945377111435,0.00964503654684775
70671,353237,0,353237,11577.863404750824,0.009631228265267692
70771,353737,0,353737,11587.745622873306,0.009617448440510861
70871,354237,0,354237,11597.881050825119,0.009603696990742629
70971,354737,0,354737,11607.897282838821,0.00958997383444859
71071,355237,0,355237,11618.466060876846,0.009576278890432836
71171,355737,0,355737,11630.501217126846,0.009562612077815969
71271,356237,0,356237,11641.333519935608,0.009548973316033592
71371,356737,0,356737,11652.32924079895,0.00953536252483438
71471,357237,0,357237,11663.648709774017,0.009521779624278486
71572,357742,0,357742,11674.483215808868,0.009508089124017292
71672,358242,0,358242,11683.940743923187,0.009494562043083053
71772,358742,0,358742,11694.419682741165,0.009481062614035508
71872,359242,0,359242,11704.739424943924,0.009467590758166729
71972,359742,0,359742,11858.060126066208,0.009454146397071614
72072,360242,0,360242,11870.410477876663,0.00944072945264662
72172,360742,0,360742,11880.718903779984,0.009427339847087882
72272,361242,0,361242,11890.213956832886,0.009413977502889696
72372,361742,0,361742,11900.395734786987,0.009400642342842902
72472,362242,0,362242,11912.137720823288,0.009387334290033298
72573,362747,0,362747,11922.545905828476,0.009373920593864169
72673,363247,0,363247,11933.32832288742,0.009360666795116655
72773,363747,0,363747,11946.424739837646,0.00934743987385884
72873,364247,0,364247,11959.48798084259,0.009334239754343675
72973,364747,0,364747,11970.289983034134,0.009321066361111194
73073,365247,0,365247,11980.020337820053,0.00930791961898726
73173,365747,0,365747,11989.362310886383,0.009294799453081844
73273,366247,0,366247,11999.604336977005,0.00928170578878762
73373,366747,0,366747,12009.886146783829,0.009268638551778471
73473,367247,0,367247,12020.363102912903,0.009255597668008087
73574,367752,0,367752,12032.291608810425,0.0092424530501279
73674,368252,0,368252,12044.373602867126,0.0092294649134975
73774,368752,0,368752,12054.628666877747,0.009216502908900139
73874,369252,0,369252,12064.524953842163,0.009203566963396942
73974,369752,0,369752,12074.676825761795,0.009190657004321437
74074,370252,0,370252,12084.651273965836,0.009177772959278449
74174,370752,0,370752,12094.500089883804,0.009164914756142605
74274,371252,0,371252,12104.051033973694,0.009152082323056926
74374,371752,0,371752,12113.583316087723,0.009139275588431556
74474,372252,0,372252,12123.17876291275,0.009126494480942193
74575,372757,0,372757,12133.364844799042,0.009113611502833364
74675,373257,0,373257,12143.433889865875,0.009100881691195857
74775,373757,0,373757,12153.24691581726,0.00908817729359864
74875,374257,0,374257,12162.93075799942,0.009075498239769579
74975,374757,0,374757,12172.653393983841,0.009062844459695595
75075,375257,0,375257,12182.241153001785,0.009050215883621465
75175,375757,0,375757,12192.114384889603,0.009037612442048298
75275,376257,0,376257,12201.910492897034,0.009025034065732537
75375,376757,0,376757,12211.556963920593,0.009012480685684554
75475,377257,0,377257,12223.015185832977,0.008999952233167345
75576,377762,0,377762,12233.967998981476,0.00898732372906778
75676,378262,0,378262,12244.232633829117,0.008974845173970078
75776,378762,0,378762,12253.928231954575,0.00896239134101734
75876,379262,0,379262,12263.73308801651,0.008949962162473353
75976,379762,0,379762,12273.298439979553,0.008937557570848572
76076,380262,0,380262,12282.897511005402,0.008925177498898616
76176,380762,0,380762,12292.453680992126,0.008912821879623369
76276,381262,0,381262,12303.155387878418,0.008900490646265528
76376,381762,0,381762,12312.657185792923,0.008888183732309636
76476,382262,0,382262,12322.564269781113,0.008875901071480823
76577,382767,0,382767,12334.046644926071,0.008863520134928261
76677,383267,0,383267,12344.250470876694,0.00885128602336697
76777,383767,0,383767,12354.353832960129,0.00883907596688567
76877,384267,0,384267,12365.246877908707,0.008826889900162714
76977,384767,0,384767,12375.282857894897,0.00881472775811127
77077,385267,0,385267,12385.18101477623,0.008802589475878288
77177,385767,0,385767,12395.753201007843,0.008790474988843324
77277,386267,0,386267,12406.077651977539,0.008778384232617462
77377,386767,0,386767,12415.72970199585,0.008766317143042213
77477,387267,0,387267,12426.66630411148,0.008754273656188475
77578,387772,0,387772,12437.256542921066,0.008742133627534144
77678,388272,0,388272,12447.806750059128,0.008730137389683685
77778,388772,0,388772,12458.746620893478,0.008718164563501302
77878,389272,0,389272,12469.348270893097,0.008706215085966727
77978,389772,0,389772,12479.718670845032,0.008694288894283768
78078,390272,0,390272,12489.988988876343,0.00868238592587914
78178,390772,0,390772,12500.18431186676,0.008670506118401441
78278,391272,0,391272,12510.168486833572,0.008658649409720299
78378,391772,0,391772,12521.988092899323,0.00864681573792507
78478,392272,0,392272,12532.61269569397,0.008635005041324043
78579,392777,0,392777,12542.731447696686,0.008623099496121365
78679,393277,0,393277,12552.61932182312,0.008611334793919933
78779,393777,0,393777,12561.961922883987,0.008599592882531265
78879,394277,0,394277,12574.220978021622,0.008587873701131213
78979,394777,0,394777,12591.14508485794,0.008576177189109406
79079,395277,0,395277,12602.095505952835,0.00856450328606849
79179,395777,0,395777,12612.612853050232,0.00855285193182291
79279,396277,0,396277,12625.271368980408,0.00854122306639819
79379,396777,0,396777,12637.811251878738,0.008529616630029812
79479,397277,0,397277,12648.869386911392,0.00851803256316229
79580,397782,0,397782,12660.23443889618,0.008506355301347166
79680,398282,0,398282,12671.577410936356,0.008494816017858713
79780,398782,0,398782,12681.931404829025,0.008483298925861395
79880,399282,0,399282,12694.247112989426,0.008471803966628642
79980,399782,0,399782,12703.817835092545,0.008460331081638335
80080,400282,0,400282,12713.264189958572,0.008448880212571787
80180,400782,0,400782,12723.853051900864,0.0084374513013129
80280,401282,0,401282,12733.579011917114,0.008426044289947223
80380,401782,0,401782,12743.502896785736,0.00841465912076111
80480,402282,0,402282,12753.524314880371,0.008403295736240804
80581,402787,0,402787,12763.415397882462,0.008391840772029537
80681,403287,0,403287,12773.16028380394,0.008380521001509248
80781,403787,0,403787,12783.206682920456,0.008369222843735764
80881,404287,0,404287,12794.610837936401,0.008357946241988035
80981,404787,0,404787,12806.897563934326,0.008346691139740556
81081,405287,0,405287,12818.268851041794,0.008335457480662466
81181,405787,0,405787,12829.871589899063,0.008324245208616701
81281,406287,0,406287,12841.061709880829,0.008313054267659136
81381,406787,0,406787,12851.428687810898,0.008301884602037818
81481,407287,0,407287,12861.72916483879,0.008290736156192073
81582,407792,0,407792,12872.992948055267,0.00827949770863063
81682,408292,0,408292,12883.369881868362,0.00826839174722913
81782,408792,0,408792,12895.631880044937,0.008257306839511638
81882,409292,0,409292,12906.072833061218,0.008246242930676172
81982,409792,0,409792,12917.561244010925,0.008235199966108064
82082,410292,0,410292,12928.737320899963,0.008224177891378928
82182,410792,0,410792,12940.106654882431,0.008213176652245989
82282,411292,0,411292,12951.685611009598,0.008202196194651235
82382,411792,0,411792,12961.962002038956,0.00819123646472067
82482,412292,0,412292,12972.195574045181,0.008180297408763517
82583,412797,0,412797,12982.069355010986,0.008169269892869238
82683,413297,0,413297,12992.01236486435,0.008158372229918127
82783,413797,0,413797,13001.890798807144,0.008147495080428932
82883,414297,0,414297,13012.753487825394,0.008136638391437702
82983,414797,0,414797,13023.096176862717,0.008125802110159891
83083,415297,0,415297,13034.685487985611,0.008114986183989498
83183,415797,0,415797,13045.602393865585,0.008104190560498365
83283,416297,0,416297,13056.647297143936,0.00809341518743536
83383,416797,0,416797,13067.446592092514,0.008082660012725782
83483,417297,0,417297,13077.734493970871,0.008071924984470532
83584,417802,0,417802,13087.33752989769,0.008061103002913819
83684,418302,0,418302,13098.572657823563,0.008050408312740509
83784,418802,0,418802,13109.415833950043,0.008039733613857488
83884,419302,0,419302,13120.74457192421,0.00802907885506238
83984,419802,0,419802,13131.119787693024,0.008018443985324891
84084,420302,0,420302,13141.35398197174,0.00800782895378588
84184,420802,0,420802,13152.292392969131,0.00799723370975684
84284,421302,0,421302,13165.624024868011,0.007986658202718997
84384,421802,0,421802,13176.336890935898,0.007976102382322723
84484,422302,0,422302,13188.248998880386,0.00796556619838685
84585,422807,0,422807,13198.215997934341,0.007954944533665867
84685,423307,0,423307,13207.83170390129,0.007944447667892422
84785,423807,0,423807,13217.324961900711,0.007933970288543597
84885,424307,0,424307,13227.471884727478,0.007923512346106694
84985,424807,0,424807,13239.36557173729,0.007913073791234043
85085,425307,0,425307,13250.704677820206,0.00790265457474222
85185,425807,0,425807,13260.59997177124,0.007892254647611542
85285,426307,0,426307,13270.823391914368,0.007881873960985272
85385,426807,0,426807,13282.479831695557,0.007871512466168936
85485,427307,0,427307,13292.75188589096,0.007861170114629865
85586,427812,0,427812,13304.172152757645,0.007850743721695924
85686,428312,0,428312,13314.584637880325,0.007840439701980386
85786,428812,0,428812,13324.330173969269,0.007830154680427536
85886,429312,0,429312,15087.304672002792,0.007819888609146272
85986,429812,0,429812,15095.892345905304,0.007809641440404051
86086,430312,0,430312,15104.568359851837,0.0077994131266259144
86186,430812,0,430812,15113.906498908997,0.0077892036203942
86286,431312,0,431312,15122.520075082779,0.007779012874447677
86386,431812,0,431812,15131.858960866928,0.007768840841681057
86486,432312,0,432312,15142.028854846954,0.007758687475144215
86587,432817,0,432817,15155.241741895676,0.007748451474440908
86687,433317,0,433317,15461.041640043259,0.00773833548562429
86787,433817,0,433817,15472.429379940033,0.007728238022648513
86887,434317,0,434317,15481.12131690979,0.0077181590391798074
86987,434817,0,434817,15490.189616918564,0.007708098489036773
87087,435317,0,435317,15499.855998039246,0.007698056326189408
87187,435817,0,435817,15509.65214395523,0.007688032504758776
87287,436317,0,436317,15518.601984977722,0.007678026979016267
87387,436817,0,436817,15531.033084869385,0.007668039703383057
87487,437317,0,437317,15542.000818014145,0.00765807063242958
87588,437822,0,437822,15553.572204828262,0.0076480203033114065
87688,438322,0,438322,15563.030554771423,0.007638087686937562
87788,438822,0,438822,15572.761148929596,0.007628173139394758
87888,439322,0,439322,15582.102011919022,0.007618276615845734
87988,439822,0,439822,15591.982543945312,0.007608398071599532
88088,440322,0,440322,15601.266079902649,0.007598537462110887
88188,440822,0,440822,16824.69021987915,0.007588694742979678
88288,441322,0,441322,16833.946037054062,0.007578869869950294
88388,441822,0,441822,16842.3015229702,0.007569062798911131
88488,442322,0,442322,16850.672110795975,0.007559273485894136
88589,442827,0,442827,16860.1533100605,0.007549404260394502
88689,443327,0,443327,16869.99819803238,0.007539650508573227
88789,443827,0,443827,16880.72551393509,0.007529914383289964
88889,444327,0,444327,16890.48481988907,0.0075201958411461635
88989,444827,0,444827,16899.928216934204,0.007510494838883947
89089,445327,0,445327,17370.99649000168,0.007500811333385456
89189,445827,0,445827,17380.454955101013,0.007491145281672662
89289,446327,0,446327,17388.93695998192,0.007481496640906325
89389,446827,0,446827,17397.431469917297,0.007471865368385775
89489,447327,0,447327,17406.18833589554,0.0074622514215483765
89590,447832,0,447832,17415.450124025345,0.007452558878470288
89690,448332,0,448332,17424.941165924072,0.007442979628056925
89790,448832,0,448832,17435.632968902588,0.007433417576040308
89890,449332,0,449332,17445.69460296631,0.0074238726804056925
89990,449832,0,449832,17455.73383307457,0.007414344899273755
90090,450332,0,450332,17466.071660757065,0.00740483419089985
90190,450832,0,450832,17476.645174741745,0.007395340513673718
90290,451332,0,451332,17486.81414294243,0.007385863826118839
90390,451832,0,451832,17495.84269595146,0.00737640408689199
90490,452332,0,452332,17505.84803891182,0.007366961254782764
90591,452837,0,452837,17515.66375684738,0.0073574411140870585
90691,453337,0,453337,17525.394073963165,0.007348032141154787
90791,453837,0,453837,17535.555070877075,0.007338639952092819
90891,454337,0,454337,17545.49502801895,0.007329264506218072
90991,454837,0,454837,17554.885261774063,0.0073199057629777225
91091,455337,0,455337,17564.64334177971,0.007310563681948621
91191,455837,0,455837,17574.296652793884,0.007301238222837031
91291,456337,0,456337,17583.75923895836,0.007291929345477963
91391,456837,0,456837,17593.51507472992,0.007282637009834631
91491,457337,0,457337,17603.02508497238,0.007273361175998208
91592,457842,0,457842,17612.72210097313,0.0072640092934679315
91692,458342,0,458342,17622.229910850525,0.007254766508051344
91792,458842,0,458842,17631.57049393654,0.007245540105082393
91892,459342,0,459342,17641.12450194359,0.007236330045159958
91992,459842,0,459842,17650.448009967804,0.0072271362890082265
92092,460342,0,460342,17660.037187814713,0.007217958797476529
92192,460842,0,460842,17669.44623374939,0.0072087975315385
92292,461342,0,461342,17678.822188854218,0.007199652452291912
92392,461842,0,461842,17688.17142391205,0.007190523520958018
92492,462342,0,462342,17697.514234781265,0.0071814106988812455
92593,462847,0,462847,17707.074559926987,0.007172223061042053
92693,463347,0,463347,17716.44420981407,0.007163142502132242
92793,463847,0,463847,17726.087445020676,0.007154077936864347
92893,464347,0,464347,17735.72278571129,0.0071450293270718425
92993,464847,0,464847,17747.433388710022,0.007135996634708912
93093,465347,0,465347,17757.99951696396,0.0071269798218501655
93193,465847,0,465847,17768.26766705513,0.00711797885069003
93293,466347,0,466347,17778.4398458004,0.007108993683542557
93393,466847,0,466847,17790.06019592285,0.007100024282840741
93493,467347,0,467347,17801.919726848602,0.007091070611136209
93594,467852,0,467852,17813.336525917053,0.007082043330415176
93694,468352,0,468352,17825.16347503662,0.007073121161189108
93794,468852,0,468852,17834.8581738472,0.007064214608951908
93894,469352,0,469352,17844.179510831833,0.007055323636726295
93994,469852,0,469852,17853.6309838295,0.007046448207651482
94094,470352,0,470352,17863.161146879196,0.007037588284982597
94194,470852,0,470852,17874.401653051376,0.007028743832090383
94294,471352,0,471352,17884.576715946198,0.0070199148124606295
94394,471852,0,471852,17894.132405996323,0.007011101189693909
94494,472352,0,472352,17905.13010287285,0.007002302927505031
94595,472857,0,472857,17915.84119772911,0.006993432237611076
94695,473357,0,473357,17926.112967014313,0.00698466474087926
94795,473857,0,473857,17936.278655052185,0.00697591249619243
94895,474357,0,474357,17945.845795869827,0.006967175467719562
94995,474857,0,474857,17955.441718816757,0.006958453619741743
95095,475357,0,475357,17965.01329112053,0.006949746916651864
95195,475857,0,475857,17974.588701963425,0.006941055322954289
95295,476357,0,476357,17984.068623781204,0.006932378803264259
95395,476857,0,476857,17993.701808929443,0.006923717322307627
95495,477357,0,477357,18003.255145072937,0.006915070844920406
95596,477862,0,477862,18012.97402191162,0.006906353096432363
95696,478362,0,478362,18022.504853963852,0.006897736670290314
95796,478862,0,478862,18032.14077591896,0.006889135142534957
95896,479362,0,479362,18041.745065927505,0.006880548478440099
95996,479862,0,479862,18051.30794596672,0.006871976643387665
96096,480362,0,480362,18060.829210996628,0.006863419602867391
96196,480862,0,480862,18070.32433271408,0.0068548773224764385
96296,481362,0,481362,18079.94973707199,0.006846349767918926
96396,481862,0,481862,18089.555818080902,0.006837836905005648
96496,482362,0,482362,18099.007297754288,0.006829338699653576
96597,482867,0,482867,18109.5432677269,0.006820770355802233
96697,483367,0,483367,18119.607299804688,0.006812301509472928
96797,483867,0,483867,18129.147530078888,0.006803847218752175
96897,484367,0,484367,18138.62798690796,0.006795407449979118
96997,484867,0,484867,18148.823266744614,0.0067869821695972134
97097,485367,0,485367,18158.723965883255,0.0067785713441538
97197,485867,0,485867,18168.208043813705,0.006770174940299822
97297,486367,0,486367,18178.21631169319,0.006761792924789532
97397,486867,0,486867,18188.72185778618,0.006753425264479824
97497,487367,0,487367,18199.72372198105,0.006745071926330205
97598,487872,0,487872,18210.52154994011,0.00673664955896222
97698,488372,0,488372,18221.143618822098,0.0067283249088173165
97798,488872,0,488872,18231.155718803406,0.006720014481995018
97898,489372,0,489372,18241.412020921707,0.006711718245861882
97998,489872,0,489872,18251.454318761826,0.006703436167885163
98098,490372,0,490372,18261.516823768616,0.00669516821563234
98198,490872,0,490872,18272.45702981949,0.006686914356770828
98298,491372,0,491372,18284.328454971313,0.006678674559067552
98398,491872,0,491872,18295.765505075455,0.006670448790388656
98498,492372,0,492372,18306.535614967346,0.006662237018699133
98599,492877,0,492877,18316.013466835022,0.006653957304411834
98699,493377,0,493377,18325.755074739456,0.006645773570161275
98799,493877,0,493877,18335.480105876923,0.006637603737067666
98899,494377,0,494377,18345.098648786545,0.006629447773488743
98999,494877,0,494877,18355.9884288311,0.006621305647879393
99099,495377,0,495377,18365.758004903793,0.006613177328791244
99199,495877,0,495877,18375.88257598877,0.006605062784872306
99299,496377,0,496377,18387.318913698196,0.0065969619848665765
99399,496877,0,496877,18397.86950492859,0.006588874897613887
99499,497377,0,497377,18408.301431894302,0.0065808014920493456
99600,497882,0,497882,18418.195657014847,0.00657266120848623
99700,498382,0,498382,18427.903971910477,0.006564615209526012
99800,498882,0,498882,18439.140279769897,0.006556582799320839
99900,499382,0,499382,18451.404489040375,0.006548563947184871
100000,499882,0,499882,18461.5774269104,0.006540558622526011


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha0/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0014910697937011719,30.358099469249375
200,201,200,401,0.1721489429473877,2.443647106553536
400,401,400,801,0.34951090812683105,1.4623020054181544
601,602,601,1203,0.5220968723297119,1.0864359863509294
801,802,801,1603,0.6736180782318115,0.884172469333225
1001,1002,1001,2003,1.1403388977050781,0.756423386206226
1201,1202,1201,2403,1.335745096206665,0.6677556741322215
1401,1402,1401,2803,1.4906928539276123,0.6018803012446704
1602,1603,1602,3205,1.6921212673187256,0.5501556568527358
1802,1803,1802,3605,1.9836199283599854,0.5083939523309472
2002,2003,2002,4005,2.1715409755706787,0.4735281727112222
2202,2203,2202,4405,2.31919002532959,0.44380632430760936
2402,2403,2402,4805,2.564152240753174,0.41806194377676287
2603,2604,2603,5207,2.7299749851226807,0.3953741725141351
2803,2804,2803,5607,2.8932979106903076,0.37537408529409977
3003,3004,3003,6007,3.1782779693603516,0.3574967775454968
3203,3204,3203,6407,3.357166051864624,0.34139925351073
3403,3404,3403,6807,3.551548957824707,0.32681143125199247
3604,3605,3604,7209,3.7118289470672607,0.31345351992341636
3804,3805,3804,7609,3.8677680492401123,0.3012822006287603
4004,4005,4004,8009,4.030489921569824,0.29008382263827337
4204,4205,4204,8409,4.224907159805298,0.279738735984933
4404,4405,4404,8809,4.38552713394165,0.2701466855862572
4605,4606,4605,9211,4.5640881061553955,0.26117989625642984
4805,4806,4805,9611,4.792270183563232,0.25285519172052956
5005,5006,5005,10011,4.97637414932251,0.24506456097986604
5205,5206,5205,10411,5.165646076202393,0.2377546752075857
5405,5406,5405,10811,5.488664150238037,0.23087923832463025
5606,5607,5606,11213,5.897052049636841,0.22436636221942408
5806,5807,5806,11613,6.258732080459595,0.21824526706125563
6006,6007,6006,12013,6.574193954467773,0.21245137964008523
6206,6207,6206,12413,6.776195049285889,0.20695707567728125
6406,6407,6406,12813,6.952604055404663,0.2017378176032389
6607,6608,6607,13215,7.166656970977783,0.19674750585888232
6807,6808,6807,13615,7.338606119155884,0.19201616179110503
7007,7008,7007,14015,7.5286102294921875,0.18750081290361562
7207,7208,7207,14415,7.729483127593994,0.18318569600874168
7407,7408,7407,14815,7.881656169891357,0.17905660071913546
7608,7609,7608,15217,8.065749168395996,0.17508132201764354
7808,7809,7808,15617,8.232303857803345,0.17128774083740186
8008,8009,8008,16017,8.402020931243896,0.1676451094270218
8208,8209,8208,16417,8.578912019729614,0.1641438367768636
8408,8409,8408,16817,8.735471963882446,0.16077518492537093
8609,8610,8609,17219,8.901782989501953,0.15751525889048315
8809,8810,8809,17619,9.06904411315918,0.1543891739329465
9009,9010,9009,18019,9.23555302619934,0.15137372855239975
9209,9210,9209,18419,9.37932801246643,0.14846279486717895
9409,9410,9409,18819,9.580969095230103,0.14565073983046334
9610,9611,9610,19221,9.86003589630127,0.14291901173762436
9810,9811,9810,19621,10.053208112716675,0.1402899883101414
10010,10011,10010,20021,10.23738408088684,0.13774542960476252
10210,10211,10210,20421,10.430102109909058,0.13528124533194744
10410,10411,10410,20821,10.600186824798584,0.13289364321357225
10611,10612,10611,21223,10.757214069366455,0.13056770656886155
10811,10812,10811,21623,10.958417892456055,0.12832328956712113
11011,11012,11011,22023,11.114824056625366,0.1261455885687076
11211,11212,11211,22423,11.28009295463562,0.12403175478829191
11411,11412,11411,22823,11.430287837982178,0.12197912473265268
11612,11613,11612,23225,11.577897071838379,0.11997537797070633
11812,11813,11812,23625,11.732659101486206,0.11803810315282258
12012,12013,12012,24025,11.89461612701416,0.11615498909882122
12212,12213,12212,24425,12.042931079864502,0.11432396789326375
12412,12413,12412,24825,12.187634944915771,0.11254309058936256
12613,12614,12613,25227,12.340112924575806,0.110801973111828
12813,12814,12813,25627,12.48270297050476,0.1091161940007785
13013,13014,13013,26027,12.627492904663086,0.10747532590128248
13213,13214,13213,26427,12.77098798751831,0.10587780854087535
13413,13414,13413,26827,12.917166233062744,0.10432216072143556
13614,13615,13614,27229,13.062029123306274,0.1027994978932257
13814,13815,13814,27629,13.206346988677979,0.10132362536127505
14014,14015,14014,28029,13.367260932922363,0.09988559085904321
14214,14215,14214,28429,13.528511047363281,0.09848417612377038
14414,14415,14414,28829,13.671755075454712,0.09711821743955897
14615,14616,14615,29231,13.819056034088135,0.0957800283723399
14815,14816,14815,29631,14.055022239685059,0.09448185460311487
15015,15016,15015,30031,14.202134132385254,0.09321593291789647
15215,15216,15215,30431,14.392217874526978,0.09198128436427426
15415,15416,15415,30831,14.539200067520142,0.09077696909114973
15616,15617,15616,31233,14.685840845108032,0.08959628204623568
15816,15817,15816,31633,14.890947818756104,0.08845009932042187
16016,16017,16016,32033,15.037644147872925,0.08733163829440838
16216,16217,16216,32433,15.185374021530151,0.08624009403053348
16416,16417,16416,32833,15.332825899124146,0.08517469069943166
16617,16618,16617,33235,15.512036085128784,0.08412954255472277
16817,16818,16817,33635,15.662084817886353,0.08311432399365244
17017,17018,17017,34035,15.816444873809814,0.0821230752025654
17217,17218,17217,34435,15.965311050415039,0.08115512255151293
17417,17418,17417,34835,16.122087001800537,0.0802098148541593
17618,17619,17618,35237,16.277503967285156,0.07928196013273325
17818,17819,17818,35637,16.43550395965576,0.078380178893659
18018,18019,18018,36037,16.590744018554688,0.07749921063335644
18218,18219,18218,36437,16.734294176101685,0.07663848419961432
18418,18419,18418,36837,16.8800048828125,0.07579744628785841
18619,18620,18619,37239,17.031764030456543,0.07497149851088454
18819,18820,18819,37639,17.17979907989502,0.0741683373353586
19019,19020,19019,38039,17.324185848236084,0.07338330217372391
19219,19220,19219,38439,17.491147994995117,0.0726159042077601
19419,19420,19419,38839,17.63406491279602,0.07186566918245992
19620,19621,19620,39241,17.77882409095764,0.07112851041108008
19820,19821,19820,39641,17.93207812309265,0.07041131424899968
20020,20021,20020,40041,18.074905157089233,0.06970993822399434
20220,20221,20220,40441,18.223223209381104,0.06902396125842604
20420,20421,20420,40841,18.38381600379944,0.06835297440345825
20621,20622,20621,41243,18.528983116149902,0.06769333446935327
20821,20822,20821,41643,18.673547983169556,0.06705121754971857
21021,21022,21021,42043,18.829493045806885,0.06642293080248314
21221,21222,21221,42443,18.98547101020813,0.06580810992625838
21421,21422,21421,42843,19.160052061080933,0.0652064008787552
21622,21623,21622,43245,19.315546989440918,0.0646145463605294
21822,21823,21822,43645,19.46136713027954,0.064038099621106
22022,22023,22022,44045,19.60757303237915,0.06347375937579187
22222,22223,22222,44445,19.761258125305176,0.06292120957063496
22422,22423,22422,44845,19.95094394683838,0.06238014292701027
22623,22624,22623,45247,20.095844984054565,0.06184763887898292
22823,22824,22823,45647,20.240041971206665,0.06132870428205937
23023,23024,23023,46047,20.403598070144653,0.060820379709791594
23223,23224,23223,46447,20.609939098358154,0.06032239051084022
23423,23424,23423,46847,20.763883113861084,0.05983446959782742
23624,23625,23624,47249,20.948374032974243,0.05935399088605918
23824,23825,23824,47649,21.101516008377075,0.05888548162126789
24024,24025,24024,48049,21.29066801071167,0.05842628142641032
24224,24225,24224,48449,21.436206817626953,0.05797615141237147
24424,24425,24424,48849,21.586517095565796,0.05753485924196196
24625,24626,24625,49251,21.731067895889282,0.05710003681135416
24825,24826,24825,49651,21.91562008857727,0.05667579003434358
25025,25026,25025,50051,22.062901973724365,0.05625972054690382
25225,25226,25225,50451,22.207606077194214,0.0558516204757849
25425,25426,25425,50851,22.352801084518433,0.05545128763916859
25626,25627,25626,51253,22.500121116638184,0.055056580276372336
25826,25827,25826,51653,22.657701015472412,0.05467123377464037
26026,26027,26026,52053,22.810935020446777,0.054293079648154545
26226,26227,26226,52453,22.965838193893433,0.053921936982787105
26426,26427,26426,52853,23.112565994262695,0.05355762981499894
26627,26628,26627,53255,23.25819492340088,0.05319821524473985
26827,26828,26827,53655,23.405689239501953,0.052847102387807154
27027,27028,27027,54055,23.55393099784851,0.05250232470432488
27227,27228,27227,54455,23.6998770236969,0.05216372473443906
27427,27428,27427,54855,23.847538948059082,0.05183114932581228
27628,27629,27628,55257,23.99309015274048,0.05150283053382608
27828,27829,27828,55657,24.13757610321045,0.05118188972906709
28028,28029,28028,56057,24.289198875427246,0.05086653801236315
28228,28229,28228,56457,24.441261053085327,0.05055663832946747
28428,28429,28428,56857,24.590600967407227,0.05025205737277767
28629,28630,28629,57259,24.74024510383606,0.0499511813428624
28829,28830,28829,57659,24.896986961364746,0.049656877392330066
29029,29030,29029,58059,25.041050910949707,0.0493675131009554
29229,29230,29229,58459,25.185364961624146,0.049082969158376004
29429,29430,29429,58859,25.326876878738403,0.048803129510607654
29630,29631,29630,59261,25.477782011032104,0.048526516378772415
29830,29831,29830,59661,25.623910903930664,0.04825577187211327
30030,30031,30030,60061,25.76947593688965,0.04798940161853438
30230,30231,30230,60461,25.91222882270813,0.04772730172426648
30430,30431,30430,60861,26.059629201889038,0.04746937112319351
30631,30632,30631,61263,26.207449913024902,0.04721425226639098
30831,30832,30831,61663,26.35277485847473,0.046964387612019744
31031,31032,31031,62063,26.498263120651245,0.04671840478045996
31231,31232,31231,62463,26.64272427558899,0.04647621325984695
31431,31432,31431,62863,26.78769302368164,0.04623772499135371
31632,31633,31632,63265,26.947783946990967,0.046001688895038945
31832,31833,31832,63665,27.112432956695557,0.04577036988910864
32032,32033,32032,64065,27.258835077285767,0.04554250359696158
32232,32233,32232,64465,27.410036087036133,0.04531801111171686
32432,32433,32432,64865,27.561098098754883,0.04509681565269014
32633,32634,32633,65267,27.716853141784668,0.0448777606127259
32833,32834,32833,65667,27.864712953567505,0.0446629526387775
33033,33034,33033,66067,28.01070213317871,0.04445122316461319
33233,33234,33233,66467,28.166537046432495,0.04424250333914123
33433,33434,33433,66867,28.311180114746094,0.044036726152848336
33634,33635,33634,67269,28.457129955291748,0.04383281900891723
33834,33835,33834,67669,28.60214900970459,0.04363274709200168
34034,34035,34034,68069,28.745763063430786,0.0434354270151071
34234,34235,34234,68469,28.88890504837036,0.04324079863493503
34434,34435,34434,68869,29.041901111602783,0.043048803402420996
34635,34636,34635,69271,29.2080020904541,0.04285844360072434
34835,34836,34835,69671,29.358524084091187,0.04267155763409157
35035,35036,35035,70071,29.503119945526123,0.04248713801960008
35235,35236,35235,70471,29.657550811767578,0.04230513215120475
35435,35436,35435,70871,29.800734043121338,0.042125488802573635
35636,35637,35636,71273,29.950026035308838,0.041947277162603804
35836,35837,35836,71673,30.105008840560913,0.04177222169836566
36036,36037,36036,72073,30.249951124191284,0.04159938273239527
36236,36237,36236,72473,30.393401861190796,0.04142871418144415
36436,36437,36436,72873,30.53843903541565,0.04126017115626857
36637,36638,36637,73275,30.683300256729126,0.04109288278002668
36837,36838,36837,73675,30.826402187347412,0.04092847083658302
37037,37038,37037,74075,30.99558401107788,0.04076605637549582
37237,37238,37237,74475,31.18208909034729,0.04060559895868889
37437,37438,37437,74875,31.34405207633972,0.04044705918159016
37638,37639,37638,75277,31.49356698989868,0.040289619999451236
37838,37839,37838,75677,31.657145977020264,0.040134810392883795
38038,38039,38038,76077,31.81377410888672,0.039981805944153945
38238,38239,38238,76477,31.96026611328125,0.03983057110228058
38438,38439,38438,76877,32.10705804824829,0.03968107121126238
38639,38640,38639,77279,32.25269889831543,0.039532537709657874
38839,38840,38839,77679,32.399226903915405,0.039386415466236425
39039,39040,39039,78079,32.54489207267761,0.039241929167629405
39239,39240,39239,78479,32.69813513755798,0.039099047495965364
39439,39440,39439,78879,32.88307523727417,0.03895773990892605
39640,39641,39640,79281,33.03171110153198,0.038817281632442746
39840,39841,39840,79681,33.17893314361572,0.038679041085945186
40040,40041,40040,80081,33.32568311691284,0.03854228729564062
40240,40241,40240,80481,33.49166011810303,0.038406992613132955
40440,40441,40440,80881,33.63779401779175,0.038273130062700625
40641,40642,40641,81283,33.78247880935669,0.03814001452752626
40841,40842,40841,81683,33.93452501296997,0.03800894474858745
41041,41042,41041,82083,34.07732892036438,0.03787922990179488
41241,41242,41241,82483,34.22087812423706,0.037750845522796
41441,41442,41441,82883,34.3671932220459,0.03762376773133308
41642,41643,41642,83285,34.51578497886658,0.03749734742828437
41842,41843,41842,83685,34.68741989135742,0.03737281967346745
42042,42043,42042,84085,34.86278510093689,0.037249530100944415
42242,42243,42242,84485,35.02073907852173,0.03712745701249274
42442,42443,42442,84885,35.17447805404663,0.03700657921773478
42643,42644,42643,85287,35.3259642124176,0.03688628042127037
42843,42844,42843,85687,35.47142720222473,0.03676773732690133
43043,43044,43043,86087,35.633002042770386,0.03665032876749169
43243,43244,43243,86487,35.788504123687744,0.03653403545120651
43443,43444,43443,86887,35.93386697769165,0.03641883852841708
43644,43645,43644,87289,36.078866958618164,0.03630415166299038
43844,43845,43844,87689,36.223310232162476,0.036191097942920594
44044,44045,44044,88089,36.37023901939392,0.03607908651570536
44244,44245,44244,88489,36.51558208465576,0.035968100186186944
44444,44445,44444,88889,36.66073703765869,0.03585812214489164
44645,44646,44645,89291,36.80644989013672,0.03574859349167758
44845,44846,44845,89691,36.95969891548157,0.0356405879290156
45045,45046,45045,90091,37.12867212295532,0.035533542360903794
45245,45246,45245,90491,37.30207586288452,0.035427441422120065
45445,45446,45445,90891,37.446547985076904,0.035322270084430264
45646,45647,45646,91293,37.59386205673218,0.03521749463992091
45846,45847,45846,91693,37.780027866363525,0.03511414319045893
46046,46047,46046,92093,37.92984986305237,0.035011678122097524
46246,46247,46246,92493,38.075993061065674,0.034910085669676794
46446,46447,46446,92893,38.221956968307495,0.034809352363038934
46647,46648,46647,93295,38.36754107475281,0.034708967686338764
46847,46848,46847,93695,38.51212501525879,0.03460991753600919
47047,47048,47047,94095,38.655054807662964,0.03451168775291461
47247,47248,47247,94495,38.80659198760986,0.03441426597369256
47447,47448,47447,94895,38.9509482383728,0.03431764009374857
47648,47649,47648,95297,39.09393095970154,0.03422132100179268
47848,47849,47848,95697,39.26690602302551,0.03412625544220422
48048,48049,48048,96097,39.423166036605835,0.03403195089917383
48248,48249,48248,96497,39.570794105529785,0.033938396239960346
48448,48449,48448,96897,39.715779066085815,0.03384558055928565
48649,48650,48649,97299,39.872374057769775,0.033753034548853804
48849,48850,48849,97699,40.03850197792053,0.03366166855399277
49049,49050,49049,98099,40.185940980911255,0.03357101007938353
49249,49250,49249,98499,40.338980197906494,0.03348104907494266
49449,49450,49449,98899,40.486855030059814,0.03339177569096829
49650,49651,49650,99301,40.63190293312073,0.03330273898351182
49850,49851,49850,99701,40.777180910110474,0.0332148153872823
50050,50051,50050,100101,40.92346000671387,0.033127550969873985
50250,50251,50250,100501,41.0677809715271,0.03304093663579046
50450,50451,50450,100901,41.21245503425598,0.0329549634664552
50651,50652,50651,101303,41.35889911651611,0.03286919758663817
50851,50852,50851,101703,41.503172874450684,0.032784483775300924
51051,51052,51051,102103,41.64769005775452,0.03270038535043529
51251,51252,51251,102503,41.8093581199646,0.032616894060114525
51451,51452,51451,102903,41.957218170166016,0.03253400180897552
51652,51653,51652,103305,42.11891794204712,0.03245129062069263
51852,51853,51852,103705,42.26580786705017,0.03236957566668825
52052,52053,52052,104105,42.45754098892212,0.03228843633043651
52252,52253,52252,104505,42.61540603637695,0.03220786510719228
52452,52453,52452,104905,42.761038064956665,0.03212785463108102
52653,52654,52653,105307,42.908485889434814,0.03204800176579049
52853,52854,52853,105707,43.053614139556885,0.03196909394012309
53053,53054,53053,106107,43.20104002952576,0.03189072553060704
53253,53254,53253,106507,43.34565711021423,0.03181288969584784
53453,53454,53453,106907,43.50075602531433,0.03173557971791675
53654,53655,53654,107309,43.645997047424316,0.0316584063396373
53854,53855,53854,107709,43.793062925338745,0.03158213094916858
54054,54055,54054,108109,43.93716096878052,0.03150636194305282
54254,54255,54254,108509,44.08216309547424,0.03143109307020482
54454,54455,54454,108909,44.236693143844604,0.031356318189567724
54655,54656,54655,109311,44.390405893325806,0.031281661049028214
54855,54856,54855,109711,44.53461503982544,0.03120785855288486
55055,55056,55055,110111,44.67984199523926,0.031134532232669453
55255,55256,55255,110511,44.825031995773315,0.03106167636384517
55455,55456,55455,110911,44.96980309486389,0.03098928532016012
55656,55657,55656,111313,45.116421937942505,0.030916995057551307
55856,55857,55856,111713,45.270655155181885,0.030845519423554735
56056,56057,56056,112113,45.41688513755798,0.030774492277794035
56256,56257,56256,112513,45.56502413749695,0.030703908366513225
56456,56457,56456,112913,45.71100187301636,0.030633762523957244
56657,56658,56657,113315,45.85827422142029,0.030563702185668725
56857,56858,56857,113715,46.0038640499115,0.03049441945341709
57057,57058,57057,114115,46.148810148239136,0.030425559777533903
57257,57258,57257,114515,46.31422209739685,0.030357118326168723
57457,57458,57457,114915,46.47625494003296,0.03028909034644813
57658,57659,57658,115317,46.64840817451477,0.030221134086234405
57858,57859,57858,115717,46.83412194252014,0.03015392110834263
58058,58059,58058,116117,46.98229789733887,0.030087107778424313
58258,58259,58258,116517,47.14052104949951,0.030020689643612493
58458,58459,58458,116917,47.285582065582275,0.029954662322081667
58659,58660,58659,117319,47.45509195327759,0.029888694261406282
58859,58860,58859,117719,47.6107861995697,0.02982343759855683
59059,59060,59059,118119,47.75490403175354,0.02975855899453978
59259,59260,59259,118519,47.901166915893555,0.029694054337697912
59459,59460,59459,118919,48.047029972076416,0.029629919580423218
59660,59661,59660,119321,48.20169496536255,0.02956583280639606
59860,59861,59860,119721,48.389853954315186,0.029502427755384367
60060,60061,60060,120121,48.54690909385681,0.029439380813448743
60260,60261,60260,120521,48.7493371963501,0.029376688176829046
60460,60461,60460,120921,48.91277813911438,0.02931434609963969
60661,60662,60661,121323,49.06389617919922,0.029252041782077156
60861,60862,60861,121723,49.210273027420044,0.029190391519037764
61061,61062,61061,122123,49.37461709976196,0.02912908089594321
61261,61262,61261,122523,49.520103931427,0.029068106387489193
61461,61462,61461,122923,49.665579080581665,0.029007464520781623
61662,61663,61662,123325,49.867257833480835,0.028946851132574117
61862,61863,61862,123725,50.023386001586914,0.028886865956128206
62062,62063,62062,124125,50.1683509349823,0.028827203290694058
62262,62263,62262,124525,50.31146717071533,0.028767859863347005
62462,62463,62462,124925,50.495718002319336,0.028708832448727063
62663,62664,62663,125327,50.65342116355896,0.02864982507595059
62863,62864,62863,125727,50.81220507621765,0.02859142173718802
63063,63064,63063,126127,50.960427045822144,0.028533324996223377
63263,63264,63263,126527,51.10419297218323,0.028475531809367304
63463,63464,63463,126927,51.27660393714905,0.028418039176188254
63664,63665,63664,127329,51.420865058898926,0.028360558906318195
63864,63865,63864,127729,51.56771802902222,0.028303660014377258
64064,64065,64064,128129,51.71280097961426,0.028247052912161407
64264,64265,64264,128529,51.858356952667236,0.028190734764629403
64464,64465,64464,128929,52.00304317474365,0.02813470277616253
64665,64666,64665,129331,52.14745807647705,0.028078676154383548
64865,64866,64865,129731,52.29981017112732,0.028023209647965723
65065,65066,65065,130131,52.44391894340515,0.027968021129900187
65265,65266,65265,130531,52.613439083099365,0.02791310795544317
65465,65466,65465,130931,52.76088809967041,0.02785846751584931
65666,65667,65666,131333,52.92721486091614,0.027803826060845374
65866,65867,65866,131733,53.098570108413696,0.027749724737346673
66066,66067,66066,132133,53.24498510360718,0.02769588851970521
66266,66267,66266,132533,53.389366149902344,0.02764231493708164
66466,66467,66466,132933,53.5340838432312,0.027589001551572824
66667,66668,66667,133335,53.68196415901184,0.02753568132337202
66867,66868,66867,133735,53.82524609565735,0.027482882418456027
67067,67068,67067,134135,53.97227907180786,0.0274303365772643
67267,67268,67267,134535,54.12544393539429,0.027378041488187697
67467,67468,67467,134935,54.2680242061615,0.027325994869808547
67668,67669,67668,135337,54.42033100128174,0.02727393608327075
67868,67869,67868,135737,54.56872606277466,0.027222380894687342
68068,68069,68068,136137,54.724679946899414,0.02717106749771543
68268,68269,68268,136537,54.87518811225891,0.027119993726812338
68468,68469,68468,136937,55.030369997024536,0.02706915744416197
68669,68670,68669,137339,55.233251094818115,0.027018304122564073
68869,68870,68869,137739,55.40829801559448,0.026967937672853978
69069,69070,69069,138139,55.55328011512756,0.026917802449511842
69269,69270,69269,138539,55.69691705703735,0.026867896421229432
69469,69470,69469,138939,55.879064083099365,0.026818217582206205
69670,69671,69670,139341,56.02959585189819,0.02676851724612232
69870,69871,69870,139741,56.17482900619507,0.026719287979562044
70070,70071,70070,140141,56.31904482841492,0.026670280024185245
70270,70271,70270,140541,56.46415400505066,0.026621491472260554
70470,70471,70470,140941,56.6119749546051,0.026572920439563243
70671,70672,70671,141343,56.75709390640259,0.026524323826871515
70871,70872,70871,141743,56.909610986709595,0.026476183336627983
71071,71072,71071,142143,57.053694009780884,0.026428254841232568
71271,71272,71271,142543,57.22221493721008,0.026380536546912005
71471,71472,71471,142943,57.370487213134766,0.026333026681591643
71672,71673,71672,143345,57.516215085983276,0.026285487494986652
71872,71873,71872,143745,57.660582065582275,0.026238390276976633
72072,72073,72072,144145,57.80519104003906,0.02619149629007485
72272,72273,72272,144545,57.94912910461426,0.026144803845767835
72472,72473,72472,144945,58.09306287765503,0.02609831127560433
72673,72674,72673,145347,58.23859405517578,0.026051785954460557
72873,72874,72873,145747,58.38152098655701,0.02600568918486195
73073,73074,73073,146147,58.527925968170166,0.025959787393368128
73273,73274,73273,146547,58.67115497589111,0.025914078988845155
73473,73474,73473,146947,58.81699514389038,0.02586856239873594
73674,73675,73674,147349,58.961143016815186,0.02582300991257253
73874,73875,73874,147749,59.105080127716064,0.025777873246323864
74074,74075,74074,148149,59.296574115753174,0.025732923777959413
74274,74275,74274,148549,59.463916063308716,0.025688160006570537
74474,74475,74474,148949,59.60796284675598,0.025643580448476134
74675,74676,74675,149351,59.753445863723755,0.02559896210961971
74875,74876,74875,149751,59.899775981903076,0.025554747497581246
75075,75076,75075,150151,60.04368996620178,0.025510712741510854
75275,75276,75275,150551,60.18608117103577,0.025466856424219003
75475,75476,75475,150951,60.33824396133423,0.02542317714451537
75676,75677,75676,151353,60.48305416107178,0.025379456437858338
75876,75877,75876,151753,60.62781119346619,0.025336127960596044
76076,76077,76076,152153,60.770721197128296,0.025292972404311383
76276,76277,76276,152553,60.93907594680786,0.025249988429606376
76476,76477,76476,152953,61.08324098587036,0.025207174711961728
76677,76678,76677,153355,61.23025107383728,0.025164317139971276
76877,76878,76877,153755,61.37714600563049,0.02512184085637671
77077,77078,77077,154155,61.536519050598145,0.02507953093708606
77277,77278,77277,154555,61.68795394897461,0.025037386115082563
77477,77478,77477,154955,61.83451294898987,0.024995405137204354
77678,77679,77678,155357,62.00006723403931,0.02495337807856421
77878,77879,77878,155757,62.14507603645325,0.024911721887739973
78078,78079,78078,156157,62.28817319869995,0.02487022585673279
78278,78279,78278,156557,62.4317991733551,0.02482888878596061
78478,78479,78478,156957,62.57485914230347,0.024787709488759215
78679,78680,78679,157359,62.72279095649719,0.024746482069218284
78879,78880,78879,157759,62.86543607711792,0.02470561558424707
79079,79080,79079,158159,63.00995111465454,0.0246649033828868
79279,79280,79279,158559,63.156569957733154,0.02462434432845971
79479,79480,79479,158959,63.30122089385986,0.024583937296346954
79680,79681,79680,159361,63.44505715370178,0.024543480270519773
79880,79881,79880,159761,63.58997416496277,0.024503374702898924
80080,80081,80080,160161,63.75097393989563,0.024463417849054953
80280,80281,80280,160561,63.89435911178589,0.024423608631058615
80480,80481,80480,160961,64.05810403823853,0.024383945982250764
80681,80682,80681,161363,64.2038049697876,0.024344231625261305
80881,80882,80881,161763,64.3485472202301,0.024304859678926337
81081,81082,81081,162163,64.49523997306824,0.02426563116279573
81281,81282,81281,162563,64.68703103065491,0.02422654505387042
81481,81482,81481,162963,64.86237001419067,0.024187600339695938
81682,81683,81682,163365,65.0089659690857,0.024148602347684355
81882,81883,81882,163765,65.15400505065918,0.024109938121669453
82082,82083,82082,164165,65.32472395896912,0.024071412310059215
82282,82283,82282,164565,65.47256398200989,0.024033023941270815
82482,82483,82482,164965,65.618155002594,0.02399477205359773
82683,82684,82683,165367,65.77394104003906,0.023956465452220882
82883,82884,82883,165767,65.95595407485962,0.02391848435111394
83083,83084,83083,166167,66.09992599487305,0.023880636899360104
83283,83284,83283,166567,66.24738788604736,0.023842922173554222
83483,83484,83483,166967,66.39188885688782,0.023805339259551344
83684,83685,83684,167369,66.5388810634613,0.02376770031970814
83884,83885,83884,167769,66.6840169429779,0.023730378971149334
84084,84085,84084,168169,66.83482503890991,0.02369318674194137
84284,84285,84284,168569,66.97942209243774,0.023656122753867637
84484,84485,84484,168969,67.12439393997192,0.02361918613740254
84685,84686,84685,169371,67.27791118621826,0.023582192297496748
84885,84886,84885,169771,67.48792600631714,0.02354550847605718
85085,85086,85085,170171,67.64093494415283,0.023508949464517127
85285,85286,85285,170571,67.79163002967834,0.02347251442708628
85485,85486,85485,170971,67.94395303726196,0.023436202536138387
85686,85687,85686,171373,68.1066780090332,0.023399832330270882
85886,85887,85886,171773,68.25006794929504,0.023363764887116164
86086,86087,86086,172173,68.39575505256653,0.023327818151553645
86286,86287,86286,172573,68.57274389266968,0.023291991327662267
86486,86487,86486,172973,68.71927881240845,0.023256283627197154
86687,86688,86687,173375,68.86592316627502,0.023220516618742672
86887,86888,86887,173775,69.0448808670044,0.02318504541655343
87087,87088,87087,174175,69.19160413742065,0.023149691014377808
87287,87288,87287,174575,69.3385169506073,0.02311445265379425
87487,87488,87487,174975,69.48255324363708,0.023079329583604948
87688,87689,87688,175377,69.63171696662903,0.023044146303687254
87888,87889,87888,175777,69.81081509590149,0.023009252156363423
88088,88089,88088,176177,69.9568829536438,0.02297447108469143
88288,88289,88288,176577,70.10617399215698,0.022939802365550592
88488,88489,88488,176977,70.28427815437317,0.02290524528262353
88689,88690,88689,177379,70.46723508834839,0.022870627173054606
88889,88890,88889,177779,70.61145496368408,0.022836291789779976
89089,89090,89089,178179,70.7601969242096,0.022802065930324977
89289,89290,89289,178579,70.94643521308899,0.022767948904826824
89489,89490,89489,178979,71.09942507743835,0.022733940029835305
89690,89691,89690,179381,71.24540495872498,0.022699869390128184
89890,89891,89890,179781,71.38959908485413,0.022666075323415778
90090,90091,90090,180181,71.53361701965332,0.02263238739128656
90290,90291,90290,180581,71.68002510070801,0.022598804935235167
90490,90491,90490,180981,71.8209958076477,0.02256532730280536
90691,90692,90691,181383,71.97346997261047,0.02253178724091115
90891,90892,90891,181783,72.11741709709167,0.02249851783828896
91091,91092,91091,182183,72.33427786827087,0.022465351334364565
91291,91292,91291,182583,72.48896384239197,0.022432287100220567
91491,91492,91491,182983,72.63413906097412,0.022399324512650004
91692,91693,91692,183385,72.77975821495056,0.022366298899103878
91892,91893,91892,183785,72.94000697135925,0.022333538258133594
92092,92093,92092,184185,73.08689403533936,0.022300877424714302
92292,92293,92292,184585,73.26979613304138,0.022268315797867092
92492,92493,92492,184985,73.41590404510498,0.02223585278200714
92693,92694,92693,185387,73.56088304519653,0.022203326207200454
92893,92894,92893,185787,73.70901799201965,0.02217105913355348
93093,93094,93093,186187,73.8532440662384,0.022138888913017123
93293,93294,93293,186587,73.9967110157013,0.02210681497101136
93493,93494,93493,186987,74.14053416252136,0.022074836738055006
93694,93695,93694,187389,74.33741021156311,0.022042794472377135
93894,93895,93894,187789,74.63045310974121,0.02201100644071868
94094,94095,94094,188189,74.9087188243866,0.021979312436937914
94294,94295,94294,188589,75.20732021331787,0.021947711911415337
94494,94495,94494,188989,75.44865012168884,0.021916204319354645
94695,94696,94695,189391,75.66354990005493,0.02188463227597407
94895,94896,94895,189791,75.85635805130005,0.021853309393429936
95095,95096,95095,190191,76.00604605674744,0.021822077835729637
95295,95296,95295,190591,76.15144920349121,0.021790937076869497
95495,95496,95495,190991,76.32559490203857,0.021759886595411046
95696,95697,95696,191393,76.549880027771,0.02172877129548686
95896,95897,95896,191793,76.73746705055237,0.021697900267488288
96096,96097,96096,192193,77.00180196762085,0.02166711797694334
96296,96297,96296,192593,77.23951387405396,0.021636423920205743
96496,96497,96496,192993,77.43079805374146,0.021605817597952125
96697,96698,96697,193395,77.66598606109619,0.021575146138085165
96897,96898,96897,193795,77.93670701980591,0.021544714236408004
97097,97098,97097,194195,78.19677805900574,0.021514368594300223
97297,97298,97297,194595,78.36417317390442,0.02148410872929325
97497,97498,97497,194995,78.54626417160034,0.02145393416301556
97698,97699,97698,195397,78.7552490234375,0.021423694184768718
97898,97899,97898,195797,78.98840498924255,0.021393689217598464
98098,98099,98098,196197,79.13775396347046,0.021363768135867073
98298,98299,98298,196597,79.30823516845703,0.021333930477178447
98498,98499,98498,196997,79.48175382614136,0.021304175783020872
98699,98700,98699,197399,79.658362865448,0.02127435544435141
98899,98900,98899,197799,80.01540303230286,0.021244765728221073
99099,99100,99099,198199,80.32066202163696,0.021215257621758108
99299,99300,99299,198599,80.61465406417847,0.02118583068160165
99499,99500,99499,198999,81.12660098075867,0.0211564844680754
99700,99701,99700,199401,81.3901309967041,0.021127072416536986
99900,99901,99900,199801,81.81817698478699,0.021097886749999017
100100,100101,100100,200201,82.06132197380066,0.021068780510652408
100300,100301,100300,200601,82.37980103492737,0.021039753273197036
100501,100502,100501,201003,82.71208190917969,0.021010660069271752
100701,100702,100701,201403,82.8975019454956,0.02098178996341439
100901,100902,100901,201803,83.06662893295288,0.020952997602320545
101101,101102,101101,202203,83.23614120483398,0.02092428257448031
101301,101302,101301,202603,83.42758798599243,0.02089564447173891
101502,101503,101502,203005,83.66565895080566,0.020866940272931584
101702,101703,101702,203405,84.14139914512634,0.020838455188762917
101902,101903,101902,203805,84.50460815429688,0.020810045823034595
102102,102103,102102,204205,84.81919598579407,0.020781711780688713
102302,102303,102302,204605,85.1617579460144,0.02075345266985473
102503,102504,102503,205007,85.47239303588867,0.020725127365616724
102703,102704,102703,205407,85.7914400100708,0.02069701732460451
102903,102904,102903,205807,86.01125192642212,0.020668981056389424
103103,103104,103103,206207,86.30404615402222,0.02064101818154518
103303,103304,103303,206607,86.49008417129517,0.020613128323674873
103504,103505,103504,207009,86.6409637928009,0.02058517220520253
103704,103705,103704,207409,86.79329705238342,0.020557427624493984
103904,103905,103904,207809,87.09816002845764,0.02052975494761059
104104,104105,104104,208209,87.56422090530396,0.020502153809985553
104304,104305,104304,208609,87.85783004760742,0.020474623849932278
104505,104506,104505,209011,88.19082903862,0.020447027590242448
104705,104706,104705,209411,88.50776100158691,0.02041963926307493
104905,104906,104905,209811,88.82140398025513,0.020392321043656736
105105,105106,105105,210211,89.19775009155273,0.020365072581552512
105305,105306,105305,210611,89.75777697563171,0.020337893529066852
105506,105507,105506,211013,90.24157404899597,0.020310648164226914
105706,105707,105706,211413,90.62009716033936,0.02028360724147293
105906,105907,105906,211813,90.87632703781128,0.020256634699730023
106106,106107,106106,212213,91.10560393333435,0.020229730202008103
106306,106307,106306,212613,91.5157859325409,0.020202893413924592
106507,106508,106507,213015,91.95376420021057,0.02017599032536053
106707,106708,106707,213415,92.47454595565796,0.020149288298128884
106907,106908,106907,213815,92.7461051940918,0.020122652991151957
107107,107108,107107,214215,93.06649708747864,0.020096084080237445
107307,107308,107307,214615,93.25553894042969,0.02006958124367558
107508,107509,107508,215017,93.4267930984497,0.020043012141484632
107708,107709,107708,215417,93.6297459602356,0.02001664082470869
107908,107909,107908,215817,93.81002807617188,0.019990334630246288
108108,108109,108108,216217,94.0137369632721,0.019964093246091698
108308,108309,108308,216617,94.2135272026062,0.01993791636260392
108509,108510,108509,217019,94.41410422325134,0.019911673269805932
108709,108710,108709,217419,94.60288381576538,0.01988562478675329
108909,108910,108909,217819,94.78238701820374,0.019859639887898215
109109,109110,109109,218219,94.95816802978516,0.019833718272844497
109309,109310,109309,218619,95.13093209266663,0.019807859643449135
109510,109511,109510,219021,95.31779217720032,0.019781934881116445
109710,109711,109710,219421,95.50830912590027,0.019756201648760182
109910,109911,109910,219821,95.6895260810852,0.019730530519486488
110110,110111,110110,220221,95.87189197540283,0.019704921203963034
110310,110311,110310,220621,96.06289482116699,0.01967937341500557
110511,110512,110511,221023,96.25576090812683,0.01965375958821328
110711,110712,110711,221423,96.43538212776184,0.019628334303410103
110911,110912,110911,221823,96.65899014472961,0.01960296969490564
111111,111112,111111,222223,96.82693409919739,0.019577665483915933
111311,111312,111311,222623,97.01247906684875,0.019552421393705496
111512,111513,111512,223025,97.19070792198181,0.01952711137825143
111712,111713,111712,223425,97.37936210632324,0.019501987004674468
111912,111913,111912,223825,97.56143403053284,0.019476921932419247
112112,112113,112112,224225,97.76227903366089,0.019451915892762284
112312,112313,112312,224625,97.95990204811096,0.019426968618934372
112513,112514,112513,225027,98.13153791427612,0.019401955548779173
112713,112714,112713,225427,98.30627799034119,0.01937712530455918
112913,112914,112913,225827,98.47410416603088,0.019352353036102266
113113,113114,113113,226227,98.65419101715088,0.019327638484284045
113313,113314,113313,226627,98.8318841457367,0.019302981391844724
113514,113515,113514,227029,99.01250004768372,0.019278258647228156
113714,113715,113714,227429,99.18897199630737,0.01925371599325822
113914,113915,113914,227829,99.37077903747559,0.019229230036650467
114114,114115,114114,228229,99.61290717124939,0.01920480052744221
114314,114315,114314,228629,99.87265491485596,0.019180427217451
114515,114516,114515,229031,100.23680210113525,0.019155988413642223
114715,114716,114715,229431,100.47864818572998,0.01913172704250599
114915,114916,114915,229831,100.67521595954895,0.01910752113534766
115115,115116,115115,230231,100.88848114013672,0.01908337045095245
115315,115316,115315,230631,101.095134973526,0.019059274749805576
115516,115517,115516,231033,101.2664909362793,0.019035113726448963
115716,115717,115716,231433,101.43588900566101,0.019011127551933474
115916,115917,115916,231833,101.61319208145142,0.0189871956510003
116116,116117,116116,232233,101.79511094093323,0.01896331779078996
116316,116317,116316,232633,101.96328806877136,0.018939493740067266
116517,116518,116517,233035,102.1286768913269,0.01891560455108807
116717,116718,116717,233435,102.31941604614258,0.018891887698247435
116917,116918,116917,233835,102.49638414382935,0.01886822396965953
117117,117118,117117,234235,102.67105317115784,0.01884461314044846
117317,117318,117317,234635,102.90744400024414,0.018821054987290517
117518,117519,117518,235037,103.16175603866577,0.018797431891326603
117718,117719,117718,235437,103.37848401069641,0.018773978687062175
117918,117919,117918,235837,103.60213088989258,0.018750577496964436
118118,118119,118118,236237,103.77558207511902,0.018727228103788053
118318,118319,118318,236637,103.97674798965454,0.018703930291771757
118519,118520,118519,237039,104.17846989631653,0.018680567743100486
118719,118720,118719,237439,104.34484004974365,0.0186573727072281
118919,118920,118919,237839,104.54178786277771,0.01863422861295066
119119,119120,119119,238239,104.70593309402466,0.01861113525031887
119319,119320,119319,238639,104.85725283622742,0.018588092410802587
119520,119521,119520,239041,105.02472615242004,0.018564985050733673
119720,119721,119720,239441,105.19577193260193,0.01854204288750886
119920,119921,119920,239841,105.36012196540833,0.01851915062918099
120120,120121,120120,240241,105.51761102676392,0.01849630807277906
120320,120321,120320,240641,105.66812491416931,0.018473515016689774
120521,120522,120521,241043,105.81609296798706,0.018450657665397007
120721,120722,120721,241443,105.9718668460846,0.018427963255472003
120921,120922,120921,241843,106.12227988243103,0.018405317748062047
121121,121122,121121,242243,106.27423906326294,0.018382720946873002
121321,121322,121321,242643,106.4192111492157,0.01836017265690967
121522,121523,121522,243045,106.58080220222473,0.018337560305676757
121722,121723,121722,243445,106.73410320281982,0.01831510869846413
121922,121923,121922,243845,106.88154911994934,0.01829270502422189
122122,122123,122122,244245,107.03662896156311,0.018270349093046007
122322,122323,122322,244645,107.18932604789734,0.01824804071627606
122523,122524,122523,245047,107.34285593032837,0.018225668520131973
122723,122724,122723,245447,107.50798010826111,0.018203454926551815
122923,122924,122923,245847,107.65634894371033,0.018181288327829507
123123,123124,123123,246247,107.80871510505676,0.018159168540178933
123323,123324,123323,246647,107.95928907394409,0.01813709538100483
123524,123525,123524,247049,108.1122510433197,0.018114958651727256
123724,123725,123724,247449,108.26519203186035,0.018092978437316373
123924,123925,123924,247849,108.41017293930054,0.018071044309747725
124124,124125,124124,248249,108.56620121002197,0.01804915609109422
124324,124325,124324,248649,108.71780800819397,0.018027313604569765
124525,124526,124525,249051,108.86403894424438,0.018005407804036002
124725,124726,124725,249451,109.01729416847229,0.017983656482398552
124925,124926,124925,249851,109.17241716384888,0.017961950368415185
125125,125126,125125,250251,109.3513731956482,0.017940289289771996
125325,125326,125325,250651,109.54384016990662,0.0179186730752483
125526,125527,125526,251053,109.73314094543457,0.017896993809113654
125726,125727,125726,251453,109.89602518081665,0.017875467035694384
125926,125927,125926,251853,110.05623507499695,0.01785398461836148
126126,126127,126126,252253,110.21472811698914,0.017832546390180205
126326,126327,126326,252653,110.36692786216736,0.01781115218526362
126527,126528,126527,253055,110.52819681167603,0.017789695196949878
126727,126728,126727,253455,110.69402289390564,0.017768388763111733
126927,126928,126927,253855,110.85124516487122,0.01774712586026452
127127,127128,127127,254255,111.01627016067505,0.017725906326630136
127327,127328,127327,254655,111.17286515235901,0.017704730001434802
127528,127529,127528,255057,111.32887983322144,0.01768349116641106
127728,127729,127728,255457,111.48809599876404,0.017662400993801224
127928,127929,127928,255857,111.67101216316223,0.017641353552466602
128128,128129,128128,256257,111.84167003631592,0.017620348685573644
128328,128329,128328,256657,111.99901223182678,0.017599386237252088
128529,128530,128529,257059,112.15100121498108,0.017578361557592338
128729,128730,128729,257459,112.2999210357666,0.017557483692780127
128929,128930,128929,257859,112.45570993423462,0.017536647783867064
129129,129130,129129,258259,112.62201714515686,0.017515853678762478
129329,129330,129329,258659,112.78935194015503,0.017495101226299718
129530,129531,129530,259061,112.9758632183075,0.01747428682550234
129730,129731,129730,259461,113.1497311592102,0.017453617434874686
129930,129931,129930,259861,113.31706309318542,0.017432989248119635
130130,130131,130130,260261,113.50125503540039,0.017412402117697078
130330,130331,130330,260661,113.65484285354614,0.017391855896953967
130531,130532,130531,261063,113.81499695777893,0.01737124801500831
130731,130732,130731,261463,113.99158191680908,0.017350783379909175
130931,130932,130931,261863,114.1657350063324,0.017330359219062202
131131,131132,131131,262263,114.71819496154785,0.017309975389295077
131331,131332,131331,262663,115.2302758693695,0.01728963174828689
131532,131533,131532,263065,115.5592520236969,0.017269226736975007
131732,131733,131732,263465,115.87081098556519,0.01724896324907479
131932,131933,131932,263865,116.1800148487091,0.017228739527314234
132132,132133,132132,264265,116.39066815376282,0.017208555432714115
132332,132333,132332,264665,116.65201306343079,0.01718841082711301
132533,132534,132533,265067,116.8627541065216,0.01716820514553219
132733,132734,132733,265467,117.05178189277649,0.017148139302416307
132933,132934,132933,265867,117.24356889724731,0.017128112537978787
133133,133134,133133,266267,117.4433491230011,0.017108124717267505
133333,133334,133333,266667,117.61293196678162,0.017088175706115843
133534,133535,133534,267069,117.79211807250977,0.017068165916412272
133734,133735,133734,267469,118.02055311203003,0.017048294317375944
133934,133935,133934,267869,118.30064010620117,0.01702846112939173
134134,134135,134134,268269,118.610524892807,0.01700866622137614
134334,134335,134334,268669,118.8448588848114,0.016988909463000308
134535,134536,134535,269071,119.13627195358276,0.01696909222630119
134735,134736,134735,269471,119.58361411094666,0.016949411568340487
134935,134936,134935,269871,119.84097599983215,0.016929768672862312
135135,135136,135135,270271,120.04284024238586,0.01691016341250063
135335,135336,135335,270671,120.25642013549805,0.01689059566061461
135536,135537,135536,271073,120.43568897247314,0.01687096773314944
135736,135737,135736,271473,120.62568807601929,0.016851474807138087
135936,135937,135936,271873,120.77935004234314,0.016832019013353957
136136,136137,136136,272273,120.96827101707458,0.01681260022800411
136336,136337,136336,272673,121.12147521972656,0.01679321832799294
136537,136538,136537,273075,121.28461003303528,0.01677377655739345
136737,136738,136737,273475,121.48669505119324,0.01675446824443602
136937,136938,136937,273875,121.70843505859375,0.01673519645105615
137137,137138,137137,274275,121.86726999282837,0.016715961056896576
137337,137338,137337,274675,122.07329487800598,0.01669676194227066
137538,137539,137538,275077,122.34273600578308,0.016677503264040557
137738,137739,137738,275477,122.72558689117432,0.016658376531992113
137938,137939,137938,275877,123.1265161037445,0.016639285723801425
138138,138139,138138,276277,123.38740611076355,0.016620230722415596
138338,138339,138338,276677,123.83141803741455,0.016601211411426512
138539,138540,138539,277079,124.49972200393677,0.016582132845572133
138739,138740,138739,277479,124.88034200668335,0.016563184745717146
138939,138940,138939,277879,125.22710514068604,0.016544271990284538
139139,139140,139139,278279,125.71898698806763,0.016525394465400304
139339,139340,139339,278679,126.23578000068665,0.01650655205781082
139540,139541,139540,279081,126.5786828994751,0.016487650705624704
139740,139741,139740,279481,126.86967992782593,0.01646887836950588
139940,139941,139940,279881,127.22705316543579,0.016450140814042353
140140,140141,140140,280281,127.53091502189636,0.01643143792841908
140340,140341,140340,280681,127.75574827194214,0.016412769602418446
140541,140542,140541,281083,127.92901611328125,0.016394042643407807
140741,140742,140741,281483,128.1114649772644,0.016375443279798008
140941,140942,140941,281883,128.27822494506836,0.01635687814815601
141141,141142,141141,282283,128.4381959438324,0.016338347140611515
141341,141342,141341,282683,128.61757111549377,0.016319850149869385
141542,141543,141542,283085,128.80689311027527,0.016301294838822408
141742,141743,141742,283485,128.98598790168762,0.016282865730831965
141942,141943,141942,283885,129.1663420200348,0.01626447032063926
142142,142143,142142,284285,129.49136114120483,0.016246108503209424
142342,142343,142342,284685,129.82109117507935,0.01622778017406136
142543,142544,142543,285087,130.1201310157776,0.01620939383824413
142743,142744,142743,285487,130.4587049484253,0.016191132340557263
142943,142944,142943,285887,130.70747184753418,0.016172904020478093
143143,143144,143143,286287,130.9761140346527,0.016154708775702725
143343,143344,143343,286687,131.17097806930542,0.0161365465044607
143544,143545,143544,287089,131.365327835083,0.01611832654093865
143744,143745,143744,287489,131.65677189826965,0.01610023007717204
143944,143945,143944,287889,131.90359711647034,0.016082166284289594
144144,144145,144144,288289,132.22609305381775,0.016064135062618397
144344,144345,144344,288689,132.51507306098938,0.016046136312999705
144545,144546,144545,289091,132.7636160850525,0.016028080186077015
144745,144746,144745,289491,133.0052990913391,0.016010146246254867
144945,144946,144945,289891,133.1956820487976,0.015992244483568716
145145,145146,145145,290291,133.35949110984802,0.015974374800881243
145345,145346,145345,290691,133.54571390151978,0.015956537101550528
145546,145547,145546,291093,133.7086570262909,0.01593864234032183
145746,145747,145746,291493,133.86085510253906,0.015920868478461383
145946,145947,145946,291893,134.02755522727966,0.015903126312494586
146146,146147,146146,292293,134.19387102127075,0.01588541574772831
146346,146347,146346,292693,134.34757781028748,0.01586773668994704
146547,146548,146547,293095,134.51984906196594,0.015850000885955833
146747,146748,146747,293495,134.76410508155823,0.015832384717758295
146947,146948,146947,293895,134.9617109298706,0.015814799776268592
147147,147148,147147,294295,135.14457297325134,0.015797245969150258
147347,147348,147347,294695,135.31169414520264,0.015779723204527703
147548,147549,147548,295097,135.46246099472046,0.015762144009526545
147748,147749,147748,295497,135.6378300189972,0.015744683210167636
147948,147949,147948,295897,135.81058597564697,0.015727253179957493
148148,148149,148148,296297,136.14891815185547,0.015709853828832755
148348,148349,148348,296697,136.29900813102722,0.015692485067174616
148549,148550,148549,297099,136.50564312934875,0.01567506019098154
148749,148750,148749,297499,136.72690796852112,0.01565775249299771
148949,148950,148949,297899,136.88738799095154,0.01564047511781886
149149,149150,149149,298299,137.04393100738525,0.015623227977574705
149349,149350,149349,298699,137.21404504776,0.015606010984823967
149550,149551,149550,299101,137.5362000465393,0.015588738193271088
149750,149751,149750,299501,137.88937187194824,0.01557158138453604
149950,149951,149950,299901,138.20247888565063,0.015554454463083543
150150,150151,150150,300301,138.47727394104004,0.01553735734315997
150350,150351,150350,300701,138.68938183784485,0.015520289939425365
150551,150552,150551,301103,138.84492015838623,0.015503167052395052
150751,150752,150751,301503,138.99984407424927,0.01548615897418229
150951,150952,150951,301903,139.15181708335876,0.015469180358174218
151151,151152,151151,302303,139.46476006507874,0.015452231120660161
151351,151352,151351,302703,139.6172649860382,0.01543531117832888
151552,151553,151552,303105,139.78192496299744,0.015418336067872964
151752,151753,151752,303505,139.93382096290588,0.015401474613000838
151952,151953,151952,303905,140.17891907691956,0.01538464220533878
152152,152153,152152,304305,140.40819215774536,0.015367838763148707
152352,152353,152352,304705,140.58041501045227,0.015351064205078464
152553,152554,152553,305107,140.74355006217957,0.015334234793617153
152753,152754,152753,305507,140.9064269065857,0.015317517904671849
152953,152954,152953,305907,141.06758999824524,0.015300829657679208
153153,153154,153153,306307,141.22729206085205,0.01528416997280646
153353,153354,153353,306707,141.43145203590393,0.015267538770593631
153554,153555,153554,307109,141.68973183631897,0.01525085302918961
153754,153755,153754,307509,141.8783519268036,0.015234278696822683
153954,153955,153954,307909,142.04777002334595,0.015217732610556657
154154,154155,154154,308309,142.21890211105347,0.015201214692399627
154354,154355,154354,308709,142.38844108581543,0.015184724864719704
154555,154556,154555,309111,142.54863381385803,0.015168180811424514
154755,154756,154755,309511,142.70023608207703,0.01515174707272128
154955,154956,154955,309911,142.91387009620667,0.015135341193355243
155155,155156,155155,310311,143.12122297286987,0.015118963097113238
155355,155356,155355,310711,143.2969090938568,0.015102612708130257
155556,155557,155556,311113,143.4691789150238,0.015086208406399376
155756,155757,155756,311513,143.6172239780426,0.015069913343315196
155956,155957,155956,311913,143.7619960308075,0.015053645761587743
156156,156157,156156,312313,143.90876126289368,0.015037405586723394
156356,156357,156356,312713,144.0804841518402,0.015021192744564978
156557,156558,156557,313115,144.28727102279663,0.015004926301738056
156757,156758,156757,313515,144.4692840576172,0.01498876803959884
156957,156958,156957,313915,144.61916399002075,0.014972636889327111
157157,157158,157157,314315,144.76444697380066,0.014956532778091695
157357,157358,157357,314715,144.91650319099426,0.01494045563338711
157558,157559,157558,315117,145.08203196525574,0.014924325199230664
157758,157759,157758,315517,145.23880410194397,0.014908301905294985
157958,157959,157958,315917,145.4051170349121,0.014892305361948495
158158,158159,158158,316317,145.5800530910492,0.014876335497968062
158358,158359,158358,316717,145.74273419380188,0.01486039224244552
158559,158560,158559,317119,145.9043550491333,0.014844396007755426
158759,158760,158759,317519,146.25039911270142,0.014828505889835244
158959,158960,158959,317919,146.4655740261078,0.014812642169168208
159159,159160,159159,318319,146.66415214538574,0.014796804776086773
159359,159360,159359,318719,146.8201081752777,0.014780993641228092
159560,159561,159560,319121,146.9780809879303,0.014765129836488408
159760,159761,159760,319521,147.15531706809998,0.014749371141625759
159960,159961,159960,319921,147.41854691505432,0.014733638498364414
160160,160161,160160,320321,147.58690404891968,0.014717931838542293
160360,160361,160360,320721,147.8507149219513,0.014702251094292056
160561,160562,160561,321123,148.14994096755981,0.014686517988388263
160761,160762,160761,321523,148.53721499443054,0.014670889001585228
160961,160962,160961,321923,148.79797315597534,0.01465528572816858
161161,161162,161161,322323,149.01392221450806,0.014639708101433143
161361,161362,161361,322723,149.1786229610443,0.014624156054959366
161562,161563,161562,323125,149.34968090057373,0.014608551953943116
161762,161763,161762,323525,149.68451523780823,0.014593050996943122
161962,161963,161962,323925,149.84952998161316,0.014577575422313457
162162,162163,162162,324325,150.012864112854,0.014562125164759954
162362,162363,162362,324725,150.16230511665344,0.01454670015926456
162563,162564,162563,325127,150.38920903205872,0.014531223405168
162763,162764,162763,325527,150.62011694908142,0.014515848835284985
162963,162964,162963,325927,150.8484091758728,0.014500499323727394
163163,163164,163163,326327,151.03194904327393,0.014485174806567074
163363,163364,163363,326727,151.23158407211304,0.014469875220143699
163564,163565,163564,327129,151.4066240787506,0.014454524189840648
163764,163765,163764,327529,151.66316199302673,0.01443927439883565
163964,163965,163964,327929,151.8793239593506,0.01442404934886278
164164,164165,164164,328329,152.04515314102173,0.014408848977317415
164364,164365,164364,328729,152.2441601753235,0.014393673221854256
164565,164566,164565,329131,152.43265104293823,0.014378446325966611
164765,164766,164765,329531,152.64070105552673,0.014363319738968011
164965,164966,164965,329931,152.79958200454712,0.014348217582249327
165165,165166,165165,330331,152.95859909057617,0.014333139794488374
165365,165366,165365,330731,153.11702704429626,0.01431808631461438
165566,165567,165566,331133,153.36847496032715,0.014302981996461298
165766,165767,165766,331533,153.7010498046875,0.01428797707092742
165966,165967,165966,331933,154.18773007392883,0.014272996271260266
166166,166167,166166,332333,154.35868906974792,0.014258039537380442
166366,166367,166366,332733,154.69493889808655,0.01424310680945244
166567,166568,166567,333135,154.96888303756714,0.01422812354404065
166767,166768,166767,333535,155.18236017227173,0.014213238768763469
166967,166968,166967,333935,155.56017112731934,0.014198377821084076
167167,167168,167167,334335,155.75552701950073,0.014183540642128204
167367,167368,167367,334735,155.92896604537964,0.014168727173257845
167568,167569,167568,335137,156.20543384552002,0.014153863466311117
167768,167769,167768,335537,156.46810293197632,0.014139097360458012
167968,167969,167968,335937,156.62174105644226,0.014124354789891257
168168,168169,168168,336337,156.86052203178406,0.014109635696905064
168368,168369,168368,336737,157.14733123779297,0.014094940024022957
168569,168570,168569,337139,157.42311310768127,0.014080194411049447
168769,168770,168769,337539,157.84897994995117,0.014065545523242238
168969,168970,168969,337939,158.2048032283783,0.014050919884187666
169169,169170,169169,338339,158.6185359954834,0.01403631743731344
169369,169370,169369,338739,158.9317979812622,0.014021738126269712
169570,169571,169570,339141,159.16430020332336,0.014007109171664653
169770,169771,169770,339541,159.3924059867859,0.01399257607909387
169970,169971,169970,339941,159.56525111198425,0.013978065954346936
170170,170171,170170,340341,159.71751403808594,0.01396357874195131
170370,170371,170370,340741,160.04846906661987,0.013949114386650249
170571,170572,170571,341143,160.39174509048462,0.013934600682833198
170771,170772,170771,341543,160.8002769947052,0.013920181990406436
170971,170972,170971,341943,161.1066062450409,0.013905785990313307
171171,171172,171171,342343,161.28786301612854,0.013891412628148622
171371,171372,171371,342743,161.44521713256836,0.013877061849716453
171572,171573,171572,343145,161.81622314453125,0.013862662016301429
171772,171773,171772,343545,161.9832468032837,0.013848356355823693
171972,171973,171972,343945,162.15621709823608,0.013834073117468116
172172,172173,172172,344345,162.3104109764099,0.013819812247865385
172372,172373,172372,344745,162.45834302902222,0.013805573693849686
172573,172574,172573,345147,162.60726499557495,0.013791286376846467
172773,172774,172773,345547,162.79657912254333,0.013777092406231706
172973,172974,172973,345947,163.13076210021973,0.013762920592652243
173173,173174,173173,346347,163.48642587661743,0.013748770883744857
173373,173374,173373,346747,163.6594569683075,0.013734643227343675
173574,173575,173574,347149,163.83354306221008,0.013720467098389266
173774,173775,173774,347549,164.02900004386902,0.013706383500901462
173974,173975,173974,347949,164.19817185401917,0.013692321800338587
174174,174175,174174,348349,164.37744808197021,0.01367828194531447
174374,174375,174374,348749,164.54338693618774,0.013664263884634634
174575,174576,174575,349151,164.7053210735321,0.013650197640253452
174775,174776,174775,349551,164.86615085601807,0.013636223123776088
174975,174976,174975,349951,165.03352189064026,0.01362227024894711
175175,175176,175175,350351,165.18846917152405,0.013608338965329427
175375,175376,175375,350751,165.35198283195496,0.013594429222672419
175576,175577,175576,351153,165.50966095924377,0.013580471583563876
175776,175777,175776,351553,165.65728998184204,0.013566604879896318
175976,175977,175976,351953,165.85201692581177,0.013552759567297087
176176,176177,176176,352353,166.03105998039246,0.013538935596251295
176376,176377,176376,352753,166.17734503746033,0.01352513291742541
176577,176578,176577,353155,166.32454895973206,0.01351128262777808
176777,176778,176777,353555,166.5005021095276,0.01349752249195837
176977,176978,176977,353955,166.65226912498474,0.013483783501190873
177177,177178,177177,354355,166.99047899246216,0.013470065606857288
177377,177378,177377,354755,167.26576805114746,0.01345636876051547
177578,177579,177578,355157,167.43769192695618,0.013442624587346162
177778,177779,177778,355557,167.6031711101532,0.01342896979699826
177978,177979,177978,355957,167.76939392089844,0.013415335910123028
178178,178179,178178,356357,167.95436692237854,0.01340172287897384
178378,178379,178378,356757,168.11885809898376,0.013388130655975128
178579,178580,178579,357159,168.28612804412842,0.013374491388492452
178779,178780,178779,357559,168.4530692100525,0.013360940743197557
178979,178980,178979,357959,168.63531303405762,0.013347410764109634
179179,179180,179179,358359,168.85060000419617,0.01333390140432948
179379,179380,179379,358759,169.2741892337799,0.01332041261712447
179580,179581,179580,359161,169.63185787200928,0.01330687706611521
179780,179781,179780,359561,169.94374108314514,0.013293429386805838
179980,179981,179980,359961,170.2794508934021,0.01328000214063301
180180,180181,180180,360361,170.44016098976135,0.013266595281521893
180380,180381,180380,360761,170.65238094329834,0.01325320876355983
180581,180582,180581,361163,170.9646019935608,0.01323977576079786
180781,180782,180781,361563,171.24908804893494,0.013226429889173861
180981,180982,180981,361963,171.53779196739197,0.013213104221697108
181181,181182,181181,362363,171.8571000099182,0.01319979871309497
181381,181382,181381,362763,172.1307249069214,0.01318651331825238
181582,181583,181582,363165,172.40933108329773,0.013173181715928505
181782,181783,181782,363565,172.6954231262207,0.013159936513894015
181982,181983,181982,363965,172.99497199058533,0.013146711290988617
182182,182183,182182,364365,173.2867729663849,0.013133506002720226
182382,182383,182382,364765,173.56283497810364,0.013120320604750199
182583,182584,182583,365167,173.86382222175598,0.013107089274922568
182783,182784,182783,365567,174.12664914131165,0.01309394362404301
182983,182984,182983,365967,174.4371621608734,0.013080817731139309
183183,183184,183183,366367,174.70014691352844,0.013067711552479296
183383,183384,183383,366767,174.95543313026428,0.013054625044480014
183584,183585,183584,367169,175.24494695663452,0.013041492878544045
183784,183785,183784,367569,175.51670718193054,0.0130284456795225
183984,183985,183984,367969,175.81583380699158,0.013015418021086265
184184,184185,184184,368369,176.07255101203918,0.013002409860242843
184384,184385,184384,368769,176.32972502708435,0.012989421154145319
184585,184586,184585,369171,176.59699892997742,0.012976387062322368
184785,184786,184785,369571,176.8660809993744,0.012963437234494451
184985,184986,184985,369971,177.13706493377686,0.012950506733525043
185185,185186,185185,370371,177.4492380619049,0.012937595517142115
185385,185386,185385,370771,177.73463821411133,0.012924703543215408
185586,185587,185586,371173,177.98808598518372,0.012911766454059235
185786,185787,185786,371573,178.251060962677,0.012898912934905625
185986,185987,185986,371973,178.51727318763733,0.012886078532452105
186186,186187,186186,372373,178.78109908103943,0.012873263205128554
186386,186387,186386,372773,179.08431696891785,0.012860466911502982
186587,186588,186587,373175,179.34046387672424,0.012847625771423796
186787,186788,186787,373575,179.61219310760498,0.012834867516099666
186987,186988,186987,373975,179.871906042099,0.012822128170793754
187187,187188,187187,374375,180.14872908592224,0.012809407694619851
187387,187388,187387,374775,180.40133714675903,0.012796706046826107
187588,187589,187588,375177,180.65937900543213,0.012783959819630803
187788,187789,187788,375577,180.9085350036621,0.012771295800512016
187988,187989,187988,375977,181.16794800758362,0.012758650488117097
188188,188189,188188,376377,181.41744303703308,0.012746023842226367
188388,188389,188388,376777,181.6872899532318,0.012733415822751162
188589,188590,188589,377179,181.9435751438141,0.012720763489199705
188789,188790,188789,377579,182.2555022239685,0.01270819269544401
188989,188990,188989,377979,182.59690594673157,0.01269564040841988
189189,189190,189189,378379,182.8854100704193,0.012683106588557138
189389,189390,189389,378779,183.15725111961365,0.012670591196413564
189590,189591,189590,379181,183.49442791938782,0.012658031753790431
189790,189791,189790,379581,183.78661799430847,0.01264555319091445
189990,189991,189990,379981,184.0613009929657,0.012633092937996618
190190,190191,190190,380381,184.33464908599854,0.012620650956100207
190390,190391,190390,380781,184.60978603363037,0.012608227206413303
190591,190592,190591,381183,184.88445401191711,0.012595759668113684
190791,190792,190791,381583,185.1632890701294,0.01258337235758367
190991,190992,190991,381983,185.4648699760437,0.012571003163377328
191191,191192,191191,382383,185.75304293632507,0.012558652047175819
191391,191392,191391,382783,186.02570009231567,0.012546318970781947
191592,191593,191592,383185,186.27959203720093,0.012533942365911765
191792,191793,191792,383585,186.54488921165466,0.01252164534474869
191992,191993,191992,383985,186.80352997779846,0.012509366249336453
192192,192193,192192,384385,187.0598659515381,0.012497105041958905
192392,192393,192392,384785,187.3183000087738,0.012484861685018573
192593,192594,192593,385187,187.5782721042633,0.012472575058008382
192793,192794,192793,385587,187.8343629837036,0.01246036737840599
192993,192994,192993,385987,188.11197113990784,0.012448177436968485
193193,193194,193193,386387,188.39670515060425,0.01243600519656792
193393,193394,193393,386787,188.71788001060486,0.012423850620191823
193594,193595,193594,387189,189.029855966568,0.0124116530304233
193794,193795,193794,387589,189.2832431793213,0.012399533759379243
193994,193995,193994,387989,189.56267714500427,0.01238743204182887
194194,194195,194194,388389,189.82626008987427,0.012375347841218022
194394,194395,194394,388789,190.09212017059326,0.012363281121105529
194595,194596,194595,389191,190.3741340637207,0.012351171642550602
194795,194796,194795,389591,190.6549220085144,0.012339139861509708
194995,194996,194995,389991,190.90519094467163,0.012327125452136108
195195,195196,195195,390391,191.16355109214783,0.012315128378435855
195395,195396,195395,390791,191.4142370223999,0.01230314860452532
195596,195597,195596,391193,191.78357315063477,0.012291126325397235
195796,195797,195796,391593,192.1901478767395,0.012279181129906532
195996,195997,195996,391993,192.5356171131134,0.012267253127034037
196196,196197,196196,392393,192.85761404037476,0.012255342281332869
196396,196397,196396,392793,193.13268613815308,0.012243448557463772
196597,196598,196597,393195,193.41151213645935,0.012231512579879523
196797,196798,196797,393595,193.67630290985107,0.012219653079254817
196997,196998,196997,393995,193.94125699996948,0.012207810594911227
197197,197198,197197,394395,194.21065711975098,0.012195985091936068
197397,197398,197397,394795,194.50506401062012,0.01218417653552182
197598,197599,197598,395197,194.85397791862488,0.012172325975175915
197798,197799,197798,395597,195.1694757938385,0.012160551292179151
197998,197999,197998,395997,195.46474027633667,0.012148793451775195
198198,198199,198198,396397,195.77117800712585,0.012137052419573156
198398,198399,198398,396797,196.05830192565918,0.01212532816128502
198599,198600,198599,397199,196.35362887382507,0.012113562147133486
198799,198800,198799,397599,196.60926222801208,0.012101871417660505
198999,199000,198999,397999,196.90903496742249,0.012090197359679635
199199,199200,199199,398399,197.18434596061707,0.012078539939309909
199399,199400,199399,398799,197.4826738834381,0.012066899122770751
199600,199601,199600,399201,197.9259111881256,0.012055216796725702
199800,199801,199800,399601,198.25263381004333,0.01204360916950424
200000,200001,200000,400001,198.56298303604126,0.012032018045202673


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007648468017578125,30.358106049564984
200,201,200,401,0.07058382034301758,1.5266697976090917
400,401,400,801,0.14265894889831543,0.9949572917608964
601,602,601,1203,0.21718192100524902,0.654469703896404
801,802,801,1603,0.28324294090270996,0.5449375577615801
1001,1002,1001,2003,0.3540990352630615,0.466558339137924
1201,1202,1201,2403,0.41872286796569824,0.40790445856812785
1401,1402,1401,2803,0.49037909507751465,0.36324839772486234
1602,1603,1602,3205,0.5683107376098633,0.332410758519307
1802,1803,1802,3605,0.6348049640655518,0.2959221037316122
2002,2003,2002,4005,0.7040529251098633,0.3178597359959202
2202,2203,2202,4405,0.7678680419921875,0.25472097014152784
2402,2403,2402,4805,0.8338320255279541,0.29365243117227025
2603,2604,2603,5207,0.8970508575439453,0.22189710215379213
2803,2804,2803,5607,0.9613039493560791,0.2068581685238522
3003,3004,3003,6007,1.0259227752685547,0.20204829271238317
3203,3204,3203,6407,1.0907468795776367,0.1826780936969815
3403,3404,3403,6807,1.172070026397705,0.17350693079852542
3604,3605,3604,7209,1.2582969665527344,0.16618529329681433
3804,3805,3804,7609,1.3289129734039307,0.1559774946123097
4004,4005,4004,8009,1.3955929279327393,0.1479860340576209
4204,4205,4204,8409,1.477985143661499,0.1420812036193549
4404,4405,4404,8809,1.5451500415802002,0.1354867762288171
4605,4606,4605,9211,1.6106619834899902,0.12804190617601624
4805,4806,4805,9611,1.683297872543335,0.14492790348498927
5005,5006,5005,10011,1.7669079303741455,0.11843714281990657
5205,5206,5205,10411,1.8366169929504395,0.1355149934683695
5405,5406,5405,10811,1.9066479206085205,0.10967509053331728
5606,5607,5606,11213,1.9756591320037842,0.1047390441099821
5806,5807,5806,11613,2.045254945755005,0.11116670419397351
6006,6007,6006,12013,2.1133010387420654,0.1104731554284347
6206,6207,6206,12413,2.188856840133667,0.11339589037345801
6406,6407,6406,12813,2.261047840118408,0.08959043022299047
6607,6608,6607,13215,2.329741954803467,0.08790212998533639
6807,6808,6807,13615,2.398026943206787,0.09725045222241159
7007,7008,7007,14015,2.4656009674072266,0.08069814582142183
7207,7208,7207,14415,2.5341639518737793,0.0779170467991856
7407,7408,7407,14815,2.605954885482788,0.07497417734907265
7608,7609,7608,15217,2.6990559101104736,0.07228850125978122
7808,7809,7808,15617,2.7877659797668457,0.0705158943683833
8008,8009,8008,16017,2.8560547828674316,0.0679033528756303
8208,8209,8208,16417,2.925092935562134,0.06556943872126361
8408,8409,8408,16817,2.9941329956054688,0.06338593380502335
8609,8610,8609,17219,3.062572717666626,0.06190721473282491
8809,8810,8809,17619,3.132429838180542,0.05959173999795306
9009,9010,9009,18019,3.2028727531433105,0.060609997754527266
9209,9210,9209,18419,3.270448923110962,0.05630214481997626
9409,9410,9409,18819,3.3394088745117188,0.055273169854554924
9610,9611,9610,19221,3.4086318016052246,0.060694624115735125
9810,9811,9810,19621,3.47737193107605,0.06022217748508646
10010,10011,10010,20021,3.5437488555908203,0.05237237177653837
10210,10211,10210,20421,3.60870099067688,0.04917242783563536
10410,10411,10410,20821,3.677323818206787,0.04802124407245041
10611,10612,10611,21223,3.751830816268921,0.04673826584019885
10811,10812,10811,21623,3.8200840950012207,0.046157854104341846
11011,11012,11011,22023,3.8845887184143066,0.04441507929785954
11211,11212,11211,22423,3.9493319988250732,0.05715923333272001
11411,11412,11411,22823,4.015138864517212,0.04361524161548882
11612,11613,11612,23225,4.083329916000366,0.04145315231159302
11812,11813,11812,23625,4.174379110336304,0.04103833274219849
12012,12013,12012,24025,4.269699811935425,0.04152388108257078
12212,12213,12212,24425,4.353366136550903,0.039097157612056385
12412,12413,12412,24825,4.431055784225464,0.037917942679045025
12613,12614,12613,25227,4.51396107673645,0.037175633239289456
12813,12814,12813,25627,4.590471029281616,0.03648102445539223
13013,13014,13013,26027,4.667370080947876,0.035984507698872216
13213,13214,13213,26427,4.766811847686768,0.0352288901109299
13413,13414,13413,26827,4.851867914199829,0.034248478249940977
13614,13615,13614,27229,4.929779052734375,0.03353697604508712
13814,13815,13814,27629,5.002672910690308,0.03819334980340488
14014,14015,14014,28029,5.079078912734985,0.0325092445410024
14214,14215,14214,28429,5.159695863723755,0.03167357404618877
14414,14415,14414,28829,5.246571063995361,0.03132145035056967
14615,14616,14615,29231,5.326661825180054,0.03841943100962133
14815,14816,14815,29631,5.393293857574463,0.03149950765100605
15015,15016,15015,30031,5.464583873748779,0.029597435605700283
15215,15216,15215,30431,5.53377103805542,0.029165739782345785
15415,15416,15415,30831,5.601186752319336,0.028491164325146364
15616,15617,15616,31233,5.671533823013306,0.02851613638181219
15816,15817,15816,31633,5.7581799030303955,0.027993301187548506
16016,16017,16016,32033,5.83270788192749,0.02703679477218751
16216,16217,16216,32433,5.9094390869140625,0.026840158619861415
16416,16417,16416,32833,5.991601943969727,0.027075123915141455
16617,16618,16617,33235,6.076669931411743,0.025867205065584178
16817,16818,16817,33635,6.153759956359863,0.02565841084456606
17017,17018,17017,34035,6.237292766571045,0.02510285720067962
17217,17218,17217,34435,6.306429862976074,0.024945733381901144
17417,17418,17417,34835,6.388155937194824,0.02460658271122539
17618,17619,17618,35237,6.45967173576355,0.024043042391285803
17818,17819,17818,35637,6.532362937927246,0.024140354635167706
18018,18019,18018,36037,6.6014978885650635,0.023224035515757097
18218,18219,18218,36437,6.674348831176758,0.02837802755604619
18418,18419,18418,36837,6.763919830322266,0.022630684792705146
18619,18620,18619,37239,6.842882871627808,0.028489056280565198
18819,18820,18819,37639,6.941777944564819,0.022012179950758437
19019,19020,19019,38039,7.02716588973999,0.021879992934182038
19219,19220,19219,38439,7.098832845687866,0.021379257636480943
19419,19420,19419,38839,7.1653358936309814,0.0211590445178449
19620,19621,19620,39241,7.248676776885986,0.02101117273983544
19820,19821,19820,39641,7.316822052001953,0.02060057744243322
20020,20021,20020,40041,7.38716197013855,0.021566496480300155
20220,20221,20220,40441,7.457338809967041,0.02329234709472489
20420,20421,20420,40841,7.5306408405303955,0.01966194102571158
20621,20622,20621,41243,7.6009838581085205,0.01939121445690968
20821,20822,20821,41643,7.686722755432129,0.021866674330809285
21021,21022,21021,42043,7.76284384727478,0.021319881520695454
21221,21222,21221,42443,7.832942962646484,0.018911686871858128
21421,21422,21421,42843,7.905105829238892,0.018525947804047094
21622,21623,21622,43245,7.989865064620972,0.018143955833611978
21822,21823,21822,43645,8.065656900405884,0.018002548560382317
22022,22023,22022,44045,8.140564918518066,0.017729104951395253
22222,22223,22222,44445,8.231756925582886,0.02169050636890875
22422,22423,22422,44845,8.305401802062988,0.017236578274391543
22623,22624,22623,45247,8.378979921340942,0.017171275398090772
22823,22824,22823,45647,8.443895816802979,0.01723805741314565
23023,23024,23023,46047,8.50954794883728,0.016654232836777864
23223,23224,23223,46447,8.603161811828613,0.01637114345988508
23423,23424,23423,46847,8.726433753967285,0.016227383642620392
23624,23625,23624,47249,8.870965003967285,0.016374949911371936
23824,23825,23824,47649,8.973904848098755,0.015916322428547805
24024,24025,24024,48049,9.084212064743042,0.015611470770124466
24224,24225,24224,48449,9.200434923171997,0.01555084344791199
24424,24425,24424,48849,9.312075138092041,0.015342097353781697
24625,24626,24625,49251,9.386159896850586,0.015391270753840378
24825,24826,24825,49651,9.456448078155518,0.015486797363564774
25025,25026,25025,50051,9.526516914367676,0.014677686574071513
25225,25226,25225,50451,9.606059074401855,0.01534233015075886
25425,25426,25425,50851,9.678344011306763,0.01556508241279493
25626,25627,25626,51253,9.752928018569946,0.014207276405747475
25826,25827,25826,51653,9.820349931716919,0.014142692041634954
26026,26027,26026,52053,9.892266988754272,0.014088435968873334
26226,26227,26226,52453,9.959378004074097,0.016665082548559758
26426,26427,26426,52853,10.028705835342407,0.013678763379293758
26627,26628,26627,53255,10.094225883483887,0.01369319682065927
26827,26828,26827,53655,10.159865856170654,0.01328961165000624
27027,27028,27027,54055,10.23310899734497,0.013220549972175111
27227,27228,27227,54455,10.29791808128357,0.013591861749911147
27427,27428,27427,54855,10.364189863204956,0.013831233353945824
27628,27629,27628,55257,10.43020486831665,0.014749725228936158
27828,27829,27828,55657,10.494779825210571,0.01256930069071054
28028,28029,28028,56057,10.556712865829468,0.012629597210061889
28228,28229,28228,56457,10.61829400062561,0.012300447149308504
28428,28429,28428,56857,10.689611911773682,0.01231187615166595
28629,28630,28629,57259,10.759116888046265,0.012458374687134907
28829,28830,28829,57659,10.823574781417847,0.014645047653422776
29029,29030,29029,58059,10.889255046844482,0.011795066129494085
29229,29230,29229,58459,10.95370078086853,0.011668990359557234
29429,29430,29429,58859,11.018799781799316,0.011615872707566222
29630,29631,29630,59261,11.08354902267456,0.011457230857455845
29830,29831,29830,59661,11.148549795150757,0.011421642485357902
30030,30031,30030,60061,11.243512868881226,0.011334904959888356
30230,30231,30230,60461,11.31685996055603,0.011225895298390203
30430,30431,30430,60861,11.38327693939209,0.010993701864656555
30631,30632,30631,61263,11.448609828948975,0.010913376892857702
30831,30832,30831,61663,11.512871026992798,0.010747762786247785
31031,31032,31031,62063,11.575301885604858,0.01073682524299021
31231,31232,31231,62463,11.63721489906311,0.010730464815948637
31431,31432,31431,62863,11.706426858901978,0.010854346578810811
31632,31633,31632,63265,11.772215843200684,0.010411782149919039
31832,31833,31832,63665,11.834995031356812,0.010152821733948561
32032,32033,32032,64065,11.899375915527344,0.010511679414757436
32232,32233,32232,64465,11.963735818862915,0.010064149640755443
32432,32433,32432,64865,12.027154922485352,0.009914715275102915
32633,32634,32633,65267,12.09280276298523,0.00977876819260044
32833,32834,32833,65667,12.155019760131836,0.011954528918934865
33033,33034,33033,66067,12.224967956542969,0.009664945259027457
33233,33234,33233,66467,12.289203882217407,0.009554960255956228
33433,33434,33433,66867,12.352880954742432,0.009444683517121213
33634,33635,33634,67269,12.416938066482544,0.009212533363045217
33834,33835,33834,67669,12.481770038604736,0.009180858805514457
34034,34035,34034,68069,12.545536994934082,0.009070482856211867
34234,34235,34234,68469,12.609080791473389,0.009000496104865696
34434,34435,34434,68869,12.677753925323486,0.010391459253913101
34635,34636,34635,69271,12.747344970703125,0.009174443415102351
34835,34836,34835,69671,12.811465978622437,0.008735193068431655
35035,35036,35035,70071,12.874258041381836,0.00928060929193001
35235,35236,35235,70471,12.93698787689209,0.008593752526951411
35435,35436,35435,70871,13.001312017440796,0.009870002714740315
35636,35637,35636,71273,13.064252853393555,0.009788365239237392
35836,35837,35836,71673,13.127983808517456,0.008403676416654269
36036,36037,36036,72073,13.199471950531006,0.008436883971701758
36236,36237,36236,72473,13.26845383644104,0.008169385430545057
36436,36437,36436,72873,13.346472978591919,0.008023441650148011
36637,36638,36637,73275,13.425243854522705,0.007995745222023636
36837,36838,36837,73675,13.488154888153076,0.007959178876352183
37037,37038,37037,74075,13.554846048355103,0.0078077471474318665
37237,37238,37237,74475,13.621104001998901,0.007775713071278348
37437,37438,37437,74875,13.690204858779907,0.007821110627525184
37638,37639,37638,75277,13.759541988372803,0.007615333998271852
37838,37839,37838,75677,13.82467007637024,0.0075492781256574475
38038,38039,38038,76077,13.891592025756836,0.00922783902817441
38238,38239,38238,76477,13.959971904754639,0.0073557743007614555
38438,38439,38438,76877,14.025761127471924,0.008778804720289588
38639,38640,38639,77279,14.090030908584595,0.007238039933108067
38839,38840,38839,77679,14.154340982437134,0.007204657438835355
39039,39040,39039,78079,14.231267929077148,0.0073630940174610705
39239,39240,39239,78479,14.297241926193237,0.007026960416637018
39439,39440,39439,78879,14.362963914871216,0.007017946115219119
39640,39641,39640,79281,14.42605972290039,0.006883763708289022
39840,39841,39840,79681,14.490798950195312,0.007184939890910387
40040,40041,40040,80081,14.555286884307861,0.006723037949343745
40240,40241,40240,80481,14.620985984802246,0.006882357757456093
40440,40441,40440,80881,14.696257829666138,0.0066258467979763555
40641,40642,40641,81283,14.789479970932007,0.006564814215815098
40841,40842,40841,81683,14.89287781715393,0.008178163031538722
41041,41042,41041,82083,14.986050844192505,0.006528907249864797
41241,41242,41241,82483,15.068204164505005,0.0063335389213702645
41441,41442,41441,82883,15.140449047088623,0.006314806052776884
41642,41643,41642,83285,15.222745895385742,0.006223445179829302
41842,41843,41842,83685,15.304805994033813,0.006199636624925208
42042,42043,42042,84085,15.392822742462158,0.0064046066167128355
42242,42243,42242,84485,15.504727840423584,0.00610804918979095
42442,42443,42442,84885,15.59882402420044,0.006041011956911219
42643,42644,42643,85287,15.683449983596802,0.0075950802945418385
42843,42844,42843,85687,15.766734838485718,0.007055789738607428
43043,43044,43043,86087,15.83751392364502,0.005834122826214432
43243,43244,43243,86487,15.912606000900269,0.00694474369668056
43443,43444,43443,86887,15.99439787864685,0.005736101214718079
43644,43645,43644,87289,16.072885036468506,0.0056928854547508186
43844,43845,43844,87689,16.148908853530884,0.005672448661857534
44044,44045,44044,88089,16.258142948150635,0.005627258336581377
44244,44245,44244,88489,16.34809184074402,0.005509747309315578
44444,44445,44444,88889,16.440847873687744,0.005473784102890646
44645,44646,44645,89291,16.529570817947388,0.0054048743362980975
44845,44846,44845,89691,16.62104892730713,0.005324414430335031
45045,45046,45045,90091,16.721986770629883,0.0052861248235699055
45245,45246,45245,90491,16.810781955718994,0.00637676824949535
45445,45446,45445,90891,16.90523076057434,0.005469393148718725
45646,45647,45646,91293,16.995255947113037,0.005210261815777803
45846,45847,45846,91693,17.075894117355347,0.005184262453052653
46046,46047,46046,92093,17.154412746429443,0.005037390976195141
46246,46247,46246,92493,17.241500854492188,0.005045379447369975
46446,46447,46446,92893,17.325258016586304,0.005448903738972202
46647,46648,46647,93295,17.408763885498047,0.004882146582864415
46847,46848,46847,93695,17.48288583755493,0.004853254380033408
47047,47048,47047,94095,17.55060887336731,0.004817968873446524
47247,47248,47247,94495,17.640344858169556,0.004796794497335832
47447,47448,47447,94895,17.732635974884033,0.004784359936242819
47648,47649,47648,95297,17.825819969177246,0.0047058598691657955
47848,47849,47848,95697,17.919836044311523,0.0047183983197354685
48048,48049,48048,96097,17.995261907577515,0.004660405774696224
48248,48249,48248,96497,18.081974744796753,0.004574980937427125
48448,48449,48448,96897,18.15975785255432,0.005159583751182835
48649,48650,48649,97299,18.236470699310303,0.004494401066177711
48849,48850,48849,97699,18.305125951766968,0.004421364876352003
49049,49050,49049,98099,18.372591972351074,0.0044448900327837635
49249,49250,49249,98499,18.4457049369812,0.004359621142493204
49449,49450,49449,98899,18.519243717193604,0.004307696151307247
49650,49651,49650,99301,18.61645197868347,0.005022210110713118
49850,49851,49850,99701,18.785408973693848,0.004242293444367986
50050,50051,50050,100101,18.859556913375854,0.004314994502392726
50250,50251,50250,100501,18.930732011795044,0.004176033581827324
50450,50451,50450,100901,18.998551845550537,0.004128143289650036
50651,50652,50651,101303,19.20180583000183,0.0041339792521615185
50851,50852,50851,101703,19.30881690979004,0.004090779154477809
51051,51052,51051,102103,19.401330947875977,0.004540151194279124
51251,51252,51251,102503,19.467595100402832,0.003997643491167043
51451,51452,51451,102903,19.540467023849487,0.004016891260842929
51652,51653,51652,103305,19.612465858459473,0.003923721621086954
51852,51853,51852,103705,19.683265924453735,0.004033590827142122
52052,52053,52052,104105,19.77008581161499,0.003854374146784114
52252,52253,52252,104505,19.849427938461304,0.00382778701247259
52452,52453,52452,104905,19.919520139694214,0.0038141899436616206
52653,52654,52653,105307,19.985893964767456,0.003747986112886527
52853,52854,52853,105707,20.05150604248047,0.004460738481297694
53053,53054,53053,106107,20.116740942001343,0.0036757285816074185
53253,53254,53253,106507,20.188909769058228,0.003637104726922998
53453,53454,53453,106907,20.256837844848633,0.003995768159929085
53654,53655,53654,107309,20.322123050689697,0.0035756642346731204
53854,53855,53854,107709,20.386443853378296,0.003573966665545678
54054,54055,54054,108109,20.453223943710327,0.0035404520710186098
54254,54255,54254,108509,20.516972064971924,0.0034997189135236814
54454,54455,54454,108909,20.60979700088501,0.0034448207345215824
54655,54656,54655,109311,20.687989950180054,0.003426571604658671
54855,54856,54855,109711,20.75858211517334,0.004015792697265188
55055,55056,55055,110111,20.825946807861328,0.003410811756743703
55255,55256,55255,110511,20.895997047424316,0.0033149110083684195
55455,55456,55455,110911,20.967813968658447,0.0038234971026624765
55656,55657,55656,111313,21.048868894577026,0.0032725110883480963
55856,55857,55856,111713,21.11504888534546,0.003225975893467207
56056,56057,56056,112113,21.1821928024292,0.0032021457962409035
56256,56257,56256,112513,21.265304803848267,0.0032830659578713508
56456,56457,56456,112913,21.336288928985596,0.00313358158283242
56657,56658,56657,113315,21.40790295600891,0.0031038112335010836
56857,56858,56857,113715,21.475820064544678,0.003068666183747005
57057,57058,57057,114115,21.54113483428955,0.0030822686207365277
57257,57258,57257,114515,21.61165690422058,0.003164432014817304
57457,57458,57457,114915,21.68510890007019,0.003050757363447427
57658,57659,57658,115317,21.761884927749634,0.0029547128947588278
57858,57859,57858,115717,21.831382036209106,0.0029595848542652054
58058,58059,58058,116117,21.917004823684692,0.002948310317680173
58258,58259,58258,116517,21.997490882873535,0.0028914202693623367
58458,58459,58458,116917,22.06484580039978,0.0028542302821310877
58659,58660,58659,117319,22.1301908493042,0.0028519728113630865
58859,58860,58859,117719,22.195585012435913,0.0028124123956395175
59059,59060,59059,118119,22.263853788375854,0.003193031212689097
59259,59260,59259,118519,22.327585697174072,0.00278173229810129
59459,59460,59459,118919,22.390971899032593,0.0027773343329458217
59660,59661,59660,119321,22.454447984695435,0.0026988259601007573
59860,59861,59860,119721,22.51838707923889,0.0027471317469777118
60060,60061,60060,120121,22.582087993621826,0.003181692819311271
60260,60261,60260,120521,22.64557385444641,0.002669606356282548
60460,60461,60460,120921,22.7260160446167,0.002624876205875502
60661,60662,60661,121323,22.816571950912476,0.0025962358122678915
60861,60862,60861,121723,22.89116096496582,0.0028076605843462324
61061,61062,61061,122123,22.95526695251465,0.0028074716422748073
61261,61262,61261,122523,23.019766092300415,0.00254828190463533
61461,61462,61461,122923,23.084678888320923,0.00318563405813102
61662,61663,61662,123325,23.150120973587036,0.0024778961399352724
61862,61863,61862,123725,23.223878860473633,0.0029140708423549704
62062,62063,62062,124125,23.299428939819336,0.002452993365505163
62262,62263,62262,124525,23.36921191215515,0.0024264842511566515
62462,62463,62462,124925,23.434172868728638,0.0023942474532321536
62663,62664,62663,125327,23.507672786712646,0.002441924424476341
62863,62864,62863,125727,23.5724880695343,0.0023417762048479358
63063,63064,63063,126127,23.64223599433899,0.002833884411476546
63263,63264,63263,126527,23.711061000823975,0.002357950099527221
63463,63464,63463,126927,23.783836841583252,0.0023047279434673796
63664,63665,63664,127329,23.852894067764282,0.0022688397453119328
63864,63865,63864,127729,23.917147874832153,0.002308256475268803
64064,64065,64064,128129,24.010740041732788,0.002582592843548127
64264,64265,64264,128529,24.151176929473877,0.002226765580596944
64464,64465,64464,128929,24.251598834991455,0.0021978579451071172
64665,64666,64665,129331,24.33493399620056,0.0021853380456726035
64865,64866,64865,129731,24.404742002487183,0.002604607519962246
65065,65066,65065,130131,24.474050760269165,0.0021531408089884613
65265,65266,65265,130531,24.54742980003357,0.0021206520081071887
65465,65466,65465,130931,24.613870859146118,0.002086560712841971
65666,65667,65666,131333,24.68449091911316,0.002165790937774461
65866,65867,65866,131733,24.75597381591797,0.0023925285189972524
66066,66067,66066,132133,24.823237895965576,0.0023525402657535114
66266,66267,66266,132533,24.893287897109985,0.0023846004288762546
66466,66467,66466,132933,24.960285902023315,0.001992598457079472
66667,66668,66667,133335,25.02826189994812,0.002337947473440871
66867,66868,66867,133735,25.09685492515564,0.0021039676693394155
67067,67068,67067,134135,25.164212942123413,0.0019623741433012825
67267,67268,67267,134535,25.236160039901733,0.0019258740897910005
67467,67468,67467,134935,25.302230834960938,0.0019376569302019043
67668,67669,67668,135337,25.372169971466064,0.001911136566718753
67868,67869,67868,135737,25.438562870025635,0.001891672979873212
68068,68069,68068,136137,25.504350900650024,0.0018745668576293179
68268,68269,68268,136537,25.570355892181396,0.0018530288909395798
68468,68469,68468,136937,25.63900089263916,0.001837330898563454
68669,68670,68669,137339,25.749825716018677,0.0018137680102064703
68869,68870,68869,137739,25.867790937423706,0.0017969900262357198
69069,69070,69069,138139,25.967891931533813,0.0018039159747469103
69269,69270,69269,138539,26.042635917663574,0.001770846421773793
69469,69470,69469,138939,26.119290828704834,0.00207024027663629
69670,69671,69670,139341,26.207242012023926,0.0018858783838663878
69870,69871,69870,139741,26.293115854263306,0.0017299934099322858
70070,70071,70070,140141,26.36950993537903,0.0017123410169292488
70270,70271,70270,140541,26.449445962905884,0.0017040543167285227
70470,70471,70470,140941,26.525012016296387,0.0016892286019085452
70671,70672,70671,141343,26.597505807876587,0.0016711880487108768
70871,70872,70871,141743,26.666029930114746,0.0016556449301216329
71071,71072,71071,142143,26.82124900817871,0.0016554248251239646
71271,71272,71271,142543,26.927687883377075,0.0016215431188463794
71471,71472,71471,142943,27.0234477519989,0.0016102418672560433
71672,71673,71672,143345,27.096342086791992,0.0015974073694012484
71872,71873,71872,143745,27.164005994796753,0.001578047951775619
72072,72073,72072,144145,27.247804880142212,0.001648645113678236
72272,72273,72272,144545,27.317007780075073,0.0015686714573804894
72472,72473,72472,144945,27.388449907302856,0.0016259957829209304
72673,72674,72673,145347,27.454643964767456,0.0015339215429024933
72873,72874,72873,145747,27.520258903503418,0.0017087978179110028
73073,73074,73073,146147,27.587308883666992,0.0014991866267269245
73273,73274,73273,146547,27.654689073562622,0.0014865607022882153
73473,73474,73473,146947,27.729750871658325,0.0014810440750317052
73674,73675,73674,147349,27.796249866485596,0.0014696465353717996
73874,73875,73874,147749,27.863275051116943,0.0014498492895373702
74074,74075,74074,148149,27.929237127304077,0.0014344159097007775
74274,74275,74274,148549,27.99513602256775,0.0014283313859918445
74474,74475,74474,148949,28.062901973724365,0.001491166883556748
74675,74676,74675,149351,28.12894296646118,0.0014157961336949336
74875,74876,74875,149751,28.211358070373535,0.0013898441223984133
75075,75076,75075,150151,28.285249710083008,0.0013650476288958441
75275,75276,75275,150551,28.36661195755005,0.0013784488199792759
75475,75476,75475,150951,28.45638394355774,0.0015164276592423446
75676,75677,75676,151353,28.534773111343384,0.0013289431458864361
75876,75877,75876,151753,28.599914073944092,0.0013325628600834502
76076,76077,76076,152153,28.668128967285156,0.0013213682093171186
76276,76277,76276,152553,28.74641990661621,0.0015468465679421067
76476,76477,76476,152953,28.813735961914062,0.0013148445430109102
76677,76678,76677,153355,28.880621910095215,0.0012853842079396524
76877,76878,76877,153755,28.947283029556274,0.001320721497792898
77077,77078,77077,154155,29.020328044891357,0.0012861340208206746
77277,77278,77277,154555,29.090600967407227,0.0014294178260157717
77477,77478,77477,154955,29.252268075942993,0.0012499461922213144
77678,77679,77678,155357,29.37106680870056,0.0012171055006695505
77878,77879,77878,155757,29.46290373802185,0.0012131845461831254
78078,78079,78078,156157,29.5429368019104,0.001203724167682169
78278,78279,78278,156557,29.609725952148438,0.0012029701152497963
78478,78479,78478,156957,29.68287992477417,0.0013968161589793567
78679,78680,78679,157359,29.76009202003479,0.0011711489114842977
78879,78880,78879,157759,29.82782793045044,0.0011666695324699192
79079,79080,79079,158159,29.89389705657959,0.0011939322695306825
79279,79280,79279,158559,29.96120285987854,0.0011572430973980875
79479,79480,79479,158959,30.025644779205322,0.0011822069778385919
79680,79681,79680,159361,30.092138051986694,0.0011191015910363014
79880,79881,79880,159761,30.158751010894775,0.0011296573052424674
80080,80081,80080,160161,30.23062777519226,0.0011143579502772409
80280,80281,80280,160561,30.296111822128296,0.0011636204332137114
80480,80481,80480,160961,30.362751007080078,0.0012157709469575808
80681,80682,80681,161363,30.43578290939331,0.0010721082027020353
80881,80882,80881,161763,30.51568102836609,0.0010744123509593773
81081,81082,81081,162163,30.586927890777588,0.0011354488638184678
81281,81282,81281,162563,30.65473175048828,0.0010638817804371173
81481,81482,81481,162963,30.738807916641235,0.0010450378790161315
81682,81683,81682,163365,30.804508924484253,0.0010270518758330998
81882,81883,81882,163765,30.872061014175415,0.0010161208792489568
82082,82083,82082,164165,30.942807912826538,0.0011430844999268841
82282,82283,82282,164565,31.011684894561768,0.0010077093732481514
82482,82483,82482,164965,31.07704997062683,0.001010810569371863
82683,82684,82683,165367,31.143462896347046,0.0011804711262358462
82883,82884,82883,165767,31.213510990142822,0.0011773922194710325
83083,83084,83083,166167,31.28351378440857,0.0009733440183544112
83283,83284,83283,166567,31.352479934692383,0.0009605642811630366
83483,83484,83483,166967,31.421129941940308,0.0009664882428141598
83684,83685,83684,167369,31.491182804107666,0.0009448851639991226
83884,83885,83884,167769,31.59106683731079,0.0011003214330268336
84084,84085,84084,168169,31.66012692451477,0.0009265574902956548
84284,84285,84284,168569,31.737135887145996,0.0009652703345799466
84484,84485,84484,168969,31.82335090637207,0.00091640678821691
84685,84686,84685,169371,31.901907920837402,0.0009285919016374308
84885,84886,84885,169771,31.968256950378418,0.0009248315463882673
85085,85086,85085,170171,32.03635597229004,0.001059902085054254
85285,85286,85285,170571,32.10348296165466,0.0008905256652327223
85485,85486,85485,170971,32.17238402366638,0.0009701047042841164
85686,85687,85686,171373,32.24503779411316,0.0008651777349804145
85886,85887,85886,171773,32.310100078582764,0.0008680604197107588
86086,86087,86086,172173,32.37353301048279,0.0008565030322585804
86286,86287,86286,172573,32.43905186653137,0.0008448046842769668
86486,86487,86486,172973,32.50310683250427,0.0008387022794562168
86687,86688,86687,173375,32.57859492301941,0.000875066704367894
86887,86888,86887,173775,32.659955978393555,0.0010023588171795435
87087,87088,87087,174175,32.73519587516785,0.0008295156535442173
87287,87288,87287,174575,32.80304193496704,0.0008175970618709544
87487,87488,87487,174975,32.86812973022461,0.0008052802023323822
87688,87689,87688,175377,32.935343980789185,0.0008000983363289993
87888,87889,87888,175777,33.00088882446289,0.0008014624912253244
88088,88089,88088,176177,33.06593680381775,0.0007866351780767682
88288,88289,88288,176577,33.13161611557007,0.0007794580165739173
88488,88489,88488,176977,33.211360931396484,0.0007788527266861594
88689,88690,88689,177379,33.27821493148804,0.0007671347477646322
88889,88890,88889,177779,33.34786891937256,0.0007561657409285105
89089,89090,89089,178179,33.438294887542725,0.0007483303111641605
89289,89290,89289,178579,33.50483798980713,0.0007490567879696018
89489,89490,89489,178979,33.56978893280029,0.0007829541762407832
89690,89691,89690,179381,33.63518810272217,0.0007363015416707622
89890,89891,89890,179781,33.70776295661926,0.0007231589573518299
90090,90091,90090,180181,33.77466893196106,0.000730531819713983
90290,90291,90290,180581,33.83894991874695,0.0007225465148316321
90490,90491,90490,180981,33.90539503097534,0.0007143109795995234
90691,90692,90691,181383,33.97271394729614,0.0008081588432625499
90891,90892,90891,181783,34.03639197349548,0.0007453443755951767
91091,91092,91091,182183,34.10164475440979,0.0009470296869915553
91291,91292,91291,182583,34.16637086868286,0.0006863479038542696
91491,91492,91491,182983,34.24159383773804,0.0006805103096089165
91692,91693,91692,183385,34.30829191207886,0.0006748041521433704
91892,91893,91892,183785,34.37256193161011,0.0006659536155933086
92092,92093,92092,184185,34.43748092651367,0.0006825730077668522
92292,92293,92292,184585,34.51169395446777,0.0008026629843615761
92492,92493,92492,184985,34.64661002159119,0.0006553079695202399
92693,92694,92693,185387,34.75331687927246,0.0006503418122260605
92893,92894,92893,185787,34.84022498130798,0.0006413345148204258
93093,93094,93093,186187,34.915302991867065,0.0006336012382768772
93293,93294,93293,186587,34.991076946258545,0.000706838769011653
93493,93494,93493,186987,35.08476972579956,0.0006283195705348358
93694,93695,93694,187389,35.157965898513794,0.0006209445123949274
93894,93895,93894,187789,35.23479890823364,0.0006128555084708953
94094,94095,94094,188189,35.313117027282715,0.0006117315879973153
94294,94295,94294,188589,35.389585971832275,0.0006033332826324221
94494,94495,94494,188989,35.45924687385559,0.0006224920253842942
94695,94696,94695,189391,35.526110887527466,0.0005938602037109243
94895,94896,94895,189791,35.591460943222046,0.0005987093636249723
95095,95096,95095,190191,35.662808895111084,0.0005900435391081641
95295,95296,95295,190591,35.76694989204407,0.0005872105580052622
95495,95496,95495,190991,35.84499788284302,0.0005798798529917621
95696,95697,95696,191393,35.91755700111389,0.00057690175363858
95896,95897,95896,191793,35.994006872177124,0.0005641953689872038
96096,96097,96096,192193,36.06928896903992,0.0005812790334422416
96296,96297,96296,192593,36.1491117477417,0.0005584327763594603
96496,96497,96496,192993,36.231634855270386,0.0005564439260513722
96697,96698,96697,193395,36.308435916900635,0.0005504497653999888
96897,96898,96897,193795,36.385339975357056,0.0005360268359049048
97097,97098,97097,194195,36.45727586746216,0.0006468484726535112
97297,97298,97297,194595,36.52602791786194,0.0005375701727467738
97497,97498,97497,194995,36.59143781661987,0.0005262813840142763
97698,97699,97698,195397,36.65985703468323,0.0005258084264976563
97898,97899,97898,195797,36.73699998855591,0.0005711344108401231
98098,98099,98098,196197,36.80221486091614,0.0005999564651891176
98298,98299,98298,196597,36.882944107055664,0.0005174432666217847
98498,98499,98498,196997,36.9634907245636,0.0005149795138194943
98699,98700,98699,197399,37.03633379936218,0.0005031968920002441
98899,98900,98899,197799,37.103511810302734,0.0005266223574202575
99099,99100,99099,198199,37.169431924819946,0.0004909474612806615
99299,99300,99299,198599,37.244560956954956,0.0005768510059589779
99499,99500,99499,198999,37.31195592880249,0.0004838628707059759
99700,99701,99700,199401,37.38048791885376,0.00048621886713974403
99900,99901,99900,199801,37.4457049369812,0.00047859867076574563
100100,100101,100100,200201,37.51304507255554,0.0005093230922730786
100300,100301,100300,200601,37.580482721328735,0.0005452480449979306
100501,100502,100501,201003,37.64610695838928,0.00046411700233118993
100701,100702,100701,201403,37.72410988807678,0.0005273829662152502
100901,100902,100901,201803,37.790788888931274,0.00045771420397045756
101101,101102,101101,202203,37.85646295547485,0.00045371688074914376
101301,101302,101301,202603,37.920788049697876,0.00045324498048581157
101502,101503,101502,203005,37.99383997917175,0.00044891638162703265
101702,101703,101702,203405,38.057262897491455,0.00044276882321106096
101902,101903,101902,203805,38.119335889816284,0.00043991763267018475
102102,102103,102102,204205,38.18784284591675,0.0004341588763127202
102302,102303,102302,204605,38.25527286529541,0.0004995534290153268
102503,102504,102503,205007,38.31994605064392,0.0004280087043108906
102703,102704,102703,205407,38.395545959472656,0.00042676931478402054
102903,102904,102903,205807,38.459924936294556,0.0004200103882236883
103103,103104,103103,206207,38.52315282821655,0.00042058750693246453
103303,103304,103303,206607,38.58637595176697,0.0004730756125101285
103504,103505,103504,207009,38.648892879486084,0.00040884644695077737
103704,103705,103704,207409,38.71822500228882,0.00041280217148092195
103904,103905,103904,207809,38.78163003921509,0.000485063812090237
104104,104105,104104,208209,38.84443187713623,0.0003993037801619884
104304,104305,104304,208609,38.90769290924072,0.00039658590979544365
104505,104506,104505,209011,38.979599952697754,0.00041561692300329424
104705,104706,104705,209411,39.059484004974365,0.00040630497048711365
104905,104906,104905,209811,39.12865114212036,0.0003925000042432693
105105,105106,105105,210211,39.2020218372345,0.0004656458797485168
105305,105306,105305,210611,39.26526498794556,0.00038922669148773806
105506,105507,105506,211013,39.327977895736694,0.0003776014906903302
105706,105707,105706,211413,39.39116811752319,0.0003729140047258833
105906,105907,105906,211813,39.453896045684814,0.0003744338502468438
106106,106107,106106,212213,39.51564693450928,0.0003721521331152258
106306,106307,106306,212613,39.57726287841797,0.00036792596837777793
106507,106508,106507,213015,39.640625,0.0003618501557837311
106707,106708,106707,213415,39.71079993247986,0.0003574074158582934
106907,106908,106907,213815,39.77424192428589,0.00036173967681687086
107107,107108,107107,214215,39.83814883232117,0.0003692788365756077
107307,107308,107307,214615,39.90148401260376,0.00035124457813046555
107508,107509,107508,215017,39.96787691116333,0.0003806432753762807
107708,107709,107708,215417,40.03036284446716,0.0003468769586082119
107908,107909,107908,215817,40.09519386291504,0.00034768591092550276
108108,108109,108108,216217,40.15775799751282,0.0003894305694058081
108308,108309,108308,216617,40.22933292388916,0.0003376787571690502
108509,108510,108509,217019,40.29369306564331,0.00033419879609328555
108709,108710,108709,217419,40.35649394989014,0.000340119642561156
108909,108910,108909,217819,40.41839599609375,0.0003495444154893001
109109,109110,109109,218219,40.48121976852417,0.00032450634771038816
109309,109310,109309,218619,40.54380393028259,0.00037054407615513243
109510,109511,109510,219021,40.6086699962616,0.0003199344625380786
109710,109711,109710,219421,40.674763917922974,0.00032797617539243756
109910,109911,109910,219821,40.74669790267944,0.00031848523012838935
110110,110111,110110,220221,40.80939197540283,0.00036160632052969447
110310,110311,110310,220621,40.8718957901001,0.00032356089159483027
110511,110512,110511,221023,40.93637299537659,0.0003045955283471815
110711,110712,110711,221423,40.9999098777771,0.0003057225511695573
110911,110912,110911,221823,41.065775871276855,0.00040580979723856995
111111,111112,111111,222223,41.147236824035645,0.00029872505376238366
111311,111312,111311,222623,41.227372884750366,0.0002983452908101658
111512,111513,111512,223025,41.293051958084106,0.0002921991658618583
111712,111713,111712,223425,41.35870289802551,0.0002920190499410021
111912,111913,111912,223825,41.42456674575806,0.0002988139353219697
112112,112113,112112,224225,41.49069690704346,0.00029122983914017363
112312,112313,112312,224625,41.55626392364502,0.00028547472690218387
112513,112514,112513,225027,41.62075185775757,0.00029322007910188847
112713,112714,112713,225427,41.695317029953,0.00028415621452410327
112913,112914,112913,225827,41.76138091087341,0.00028034909040907914
113113,113114,113113,226227,41.82507300376892,0.0002862537698865424
113313,113314,113313,226627,41.889673948287964,0.00027207281238986376
113514,113515,113514,227029,41.95430779457092,0.000271094254250346
113714,113715,113714,227429,42.019113063812256,0.0003186256043844505
113914,113915,113914,227829,42.084091901779175,0.0002940680931066336
114114,114115,114114,228229,42.14868783950806,0.00026589660364078287
114314,114315,114314,228629,42.21989393234253,0.0003112575460793506
114515,114516,114515,229031,42.28494071960449,0.0002622830677987649
114715,114716,114715,229431,42.35090494155884,0.00026069893989963785
114915,114916,114915,229831,42.41645073890686,0.00025561258378783763
115115,115116,115115,230231,42.48042893409729,0.0002650900876431717
115315,115316,115315,230631,42.544599771499634,0.000251187410798559
115516,115517,115516,231033,42.60983681678772,0.0002589538945950648
115716,115717,115716,231433,42.67655086517334,0.00025833014521034454
115916,115917,115916,231833,42.74566102027893,0.00028810770226381097
116116,116117,116116,232233,42.80987811088562,0.00025000880134558453
116316,116317,116316,232633,42.875152826309204,0.00024181192021742608
116517,116518,116517,233035,42.93953490257263,0.00024206343260350897
116717,116718,116717,233435,43.00589394569397,0.00023664808074604134
116917,116918,116917,233835,43.06930994987488,0.00023643825461349655
117117,117118,117117,234235,43.13277292251587,0.0002347528403456462
117317,117318,117317,234635,43.20738482475281,0.0002316841126644065
117518,117519,117518,235037,43.30873203277588,0.00022917684722461584
117718,117719,117718,235437,43.384952783584595,0.00023571330638898834
117918,117919,117918,235837,43.47274875640869,0.00023293782471396992
118118,118119,118118,236237,43.55723977088928,0.00023206164036119505
118318,118319,118318,236637,43.6293568611145,0.00023228138934603245
118519,118520,118519,237039,43.6984589099884,0.0002727569651125273
118719,118720,118719,237439,43.77105689048767,0.00021787300175039707
118919,118920,118919,237839,43.84252691268921,0.0002595203062734971
119119,119120,119119,238239,43.91203308105469,0.00024078617837036817
119319,119320,119319,238639,43.9750919342041,0.00021417634608272707
119520,119521,119520,239041,44.044665813446045,0.00024361903579351283
119720,119721,119720,239441,44.12766480445862,0.00020939717310639164
119920,119921,119920,239841,44.22193384170532,0.00021076439761725846
120120,120121,120120,240241,44.315502882003784,0.00020444864485875212
120320,120321,120320,240641,44.41967010498047,0.0002037651599473274
120521,120522,120521,241043,44.505435943603516,0.00020219273679139798
120721,120722,120721,241443,44.585729122161865,0.00020061219543260895
120921,120922,120921,241843,44.66915988922119,0.00020408220176145676
121121,121122,121121,242243,44.7483549118042,0.00020778093101333895
121321,121322,121321,242643,44.82202506065369,0.00019472973647033083
121522,121523,121522,243045,44.899247884750366,0.0001938774921903541
121722,121723,121722,243445,44.970491886138916,0.000192182138278952
121922,121923,121922,243845,45.036351919174194,0.00019126463450956665
122122,122123,122122,244245,45.103529930114746,0.0001888029252405674
122322,122323,122322,244645,45.17131590843201,0.0001923083039550761
122523,122524,122523,245047,45.247586727142334,0.00018670612531901428
122723,122724,122723,245447,45.32976484298706,0.00018473246330555834
122923,122924,122923,245847,45.489752769470215,0.00018204205253217188
123123,123124,123123,246247,45.582329988479614,0.00022656400138616766
123323,123324,123323,246647,45.67662501335144,0.00018368106136972635
123524,123525,123524,247049,45.74907088279724,0.00017869721073357302
123724,123725,123724,247449,45.86841702461243,0.00017872187989690147
123924,123925,123924,247849,45.942789793014526,0.0001769575066423175
124124,124125,124124,248249,46.02781701087952,0.0001739732840351933
124324,124325,124324,248649,46.09930992126465,0.00017260085259708987
124525,124526,124525,249051,46.163562059402466,0.00017445859572388155
124725,124726,124725,249451,46.232691049575806,0.00018882061041088186
124925,124926,124925,249851,46.2977659702301,0.0001673700468897207
125125,125126,125125,250251,46.363986015319824,0.0001672240356612481
125325,125326,125325,250651,46.42899203300476,0.00018962410112142368
125526,125527,125526,251053,46.49412417411804,0.00016421675173464224
125726,125727,125726,251453,46.56040406227112,0.00019649398922978032
125926,125927,125926,251853,46.625303745269775,0.0001654520561215418
126126,126127,126126,252253,46.70616388320923,0.0001626108975080058
126326,126327,126326,252653,46.7737820148468,0.00018690661512672956
126527,126528,126527,253055,46.83810591697693,0.00016468691847333758
126727,126728,126727,253455,46.90501880645752,0.0001564688083674855
126927,126928,126927,253855,46.97080612182617,0.0001840954686455205
127127,127128,127127,254255,47.036515951156616,0.00017376515485707198
127327,127328,127327,254655,47.102067947387695,0.00015146344895175268
127528,127529,127528,255057,47.168529987335205,0.00015935304609455208
127728,127729,127728,255457,47.24303698539734,0.0001497470880243413
127928,127929,127928,255857,47.31846499443054,0.00014809913545038429
128128,128129,128128,256257,47.4066059589386,0.000149256290112432
128328,128329,128328,256657,47.475172996520996,0.0001471485472175194
128529,128530,128529,257059,47.54940605163574,0.00014502711338056816
128729,128730,128729,257459,47.63383984565735,0.00014457830352967364
128929,128930,128929,257859,47.71554493904114,0.00016347542788958572
129129,129130,129129,258259,47.785337924957275,0.00016660390842092158
129329,129330,129329,258659,47.8507719039917,0.00014167591996885868
129530,129531,129530,259061,47.918423891067505,0.00013921868339999437
129730,129731,129730,259461,47.994534969329834,0.00013952844089690482
129930,129931,129930,259861,48.10513210296631,0.00013691912705496995
130130,130131,130130,260261,48.23697209358215,0.00013567999040744826
130330,130331,130330,260661,48.325045108795166,0.00016897389028923767
130531,130532,130531,261063,48.411322832107544,0.0001323561823563359
130731,130732,130731,261463,48.47838377952576,0.00013312171444892666
130931,130932,130931,261863,48.54245209693909,0.0001387492538816508
131131,131132,131131,262263,48.61523103713989,0.00012959465072680596
131331,131332,131331,262663,48.68899583816528,0.00012987401090343534
131532,131533,131532,263065,48.75428581237793,0.0001311729586442298
131732,131733,131732,263465,48.82112693786621,0.00015364622017195276
131932,131933,131932,263865,48.885615825653076,0.00013999881335071294
132132,132133,132132,264265,48.95142197608948,0.00013518138362311353
132332,132333,132332,264665,49.02133297920227,0.00012336901765903064
132533,132534,132533,265067,49.10306906700134,0.00012375024302195965
132733,132734,132733,265467,49.17459988594055,0.00012196954970905207
132933,132934,132933,265867,49.25077676773071,0.00012043612322105873
133133,133134,133133,266267,49.31604194641113,0.00011981585083038713
133333,133334,133333,266667,49.3808319568634,0.0001198250690442835
133534,133535,133534,267069,49.44689702987671,0.00011961563522740877
133734,133735,133734,267469,49.51091694831848,0.00011752697316186241
133934,133935,133934,267869,49.57864785194397,0.0001166181711923264
134134,134135,134134,268269,49.64753580093384,0.0001160422312848565
134334,134335,134334,268669,49.74508190155029,0.00011392885901520261
134535,134536,134535,269071,49.89667987823486,0.00011373807145986395
134735,134736,134735,269471,49.986222982406616,0.00012856258416784401
134935,134936,134935,269871,50.07552170753479,0.00011339916194495924
135135,135136,135135,270271,50.14086890220642,0.00011379903715873143
135335,135336,135335,270671,50.212599754333496,0.00011001481322224674
135536,135537,135536,271073,50.28650879859924,0.00011679720869627482
135736,135737,135736,271473,50.35615277290344,0.00010763387762289136
135936,135937,135936,271873,50.4236319065094,0.00013187356045771343
136136,136137,136136,272273,50.49057579040527,0.00010654864477437506
136336,136337,136336,272673,50.55665683746338,0.00013258091895106274
136537,136538,136537,273075,50.62621593475342,0.00010646439757504464
136737,136738,136737,273475,50.698668003082275,0.00010389703825020822
136937,136938,136937,273875,50.768314838409424,0.00010299086095545126
137137,137138,137137,274275,50.83277177810669,0.0001021330450886693
137337,137338,137337,274675,50.89908576011658,0.00010217630618454856
137538,137539,137538,275077,50.963984966278076,0.00010166933861882493
137738,137739,137738,275477,51.031566858291626,9.897784705146196e-05
137938,137939,137938,275877,51.09869194030762,9.853501545935032e-05
138138,138139,138138,276277,51.16286897659302,9.874414059854649e-05
138338,138339,138338,276677,51.23936891555786,0.00010291121056961455
138539,138540,138539,277079,51.304250955581665,9.582742988463976e-05
138739,138740,138739,277479,51.37292504310608,9.653339325814909e-05
138939,138940,138939,277879,51.44041991233826,0.00010312680411150754
139139,139140,139139,278279,51.505654096603394,9.37560019873352e-05
139339,139340,139339,278679,51.57122588157654,9.371176399321355e-05
139540,139541,139540,279081,51.63642978668213,9.174452155919e-05
139740,139741,139740,279481,51.71177697181702,9.194929497338977e-05
139940,139941,139940,279881,51.775707960128784,9.092507693284067e-05
140140,140141,140140,280281,51.85531187057495,9.002930812843955e-05
140340,140341,140340,280681,51.93307089805603,9.949210621541076e-05
140541,140542,140541,281083,51.998334884643555,8.783333304017521e-05
140741,140742,140741,281483,52.066540002822876,8.824524089881631e-05
140941,140942,140941,281883,52.13166809082031,0.00010429493791617036
141141,141142,141141,282283,52.20343613624573,8.875151496493305e-05
141341,141342,141341,282683,52.26841711997986,8.586632713388242e-05
141542,141543,141542,283085,52.335808992385864,8.500046136241476e-05
141742,141743,141742,283485,52.40011286735535,8.537487712826522e-05
141942,141943,141942,283885,52.46521186828613,9.783945090103757e-05
142142,142143,142142,284285,52.52998900413513,8.382210024623598e-05
142342,142343,142342,284685,52.59608292579651,8.255641495883449e-05
142543,142544,142543,285087,52.660836935043335,9.484831784373542e-05
142743,142744,142743,285487,52.73432397842407,8.624334365519478e-05
142943,142944,142943,285887,52.80699396133423,8.050110647744244e-05
143143,143144,143143,286287,52.87541198730469,7.962263428846227e-05
143343,143344,143343,286687,52.93836808204651,9.523532753013052e-05
143544,143545,143544,287089,53.00574994087219,7.894442558028543e-05
143744,143745,143744,287489,53.0689480304718,7.854699685926919e-05
143944,143945,143944,287889,53.13272976875305,7.797565308734925e-05
144144,144145,144144,288289,53.199896812438965,8.956701960178264e-05
144344,144345,144344,288689,53.26440405845642,7.60104307585942e-05
144545,144546,144545,289091,53.32704997062683,7.612520764377942e-05
144745,144746,144745,289491,53.3878059387207,7.476055761411095e-05
144945,144946,144945,289891,53.451897859573364,7.365727497367591e-05
145145,145146,145145,290291,53.51666784286499,7.357659630272369e-05
145345,145346,145345,290691,53.57898497581482,7.292173248920831e-05
145546,145547,145546,291093,53.64110493659973,7.244695901604426e-05
145746,145747,145746,291493,53.70946002006531,7.150598810829629e-05
145946,145947,145946,291893,53.77152991294861,7.190262367510043e-05
146146,146147,146146,292293,53.83381414413452,7.091588383066895e-05
146346,146347,146346,292693,53.89574980735779,7.070186259317419e-05
146547,146548,146547,293095,53.96789574623108,6.980497573878492e-05
146747,146748,146747,293495,54.04617786407471,6.865439936298941e-05
146947,146948,146947,293895,54.1124370098114,7.029299049303743e-05
147147,147148,147147,294295,54.175220012664795,6.813462482619054e-05
147347,147348,147347,294695,54.24706792831421,6.761817277109127e-05
147548,147549,147548,295097,54.31199598312378,7.229710238902535e-05
147748,147749,147748,295497,54.37777805328369,6.618031424898521e-05
147948,147949,147948,295897,54.44094896316528,7.590045673125923e-05
148148,148149,148148,296297,54.504169940948486,6.563465571551925e-05
148348,148349,148348,296697,54.56735706329346,6.42599719903498e-05
148549,148550,148549,297099,54.63081693649292,6.593522288403782e-05
148749,148750,148749,297499,54.70032286643982,6.325158291457148e-05
148949,148950,148949,297899,54.76271080970764,6.357234306901179e-05
149149,149150,149149,298299,54.82577109336853,6.247986568539039e-05
149349,149350,149349,298699,54.88940501213074,7.559154613027303e-05
149550,149551,149550,299101,54.95313382148743,6.155013848095213e-05
149750,149751,149750,299501,55.016305923461914,6.121710661037563e-05
149950,149951,149950,299901,55.07974410057068,6.0689623661091054e-05
150150,150151,150150,300301,55.14231204986572,6.043805943900582e-05
150350,150351,150350,300701,55.21337080001831,6.389810328122044e-05
150551,150552,150551,301103,55.277997732162476,5.9505227477730134e-05
150751,150752,150751,301503,55.34183192253113,5.8558413861974257e-05
150951,150952,150951,301903,55.405694007873535,5.7695682747601486e-05
151151,151152,151151,302303,55.46881175041199,5.821052533332896e-05
151351,151352,151351,302703,55.532275915145874,7.055893709483815e-05
151552,151553,151552,303105,55.59876894950867,5.663685507499758e-05
151752,151753,151752,303505,55.66244101524353,6.46073997313166e-05
151952,151953,151952,303905,55.733946800231934,5.5498772173815967e-05
152152,152153,152152,304305,55.7957718372345,5.685822681347772e-05
152352,152353,152352,304705,55.861167907714844,6.335323923990663e-05
152553,152554,152553,305107,55.92494177818298,5.4643817163495384e-05
152753,152754,152753,305507,55.988762855529785,5.3472253407157616e-05
152953,152954,152953,305907,56.050609827041626,6.576487144240396e-05
153153,153154,153153,306307,56.12912106513977,5.344167851059788e-05
153353,153354,153353,306707,56.20781898498535,5.296115449199122e-05
153554,153555,153554,307109,56.272642850875854,5.247286026512555e-05
153754,153755,153754,307509,56.33785891532898,5.401221460655201e-05
153954,153955,153954,307909,56.40167307853699,5.208557055054735e-05
154154,154155,154154,308309,56.466338872909546,6.0809321170391063e-05
154354,154355,154354,308709,56.53033185005188,5.123187742822885e-05
154555,154556,154555,309111,56.59428882598877,5.064422381215114e-05
154755,154756,154755,309511,56.65813899040222,4.96468975112124e-05
154955,154956,154955,309911,56.73147487640381,4.9450662490294586e-05
155155,155156,155155,310311,56.79628801345825,4.952027156469974e-05
155355,155356,155355,310711,56.86235594749451,4.8499185328768754e-05
155556,155557,155556,311113,56.92832589149475,4.820176692408304e-05
155756,155757,155756,311513,56.9948890209198,4.8707388151135155e-05
155956,155957,155956,311913,57.05992603302002,4.718544870468868e-05
156156,156157,156156,312313,57.127805948257446,4.736685199020415e-05
156356,156357,156356,312713,57.1995689868927,4.903274832668688e-05
156557,156558,156557,313115,57.26588296890259,4.598288153326294e-05
156757,156758,156757,313515,57.331905126571655,5.488755141257684e-05
156957,156958,156957,313915,57.397989988327026,4.54819404849507e-05
157157,157158,157157,314315,57.4629020690918,4.530840716274448e-05
157357,157358,157357,314715,57.527161836624146,4.457333206695802e-05
157558,157559,157558,315117,57.59168291091919,4.4149445541578824e-05
157758,157759,157758,315517,57.65585494041443,4.4886397726325016e-05
157958,157959,157958,315917,57.73095512390137,4.377038644154132e-05
158158,158159,158158,316317,57.79482984542847,4.340185998662825e-05
158358,158359,158358,316717,57.85910892486572,4.295343654740348e-05
158559,158560,158559,317119,57.92373299598694,4.334195481395645e-05
158759,158760,158759,317519,57.98809790611267,4.236399749430526e-05
158959,158960,158959,317919,58.05095887184143,4.219640791919178e-05
159159,159160,159159,318319,58.11596083641052,4.211685264975678e-05
159359,159360,159359,318719,58.187220096588135,4.1497683069042795e-05
159560,159561,159560,319121,58.27242994308472,4.1228167840209144e-05
159760,159761,159760,319521,58.34707999229431,4.10776669055825e-05
159960,159961,159960,319921,58.4101357460022,4.050731097462188e-05
160160,160161,160160,320321,58.47441792488098,4.7889674645347517e-05
160360,160361,160360,320721,58.53868293762207,4.16235000580039e-05
160561,160562,160561,321123,58.60433888435364,3.942638949358079e-05
160761,160762,160761,321523,58.67130398750305,3.957494080266781e-05
160961,160962,160961,321923,58.74077892303467,3.89679406236358e-05
161161,161162,161161,322323,58.80508804321289,3.8759420575968616e-05
161361,161362,161361,322723,58.8703179359436,4.775163004515131e-05
161562,161563,161562,323125,58.93441104888916,3.781668470206771e-05
161762,161763,161762,323525,59.00938296318054,3.774555158683405e-05
161962,161963,161962,323925,59.11662793159485,3.739959460676e-05
162162,162163,162162,324325,59.21823000907898,3.6878560468410325e-05
162362,162363,162362,324725,59.29449200630188,3.8942412863417256e-05
162563,162564,162563,325127,59.37088108062744,4.029531178497658e-05
162763,162764,162763,325527,59.44822883605957,3.6046697066374674e-05
162963,162964,162963,325927,59.52490496635437,4.7983650867463446e-05
163163,163164,163163,326327,59.60086512565613,3.61455247369907e-05
163363,163364,163363,326727,59.67850089073181,3.542471727001728e-05
163564,163565,163564,327129,59.754008769989014,3.8572733388331275e-05
163764,163765,163764,327529,59.8246009349823,3.485210946053706e-05
163964,163965,163964,327929,59.89461302757263,4.287172400246614e-05
164164,164165,164164,328329,59.96113681793213,3.8762512938776434e-05
164364,164365,164364,328729,60.02522301673889,3.479940562906852e-05
164565,164566,164565,329131,60.08925914764404,3.3740316865595474e-05
164765,164766,164765,329531,60.15424394607544,3.685925617577931e-05
164965,164966,164965,329931,60.22800397872925,3.3036973596040614e-05
165165,165166,165165,330331,60.29315900802612,3.316160679008095e-05
165365,165366,165365,330731,60.368370056152344,3.25970272668575e-05
165566,165567,165566,331133,60.44872498512268,3.224205119466628e-05
165766,165767,165766,331533,60.51491594314575,3.207661430411782e-05
165966,165967,165966,331933,60.580278158187866,3.793423523419757e-05
166166,166167,166166,332333,60.645028829574585,3.384054230804874e-05
166366,166367,166366,332733,60.71939301490784,3.135095878803887e-05
166567,166568,166567,333135,60.78639483451843,3.073874549646531e-05
166767,166768,166767,333535,60.851516008377075,3.0889570161048815e-05
166967,166968,166967,333935,60.91677808761597,3.019311715120866e-05
167167,167168,167167,334335,60.983717918395996,3.0501004857513827e-05
167367,167368,167367,334735,61.04768180847168,2.9898613313477533e-05
167568,167569,167568,335137,61.114166021347046,2.9994861530625792e-05
167768,167769,167768,335537,61.178767919540405,2.9485648890471344e-05
167968,167969,167968,335937,61.255982875823975,2.9270166525021802e-05
168168,168169,168168,336337,61.321362018585205,2.921109351677763e-05
168368,168369,168368,336737,61.38575077056885,2.90116860066858e-05
168569,168570,168569,337139,61.44992685317993,2.8699747176317407e-05
168769,168770,168769,337539,61.51311683654785,2.8539617010191023e-05
168969,168970,168969,337939,61.578359842300415,2.8251129845524487e-05
169169,169170,169169,338339,61.64324998855591,2.7867727534734185e-05
169369,169370,169369,338739,61.71668791770935,2.7733557361142062e-05
169570,169571,169570,339141,61.78283190727234,2.750858122068453e-05
169770,169771,169770,339541,61.849544048309326,2.7137618176971612e-05
169970,169971,169970,339941,61.91417098045349,2.6794160439180114e-05
170170,170171,170170,340341,61.97864890098572,2.6811890973119676e-05
170370,170371,170370,340741,62.043203830718994,2.6555661475857818e-05
170571,170572,170571,341143,62.107940912246704,2.9500873688809605e-05
170771,170772,170771,341543,62.173826932907104,2.5924761213001017e-05
170971,170972,170971,341943,62.24441409111023,2.624943519500069e-05
171171,171172,171171,342343,62.310006856918335,2.9446236434885365e-05
171371,171372,171371,342743,62.37576389312744,2.560293982990846e-05
171572,171573,171572,343145,62.44026589393616,2.513015187492961e-05
171772,171773,171772,343545,62.51561498641968,2.4978042069918828e-05
171972,171973,171972,343945,62.594982862472534,2.5045130636507086e-05
172172,172173,172172,344345,62.66012907028198,2.474149762171939e-05
172372,172373,172372,344745,62.730653047561646,2.5613411048983442e-05
172573,172574,172573,345147,62.797780990600586,2.4236135827244624e-05
172773,172774,172773,345547,62.86223006248474,2.4169759976764823e-05
172973,172974,172973,345947,62.92622900009155,2.4051798011853342e-05
173173,173174,173173,346347,62.99005079269409,2.3741525919557993e-05
173373,173374,173373,346747,63.05427575111389,2.3533094468429617e-05
173574,173575,173574,347149,63.119022846221924,2.3333359789382096e-05
173774,173775,173774,347549,63.18737292289734,2.3569148767226634e-05
173974,173975,173974,347949,63.25644493103027,2.2880205090162753e-05
174174,174175,174174,348349,63.32080101966858,2.3120261769558065e-05
174374,174375,174374,348749,63.38904094696045,2.2905250313062878e-05
174575,174576,174575,349151,63.45304298400879,2.2577638718334215e-05
174775,174776,174775,349551,63.518380880355835,2.2471148524402526e-05
174975,174976,174975,349951,63.5821897983551,2.2309096282710858e-05
175175,175176,175175,350351,63.64787697792053,2.912658334063008e-05
175375,175376,175375,350751,63.72519493103027,2.1911951693096282e-05
175576,175577,175576,351153,63.79039001464844,2.256764661607228e-05
175776,175777,175776,351553,63.855058908462524,2.138114943855892e-05
175976,175977,175976,351953,63.91907787322998,2.4373396124255646e-05
176176,176177,176176,352353,63.985265016555786,2.161799147950915e-05
176376,176377,176376,352753,64.05079293251038,2.089273971244562e-05
176577,176578,176577,353155,64.11640501022339,2.0806740788502674e-05
176777,176778,176777,353555,64.18282508850098,2.07193010267432e-05
176977,176978,176977,353955,64.2518539428711,2.048667615696006e-05
177177,177178,177177,354355,64.31975507736206,2.0511692739726507e-05
177377,177378,177377,354755,64.38561272621155,2.0141987445730457e-05
177578,177579,177578,355157,64.45244288444519,1.989507723900504e-05
177778,177779,177778,355557,64.51903295516968,1.9928621446447497e-05
177978,177979,177978,355957,64.58805394172668,1.9508542716461334e-05
178178,178179,178178,356357,64.67279291152954,2.0310836983707785e-05
178378,178379,178378,356757,64.75750780105591,1.9352746862370587e-05
178579,178580,178579,357159,64.8254930973053,1.911042073546386e-05
178779,178780,178779,357559,64.89472484588623,1.91750904262206e-05
178979,178980,178979,357959,64.96158003807068,2.1901674461263277e-05
179179,179180,179179,358359,65.02745389938354,1.8621537103763344e-05
179379,179380,179379,358759,65.09559988975525,2.037920447658315e-05
179580,179581,179580,359161,65.16385889053345,1.8353550081400794e-05
179780,179781,179780,359561,65.23386287689209,2.2428986924702833e-05
179980,179981,179980,359961,65.30101108551025,2.0689661561384377e-05
180180,180181,180180,360361,65.36806893348694,1.8767157968672402e-05
180380,180381,180380,360761,65.43474888801575,2.0330757195062246e-05
180581,180582,180581,361163,65.50270175933838,1.7810137691829764e-05
180781,180782,180781,361563,65.56873393058777,1.8084036402242967e-05
180981,180982,180981,361963,65.63504600524902,1.7376074792103355e-05
181181,181182,181181,362363,65.71305394172668,1.7204857063559666e-05
181381,181382,181381,362763,65.78161478042603,1.7208030494893437e-05
181582,181583,181582,363165,65.8492329120636,1.6788371424648805e-05
181782,181783,181782,363565,65.91516184806824,2.0364829746733358e-05
181982,181983,181982,363965,65.981684923172,1.6613792954431888e-05
182182,182183,182182,364365,66.05102181434631,2.0048395887529046e-05
182382,182383,182382,364765,66.12112188339233,1.656824197009149e-05
182583,182584,182583,365167,66.19386506080627,1.6306846581755764e-05
182783,182784,182783,365567,66.26604390144348,1.78045986804804e-05
182983,182984,182983,365967,66.33778214454651,1.6052021123486903e-05
183183,183184,183183,366367,66.40486788749695,1.577891809696849e-05
183383,183384,183383,366767,66.47479605674744,1.8559509973725917e-05
183584,183585,183584,367169,66.5418770313263,1.5682180395720893e-05
183784,183785,183784,367569,66.60933208465576,1.8699574711081203e-05
183984,183985,183984,367969,66.68280100822449,1.5886148912080177e-05
184184,184185,184184,368369,66.75842380523682,1.5351065367949774e-05
184384,184385,184384,368769,66.83759593963623,1.5053285110781263e-05
184585,184586,184585,369171,66.91258597373962,1.5333486812535775e-05
184785,184786,184785,369571,66.97915697097778,1.4918711384618207e-05
184985,184986,184985,369971,67.04396176338196,1.4821562690640722e-05
185185,185186,185185,370371,67.1088080406189,1.4990328260285264e-05
185385,185386,185385,370771,67.1764030456543,1.4639564064734033e-05
185586,185587,185586,371173,67.25073289871216,1.4434035462804549e-05
185786,185787,185786,371573,67.31569600105286,1.4941743980228804e-05
185986,185987,185986,371973,67.38059878349304,1.4365393082150865e-05
186186,186187,186186,372373,67.44461584091187,1.7308601515036298e-05
186386,186387,186386,372773,67.50939869880676,1.71825674589924e-05
186587,186588,186587,373175,67.57413482666016,1.3913155568583969e-05
186787,186788,186787,373575,67.63936686515808,1.368197728838774e-05
186987,186988,186987,373975,67.71131610870361,1.3752062352254422e-05
187187,187188,187187,374375,67.77591609954834,1.3631643372238521e-05
187387,187388,187387,374775,67.84269189834595,1.3453417608744274e-05
187588,187589,187588,375177,67.908038854599,1.3320052046459817e-05
187788,187789,187788,375577,67.97315192222595,1.323098971307281e-05
187988,187989,187988,375977,68.03631806373596,1.3100265765192315e-05
188188,188189,188188,376377,68.10023188591003,1.3183846584495748e-05
188388,188389,188388,376777,68.16347885131836,1.3319921349469084e-05
188589,188590,188589,377179,68.23658990859985,1.4336921071725118e-05
188789,188790,188789,377579,68.30802202224731,1.2705460722879558e-05
188989,188990,188989,377979,68.37816405296326,1.264104266709439e-05
189189,189190,189189,378379,68.4495370388031,1.3926855003709742e-05
189389,189390,189389,378779,68.52197980880737,1.2383667320245366e-05
189590,189591,189590,379181,68.5885419845581,1.2706340624772496e-05
189790,189791,189790,379581,68.65622186660767,1.266978576459434e-05
189990,189991,189990,379981,68.73620676994324,1.2127715141789028e-05
190190,190191,190190,380381,68.80706000328064,1.2445643558535981e-05
190390,190391,190390,380781,68.87924790382385,1.1960891804182084e-05
190591,190592,190591,381183,68.96231198310852,1.4877585302126947e-05
190791,190792,190791,381583,69.0361099243164,1.1743689272225778e-05
190991,190992,190991,381983,69.10325789451599,1.1649748350356186e-05
191191,191192,191191,382383,69.16712999343872,1.164688106998137e-05
191391,191392,191391,382783,69.23829793930054,1.145533809433758e-05
191592,191593,191592,383185,69.30279088020325,1.1338258257270108e-05
191792,191793,191792,383585,69.36959075927734,1.1319544318632654e-05
191992,191993,191992,383985,69.43322777748108,1.1457282133390425e-05
192192,192193,192192,384385,69.49620580673218,1.1100461992951215e-05
192392,192393,192392,384785,69.55876302719116,1.1086976985472297e-05
192593,192594,192593,385187,69.6212067604065,1.0957293136732626e-05
192793,192794,192793,385587,69.69252896308899,1.07879278532948e-05
192993,192994,192993,385987,69.75531888008118,1.0715072531270601e-05
193193,193194,193193,386387,69.81832098960876,1.2122374718399783e-05
193393,193394,193393,386787,69.88072896003723,1.0578543209430875e-05
193594,193595,193594,387189,69.94338989257812,1.054329478714354e-05
193794,193795,193794,387589,70.00741696357727,1.053031180390229e-05
193994,193995,193994,387989,70.06862378120422,1.032134338534349e-05
194194,194195,194194,388389,70.13046097755432,1.030193891597823e-05
194394,194395,194394,388789,70.20085883140564,1.0129029535373847e-05
194595,194596,194595,389191,70.2649998664856,1.1552154485315494e-05
194795,194796,194795,389591,70.32689595222473,1.1472556047323885e-05
194995,194996,194995,389991,70.38975501060486,1.0098606268895488e-05
195195,195196,195195,390391,70.4525740146637,9.999383471381214e-06
195395,195396,195395,390791,70.51463794708252,9.827421135950824e-06
195596,195597,195596,391193,70.57807183265686,9.718608837140094e-06
195796,195797,195796,391593,70.63890480995178,9.585797405985884e-06
195996,195997,195996,391993,70.70722579956055,9.574691747991579e-06
196196,196197,196196,392393,70.77061486244202,9.503125260895581e-06
196396,196397,196396,392793,70.83236575126648,9.346109612510969e-06
196597,196598,196597,393195,70.89644384384155,9.361326313287235e-06
196797,196798,196797,393595,70.95899200439453,9.342742635101381e-06
196997,196998,196997,393995,71.0295958518982,9.243965484742884e-06
197197,197198,197197,394395,71.11311602592468,1.1076624156361041e-05
197397,197398,197397,394795,71.19796991348267,9.05124975085931e-06
197598,197599,197598,395197,71.26477980613708,9.072644958385547e-06
197798,197799,197798,395597,71.3312668800354,8.985084254281026e-06
197998,197999,197998,395997,71.39227890968323,8.808044456682028e-06
198198,198199,198198,396397,71.45394492149353,8.782904120895869e-06
198398,198399,198398,396797,71.51484894752502,8.958245860313968e-06
198599,198600,198599,397199,71.57707595825195,1.0813126203080966e-05
198799,198800,198799,397599,71.63833713531494,8.695899320432537e-06
198999,199000,198999,397999,71.71731781959534,8.507299181512479e-06
199199,199200,199199,398399,71.79246807098389,9.596035632475866e-06
199399,199400,199399,398799,71.85807704925537,8.337505548866718e-06
199600,199601,199600,399201,71.92366909980774,8.367295817649188e-06
199800,199801,199800,399601,71.98608899116516,8.258122890338423e-06
200000,200001,200000,400001,72.0513129234314,8.177125483508661e-06


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/eag-c.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007338523864746094,30.358106049564984
100,201,0,201,0.1048591136932373,6.493450136861272
200,401,0,401,0.18327093124389648,3.177507289781097
300,601,0,601,0.2569589614868164,2.0200540878033326
400,801,0,801,0.32503795623779297,1.4973870829094331
501,1003,0,1003,0.3924698829650879,1.2077208389856788
601,1203,0,1203,0.467242956161499,0.989316830878674
701,1403,0,1403,0.5347979068756104,0.8233653449454962
801,1603,0,1603,0.6016550064086914,0.7043998342234868
901,1803,0,1803,0.6758987903594971,0.6522505355825833
1001,2003,0,2003,0.7689969539642334,0.5753800609690223
1101,2203,0,2203,0.841871976852417,0.5126912067869833
1201,2403,0,2403,0.9125769138336182,0.45466603800015104
1301,2603,0,2603,0.9789519309997559,0.43864535988365744
1401,2803,0,2803,1.0438988208770752,0.3960641705985294
1502,3005,0,3005,1.106048822402954,0.36800860768665794
1602,3205,0,3205,1.17116379737854,0.3439575007189226
1702,3405,0,3405,1.2306506633758545,0.3210982972833532
1802,3605,0,3605,1.2873649597167969,0.29907689517926345
1902,3805,0,3805,1.3432068824768066,0.27792100029923855
2002,4005,0,4005,1.3986527919769287,0.2664558386879063
2102,4205,0,4205,1.45784592628479,0.2569607227315315
2202,4405,0,4405,1.5139529705047607,0.2525404359365554
2302,4605,0,4605,1.5709469318389893,0.24348000315202725
2402,4805,0,4805,1.6382169723510742,0.2294540764756248
2503,5007,0,5007,1.7050459384918213,0.22096504244071943
2603,5207,0,5207,1.773900032043457,0.20933355408296336
2703,5407,0,5407,1.8667550086975098,0.2003706010584758
2803,5607,0,5607,1.9311738014221191,0.19409314830020635
2903,5807,0,5807,1.9882957935333252,0.18758713015755707
3003,6007,0,6007,2.0513458251953125,0.17936651120038055
3103,6207,0,6207,2.127657890319824,0.17151651282570124
3203,6407,0,6407,2.1956210136413574,0.16648509708971368
3303,6607,0,6607,2.2529866695404053,0.16243960781487446
3403,6807,0,6807,2.3101680278778076,0.15685359329638138
3504,7009,0,7009,2.3786909580230713,0.15145019004331028
3604,7209,0,7209,2.443467855453491,0.1489031461598561
3704,7409,0,7409,2.5167369842529297,0.14421961397682728
3804,7609,0,7609,2.580432891845703,0.13933800424958753
3904,7809,0,7809,2.6425321102142334,0.13643824780422475
4004,8009,0,8009,2.700342893600464,0.13412666254906758
4104,8209,0,8209,2.766908884048462,0.13205883724844866
4204,8409,0,8409,2.832261800765991,0.13040429550311303
4304,8609,0,8609,2.893021821975708,0.12518696134067447
4404,8809,0,8809,2.9549429416656494,0.12120779775877681
4505,9011,0,9011,3.015314817428589,0.11793867947372813
4605,9211,0,9211,3.078489065170288,0.11514283592056614
4705,9411,0,9411,3.1398088932037354,0.11160654494049432
4805,9611,0,9611,3.200960874557495,0.10996968850546354
4905,9811,0,9811,3.2702958583831787,0.10801958387209429
5005,10011,0,10011,3.331705093383789,0.10548909035279165
5105,10211,0,10211,3.3897409439086914,0.10221391810925645
5205,10411,0,10411,3.4467618465423584,0.1010294983374759
5305,10611,0,10611,3.51163387298584,0.09970007478805022
5405,10811,0,10811,3.585360050201416,0.09881179743007851
5506,11013,0,11013,3.649481773376465,0.09570070788914996
5606,11213,0,11213,3.7157979011535645,0.09374846854657858
5706,11413,0,11413,3.792156934738159,0.0940464827703189
5806,11613,0,11613,3.869720935821533,0.09174830703767393
5906,11813,0,11813,3.9345688819885254,0.08924541998206977
6006,12013,0,12013,3.9989490509033203,0.08850053343835623
6106,12213,0,12213,4.063514947891235,0.08687853786897974
6206,12413,0,12413,4.132277011871338,0.0852908463906032
6306,12613,0,12613,4.197494029998779,0.08284840439442
6406,12813,0,12813,4.289319753646851,0.08079935314962451
6507,13015,0,13015,4.394905090332031,0.07899258511759796
6607,13215,0,13215,4.495901823043823,0.07787498942184042
6707,13415,0,13415,4.592221736907959,0.07632367495431167
6807,13615,0,13615,4.670635938644409,0.0759460752235735
6907,13815,0,13815,4.756820917129517,0.07584697075460098
7007,14015,0,14015,4.8478288650512695,0.07453511218689807
7107,14215,0,14215,4.9284327030181885,0.07336599203349224
7207,14415,0,14415,4.988650798797607,0.07340253199369183
7307,14615,0,14615,5.050331115722656,0.07290157202157466
7407,14815,0,14815,5.11274790763855,0.07153615631743382
7508,15017,0,15017,5.1749889850616455,0.06985831748037355
7608,15217,0,15217,5.237165927886963,0.06893807749832585
7708,15417,0,15417,5.302053689956665,0.06797271403369433
7808,15617,0,15617,5.364564895629883,0.06723807472828548
7908,15817,0,15817,5.446307897567749,0.06630195961927388
8008,16017,0,16017,5.50873589515686,0.06524329737100265
8108,16217,0,16217,5.570310831069946,0.06456382281314012
8208,16417,0,16417,5.634135007858276,0.0629767120173992
8308,16617,0,16617,5.695662021636963,0.06146963170293714
8408,16817,0,16817,5.757710933685303,0.06105128835195123
8509,17019,0,17019,5.819674968719482,0.06059338471273952
8609,17219,0,17219,5.881176948547363,0.0598431014110998
8709,17419,0,17419,5.951133966445923,0.05911898717921063
8809,17619,0,17619,6.0178139209747314,0.05873404789957919
8909,17819,0,17819,6.078969955444336,0.05863766599263057
9009,18019,0,18019,6.1383748054504395,0.057894940882902264
9109,18219,0,18219,6.197645902633667,0.057150907916840105
9209,18419,0,18419,6.257231950759888,0.05711564635271991
9309,18619,0,18619,6.3178510665893555,0.05677012916598475
9409,18819,0,18819,6.393862724304199,0.055767262439525386
9510,19021,0,19021,6.470256090164185,0.05484772960673859
9610,19221,0,19221,6.5312769412994385,0.05423758049087429
9710,19421,0,19421,6.59601092338562,0.05381902319484677
9810,19621,0,19621,6.664269924163818,0.05310568959428667
9910,19821,0,19821,6.724441051483154,0.05251756126365489
10010,20021,0,20021,6.785211801528931,0.05202112985688373
10110,20221,0,20221,6.842751979827881,0.05113442285242482
10210,20421,0,20421,6.903863906860352,0.050170814328476504
10310,20621,0,20621,6.963104009628296,0.049559061615367966
10410,20821,0,20821,7.022135019302368,0.04954515670001858
10511,21023,0,21023,7.080155849456787,0.04946131894130097
10611,21223,0,21223,7.138887882232666,0.04895753711135221
10711,21423,0,21423,7.197191953659058,0.04858863825436371
10811,21623,0,21623,7.255569934844971,0.048386863253826226
10911,21823,0,21823,7.313831806182861,0.04801247066539187
11011,22023,0,22023,7.374481916427612,0.04717683486265263
11111,22223,0,22223,7.440400123596191,0.04645725156277679
11211,22423,0,22423,7.507816791534424,0.046240757861431524
11311,22623,0,22623,7.573101997375488,0.04587148810738096
11411,22823,0,22823,7.632601976394653,0.044945876521436924
11512,23025,0,23025,7.691704034805298,0.04424786232894383
11612,23225,0,23225,7.754400968551636,0.044086267051293995
11712,23425,0,23425,7.815758943557739,0.04367249224835261
11812,23625,0,23625,7.875954866409302,0.04304100055155869
11912,23825,0,23825,7.938638925552368,0.04285121358920512
12012,24025,0,24025,7.997853755950928,0.04293031836131672
12112,24225,0,24225,8.057036876678467,0.042827151959074335
12212,24425,0,24425,8.11679482460022,0.04247002207493495
12312,24625,0,24625,8.17540192604065,0.04221675633652936
12412,24825,0,24825,8.233855962753296,0.041896213469312986
12513,25027,0,25027,8.293205976486206,0.04118777502728249
12613,25227,0,25227,8.351789951324463,0.04060350594824031
12713,25427,0,25427,8.409115076065063,0.04059383070041453
12813,25627,0,25627,8.468544006347656,0.0406103244830042
12913,25827,0,25827,8.54479694366455,0.040222491379367314
13013,26027,0,26027,8.61377501487732,0.039714453252492746
13113,26227,0,26227,8.67233681678772,0.03924484088077877
13213,26427,0,26427,8.729663848876953,0.03874781288387245
13313,26627,0,26627,8.78616189956665,0.03838444957203775
13413,26827,0,26827,8.843533039093018,0.03819813983779849
13514,27029,0,27029,8.901780843734741,0.03789297249811301
13614,27229,0,27229,8.962234735488892,0.037510380513344974
13714,27429,0,27429,9.02123212814331,0.03739576969169575
13814,27629,0,27629,9.077712774276733,0.03753807996642545
13914,27829,0,27829,9.136817932128906,0.037761064009475924
14014,28029,0,28029,9.200476884841919,0.03774299003687111
14114,28229,0,28229,9.257323980331421,0.03734377079737995
14214,28429,0,28429,9.314065933227539,0.03685797290551392
14314,28629,0,28629,9.373105764389038,0.03637333766629744
14414,28829,0,28829,9.43221402168274,0.035834183972586406
14515,29031,0,29031,9.491670846939087,0.03534846475132066
14615,29231,0,29231,9.549797773361206,0.03500427217938494
14715,29431,0,29431,9.608212947845459,0.034833754704270595
14815,29631,0,29631,9.668735980987549,0.03472558058408438
14915,29831,0,29831,9.728851795196533,0.0344579493769088
15015,30031,0,30031,9.787823915481567,0.03409658761431861
15115,30231,0,30231,9.848418951034546,0.033864512486068934
15215,30431,0,30431,9.90700387954712,0.03373298390191974
15315,30631,0,30631,9.966417789459229,0.033565919555018066
15415,30831,0,30831,10.026336908340454,0.03333822902925942
15516,31033,0,31033,10.086672067642212,0.03310810334141374
15616,31233,0,31233,10.14652681350708,0.03290241684355466
15716,31433,0,31433,10.207526922225952,0.03279683987739169
15816,31633,0,31633,10.270567893981934,0.03289865625135315
15916,31833,0,31833,10.329388856887817,0.033026082338673164
16016,32033,0,32033,10.38875699043274,0.03285544629813413
16116,32233,0,32233,10.450913906097412,0.03233679960845518
16216,32433,0,32433,10.512165784835815,0.03175743640624014
16316,32633,0,32633,10.57535195350647,0.0313589115493064
16416,32833,0,32833,10.644627809524536,0.03106260820852627
16517,33035,0,33035,10.71979284286499,0.03073466043598325
16617,33235,0,33235,10.790297985076904,0.03048290037772186
16717,33435,0,33435,10.849900007247925,0.03043170726562068
16817,33635,0,33635,10.909243822097778,0.030428124358431837
16917,33835,0,33835,10.969339847564697,0.030290627457881737
17017,34035,0,34035,11.028676986694336,0.030140520317679664
17117,34235,0,34235,11.090879917144775,0.030153790900751137
17217,34435,0,34435,11.15061092376709,0.030184430609046603
17317,34635,0,34635,11.20901870727539,0.02999649717802615
17417,34835,0,34835,11.267674922943115,0.02966875149034884
17518,35037,0,35037,11.326984882354736,0.029358972453177232
17618,35237,0,35237,11.391083002090454,0.029084109708836348
17718,35437,0,35437,11.451097965240479,0.028852334473472123
17818,35637,0,35637,11.509781837463379,0.028708187377669923
17918,35837,0,35837,11.569560050964355,0.028609977284311902
18018,36037,0,36037,11.629380941390991,0.02839569974855992
18118,36237,0,36237,11.686888933181763,0.028051743783738453
18218,36437,0,36437,11.746120929718018,0.027794924366970925
18318,36637,0,36637,11.804812908172607,0.02767626478551603
18418,36837,0,36837,11.866729974746704,0.027557560636513892
18519,37039,0,37039,11.9271080493927,0.027420607830366865
18619,37239,0,37239,11.98679804801941,0.027333681249766553
18719,37439,0,37439,12.04630970954895,0.027260816004700896
18819,37639,0,37639,12.10727071762085,0.027170525439944963
18919,37839,0,37839,12.171175956726074,0.02710689243810413
19019,38039,0,38039,12.236690759658813,0.027046412034836546
19119,38239,0,38239,12.31233286857605,0.026898664181944625
19219,38439,0,38439,12.396403789520264,0.02665161118030196
19319,38639,0,38639,12.47156286239624,0.0263749707542372
19419,38839,0,38839,12.532453060150146,0.026129407395588417
19520,39041,0,39041,12.593605041503906,0.025920630669609878
19620,39241,0,39241,12.65378189086914,0.02576008635326071
19720,39441,0,39441,12.711575031280518,0.025699577917577262
19820,39641,0,39641,12.778547763824463,0.025716225642238483
19920,39841,0,39841,12.854021787643433,0.0256549453913596
20020,40041,0,40041,12.924274921417236,0.02544924349488219
20120,40241,0,40241,12.98586893081665,0.02523030938098149
20220,40441,0,40441,13.043525695800781,0.025138858919045336
20320,40641,0,40641,13.101611852645874,0.025159752558046682
20420,40841,0,40841,13.169097900390625,0.025179805492266012
20521,41043,0,41043,13.23695683479309,0.025125779467433156
20621,41243,0,41243,13.294464826583862,0.02499131737954627
20721,41443,0,41443,13.35439682006836,0.02478939281786251
20821,41643,0,41643,13.413368940353394,0.02457934912691372
20921,41843,0,41843,13.47173810005188,0.02445842505472295
21021,42043,0,42043,13.52979588508606,0.024416880307477993
21121,42243,0,42243,13.588018894195557,0.024314961087311328
21221,42443,0,42443,13.645341873168945,0.024084617053506983
21321,42643,0,42643,13.703597068786621,0.023840979818897906
21421,42843,0,42843,13.76629090309143,0.023718554677641834
21522,43045,0,43045,13.82770299911499,0.02369414846280551
21622,43245,0,43245,13.88621473312378,0.023677310346186517
21722,43445,0,43445,13.944880723953247,0.023639853778932216
21822,43645,0,43645,14.001960754394531,0.0235796095178903
21922,43845,0,43845,14.06073784828186,0.023468162526206347
22022,44045,0,44045,14.122384071350098,0.02327975972881778
22122,44245,0,44245,14.202729940414429,0.02307577106376024
22222,44445,0,44445,14.271947860717773,0.022983367189758165
22322,44645,0,44645,14.335178852081299,0.023017729620847555
22422,44845,0,44845,14.392729043960571,0.023043878449885407
22523,45047,0,45047,14.45179009437561,0.0229619275014972
22623,45247,0,45247,14.515070915222168,0.02280308834227863
22723,45447,0,45447,14.576184034347534,0.02262047460606344
22823,45647,0,45647,14.636901140213013,0.0224262429231567
22923,45847,0,45847,14.69775390625,0.02224427244348681
23023,46047,0,46047,14.75629997253418,0.02211054437688033
23123,46247,0,46247,14.81484580039978,0.02199153129407551
23223,46447,0,46447,14.889219045639038,0.021824858028409087
23323,46647,0,46647,14.987433910369873,0.02164568683903626
23423,46847,0,46847,15.05506181716919,0.021555633631657745
23524,47049,0,47049,15.114195823669434,0.021580969113077778
23624,47249,0,47249,15.171954870223999,0.021636693489933006
23724,47449,0,47449,15.230187892913818,0.02164022553079419
23824,47649,0,47649,15.288805723190308,0.021575359795960713
23924,47849,0,47849,15.348649978637695,0.02144930247069973
24024,48049,0,48049,15.409942865371704,0.021288811201526803
24124,48249,0,48249,15.47545599937439,0.021156154408774882
24224,48449,0,48449,15.544080018997192,0.0210849817338012
24324,48649,0,48649,15.605079889297485,0.021034993926427017
24424,48849,0,48849,15.66410493850708,0.020957618113806267
24525,49051,0,49051,15.722323894500732,0.020858089013003407
24625,49251,0,49251,15.783370971679688,0.020762111311030666
24725,49451,0,49451,15.841320753097534,0.02067131968520767
24825,49651,0,49651,15.899703025817871,0.02058622266616884
24925,49851,0,49851,15.954837799072266,0.020498677311905744
25025,50051,0,50051,16.011334896087646,0.020371107425787387
25125,50251,0,50251,16.067996740341187,0.020186823664900336
25225,50451,0,50451,16.12308979034424,0.02001152416491854
25325,50651,0,50651,16.17862296104431,0.019940533820777578
25425,50851,0,50851,16.234494924545288,0.019981704092350745
25526,51053,0,51053,16.289469957351685,0.02004673463452749
25626,51253,0,51253,16.344926834106445,0.020052145884274925
25726,51453,0,51453,16.39993190765381,0.019978373039478668
25826,51653,0,51653,16.456936836242676,0.01984050088941162
25926,51853,0,51853,16.5141818523407,0.019669868507508348
26026,52053,0,52053,16.572908878326416,0.01950550006373346
26126,52253,0,52253,16.628321886062622,0.019380214861140273
26226,52453,0,52453,16.686492919921875,0.019309285231855437
26326,52653,0,52653,16.74790072441101,0.019283459901069413
26426,52853,0,52853,16.808418035507202,0.019280157726637968
26527,53055,0,53055,16.86550807952881,0.01927425484247622
26627,53255,0,53255,16.922626972198486,0.019232670284111807
26727,53455,0,53455,16.980002880096436,0.01913339643183112
26827,53655,0,53655,17.03870987892151,0.019000087467065527
26927,53855,0,53855,17.10796284675598,0.018882153540277495
27027,54055,0,54055,17.173404932022095,0.01879275596720773
27127,54255,0,54255,17.228379726409912,0.018709809952036083
27227,54455,0,54455,17.285077810287476,0.018638289412378627
27327,54655,0,54655,17.341936826705933,0.01860480387168761
27427,54855,0,54855,17.398530960083008,0.01859216781350349
27528,55057,0,55057,17.45945906639099,0.018544704494266734
27628,55257,0,55257,17.522567749023438,0.018438044904286018
27728,55457,0,55457,17.582704067230225,0.018292609915055567
27828,55657,0,55657,17.63833785057068,0.018138041955773496
27928,55857,0,55857,17.695989847183228,0.018004912078191555
28028,56057,0,56057,17.751610040664673,0.017932120121679825
28128,56257,0,56257,17.80669093132019,0.017933853916027087
28228,56457,0,56457,17.861888885498047,0.017977756925577393
28328,56657,0,56657,17.918412923812866,0.018021628087101546
28428,56857,0,56857,17.97753071784973,0.018042635866574928
28529,57059,0,57059,18.03495502471924,0.018021752807430024
28629,57259,0,57259,18.091931104660034,0.017939971020218468
28729,57459,0,57459,18.14798593521118,0.017803406729614103
28829,57659,0,57659,18.205467700958252,0.017653927696853842
28929,57859,0,57859,18.26340079307556,0.017536491299037758
29029,58059,0,58059,18.319134950637817,0.01746137680867546
29129,58259,0,58259,18.375683069229126,0.017413363779105004
29229,58459,0,58459,18.43251609802246,0.0173816952989395
29329,58659,0,58659,18.48864984512329,0.017355041399424412
29429,58859,0,58859,18.547055959701538,0.01730370652956164
29530,59061,0,59061,18.603786945343018,0.017198577432622486
29630,59261,0,59261,18.663089752197266,0.01705303841661969
29730,59461,0,59461,18.719273805618286,0.01691061120626897
29830,59661,0,59661,18.775563955307007,0.0168100581368708
29930,59861,0,59861,18.834040880203247,0.0167704820639451
30030,60061,0,60061,18.898255109786987,0.016794060014096338
30130,60261,0,60261,18.96183180809021,0.016855402988974474
30230,60461,0,60461,19.020549774169922,0.016908765293439203
30330,60661,0,60661,19.07852005958557,0.01692488790054963
30430,60861,0,60861,19.134845972061157,0.016902160314933117
30531,61063,0,61063,19.205026865005493,0.016842887715150606
30631,61263,0,61263,19.27654480934143,0.016752720399801812
30731,61463,0,61463,19.337794065475464,0.01664984792970389
30831,61663,0,61663,19.39590072631836,0.01655171899535322
30931,61863,0,61863,19.455347776412964,0.016452096738699826
31031,62063,0,62063,19.513372898101807,0.01633476712879096
31131,62263,0,62263,19.57232403755188,0.016203729221512798
31231,62463,0,62463,19.630377769470215,0.01608608011933965
31331,62663,0,62663,19.68768286705017,0.016006817105991705
31431,62863,0,62863,19.74578881263733,0.015967907789441387
31532,63065,0,63065,19.807383060455322,0.015951001587740734
31632,63265,0,63265,19.87288999557495,0.015936944993008243
31732,63465,0,63465,19.934342861175537,0.01592240456960927
31832,63665,0,63665,19.994480848312378,0.015917961362566277
31932,63865,0,63865,20.054110765457153,0.01592903947671259
32032,64065,0,64065,20.11510396003723,0.015945864179848168
32132,64265,0,64265,20.17277193069458,0.015949275982233252
32232,64465,0,64465,20.232053995132446,0.01592228614983197
32332,64665,0,64665,20.290992736816406,0.015860958861401375
32432,64865,0,64865,20.357630968093872,0.01577562495562067
32533,65067,0,65067,20.419798851013184,0.015680988263899107
32633,65267,0,65267,20.482417821884155,0.015593713082745228
32733,65467,0,65467,20.546449899673462,0.015524975110512186
32833,65667,0,65667,20.63054394721985,0.015478368034192422
32933,65867,0,65867,20.695467948913574,0.015442003371100488
33033,66067,0,66067,20.755472898483276,0.015395178244318611
33133,66267,0,66267,20.81645894050598,0.01533041885680635
33233,66467,0,66467,20.87836194038391,0.015267287065115298
33333,66667,0,66667,20.94036889076233,0.015233899131623783
33433,66867,0,66867,21.002001762390137,0.015232736474147414
33534,67069,0,67069,21.061830759048462,0.015235903757457899
33634,67269,0,67269,21.121252059936523,0.015216193310743625
33734,67469,0,67469,21.180259943008423,0.015171602821131185
33834,67669,0,67669,21.24015498161316,0.015115967626649116
33934,67869,0,67869,21.301931858062744,0.01505916076807911
34034,68069,0,68069,21.378523111343384,0.015001289992075584
34134,68269,0,68269,21.462382078170776,0.01493578930057414
34234,68469,0,68469,21.527481079101562,0.014851476926887448
34334,68669,0,68669,21.597272872924805,0.014743263628310686
34434,68869,0,68869,21.658897876739502,0.01462745667545257
34535,69071,0,69071,21.72029685974121,0.014533519250429795
34635,69271,0,69271,21.782367944717407,0.014481322506551092
34735,69471,0,69471,21.84491276741028,0.014466455654823735
34835,69671,0,69671,21.90491795539856,0.014475680813181
34935,69871,0,69871,21.96626305580139,0.014492784929933637
35035,70071,0,70071,22.02590298652649,0.014501068085698577
35135,70271,0,70271,22.087218761444092,0.014491143625437143
35235,70471,0,70471,22.147265911102295,0.01446526130181465
35335,70671,0,70671,22.207313776016235,0.014430427786110204
35435,70871,0,70871,22.26609492301941,0.014391163902417622
35536,71073,0,71073,22.43672800064087,0.014347688051080488
35636,71273,0,71273,22.50159001350403,0.014296018525278677
35736,71473,0,71473,22.561421871185303,0.014229045522591962
35836,71673,0,71673,22.62057375907898,0.014151555839997615
35936,71873,0,71873,22.68016791343689,0.014081308678462075
36036,72073,0,72073,22.743097066879272,0.014026467939148628
36136,72273,0,72273,22.807029008865356,0.013971811722765227
36236,72473,0,72473,22.86996293067932,0.013900654975927679
36336,72673,0,72673,22.930275917053223,0.013820804877356693
36436,72873,0,72873,22.991225957870483,0.013756838310642528
36537,73075,0,73075,23.052356004714966,0.01372597870996677
36637,73275,0,73275,23.11270809173584,0.01373097745024174
36737,73475,0,73475,23.174161911010742,0.013760824776911656
36837,73675,0,73675,23.233861684799194,0.013793008327880838
36937,73875,0,73875,23.303188800811768,0.013803767400256056
37037,74075,0,74075,23.38690495491028,0.013787993250131325
37137,74275,0,74275,23.45000386238098,0.0137599538493293
37237,74475,0,74475,23.525381088256836,0.013730172714679363
37337,74675,0,74675,23.59705376625061,0.01369213003246609
37437,74875,0,74875,23.65492606163025,0.013633781415766289
37538,75077,0,75077,23.71427869796753,0.013549438974218946
37638,75277,0,75277,23.773251056671143,0.013444374719117696
37738,75477,0,75477,23.85354495048523,0.013330483862197822
37838,75677,0,75677,23.929778814315796,0.013230981252340838
37938,75877,0,75877,23.99554991722107,0.013168810857294952
38038,76077,0,76077,24.054109811782837,0.01314764661795424
38138,76277,0,76277,24.112834930419922,0.013149057885518796
38238,76477,0,76477,24.17127275466919,0.013152027446406141
38338,76677,0,76677,24.22957682609558,0.013150257780348246
38438,76877,0,76877,24.291014909744263,0.01314838097384909
38539,77079,0,77079,24.349254846572876,0.013148047316145675
38639,77279,0,77279,24.407803773880005,0.01314337960076272
38739,77479,0,77479,24.466187953948975,0.01312779409481676
38839,77679,0,77679,24.523308038711548,0.013100575190709325
38939,77879,0,77879,24.585474967956543,0.013067362754982794
39039,78079,0,78079,24.644478797912598,0.013036315478978202
39139,78279,0,78279,24.702456951141357,0.01301153583082338
39239,78479,0,78479,24.760849714279175,0.012987422746797107
39339,78679,0,78679,24.822677850723267,0.012951757300121236
39439,78879,0,78879,24.882494926452637,0.012896824579535322
39540,79081,0,79081,24.94611096382141,0.012824944589761824
39640,79281,0,79281,25.021371841430664,0.01274740713587557
39740,79481,0,79481,25.093785047531128,0.01267454698349436
39840,79681,0,79681,25.153040885925293,0.012616986999912665
39940,79881,0,79881,25.210163831710815,0.012582711255122262
40040,80081,0,80081,25.267971992492676,0.01257275859448868
40140,80281,0,80281,25.326634883880615,0.012579811327479462
40240,80481,0,80481,25.38430404663086,0.012591853533341099
40340,80681,0,80681,25.442384004592896,0.01259742017533472
40440,80881,0,80881,25.50052809715271,0.01258849190341614
40541,81083,0,81083,25.571687936782837,0.012560541913467603
40641,81283,0,81283,25.658350944519043,0.012514174766199287
40741,81483,0,81483,25.729399919509888,0.012455248374482742
40841,81683,0,81683,25.789623022079468,0.012396846616790623
40941,81883,0,81883,25.848505973815918,0.01235398096053491
41041,82083,0,82083,25.90678906440735,0.012331918929629492
41141,82283,0,82283,25.963871955871582,0.012318793236578474
41241,82483,0,82483,26.0235378742218,0.01229335439518043
41341,82683,0,82683,26.10819697380066,0.012243316292336999
41441,82883,0,82883,26.173155069351196,0.012177252007486651
41542,83085,0,83085,26.233048915863037,0.012118010425831119
41642,83285,0,83285,26.292101860046387,0.012087090460390948
41742,83485,0,83485,26.34912896156311,0.012088127312532573
41842,83685,0,83685,26.40723490715027,0.012110371833813933
41942,83885,0,83885,26.46609878540039,0.012135932239867675
42042,84085,0,84085,26.523667812347412,0.012147828630524984
42142,84285,0,84285,26.58194088935852,0.012136180513043398
42242,84485,0,84485,26.64787983894348,0.0121001820674274
42342,84685,0,84685,26.72251009941101,0.012044754084458532
42442,84885,0,84885,26.78745174407959,0.011976185315968956
42543,85087,0,85087,26.845487117767334,0.011900281583547345
42643,85287,0,85287,26.90305995941162,0.011826030360169054
42743,85487,0,85487,26.960463047027588,0.011760251744006477
42843,85687,0,85687,27.018021821975708,0.011709484257061179
42943,85887,0,85887,27.07562804222107,0.011678161181881907
43043,86087,0,86087,27.1333589553833,0.011665284912635208
43143,86287,0,86287,27.19233202934265,0.011661557046158623
43243,86487,0,86487,27.25080895423889,0.011654251647284975
43343,86687,0,86687,27.31066393852234,0.011638139887697936
43443,86887,0,86887,27.369441032409668,0.011620426126678702
43544,87089,0,87089,27.43018889427185,0.011613182061582477
43644,87289,0,87289,27.49273180961609,0.011620954996574983
43744,87489,0,87489,27.56327486038208,0.011635423697052902
43844,87689,0,87689,27.626671075820923,0.011642043944076405
43944,87889,0,87889,27.685884714126587,0.011629010495441568
44044,88089,0,88089,27.748373985290527,0.011592024496400686
44144,88289,0,88289,27.820713996887207,0.011534680568930086
44244,88489,0,88489,27.891062021255493,0.011466320788135588
44344,88689,0,88689,27.95071291923523,0.011397536868197866
44444,88889,0,88889,28.012284755706787,0.011335486160834109
44545,89091,0,89091,28.078927040100098,0.01128284361526051
44645,89291,0,89291,28.14059591293335,0.011243375601964594
44745,89491,0,89491,28.20009994506836,0.011220761802009007
44845,89691,0,89691,28.25770902633667,0.01121746067995878
44945,89891,0,89891,28.314608812332153,0.011229293587269767
45045,90091,0,90091,28.37148380279541,0.011245097228247812
45145,90291,0,90291,28.428205966949463,0.011251871740763758
45245,90491,0,90491,28.486281871795654,0.011241843654263232
45345,90691,0,90691,28.549630880355835,0.01121686892123499
45445,90891,0,90891,28.60671591758728,0.01118656187702132
45546,91093,0,91093,28.663472890853882,0.011160249748534945
45646,91293,0,91293,28.719721794128418,0.011140194340159842
45746,91493,0,91493,28.776439905166626,0.01111930314035044
45846,91693,0,91693,28.83249592781067,0.011088771340286978
45946,91893,0,91893,28.887523889541626,0.011044707465559092
46046,92093,0,92093,28.943612813949585,0.01098984467688487
46146,92293,0,92293,29.001101970672607,0.010930643704773547
46246,92493,0,92493,29.061012983322144,0.010873694523576862
46346,92693,0,92693,29.119663953781128,0.01082380548721227
46446,92893,0,92893,29.17910599708557,0.010783799089033042
46547,93095,0,93095,29.237950801849365,0.010754718881999654
46647,93295,0,93295,29.29659390449524,0.010736986488226635
46747,93495,0,93495,29.35502791404724,0.010728629818643321
46847,93695,0,93695,29.411854028701782,0.010727019924492298
46947,93895,0,93895,29.467697858810425,0.010728965033804052
47047,94095,0,94095,29.523905038833618,0.010730000831684327
47147,94295,0,94295,29.581729888916016,0.0107240351026295
47247,94495,0,94495,29.63773488998413,0.010706450883217408
47347,94695,0,94695,29.692798852920532,0.010678777959679388
47447,94895,0,94895,29.74857783317566,0.01064818883866156
47548,95097,0,95097,29.804638862609863,0.010620516735535754
47648,95297,0,95297,29.86134910583496,0.010596177674995228
47748,95497,0,95497,29.937216997146606,0.010570355682742946
47848,95697,0,95697,30.006205797195435,0.010539022967456207
47948,95897,0,95897,30.06705594062805,0.010501730332484763
48048,96097,0,96097,30.12835693359375,0.010462734800943467
48148,96297,0,96297,30.187551975250244,0.01043010513085045
48248,96497,0,96497,30.247389793395996,0.0104116521722781
48348,96697,0,96697,30.307400941848755,0.010409880958250434
48448,96897,0,96897,30.36747694015503,0.01042037546379682
48549,97099,0,97099,30.426774978637695,0.010434267562523369
48649,97299,0,97299,30.485368013381958,0.010441058806138433
48749,97499,0,97499,30.545423984527588,0.010432928440863113
48849,97699,0,97699,30.605193853378296,0.010407114079506216
48949,97899,0,97899,30.664292097091675,0.010366716716095693
49049,98099,0,98099,30.72211503982544,0.010318096482632004
49149,98299,0,98299,30.77842402458191,0.01026769768614067
49249,98499,0,98499,30.836700916290283,0.010220756251457273
49349,98699,0,98699,30.897849082946777,0.010181201622673683
49449,98899,0,98899,30.956984996795654,0.010151357804525554
49550,99101,0,99101,31.019827842712402,0.010131345942205258
49650,99301,0,99301,31.081645965576172,0.010119764719979418
49750,99501,0,99501,31.141824960708618,0.010113155924813612
49850,99701,0,99701,31.207668781280518,0.010108054805557778
49950,99901,0,99901,31.266979932785034,0.010102099529774842
50050,100101,0,100101,31.3242449760437,0.010094850227981282
50150,100301,0,100301,31.3831889629364,0.010087549177962243
50250,100501,0,100501,31.44161081314087,0.010081936442045393
50350,100701,0,100701,31.498867988586426,0.010078588344514266
50450,100901,0,100901,31.556868076324463,0.010075515692014154
50551,101103,0,101103,31.617185831069946,0.010067978668233897
50651,101303,0,101303,31.675770044326782,0.010050676222643046
50751,101503,0,101503,31.73632001876831,0.010020317179777671
50851,101703,0,101703,31.7973690032959,0.00997796358476609
50951,101903,0,101903,31.859923839569092,0.00992897930183474
51051,102103,0,102103,31.918441772460938,0.009880793242002436
51151,102303,0,102303,31.983218908309937,0.009839848554861003
51251,102503,0,102503,32.05856204032898,0.009809776476626992
51351,102703,0,102703,32.139697790145874,0.009791614168874984
51451,102903,0,102903,32.20601010322571,0.009784783451054603
51552,103105,0,103105,32.27678298950195,0.009787186820364233
51652,103305,0,103305,32.34217596054077,0.009794241275637485
51752,103505,0,103505,32.404431104660034,0.009799329806767938
51852,103705,0,103705,32.465680837631226,0.009796122861830327
51952,103905,0,103905,32.52687883377075,0.00978193423058491
52052,104105,0,104105,32.587557792663574,0.009759385620641454
52152,104305,0,104305,32.64889693260193,0.00973437959087421
52252,104505,0,104505,32.708656787872314,0.009711593241208185
52352,104705,0,104705,32.780293703079224,0.009691426212141223
52452,104905,0,104905,32.8442018032074,0.009670917717797904
52553,105107,0,105107,32.90506386756897,0.009646576410917958
52653,105307,0,105307,32.967296838760376,0.00961722411200527
52753,105507,0,105507,33.02649283409119,0.009582394451196366
52853,105707,0,105707,33.08771085739136,0.009542799487996762
52953,105907,0,105907,33.16471076011658,0.009500359302009185
53053,106107,0,106107,33.239099740982056,0.009458474681742261
53153,106307,0,106307,33.30424690246582,0.009421856755248283
53253,106507,0,106507,33.36993193626404,0.009395915501364949
53353,106707,0,106707,33.43184995651245,0.009385310563629866
53453,106907,0,106907,33.495574951171875,0.009391548110275202
53554,107109,0,107109,33.55557584762573,0.009411072457460702
53654,107309,0,107309,33.61705493927002,0.00943419536432631
53754,107509,0,107509,33.67711877822876,0.00944912820161948
53854,107709,0,107709,33.74218797683716,0.009446093078997672
53954,107909,0,107909,33.81305909156799,0.009422107841772777
54054,108109,0,108109,33.897191762924194,0.009382360344359863
54154,108309,0,108309,33.957801818847656,0.009336810375311424
54254,108509,0,108509,34.01818108558655,0.00929427135758262
54354,108709,0,108709,34.0782949924469,0.009258522867911774
54454,108909,0,108909,34.13970398902893,0.009228811124972792
54555,109111,0,109111,34.21723008155823,0.009202596807682553
54655,109311,0,109311,34.290260791778564,0.009178828227337144
54755,109511,0,109511,34.351677894592285,0.009156802884742335
54855,109711,0,109711,34.42925477027893,0.009136660725316645
54955,109911,0,109911,34.51308989524841,0.00911875986228487
55055,110111,0,110111,34.57393407821655,0.009103842066035372
55155,110311,0,110311,34.63504099845886,0.00909317139789591
55255,110511,0,110511,34.695016860961914,0.009087997126030018
55355,110711,0,110711,34.75754475593567,0.00908844933787792
55455,110911,0,110911,34.8187198638916,0.009092617388602002
55556,111113,0,111113,34.88218092918396,0.009096407742470185
55656,111313,0,111313,34.94228792190552,0.00909425669420223
55756,111513,0,111513,35.0039598941803,0.009081550495760288
55856,111713,0,111713,35.06560683250427,0.009057153480114162
55956,111913,0,111913,35.12426781654358,0.009024857757038924
56056,112113,0,112113,35.184958934783936,0.008991625747655088
56156,112313,0,112313,35.24343395233154,0.008963439897264922
56256,112513,0,112513,35.30313181877136,0.008941959049597503
56356,112713,0,112713,35.36354303359985,0.008924641593044305
56456,112913,0,112913,35.42447304725647,0.008908045328560928
56557,113115,0,113115,35.4864559173584,0.008891264505246181
56657,113315,0,113315,35.55115103721619,0.008877386429474528
56757,113515,0,113515,35.61001491546631,0.008869639102887246
56857,113715,0,113715,35.67106509208679,0.008868356751634032
56957,113915,0,113915,35.73099207878113,0.008869889185627759
57057,114115,0,114115,35.79543900489807,0.008869293833110402
57157,114315,0,114315,35.85559701919556,0.008863673051179213
57257,114515,0,114515,35.91524076461792,0.008852915396300908
57357,114715,0,114715,35.97946381568909,0.00883787178734264
57457,114915,0,114915,36.036499977111816,0.008818550505109582
57558,115117,0,115117,36.09719395637512,0.00879385957034237
57658,115317,0,115317,36.15493297576904,0.008764060965915617
57758,115517,0,115517,36.22045373916626,0.00873077453460896
57858,115717,0,115717,36.278778076171875,0.008698285125955298
57958,115917,0,115917,36.35150408744812,0.008671913545105497
58058,116117,0,116117,36.421327114105225,0.00865504459304375
58158,116317,0,116317,36.48056888580322,0.008646641211054728
58258,116517,0,116517,36.539146900177,0.008641745002057164
58358,116717,0,116717,36.59872889518738,0.008635029316991108
58458,116917,0,116917,36.656533002853394,0.008624477304093159
58559,117119,0,117119,36.71570086479187,0.008611980946762743
58659,117319,0,117319,36.77411603927612,0.008601260689291576
58759,117519,0,117519,36.8334219455719,0.008593572397725983
58859,117719,0,117719,36.892021894454956,0.008586778771436394
58959,117919,0,117919,36.955410957336426,0.008576794606098668
59059,118119,0,118119,37.013378858566284,0.00856068599414247
59159,118319,0,118319,37.070536851882935,0.008538731500761284
59259,118519,0,118519,37.13079380989075,0.008513888543393513
59359,118719,0,118719,37.1904239654541,0.008489404000839883
59459,118919,0,118919,37.24812197685242,0.008466879924593705
59560,119121,0,119121,37.30629301071167,0.008446156616738426
59660,119321,0,119321,37.364428997039795,0.008427536476468628
59760,119521,0,119521,37.42911887168884,0.008411546756467375
59860,119721,0,119721,37.511812925338745,0.008399538163253178
59960,119921,0,119921,37.57483100891113,0.008392508542412209
60060,120121,0,120121,37.63401007652283,0.008390118272212626
60160,120321,0,120321,37.69202494621277,0.008390217268757667
60260,120521,0,120521,37.75257682800293,0.008389399843624358
60360,120721,0,120721,37.81327509880066,0.008384529028844144
60460,120921,0,120921,37.87101483345032,0.008374148006962285
60561,121123,0,121123,37.930497884750366,0.008358437768991745
60661,121323,0,121323,37.98843193054199,0.008338831265213073
60761,121523,0,121523,38.051620960235596,0.008316050103701327
60861,121723,0,121723,38.113778829574585,0.008290772274662472
60961,121923,0,121923,38.17318797111511,0.008264392935395931
61061,122123,0,122123,38.23195195198059,0.008239464058084029
61161,122323,0,122323,38.28912091255188,0.008218811913607873
61261,122523,0,122523,38.347200870513916,0.008203856759050901
61361,122723,0,122723,38.40511393547058,0.008193636846330265
61461,122923,0,122923,38.47827386856079,0.008185550279572806
61562,123125,0,123125,38.55898094177246,0.008177208211007935
61662,123325,0,123325,38.61817288398743,0.008168280889727262
61762,123525,0,123525,38.67889595031738,0.008159784506111377
61862,123725,0,123725,38.73768496513367,0.0081527302888562
61962,123925,0,123925,38.8012809753418,0.008146574457245271
62062,124125,0,124125,38.86097979545593,0.008139313373725462
62162,124325,0,124325,38.920379877090454,0.008128958687563971
62262,124525,0,124525,38.98643183708191,0.008114985073655382
62362,124725,0,124725,39.0489399433136,0.008098585694314937
62462,124925,0,124925,39.11163091659546,0.008081718980543
62563,125127,0,125127,39.18022298812866,0.00806566026323462
62663,125327,0,125327,39.23856568336487,0.008050938447781866
62763,125527,0,125527,39.29608082771301,0.008036718809978216
62863,125727,0,125727,39.35888886451721,0.008022436566841503
62963,125927,0,125927,39.41777992248535,0.008008376872473362
63063,126127,0,126127,39.475050926208496,0.007995498217915745
63163,126327,0,126327,39.532957792282104,0.00798443917076437
63263,126527,0,126527,39.59140872955322,0.00797463550190673
63363,126727,0,126727,39.6503427028656,0.007964494618723894
63463,126927,0,126927,39.70822191238403,0.00795259788605402
63564,127129,0,127129,39.76776695251465,0.007938716998042907
63664,127329,0,127329,39.82600498199463,0.007924458292761012
63764,127529,0,127529,39.882359981536865,0.007911366017282132
63864,127729,0,127729,39.94049596786499,0.007900195708787371
63964,127929,0,127929,40.00132608413696,0.007890208253394872
64064,128129,0,128129,40.06131196022034,0.0078796292244711
64164,128329,0,128329,40.12240409851074,0.007866866990561395
64264,128529,0,128529,40.18260598182678,0.007851684943009597
64364,128729,0,128729,40.24278283119202,0.007835404840250538
64464,128929,0,128929,40.303375005722046,0.007819928313755078
64565,129131,0,129131,40.371562004089355,0.0078063123957002375
64665,129331,0,129331,40.43684196472168,0.007794756342410101
64765,129531,0,129531,40.50225591659546,0.007784270154336194
64865,129731,0,129731,40.56979703903198,0.0077740387715886546
64965,129931,0,129931,40.64959788322449,0.007763691083291243
65065,130131,0,130131,40.721349000930786,0.007753114028405276
65165,130331,0,130331,40.787142753601074,0.007741911868765912
65265,130531,0,130531,40.85050702095032,0.007729068728458717
65365,130731,0,130731,40.91455888748169,0.007713310803468315
65465,130931,0,130931,40.97849178314209,0.007694026173873848
65566,131133,0,131133,41.03638792037964,0.007671718853971496
65666,131333,0,131333,41.10054397583008,0.007648748658338769
65766,131533,0,131533,41.16223978996277,0.007627125665096509
65866,131733,0,131733,41.23462986946106,0.007608570456612985
65966,131933,0,131933,41.30830693244934,0.007593980306732783
66066,132133,0,132133,41.37694478034973,0.007583528865600308
66166,132333,0,132333,41.43973183631897,0.007576836481283961
66266,132533,0,132533,41.50126886367798,0.007572924457868866
66366,132733,0,132733,41.56327295303345,0.007570054165316188
66466,132933,0,132933,41.62948298454285,0.007565931664868809
66567,133135,0,133135,41.69281983375549,0.00755849912675663
66667,133335,0,133335,41.75550293922424,0.007547440245384631
66767,133535,0,133535,41.821499824523926,0.007534294067707244
66867,133735,0,133735,41.88503289222717,0.007522022028853063
66967,133935,0,133935,41.94787383079529,0.007513283269721713
67067,134135,0,134135,42.0118887424469,0.007508679212265767
67167,134335,0,134335,42.07460808753967,0.0075059912699163844
67267,134535,0,134535,42.13754391670227,0.0075010316262593595
67367,134735,0,134735,42.196656703948975,0.007489770051496491
67467,134935,0,134935,42.25996494293213,0.007470557468473313
67568,135137,0,135137,42.32095289230347,0.007444938243277958
67668,135337,0,135337,42.3879017829895,0.007418143938868498
67768,135537,0,135537,42.44826889038086,0.007395531627407984
67868,135737,0,135737,42.51859784126282,0.007381259739505908
67968,135937,0,135937,42.58176589012146,0.007376550128270628
68068,136137,0,136137,42.64091992378235,0.007379625699092857
68168,136337,0,136337,42.70161509513855,0.00738675278434639
68268,136537,0,136537,42.77451682090759,0.007393523733379229
68368,136737,0,136737,42.84514284133911,0.00739592150847186
68468,136937,0,136937,42.90839600563049,0.007391300476336427
68569,137139,0,137139,42.97109603881836,0.007379146992632278
68669,137339,0,137339,43.03500199317932,0.007361951396987905
68769,137539,0,137539,43.09627103805542,0.00734356504381411
68869,137739,0,137739,43.16517972946167,0.007327800931907256
68969,137939,0,137939,43.227736949920654,0.007316631763900394
69069,138139,0,138139,43.28911995887756,0.007309529614787006
69169,138339,0,138339,43.35026979446411,0.007304022636236255
69269,138539,0,138539,43.41263389587402,0.0072969470711801545
69369,138739,0,138739,43.47513484954834,0.007285798279211084
69469,138939,0,138939,43.549519062042236,0.007269808260700402
69570,139141,0,139141,43.628785848617554,0.007250236639896668
69670,139341,0,139341,43.690653800964355,0.007230770528532205
69770,139541,0,139541,43.75343680381775,0.007214938155404445
69870,139741,0,139741,43.812532901763916,0.007205144090509089
69970,139941,0,139941,43.870720863342285,0.007201314247952143
70070,140141,0,140141,43.92833685874939,0.007200943119254834
70170,140341,0,140341,43.98700475692749,0.007200314375620685
70270,140541,0,140541,44.075368881225586,0.007196209665670404
70370,140741,0,140741,44.1864218711853,0.0071872218522481025
70470,140941,0,140941,44.300132036209106,0.00717407704365403
70571,141143,0,141143,44.41515803337097,0.007158786495265605
70671,141343,0,141343,44.500794887542725,0.007144044763525589
70771,141543,0,141543,44.64507269859314,0.00713118422212801
70871,141743,0,141743,44.7812979221344,0.007120324195044202
70971,141943,0,141943,44.922796964645386,0.007110513928758536
71071,142143,0,142143,45.00236797332764,0.007100518047407643
71171,142343,0,142343,45.0625159740448,0.007089584315541332
71271,142543,0,142543,45.123570919036865,0.0070777548822075894
71371,142743,0,142743,45.18486499786377,0.007065679810021526
71471,142943,0,142943,45.246872901916504,0.007054237575246948
71572,143145,0,143145,45.309454917907715,0.007044131004119543
71672,143345,0,143345,45.3707058429718,0.007035998909686463
71772,143545,0,143545,45.43130278587341,0.00702947289088109
71872,143745,0,143745,45.493982791900635,0.007023353311468679
71972,143945,0,143945,45.55838394165039,0.007015700281112519
72072,144145,0,144145,45.620276927948,0.007004619222931381
72172,144345,0,144345,45.680861949920654,0.006989253281603668
72272,144545,0,144545,45.74539494514465,0.006970323959531712
72372,144745,0,144745,45.83016276359558,0.006949854181600146
72472,144945,0,144945,46.028889894485474,0.006930297860325547
72573,145147,0,145147,46.15583086013794,0.006913487436533727
72673,145347,0,145347,46.221725940704346,0.006900753721687424
72773,145547,0,145547,46.28430414199829,0.006891879031289255
72873,145747,0,145747,46.34586000442505,0.0068860953682525535
72973,145947,0,145947,46.407212018966675,0.00688228880743852
73073,146147,0,146147,46.46871995925903,0.0068793486117229175
73173,146347,0,146347,46.52868700027466,0.006876429026804945
73273,146547,0,146547,46.590110778808594,0.0068730977688470085
73373,146747,0,146747,46.65826392173767,0.006869306088026997
73473,146947,0,146947,46.718008041381836,0.006865138305280393
73574,147149,0,147149,46.78008580207825,0.006860376845665334
73674,147349,0,147349,46.84416580200195,0.006854380787444337
73774,147549,0,147549,46.96904683113098,0.006845791731786861
73874,147749,0,147749,47.10303473472595,0.006833104297550502
73974,147949,0,147949,47.18367671966553,0.006815379017061515
74074,148149,0,148149,47.25083589553833,0.006793051817513773
74174,148349,0,148349,47.31292200088501,0.006768281771649881
74274,148549,0,148549,47.380316734313965,0.006744464128574958
74374,148749,0,148749,47.44466185569763,0.006725054177901147
74474,148949,0,148949,47.50959897041321,0.006712342451137187
74575,149151,0,149151,47.573077917099,0.006706809677988415
74675,149351,0,149351,47.65765595436096,0.006707415662442803
74775,149551,0,149551,47.72567296028137,0.006711900739219873
74875,149751,0,149751,47.7928409576416,0.006717709306782018
74975,149951,0,149951,47.85724592208862,0.006722380954435715
75075,150151,0,150151,47.92622995376587,0.006723944499778406
75175,150351,0,150351,47.99016284942627,0.006721295573593966
75275,150551,0,150551,48.05873775482178,0.006714440080525755
75375,150751,0,150751,48.14179491996765,0.0067043739097575735
75475,150951,0,150951,48.215879917144775,0.006692528711834919
75576,151153,0,151153,48.289658069610596,0.0066799108345765865
75676,151353,0,151353,48.34842801094055,0.006667117829434347
75776,151553,0,151553,48.406288146972656,0.0066536456949247355
75876,151753,0,151753,48.471709966659546,0.0066389633321500535
75976,151953,0,151953,48.60356283187866,0.006623135417455093
76076,152153,0,152153,48.79920983314514,0.006607276601182124
76176,152353,0,152353,48.91937184333801,0.0065933515810765505
76276,152553,0,152553,49.00571894645691,0.006583330443035823
76376,152753,0,152753,49.107178926467896,0.006578167301260679
76476,152953,0,152953,49.20204281806946,0.006577243849496588
76577,153155,0,153155,49.28557085990906,0.006578627385069742
76677,153355,0,153355,49.35515284538269,0.006579815926972762
76777,153555,0,153555,49.4372398853302,0.006578736850265117
76877,153755,0,153755,49.504010915756226,0.006574181476056478
76977,153955,0,153955,49.5633749961853,0.006565875733439574
77077,154155,0,154155,49.6264328956604,0.006554333835824532
77177,154355,0,154355,49.6840717792511,0.006540691750363322
77277,154555,0,154555,49.740955114364624,0.006526489431994804
77377,154755,0,154755,49.79803276062012,0.006513258191939193
77477,154955,0,154955,49.856268882751465,0.006501939956851516
77578,155157,0,155157,49.91542196273804,0.006492363508745275
77678,155357,0,155357,49.97348499298096,0.006483685405936677
77778,155557,0,155557,50.03473496437073,0.006474519071467548
77878,155757,0,155757,50.10678696632385,0.0064642082835428775
77978,155957,0,155957,50.168789863586426,0.006453209584259463
78078,156157,0,156157,50.23889493942261,0.006442810793705656
78178,156357,0,156357,50.30047583580017,0.006434253029869735
78278,156557,0,156557,50.365375995635986,0.006427870533849245
78378,156757,0,156757,50.43112897872925,0.006422841146226097
78478,156957,0,156957,50.49474787712097,0.006417669582351367
78579,157159,0,157159,50.56021189689636,0.006410937843777352
78679,157359,0,157359,50.62605309486389,0.006402211862557696
78779,157559,0,157559,50.691579818725586,0.0063917322546618175
78879,157759,0,157759,50.772785902023315,0.006380258567283409
78979,157959,0,157959,50.83979272842407,0.006368515630427897
79079,158159,0,158159,50.910902976989746,0.006357004488378025
79179,158359,0,158359,50.97817587852478,0.006346226200388647
79279,158559,0,158559,51.04487705230713,0.006336999685115724
79379,158759,0,158759,51.13918209075928,0.006330413577212286
79479,158959,0,158959,51.23459601402283,0.006327271775837482
79580,159161,0,159161,51.31260371208191,0.00632740443821423
79680,159361,0,159361,51.401349782943726,0.006329342729805803
79780,159561,0,159561,51.463939905166626,0.006330813851845528
79880,159761,0,159761,51.523271799087524,0.006329738140063581
79980,159961,0,159961,51.594330072402954,0.006325092835385952
80080,160161,0,160161,51.65858197212219,0.006317122940496106
80180,160361,0,160361,51.724153995513916,0.006306800561403505
80280,160561,0,160561,51.79211211204529,0.006295007089784566
80380,160761,0,160761,51.85697674751282,0.0062820854308129155
80480,160961,0,160961,51.91534686088562,0.006268037078644111
80581,161163,0,161163,51.972330808639526,0.00625291267142599
80681,161363,0,161363,52.05174493789673,0.006237760268742908
80781,161563,0,161563,52.13692593574524,0.006223538031024847
80881,161763,0,161763,52.20077085494995,0.006211200134098993
80981,161963,0,161963,52.2591028213501,0.006201164968657516
81081,162163,0,162163,52.315762758255005,0.006193363718402701
81181,162363,0,162363,52.37102484703064,0.006187625782028468
81281,162563,0,162563,52.42745900154114,0.006183987463252627
81381,162763,0,162763,52.489274740219116,0.006182574323561393
81481,162963,0,162963,52.55641579627991,0.0061831137879147235
81582,163165,0,163165,52.634567737579346,0.006184537046620509
81682,163365,0,163365,52.695019006729126,0.006185017612347482
81782,163565,0,163565,52.76571583747864,0.006182742342665173
81882,163765,0,163765,52.841062784194946,0.0061766169792434825
81982,163965,0,163965,52.90946984291077,0.006166664472020179
82082,164165,0,164165,53.019059896469116,0.006153859411214947
82182,164365,0,164365,53.10757279396057,0.006139633799702057
82282,164565,0,164565,53.20490288734436,0.0061254006253893024
82382,164765,0,164765,53.33006572723389,0.006112278575012047
82482,164965,0,164965,53.38868188858032,0.006100980846818899
82583,165167,0,165167,53.45101189613342,0.006091678814200914
82683,165367,0,165367,53.52882194519043,0.006084326190826553
82783,165567,0,165567,53.61269807815552,0.006078196839987096
82883,165767,0,165767,53.733647108078,0.0060725231814704956
82983,165967,0,165967,53.79172873497009,0.0060667427637404675
83083,166167,0,166167,53.849623918533325,0.006060770691237532
83183,166367,0,166367,53.908535957336426,0.006055006466621789
83283,166567,0,166567,53.968082904815674,0.00605001569575465
83383,166767,0,166767,54.02493381500244,0.006046039570402898
83483,166967,0,166967,54.08955001831055,0.006042636499109429
83584,167169,0,167169,54.15880012512207,0.006038666314505754
83684,167369,0,167369,54.322656869888306,0.00603288532128104
83784,167569,0,167569,54.50905084609985,0.006024319511563222
83884,167769,0,167769,54.67722487449646,0.006012797186594294
83984,167969,0,167969,54.73674273490906,0.005998931857247583
84084,168169,0,168169,54.79460096359253,0.0059838283176214145
84184,168369,0,168369,54.861488819122314,0.005968713208247137
84284,168569,0,168569,54.936309814453125,0.0059546905452422015
84384,168769,0,168769,55.07400393486023,0.0059426467692178615
84484,168969,0,168969,55.15817904472351,0.0059332001706545005
84585,169171,0,169171,55.238380908966064,0.005926567043396884
84685,169371,0,169371,55.34575891494751,0.005922710538937718
84785,169571,0,169571,55.41110181808472,0.005920943028175706
84885,169771,0,169771,55.47823882102966,0.005920317878003945
84985,169971,0,169971,55.53898000717163,0.005919732673488156
85085,170171,0,170171,55.61734175682068,0.005918155798456033
85185,170371,0,170371,55.690253019332886,0.005914834954634404
85285,170571,0,170571,55.7512948513031,0.005909411892869939
85385,170771,0,170771,55.80970287322998,0.005901907530898961
85485,170971,0,170971,55.86982583999634,0.0058926221881736825
85586,171173,0,171173,55.97798490524292,0.005881923811601864
85686,171373,0,171373,56.077223777770996,0.00587062522168571
85786,171573,0,171573,56.188347816467285,0.005859294641033896
85886,171773,0,171773,56.3428111076355,0.005848604498415193
85986,171973,0,171973,56.45743680000305,0.00583913806808359
86086,172173,0,172173,56.52031683921814,0.005831308960912624
86186,172373,0,172373,56.581559896469116,0.005825322830233905
86286,172573,0,172573,56.64234375953674,0.005821168032310239
86386,172773,0,172773,56.71188282966614,0.005818601001814395
86486,172973,0,172973,56.771047830581665,0.005817126994080715
86587,173175,0,173175,56.83198094367981,0.005816014046640073
86687,173375,0,173375,56.89234685897827,0.005814445508239555
86787,173575,0,173575,56.95396590232849,0.0058116438428099096
86887,173775,0,173775,57.01354789733887,0.005807067710837212
86987,173975,0,173975,57.07573390007019,0.005800480224528795
87087,174175,0,174175,57.13900375366211,0.005791950234930695
87187,174375,0,174375,57.19788885116577,0.005781811875236365
87287,174575,0,174575,57.35693097114563,0.005770606630741553
87387,174775,0,174775,57.535736083984375,0.005759008093047142
87487,174975,0,174975,57.617923974990845,0.0057477316857425294
87588,175177,0,175177,57.68238592147827,0.005737355473919624
87688,175377,0,175377,57.75417995452881,0.005728667339739714
87788,175577,0,175577,57.831946849823,0.005722008654751628
87888,175777,0,175777,57.891886949539185,0.005717660494168233
87988,175977,0,175977,57.94994592666626,0.005715660451452239
88088,176177,0,176177,58.00777888298035,0.005715722673143242
88188,176377,0,176377,58.065287828445435,0.0057172097050312435
88288,176577,0,176577,58.125372886657715,0.0057191899739203085
88388,176777,0,176777,58.185404777526855,0.005720563860147484
88488,176977,0,176977,58.24121904373169,0.005720222478877015
88589,177179,0,177179,58.29753375053406,0.00571718083201398
88689,177379,0,177379,58.35325789451599,0.005710924526099272
88789,177579,0,177579,58.40887689590454,0.005701413356890998
88889,177779,0,177779,58.466187953948975,0.005689226055388126
88989,177979,0,177979,58.52672982215881,0.005675416373485961
89089,178179,0,178179,58.59200096130371,0.0056612132705200265
89189,178379,0,178379,58.65049481391907,0.005647672322363392
89289,178579,0,178579,58.710103034973145,0.005635439724838899
89389,178779,0,178779,58.76986384391785,0.005624733518825825
89489,178979,0,178979,58.826204776763916,0.005615527377784496
89590,179181,0,179181,58.885822772979736,0.005607739954246668
89690,179381,0,179381,58.94602108001709,0.005601693943797764
89790,179581,0,179581,59.00799894332886,0.005597604118614028
89890,179781,0,179781,59.08019709587097,0.005595653441929693
89990,179981,0,179981,59.14371991157532,0.005595597276718549
90090,180181,0,180181,59.20821285247803,0.005596584856012616
90190,180381,0,180381,59.26894783973694,0.005597253885880519
90290,180581,0,180581,59.327499866485596,0.0055960866036244205
90390,180781,0,180781,59.387425899505615,0.005591863564624203
90490,180981,0,180981,59.443504095077515,0.005584010503220677
90591,181183,0,181183,59.50449776649475,0.00557259645155361
90691,181383,0,181383,59.56158685684204,0.005558746212822594
90791,181583,0,181583,59.62523102760315,0.005543743258983847
90891,181783,0,181783,59.68232274055481,0.0055291874545232225
90991,181983,0,181983,59.73874092102051,0.005516596925405587
91091,182183,0,182183,59.79445195198059,0.0055071025103751526
91191,182383,0,182383,59.85331392288208,0.005501204347254055
91291,182583,0,182583,59.92333388328552,0.005498673297552836
91391,182783,0,182783,59.990679025650024,0.005498643484430579
91491,182983,0,182983,60.0522198677063,0.005499867238591489
91592,183185,0,183185,60.11906695365906,0.005501044618695045
91692,183385,0,183385,60.178921937942505,0.005501054058664265
91792,183585,0,183585,60.2383987903595,0.0054991938166189845
91892,183785,0,183785,60.29708480834961,0.0054951414124938085
91992,183985,0,183985,60.354623794555664,0.005488902161121889
92092,184185,0,184185,60.41201400756836,0.0054807186733045925
92192,184385,0,184385,60.46904802322388,0.005470995085045587
92292,184585,0,184585,60.526187896728516,0.005460240397625913
92392,184785,0,184785,60.58510684967041,0.005449017392084609
92492,184985,0,184985,60.64248085021973,0.005437890116056643
92593,185187,0,185187,60.69886898994446,0.005427275518267758
92693,185387,0,185387,60.75572395324707,0.0054178233125894565
92793,185587,0,185587,60.81301403045654,0.005409758919085763
92893,185787,0,185787,60.869855880737305,0.005403301163180252
92993,185987,0,185987,60.92565989494324,0.00539852713865669
93093,186187,0,186187,60.98336577415466,0.005395323499740656
93193,186387,0,186387,61.04075884819031,0.005393331017795206
93293,186587,0,186587,61.11120676994324,0.005391930482023636
93393,186787,0,186787,61.171475887298584,0.005390321149126888
93493,186987,0,186987,61.22734785079956,0.005387700515157615
93594,187189,0,187189,61.283955812454224,0.0053834398714257305
93694,187389,0,187389,61.33971405029297,0.0053774504937556195
93794,187589,0,187589,61.39638686180115,0.005369978520308289
93894,187789,0,187789,61.453266859054565,0.005361637684975971
93994,187989,0,187989,61.510132789611816,0.005353153887437914
94094,188189,0,188189,61.566473960876465,0.005345141080713081
94194,188389,0,188389,61.62502384185791,0.005337967722451684
94294,188589,0,188589,61.68226599693298,0.005331740623447432
94394,188789,0,188789,61.74195384979248,0.005326367464065984
94494,188989,0,188989,61.803133964538574,0.0053216428161738
94595,189191,0,189191,61.86123204231262,0.005317289439703156
94695,189391,0,189391,61.91892385482788,0.005313208184613084
94795,189591,0,189591,61.97979378700256,0.005309293393753237
94895,189791,0,189791,62.05171084403992,0.0053056223589581335
94995,189991,0,189991,62.12613487243652,0.005302317679326149
95095,190191,0,190191,62.18473696708679,0.005299352112559907
95195,190391,0,190391,62.2432599067688,0.00529636113764621
95295,190591,0,190591,62.301405906677246,0.005292627508405846
95395,190791,0,190791,62.35898804664612,0.005287325316621155
95495,190991,0,190991,62.421345949172974,0.00527993261485608
95596,191193,0,191193,62.4806969165802,0.0052704765342773815
95696,191393,0,191393,62.538455963134766,0.005259989968454442
95796,191593,0,191593,62.598809003829956,0.005249646040618858
95896,191793,0,191793,62.657179832458496,0.005240631331917189
95996,191993,0,191993,62.71567392349243,0.005233629392546392
96096,192193,0,192193,62.77440571784973,0.005228645098702569
96196,192393,0,192393,62.83569288253784,0.0052251286552501665
96296,192593,0,192593,62.89667081832886,0.0052222879537750025
96396,192793,0,192793,62.95800185203552,0.0052194160286189615
96496,192993,0,192993,63.01988077163696,0.005216102206355348
96597,193195,0,193195,63.08355402946472,0.005212243055105286
96697,193395,0,193395,63.14274501800537,0.0052081177949299205
96797,193595,0,193595,63.20288395881653,0.00520398702169877
96897,193795,0,193795,63.26231074333191,0.00520004424728759
96997,193995,0,193995,63.31996989250183,0.0051962131578217816
97097,194195,0,194195,63.37672686576843,0.005192083295763352
97197,194395,0,194395,63.43492293357849,0.005187013862526274
97297,194595,0,194595,63.493138790130615,0.0051804108162943905
97397,194795,0,194795,63.552156925201416,0.005172075470399447
97497,194995,0,194995,63.61806583404541,0.005162438383244741
97598,195197,0,195197,63.67643213272095,0.0051524183020271635
97698,195397,0,195397,63.736480951309204,0.005143481166171602
97798,195597,0,195597,63.79411506652832,0.005136543719886977
97898,195797,0,195797,63.85253190994263,0.0051320146477682165
97998,195997,0,195997,63.90936803817749,0.005129609302065471
98098,196197,0,196197,63.966535806655884,0.005128541084653189
98198,196397,0,196397,64.02423787117004,0.0051278443046347
98298,196597,0,196597,64.08372712135315,0.005126663800300864
98398,196797,0,196797,64.15274691581726,0.005124425809643827
98498,196997,0,196997,64.22431683540344,0.005120893229623032
98599,197199,0,197199,64.29015684127808,0.005116088785268417
98699,197399,0,197399,64.35843300819397,0.005110415494816555
98799,197599,0,197599,64.42149710655212,0.005104227058415538
98899,197799,0,197799,64.48144507408142,0.005097841201350138
98999,197999,0,197999,64.53929686546326,0.005091371797212367
99099,198199,0,198199,64.61247205734253,0.005084724362292203
99199,198399,0,198399,64.70184183120728,0.005077737566869527
99299,198599,0,198599,64.78288674354553,0.00507039631052385
99399,198799,0,198799,64.8698480129242,0.00506297460937025
99499,198999,0,198999,64.97063398361206,0.00505599421150402
99600,199201,0,199201,65.08398413658142,0.0050499475735867085
99700,199401,0,199401,65.23796391487122,0.0050452487255632636
99800,199601,0,199601,65.32781982421875,0.005041712194349829
99900,199801,0,199801,65.40050387382507,0.005038869882085438
100000,200001,0,200001,65.46437382698059,0.005036140328868398


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007221698760986328,30.358106049564984
100,201,200,401,0.07111811637878418,1.7063375198016169
200,401,400,801,0.15479707717895508,1.0108894113540814
300,601,600,1201,0.22110509872436523,0.7489939892258344
400,801,800,1601,0.28597021102905273,0.6081938727196392
501,1003,1002,2005,0.3430659770965576,0.5168895867181229
601,1203,1202,2405,0.399658203125,0.452278382327617
701,1403,1402,2805,0.45823097229003906,0.40291992726905773
801,1603,1602,3205,0.5149731636047363,0.3634630940471491
901,1803,1802,3605,0.5751190185546875,0.33097564129661755
1001,2003,2002,4005,0.6394898891448975,0.3037093528611154
1101,2203,2202,4405,0.6969859600067139,0.2803953971483973
1201,2403,2402,4805,0.7553591728210449,0.26019451460291226
1301,2603,2602,5205,0.8123140335083008,0.24250818197445992
1401,2803,2802,5605,0.8706750869750977,0.22685332490806293
1502,3005,3004,6009,0.9271430969238281,0.2127929708960007
1602,3205,3204,6409,0.9837710857391357,0.20030755961093588
1702,3405,3404,6809,1.0433928966522217,0.18902363243190226
1802,3605,3604,7209,1.1205999851226807,0.17874588608055825
1902,3805,3804,7609,1.190566062927246,0.16936686708805634
2002,4005,4004,8009,1.253993034362793,0.16078928006504323
2102,4205,4204,8409,1.315399169921875,0.15289388141740703
2202,4405,4404,8809,1.377676010131836,0.1455894973020299
2302,4605,4604,9209,1.4560480117797852,0.13880996643974702
2402,4805,4804,9609,1.5163989067077637,0.13250544845542997
2503,5007,5006,10013,1.5813071727752686,0.12658272496808612
2603,5207,5206,10413,1.6557328701019287,0.12107898410631822
2703,5407,5406,10813,1.7226440906524658,0.11592039425419869
2803,5607,5606,11213,1.7872650623321533,0.11108349163202878
2903,5807,5806,11613,1.8494648933410645,0.10652119458942605
3003,6007,6006,12013,1.909250020980835,0.10222880204007911
3103,6207,6206,12413,1.9699392318725586,0.09818713706730445
3203,6407,6406,12813,2.0313398838043213,0.09436920147170691
3303,6607,6606,13213,2.096950054168701,0.09073320222110537
3403,6807,6806,13613,2.1620609760284424,0.08729857820057606
3504,7009,7008,14017,2.2354400157928467,0.08401838454826126
3604,7209,7208,14417,2.312311887741089,0.08093927928962326
3704,7409,7408,14817,2.374199867248535,0.07800912151469362
3804,7609,7608,15217,2.4395711421966553,0.0752232971485176
3904,7809,7808,15617,2.500128984451294,0.07257609242688355
4004,8009,8008,16017,2.5602238178253174,0.07005957569801338
4104,8209,8208,16417,2.632909059524536,0.06766082262576223
4204,8409,8408,16817,2.6967039108276367,0.0653627511027669
4304,8609,8608,17217,2.7577710151672363,0.06318097775381688
4404,8809,8808,17617,2.8185360431671143,0.06110300953777403
4505,9011,9010,18021,2.8820929527282715,0.0590937428271714
4605,9211,9210,18421,2.944782018661499,0.05717733161162599
4705,9411,9410,18821,3.007866144180298,0.05535773017085458
4805,9611,9610,19221,3.0684731006622314,0.05361798797459647
4905,9811,9810,19621,3.1422371864318848,0.05194900886724691
5005,10011,10010,20021,3.2039499282836914,0.05035243765185992
5105,10211,10210,20421,3.2653040885925293,0.04882063373100812
5205,10411,10410,20821,3.3260772228240967,0.047359071023488915
5305,10611,10610,21221,3.3886728286743164,0.045955467781552156
5405,10811,10810,21621,3.4485411643981934,0.04461009631068081
5506,11013,11012,22025,3.515192985534668,0.043314099629270165
5606,11213,11212,22425,3.5777299404144287,0.04207838125332836
5706,11413,11412,22825,3.6468799114227295,0.040893441689385045
5806,11613,11612,23225,3.7094480991363525,0.039758063729968526
5906,11813,11812,23625,3.770732879638672,0.03866727459590865
6006,12013,12012,24025,3.8318021297454834,0.03762274291255587
6106,12213,12212,24425,3.894062042236328,0.036611040471708
6206,12413,12412,24825,3.9540770053863525,0.03562856314436133
6306,12613,12612,25225,4.015941143035889,0.03469692269248736
6406,12813,12812,25625,4.07974910736084,0.033799683286082904
6507,13015,13014,26029,4.142674207687378,0.032929696359171264
6607,13215,13214,26429,4.2083611488342285,0.03210090886963369
6707,13415,13414,26829,4.292970895767212,0.03129562467976816
6807,13615,13614,27229,4.390583038330078,0.030518070810675323
6907,13815,13814,27629,4.473135948181152,0.02976476100537671
7007,14015,14014,28029,4.543805122375488,0.029042946413349643
7107,14215,14214,28429,4.625964879989624,0.028345043787213003
7207,14415,14414,28829,4.70111608505249,0.0276787893149401
7307,14615,14614,29229,4.772382020950317,0.027025990891256242
7407,14815,14814,29629,4.85260796546936,0.02639680752696954
7508,15017,15016,30033,4.928344011306763,0.025790202933365928
7608,15217,15216,30433,5.000643968582153,0.025208342940185372
7708,15417,15416,30833,5.073904037475586,0.024644675806295535
7808,15617,15616,31233,5.149876832962036,0.024097814611134232
7908,15817,15816,31633,5.22419810295105,0.023566249852129673
8008,16017,16016,32033,5.298389911651611,0.02305376193088568
8108,16217,16216,32433,5.364605188369751,0.022559992497924237
8208,16417,16416,32833,5.4363110065460205,0.022127591431272717
8308,16617,16616,33233,5.499424934387207,0.02183072302642047
8408,16817,16816,33633,5.56223201751709,0.021543699371941685
8509,17019,17018,34037,5.635188817977905,0.021261309515999933
8609,17219,17218,34437,5.6984312534332275,0.02098255850015554
8709,17419,17418,34837,5.761754035949707,0.020702356282380815
8809,17619,17618,35237,5.82614803314209,0.020420375359117754
8909,17819,17818,35637,5.891563892364502,0.020138484850655773
9009,18019,18018,36037,5.968167066574097,0.019856479540637278
9109,18219,18218,36437,6.0351080894470215,0.019579994634302125
9209,18419,18418,36837,6.106342077255249,0.019317725373640755
9309,18619,18618,37237,6.17547607421875,0.01905872209024548
9409,18819,18818,37637,6.247542858123779,0.01879995540818351
9510,19021,19020,38041,6.312247037887573,0.01854074106529157
9610,19221,19220,38441,6.376391172409058,0.018285940160676868
9710,19421,19420,38841,6.442178964614868,0.018033973880335365
9810,19621,19620,39241,6.522934913635254,0.017784346530271056
9910,19821,19820,39641,6.61003303527832,0.01754157169669738
10010,20021,20020,40041,6.683986186981201,0.017298410407666644
10110,20221,20220,40441,6.761784076690674,0.017056909972164882
10210,20421,20420,40841,6.838958024978638,0.016821123610325783
10310,20621,20620,41241,6.9127678871154785,0.016589128045374983
10410,20821,20820,41641,6.979252815246582,0.016354305165659166
10511,21023,21022,42045,7.045183897018433,0.016116668275785968
10611,21223,21222,42445,7.123002052307129,0.015890884021779093
10711,21423,21422,42845,7.190722942352295,0.015665347331383236
10811,21623,21622,43245,7.256376028060913,0.015434709267468974
10911,21823,21822,43645,7.320688962936401,0.015212370568155185
11011,22023,22022,44045,7.389062166213989,0.014993947575038701
11111,22223,22222,44445,7.460387945175171,0.014771376883042104
11211,22423,22422,44845,7.537173271179199,0.014550765644058933
11311,22623,22622,45245,7.622260808944702,0.014334080098261178
11411,22823,22822,45645,7.703177213668823,0.014116158028222484
11512,23025,23024,46049,7.7780539989471436,0.013902809895313464
11612,23225,23224,46449,7.840038061141968,0.013695643382817462
11712,23425,23424,46849,7.9021852016448975,0.013484527177849842
11812,23625,23624,47249,7.9816858768463135,0.01328034081915178
11912,23825,23824,47649,8.047395944595337,0.013080685802734427
12012,24025,24024,48049,8.113860130310059,0.012879287348580218
12112,24225,24224,48449,8.175557136535645,0.012688001335773287
12212,24425,24424,48849,8.241299152374268,0.012500327290257563
12312,24625,24624,49249,8.310078144073486,0.012310316549936438
12412,24825,24824,49649,8.38286304473877,0.012127368917885458
12513,25027,25026,50053,8.45032000541687,0.011942693247676607
12613,25227,25226,50453,8.513161182403564,0.011759630765673523
12713,25427,25426,50853,8.577107191085815,0.011577998632949813
12813,25627,25626,51253,8.665873050689697,0.011398773287604
12913,25827,25826,51653,8.751668214797974,0.011225178439008686
13013,26027,26026,52053,8.829296112060547,0.011052352318824609
13113,26227,26226,52453,8.898505210876465,0.010881101841824966
13213,26427,26426,52853,8.976408958435059,0.010711517925130679
13313,26627,26626,53253,9.050190925598145,0.01053970825186124
13413,26827,26826,53653,9.129212141036987,0.010373069909673675
13514,27029,27028,54057,9.199381828308105,0.010208010736618077
13614,27229,27228,54457,9.267427921295166,0.010047203235739155
13714,27429,27428,54857,9.33531904220581,0.009886819102132356
13814,27629,27628,55257,9.420829057693481,0.009727176920220567
13914,27829,27828,55657,9.537475109100342,0.009571825961645079
14014,28029,28028,56057,9.689951181411743,0.009420559812505053
14114,28229,28228,56457,9.78522515296936,0.009264481496922659
14214,28429,28428,56857,9.88527512550354,0.009111795150308254
14314,28629,28628,57257,9.986868858337402,0.008960426757708433
14414,28829,28828,57657,10.092884063720703,0.008811356820738444
14515,29031,29030,58061,10.16550588607788,0.008661971411963471
14615,29231,29230,58461,10.231786251068115,0.0085147352050275
14715,29431,29430,58861,10.297982215881348,0.008371399791506053
14815,29631,29630,59261,10.361873149871826,0.008230277060289374
14915,29831,29830,59661,10.435137033462524,0.008088785214119236
15015,30031,30030,60061,10.5000638961792,0.007957725611132869
15115,30231,30230,60461,10.563796043395996,0.007828766165637954
15215,30431,30430,60861,10.637076139450073,0.007702214071622525
15315,30631,30630,61261,10.709483861923218,0.007579056214627207
15415,30831,30830,61661,10.788156032562256,0.007458542171695687
15516,31033,31032,62065,10.865755081176758,0.007338314326559178
15616,31233,31232,62465,10.929435968399048,0.007220560957340546
15716,31433,31432,62865,10.995519161224365,0.007104786479107159
15816,31633,31632,63265,11.059489965438843,0.006993305890992013
15916,31833,31832,63665,11.12909197807312,0.006883644391807818
16016,32033,32032,64065,11.193243026733398,0.006775302164585744
16116,32233,32232,64465,11.256379127502441,0.006668338416285847
16216,32433,32432,64865,11.319308042526245,0.006564102840771003
16316,32633,32632,65265,11.38358211517334,0.00646168482265777
16416,32833,32832,65665,11.443063974380493,0.00636063742741675
16517,33035,33034,66069,11.504501819610596,0.006261352045845996
16617,33235,33234,66469,11.56729793548584,0.00616446061075423
16717,33435,33434,66869,11.638481140136719,0.006068326088936202
16817,33635,33634,67269,11.697715044021606,0.00597415591209079
16917,33835,33834,67669,11.760159254074097,0.005881769753432209
17017,34035,34034,68069,11.822763919830322,0.00579088832402879
17117,34235,34234,68469,11.88634991645813,0.005700441037070479
17217,34435,34434,68869,11.948215007781982,0.00561125633315622
17317,34635,34634,69269,12.009923934936523,0.005523652669130749
17417,34835,34834,69669,12.069901943206787,0.005438853698557275
17518,35037,35036,70073,12.145321130752563,0.00535317600669035
17618,35237,35236,70473,12.203764200210571,0.005268893774460433
17718,35437,35436,70873,12.266256093978882,0.005187057729373812
17818,35637,35636,71273,12.326190948486328,0.005106914522064102
17918,35837,35836,71673,12.386100053787231,0.005027095355570396
18018,36037,36036,72073,12.44614315032959,0.004950044526937833
18118,36237,36236,72473,12.507622003555298,0.004873844016375647
18218,36437,36436,72873,12.571474075317383,0.004799462694000384
18318,36637,36636,73273,12.645108938217163,0.004727414678885444
18418,36837,36836,73673,12.707042932510376,0.004655481375666323
18519,37039,37038,74077,12.767330884933472,0.0045841911071727815
18619,37239,37238,74477,12.828294038772583,0.004514961509392858
18719,37439,37438,74877,12.896565914154053,0.004446586256726498
18819,37639,37638,75277,12.971626043319702,0.004380327440970527
18919,37839,37838,75677,13.036288022994995,0.0043153148028974115
19019,38039,38038,76077,13.098992109298706,0.00425092402749638
19119,38239,38238,76477,13.165167093276978,0.004187519836059987
19219,38439,38438,76877,13.235447883605957,0.0041249477063166114
19319,38639,38638,77277,13.30347990989685,0.004063816790596845
19419,38839,38838,77677,13.37231993675232,0.004003700540499531
19520,39041,39040,78081,13.439068078994751,0.003943925277498849
19620,39241,39240,78481,13.505311965942383,0.003884819167590979
19720,39441,39440,78881,13.57625412940979,0.0038269317385694777
19820,39641,39640,79281,13.652884244918823,0.0037708737474745195
19920,39841,39840,79681,13.723875045776367,0.0037145532579593273
20020,40041,40040,80081,13.798302173614502,0.0036584291949138853
20120,40241,40240,80481,13.858078241348267,0.003603366768594275
20220,40441,40440,80881,13.919543981552124,0.0035489978910629868
20320,40641,40640,81281,13.983485221862793,0.003495686226694369
20420,40841,40840,81681,14.048204898834229,0.0034434990275128852
20521,41043,41042,82085,14.118958950042725,0.0033915132480723444
20621,41243,41242,82485,14.183348178863525,0.00334116452748544
20721,41443,41442,82885,14.248977184295654,0.0032915124515810216
20821,41643,41642,83285,14.309129238128662,0.0032425950542720214
20921,41843,41842,83685,14.370642185211182,0.0031948643660281817
21021,42043,42042,84085,14.43604588508606,0.0031476492059488745
21121,42243,42242,84485,14.501023054122925,0.00310126261251773
21221,42443,42442,84885,14.562581062316895,0.003056129359842945
21321,42643,42642,85285,14.636733055114746,0.0030119612035079987
21421,42843,42842,85685,14.699596881866455,0.002968074746125493
21522,43045,43044,86089,14.76484489440918,0.002924371116217384
21622,43245,43244,86489,14.8334219455719,0.002881569865576798
21722,43445,43444,86889,14.898208856582642,0.002839747643428888
21822,43645,43644,87289,14.967154026031494,0.0027993270866922136
21922,43845,43844,87689,15.048724174499512,0.0027593892451250423
22022,44045,44044,88089,15.132683992385864,0.0027192847850162744
22122,44245,44244,88489,15.204129934310913,0.002679927023142476
22222,44445,44444,88889,15.268203020095825,0.0026419890819075124
22322,44645,44644,89289,15.332620859146118,0.002604373986547768
22422,44845,44844,89689,15.396627187728882,0.002566633685588737
22523,45047,45046,90093,15.461143970489502,0.002528809218388413
22623,45247,45246,90493,15.525268077850342,0.002492101292504614
22723,45447,45446,90893,15.597223043441772,0.002456077738520633
22823,45647,45646,91293,15.662830114364624,0.0024203499482636833
22923,45847,45846,91693,15.72950792312622,0.00238499805154855
23023,46047,46046,92093,15.792171001434326,0.00235038580587238
23123,46247,46246,92493,15.853379964828491,0.0023159784172378144
23223,46447,46446,92893,15.915328025817871,0.0022817855748038618
23323,46647,46646,93293,15.978865146636963,0.002248907300292022
23423,46847,46846,93693,16.042865991592407,0.0022164926452908577
23524,47049,47048,94097,16.111135244369507,0.002183712668552709
23624,47249,47248,94497,16.173521995544434,0.002151878226282065
23724,47449,47448,94897,16.236832857131958,0.002120901752936091
23824,47649,47648,95297,16.302364110946655,0.002090389310674898
23924,47849,47848,95697,16.36510992050171,0.0020602076568302114
24024,48049,48048,96097,16.426560878753662,0.0020300358244441674
24124,48249,48248,96497,16.490967988967896,0.0020007501763382183
24224,48449,48448,96897,16.552967071533203,0.0019725999537984077
24324,48649,48648,97297,16.62134599685669,0.0019446288771185157
24424,48849,48848,97697,16.685590028762817,0.0019167010082839434
24525,49051,49050,98101,16.748387098312378,0.001889088983518954
24625,49251,49250,98501,16.81114625930786,0.0018623959407974152
24725,49451,49450,98901,16.872386932373047,0.0018362003689114308
24825,49651,49650,99301,16.933897256851196,0.0018102601128650523
24925,49851,49850,99701,16.99528408050537,0.0017846602201538415
25025,50051,50050,100101,17.057823181152344,0.0017593600818294342
25125,50251,50250,100501,17.12725305557251,0.001734419535061171
25225,50451,50450,100901,17.204463005065918,0.0017098739985286888
25325,50651,50650,101301,17.28036403656006,0.0016857110768930476
25425,50851,50850,101701,17.341629028320312,0.0016620538342593714
25526,51053,51052,102105,17.40421485900879,0.0016380740395514435
25626,51253,51252,102505,17.466536045074463,0.0016144983521808722
25726,51453,51452,102905,17.526948928833008,0.0015918118810752276
25826,51653,51652,103305,17.594922065734863,0.0015693254066215358
25926,51853,51852,103705,17.659789085388184,0.0015467781832337205
26026,52053,52052,104105,17.722559928894043,0.0015244602389677497
26126,52253,52252,104505,17.784492015838623,0.0015026502572782145
26226,52453,52452,104905,17.84726905822754,0.001481330595269735
26326,52653,52652,105305,17.914132118225098,0.001460079165254246
26426,52853,52852,105705,17.97667694091797,0.0014389821807388493
26527,53055,53054,106109,18.04431700706482,0.0014182443538461934
26627,53255,53254,106509,18.111519813537598,0.0013982646585259067
26727,53455,53454,106909,18.176138877868652,0.0013783474126149002
26827,53655,53654,107309,18.239681005477905,0.0013585571513145516
26927,53855,53854,107709,18.300904035568237,0.0013393216720983194
27027,54055,54054,108109,18.361008167266846,0.0013204230171340332
27127,54255,54254,108509,18.42322087287903,0.0013017306960680928
27227,54455,54454,108909,18.486028909683228,0.0012834669603326036
27327,54655,54654,109309,18.548516988754272,0.0012655251522662237
27427,54855,54854,109709,18.6266610622406,0.0012478452688603019
27528,55057,55056,110113,18.69686484336853,0.0012302125465743373
27628,55257,55256,110513,18.760345935821533,0.0012132053247634216
27728,55457,55456,110913,18.820992946624756,0.0011966904873274232
27828,55657,55656,111313,18.882877111434937,0.0011802019934684825
27928,55857,55856,111713,18.945513248443604,0.0011637458216228502
28028,56057,56056,112113,19.007467031478882,0.0011476477124180966
28128,56257,56256,112513,19.071022987365723,0.0011320792744783767
28228,56457,56456,112913,19.139606952667236,0.0011165924841270373
28328,56657,56656,113313,19.202129125595093,0.0011009499922181403
28428,56857,56856,113713,19.2660551071167,0.0010854847205532423
28529,57059,57058,114117,19.342783212661743,0.0010701102187086783
28629,57259,57258,114517,19.41591215133667,0.0010551348959841258
28729,57459,57458,114917,19.47808599472046,0.0010403849838116121
28829,57659,57658,115317,19.541871070861816,0.0010256658519945917
28929,57859,57858,115717,19.612452030181885,0.0010111866354786103
29029,58059,58058,116117,19.67368793487549,0.0009969480513930067
29129,58259,58258,116517,19.734447956085205,0.0009829123913166627
29229,58459,58458,116917,19.79522204399109,0.0009690605140732158
29329,58659,58658,117317,19.856840133666992,0.0009553096585697534
29429,58859,58858,117717,19.920674085617065,0.0009418003635743267
29530,59061,59060,118121,19.98335099220276,0.0009284304652033482
29630,59261,59260,118521,20.047746896743774,0.0009154142986187284
29730,59461,59460,118921,20.11328101158142,0.0009026317855767636
29830,59661,59660,119321,20.1770441532135,0.0008899873045686885
29930,59861,59860,119721,20.243183135986328,0.0008775041211860132
30030,60061,60060,120121,20.30452013015747,0.0008653225516324965
30130,60261,60260,120521,20.366421937942505,0.0008535461698688634
30230,60461,60460,120921,20.427445888519287,0.0008419674667357488
30330,60661,60660,121321,20.488420009613037,0.0008303386774036522
30430,60861,60860,121721,20.55075693130493,0.0008188580681519754
30531,61063,61062,122125,20.621551036834717,0.0008076775110276781
30631,61263,61262,122525,20.682762145996094,0.0007968731855088166
30731,61463,61462,122925,20.74382996559143,0.0007860349944779897
30831,61663,61662,123325,20.804694890975952,0.0007751927084849044
30931,61863,61862,123725,20.86746907234192,0.0007645015410756932
31031,62063,62062,124125,20.940480947494507,0.0007540276429651918
31131,62263,62262,124525,21.005068063735962,0.0007437460770822886
31231,62463,62462,124925,21.06995391845703,0.0007335321327945892
31331,62663,62662,125325,21.142383098602295,0.0007233619219762391
31431,62863,62862,125725,21.205503940582275,0.0007132575624108962
31532,63065,63064,126129,21.271016120910645,0.0007031791518934151
31632,63265,63264,126529,21.33330202102661,0.000693407276131615
31732,63465,63464,126929,21.396509170532227,0.0006837682224038886
31832,63665,63664,127329,21.474234104156494,0.0006742308091293568
31932,63865,63864,127729,21.548655033111572,0.0006647500198807649
32032,64065,64064,128129,21.622551918029785,0.000655433217201054
32132,64265,64264,128529,21.703758001327515,0.0006463353889688796
32232,64465,64464,128929,21.86014723777771,0.000637319651456879
32332,64665,64664,129329,21.934923887252808,0.0006283514193170035
32432,64865,64864,129729,21.997992038726807,0.0006194827952186915
32533,65067,65066,130133,22.061700105667114,0.0006108092191794662
32633,65267,65266,130533,22.141151189804077,0.0006024799485118703
32733,65467,65466,130933,22.208763122558594,0.0005941212182405992
32833,65667,65666,131333,22.27108120918274,0.0005857944968891536
32933,65867,65866,131733,22.333060026168823,0.0005777440995846808
33033,66067,66066,132133,22.39333701133728,0.0005699266972724137
33133,66267,66266,132533,22.458478927612305,0.0005621643248891333
33233,66467,66466,132933,22.52424907684326,0.0005544437387228325
33333,66667,66666,133333,22.59811019897461,0.0005468635377227691
33433,66867,66866,133733,22.664429903030396,0.0005394013065281456
33534,67069,67068,134137,22.730762243270874,0.00053198819381291
33634,67269,67268,134537,22.797364950180054,0.0005247955643287588
33734,67469,67468,134937,22.8648841381073,0.0005177029627606521
33834,67669,67668,135337,22.945531129837036,0.0005106466347315166
33934,67869,67868,135737,23.018501043319702,0.0005035834270797113
34034,68069,68068,136137,23.09039807319641,0.0004966855250277016
34134,68269,68268,136537,23.16755509376526,0.0004900003000226095
34234,68469,68468,136937,23.24531126022339,0.00048332097387309884
34334,68669,68668,137337,23.31636905670166,0.00047661937030205715
34434,68869,68868,137737,23.38484287261963,0.0004700321654022045
34535,69071,69070,138141,23.46036696434021,0.0004635443572416771
34635,69271,69270,138541,23.529834270477295,0.0004571787334096308
34735,69471,69470,138941,23.6158230304718,0.0004508047311539187
34835,69671,69670,139341,23.694399118423462,0.00044452928748924935
34935,69871,69870,139741,23.792896032333374,0.000438393552017286
35035,70071,70070,140141,23.933488130569458,0.00043236688364006173
35135,70271,70270,140541,24.024163961410522,0.00042636610962974963
35235,70471,70470,140941,24.117117166519165,0.00042040513674547903
35335,70671,70670,141341,24.180429935455322,0.00041459402541517236
35435,70871,70870,141741,24.24325704574585,0.000408864711072116
35536,71073,71072,142145,24.312637090682983,0.000403132403442468
35636,71273,71272,142545,24.37627410888672,0.0003975786292588106
35736,71473,71472,142945,24.439263105392456,0.0003921131712407527
35836,71673,71672,143345,24.49909806251526,0.00038673475432789335
35936,71873,71872,143745,24.563776969909668,0.0003814759245695828
36036,72073,72072,144145,24.631532907485962,0.0003763491886690569
36136,72273,72272,144545,24.69352698326111,0.0003712963254442391
36236,72473,72472,144945,24.75804090499878,0.00036626315303797457
36336,72673,72672,145345,24.81902503967285,0.0003613073808415068
36436,72873,72872,145745,24.886712074279785,0.0003564998014459769
36537,73075,73074,146149,24.960304975509644,0.0003517684228451117
36637,73275,73274,146549,25.045418977737427,0.0003470859518399967
36737,73475,73474,146949,25.154603004455566,0.00034238542432181635
36837,73675,73674,147349,25.23512315750122,0.0003377721888417434
36937,73875,73874,147749,25.311609983444214,0.00033324931614373926
37037,74075,74074,148149,25.387518167495728,0.00032877466863530646
37137,74275,74274,148549,25.46184206008911,0.00032432875466882036
37237,74475,74474,148949,25.529502153396606,0.0003199121004637346
37337,74675,74674,149349,25.607481956481934,0.00031556178091294234
37437,74875,74874,149749,25.67674422264099,0.00031127821212167646
37538,75077,75076,150153,25.760698080062866,0.0003069851531376528
37638,75277,75276,150553,25.841336965560913,0.00030276286615262644
37738,75477,75476,150953,25.905210971832275,0.0002985986174564337
37838,75677,75676,151353,25.96740698814392,0.0002944822463885652
37938,75877,75876,151753,26.03170609474182,0.0002904160362283441
38038,76077,76076,152153,26.10307812690735,0.0002864124403290968
38138,76277,76276,152553,26.17518401145935,0.00028244167543167503
38238,76477,76476,152953,26.23824191093445,0.00027852478478472456
38338,76677,76676,153353,26.300260066986084,0.0002747069173555146
38438,76877,76876,153753,26.36370015144348,0.0002709858114772953
38539,77079,77078,154157,26.429996967315674,0.0002672924926913349
38639,77279,77278,154557,26.49428915977478,0.00026366082676329935
38739,77479,77478,154957,26.55736207962036,0.000260081088605521
38839,77679,77678,155357,26.628175020217896,0.00025660497097583425
38939,77879,77878,155757,26.69702911376953,0.0002532170740752753
39039,78079,78078,156157,26.762163162231445,0.000249862105894635
39139,78279,78278,156557,26.82266902923584,0.0002465091480622687
39239,78479,78478,156957,26.8856520652771,0.00024319187606019246
39339,78679,78678,157357,26.949084043502808,0.00023995092088109765
39439,78879,78878,157757,27.01382327079773,0.00023679246371633084
39540,79081,79080,158161,27.07866406440735,0.00023363741432170235
39640,79281,79280,158561,27.156179189682007,0.0002304928539276233
39740,79481,79480,158961,27.221257209777832,0.00022736031600356234
39840,79681,79680,159361,27.28466010093689,0.00022429472809569855
39940,79881,79880,159761,27.348665952682495,0.0002212867186009496
40040,80081,80080,160161,27.410118103027344,0.00021831011598046925
40140,80281,80280,160561,27.473133087158203,0.00021535368556492132
40240,80481,80480,160961,27.53454613685608,0.00021241060690121028
40340,80681,80680,161361,27.60273027420044,0.00020949154846723123
40440,80881,80880,161761,27.665507078170776,0.00020661824863053065
40541,81083,81082,162165,27.727718114852905,0.00020375826404380435
40641,81283,81282,162565,27.794356107711792,0.0002009538471022078
40741,81483,81482,162965,27.866849899291992,0.00019817875758919694
40841,81683,81682,163365,27.942869186401367,0.00019544804153826215
40941,81883,81882,163765,28.00429892539978,0.00019278533445070357
41041,82083,82082,164165,28.066054105758667,0.00019015671141277296
41141,82283,82282,164565,28.138342142105103,0.00018753012692844666
41241,82483,82482,164965,28.198880910873413,0.00018495469044205076
41341,82683,82682,165365,28.261354207992554,0.0001824572218249232
41441,82883,82882,165765,28.326224088668823,0.00018000883348511461
41542,83085,83084,166169,28.39138913154602,0.00017754663065170265
41642,83285,83284,166569,28.453316926956177,0.00017511878633630218
41742,83485,83484,166969,28.514064073562622,0.0001727470353796481
41842,83685,83684,167369,28.57817006111145,0.00017044773814906474
41942,83885,83884,167769,28.645754098892212,0.000168192474392055
42042,84085,84084,168169,28.706175804138184,0.00016594484112919473
42142,84285,84284,168569,28.768144130706787,0.0001637009127920054
42242,84485,84484,168969,28.828400135040283,0.00016148554606379298
42342,84685,84684,169369,28.88987112045288,0.00015931595937799484
42442,84885,84884,169769,28.951460123062134,0.00015720535074066857
42543,85087,85086,170173,29.01414203643799,0.00015510712129106604
42643,85287,85286,170573,29.07933497428894,0.00015301902981589138
42743,85487,85486,170973,29.150655269622803,0.0001509367516719879
42843,85687,85686,171373,29.213417053222656,0.00014889851699325993
42943,85887,85886,171773,29.27625584602356,0.0001469105714322364
43043,86087,86086,172173,29.342037200927734,0.0001449367195781464
43143,86287,86286,172573,29.40394616127014,0.00014295863287460748
43243,86487,86486,172973,29.465830087661743,0.00014100991283424506
43343,86687,86686,173373,29.52681303024292,0.00013910681993530323
43443,86887,86886,173773,29.594522953033447,0.00013722626148631592
43544,87089,87088,174177,29.660703897476196,0.000135330376518051
43644,87289,87288,174577,29.719914197921753,0.0001334722217873584
43744,87489,87488,174977,29.779982089996338,0.00013165091614106763
43844,87689,87688,175377,29.84107995033264,0.00012985707738058373
43944,87889,87888,175777,29.90396213531494,0.00012808233222352916
44044,88089,88088,176177,29.968348026275635,0.00012632859787115798
44144,88289,88288,176577,30.041334867477417,0.00012460328112476625
44244,88489,88488,176977,30.11862802505493,0.00012291591583379693
44344,88689,88688,177377,30.17786693572998,0.00012126476652245682
44444,88889,88888,177777,30.23773193359375,0.00011963918984645939
44545,89091,89090,178181,30.29670810699463,0.0001180115232430339
44645,89291,89290,178581,30.35511589050293,0.00011642165919494814
44745,89491,89490,178981,30.415800094604492,0.00011487050360592513
44845,89691,89690,179381,30.47470498085022,0.0001133586478329886
44945,89891,89890,179781,30.536998987197876,0.00011187049871040026
45045,90091,90090,180181,30.60517120361328,0.00011038597274011977
45145,90291,90290,180581,30.665380001068115,0.00010891380767797004
45245,90491,90490,180981,30.72723913192749,0.00010747689955334446
45345,90691,90690,181381,30.78827404975891,0.00010607221084003018
45445,90891,90890,181781,30.853456020355225,0.00010468177171523861
45546,91093,91092,182185,30.9131019115448,0.00010328126335128754
45646,91293,91292,182585,30.972707986831665,0.00010190659295263786
45746,91493,91492,182985,31.031719207763672,0.00010055628125608383
45846,91693,91692,183385,31.101589918136597,9.92241229077307e-05
45946,91893,91892,183785,31.16430926322937,9.790250789804027e-05
46046,92093,92092,184185,31.222779035568237,9.659153629019783e-05
46146,92293,92292,184585,31.282708168029785,9.529140614959256e-05
46246,92493,92492,184985,31.354470014572144,9.400391902551128e-05
46346,92693,92692,185385,31.456881999969482,9.27287251912711e-05
46446,92893,92892,185785,31.531164169311523,9.146443006662153e-05
46547,93095,93094,186189,31.605782985687256,9.020271076744699e-05
46647,93295,93294,186589,31.674801111221313,8.897630178099456e-05
46747,93495,93494,186989,31.742414951324463,8.777381094506822e-05
46847,93695,93694,187389,31.813075065612793,8.658846118821059e-05
46947,93895,93894,187789,31.88187313079834,8.541711280645088e-05
47047,94095,94094,188189,31.95291805267334,8.426705601910498e-05
47147,94295,94294,188589,32.02509903907776,8.3142579848123e-05
47247,94495,94494,188989,32.09729290008545,8.20371103771542e-05
47347,94695,94694,189389,32.18608617782593,8.09461441831052e-05
47447,94895,94894,189789,32.25328707695007,7.986790705155107e-05
47548,95097,95096,190193,32.31927704811096,7.87933300547785e-05
47648,95297,95296,190593,32.38481593132019,7.775255755500025e-05
47748,95497,95496,190993,32.4462571144104,7.673850706710915e-05
47848,95697,95696,191393,32.50702404975891,7.574244841671685e-05
47948,95897,95896,191793,32.56598711013794,7.474644786992331e-05
48048,96097,96096,192193,32.63795304298401,7.37476297947579e-05
48148,96297,96296,192593,32.70254397392273,7.276879183600468e-05
48248,96497,96496,192993,32.764564037323,7.18187705444913e-05
48348,96697,96696,193393,32.82630896568298,7.088018018560328e-05
48448,96897,96896,193793,32.88952898979187,6.993998250413446e-05
48549,97099,97098,194197,32.95270109176636,6.899415075101884e-05
48649,97299,97298,194597,33.01601696014404,6.807162562031932e-05
48749,97499,97498,194997,33.07984924316406,6.716226835834011e-05
48849,97699,97698,195397,33.148359060287476,6.626242939790226e-05
48949,97899,97898,195797,33.2096049785614,6.537060257053136e-05
49049,98099,98098,196197,33.27069091796875,6.448441349648132e-05
49149,98299,98298,196597,33.34979009628296,6.360437385327254e-05
49249,98499,98498,196997,33.41513109207153,6.27370202351133e-05
49349,98699,98698,197397,33.47600293159485,6.188935257025183e-05
49449,98899,98898,197797,33.53846216201782,6.105386954099493e-05
49550,99101,99100,198201,33.606016874313354,6.021347451309473e-05
49650,99301,99300,198601,33.66944098472595,5.939477914033675e-05
49750,99501,99500,199001,33.73003101348877,5.8596880940775086e-05
49850,99701,99700,199401,33.79337406158447,5.78095514535441e-05
49950,99901,99900,199801,33.855968952178955,5.702430316514268e-05
50050,100101,100100,200201,33.91671419143677,5.625085952137154e-05
50150,100301,100300,200601,33.98117280006409,5.550218145903701e-05
50250,100501,100500,201001,34.05390405654907,5.47715840925131e-05
50350,100701,100700,201401,34.12641406059265,5.404165415300788e-05
50450,100901,100900,201801,34.1874520778656,5.330900168319847e-05
50551,101103,101102,202205,34.25862693786621,5.258362986721415e-05
50651,101303,101302,202605,34.33473300933838,5.1891280024244815e-05
50751,101503,101502,203005,34.40293002128601,5.121517489468884e-05
50851,101703,101702,203405,34.465912103652954,5.054302430131499e-05
50951,101903,101902,203805,34.52834701538086,4.9869805247115786e-05
51051,102103,102102,204205,34.5994610786438,4.919962326813747e-05
51151,102303,102302,204605,34.6715190410614,4.8542907552255166e-05
51251,102503,102502,205005,34.7339301109314,4.7903805839046464e-05
51351,102703,102702,205405,34.79580783843994,4.7275188382929695e-05
51451,102903,102902,205805,34.863425970077515,4.6645444226357086e-05
51552,103105,103104,206209,34.93513011932373,4.600790896694399e-05
51652,103305,103304,206609,34.99431800842285,4.538790974174408e-05
51752,103505,103504,207009,35.055480003356934,4.478528964614289e-05
51852,103705,103704,207409,35.125855922698975,4.419048837744402e-05
51952,103905,103904,207809,35.18850111961365,4.3593100219979635e-05
52052,104105,104104,208209,35.25419306755066,4.3000121795820345e-05
52152,104305,104304,208609,35.31726312637329,4.242106793022669e-05
52252,104505,104504,209009,35.38417911529541,4.1849358053769155e-05
52352,104705,104704,209409,35.44851112365723,4.127925059440351e-05
52452,104905,104904,209809,35.51094388961792,4.071679436286542e-05
52553,105107,105106,210213,35.57446813583374,4.0162450637070424e-05
52653,105307,105306,210613,35.64508605003357,3.962534499645836e-05
52753,105507,105506,211013,35.71227788925171,3.909372862896381e-05
52853,105707,105706,211413,35.775182008743286,3.856626123627558e-05
52953,105907,105906,211813,35.84217596054077,3.8047723509301315e-05
53053,106107,106106,212213,35.90400290489197,3.7540968902855066e-05
53153,106307,106306,212613,35.96542191505432,3.7045041913201895e-05
53253,106507,106506,213013,36.02898406982422,3.655809932056742e-05
53353,106707,106706,213413,36.0948269367218,3.6075458184646713e-05
53453,106907,106906,213813,36.15817594528198,3.559490123886709e-05
53554,107109,107108,214217,36.22224402427673,3.5118493460720987e-05
53654,107309,107308,214617,36.287328004837036,3.4660711534279084e-05
53754,107509,107508,215017,36.350005865097046,3.421245636981651e-05
53854,107709,107708,215417,36.4267361164093,3.376704634216113e-05
53954,107909,107908,215817,36.50159811973572,3.332276737184541e-05
54054,108109,108108,216217,36.56227898597717,3.2884403631103596e-05
54154,108309,108308,216617,36.63444209098816,3.245579737633296e-05
54254,108509,108508,217017,36.69692397117615,3.2033869085343e-05
54354,108709,108708,217417,36.75911211967468,3.1613480934277026e-05
54454,108909,108908,217817,36.82325601577759,3.1194518887740196e-05
54555,109111,109110,218221,36.88676595687866,3.0776372601044885e-05
54655,109311,109310,218621,36.94714093208313,3.036802552294471e-05
54755,109511,109510,219021,37.01154398918152,2.9963686866388003e-05
54855,109711,109710,219421,37.07317113876343,2.956257478028908e-05
54955,109911,109910,219821,37.145703077316284,2.9165464605280825e-05
55055,110111,110110,220221,37.208394050598145,2.8773619442781398e-05
55155,110311,110310,220621,37.27583980560303,2.8386589314722217e-05
55255,110511,110510,221021,37.34181809425354,2.800494489162376e-05
55355,110711,110710,221421,37.408133029937744,2.7631059997973393e-05
55455,110911,110910,221821,37.47089409828186,2.726392266646076e-05
55556,111113,111112,222225,37.533912897109985,2.6897065123078456e-05
55656,111313,111312,222625,37.59982395172119,2.653832313575744e-05
55756,111513,111512,223025,37.66287708282471,2.6185534068532448e-05
55856,111713,111712,223425,37.72564911842346,2.5837702618988175e-05
55956,111913,111912,223825,37.78809404373169,2.5494838960718564e-05
56056,112113,112112,224225,37.85161900520325,2.5159354731689546e-05
56156,112313,112312,224625,37.91311812400818,2.4831966216797645e-05
56256,112513,112512,225025,37.978302240371704,2.4509057222825604e-05
56356,112713,112712,225425,38.03989791870117,2.418681248729199e-05
56456,112913,112912,225825,38.110198974609375,2.3868444022129383e-05
56557,113115,113114,226229,38.17477798461914,2.3556191364100272e-05
56657,113315,113314,226629,38.23762607574463,2.32534513938797e-05
56757,113515,113514,227029,38.30114698410034,2.2951018693094992e-05
56857,113715,113714,227429,38.36210918426514,2.2648708787882594e-05
56957,113915,113914,227829,38.4267361164093,2.2350633422186926e-05
57057,114115,114114,228229,38.4897198677063,2.205838726543763e-05
57157,114315,114314,228629,38.565540075302124,2.1769862680747687e-05
57257,114515,114514,229029,38.64131283760071,2.148277781867182e-05
57357,114715,114714,229429,38.70189881324768,2.1196788944415933e-05
57457,114915,114914,229829,38.76415705680847,2.0913232059006286e-05
57558,115117,115116,230233,38.825916051864624,2.0630572754566984e-05
57658,115317,115316,230633,38.88910984992981,2.0355435530547253e-05
57758,115517,115516,231033,38.95036602020264,2.0084670740451143e-05
57858,115717,115716,231433,39.01076292991638,1.9815118005125117e-05
57958,115917,115916,231833,39.073758125305176,1.9546345144101378e-05
58058,116117,116116,232233,39.14449715614319,1.9282543162836305e-05
58158,116317,116316,232633,39.20508003234863,1.9025150872184732e-05
58258,116517,116516,233033,39.26600694656372,1.877090736336764e-05
58358,116717,116716,233433,39.3273069858551,1.8517925372826664e-05
58458,116917,116916,233833,39.389875173568726,1.8269186960708648e-05
58559,117119,117118,234237,39.45094108581543,1.8024862487983653e-05
58659,117319,117318,234637,39.511905908584595,1.7786248144470147e-05
58759,117519,117518,235037,39.57428812980652,1.754725716304952e-05
58859,117719,117718,235437,39.64064908027649,1.731171578395909e-05
58959,117919,117918,235837,39.708184003829956,1.708469970895182e-05
59059,118119,118118,236237,39.76994299888611,1.6863221199562754e-05
59159,118319,118318,236637,39.83060598373413,1.6641336201894356e-05
59259,118519,118518,237037,39.895217180252075,1.641927382851309e-05
59359,118719,118718,237437,39.95704793930054,1.6201047542240282e-05
59459,118919,118918,237837,40.01704692840576,1.598856763751764e-05
59560,119121,119120,238241,40.08372116088867,1.5779008401789754e-05
59660,119321,119320,238641,40.15004205703735,1.557431044986517e-05
59760,119521,119520,239041,40.2139630317688,1.536968477946451e-05
59860,119721,119720,239441,40.27495312690735,1.5164558149519381e-05
59960,119921,119920,239841,40.33594298362732,1.4962404983243916e-05
60060,120121,120120,240241,40.398828983306885,1.4766685971927884e-05
60160,120321,120320,240641,40.46017408370972,1.457505770578934e-05
60260,120521,120520,241041,40.5226411819458,1.4382059827067614e-05
60360,120721,120720,241441,40.58719086647034,1.4187539157506675e-05
60460,120921,120920,241841,40.66245698928833,1.3996562486301185e-05
60561,121123,121122,242245,40.73913311958313,1.3808914828650358e-05
60661,121323,121322,242645,40.80331110954285,1.3625179787876983e-05
60761,121523,121522,243045,40.86395311355591,1.344206446166368e-05
60861,121723,121722,243445,40.92599105834961,1.326128379466981e-05
60961,121923,121922,243845,40.98927712440491,1.308392771305674e-05
61061,122123,122122,244245,41.05084705352783,1.2908697534080166e-05
61161,122323,122322,244645,41.11640000343323,1.273450965751624e-05
61261,122523,122522,245045,41.18063926696777,1.2562947305821196e-05
61361,122723,122722,245445,41.24595499038696,1.2395661101612578e-05
61461,122923,122922,245845,41.30947399139404,1.2231749394925177e-05
61562,123125,123124,246249,41.37196397781372,1.2068110216465646e-05
61662,123325,123324,246649,41.43293499946594,1.190761661267762e-05
61762,123525,123524,247049,41.49506115913391,1.1748879106988308e-05
61862,123725,123724,247449,41.55664610862732,1.1592878919587142e-05
61962,123925,123924,247849,41.62825322151184,1.1441064976767601e-05
62062,124125,124124,248249,41.68939208984375,1.129329834429313e-05
62162,124325,124324,248649,41.75192999839783,1.1147214705800233e-05
62262,124525,124524,249049,41.81422805786133,1.1001034686926076e-05
62362,124725,124724,249449,41.87589120864868,1.0856280824629917e-05
62462,124925,124924,249849,41.937427043914795,1.0715669831420112e-05
62563,125127,125126,250253,42.00268602371216,1.0577419157284645e-05
62663,125327,125326,250653,42.06531023979187,1.0441099034850115e-05
62763,125527,125526,251053,42.13240098953247,1.0304129621921061e-05
62863,125727,125726,251453,42.19511604309082,1.016850405473781e-05
62963,125927,125926,251853,42.255818128585815,1.003590734087636e-05
63063,126127,126126,252253,42.31610417366028,9.905663515528842e-06
63163,126327,126326,252653,42.37799406051636,9.776231674630495e-06
63263,126527,126526,253053,42.439424991607666,9.646969993890194e-06
63363,126727,126726,253453,42.50305199623108,9.518397385894576e-06
63463,126927,126926,253853,42.563010931015015,9.391345600739486e-06
63564,127129,127128,254257,42.63484311103821,9.265171867246204e-06
63664,127329,127328,254657,42.69580101966858,9.142481799285115e-06
63764,127529,127528,255057,42.76039791107178,9.021334224134595e-06
63864,127729,127728,255457,42.83613109588623,8.901121562321754e-06
63964,127929,127928,255857,42.908565282821655,8.782294051120254e-06
64064,128129,128128,256257,42.97164988517761,8.665488081012583e-06
64164,128329,128328,256657,43.03434991836548,8.550460750440408e-06
64264,128529,128528,257057,43.09929895401001,8.43674364180119e-06
64364,128729,128728,257457,43.16047501564026,8.324758719936274e-06
64464,128929,128928,257857,43.22327995300293,8.215242654047104e-06
64565,129131,129130,258261,43.28415393829346,8.106802506795829e-06
64665,129331,129330,258661,43.344380140304565,8.000536206253941e-06
64765,129531,129530,259061,43.40612602233887,7.895380604105163e-06
64865,129731,129730,259461,43.47316384315491,7.792696216688844e-06
64965,129931,129930,259861,43.53782391548157,7.692953330640033e-06
65065,130131,130130,260261,43.60539412498474,7.594610385406215e-06
65165,130331,130330,260661,43.66908311843872,7.496273077682297e-06
65265,130531,130530,261061,43.73137903213501,7.398593347159155e-06
65365,130731,130730,261461,43.792842864990234,7.302999744868574e-06
65465,130931,130930,261861,43.856045961380005,7.209465408994336e-06
65566,131133,131132,262265,43.920734167099,7.115722701213056e-06
65666,131333,131332,262665,43.98829197883606,7.0229707376554675e-06
65766,131533,131532,263065,44.049681186676025,6.930881685774421e-06
65866,131733,131732,263465,44.11652398109436,6.8400844726079e-06
65966,131933,131932,263865,44.17905807495117,6.750581686664404e-06
66066,132133,132132,264265,44.242534160614014,6.66209894777586e-06
66166,132333,132332,264665,44.3046350479126,6.5741509130985995e-06
66266,132533,132532,265065,44.36621809005737,6.48645199468879e-06
66366,132733,132732,265465,44.42738199234009,6.399695302363347e-06
66466,132933,132932,265865,44.487658977508545,6.314753666567243e-06
66567,133135,133134,266269,44.551188230514526,6.230391419451172e-06
66667,133335,133334,266669,44.62120699882507,6.147231091210102e-06
66767,133535,133534,267069,44.68229699134827,6.064590273535045e-06
66867,133735,133734,267469,44.743597984313965,5.983633197660427e-06
66967,133935,133934,267869,44.805083990097046,5.904500097168502e-06
67067,134135,134134,268269,44.86585307121277,5.8261195620669355e-06
67167,134335,134334,268669,44.934552907943726,5.7483127715344485e-06
67267,134535,134534,269069,45.011234998703,5.6722020976153525e-06
67367,134735,134734,269469,45.07902002334595,5.59811751231062e-06
67467,134935,134934,269869,45.14584684371948,5.524869320789642e-06
67568,135137,135136,270273,45.210299015045166,5.451012558301816e-06
67668,135337,135336,270673,45.271103858947754,5.378938124540822e-06
67768,135537,135536,271073,45.33196210861206,5.3088875837808785e-06
67868,135737,135736,271473,45.40041422843933,5.240498582477052e-06
67968,135937,135936,271873,45.47211313247681,5.172779183017556e-06
68068,136137,136136,272273,45.54034614562988,5.1052908066521035e-06
68168,136337,136336,272673,45.60788917541504,5.038372022308147e-06
68268,136537,136536,273073,45.67269587516785,4.972691850730634e-06
68368,136737,136736,273473,45.73454809188843,4.908635577391338e-06
68468,136937,136936,273873,45.79585289955139,4.845681559774986e-06
68569,137139,137138,274277,45.85769200325012,4.781987861208881e-06
68669,137339,137338,274677,45.9191529750824,4.718427398654161e-06
68769,137539,137538,275077,45.988105058670044,4.655627763733472e-06
68869,137739,137738,275477,46.052348136901855,4.5947647018922884e-06
68969,137939,137938,275877,46.13656687736511,4.5351459607733985e-06
69069,138139,138138,276277,46.24317717552185,4.475362057572486e-06
69169,138339,138338,276677,46.3341338634491,4.415412801732109e-06
69269,138539,138538,277077,46.42189884185791,4.356381009844091e-06
69369,138739,138738,277477,46.50967597961426,4.2986476065856275e-06
69469,138939,138938,277877,46.60119700431824,4.241636799821523e-06
69570,139141,139140,278281,46.713606119155884,4.184458058229318e-06
69670,139341,139340,278681,46.833035945892334,4.128573691093181e-06
69770,139541,139540,279081,47.00057792663574,4.073628937244107e-06
69870,139741,139740,279481,47.163334131240845,4.019384169356878e-06
69970,139941,139940,279881,47.26028895378113,3.9656849566078106e-06
70070,140141,140140,280281,47.35255408287048,3.912716865861502e-06
70170,140341,140340,280681,47.52888107299805,3.860739730706228e-06
70270,140541,140540,281081,47.682695150375366,3.8099352109141677e-06
70370,140741,140740,281481,47.79028105735779,3.7602608635376523e-06
70470,140941,140940,281881,47.89018988609314,3.711283297876071e-06
70571,141143,141142,282285,48.01051902770996,3.6621119616174e-06
70671,141343,141342,282685,48.13720202445984,3.6140261599831843e-06
70771,141543,141542,283085,48.28184103965759,3.5672574638238214e-06
70871,141743,141742,283485,48.451282024383545,3.5218198378121066e-06
70971,141943,141942,283885,48.55519199371338,3.4767756128437345e-06
71071,142143,142142,284285,48.64660286903381,3.4314777890495462e-06
71171,142343,142342,284685,48.73191499710083,3.3865220333733076e-06
71271,142543,142542,285085,48.851682901382446,3.342875262033436e-06
71371,142743,142742,285485,48.950061082839966,3.300474337122758e-06
71471,142943,142942,285885,49.062719106674194,3.258373914769819e-06
71572,143145,143144,286289,49.14175605773926,3.2155494402842386e-06
71672,143345,143344,286689,49.20627808570862,3.173140221056529e-06
71772,143545,143544,287089,49.277894020080566,3.131373868268516e-06
71872,143745,143744,287489,49.34457993507385,3.0905167018022717e-06
71972,143945,143944,287889,49.404491901397705,3.0502612173691828e-06
72072,144145,144144,288289,49.46297526359558,3.0101730893575022e-06
72172,144345,144344,288689,49.52546405792236,2.9702133934267824e-06
72272,144545,144544,289089,49.59100008010864,2.930729137943508e-06
72372,144745,144744,289489,49.6502890586853,2.891960787883277e-06
72472,144945,144944,289889,49.709312915802,2.853758575963227e-06
72573,145147,145146,290293,49.76775789260864,2.8154894636607945e-06
72673,145347,145346,290693,49.826874017715454,2.7779771944394187e-06
72773,145547,145546,291093,49.885855197906494,2.7411133582366744e-06
72873,145747,145746,291493,49.94642901420593,2.704941901160451e-06
72973,145947,145946,291893,50.0100839138031,2.669262329436456e-06
73073,146147,146146,292293,50.06869697570801,2.6340008269975367e-06
73173,146347,146346,292693,50.13275098800659,2.5993981340683537e-06
73273,146547,146546,293093,50.19088411331177,2.5657203667815465e-06
73373,146747,146746,293493,50.24940609931946,2.532789066555339e-06
73473,146947,146946,293893,50.30942106246948,2.50011134279012e-06
73574,147149,147148,294297,50.369611978530884,2.467259826246608e-06
73674,147349,147348,294697,50.42786192893982,2.4353362963411973e-06
73774,147549,147548,295097,50.48671293258667,2.4043138531598285e-06
73874,147749,147748,295497,50.547229051589966,2.37386541896849e-06
73974,147949,147948,295897,50.61403799057007,2.3434816861004225e-06
74074,148149,148148,296297,50.674803018569946,2.3131430997051076e-06
74174,148349,148348,296697,50.74156618118286,2.283247669469385e-06
74274,148549,148548,297097,50.806737184524536,2.253975807006888e-06
74374,148749,148748,297497,50.87626004219055,2.2250664127367224e-06
74474,148949,148948,297897,50.943613052368164,2.196226531684181e-06
74575,149151,149150,298301,51.01614189147949,2.1671703462334003e-06
74675,149351,149350,298701,51.08936524391174,2.1386841571338265e-06
74775,149551,149550,299101,51.16186785697937,2.1106847409432683e-06
74875,149751,149750,299501,51.22897696495056,2.083160119411901e-06
74975,149951,149950,299901,51.29247808456421,2.055870114067057e-06
75075,150151,150150,300301,51.37346601486206,2.0286581622842124e-06
75175,150351,150350,300701,51.46055793762207,2.001678594610852e-06
75275,150551,150550,301101,51.52391004562378,1.9751612161495315e-06
75375,150751,150750,301501,51.58907103538513,1.9490634140730767e-06
75475,150951,150950,301901,51.65888595581055,1.9231725683858647e-06
75576,151153,151152,302305,51.73671317100525,1.897276205675667e-06
75676,151353,151352,302705,51.82238817214966,1.8721762234944973e-06
75776,151553,151552,303105,51.91272211074829,1.8476386645876327e-06
75876,151753,151752,303505,51.99655795097351,1.8233658248114926e-06
75976,151953,151952,303905,52.083575963974,1.7992795376471934e-06
76076,152153,152152,304305,52.174535036087036,1.7756602025019653e-06
76176,152353,152352,304705,52.25943207740784,1.7526567163773291e-06
76276,152553,152552,305105,52.343437910079956,1.730046675658995e-06
76376,152753,152752,305505,52.4360671043396,1.7075830281189038e-06
76476,152953,152952,305905,52.51924705505371,1.6853197299998661e-06
76577,153155,153154,306309,52.60535407066345,1.6632740162371466e-06
76677,153355,153354,306709,52.7059428691864,1.641958314212697e-06
76777,153555,153554,307109,52.807437896728516,1.6209768166841254e-06
76877,153755,153754,307509,52.89422607421875,1.6001114613554674e-06
76977,153955,153954,307909,52.966979026794434,1.5793171581909331e-06
77077,154155,154154,308309,53.04375910758972,1.5587758224610203e-06
77177,154355,154354,308709,53.11430311203003,1.5387101828945736e-06
77277,154555,154554,309109,53.18322491645813,1.5190614429729995e-06
77377,154755,154754,309509,53.249943017959595,1.499491205619686e-06
77477,154955,154954,309909,53.32708406448364,1.479828142619619e-06
77578,155157,155156,310313,53.40073585510254,1.4601140259797666e-06
77678,155357,155356,310713,53.469146966934204,1.4410305389634888e-06
77778,155557,155556,311113,53.55173707008362,1.4223108037130692e-06
77878,155757,155756,311513,53.63024401664734,1.4036687264117373e-06
77978,155957,155956,311913,53.698304891586304,1.3850540833661777e-06
78078,156157,156156,312313,53.76786017417908,1.3667010044589633e-06
78178,156357,156356,312713,53.840993881225586,1.3487264235601684e-06
78278,156557,156556,313113,53.911596059799194,1.3309778004710473e-06
78378,156757,156756,313513,53.9773850440979,1.3133286935518504e-06
78478,156957,156956,313913,54.04286813735962,1.2958550399914074e-06
78579,157159,157158,314317,54.112529039382935,1.2785058880452096e-06
78679,157359,157358,314717,54.21315598487854,1.2616366022587691e-06
78779,157559,157558,315117,54.3035409450531,1.2450022667915494e-06
78879,157759,157758,315517,54.407307863235474,1.228564228909038e-06
78979,157959,157958,315917,54.550549268722534,1.2123972180442847e-06
79079,158159,158158,316317,54.69971203804016,1.1966345570892125e-06
79179,158359,158358,316717,54.81678605079651,1.1812765634458496e-06
79279,158559,158558,317117,54.9197359085083,1.1661133984540584e-06
79379,158759,158758,317517,55.053932905197144,1.1509604386044877e-06
79479,158959,158958,317917,55.3762149810791,1.1359297236404193e-06
79580,159161,159160,318321,55.515713930130005,1.1211606615215198e-06
79680,159361,159360,318721,55.788756132125854,1.106994003751121e-06
79780,159561,159560,319121,55.90830707550049,1.0930002808288197e-06
79880,159761,159760,319521,56.0097599029541,1.0789334353930932e-06
79980,159961,159960,319921,56.10833501815796,1.0648759325701037e-06
80080,160161,160160,320321,56.21704697608948,1.0511011777225084e-06
80180,160361,160360,320721,56.333479166030884,1.037718651993088e-06
80280,160561,160560,321121,56.413639068603516,1.02453581122427e-06
80380,160761,160760,321521,56.48496913909912,1.0113074792462165e-06
80480,160961,160960,321921,56.55391502380371,9.980409102504748e-07
80581,161163,161162,322325,56.62382984161377,9.84812725307809e-07
80681,161363,161362,322725,56.687779903411865,9.71989968978785e-07
80781,161563,161562,323125,56.75088405609131,9.59338485035773e-07
80881,161763,161762,323525,56.81665015220642,9.467388385549771e-07
80981,161963,161962,323925,56.881009101867676,9.342113440382171e-07
81081,162163,162162,324325,56.94509315490723,9.218428893081178e-07
81181,162363,162362,324725,57.011871099472046,9.096524955728146e-07
81281,162563,162562,325125,57.079885959625244,8.975950408413405e-07
81381,162763,162762,325525,57.14629101753235,8.856597116835539e-07
81481,162963,162962,325925,57.212536096572876,8.739086048007357e-07
81582,163165,163164,326329,57.28051018714905,8.623056274364478e-07
81682,163365,163364,326729,57.34314298629761,8.510728628959714e-07
81782,163565,163564,327129,57.404136180877686,8.399859576997568e-07
81882,163765,163764,327529,57.46626019477844,8.28973399623453e-07
81982,163965,163964,327929,57.528002977371216,8.18121036949982e-07
82082,164165,164164,328329,57.5944390296936,8.07562756459861e-07
82182,164365,164364,328729,57.672703981399536,7.972682338575978e-07
82282,164565,164564,329129,57.80600118637085,7.870567860262749e-07
82382,164765,164764,329529,57.9662880897522,7.76845055511189e-07
82482,164965,164964,329929,58.10435509681702,7.667710316043862e-07
82583,165167,165166,330333,58.20024108886719,7.56899448496898e-07
82683,165367,165366,330733,58.339402198791504,7.473681430137038e-07
82783,165567,165566,331133,58.41625690460205,7.378826751550724e-07
82883,165767,165766,331533,58.48291492462158,7.283698627410048e-07
82983,165967,165966,331933,58.555341958999634,7.189291587429368e-07
83083,166167,166166,332333,58.62894606590271,7.096616351320971e-07
83183,166367,166366,332733,58.69477295875549,7.005564449327429e-07
83283,166567,166566,333133,58.76033806800842,6.915363164143912e-07
83383,166767,166766,333533,58.82162809371948,6.825485567282871e-07
83483,166967,166966,333933,58.88571619987488,6.736054163060824e-07
83584,167169,167168,334337,58.948275089263916,6.64675622170777e-07
83684,167369,167368,334737,59.00863003730774,6.559731621402759e-07
83784,167569,167568,335137,59.07350206375122,6.473728992648623e-07
83884,167769,167768,335537,59.14472699165344,6.388193986135177e-07
83984,167969,167968,335937,59.20524621009827,6.303404185190975e-07
84084,168169,168168,336337,59.26683211326599,6.220153400005334e-07
84184,168369,168368,336737,59.32881307601929,6.138386465811043e-07
84284,168569,168568,337137,59.3892240524292,6.057323681299346e-07
84384,168769,168768,337537,59.44555401802063,5.976997003102e-07
84484,168969,168968,337937,59.50339126586914,5.898358063044231e-07
84585,169171,169170,338341,59.56257605552673,5.820911172253894e-07
84685,169371,169370,338741,59.640340089797974,5.745292798689279e-07
84785,169571,169570,339141,59.697405099868774,5.670188052183681e-07
84885,169771,169770,339541,59.75347399711609,5.596269024825933e-07
84985,169971,169970,339941,59.812660932540894,5.524269980773158e-07
85085,170171,170170,340341,59.870933055877686,5.453812953359679e-07
85185,170371,170370,340741,59.92925190925598,5.384007097581502e-07
85285,170571,170570,341141,59.98823308944702,5.314629742103067e-07
85385,170771,170770,341541,60.057323932647705,5.246125249619598e-07
85485,170971,170970,341941,60.138755083084106,5.178940241492014e-07
85586,171173,171172,342345,60.19812226295471,5.112461401192589e-07
85686,171373,171372,342745,60.25745511054993,5.047510456620906e-07
85786,171573,171572,343145,60.3152060508728,4.98279971848266e-07
85886,171773,171772,343545,60.37279200553894,4.918378873496897e-07
85986,171973,171972,343945,60.430197954177856,4.855003412850737e-07
86086,172173,172172,344345,60.488065004348755,4.793014542702111e-07
86186,172373,172372,344745,60.54468107223511,4.731707162234944e-07
86286,172573,172572,345145,60.61127591133118,4.6703370544062936e-07
86386,172773,172772,345545,60.66874313354492,4.6092387943038116e-07
86486,172973,172972,345945,60.72702097892761,4.549208125067141e-07
86587,173175,173174,346349,60.79018211364746,4.489617986992717e-07
86687,173375,173374,346749,60.84961915016174,4.4309639238041163e-07
86787,173575,173574,347149,60.90852117538452,4.372536356281754e-07
86887,173775,173774,347549,60.96709609031677,4.3148845364379756e-07
86987,173975,173974,347949,61.02718806266785,4.2582792364123674e-07
87087,174175,174174,348349,61.09632921218872,4.202407683102412e-07
87187,174375,174374,348749,61.16103219985962,4.1470201511649623e-07
87287,174575,174574,349149,61.221421003341675,4.0923929625836375e-07
87387,174775,174774,349549,61.28217792510986,4.038954064719308e-07
87487,174975,174974,349949,61.34342002868652,3.9866535927738726e-07
87588,175177,175176,350353,61.40755915641785,3.934479138385259e-07
87688,175377,175376,350753,61.46937298774719,3.8831585236473277e-07
87788,175577,175576,351153,61.53162622451782,3.8324783431102253e-07
87888,175777,175776,351553,61.59987282752991,3.783014300808727e-07
87988,175977,175976,351953,61.66361403465271,3.7349043189766426e-07
88088,176177,176176,352353,61.728219985961914,3.687543516557307e-07
88188,176377,176376,352753,61.793983936309814,3.6402077382938554e-07
88288,176577,176576,353153,61.85445499420166,3.592973850894314e-07
88388,176777,176776,353553,61.913514137268066,3.5466825079840123e-07
88488,176977,176976,353953,61.97700500488281,3.501833935038594e-07
88589,177179,177178,354357,62.03881001472473,3.457401211960559e-07
88689,177379,177378,354757,62.10493302345276,3.413307633637492e-07
88789,177579,177578,355157,62.17434000968933,3.3690559595217554e-07
88889,177779,177778,355557,62.2491180896759,3.325447541066129e-07
88989,177979,177978,355957,62.31930208206177,3.2829432744079283e-07
89089,178179,178178,356357,62.38290095329285,3.241100511424351e-07
89189,178379,178378,356757,62.445334911346436,3.1992958901349495e-07
89289,178579,178578,357157,62.50740385055542,3.157490857419479e-07
89389,178779,178778,357557,62.57143998146057,3.1160703902677945e-07
89489,178979,178978,357957,62.639281034469604,3.075258219620171e-07
89590,179181,179180,358361,62.70172095298767,3.034554244735506e-07
89690,179381,179380,358761,62.763108015060425,2.994642989567752e-07
89790,179581,179580,359161,62.82370710372925,2.955189481870578e-07
89890,179781,179780,359561,62.88573718070984,2.916317893811425e-07
89990,179981,179980,359961,62.94618320465088,2.878017806375548e-07
90090,180181,180180,360361,63.008506059646606,2.840178070243734e-07
90190,180381,180380,360761,63.06947708129883,2.802761809596499e-07
90290,180581,180580,361161,63.13551092147827,2.7659266984286624e-07
90390,180781,180780,361561,63.199581146240234,2.729884454726329e-07
90490,180981,180980,361961,63.260847091674805,2.694570228341854e-07
90591,181183,181182,362365,63.32175087928772,2.659236718974791e-07
90691,181383,181382,362765,63.38357400894165,2.6243452007327257e-07
90791,181583,181582,363165,63.44469404220581,2.58993114677176e-07
90891,181783,181782,363565,63.505364179611206,2.5566217880270534e-07
90991,181983,181982,363965,63.56713104248047,2.5243783962857854e-07
91091,182183,182182,364365,63.638176918029785,2.4924061306646697e-07
91191,182383,182382,364765,63.70151996612549,2.4601781448732245e-07
91291,182583,182582,365165,63.76726007461548,2.428088448939167e-07
91391,182783,182782,365565,63.829344034194946,2.3968076488781484e-07
91491,182983,182982,365965,63.890239238739014,2.3664058088134135e-07
91592,183185,183184,366369,63.95210099220276,2.3361125845763882e-07
91692,183385,183384,366769,64.01482892036438,2.306154779676401e-07
91792,183585,183584,367169,64.08338809013367,2.2762646922499224e-07
91892,183785,183784,367569,64.15010404586792,2.2467076897077982e-07
91992,183985,183984,367969,64.21209907531738,2.2176874456018583e-07
92092,184185,184184,368369,64.27449011802673,2.1891465319048568e-07
92192,184385,184384,368769,64.35121083259583,2.160808283472879e-07
92292,184585,184584,369169,64.42587995529175,2.132515083416634e-07
92392,184785,184784,369569,64.4876389503479,2.1044556050318778e-07
92492,184985,184984,369969,64.54858899116516,2.0768665827082568e-07
92593,185187,185186,370373,64.61726188659668,2.049393320298659e-07
92693,185387,185386,370773,64.67952394485474,2.0223895870476415e-07
92793,185587,185586,371173,64.73956108093262,1.9956986565865546e-07
92893,185787,185786,371573,64.80754017829895,1.9695624011774926e-07
92993,185987,185986,371973,64.87872195243835,1.9439022761319223e-07
93093,186187,186186,372373,64.93885827064514,1.9184348751990393e-07
93193,186387,186386,372773,65.00127601623535,1.8931807932418783e-07
93293,186587,186586,373173,65.06279993057251,1.8684723828702833e-07
93393,186787,186786,373573,65.13407516479492,1.8444155622733132e-07
93493,186987,186986,373973,65.19764590263367,1.8207093099068698e-07
93594,187189,187188,374377,65.26067900657654,1.7968696706717006e-07
93694,187389,187388,374777,65.32538414001465,1.773497535135692e-07
93794,187589,187588,375177,65.39113807678223,1.750610675730683e-07
93894,187789,187788,375577,65.4549069404602,1.7282639514493302e-07
93994,187989,187988,375977,65.51540112495422,1.7063077085102618e-07
94094,188189,188188,376377,65.57798600196838,1.6845547286051536e-07
94194,188389,188388,376777,65.64220094680786,1.662951619960348e-07
94294,188589,188588,377177,65.70305395126343,1.6416455155661717e-07
94394,188789,188788,377577,65.76529288291931,1.620813442127127e-07
94494,188989,188988,377977,65.8293149471283,1.6003768625909009e-07
94595,189191,189190,378381,65.89374089241028,1.5798376968129012e-07
94695,189391,189390,378781,65.95532894134521,1.5594927282129926e-07
94795,189591,189590,379181,66.0213840007782,1.5393724878015208e-07
94895,189791,189790,379581,66.09096693992615,1.5196762477585909e-07
94995,189991,189990,379981,66.15965104103088,1.500259445314524e-07
95095,190191,190190,380381,66.22487902641296,1.4808877558474724e-07
95195,190391,190390,380781,66.28939414024353,1.461591711799253e-07
95295,190591,190590,381181,66.35283493995667,1.4425512259684798e-07
95395,190791,190790,381581,66.41977000236511,1.4237927665839035e-07
95495,190991,190990,381981,66.49664902687073,1.4052204863592887e-07
95596,191193,191192,382385,66.57035994529724,1.3866669116723945e-07
95696,191393,191392,382785,66.64188313484192,1.36861693201495e-07
95796,191593,191592,383185,66.70394110679626,1.3508902453702186e-07
95896,191793,191792,383585,66.76589703559875,1.3333551394461236e-07
95996,191993,191992,383985,66.82851600646973,1.3159468565300743e-07
96096,192193,192192,384385,66.88961505889893,1.298758445492291e-07
96196,192393,192392,384785,66.95433688163757,1.2819087595875126e-07
96296,192593,192592,385185,67.01899695396423,1.2654030129500964e-07
96396,192793,192792,385585,67.09030389785767,1.2491296775374385e-07
96496,192993,192992,385985,67.15491914749146,1.232975807588221e-07
96597,193195,193194,386389,67.21621489524841,1.21681086645127e-07
96697,193395,193394,386789,67.27611207962036,1.2011397492136512e-07
96797,193595,193594,387189,67.33674001693726,1.1859255832053948e-07
96897,193795,193794,387589,67.39828491210938,1.1710314294690344e-07
96997,193995,193994,387989,67.46118593215942,1.1561863928819943e-07
97097,194195,194194,388389,67.52262115478516,1.1413259145640853e-07
97197,194395,194394,388789,67.58765411376953,1.1266647268651179e-07
97297,194595,194594,389189,67.65419793128967,1.1123815389220658e-07
97397,194795,194794,389589,67.71676707267761,1.0983707308542618e-07
97497,194995,194994,389989,67.77789402008057,1.0844044261370887e-07
97598,195197,195196,390393,67.84028601646423,1.0702971110083916e-07
97698,195397,195396,390793,67.9024760723114,1.0564846004107998e-07
97798,195597,195596,391193,67.96525812149048,1.0429443531656666e-07
97898,195797,195796,391593,68.02767515182495,1.0296136319101379e-07
97998,195997,195996,391993,68.09445810317993,1.0163519263577301e-07
98098,196197,196196,392393,68.15877223014832,1.0031055309750041e-07
98198,196397,196396,392793,68.220046043396,9.899313081771302e-08
98298,196597,196596,393193,68.28225922584534,9.769131601394468e-08
98398,196797,196796,393593,68.34306192398071,9.641004054117868e-08
98498,196997,196996,393993,68.40409517288208,9.514998789068313e-08
98599,197199,197198,394397,68.46648097038269,9.389684417067932e-08
98699,197399,197398,394797,68.52869296073914,9.267288763188241e-08
98799,197599,197598,395197,68.60963296890259,9.146341848563611e-08
98899,197799,197798,395597,68.68404603004456,9.026603997886941e-08
98999,197999,197998,395997,68.74426889419556,8.908089308017963e-08
99099,198199,198198,396397,68.80768084526062,8.791512840493742e-08
99199,198399,198398,396797,68.87003302574158,8.677837459261317e-08
99299,198599,198598,397197,68.93086504936218,8.566834892541664e-08
99399,198799,198798,397597,68.99082899093628,8.456765038740797e-08
99499,198999,198998,397997,69.05367422103882,8.346420550597914e-08
99600,199201,199200,398401,69.12402701377869,8.235951600078817e-08
99700,199401,199400,398801,69.1858160495758,8.129874259265131e-08
99800,199601,199600,399201,69.24980020523071,8.027370658637301e-08
99900,199801,199800,399601,69.31107902526855,7.926245077442256e-08
100000,200001,200000,400001,69.37177109718323,7.824581526884113e-08


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0006909370422363281,30.358106049564984
100,201,200,401,0.06297898292541504,1.7063375198016169
200,401,400,801,0.12068986892700195,1.0108894113540814
300,601,600,1201,0.1797010898590088,0.7489939892258344
400,801,800,1601,0.2371671199798584,0.6081938727196392
501,1003,1002,2005,0.29901909828186035,0.5168895867181229
601,1203,1202,2405,0.3597109317779541,0.452278382327617
701,1403,1402,2805,0.4363288879394531,0.40291992726905773
801,1603,1602,3205,0.5007870197296143,0.3634630940471491
901,1803,1802,3605,0.5554502010345459,0.33097564129661755
1001,2003,2002,4005,0.612037181854248,0.3037093528611154
1101,2203,2202,4405,0.6704959869384766,0.2803953971483973
1201,2403,2402,4805,0.731205940246582,0.26019451460291226
1301,2603,2602,5205,0.7891478538513184,0.24250818197445992
1401,2803,2802,5605,0.8446431159973145,0.22685332490806293
1502,3005,3004,6009,0.8997559547424316,0.2127929708960007
1602,3205,3204,6409,0.9590818881988525,0.20030755961093588
1702,3405,3404,6809,1.0188090801239014,0.18902363243190226
1802,3605,3604,7209,1.1354889869689941,0.17874588608055825
1902,3805,3804,7609,1.1929447650909424,0.16936686708805634
2002,4005,4004,8009,1.2480969429016113,0.16078928006504323
2102,4205,4204,8409,1.3040919303894043,0.15289388141740703
2202,4405,4404,8809,1.3596839904785156,0.1455894973020299
2302,4605,4604,9209,1.4141571521759033,0.13880996643974702
2402,4805,4804,9609,1.471203088760376,0.13250544845542997
2503,5007,5006,10013,1.527184009552002,0.12658272496808612
2603,5207,5206,10413,1.5825860500335693,0.12107898410631822
2703,5407,5406,10813,1.639333963394165,0.11592039425419869
2803,5607,5606,11213,1.6979539394378662,0.11108349163202878
2903,5807,5806,11613,1.770596981048584,0.10652119458942605
3003,6007,6006,12013,1.842939853668213,0.10222880204007911
3103,6207,6206,12413,1.9022667407989502,0.09818713706730445
3203,6407,6406,12813,1.964468002319336,0.09436920147170691
3303,6607,6606,13213,2.0247550010681152,0.09073320222110537
3403,6807,6806,13613,2.0829389095306396,0.08729857820057606
3504,7009,7008,14017,2.1414718627929688,0.08401838454826126
3604,7209,7208,14417,2.202371120452881,0.08093927928962326
3704,7409,7408,14817,2.260944128036499,0.07800912151469362
3804,7609,7608,15217,2.3210020065307617,0.0752232971485176
3904,7809,7808,15617,2.3794310092926025,0.07257609242688355
4004,8009,8008,16017,2.437541961669922,0.07005957569801338
4104,8209,8208,16417,2.5040807723999023,0.06766082262576223
4204,8409,8408,16817,2.5689220428466797,0.0653627511027669
4304,8609,8608,17217,2.628204107284546,0.06318097775381688
4404,8809,8808,17617,2.686371088027954,0.06110300953777403
4505,9011,9010,18021,2.7455148696899414,0.0590937428271714
4605,9211,9210,18421,2.809199094772339,0.05717733161162599
4705,9411,9410,18821,2.868955135345459,0.05535773017085458
4805,9611,9610,19221,2.930063009262085,0.05361798797459647
4905,9811,9810,19621,2.9879109859466553,0.05194900886724691
5005,10011,10010,20021,3.047333002090454,0.05035243765185992
5105,10211,10210,20421,3.1072051525115967,0.04882063373100812
5205,10411,10410,20821,3.167013168334961,0.047359071023488915
5305,10611,10610,21221,3.2246079444885254,0.045955467781552156
5405,10811,10810,21621,3.281989812850952,0.04461009631068081
5506,11013,11012,22025,3.3391427993774414,0.043314099629270165
5606,11213,11212,22425,3.396791934967041,0.04207838125332836
5706,11413,11412,22825,3.453721046447754,0.040893441689385045
5806,11613,11612,23225,3.5102310180664062,0.039758063729968526
5906,11813,11812,23625,3.5669801235198975,0.03866727459590865
6006,12013,12012,24025,3.623012065887451,0.03762274291255587
6106,12213,12212,24425,3.6800589561462402,0.036611040471708
6206,12413,12412,24825,3.73641300201416,0.03562856314436133
6306,12613,12612,25225,3.7920429706573486,0.03469692269248736
6406,12813,12812,25625,3.847104072570801,0.033799683286082904
6507,13015,13014,26029,3.916735887527466,0.032929696359171264
6607,13215,13214,26429,3.986114978790283,0.03210090886963369
6707,13415,13414,26829,4.0440239906311035,0.03129562467976816
6807,13615,13614,27229,4.101706027984619,0.030518070810675323
6907,13815,13814,27629,4.159929990768433,0.02976476100537671
7007,14015,14014,28029,4.215943813323975,0.029042946413349643
7107,14215,14214,28429,4.273210763931274,0.028345043787213003
7207,14415,14414,28829,4.332073926925659,0.0276787893149401
7307,14615,14614,29229,4.389107942581177,0.027025990891256242
7407,14815,14814,29629,4.444912910461426,0.02639680752696954
7508,15017,15016,30033,4.501189947128296,0.025790202933365928
7608,15217,15216,30433,4.556909084320068,0.025208342940185372
7708,15417,15416,30833,4.618888854980469,0.024644675806295535
7808,15617,15616,31233,4.677147150039673,0.024097814611134232
7908,15817,15816,31633,4.733443021774292,0.023566249852129673
8008,16017,16016,32033,4.789669036865234,0.02305376193088568
8108,16217,16216,32433,4.846141815185547,0.022559992497924237
8208,16417,16416,32833,4.908447027206421,0.02207759737706084
8308,16617,16616,33233,4.984722852706909,0.02161238570044299
8408,16817,16816,33633,5.062398910522461,0.021164310044291958
8509,17019,17018,34037,5.142366886138916,0.020719969130055856
8609,17219,17218,34437,5.212211847305298,0.020289142488751587
8709,17419,17418,34837,5.279783010482788,0.019873623405900084
8809,17619,17618,35237,5.348188877105713,0.019475522501521056
8909,17819,17818,35637,5.415401935577393,0.019087241660711515
9009,18019,18018,36037,5.503641128540039,0.018709462863585432
9109,18219,18218,36437,5.573260068893433,0.01834242177141693
9209,18419,18418,36837,5.632857084274292,0.017986694060080653
9309,18619,18618,37237,5.694960832595825,0.017639570923587207
9409,18819,18818,37637,5.756062030792236,0.017304090160352722
9510,19021,19020,38041,5.8246400356292725,0.01697037256681031
9610,19221,19220,38441,5.888021945953369,0.016650869536836047
9710,19421,19420,38841,5.954566955566406,0.016338428904114157
9810,19621,19620,39241,6.032789945602417,0.016032065561002222
9910,19821,19820,39641,6.127771854400635,0.015736215804187048
10010,20021,20020,40041,6.189207077026367,0.015443306257313391
10110,20221,20220,40441,6.24676513671875,0.015159276298873113
10210,20421,20420,40841,6.303054094314575,0.014880353086775216
10310,20621,20620,41241,6.359117031097412,0.014610834315845698
10410,20821,20820,41641,6.417567014694214,0.01434706491684801
10511,21023,21022,42045,6.476357936859131,0.014085199618959468
10611,21223,21222,42445,6.544482946395874,0.013835652154810913
10711,21423,21422,42845,6.605547904968262,0.013589342281853576
10811,21623,21622,43245,6.6685590744018555,0.013354002367906608
10911,21823,21822,43645,6.734792947769165,0.013122741296041598
11011,22023,22022,44045,6.803910970687866,0.012897126910157219
11111,22223,22222,44445,6.863466024398804,0.01267746338992712
11211,22423,22422,44845,6.920316934585571,0.012460920442064519
11311,22623,22622,45245,6.983184099197388,0.012248712357741501
11411,22823,22822,45645,7.046810150146484,0.0120408501101333
11512,23025,23024,46049,7.1042139530181885,0.01183763020113523
11612,23225,23224,46449,7.1639931201934814,0.01164006612654538
11712,23425,23424,46849,7.2256200313568115,0.0114466669419765
11812,23625,23624,47249,7.294600963592529,0.011256805141840357
11912,23825,23824,47649,7.368479013442993,0.011068964054448644
12012,24025,24024,48049,7.446143865585327,0.010886822962676155
12112,24225,24224,48449,7.520823955535889,0.010708973654508593
12212,24425,24424,48849,7.58391809463501,0.010535118108427515
12312,24625,24624,49249,7.648624897003174,0.01036397438479419
12412,24825,24824,49649,7.719846963882446,0.010195631666659726
12513,25027,25026,50053,7.783802032470703,0.010030569936909036
12613,25227,25226,50453,7.8466479778289795,0.009871252990260712
12713,25427,25426,50853,7.9123311042785645,0.009711746042621023
12813,25627,25626,51253,7.975193977355957,0.009556048647357459
12913,25827,25826,51653,8.044059991836548,0.009403642583312196
13013,26027,26026,52053,8.1022047996521,0.00925358377989855
13113,26227,26226,52453,8.180286884307861,0.009106999391905887
13213,26427,26426,52853,8.257080078125,0.008961927882435695
13313,26627,26626,53253,8.322768926620483,0.008819693970361838
13413,26827,26826,53653,8.385426998138428,0.008681359896065092
13514,27029,27028,54057,8.449901103973389,0.008543950765493025
13614,27229,27228,54457,8.524857997894287,0.008409233988912568
13714,27429,27428,54857,8.595554113388062,0.008279902665875727
13814,27629,27628,55257,8.669323921203613,0.008152617209461761
13914,27829,27828,55657,8.750864028930664,0.008026512120131583
14014,28029,28028,56057,8.840687990188599,0.007903728658445882
14114,28229,28228,56457,8.916973114013672,0.007783622588777366
14214,28429,28428,56857,8.985424041748047,0.007665939539988106
14314,28629,28628,57257,9.051099061965942,0.0075494264729885005
14414,28829,28828,57657,9.114238977432251,0.00743439393415637
14515,29031,29030,58061,9.174548864364624,0.007320070375111831
14615,29231,29230,58461,9.250110864639282,0.007210816307447554
14715,29431,29430,58861,9.338696956634521,0.0071037168090751475
14815,29631,29630,59261,9.445648193359375,0.0069978140175911705
14915,29831,29830,59661,9.544960021972656,0.006893302443676335
15015,30031,30030,60061,9.64279294013977,0.006790653764443709
15115,30231,30230,60461,9.73103404045105,0.006690559735818359
15215,30431,30430,60861,9.828573942184448,0.0065917079510694355
15315,30631,30630,61261,9.921413898468018,0.006494426826239039
15415,30831,30830,61661,9.998661041259766,0.0063998511647646306
15516,31033,31032,62065,10.06583285331726,0.006305414231237228
15616,31233,31232,62465,10.129904985427856,0.006212675033630323
15716,31433,31432,62865,10.193603038787842,0.006121818345902143
15816,31633,31632,63265,10.257379055023193,0.006032477348766477
15916,31833,31832,63665,10.338679075241089,0.005944909152241164
16016,32033,32032,64065,10.41720199584961,0.005857863671652319
16116,32233,32232,64465,10.484701871871948,0.005771793092418668
16216,32433,32432,64865,10.547355890274048,0.005686836282398767
16316,32633,32632,65265,10.610591888427734,0.005603883184672335
16416,32833,32832,65665,10.674334049224854,0.005523094010000106
16517,33035,33034,66069,10.736692905426025,0.005441233723712932
16617,33235,33234,66469,10.80310606956482,0.005360929256303944
16717,33435,33434,66869,10.866544008255005,0.005282785119962842
16817,33635,33634,67269,10.933731079101562,0.005206396925919889
16917,33835,33834,67669,10.993803024291992,0.0051302409911087345
17017,34035,34034,68069,11.054204940795898,0.005055965898887682
17117,34235,34234,68469,11.114509105682373,0.004983635292561712
17217,34435,34434,68869,11.174429893493652,0.004911618144718041
17317,34635,34634,69269,11.23395299911499,0.0048421856219658796
17417,34835,34834,69669,11.292272090911865,0.004773995674033953
17518,35037,35036,70073,11.352333068847656,0.004705333144626182
17618,35237,35236,70473,11.41235613822937,0.004638693046376321
17718,35437,35436,70873,11.4688880443573,0.004573244929095878
17818,35637,35636,71273,11.525978088378906,0.004508469981765339
17918,35837,35836,71673,11.583799123764038,0.004445483827106951
18018,36037,36036,72073,11.640419960021973,0.00438394267520254
18118,36237,36236,72473,11.697082757949829,0.004322926095325923
18218,36437,36436,72873,11.753015041351318,0.0042627725542947305
18318,36637,36636,73273,11.809151887893677,0.004203371011086959
18418,36837,36836,73673,11.865689992904663,0.004144912239114603
18519,37039,37038,74077,11.923050880432129,0.0040871017415159425
18619,37239,37238,74477,11.980955123901367,0.004030763356925354
18719,37439,37438,74877,12.03951096534729,0.003975243272120712
18819,37639,37638,75277,12.096816778182983,0.00391979960089009
18919,37839,37838,75677,12.153985977172852,0.003865249257327049
19019,38039,38038,76077,12.209196090698242,0.003812422175678236
19119,38239,38238,76477,12.266581058502197,0.003759977232970467
19219,38439,38438,76877,12.330405950546265,0.0037071795738251047
19319,38639,38638,77277,12.39159083366394,0.003655243445506932
19419,38839,38838,77677,12.457733154296875,0.0036040650125742524
19520,39041,39040,78081,12.529053926467896,0.0035530551680510373
19620,39241,39240,78481,12.590693950653076,0.003503527828498237
19720,39441,39440,78881,12.646501779556274,0.003454955033293234
19820,39641,39640,79281,12.706362962722778,0.0034069870116554025
19920,39841,39840,79681,12.7659010887146,0.0033599647905396923
20020,40041,40040,80081,12.822373867034912,0.0033136982134211444
20120,40241,40240,80481,12.876863956451416,0.0032678620157086794
20220,40441,40440,80881,12.930071115493774,0.003223120084991087
20320,40641,40640,81281,12.989405870437622,0.0031790344510985186
20420,40841,40840,81681,13.04877495765686,0.0031354275182303225
20521,41043,41042,82085,13.11289095878601,0.0030922796795635156
20621,41243,41242,82485,13.177001953125,0.003050653756733758
20721,41443,41442,82885,13.24402403831482,0.0030097410406953982
20821,41643,41642,83285,13.30899715423584,0.0029690653918482655
20921,41843,41842,83685,13.372453212738037,0.002928941552300115
21021,42043,42042,84085,13.436490058898926,0.0028892309435148283
21121,42243,42242,84485,13.4984130859375,0.0028502035305651967
21221,42443,42442,84885,13.55840802192688,0.002812368444327073
21321,42643,42642,85285,13.617565870285034,0.0027753887202941023
21421,42843,42842,85685,13.677345037460327,0.0027383639017034803
21522,43045,43044,86089,13.737701892852783,0.002701066335187053
21622,43245,43244,86489,13.796871900558472,0.00266506837031242
21722,43445,43444,86889,13.852432012557983,0.002630204759457289
21822,43645,43644,87289,13.908066987991333,0.002595477065467895
21922,43845,43844,87689,13.96227502822876,0.0025606755089754452
22022,44045,44044,88089,14.017725944519043,0.0025261160067499896
22122,44245,44244,88489,14.072899103164673,0.0024921225384463733
22222,44445,44444,88889,14.126906871795654,0.0024588130892679687
22322,44645,44644,89289,14.182556867599487,0.002425832369400067
22422,44845,44844,89689,14.239289999008179,0.002393106439487853
22523,45047,45046,90093,14.294556856155396,0.0023605301690849414
22623,45247,45246,90493,14.35108995437622,0.0023288843176608766
22723,45447,45446,90893,14.413082122802734,0.0022972369973633788
22823,45647,45646,91293,14.480237007141113,0.002265961526679049
22923,45847,45846,91693,14.545683860778809,0.002235816087229212
23023,46047,46046,92093,14.616159915924072,0.0022060734692023747
23123,46247,46246,92493,14.684607982635498,0.0021762834304517465
23223,46447,46446,92893,14.740747928619385,0.0021468772759382663
23323,46647,46646,93293,14.800012111663818,0.0021182539411345163
23423,46847,46846,93693,14.857270002365112,0.0020901150321934697
23524,47049,47048,94097,14.915755987167358,0.00206207789073199
23624,47249,47248,94497,14.971490144729614,0.0020344391567394537
23724,47449,47448,94897,15.026384115219116,0.002006940904425779
23824,47649,47648,95297,15.08187484741211,0.0019803639994873975
23924,47849,47848,95697,15.137509822845459,0.0019546652026762577
24024,48049,48048,96097,15.194405794143677,0.0019290901174034071
24124,48249,48248,96497,15.251051902770996,0.001903528857177315
24224,48449,48448,96897,15.30784296989441,0.0018784219515933262
24324,48649,48648,97297,15.369674921035767,0.0018538691308578855
24424,48849,48848,97697,15.431391954421997,0.0018297957217538296
24525,49051,49050,98101,15.492722988128662,0.0018057761889676575
24625,49251,49250,98501,15.552910089492798,0.0017822167607118604
24725,49451,49450,98901,15.609447956085205,0.001758972691668677
24825,49651,49650,99301,15.663542032241821,0.0017359592620280221
24925,49851,49850,99701,15.719966888427734,0.0017132828288529494
25025,50051,50050,100101,15.774657964706421,0.0016909282912083354
25125,50251,50250,100501,15.829487085342407,0.0016688915753794746
25225,50451,50450,100901,15.883656024932861,0.001647304466976178
25325,50651,50650,101301,15.945784091949463,0.00162574981053356
25425,50851,50850,101701,16.009171962738037,0.0016041325357932313
25526,51053,51052,102105,16.06874108314514,0.0015829334740507929
25626,51253,51252,102505,16.12596607208252,0.001562492810147561
25726,51453,51452,102905,16.184367179870605,0.0015420038491380406
25826,51653,51652,103305,16.245408058166504,0.0015215474186297943
25926,51853,51852,103705,16.307536125183105,0.0015013343540489692
26026,52053,52052,104105,16.368361949920654,0.0014815744346237615
26126,52253,52252,104505,16.428653955459595,0.0014622147309564825
26226,52453,52452,104905,16.495178937911987,0.0014429248404153458
26326,52653,52652,105305,16.563716173171997,0.0014237214420007012
26426,52853,52852,105705,16.62933921813965,0.0014049123676458826
26527,53055,53054,106109,16.694168090820312,0.0013864561895997449
26627,53255,53254,106509,16.770139932632446,0.0013684126049319189
26727,53455,53454,106909,16.842320919036865,0.0013503584389416101
26827,53655,53654,107309,16.900689840316772,0.0013325648333129781
26927,53855,53854,107709,16.959105014801025,0.001315245020235094
27027,54055,54054,108109,17.016618013381958,0.0012981464405400504
27127,54255,54254,108509,17.07396411895752,0.0012812362433527523
27227,54455,54454,108909,17.131526947021484,0.0012646847846415278
27327,54655,54654,109309,17.191128969192505,0.001248413516773543
27427,54855,54854,109709,17.24991798400879,0.001232365332832007
27528,55057,55056,110113,17.31125807762146,0.0012163422628432249
27628,55257,55256,110513,17.37301206588745,0.0012007487414121831
27728,55457,55456,110913,17.434780836105347,0.0011856211157098915
27828,55657,55656,111313,17.49788999557495,0.0011707441759108525
27928,55857,55856,111713,17.566428899765015,0.001155830152379695
28028,56057,56056,112113,17.62775707244873,0.001140997998677747
28128,56257,56256,112513,17.689734935760498,0.0011264985706258485
28228,56457,56456,112913,17.75053381919861,0.0011124366296351694
28328,56657,56656,113313,17.836575031280518,0.0010984739176887336
28428,56857,56856,113713,17.899847984313965,0.0010843713433919646
28529,57059,57058,114117,17.959800004959106,0.001070209207251639
28629,57259,57258,114517,18.0197970867157,0.0010564074790777433
28729,57459,57458,114917,18.078557014465332,0.0010427852142414643
28829,57659,57658,115317,18.185598850250244,0.001029395984928758
28929,57859,57858,115717,18.259788036346436,0.0010161170668409893
29029,58059,58058,116117,18.317878007888794,0.0010028852735070662
29129,58259,58258,116517,18.375805854797363,0.0009898803582890777
29229,58459,58458,116917,18.43610119819641,0.0009770654043842024
29329,58659,58658,117317,18.49589991569519,0.0009644180681854901
29429,58859,58858,117717,18.553328037261963,0.0009519341434160016
29530,59061,59060,118121,18.61894392967224,0.0009394078877329043
29630,59261,59260,118521,18.679674863815308,0.0009271719139192254
29730,59461,59460,118921,18.757979154586792,0.0009151672911712378
29830,59661,59660,119321,18.82108497619629,0.0009033591387170011
29930,59861,59860,119721,18.90194606781006,0.0008917409664697023
30030,60061,60060,120121,18.973127841949463,0.0008802988455081966
30130,60261,60260,120521,19.031333923339844,0.0008689573566629654
30230,60461,60460,120921,19.089675903320312,0.0008577630739799271
30330,60661,60660,121321,19.147475957870483,0.0008468217024087507
30430,60861,60860,121721,19.204583883285522,0.000836213587043217
30531,61063,61062,122125,19.263252019882202,0.0008257063914645861
30631,61263,61262,122525,19.32655906677246,0.0008152790889900327
30731,61463,61462,122925,19.38561201095581,0.0008048872648082177
30831,61663,61662,123325,19.444437980651855,0.0007947666008145213
30931,61863,61862,123725,19.50159215927124,0.0007849734815241334
31031,62063,62062,124125,19.55939507484436,0.0007752914069039619
31131,62263,62262,124525,19.624118089675903,0.0007655604481768055
31231,62463,62462,124925,19.689514875411987,0.0007558522460640074
31331,62663,62662,125325,19.755456924438477,0.0007462777872553389
31431,62863,62862,125725,19.82245182991028,0.0007368841449350017
31532,63065,63064,126129,19.882932901382446,0.0007275646600866449
31632,63265,63264,126529,19.94701600074768,0.000718412068472922
31732,63465,63464,126929,20.005971908569336,0.0007092889757316277
31832,63665,63664,127329,20.06532597541809,0.0007002188384096632
31932,63865,63864,127729,20.123368978500366,0.0006912156096667298
32032,64065,64064,128129,20.182201147079468,0.0006823576365028392
32132,64265,64264,128529,20.25461983680725,0.000673656100169962
32232,64465,64464,128929,20.31817603111267,0.000665055300941808
32332,64665,64664,129329,20.377231121063232,0.0006565317276488504
32432,64865,64864,129729,20.43596601486206,0.0006480549560862117
32533,65067,65066,130133,20.496307849884033,0.0006396228151107925
32633,65267,65266,130533,20.55435585975647,0.0006314627450635855
32733,65467,65466,130933,20.613343954086304,0.0006233959751778609
32833,65667,65666,131333,20.67063593864441,0.0006153678410492319
32933,65867,65866,131733,20.73310112953186,0.0006073919539786686
33033,66067,66066,132133,20.793298959732056,0.0005995633916072135
33133,66267,66266,132533,20.85431694984436,0.000591997289100956
33233,66467,66466,132933,20.912963151931763,0.000584575855427674
33333,66667,66666,133333,20.98826789855957,0.0005771084756582733
33433,66867,66866,133733,21.058488130569458,0.0005696863929570546
33534,67069,67068,134137,21.124410152435303,0.0005624184792915367
33634,67269,67268,134537,21.182942867279053,0.0005554280076784693
33734,67469,67468,134937,21.242225885391235,0.0005485061715251781
33834,67669,67668,135337,21.30128502845764,0.0005416028141252545
33934,67869,67868,135737,21.35988187789917,0.0005347875483740765
34034,68069,68068,136137,21.41763997077942,0.0005280879963183113
34134,68269,68268,136537,21.480144023895264,0.0005214761486977644
34234,68469,68468,136937,21.540777921676636,0.0005149780357951228
34334,68669,68668,137337,21.599519968032837,0.0005085924872539106
34434,68869,68868,137737,21.673937797546387,0.000502283302734517
34535,69071,69070,138141,21.750813961029053,0.0004959370176206457
34635,69271,69270,138541,21.829829216003418,0.0004896480072764031
34735,69471,69470,138941,21.897983074188232,0.0004834708223313215
34835,69671,69670,139341,21.95793104171753,0.0004774844483334934
34935,69871,69870,139741,22.02361297607422,0.00047155902265240136
35035,70071,70070,140141,22.084518909454346,0.0004655961549946899
35135,70271,70270,140541,22.15023112297058,0.0004596667679794084
35235,70471,70470,140941,22.215925931930542,0.0004538614263627269
35335,70671,70670,141341,22.279546976089478,0.0004481761276762892
35435,70871,70870,141741,22.351382970809937,0.0004425184464727837
35536,71073,71072,142145,22.42578101158142,0.00043680176754632056
35636,71273,71272,142545,22.491870880126953,0.0004312203765765617
35736,71473,71472,142945,22.55123996734619,0.00042575428452023656
35836,71673,71672,143345,22.611583948135376,0.00042038476598061774
35936,71873,71872,143745,22.672756910324097,0.00041505590545173237
36036,72073,72072,144145,22.73304009437561,0.00040973613464931807
36136,72273,72272,144545,22.792383909225464,0.0004045053016307405
36236,72473,72472,144945,22.851099967956543,0.00039938870744720605
36336,72673,72672,145345,22.913501977920532,0.0003943161478983263
36436,72873,72872,145745,22.974884033203125,0.00038930292427483316
36537,73075,73074,146149,23.033108949661255,0.0003843384904795294
36637,73275,73274,146549,23.093466997146606,0.00037949383715535454
36737,73475,73474,146949,23.167191982269287,0.00037471805399694864
36837,73675,73674,147349,23.240005016326904,0.00037003549227508593
36937,73875,73874,147749,23.298479080200195,0.00036546155835562636
37037,74075,74074,148149,23.357487201690674,0.00036096921619585884
37137,74275,74274,148549,23.414644956588745,0.0003565014206840077
37237,74475,74474,148949,23.476386070251465,0.000352062057915611
37337,74675,74674,149349,23.53265690803528,0.0003477120342057831
37437,74875,74874,149749,23.589515924453735,0.00034348744847546874
37538,75077,75076,150153,23.653085947036743,0.0003393050059050072
37638,75277,75276,150553,23.714929819107056,0.0003351577637960295
37738,75477,75476,150953,23.7754909992218,0.0003309970271766664
37838,75677,75676,151353,23.8392550945282,0.000326900350872223
37938,75877,75876,151753,23.900689840316772,0.0003228846532448041
38038,76077,76076,152153,23.962080001831055,0.0003189160308931518
38138,76277,76276,152553,24.02362895011902,0.0003149758244353602
38238,76477,76476,152953,24.084390878677368,0.00031105373060227745
38338,76677,76676,153353,24.14223313331604,0.00030716800811117354
38438,76877,76876,153753,24.1994891166687,0.000303341062980693
38539,77079,77078,154157,24.262148141860962,0.00029952467808556975
38639,77279,77278,154557,24.32418394088745,0.000295770123073343
38739,77479,77478,154957,24.385011911392212,0.0002920403117529768
38839,77679,77678,155357,24.44435715675354,0.0002883565324695118
38939,77879,77878,155757,24.50125789642334,0.0002847147761708351
39039,78079,78078,156157,24.55760884284973,0.00028111084788081915
39139,78279,78278,156557,24.616069078445435,0.0002775582991780617
39239,78479,78478,156957,24.67562484741211,0.00027404218510427046
39339,78679,78678,157357,24.73312211036682,0.0002705538266859334
39439,78879,78878,157757,24.79091787338257,0.00026712591648868713
39540,79081,79080,158161,24.848469972610474,0.0002637482063303302
39640,79281,79280,158561,24.90454387664795,0.0002604784557069851
39740,79481,79480,158961,24.9617760181427,0.00025725518783974654
39840,79681,79680,159361,25.0186870098114,0.0002540514538603606
39940,79881,79880,159761,25.075504779815674,0.0002508852192821218
40040,80081,80080,160161,25.132127046585083,0.00024779788249145465
40140,80281,80280,160561,25.18770408630371,0.0002447909742628181
40240,80481,80480,160961,25.248164176940918,0.00024182806361832822
40340,80681,80680,161361,25.32140588760376,0.00023887223116086424
40440,80881,80880,161761,25.393603086471558,0.00023592433769801732
40541,81083,81082,162165,25.45724320411682,0.00023299001283526215
40641,81283,81282,162565,25.516025066375732,0.00023015205982570444
40741,81483,81482,162965,25.575045824050903,0.00022737815731754086
40841,81683,81682,163365,25.635541915893555,0.00022462806821962373
40941,81883,81882,163765,25.698019981384277,0.00022186189036798443
41041,82083,82082,164165,25.757588863372803,0.00021909822002065988
41141,82283,82282,164565,25.819732904434204,0.0002163819483350431
41241,82483,82482,164965,25.884191036224365,0.00021371975005363353
41341,82683,82682,165365,25.949743032455444,0.00021109100878277169
41441,82883,82882,165765,26.009356021881104,0.00020848231493860272
41542,83085,83084,166169,26.069872856140137,0.00020586057062015395
41642,83285,83284,166569,26.164395093917847,0.000203276428634973
41742,83485,83484,166969,26.243167877197266,0.00020071608930321316
41842,83685,83684,167369,26.301923990249634,0.00019819393778978066
41942,83885,83884,167769,26.360217094421387,0.00019570568988827228
42042,84085,84084,168169,26.42016887664795,0.00019323998709289668
42142,84285,84284,168569,26.47700309753418,0.0001907964104118274
42242,84485,84484,168969,26.537559032440186,0.00018838356809352383
42342,84685,84684,169369,26.597509145736694,0.00018602079675367187
42442,84885,84884,169769,26.655256032943726,0.0001837037199078083
42543,85087,85086,170173,26.713130950927734,0.0001813725643109436
42643,85287,85286,170573,26.77079486846924,0.0001790752341245966
42743,85487,85486,170973,26.83228898048401,0.0001768292416121034
42843,85687,85686,171373,26.893616914749146,0.00017464499844021015
42943,85887,85886,171773,26.95403790473938,0.0001724984090081392
43043,86087,86086,172173,27.021099090576172,0.00017036015715322754
43143,86287,86286,172573,27.081203937530518,0.0001682264437269874
43243,86487,86486,172973,27.143790006637573,0.00016612877051334118
43343,86687,86686,173373,27.20639419555664,0.0001640901907504747
43443,86887,86886,173773,27.2626690864563,0.00016209982549336856
43544,87089,87088,174177,27.327502965927124,0.00016010996865951747
43644,87289,87288,174577,27.39045286178589,0.00015814021033291694
43744,87489,87488,174977,27.46026110649109,0.00015617824455206657
43844,87689,87688,175377,27.526331901550293,0.00015424229798519386
43944,87889,87888,175777,27.583168983459473,0.00015234525595818335
44044,88089,88088,176177,27.639450073242188,0.00015049565825211848
44144,88289,88288,176577,27.697808980941772,0.00014867539777357647
44244,88489,88488,176977,27.754178047180176,0.00014685057794439226
44344,88689,88688,177377,27.81309199333191,0.0001450222279675677
44444,88889,88888,177777,27.882429838180542,0.0001432193365019815
44545,89091,89090,178181,27.957441091537476,0.00014144207418414795
44645,89291,89290,178581,28.016216039657593,0.00013971263705615558
44745,89491,89490,178981,28.07327103614807,0.00013798442866319154
44845,89691,89690,179381,28.13095712661743,0.00013625729341167262
44945,89891,89890,179781,28.187152862548828,0.0001345574945113164
45045,90091,90090,180181,28.244781970977783,0.00013289356624013315
45145,90291,90290,180581,28.30297017097473,0.00013124863589701358
45245,90491,90490,180981,28.362141847610474,0.00012960722090503565
45345,90691,90690,181381,28.4181911945343,0.0001279765553778598
45445,90891,90890,181781,28.475268125534058,0.00012637317921053898
45546,91093,91092,182185,28.53309202194214,0.00012478124938241402
45646,91293,91292,182585,28.58947515487671,0.0001232226103641434
45746,91493,91492,182985,28.645385026931763,0.0001216789573696633
45846,91693,91692,183385,28.701069116592407,0.00012015315637023151
45946,91893,91892,183785,28.757527112960815,0.00011865199055657371
46046,92093,92092,184185,28.81669592857361,0.00011718150186085775
46146,92293,92292,184585,28.87310791015625,0.00011573985523195458
46246,92493,92492,184985,28.930819988250732,0.00011431914546291289
46346,92693,92692,185385,28.991714000701904,0.00011291029269743087
46446,92893,92892,185785,29.045536041259766,0.00011151509618881839
46547,93095,93094,186189,29.10007095336914,0.00011013293195193942
46647,93295,93294,186589,29.155529022216797,0.00010879776392846443
46747,93495,93494,186989,29.211116075515747,0.00010748995831141965
46847,93695,93694,187389,29.267162084579468,0.00010619429652382873
46947,93895,93894,187789,29.3270001411438,0.00010490064689802641
47047,94095,94094,188189,29.383702993392944,0.0001036202161873568
47147,94295,94294,188589,29.441559076309204,0.00010236838243776943
47247,94495,94494,188989,29.499955892562866,0.00010114275966565546
47347,94695,94694,189389,29.573400020599365,9.993016057126198e-05
47447,94895,94894,189789,29.641712188720703,9.872110501904615e-05
47548,95097,95096,190193,29.70058012008667,9.75059895762616e-05
47648,95297,95296,190593,29.755668878555298,9.631948607871723e-05
47748,95497,95496,190993,29.813584089279175,9.515161555636806e-05
47848,95697,95696,191393,29.87356686592102,9.399530073302256e-05
47948,95897,95896,191793,29.931760787963867,9.28471926355752e-05
48048,96097,96096,192193,29.985819816589355,9.170756160305401e-05
48148,96297,96296,192593,30.039971113204956,9.057703727985186e-05
48248,96497,96496,192993,30.096269130706787,8.945683711013203e-05
48348,96697,96696,193393,30.150660037994385,8.834664826830426e-05
48448,96897,96896,193793,30.20555281639099,8.724529971294314e-05
48549,97099,97098,194197,30.26754403114319,8.614377724831555e-05
48649,97299,97298,194597,30.324755907058716,8.506922825433246e-05
48749,97499,97498,194997,30.381598949432373,8.401407780519597e-05
48849,97699,97698,195397,30.438168048858643,8.297560476609393e-05
48949,97899,97898,195797,30.494565963745117,8.194880047050278e-05
49049,98099,98098,196197,30.55080795288086,8.093404397391337e-05
49149,98299,98298,196597,30.60677695274353,7.993719206597883e-05
49249,98499,98498,196997,30.665284156799316,7.896040056880056e-05
49349,98699,98698,197397,30.72007393836975,7.799917656674808e-05
49449,98899,98898,197797,30.777384996414185,7.704973967353492e-05
49550,99101,99100,198201,30.831660985946655,7.610103818764431e-05
49650,99301,99300,198601,30.88604497909546,7.517184384615252e-05
49750,99501,99500,199001,30.941736936569214,7.425796140602551e-05
49850,99701,99700,199401,30.997534036636353,7.336513538575964e-05
49950,99901,99900,199801,31.051828861236572,7.249215031877041e-05
50050,100101,100100,200201,31.10466194152832,7.162912904509873e-05
50150,100301,100300,200601,31.16011118888855,7.076374828155986e-05
50250,100501,100500,201001,31.21823215484619,6.989779254409602e-05
50350,100701,100700,201401,31.279018878936768,6.904789460229943e-05
50450,100901,100900,201801,31.341397047042847,6.822109192835934e-05
50551,101103,101102,202205,31.404046058654785,6.739825052923212e-05
50651,101303,101302,202605,31.460876941680908,6.658374608708562e-05
50751,101503,101502,203005,31.518566846847534,6.5769342162764e-05
50851,101703,101702,203405,31.583723068237305,6.496287089872317e-05
50951,101903,101902,203805,31.648922204971313,6.416833091828788e-05
51051,102103,102102,204205,31.726086854934692,6.338345579829246e-05
51151,102303,102302,204605,31.7989718914032,6.260605350774292e-05
51251,102503,102502,205005,31.861091136932373,6.183457044517785e-05
51351,102703,102702,205405,31.92189311981201,6.106720440061781e-05
51451,102903,102902,205805,31.977428913116455,6.03044512704491e-05
51552,103105,103104,206209,32.0339560508728,5.9543515796248956e-05
51652,103305,103304,206609,32.0915892124176,5.88052090248075e-05
51752,103505,103504,207009,32.14947986602783,5.807945163953757e-05
51852,103705,103704,207409,32.20608305931091,5.735804563044207e-05
51952,103905,103904,207809,32.26321887969971,5.6642141078523705e-05
52052,104105,104104,208209,32.318832874298096,5.594056268989919e-05
52152,104305,104304,208609,32.37707281112671,5.5253799854957306e-05
52252,104505,104504,209009,32.4332070350647,5.4573053162603945e-05
52352,104705,104704,209409,32.489898920059204,5.38941665184917e-05
52452,104905,104904,209809,32.54667806625366,5.322499244773153e-05
52553,105107,105106,210213,32.60425806045532,5.256861249834601e-05
52653,105307,105306,210613,32.65957713127136,5.1935010621913895e-05
52753,105507,105506,211013,32.71627497673035,5.130504389247485e-05
52853,105707,105706,211413,32.77573299407959,5.067170372996229e-05
52953,105907,105906,211813,32.83437395095825,5.004264910824949e-05
53053,106107,106106,212213,32.889896869659424,4.943097693078666e-05
53153,106307,106306,212613,32.9466450214386,4.8838420422606406e-05
53253,106507,106506,213013,33.004218101501465,4.825600154277218e-05
53353,106707,106706,213413,33.063244104385376,4.7675519375717334e-05
53453,106907,106906,213813,33.120627880096436,4.709396250384261e-05
53554,107109,107108,214217,33.176679849624634,4.65088751547906e-05
53654,107309,107308,214617,33.23550009727478,4.593947365555237e-05
53754,107509,107508,215017,33.29430079460144,4.538427313598944e-05
53854,107709,107708,215417,33.35377097129822,4.4839924568434876e-05
53954,107909,107908,215817,33.41346096992493,4.429786408307091e-05
54054,108109,108108,216217,33.47206711769104,4.3752986327879746e-05
54154,108309,108308,216617,33.52920389175415,4.3210486002077905e-05
54254,108509,108508,217017,33.58775496482849,4.267955958200301e-05
54354,108709,108708,217417,33.645511865615845,4.2161652558707596e-05
54454,108909,108908,217817,33.70328092575073,4.164867775421944e-05
54555,109111,109110,218221,33.76313495635986,4.112885835827202e-05
54655,109311,109310,218621,33.832813024520874,4.0617115059512164e-05
54755,109511,109510,219021,33.90419888496399,4.011556600117012e-05
54855,109711,109710,219421,33.96665382385254,3.962175682848879e-05
54955,109911,109910,219821,34.028241872787476,3.912986292665664e-05
55055,110111,110110,220221,34.08597183227539,3.8641230415958725e-05
55155,110311,110310,220621,34.14530611038208,3.8161329532574645e-05
55255,110511,110510,221021,34.20331907272339,3.7692351736237234e-05
55355,110711,110710,221421,34.260704040527344,3.7231349641486495e-05
55455,110911,110910,221821,34.32121181488037,3.6774056160339804e-05
55556,111113,111112,222225,34.383376121520996,3.631561794124037e-05
55656,111313,111312,222625,34.44138288497925,3.586853618338635e-05
55756,111513,111512,223025,34.5012788772583,3.543063896381011e-05
55856,111713,111712,223425,34.55884385108948,3.5001678275984944e-05
55956,111913,111912,223825,34.622671127319336,3.458036953387617e-05
56056,112113,112112,224225,34.68872022628784,3.4163923529434016e-05
56156,112313,112312,224625,34.75506615638733,3.3749151866548185e-05
56256,112513,112512,225025,34.820693016052246,3.333767616873116e-05
56356,112713,112712,225425,34.88981819152832,3.2935047409620035e-05
56456,112913,112912,225825,34.94925498962402,3.254313896618875e-05
56557,113115,113114,226229,35.00871801376343,3.2154292626006215e-05
56657,113315,113314,226629,35.067848920822144,3.177133310919726e-05
56757,113515,113514,227029,35.128411054611206,3.138908123423236e-05
56857,113715,113714,227429,35.19170618057251,3.101070281404708e-05
56957,113915,113914,227829,35.25103688240051,3.063970639219593e-05
57057,114115,114114,228229,35.31182098388672,3.0275373577068552e-05
57157,114315,114314,228629,35.38250803947449,2.991388537029835e-05
57257,114515,114514,229029,35.44860601425171,2.955302671387017e-05
57357,114715,114714,229429,35.5103440284729,2.9194265670138282e-05
57457,114915,114914,229829,35.56964612007141,2.883980869161243e-05
57558,115117,115116,230233,35.63014602661133,2.8486187328171287e-05
57658,115317,115316,230633,35.689621925354004,2.813926683908595e-05
57758,115517,115516,231033,35.748201847076416,2.779495508601753e-05
57858,115717,115716,231433,35.80846905708313,2.745369249468967e-05
57958,115917,115916,231833,35.873023986816406,2.7116351653188816e-05
58058,116117,116116,232233,35.94576096534729,2.678291896668392e-05
58158,116317,116316,232633,36.029350996017456,2.645333939183334e-05
58258,116517,116516,233033,36.09479904174805,2.612901913459722e-05
58358,116717,116716,233433,36.157835960388184,2.58107745199425e-05
58458,116917,116916,233833,36.21775197982788,2.5497007013748194e-05
58559,117119,117118,234237,36.27802491188049,2.5183129971058986e-05
58659,117319,117318,234637,36.336517095565796,2.4876044596642697e-05
58759,117519,117518,235037,36.4106879234314,2.457347765599679e-05
58859,117719,117718,235437,36.47808790206909,2.4274853671780186e-05
58959,117919,117918,235837,36.55821108818054,2.398003763226692e-05
59059,118119,118118,236237,36.62785291671753,2.369053102535686e-05
59159,118319,118318,236637,36.68765687942505,2.3407479214200692e-05
59259,118519,118518,237037,36.746947050094604,2.3129425461007423e-05
59359,118719,118718,237437,36.808470010757446,2.2853056793730952e-05
59459,118919,118918,237837,36.86618113517761,2.257753619579934e-05
59560,119121,119120,238241,36.923264026641846,2.230378247370312e-05
59660,119321,119320,238641,36.9802188873291,2.203996402099865e-05
59760,119521,119520,239041,37.04773497581482,2.1780738696627824e-05
59860,119721,119720,239441,37.12630081176758,2.1521899919741736e-05
59960,119921,119920,239841,37.1899049282074,2.1262925510155518e-05
60060,120121,120120,240241,37.24769902229309,2.100657189920181e-05
60160,120321,120320,240641,37.30599904060364,2.0754818000468815e-05
60260,120521,120520,241041,37.36414694786072,2.0506905544200124e-05
60360,120721,120720,241441,37.42199492454529,2.0260907500736043e-05
60460,120921,120920,241841,37.47836494445801,2.0015703200571263e-05
60561,121123,121122,242245,37.535022020339966,1.9769142415078984e-05
60661,121323,121322,242645,37.59245014190674,1.95271560438472e-05
60761,121523,121522,243045,37.64995980262756,1.9288216974140812e-05
60861,121723,121722,243445,37.70765686035156,1.9053059032174804e-05
60961,121923,121922,243845,37.76319098472595,1.8821337750601712e-05
61061,122123,122122,244245,37.82112002372742,1.859094706708093e-05
61161,122323,122322,244645,37.87753176689148,1.8360908210656085e-05
61261,122523,122522,245045,37.936439037323,1.813353036416554e-05
61361,122723,122722,245445,37.993499994277954,1.7911140701155434e-05
61461,122923,122922,245845,38.048762798309326,1.7692781977111633e-05
61562,123125,123124,246249,38.11831712722778,1.747383818606132e-05
61662,123325,123324,246649,38.194157123565674,1.7258481408639023e-05
61762,123525,123524,247049,38.2535080909729,1.704703743092231e-05
61862,123725,123724,247449,38.314889907836914,1.684069277206451e-05
61962,123925,123924,247849,38.37279796600342,1.6636866760599375e-05
62062,124125,124124,248249,38.42946791648865,1.6432933169106245e-05
62162,124325,124324,248649,38.486958026885986,1.6230787858329705e-05
62262,124525,124524,249049,38.5439190864563,1.6034483921626006e-05
62362,124725,124724,249449,38.60022592544556,1.5844054850809136e-05
62462,124925,124924,249849,38.65756797790527,1.5655322456021593e-05
62563,125127,125126,250253,38.7193877696991,1.5463800228088604e-05
62663,125327,125326,250653,38.77476716041565,1.527490295176856e-05
62763,125527,125526,251053,38.83280301094055,1.5089518052572588e-05
62863,125727,125726,251453,38.88856387138367,1.490874251698392e-05
62963,125927,125926,251853,38.944035053253174,1.4731912971443898e-05
63063,126127,126126,252253,39.00144100189209,1.4557331629105517e-05
63163,126327,126326,252653,39.05631685256958,1.4382971086898616e-05
63263,126527,126526,253053,39.11260008811951,1.4207992781036855e-05
63363,126727,126726,253453,39.16908001899719,1.4034193211534196e-05
63463,126927,126926,253853,39.22593092918396,1.3864633190085699e-05
63564,127129,127128,254257,39.28409504890442,1.3698226329689802e-05
63664,127329,127328,254657,39.34245991706848,1.3535004997494248e-05
63764,127529,127528,255057,39.401139974594116,1.337016634326633e-05
63864,127729,127728,255457,39.46233081817627,1.3204777443682471e-05
63964,127929,127928,255857,39.519351959228516,1.3042338690329268e-05
64064,128129,128128,256257,39.57603311538696,1.2883874802985627e-05
64164,128329,128328,256657,39.63296580314636,1.2727393250809385e-05
64264,128529,128528,257057,39.69308590888977,1.2571467360142818e-05
64364,128729,128728,257457,39.74922490119934,1.2416855998330114e-05
64464,128929,128928,257857,39.805294036865234,1.226474162350922e-05
64565,129131,129130,258261,39.86303091049194,1.2113403151036171e-05
64665,129331,129330,258661,39.91895604133606,1.196468836691997e-05
64765,129531,129530,259061,39.97746992111206,1.181703522784001e-05
64865,129731,129730,259461,40.03536510467529,1.1671817670465344e-05
64965,129931,129930,259861,40.09169793128967,1.1529884131356623e-05
65065,130131,130130,260261,40.145890951156616,1.1390525546333348e-05
65165,130331,130330,260661,40.200434923172,1.1252672981294376e-05
65265,130531,130530,261061,40.27051281929016,1.1115931871594509e-05
65365,130731,130730,261461,40.339536905288696,1.0980426805545521e-05
65465,130931,130930,261861,40.39665985107422,1.084674026435279e-05
65566,131133,131132,262265,40.4542510509491,1.0714629587763982e-05
65666,131333,131332,262665,40.51187515258789,1.0587298622667517e-05
65766,131533,131532,263065,40.56867980957031,1.0462491711023173e-05
65866,131733,131732,263465,40.62665390968323,1.0338359466017731e-05
65966,131933,131932,263865,40.68463683128357,1.0214164794199344e-05
66066,132133,132132,264265,40.742563009262085,1.0091304726756888e-05
66166,132333,132332,264665,40.81301188468933,9.971637656672554e-06
66266,132533,132532,265065,40.891687870025635,9.855010388847102e-06
66366,132733,132732,265465,40.97929000854492,9.739335207116926e-06
66466,132933,132932,265865,41.0387818813324,9.62316683784727e-06
66567,133135,133134,266269,41.09726309776306,9.50610647254751e-06
66667,133335,133334,266669,41.15543508529663,9.392095066044943e-06
66767,133535,133534,267069,41.21656918525696,9.280424253491105e-06
66867,133735,133734,267469,41.275416135787964,9.170239306057968e-06
66967,133935,133934,267869,41.338168144226074,9.060523613700948e-06
67067,134135,134134,268269,41.40409183502197,8.950957972531323e-06
67167,134335,134334,268669,41.47491717338562,8.841936371605017e-06
67267,134535,134534,269069,41.53999590873718,8.734071405446393e-06
67367,134735,134734,269469,41.595649003982544,8.627825823699079e-06
67467,134935,134934,269869,41.65282893180847,8.523341225358271e-06
67568,135137,135136,270273,41.7100830078125,8.419241955921861e-06
67668,135337,135336,270673,41.767356872558594,8.317036260076293e-06
67768,135537,135536,271073,41.82347011566162,8.215638493292519e-06
67868,135737,135736,271473,41.878671169281006,8.115523509994341e-06
67968,135937,135936,271873,41.93357491493225,8.016963483756674e-06
68068,136137,136136,272273,41.990293979644775,7.919697759081764e-06
68168,136337,136336,272673,42.04576897621155,7.823480169844544e-06
68268,136537,136536,273073,42.101075887680054,7.728619256198935e-06
68368,136737,136736,273473,42.1570041179657,7.635601207358444e-06
68468,136937,136936,273873,42.21132278442383,7.54430973431086e-06
68569,137139,137138,274277,42.26684808731079,7.453148381780344e-06
68669,137339,137338,274677,42.32094597816467,7.3635964668142864e-06
68769,137539,137538,275077,42.389569997787476,7.27542146253942e-06
68869,137739,137738,275477,42.45802593231201,7.189484388474654e-06
68969,137939,137938,275877,42.517159938812256,7.1055288487371216e-06
69069,138139,138138,276277,42.57176399230957,7.022312705499155e-06
69169,138339,138338,276677,42.62604117393494,6.939098886723639e-06
69269,138539,138538,277077,42.67967200279236,6.856455544096988e-06
69369,138739,138738,277477,42.735495805740356,6.775378889890081e-06
69469,138939,138938,277877,42.79190993309021,6.695987965602475e-06
69570,139141,139140,278281,42.84895205497742,6.616655930332594e-06
69670,139341,139340,278681,42.90510702133179,6.538226471548594e-06
69770,139541,139540,279081,42.959882974624634,6.460030861001193e-06
69870,139741,139740,279481,43.01756691932678,6.382613441749748e-06
69970,139941,139940,279881,43.07386493682861,6.306259823450284e-06
70070,140141,140140,280281,43.13016486167908,6.230892851423573e-06
70170,140341,140340,280681,43.18636393547058,6.156249624909426e-06
70270,140541,140540,281081,43.24262499809265,6.081959454547285e-06
70370,140741,140740,281481,43.30242609977722,6.007875543194663e-06
70470,140941,140940,281881,43.35768008232117,5.934462161537935e-06
70571,141143,141142,282285,43.41320180892944,5.861652838489431e-06
70671,141343,141342,282685,43.47144913673401,5.790838125308727e-06
70771,141543,141542,283085,43.52771306037903,5.720581615096783e-06
70871,141743,141742,283485,43.58302593231201,5.650543197181403e-06
70971,141943,141942,283885,43.640198945999146,5.581282776119708e-06
71071,142143,142142,284285,43.69596481323242,5.513459814412596e-06
71171,142343,142342,284685,43.75305104255676,5.44685617676832e-06
71271,142543,142542,285085,43.808547019958496,5.380767811599903e-06
71371,142743,142742,285485,43.86606216430664,5.3151780693665394e-06
71471,142943,142942,285885,43.924400091171265,5.250825918860528e-06
71572,143145,143144,286289,43.98071908950806,5.1874131901174406e-06
71672,143345,143344,286689,44.03733205795288,5.125518230870441e-06
71772,143545,143544,287089,44.09349799156189,5.0637814364658e-06
71872,143745,143744,287489,44.1505331993103,5.0024513766612885e-06
71972,143945,143944,287889,44.20655417442322,4.94236750504133e-06
72072,144145,144144,288289,44.26260185241699,4.883853912679247e-06
72172,144345,144344,288689,44.31959080696106,4.826416012203579e-06
72272,144545,144544,289089,44.376242876052856,4.769375478264605e-06
72372,144745,144744,289489,44.4318368434906,4.712488852995498e-06
72472,144945,144944,289889,44.49554896354675,4.656024305780815e-06
72573,145147,145146,290293,44.5655779838562,4.599931985925764e-06
72673,145347,145346,290693,44.62777805328369,4.545656886890169e-06
72773,145547,145546,291093,44.68605589866638,4.492411346688132e-06
72873,145747,145746,291493,44.74427890777588,4.439407275639548e-06
72973,145947,145946,291893,44.803394079208374,4.386006831905729e-06
73073,146147,146146,292293,44.85916805267334,4.332545884219682e-06
73173,146347,146346,292693,44.915178060531616,4.280074221116293e-06
73273,146547,146546,293093,44.97339606285095,4.229084003681615e-06
73373,146747,146746,293493,45.030192136764526,4.17890006971674e-06
73473,146947,146946,293893,45.08670496940613,4.1286033338218005e-06
73574,147149,147148,294297,45.1425199508667,4.077661664965336e-06
73674,147349,147348,294697,45.19752502441406,4.02779468290231e-06
73774,147549,147548,295097,45.25349712371826,3.978923750967165e-06
73874,147749,147748,295497,45.310160875320435,3.930799654075014e-06
73974,147949,147948,295897,45.36684584617615,3.88304790887971e-06
74074,148149,148148,296297,45.4257447719574,3.835693206481368e-06
74174,148349,148348,296697,45.481691122055054,3.788979237704592e-06
74274,148549,148548,297097,45.53824305534363,3.7429383792721963e-06
74374,148749,148748,297497,45.59435701370239,3.6973933638966984e-06
74474,148949,148948,297897,45.6505970954895,3.6522737645715735e-06
74575,149151,149150,298301,45.70987606048584,3.607274416361103e-06
74675,149351,149350,298701,45.76693081855774,3.563482168429292e-06
74775,149551,149550,299101,45.82470917701721,3.5205864102551228e-06
74875,149751,149750,299501,45.88205695152283,3.4785840333324177e-06
74975,149951,149950,299901,45.940165758132935,3.437232033917708e-06
75075,150151,150150,300301,45.99926996231079,3.396183273743073e-06
75175,150351,150350,300701,46.0587899684906,3.3553860780812256e-06
75275,150551,150550,301101,46.11621809005737,3.3152474957659398e-06
75375,150751,150750,301501,46.1750111579895,3.27619188733722e-06
75475,150951,150950,301901,46.232362031936646,3.2380646459740446e-06
75576,151153,151152,302305,46.292336225509644,3.199811534489327e-06
75676,151353,151352,302705,46.35120987892151,3.1617547769410877e-06
75776,151553,151552,303105,46.41008901596069,3.123862331596677e-06
75876,151753,151752,303505,46.474480867385864,3.0868381291892873e-06
75976,151953,151952,303905,46.535008907318115,3.050891933502293e-06
76076,152153,152152,304305,46.595513105392456,3.015519454078934e-06
76176,152353,152352,304705,46.66762018203735,2.980087313997555e-06
76276,152553,152552,305105,46.739147901535034,2.9444371836527494e-06
76376,152753,152752,305505,46.796468019485474,2.9089164427503043e-06
76476,152953,152952,305905,46.853739976882935,2.873964365160425e-06
76577,153155,153154,306309,46.91430187225342,2.839374636206642e-06
76677,153355,153354,306709,46.972999811172485,2.8056021503826897e-06
76777,153555,153554,307109,47.03123879432678,2.7719913898512007e-06
76877,153755,153754,307509,47.08911204338074,2.7384654014684527e-06
76977,153955,153954,307909,47.14860486984253,2.7052216726317153e-06
77077,154155,154154,308309,47.20912504196167,2.6724856093026847e-06
77177,154355,154354,308709,47.26658892631531,2.640266871948551e-06
77277,154555,154554,309109,47.326213121414185,2.6083904100481276e-06
77377,154755,154754,309509,47.38679099082947,2.5767476251300735e-06
77477,154955,154954,309909,47.44647288322449,2.5454416752342155e-06
77578,155157,155156,310313,47.50515294075012,2.514332615142905e-06
77678,155357,155356,310713,47.56483292579651,2.484043679463038e-06
77778,155557,155556,311113,47.62333583831787,2.454131113219411e-06
77878,155757,155756,311513,47.680959939956665,2.424531709374477e-06
77978,155957,155956,311913,47.741377115249634,2.39538126672463e-06
78078,156157,156156,312313,47.80099105834961,2.3668899806164365e-06
78178,156357,156356,312713,47.859477043151855,2.3390592183608774e-06
78278,156557,156556,313113,47.917937994003296,2.311600961737528e-06
78378,156757,156756,313513,47.977883100509644,2.284248279986976e-06
78478,156957,156956,313913,48.03696298599243,2.257089860950576e-06
78579,157159,157158,314317,48.09598207473755,2.2301987948627292e-06
78679,157359,157358,314717,48.15446591377258,2.204255759855994e-06
78779,157559,157558,315117,48.2147159576416,2.1787470364288214e-06
78879,157759,157758,315517,48.27278804779053,2.1533181734215166e-06
78979,157959,157958,315917,48.33109188079834,2.1278972232336987e-06
79079,158159,158158,316317,48.38876795768738,2.1027236570610617e-06
79179,158359,158358,316717,48.449328899383545,2.0780145237559054e-06
79279,158559,158558,317117,48.50731587409973,2.0537082068619643e-06
79379,158759,158758,317517,48.565123081207275,2.029572080373028e-06
79479,158959,158958,317917,48.622811794281006,2.005466593302359e-06
79580,159161,159160,318321,48.682340145111084,1.9812061757979417e-06
79680,159361,159360,318721,48.74190306663513,1.957436420804103e-06
79780,159561,159560,319121,48.81387495994568,1.9340506022440755e-06
79880,159761,159760,319521,48.88178205490112,1.9110343604610897e-06
79980,159961,159960,319921,48.93891000747681,1.8882278700788334e-06
80080,160161,160160,320321,48.99518799781799,1.8654956029839672e-06
80180,160361,160360,320721,49.055476903915405,1.84288459661759e-06
80280,160561,160560,321121,49.114808082580566,1.8205615113476113e-06
80380,160761,160760,321521,49.171207904815674,1.7985967443388238e-06
80480,160961,160960,321921,49.22890901565552,1.7768822480899738e-06
80581,161163,161162,322325,49.286808013916016,1.7550968820435613e-06
80681,161363,161362,322725,49.34321308135986,1.7337630722222715e-06
80781,161563,161562,323125,49.40301012992859,1.7128444775480456e-06
80881,161763,161762,323525,49.467808961868286,1.69233877985594e-06
80981,161963,161962,323925,49.52469205856323,1.6720580518476242e-06
81081,162163,162162,324325,49.58422088623047,1.6519175810706472e-06
81181,162363,162362,324725,49.64551591873169,1.6320669099062695e-06
81281,162563,162562,325125,49.70415210723877,1.6126683350884614e-06
81381,162763,162762,325525,49.77119588851929,1.5936662567809742e-06
81481,162963,162962,325925,49.83410692214966,1.5748616763579407e-06
81582,163165,163164,326329,49.897356033325195,1.5559683386047738e-06
81682,163365,163364,326729,49.95923089981079,1.5374564417569558e-06
81782,163565,163564,327129,50.02065110206604,1.519293092644214e-06
81882,163765,163764,327529,50.08230710029602,1.50151075505598e-06
81982,163965,163964,327929,50.14322304725647,1.4839881080529522e-06
82082,164165,164164,328329,50.20658302307129,1.4665680444731932e-06
82182,164365,164364,328729,50.267874002456665,1.4491922368872726e-06
82282,164565,164564,329129,50.32859802246094,1.4319541090504765e-06
82382,164765,164764,329529,50.385550022125244,1.4150245506421163e-06
82482,164965,164964,329929,50.44566202163696,1.398469566077759e-06
82583,165167,165166,330333,50.50911211967468,1.3819754764775833e-06
82683,165367,165366,330733,50.56925392150879,1.3656398166042768e-06
82783,165567,165566,331133,50.63046193122864,1.3492558431596208e-06
82883,165767,165766,331533,50.68891215324402,1.333012304645386e-06
82983,165967,165966,331933,50.74998998641968,1.3170952876362194e-06
83083,166167,166166,332333,50.808692932128906,1.3014693974912791e-06
83183,166367,166366,332733,50.86673617362976,1.285946154819672e-06
83283,166567,166566,333133,50.94594407081604,1.2704370756107218e-06
83383,166767,166766,333533,51.03136897087097,1.2550541174487275e-06
83483,166967,166966,333933,51.08991098403931,1.2399378091000795e-06
83584,167169,167168,334337,51.14828014373779,1.2249248579436813e-06
83684,167369,167368,334737,51.20559906959534,1.210193380828141e-06
83784,167569,167568,335137,51.26391100883484,1.1955466545686345e-06
83884,167769,167768,335537,51.32126498222351,1.1810477825428527e-06
83984,167969,167968,335937,51.38298487663269,1.1667702203684663e-06
84084,168169,168168,336337,51.4657940864563,1.1527200880534965e-06
84184,168369,168368,336737,51.53338289260864,1.1388506085924966e-06
84284,168569,168568,337137,51.59806680679321,1.125128099406927e-06
84384,168769,168768,337537,51.65502214431763,1.1115867961346459e-06
84484,168969,168968,337937,51.713643074035645,1.0983170826698765e-06
84585,169171,169170,338341,51.77281618118286,1.0852439558232223e-06
84685,169371,169370,338741,51.83971881866455,1.072548792244412e-06
84785,169571,169570,339141,51.899137020111084,1.059936933322973e-06
84885,169771,169770,339541,51.95536994934082,1.047330660994618e-06
84985,169971,169970,339941,52.01953601837158,1.0348436064616e-06
85085,170171,170170,340341,52.07485103607178,1.0226645380021594e-06
85185,170371,170370,340741,52.13043403625488,1.010832983269347e-06
85285,170571,170570,341141,52.20146989822388,9.99178229461375e-07
85385,170771,170770,341541,52.26221585273743,9.875010076943707e-07
85485,170971,170970,341941,52.31873416900635,9.757801452259015e-07
85586,171173,171172,342345,52.376686096191406,9.640626074038956e-07
85686,171373,171372,342745,52.43189811706543,9.527427857566978e-07
85786,171573,171572,343145,52.48674702644348,9.416911920594927e-07
85886,171773,171772,343545,52.54271411895752,9.307391423669506e-07
85986,171973,171972,343945,52.59853792190552,9.197445803809259e-07
86086,172173,172172,344345,52.65353298187256,9.087329804441159e-07
86186,172373,172372,344745,52.708779096603394,8.978422577979304e-07
86286,172573,172572,345145,52.763787031173706,8.871564333162901e-07
86386,172773,172772,345545,52.82499980926514,8.766308807481549e-07
86486,172973,172972,345945,52.88568711280823,8.661736296787638e-07
86587,173175,173174,346349,52.94337511062622,8.556525158306274e-07
86687,173375,173374,346749,52.999096155166626,8.45321449677144e-07
86787,173575,173574,347149,53.06352400779724,8.351200297068377e-07
86887,173775,173774,347549,53.15099501609802,8.250424542315373e-07
86987,173975,173974,347949,53.223780155181885,8.150602593278484e-07
87087,174175,174174,348349,53.28210210800171,8.051750218774361e-07
87187,174375,174374,348749,53.33717608451843,7.954323645021531e-07
87287,174575,174574,349149,53.394065856933594,7.858838602241302e-07
87387,174775,174774,349549,53.450072050094604,7.765301579008759e-07
87487,174975,174974,349949,53.50781321525574,7.673062606232353e-07
87588,175177,175176,350353,53.56339502334595,7.580544056193875e-07
87688,175377,175376,350753,53.619112968444824,7.489751482107979e-07
87788,175577,175576,351153,53.673758029937744,7.400693693352457e-07
87888,175777,175776,351553,53.73484206199646,7.31391980703694e-07
87988,175977,175976,351953,53.804786920547485,7.228777660174844e-07
88088,176177,176176,352353,53.85926699638367,7.144046670104168e-07
88188,176377,176376,352753,53.91450381278992,7.059364633497453e-07
88288,176577,176576,353153,53.96984505653381,6.975692796330037e-07
88388,176777,176776,353553,54.024659872055054,6.89416427342105e-07
88488,176977,176976,353953,54.080551862716675,6.814691083508181e-07
88589,177179,177178,354357,54.13791584968567,6.735275193521018e-07
88689,177379,177378,354757,54.19391417503357,6.656533138892045e-07
88789,177579,177578,355157,54.24929618835449,6.577873098848816e-07
88889,177779,177778,355557,54.30608105659485,6.500120907498784e-07
88989,177979,177978,355957,54.36630082130432,6.423747085292166e-07
89089,178179,178178,356357,54.422404050827026,6.348526156295191e-07
89189,178379,178378,356757,54.47751593589783,6.273913774085267e-07
89289,178579,178578,357157,54.53214693069458,6.199554915866075e-07
89389,178779,178778,357557,54.58626103401184,6.125515655286833e-07
89489,178979,178978,357957,54.640592098236084,6.052174083098207e-07
89590,179181,179180,358361,54.695703983306885,5.979130086102331e-07
89690,179381,179380,358761,54.75102996826172,5.907730523524126e-07
89790,179581,179580,359161,54.810559034347534,5.836845864861313e-07
89890,179781,179780,359561,54.86387085914612,5.766346507718779e-07
89990,179981,179980,359961,54.91804480552673,5.696635572283088e-07
90090,180181,180180,360361,54.973772048950195,5.628111482474999e-07
90190,180381,180380,360761,55.02847695350647,5.56058189399204e-07
90290,180581,180580,361161,55.08458995819092,5.493586766951103e-07
90390,180781,180780,361561,55.140880823135376,5.42718415155775e-07
90490,180981,180980,361961,55.20684599876404,5.361959827254872e-07
90591,181183,181182,362365,55.27693009376526,5.297568661274034e-07
90691,181383,181382,362765,55.337804079055786,5.234841580130019e-07
90791,181583,181582,363165,55.40873384475708,5.172588115196956e-07
90891,181783,181782,363565,55.484740018844604,5.110912350881152e-07
90991,181983,181982,363965,55.55750489234924,5.050398418078285e-07
91091,182183,182182,364365,55.61807990074158,4.991300116461012e-07
91191,182383,182382,364765,55.676182985305786,4.933209744936856e-07
91291,182583,182582,365165,55.733349084854126,4.875567713044838e-07
91391,182783,182782,365565,55.790714740753174,4.818242773626119e-07
91491,182983,182982,365965,55.847482204437256,4.761525891898084e-07
91592,183185,183184,366369,55.90445590019226,4.705210408575822e-07
91692,183385,183384,366769,55.96260404586792,4.6505153643708156e-07
91792,183585,183584,367169,56.021775007247925,4.596626586778346e-07
91892,183785,183784,367569,56.07817602157593,4.543090846393008e-07
91992,183985,183984,367969,56.13455295562744,4.489680542075586e-07
92092,184185,184184,368369,56.19244909286499,4.436687872582898e-07
92192,184385,184384,368769,56.25176811218262,4.3846155321911535e-07
92292,184585,184584,369169,56.308927059173584,4.33352780368806e-07
92392,184785,184784,369569,56.378578901290894,4.282909121109862e-07
92492,184985,184984,369969,56.43732190132141,4.2322909376327765e-07
92593,185187,185186,370373,56.49701404571533,4.181329603788996e-07
92693,185387,185386,370773,56.55479192733765,4.131559665817443e-07
92793,185587,185586,371173,56.6130428314209,4.082632033682309e-07
92893,185787,185786,371573,56.66951084136963,4.034187034706379e-07
92993,185987,185986,371973,56.728158950805664,3.985916245233719e-07
93093,186187,186186,372373,56.78599715232849,3.937975922901961e-07
93193,186387,186386,372773,56.8431670665741,3.8907122174639353e-07
93293,186587,186586,373173,56.90111994743347,3.8441927296461854e-07
93393,186787,186786,373573,56.9732449054718,3.7981954445602524e-07
93493,186987,186986,373973,57.03116488456726,3.7525845597535504e-07
93594,187189,187188,374377,57.08942890167236,3.7070867586690696e-07
93694,187389,187388,374777,57.14697599411011,3.662888906221662e-07
93794,187589,187588,375177,57.203441858291626,3.619575877507921e-07
93894,187789,187788,375577,57.25941491127014,3.5768672225747386e-07
93994,187989,187988,375977,57.32280492782593,3.5344565669422275e-07
94094,188189,188188,376377,57.39587616920471,3.492347546739041e-07
94194,188389,188388,376777,57.462379932403564,3.4508773212149264e-07
94294,188589,188588,377177,57.518900871276855,3.4103909026113684e-07
94394,188789,188788,377577,57.574923038482666,3.37085531076439e-07
94494,188989,188988,377977,57.630714893341064,3.3318082584499075e-07
94595,189191,189190,378381,57.68688106536865,3.2923862170050655e-07
94695,189391,189390,378781,57.747523069381714,3.2533952460003263e-07
94795,189591,189590,379181,57.80948805809021,3.214977312434846e-07
94895,189791,189790,379581,57.87031388282776,3.1775956604912793e-07
94995,189991,189990,379981,57.92848515510559,3.14110023343391e-07
95095,190191,190190,380381,57.99215316772461,3.1048573131058114e-07
95195,190391,190390,380781,58.050256967544556,3.068440555883996e-07
95295,190591,190590,381181,58.108142137527466,3.032072396505976e-07
95395,190791,190790,381581,58.1653528213501,2.996300069060547e-07
95495,190991,190990,381981,58.2395179271698,2.9613407849212896e-07
95596,191193,191192,382385,58.31120681762695,2.9265440062324074e-07
95696,191393,191392,382785,58.377326011657715,2.8921730647704145e-07
95796,191593,191592,383185,58.43732500076294,2.857782416067841e-07
95896,191793,191792,383585,58.49573612213135,2.823587629851113e-07
95996,191993,191992,383985,58.556060791015625,2.7898097333163993e-07
96096,192193,192192,384385,58.61667084693909,2.756476156238138e-07
96196,192393,192392,384785,58.675390005111694,2.72349630487867e-07
96296,192593,192592,385185,58.73500108718872,2.69083354886126e-07
96396,192793,192792,385585,58.79481911659241,2.6585464550193153e-07
96496,192993,192992,385985,58.85456681251526,2.6266918325117704e-07
96597,193195,193194,386389,58.91514015197754,2.594933049732299e-07
96697,193395,193394,386789,58.97560501098633,2.563825507026551e-07
96797,193595,193594,387189,59.03331780433655,2.5330324488576193e-07
96897,193795,193794,387589,59.09281516075134,2.5026511118370755e-07
96997,193995,193994,387989,59.15105104446411,2.472831493770019e-07
97097,194195,194194,388389,59.21201205253601,2.443597490981179e-07
97197,194395,194394,388789,59.28445887565613,2.4147455799511677e-07
97297,194595,194594,389189,59.35992503166199,2.386011384964809e-07
97397,194795,194794,389589,59.42307186126709,2.3573956436651094e-07
97497,194995,194994,389989,59.49651789665222,2.3292593978037373e-07
97598,195197,195196,390393,59.57461094856262,2.3017015707292656e-07
97698,195397,195396,390793,59.63399386405945,2.2751776349706035e-07
97798,195597,195596,391193,59.69600510597229,2.2488909301872662e-07
97898,195797,195796,391593,59.75695204734802,2.22244563497206e-07
97998,195997,195996,391993,59.81830596923828,2.195981575788809e-07
98098,196197,196196,392393,59.87866401672363,2.1699600910404e-07
98198,196397,196396,392793,59.937726974487305,2.1446359062865682e-07
98298,196597,196596,393193,59.99684000015259,2.119844681379751e-07
98398,196797,196796,393593,60.05543303489685,2.095247981742123e-07
98498,196997,196996,393993,60.117424964904785,2.0706618745094666e-07
98599,197199,197198,394397,60.182496070861816,2.0459068060364503e-07
98699,197399,197398,394797,60.267776012420654,2.0216660642634568e-07
98799,197599,197598,395197,60.3420889377594,1.9978337868365573e-07
98899,197799,197798,395597,60.410048961639404,1.974380034542728e-07
98999,197999,197998,395997,60.468979835510254,1.9511284662155972e-07
99099,198199,198198,396397,60.52646803855896,1.9279331230797625e-07
99199,198399,198398,396797,60.58385396003723,1.9048403478150112e-07
99299,198599,198598,397197,60.64099884033203,1.8820207742954967e-07
99399,198799,198798,397597,60.70054602622986,1.859541448470476e-07
99499,198999,198998,397997,60.77490997314453,1.8373022571709705e-07
99600,199201,199200,398401,60.85618615150452,1.8150118851289065e-07
99700,199401,199400,398801,60.91706299781799,1.79321443504642e-07
99800,199601,199600,399201,60.975502014160156,1.771818899670854e-07
99900,199801,199800,399601,61.03328895568848,1.7507729766674394e-07
100000,200001,200000,400001,61.0918710231781,1.7299025675631476e-07


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/flex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.001444101333618164,30.358106049564984
100,459,0,459,1.3437139987945557,0.4177783180862636
200,946,0,946,2.6486191749572754,0.14175932992192242
300,1438,0,1438,3.8425540924072266,0.07601728769773797
400,1938,0,1938,5.278935194015503,0.0725310775598768
501,2437,0,2437,6.596522092819214,0.04538065490306894
601,2937,0,2937,7.757116317749023,0.044068625079784526
701,3433,0,3433,8.949284076690674,0.03533688712286274
801,3932,0,3932,10.12729811668396,0.02924057673082615
901,4432,0,4432,11.279781103134155,0.028390523873332518
1001,4932,0,4932,12.379555225372314,0.027765611371221067
1101,5430,0,5430,13.49347996711731,0.025054014706036555
1201,5930,0,5930,14.596665143966675,0.023414283276782594
1301,6430,0,6430,15.710084199905396,0.022681373934310387
1401,6928,0,6928,16.8121120929718,0.01990069636099634
1502,7433,0,7433,17.952710151672363,0.019121594206419255
1602,7933,0,7933,19.07693910598755,0.01858096791255499
1702,8433,0,8433,20.180617094039917,0.018144552419579744
1802,8929,0,8929,21.27962899208069,0.015316418393985001
1902,9429,0,9429,22.385278940200806,0.013597420394604117
2002,9929,0,9929,23.636065006256104,0.01315521950758562
2102,10429,0,10429,24.871247053146362,0.012806038390595714
2202,10928,0,10928,25.925913095474243,0.011881428256675928
2302,11428,0,11428,26.899526119232178,0.011480478014737422
2402,11928,0,11928,27.853302001953125,0.011214057586319317
2503,12432,0,12432,28.869408130645752,0.010327181404105597
2603,12932,0,12932,29.957327127456665,0.010045841745684337
2703,13431,0,13431,31.071592092514038,0.009314577543619739
2803,13931,0,13931,32.31199526786804,0.008984460058306986
2903,14431,0,14431,33.474244117736816,0.008797737119575492
3003,14929,0,14929,34.5835599899292,0.007795128751181283
3103,15429,0,15429,35.681008100509644,0.007402164356026432
3203,15929,0,15929,36.79555296897888,0.007164753451444441
3303,16429,0,16429,37.94761109352112,0.006977696664473585
3403,16929,0,16929,39.20013999938965,0.006822265438383189
3504,17432,0,17432,40.3418550491333,0.006299274488423881
3604,17932,0,17932,41.46460318565369,0.00594520532488727
3704,18432,0,18432,42.68791198730469,0.0057305625896245
3804,18932,0,18932,43.79246807098389,0.0055721034066578716
3904,19432,0,19432,45.004515171051025,0.005445026156827749
4004,19931,0,19931,46.117182970047,0.005114177517521077
4104,20431,0,20431,47.24500513076782,0.00495361539262455
4204,20931,0,20931,48.64005923271179,0.0048415489454242755
4304,21431,0,21431,49.85076093673706,0.004751275876701585
4404,21930,0,21930,51.281538009643555,0.004404655749844648
4505,22435,0,22435,52.51587104797363,0.004291968948930966
4605,22934,0,22934,53.79017496109009,0.004042927019732852
4705,23434,0,23434,55.138615131378174,0.0039104690294445976
4805,23934,0,23934,56.236714124679565,0.003831582489277955
4905,24434,0,24434,57.356343030929565,0.0037687916076420106
5005,24934,0,24934,58.45380520820618,0.0037140079593162567
5105,25434,0,25434,59.57071304321289,0.0036637177711404166
5205,25933,0,25933,60.664454221725464,0.0034308828938173887
5305,26433,0,26433,61.76676607131958,0.0033183566038330276
5405,26933,0,26933,62.86151719093323,0.0032534607671240515
5506,27434,0,27434,63.97145128250122,0.002601333708075385
5606,27934,0,27934,65.06941103935242,0.002461351895938841
5706,28434,0,28434,66.18212413787842,0.0023769331894139428
5806,28934,0,28934,67.34075117111206,0.0023126743631039413
5906,29434,0,29434,68.47047710418701,0.002260107506134496
6006,29934,0,29934,69.6246280670166,0.002214863776737378
6106,30434,0,30434,70.80647921562195,0.0021747861671821147
6206,30934,0,30934,71.95562601089478,0.002138376884605648
6306,31434,0,31434,73.09168219566345,0.0021045387067470957
6406,31931,0,31931,74.19195508956909,0.001768305579215513
6507,32436,0,32436,75.29798197746277,0.0016444399345383839
6607,32936,0,32936,76.42410230636597,0.00158055689094123
6707,33436,0,33436,77.52315211296082,0.0015376571350073102
6807,33936,0,33936,78.64048218727112,0.0015042413216694644
6907,34436,0,34436,79.77792692184448,0.0014757756509199908
7007,34936,0,34936,80.92021918296814,0.001450372558477935
7107,35436,0,35436,82.03440809249878,0.0014271372478449598
7207,35936,0,35936,83.14057302474976,0.0014054709197256073
7307,36436,0,36436,84.2688980102539,0.0013852217253169
7407,36935,0,36935,85.36927223205566,0.0013174525609556354
7508,37440,0,37440,86.52415800094604,0.001271514913751273
7608,37940,0,37940,87.6423671245575,0.001241946102043871
7708,38440,0,38440,88.73730206489563,0.00121903349112773
7808,38940,0,38940,89.87076997756958,0.0011995365763850234
7908,39438,0,39438,91.02064418792725,0.0010934910665205695
8008,39938,0,39938,92.12119197845459,0.0010382455800063799
8108,40438,0,40438,93.21584796905518,0.0010079355365055036
8208,40938,0,40938,94.46010613441467,0.0009860915212939875
8308,41438,0,41438,95.6563949584961,0.0009681037842690677
8408,41938,0,41938,96.89652991294861,0.0009523147156473299
8509,42443,0,42443,98.17666101455688,0.0009377770408143001
8609,42943,0,42943,99.4133551120758,0.000924456937117362
8709,43443,0,43443,100.9830310344696,0.0009119188525692536
8809,43943,0,43943,102.34749794006348,0.0009000652893896586
8909,44443,0,44443,103.57060194015503,0.0008886739611242621
9009,44942,0,44942,104.90580916404724,0.0008443116261274162
9109,45442,0,45442,106.14191794395447,0.0008210645325951795
9209,45942,0,45942,107.44775819778442,0.0008036742749053365
9309,46442,0,46442,108.69150018692017,0.0007892526970755217
9409,46942,0,46942,109.91604709625244,0.0007766510134182753
9510,47447,0,47447,111.1652340888977,0.0007651295061535939
9610,47947,0,47947,112.29032492637634,0.0007545677099223517
9710,48446,0,48446,113.52125906944275,0.0007324156725780625
9810,48946,0,48946,114.67651510238647,0.0007014458974664369
9910,49446,0,49446,115.83966898918152,0.0006852987940345988
10010,49946,0,49946,117.16943216323853,0.0006733674818009415
10110,50446,0,50446,118.36485004425049,0.0006631582277245041
10210,50946,0,50946,119.5842182636261,0.0006538674943510608
10310,51446,0,51446,120.76018905639648,0.0006451683380868496
10410,51946,0,51946,122.0774872303009,0.0006368829577454346
10511,52451,0,52451,123.30457806587219,0.0006288208138258747
10611,52951,0,52951,124.40029501914978,0.0006211169030631502
10711,53451,0,53451,125.4135811328888,0.0006136395843641378
10811,53951,0,53951,126.49870014190674,0.0006063908319252937
10911,54451,0,54451,127.75040626525879,0.0005992932638615387
11011,54950,0,54950,129.09409308433533,0.0005620960651881439
11111,55450,0,55450,130.3426811695099,0.0005473522747839182
11211,55950,0,55950,131.60787892341614,0.0005374317940319283
11311,56450,0,56450,132.99244594573975,0.0005293268932826646
11411,56950,0,56950,134.60720205307007,0.0005221184689501902
11512,57455,0,57455,135.9972381591797,0.0005153643422958937
11612,57955,0,57955,137.35430717468262,0.0005090204624176557
11712,58455,0,58455,138.8443431854248,0.0005029207592326038
11812,58955,0,58955,140.2047061920166,0.0004970207468232001
11912,59455,0,59455,141.39050388336182,0.000491300283093536
12012,59955,0,59955,142.71889424324036,0.00048573766154281497
12112,60455,0,60455,144.04824805259705,0.0004803182608662925
12212,60954,0,60954,145.46413111686707,0.0004563348145047628
12312,61454,0,61454,146.68298387527466,0.00044436700353847494
12412,61954,0,61954,148.17941212654114,0.00043649320553683217
12513,62459,0,62459,149.3172469139099,0.0004300656099434651
12613,62959,0,62959,150.4829502105713,0.00042438606294749933
12713,63459,0,63459,151.7871081829071,0.0004190957602749606
12813,63959,0,63959,153.04019403457642,0.0004140468736639998
12913,64459,0,64459,154.41687393188477,0.0004091800198050311
13013,64959,0,64959,156.07093000411987,0.0004044434858118401
13113,65459,0,65459,157.75449919700623,0.00039980169698236893
13213,65959,0,65959,160.0249059200287,0.00039525038160553
13313,66459,0,66459,161.69914603233337,0.00039076420679845525
13413,66959,0,66959,163.48623895645142,0.00038635133171211817
13514,67464,0,67464,165.0318672657013,0.0003819460308852868
13614,67964,0,67964,166.36785411834717,0.0003776505137463102
13714,68464,0,68464,167.63716506958008,0.00037340694758298117
13814,68964,0,68964,169.11024808883667,0.0003692209066811099
13914,69464,0,69464,170.3735601902008,0.00036510333860995635
14014,69964,0,69964,171.77043509483337,0.00036103490449362414
14114,70464,0,70464,173.04830312728882,0.00035703451515604174
14214,70964,0,70964,174.4976770877838,0.0003530803603711334
14314,71464,0,71464,176.26417422294617,0.0003491786256077799
14414,71964,0,71964,177.54377698898315,0.0003453250709973222
14515,72468,0,72468,178.73351192474365,0.00033438566170958576
14615,72968,0,72968,180.18937397003174,0.0003256733222885569
14715,73468,0,73468,181.6072871685028,0.00031889909115047983
14815,73968,0,73968,182.8272180557251,0.000313323314360583
14915,74468,0,74468,184.04116916656494,0.0003085027848760246
15015,74968,0,74968,185.24681496620178,0.00030417286917158037
15115,75468,0,75468,186.50020623207092,0.00030018353704620247
15215,75968,0,75968,187.90470814704895,0.00029642753700423284
15315,76468,0,76468,189.4217710494995,0.00029283841574578395
15415,76968,0,76968,190.89225697517395,0.0002893826395526868
15516,77473,0,77473,192.13032007217407,0.00028598247437223615
15616,77973,0,77973,193.6739902496338,0.0002826946981087163
15716,78473,0,78473,195.1978461742401,0.0002794712137918587
15816,78973,0,78973,196.79899406433105,0.00027629751150990453
15916,79473,0,79473,198.27394723892212,0.0002731705321914717
16016,79973,0,79973,199.80794215202332,0.00027008693640050125
16116,80473,0,80473,201.13425207138062,0.0002670446304588568
16216,80973,0,80973,202.38352012634277,0.00026404001567025963
16316,81473,0,81473,203.59275603294373,0.00026107951000241465
16416,81973,0,81973,204.84079003334045,0.0002581564813065858
16517,82478,0,82478,206.31258010864258,0.0002552462808488027
16617,82978,0,82978,207.58086705207825,0.0002524050521029749
16717,83478,0,83478,208.93677496910095,0.00024960119026006526
16817,83978,0,83978,210.2335660457611,0.00024683866603185525
16917,84478,0,84478,212.07190918922424,0.00024411248382455884
17017,84978,0,84978,214.2612280845642,0.00024142666906205965
17117,85478,0,85478,216.1512451171875,0.00023878212756152758
17217,85978,0,85978,217.5940990447998,0.0002361746668935683
17317,86478,0,86478,218.87350511550903,0.00023361317058781127
17417,86978,0,86978,220.64686012268066,0.00023108962894049834
17518,87483,0,87483,222.1141140460968,0.00022858497820521425
17618,87983,0,87983,223.50740313529968,0.0002261444358158042
17718,88483,0,88483,225.2631549835205,0.00022374153408966625
17818,88983,0,88983,227.03921008110046,0.00022137357621910511
17918,89482,0,89482,228.8451452255249,0.0002155168875996505
18018,89982,0,89982,230.73800706863403,0.00021083043928781856
18118,90482,0,90482,232.11134099960327,0.00020684969946099986
18218,90982,0,90982,233.66431427001953,0.00020336187707748732
18318,91482,0,91482,234.99761509895325,0.00020024622982228057
18418,91982,0,91982,236.40107321739197,0.00019739572932560512
18519,92487,0,92487,237.69369220733643,0.0001947157209637144
18619,92987,0,92987,238.94412422180176,0.00019221221107425495
18719,93487,0,93487,240.4250612258911,0.0001898185981769276
18819,93987,0,93987,241.9810061454773,0.00018751631835416916
18919,94487,0,94487,243.17607927322388,0.00018529069359485832
19019,94987,0,94987,244.25333499908447,0.00018312069041499755
19119,95487,0,95487,245.42418217658997,0.0001810091211522038
19219,95987,0,95987,246.6499960422516,0.00017893778333190536
19319,96487,0,96487,247.79554319381714,0.00017691253864272224
19419,96987,0,96987,248.94996404647827,0.0001749222375333678
19520,97492,0,97492,250.24643301963806,0.00017295354273458966
19620,97992,0,97992,251.44610214233398,0.00017103491865520966
19720,98492,0,98492,252.99484014511108,0.00016915081471442455
19820,98992,0,98992,254.39477610588074,0.000167300366168136
19920,99492,0,99492,255.65587401390076,0.00016547689978376978
20020,99992,0,99992,256.7851951122284,0.00016368722019534468
20120,100492,0,100492,257.88951301574707,0.00016192382266078174
20220,100992,0,100992,259.09400820732117,0.0001601862650150349
20320,101492,0,101492,260.32452416419983,0.00015847404154761398
20420,101992,0,101992,261.4506139755249,0.00015678359310343867
20521,102497,0,102497,262.6436128616333,0.00015510021801141535
20621,102997,0,102997,264.1100420951843,0.00015345134606217754
20721,103497,0,103497,265.4151191711426,0.00015182013742909097
20821,103997,0,103997,266.8133592605591,0.00015020498991846754
20921,104497,0,104497,268.05882024765015,0.00014860336021587476
21021,104997,0,104997,269.2431321144104,0.0001470157093916856
21121,105497,0,105497,270.36021995544434,0.00014544042156765767
21221,105997,0,105997,271.58097219467163,0.00014387567760265006
21321,106497,0,106497,272.7089989185333,0.00014232258250607304
21421,106997,0,106997,273.89279413223267,0.00014078150182636855
21522,107502,0,107502,275.1102452278137,0.00013923581265492196
21622,108002,0,108002,276.29761719703674,0.00013771666997906994
21722,108502,0,108502,277.49145007133484,0.00013621260987070301
21822,109002,0,109002,278.6788651943207,0.00013472124940212642
21922,109502,0,109502,279.95566415786743,0.0001332453210948506
22022,110002,0,110002,281.20237493515015,0.00013178703065396482
22122,110502,0,110502,282.27047085762024,0.0001303441077582096
22222,111002,0,111002,283.5417721271515,0.00012891935454397417
22322,111502,0,111502,284.70920610427856,0.00012751316206831967
22422,112002,0,112002,285.8222200870514,0.00012612426406327691
22523,112507,0,112507,287.01996326446533,0.0001247398451410863
22623,113006,0,113006,288.302855014801,0.0001219657756015339
22723,113506,0,113506,289.4547052383423,0.0001192346332761072
22823,114006,0,114006,290.5561349391937,0.00011687087247224473
22923,114506,0,114506,291.71707010269165,0.00011478003341600703
23023,115006,0,115006,292.92033314704895,0.00011289891523710435
23123,115506,0,115506,294.05291223526,0.00011118691534247451
23223,116006,0,116006,295.2617530822754,0.00010960693505900789
23323,116506,0,116506,296.5679852962494,0.00010812648506114296
23423,117006,0,117006,297.76085805892944,0.0001067246270977538
23524,117511,0,117511,298.93977308273315,0.00010537409894352683
23624,118011,0,118011,300.2640380859375,0.00010408742653686867
23724,118511,0,118511,301.40400218963623,0.00010284182505709286
23824,119011,0,119011,302.6144971847534,0.00010163698539779948
23924,119511,0,119511,303.80491399765015,0.00010046050819300394
24024,120011,0,120011,304.98391103744507,9.930408893726373e-05
24124,120511,0,120511,306.0897569656372,9.817126151220233e-05
24224,121011,0,121011,307.19545006752014,9.705915282310924e-05
24324,121511,0,121511,308.28785514831543,9.596430722778784e-05
24424,122011,0,122011,309.39580488204956,9.488622230077426e-05
24525,122516,0,122516,310.5050871372223,9.381386532289594e-05
24625,123016,0,123016,311.6967911720276,9.276572470910681e-05
24725,123516,0,123516,312.80940222740173,9.173063275885457e-05
24825,124016,0,124016,313.90950202941895,9.071297074896527e-05
24925,124516,0,124516,315.00067615509033,8.970884883966132e-05
25025,125016,0,125016,316.10490918159485,8.871666237168206e-05
25125,125516,0,125516,317.2046048641205,8.774064529236145e-05
25225,126016,0,126016,318.3036811351776,8.677980866962623e-05
25325,126516,0,126516,319.39744424819946,8.582937053546485e-05
25425,127016,0,127016,320.50361800193787,8.48955757202122e-05
25526,127521,0,127521,321.6128010749817,8.39687798843142e-05
25626,128021,0,128021,322.7121069431305,8.306106069174072e-05
25726,128521,0,128521,323.80378818511963,8.216805926327842e-05
25826,129021,0,129021,324.9125680923462,8.128919739224383e-05
25926,129521,0,129521,326.01856803894043,8.042003796319915e-05
26026,130021,0,130021,327.20936822891235,7.956288142042239e-05
26126,130521,0,130521,328.34621596336365,7.87171528088483e-05
26226,131021,0,131021,329.44941306114197,7.78789414092479e-05
26326,131521,0,131521,330.5596580505371,7.705167112803877e-05
26426,132021,0,132021,331.6555550098419,7.623337710794204e-05
26527,132526,0,132526,332.7722361087799,7.541157643651911e-05
26627,133026,0,133026,333.8605649471283,7.460622772078033e-05
26727,133526,0,133526,334.9705421924591,7.380995793479146e-05
26827,134026,0,134026,336.067675113678,7.30190492240955e-05
26927,134526,0,134526,337.1739110946655,7.223385281532876e-05
27027,135026,0,135026,338.26326608657837,7.14554312265782e-05
27127,135526,0,135526,339.477441072464,7.068458652004796e-05
27227,136026,0,136026,340.62790513038635,6.991971092065215e-05
27327,136526,0,136526,341.8284249305725,6.916301012470776e-05
27427,137026,0,137026,343.0550148487091,6.841555453601123e-05
27528,137531,0,137531,344.2509171962738,6.766803018466e-05
27628,138031,0,138031,345.36024618148804,6.693574791512647e-05
27728,138531,0,138531,346.46640515327454,6.621359794780738e-05
27828,139031,0,139031,347.5654022693634,6.550048252689829e-05
27928,139531,0,139531,348.6863172054291,6.47964029500481e-05
28028,140031,0,140031,349.78642320632935,6.41021997713222e-05
28128,140531,0,140531,350.9590232372284,6.341535689360674e-05
28228,141031,0,141031,352.2096121311188,6.27362524787659e-05
28328,141531,0,141531,353.37068223953247,6.206724113449434e-05
28428,142031,0,142031,354.50374603271484,6.140669338183834e-05
28529,142536,0,142536,355.6264362335205,6.074685561704041e-05
28629,143036,0,143036,356.7418580055237,6.010014450474079e-05
28729,143536,0,143536,357.8444890975952,5.946024030645318e-05
28829,144036,0,144036,359.020467042923,5.8827617649597955e-05
28929,144536,0,144536,360.1247491836548,5.8200998472433624e-05
29029,145036,0,145036,361.262971162796,5.7580150303739074e-05
29129,145536,0,145536,362.36615085601807,5.696491601605392e-05
29229,146036,0,146036,363.48220205307007,5.635382166322748e-05
29329,146536,0,146536,364.6006200313568,5.574845768244752e-05
29429,147036,0,147036,365.75716829299927,5.5148876508038447e-05
29530,147541,0,147541,366.8916952610016,5.454668860012277e-05
29630,148041,0,148041,368.1958529949188,5.395511398766742e-05
29730,148541,0,148541,369.394602060318,5.3369513084395924e-05
29830,149041,0,149041,370.50001096725464,5.278793963577943e-05
29930,149541,0,149541,371.60943698883057,5.221111654658672e-05
30030,150041,0,150041,372.7125220298767,5.164013549641547e-05
30130,150541,0,150541,373.81547713279724,5.107447867883836e-05
30230,151041,0,151041,374.90629601478577,5.051551635517621e-05
30330,151541,0,151541,376.00977897644043,4.996345977756957e-05
30430,152041,0,152041,377.1147041320801,4.9417322109135715e-05
30531,152546,0,152546,378.22979521751404,4.8873001649191144e-05
30631,153046,0,153046,379.3265149593353,4.834182106417658e-05
30731,153546,0,153546,380.42329597473145,4.781706619897961e-05
30831,154046,0,154046,381.52603006362915,4.7299173016522024e-05
30931,154546,0,154546,382.6278142929077,4.678882397764038e-05
31031,155046,0,155046,383.71620512008667,4.6285255072989336e-05
31131,155546,0,155546,384.8272111415863,4.5787709052220686e-05
31231,156046,0,156046,385.91948413848877,4.5296705020198724e-05
31331,156546,0,156546,387.02377820014954,4.481258660975853e-05
31431,157046,0,157046,388.18974709510803,4.4334317480227565e-05
31532,157551,0,157551,389.43935799598694,4.3856803884512845e-05
31632,158051,0,158051,390.6116752624512,4.3389859810586404e-05
31732,158551,0,158551,391.7695748806,4.292810598805867e-05
31832,159051,0,159051,393.0380349159241,4.247120840025504e-05
31932,159551,0,159551,394.16399788856506,4.201923426372581e-05
32032,160051,0,160051,395.45793318748474,4.157134146272643e-05
32132,160551,0,160551,396.6441011428833,4.1127112315303414e-05
32232,161051,0,161051,397.82328701019287,4.0687236378794365e-05
32332,161551,0,161551,398.98485708236694,4.0251435204314086e-05
32432,162051,0,162051,400.14693808555603,3.981927041455882e-05
32533,162556,0,162556,401.3103759288788,3.938671245407388e-05
32633,163056,0,163056,402.4476249217987,3.8962296806084434e-05
32733,163556,0,163556,403.70908403396606,3.8541840517381724e-05
32833,164056,0,164056,404.925833940506,3.8125571125778e-05
32933,164556,0,164556,406.1161060333252,3.77137137044239e-05
33033,165056,0,165056,407.3067798614502,3.730651175474961e-05
33133,165556,0,165556,408.6058192253113,3.690387241427071e-05
33233,166056,0,166056,409.7139341831207,3.6506091315853715e-05
33333,166556,0,166556,410.819699048996,3.611349689655464e-05
33433,167056,0,167056,411.9143600463867,3.572614335949348e-05
33534,167561,0,167561,413.02788519859314,3.534042359211925e-05
33634,168061,0,168061,414.140593290329,3.496377120346445e-05
33734,168561,0,168561,415.40378308296204,3.459184043731972e-05
33834,169061,0,169061,416.6263520717621,3.422499397078352e-05
33934,169561,0,169561,417.7780559062958,3.3863431683571225e-05
34034,170061,0,170061,418.88633608818054,3.350619492469981e-05
34134,170561,0,170561,420.140114068985,3.3152904294663406e-05
34234,171061,0,171061,421.3447461128235,3.280382950337981e-05
34334,171561,0,171561,422.40831422805786,3.2458523992637095e-05
34434,172061,0,172061,423.59988713264465,3.211653296004344e-05
34535,172566,0,172566,424.7572650909424,3.1774177407125385e-05
34635,173066,0,173066,425.8721332550049,3.1437892288382413e-05
34735,173566,0,173566,426.9955220222473,3.1104364938236076e-05
34835,174066,0,174066,428.1071779727936,3.0773635760124096e-05
34935,174566,0,174566,429.20178627967834,3.044529487963321e-05
35035,175066,0,175066,430.3812119960785,3.0119233678843722e-05
35135,175566,0,175566,431.53869915008545,2.9795992019045267e-05
35235,176066,0,176066,432.6748080253601,2.947575054294454e-05
35335,176566,0,176566,433.771931886673,2.915824954069372e-05
35435,177066,0,177066,434.906023979187,2.8843605479757906e-05
35536,177571,0,177571,436.02695202827454,2.852901007438208e-05
35636,178071,0,178071,437.13678216934204,2.8220720793562377e-05
35736,178571,0,178571,438.24673199653625,2.7915647927604747e-05
35836,179071,0,179071,439.36513209342957,2.7614011920278146e-05
35936,179571,0,179571,440.453910112381,2.7315891781905105e-05
36036,180071,0,180071,441.56283712387085,2.7021301315368236e-05
36136,180571,0,180571,442.6819839477539,2.6730381151970066e-05
36236,181071,0,181071,443.80851006507874,2.64431347746308e-05
36336,181567,0,181567,444.9054489135742,2.4758139166353404e-05
36436,182067,0,182067,446.13187193870544,2.4469446948454398e-05
36537,182572,0,182572,447.40120911598206,2.4184550018347918e-05
36637,183072,0,183072,448.5311322212219,2.3904667681089315e-05
36737,183572,0,183572,449.66693210601807,2.3630675006035834e-05
36837,184072,0,184072,450.9198820590973,2.336107354573459e-05
36937,184572,0,184572,452.0492310523987,2.3093597436580734e-05
37037,185072,0,185072,453.14620327949524,2.2830130498251928e-05
37137,185572,0,185572,454.2426931858063,2.2571112477224215e-05
37237,186072,0,186072,455.39273715019226,2.2315598689357874e-05
37337,186572,0,186572,456.7113561630249,2.2062388797824966e-05
37437,187072,0,187072,458.0724730491638,2.1811888098543773e-05
37538,187577,0,187577,459.56900215148926,2.1563625478502556e-05
37638,188077,0,188077,460.6954290866852,2.1320250500516268e-05
37738,188577,0,188577,461.84151816368103,2.107872049068823e-05
37838,189077,0,189077,463.3122401237488,2.084160383876619e-05
37938,189577,0,189577,464.6571829319,2.060663066464926e-05
38038,190077,0,190077,466.1898310184479,2.0372314453985773e-05
38138,190577,0,190577,467.66381907463074,2.014342031196946e-05
38238,191077,0,191077,468.868243932724,1.9916955741012533e-05
38338,191577,0,191577,470.0531499385834,1.9691330357419506e-05
38438,192077,0,192077,471.22212505340576,1.947050083882645e-05
38539,192582,0,192582,472.67108607292175,1.924966067524094e-05
38639,193082,0,193082,473.829430103302,1.903288005243698e-05
38739,193582,0,193582,475.1398551464081,1.8821127446457076e-05
38839,194082,0,194082,476.49254298210144,1.861171809428198e-05
38939,194582,0,194582,477.6452660560608,1.8404191265212173e-05
39039,195082,0,195082,479.0962071418762,1.8200850302727075e-05
39139,195582,0,195582,480.26216411590576,1.800075789666051e-05
39239,196082,0,196082,481.73844504356384,1.7802422524324302e-05
39339,196582,0,196582,483.19166707992554,1.7607417973754064e-05
39439,197082,0,197082,484.4575791358948,1.74156142538411e-05
39540,197587,0,197587,485.99728202819824,1.7224118202948158e-05
39640,198087,0,198087,487.11669993400574,1.7037157341547638e-05
39740,198587,0,198587,488.4004611968994,1.6852511050901508e-05
39840,199087,0,199087,489.82164192199707,1.6670016156615018e-05
39940,199587,0,199587,490.928111076355,1.6489118675185517e-05
40040,200087,0,200087,492.0403730869293,1.631086879528157e-05
40140,200587,0,200587,493.1430780887604,1.61352835984699e-05
40240,201087,0,201087,494.33528304100037,1.596035824198345e-05
40340,201587,0,201587,495.5726180076599,1.578714394595393e-05
40440,202087,0,202087,496.6937780380249,1.561610088306341e-05
40541,202592,0,202592,497.8550579547882,1.5444942817258926e-05
40641,203092,0,203092,498.96627616882324,1.5277682043544248e-05
40741,203592,0,203592,500.0883550643921,1.511214688382398e-05
40841,204092,0,204092,501.42877221107483,1.4947787394190242e-05
40941,204592,0,204592,502.6802680492401,1.4784939211747223e-05
41041,205092,0,205092,503.86689710617065,1.4624214532359079e-05
41141,205592,0,205592,505.3698959350586,1.446558141684178e-05
41241,206092,0,206092,506.62630915641785,1.430869176679836e-05
41341,206592,0,206592,507.78914618492126,1.4153384217204847e-05
41441,207092,0,207092,509.14081621170044,1.400006063232184e-05
41542,207597,0,207597,510.4381241798401,1.3847053831841963e-05
41642,208097,0,208097,512.0749409198761,1.369756240558973e-05
41742,208597,0,208597,513.5662100315094,1.35506180790394e-05
41842,209097,0,209097,514.7336041927338,1.3405192571801446e-05
41942,209597,0,209597,516.0427210330963,1.32609326834922e-05
42042,210097,0,210097,517.3415009975433,1.3119066120366419e-05
42142,210597,0,210597,518.7288720607758,1.297907002693116e-05
42242,211097,0,211097,520.1692962646484,1.2840392779078467e-05
42342,211597,0,211597,521.3566892147064,1.2703684297929615e-05
42442,212097,0,212097,522.5749711990356,1.2568365212262749e-05
42543,212602,0,212602,524.1707429885864,1.2432700312574631e-05
42643,213102,0,213102,525.5208430290222,1.2300135104970066e-05
42743,213602,0,213602,526.7800760269165,1.2168930976972997e-05
42843,214102,0,214102,528.101722240448,1.2038432346894075e-05
42943,214602,0,214602,529.1917371749878,1.190922197178555e-05
43043,215102,0,215102,530.2155709266663,1.1781110989271377e-05
43143,215602,0,215602,531.330225944519,1.165367766608862e-05
43243,216102,0,216102,532.607565164566,1.1527504201565588e-05
43343,216602,0,216602,534.0210120677948,1.1402599783942539e-05
43443,217102,0,217102,535.4736812114716,1.1278615848864776e-05
43544,217607,0,217607,536.7904171943665,1.1154699707662718e-05
43644,218107,0,218107,537.9828369617462,1.1033741065935602e-05
43744,218607,0,218607,539.3387341499329,1.0913911730099933e-05
43844,219107,0,219107,540.7572391033173,1.079504229435253e-05
43944,219607,0,219607,541.9644842147827,1.0677788708144172e-05
44044,220107,0,220107,543.3072640895844,1.056202118274933e-05
44144,220607,0,220607,544.7767701148987,1.0447523140499555e-05
44244,221107,0,221107,546.2127890586853,1.033445795302614e-05
44344,221607,0,221607,547.4186842441559,1.0222578304510024e-05
44444,222107,0,222107,548.6016340255737,1.0111783868246907e-05
44545,222612,0,222612,550.0508270263672,1.0001498870790633e-05
44645,223112,0,223112,551.2722780704498,9.893952869875802e-06
44745,223612,0,223612,552.6659409999847,9.787657129104306e-06
44845,224112,0,224112,553.9673020839691,9.68257563538978e-06
44945,224612,0,224612,555.337159872055,9.578706777845712e-06
45045,225112,0,225112,556.5738251209259,9.476125578111888e-06
45145,225612,0,225612,557.8944320678711,9.374897006080215e-06
45245,226112,0,226112,559.1110031604767,9.274821855774882e-06
45345,226612,0,226612,560.355978012085,9.175674678850745e-06
45445,227112,0,227112,561.7197189331055,9.077296727833068e-06
45546,227617,0,227617,562.9068269729614,8.978814620662631e-06
45646,228117,0,228117,564.3138749599457,8.882527169408377e-06
45746,228617,0,228617,565.7685790061951,8.787227697704095e-06
45846,229117,0,229117,567.3318920135498,8.692570000329447e-06
45946,229617,0,229617,569.1224598884583,8.598733243853218e-06
46046,230117,0,230117,570.732990026474,8.505680711096603e-06
46146,230617,0,230617,571.9922111034393,8.413416227556367e-06
46246,231117,0,231117,573.3036210536957,8.322285798499552e-06
46346,231617,0,231617,574.7364768981934,8.232094221539659e-06
46446,232117,0,232117,575.9339289665222,8.142510877800837e-06
46547,232622,0,232622,577.4758882522583,8.053018364660047e-06
46647,233122,0,233122,578.7865509986877,7.965549155284193e-06
46747,233622,0,233622,580.0548889636993,7.879072191243845e-06
46847,234122,0,234122,581.7701930999756,7.793759723184333e-06
46947,234622,0,234622,583.3120901584625,7.709576091986175e-06
47047,235122,0,235122,585.1055092811584,7.626335744686339e-06
47147,235622,0,235622,586.4364020824432,7.544207552546298e-06
47247,236122,0,236122,587.9403269290924,7.463289250335407e-06
47347,236622,0,236622,589.436517238617,7.383386638930977e-06
47447,237122,0,237122,590.895565032959,7.304460610108644e-06
47548,237627,0,237627,592.200010061264,7.225792707767383e-06
47648,238127,0,238127,593.4756910800934,7.14884092621591e-06
47748,238627,0,238627,594.9542169570923,7.072793744541637e-06
47848,239127,0,239127,596.4605782032013,6.9976511787271436e-06
47948,239627,0,239627,597.6695930957794,6.923314425945499e-06
48048,240127,0,240127,599.1140029430389,6.849790007182898e-06
48148,240627,0,240627,600.551351070404,6.777201605451543e-06
48248,241127,0,241127,602.184112071991,6.705407334108922e-06
48348,241627,0,241627,603.6099870204926,6.634146783057482e-06
48448,242127,0,242127,605.1305811405182,6.563493932586385e-06
48549,242632,0,242632,606.3585002422333,6.492886823556212e-06
48649,243132,0,243132,607.4993751049042,6.423674063546567e-06
48749,243632,0,243632,608.6822011470795,6.355112350079974e-06
48849,244132,0,244132,609.9928300380707,6.28709163586412e-06
48949,244632,0,244632,611.1296110153198,6.219529692078332e-06
49049,245132,0,245132,612.1762969493866,6.152609529540781e-06
49149,245632,0,245632,613.2930839061737,6.086510876243468e-06
49249,246132,0,246132,614.4515080451965,6.0211948925853215e-06
49349,246632,0,246632,615.6385731697083,5.956518357559711e-06
49449,247132,0,247132,616.8118500709534,5.89244063486401e-06
49550,247637,0,247637,618.0155708789825,5.828433434927389e-06
49650,248137,0,248137,619.2043631076813,5.765914393117245e-06
49750,248637,0,248637,620.4580931663513,5.704284944771898e-06
49850,249137,0,249137,621.8597140312195,5.643427604310878e-06
49950,249637,0,249637,623.030601978302,5.583230683097488e-06
50050,250137,0,250137,624.2044270038605,5.523685846079038e-06
50150,250637,0,250637,625.4220752716064,5.4649257358620515e-06
50250,251137,0,251137,626.8180379867554,5.406970412073335e-06
50350,251637,0,251637,628.2238001823425,5.349641367533867e-06
50450,252137,0,252137,629.602462053299,5.292879735346801e-06
50551,252642,0,252642,631.085942029953,5.236121298926422e-06
50651,253142,0,253142,632.3479082584381,5.180442810130622e-06
50751,253642,0,253642,633.7183170318604,5.125309556299008e-06
50851,254142,0,254142,634.9585840702057,5.070704491540264e-06
50951,254642,0,254642,636.180006980896,5.016512455800144e-06
51051,255142,0,255142,637.3791260719299,4.962734851058347e-06
51151,255642,0,255642,638.9390542507172,4.909446702543266e-06
51251,256142,0,256142,640.076336145401,4.856630884357071e-06
51351,256642,0,256642,641.2633411884308,4.804292390243072e-06
51451,257142,0,257142,642.4672420024872,4.752458312717086e-06
51552,257647,0,257647,643.6414220333099,4.700579900590139e-06
51652,258147,0,258147,644.8333592414856,4.649687520125507e-06
51752,258647,0,258647,646.0264592170715,4.5993004555764e-06
51852,259147,0,259147,647.5063440799713,4.54938739374054e-06
51952,259647,0,259647,648.6776130199432,4.499935824229093e-06
52052,260147,0,260147,649.997040271759,4.451000921406495e-06
52152,260647,0,260647,651.2552120685577,4.402613685668961e-06
52252,261147,0,261147,652.4635081291199,4.354763297578256e-06
52352,261647,0,261647,653.7326469421387,4.307472928879753e-06
52452,262147,0,262147,655.094722032547,4.260760688189293e-06
52553,262652,0,262652,656.2899420261383,4.214178224397701e-06
52653,263152,0,263152,657.4762830734253,4.168719244035852e-06
52753,263652,0,263652,658.7085950374603,4.123926758411941e-06
52853,264152,0,264152,659.9352209568024,4.07968454676253e-06
52953,264652,0,264652,661.1873750686646,4.035936273349656e-06
53053,265152,0,265152,662.6879460811615,3.992730931437731e-06
53153,265652,0,265652,663.8382489681244,3.950083229128714e-06
53253,266152,0,266152,664.9742422103882,3.907970731733579e-06
53353,266652,0,266652,666.2713451385498,3.866339973221415e-06
53453,267152,0,267152,667.4203140735626,3.825107616081232e-06
53554,267657,0,267657,668.8276031017303,3.783854811990382e-06
53654,268157,0,268157,670.1129860877991,3.7434435340904455e-06
53754,268657,0,268657,671.2189040184021,3.70348029452732e-06
53854,269157,0,269157,672.3195662498474,3.6639227884685946e-06
53954,269657,0,269657,673.485405921936,3.624702255017439e-06
54054,270157,0,270157,674.6021802425385,3.585800921864586e-06
54154,270657,0,270657,675.7524642944336,3.547256348220438e-06
54254,271157,0,271157,676.9088032245636,3.5091020479121405e-06
54354,271657,0,271657,678.0899262428284,3.4713340217678622e-06
54454,272157,0,272157,679.2746822834015,3.43392024959705e-06
54555,272662,0,272662,680.4837760925293,3.3964697104966667e-06
54655,273162,0,273162,681.6685838699341,3.3597691136665096e-06
54755,273662,0,273662,682.8344540596008,3.3235108893186466e-06
54855,274162,0,274162,684.0618412494659,3.2876922516835745e-06
54955,274662,0,274662,685.1641721725464,3.252291008176687e-06
55055,275162,0,275162,686.2957921028137,3.217302299311481e-06
55155,275662,0,275662,687.4388899803162,3.1827223493908774e-06
55255,276162,0,276162,688.6692910194397,3.1485724731475995e-06
55355,276662,0,276662,689.8090550899506,3.11486951630993e-06
55455,277162,0,277162,691.0313301086426,3.0815865990125865e-06
55556,277667,0,277667,692.4643530845642,3.048375143167118e-06
55656,278167,0,278167,693.8435909748077,3.015903328397608e-06
55756,278667,0,278667,695.0714020729065,2.983845248792869e-06
55856,279167,0,279167,696.3174510002136,2.9521879575373566e-06
55956,279667,0,279667,697.7693231105804,2.9209188025561865e-06
56056,280167,0,280167,699.5180361270905,2.8900172442733567e-06
56156,280667,0,280667,701.106761932373,2.8594576786021798e-06
56256,281167,0,281167,702.3628122806549,2.829224517237732e-06
56356,281667,0,281667,703.8369920253754,2.7992897396153717e-06
56456,282167,0,282167,705.1463899612427,2.769612752245971e-06
56557,282672,0,282672,706.500214099884,2.739887156767084e-06
56657,283172,0,283172,707.7341680526733,2.710712553700366e-06
56757,283672,0,283672,709.0301020145416,2.6817900837441286e-06
56857,284172,0,284172,710.2775540351868,2.6531072069180945e-06
56957,284672,0,284672,711.5293231010437,2.624659963102356e-06
57057,285172,0,285172,712.8238871097565,2.596455687108258e-06
57157,285672,0,285672,714.1425909996033,2.5685278529025478e-06
57257,286172,0,286172,715.3020920753479,2.5409120285667194e-06
57357,286672,0,286672,716.5518610477448,2.513597678007661e-06
57457,287172,0,287172,717.8724591732025,2.4865542317522048e-06
57558,287677,0,287677,719.2196769714355,2.4595210038146708e-06
57658,288177,0,288177,720.484857082367,2.4330650476121033e-06
57758,288677,0,288677,721.776330947876,2.4069395385034546e-06
57858,289177,0,289177,722.9995710849762,2.3811411544842593e-06
57958,289677,0,289677,724.2573821544647,2.355642481194301e-06
58058,290177,0,290177,725.607017993927,2.3304266351697466e-06
58158,290677,0,290677,727.0561451911926,2.305507406843027e-06
58258,291177,0,291177,728.4293241500854,2.2809041912074893e-06
58358,291677,0,291677,730.0410740375519,2.2566101276976258e-06
58458,292177,0,292177,731.1794831752777,2.232591363131543e-06
58559,292682,0,292682,732.4047412872314,2.2085802823311447e-06
58659,293182,0,293182,733.711837053299,2.18504535220302e-06
58759,293682,0,293682,735.0189161300659,2.1617560171912653e-06
58859,294182,0,294182,736.4402911663055,2.138715567453138e-06
58959,294682,0,294682,737.5500569343567,2.115910359983238e-06
59059,295182,0,295182,738.672749042511,2.0933188463638463e-06
59159,295682,0,295682,739.8101010322571,2.070932134942229e-06
59259,296182,0,296182,740.9286830425262,2.0487537693900075e-06
59359,296682,0,296682,742.0417320728302,2.0267769814991227e-06
59459,297182,0,297182,743.1364369392395,2.0049843102786204e-06
59560,297687,0,297687,744.275778055191,1.983154072163781e-06
59660,298187,0,298187,745.4090020656586,1.9617197432343142e-06
59760,298687,0,298687,746.5111691951752,1.940465844698492e-06
59860,299187,0,299187,747.613970041275,1.919398664091869e-06
59960,299687,0,299687,748.7269592285156,1.8985245914405751e-06
60060,300187,0,300187,749.8192069530487,1.8778517757200504e-06
60160,300687,0,300687,750.9204621315002,1.8573968346508762e-06
60260,301187,0,301187,752.0272481441498,1.8371758450952007e-06
60360,301687,0,301687,753.1747372150421,1.8171957321028884e-06
60460,302187,0,302187,754.3466281890869,1.7974622734397234e-06
60561,302692,0,302692,755.5574929714203,1.7777878963175178e-06
60661,303192,0,303192,756.7267861366272,1.7585629416855465e-06
60761,303692,0,303692,757.9780879020691,1.7395915348907301e-06
60861,304192,0,304192,759.5097260475159,1.7208696471669597e-06
60961,304692,0,304692,760.6648828983307,1.7023852443145815e-06
61061,305192,0,305192,761.8683881759644,1.6841310014724146e-06
61161,305692,0,305692,762.9726221561432,1.666107461913062e-06
61261,306192,0,306192,764.1426281929016,1.648312293064047e-06
61361,306692,0,306692,765.3440041542053,1.6307369013636357e-06
61461,307192,0,307192,766.6034359931946,1.6133699854806846e-06
61562,307697,0,307697,767.8217039108276,1.596030097821916e-06
61662,308197,0,308197,768.9660580158234,1.5790546241561168e-06
61762,308697,0,308697,770.2983989715576,1.56226855175351e-06
61862,309197,0,309197,771.380392074585,1.5456617706098238e-06
61962,309697,0,309697,772.3771729469299,1.5292151046108995e-06
62062,310197,0,310197,773.9125680923462,1.5129155286745008e-06
62162,310697,0,310697,775.2344450950623,1.4967636708336828e-06
62262,311197,0,311197,776.4098889827728,1.4807653824030726e-06
62362,311697,0,311697,777.9692978858948,1.4649224020491598e-06
62462,312197,0,312197,779.035001039505,1.4492310340943158e-06
62563,312702,0,312702,780.2772641181946,1.4335322534561939e-06
62663,313202,0,313202,781.4909110069275,1.4181384309461403e-06
62763,313702,0,313702,782.7617359161377,1.4029015400270456e-06
62863,314202,0,314202,783.9474971294403,1.3878284588765156e-06
62963,314702,0,314702,785.1676530838013,1.372917683004314e-06
63063,315202,0,315202,786.522607088089,1.3581651685270229e-06
63163,315702,0,315702,787.9034571647644,1.343574266252901e-06
63263,316202,0,316202,789.2312331199646,1.3291535375019734e-06
63363,316702,0,316702,790.6810302734375,1.3149102227338883e-06
63463,317202,0,317202,792.4052650928497,1.300847728933644e-06
63564,317707,0,317707,793.6700432300568,1.2868271288751973e-06
63664,318207,0,318207,795.028017282486,1.273124112667211e-06
63764,318707,0,318707,796.1452040672302,1.2595983232861884e-06
63864,319207,0,319207,797.2306351661682,1.246245674252732e-06
63964,319707,0,319707,798.5016980171204,1.2330560630652104e-06
64064,320207,0,320207,799.7373292446136,1.220017727777629e-06
64164,320707,0,320707,801.1655292510986,1.2071203141340176e-06
64264,321207,0,321207,802.4481720924377,1.1943543120133008e-06
64364,321707,0,321707,803.6061880588531,1.1817107691135147e-06
64464,322207,0,322207,804.7187671661377,1.1691810338006463e-06
64565,322712,0,322712,805.8359370231628,1.1566347794900402e-06
64665,323212,0,323212,806.9315211772919,1.1443183832653459e-06
64765,323712,0,323712,808.0164921283722,1.1321079286975326e-06
64865,324212,0,324212,809.1929879188538,1.1200035742706644e-06
64965,324712,0,324712,810.4263648986816,1.1080049605588141e-06
65065,325212,0,325212,811.6726689338684,1.096113182685053e-06
65165,325712,0,325712,812.971687078476,1.0843296767510358e-06
65265,326212,0,326212,814.269366979599,1.0726561183002456e-06
65365,326712,0,326712,815.7760078907013,1.061095014062317e-06
65465,327212,0,327212,817.1639502048492,1.0496470246169862e-06
65566,327717,0,327717,818.5193231105804,1.0381999563225477e-06
65666,328217,0,328217,819.728935956955,1.0269847576143703e-06
65766,328717,0,328717,820.9627850055695,1.0158925689194452e-06
65866,329217,0,329217,822.1954131126404,1.0049259481510315e-06
65966,329717,0,329717,823.3959438800812,9.940855267346418e-07
66066,330217,0,330217,824.8061690330505,9.833719876582508e-07
66166,330717,0,330717,826.0516889095306,9.727880520583622e-07
66266,331217,0,331217,827.1310141086578,9.623374351265779e-07
66366,331717,0,331717,828.5359020233154,9.520207180885351e-07
66466,332217,0,332217,829.8170540332794,9.418336128162383e-07
66567,332722,0,332722,831.1911280155182,9.316700240749915e-07
66667,333222,0,333222,832.4936230182648,9.217271623936702e-07
66767,333722,0,333722,833.8469939231873,9.11900973918843e-07
66867,334222,0,334222,835.01664686203,9.021860095887457e-07
66967,334722,0,334722,836.3188381195068,8.925742305820325e-07
67067,335222,0,335222,837.9499042034149,8.830583492669215e-07
67167,335722,0,335722,839.3354511260986,8.736334425874546e-07
67267,336222,0,336222,840.7900710105896,8.642967840073961e-07
67367,336722,0,336722,842.2618980407715,8.550463039981891e-07
67467,337222,0,337222,843.6369421482086,8.458785940951659e-07
67568,337727,0,337727,844.939572095871,8.366993440625389e-07
67668,338227,0,338227,846.3133561611176,8.27688677308282e-07
67768,338727,0,338727,847.7448298931122,8.18755980318171e-07
67868,339227,0,339227,848.8757572174072,8.099026085895654e-07
67968,339727,0,339727,850.1825132369995,8.011302377917576e-07
68068,340227,0,340227,851.5032961368561,7.924414715768279e-07
68168,340727,0,340727,852.7664840221405,7.838404281018891e-07
68268,341227,0,341227,853.9650990962982,7.753324173023301e-07
68368,341727,0,341727,855.1945641040802,7.669213846430057e-07
68468,342227,0,342227,856.3974311351776,7.586078537484956e-07
68569,342732,0,342732,857.7091052532196,7.503095311112588e-07
68669,343232,0,343232,859.1275510787964,7.421920083133684e-07
68769,343732,0,343732,860.2548019886017,7.34174652470198e-07
68869,344232,0,344232,861.4629671573639,7.262580664381888e-07
68969,344732,0,344732,862.5710980892181,7.184413830674902e-07
69069,345232,0,345232,863.6713888645172,7.107234815614449e-07
69169,345732,0,345732,864.7739901542664,7.031041351747459e-07
69269,346232,0,346232,866.1137421131134,6.955832124596854e-07
69369,346732,0,346732,867.3621790409088,6.881590632382932e-07
69469,347232,0,347232,868.5072388648987,6.80828915953804e-07
69570,347737,0,347737,869.6841771602631,6.735181579151269e-07
69670,348237,0,348237,870.8883509635925,6.663685179595736e-07
69770,348737,0,348737,872.0507090091705,6.593027248894223e-07
69870,349237,0,349237,873.1298530101776,6.523151435487793e-07
69970,349737,0,349737,874.348197221756,6.454002002365713e-07
70070,350237,0,350237,875.5348181724548,6.385538337749787e-07
70170,350737,0,350737,876.8410220146179,6.317739874753919e-07
70270,351237,0,351237,878.1292741298676,6.250590924957788e-07
70370,351737,0,351737,879.5745780467987,6.18406469376686e-07
70470,352237,0,352237,880.8100821971893,6.118130803177087e-07
70571,352742,0,352742,881.9977641105652,6.052126087688966e-07
70671,353242,0,353242,883.3625910282135,5.987371272322172e-07
70771,353742,0,353742,884.7426512241364,5.923232533738532e-07
70871,354242,0,354242,886.0685188770294,5.859719379929252e-07
70971,354742,0,354742,887.6396610736847,5.79682969630108e-07
71071,355242,0,355242,888.7544991970062,5.734572256210388e-07
71171,355742,0,355742,889.9984481334686,5.672980778254223e-07
71271,356242,0,356242,891.528430223465,5.612100452919797e-07
71371,356742,0,356742,892.8338010311127,5.551961002915604e-07
71471,357242,0,357242,894.2078430652618,5.492566417481415e-07
71572,357747,0,357747,895.3448770046234,5.433325783386095e-07
71672,358247,0,358247,896.5125141143799,5.375405726517072e-07
71772,358747,0,358747,897.6940412521362,5.31820978206146e-07
71872,359247,0,359247,898.8109750747681,5.261721461709098e-07
71972,359747,0,359747,899.946475982666,5.205905248497584e-07
72072,360247,0,360247,901.1907262802124,5.150714020625476e-07
72172,360747,0,360747,902.3855590820312,5.096110004691253e-07
72272,361247,0,361247,903.6012489795685,5.042072646492409e-07
72372,361747,0,361747,904.9967851638794,4.988586021967168e-07
72472,362247,0,362247,906.4272162914276,4.935628346604749e-07
72573,362752,0,362752,907.6680572032928,4.882654528657139e-07
72673,363252,0,363252,909.1285061836243,4.830696874710901e-07
72773,363752,0,363752,910.2853510379791,4.779217151643314e-07
72873,364252,0,364252,911.7562811374664,4.7282023909427746e-07
72973,364752,0,364752,913.8338840007782,4.677634359780377e-07
73073,365252,0,365252,915.5222232341766,4.6274950986825224e-07
73173,365752,0,365752,917.3557231426239,4.5777760280808976e-07
73273,366252,0,366252,919.2206149101257,4.5284780451463425e-07
73373,366752,0,366752,920.8000400066376,4.4796048281614885e-07
73473,367252,0,367252,922.6352829933167,4.431161211775417e-07
73574,367757,0,367757,924.2834870815277,4.382679443680102e-07
73674,368257,0,368257,925.9735641479492,4.335138917638465e-07
73774,368757,0,368757,927.7830860614777,4.28808411545749e-07
73874,369257,0,369257,929.2755930423737,4.241540818848665e-07
73974,369757,0,369757,931.1942729949951,4.1955297033080294e-07
74074,370257,0,370257,932.6176381111145,4.1500699046842446e-07
74174,370757,0,370757,933.995364189148,4.1051775539140377e-07
74274,371257,0,371257,935.3330659866333,4.0608577355642756e-07
74374,371757,0,371757,936.7164940834045,4.0171017541439516e-07
74474,372257,0,372257,938.1453161239624,3.97389361630678e-07
74575,372762,0,372762,939.5851151943207,3.930795785906087e-07
74675,373262,0,373262,941.2376089096069,3.8886555044741166e-07
74775,373762,0,373762,942.7373330593109,3.847038269104982e-07
74875,374262,0,374262,944.8398399353027,3.805928897538682e-07
74975,374762,0,374762,946.4137001037598,3.765300579367665e-07
75075,375262,0,375262,947.932361125946,3.7251254896109623e-07
75175,375762,0,375762,949.5506980419159,3.6853859679069454e-07
75275,376262,0,376262,950.8452560901642,3.6460725536611033e-07
75375,376762,0,376762,952.3972039222717,3.607170845970729e-07
75475,377262,0,377262,953.7450549602509,3.568654882258914e-07
75576,377767,0,377767,955.127965927124,3.5301169792769407e-07
75676,378267,0,378267,956.3969552516937,3.492306163246594e-07
75776,378767,0,378767,957.6851599216461,3.454842474717345e-07
75876,379267,0,379267,958.9495980739594,3.417733468821678e-07
75976,379767,0,379767,960.2265720367432,3.380977784564849e-07
76076,380267,0,380267,961.5105290412903,3.3445678396509216e-07
76176,380767,0,380767,962.7736341953278,3.308502241693137e-07
76276,381267,0,381267,964.0410890579224,3.2727904260973124e-07
76376,381767,0,381767,965.3070380687714,3.237445262706469e-07
76476,382267,0,382267,966.6593432426453,3.202473806887258e-07
76577,382772,0,382772,968.4219992160797,3.1675322385484505e-07
76677,383272,0,383272,969.8314712047577,3.1333142841406253e-07
76777,383772,0,383772,971.2163372039795,3.0994822648801524e-07
76877,384272,0,384272,972.6924481391907,3.066050600212221e-07
76977,384772,0,384772,974.1578528881073,3.0330295431052714e-07
77077,385272,0,385272,975.8345630168915,3.0004234658145314e-07
77177,385772,0,385772,977.39923620224,2.9682355758550837e-07
77277,386272,0,386272,979.0857059955597,2.936470343978693e-07
77377,386772,0,386772,980.7823450565338,2.90512900577482e-07
77477,387272,0,387272,982.5395820140839,2.874203035996396e-07
77578,387777,0,387777,984.6919181346893,2.8433710807050587e-07
77678,388277,0,388277,986.7006452083588,2.813223085813156e-07
77778,388777,0,388777,988.5044801235199,2.7834334007996905e-07
77878,389277,0,389277,989.9508941173553,2.753983415705869e-07
77978,389777,0,389777,991.5994391441345,2.724851945866657e-07
78078,390277,0,390277,993.3086750507355,2.69601786143182e-07
78178,390777,0,390777,994.9976019859314,2.667464765234163e-07
78278,391277,0,391277,996.9593873023987,2.6391813193734857e-07
78378,391777,0,391777,998.520268201828,2.6111566473942905e-07
78478,392277,0,392277,1000.2901840209961,2.58337802164423e-07
78579,392782,0,392782,1002.0880541801453,2.555561782408286e-07
78679,393282,0,393282,1003.7121760845184,2.528259361608583e-07
78779,393782,0,393782,1005.6193599700928,2.501203306519358e-07
78879,394282,0,394282,1007.3233091831207,2.474402599637395e-07
78979,394782,0,394782,1008.8062300682068,2.44786097395252e-07
79079,395282,0,395282,1010.2384760379791,2.4215808811323914e-07
79179,395782,0,395782,1011.660177230835,2.3955704003237335e-07
79279,396282,0,396282,1013.0586822032928,2.369843150730864e-07
79379,396782,0,396782,1014.4697642326355,2.3444098451284756e-07
79479,397282,0,397282,1015.9024691581726,2.319271164825373e-07
79580,397787,0,397787,1017.3222389221191,2.2941737371723322e-07
79680,398287,0,398287,1018.7383649349213,2.2696109624584757e-07
79780,398787,0,398787,1020.3676810264587,2.2453366048435663e-07
79880,399287,0,399287,1022.3726091384888,2.2213554443704942e-07
79980,399787,0,399787,1024.2603340148926,2.1976650649725233e-07
80080,400287,0,400287,1026.0705962181091,2.1742556138219275e-07
80180,400787,0,400787,1028.650446176529,2.151116692584531e-07
80280,401287,0,401287,1030.3638241291046,2.1282422158841604e-07
80380,401787,0,401787,1032.063333272934,2.105627699539956e-07
80480,402287,0,402287,1033.6501660346985,2.0832641849530947e-07
80581,402792,0,402792,1035.22500705719,2.0609165413513596e-07
80681,403292,0,403292,1036.8531498908997,2.0390105832040527e-07
80781,403792,0,403792,1038.736699104309,2.017310596775534e-07
80881,404292,0,404292,1040.3302111625671,1.9958071061103183e-07
80981,404792,0,404792,1041.9483880996704,1.974491858869539e-07
81081,405292,0,405292,1043.6014242172241,1.9533560406603796e-07
81181,405792,0,405792,1045.4311010837555,1.932391696408168e-07
81281,406292,0,406292,1047.0285680294037,1.9115949736179776e-07
81381,406792,0,406792,1048.5969669818878,1.8909673978364401e-07
81481,407292,0,407292,1050.1837491989136,1.8705140147130446e-07
81582,407797,0,407797,1051.805017232895,1.8500395611322046e-07
81682,408297,0,408297,1053.4021861553192,1.829957422257774e-07
81782,408797,0,408797,1054.9698412418365,1.8100733966442422e-07
81882,409297,0,409297,1056.5558788776398,1.7903970858366988e-07
81982,409797,0,409797,1058.1505391597748,1.7709361365501961e-07
82082,410297,0,410297,1059.7654480934143,1.7516956844360552e-07
82182,410797,0,410797,1061.3488171100616,1.732679994081638e-07
82282,411297,0,411297,1062.9395849704742,1.7138936428328358e-07
82382,411797,0,411797,1064.5247910022736,1.6953401577948357e-07
82482,412297,0,412297,1066.1033971309662,1.6770200626748427e-07
82583,412802,0,412802,1067.6997339725494,1.658751496211222e-07
82683,413302,0,413302,1069.290580034256,1.640893765127288e-07
82783,413802,0,413802,1070.8786671161652,1.6232634020806648e-07
82883,414302,0,414302,1072.4616770744324,1.605858293473245e-07
82983,414802,0,414802,1074.0512311458588,1.5886733224531213e-07
83083,415302,0,415302,1075.639983177185,1.571700695377117e-07
83183,415802,0,415802,1077.2212760448456,1.5549325045732196e-07
83283,416302,0,416302,1078.8043360710144,1.538361977149693e-07
83383,416802,0,416802,1080.4100461006165,1.5219817603018555e-07
83483,417302,0,417302,1082.0035572052002,1.5057818932078878e-07
83584,417807,0,417807,1083.5997860431671,1.489591377779871e-07
83684,418307,0,418307,1085.1817240715027,1.4737214785214525e-07
83784,418807,0,418807,1086.7700581550598,1.4580066753788848e-07
83884,419307,0,419307,1088.3592519760132,1.4424458891379322e-07
83984,419807,0,419807,1089.9345531463623,1.4270371127421584e-07
84084,420307,0,420307,1091.5313630104065,1.4117751928112094e-07
84184,420807,0,420807,1093.1178810596466,1.3966542322879032e-07
84284,421307,0,421307,1094.7311081886292,1.3816717373656054e-07
84384,421807,0,421807,1096.3240802288055,1.3668295928903521e-07
84484,422307,0,422307,1097.945808172226,1.352131078965057e-07
84585,422812,0,422812,1099.5643410682678,1.3374333530404756e-07
84685,423312,0,423312,1101.1429080963135,1.3230290905467397e-07
84785,423812,0,423812,1102.736577987671,1.3087764695245663e-07
84885,424312,0,424312,1104.4204270839691,1.2946836026184611e-07
84985,424812,0,424812,1106.1351101398468,1.280759217099276e-07
85085,425312,0,425312,1107.8310191631317,1.2670087325426363e-07
85185,425812,0,425812,1109.5269072055817,1.2534333765623355e-07
85285,426312,0,426312,1111.3066291809082,1.2400321172538125e-07
85385,426812,0,426812,1112.9040920734406,1.2268032333935662e-07
85485,427312,0,427312,1114.4855270385742,1.2137439402136777e-07
85586,427817,0,427817,1116.0740151405334,1.2007212121651653e-07
85686,428317,0,428317,1117.6682181358337,1.1879860492874518e-07
85786,428817,0,428817,1119.2727680206299,1.1754014370768598e-07
85886,429317,0,429317,1120.8516192436218,1.1629606350237402e-07
85986,429817,0,429817,1122.5073821544647,1.1506568257806039e-07
86086,430317,0,430317,1124.1513350009918,1.1384822756141683e-07
86186,430817,0,430817,1125.7959260940552,1.1264289975567055e-07
86286,431317,0,431317,1127.414796113968,1.1144904631032075e-07
86386,431817,0,431817,1128.9994912147522,1.1026622766645966e-07
86486,432317,0,432317,1130.621407032013,1.0909411811604476e-07
86587,432822,0,432822,1132.2306640148163,1.0792084519753453e-07
86687,433322,0,433322,1133.8134751319885,1.0676940440432179e-07
86787,433822,0,433822,1135.4172701835632,1.0562807228160408e-07
86887,434322,0,434322,1136.9975781440735,1.0449695369204678e-07
86987,434822,0,434822,1138.5855731964111,1.0337616993505784e-07
87087,435322,0,435322,1140.1556041240692,1.0226577602820133e-07
87187,435822,0,435822,1141.7396240234375,1.0116583872930589e-07
87287,436322,0,436322,1143.3182721138,1.0007656176555969e-07
87387,436822,0,436822,1144.9098958969116,9.899828792728952e-08
87487,437322,0,437322,1146.494590997696,9.79313684574609e-08
87588,437827,0,437827,1148.1045010089874,9.686557205223534e-08
87688,438327,0,438327,1149.68931722641,9.582223633488851e-08
87788,438827,0,438827,1151.2641341686249,9.479106385389852e-08
87888,439327,0,439327,1152.8641331195831,9.37724231224351e-08
87988,439827,0,439827,1154.457337141037,9.276654578127547e-08
88088,440327,0,440327,1156.0410749912262,9.177336598869574e-08
88188,440827,0,440827,1157.6006231307983,9.079255908547777e-08
88288,441327,0,441327,1159.1943318843842,8.982371127793521e-08
88388,441827,0,441827,1160.7793788909912,8.886641747962162e-08
88488,442327,0,442327,1162.3613948822021,8.792022357791811e-08
88589,442832,0,442832,1163.951495885849,8.697523106061668e-08
88689,443332,0,443332,1165.5525150299072,8.604946233965795e-08
88789,443832,0,443832,1167.132344007492,8.513290304670765e-08
88889,444332,0,444332,1168.6859872341156,8.422513737655318e-08
88989,444832,0,444832,1170.306384086609,8.33258908517979e-08
89089,445332,0,445332,1172.1851279735565,8.243490841931046e-08
89189,445832,0,445832,1173.7761180400848,8.155190875416452e-08
89289,446332,0,446332,1175.3497650623322,8.067664487432395e-08
89389,446832,0,446832,1176.9403901100159,7.980898052170264e-08
89489,447332,0,447332,1178.527932882309,7.89489005210313e-08
89590,447837,0,447837,1180.1413979530334,7.808798205228035e-08
89690,448337,0,448337,1181.742887020111,7.724338356573574e-08
89790,448837,0,448837,1183.330794095993,7.640670443715367e-08
89890,449337,0,449337,1184.9271869659424,7.557815897630344e-08
89990,449837,0,449837,1186.5108571052551,7.475798541877854e-08
90090,450337,0,450337,1188.0815312862396,7.394641513045673e-08
90190,450837,0,450837,1189.667550086975,7.314366529759329e-08
90290,451337,0,451337,1191.261766910553,7.234994511926245e-08
90390,451837,0,451837,1192.8410739898682,7.156545233708477e-08
90490,452337,0,452337,1194.432615995407,7.07903512866788e-08
90591,452842,0,452842,1196.0304062366486,7.001714492380071e-08
90691,453342,0,453342,1197.6096460819244,6.926120834847599e-08
90791,453842,0,453842,1199.1888101100922,6.851487782755482e-08
90891,454342,0,454342,1200.784882068634,6.777816971003707e-08
90991,454842,0,454842,1202.3526380062103,6.705103970488444e-08
91091,455342,0,455342,1203.914447069168,6.633334226418673e-08
91191,455842,0,455842,1205.4939231872559,6.562483866422212e-08
91291,456342,0,456342,1207.077977180481,6.49252524811353e-08
91391,456842,0,456842,1208.666519165039,6.42343104866385e-08
91491,457342,0,457342,1210.2492291927338,6.355172145956567e-08
91592,457847,0,457847,1211.8372721672058,6.287041737365335e-08
91692,458347,0,458347,1213.4085400104523,6.220344669719794e-08
91792,458847,0,458847,1214.989984035492,6.154356253289933e-08
91892,459347,0,459347,1216.551996231079,6.089033949338582e-08
91992,459847,0,459847,1218.1395750045776,6.024340524160767e-08
92092,460347,0,460347,1219.718641281128,5.9602437652332105e-08
92192,460847,0,460847,1221.3043801784515,5.8967191993712113e-08
92292,461347,0,461347,1222.8735330104828,5.833755447657805e-08
92392,461847,0,461847,1224.4757282733917,5.771356289967479e-08
92492,462347,0,462347,1226.057590007782,5.709535845468965e-08
92593,462852,0,462852,1227.6372311115265,5.6477015936762434e-08
92693,463352,0,463352,1229.2176880836487,5.5870934565764556e-08
92793,463852,0,463852,1230.8034081459045,5.5271121619224754e-08
92893,464352,0,464352,1232.4111471176147,5.467776851502992e-08
92993,464852,0,464852,1233.9784710407257,5.409107684263335e-08
93093,465352,0,465352,1235.5743391513824,5.3511198524894656e-08
93193,465852,0,465852,1237.1547572612762,5.2938198200698075e-08
93293,466352,0,466352,1238.7348201274872,5.237207621662884e-08
93393,466852,0,466852,1240.3060281276703,5.181281910158578e-08
93493,467352,0,467352,1241.8969662189484,5.126041202478091e-08
93594,467857,0,467857,1243.493881225586,5.070937672949822e-08
93694,468357,0,468357,1245.0592849254608,5.01704836030814e-08
93794,468857,0,468857,1246.6399500370026,4.9638021400772925e-08
93894,469357,0,469357,1248.2302031517029,4.9111728970494083e-08
93994,469857,0,469857,1249.8091831207275,4.85913450270099e-08
94094,470357,0,470357,1251.3814179897308,4.807661898807941e-08
94194,470857,0,470857,1252.9555351734161,4.756730471856346e-08
94294,471357,0,471357,1254.5765330791473,4.7063158869899435e-08
94394,471857,0,471857,1256.1558530330658,4.6563946765815976e-08
94494,472357,0,472357,1257.7291841506958,4.606944630958849e-08
94595,472862,0,472862,1259.3346712589264,4.557457024401372e-08
94695,473362,0,473362,1260.9222321510315,4.508892520046027e-08
94795,473862,0,473862,1262.4950630664825,4.4607430812461174e-08
94895,474362,0,474362,1264.0768041610718,4.412997718660471e-08
94995,474862,0,474862,1265.6605050563812,4.365650664513423e-08
95095,475362,0,475362,1267.470115184784,4.318700574747207e-08
95195,475862,0,475862,1269.1050810813904,4.272150611444266e-08
95295,476362,0,476362,1270.6918790340424,4.226010616267049e-08
95395,476862,0,476862,1272.2772579193115,4.1802989731364147e-08
95495,477362,0,477362,1273.8635420799255,4.135040698391273e-08
95596,477867,0,477867,1275.4421200752258,4.089816700860786e-08
95696,478367,0,478367,1277.0229880809784,4.0455448953385145e-08
95796,478867,0,478867,1278.6083211898804,4.001791203536293e-08
95896,479367,0,479367,1280.1899890899658,3.958565578190874e-08
95996,479867,0,479867,1281.7630190849304,3.9158716211616864e-08
96096,480367,0,480367,1283.3571269512177,3.87370660156384e-08
96196,480867,0,480867,1284.9581551551819,3.83206289114138e-08
96296,481367,0,481367,1286.5195109844208,3.790930486674825e-08
96396,481867,0,481867,1288.145518064499,3.750298885396706e-08
96496,482367,0,482367,1289.7459170818329,3.7101572269938415e-08
96597,482872,0,482872,1291.430762052536,3.670099122870077e-08
96697,483372,0,483372,1293.0140390396118,3.6309036831582725e-08
96797,483872,0,483872,1294.6020259857178,3.5921561709229526e-08
96897,484372,0,484372,1296.1947910785675,3.553839422848413e-08
96997,484872,0,484872,1297.7837541103363,3.5159347923588836e-08
97097,485372,0,485372,1299.3578329086304,3.4784222109441415e-08
97197,485872,0,485872,1300.9443500041962,3.441281657496174e-08
97297,486372,0,486372,1302.52738904953,3.4044959312246065e-08
97397,486872,0,486872,1304.0981419086456,3.368052747784616e-08
97497,487372,0,487372,1305.6792619228363,3.331944530141719e-08
97598,487877,0,487877,1307.2851340770721,3.295810436247961e-08
97698,488377,0,488377,1308.8756980895996,3.2603627596715596e-08
97798,488877,0,488877,1310.4458711147308,3.2252406392916555e-08
97898,489377,0,489377,1312.035521030426,3.1904452685634734e-08
97998,489877,0,489877,1313.6236779689789,3.1559805654004965e-08
98098,490377,0,490377,1315.2228360176086,3.121852230611505e-08
98198,490877,0,490877,1316.797294139862,3.0880668825624187e-08
98298,491377,0,491377,1318.3908851146698,3.054631967917101e-08
98398,491877,0,491877,1319.9855270385742,3.021555948709407e-08
98498,492377,0,492377,1321.5605518817902,2.9888480738356374e-08
98599,492882,0,492882,1323.153531074524,2.9561964792174407e-08
98699,493382,0,493382,1324.730191230774,2.9242572997470586e-08
98799,493882,0,493882,1326.3234610557556,2.892714749025802e-08
98899,494382,0,494382,1327.8999559879303,2.8615771893396364e-08
98999,494882,0,494882,1329.4905610084534,2.83084972401931e-08
99099,495382,0,495382,1331.0588071346283,2.8005320775437747e-08
99199,495882,0,495882,1332.6506271362305,2.770618214474585e-08
99299,496382,0,496382,1334.2306282520294,2.7410975683418705e-08
99399,496882,0,496882,1335.7188980579376,2.7119562772877072e-08
99499,497382,0,497382,1337.20174908638,2.683177513919919e-08
99600,497887,0,497887,1338.9910521507263,2.654458979816938e-08
99700,498387,0,498387,1340.5689561367035,2.6263480033161935e-08
99800,498887,0,498887,1342.2582149505615,2.598538006390332e-08
99900,499387,0,499387,1343.8986320495605,2.5710111389207502e-08
100000,499887,0,499887,1345.763931274414,2.543753277181282e-08


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/flex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002183198928833008,30.358106049564984
81,243,0,243,1.5511021614074707,0.3480833949950039
161,483,0,483,2.8602840900421143,0.1404995373723559
242,726,0,726,4.128584146499634,0.0657505266695044
323,969,0,969,5.4588141441345215,0.047872603732171684
404,1212,0,1212,6.717121124267578,0.040075349061280297
484,1452,0,1452,7.978608131408691,0.0349076173897176
565,1695,0,1695,9.15440320968628,0.027651117536782024
646,1938,0,1938,10.332130193710327,0.025409925734020556
726,2178,0,2178,11.478452205657959,0.0231275888349837
807,2421,0,2421,12.613002300262451,0.020163481540391753
888,2664,0,2664,13.759902238845825,0.0175729995196827
969,2907,0,2907,14.921958208084106,0.016525311952617056
1049,3147,0,3147,16.04424023628235,0.015535577115170254
1130,3390,0,3390,17.195394039154053,0.014592647167650692
1211,3633,0,3633,18.31826615333557,0.013980455794172727
1291,3873,0,3873,19.430898189544678,0.013197949521073149
1372,4116,0,4116,20.578806161880493,0.01176124001048875
1453,4359,0,4359,21.75723624229431,0.009922311591465031
1534,4602,0,4602,22.946632146835327,0.008414422846928291
1614,4842,0,4842,24.036660194396973,0.007605961060768524
1695,5085,0,5085,25.139055252075195,0.006937635577089381
1776,5328,0,5328,26.222589254379272,0.006305743416037854
1856,5568,0,5568,27.313225269317627,0.0058652162185436904
1937,5811,0,5811,28.428125143051147,0.0054911984702519295
2018,6054,0,6054,29.530946016311646,0.005194270247685958
2099,6297,0,6297,30.631890296936035,0.0049487176596587
2179,6537,0,6537,31.722941160202026,0.00475622538625983
2260,6780,0,6780,32.82115316390991,0.00430966740160458
2341,7023,0,7023,33.96980619430542,0.0037520236708764127
2421,7263,0,7263,35.05737614631653,0.0034737644520284163
2502,7506,0,7506,36.16252899169922,0.0033426259493403603
2583,7749,0,7749,37.258249282836914,0.0032097501407459526
2664,7992,0,7992,38.362269163131714,0.0030874382573407373
2744,8232,0,8232,39.528802156448364,0.0029493325518515677
2825,8475,0,8475,40.66103219985962,0.0028080108482399554
2906,8718,0,8718,41.77852511405945,0.0027087765236887096
2986,8958,0,8958,42.87853527069092,0.0026184777362827836
3067,9201,0,9201,43.98224925994873,0.002551425503315686
3148,9444,0,9444,45.102431297302246,0.0024903413663226
3229,9687,0,9687,46.20412635803223,0.0024307605944403916
3309,9927,0,9927,47.307706117630005,0.002340125866489356
3390,10170,0,10170,48.506089210510254,0.0022070913495341364
3471,10413,0,10413,49.713144063949585,0.0021438371877831697
3551,10653,0,10653,50.81929922103882,0.0020936678965963827
3632,10896,0,10896,51.95348310470581,0.002042137449285472
3713,11139,0,11139,53.07148814201355,0.0019933598396542664
3794,11382,0,11382,54.21267032623291,0.0019348643384052891
3874,11622,0,11622,55.31523609161377,0.0018941166766654426
3955,11865,0,11865,56.447652101516724,0.0018347022448073828
4036,12108,0,12108,57.58098316192627,0.0017933055308741582
4117,12351,0,12351,58.70805907249451,0.0017525719468298665
4197,12591,0,12591,59.803715229034424,0.001692363084264814
4278,12834,0,12834,60.954116106033325,0.0016194349172522523
4359,13077,0,13077,62.0742461681366,0.0015844956675461694
4439,13317,0,13317,63.18284225463867,0.0015493031402927574
4520,13560,0,13560,64.3548800945282,0.0015067512068902128
4601,13803,0,13803,65.49377822875977,0.001479513069900397
4682,14046,0,14046,66.62090802192688,0.0014514051485658693
4762,14286,0,14286,67.71512699127197,0.0014172538953305632
4843,14529,0,14529,68.82560110092163,0.0013888605372912133
4924,14772,0,14772,69.927894115448,0.0013649907855192208
5004,15012,0,15012,71.07868218421936,0.0013329083575399142
5085,15255,0,15255,72.19899916648865,0.001287879628891363
5166,15498,0,15498,73.31371426582336,0.0012620309310185413
5247,15741,0,15741,74.43545126914978,0.0012406644968982114
5327,15981,0,15981,75.54670214653015,0.0012154280546489821
5408,16224,0,16224,76.70524525642395,0.0011939858625329626
5489,16467,0,16467,77.85846495628357,0.0011791180555029237
5569,16707,0,16707,79.17857813835144,0.0011646149078970568
5650,16950,0,16950,80.61054825782776,0.0011475629474139754
5731,17193,0,17193,81.73575806617737,0.0011244273343234315
5812,17436,0,17436,82.85056710243225,0.0011050408593391368
5892,17676,0,17676,83.98881506919861,0.0010909641582438373
5973,17919,0,17919,85.07292795181274,0.0010764608033646654
6054,18162,0,18162,86.10837602615356,0.0010593142855032129
6134,18402,0,18402,87.19927906990051,0.001046074730011907
6215,18645,0,18645,88.2378671169281,0.0010319213713828154
6296,18888,0,18888,89.40985321998596,0.001016436659764876
6377,19131,0,19131,90.4904272556305,0.0010024952711078503
6457,19371,0,19371,91.51207327842712,0.0009902603524803153
6538,19614,0,19614,92.5363540649414,0.000978603307830104
6619,19857,0,19857,93.5622010231018,0.0009653271236132528
6699,20097,0,20097,94.55389428138733,0.0009542165888680154
6780,20340,0,20340,95.64333629608154,0.0009418272319643379
6861,20583,0,20583,96.693115234375,0.0009283668819297392
6942,20826,0,20826,97.79451632499695,0.0009179293019847279
7022,21066,0,21066,98.83344316482544,0.0009062454956422808
7103,21309,0,21309,99.86559319496155,0.0008933913286452246
7184,21552,0,21552,101.05973720550537,0.0008831299576373038
7264,21792,0,21792,102.25181913375854,0.0008732393841611175
7345,22035,0,22035,103.34003520011902,0.0008630413507915407
7426,22278,0,22278,104.39491128921509,0.000852657788352591
7507,22521,0,22521,105.4545750617981,0.000842431876865029
7587,22761,0,22761,106.51916217803955,0.0008324927626706043
7668,23004,0,23004,107.63288521766663,0.0008205478420038041
7749,23247,0,23247,108.7430510520935,0.0008107502036878812
7829,23487,0,23487,109.81752228736877,0.0008014040290956084
7910,23730,0,23730,110.85525417327881,0.0007923219829443787
7991,23973,0,23973,111.92157816886902,0.0007819872876492861
8072,24216,0,24216,113.03729104995728,0.0007715269636013926
8152,24456,0,24456,114.12199330329895,0.0007629054157914433
8233,24699,0,24699,115.30718612670898,0.000753605057822457
8314,24942,0,24942,116.43123316764832,0.0007434144871642799
8394,25182,0,25182,117.53237724304199,0.0007341388558184425
8475,25425,0,25425,118.63340210914612,0.0007255801754850654
8556,25668,0,25668,119.76549124717712,0.0007169783373218987
8637,25911,0,25911,120.86697006225586,0.0007076856209678048
8717,26151,0,26151,122.00175523757935,0.0006967875219464598
8798,26394,0,26394,123.0933129787445,0.0006864184852366698
8879,26637,0,26637,124.25888299942017,0.0006774085551221286
8959,26877,0,26877,125.35234093666077,0.0006691258840228312
9040,27120,0,27120,126.51745915412903,0.0006563078502706747
9121,27363,0,27363,127.66072916984558,0.0006360079096048793
9202,27606,0,27606,128.7800953388214,0.0006236128457970461
9282,27846,0,27846,129.799574136734,0.0006156028827488595
9363,28089,0,28089,130.83956813812256,0.0006086584416160589
9444,28332,0,28332,131.88965511322021,0.0006019502883541746
9524,28572,0,28572,132.93441820144653,0.000595437722671563
9605,28815,0,28815,133.97568321228027,0.0005880241250489464
9686,29058,0,29058,135.04152011871338,0.0005789848691005312
9767,29301,0,29301,136.0813512802124,0.0005699611163116421
9847,29541,0,29541,137.12313604354858,0.000563476868005442
9928,29784,0,29784,138.169753074646,0.0005566992028133563
10009,30027,0,30027,139.2357861995697,0.000549361208313688
10089,30267,0,30267,140.2457892894745,0.0005389991292516782
10170,30510,0,30510,141.28163027763367,0.0005311179557140108
10251,30753,0,30753,142.32065200805664,0.0005246627503710169
10332,30996,0,30996,143.35987210273743,0.0005187066290061334
10412,31236,0,31236,144.3734781742096,0.0005129441058615777
10493,31479,0,31479,145.4150640964508,0.0005069189540784983
10574,31722,0,31722,146.44230604171753,0.000500557188628404
10654,31962,0,31962,147.4693250656128,0.000494321487813889
10735,32205,0,32205,148.49873614311218,0.0004871345955917951
10816,32448,0,32448,149.54499912261963,0.0004809525501577373
10897,32691,0,32691,150.57236409187317,0.0004724174831837188
10977,32931,0,32931,151.57052206993103,0.0004650943285123979
11058,33174,0,33174,152.60595726966858,0.0004596190610330869
11139,33417,0,33417,153.62273812294006,0.0004538377614646511
11219,33657,0,33657,154.63517832756042,0.0004480610509165946
11300,33900,0,33900,155.66501235961914,0.00044262094766303145
11381,34143,0,34143,156.70185232162476,0.00043738163372860245
11462,34386,0,34386,157.70102906227112,0.0004322526714794509
11542,34626,0,34626,158.71261310577393,0.0004270684125982953
11623,34869,0,34869,159.7472870349884,0.00042198749392822257
11704,35112,0,35112,160.7873411178589,0.0004170153266451099
11784,35352,0,35352,161.80606508255005,0.0004121512550797726
11865,35595,0,35595,162.867445230484,0.00040459431522320353
11946,35838,0,35838,163.90884518623352,0.00039483475750917246
12027,36081,0,36081,164.9715051651001,0.0003898953417790388
12107,36321,0,36321,165.98597121238708,0.0003852391753859573
12188,36564,0,36564,166.9994490146637,0.0003808049197300928
12269,36807,0,36807,168.19934821128845,0.00037618283544764474
12350,37050,0,37050,169.23240613937378,0.0003711538071010317
12430,37290,0,37290,170.2794930934906,0.00036634773908470765
12511,37533,0,37533,171.32184720039368,0.0003613622473801487
12592,37776,0,37776,172.5373091697693,0.00035581963717513937
12672,38016,0,38016,174.19309425354004,0.00035152571980898335
12753,38259,0,38259,175.5674023628235,0.0003473956500269698
12834,38502,0,38502,176.6374740600586,0.00034325282691448366
12915,38745,0,38745,177.659850358963,0.0003391186427016064
12995,38985,0,38985,178.6923942565918,0.0003352556959642115
13076,39228,0,39228,179.69052124023438,0.000331361757590497
13157,39471,0,39471,180.6965880393982,0.0003273418136440311
13237,39711,0,39711,181.7023961544037,0.0003236567029578451
13318,39954,0,39954,182.71415495872498,0.00031991290125473897
13399,40197,0,40197,183.73569202423096,0.0003162992426817924
13480,40440,0,40440,184.85821723937988,0.00031258998694652743
13560,40680,0,40680,185.94151496887207,0.0003089953941341313
13641,40923,0,40923,187.13082909584045,0.00030505235181169706
13722,41166,0,41166,188.18464732170105,0.0003009121339056543
13802,41406,0,41406,189.19853115081787,0.0002970371314844219
13883,41649,0,41649,190.31761026382446,0.00029351706635609415
13964,41892,0,41892,191.35679006576538,0.0002901038402527842
14045,42135,0,42135,192.38454604148865,0.000286316192439031
14125,42375,0,42375,193.3949031829834,0.0002812103707274026
14206,42618,0,42618,194.39420533180237,0.00027438895396675013
14287,42861,0,42861,195.4131100177765,0.0002698194946365138
14367,43101,0,43101,196.40215921401978,0.0002645065976453638
14448,43344,0,43344,197.40798616409302,0.0002565766411141783
14529,43587,0,43587,198.41477513313293,0.0002523658368973472
14610,43830,0,43830,199.41171026229858,0.0002492435430270792
14690,44070,0,44070,200.41243529319763,0.00024616974378079246
14771,44313,0,44313,201.41702127456665,0.0002433569783411979
14852,44556,0,44556,202.46815609931946,0.00024064972695210404
14932,44796,0,44796,203.46481728553772,0.0002378600725601445
15013,45039,0,45039,204.47644329071045,0.00023495222214183845
15094,45282,0,45282,205.4812400341034,0.0002318830676390698
15175,45525,0,45525,206.49949622154236,0.00022853534919956196
15255,45765,0,45765,207.51059412956238,0.00022572032577562238
15336,46008,0,46008,208.57741832733154,0.00022325248879972445
15417,46251,0,46251,209.5733962059021,0.00022081785397212616
15497,46491,0,46491,210.562509059906,0.0002184259510267074
15578,46734,0,46734,211.55107712745667,0.0002159613382976906
15659,46977,0,46977,212.54403519630432,0.0002133262531584226
15740,47220,0,47220,213.53955912590027,0.00021083353443803428
15820,47460,0,47460,214.51433801651,0.00020853210428045096
15901,47703,0,47703,215.53128910064697,0.00020587175692144647
15982,47946,0,47946,216.5468032360077,0.00020294551722523085
16062,48186,0,48186,217.5576560497284,0.00020066383758018952
16143,48429,0,48429,218.58622312545776,0.00019820749834460912
16224,48672,0,48672,219.63318514823914,0.00019519955053906438
16305,48915,0,48915,220.63932418823242,0.00019276478795614418
16385,49155,0,49155,221.63673210144043,0.00019033882298879974
16466,49398,0,49398,222.63009214401245,0.0001881164406934317
16547,49641,0,49641,223.6370050907135,0.0001859763901271092
16627,49881,0,49881,224.62501502037048,0.00018388594167621057
16708,50124,0,50124,225.6299183368683,0.00018165638644415357
16789,50367,0,50367,226.63575720787048,0.00017885793680569236
16870,50610,0,50610,227.64129114151,0.00017556143848836855
16950,50850,0,50850,228.62742400169373,0.00017331529282015853
17031,51093,0,51093,229.62489128112793,0.00017117557187565526
17112,51336,0,51336,230.6423442363739,0.00016906705749047786
17192,51576,0,51576,231.61991715431213,0.00016693615311487708
17273,51819,0,51819,232.6099100112915,0.00016494175197668702
17354,52062,0,52062,233.59377312660217,0.0001630802083147647
17435,52305,0,52305,234.61081910133362,0.00016106438893092944
17515,52545,0,52545,235.59733605384827,0.00015920823715108703
17596,52788,0,52788,236.621502161026,0.0001573198240797075
17677,53031,0,53031,237.64499020576477,0.0001553698787248588
17757,53271,0,53271,238.63878393173218,0.00015348496679289152
17838,53514,0,53514,239.6476480960846,0.00015130682657987297
17919,53757,0,53757,240.64684534072876,0.00014769479201195968
18000,54000,0,54000,241.65408301353455,0.0001440894166964002
18080,54240,0,54240,242.65068221092224,0.00014204715164550937
18161,54483,0,54483,243.67315196990967,0.00014015644186687447
18242,54726,0,54726,244.6621961593628,0.00013843070752574994
18322,54966,0,54966,245.65150833129883,0.0001368689682768621
18403,55209,0,55209,246.6627161502838,0.0001352858688683965
18484,55452,0,55452,247.67483806610107,0.00013376239237667474
18565,55695,0,55695,248.6858789920807,0.00013222428960784325
18645,55935,0,55935,249.6871359348297,0.00013058945285524508
18726,56178,0,56178,250.66064715385437,0.00012900180809092665
18807,56421,0,56421,251.6620500087738,0.000127487221399713
18887,56661,0,56661,252.6582682132721,0.00012582842172339603
18968,56904,0,56904,253.65658521652222,0.00012429743170148822
19049,57147,0,57147,254.6764793395996,0.00012276416402801405
19130,57390,0,57390,255.6793510913849,0.00012059262508771417
19210,57630,0,57630,256.6831040382385,0.00011873127393593348
19291,57873,0,57873,257.69016909599304,0.00011715380222171674
19372,58116,0,58116,258.70229291915894,0.00011562619806928655
19452,58356,0,58356,259.7204101085663,0.00011427699908216215
19533,58599,0,58599,260.7401351928711,0.00011290318341274583
19614,58842,0,58842,261.7422614097595,0.00011157694985924556
19695,59085,0,59085,262.7472622394562,0.00011019848183511988
19775,59325,0,59325,263.738801240921,0.00010893736381904522
19856,59568,0,59568,264.738893032074,0.00010769228280468276
19937,59811,0,59811,265.7466821670532,0.00010643963068289392
20017,60051,0,60051,266.73356008529663,0.0001052417436760213
20098,60294,0,60294,267.7583432197571,0.00010400426853815942
20179,60537,0,60537,268.7591972351074,0.00010270571771308619
20260,60780,0,60780,269.7559931278229,0.000101453774232364
20340,61020,0,61020,270.72467017173767,0.00010013113492921062
20421,61263,0,61263,271.7163722515106,9.884687866337915e-05
20502,61506,0,61506,272.7210052013397,9.765142930127606e-05
20583,61749,0,61749,273.72799921035767,9.652200986396901e-05
20663,61989,0,61989,274.71843123435974,9.543741294682565e-05
20744,62232,0,62232,275.73053908348083,9.436679898310941e-05
20825,62475,0,62475,276.7325723171234,9.326272625436728e-05
20905,62715,0,62715,277.7238802909851,9.221343484757358e-05
20986,62958,0,62958,278.7429041862488,9.115338343630033e-05
21067,63201,0,63201,279.7533302307129,9.010513041497147e-05
21148,63444,0,63444,280.7482521533966,8.896593034037422e-05
21228,63684,0,63684,281.73161005973816,8.794131308085983e-05
21309,63927,0,63927,282.74293303489685,8.690321942002466e-05
21390,64170,0,64170,283.7485980987549,8.584858676211071e-05
21470,64410,0,64410,284.72904419898987,8.486354484163871e-05
21551,64653,0,64653,285.7178521156311,8.384445923772092e-05
21632,64896,0,64896,286.7209703922272,8.286669231782388e-05
21713,65139,0,65139,287.72909212112427,8.175152566669745e-05
21793,65379,0,65379,288.7223081588745,8.08099343620428e-05
21874,65622,0,65622,289.7378532886505,7.983613033651663e-05
21955,65865,0,65865,290.73622703552246,7.882327023134608e-05
22035,66105,0,66105,291.7217471599579,7.79210800748475e-05
22116,66348,0,66348,292.7185592651367,7.688894236694817e-05
22197,66591,0,66591,293.7129020690918,7.580312029928105e-05
22278,66834,0,66834,294.7150902748108,7.474882939542122e-05
22358,67074,0,67074,295.71956610679626,7.368447894603685e-05
22439,67317,0,67317,296.70524525642395,7.273540722686048e-05
22520,67560,0,67560,297.72329211235046,7.19117932111266e-05
22600,67800,0,67800,298.69623708724976,7.109332093593545e-05
22681,68043,0,68043,299.69451427459717,7.02210764796654e-05
22762,68286,0,68286,300.6804132461548,6.935403462450602e-05
22843,68529,0,68529,301.73746514320374,6.855452752846548e-05
22923,68769,0,68769,303.03819012641907,6.764574250161276e-05
23004,69012,0,69012,304.28361535072327,6.684309292097991e-05
23085,69255,0,69255,305.29205226898193,6.60367468970667e-05
23165,69495,0,69495,306.294575214386,6.528072078011078e-05
23246,69738,0,69738,307.29644322395325,6.450033463594196e-05
23327,69981,0,69981,308.3106791973114,6.366513487286744e-05
23408,70224,0,70224,309.67106914520264,6.28909739021375e-05
23488,70464,0,70464,310.87833428382874,6.217787765426251e-05
23569,70707,0,70707,312.07445216178894,6.131778474558084e-05
23650,70950,0,70950,313.25587129592896,6.052421693301976e-05
23730,71190,0,71190,314.3217062950134,5.9836603184543235e-05
23811,71433,0,71433,315.3923850059509,5.913060171143436e-05
23892,71676,0,71676,316.5373842716217,5.804925160000002e-05
23973,71919,0,71919,317.6277141571045,5.6626734482117294e-05
24053,72159,0,72159,318.6751160621643,5.577750301902754e-05
24134,72402,0,72402,319.6919243335724,5.483569275140096e-05
24215,72645,0,72645,320.6942801475525,5.393351487467421e-05
24295,72885,0,72885,321.69396018981934,5.326755589713977e-05
24376,73128,0,73128,322.7020699977875,5.261703233331714e-05
24457,73371,0,73371,323.7109181880951,5.195767573246348e-05
24538,73614,0,73614,324.7109582424164,5.1350832589576785e-05
24618,73854,0,73854,325.70325922966003,5.0761260851757245e-05
24699,74097,0,74097,326.70745611190796,5.0182901442732845e-05
24780,74340,0,74340,327.7100751399994,4.959823385494271e-05
24860,74580,0,74580,328.6913080215454,4.89249340572144e-05
24941,74823,0,74823,329.92508721351624,4.8288367492714105e-05
25022,75066,0,75066,331.0930211544037,4.773165700396556e-05
25103,75309,0,75309,332.1798713207245,4.718080259267982e-05
25183,75549,0,75549,333.3665962219238,4.6625177760142904e-05
25264,75792,0,75792,334.57836532592773,4.6067887889297795e-05
25345,76035,0,76035,335.58521604537964,4.545699846186177e-05
25425,76275,0,76275,336.6897542476654,4.490278357197959e-05
25506,76518,0,76518,337.75656509399414,4.435942823501054e-05
25587,76761,0,76761,338.80293226242065,4.384423437992647e-05
25668,77004,0,77004,339.87396121025085,4.3339895540573765e-05
25748,77244,0,77244,340.96864008903503,4.282730115696036e-05
25829,77487,0,77487,341.946475982666,4.2246794214487655e-05
25910,77730,0,77730,342.9587562084198,4.1745227028838506e-05
25990,77970,0,77970,343.9479591846466,4.126926077580295e-05
26071,78213,0,78213,344.92587208747864,4.077754377003677e-05
26152,78456,0,78456,346.0445611476898,4.026007059936987e-05
26233,78699,0,78699,347.12242126464844,3.9786469556692846e-05
26313,78939,0,78939,348.1221241950989,3.9341221188743484e-05
26394,79182,0,79182,349.2408859729767,3.888561477938234e-05
26475,79425,0,79425,350.2558183670044,3.842212777506334e-05
26555,79665,0,79665,351.3674931526184,3.798493575878026e-05
26636,79908,0,79908,352.44785714149475,3.750993664911282e-05
26717,80151,0,80151,353.46881914138794,3.706697913017369e-05
26798,80394,0,80394,354.4790372848511,3.662937575078214e-05
26878,80634,0,80634,355.5020351409912,3.617319235938368e-05
26959,80877,0,80877,356.6347529888153,3.5491025947757096e-05
27040,81120,0,81120,357.73149514198303,3.4951747630693016e-05
27120,81360,0,81360,358.7254741191864,3.452896759032316e-05
27201,81603,0,81603,359.72897720336914,3.4126156664960286e-05
27282,81846,0,81846,360.72215127944946,3.373644690337386e-05
27363,82089,0,82089,361.71445417404175,3.3309375571912514e-05
27443,82329,0,82329,362.70174622535706,3.289868780931361e-05
27524,82572,0,82572,363.7013213634491,3.2514000228160875e-05
27605,82815,0,82815,364.6896231174469,3.214111021901643e-05
27685,83055,0,83055,365.6794981956482,3.1788719351803576e-05
27766,83298,0,83298,366.68666315078735,3.1435471623784446e-05
27847,83541,0,83541,367.68260502815247,3.107662438464155e-05
27928,83784,0,83784,368.69050312042236,3.072865552686948e-05
28008,84024,0,84024,369.70672512054443,3.0371425966312114e-05
28089,84267,0,84267,370.70838022232056,3.0028480063761294e-05
28170,84510,0,84510,371.73922204971313,2.9680389177130735e-05
28251,84753,0,84753,372.74231910705566,2.9310600512236267e-05
28331,84993,0,84993,373.7961163520813,2.892946494695495e-05
28412,85236,0,85236,374.88393807411194,2.8600159630833536e-05
28493,85479,0,85479,376.0805969238281,2.8269741843215465e-05
28573,85719,0,85719,377.0465130805969,2.7905800327059594e-05
28654,85962,0,85962,378.19972825050354,2.7516827776140224e-05
28735,86205,0,86205,379.19451427459717,2.7147068279837557e-05
28816,86448,0,86448,380.319402217865,2.6724471411860252e-05
28896,86688,0,86688,381.405225276947,2.6364157950300775e-05
28977,86931,0,86931,382.47104716300964,2.6054803774373826e-05
29058,87174,0,87174,383.50255823135376,2.5713447092804537e-05
29138,87414,0,87414,384.49383330345154,2.539230328724914e-05
29219,87657,0,87657,385.4778561592102,2.507752513783104e-05
29300,87900,0,87900,386.4810471534729,2.4759487937193936e-05
29381,88143,0,88143,387.58067297935486,2.4382195385001114e-05
29461,88383,0,88383,388.58602023124695,2.4083819736067054e-05
29542,88626,0,88626,389.5854630470276,2.3783331904976318e-05
29623,88869,0,88869,390.5810480117798,2.3507866765853092e-05
29703,89109,0,89109,391.5706133842468,2.323306413788995e-05
29784,89352,0,89352,392.5705201625824,2.2962806365873374e-05
29865,89595,0,89595,393.5686902999878,2.268699826851181e-05
29946,89838,0,89838,394.53045296669006,2.2413484733804996e-05
30026,90078,0,90078,395.49812602996826,2.2152304709010987e-05
30107,90321,0,90321,396.4732060432434,2.184974996862894e-05
30188,90564,0,90564,397.46104526519775,2.1588154818590982e-05
30268,90804,0,90804,398.44334411621094,2.1313923877411837e-05
30349,91047,0,91047,399.4220151901245,2.1064409238123383e-05
30430,91290,0,91290,400.4154040813446,2.0820607422987357e-05
30511,91533,0,91533,401.40441608428955,2.056537502090521e-05
30591,91773,0,91773,402.3901810646057,2.0331487325499936e-05
30672,92016,0,92016,403.37318325042725,2.00896469477783e-05
30753,92259,0,92259,404.3657112121582,1.9830321492929204e-05
30833,92499,0,92499,405.332288980484,1.960268171194981e-05
30914,92742,0,92742,406.3223023414612,1.9358013675140125e-05
30995,92985,0,92985,407.3064031600952,1.9129679309168815e-05
31076,93228,0,93228,408.2994501590729,1.8864469590073645e-05
31156,93468,0,93468,409.27315306663513,1.8633055719927125e-05
31237,93711,0,93711,410.26085233688354,1.8397792556940768e-05
31318,93954,0,93954,411.25450325012207,1.8136441459436326e-05
31398,94194,0,94194,412.22276306152344,1.7922468355413082e-05
31479,94437,0,94437,413.22021412849426,1.7719455839225505e-05
31560,94680,0,94680,414.2051491737366,1.7497808917485034e-05
31641,94923,0,94923,415.20734310150146,1.729721390360899e-05
31721,95163,0,95163,416.17994117736816,1.7099901888310084e-05
31802,95406,0,95406,417.169291973114,1.6903944065220988e-05
31883,95649,0,95649,418.1574110984802,1.67055150923507e-05
31963,95889,0,95889,419.1426901817322,1.6509435010491178e-05
32044,96132,0,96132,420.1482172012329,1.6313702584413172e-05
32125,96375,0,96375,421.1392431259155,1.6108442439274954e-05
32206,96618,0,96618,422.1378049850464,1.5917947440241218e-05
32286,96858,0,96858,423.1086571216583,1.5718280786315898e-05
32367,97101,0,97101,424.106014251709,1.553754029472218e-05
32448,97344,0,97344,425.08945417404175,1.5358210560541707e-05
32528,97584,0,97584,426.0707960128784,1.5179370710831978e-05
32609,97827,0,97827,427.04850912094116,1.4996856546583724e-05
32690,98070,0,98070,428.04015827178955,1.4804636692068353e-05
32771,98313,0,98313,429.02504229545593,1.4632695414654816e-05
32851,98553,0,98553,429.9937391281128,1.4466080321907063e-05
32932,98796,0,98796,430.98203706741333,1.4297971562023328e-05
33013,99039,0,99039,431.96419501304626,1.4128421881986545e-05
33093,99279,0,99279,432.96157002449036,1.396300861817067e-05
33174,99522,0,99522,433.9469401836395,1.3803580728999722e-05
33255,99765,0,99765,434.9406931400299,1.3641305382086006e-05
33336,100008,0,100008,435.91919922828674,1.3486643919244949e-05
33416,100248,0,100248,436.90220618247986,1.333596704555e-05
33497,100491,0,100491,437.881019115448,1.3181252095529816e-05
33578,100734,0,100734,438.86767411231995,1.3034848709717255e-05
33658,100974,0,100974,439.8311142921448,1.2888583599515774e-05
33739,101217,0,101217,440.8067891597748,1.2741068092395331e-05
33820,101460,0,101460,441.79656434059143,1.25962045420259e-05
33901,101703,0,101703,442.77802634239197,1.2448407627698665e-05
33981,101943,0,101943,443.7732231616974,1.2297794034184826e-05
34062,102186,0,102186,444.7457482814789,1.214995088574474e-05
34143,102429,0,102429,445.738144159317,1.2012858770584548e-05
34223,102669,0,102669,446.70521116256714,1.1875434581513134e-05
34304,102912,0,102912,447.7086272239685,1.1721679148438922e-05
34385,103155,0,103155,448.73030614852905,1.1578691461957041e-05
34466,103398,0,103398,449.7541871070862,1.1444507159184726e-05
34546,103638,0,103638,450.7795560359955,1.1316756803044628e-05
34627,103881,0,103881,451.86549496650696,1.1187126772036785e-05
34708,104124,0,104124,452.916561126709,1.1060564422469409e-05
34788,104364,0,104364,453.96685004234314,1.0935796478948367e-05
34869,104607,0,104607,455.08161520957947,1.0810435346712288e-05
34950,104850,0,104850,456.3198971748352,1.066277604550648e-05
35031,105093,0,105093,457.3217830657959,1.0543031327776853e-05
35111,105333,0,105333,458.47629618644714,1.0426358078966089e-05
35192,105576,0,105576,459.47779512405396,1.030232311509309e-05
35273,105819,0,105819,460.57184624671936,1.017216764530965e-05
35353,106059,0,106059,461.6829752922058,1.003106833671925e-05
35434,106302,0,106302,462.7608313560486,9.912552580902047e-06
35515,106545,0,106545,463.8195900917053,9.789141025901564e-06
35596,106788,0,106788,464.90858125686646,9.659530913826953e-06
35676,107028,0,107028,465.9392640590668,9.546824278436659e-06
35757,107271,0,107271,467.15995812416077,9.42949094142981e-06
35838,107514,0,107514,468.28589820861816,9.30452537614298e-06
35918,107754,0,107754,469.32843017578125,9.198173784576179e-06
35999,107997,0,107997,470.3499183654785,9.089694468147069e-06
36080,108240,0,108240,471.3821151256561,8.982271140477139e-06
36161,108483,0,108483,472.59742307662964,8.877927029527435e-06
36241,108723,0,108723,473.57861328125,8.778312658028272e-06
36322,108966,0,108966,474.57728719711304,8.674768186915056e-06
36403,109209,0,109209,475.5578501224518,8.572784522253109e-06
36484,109452,0,109452,476.5504550933838,8.469096228245093e-06
36564,109692,0,109692,477.53798508644104,8.372800779324935e-06
36645,109935,0,109935,478.52973103523254,8.276328858712707e-06
36726,110178,0,110178,479.5154240131378,8.164936115686671e-06
36806,110418,0,110418,480.5014691352844,8.068857401124506e-06
36887,110661,0,110661,481.490825176239,7.971394181075959e-06
36968,110904,0,110904,482.49268221855164,7.878781279266806e-06
37049,111147,0,111147,483.4776861667633,7.790963084969156e-06
37129,111387,0,111387,484.46276807785034,7.69814058079229e-06
37210,111630,0,111630,485.44458413124084,7.603767493297982e-06
37291,111873,0,111873,486.4378023147583,7.516190630504553e-06
37371,112113,0,112113,487.4167082309723,7.4291088701261104e-06
37452,112356,0,112356,488.414626121521,7.330639606357164e-06
37533,112599,0,112599,489.4115061759949,7.243702494262601e-06
37614,112842,0,112842,490.39718413352966,7.16090653030799e-06
37694,113082,0,113082,491.3780152797699,7.0775820284440175e-06
37775,113325,0,113325,492.37753534317017,6.974460879413449e-06
37856,113568,0,113568,493.38250637054443,6.861737413431167e-06
37936,113808,0,113808,494.3638062477112,6.777370080906541e-06
38017,114051,0,114051,495.5393841266632,6.6925485694316516e-06
38098,114294,0,114294,496.62904596328735,6.604054151819736e-06
38179,114537,0,114537,497.76621317863464,6.525508454115682e-06
38259,114777,0,114777,498.72698616981506,6.451327240845057e-06
38340,115020,0,115020,499.7084562778473,6.374536659661261e-06
38421,115263,0,115263,500.6922962665558,6.294882705913517e-06
38501,115503,0,115503,501.76667308807373,6.2209958371075235e-06
38582,115746,0,115746,502.909704208374,6.146003618881788e-06
38663,115989,0,115989,504.0024423599243,6.0725467140564985e-06
38744,116232,0,116232,505.01033210754395,5.994846427250902e-06
38824,116472,0,116472,505.98405027389526,5.917935471827616e-06
38905,116715,0,116715,506.996707201004,5.84449623092824e-06
38986,116958,0,116958,507.99892711639404,5.778183855286883e-06
39066,117198,0,117198,508.98318219184875,5.712463532768936e-06
39147,117441,0,117441,509.96777415275574,5.643177639870138e-06
39228,117684,0,117684,510.9651691913605,5.576572574632584e-06
39309,117927,0,117927,511.94584608078003,5.513004071254282e-06
39389,118167,0,118167,512.9355492591858,5.449859997806579e-06
39470,118410,0,118410,513.9207742214203,5.386782543632739e-06
39551,118653,0,118653,514.9121601581573,5.305184200563142e-06
39631,118893,0,118893,515.882336139679,5.1952171040937725e-06
39712,119136,0,119136,516.8657021522522,5.107011361411317e-06
39793,119379,0,119379,517.8577802181244,5.043105291727307e-06
39874,119622,0,119622,518.839380979538,4.981029334425426e-06
39954,119862,0,119862,519.8264021873474,4.9259275455891106e-06
40035,120105,0,120105,520.8181781768799,4.868950731890643e-06
40116,120348,0,120348,521.8135211467743,4.812105380814399e-06
40196,120588,0,120588,522.7836112976074,4.7556688805809696e-06
40277,120831,0,120831,523.7744960784912,4.7002915497162505e-06
40358,121074,0,121074,524.7611091136932,4.646630556745637e-06
40439,121317,0,121317,525.7504560947418,4.592639138226357e-06
40519,121557,0,121557,526.7286560535431,4.536541303425066e-06
40600,121800,0,121800,527.7126572132111,4.483285029957933e-06
40681,122043,0,122043,528.7088482379913,4.430665616845248e-06
40761,122283,0,122283,529.6794052124023,4.3806830164190065e-06
40842,122526,0,122526,530.674149274826,4.325944878371009e-06
40923,122769,0,122769,531.6569261550903,4.269307961701926e-06
41004,123012,0,123012,532.6445531845093,4.2203116210449425e-06
41084,123252,0,123252,533.6206901073456,4.173335790237046e-06
41165,123495,0,123495,534.6176760196686,4.125790922507842e-06
41246,123738,0,123738,535.6002812385559,4.07462278373258e-06
41326,123978,0,123978,536.572859287262,4.004806163674379e-06
41407,124221,0,124221,537.5674123764038,3.949785081762136e-06
41488,124464,0,124464,538.5529420375824,3.898757514934125e-06
41569,124707,0,124707,539.550065279007,3.85105043482576e-06
41649,124947,0,124947,540.5191342830658,3.8080679536999403e-06
41730,125190,0,125190,541.5175712108612,3.7650065270523733e-06
41811,125433,0,125433,542.5084342956543,3.7221101954751793e-06
41891,125673,0,125673,543.5013191699982,3.6773692759432235e-06
41972,125916,0,125916,544.4991521835327,3.6333210448344737e-06
42053,126159,0,126159,545.4977152347565,3.5915500720841957e-06
42134,126402,0,126402,546.4851629734039,3.547497774184947e-06
42214,126642,0,126642,547.4647271633148,3.505810601549735e-06
42295,126885,0,126885,548.4699392318726,3.464202339101528e-06
42376,127128,0,127128,549.4580552577972,3.4254670274310923e-06
42456,127368,0,127368,550.445127248764,3.383381073977785e-06
42537,127611,0,127611,551.4251942634583,3.339953752526385e-06
42618,127854,0,127854,552.4174520969391,3.296653397812262e-06
42699,128097,0,128097,553.4000582695007,3.2569650575195574e-06
42779,128337,0,128337,554.3733742237091,3.218130408205287e-06
42860,128580,0,128580,555.3446731567383,3.1817309949065857e-06
42941,128823,0,128823,556.3499729633331,3.145859852311753e-06
43021,129063,0,129063,557.3203711509705,3.1039335142812648e-06
43102,129306,0,129306,558.3154852390289,3.0638299570646425e-06
43183,129549,0,129549,559.3081841468811,3.0276636767022087e-06
43264,129792,0,129792,560.2915840148926,2.9912533637749195e-06
43344,130032,0,130032,561.2793362140656,2.9550753583892913e-06
43425,130275,0,130275,562.2681651115417,2.9155053966169555e-06
43506,130518,0,130518,563.290999174118,2.8797132322106536e-06
43586,130758,0,130758,564.313826084137,2.8467581667527964e-06
43667,131001,0,131001,565.3783621788025,2.814351060176646e-06
43748,131244,0,131244,566.4447801113129,2.7812684763341036e-06
43829,131487,0,131487,567.5328731536865,2.7483534505353716e-06
43909,131727,0,131727,568.5715272426605,2.717339117434181e-06
43990,131970,0,131970,569.7272822856903,2.687341087273499e-06
44071,132213,0,132213,570.8267493247986,2.6580473330266395e-06
44151,132453,0,132453,571.9362041950226,2.6292051877188426e-06
44232,132696,0,132696,572.9201972484589,2.5990160801490853e-06
44313,132939,0,132939,573.9195981025696,2.5696768386558515e-06
44394,133182,0,133182,574.9004023075104,2.540535613556355e-06
44474,133422,0,133422,575.8868641853333,2.511425752217734e-06
44555,133665,0,133665,576.8737301826477,2.476963256858052e-06
44636,133908,0,133908,577.8673651218414,2.4439046094495586e-06
44717,134151,0,134151,578.8606061935425,2.4159597871380704e-06
44797,134391,0,134391,579.8386559486389,2.3870209544701467e-06
44878,134634,0,134634,580.8108870983124,2.3582179198052154e-06
44959,134877,0,134877,581.7723062038422,2.3310056519484826e-06
45039,135117,0,135117,582.7570853233337,2.3054905022667085e-06
45120,135360,0,135360,583.788378238678,2.2760985210683383e-06
45201,135603,0,135603,584.8166661262512,2.246838849922501e-06
45282,135846,0,135846,585.9969210624695,2.218583817647409e-06
45362,136086,0,136086,587.0682570934296,2.1929160267368603e-06
45443,136329,0,136329,588.1360101699829,2.165039811039391e-06
45524,136572,0,136572,589.2299160957336,2.1390512170092195e-06
45604,136812,0,136812,590.2660903930664,2.1122002977007046e-06
45685,137055,0,137055,591.3235011100769,2.08389359839177e-06
45766,137298,0,137298,592.3143889904022,2.054277239796439e-06
45847,137541,0,137541,593.3570771217346,2.0254278804145765e-06
45927,137781,0,137781,594.3408010005951,2.0003122069640575e-06
46008,138024,0,138024,595.3371713161469,1.9747356389313396e-06
46089,138267,0,138267,596.3343861103058,1.9508156059295617e-06
46169,138507,0,138507,597.3399653434753,1.9289966372014855e-06
46250,138750,0,138750,598.3445491790771,1.9065026415173665e-06
46331,138993,0,138993,599.3334031105042,1.8817989852913878e-06
46412,139236,0,139236,600.3358392715454,1.8551198445229599e-06
46492,139476,0,139476,601.3123240470886,1.8286276625046594e-06
46573,139719,0,139719,602.3024210929871,1.800172997757878e-06
46654,139962,0,139962,603.2855112552643,1.775507334919584e-06
46734,140202,0,140202,604.318695306778,1.754338216040686e-06
46815,140445,0,140445,605.3022420406342,1.7339778612371382e-06
46896,140688,0,140688,606.3725731372833,1.713938328697328e-06
46977,140931,0,140931,607.4828369617462,1.6937291474414172e-06
47057,141171,0,141171,608.6061222553253,1.672929663751161e-06
47138,141414,0,141414,609.6034822463989,1.6532248181551918e-06
47219,141657,0,141657,610.6025810241699,1.6337047302845793e-06
47299,141897,0,141897,611.5785751342773,1.6143008751226381e-06
47380,142140,0,142140,612.5867691040039,1.5941931027234638e-06
47461,142383,0,142383,613.6422362327576,1.5756029149938633e-06
47542,142626,0,142626,614.6401782035828,1.5574277344647955e-06
47622,142866,0,142866,615.6435701847076,1.5391043407276238e-06
47703,143109,0,143109,616.6570081710815,1.5207355853545207e-06
47784,143352,0,143352,617.6696441173553,1.5018424914184847e-06
47864,143592,0,143592,618.6462602615356,1.4822890677003447e-06
47945,143835,0,143835,619.6406271457672,1.4644707237319372e-06
48026,144078,0,144078,620.6160712242126,1.4482137657948267e-06
48107,144321,0,144321,621.6256561279297,1.4318634882901794e-06
48187,144561,0,144561,622.591203212738,1.416209444295558e-06
48268,144804,0,144804,623.6069769859314,1.400075257412946e-06
48349,145047,0,145047,624.5913331508636,1.384170384821825e-06
48429,145287,0,145287,625.5534262657166,1.3678126615761397e-06
48510,145530,0,145530,626.5401482582092,1.352119663080252e-06
48591,145773,0,145773,627.5456502437592,1.336588058555002e-06
48672,146016,0,146016,628.5441591739655,1.3206623307852659e-06
48752,146256,0,146256,629.5175621509552,1.3046334958130003e-06
48833,146499,0,146499,630.5151772499084,1.2897106748200752e-06
48914,146742,0,146742,631.5027372837067,1.2724126683406458e-06
48994,146982,0,146982,632.4979650974274,1.25588510396962e-06
49075,147225,0,147225,633.4896550178528,1.2415535494651558e-06
49156,147468,0,147468,634.4882972240448,1.227265020945802e-06
49237,147711,0,147711,635.4705860614777,1.2127183240405117e-06
49317,147951,0,147951,636.4399790763855,1.1974930573805572e-06
49398,148194,0,148194,637.4367311000824,1.1830632709300124e-06
49479,148437,0,148437,638.4227902889252,1.1689268673827813e-06
49559,148677,0,148677,639.3977062702179,1.154674940153797e-06
49640,148920,0,148920,640.3873162269592,1.141339254140654e-06
49721,149163,0,149163,641.385968208313,1.1283144951290247e-06
49802,149406,0,149406,642.3781070709229,1.1149751705220813e-06
49882,149646,0,149646,643.3621480464935,1.1020176451849843e-06
49963,149889,0,149889,644.3429291248322,1.0884635170054324e-06
50044,150132,0,150132,645.338002204895,1.0760069870229254e-06
50124,150372,0,150372,646.312420129776,1.063832572394624e-06
50205,150615,0,150615,647.3113222122192,1.0500598086842157e-06
50286,150858,0,150858,648.3101880550385,1.0361464339956899e-06
50367,151101,0,151101,649.3039462566376,1.0242813514072417e-06
50447,151341,0,151341,650.3052232265472,1.012282270209607e-06
50528,151584,0,151584,651.2864303588867,1.0000825344819094e-06
50609,151827,0,151827,652.2849702835083,9.857774770479197e-07
50689,152067,0,152067,653.258807182312,9.747615128821186e-07
50770,152310,0,152310,654.2617189884186,9.633936066798772e-07
50851,152553,0,152553,655.2449593544006,9.525369999142846e-07
50932,152796,0,152796,656.2333052158356,9.409997820904622e-07
51012,153036,0,153036,657.2026791572571,9.28685368563375e-07
51093,153279,0,153279,658.2032833099365,9.176568051338674e-07
51174,153522,0,153522,659.2006442546844,9.071292450392671e-07
51254,153762,0,153762,660.1787431240082,8.967201197550455e-07
51335,154005,0,154005,661.1769931316376,8.856038895295746e-07
51416,154248,0,154248,662.1669580936432,8.754610493591227e-07
51497,154491,0,154491,663.1600000858307,8.653501536959438e-07
51577,154731,0,154731,664.1340799331665,8.551723924579907e-07
51658,154974,0,154974,665.126894235611,8.444906243868554e-07
51739,155217,0,155217,666.1021921634674,8.345873657928628e-07
51819,155457,0,155457,667.0892651081085,8.251075196219255e-07
51900,155700,0,155700,668.0657069683075,8.150025131154973e-07
51981,155943,0,155943,669.0547392368317,8.038387820371657e-07
52062,156186,0,156186,670.0783972740173,7.927025977729405e-07
52142,156426,0,156426,671.1294510364532,7.824188154935469e-07
52223,156669,0,156669,672.1847763061523,7.720247504876115e-07
52304,156912,0,156912,673.2872252464294,7.62777208210536e-07
52384,157152,0,157152,674.3247621059418,7.542963802853742e-07
52465,157395,0,157395,675.3729913234711,7.451683453291219e-07
52546,157638,0,157638,676.4834370613098,7.358871316996487e-07
52627,157881,0,157881,677.6013412475586,7.273296953220709e-07
52707,158121,0,158121,678.5831651687622,7.183285353846352e-07
52788,158364,0,158364,679.5665531158447,7.102297492426302e-07
52869,158607,0,158607,680.5524532794952,7.015345280907807e-07
52950,158850,0,158850,681.5393903255463,6.931859385008576e-07
53030,159090,0,159090,682.5205721855164,6.848536703035208e-07
53111,159333,0,159333,683.5106720924377,6.76592780164335e-07
53192,159576,0,159576,684.5133621692657,6.685322377283015e-07
53272,159816,0,159816,685.4830090999603,6.609721557212757e-07
53353,160059,0,160059,686.4684300422668,6.53190783038286e-07
53434,160302,0,160302,687.4643051624298,6.444101469713111e-07
53515,160545,0,160545,688.5540981292725,6.345573731878413e-07
53595,160785,0,160785,689.5366570949554,6.268683482987676e-07
53676,161028,0,161028,690.9589900970459,6.195282978816697e-07
53757,161271,0,161271,692.0919380187988,6.108528238908876e-07
53837,161511,0,161511,693.366800069809,6.036398058803796e-07
53918,161754,0,161754,694.8188591003418,5.967888560723387e-07
53999,161997,0,161997,695.8806340694427,5.8986865712815e-07
54080,162240,0,162240,697.0360932350159,5.829917207635249e-07
54160,162480,0,162480,698.394314289093,5.761449852414903e-07
54241,162723,0,162723,699.7002260684967,5.696900897846539e-07
54322,162966,0,162966,700.8361411094666,5.631720237044722e-07
54402,163206,0,163206,701.9322690963745,5.562354508349563e-07
54483,163449,0,163449,703.178697347641,5.491779533172514e-07
54564,163692,0,163692,704.4039573669434,5.417849802516875e-07
54645,163935,0,163935,705.4299902915955,5.355417340665507e-07
54725,164175,0,164175,706.4324793815613,5.294077620656792e-07
54806,164418,0,164418,707.4213533401489,5.232025362290644e-07
54887,164661,0,164661,708.8366861343384,5.170973240367281e-07
54967,164901,0,164901,710.0430183410645,5.103656287696002e-07
55048,165144,0,165144,712.2740621566772,5.040910389981217e-07
55129,165387,0,165387,713.440838098526,4.981761704679595e-07
55210,165630,0,165630,714.4303641319275,4.920856159495648e-07
55290,165870,0,165870,715.3984682559967,4.842862677465382e-07
55371,166113,0,166113,716.3865621089935,4.780132558572223e-07
55452,166356,0,166356,717.3941791057587,4.7261891219334875e-07
55532,166596,0,166596,718.3516461849213,4.6723049545346854e-07
55613,166839,0,166839,719.3443331718445,4.6118734036549435e-07
55694,167082,0,167082,720.3341870307922,4.5543679123839807e-07
55775,167325,0,167325,721.3388242721558,4.4966458826716333e-07
55855,167565,0,167565,722.3323471546173,4.443960187642256e-07
55936,167808,0,167808,723.3315541744232,4.3917499300391026e-07
56017,168051,0,168051,724.3307361602783,4.331567288297316e-07
56097,168291,0,168291,725.2836892604828,4.2811466370458605e-07
56178,168534,0,168534,726.2833631038666,4.229555106405524e-07
56259,168777,0,168777,727.2821941375732,4.178855383136236e-07
56340,169020,0,169020,728.290271282196,4.123678156457122e-07
56420,169260,0,169260,729.2672202587128,4.0701891790617744e-07
56501,169503,0,169503,730.2565021514893,4.021092981070933e-07
56582,169746,0,169746,731.2749791145325,3.97482757197119e-07
56662,169986,0,169986,732.2651121616364,3.929093839380588e-07
56743,170229,0,170229,733.2722842693329,3.8810059825777276e-07
56824,170472,0,170472,734.258542060852,3.8329029460917905e-07
56905,170715,0,170715,735.2864460945129,3.789196274504232e-07
56985,170955,0,170955,736.2234652042389,3.7474946102372676e-07
57066,171198,0,171198,737.1540122032166,3.705765794104164e-07
57147,171441,0,171441,738.1473162174225,3.6581798770025556e-07
57227,171681,0,171681,739.0753161907196,3.616727307468893e-07
57308,171924,0,171924,740.0186631679535,3.574073761167997e-07
57389,172167,0,172167,741.130410194397,3.532930132143596e-07
57470,172410,0,172410,742.1465473175049,3.4896743849081536e-07
57550,172650,0,172650,743.2979121208191,3.4457472537339574e-07
57631,172893,0,172893,744.275003194809,3.406646881496375e-07
57712,173136,0,173136,745.2067880630493,3.365410368443703e-07
57792,173376,0,173376,746.2421622276306,3.3260120562625696e-07
57873,173619,0,173619,747.2854731082916,3.288316115146902e-07
57954,173862,0,173862,748.4614503383636,3.24385676914022e-07
58035,174105,0,174105,749.6896362304688,3.2029700987513944e-07
58115,174345,0,174345,750.7308542728424,3.16353530268085e-07
58196,174588,0,174588,751.640691280365,3.121084637219063e-07
58277,174831,0,174831,752.7389991283417,3.0752353394147807e-07
58357,175071,0,175071,753.7435622215271,3.034655134822391e-07
58438,175314,0,175314,754.7611210346222,2.998011910276632e-07
58519,175557,0,175557,755.7262289524078,2.9640670334813917e-07
58600,175800,0,175800,756.7333121299744,2.930425502738339e-07
58680,176040,0,176040,757.8145883083344,2.8974465218015807e-07
58761,176283,0,176283,758.8414142131805,2.8646740713654845e-07
58842,176526,0,176526,759.8256561756134,2.8315112751013534e-07
58922,176766,0,176766,760.7830011844635,2.799841843470536e-07
59003,177009,0,177009,761.7333731651306,2.7672873102074534e-07
59084,177252,0,177252,762.7039411067963,2.73366498304352e-07
59165,177495,0,177495,763.7061471939087,2.6980408090337326e-07
59245,177735,0,177735,764.6685853004456,2.666589701422103e-07
59326,177978,0,177978,765.7294273376465,2.6329456249310113e-07
59407,178221,0,178221,766.9089632034302,2.599373571320903e-07
59487,178461,0,178461,767.9071569442749,2.568658456677521e-07
59568,178704,0,178704,768.9965691566467,2.5391655088783036e-07
59649,178947,0,178947,770.0086901187897,2.5087813238071466e-07
59730,179190,0,179190,771.0857400894165,2.480398514840979e-07
59810,179430,0,179430,772.1357712745667,2.4515864562589214e-07
59891,179673,0,179673,773.1282851696014,2.4204524705923046e-07
59972,179916,0,179916,774.1434643268585,2.384537584082937e-07
60052,180156,0,180156,775.110062122345,2.3569305239509883e-07
60133,180399,0,180399,776.100554227829,2.3288328204405646e-07
60214,180642,0,180642,777.1297471523285,2.301220472936791e-07
60295,180885,0,180885,778.4257509708405,2.2761838423037262e-07
60375,181125,0,181125,779.537750005722,2.2510447860266348e-07
60456,181368,0,181368,780.4747681617737,2.226485676463608e-07
60537,181611,0,181611,781.425555229187,2.2005455878438145e-07
60618,181854,0,181854,782.3729200363159,2.1711498985962484e-07
60698,182094,0,182094,783.7717821598053,2.1428840214563683e-07
60779,182337,0,182337,784.71679520607,2.1182461985121644e-07
60860,182580,0,182580,785.7127270698547,2.0932082245471687e-07
60940,182820,0,182820,786.7180693149567,2.0655531793868869e-07
61021,183063,0,183063,787.6297290325165,2.03687350396514e-07
61102,183306,0,183306,788.5424020290375,2.0083105964705568e-07
61183,183549,0,183549,789.4383971691132,1.9837069570249646e-07
61263,183789,0,183789,790.3205230236053,1.960681682502312e-07
61344,184032,0,184032,791.2082500457764,1.9380221026041903e-07
61425,184275,0,184275,792.1162922382355,1.914213906781907e-07
61505,184515,0,184515,792.999231338501,1.889490526219643e-07
61586,184758,0,184758,793.904886007309,1.8647909472855743e-07
61667,185001,0,185001,794.7955513000488,1.8414100213942238e-07
61748,185244,0,185244,795.6897232532501,1.8168531677891274e-07
61828,185484,0,185484,796.5779991149902,1.7918745356072573e-07
61909,185727,0,185727,797.4542970657349,1.7699874569812475e-07
61990,185970,0,185970,798.3603000640869,1.7493854717802205e-07
62070,186210,0,186210,799.2428662776947,1.7283693764233066e-07
62151,186453,0,186453,800.1415662765503,1.707475390426392e-07
62232,186696,0,186696,801.0521941184998,1.6822070454473353e-07
62313,186939,0,186939,801.9395792484283,1.659116614122422e-07
62393,187179,0,187179,802.8329961299896,1.640803637433141e-07
62474,187422,0,187422,803.7210080623627,1.622409383036632e-07
62555,187665,0,187665,804.6258392333984,1.603377094925803e-07
62635,187905,0,187905,805.5011200904846,1.5847400954422034e-07
62716,188148,0,188148,806.3941969871521,1.5661166876264622e-07
62797,188391,0,188391,807.3030190467834,1.54784682078637e-07
62878,188634,0,188634,808.2108919620514,1.530140584012006e-07
62958,188874,0,188874,809.0977461338043,1.5125703032099004e-07
63039,189117,0,189117,809.9855341911316,1.493858275202795e-07
63120,189360,0,189360,810.885231256485,1.4766132196910677e-07
63200,189600,0,189600,811.7747230529785,1.4591003063699802e-07
63281,189843,0,189843,812.6731812953949,1.4371290268303773e-07
63362,190086,0,190086,813.5707061290741,1.411730368744625e-07
63443,190329,0,190329,814.4591763019562,1.3937780931911772e-07
63523,190569,0,190569,815.3492243289948,1.3775291896540768e-07
63604,190812,0,190812,816.2356312274933,1.361053015458188e-07
63685,191055,0,191055,817.1282112598419,1.3452566065759986e-07
63765,191295,0,191295,818.01629114151,1.3282280450028082e-07
63846,191538,0,191538,818.896154165268,1.3103260508998937e-07
63927,191781,0,191781,819.7943332195282,1.2913198554346628e-07
64008,192024,0,192024,820.6799993515015,1.275551484503531e-07
64088,192264,0,192264,821.5602931976318,1.261288538125974e-07
64169,192507,0,192507,822.4531493186951,1.245466841942326e-07
64250,192750,0,192750,823.346363067627,1.2307443963351046e-07
64330,192990,0,192990,824.2311992645264,1.216691135622767e-07
64411,193233,0,193233,825.1230940818787,1.2026082913519838e-07
64492,193476,0,193476,826.0184302330017,1.1879253609512997e-07
64573,193719,0,193719,826.9060142040253,1.1731350665115544e-07
64653,193959,0,193959,827.7846562862396,1.1597610811712089e-07
64734,194202,0,194202,828.6886100769043,1.1439343738628103e-07
64815,194445,0,194445,829.5693881511688,1.1277220252803983e-07
64895,194685,0,194685,830.4513840675354,1.1146708940159478e-07
64976,194928,0,194928,831.3469862937927,1.0999367326196501e-07
65057,195171,0,195171,832.2451839447021,1.0864063410145678e-07
65138,195414,0,195414,833.1444611549377,1.0741466265813645e-07
65218,195654,0,195654,834.0250751972198,1.0616228978460562e-07
65299,195897,0,195897,834.9196982383728,1.048043789172652e-07
65380,196140,0,196140,835.8142120838165,1.0331376381481127e-07
65460,196380,0,196380,836.6991271972656,1.0203899318043924e-07
65541,196623,0,196623,837.6158950328827,1.0087713134729978e-07
65622,196866,0,196866,838.5025551319122,9.967445721723814e-08
65703,197109,0,197109,839.3966012001038,9.842182255896307e-08
65783,197349,0,197349,840.2716221809387,9.722999298187672e-08
65864,197592,0,197592,841.1786532402039,9.594968141429208e-08
65945,197835,0,197835,842.0728101730347,9.485143009494407e-08
66025,198075,0,198075,842.9539232254028,9.378736138119117e-08
66106,198318,0,198318,843.8665761947632,9.275113164200344e-08
66187,198561,0,198561,844.755383014679,9.170653319626913e-08
66268,198804,0,198804,845.6631932258606,9.047328194170179e-08
66348,199044,0,199044,846.5485641956329,8.934296367465562e-08
66429,199287,0,199287,847.4766161441803,8.825656572199044e-08
66510,199530,0,199530,848.4170973300934,8.726374681672423e-08
66590,199770,0,199770,849.3428809642792,8.627005840726135e-08
66671,200013,0,200013,850.2901382446289,8.523167595327812e-08
66752,200256,0,200256,851.3643431663513,8.413217722554494e-08
66833,200499,0,200499,852.3970251083374,8.314343353263649e-08
66913,200739,0,200739,853.4421119689941,8.220968025891248e-08
66994,200982,0,200982,854.4272701740265,8.127675103929872e-08
67075,201225,0,201225,855.401015996933,8.034020024903309e-08
67155,201465,0,201465,856.2893822193146,7.939087165154297e-08
67236,201708,0,201708,857.1936461925507,7.840776762828963e-08
67317,201951,0,201951,858.0894801616669,7.747101934239955e-08
67398,202194,0,202194,858.9889500141144,7.651144741368084e-08
67478,202434,0,202434,859.8760361671448,7.561744499674314e-08
67559,202677,0,202677,860.7791132926941,7.461839420123173e-08
67640,202920,0,202920,861.6829171180725,7.372503051204359e-08
67720,203160,0,203160,862.5788090229034,7.27740197945749e-08
67801,203403,0,203403,863.4820141792297,7.184414798084608e-08
67882,203646,0,203646,864.3759431838989,7.100047326043176e-08
67963,203889,0,203889,865.2836573123932,7.015618172931456e-08
68043,204129,0,204129,866.1980781555176,6.9275620240548e-08
68124,204372,0,204372,867.1347062587738,6.844582915182549e-08
68205,204615,0,204615,868.0553162097931,6.762369820951593e-08
68285,204855,0,204855,868.9522061347961,6.680619879652525e-08
68366,205098,0,205098,869.8875381946564,6.598579765181763e-08
68447,205341,0,205341,870.8010311126709,6.50970854179892e-08
68528,205584,0,205584,871.6998870372772,6.417230550111293e-08
68608,205824,0,205824,872.5895352363586,6.322064581419618e-08
68689,206067,0,206067,873.4815862178802,6.246798015815812e-08
68770,206310,0,206310,874.3842780590057,6.173915548540316e-08
68851,206553,0,206553,875.2757661342621,6.103128208768966e-08
68931,206793,0,206793,876.2571151256561,6.021681120988601e-08
69012,207036,0,207036,877.2488460540771,5.9462287544064524e-08
69093,207279,0,207279,878.2985022068024,5.872782723079215e-08
69173,207519,0,207519,879.3276510238647,5.8071082840882155e-08
69254,207762,0,207762,880.2783091068268,5.7425757764555105e-08
69335,208005,0,208005,881.1787111759186,5.669042997340267e-08
69416,208248,0,208248,882.0666670799255,5.602749842638723e-08
69496,208488,0,208488,882.9534740447998,5.5334386428442945e-08
69577,208731,0,208731,883.8438541889191,5.460730286144479e-08
69658,208974,0,208974,884.7442831993103,5.3958838117421334e-08
69738,209214,0,209214,885.6200833320618,5.3350382333485885e-08
69819,209457,0,209457,886.5098810195923,5.272420893086978e-08
69900,209700,0,209700,887.4059519767761,5.213624955905513e-08
69981,209943,0,209943,888.2991251945496,5.1541687998789754e-08
70061,210183,0,210183,889.1910603046417,5.096549524639667e-08
70142,210426,0,210426,890.0832660198212,5.036282007678217e-08
70223,210669,0,210669,890.9808020591736,4.975114074513109e-08
70303,210909,0,210909,891.8596971035004,4.920730415449812e-08
70384,211152,0,211152,892.8581602573395,4.8599692927177735e-08
70465,211395,0,211395,893.8521473407745,4.8016123802964405e-08
70546,211638,0,211638,894.843120098114,4.744508631807766e-08
70626,211878,0,211878,895.852833032608,4.6817385237339666e-08
70707,212121,0,212121,896.7379519939423,4.622697879538841e-08
70788,212364,0,212364,897.6573832035065,4.565483132322711e-08
70868,212604,0,212604,898.536609172821,4.4982464995962364e-08
70949,212847,0,212847,899.4941880702972,4.442499848653815e-08
71030,213090,0,213090,900.5119481086731,4.3906829197186e-08
71111,213333,0,213333,901.4683382511139,4.340852776790437e-08
71191,213573,0,213573,902.4826669692993,4.28563804677737e-08
71272,213816,0,213816,903.4250411987305,4.229989661372699e-08
71353,214059,0,214059,904.4631900787354,4.1783894499687114e-08
71433,214299,0,214299,905.3453192710876,4.131211693243385e-08
71514,214542,0,214542,906.2552759647369,4.079849018701583e-08
71595,214785,0,214785,907.145524263382,4.029268576313134e-08
71676,215028,0,215028,908.0431361198425,3.980364424154585e-08
71756,215268,0,215268,908.9218831062317,3.932720844991519e-08
71837,215511,0,215511,909.8020341396332,3.8869000321816135e-08
71918,215754,0,215754,910.7006492614746,3.842876770361828e-08
71998,215994,0,215994,911.5829241275787,3.7980681929652913e-08
72079,216237,0,216237,912.4732391834259,3.7546482522007253e-08
72160,216480,0,216480,913.3706691265106,3.711347581153508e-08
72241,216723,0,216723,914.3204343318939,3.667461660360431e-08
72321,216963,0,216963,915.2077231407166,3.617939454079023e-08
72402,217206,0,217206,916.0965051651001,3.555883715436353e-08
72483,217449,0,217449,916.9889063835144,3.4947607798421336e-08
72563,217689,0,217689,917.8731231689453,3.44778624947751e-08
72644,217932,0,217932,918.7665781974792,3.394426893242253e-08
72725,218175,0,218175,919.6686503887177,3.3283202926847035e-08
72806,218418,0,218418,920.5633180141449,3.273628802023906e-08
72886,218658,0,218658,921.4538552761078,3.2286211000274716e-08
72967,218901,0,218901,922.346931219101,3.179364417376546e-08
73048,219144,0,219144,923.2418763637543,3.143405094321134e-08
73128,219384,0,219384,924.1402730941772,3.108439357310815e-08
73209,219627,0,219627,925.0333223342896,3.073047098253282e-08
73290,219870,0,219870,925.930474281311,3.032583525922226e-08
73371,220113,0,220113,926.8320572376251,2.9869238065072715e-08
73451,220353,0,220353,927.7272613048553,2.948117226163062e-08
73532,220596,0,220596,928.6513311862946,2.912865853022082e-08
73613,220839,0,220839,929.634124994278,2.8798981517619408e-08
73693,221079,0,221079,930.6359171867371,2.846592926320367e-08
73774,221322,0,221322,931.6143500804901,2.8120889992762496e-08
73855,221565,0,221565,932.6448712348938,2.7781170829488354e-08
73936,221808,0,221808,933.631637096405,2.7460182085864134e-08
74016,222048,0,222048,934.6681971549988,2.7113386665776168e-08
74097,222291,0,222291,935.5930511951447,2.6795461852781946e-08
74178,222534,0,222534,936.4768922328949,2.648749729408174e-08
74258,222774,0,222774,937.3712959289551,2.6188639833127655e-08
74339,223017,0,223017,938.257847070694,2.588775224888217e-08
74420,223260,0,223260,939.1635823249817,2.5581937493622185e-08
74501,223503,0,223503,940.0458722114563,2.5286001196021694e-08
74581,223743,0,223743,940.9175040721893,2.4996339525114803e-08
74662,223986,0,223986,941.8085989952087,2.4708454261052366e-08
74743,224229,0,224229,942.698046207428,2.438224805882196e-08
74823,224469,0,224469,943.5903143882751,2.4101975945417076e-08
74904,224712,0,224712,944.4715812206268,2.382593011658333e-08
74985,224955,0,224955,945.3793902397156,2.3531850532307275e-08
75066,225198,0,225198,946.2704360485077,2.32473371104662e-08
75146,225438,0,225438,947.147613286972,2.2993404570718276e-08
75227,225681,0,225681,948.0486409664154,2.2730758060572946e-08
75308,225924,0,225924,948.933895111084,2.2456378706610354e-08
75388,226164,0,226164,949.8181862831116,2.2202634766342186e-08
75469,226407,0,226407,950.7102739810944,2.1945767546257168e-08
75550,226650,0,226650,951.6000211238861,2.1687041993568232e-08
75631,226893,0,226893,952.5021879673004,2.1423387085598933e-08
75711,227133,0,227133,953.3836002349854,2.1165586559640587e-08
75792,227376,0,227376,954.2918100357056,2.090796533456048e-08
75873,227619,0,227619,955.1829102039337,2.0636906427955986e-08
75953,227859,0,227859,956.071857213974,2.039474474267415e-08
76034,228102,0,228102,957.0384492874146,2.013865225231108e-08
76115,228345,0,228345,958.0832431316376,1.9882123355551508e-08
76196,228588,0,228588,959.0511300563812,1.9650182963491314e-08
76276,228828,0,228828,959.9987812042236,1.9352941227185247e-08
76357,229071,0,229071,960.9558181762695,1.905149810137536e-08
76438,229314,0,229314,961.880232334137,1.8810116085819577e-08
76518,229554,0,229554,962.7731292247772,1.857031161521524e-08
76599,229797,0,229797,963.75923204422,1.835286446940648e-08
76680,230040,0,230040,964.7330982685089,1.8116928411561804e-08
76761,230283,0,230283,965.6753401756287,1.790102374793967e-08
76841,230523,0,230523,966.6430780887604,1.769605136685407e-08
76922,230766,0,230766,967.8439872264862,1.750086847176048e-08
77003,231009,0,231009,968.938285112381,1.7293304750605303e-08
77084,231252,0,231252,969.9148080348969,1.707323564593434e-08
77164,231492,0,231492,970.7939450740814,1.6860575943072575e-08
77245,231735,0,231735,971.772824048996,1.666694147247108e-08
77326,231978,0,231978,972.7700700759888,1.6473731370733043e-08
77406,232218,0,232218,973.7786569595337,1.6288383180934982e-08
77487,232461,0,232461,974.7079651355743,1.6079929009122865e-08
77568,232704,0,232704,975.6153931617737,1.5884814519790404e-08
77649,232947,0,232947,976.531387090683,1.5687028394155958e-08
77729,233187,0,233187,977.4122381210327,1.550140947647424e-08
77810,233430,0,233430,978.3476121425629,1.5322697615034088e-08
77891,233673,0,233673,979.2634701728821,1.5137867583922058e-08
77971,233913,0,233913,980.1705992221832,1.4949784230970968e-08
78052,234156,0,234156,981.0737912654877,1.4764333878209806e-08
78133,234399,0,234399,981.9776341915131,1.4595799188839316e-08
78214,234642,0,234642,982.8995640277863,1.44227494772913e-08
78294,234882,0,234882,983.8446581363678,1.4203783118124382e-08
78375,235125,0,235125,984.8703191280365,1.4026971509176022e-08
78456,235368,0,235368,985.8847050666809,1.3864044978239717e-08
78536,235608,0,235608,986.8831751346588,1.3710428744989397e-08
78617,235851,0,235851,987.8936071395874,1.3538694675089312e-08
78698,236094,0,236094,988.9774310588837,1.3384367107067192e-08
78779,236337,0,236337,989.9961311817169,1.3231282214232228e-08
78859,236577,0,236577,991.118643283844,1.3082167738669648e-08
78940,236820,0,236820,992.2337710857391,1.2930103243473856e-08
79021,237063,0,237063,993.4094982147217,1.2780094255332154e-08
79101,237303,0,237303,994.445652961731,1.2630310375081759e-08
79182,237546,0,237546,995.439070224762,1.248200718940627e-08
79263,237789,0,237789,996.5035660266876,1.2329955482837858e-08
79344,238032,0,238032,997.4391143321991,1.2184661761036052e-08
79424,238272,0,238272,998.3659310340881,1.2043795017026338e-08
79505,238515,0,238515,999.5904240608215,1.1884258677019082e-08
79586,238758,0,238758,1000.7630572319031,1.1724532862008892e-08
79666,238998,0,238998,1001.7329850196838,1.1589404179443818e-08
79747,239241,0,239241,1002.6943731307983,1.1448631747648767e-08
79828,239484,0,239484,1003.6987042427063,1.1293209519242333e-08
79909,239727,0,239727,1004.7500221729279,1.11517584708479e-08
79989,239967,0,239967,1005.6809930801392,1.1012320240755549e-08
80070,240210,0,240210,1007.3818881511688,1.0888540684155097e-08
80151,240453,0,240453,1008.7387020587921,1.076349191687153e-08
80231,240693,0,240693,1010.0119452476501,1.064183705219615e-08
80312,240936,0,240936,1011.1586651802063,1.0498198560384532e-08
80393,241179,0,241179,1012.2761881351471,1.0358514538174821e-08
80474,241422,0,241422,1013.341117143631,1.0236379903292454e-08
80554,241662,0,241662,1014.4755623340607,1.0114850702076874e-08
80635,241905,0,241905,1015.5418121814728,9.999789548452178e-09


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/flex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0006730556488037109,30.358106049564984
100,423,0,423,9.699470043182373,0.6740708090137648
200,904,0,904,19.293302059173584,0.36479367437778243
300,1398,0,1398,30.14501118659973,0.3011071376998588
400,1898,0,1898,41.2958869934082,0.27284904918698316
501,2403,0,2403,51.33675408363342,0.2513713270154871
601,2903,0,2903,62.01597213745117,0.234106610900458
701,3403,0,3403,72.63560199737549,0.21948271100161407
801,3903,0,3903,83.10749697685242,0.20671330437256502
901,4403,0,4403,93.06895780563354,0.19533775315508978
1001,4903,0,4903,102.56371402740479,0.18508769923021168
1101,5403,0,5403,112.03076696395874,0.17574157451435118
1201,5903,0,5903,121.87506914138794,0.16718224618280828
1301,6403,0,6403,132.27479004859924,0.1592768985844412
1401,6903,0,6903,144.16654109954834,0.1519401173686006
1502,7408,0,7408,154.95235800743103,0.14506500219313892
1602,7908,0,7908,167.59047603607178,0.1387179106376333
1702,8408,0,8408,180.78743600845337,0.13278191151715082
1802,8908,0,8908,191.2439830303192,0.12719265855275141
1902,9408,0,9408,201.48468589782715,0.1219400560136374
2002,9908,0,9908,211.64182591438293,0.11701191228993676
2102,10408,0,10408,223.53338313102722,0.11236629569478193
2202,10908,0,10908,234.19905924797058,0.1079741884630845
2302,11408,0,11408,244.99614310264587,0.10381508154336361
2402,11908,0,11908,255.05940914154053,0.09987308583851982
2503,12413,0,12413,265.158056974411,0.09610822382464428
2603,12913,0,12913,276.82814717292786,0.09255337945643131
2703,13413,0,13413,288.7055678367615,0.08917858033816427
2803,13913,0,13913,298.69650411605835,0.08597224804076486
2903,14413,0,14413,309.3056402206421,0.08291247365497094
3003,14913,0,14913,319.35656118392944,0.08000772731563129
3103,15413,0,15413,329.2388961315155,0.07724586090048079
3203,15913,0,15913,339.0263350009918,0.07461367196444577
3303,16413,0,16413,348.7440061569214,0.07208114636080319
3403,16913,0,16913,358.83766198158264,0.06967606694973875
3504,17418,0,17418,368.7782881259918,0.06735533287282698
3604,17918,0,17918,380.54287099838257,0.0651705839756705
3704,18418,0,18418,391.6623890399933,0.06307331943822765
3804,18918,0,18918,401.6895110607147,0.061069200263926635
3904,19418,0,19418,412.3128261566162,0.059158459188021435
4004,19918,0,19918,422.791640996933,0.05732596943137648
4104,20418,0,20418,433.3351631164551,0.05557071732301238
4204,20918,0,20918,443.52463603019714,0.05388292866896858
4304,21418,0,21418,453.3360779285431,0.05226988215909881
4404,21918,0,21918,463.94493794441223,0.05073371062024936
4505,22423,0,22423,473.92792320251465,0.049239908680385955
4605,22923,0,22923,484.96298480033875,0.047811337373014344
4705,23423,0,23423,495.05528497695923,0.04644612916767309
4805,23923,0,23923,505.56760907173157,0.045138535468762855
4905,24423,0,24423,516.5812230110168,0.043876713568457695
5005,24923,0,24923,527.3454110622406,0.042667078190062255
5105,25423,0,25423,538.0618500709534,0.04150156967641493
5205,25923,0,25923,548.302276134491,0.040382780754147994
5305,26423,0,26423,558.2923929691315,0.03930801613506081
5405,26923,0,26923,569.6716032028198,0.038272359434075295
5506,27428,0,27428,580.1642160415649,0.03727117225157682
5606,27928,0,27928,591.4966111183167,0.036313514972909265
5706,28428,0,28428,603.2202050685883,0.03539102472124249
5806,28928,0,28928,615.5168859958649,0.03450565883793069
5906,29428,0,29428,626.8991320133209,0.03365118833915721
6006,29928,0,29928,638.1180880069733,0.03282710655393964
6106,30428,0,30428,649.4500699043274,0.032030826600110085
6206,30928,0,30928,660.9912848472595,0.031251986584151854
6306,31428,0,31428,671.9112968444824,0.030508918236367304
6406,31928,0,31928,681.8826060295105,0.029793637817455157
6507,32433,0,32433,692.0171658992767,0.029095611888973298
6607,32933,0,32933,701.9363031387329,0.02843036289544006
6707,33433,0,33433,711.8595790863037,0.027781592628328324
6807,33933,0,33933,721.8995070457458,0.027152829857074155
6907,34433,0,34433,731.6549100875854,0.026538935137007263
7007,34933,0,34933,741.6377792358398,0.02595172271031554
7107,35433,0,35433,751.6755850315094,0.02538157140054715
7207,35933,0,35933,761.9250719547272,0.024834885215656122
7307,36433,0,36433,772.5627608299255,0.024298489003464614
7407,36933,0,36933,783.2905461788177,0.02377729330308051
7508,37438,0,37438,794.0686919689178,0.023275230739235382
7608,37938,0,37938,805.6115131378174,0.02279203498650222
7708,38438,0,38438,817.3950800895691,0.022322806772084865
7808,38938,0,38938,829.3922560214996,0.021865528571221024
7908,39438,0,39438,840.5269300937653,0.021419479492325068
8008,39938,0,39938,850.5700421333313,0.02098867118647162
8108,40438,0,40438,860.5083179473877,0.020572205964901655
8208,40938,0,40938,870.4831459522247,0.02016582322980434
8308,41438,0,41438,880.3280801773071,0.01977047541984274
8408,41938,0,41938,890.2508971691132,0.019389799980957342
8509,42443,0,42443,901.1762101650238,0.019011432923092448
8609,42943,0,42943,911.14927983284,0.018643052388337335
8709,43443,0,43443,921.5642149448395,0.018285644353247893
8809,43943,0,43943,931.7266509532928,0.01794423210894945
8909,44443,0,44443,944.0602648258209,0.017609809355168732
9009,44943,0,44943,955.7249300479889,0.017283162120705936
9109,45443,0,45443,968.0701911449432,0.016964699513328976
9209,45943,0,45943,979.5202269554138,0.016655877057779756
9309,46443,0,46443,990.6654980182648,0.016353440897675802
9409,46943,0,46943,1000.8383059501648,0.016060743806844174
9510,47448,0,47448,1012.6331398487091,0.015769300195604255
9610,47948,0,47948,1024.1976990699768,0.015487873408863198
9710,48448,0,48448,1037.8917889595032,0.01521403141112706
9810,48948,0,48948,1049.1274650096893,0.014943237769159498
9910,49448,0,49448,1060.8081979751587,0.014682259050626364
10010,49948,0,49948,1071.976175069809,0.014423437798893483
10110,50448,0,50448,1084.1940269470215,0.014171277133404974
10210,50948,0,50948,1095.340166091919,0.01392333594599989
10310,51448,0,51448,1106.6179921627045,0.013682338157944274
10410,51948,0,51948,1118.0536391735077,0.013447507339058948
10511,52453,0,52453,1128.1963860988617,0.01321293134250753
10611,52953,0,52953,1138.5358068943024,0.012989574657526023
10711,53453,0,53453,1149.5386338233948,0.012768769040499405
10811,53953,0,53953,1159.6291601657867,0.012556441467346625
10911,54453,0,54453,1169.4987869262695,0.012349143740692738
11011,54953,0,54953,1179.5461390018463,0.01214524355860213
11111,55453,0,55453,1189.547888994217,0.011947266766893203
11211,55953,0,55953,1199.7248990535736,0.011751695137031887
11311,56453,0,56453,1210.1026470661163,0.011559599614786942
11411,56953,0,56953,1221.7343001365662,0.011371096600628265
11512,57458,0,57458,1234.2979729175568,0.011186639526794611
11612,57958,0,57958,1245.2664771080017,0.0110072713543146
11712,58458,0,58458,1256.0167319774628,0.010831155361876243
11812,58958,0,58958,1268.3479030132294,0.010658408334752617
11912,59458,0,59458,1279.9490900039673,0.010486890162832036
12012,59958,0,59958,1290.2467019557953,0.010320351943382359
12112,60458,0,60458,1300.134365081787,0.010157743210582122
12212,60958,0,60958,1310.082113981247,0.009998570256356795
12312,61458,0,61458,1319.9124610424042,0.00984163501184768
12412,61958,0,61958,1329.6916460990906,0.009687127901705582
12513,62463,0,62463,1340.343815088272,0.009534941649700859
12613,62963,0,62963,1350.4492959976196,0.00938868992799043
12713,63463,0,63463,1360.2311689853668,0.009241979730494933
12813,63963,0,63963,1369.8919689655304,0.009097986425696137
12913,64463,0,64463,1379.7811110019684,0.008957248416518902
13013,64963,0,64963,1389.614872932434,0.008818201482802683
13113,65463,0,65463,1399.2509980201721,0.00868249810425601
13213,65963,0,65963,1409.0612919330597,0.008548064509870506
13313,66463,0,66463,1418.9324080944061,0.008416005396848438
13413,66963,0,66963,1428.7228798866272,0.008287377199784856
13514,67468,0,67468,1438.553619146347,0.008159888099818451
13614,67968,0,67968,1448.5758690834045,0.008034419436160416
13714,68468,0,68468,1459.4919679164886,0.007913611752316004
13814,68968,0,68968,1469.9276340007782,0.007795390316821144
13914,69468,0,69468,1480.1929891109467,0.007677743815105847
14014,69968,0,69968,1490.2318949699402,0.007562860481353119
14114,70468,0,70468,1500.4205849170685,0.007450605242903559
14214,70968,0,70968,1512.4886538982391,0.007340636657919483
14314,71468,0,71468,1523.2430560588837,0.007231841509013097
14414,71968,0,71968,1534.38387799263,0.00712416435095943
14515,72473,0,72473,1545.5344948768616,0.007017012543646849
14615,72973,0,72973,1557.550113916397,0.006914271553971753
14715,73473,0,73473,1571.8863739967346,0.006814068949784387
14815,73973,0,73973,1585.2750871181488,0.006714731852956441
14915,74473,0,74473,1596.212457895279,0.006616603931633526
15015,74973,0,74973,1606.6555409431458,0.006520031544543469
15115,75473,0,75473,1616.9285678863525,0.006425897019206822
15215,75973,0,75973,1627.102919101715,0.006332988037277899
15315,76473,0,76473,1637.5276579856873,0.0062413727734129
15415,76973,0,76973,1648.013345003128,0.006152090206288771
15516,77478,0,77478,1659.0314919948578,0.006063241357561435
15616,77978,0,77978,1669.8793561458588,0.0059757368861365805
15716,78478,0,78478,1679.9648249149323,0.005889920085292591
15816,78978,0,78978,1690.3627171516418,0.0058055010224595084
15916,79478,0,79478,1700.636183977127,0.005722752804225829
16016,79978,0,79978,1710.8188710212708,0.005640623693481606
16116,80478,0,80478,1723.4660189151764,0.005559186804897125
16216,80978,0,80978,1735.31405210495,0.005478765407526689
16316,81478,0,81478,1746.2166528701782,0.005399980840299835
16416,81978,0,81978,1757.2159872055054,0.0053234970975538495
16517,82483,0,82483,1767.9029412269592,0.005246187465325018
16617,82983,0,82983,1777.981750011444,0.005169919168812627
16717,83483,0,83483,1788.2994439601898,0.005095591710316658
16817,83983,0,83983,1798.3705258369446,0.005023072144022762
16917,84483,0,84483,1808.396311044693,0.004950929151437472
17017,84983,0,84983,1818.3841049671173,0.004880086256069801
17117,85483,0,85483,1828.5262398719788,0.004811328271177826
17217,85983,0,85983,1839.1046750545502,0.004742862582062508
17317,86483,0,86483,1849.5185267925262,0.004676545072588412
17417,86983,0,86983,1859.5849928855896,0.004611783740845919
17518,87488,0,87488,1869.7007129192352,0.0045464589241467615
17618,87988,0,87988,1879.7228882312775,0.004482863327512462
17718,88488,0,88488,1889.8140211105347,0.004420565297487159
17818,88988,0,88988,1900.3921859264374,0.004358859020481772
17918,89488,0,89488,1911.3747289180756,0.004298649030839239
18018,89988,0,89988,1922.3947660923004,0.004239974742757932
18118,90488,0,90488,1934.451828956604,0.004181856626744563
18218,90988,0,90988,1946.0246698856354,0.0041244299516009445
18318,91488,0,91488,1957.5522480010986,0.004067760539698059
18418,91988,0,91988,1968.596971988678,0.0040118943588045184
18519,92493,0,92493,1979.6483471393585,0.003956686811520169
18619,92993,0,92993,1989.5692410469055,0.0039028743511904385
18719,93493,0,93493,2000.7066910266876,0.0038498559976971668
18819,93993,0,93993,2011.4981219768524,0.00379690826235795
18919,94493,0,94493,2023.023059129715,0.0037446131980354196
19019,94993,0,94993,2033.502333164215,0.003693937852466599
19119,95493,0,95493,2044.1939160823822,0.003643936854438327
19219,95993,0,95993,2054.6254019737244,0.0035934791019181455
19319,96493,0,96493,2065.5397329330444,0.0035436462446997857
19419,96993,0,96993,2076.525779247284,0.0034946011434185665
19520,97498,0,97498,2088.421856880188,0.0034456566818429034
19620,97998,0,97998,2099.9350969791412,0.0033980930796209544
19720,98498,0,98498,2111.536989927292,0.00335146003228404
19820,98998,0,98998,2122.7096660137177,0.00330542664071531
19920,99498,0,99498,2134.9520611763,0.0032601993139334583
20020,99998,0,99998,2146.1293098926544,0.003215795253064266
20120,100498,0,100498,2156.7036378383636,0.0031717673149927856
20220,100998,0,100998,2167.7782320976257,0.0031287050460743733
20320,101498,0,101498,2178.990291118622,0.003086363301907172
20420,101998,0,101998,2189.954290151596,0.003044445551693037
20521,102503,0,102503,2201.237939119339,0.003002888075763937
20621,103003,0,103003,2212.2980678081512,0.0029627838629593117
20721,103503,0,103503,2223.615624189377,0.002923467941498095
20821,104003,0,104003,2234.6899812221527,0.0028843921347016734
20921,104503,0,104503,2246.304037094116,0.002845777648144417
21021,105003,0,105003,2257.4469170570374,0.002807604420269065
21121,105503,0,105503,2267.7689850330353,0.002769985193498142
21221,106003,0,106003,2278.3883991241455,0.002733459822412864
21321,106503,0,106503,2289.9377069473267,0.0026978773884618443
21421,107003,0,107003,2300.036851167679,0.0026623464651141624
21522,107508,0,107508,2311.3211500644684,0.0026264289794471363
21622,108008,0,108008,2323.0846149921417,0.0025916193404392565
21722,108508,0,108508,2334.5994980335236,0.0025579546784296786
21822,109008,0,109008,2344.7696890830994,0.002524605794318878
21922,109508,0,109508,2355.329129934311,0.002491127632570393
22022,110008,0,110008,2366.1014540195465,0.0024578116424554754
22122,110508,0,110508,2376.3520691394806,0.002424961584814794
22222,111008,0,111008,2387.1287038326263,0.0023927861578514503
22322,111508,0,111508,2398.808699131012,0.0023609871178997513
22422,112008,0,112008,2409.445496082306,0.0023294175969082037
22523,112513,0,112513,2420.378399848938,0.002297924573733798
22623,113013,0,113013,2431.156378030777,0.0022673511708853006
22723,113513,0,113513,2441.5369188785553,0.0022368688187186956
22823,114013,0,114013,2452.4181020259857,0.0022065841664088244
22923,114513,0,114513,2463.393405199051,0.0021773461430529164
23023,115013,0,115013,2474.069747209549,0.002148654163350126
23123,115513,0,115513,2484.856570959091,0.0021199231946575975
23223,116013,0,116013,2496.0955300331116,0.0020914531135217424
23323,116513,0,116513,2507.2227470874786,0.002063706162551783
23423,117013,0,117013,2518.055771112442,0.002036499504599918
23524,117518,0,117518,2529.393872976303,0.0020093881755093514
23624,118018,0,118018,2540.6054809093475,0.001982709735082616
23724,118518,0,118518,2551.240509033203,0.0019561014206939077
23824,119018,0,119018,2562.076261997223,0.0019302603745496515
23924,119518,0,119518,2573.6392302513123,0.0019053454353859243
24024,120018,0,120018,2584.430788040161,0.0018806693008264134
24124,120518,0,120518,2595.309977054596,0.0018559450999957043
24224,121018,0,121018,2606.504457950592,0.0018315873716478475
24324,121518,0,121518,2617.153336048126,0.0018077804981858035
24424,122018,0,122018,2627.7042989730835,0.001784454642912226
24525,122523,0,122523,2638.1886451244354,0.001761209015094746
24625,123023,0,123023,2652.4952681064606,0.001738391988894958
24725,123523,0,123523,2664.1773421764374,0.00171586423485638
24825,124023,0,124023,2675.329486131668,0.0016935761857893345
24925,124523,0,124523,2685.6356739997864,0.0016715839296080578
25025,125023,0,125023,2695.5852320194244,0.0016499198063745875
25125,125523,0,125523,2705.47967004776,0.0016285428820247592
25225,126023,0,126023,2715.3987679481506,0.0016075924236171844
25325,126523,0,126523,2725.428989171982,0.0015867531763290267
25425,127023,0,127023,2735.258108139038,0.0015658059260057534
25526,127528,0,127528,2746.1808359622955,0.0015451444418893383
25626,128028,0,128028,2757.429119825363,0.0015253098082737766
25726,128528,0,128528,2769.2243649959564,0.0015054972300539602
25826,129028,0,129028,2779.19335603714,0.001485658988449537
25926,129528,0,129528,2789.3767268657684,0.0014660199308520123
26026,130028,0,130028,2799.4655232429504,0.0014467936258351932
26126,130528,0,130528,2810.6020560264587,0.001427990732161791
26226,131028,0,131028,2822.444680929184,0.0014092965002787707
26326,131528,0,131528,2833.286127090454,0.0013906476526894666
26426,132028,0,132028,2844.106440782547,0.001372328535017738
26527,132533,0,132533,2854.1336619853973,0.0013543540128066133
26627,133033,0,133033,2865.0407269001007,0.0013368473809247214
26727,133533,0,133533,2875.7185368537903,0.0013193386765255664
26827,134033,0,134033,2886.70029091835,0.0013020111015608902
26927,134533,0,134533,2897.2351191043854,0.0012851365408325561
27027,135033,0,135033,2909.5016429424286,0.0012685326536822016
27127,135533,0,135533,2920.6220610141754,0.0012520846679355017
27227,136033,0,136033,2932.4789202213287,0.0012359650670930196
27327,136533,0,136533,2944.3751668930054,0.0012201408011003109
27427,137033,0,137033,2956.187180042267,0.0012045337051295054
27528,137538,0,137538,2967.347860813141,0.0011889538197235156
27628,138038,0,138038,2978.3903341293335,0.0011737633960006634
27728,138538,0,138538,2988.4745378494263,0.001159006846744811
27828,139038,0,139038,2998.5308899879456,0.0011445533289527732
27928,139538,0,139538,3008.649559020996,0.0011300831995496015
28028,140038,0,140038,3019.242676973343,0.0011156508556234065
28128,140538,0,140538,3029.5465109348297,0.0011014996204924891
28228,141038,0,141038,3039.560481071472,0.0010877816852691465
28328,141538,0,141538,3049.548295021057,0.0010742364195470795
28428,142038,0,142038,3059.584760904312,0.001060561563204573
28529,142543,0,142543,3069.873728990555,0.0010467721196679356
28629,143043,0,143043,3082.125308036804,0.0010333276400003775
28729,143543,0,143543,3094.005252122879,0.001020061240369355
28829,144043,0,144043,3104.0048570632935,0.0010070101018600408
28929,144543,0,144543,3113.9865849018097,0.0009940971974781159
29029,145043,0,145043,3123.9651350975037,0.000981219744957462
29129,145543,0,145543,3134.2727541923523,0.0009685331546077873
29229,146043,0,146043,3145.138696193695,0.0009560472782302953
29329,146543,0,146543,3155.305980205536,0.0009437195548886938
29429,147043,0,147043,3165.5753259658813,0.0009315581817663742
29530,147548,0,147548,3175.7362768650055,0.0009193600921322451
29630,148048,0,148048,3186.603451013565,0.0009074241261998246
29730,148548,0,148548,3197.3450758457184,0.0008957086455786554
29830,149048,0,149048,3208.7932970523834,0.0008841907846550142
29930,149548,0,149548,3220.082731962204,0.0008728574992763401
30030,150048,0,150048,3231.5073561668396,0.0008617020424861686
30130,150548,0,150548,3242.758847951889,0.0008506497334819705
30230,151048,0,151048,3253.341505050659,0.0008397281367189477
30330,151548,0,151548,3263.9292089939117,0.0008290370498930587
30430,152048,0,152048,3275.066766023636,0.0008186622279307561
30531,152553,0,152553,3286.536719083786,0.0008084208423240097
30631,153053,0,153053,3297.751591205597,0.000798282359315857
30731,153553,0,153553,3307.9708340168,0.000788147202886754
30831,154053,0,154053,3319.026332139969,0.0007782398130713101
30931,154553,0,154553,3329.44251704216,0.0007686620024254315
31031,155053,0,155053,3340.012946128845,0.0007592367536939216
31131,155553,0,155553,3350.8919909000397,0.0007497737075312852
31231,156053,0,156053,3361.204619884491,0.0007403085738802685
31331,156553,0,156553,3372.3822388648987,0.0007309587843850111
31431,157053,0,157053,3384.4223189353943,0.0007217810233619198
31532,157558,0,157558,3396.237493991852,0.000712683668522996
31632,158058,0,158058,3406.8846728801727,0.0007037663169281105
31732,158558,0,158558,3419.962462902069,0.0006948741795556393
31832,159058,0,159058,3431.159548997879,0.0006860266726231893
31932,159558,0,159558,3441.3197770118713,0.0006772414696078435
32032,160058,0,160058,3451.2048139572144,0.0006685827834672235
32132,160558,0,160558,3461.5287709236145,0.000660081657837168
32232,161058,0,161058,3472.9723591804504,0.0006516862415802117
32332,161558,0,161558,3484.501163959503,0.0006433685659208209
32432,162058,0,162058,3495.945027112961,0.0006350972787162443
32533,162563,0,162563,3507.18661403656,0.0006268495826922653
32633,163063,0,163063,3519.25572180748,0.0006188660737521514
32733,163563,0,163563,3531.4071238040924,0.0006109919566066389
32833,164063,0,164063,3541.318706035614,0.0006031590939862547
32933,164563,0,164563,3551.117156982422,0.0005953726448863385
33033,165063,0,165063,3561.048539161682,0.0005877081411343943
33133,165563,0,165563,3570.868008852005,0.0005802879828078687
33233,166063,0,166063,3581.6455929279327,0.0005730434328837904
33333,166563,0,166563,3592.8631222248077,0.0005657733459171801
33433,167063,0,167063,3604.600296020508,0.0005585136075059691
33534,167568,0,167568,3616.593600988388,0.0005513825762683625
33634,168068,0,168068,3627.925632953644,0.0005445406263639869
33734,168568,0,168568,3641.015226125717,0.0005377888213738135
33834,169068,0,169068,3655.4783000946045,0.0005310529670369452
33934,169568,0,169568,3669.0734169483185,0.0005243854838288612
34034,170068,0,170068,3682.604264974594,0.000517831328721706
34134,170568,0,170568,3696.2952330112457,0.0005113676747452104
34234,171068,0,171068,3707.7795989513397,0.0005050098629617553
34334,171568,0,171568,3719.447010040283,0.00049876465823154
34434,172068,0,172068,3731.1519269943237,0.00049259800225575
34535,172573,0,172573,3742.3255751132965,0.00048640436343996184
34635,173073,0,173073,3752.4785430431366,0.0004802655788187519
34735,173573,0,173573,3762.590150117874,0.0004742093471004622
34835,174073,0,174073,3773.7791390419006,0.00046833814235534523
34935,174573,0,174573,3784.5149841308594,0.00046255593506026025
35035,175073,0,175073,3794.9408628940582,0.0004567417559355909
35135,175573,0,175573,3806.5286231040955,0.0004509403254617686
35235,176073,0,176073,3818.0886929035187,0.0004452489705895118
35335,176573,0,176573,3829.545721054077,0.00043968320882483726
35435,177073,0,177073,3840.4341008663177,0.0004341618047082116
35536,177578,0,177578,3850.8316111564636,0.0004285787620269132
35636,178078,0,178078,3861.076411008835,0.0004231109704062924
35736,178578,0,178578,3871.5602831840515,0.000417754151896793
35836,179078,0,179078,3881.842430114746,0.0004124976682262871
35936,179578,0,179578,3892.650361061096,0.0004072915540156594
36036,180078,0,180078,3902.9509768486023,0.00040209175212119734
36136,180578,0,180578,3913.0800700187683,0.0003969624072696761
36236,181078,0,181078,3923.2705760002136,0.00039194998090848215
36336,181578,0,181578,3933.602425098419,0.0003869921380551484
36436,182078,0,182078,3944.1750168800354,0.0003820833837071302
36537,182583,0,182583,3954.5932910442352,0.00037721896684675903
36637,183083,0,183083,3964.9579350948334,0.00037247645990617516
36737,183583,0,183583,3975.144170999527,0.0003677983537082144
36837,184083,0,184083,3985.300096988678,0.0003632073892757746
36937,184583,0,184583,3995.521896123886,0.00035872169287079296
37037,185083,0,185083,4005.375247001648,0.0003543231172937472
37137,185583,0,185583,4015.2529859542847,0.0003499555631106733
37237,186083,0,186083,4025.297404050827,0.0003456091543287095
37337,186583,0,186583,4035.3080911636353,0.00034133904036296543
37437,187083,0,187083,4047.33403301239,0.0003371897041997399
37538,187588,0,187588,4061.1254189014435,0.0003330940770030127
37638,188088,0,188088,4074.0332090854645,0.00032904613341672536
37738,188588,0,188588,4086.394381046295,0.0003249776189030221
37838,189088,0,189088,4102.193630933762,0.00032095873374849646
37938,189588,0,189588,4119.534715175629,0.00031702222306425227
38038,190088,0,190088,4135.752055883408,0.00031313764609344373
38138,190588,0,190588,4151.646120786667,0.00030928319204809014
38238,191088,0,191088,4167.047230243683,0.0003054462282524585
38338,191588,0,191588,4182.352931022644,0.0003016392954409308
38438,192088,0,192088,4197.769783973694,0.0002978876644134703
38539,192593,0,192593,4213.78545498848,0.00029414997270711386
38639,193093,0,193093,4230.038600921631,0.0002904760483259826
38739,193593,0,193593,4246.434118032455,0.0002868238988232153
38839,194093,0,194093,4262.640264034271,0.0002832135956908058
38939,194593,0,194593,4279.589560031891,0.0002796467182235892
39039,195093,0,195093,4296.195240974426,0.0002761159716255151
39139,195593,0,195593,4312.778830051422,0.00027263345480684793
39239,196093,0,196093,4328.883623123169,0.00026919021860002734
39339,196593,0,196593,4346.072429895401,0.0002657728031629332
39439,197093,0,197093,4361.5704691410065,0.00026240807660154433
39540,197598,0,197598,4377.396242141724,0.0002590910973433425
39640,198098,0,198098,4393.116788864136,0.00025588265341784086
39740,198598,0,198598,4409.757657051086,0.0002527241050797486
39840,199098,0,199098,4425.880966186523,0.0002495867002298357
39940,199598,0,199598,4441.948101043701,0.0002464799047741714
40040,200098,0,200098,4458.030071973801,0.00024344507406500032
40140,200598,0,200598,4474.289134979248,0.00024049217401295308
40240,201098,0,201098,4490.09783911705,0.00023758925035202111
40340,201598,0,201598,4505.819542884827,0.0002346974720580825
40440,202098,0,202098,4522.433734178543,0.00023181002222996108
40541,202603,0,202603,4538.322981119156,0.00022892956364527054
40641,203103,0,203103,4554.054399967194,0.00022614114331804207
40741,203603,0,203603,4570.510680913925,0.00022341837448286615
40841,204103,0,204103,4586.327925920486,0.00022072753023352708
40941,204603,0,204603,4601.550536155701,0.00021802439763574777
41041,205103,0,205103,4616.743934869766,0.0002153160438144532
41141,205603,0,205603,4632.020478248596,0.00021264765748837884
41241,206103,0,206103,4647.64825797081,0.0002100345412956692
41341,206603,0,206603,4663.386606931686,0.00020745813187193632
41441,207103,0,207103,4679.035411834717,0.00020490261520566503
41542,207608,0,207608,4694.72914814949,0.00020233465972032793
41642,208108,0,208108,4710.382244110107,0.000199802884274177
41742,208608,0,208608,4727.360029935837,0.00019729182682935609
41842,209108,0,209108,4744.93544793129,0.00019481621710768968
41942,209608,0,209608,4761.359313011169,0.0001923755958623994
42042,210108,0,210108,4777.545238018036,0.0001899588719947242
42142,210608,0,210608,4793.727998256683,0.00018756344101920325
42242,211108,0,211108,4809.673326015472,0.0001851956797072706
42342,211608,0,211608,4825.901910066605,0.0001828731912447905
42442,212108,0,212108,4842.284168243408,0.00018059845025777968
42543,212613,0,212613,4858.905063152313,0.00017831601776185699
42643,213113,0,213113,4875.176419019699,0.00017606275381638659
42743,213613,0,213613,4891.423650979996,0.00017385303972389696
42843,214113,0,214113,4907.281273126602,0.00017170521327511962
42943,214613,0,214613,4923.398113965988,0.00016959968472830621
43043,215113,0,215113,4938.465106010437,0.00016750607326702926
43143,215613,0,215613,4953.645373106003,0.00016541434271077386
43243,216113,0,216113,4968.637050151825,0.00016335144342275186
43343,216613,0,216613,4984.335066080093,0.00016134497849539813
43443,217113,0,217113,5000.016824007034,0.0001593898471032139
43544,217618,0,217618,5016.038820981979,0.0001574400345603422
43644,218118,0,218118,5031.447181940079,0.00015551106209193895
43744,218618,0,218618,5046.764511823654,0.0001535865154520082
43844,219118,0,219118,5060.537490129471,0.00015168479499473708
43944,219618,0,219618,5071.468253850937,0.00014981951633575002
44044,220118,0,220118,5084.250503063202,0.00014800011208480985
44144,220618,0,220618,5095.068859100342,0.00014621436322828963
44244,221118,0,221118,5105.955325126648,0.00014442878139451362
44344,221618,0,221618,5116.180061101913,0.00014263665106754294
44444,222118,0,222118,5126.776809930801,0.00014086422000602705
44545,222623,0,222623,5136.680850028992,0.00013911567700658194
44645,223123,0,223123,5149.801614046097,0.0001374183201096502
44745,223623,0,223623,5160.80236697197,0.00013572641144805178
44845,224123,0,224123,5171.212321996689,0.0001340328188139223
44945,224623,0,224623,5182.8889808654785,0.00013236112328072992
45045,225123,0,225123,5193.261703014374,0.00013072490474152403
45145,225623,0,225623,5204.158057928085,0.00012911114446064365
45245,226123,0,226123,5214.659335136414,0.0001275024555124265
45345,226623,0,226623,5225.636590957642,0.00012590161085567313
45445,227123,0,227123,5235.858992099762,0.0001243253689193958
45546,227628,0,227628,5246.176659107208,0.00012276184114542522
45646,228128,0,228128,5256.821223020554,0.00012123236403793853
45746,228628,0,228628,5268.682576179504,0.00011971705681063681
45846,229128,0,229128,5279.8755848407745,0.00011821828297044659
45946,229628,0,229628,5290.658276081085,0.00011674246354088736
46046,230128,0,230128,5302.027095079422,0.00011529636776283101
46146,230628,0,230628,5312.606182098389,0.00011387938281053799
46246,231128,0,231128,5323.567645072937,0.00011248413550743903
46346,231628,0,231628,5333.8440721035,0.00011110133225261212
46446,232128,0,232128,5345.98227596283,0.00010973060229597501
46547,232633,0,232633,5357.968587875366,0.00010837044060160703
46647,233133,0,233133,5369.910881996155,0.00010705609787735993
46747,233633,0,233633,5380.724584102631,0.00010577023960898871
46847,234133,0,234133,5391.075186014175,0.00010449901468025544
46947,234633,0,234633,5402.657609939575,0.00010323012198943327
47047,235133,0,235133,5414.355530977249,0.0001019711063233136
47147,235633,0,235633,5425.338212013245,0.00010073847118361565
47247,236133,0,236133,5436.322461843491,9.95332678283808e-05
47347,236633,0,236633,5447.608019113541,9.834313200863676e-05
47447,237133,0,237133,5459.032230138779,9.715722569053257e-05
47548,237638,0,237638,5468.938488006592,9.596396705510397e-05
47648,238138,0,238138,5480.643612146378,9.479710229733944e-05
47748,238638,0,238638,5491.835803985596,9.364910772111053e-05
47848,239138,0,239138,5502.464318037033,9.251380757307025e-05
47948,239638,0,239638,5513.385139226913,9.13867477461328e-05
48048,240138,0,240138,5524.085081100464,9.026786264199883e-05
48148,240638,0,240638,5534.6294901371,8.915781353468074e-05
48248,241138,0,241138,5545.310627937317,8.805773416627259e-05
48348,241638,0,241638,5556.044322013855,8.69675689652116e-05
48448,242138,0,242138,5566.0253229141235,8.588622089057175e-05
48549,242643,0,242643,5576.991172075272,8.480414492731312e-05
48649,243143,0,243143,5586.782181978226,8.374749475827166e-05
48749,243643,0,243643,5596.789686918259,8.270959085165348e-05
48849,244143,0,244143,5608.708170890808,8.168875746491998e-05
48949,244643,0,244643,5619.888361930847,8.06798311353179e-05
49049,245143,0,245143,5630.383345127106,7.968206226361594e-05
49149,245643,0,245643,5640.4056968688965,7.870088224222207e-05
49249,246143,0,246143,5650.5806131362915,7.773961196312214e-05
49349,246643,0,246643,5664.6444981098175,7.679457098557647e-05
49449,247143,0,247143,5675.3483710289,7.586140452421898e-05
49550,247648,0,247648,5686.687590122223,7.492898581986418e-05
49650,248148,0,248148,5697.687673091888,7.401539953566568e-05
49750,248648,0,248648,5709.435055017471,7.311576962833046e-05
49850,249148,0,249148,5720.492058038712,7.223622243787864e-05
49950,249648,0,249648,5731.650343179703,7.137692837144109e-05
50050,250148,0,250148,5742.451267004013,7.052945389542406e-05
50150,250648,0,250648,5754.456598997116,6.96812230872659e-05
50250,251148,0,251148,5766.383048057556,6.883077822095232e-05
50350,251648,0,251648,5776.532115936279,6.799313079537122e-05
50450,252148,0,252148,5788.189209938049,6.717832156914836e-05
50551,252653,0,252653,5799.261986017227,6.63699769841229e-05
50651,253153,0,253153,5811.425168991089,6.557122498319466e-05
50751,253653,0,253653,5822.612858057022,6.477172120144465e-05
50851,254153,0,254153,5833.877405166626,6.39785325928235e-05
50951,254653,0,254653,5845.606907129288,6.3196892000334e-05
51051,255153,0,255153,5856.48584318161,6.242540291110463e-05
51151,255653,0,255653,5866.708245038986,6.166159549818611e-05
51251,256153,0,256153,5876.728462934494,6.090383717036853e-05
51351,256653,0,256653,5887.35281920433,6.015023768958237e-05
51451,257153,0,257153,5898.7205810546875,5.940073889040863e-05
51552,257658,0,257658,5911.1345472335815,5.8651865665582604e-05
51652,258158,0,258158,5925.064723968506,5.792444861161008e-05
51752,258658,0,258658,5939.021440029144,5.721048972807709e-05
51852,259158,0,259158,5950.682116031647,5.6502167509600485e-05
51952,259658,0,259658,5961.630486965179,5.5798308658219694e-05
52052,260158,0,260158,5972.797118902206,5.510701241845707e-05
52152,260658,0,260658,5984.750582933426,5.443082609636523e-05
52252,261158,0,261158,5996.236657142639,5.376211681440372e-05
52352,261658,0,261658,6006.32682800293,5.309523238551592e-05
52452,262158,0,262158,6016.70072221756,5.243602968171447e-05
52553,262663,0,262663,6029.032459020615,5.178827310196105e-05
52653,263163,0,263163,6041.968382835388,5.116432646511327e-05
52753,263663,0,263663,6052.81179690361,5.0546094355125655e-05
52853,264163,0,264163,6064.334852933884,4.992475474952824e-05
52953,264663,0,264663,6076.129531145096,4.9305458189211e-05
53053,265163,0,265163,6086.65403008461,4.870146174345732e-05
53153,265663,0,265663,6097.275139093399,4.811701072913669e-05
53253,266163,0,266163,6109.2286829948425,4.754425147170306e-05
53353,266663,0,266663,6119.959048986435,4.6974322415576416e-05
53453,267163,0,267163,6133.7770228385925,4.6403347753107346e-05
53554,267668,0,267668,6146.680429935455,4.582793347846726e-05
53654,268168,0,268168,6158.142493009567,4.52666957593962e-05
53754,268668,0,268668,6170.289953947067,4.4719194940977955e-05
53854,269168,0,269168,6181.105171918869,4.4183427521040305e-05
53954,269668,0,269668,6192.268524885178,4.365136830142839e-05
54054,270168,0,270168,6204.213971853256,4.31167376149825e-05
54154,270668,0,270668,6215.025235176086,4.258290992679035e-05
54254,271168,0,271168,6225.477875947952,4.205908285827396e-05
54354,271668,0,271668,6236.485089063644,4.1548568653170534e-05
54454,272168,0,272168,6246.922183036804,4.104464310971055e-05
54555,272673,0,272673,6257.59080696106,4.053456050487089e-05
54655,273173,0,273173,6268.075711011887,4.003101014439587e-05
54755,273673,0,273673,6279.13339805603,3.9536609048265145e-05
54855,274173,0,274173,6290.79912686348,3.905074868028278e-05
54955,274673,0,274673,6302.76767206192,3.856746088754561e-05
55055,275173,0,275173,6313.452828168869,3.808667433350143e-05
55155,275673,0,275673,6324.294550895691,3.761361509352135e-05
55255,276173,0,276173,6336.340926170349,3.715133146176335e-05
55355,276673,0,276673,6346.533806085587,3.669761805121421e-05
55455,277173,0,277173,6357.025889873505,3.624803255944671e-05
55556,277678,0,277678,6367.056698083878,3.579695148717814e-05
55656,278178,0,278178,6379.1499218940735,3.535638456565927e-05
55756,278678,0,278678,6391.788635015488,3.492468851005458e-05
55856,279178,0,279178,6402.51203083992,3.4501966117265636e-05
55956,279678,0,279678,6412.714081048965,3.408698164918513e-05
56056,280178,0,280178,6424.369830131531,3.367725370251476e-05
56156,280678,0,280678,6436.093647956848,3.3269482232394996e-05
56256,281178,0,281178,6447.307321071625,3.286428965720167e-05
56356,281678,0,281678,6459.3706040382385,3.24669249857232e-05
56456,282178,0,282178,6471.490961074829,3.208024682398501e-05
56557,282683,0,282683,6482.914742946625,3.169744112148325e-05
56657,283183,0,283183,6494.129553079605,3.1321034590272914e-05
56757,283683,0,283683,6505.204050064087,3.094515801096704e-05
56857,284183,0,284183,6515.903891086578,3.057238034810527e-05
56957,284683,0,284683,6526.247464895248,3.020649591614506e-05
57057,285183,0,285183,6536.924968957901,2.9847595156331716e-05
57157,285683,0,285683,6546.851748943329,2.9492154503065965e-05
57257,286183,0,286183,6556.6168801784515,2.913746429593703e-05
57357,286683,0,286683,6566.864846944809,2.8784420646033977e-05
57457,287183,0,287183,6577.05441904068,2.843532848160415e-05
57558,287688,0,287688,6587.2089920043945,2.8087189030733185e-05
57658,288188,0,288188,6597.35404419899,2.7745860106050404e-05
57758,288688,0,288688,6607.326265096664,2.7407162839921218e-05
57858,289188,0,289188,6617.126899957657,2.7071326266381847e-05
57958,289688,0,289688,6627.1219618320465,2.6739190178275027e-05
58058,290188,0,290188,6637.546228885651,2.6410925229716104e-05
58158,290688,0,290688,6648.207372903824,2.6086367958370422e-05
58258,291188,0,291188,6659.602993011475,2.5766683252885666e-05
58358,291688,0,291688,6670.1374168396,2.5452975440638598e-05
58458,292188,0,292188,6681.113091945648,2.514404787451879e-05
58559,292693,0,292693,6692.361999034882,2.4835147731110157e-05
58659,293193,0,293193,6703.0110239982605,2.453267844457917e-05
58759,293693,0,293693,6713.4556839466095,2.423452607592489e-05
58859,294193,0,294193,6723.779681921005,2.3940369527728506e-05
58959,294693,0,294693,6733.762773990631,2.3649905073596144e-05
59059,295193,0,295193,6744.086612939835,2.3364383810442608e-05
59159,295693,0,295693,6753.886604070663,2.3085114829939177e-05
59259,296193,0,296193,6763.924510002136,2.2811124086163103e-05
59359,296693,0,296693,6774.61822104454,2.2539297566656647e-05
59459,297193,0,297193,6784.747424840927,2.2268166985798894e-05
59560,297698,0,297698,6795.346617937088,2.1998025226468197e-05
59660,298198,0,298198,6805.752916812897,2.1737482353724425e-05
59760,298698,0,298698,6816.246340036392,2.1482166447829375e-05
59860,299198,0,299198,6826.596555948257,2.122781924720474e-05
59960,299698,0,299698,6837.983086109161,2.0973127821090152e-05
60060,300198,0,300198,6849.00009894371,2.072045241848122e-05
60160,300698,0,300698,6859.638548851013,2.0472132603119684e-05
60260,301198,0,301198,6870.9410190582275,2.0227903076502737e-05
60360,301698,0,301698,6881.027704954147,1.99859004894402e-05
60460,302198,0,302198,6893.978182077408,1.9744752980151056e-05
60561,302703,0,302703,6905.232540130615,1.9502097143049546e-05
60661,303203,0,303203,6916.065119981766,1.9263740048814972e-05
60761,303703,0,303703,6926.609055995941,1.9028254320624857e-05
60861,304203,0,304203,6936.42778801918,1.879640352376301e-05
60961,304703,0,304703,6949.411941051483,1.856810872955397e-05
61061,305203,0,305203,6959.861864089966,1.834152653927029e-05
61161,305703,0,305703,6969.767720937729,1.8115267056308347e-05
61261,306203,0,306203,6979.71617102623,1.7891078537923152e-05
61361,306703,0,306703,6992.218241930008,1.7671529500087545e-05
61461,307203,0,307203,7002.830684185028,1.7456300651615e-05
61562,307708,0,307708,7014.223702907562,1.724088864167901e-05
61662,308208,0,308208,7025.016810894012,1.702883657183779e-05
61762,308708,0,308708,7035.705771923065,1.6820139487432884e-05
61862,309208,0,309208,7046.708790063858,1.6616437198468514e-05
61962,309708,0,309708,7057.425010204315,1.6415781455011375e-05
62062,310208,0,310208,7068.179789066315,1.6215269491729208e-05
62162,310708,0,310708,7079.070896148682,1.6015926923471743e-05
62262,311208,0,311208,7089.849462985992,1.5821743945411168e-05
62362,311708,0,311708,7100.450437068939,1.5633682532013225e-05
62462,312208,0,312208,7110.686372041702,1.5448057925095894e-05
62563,312713,0,312713,7120.846509933472,1.5259823138989655e-05
62663,313213,0,313213,7131.936958789825,1.5073660432910923e-05
62763,313713,0,313713,7143.246261835098,1.4890539453984543e-05
62863,314213,0,314213,7153.255699872971,1.471194688591665e-05
62963,314713,0,314713,7164.991657972336,1.4537473343843078e-05
63063,315213,0,315213,7175.849265098572,1.4365525927233611e-05
63163,315713,0,315713,7186.353193998337,1.419406376977266e-05
63263,316213,0,316213,7197.1034190654755,1.4021966492575e-05
63363,316713,0,316713,7207.352340936661,1.3850582501577993e-05
63463,317213,0,317213,7217.210174798965,1.3682926077482154e-05
63564,317718,0,317718,7227.301638126373,1.351854427035557e-05
63664,318218,0,318218,7237.692618846893,1.3358002802942096e-05
63764,318718,0,318718,7248.437001943588,1.3196208161531564e-05
63864,319218,0,319218,7259.534518957138,1.3033401960233011e-05
63964,319718,0,319718,7269.617192029953,1.2872915895864413e-05
64064,320218,0,320218,7280.072406053543,1.2716411538794653e-05
64164,320718,0,320718,7290.092262983322,1.256229329689525e-05
64264,321218,0,321218,7300.259962081909,1.240884540457742e-05
64364,321718,0,321718,7311.23024892807,1.2256464403812075e-05
64464,322218,0,322218,7322.2292058467865,1.2106384198338822e-05
64565,322723,0,322723,7333.1550278663635,1.1957185940358784e-05
64665,323223,0,323223,7345.096871137619,1.1810736102235363e-05
64765,323723,0,323723,7357.874403953552,1.1665225775315255e-05
64865,324223,0,324223,7369.435894012451,1.1521857854975412e-05
64965,324723,0,324723,7380.838091850281,1.1381684996550782e-05
65065,325223,0,325223,7391.244906902313,1.1244233793864254e-05
65165,325723,0,325723,7402.2139530181885,1.110839091237824e-05
65265,326223,0,326223,7415.348847150803,1.0973628399049542e-05
65365,326723,0,326723,7426.652863025665,1.084002190681997e-05
65465,327223,0,327223,7437.020606994629,1.070808932479147e-05
65566,327728,0,327728,7447.504498004913,1.0577548709982288e-05
65666,328228,0,328228,7457.638253927231,1.0451705231888057e-05
65766,328728,0,328728,7467.821354866028,1.032857305839718e-05
65866,329228,0,329228,7480.227919101715,1.0206369491877351e-05
65966,329728,0,329728,7491.062546014786,1.0084085694189604e-05
66066,330228,0,330228,7502.000921964645,9.962796521261307e-06
66166,330728,0,330728,7512.096980810165,9.844425337186806e-06
66266,331228,0,331228,7522.149739027023,9.729233141456767e-06
66366,331728,0,331728,7532.883182048798,9.615360798668503e-06
66466,332228,0,332228,7544.056796073914,9.501110706701497e-06
66567,332733,0,332733,7555.87803196907,9.385727062177156e-06
66667,333233,0,333233,7566.945299863815,9.273100846351122e-06
66767,333733,0,333733,7579.952338218689,9.162812309478779e-06
66867,334233,0,334233,7591.248291969299,9.05419126298213e-06
66967,334733,0,334733,7601.962802171707,8.946185400333436e-06
67067,335233,0,335233,7612.834730863571,8.838327949177462e-06
67167,335733,0,335733,7622.906352043152,8.7309013665276e-06
67267,336233,0,336233,7632.966763019562,8.624506803984673e-06
67367,336733,0,336733,7644.047981023788,8.519646962427412e-06
67467,337233,0,337233,7654.224003076553,8.416529560453575e-06
67568,337738,0,337738,7664.681875944138,8.313879931990155e-06
67668,338238,0,338238,7674.693104982376,8.213176903991008e-06
67768,338738,0,338738,7685.22611284256,8.113231147006209e-06
67868,339238,0,339238,7696.519285917282,8.014448500882732e-06
67968,339738,0,339738,7707.783769130707,7.917174008170553e-06
68068,340238,0,340238,7718.804968833923,7.821235962083843e-06
68168,340738,0,340738,7731.059731245041,7.726353490189221e-06
68268,341238,0,341238,7743.393457174301,7.632733335193862e-06
68368,341738,0,341738,7754.452805042267,7.540857793780057e-06
68468,342238,0,342238,7765.899022102356,7.450726400350624e-06
68569,342743,0,342743,7777.555006027222,7.360829704940503e-06
68669,343243,0,343243,7788.8782551288605,7.272520826994498e-06
68769,343743,0,343743,7799.497274160385,7.185416877213837e-06
68869,344243,0,344243,7809.913864850998,7.10041092511972e-06
68969,344743,0,344743,7820.662106990814,7.017476141930946e-06
69069,345243,0,345243,7831.939733982086,6.935487419753565e-06
69169,345743,0,345743,7843.548296928406,6.853546824655216e-06
69269,346243,0,346243,7854.345700979233,6.772003892192333e-06
69369,346743,0,346743,7865.363977909088,6.6918603396319896e-06
69469,347243,0,347243,7876.952253103256,6.613439390162124e-06
69570,347748,0,347748,7888.399921178818,6.535255410034448e-06
69670,348248,0,348248,7898.362425088882,6.4580355621939035e-06
69770,348748,0,348748,7908.906986951828,6.380964256554013e-06
69870,349248,0,349248,7919.775504112244,6.304562553291221e-06
69970,349748,0,349748,7931.08017706871,6.229197731588296e-06
70070,350248,0,350248,7942.179601192474,6.154844301725254e-06
70170,350748,0,350748,7953.288635015488,6.0812530919903525e-06
70270,351248,0,351248,7963.603061914444,6.008062867164837e-06
70370,351748,0,351748,7973.745256900787,5.9350679201890356e-06
70470,352248,0,352248,7983.8870260715485,5.862624598788322e-06
70571,352753,0,352753,7994.222963094711,5.790686639940149e-06
70671,353253,0,353253,8004.237703084946,5.720781203751951e-06
70771,353753,0,353753,8014.349300861359,5.6515601315417865e-06
70871,354253,0,354253,8025.310355901718,5.58256227896653e-06
70971,354753,0,354753,8036.551556110382,5.514191688115782e-06
71071,355253,0,355253,8046.803771018982,5.4471488303813e-06
71171,355753,0,355753,8056.950939178467,5.381394753226443e-06
71271,356253,0,356253,8067.050184965134,5.3162605959038245e-06
71371,356753,0,356753,8077.116829872131,5.25156318847827e-06
71471,357253,0,357253,8087.104264974594,5.187943077863158e-06
71572,357758,0,357758,8097.886803150177,5.1252439720202605e-06
71672,358258,0,358258,8107.884136199951,5.064192259549665e-06
71772,358758,0,358758,8117.938899040222,5.003372443879174e-06
71872,359258,0,359258,8127.939598083496,4.942844028802305e-06
71972,359758,0,359758,8138.028110980988,4.883403931652314e-06
72072,360258,0,360258,8148.109980106354,4.825517142315816e-06
72172,360758,0,360758,8159.7845339775085,4.768811951364597e-06
72272,361258,0,361258,8170.136236906052,4.712590234626802e-06
72372,361758,0,361758,8180.233290910721,4.656510941771423e-06
72472,362258,0,362258,8190.700958967209,4.600771635839923e-06
72573,362763,0,362763,8200.763972997665,4.545319161800006e-06
72673,363263,0,363263,8211.475556135178,4.49163768046558e-06
72773,363763,0,363763,8222.078131198883,4.4390485475585575e-06
72873,364263,0,364263,8232.09399485588,4.386838637899525e-06
72973,364763,0,364763,8242.248409032822,4.3342982188364444e-06
73073,365263,0,365263,8252.175286054611,4.281576131095425e-06
73173,365763,0,365763,8262.2346200943,4.2296501639935e-06
73273,366263,0,366263,8272.853219985962,4.179175764370202e-06
73373,366763,0,366763,8282.893640041351,4.129668929193826e-06
73473,367263,0,367263,8293.163993120193,4.080178785002099e-06
73574,367768,0,367768,8303.254494905472,4.029990904521975e-06
73674,368268,0,368268,8313.2496240139,3.980724361220513e-06
73774,368768,0,368768,8323.32605791092,3.9324068003479145e-06
73874,369268,0,369268,8333.296340942383,3.884900283850381e-06
73974,369768,0,369768,8343.209218978882,3.8378132522559294e-06
74074,370268,0,370268,8353.231389045715,3.7910883191817865e-06
74174,370768,0,370768,8363.285363912582,3.74495270750956e-06
74274,371268,0,371268,8373.239120006561,3.6994887306868326e-06
74374,371768,0,371768,8383.127228021622,3.6545402768982055e-06
74474,372268,0,372268,8394.748512983322,3.610004437295071e-06
74575,372773,0,372773,8404.862775087357,3.5655550728876476e-06
74675,373273,0,373273,8415.010241985321,3.522271888103921e-06
74775,373773,0,373773,8425.035134792328,3.479859715581925e-06
74875,374273,0,374273,8434.977724075317,3.438335872023861e-06
74975,374773,0,374773,8444.935008049011,3.3974942134196173e-06
75075,375273,0,375273,8455.660915136337,3.3569935744140695e-06
75175,375773,0,375773,8465.624948978424,3.3167215376770292e-06
75275,376273,0,376273,8475.508156061172,3.2770191808049407e-06
75375,376773,0,376773,8485.63809299469,3.238339314663213e-06
75475,377273,0,377273,8495.793001890182,3.200639849545891e-06
75576,377778,0,377778,8505.812535047531,3.162932581585882e-06
75676,378278,0,378278,8515.849556922913,3.1254453042316184e-06
75776,378778,0,378778,8525.805340051651,3.088018220483115e-06
75876,379278,0,379278,8535.830066204071,3.0513405285614642e-06
75976,379778,0,379778,8546.097909927368,3.0157423691184174e-06
76076,380278,0,380278,8556.045169115067,2.98082563734777e-06
76176,380778,0,380778,8565.912060022354,2.945938597627906e-06
76276,381278,0,381278,8576.694001197815,2.910823892473102e-06
76376,381778,0,381778,8586.789266109467,2.8757570416664807e-06
76476,382278,0,382278,8596.813979148865,2.841188117774775e-06
76577,382783,0,382783,8607.062808036804,2.806981833913361e-06
76677,383283,0,383283,8618.327803134918,2.773639887322699e-06
76777,383783,0,383783,8629.469297170639,2.7405040231281728e-06
76877,384283,0,384283,8640.240701198578,2.7074447669029232e-06
76977,384783,0,384783,8651.925164937973,2.6746186950540377e-06
77077,385283,0,385283,8663.439660072327,2.6422625148284447e-06
77177,385783,0,385783,8674.401023864746,2.610430148248178e-06
77277,386283,0,386283,8684.361283063889,2.5789694714312174e-06
77377,386783,0,386783,8694.284075021744,2.5477477899275487e-06
77477,387283,0,387283,8704.403366088867,2.516831377958988e-06
77578,387788,0,387788,8714.516211986542,2.486082510242937e-06
77678,388288,0,388288,8724.568189144135,2.4561477478741123e-06
77778,388788,0,388788,8735.094249010086,2.4266042053456264e-06
77878,389288,0,389288,8745.520187139511,2.397370447835066e-06
77978,389788,0,389788,8755.776276826859,2.368549404643999e-06
78078,390288,0,390288,8765.844856977463,2.340348034409946e-06
78178,390788,0,390788,8776.663370847702,2.312812525989693e-06
78278,391288,0,391288,8786.695687055588,2.285697881548084e-06
78378,391788,0,391788,8796.759368896484,2.2587148143703633e-06
78478,392288,0,392288,8807.548408985138,2.231885488289706e-06
78579,392793,0,392793,8817.613168001175,2.205262114083957e-06
78679,393293,0,393293,8827.852659225464,2.179574121104268e-06
78779,393793,0,393793,8838.93760895729,2.1543737990090806e-06
78879,394293,0,394293,8849.883383989334,2.1293016375157224e-06
78979,394793,0,394793,8862.190739870071,2.104223237199212e-06
79079,395293,0,395293,8872.50890994072,2.0793378899130188e-06
79179,395793,0,395793,8883.631740093231,2.0548897962925964e-06
79279,396293,0,396293,8895.347617864609,2.0308694285468953e-06
79379,396793,0,396793,8907.007479906082,2.0070570583497095e-06
79479,397293,0,397293,8918.976606845856,1.983284126090729e-06
79580,397798,0,397798,8929.980680942535,1.959337509116158e-06
79680,398298,0,398298,8940.948719024658,1.9358471423802834e-06
79780,398798,0,398798,8951.548768997192,1.9127221340013505e-06
79880,399298,0,399298,8963.385838985443,1.8899760287855021e-06
79980,399798,0,399798,8976.452963113785,1.8674683572181417e-06
80080,400298,0,400298,8986.675666093826,1.84504911630453e-06
80180,400798,0,400798,8997.288135051727,1.822730084517522e-06
80280,401298,0,401298,9008.043860912323,1.8006650704767812e-06
80380,401798,0,401798,9019.685525894165,1.7789510774956006e-06
80480,402298,0,402298,9031.002485990524,1.7575092766457708e-06
80581,402803,0,402803,9041.957247018814,1.736008377650817e-06
80681,403303,0,403303,9053.494703054428,1.7149256615739081e-06
80781,403803,0,403803,9064.679111003876,1.694224009211713e-06
80881,404303,0,404303,9076.675405979156,1.6739433017325245e-06
80981,404803,0,404803,9088.728958129883,1.653918615837566e-06
81081,405303,0,405303,9100.076959848404,1.6340323035835647e-06
81181,405803,0,405803,9110.291207075119,1.614396647301692e-06
81281,406303,0,406303,9120.585021018982,1.595188215227578e-06
81381,406803,0,406803,9130.671277046204,1.576394034450736e-06
81481,407303,0,407303,9141.113435029984,1.5578271858809005e-06
81582,407808,0,407808,9153.397113084793,1.539174287682051e-06
81682,408308,0,408308,9164.156883239746,1.5208703338087525e-06
81782,408808,0,408808,9174.789902925491,1.5028880935384535e-06
81882,409308,0,409308,9184.785419940948,1.4852880986081142e-06
81982,409808,0,409808,9194.869901895523,1.467969979540936e-06
82082,410308,0,410308,9205.201012849808,1.4507735754026616e-06
82182,410808,0,410808,9216.057704210281,1.4336198508094424e-06
82282,411308,0,411308,9226.316649913788,1.4165787062829164e-06
82382,411808,0,411808,9237.442347049713,1.3998155182539427e-06
82482,412308,0,412308,9248.875534057617,1.3834235588149686e-06
82583,412813,0,412813,9260.516491889954,1.367128533762217e-06
82683,413313,0,413313,9273.894635915756,1.3510243339280215e-06
82783,413813,0,413813,9288.989939212799,1.3348636529034483e-06
82883,414313,0,414313,9307.07862997055,1.3188013965027595e-06
82983,414813,0,414813,9321.508517026901,1.3030399118081953e-06
83083,415313,0,415313,9335.148608922958,1.2875877165294154e-06
83183,415813,0,415813,9347.1849629879,1.272271387542137e-06
83283,416313,0,416313,9359.586441993713,1.2569718792905136e-06
83383,416813,0,416813,9370.791877985,1.241768459846931e-06
83483,417313,0,417313,9385.862338066101,1.226809561698296e-06
83584,417818,0,417818,9401.746915102005,1.2119654003170777e-06
83684,418318,0,418318,9417.44703412056,1.1974202555366888e-06
83784,418818,0,418818,9434.063554048538,1.1829598561404605e-06
83884,419318,0,419318,9451.605717897415,1.1686310679546217e-06
83984,419818,0,419818,9466.542996883392,1.1545103355095708e-06
84084,420318,0,420318,9479.290688037872,1.1406150658179736e-06
84184,420818,0,420818,9492.005101919174,1.126904111113114e-06
84284,421318,0,421318,9504.622109889984,1.1133391927262904e-06
84384,421818,0,421818,9520.028578996658,1.0999434662189247e-06
84484,422318,0,422318,9533.47388792038,1.08680125591519e-06
84585,422823,0,422823,9547.546399831772,1.0738497766797403e-06
84685,423323,0,423323,9561.360790967941,1.0612907740686426e-06
84785,423823,0,423823,9574.861290931702,1.0488388533110951e-06
84885,424323,0,424323,9588.487112045288,1.0363937218026013e-06
84985,424823,0,424823,9601.15775513649,1.0240374727506334e-06
85085,425323,0,425323,9615.091645002365,1.0119574546266437e-06
85185,425823,0,425823,9627.830102920532,1.0002279036832895e-06
85285,426323,0,426323,9642.542552947998,9.88709477066939e-07
85385,426823,0,426823,9655.59915304184,9.771949083304086e-07
85485,427323,0,427323,9669.32161617279,9.656266706509858e-07
85586,427828,0,427828,9682.696079015732,9.540283847683607e-07
85686,428328,0,428328,9695.490464925766,9.428041318476358e-07
85786,428828,0,428828,9708.276285171509,9.318601359038285e-07
85886,429328,0,429328,9722.775444984436,9.21047590502841e-07
85986,429828,0,429828,9736.677142858505,9.102091743055808e-07
86086,430328,0,430328,9751.191452026367,8.993390385924364e-07
86186,430828,0,430828,9764.710792064667,8.885633598470528e-07
86286,431328,0,431328,9778.272904872894,8.779833926057646e-07
86386,431828,0,431828,9791.593980073929,8.675763132781875e-07
86486,432328,0,432328,9804.823837041855,8.572519797554856e-07
86587,432833,0,432833,9818.734462022781,8.468645578197761e-07
86687,433333,0,433333,9832.866523981094,8.366543974243173e-07
86787,433833,0,433833,9846.515981912613,8.265660551735608e-07
86887,434333,0,434333,9860.538617134094,8.166024854378622e-07
86987,434833,0,434833,9874.071400880814,8.067367722541181e-07
87087,435333,0,435333,9887.07683300972,7.969640997202253e-07
87187,435833,0,435833,9900.298805952072,7.873236356098735e-07
87287,436333,0,436333,9913.12799501419,7.778678890753506e-07
87387,436833,0,436833,9925.999376058578,7.686071819970119e-07
87487,437333,0,437333,9939.52075791359,7.594861394654874e-07
87588,437838,0,437838,9952.78317785263,7.503447309879999e-07
87688,438338,0,438338,9965.406202077866,7.413655187322485e-07
87788,438838,0,438838,9978.333084106445,7.325415044509022e-07
87888,439338,0,439338,9991.488641023636,7.239395544253552e-07
87988,439838,0,439838,10004.347578048706,7.155149277502511e-07
88088,440338,0,440338,10017.165160179138,7.071486520630352e-07
88188,440838,0,440838,10030.396478176117,6.987842483304137e-07
88288,441338,0,441338,10043.297369003296,6.904980867258026e-07
88388,441838,0,441838,10056.026651144028,6.824094175438729e-07
88488,442338,0,442338,10069.02336883545,6.745346444418822e-07
88589,442843,0,442843,10082.082602977753,6.666886989286523e-07
88689,443343,0,443343,10095.540673017502,6.589189160145157e-07
88789,443843,0,443843,10108.25803399086,6.511470289268204e-07
88889,444343,0,444343,10121.039928913116,6.434507722597442e-07
88989,444843,0,444843,10134.374951124191,6.358876324817013e-07
89089,445343,0,445343,10148.264940977097,6.284461048901472e-07
89189,445843,0,445843,10161.012730121613,6.21073984934571e-07
89289,446343,0,446343,10173.661363124847,6.137305530707677e-07
89389,446843,0,446843,10186.471033096313,6.064151666382232e-07
89489,447343,0,447343,10199.385757923126,5.991615201109122e-07
89590,447848,0,447848,10212.901964902878,5.919333547295761e-07
89690,448348,0,448348,10225.714333057404,5.848721390347853e-07
89790,448848,0,448848,10238.403115034103,5.778690989340779e-07
89890,449348,0,449348,10251.078357934952,5.709035383388992e-07
89990,449848,0,449848,10263.78957104683,5.640067020564769e-07
90090,450348,0,450348,10276.35076713562,5.572220934647574e-07
90190,450848,0,450848,10289.064678192139,5.505419988977327e-07
90290,451348,0,451348,10301.83118891716,5.439215470794279e-07
90390,451848,0,451848,10314.52474784851,5.373548007262276e-07
90490,452348,0,452348,10327.07319688797,5.30893855805643e-07
90591,452853,0,452853,10340.449472904205,5.245140751246722e-07
90691,453353,0,453353,10353.376642942429,5.183089174233402e-07
90791,453853,0,453853,10367.045224189758,5.121567061821848e-07
90891,454353,0,454353,10379.859923124313,5.060548737970674e-07
90991,454853,0,454853,10392.486715078354,5.000575152824616e-07
91091,455353,0,455353,10405.314053058624,4.94199881362548e-07
91191,455853,0,455853,10417.923154115677,4.884514677237207e-07
91291,456353,0,456353,10430.571514129639,4.827546020805439e-07
91391,456853,0,456853,10444.262926101685,4.77087146026773e-07
91491,457353,0,457353,10456.925355911255,4.7147303006827536e-07
91592,457858,0,457858,10469.738337039948,4.658935648248148e-07
91692,458358,0,458358,10482.222696065903,4.6047473921125185e-07
91792,458858,0,458858,10494.986747980118,4.5514144822299656e-07
91892,459358,0,459358,10508.133114099503,4.498502128584671e-07
91992,459858,0,459858,10521.504952907562,4.445722638312317e-07
92092,460358,0,460358,10534.521472930908,4.393279957765096e-07
92192,460858,0,460858,10547.328594207764,4.341673887932187e-07
92292,461358,0,461358,10560.223947048187,4.291073454532109e-07
92392,461858,0,461858,10573.135232925415,4.241047301347092e-07
92492,462358,0,462358,10586.174937009811,4.1910748674936426e-07
92593,462863,0,462863,10599.007339000702,4.140695833550609e-07
92693,463363,0,463363,10612.064541816711,4.091405825935459e-07
92793,463863,0,463863,10624.618805885315,4.042958343224479e-07
92893,464363,0,464363,10637.746643066406,3.9950695492971593e-07
92993,464863,0,464863,10654.493494987488,3.9473872726521834e-07
93093,465363,0,465363,10669.731975078583,3.8999822328826155e-07
93193,465863,0,465863,10685.405428886414,3.853191905985674e-07
93293,466363,0,466363,10700.866775989532,3.8071448934806765e-07
93393,466863,0,466863,10714.122199058533,3.761654550541832e-07
93493,467363,0,467363,10728.293938159943,3.7165515673551745e-07
93594,467868,0,467868,10741.697640895844,3.6715155353449804e-07
93694,468368,0,468368,10754.912420034409,3.627723516319842e-07
93794,468868,0,468868,10768.439208984375,3.584817718186077e-07
93894,469368,0,469368,10781.25291800499,3.5425617427110855e-07
93994,469868,0,469868,10793.950731992722,3.5006336378189063e-07
94094,470368,0,470368,10806.909447193146,3.4589761576338323e-07
94194,470868,0,470868,10820.22015094757,3.41788180926873e-07
94294,471368,0,471368,10833.476355075836,3.377716317616492e-07
94394,471868,0,471868,10846.660092115402,3.338523163528971e-07
94494,472368,0,472368,10859.99115896225,3.299900266084305e-07
94595,472873,0,472873,10874.136531114578,3.2609612514685875e-07
94695,473373,0,473373,10887.7418050766,3.222403130137195e-07
94795,473873,0,473873,10901.060275793076,3.184308192479056e-07
94895,474373,0,474373,10914.09284901619,3.147189226859762e-07
94995,474873,0,474873,10926.993079900742,3.1110138488153563e-07
95095,475373,0,475373,10941.072956085205,3.0752029780828136e-07
95195,475873,0,475873,10954.160082101822,3.039257673050809e-07
95295,476373,0,476373,10967.299841880798,3.0032870180524155e-07
95395,476873,0,476873,10981.056184053421,2.967816506133494e-07
95495,477373,0,477373,10994.007575035095,2.93314823603615e-07
95596,477878,0,477878,11007.013916015625,2.898717945610179e-07
95696,478378,0,478378,11020.664552927017,2.864773027479392e-07
95796,478878,0,478878,11034.746318101883,2.830801499500689e-07
95896,479378,0,479378,11047.868606805801,2.79697442317601e-07
95996,479878,0,479878,11060.411998987198,2.763528094948653e-07
96096,480378,0,480378,11073.8444378376,2.7305283433312867e-07
96196,480878,0,480878,11086.450933933258,2.6978984696796766e-07
96296,481378,0,481378,11099.651950120926,2.665586193558936e-07
96396,481878,0,481878,11112.449972867966,2.6336339553895497e-07
96496,482378,0,482378,11125.6771838665,2.60210085782993e-07
96597,482883,0,482883,11138.553885936737,2.5706654168937546e-07
96697,483383,0,483383,11152.460648059845,2.5398810678479437e-07
96797,483883,0,483883,11165.196208000183,2.5094041796416254e-07
96897,484383,0,484383,11177.777813911438,2.479315489293004e-07
96997,484883,0,484883,11190.917102098465,2.4497626599950387e-07
97097,485383,0,485383,11204.116236925125,2.420795392259713e-07
97197,485883,0,485883,11217.065440893173,2.3922438097890714e-07
97297,486383,0,486383,11229.770483970642,2.3638398417627645e-07
97397,486883,0,486883,11242.722643852234,2.3355292838287652e-07
97497,487383,0,487383,11255.535018920898,2.307621329794332e-07
97598,487888,0,487888,11268.552514076233,2.2802403602709497e-07
97698,488388,0,488388,11281.13172698021,2.253929128398195e-07
97798,488888,0,488888,11293.737134933472,2.2279463636503166e-07
97898,489388,0,489388,11306.471274852753,2.2018443844183878e-07
97998,489888,0,489888,11319.118954896927,2.1756671343567745e-07
98098,490388,0,490388,11332.065693855286,2.1498479523494467e-07
98198,490888,0,490888,11344.99044919014,2.1247019592222995e-07
98298,491388,0,491388,11357.652485132217,2.100133635687261e-07
98398,491888,0,491888,11370.233179092407,2.0758136485339637e-07
98498,492388,0,492388,11382.912325143814,2.0515183591758173e-07
98599,492893,0,492893,11395.797316074371,2.0270312197099453e-07
98699,493393,0,493393,11410.707262992859,2.0030192815790147e-07
98799,493893,0,493893,11424.639863014221,1.9793972521497838e-07
98899,494393,0,494393,11439.30077791214,1.9561670399271592e-07
98999,494893,0,494893,11455.605652809143,1.9331718154504723e-07
99099,495393,0,495393,11469.480743169785,1.9102492818857112e-07
99199,495893,0,495893,11483.159214019775,1.8874075588192863e-07
99299,496393,0,496393,11495.787558078766,1.8648043337005755e-07
99399,496893,0,496893,11508.550247192383,1.8425358087527368e-07
99499,497393,0,497393,11524.668349027634,1.820528808003072e-07
99600,497898,0,497898,11538.51731300354,1.798478277600863e-07
99700,498398,0,498398,11551.692916870117,1.7768914180874953e-07
99800,498898,0,498898,11565.631859064102,1.7556845899534468e-07
99900,499398,0,499398,11579.3521630764,1.734841473779228e-07
100000,499898,0,499898,11592.777736902237,1.7141988818164217e-07


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007808208465576172,30.358106049564984
200,201,200,401,0.0998227596282959,2.414250482001093
400,401,400,801,0.22975373268127441,1.4275908626167872
601,602,601,1203,0.3741638660430908,1.0481327108822946
801,802,801,1603,0.4691016674041748,0.8429375202786947
1001,1002,1001,2003,0.5529468059539795,0.712546757650721
1201,1202,1201,2403,0.6229298114776611,0.6216049129860671
1401,1402,1401,2803,0.6938376426696777,0.5537429058139829
1602,1603,1602,3205,0.7582828998565674,0.5000986009063654
1802,1803,1802,3605,0.826683759689331,0.45667916724582736
2002,2003,2002,4005,0.8925986289978027,0.4202781269214063
2202,2203,2202,4405,0.9591360092163086,0.3891795414674984
2402,2403,2402,4805,1.0277667045593262,0.3622391831349261
2603,2604,2603,5207,1.0952939987182617,0.3384582011656795
2803,2804,2803,5607,1.1621119976043701,0.31752317710822264
3003,3004,3003,6007,1.2292418479919434,0.29883215313746203
3203,3204,3203,6407,1.2940788269042969,0.2819775426177739
3403,3404,3403,6807,1.3601548671722412,0.26670561631211803
3604,3605,3604,7209,1.4431788921356201,0.25276560852787017
3804,3805,3804,7609,1.5205450057983398,0.2401055723226409
4004,4005,4004,8009,1.585622787475586,0.22846023614234734
4204,4205,4204,8409,1.655843734741211,0.21770086095284105
4404,4405,4404,8809,1.7517130374908447,0.20775800709081435
4605,4606,4605,9211,1.8446357250213623,0.1985038770076265
4805,4806,4805,9611,1.9472477436065674,0.18990251157422125
5005,5006,5005,10011,2.0685219764709473,0.1818747411628254
5205,5206,5205,10411,2.2111048698425293,0.17434340626448766
5405,5406,5405,10811,2.3722238540649414,0.16728300153126816
5606,5607,5606,11213,2.5538408756256104,0.160633268379683
5806,5807,5806,11613,2.6838557720184326,0.15441655428221882
6006,6007,6006,12013,2.795325994491577,0.14851457510308494
6206,6207,6206,12413,2.8963546752929688,0.14294923202773954
6406,6407,6406,12813,3.02213191986084,0.13771396492213575
6607,6608,6607,13215,3.1218698024749756,0.1327078081501456
6807,6808,6807,13615,3.197584867477417,0.1279733204842423
7007,7008,7007,14015,3.270822763442993,0.1234929697394868
7207,7208,7207,14415,3.33375883102417,0.11924831821808715
7407,7408,7407,14815,3.3939709663391113,0.11520151401373714
7608,7609,7608,15217,3.4551918506622314,0.11130828412606891
7808,7809,7808,15617,3.5261318683624268,0.10763225790397134
8008,8009,8008,16017,3.587575674057007,0.10410544232711587
8208,8209,8208,16417,3.6487040519714355,0.1007179744877205
8408,8409,8408,16817,3.711887836456299,0.09746696840937676
8609,8610,8609,17219,3.772451877593994,0.09434882795438675
8809,8810,8809,17619,3.8359789848327637,0.09137534470607764
9009,9010,9009,18019,3.8959407806396484,0.0885193771554489
9209,9210,9209,18419,3.9575066566467285,0.08578457445722024
9409,9410,9409,18819,4.021582841873169,0.08316491320092234
9610,9611,9610,19221,4.085938930511475,0.08062202500580945
9810,9811,9810,19621,4.148967981338501,0.0781987404264939
10010,10011,10010,20021,4.216129779815674,0.07587040387611937
10210,10211,10210,20421,4.282110929489136,0.07362716634542461
10410,10411,10410,20821,4.3428590297698975,0.07146898013709031
10611,10612,10611,21223,4.4074718952178955,0.06939222244711075
10811,10812,10811,21623,4.470516920089722,0.06740602586817149
11011,11012,11011,22023,4.540755987167358,0.06547371912052025
11211,11212,11211,22423,4.616089820861816,0.06359931972978485
11411,11412,11411,22823,4.691934823989868,0.0618161493160939
11612,11613,11612,23225,4.77783989906311,0.06008443835215906
11812,11813,11812,23625,4.863937616348267,0.05842555290063512
12012,12013,12012,24025,4.940488815307617,0.05681918985701662
12212,12213,12212,24425,5.0184009075164795,0.05526606485487973
12412,12413,12412,24825,5.091875791549683,0.05375274885738671
12613,12614,12613,25227,5.164814710617065,0.05228513371423172
12813,12814,12813,25627,5.241544961929321,0.05087511391319227
13013,13014,13013,26027,5.328923940658569,0.049522783486822604
13213,13214,13213,26427,5.402685880661011,0.04820197361145632
13413,13414,13413,26827,5.47279691696167,0.04693521698349971
13614,13615,13614,27229,5.550067901611328,0.045706745813395094
13814,13815,13814,27629,5.628948926925659,0.04452360855372407
14014,14015,14014,28029,5.703023910522461,0.0433763721780153
14214,14215,14214,28429,5.770842790603638,0.04226061105568543
14414,14415,14414,28829,5.833544969558716,0.04118127656962729
14615,14616,14615,29231,5.907144784927368,0.0401316692196825
14815,14816,14815,29631,5.976404905319214,0.03911041866917804
15015,15016,15015,30031,6.049389839172363,0.03813405903053661
15215,15216,15215,30431,6.112715005874634,0.03719165623735689
15415,15416,15415,30831,6.176487922668457,0.03626697015308906
15616,15617,15616,31233,6.251130819320679,0.03535864291108896
15816,15817,15816,31633,6.320572853088379,0.034494222993455295
16016,16017,16016,32033,6.394276857376099,0.03365678154923456
16216,16217,16216,32433,6.469841957092285,0.032845838033466045
16416,16417,16416,32833,6.5453996658325195,0.032061208749318754
16617,16618,16617,33235,6.612817764282227,0.03129721841714124
16817,16818,16817,33635,6.7028748989105225,0.030556098940941044
17017,17018,17017,34035,6.790320873260498,0.02984051176722835
17217,17218,17217,34435,6.862180709838867,0.029142401033406744
17417,17418,17417,34835,6.929933786392212,0.028470800358547748
17618,17619,17618,35237,7.0103278160095215,0.027805739275565008
17818,17819,17818,35637,7.085132837295532,0.027168587461877294
18018,18019,18018,36037,7.172886610031128,0.026542462800522252
18218,18219,18218,36437,7.241873741149902,0.025937138597594767
18418,18419,18418,36837,7.304742813110352,0.025348137806732438
18619,18620,18619,37239,7.36555290222168,0.024778349241448845
18819,18820,18819,37639,7.432898759841919,0.024220654667310187
19019,19020,19019,38039,7.508040904998779,0.023678878924503273
19219,19220,19219,38439,7.588047742843628,0.02315031703978796
19419,19420,19419,38839,7.655030727386475,0.02264257839251141
19620,19621,19620,39241,7.72562575340271,0.022151147579476792
19820,19821,19820,39641,7.7916176319122314,0.021672090117837047
20020,20021,20020,40041,7.858196973800659,0.02120921831064929
20220,20221,20220,40441,7.925842761993408,0.02075570698828225
20420,20421,20420,40841,8.008630752563477,0.02031370878660496
20621,20622,20621,41243,8.07701563835144,0.019879977638748533
20821,20822,20821,41643,8.145489931106567,0.019461332292364485
21021,21022,21021,42043,8.210661888122559,0.01905270173018761
21221,21222,21221,42443,8.284356832504272,0.018655438567671153
21421,21422,21421,42843,8.36153769493103,0.01826461329502448
21622,21623,21622,43245,8.431259870529175,0.017883178399155375
21822,21823,21822,43645,8.51243281364441,0.017513143034382662
22022,22023,22022,44045,8.596333742141724,0.01715455890696065
22222,22223,22222,44445,8.66556978225708,0.016803639978213655
22422,22423,22422,44845,8.735138654708862,0.016460030699083934
22623,22624,22623,45247,8.817302703857422,0.016127447412081736
22823,22824,22823,45647,8.91060996055603,0.015801860181463883
23023,23024,23023,46047,9.005409002304077,0.015485163393882322
23223,23224,23223,46447,9.101175785064697,0.015178813136378878
23423,23424,23423,46847,9.214393854141235,0.014878525182719083
23624,23625,23624,47249,9.30024766921997,0.014585243934590297
23824,23825,23824,47649,9.389579057693481,0.014297362178958349
24024,24025,24024,48049,9.479281902313232,0.01401645597216914
24224,24225,24224,48449,9.575916767120361,0.013744226255763914
24424,24425,24424,48849,9.639563798904419,0.013477770026210168
24625,24626,24625,49251,9.702123880386353,0.01321594361264385
24825,24826,24825,49651,9.763345956802368,0.01296429246837232
25025,25026,25025,50051,9.831681728363037,0.012717620000985775
25225,25226,25225,50451,9.897501945495605,0.012478225383583879
25425,25426,25425,50851,9.965598821640015,0.012244582484215888
25626,25627,25626,51253,10.038213729858398,0.012015557704819681
25826,25827,25826,51653,10.103692770004272,0.01179130703147413
26026,26027,26026,52053,10.171680927276611,0.011571882118872726
26226,26227,26226,52453,10.236456871032715,0.011355654830260733
26426,26427,26426,52853,10.299535751342773,0.011148219667720513
26627,26628,26627,53255,10.36247181892395,0.010943676907023008
26827,26828,26827,53655,10.42749285697937,0.01074522513160762
27027,27028,27027,54055,10.489075899124146,0.010548775920777511
27227,27228,27227,54455,10.556520938873291,0.010358722082939848
27427,27428,27427,54855,10.620369911193848,0.010172159658524638
27628,27629,27628,55257,10.68336796760559,0.009988764060444055
27828,27829,27828,55657,10.745329856872559,0.009813163371585729
28028,28029,28028,56057,10.803769826889038,0.009638983575030355
28228,28229,28228,56457,10.866344928741455,0.009467965790070835
28428,28429,28428,56857,10.93319582939148,0.009300625776855543
28629,28630,28629,57259,11.009480953216553,0.009136602769963467
28829,28830,28829,57659,11.078519821166992,0.008975902937212192
29029,29030,29029,58059,11.13966679573059,0.008818024394642158
29229,29230,29229,58459,11.197703838348389,0.00866292883888886
29429,29430,29429,58859,11.257059812545776,0.008511678026513717
29630,29631,29630,59261,11.31827998161316,0.008363218844996047
29830,29831,29830,59661,11.378100872039795,0.008216051498970374
30030,30031,30030,60061,11.437477827072144,0.008073663848700455
30230,30231,30230,60461,11.497763872146606,0.007934750631176627
30430,30431,30430,60861,11.563050985336304,0.007798140666873259
30631,30632,30631,61263,11.625550746917725,0.007662623076051517
30831,30832,30831,61663,11.689152956008911,0.007533805220532293
31031,31032,31031,62063,11.749683856964111,0.007404610967447344
31231,31232,31231,62463,11.808461666107178,0.00728022952838245
31431,31432,31431,62863,11.86711072921753,0.007158144334321176
31632,31633,31632,63265,11.92573595046997,0.007037952484911452
31832,31833,31832,63665,11.988050937652588,0.006920325767066486
32032,32033,32032,64065,12.052917957305908,0.0068042998434466595
32232,32233,32232,64465,12.116415023803711,0.0066914444469923905
32432,32433,32432,64865,12.217423915863037,0.006581723560901589
32633,32634,32633,65267,12.290897846221924,0.006472507824112722
32833,32834,32833,65667,12.361841917037964,0.006366363710213357
33033,33034,33033,66067,12.437455892562866,0.006262015618217894
33233,33234,33233,66467,12.52313494682312,0.006159532537137357
33433,33434,33433,66867,12.603120803833008,0.006058832312036503
33634,33635,33634,67269,12.680173873901367,0.0059606195867872
33834,33835,33834,67669,12.752911806106567,0.005864351565763597
34034,34035,34034,68069,12.827451944351196,0.005768973366694284
34234,34235,34234,68469,12.890244722366333,0.005675764774787819
34434,34435,34434,68869,12.951738834381104,0.005584832012078923
34635,34636,34635,69271,13.018412828445435,0.005493306709717078
34835,34836,34835,69671,13.12154769897461,0.00540449770885505
35035,35036,35035,70071,13.20741081237793,0.005317348312845285
35235,35236,35235,70471,13.277415752410889,0.005231947250737163
35435,35436,35435,70871,13.345885992050171,0.00514782201418232
35636,35637,35636,71273,13.421756744384766,0.005065554524006182
35836,35837,35836,71673,13.503736734390259,0.00498479457631076
36036,36037,36036,72073,13.583715677261353,0.004906358614123558
36236,36237,36236,72473,13.660415887832642,0.004827827470599538
36436,36437,36436,72873,13.754400968551636,0.004752128129901982
36637,36638,36637,73275,13.822187900543213,0.004676998180425202
36837,36838,36837,73675,13.892031908035278,0.004603554237245189
37037,37038,37037,74075,13.959884643554688,0.004531881341661738
37237,37238,37237,74475,14.033780813217163,0.004462223226885377
37437,37438,37437,74875,14.132718801498413,0.004393187752783643
37638,37639,37638,75277,14.233873844146729,0.00432441711561532
37838,37839,37838,75677,14.371985912322998,0.004256883467388916
38038,38039,38038,76077,14.462279796600342,0.004190689686153657
38238,38239,38238,76477,14.563907861709595,0.004126787870819854
38438,38439,38438,76877,14.656815767288208,0.00406433357007835
38639,38640,38639,77279,14.748534679412842,0.004001716479706899
38839,38840,38839,77679,14.809635877609253,0.003940384703575844
39039,39040,39039,78079,14.880784749984741,0.003880924798548449
39239,39240,39239,78479,14.945762634277344,0.0038228121366734066
39439,39440,39439,78879,15.009676694869995,0.003764360096574885
39640,39641,39640,79281,15.076802730560303,0.0037067996330946997
39840,39841,39840,79681,15.14657998085022,0.003650440390922143
40040,40041,40040,80081,15.220487833023071,0.0035954524551109544
40240,40241,40240,80481,15.304881811141968,0.003540610701209632
40440,40441,40440,80881,15.374084711074829,0.0034867425605838265
40641,40642,40641,81283,15.438676834106445,0.0034334999285360987
40841,40842,40841,81683,15.511445045471191,0.003381513462800075
41041,41042,41041,82083,15.584027767181396,0.0033291338453381785
41241,41242,41241,82483,15.647459745407104,0.0032788073218907184
41441,41442,41441,82883,15.718439817428589,0.0032295807210981444
41642,41643,41642,83285,15.786356925964355,0.0031803058117023703
41842,41843,41842,83685,15.851436853408813,0.003131895555236221
42042,42043,42042,84085,15.920766830444336,0.003085091861613188
42242,42243,42242,84485,15.986969709396362,0.0030386227745741803
42442,42443,42442,84885,16.05426788330078,0.0029931437585829397
42643,42644,42643,85287,16.123273849487305,0.002947558377769868
42843,42844,42843,85687,16.189010858535767,0.0029029578458183844
43043,43044,43043,86087,16.25371789932251,0.0028602814351204155
43243,43244,43243,86487,16.3186297416687,0.0028183875158611428
43443,43444,43443,86887,16.392581939697266,0.0027765025285384957
43644,43645,43644,87289,16.459617614746094,0.0027351757125747317
43844,43845,43844,87689,16.530570030212402,0.0026948025095869
44044,44045,44044,88089,16.59780478477478,0.0026554861101548404
44244,44245,44244,88489,16.667418718338013,0.0026166536366824178
44444,44445,44444,88889,16.73674964904785,0.0025781487494501874
44645,44646,44645,89291,16.804128885269165,0.0025401004267223575
44845,44846,44845,89691,16.868340969085693,0.002502670875081852
45045,45046,45045,90091,16.942838668823242,0.0024660908620435257
45245,45246,45245,90491,17.01849389076233,0.0024297484740241023
45445,45446,45445,90891,17.092187881469727,0.0023945898657533634
45646,45647,45646,91293,17.17642879486084,0.002359495924673806
45846,45847,45846,91693,17.25420379638672,0.002324312954622752
46046,46047,46046,92093,17.325815677642822,0.0022905734822706177
46246,46247,46246,92493,17.416401863098145,0.0022572288759543264
46446,46447,46446,92893,17.493868827819824,0.0022240926990488748
46647,46648,46647,93295,17.56468892097473,0.0021912751721729594
46847,46848,46847,93695,17.639939785003662,0.002159044420522511
47047,47048,47047,94095,17.706451892852783,0.0021277474055163763
47247,47248,47247,94495,17.776371955871582,0.0020967624176808928
47447,47448,47447,94895,17.853158950805664,0.0020660158741620228
47648,47649,47648,95297,17.922785758972168,0.0020357121738329887
47848,47849,47848,95697,17.98897385597229,0.0020065025203099933
48048,48049,48048,96097,18.06256103515625,0.0019774418100411977
48248,48249,48248,96497,18.125463724136353,0.0019484401490789073
48448,48449,48448,96897,18.193220853805542,0.001920249382427428
48649,48650,48649,97299,18.25882601737976,0.0018925841498516108
48849,48850,48849,97699,18.358308792114258,0.0018651858688157736
49049,49050,49049,98099,18.448017835617065,0.00183845475060204
49249,49250,49249,98499,18.546611785888672,0.0018120057084521023
49449,49450,49449,98899,18.660993814468384,0.0017861424962992067
49650,49651,49650,99301,18.77947187423706,0.0017604834723886778
49850,49851,49850,99701,18.95735502243042,0.001735423415429767
50050,50051,50050,100101,19.12859082221985,0.0017113103824172341
50250,50251,50250,100501,19.23507571220398,0.0016872408695702877
50450,50451,50450,100901,19.334600925445557,0.0016633012642137846
50651,50652,50651,101303,19.427254676818848,0.0016396682472135512
50851,50852,50851,101703,19.556941747665405,0.0016169950820499877
51051,51052,51051,102103,19.700292825698853,0.0015944675560115307
51251,51252,51251,102503,19.783323764801025,0.0015716622090984887
51451,51452,51451,102903,19.857956886291504,0.0015492553900764248
51652,51653,51652,103305,19.921722888946533,0.001527176303403981
51852,51853,51852,103705,19.98626685142517,0.001505445349073074
52052,52053,52052,104105,20.058103799819946,0.001484245856792927
52252,52253,52252,104505,20.118204832077026,0.0014629445411834046
52452,52453,52452,104905,20.180480003356934,0.0014421049889295926
52653,52654,52653,105307,20.24366593360901,0.0014214444338141385
52853,52854,52853,105707,20.344700813293457,0.0014011662784877354
53053,53054,53053,106107,20.460314750671387,0.0013813471286380874
53253,53254,53253,106507,20.64758563041687,0.001361516242499634
53453,53454,53453,106907,20.795440912246704,0.0013420694852652086
53654,53655,53654,107309,20.950684785842896,0.0013229857804086388
53854,53855,53854,107709,21.072896003723145,0.0013041680220790717
54054,54055,54054,108109,21.162375926971436,0.001285681193302624
54254,54255,54254,108509,21.254411697387695,0.0012674397307182532
54454,54455,54454,108909,21.340853929519653,0.0012494631133587516
54655,54656,54655,109311,21.430083751678467,0.0012317951624588018
54855,54856,54855,109711,21.56891703605652,0.001214740451435602
55055,55056,55055,110111,21.681241750717163,0.001198068908133733
55255,55256,55255,110511,21.870383739471436,0.0011813586308002065
55455,55456,55455,110911,22.005879640579224,0.001164898014376947
55656,55657,55656,111313,22.10655164718628,0.0011489008558959466
55856,55857,55856,111713,22.19888472557068,0.001133360041498177
56056,56057,56056,112113,22.285945892333984,0.0011177788184968504
56256,56257,56256,112513,22.34503984451294,0.0011022341200223466
56456,56457,56456,112913,22.420657873153687,0.0010869053952228757
56657,56658,56657,113315,22.573540687561035,0.0010717393145513415
56857,56858,56857,113715,22.677367687225342,0.001056993589320401
57057,57058,57057,114115,22.77505373954773,0.0010423515497593968
57257,57258,57257,114515,22.86415982246399,0.0010278089335622775
57457,57458,57457,114915,22.97651982307434,0.0010133800167104817
57658,57659,57658,115317,23.078893661499023,0.0009990405303262366
57858,57859,57858,115717,23.18005394935608,0.000985171225215665
58058,58059,58058,116117,23.34823489189148,0.0009713478109232805
58258,58259,58258,116517,23.484036684036255,0.0009578258157588103
58458,58459,58458,116917,23.582965850830078,0.000944344056779163
58659,58660,58659,117319,23.686124086380005,0.0009310880523488776
58859,58860,58859,117719,23.769497871398926,0.0009181986036367689
59059,59060,59059,118119,23.84630298614502,0.0009053506535363928
59259,59260,59259,118519,23.92694401741028,0.0008926713870727155
59459,59460,59459,118919,23.986445665359497,0.0008800631211703855
59660,59661,59660,119321,24.05625081062317,0.000867757824119764
59860,59861,59860,119721,24.115604877471924,0.0008559232080171846
60060,60061,60060,120121,24.175585746765137,0.0008439675461950424
60260,60261,60260,120521,24.236061811447144,0.0008321523330809723
60460,60461,60460,120921,24.297268867492676,0.0008207510878751708
60661,60662,60661,121323,24.358999729156494,0.000809543933693382
60861,60862,60861,121723,24.422651767730713,0.0007984087943771305
61061,61062,61061,122123,24.4853777885437,0.000787401761296789
61261,61262,61261,122523,24.550297737121582,0.0007766897090699121
61461,61462,61461,122923,24.617421865463257,0.0007660440878736943
61662,61663,61662,123325,24.68082571029663,0.0007555310694615147
61862,61863,61862,123725,24.74148988723755,0.0007453060022503595
62062,62063,62062,124125,24.7999107837677,0.0007352070737036983
62262,62263,62262,124525,24.855523824691772,0.0007252083327034155
62462,62463,62462,124925,24.91512179374695,0.0007151117086181869
62663,62664,62663,125327,24.976260900497437,0.0007052874783128918
62863,62864,62863,125727,25.04423499107361,0.000695812412316171
63063,63064,63063,126127,25.10442280769348,0.0006862675044512559
63263,63264,63263,126527,25.162450790405273,0.0006767757209854186
63463,63464,63463,126927,25.224589824676514,0.0006674786788505068
63664,63665,63664,127329,25.285412788391113,0.0006583418685454106
63864,63865,63864,127729,25.344217777252197,0.000649294656981525
64064,64065,64064,128129,25.406036853790283,0.0006402167772949971
64264,64265,64264,128529,25.466083765029907,0.0006314111760917227
64464,64465,64464,128929,25.531226873397827,0.0006227022062097387
64665,64666,64665,129331,25.59368872642517,0.0006141548347277872
64865,64866,64865,129731,25.653435945510864,0.0006056621845365376
65065,65066,65065,130131,25.716009855270386,0.0005972326087198623
65265,65266,65265,130531,25.778077840805054,0.0005890812087043755
65465,65466,65465,130931,25.840853929519653,0.0005809251161722342
65666,65667,65666,131333,25.901893854141235,0.0005728011393250753
65866,65867,65866,131733,25.978290796279907,0.0005649453908827207
66066,66067,66066,132133,26.05366086959839,0.0005571700505206695
66266,66267,66266,132533,26.11438274383545,0.0005495749505089508
66466,66467,66466,132933,26.17395782470703,0.0005421377525967819
66667,66668,66667,133335,26.23481774330139,0.0005348393249119986
66867,66868,66867,133735,26.295796871185303,0.0005276507513632958
67067,67068,67067,134135,26.354442834854126,0.0005205129190188357
67267,67268,67267,134535,26.41383385658264,0.0005135457681473184
67467,67468,67467,134935,26.470966815948486,0.000506764725224965
67668,67669,67668,135337,26.535094738006592,0.0005000928247213803
67868,67869,67868,135737,26.602425813674927,0.0004934188469972313
68068,68069,68068,136137,26.669710874557495,0.0004867385232472511
68268,68269,68268,136537,26.744807958602905,0.00048024995466902827
68468,68469,68468,136937,26.81201481819153,0.0004738044266190112
68669,68670,68669,137339,26.87824273109436,0.00046742372070168254
68869,68870,68869,137739,26.943737745285034,0.000461124091922516
69069,69070,69069,138139,27.012919664382935,0.0004548786777582282
69269,69270,69269,138539,27.083574056625366,0.0004487518784170736
69469,69470,69469,138939,27.145458936691284,0.0004427236243523446
69670,69671,69670,139341,27.229451656341553,0.00043669511516001094
69870,69871,69870,139741,27.350368976593018,0.0004307362373976232
70070,70071,70070,140141,27.446368932724,0.00042489590050800763
70270,70271,70270,140541,27.520296812057495,0.00041907546041301775
70470,70471,70470,140941,27.59122896194458,0.00041333937381831564
70671,70672,70671,141343,27.65649676322937,0.0004076815185040909
70871,70872,70871,141743,27.72305679321289,0.0004020654503486046
71071,71072,71071,142143,27.78665590286255,0.000396556742976547
71271,71272,71271,142543,27.853256940841675,0.00039117311645054276
71471,71472,71471,142943,27.91619372367859,0.000385911953870524
71672,71673,71672,143345,27.981177806854248,0.00038072737128825175
71872,71873,71872,143745,28.063323736190796,0.00037559004326054394
72072,72073,72072,144145,28.147477865219116,0.000370561797002656
72272,72273,72272,144545,28.22171688079834,0.0003656758113238041
72472,72473,72472,144945,28.29997682571411,0.0003608795112190771
72673,72674,72673,145347,28.367281913757324,0.00035609170149239586
72873,72874,72873,145747,28.433165788650513,0.0003513430128400182
73073,73074,73073,146147,28.50076174736023,0.00034668513637330886
73273,73274,73273,146547,28.576075792312622,0.0003421025586494241
73473,73474,73473,146947,28.64472484588623,0.0003376295253542471
73674,73675,73674,147349,28.714691877365112,0.00033315939733987587
73874,73875,73874,147749,28.78032374382019,0.00032868956875648213
74074,74075,74074,148149,28.84452986717224,0.0003242839217397435
74274,74275,74274,148549,28.91039800643921,0.0003199796305699049
74474,74475,74474,148949,28.97793984413147,0.00031571054543250577
74675,74676,74675,149351,29.048738718032837,0.00031147335008010563
74875,74876,74875,149751,29.113420724868774,0.0003073010484012992
75075,75076,75075,150151,29.179404735565186,0.0003031494030948048
75275,75276,75275,150551,29.249295711517334,0.00029903002348332286
75475,75476,75475,150951,29.331641674041748,0.0002949852636513685
75676,75677,75676,151353,29.3995578289032,0.00029094578013623374
75876,75877,75876,151753,29.46917462348938,0.000286982384500676
76076,76077,76076,152153,29.538426876068115,0.00028306905396511915
76276,76277,76276,152553,29.61085271835327,0.0002792104289754811
76476,76477,76476,152953,29.677942752838135,0.00027548101433197907
76677,76678,76677,153355,29.74287486076355,0.0002717304334394931
76877,76878,76877,153755,29.806745767593384,0.0002680250278693373
77077,77078,77077,154155,29.874717950820923,0.0002644374612590234
77277,77278,77277,154555,29.938817024230957,0.00026090501907984683
77477,77478,77477,154955,30.00443983078003,0.00025743017560501323
77678,77679,77678,155357,30.07512879371643,0.0002539505537003658
77878,77879,77878,155757,30.142282009124756,0.00025053510697876073
78078,78079,78078,156157,30.224236726760864,0.0002472262217203472
78278,78279,78278,156557,30.320952653884888,0.0002439843296962419
78478,78479,78478,156957,30.393688678741455,0.00024077804228057434
78679,78680,78679,157359,30.461734771728516,0.0002375478298160555
78879,78880,78879,157759,30.530012845993042,0.000234376033896664
79079,79080,79079,158159,30.597282648086548,0.0002312653422273322
79279,79280,79279,158559,30.660669803619385,0.00022820904506292496
79479,79480,79479,158959,30.726417779922485,0.0002252427294164842
79680,79681,79680,159361,30.792545795440674,0.00022225844585727962
79880,79881,79880,159761,30.860062837600708,0.00021927946587457943
80080,80081,80080,160161,30.92627787590027,0.00021634930238812963
80280,80281,80280,160561,30.991522789001465,0.0002134732091149855
80480,80481,80480,160961,31.06964683532715,0.00021066211710877295
80681,80682,80681,161363,31.135995864868164,0.00020782078990606146
80881,80882,80881,161763,31.198004007339478,0.00020501839368127547
81081,81082,81081,162163,31.421247005462646,0.00020229213450807402
81281,81282,81281,162563,31.563532829284668,0.00019961007869545965
81481,81482,81481,162963,31.641480922698975,0.00019694117448136215
81682,81683,81682,163365,31.70418882369995,0.00019426424598944543
81882,81883,81882,163765,31.772944927215576,0.0001916476235991479
82082,82083,82082,164165,31.841065883636475,0.00018907448604913964
82282,82283,82282,164565,31.90999484062195,0.00018652478862011307
82482,82483,82482,164965,31.970524787902832,0.0001840166903292946
82683,82684,82683,165367,32.05263376235962,0.000181522524462458
82883,82884,82883,165767,32.114866971969604,0.00017909325462996182
83083,83084,83083,166167,32.178645849227905,0.00017671236929102637
83283,83284,83283,166567,32.24138379096985,0.0001743766204616717
83483,83484,83483,166967,32.3161838054657,0.00017207254045355536
83684,83685,83684,167369,32.39297103881836,0.00016977180754932516
83884,83885,83884,167769,32.4690728187561,0.00016753791629444398
84084,84085,84084,168169,32.53374886512756,0.00016535367966499911
84284,84285,84284,168569,32.600828886032104,0.0001632140529359304
84484,84485,84484,168969,32.67393159866333,0.00016109142354260478
84685,84686,84685,169371,32.73785972595215,0.0001589549689838746
84885,84886,84885,169771,32.802926778793335,0.00015687626017223092
85085,85086,85085,170171,32.863478660583496,0.00015484737734202268
85285,85286,85285,170571,33.06275200843811,0.00015284588505977358
85485,85486,85485,170971,33.14992380142212,0.00015086235588029624
85686,85687,85686,171373,33.23125195503235,0.0001488766919747069
85886,85887,85886,171773,33.29426097869873,0.00014693657661973524
86086,86087,86086,172173,33.35585284233093,0.00014502658759247948
86286,86287,86286,172573,33.42884564399719,0.00014312233106591744
86486,86487,86486,172973,33.4903678894043,0.00014124532704896616
86687,86688,86687,173375,33.56534194946289,0.00013936944657912147
86887,86888,86887,173775,33.627206802368164,0.0001375151858629905
87087,87088,87087,174175,33.68797588348389,0.0001356800052169127
87287,87288,87287,174575,33.74841380119324,0.00013385863911910908
87487,87488,87487,174975,33.81177091598511,0.00013205408250652198
87688,87689,87688,175377,33.871909856796265,0.00013027215991237207
87888,87889,87888,175777,33.93316888809204,0.00012853502017459755
88088,88089,88088,176177,33.994038820266724,0.00012683158912569036
88288,88289,88288,176577,34.06755304336548,0.0001251491384305391
88488,88489,88488,176977,34.129692792892456,0.00012349052317589667
88689,88690,88689,177379,34.19181180000305,0.00012186584028103135
88889,88890,88889,177779,34.251808881759644,0.00012027287603101767
89089,89090,89089,178179,34.31524085998535,0.00011869415000336098
89289,89290,89289,178579,34.375372648239136,0.00011714361051289847
89489,89490,89489,178979,34.43821477890015,0.00011560991291645352
89690,89691,89690,179381,34.50911998748779,0.00011409823814248318
89890,89891,89890,179781,34.59699892997742,0.00011262817240842538
90090,90091,90090,180181,34.660789012908936,0.00011118492744508618
90290,90291,90290,180581,34.724445819854736,0.00010975617891016497
90490,90491,90490,180981,34.783981800079346,0.00010831303405022587
90691,90692,90691,181383,34.845011949539185,0.00010688529218467811
90891,90892,90891,181783,34.90629291534424,0.00010551489052971607
91091,91092,91091,182183,34.96820282936096,0.00010416108704950234
91291,91292,91291,182583,35.038023948669434,0.00010280807289617169
91491,91492,91491,182983,35.097503900527954,0.00010145655695681298
91692,91693,91692,183385,35.157978773117065,0.00010012076502267505
91892,91893,91892,183785,35.21774482727051,9.880718901499401e-05
92092,92093,92092,184185,35.28087091445923,9.75004821291043e-05
92292,92293,92292,184585,35.342928886413574,9.620895449813824e-05
92492,92493,92492,184985,35.405704975128174,9.492811418366405e-05
92693,92694,92693,185387,35.470035791397095,9.365556703365862e-05
92893,92894,92893,185787,35.53815674781799,9.240260564614021e-05
93093,93094,93093,186187,35.60113000869751,9.117756638754565e-05
93293,93294,93293,186587,35.665966749191284,8.997766313029656e-05
93493,93494,93493,186987,35.727733850479126,8.8771635618125e-05
93694,93695,93694,187389,35.78912091255188,8.757612997979614e-05
93894,93895,93894,187789,35.850502729415894,8.642151207130415e-05
94094,94095,94094,188189,35.91406273841858,8.528485519510682e-05
94294,94295,94294,188589,35.976048946380615,8.415286765755978e-05
94494,94495,94494,188989,36.04261088371277,8.30299689787259e-05
94695,94696,94695,189391,36.10566568374634,8.193880178712148e-05
94895,94896,94895,189791,36.16950988769531,8.087893491730921e-05
95095,95096,95095,190191,36.231773853302,7.982364297143526e-05
95295,95296,95295,190591,36.2920618057251,7.87624228514586e-05
95495,95496,95495,190991,36.366238832473755,7.771620909848523e-05
95696,95697,95696,191393,36.4291877746582,7.670667108932885e-05
95896,95897,95896,191793,36.495656967163086,7.572251973128162e-05
96096,96097,96096,192193,36.563193798065186,7.474684782147175e-05
96296,96297,96296,192593,36.630066871643066,7.377343752456229e-05
96496,96497,96496,192993,36.71545076370239,7.280039418638807e-05
96697,96698,96697,193395,36.78489685058594,7.184202468711155e-05
96897,96898,96897,193795,36.8485209941864,7.091048919782164e-05
97097,97098,97097,194195,36.90989685058594,6.99970260363001e-05
97297,97298,97297,194595,36.981276750564575,6.908558276468211e-05
97497,97498,97497,194995,37.05090570449829,6.816907100040238e-05
97698,97699,97698,195397,37.11262798309326,6.726533398147265e-05
97898,97899,97898,195797,37.17632794380188,6.638904664777338e-05
98098,98099,98098,196197,37.236143827438354,6.552769550097537e-05
98298,98299,98298,196597,37.29703092575073,6.465832545740876e-05
98498,98499,98498,196997,37.35898971557617,6.378889286704535e-05
98699,98700,98699,197399,37.420153856277466,6.294496154533116e-05
98899,98900,98899,197799,37.47979497909546,6.211518222798223e-05
99099,99100,99099,198199,37.54805874824524,6.128381441590894e-05
99299,99300,99299,198599,37.61007595062256,6.0467151899641244e-05
99499,99500,99499,198999,37.66990780830383,5.966680186815877e-05
99700,99701,99700,199401,37.73011302947998,5.887957321171497e-05
99900,99901,99900,199801,37.790013790130615,5.8105150948722326e-05
100100,100101,100100,200201,37.84955286979675,5.7336257043037044e-05
100300,100301,100300,200601,37.91429781913757,5.6582861504167654e-05
100501,100502,100501,201003,37.97379779815674,5.584283652914116e-05
100701,100702,100701,201403,38.050381660461426,5.511720330360962e-05
100901,100902,100901,201803,38.11131691932678,5.440586890368439e-05
101101,101102,101101,202203,38.171793937683105,5.370455596587546e-05
101301,101302,101301,202603,38.232303857803345,5.300214814511839e-05
101502,101503,101502,203005,38.29396891593933,5.230988910939091e-05
101702,101703,101702,203405,38.35495090484619,5.164113340159465e-05
101902,101903,101902,203805,38.41509389877319,5.098268983141891e-05
102102,102103,102102,204205,38.47502374649048,5.033136035485895e-05
102302,102303,102302,204605,38.538670778274536,4.968291970495641e-05
102503,102504,102503,205007,38.60185694694519,4.9039978373801967e-05
102703,102704,102703,205407,38.6640567779541,4.841448018030458e-05
102903,102904,102903,205807,38.724607944488525,4.779731643772772e-05
103103,103104,103103,206207,38.79421901702881,4.718193771009914e-05
103303,103304,103303,206607,38.86729693412781,4.656798449963186e-05
103504,103505,103504,207009,38.931734800338745,4.596012323952167e-05
103704,103705,103704,207409,38.99436593055725,4.5362270301787345e-05
103904,103905,103904,207809,39.0641028881073,4.476877423596486e-05
104104,104105,104104,208209,39.124178886413574,4.418007522984389e-05
104304,104305,104304,208609,39.18551588058472,4.359678135619597e-05
104505,104506,104505,209011,39.24861478805542,4.302084883661207e-05
104705,104706,104705,209411,39.30854082107544,4.2454754744606647e-05
104905,104906,104905,209811,39.368504762649536,4.1894119348474885e-05
105105,105106,105105,210211,39.42807388305664,4.134734380362787e-05
105305,105306,105305,210611,39.49134373664856,4.0810808497345947e-05
105506,105507,105506,211013,39.560030937194824,4.0274739708349363e-05
105706,105707,105706,211413,39.62084984779358,3.974816206506211e-05
105906,105907,105906,211813,39.68134570121765,3.923246554957875e-05
106106,106107,106106,212213,39.74094080924988,3.872214455492361e-05
106306,106307,106306,212613,39.80156898498535,3.821798367002212e-05
106507,106508,106507,213015,39.862539768218994,3.772278860044604e-05
106707,106708,106707,213415,39.92196202278137,3.724096755943991e-05
106907,106908,106907,213815,39.982202768325806,3.676667704662083e-05
107107,107108,107107,214215,40.05090093612671,3.6291062343616e-05
107307,107308,107307,214615,40.11375594139099,3.582170345720955e-05
107508,107509,107508,215017,40.1730637550354,3.53671612117223e-05
107708,107709,107708,215417,40.234827756881714,3.492178029743362e-05
107908,107909,107908,215817,40.294973850250244,3.4474854288589036e-05
108108,108109,108108,216217,40.35436487197876,3.40294995071156e-05
108308,108309,108308,216617,40.41771864891052,3.3591607353848384e-05
108509,108510,108509,217019,40.477025747299194,3.315898945917218e-05
108709,108710,108709,217419,40.54208183288574,3.273263239382966e-05
108909,108910,108909,217819,40.60425591468811,3.2309032001612506e-05
109109,109110,109109,218219,40.663909912109375,3.188638286560343e-05
109309,109310,109309,218619,40.72731685638428,3.146923261258838e-05
109510,109511,109510,219021,40.78778600692749,3.1055075627444526e-05
109710,109711,109710,219421,40.84722280502319,3.06483763686686e-05
109910,109911,109910,219821,40.91623401641846,3.0250342983088576e-05
110110,110111,110110,220221,40.99052381515503,2.9851965056713734e-05
110310,110311,110310,220621,41.06473779678345,2.9453946396981197e-05
110511,110512,110511,221023,41.12474966049194,2.906447969107026e-05
110711,110712,110711,221423,41.18628406524658,2.8685361672851316e-05
110911,110912,110911,221823,41.24617075920105,2.8309791881153772e-05
111111,111112,111111,222223,41.30719065666199,2.793519868376379e-05
111311,111312,111311,222623,41.36850690841675,2.756709385061219e-05
111512,111513,111512,223025,41.42861270904541,2.7209345144369468e-05
111712,111713,111712,223425,41.489858865737915,2.6856382755677513e-05
111912,111913,111912,223825,41.559897899627686,2.6500766470475935e-05
112112,112113,112112,224225,41.62149977684021,2.6152504592056777e-05
112312,112313,112312,224625,41.68115782737732,2.5819325671295058e-05
112513,112514,112513,225027,41.74170184135437,2.5489445060157117e-05
112713,112714,112713,225427,41.80459499359131,2.5158092247333167e-05
112913,112914,112913,225827,41.86544680595398,2.483022924094265e-05
113113,113114,113113,226227,41.92523980140686,2.4510038193581392e-05
113313,113314,113313,226627,41.985302686691284,2.419587332316833e-05
113514,113515,113514,227029,42.05528783798218,2.3885442286206356e-05
113714,113715,113714,227429,42.11510491371155,2.3580706848808053e-05
113914,113915,113914,227829,42.175896883010864,2.327710824570571e-05
114114,114115,114114,228229,42.239330768585205,2.2973227534980313e-05
114314,114315,114314,228629,42.30159068107605,2.2674804915710805e-05
114515,114516,114515,229031,42.361777782440186,2.238453946885797e-05
114715,114716,114715,229431,42.421462059020996,2.2099449084474933e-05
114915,114916,114915,229831,42.4836049079895,2.180977521247195e-05
115115,115116,115115,230231,42.54961895942688,2.1519500463285077e-05
115315,115316,115315,230631,42.61103582382202,2.1238677804018657e-05
115516,115517,115516,231033,42.671281814575195,2.0962494835235708e-05
115716,115717,115716,231433,42.7308988571167,2.0687329974705248e-05
115916,115917,115916,231833,42.79102063179016,2.041431648426385e-05
116116,116117,116116,232233,42.85270094871521,2.014596851656732e-05
116316,116317,116316,232633,42.91355800628662,1.988266146999009e-05
116517,116518,116517,233035,42.97365188598633,1.962033701367244e-05
116717,116718,116717,233435,43.0461368560791,1.9359956486047953e-05
116917,116918,116917,233835,43.123414754867554,1.910567367206094e-05
117117,117118,117117,234235,43.19151592254639,1.8858412497266025e-05
117317,117318,117317,234635,43.2505247592926,1.8614066529843346e-05
117518,117519,117518,235037,43.31029295921326,1.8371253627111054e-05
117718,117719,117718,235437,43.3689227104187,1.8132783849439717e-05
117918,117919,117918,235837,43.429646730422974,1.789673532767881e-05
118118,118119,118118,236237,43.49250793457031,1.766461490286039e-05
118318,118319,118318,236637,43.55985999107361,1.743852663848573e-05
118519,118520,118519,237039,43.6204948425293,1.7216707430073667e-05
118719,118720,118719,237439,43.68128776550293,1.6997802784941326e-05
118919,118920,118919,237839,43.75149965286255,1.6779103041475532e-05
119119,119120,119119,238239,43.81121373176575,1.6564321561972023e-05
119319,119320,119319,238639,43.886295795440674,1.6356685286522123e-05
119520,119521,119520,239041,43.966556787490845,1.6151432781057944e-05
119720,119721,119720,239441,44.04910063743591,1.5945612527305607e-05
119920,119921,119920,239841,44.11272597312927,1.5739866418091707e-05
120120,120121,120120,240241,44.172802686691284,1.553851433457343e-05
120320,120321,120320,240641,44.2318058013916,1.5341289814167193e-05
120521,120522,120521,241043,44.29466986656189,1.5144882344943706e-05
120721,120722,120721,241443,44.35399675369263,1.4949704941051995e-05
120921,120922,120921,241843,44.414384841918945,1.4755043955947428e-05
121121,121122,121121,242243,44.47479605674744,1.4562447467048299e-05
121321,121322,121321,242643,44.53909182548523,1.4372106761909459e-05
121522,121523,121522,243045,44.600366830825806,1.4184032568775834e-05
121722,121723,121722,243445,44.65978980064392,1.4000548234215654e-05
121922,121923,121922,243845,44.720109701156616,1.3818528370447301e-05
122122,122123,122122,244245,44.77963185310364,1.3637848930070931e-05
122322,122323,122322,244645,44.84082889556885,1.346016461261688e-05
122523,122524,122523,245047,44.90179777145386,1.3284685446248557e-05
122723,122724,122723,245447,44.96177887916565,1.3111916551545706e-05
122923,122924,122923,245847,45.02664875984192,1.2940464068257475e-05
123123,123124,123123,246247,45.08845901489258,1.2772285486469118e-05
123323,123324,123323,246647,45.14738988876343,1.2608320098172464e-05
123524,123525,123524,247049,45.219958782196045,1.2446292583172009e-05
123724,123725,123724,247449,45.29409980773926,1.2286311093599653e-05
123924,123925,123924,247849,45.356268644332886,1.212859376112078e-05
124124,124125,124124,248249,45.41667890548706,1.197567135851732e-05
124324,124325,124324,248649,45.476961612701416,1.1826469258359274e-05
124525,124526,124525,249051,45.546366930007935,1.16768822811991e-05
124725,124726,124725,249451,45.60671281814575,1.1528104328762432e-05
124925,124926,124925,249851,45.6670196056366,1.1381546194638878e-05
125125,125126,125125,250251,45.72658085823059,1.1238571386144452e-05
125325,125326,125325,250651,45.788230895996094,1.1097406986620853e-05
125526,125527,125526,251053,45.84754991531372,1.0955261815643842e-05
125726,125727,125726,251453,45.90619397163391,1.0814539096459148e-05
125926,125927,125926,251853,45.96526575088501,1.0675868479583636e-05
126126,126127,126126,252253,46.032530784606934,1.0538860674751363e-05
126326,126327,126326,252653,46.094796657562256,1.040318660931943e-05
126527,126528,126527,253055,46.15490365028381,1.0268598696375037e-05
126727,126728,126727,253455,46.21890878677368,1.0135279140182757e-05
126927,126928,126927,253855,46.27927088737488,1.0002281435417993e-05
127127,127128,127127,254255,46.338499784469604,9.871722723459605e-06
127327,127328,127327,254655,46.402169704437256,9.744002680000372e-06
127528,127529,127528,255057,46.46312093734741,9.61665289956283e-06
127728,127729,127728,255457,46.524186849594116,9.489892778628001e-06
127928,127929,127928,255857,46.588220834732056,9.364846366372176e-06
128128,128129,128128,256257,46.64966678619385,9.243442205259841e-06
128328,128329,128328,256657,46.710991859436035,9.12367042457294e-06
128529,128530,128529,257059,46.77103590965271,9.003295915835782e-06
128729,128730,128729,257459,46.83199882507324,8.88562893484679e-06
128929,128930,128929,257859,46.8933207988739,8.771650341437249e-06
129129,129130,129129,258259,46.955169677734375,8.659843149925473e-06
129329,129330,129329,258659,47.02410173416138,8.54787266385816e-06
129530,129531,129530,259061,47.09418702125549,8.436113866643165e-06
129730,129731,129730,259461,47.154953956604004,8.32801029647945e-06
129930,129931,129930,259861,47.21739387512207,8.222559849159845e-06
130130,130131,130130,260261,47.27873373031616,8.11831464853367e-06
130330,130331,130330,260661,47.34968090057373,8.014772111331724e-06
130531,130532,130531,261063,47.43169569969177,7.91168205984678e-06
130731,130732,130731,261463,47.49445462226868,7.810640273877008e-06
130931,130932,130931,261863,47.55974292755127,7.711617353754715e-06
131131,131132,131131,262263,47.63801193237305,7.614713840505814e-06
131331,131332,131331,262663,47.70688486099243,7.518567731952333e-06
131532,131533,131532,263065,47.77128767967224,7.4209399919042546e-06
131732,131733,131732,263465,47.83075189590454,7.323895286212233e-06
131932,131933,131932,263865,47.892345905303955,7.229769122956267e-06
132132,132133,132132,264265,47.95261788368225,7.138375794736244e-06
132332,132333,132332,264665,48.01800179481506,7.046717227891322e-06
132533,132534,132533,265067,48.09047985076904,6.953719171646285e-06
132733,132734,132733,265467,48.15100693702698,6.86255131019586e-06
132933,132934,132933,265867,48.21178865432739,6.773653189719054e-06
133133,133134,133133,266267,48.27247166633606,6.685829351678706e-06
133333,133334,133333,266667,48.331542015075684,6.598275845722372e-06
133534,133535,133534,267069,48.39093995094299,6.511316376804007e-06
133734,133735,133734,267469,48.45172381401062,6.426538597378519e-06
133934,133935,133934,267869,48.5146267414093,6.342950500301896e-06
134134,134135,134134,268269,48.58068585395813,6.260024005570409e-06
134334,134335,134334,268669,48.64064002037048,6.178153318738682e-06
134535,134536,134535,269071,48.70200490951538,6.097140053088602e-06
134735,134736,134735,269471,48.762115716934204,6.017931854360804e-06
134935,134936,134935,269871,48.82332491874695,5.940626116836509e-06
135135,135136,135135,270271,48.885751724243164,5.8649880954584645e-06
135335,135336,135335,270671,48.947041034698486,5.79002498268552e-06
135536,135537,135536,271073,49.00969696044922,5.715211775086579e-06
135736,135737,135736,271473,49.08655071258545,5.642488123792656e-06
135936,135937,135936,271873,49.1610586643219,5.572112908137876e-06
136136,136137,136136,272273,49.238494873046875,5.502890415650309e-06
136336,136337,136336,272673,49.30309987068176,5.4332172146445835e-06
136537,136538,136537,273075,49.36418104171753,5.36324690683766e-06
136737,136738,136737,273475,49.425548791885376,5.29555988049713e-06
136937,136938,136937,273875,49.49917697906494,5.229951966662565e-06
137137,137138,137137,274275,49.582589864730835,5.164772931214835e-06
137337,137338,137337,274675,49.645219802856445,5.099144547466333e-06
137538,137539,137538,275077,49.710747957229614,5.03319326224279e-06
137738,137739,137738,275477,49.773003816604614,4.968439750193433e-06
137938,137939,137938,275877,49.83520174026489,4.904971023017556e-06
138138,138139,138138,276277,49.89748668670654,4.8425071157005245e-06
138338,138339,138338,276677,49.960121870040894,4.780337490587529e-06
138539,138540,138539,277079,50.030799865722656,4.717899547625745e-06
138739,138740,138739,277479,50.0931499004364,4.656403717616764e-06
138939,138940,138939,277879,50.15567684173584,4.596001507415269e-06
139139,139140,139139,278279,50.217352867126465,4.5365244405257544e-06
139339,139340,139339,278679,50.27994966506958,4.477411346521915e-06
139540,139541,139540,279081,50.344873905181885,4.418341416871295e-06
139740,139741,139740,279481,50.40745782852173,4.360684891394473e-06
139940,139941,139940,279881,50.46904182434082,4.304246028507933e-06
140140,140141,140140,280281,50.5456109046936,4.248564247995627e-06
140340,140341,140340,280681,50.61003279685974,4.193591393814858e-06
140541,140542,140541,281083,50.67338967323303,4.139229228976016e-06
140741,140742,140741,281483,50.736163854599,4.086548298739797e-06
140941,140942,140941,281883,50.798152923583984,4.03532747944773e-06
141141,141142,141141,282283,50.86064887046814,3.984594220651304e-06
141341,141342,141341,282683,50.92532682418823,3.933951906301062e-06
141542,141543,141542,283085,50.987836837768555,3.883895986929403e-06
141742,141743,141742,283485,51.05851483345032,3.835469243612382e-06
141942,141943,141942,283885,51.11996579170227,3.7879403018177495e-06
142142,142143,142142,284285,51.18251180648804,3.740481095173814e-06
142342,142343,142342,284685,51.24501395225525,3.693041010992595e-06
142543,142544,142543,285087,51.30893898010254,3.646088954879403e-06
142743,142744,142743,285487,51.37893891334534,3.600401307003214e-06
142943,142944,142943,285887,51.44209384918213,3.5551678471800976e-06
143143,143144,143143,286287,51.50591993331909,3.5099594176301056e-06
143343,143344,143343,286687,51.57579493522644,3.4649756250481164e-06
143544,143545,143544,287089,51.65611171722412,3.420150384363263e-06
143744,143745,143744,287489,51.730748891830444,3.3761523250988917e-06
143944,143945,143944,287889,51.792627811431885,3.3329406729572125e-06
144144,144145,144144,288289,51.85452890396118,3.290064197314144e-06
144344,144345,144344,288689,51.9156129360199,3.2472210970613423e-06
144545,144546,144545,289091,51.97831869125366,3.204534554643172e-06
144745,144746,144745,289491,52.0505108833313,3.1628178548410484e-06
144945,144946,144945,289891,52.11395883560181,3.1218451767060057e-06
145145,145146,145145,290291,52.17653679847717,3.0811733251195294e-06
145345,145346,145345,290691,52.23960590362549,3.0407507982479615e-06
145546,145547,145546,291093,52.30375671386719,3.001078858145176e-06
145746,145747,145746,291493,52.36700081825256,2.9626735072299912e-06
145946,145947,145946,291893,52.427663803100586,2.9245379736346688e-06
146146,146147,146146,292293,52.48917078971863,2.8865134397707923e-06
146346,146347,146346,292693,52.55846571922302,2.849297883626035e-06
146547,146548,146547,293095,52.61917281150818,2.8129249391549343e-06
146747,146748,146747,293495,52.6798939704895,2.777302146417527e-06
146947,146948,146947,293895,52.74266481399536,2.7419292369919155e-06
147147,147148,147147,294295,52.8097448348999,2.7068802920729257e-06
147347,147348,147347,294695,52.87354493141174,2.6725383248930564e-06
147548,147549,147548,295097,52.93374800682068,2.638854531680487e-06
147748,147749,147748,295497,52.99685478210449,2.6057969797990767e-06
147948,147949,147948,295897,53.067662715911865,2.5729477897224153e-06
148148,148149,148148,296297,53.1274778842926,2.5402633075014834e-06
148348,148349,148348,296697,53.18883991241455,2.5079049522177933e-06
148549,148550,148549,297099,53.24907684326172,2.476136025799737e-06
148749,148750,148749,297499,53.30963182449341,2.4452260116823235e-06
148949,148950,148949,297899,53.36964392662048,2.4143571316762967e-06
149149,149150,149149,298299,53.4293167591095,2.3832745014154056e-06
149349,149350,149349,298699,53.489238023757935,2.3524776276886625e-06
149550,149551,149550,299101,53.560263872146606,2.3222773307274835e-06
149750,149751,149750,299501,53.623634815216064,2.2927824916195944e-06
149950,149951,149950,299901,53.68368577957153,2.2633046514341802e-06
150150,150151,150150,300301,53.75056791305542,2.233761261888304e-06
150350,150351,150350,300701,53.823171854019165,2.204743523057599e-06
150551,150552,150551,301103,53.892369747161865,2.176259129767353e-06
150751,150752,150751,301503,53.95189571380615,2.148072818259588e-06
150951,150952,150951,301903,54.01576280593872,2.1199573870360405e-06
151151,151152,151151,302303,54.0836067199707,2.092202735698951e-06
151351,151352,151351,302703,54.14453196525574,2.0649519007327967e-06
151552,151553,151552,303105,54.20456290245056,2.038084486924125e-06
151752,151753,151752,303505,54.267946004867554,2.0117552351323047e-06
151952,151953,151952,303905,54.32860088348389,1.9857548265499217e-06
152152,152153,152152,304305,54.3891327381134,1.9601379698214323e-06
152352,152353,152352,304705,54.448476791381836,1.93512459629048e-06
152553,152554,152553,305107,54.509888887405396,1.9106915127102578e-06
152753,152754,152753,305507,54.575562953948975,1.886714272826311e-06
152953,152954,152953,305907,54.63675379753113,1.8627299201078509e-06
153153,153154,153153,306307,54.69654870033264,1.8389731052285115e-06
153353,153354,153353,306707,54.7558867931366,1.815951511223215e-06
153554,153555,153554,307109,54.81662678718567,1.793509352821652e-06
153754,153755,153754,307509,54.87687683105469,1.771288074652469e-06
153954,153955,153954,307909,54.936954736709595,1.748938889953805e-06
154154,154155,154154,308309,54.996731758117676,1.7267110426722498e-06
154354,154355,154354,308709,55.06560182571411,1.7049668350902972e-06
154555,154556,154555,309111,55.12768578529358,1.6837136711172876e-06
154755,154756,154755,309511,55.187920808792114,1.6627795349463743e-06
154955,154956,154955,309911,55.24683976173401,1.641667787480338e-06
155155,155156,155155,310311,55.307506799697876,1.6205305030376032e-06
155355,155356,155355,310711,55.36838674545288,1.5997622493536874e-06
155556,155557,155556,311113,55.430370807647705,1.5793052671669733e-06
155756,155757,155756,311513,55.48920679092407,1.5590695929271191e-06
155956,155957,155956,311913,55.55509567260742,1.5388243093847645e-06
156156,156157,156156,312313,55.61346483230591,1.5187644885157856e-06
156356,156357,156356,312713,55.67162275314331,1.4990445061076293e-06
156557,156558,156557,313115,55.73058199882507,1.4794910115911802e-06
156757,156758,156757,313515,55.788310050964355,1.4602146897990975e-06
156957,156958,156957,313915,55.84657001495361,1.4411500162480282e-06
157157,157158,157157,314315,55.92092967033386,1.422385633275846e-06
157357,157358,157357,314715,55.991414070129395,1.4040512143322632e-06
157558,157559,157558,315117,56.06198978424072,1.3860666070618404e-06
157758,157759,157758,315517,56.12020564079285,1.368401535398108e-06
157958,157959,157958,315917,56.17799973487854,1.3508324281528885e-06
158158,158159,158158,316317,56.235511779785156,1.3335530931028398e-06
158358,158359,158358,316717,56.29626774787903,1.316793952292029e-06
158559,158560,158559,317119,56.356281757354736,1.300329485565827e-06
158759,158760,158759,317519,56.415931940078735,1.283996167354821e-06
158959,158960,158959,317919,56.47360587120056,1.2676646165800633e-06
159159,159160,159159,318319,56.53683376312256,1.25165266315491e-06
159359,159360,159359,318719,56.599350690841675,1.2361798902373522e-06
159560,159561,159560,319121,56.65918588638306,1.2209033524791474e-06
159760,159761,159760,319521,56.71827673912048,1.2056296236478967e-06
159960,159961,159960,319921,56.77606391906738,1.190341052165116e-06
160160,160161,160160,320321,56.834030866622925,1.1752693185250995e-06
160360,160361,160360,320721,56.89381289482117,1.1604782089536489e-06
160561,160562,160561,321123,56.956806898117065,1.1457857039362884e-06
160761,160762,160761,321523,57.01985573768616,1.131234488928252e-06
160961,160962,160961,321923,57.07897186279297,1.1167431080956844e-06
161161,161162,161161,322323,57.136884927749634,1.1023542060902663e-06
161361,161362,161361,322723,57.19827580451965,1.0881325836548938e-06
161562,161563,161562,323125,57.2576117515564,1.0740668182164666e-06
161762,161763,161762,323525,57.315521001815796,1.0602150423936037e-06
161962,161963,161962,323925,57.37256193161011,1.0463866135990375e-06
162162,162163,162162,324325,57.431970834732056,1.0327121590505122e-06
162362,162363,162362,324725,57.48894691467285,1.0193771925717172e-06
162563,162564,162563,325127,57.553565979003906,1.0061992302395457e-06
162763,162764,162763,325527,57.612422943115234,9.931070773009517e-07
162963,162964,162963,325927,57.669928789138794,9.801370792048226e-07
163163,163164,163163,326327,57.72789978981018,9.67535781638883e-07
163363,163364,163363,326727,57.78707671165466,9.552442733616229e-07
163564,163565,163564,327129,57.84712195396423,9.429610079340143e-07
163764,163765,163764,327529,57.90556073188782,9.308083047756543e-07
163964,163965,163964,327929,57.96312594413757,9.189327350413245e-07
164164,164165,164164,328329,58.03810095787048,9.074089474913384e-07
164364,164365,164364,328729,58.11135983467102,8.960465478113089e-07
164565,164566,164565,329131,58.17171382904053,8.846701086735691e-07
164765,164766,164765,329531,58.236202001571655,8.734887753219937e-07
164965,164966,164965,329931,58.30508065223694,8.62492197246098e-07
165165,165166,165165,330331,58.36454486846924,8.516846471160357e-07
165365,165366,165365,330731,58.424694776535034,8.410797225687716e-07
165566,165567,165566,331133,58.48463988304138,8.305437919108827e-07
165766,165767,165766,331533,58.55148983001709,8.200733313725215e-07
165966,165967,165966,331933,58.61307883262634,8.096620286572932e-07
166166,166167,166166,332333,58.672852993011475,7.994789688250922e-07
166366,166367,166366,332733,58.733152866363525,7.895131555253986e-07
166567,166568,166567,333135,58.79424476623535,7.795112268536304e-07
166767,166768,166767,333535,58.854344844818115,7.695090999328867e-07
166967,166968,166967,333935,58.91391587257385,7.596304554481433e-07
167167,167168,167167,334335,58.975557804107666,7.499883839230843e-07
167367,167368,167367,334735,59.04400181770325,7.404336427758975e-07
167568,167569,167568,335137,59.105830907821655,7.307938460227386e-07
167768,167769,167768,335537,59.16838192939758,7.212766163665938e-07
167968,167969,167968,335937,59.22900986671448,7.119506513262573e-07
168168,168169,168168,336337,59.28995084762573,7.027814072030042e-07
168368,168369,168368,336737,59.351645946502686,6.936857911989809e-07
168569,168570,168569,337139,59.41222882270813,6.846197383240841e-07
168769,168770,168769,337539,59.474448919296265,6.757604887183849e-07
168969,168970,168969,337939,59.53952169418335,6.671213132957595e-07
169169,169170,169169,338339,59.601072788238525,6.586428742558714e-07
169369,169370,169369,338739,59.66215491294861,6.502269373174994e-07
169570,169571,169570,339141,59.72314190864563,6.418453016865293e-07
169770,169771,169770,339541,59.78239893913269,6.336639828602979e-07
169970,169971,169970,339941,59.84087681770325,6.257014113464206e-07
170170,170171,170170,340341,59.90053200721741,6.179362636613606e-07
170370,170371,170370,340741,59.9603316783905,6.102394559995958e-07
170571,170572,170571,341143,60.02673673629761,6.024935308915762e-07
170771,170772,170771,341543,60.089582681655884,5.948616954224373e-07
170971,170972,170971,341943,60.160029888153076,5.874504584502186e-07
171171,171172,171171,342343,60.23397088050842,5.802639811988597e-07
171371,171372,171371,342743,60.29550886154175,5.731128522499426e-07
171572,171573,171572,343145,60.35413980484009,5.658446915831294e-07
171772,171773,171772,343545,60.41728377342224,5.586594208061028e-07
171972,171973,171972,343945,60.47794985771179,5.516666896027404e-07
172172,172173,172172,344345,60.54065275192261,5.44809824612287e-07
172372,172373,172372,344745,60.60131788253784,5.379444549209167e-07
172573,172574,172573,345147,60.66133666038513,5.310236546010064e-07
172773,172774,172773,345547,60.72070670127869,5.242006534608068e-07
172973,172974,172973,345947,60.78043985366821,5.17480967287459e-07
173173,173174,173173,346347,60.841118812561035,5.108417534121768e-07
173373,173374,173373,346747,60.90516185760498,5.042424987648239e-07
173574,173575,173574,347149,60.976810932159424,4.976596913049939e-07
173774,173775,173774,347549,61.04982876777649,4.912061132788909e-07
173974,173975,173974,347949,61.11187791824341,4.848600815213234e-07
174174,174175,174174,348349,61.172563791275024,4.786043908529564e-07
174374,174375,174374,348749,61.233882904052734,4.724246854445593e-07
174575,174576,174575,349151,61.297812938690186,4.6628649103876314e-07
174775,174776,174775,349551,61.36579895019531,4.6028536766352673e-07
174975,174976,174975,349951,61.430842876434326,4.5442540031962536e-07
175175,175176,175175,350351,61.493780851364136,4.486662322018489e-07
175375,175376,175375,350751,61.563384771347046,4.429340211126801e-07
175576,175577,175576,351153,61.62601971626282,4.371969877166193e-07
175776,175777,175776,351553,61.688098669052124,4.316257988846358e-07
175976,175977,175976,351953,61.750359773635864,4.262826729148975e-07
176176,176177,176176,352353,61.811625957489014,4.210493994299217e-07
176376,176377,176376,352753,61.87491989135742,4.157573416715212e-07
176577,176578,176577,353155,61.938326835632324,4.104236325823518e-07
176777,176778,176777,353555,62.002076864242554,4.052512745619879e-07
176977,176978,176977,353955,62.07077193260193,4.002335371804569e-07
177177,177178,177177,354355,62.13396382331848,3.952737100979377e-07
177377,177378,177377,354755,62.19641184806824,3.903161444109756e-07
177578,177579,177578,355157,62.26505398750305,3.853512111404058e-07
177778,177779,177778,355557,62.34135389328003,3.8045461642645474e-07
177978,177979,177978,355957,62.412214040756226,3.756242191030937e-07
178178,178179,178178,356357,62.474151849746704,3.7087068143957036e-07
178378,178379,178378,356757,62.54298281669617,3.661680159886707e-07
178579,178580,178579,357159,62.60648488998413,3.614389773281601e-07
178779,178780,178779,357559,62.669455766677856,3.567449036002454e-07
178979,178980,178979,357959,62.7307448387146,3.5214573737304166e-07
179179,179180,179179,358359,62.79183077812195,3.476381096307733e-07
179379,179380,179379,358759,62.853513956069946,3.431408229135755e-07
179580,179581,179580,359161,62.92089605331421,3.386343021941778e-07
179780,179781,179780,359561,62.98424768447876,3.342458396868161e-07
179980,179981,179980,359961,63.053616762161255,3.2996860727917556e-07
180180,180181,180180,360361,63.123408794403076,3.2572614196233787e-07
180380,180381,180380,360761,63.187368869781494,3.214879246781353e-07
180581,180582,180581,361163,63.25515294075012,3.173100086722686e-07
180781,180782,180781,361563,63.321457862854004,3.132918228668646e-07
180981,180982,180981,361963,63.38478899002075,3.093481077540065e-07
181181,181182,181181,362363,63.4469678401947,3.054066366150126e-07
181381,181382,181381,362763,63.51300573348999,3.0150281054007786e-07
181582,181583,181582,363165,63.58309888839722,2.9766746455967676e-07
181782,181783,181782,363565,63.646214962005615,2.9393251325970226e-07
181982,181983,181982,363965,63.7078058719635,2.902615914449767e-07
182182,182183,182182,364365,63.769644021987915,2.866387313383574e-07
182382,182383,182382,364765,63.83152794837952,2.8304402320318553e-07
182583,182584,182583,365167,63.894386768341064,2.79463195030544e-07
182783,182784,182783,365567,63.956339836120605,2.7597202730253195e-07
182983,182984,182983,365967,64.03209090232849,2.725656016599168e-07
183183,183184,183183,366367,64.09457278251648,2.6918522515797925e-07
183383,183384,183383,366767,64.1571409702301,2.657850886548911e-07
183584,183585,183584,367169,64.2197036743164,2.6239189046436764e-07
183784,183785,183784,367569,64.28181886672974,2.5910270184870646e-07
183984,183985,183984,367969,64.34269165992737,2.558698754155164e-07
184184,184185,184184,368369,64.41018986701965,2.526216409068788e-07
184384,184385,184384,368769,64.48366475105286,2.4937226475776374e-07
184585,184586,184585,369171,64.55963587760925,2.4616163454001323e-07
184785,184786,184785,369571,64.6213538646698,2.430220285434953e-07
184985,184986,184985,369971,64.68664884567261,2.3990199264264543e-07
185185,185186,185185,370371,64.74654269218445,2.3679800730692766e-07
185385,185386,185385,370771,64.80782794952393,2.3374992317239174e-07
185586,185587,185586,371173,64.86886978149414,2.3075584844544786e-07
185786,185787,185786,371573,64.9288158416748,2.2780786566789327e-07
185986,185987,185986,371973,64.99002981185913,2.2487366378109202e-07
186186,186187,186186,372373,65.05838894844055,2.2197879234654386e-07
186386,186387,186386,372773,65.11838889122009,2.19142646845246e-07
186587,186588,186587,373175,65.17802286148071,2.1634846850792098e-07
186787,186788,186787,373575,65.2383668422699,2.1361475189357947e-07
186987,186988,186987,373975,65.29953169822693,2.1091119254978668e-07
187187,187188,187187,374375,65.35990881919861,2.08228818787683e-07
187387,187388,187387,374775,65.41930079460144,2.0559249209179393e-07
187588,187589,187588,375177,65.47995686531067,2.0302445857150853e-07
187788,187789,187788,375577,65.5450439453125,2.0053782900678585e-07
187988,187989,187988,375977,65.60585379600525,1.980610660771319e-07
188188,188189,188188,376377,65.66565680503845,1.9557087916446244e-07
188388,188389,188388,376777,65.72573280334473,1.931128232628215e-07
188589,188590,188589,377179,65.78593373298645,1.9071416011678247e-07
188789,188790,188789,377579,65.84458589553833,1.8837164937829967e-07
188989,188990,188989,377979,65.9072687625885,1.8602450286028056e-07
189189,189190,189189,378379,65.96752285957336,1.8367237760799064e-07
189389,189390,189389,378779,66.03352189064026,1.813507448119563e-07
189590,189591,189590,379181,66.09423589706421,1.7906443323206803e-07
189790,189791,189790,379581,66.15466976165771,1.7681787160434122e-07
189990,189991,189990,379981,66.21747875213623,1.7457407381226337e-07
190190,190191,190190,380381,66.27755379676819,1.7233343619771274e-07
190390,190391,190390,380781,66.339430809021,1.701135962645282e-07
190591,190592,190591,381183,66.40091800689697,1.6791120691909394e-07
190791,190792,190791,381583,66.46028065681458,1.657496984649122e-07
190991,190992,190991,381983,66.52766799926758,1.6361929877227506e-07
191191,191192,191191,382383,66.60428285598755,1.6151612481616844e-07
191391,191392,191391,382783,66.67480492591858,1.594374761313716e-07
191592,191593,191592,383185,66.73496603965759,1.5737710509995908e-07
191792,191793,191792,383585,66.79504895210266,1.553552481558247e-07
191992,191993,191992,383985,66.8544819355011,1.5335383015895235e-07
192192,192193,192192,384385,66.91520166397095,1.5137711944338506e-07
192392,192393,192392,384785,66.97679996490479,1.494476857872407e-07
192593,192594,192593,385187,67.04678392410278,1.4756529137405865e-07
192793,192794,192793,385587,67.10744667053223,1.4571558904610506e-07
192993,192994,192993,385987,67.16641879081726,1.438552775562191e-07
193193,193194,193193,386387,67.22728395462036,1.4200736732755282e-07
193393,193394,193393,386787,67.28616786003113,1.402206265505515e-07
193594,193595,193594,387189,67.3452160358429,1.38487841259072e-07
193794,193795,193794,387589,67.41273593902588,1.3677925045925167e-07
193994,193995,193994,387989,67.47072887420654,1.3505679888684066e-07
194194,194195,194194,388389,67.53550171852112,1.3333945257277157e-07
194394,194395,194394,388789,67.5959689617157,1.3165881002515542e-07
194595,194596,194595,389191,67.65608668327332,1.3001269738221647e-07
194795,194796,194795,389591,67.71608281135559,1.2839786550831146e-07
194995,194996,194995,389991,67.77418184280396,1.267846978808963e-07
195195,195196,195195,390391,67.8316798210144,1.2516574577409197e-07
195395,195396,195395,390791,67.88878798484802,1.235539017118894e-07
195596,195597,195596,391193,67.94821786880493,1.2196787488171025e-07
195796,195797,195796,391593,68.01076579093933,1.2042646442762324e-07
195996,195997,195996,391993,68.07212281227112,1.1889282713378138e-07
196196,196197,196196,392393,68.13036894798279,1.1735389490475789e-07
196396,196397,196396,392793,68.18715071678162,1.1583263875314402e-07
196597,196598,196597,393195,68.24531674385071,1.143396542600712e-07
196797,196798,196797,393595,68.30553984642029,1.1287178909428801e-07
196997,196998,196997,393995,68.36324572563171,1.1140457339744957e-07
197197,197198,197197,394395,68.42155861854553,1.0995729019477146e-07
197397,197398,197397,394795,68.47958397865295,1.0855053616836268e-07
197598,197599,197598,395197,68.54426598548889,1.0716217891046946e-07
197798,197799,197798,395597,68.60455083847046,1.0578118339393362e-07
197998,197999,197998,395997,68.66564083099365,1.044090346227869e-07
198198,198199,198198,396397,68.73851490020752,1.0307312692123835e-07
198398,198399,198398,396797,68.80732679367065,1.0177676074940671e-07
198599,198600,198599,397199,68.86567974090576,1.0049481413669124e-07
198799,198800,198799,397599,68.92366576194763,9.922729371176391e-08
198999,199000,198999,397999,68.98159885406494,9.796925448788079e-08
199199,199200,199199,398399,69.04638171195984,9.673107976383111e-08
199399,199400,199399,398799,69.10658097267151,9.552364641923907e-08
199600,199601,199600,399201,69.1683099269867,9.433914868353828e-08
199800,199801,199800,399601,69.2270028591156,9.317096573598365e-08
200000,200001,200000,400001,69.28586792945862,9.20000982116779e-08


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0013942718505859375,30.358106049564984
100,309,0,309,1.3257431983947754,0.6507547624690679
200,609,0,609,2.8780300617218018,0.4182419742677393
300,909,0,909,4.388712167739868,0.3110699759547583
400,1209,0,1209,5.709566354751587,0.2465004680819078
501,1512,0,1512,6.936438083648682,0.20282738540711617
601,1885,0,1885,8.291751146316528,0.12622544045254913
701,2238,0,2238,9.883986234664917,0.07743810430328488
801,2602,0,2602,11.418199062347412,0.05325129915661818
901,2986,0,2986,12.78946828842163,0.04345792423451749
1001,3371,0,3371,14.251145362854004,0.0365011017767492
1101,3773,0,3773,15.607449054718018,0.0354375508873495
1201,4160,0,4160,17.138273000717163,0.02981484593213899
1301,4560,0,4560,18.95812702178955,0.02905896039873752
1401,4960,0,4960,20.28397512435913,0.026356620340761645
1502,5364,0,5364,21.7161762714386,0.025706961200401265
1602,5763,0,5763,23.441672325134277,0.025053600169154467
1702,6163,0,6163,24.93668508529663,0.02332565854780266
1802,6563,0,6563,27.31739616394043,0.022801049042980723
1902,6963,0,6963,28.759879112243652,0.022284665871272702
2002,7363,0,7363,30.785332918167114,0.02177763200369444
2102,7763,0,7763,32.381479263305664,0.021281419981965796
2202,8163,0,8163,33.93050813674927,0.020799524693982878
2302,8563,0,8563,35.49981212615967,0.020333657755180683
2402,8963,0,8963,36.82053804397583,0.01988131965592813
2503,9367,0,9367,38.088961124420166,0.019438349041856744
2603,9767,0,9767,39.32350301742554,0.01901171937323965
2703,10167,0,10167,40.66910910606384,0.018597009783050882
2803,10567,0,10567,42.108487129211426,0.018196952675144953
2903,10967,0,10967,43.49486517906189,0.017809676412902122
3003,11367,0,11367,44.94133400917053,0.017432966796540564
3103,11767,0,11767,47.342814207077026,0.01706720342611169
3203,12167,0,12167,49.65823006629944,0.016709862949451176
3303,12567,0,12567,51.03801608085632,0.016360531159521505
3403,12967,0,12967,52.678218364715576,0.016022328460370227
3504,13371,0,13371,54.107999324798584,0.01569015604597771
3604,13771,0,13771,55.499009132385254,0.015368212120845071
3704,14171,0,14171,56.8081111907959,0.015052928956088172
3804,14571,0,14571,58.17817521095276,0.014744764608116728
3904,14971,0,14971,59.618213176727295,0.014444478515888088
4004,15371,0,15371,61.146820068359375,0.014152361288010229
4104,15771,0,15771,63.08996510505676,0.013868448132787412
4204,16171,0,16171,64.53096914291382,0.013591314333172278
4304,16571,0,16571,65.94555902481079,0.013320199854744336
4404,16971,0,16971,67.32756114006042,0.013057116876893376
4505,17375,0,17375,68.8132700920105,0.012799273959925184
4605,17775,0,17775,70.14143991470337,0.012549457965282505
4705,18175,0,18175,71.50015616416931,0.01230467586786776
4805,18575,0,18575,72.81968116760254,0.012065379068085394
4905,18975,0,18975,74.06960320472717,0.011832570205677932
5005,19375,0,19375,75.44185018539429,0.011606891903434615
5105,19775,0,19775,76.82581233978271,0.011386065924475428
5205,20175,0,20175,78.1908061504364,0.01116838840480713
5305,20575,0,20575,79.5469081401825,0.010955288799765128
5405,20975,0,20975,80.77636909484863,0.010748463182153674
5506,21379,0,21379,82.18384099006653,0.010545310546435979
5606,21779,0,21779,83.42752814292908,0.010347920470839137
5706,22179,0,22179,84.71753025054932,0.010153940681293728
5806,22579,0,22579,86.02191829681396,0.009963913005620021
5906,22979,0,22979,87.30474519729614,0.009777287850303287
6006,23379,0,23379,88.60146617889404,0.009594540981701814
6106,23779,0,23779,89.86962723731995,0.009416719337336383
6206,24179,0,24179,91.21616315841675,0.00924273978820138
6306,24579,0,24579,92.51898527145386,0.009071119409911205
6406,24979,0,24979,93.78722715377808,0.008901789677730688
6507,25383,0,25383,95.0853180885315,0.008734038825469009
6607,25783,0,25783,96.28937220573425,0.008572474705299152
6707,26183,0,26183,97.67125606536865,0.008414866243460033
6807,26583,0,26583,99.01777625083923,0.008259313311634483
6907,26983,0,26983,100.27417421340942,0.008105748721700437
7007,27383,0,27383,101.58654713630676,0.007955529562193248
7107,27783,0,27783,102.97901010513306,0.00780919373545589
7207,28183,0,28183,104.21745729446411,0.007665904501052503
7307,28583,0,28583,105.60704112052917,0.007524905359377179
7407,28983,0,28983,107.01325631141663,0.007386490077686376
7508,29387,0,29387,108.37999510765076,0.007250190828197828
7608,29787,0,29787,109.7057740688324,0.00711877034482702
7708,30187,0,30187,111.00402808189392,0.006990152600426185
7808,30587,0,30587,112.38723921775818,0.0068636568236796975
7908,30987,0,30987,113.90844798088074,0.006739364849018432
8008,31387,0,31387,115.51555132865906,0.006617919916156095
8108,31787,0,31787,117.07736229896545,0.0064998319003776615
8208,32187,0,32187,118.48056435585022,0.006384874047414578
8308,32587,0,32587,119.9318950176239,0.006272224513318704
8408,32987,0,32987,121.46299719810486,0.006161140168506875
8509,33391,0,33391,123.33060503005981,0.006050297776820639
8609,33791,0,33791,124.80073428153992,0.005942584381552453
8709,34191,0,34191,126.07985925674438,0.005837946296906162
8809,34591,0,34591,127.42879509925842,0.0057364884452167945
8909,34991,0,34991,128.8494062423706,0.005636856477054728
9009,35391,0,35391,130.11250925064087,0.0055379537288795895
9109,35791,0,35791,132.27751326560974,0.005440027801509376
9209,36191,0,36191,133.93895316123962,0.005344026836957584
9309,36591,0,36591,135.36651420593262,0.005250470711951127
9409,36991,0,36991,137.55284023284912,0.005159039462309007
9510,37395,0,37395,139.10367727279663,0.005068065405467702
9610,37795,0,37795,140.5872540473938,0.004979015991549589
9710,38195,0,38195,142.466046333313,0.0048912152740051
9810,38595,0,38595,144.0951201915741,0.004805089934748792
9910,38995,0,38995,145.5192632675171,0.004720842512797192
10010,39395,0,39395,146.92554330825806,0.004638331629492168
10110,39795,0,39795,148.28331017494202,0.00455714383273268
10210,40195,0,40195,149.83534002304077,0.004477098057683501
10310,40595,0,40595,151.33019018173218,0.004398417688785877
10410,40995,0,40995,152.90133905410767,0.004321374983913718
10511,41399,0,41399,154.7786841392517,0.004245192040503568
10611,41799,0,41799,156.38902711868286,0.004171260805560101
10711,42199,0,42199,157.9491412639618,0.00409882913631162
10811,42599,0,42599,159.3759651184082,0.004028015348708646
10911,42999,0,42999,161.26487016677856,0.003958854471329461
11011,43399,0,43399,163.67064428329468,0.0038911650450352843
11111,43799,0,43799,165.07705807685852,0.0038246051275886463
11211,44199,0,44199,166.37035632133484,0.0037590367662733385
11311,44599,0,44599,167.8639690876007,0.00369465623117031
11411,44999,0,44999,169.2154951095581,0.003631865694224254
11512,45403,0,45403,170.75410723686218,0.0035702213362157386
11612,45803,0,45803,172.03366017341614,0.0035105026751957396
11712,46203,0,46203,173.37079334259033,0.003451427439638342
11812,46603,0,46603,174.75291109085083,0.0033928517413217797
11912,47003,0,47003,176.1000051498413,0.0033352398661281664
12012,47403,0,47403,177.38842105865479,0.0032791838094821807
12112,47803,0,47803,178.6816382408142,0.0032247140975964557
12212,48203,0,48203,179.97429704666138,0.0031711376312158323
12312,48603,0,48603,181.26625418663025,0.0031179053308697043
12412,49003,0,49003,182.53753113746643,0.0030651788633711853
12513,49407,0,49407,183.87928128242493,0.003012973807248253
12613,49807,0,49807,185.3775680065155,0.0029625165749871617
12713,50207,0,50207,187.05910921096802,0.0029130463650657106
12813,50607,0,50607,188.68206310272217,0.0028641723864838153
12913,51007,0,51007,190.28484296798706,0.0028158049214479413
13013,51407,0,51407,191.79163312911987,0.002768097981770114
13113,51807,0,51807,193.80993723869324,0.0027212577206088785
13213,52207,0,52207,195.33388113975525,0.0026753701200842896
13313,52607,0,52607,196.73185205459595,0.0026304417093238703
13413,53007,0,53007,198.085853099823,0.002586291247923236
13514,53411,0,53411,199.6228699684143,0.0025423106232928968
13614,53811,0,53811,201.05761098861694,0.002499527268664444
13714,54211,0,54211,202.51929116249084,0.00245769199844635
13814,54611,0,54611,203.83179712295532,0.002416732630308154
13914,55011,0,55011,205.2480161190033,0.0023764348375698912
14014,55411,0,55411,206.5768129825592,0.0023367048497196204
14114,55811,0,55811,208.0562460422516,0.0022978003691479444
14214,56211,0,56211,209.41531205177307,0.0022598911054391158
14314,56611,0,56611,210.74947214126587,0.0022227212480486606
14414,57011,0,57011,212.01885223388672,0.0021859738234900426
14515,57415,0,57415,213.3082091808319,0.002149392905430431
14615,57815,0,57815,214.62981820106506,0.002114000215870793
14715,58215,0,58215,216.12208199501038,0.0020795752259138273
14815,58615,0,58615,217.40436124801636,0.002045863870732177
14915,59015,0,59015,218.6551992893219,0.002012520976274969
15015,59415,0,59415,219.98070120811462,0.0019795682034044327
15115,59815,0,59815,221.35109496116638,0.0019472168721430191
15215,60215,0,60215,222.71408009529114,0.0019155840479106873
15315,60615,0,60615,224.15484523773193,0.0018846100571719632
15415,61015,0,61015,225.46359515190125,0.0018541948417008939
15516,61419,0,61419,226.86920428276062,0.0018238410209070722
15616,61819,0,61819,228.1631453037262,0.0017941188364593
15716,62219,0,62219,229.4073121547699,0.0017648020716875535
15816,62619,0,62619,230.861102104187,0.0017360344126222406
15916,63019,0,63019,232.12626099586487,0.001707866608355096
16016,63419,0,63419,233.42491221427917,0.0016801305389868557
16116,63819,0,63819,234.73857617378235,0.0016526024271049096
16216,64219,0,64219,236.0356583595276,0.001625364637911422
16316,64619,0,64619,237.28669428825378,0.0015986457495929147
16416,65019,0,65019,238.64607095718384,0.0015724954517711436
16517,65423,0,65423,239.87859725952148,0.0015465410373268294
16617,65823,0,65823,241.20359706878662,0.0015211622597440433
16717,66223,0,66223,242.7109191417694,0.0014961524371583706
16817,66623,0,66623,244.05299019813538,0.0014716815971164174
16917,67023,0,67023,245.46382212638855,0.0014477048721005556
17017,67423,0,67423,246.72404313087463,0.0014240937809227533
17117,67823,0,67823,247.64771127700806,0.0014008621205052457
17217,68223,0,68223,248.84257912635803,0.0013780778521612666
17317,68623,0,68623,250.26639008522034,0.0013557930380092102
17417,69023,0,69023,251.44510221481323,0.0013339893755452302
17518,69427,0,69427,252.66408228874207,0.001312318321097196
17618,69827,0,69827,253.9125370979309,0.0012911466345974076
17718,70227,0,70227,255.10173511505127,0.0012703533072887887
17818,70627,0,70627,256.12733817100525,0.0012499921720609162
17918,71027,0,71027,257.325168132782,0.0012301403507880093
18018,71427,0,71427,258.43595814704895,0.0012107402047670326
18118,71827,0,71827,259.45753812789917,0.0011916346730938452
18218,72227,0,72227,260.50616431236267,0.0011727029709069719
18318,72627,0,72627,261.6184639930725,0.0011539753824583846
18418,73027,0,73027,262.6610600948334,0.0011356046604891988
18519,73431,0,73431,263.7278881072998,0.0011175134924743734
18619,73831,0,73831,264.8621871471405,0.0010999862408079823
18719,74231,0,74231,265.91029024124146,0.0010826272468067338
18819,74631,0,74631,267.03843927383423,0.0010653470201187137
18919,75031,0,75031,268.4012773036957,0.001048252511288985
19019,75431,0,75431,270.01831912994385,0.001031521089464909
19119,75831,0,75831,271.2057421207428,0.0010151868380032882
19219,76231,0,76231,272.3089520931244,0.0009991272976077434
19319,76631,0,76631,273.45073318481445,0.0009832007547621177
19419,77031,0,77031,274.58428621292114,0.0009673938704916476
19520,77435,0,77435,275.9043519496918,0.0009516409683803534
19620,77835,0,77835,277.00987005233765,0.0009363404548170853
19720,78235,0,78235,278.05911111831665,0.000921362703504236
19820,78635,0,78635,279.1259319782257,0.0009066758120257018
19920,79035,0,79035,280.2930450439453,0.0008922464749570341
20020,79435,0,79435,281.3099613189697,0.0008780581871527938
20120,79835,0,79835,282.8442039489746,0.0008641098500179282
20220,80235,0,80235,284.25258326530457,0.0008503922100089217
20320,80635,0,80635,285.46898913383484,0.0008368883175660513
20420,81035,0,81035,286.63552618026733,0.0008236042699702059
20521,81439,0,81439,288.07090520858765,0.0008104537164871062
20621,81839,0,81839,289.33183097839355,0.0007977362436747548
20721,82239,0,82239,290.3971881866455,0.0007853094526995712
20821,82639,0,82639,291.45324420928955,0.0007730861722539401
20921,83039,0,83039,292.6145761013031,0.0007609877975096041
21021,83439,0,83439,293.65397334098816,0.0007490204622297301
21121,83839,0,83839,294.7806692123413,0.0007372819971865592
21221,84239,0,84239,295.90140318870544,0.0007258527384648382
21321,84639,0,84639,297.01545429229736,0.0007146963311767857
21421,85039,0,85039,298.20522904396057,0.0007036754498273726
21522,85443,0,85443,299.24672627449036,0.0006925984689575183
21622,85843,0,85843,300.29191422462463,0.0006817427362606502
21722,86243,0,86243,301.3416311740875,0.0006711226004206478
21822,86643,0,86643,302.4089353084564,0.0006607801966491446
21922,87043,0,87043,303.4068253040314,0.000650636868992007
22022,87443,0,87443,304.42526721954346,0.0006405776058091096
22122,87843,0,87843,305.44574427604675,0.0006305722331827804
22222,88243,0,88243,306.5190739631653,0.0006206730587145202
22322,88643,0,88643,307.6278340816498,0.000610945042903948
22422,89043,0,89043,308.6482470035553,0.0006014150101720749
22523,89447,0,89447,309.64598321914673,0.0005919631910887146
22623,89847,0,89847,310.64476323127747,0.0005827343039487044
22723,90247,0,90247,311.70755195617676,0.0005736218683153639
22823,90647,0,90647,312.76607608795166,0.0005646507357322053
22923,91047,0,91047,313.82152223587036,0.0005558550042906865
23023,91447,0,91447,314.9217641353607,0.0005472343501870208
23123,91847,0,91847,316.0132031440735,0.0005387492039469365
23223,92247,0,92247,317.15062713623047,0.0005303746919463805
23323,92647,0,92647,318.3307251930237,0.0005221246244921503
23423,93047,0,93047,319.39635396003723,0.0005140231809636976
23524,93451,0,93451,320.46302318573,0.0005059808989078129
23624,93851,0,93851,321.4664011001587,0.0004981260379678544
23724,94251,0,94251,322.4534749984741,0.0004903765375955209
23824,94651,0,94651,323.44416403770447,0.0004827800708702784
23924,95051,0,95051,324.4483850002289,0.0004753641784925095
24024,95451,0,95451,325.439893245697,0.00046810511835460847
24124,95851,0,95851,326.4390251636505,0.0004609444542536899
24224,96251,0,96251,327.4278492927551,0.00045385860043912845
24324,96651,0,96651,328.4334282875061,0.00044688021003721617
24424,97051,0,97051,329.4233720302582,0.00044005081923466935
24525,97455,0,97455,330.4420852661133,0.0004333080267294898
24625,97855,0,97855,331.44218015670776,0.0004267498640150915
24725,98255,0,98255,332.4462089538574,0.000420273870148551
24825,98655,0,98655,333.43499517440796,0.0004138666777851403
24925,99055,0,99055,334.4527630805969,0.0004075487951987757
25025,99455,0,99455,335.4453649520874,0.0004013435912567003
25125,99855,0,99855,336.4456181526184,0.0003952591876055962
25225,100255,0,100255,337.4488501548767,0.00038926910819748805
25325,100655,0,100655,338.44034814834595,0.0003833427975293865
25425,101055,0,101055,339.4847753047943,0.0003774772172054246
25526,101459,0,101459,340.48418712615967,0.00037163947874811824
25626,101859,0,101859,341.48699736595154,0.0003659729725449927
25726,102259,0,102259,342.5179831981659,0.00036040546811693037
25826,102659,0,102659,343.5232219696045,0.00035490869049088346
25926,103059,0,103059,344.5140151977539,0.00034947369577205525
26026,103459,0,103459,345.5404930114746,0.0003441142167159695
26126,103859,0,103859,346.5290632247925,0.00033884478743114696
26226,104259,0,104259,347.5746190547943,0.00033366565119359153
26326,104659,0,104659,348.6023211479187,0.0003285623625134495
26426,105059,0,105059,349.65351819992065,0.00032353980652274715
26527,105463,0,105463,350.68159198760986,0.0003185604267722937
26627,105863,0,105863,351.6799590587616,0.00031371933830147517
26727,106263,0,106263,352.67128920555115,0.0003089547111937232
26827,106663,0,106663,353.6594431400299,0.0003042546872309285
26927,107063,0,107063,354.6641652584076,0.00029962096264257146
27027,107463,0,107463,355.65529322624207,0.00029506827443446815
27127,107863,0,107863,356.79106616973877,0.0002906055792065784
27227,108263,0,108263,357.886372089386,0.00028622549208219496
27327,108663,0,108663,358.9966812133789,0.0002819159369750738
27427,109063,0,109063,360.0048770904541,0.0002776670474268531
27528,109467,0,109467,361.075434923172,0.00027344288370076257
27628,109867,0,109867,362.10153007507324,0.00026934092248323907
27728,110267,0,110267,363.19413924217224,0.00026532895146723313
27828,110667,0,110667,364.3256850242615,0.00026138777792272333
27928,111067,0,111067,365.410117149353,0.0002574923490464453
28028,111467,0,111467,366.4783601760864,0.00025363063438622717
28128,111867,0,111867,367.58180022239685,0.0002498173679740786
28228,112267,0,112267,368.6898012161255,0.0002460785476639138
28328,112667,0,112667,369.73567509651184,0.0002424193866919694
28428,113067,0,113067,370.7259042263031,0.00023881403962149264
28529,113471,0,113471,371.74574422836304,0.00023520226694484332
28629,113871,0,113871,372.7768371105194,0.00023165407319258353
28729,114271,0,114271,373.84909415245056,0.00022814869049691638
28829,114671,0,114671,374.92775416374207,0.0002247076484011169
28929,115071,0,115071,376.01430010795593,0.00022133124997030147
29029,115471,0,115471,377.0426800251007,0.00021800847619289274
29129,115871,0,115871,378.12698698043823,0.00021473409427183202
29229,116271,0,116271,379.18932127952576,0.0002115068493260824
29329,116671,0,116671,380.28385305404663,0.00020832828602043848
29429,117071,0,117071,381.3401322364807,0.0002052019016221952
29530,117475,0,117475,382.4307670593262,0.0002020917180155017
29630,117875,0,117875,383.4690160751343,0.000199056694005001
29730,118275,0,118275,384.591924905777,0.00019606859155655275
29830,118675,0,118675,385.64229011535645,0.00019312579891759497
29930,119075,0,119075,386.6971802711487,0.0001902261216503937
30030,119475,0,119475,387.89540219306946,0.00018736527897840997
30130,119875,0,119875,389.1136722564697,0.00018453992392629458
30230,120275,0,120275,390.2558591365814,0.0001817618848748329
30330,120675,0,120675,391.4258060455322,0.0001790473959149819
30430,121075,0,121075,392.5677082538605,0.00017639893568001098
30531,121479,0,121479,394.2540521621704,0.00017377634308344243
30631,121879,0,121879,395.8938159942627,0.00017121008402431486
30731,122279,0,122279,397.1998071670532,0.00016866265796159258
30831,122679,0,122679,398.25563621520996,0.00016614825333388303
30931,123079,0,123079,399.4763581752777,0.0001636862735752721
31031,123479,0,123479,400.57799315452576,0.00016127849224959907
31131,123879,0,123879,401.90285897254944,0.000158911661910389
31231,124279,0,124279,403.03972911834717,0.000156566337465703
31331,124679,0,124679,404.0527353286743,0.00015423878029110062
31431,125079,0,125079,405.0433671474457,0.00015194383854620188
31532,125483,0,125483,406.05002617836,0.00014967728225045984
31632,125883,0,125883,406.9705812931061,0.00014748141364491927
31732,126283,0,126283,407.7231001853943,0.0001453236496155613
31832,126683,0,126683,408.81299805641174,0.00014318577820739394
31932,127083,0,127083,409.85258316993713,0.0001410630636861738
32032,127483,0,127483,410.917592048645,0.00013896495685249098
32132,127883,0,127883,411.94422221183777,0.00013690068219397215
32232,128283,0,128283,413.0728142261505,0.00013487394860806374
32332,128683,0,128683,414.21441411972046,0.00013288422901165894
32432,129083,0,129083,415.2850432395935,0.00013092481030741037
32533,129487,0,129487,416.303524017334,0.00012897076579163302
32633,129887,0,129887,417.32983922958374,0.00012706354815131054
32733,130287,0,130287,418.4362292289734,0.00012517977678015444
32833,130687,0,130687,419.4902651309967,0.00012332019549503957
32933,131087,0,131087,420.50152707099915,0.00012149010101979144
33033,131487,0,131487,421.6357972621918,0.00011969138451786213
33133,131887,0,131887,422.889475107193,0.00011792744669814292
33233,132287,0,132287,423.99755120277405,0.00011619614486706059
33333,132687,0,132687,425.22660303115845,0.00011448422249397478
33433,133087,0,133087,426.55300307273865,0.00011279029892638291
33534,133491,0,133491,428.3420422077179,0.00011110764052425343
33634,133891,0,133891,429.65023922920227,0.00010947545315292079
33734,134291,0,134291,430.98934412002563,0.00010788322633093137
33834,134691,0,134691,432.1551170349121,0.00010632222575153737
33934,135091,0,135091,433.7206072807312,0.00010477778169075889
34034,135491,0,135491,435.2484230995178,0.00010325130623508456
34134,135891,0,135891,436.99455404281616,0.00010174668960357438
34234,136291,0,136291,438.0871322154999,0.00010026908442009072
34334,136691,0,136691,439.2035140991211,9.882425639087327e-05
34434,137091,0,137091,440.3708510398865,9.740489934607251e-05
34535,137495,0,137495,442.57846331596375,9.598480524907882e-05
34635,137895,0,137895,444.6038911342621,9.459384537432654e-05
34735,138295,0,138295,446.07711720466614,9.321669210295596e-05
34835,138695,0,138695,447.1051902770996,9.186034875953142e-05
34935,139095,0,139095,448.11547207832336,9.052982550168082e-05
35035,139495,0,139495,449.10090708732605,8.92164727620526e-05
35135,139895,0,139895,450.098441362381,8.791907397811734e-05
35235,140295,0,140295,451.09479117393494,8.663904547262731e-05
35335,140695,0,140695,452.0951783657074,8.537736021308555e-05
35435,141095,0,141095,453.0814073085785,8.413637141505549e-05
35536,141499,0,141499,454.1009750366211,8.290218088452492e-05
35636,141899,0,141899,455.08919501304626,8.169775599583504e-05
35736,142299,0,142299,456.1527841091156,8.050980248098726e-05
35836,142699,0,142699,457.1680529117584,7.933879789632287e-05
35936,143099,0,143099,458.1706962585449,7.818308111840444e-05
36036,143499,0,143499,459.1510121822357,7.704229695343715e-05
36136,143899,0,143899,460.1360182762146,7.59171165284166e-05
36236,144299,0,144299,461.13270711898804,7.48103105131684e-05
36336,144699,0,144699,462.12735414505005,7.372422598790913e-05
36436,145099,0,145099,463.12385416030884,7.265879187829862e-05
36537,145503,0,145503,464.1199150085449,7.160137565200747e-05
36637,145903,0,145903,465.1146080493927,7.057174588152417e-05
36737,146303,0,146303,466.1013660430908,6.955945952849099e-05
36837,146703,0,146703,467.1002140045166,6.856652057333526e-05
36937,147103,0,147103,468.0889720916748,6.759265262571435e-05
37037,147503,0,147503,469.0820610523224,6.663467672217817e-05
37137,147903,0,147903,470.06203722953796,6.568809940505057e-05
37237,148303,0,148303,471.05312609672546,6.475095377543622e-05
37337,148703,0,148703,472.03926706314087,6.382472233856275e-05
37437,149103,0,149103,473.0179052352905,6.291342747488348e-05
37538,149507,0,149507,474.0270850658417,6.200868654269514e-05
37638,149907,0,149907,475.36258912086487,6.112581513221243e-05
37738,150307,0,150307,476.5173201560974,6.0251812479518895e-05
37838,150707,0,150707,477.52821230888367,5.938581968737049e-05
37938,151107,0,151107,478.5801191329956,5.853082032565416e-05
38038,151507,0,151507,480.0252311229706,5.769017168739846e-05
38138,151907,0,151907,481.16616010665894,5.686502208912203e-05
38238,152307,0,152307,482.3984282016754,5.605363998276093e-05
38338,152707,0,152707,483.63373017311096,5.525336418396882e-05
38438,153107,0,153107,484.94600009918213,5.446326214701382e-05
38539,153511,0,153511,486.29078912734985,5.367594125777318e-05
38639,153911,0,153911,487.6389229297638,5.2907840519948476e-05
38739,154311,0,154311,489.18898725509644,5.2151945661753104e-05
38839,154711,0,154711,490.29198932647705,5.1407917682869146e-05
38939,155111,0,155111,491.3472549915314,5.067568178899403e-05
39039,155511,0,155511,492.4073541164398,4.9954439275361084e-05
39139,155911,0,155911,493.49091601371765,4.924334693885037e-05
39239,156311,0,156311,494.7532353401184,4.8541978607420313e-05
39339,156711,0,156711,496.2634479999542,4.7851136506433944e-05
39439,157111,0,157111,497.4674801826477,4.7171751473896564e-05
39540,157515,0,157515,498.54406905174255,4.6498403011874585e-05
39640,157915,0,157915,499.63926219940186,4.5842853010942615e-05
39740,158315,0,158315,500.63603711128235,4.5196447928530915e-05
39840,158715,0,158715,501.64628314971924,4.455746233899277e-05
39940,159115,0,159115,502.6616430282593,4.39266923026386e-05
40040,159515,0,159515,503.6896412372589,4.330722491081732e-05
40140,159915,0,159915,504.7260551452637,4.2700188223661464e-05
40240,160315,0,160315,505.7306101322174,4.210478121716521e-05
40340,160715,0,160715,506.73683619499207,4.151688057124669e-05
40440,161115,0,161115,507.72879815101624,4.0933794901470184e-05
40541,161519,0,161519,508.7896182537079,4.035038955071414e-05
40641,161919,0,161919,509.8320822715759,3.9781410389822186e-05
40741,162319,0,162319,510.88662910461426,3.922359090576307e-05
40841,162719,0,162719,511.9524390697479,3.8676209565013035e-05
40941,163119,0,163119,513.0294530391693,3.8135728513416286e-05
41041,163519,0,163519,514.0424020290375,3.759931452240164e-05
41141,163919,0,163919,515.0468881130219,3.706755012762417e-05
41241,164319,0,164319,516.2123100757599,3.654310401692769e-05
41341,164719,0,164719,517.511214017868,3.602930826266534e-05
41441,165119,0,165119,518.7000062465668,3.552630053197368e-05
41542,165523,0,165523,519.7183301448822,3.502700887585216e-05
41642,165923,0,165923,520.775562286377,3.453848331963569e-05
41742,166323,0,166323,521.9549460411072,3.40545464973837e-05
41842,166723,0,166723,523.1511561870575,3.357609857912339e-05
41942,167123,0,167123,524.4625062942505,3.3105104687177495e-05
42042,167523,0,167523,525.88605427742,3.2643058733740716e-05
42142,167923,0,167923,527.1354732513428,3.218981763336597e-05
42242,168323,0,168323,528.4549281597137,3.174405997224603e-05
42342,168723,0,168723,529.6390731334686,3.130387613325087e-05
42442,169123,0,169123,530.8285531997681,3.086769732740725e-05
42543,169527,0,169527,531.9804141521454,3.0431192242622897e-05
42643,169927,0,169927,533.6264822483063,3.0004304201570393e-05
42743,170327,0,170327,534.8456251621246,2.958485139992288e-05
42843,170727,0,170727,536.2514982223511,2.9173888324019765e-05
42943,171127,0,171127,537.317253112793,2.8770464179708746e-05
43043,171527,0,171527,538.321542263031,2.8372448808121058e-05
43143,171927,0,171927,539.3156542778015,2.797807427382608e-05
43243,172327,0,172327,540.2998111248016,2.7588125409690452e-05
43343,172727,0,172727,541.3872423171997,2.720448877470487e-05
43443,173127,0,173127,542.4823281764984,2.682870052336601e-05
43544,173531,0,173531,543.7519881725311,2.645593846849383e-05
43644,173931,0,173931,544.8588061332703,2.6091094352291837e-05
43744,174331,0,174331,545.8787310123444,2.572785873359281e-05
43844,174731,0,174731,546.9218912124634,2.5366970880339185e-05
43944,175131,0,175131,548.0383841991425,2.5010573177106722e-05
44044,175531,0,175531,549.1710162162781,2.4661525675845345e-05
44144,175931,0,175931,550.2923800945282,2.4320668474522675e-05
44244,176331,0,176331,551.43421626091,2.3986592352350425e-05
44344,176731,0,176731,552.7863461971283,2.3657501962508774e-05
44444,177131,0,177131,554.0807480812073,2.3332351584105995e-05
44545,177535,0,177535,555.1927480697632,2.3008363738438773e-05
44645,177935,0,177935,556.395188331604,2.2692614418630773e-05
44745,178335,0,178335,557.4989211559296,2.2382231538718818e-05
44845,178735,0,178735,558.7036671638489,2.207622470308336e-05
44945,179135,0,179135,560.014847278595,2.1774014121078972e-05
45045,179535,0,179535,561.5879452228546,2.1474766996474042e-05
45145,179935,0,179935,562.8088240623474,2.1178689104366647e-05
45245,180335,0,180335,564.090968132019,2.0886337825348448e-05
45345,180735,0,180735,565.5297381877899,2.0598172496271158e-05
45445,181135,0,181135,566.6878509521484,2.0315056016407612e-05
45546,181539,0,181539,567.7800121307373,2.0034041301974822e-05
45646,181939,0,181939,568.9753642082214,1.9760409854259747e-05
45746,182339,0,182339,569.9647040367126,1.949068917943313e-05
45846,182739,0,182739,571.4102830886841,1.9224465537906003e-05
45946,183139,0,183139,572.5167112350464,1.896201192914267e-05
46046,183539,0,183539,573.6434030532837,1.8703711456500528e-05
46146,183939,0,183939,574.9623260498047,1.8449640067827e-05
46246,184339,0,184339,576.0870361328125,1.8199343147451876e-05
46346,184739,0,184739,577.1256680488586,1.7952264618032697e-05
46446,185139,0,185139,578.3857641220093,1.770799472806867e-05
46547,185543,0,185543,579.4220821857452,1.7464743831697954e-05
46647,185943,0,185943,580.5141031742096,1.722776873860336e-05
46747,186343,0,186343,581.3292181491852,1.6994910254835852e-05
46847,186743,0,186743,582.6953721046448,1.6765650870970367e-05
46947,187143,0,187143,583.9828500747681,1.6539186208977222e-05
47047,187543,0,187543,585.1963651180267,1.6315300860420997e-05
47147,187943,0,187943,586.4084820747375,1.6094185032023962e-05
47247,188343,0,188343,588.0410380363464,1.5876555508977693e-05
47347,188743,0,188743,589.2095663547516,1.5662663687851418e-05
47447,189143,0,189143,590.3033990859985,1.545228607945765e-05
47548,189547,0,189547,591.5232892036438,1.5243089138493048e-05
47648,189947,0,189947,592.6011960506439,1.5038979476610688e-05
47748,190347,0,190347,593.6105592250824,1.4838164235708716e-05
47848,190747,0,190747,594.6183032989502,1.4640945891980317e-05
47948,191147,0,191147,595.7158432006836,1.4447278005491406e-05
48048,191547,0,191547,596.7931661605835,1.4256848524202011e-05
48148,191947,0,191947,597.8204391002655,1.40689802950577e-05
48248,192347,0,192347,598.8248331546783,1.3883157446564332e-05
48348,192747,0,192747,599.8229801654816,1.36992177439814e-05
48448,193147,0,193147,600.8519032001495,1.351729771919296e-05
48549,193551,0,193551,601.9680330753326,1.3335837044536997e-05
48649,193951,0,193951,603.0528712272644,1.3158729742192206e-05
48749,194351,0,194351,604.0618481636047,1.2984057736325511e-05
48849,194751,0,194751,605.0527131557465,1.2811695616457415e-05
48949,195151,0,195151,606.0559799671173,1.264148639817577e-05
49049,195551,0,195551,607.0398392677307,1.2473403608076921e-05
49149,195951,0,195951,608.0317831039429,1.2307708479639038e-05
49249,196351,0,196351,609.0545401573181,1.214448625758407e-05
49349,196751,0,196751,610.0444111824036,1.1983733834179065e-05
49449,197151,0,197151,611.0636131763458,1.1825016208866703e-05
49550,197555,0,197555,612.0737330913544,1.1666644093359632e-05
49650,197955,0,197955,613.1485161781311,1.1511657256007075e-05
49750,198355,0,198355,614.1764721870422,1.135903485513368e-05
49850,198755,0,198755,615.1814641952515,1.1209135438638551e-05
49950,199155,0,199155,616.2290060520172,1.1062057889284107e-05
50050,199555,0,199555,617.2373633384705,1.0917302462094327e-05
50150,199955,0,199955,618.2452793121338,1.0774230643912528e-05
50250,200355,0,200355,619.2969691753387,1.063253491129586e-05
50350,200755,0,200755,620.2837240695953,1.0492483734337304e-05
50450,201155,0,201155,621.3276801109314,1.035474516791634e-05
50551,201559,0,201559,622.3290610313416,1.021822903828198e-05
50651,201959,0,201959,623.3441913127899,1.0085594708426323e-05
50751,202359,0,202359,624.3804280757904,9.954836535181103e-06
50851,202759,0,202759,625.3796589374542,9.825650048544928e-06
50951,203159,0,203159,626.3680601119995,9.697939698790288e-06
51051,203559,0,203559,627.3758492469788,9.571945114533722e-06
51151,203959,0,203959,628.4409573078156,9.447695721932687e-06
51251,204359,0,204359,629.5014071464539,9.324911077350676e-06
51351,204759,0,204759,630.578152179718,9.203035696461605e-06
51451,205159,0,205159,631.6558091640472,9.081650478476648e-06
51552,205563,0,205563,632.6903390884399,8.95962500118488e-06
51652,205963,0,205963,633.6959891319275,8.83985127087238e-06
51752,206363,0,206363,634.7289042472839,8.721849220794106e-06
51852,206763,0,206763,635.7285680770874,8.606096806631979e-06
51952,207163,0,207163,636.8051381111145,8.492665965099632e-06
52052,207563,0,207563,637.824969291687,8.381225596827836e-06
52152,207963,0,207963,638.8321640491486,8.271369276637015e-06
52252,208363,0,208363,639.8122990131378,8.16279965861016e-06
52352,208763,0,208763,640.8534829616547,8.055561275217626e-06
52452,209163,0,209163,641.8400650024414,7.949936598108902e-06
52553,209567,0,209567,642.8706271648407,7.845095367950762e-06
52653,209967,0,209967,643.8680372238159,7.742903785998902e-06
52753,210367,0,210367,644.8584632873535,7.642040998701366e-06
52853,210767,0,210767,645.9236991405487,7.5420329193684395e-06
52953,211167,0,211167,646.9664182662964,7.443137799215738e-06
53053,211567,0,211567,647.9657912254333,7.345820028657914e-06
53153,211967,0,211967,649.0217311382294,7.250603728363687e-06
53253,212367,0,212367,650.0586552619934,7.15766801946621e-06
53353,212767,0,212767,651.1012892723083,7.066473656269929e-06
53453,213167,0,213167,652.1935620307922,6.976346024624254e-06
53554,213571,0,213571,653.1913640499115,6.885916108395203e-06
53654,213971,0,213971,654.2576770782471,6.797099124601739e-06
53754,214371,0,214371,655.274697303772,6.7093271483412155e-06
53854,214771,0,214771,656.8361930847168,6.623070481088954e-06
53954,215171,0,215171,658.0087883472443,6.53819019410309e-06
54054,215571,0,215571,659.430251121521,6.454413882037678e-06
54154,215971,0,215971,660.6212720870972,6.371480296821456e-06
54254,216371,0,216371,662.3938090801239,6.28926962026742e-06
54354,216771,0,216771,664.0144181251526,6.2080586569873455e-06
54454,217171,0,217171,665.5412590503693,6.128068291095267e-06
54555,217575,0,217575,667.1645832061768,6.0485804600161595e-06
54655,217975,0,217975,668.675594329834,5.970969770861281e-06
54755,218375,0,218375,670.4293601512909,5.894223568229561e-06
54855,218775,0,218775,672.3742399215698,5.8180816778302945e-06
54955,219175,0,219175,674.3033351898193,5.742671881943044e-06
55055,219575,0,219575,675.4915812015533,5.6682689975973985e-06
55155,219975,0,219975,676.6361591815948,5.595117891605344e-06
55255,220375,0,220375,677.817877292633,5.523516138411069e-06
55355,220775,0,220775,678.9796681404114,5.4533916387236665e-06
55455,221175,0,221175,680.1013350486755,5.3845500601115786e-06
55556,221579,0,221579,681.5626201629639,5.316129703487026e-06
55656,221979,0,221979,682.7532021999359,5.249403219276246e-06
55756,222379,0,222379,683.8975882530212,5.1836920378081895e-06
55856,222779,0,222779,685.2395482063293,5.119123136614227e-06
55956,223179,0,223179,686.351056098938,5.0555465323844834e-06
56056,223579,0,223579,687.3846471309662,4.992782080638137e-06
56156,223979,0,223979,688.4062051773071,4.930689948811121e-06
56256,224379,0,224379,689.4379193782806,4.869135102791936e-06
56356,224779,0,224779,690.4742381572723,4.808255019351345e-06
56456,225179,0,225179,691.5622591972351,4.748228341129539e-06
56557,225583,0,225583,692.6293942928314,4.6885234610329356e-06
56657,225983,0,225983,693.6982400417328,4.630248797921739e-06
56757,226383,0,226383,694.799173116684,4.572668913662691e-06
56857,226783,0,226783,696.5837690830231,4.5156219338936226e-06
56957,227183,0,227183,698.0538511276245,4.459127358579368e-06
57057,227583,0,227583,699.2839541435242,4.40331125808424e-06
57157,227983,0,227983,700.9476132392883,4.348128492884911e-06
57257,228383,0,228383,702.1238760948181,4.293644517479232e-06
57357,228783,0,228783,703.341824054718,4.239798075609552e-06
57457,229183,0,229183,705.2493031024933,4.186517036364248e-06
57558,229587,0,229587,707.4480082988739,4.133340724856987e-06
57658,229987,0,229987,708.9408671855927,4.08139716676382e-06
57758,230387,0,230387,710.06059217453,4.030204162088082e-06
57858,230787,0,230787,711.6056010723114,3.9798110550305215e-06
57958,231187,0,231187,712.9833152294159,3.930221550922501e-06
58058,231587,0,231587,714.3864681720734,3.881311482298429e-06
58158,231987,0,231987,715.4723660945892,3.8332331369600245e-06
58258,232387,0,232387,716.6452369689941,3.7859352843292656e-06
58358,232787,0,232787,717.9499592781067,3.7394264613393535e-06
58458,233187,0,233187,719.4845969676971,3.693740422425617e-06
58559,233591,0,233591,720.7327680587769,3.648286751095104e-06
58659,233991,0,233991,721.9344301223755,3.6038327363250865e-06
58759,234391,0,234391,723.1373450756073,3.5598468900574956e-06
58859,234791,0,234791,724.2824430465698,3.5162069556923925e-06
58959,235191,0,235191,725.3549811840057,3.4729135677940472e-06
59059,235591,0,235591,726.4161510467529,3.430090824602499e-06
59159,235991,0,235991,727.7118473052979,3.387621914787003e-06
59259,236391,0,236391,728.9871249198914,3.345561302183569e-06
59359,236791,0,236791,730.4741811752319,3.3039740340263686e-06
59459,237191,0,237191,731.8067572116852,3.2627825045956263e-06
59560,237595,0,237595,733.1149852275848,3.2217623468362737e-06
59660,237995,0,237995,734.2683219909668,3.181754183696677e-06
59760,238395,0,238395,736.1057043075562,3.142352294922836e-06
59860,238795,0,238795,737.6260652542114,3.103545859882017e-06
59960,239195,0,239195,739.3872129917145,3.0652456821621016e-06
60060,239595,0,239595,740.919536113739,3.0273166125728335e-06
60160,239995,0,239995,742.6512761116028,2.989867056676196e-06
60260,240395,0,240395,743.8366949558258,2.952888321344867e-06
60360,240795,0,240795,745.287709236145,2.916320135033591e-06
60460,241195,0,241195,746.3824801445007,2.8802413999003536e-06
60561,241599,0,241599,747.4534063339233,2.8442250376086884e-06
60661,241999,0,241999,748.7622570991516,2.8089741283178198e-06
60761,242399,0,242399,749.8771481513977,2.7742600313758343e-06
60861,242799,0,242799,751.5456392765045,2.740040262608529e-06
60961,243199,0,243199,752.7018442153931,2.706389367869176e-06
61061,243599,0,243599,753.783370256424,2.6733382121301483e-06
61161,243999,0,243999,754.8596611022949,2.64069991370476e-06
61261,244399,0,244399,755.9157192707062,2.6084546714155837e-06
61361,244799,0,244799,756.9667780399323,2.5766848069360984e-06
61461,245199,0,245199,757.9608690738678,2.5452902395189833e-06
61562,245603,0,245603,759.0303871631622,2.5140911161542614e-06
61662,246003,0,246003,760.0438132286072,2.4837238245520025e-06
61762,246403,0,246403,761.0542650222778,2.4537474279728738e-06
61862,246803,0,246803,762.0401840209961,2.4242513185264145e-06
61962,247203,0,247203,763.0221741199493,2.395082194623818e-06
62062,247603,0,247603,764.1599049568176,2.3661778989874117e-06
62162,248003,0,248003,765.2604939937592,2.3377148662151028e-06
62262,248403,0,248403,766.2949151992798,2.3096265637023976e-06
62362,248803,0,248803,767.34334897995,2.281808213590547e-06
62462,249203,0,249203,768.3266880512238,2.2543788736567392e-06
62563,249607,0,249607,769.3407561779022,2.2267855488598186e-06
62663,250007,0,250007,770.4326503276825,2.199669948610493e-06
62763,250407,0,250407,771.4548561573029,2.1727766477733587e-06
62863,250807,0,250807,772.442223072052,2.1462690757759383e-06
62963,251207,0,251207,773.7432081699371,2.120178255857176e-06
63063,251607,0,251607,774.8062152862549,2.09454822417445e-06
63163,252007,0,252007,775.901123046875,2.0693017110775478e-06
63263,252407,0,252407,777.0236222743988,2.0443749484881163e-06
63363,252807,0,252807,778.0860903263092,2.0197617907224266e-06
63463,253207,0,253207,779.3427550792694,1.995493427360685e-06
63564,253611,0,253611,780.266520023346,1.97139229558571e-06
63664,254011,0,254011,781.0719332695007,1.9479418001527857e-06
63764,254411,0,254411,782.030641078949,1.924834509294109e-06
63864,254811,0,254811,783.0867431163788,1.9020028983841408e-06
63964,255211,0,255211,784.1868510246277,1.8793923292913581e-06
64064,255611,0,255611,785.2005131244659,1.8570328049087636e-06
64164,256011,0,256011,786.2473940849304,1.8349743397947918e-06
64264,256411,0,256411,787.372935295105,1.8132793296433024e-06
64364,256811,0,256811,788.4433310031891,1.7919418038348578e-06
64464,257211,0,257211,789.5576272010803,1.770918113164439e-06
64565,257615,0,257615,790.6588661670685,1.7499264036300537e-06
64665,258015,0,258015,791.7803702354431,1.7293333319452015e-06
64765,258415,0,258415,793.0903232097626,1.7089253274686808e-06
64865,258815,0,258815,794.1923530101776,1.6887238647171406e-06
64965,259215,0,259215,795.3986873626709,1.6687428933357523e-06
65065,259615,0,259615,796.4649271965027,1.6489829100005038e-06
65165,260015,0,260015,797.6697173118591,1.6293824477856277e-06
65265,260415,0,260415,798.7960503101349,1.6099276506428023e-06
65365,260815,0,260815,800.0661461353302,1.5905814654011146e-06
65465,261215,0,261215,801.3166501522064,1.5714139668683233e-06
65566,261619,0,261619,802.565092086792,1.5522837876226608e-06
65666,262019,0,262019,803.6415331363678,1.5336400666136054e-06
65766,262419,0,262419,804.6969132423401,1.515300850471348e-06
65866,262819,0,262819,805.6872119903564,1.497245275117191e-06
65966,263219,0,263219,806.6691403388977,1.4794424086375368e-06
66066,263619,0,263619,807.6774272918701,1.4618707073977875e-06
66166,264019,0,264019,808.6544580459595,1.4445520582828496e-06
66266,264419,0,264419,809.6196253299713,1.4274704444059194e-06
66366,264819,0,264819,810.8162460327148,1.4106444234349605e-06
66466,265219,0,265219,812.0272421836853,1.3940132227299357e-06
66567,265623,0,265623,813.1285643577576,1.3774039578916548e-06
66667,266023,0,266023,814.1375563144684,1.3611191454388932e-06
66767,266423,0,266423,815.2245512008667,1.345021182879363e-06
66867,266823,0,266823,816.2662572860718,1.3291447259736833e-06
66967,267223,0,267223,817.2963471412659,1.3135000798574967e-06
67067,267623,0,267623,818.3205161094666,1.2981024415150494e-06
67167,268023,0,268023,819.3667030334473,1.2829156725181327e-06
67267,268423,0,268423,820.4118509292603,1.2679262483326907e-06
67367,268823,0,268823,821.4513032436371,1.2531132991180455e-06
67467,269223,0,269223,822.4573440551758,1.2384682144442457e-06
67568,269627,0,269627,823.543799161911,1.2238452451863084e-06
67668,270027,0,270027,824.5630550384521,1.2095152150899361e-06
67768,270427,0,270427,825.6330552101135,1.1953278996768847e-06
67868,270827,0,270827,826.7277760505676,1.1812585198159799e-06
67968,271227,0,271227,827.7762720584869,1.1673167802833678e-06
68068,271627,0,271627,828.8376371860504,1.1534990541942596e-06
68168,272027,0,272027,829.8604590892792,1.1398314220677187e-06
68268,272427,0,272427,830.921168088913,1.1263105672165294e-06
68368,272827,0,272827,832.1719479560852,1.1129489175853223e-06
68468,273227,0,273227,833.3938670158386,1.0997318978161957e-06
68569,273631,0,273631,834.5086162090302,1.0865303243533404e-06
68669,274031,0,274031,835.5781490802765,1.0736133538596146e-06
68769,274431,0,274431,836.6413171291351,1.0608614281135875e-06
68869,274831,0,274831,837.6496601104736,1.0483012593675632e-06
68969,275231,0,275231,838.7254812717438,1.0359412601086447e-06
69069,275631,0,275631,839.8014409542084,1.023789525530111e-06
69169,276031,0,276031,840.9427199363708,1.011842107933497e-06
69269,276431,0,276431,842.0674731731415,1.0000944219321423e-06
69369,276831,0,276831,843.6644041538239,9.885471379049085e-07
69469,277231,0,277231,845.1625919342041,9.7718955479878e-07
69570,277635,0,277635,846.3538012504578,9.659094887044727e-07
69670,278035,0,278035,847.9398510456085,9.54903046785818e-07
69770,278435,0,278435,849.4691061973572,9.4404678818232e-07
69870,278835,0,278835,850.8184220790863,9.333108626545276e-07
69970,279235,0,279235,851.8698239326477,9.226982245004449e-07
70070,279635,0,279635,852.946702003479,9.121918523054026e-07
70170,280035,0,280035,854.1681931018829,9.017904365217595e-07
70270,280435,0,280435,855.3023171424866,8.914867277509191e-07
70370,280835,0,280835,856.3659851551056,8.812657899412108e-07
70470,281235,0,281235,857.4272072315216,8.711361565196021e-07
70571,281639,0,281639,858.5804421901703,8.609867966318388e-07
70671,282039,0,282039,859.6804389953613,8.510431707216438e-07
70771,282439,0,282439,860.7975351810455,8.411976006039792e-07
70871,282839,0,282839,861.8751800060272,8.314646398451331e-07
70971,283239,0,283239,863.0477240085602,8.218384883031475e-07
71071,283639,0,283639,864.5447962284088,8.123209272154853e-07
71171,284039,0,284039,866.1464612483978,8.029165958653523e-07
71271,284439,0,284439,867.525475025177,7.936242012795865e-07
71371,284839,0,284839,868.6835091114044,7.84454986341409e-07
71471,285239,0,285239,870.0586512088776,7.754000674016833e-07
71572,285643,0,285643,871.2820842266083,7.663821814855323e-07
71672,286043,0,286043,872.5120582580566,7.575649461618619e-07
71772,286443,0,286443,873.7398200035095,7.488728451730774e-07
71872,286843,0,286843,875.0853471755981,7.40303613269805e-07
71972,287243,0,287243,876.5599811077118,7.31869071489858e-07
72072,287643,0,287643,877.7067613601685,7.235787411459034e-07
72172,288043,0,288043,878.8241751194,7.154153025248268e-07
72272,288443,0,288443,879.9004542827606,7.073797434443381e-07
72372,288843,0,288843,881.0113611221313,6.994405857970477e-07
72472,289243,0,289243,882.0724651813507,6.91596409795027e-07
72573,289647,0,289647,883.2885921001434,6.837521241815563e-07
72673,290047,0,290047,884.7426149845123,6.76063614227455e-07
72773,290447,0,290447,885.9948070049286,6.684365460551952e-07
72873,290847,0,290847,887.1287441253662,6.608606357052393e-07
72973,291247,0,291247,888.4719820022583,6.533201527392151e-07
73073,291647,0,291647,889.6597559452057,6.458129668715352e-07
73173,292047,0,292047,890.8027250766754,6.383510968567983e-07
73273,292447,0,292447,892.1578443050385,6.309498024153505e-07
73373,292847,0,292847,893.4214472770691,6.236311401905401e-07
73473,293247,0,293247,894.4731872081757,6.164007865978117e-07
73574,293651,0,293651,895.5479040145874,6.09187964875479e-07
73674,294051,0,294051,896.8453812599182,6.021311735914442e-07
73774,294451,0,294451,897.9569911956787,5.951524542427206e-07
73874,294851,0,294851,899.3481891155243,5.88257375420663e-07
73974,295251,0,295251,900.7169382572174,5.814451520660815e-07
74074,295651,0,295651,901.9344160556793,5.747191750822218e-07
74174,296051,0,296051,902.990195274353,5.680764583261537e-07
74274,296451,0,296451,904.2461459636688,5.615087542563483e-07
74374,296851,0,296851,905.4452481269836,5.550197064147841e-07
74474,297251,0,297251,906.6694593429565,5.48611636532368e-07
74575,297655,0,297655,907.8476431369781,5.422367302184988e-07
74675,298055,0,298055,909.0447070598602,5.360308924718053e-07
74775,298455,0,298455,910.2183620929718,5.299344190555424e-07
74875,298855,0,298855,911.2995183467865,5.23939895091956e-07
74975,299255,0,299255,912.4112451076508,5.180314380096783e-07
75075,299655,0,299655,913.4860689640045,5.121924579850823e-07
75175,300055,0,300055,914.8848240375519,5.064118452941054e-07
75275,300455,0,300455,916.0268442630768,5.006896168826657e-07
75375,300855,0,300855,917.0905940532684,4.950239922248364e-07
75475,301255,0,301255,918.136744260788,4.894208573032311e-07
75576,301659,0,301659,919.264083147049,4.838201304410442e-07
75676,302059,0,302059,920.3298633098602,4.783333177991947e-07
75776,302459,0,302459,921.3424220085144,4.728986537459399e-07
75876,302859,0,302859,922.3772192001343,4.675228480748712e-07
75976,303259,0,303259,923.3843071460724,4.6220236043669274e-07
76076,303659,0,303659,924.3918220996857,4.56942263802604e-07
76176,304059,0,304059,925.3893821239471,4.5173454659227366e-07
76276,304459,0,304459,926.3973910808563,4.465713470526085e-07
76376,304859,0,304859,927.3936371803284,4.4145151777678366e-07
76476,305259,0,305259,928.4042851924896,4.3637294947482686e-07
76577,305663,0,305663,929.409585237503,4.3129788306002076e-07
76677,306063,0,306063,930.4236512184143,4.2633601200510203e-07
76777,306463,0,306463,931.4365103244781,4.2144866600397913e-07
76877,306863,0,306863,932.4453852176666,4.166373875156341e-07
76977,307263,0,307263,933.4628882408142,4.119053954311408e-07
77077,307663,0,307663,934.5746963024139,4.072453579507207e-07
77177,308063,0,308063,936.0996351242065,4.026567022653564e-07
77277,308463,0,308463,937.7437093257904,3.9813683556749264e-07
77377,308863,0,308863,938.8904850482941,3.936821479100894e-07
77477,309263,0,309263,939.9566671848297,3.8929141694876395e-07
77578,309667,0,309667,940.9691932201385,3.849181033926139e-07
77678,310067,0,310067,942.0533401966095,3.806434913733557e-07
77778,310467,0,310467,943.1178741455078,3.764251248863545e-07
77878,310867,0,310867,944.1489191055298,3.7225677148854326e-07
77978,311267,0,311267,945.3985750675201,3.681427430983257e-07
78078,311667,0,311667,946.6487441062927,3.6407689873230597e-07
78178,312067,0,312067,947.7825500965118,3.600605246330963e-07
78278,312467,0,312467,948.9133801460266,3.560850307839211e-07
78378,312867,0,312867,950.0206341743469,3.5214890799133697e-07
78478,313267,0,313267,951.1887900829315,3.482481584211923e-07
78579,313671,0,313671,952.3502221107483,3.4434168574921477e-07
78679,314071,0,314071,953.6887972354889,3.4050992210492806e-07
78779,314471,0,314471,955.1924362182617,3.3671034773279705e-07
78879,314871,0,314871,956.8400461673737,3.3294519206690856e-07
78979,315271,0,315271,957.9179210662842,3.292108782800375e-07
79079,315671,0,315671,959.1221830844879,3.2550911060341167e-07
79179,316071,0,316071,960.2934482097626,3.218395227398407e-07
79279,316471,0,316471,961.3661522865295,3.1820662474047363e-07
79379,316871,0,316871,962.3666622638702,3.1461431271844557e-07
79479,317271,0,317271,963.3950293064117,3.1106163730826524e-07
79580,317675,0,317675,964.5986909866333,3.0752429550424507e-07
79680,318075,0,318075,966.1613349914551,3.040672379606385e-07
79780,318475,0,318475,967.7474451065063,3.0066529580455973e-07
79880,318875,0,318875,969.2014091014862,2.973142055404846e-07
79980,319275,0,319275,970.7110960483551,2.9401600084151916e-07
80080,319675,0,319675,971.8899283409119,2.9076673490048286e-07
80180,320075,0,320075,972.9514880180359,2.875612438718773e-07
80280,320475,0,320475,974.9245312213898,2.8439378976916807e-07
80380,320875,0,320875,977.3543212413788,2.812588848199686e-07
80480,321275,0,321275,980.0509810447693,2.781559329971361e-07
80581,321679,0,321679,982.0676741600037,2.7504706398147847e-07
80681,322079,0,322079,983.5015389919281,2.71999773485749e-07
80781,322479,0,322479,985.3971531391144,2.689769071097198e-07
80881,322879,0,322879,988.3764650821686,2.6598275593857814e-07
80981,323279,0,323279,989.6701080799103,2.6301675240739e-07
81081,323679,0,323679,991.2975442409515,2.600799408329081e-07
81181,324079,0,324079,993.1775691509247,2.571725825193734e-07
81281,324479,0,324479,995.2193410396576,2.5429492924187986e-07
81381,324879,0,324879,996.4848623275757,2.51446044277539e-07
81481,325279,0,325279,997.5870652198792,2.486218261936775e-07
81582,325683,0,325683,998.7318289279938,2.4579569633958043e-07
81682,326083,0,326083,999.8632659912109,2.430193904617974e-07
81782,326483,0,326483,1001.394195318222,2.4026697880435034e-07
81882,326883,0,326883,1002.6235539913177,2.3753980555745512e-07
81982,327283,0,327283,1003.8423261642456,2.3483703164491856e-07
82082,327683,0,327683,1005.1575553417206,2.3216298191340907e-07
82182,328083,0,328083,1006.3331582546234,2.2951926401383224e-07
82282,328483,0,328483,1007.4084672927856,2.269087968593467e-07
82382,328883,0,328883,1008.6117062568665,2.2433209792170738e-07
82482,329283,0,329283,1010.1392540931702,2.2179468603730744e-07
82583,329687,0,329687,1011.2276751995087,2.1926664651152742e-07
82683,330087,0,330087,1012.7358913421631,2.1680084153062058e-07
82783,330487,0,330487,1013.8506863117218,2.1436801665210095e-07
82883,330887,0,330887,1015.1302771568298,2.119662457054118e-07
82983,331287,0,331287,1016.5265882015228,2.0959815876851192e-07
83083,331687,0,331687,1018.1083650588989,2.0726120171785138e-07
83183,332087,0,332087,1019.9863741397858,2.0495843331358286e-07
83283,332487,0,332487,1021.4649641513824,2.026877893109564e-07
83383,332887,0,332887,1022.6689400672913,2.0045176143843585e-07
83483,333287,0,333287,1023.9901113510132,1.982443994630695e-07
83584,333691,0,333691,1025.205542087555,1.9604628638782837e-07
83684,334091,0,334091,1026.5016911029816,1.9389606439804818e-07
83784,334491,0,334491,1027.9447782039642,1.9176870427346846e-07
83884,334891,0,334891,1029.1786050796509,1.8966417403643064e-07
83984,335291,0,335291,1030.8003282546997,1.8757449454631704e-07
84084,335691,0,335691,1031.9380910396576,1.8550118310140662e-07
84184,336091,0,336091,1033.0166010856628,1.8344146101589218e-07
84284,336491,0,336491,1034.3357932567596,1.81398277875427e-07
84384,336891,0,336891,1035.4633440971375,1.7937110694401527e-07
84484,337291,0,337291,1036.5045862197876,1.7736662695707541e-07
84585,337695,0,337695,1037.5681290626526,1.7536400398700696e-07
84685,338095,0,338095,1038.6069691181183,1.7340465970212296e-07
84785,338495,0,338495,1039.6131031513214,1.7146955118389847e-07
84885,338895,0,338895,1040.6616671085358,1.6955452625618653e-07
84985,339295,0,339295,1041.6590151786804,1.6766379965195107e-07
85085,339695,0,339695,1043.002869129181,1.6579624741978435e-07
85185,340095,0,340095,1044.4244811534882,1.6395272018562886e-07
85285,340495,0,340495,1046.1672821044922,1.6213430741596268e-07
85385,340895,0,340895,1048.534559249878,1.603423493146407e-07
85485,341295,0,341295,1050.0151982307434,1.5857443262925334e-07
85586,341699,0,341699,1051.1447081565857,1.5681517234473405e-07
85686,342099,0,342099,1052.274167060852,1.5509986516961643e-07
85786,342499,0,342499,1053.4609920978546,1.534089002977632e-07
85886,342899,0,342899,1054.474314212799,1.5174556034614455e-07
85986,343299,0,343299,1055.7289361953735,1.5010475247312503e-07
86086,343699,0,343699,1057.9921810626984,1.4848430850428215e-07
86186,344099,0,344099,1060.2575380802155,1.4688344504131224e-07
86286,344499,0,344499,1062.8989062309265,1.4529864449529885e-07
86386,344899,0,344899,1064.1817650794983,1.4372807903555653e-07
86486,345299,0,345299,1065.7103242874146,1.4217254855254989e-07
86587,345703,0,345703,1067.0061461925507,1.4061428989036337e-07
86687,346103,0,346103,1068.5022420883179,1.3908225498039293e-07
86787,346503,0,346503,1070.105339050293,1.3756139940271955e-07
86887,346903,0,346903,1071.1293580532074,1.3604743285176824e-07
86987,347303,0,347303,1072.156372308731,1.3454252422643153e-07
87087,347703,0,347703,1073.3452022075653,1.3304926794014083e-07
87187,348103,0,348103,1074.3824472427368,1.3156623749083803e-07
87287,348503,0,348503,1075.4003932476044,1.3009773316822023e-07
87387,348903,0,348903,1076.4065861701965,1.286464938143749e-07
87487,349303,0,349303,1077.437441110611,1.2721104614696963e-07
87588,349707,0,349707,1078.4747912883759,1.2577966178835254e-07
87688,350107,0,350107,1079.4963171482086,1.2438094387859732e-07
87788,350507,0,350507,1080.5023410320282,1.229991935762216e-07
87888,350907,0,350907,1081.5497682094574,1.2163643110099446e-07
87988,351307,0,351307,1082.6328670978546,1.2029139293048514e-07
88088,351707,0,351707,1083.8623220920563,1.1896061635752625e-07
88188,352107,0,352107,1084.8975591659546,1.1764813733733752e-07
88288,352507,0,352507,1085.9750430583954,1.1635133451015061e-07
88388,352907,0,352907,1087.1409599781036,1.1506990649353804e-07
88488,353307,0,353307,1088.2605140209198,1.13806669551508e-07
88589,353711,0,353711,1089.3632380962372,1.1254841742980241e-07
88689,354111,0,354111,1090.4624450206757,1.1131851544271273e-07
88789,354511,0,354511,1091.5379860401154,1.101063177997413e-07
88889,354911,0,354911,1092.62313914299,1.0890621649539111e-07
88989,355311,0,355311,1093.7232131958008,1.0771832314092281e-07
89089,355711,0,355711,1094.8296341896057,1.0654335374651037e-07
89189,356111,0,356111,1096.1392612457275,1.053759700281656e-07
89289,356511,0,356511,1097.2922360897064,1.0421716900829841e-07
89389,356911,0,356911,1098.3739030361176,1.0306856991339264e-07
89489,357311,0,357311,1099.5771770477295,1.0192665470982408e-07
89590,357715,0,357715,1101.0182111263275,1.0078184585451295e-07
89690,358115,0,358115,1102.718159198761,9.965863869115317e-08
89790,358515,0,358515,1104.093513250351,9.854282207238429e-08
89890,358915,0,358915,1105.4410872459412,9.743925169987752e-08
89990,359315,0,359315,1106.5551590919495,9.63467050150379e-08
90090,359715,0,359715,1107.7799799442291,9.526257018720066e-08
90190,360115,0,360115,1108.785926103592,9.419193935644718e-08
90290,360515,0,360515,1109.8138873577118,9.313354786771865e-08
90390,360915,0,360915,1110.8434171676636,9.208467522870625e-08
90490,361315,0,361315,1111.88347530365,9.10512516981325e-08
90591,361719,0,361719,1112.9739980697632,9.002063463121937e-08
90691,362119,0,362119,1114.0708799362183,8.901403308725061e-08
90791,362519,0,362519,1115.128065109253,8.802473281360776e-08
90891,362919,0,362919,1116.166395187378,8.704841692783936e-08
90991,363319,0,363319,1117.1768102645874,8.608767001960605e-08
91091,363719,0,363719,1118.1964461803436,8.514478683632309e-08
91191,364119,0,364119,1119.2165212631226,8.421453346511235e-08
91291,364519,0,364519,1120.2221901416779,8.32975128501969e-08
91391,364919,0,364919,1121.2344102859497,8.239677103729871e-08
91491,365319,0,365319,1122.2495033740997,8.150406982451709e-08
91592,365723,0,365723,1123.7854890823364,8.061479824915943e-08
91692,366123,0,366123,1124.9350662231445,7.974387422840997e-08
91792,366523,0,366523,1126.3274581432343,7.887948789447006e-08
91892,366923,0,366923,1127.3863141536713,7.802711139763855e-08
91992,367323,0,367323,1128.514074087143,7.718147819396633e-08
92092,367723,0,367723,1129.5837752819061,7.634159550578226e-08
92192,368123,0,368123,1130.6263892650604,7.551134497436577e-08
92292,368523,0,368523,1131.6822383403778,7.468767356755495e-08
92392,368923,0,368923,1132.8006372451782,7.387189050439875e-08
92492,369323,0,369323,1133.9880361557007,7.306421831716721e-08
92593,369727,0,369727,1135.0615921020508,7.225596467286293e-08
92693,370127,0,370127,1136.1750662326813,7.14622812174851e-08
92793,370527,0,370527,1137.2107751369476,7.06759930821609e-08
92893,370927,0,370927,1138.326689004898,6.989677117076018e-08
92993,371327,0,371327,1139.4300472736359,6.912612654031898e-08
93093,371727,0,371727,1140.6457750797272,6.836331134107448e-08
93193,372127,0,372127,1141.8034522533417,6.761064901178e-08
93293,372527,0,372527,1142.8753521442413,6.68670578513105e-08
93393,372927,0,372927,1143.9127690792084,6.613454563806163e-08
93493,373327,0,373327,1144.9707782268524,6.541222325576293e-08
93594,373731,0,373731,1146.0220091342926,6.46940292654225e-08
93694,374131,0,374131,1147.1108300685883,6.39936951211201e-08
93794,374531,0,374531,1148.1831641197205,6.330341616316238e-08
93894,374931,0,374931,1149.2012090682983,6.262325789121572e-08
93994,375331,0,375331,1150.2771520614624,6.195165795092965e-08
94094,375731,0,375731,1151.2844462394714,6.12889114372425e-08
94194,376131,0,376131,1152.2869460582733,6.063332235305462e-08
94294,376531,0,376531,1153.309261083603,5.9984956998014e-08
94394,376931,0,376931,1154.3012590408325,5.934233531774784e-08
94494,377331,0,377331,1155.3132452964783,5.870491644438914e-08
94595,377735,0,377735,1156.320237159729,5.80657044164055e-08
94695,378135,0,378135,1157.3337421417236,5.743674085479315e-08
94795,378535,0,378535,1158.3331441879272,5.6812004998798084e-08
94895,378935,0,378935,1159.349106311798,5.6191289592457075e-08
94995,379335,0,379335,1160.3232700824738,5.557543491370609e-08
95095,379735,0,379735,1161.3079252243042,5.496442636523241e-08
95195,380135,0,380135,1162.2878692150116,5.435870121136235e-08
95295,380535,0,380535,1163.2618160247803,5.375852331662496e-08
95395,380935,0,380935,1164.24946808815,5.316373849877799e-08
95495,381335,0,381335,1165.23513007164,5.2574931379234836e-08
95596,381739,0,381739,1166.2439930438995,5.1985933236070685e-08
95696,382139,0,382139,1167.22824716568,5.140887452552616e-08
95796,382539,0,382539,1168.2298302650452,5.083780943217572e-08
95896,382939,0,382939,1169.1600761413574,5.027314531429729e-08
95996,383339,0,383339,1169.8720932006836,4.971497222426046e-08
96096,383739,0,383739,1171.0124940872192,4.9164000644309835e-08
96196,384139,0,384139,1171.7770371437073,4.862067011163972e-08
96296,384539,0,384539,1172.5745720863342,4.80850914426928e-08
96396,384939,0,384939,1173.7295711040497,4.755767303250286e-08
96496,385339,0,385339,1174.8598430156708,4.703757639862222e-08
96597,385743,0,385743,1175.966480255127,4.651979405712348e-08
96697,386143,0,386143,1176.7894961833954,4.601303013606069e-08
96797,386543,0,386543,1177.5492541790009,4.551266894616704e-08
96897,386943,0,386943,1178.3781323432922,4.5017193642435716e-08
96997,387343,0,387343,1179.352536201477,4.452738903731044e-08
97097,387743,0,387743,1180.275621175766,4.4042361795700234e-08
97197,388143,0,388143,1181.02214717865,4.356238542056959e-08
97297,388543,0,388543,1181.7586982250214,4.308732859046706e-08
97397,388943,0,388943,1182.6723272800446,4.2616768134765095e-08
97497,389343,0,389343,1183.4478282928467,4.215118823121505e-08
97598,389747,0,389747,1184.644632101059,4.1685124613830125e-08
97698,390147,0,390147,1185.362755060196,4.1228433487632625e-08
97798,390547,0,390547,1186.058223247528,4.077539389436083e-08
97898,390947,0,390947,1186.8260741233826,4.032631789071949e-08
97998,391347,0,391347,1187.5545053482056,3.988070972476413e-08
98098,391747,0,391747,1188.2228801250458,3.943868396650517e-08
98198,392147,0,392147,1188.8985600471497,3.9000731195867856e-08
98298,392547,0,392547,1189.647919178009,3.856680814685892e-08
98398,392947,0,392947,1190.3186831474304,3.8138081893172694e-08
98498,393347,0,393347,1190.9794092178345,3.7714119863253e-08
98599,393751,0,393751,1191.686457157135,3.729179949919601e-08
98699,394151,0,394151,1192.3494062423706,3.687899354533666e-08
98799,394551,0,394551,1193.0217730998993,3.64720343999125e-08
98899,394951,0,394951,1193.7159841060638,3.607072189358274e-08
98999,395351,0,395351,1194.3831901550293,3.5675037623247156e-08
99099,395751,0,395751,1195.0449483394623,3.528507681533561e-08
99199,396151,0,396151,1195.72380900383,3.49004885007863e-08
99299,396551,0,396551,1196.4018700122833,3.452136691670143e-08
99399,396951,0,396951,1197.2123210430145,3.414743518920771e-08
99499,397351,0,397351,1198.0194561481476,3.377871398734246e-08
99600,397755,0,397755,1198.7835252285004,3.341149102622366e-08
99700,398155,0,398155,1199.5125889778137,3.3052810473139837e-08
99800,398555,0,398555,1200.3517112731934,3.269894022201112e-08
99900,398955,0,398955,1201.065805196762,3.234938905480299e-08
100000,399355,0,399355,1201.8951790332794,3.2003996086682737e-08


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007729530334472656,30.358106049564984
100,252,0,252,0.7068758010864258,0.2584702496066637
200,504,0,504,1.379183053970337,0.10025228889566092
300,757,0,757,2.0684399604797363,0.05354232784000942
400,1007,0,1007,2.7371439933776855,0.04118183074080015
501,1259,0,1259,3.395610809326172,0.03212008761769572
601,1511,0,1511,4.045492887496948,0.026550400741840233
701,1761,0,1761,4.715965032577515,0.022253473456958668
801,2013,0,2013,5.367310047149658,0.017617868455366646
901,2262,0,2262,6.01697301864624,0.014662611161370801
1001,2512,0,2512,6.672208786010742,0.011962667368031256
1101,2760,0,2760,7.313669919967651,0.009501045770622368
1201,3013,0,3013,7.967495918273926,0.007629167055048466
1301,3263,0,3263,8.737348794937134,0.0060928937607256884
1401,3513,0,3513,9.461069107055664,0.005125194375011903
1502,3764,0,3764,10.340143918991089,0.0043152279799267045
1602,4003,0,4003,11.070133924484253,0.0038042693624838367
1702,4249,0,4249,11.953434944152832,0.003289468275864946
1802,4498,0,4498,12.598495960235596,0.0027370060050925966
1902,4742,0,4742,13.230838060379028,0.0024009989456067883
2002,4970,0,4970,13.843727111816406,0.0022620802558184962
2102,5220,0,5220,14.467022180557251,0.001993849435343263
2202,5468,0,5468,15.116336822509766,0.0017790620894565959
2302,5694,0,5694,15.739657878875732,0.001686982584417212
2402,5921,0,5921,16.355583906173706,0.0016136342708067159
2503,6141,0,6141,16.98948097229004,0.001568348894393168
2603,6353,0,6353,17.605875968933105,0.0015383013425077706
2703,6569,0,6569,18.21681308746338,0.0014969245093177557
2803,6778,0,6778,18.826438903808594,0.0014692927979711983
2903,6978,0,6978,19.452043056488037,0.001455371015657392
3003,7178,0,7178,20.071763038635254,0.0014414202912371972
3103,7378,0,7378,20.69378399848938,0.0014291242240314893
3203,7578,0,7578,21.33190894126892,0.0014173919844090417
3303,7778,0,7778,21.9515221118927,0.0014059351458918633
3403,7982,0,7982,22.565647840499878,0.0013896522951835479
3504,8204,0,8204,23.191898107528687,0.0013468770142071734
3604,8424,0,8424,23.808932065963745,0.001309703265807277
3704,8627,0,8627,24.419151782989502,0.0012950370323156109
3804,8827,0,8827,25.123759031295776,0.0012839912619955068
3904,9027,0,9027,25.743422985076904,0.0012736515872593822
4004,9227,0,9227,26.345382928848267,0.001263644071159475
4104,9427,0,9427,27.023279190063477,0.0012538186059952879
4204,9627,0,9627,27.67383599281311,0.0012440576751176337
4304,9827,0,9827,28.302362203598022,0.0012344217955391433
4404,10027,0,10027,28.927103996276855,0.0012248451385586648
4505,10229,0,10229,29.636065006256104,0.001215275785555544
4605,10429,0,10429,30.24572992324829,0.0012058541351347418
4705,10629,0,10629,30.847866773605347,0.0011965243775971769
4805,10829,0,10829,31.444740772247314,0.001187239629111943
4905,11029,0,11029,32.08491492271423,0.0011780640177723562
5005,11229,0,11229,32.70137095451355,0.0011689179926348255
5105,11429,0,11429,33.402997970581055,0.0011598643366503097
5205,11629,0,11629,34.11725378036499,0.0011508732958342587
5305,11829,0,11829,34.7608699798584,0.0011419386771410434
5405,12029,0,12029,35.388041973114014,0.0011330806723231933
5506,12231,0,12231,36.04432415962219,0.0011241863769342836
5606,12431,0,12431,36.71251893043518,0.0011154487440146873
5706,12631,0,12631,37.392329931259155,0.0011067594856848282
5806,12831,0,12831,38.04498314857483,0.001098148373770333
5906,13031,0,13031,38.713518142700195,0.0010895849939988825
6006,13231,0,13231,39.416255950927734,0.0010811070554585178
6106,13431,0,13431,40.02256679534912,0.0010726725806420659
6206,13631,0,13631,40.651983976364136,0.0010643270736202508
6306,13831,0,13831,41.260719776153564,0.0010560548511251823
6406,14031,0,14031,41.85399913787842,0.0010478504535294789
6507,14233,0,14233,42.456090211868286,0.0010396539829893715
6607,14433,0,14433,43.06252908706665,0.0010316157105679075
6707,14633,0,14633,43.66241788864136,0.0010236619342892095
6807,14833,0,14833,44.25987887382507,0.001015788713083205
6907,15033,0,15033,44.86520981788635,0.00100800942591253
7007,15233,0,15233,45.46085000038147,0.0010002993147332677
7107,15433,0,15433,46.065337896347046,0.0009926842602501259
7207,15633,0,15633,46.67070198059082,0.000985136917510493
7307,15833,0,15833,47.28620481491089,0.000977677415512971
7407,16033,0,16033,47.888723850250244,0.0009703001268882239
7508,16235,0,16235,48.49437499046326,0.0009629107201948288
7608,16435,0,16435,49.11427092552185,0.0009556840689592388
7708,16635,0,16635,49.71981501579285,0.0009485176226957701
7808,16835,0,16835,50.322710037231445,0.0009414199962282755
7908,17035,0,17035,50.922971963882446,0.0009343843112065706
8008,17235,0,17235,51.60275197029114,0.0009274205350711474
8108,17435,0,17435,52.29482293128967,0.0009204924942285719
8208,17635,0,17635,52.92790985107422,0.0009136286913271874
8308,17835,0,17835,53.54347109794617,0.0009068068343480386
8408,18035,0,18035,54.163559913635254,0.0009000270090566092
8509,18237,0,18237,54.77231001853943,0.0008932266933670874
8609,18437,0,18437,55.382158041000366,0.000886526134108414
8709,18637,0,18637,55.991092920303345,0.0008798703917080213
8809,18837,0,18837,56.60236191749573,0.0008732388405790019
8909,19037,0,19037,57.206937074661255,0.0008666458561685062
9009,19237,0,19237,57.81745886802673,0.0008600793249633281
9109,19437,0,19437,58.43125891685486,0.0008535567535819349
9209,19637,0,19637,59.035927057266235,0.0008470499035956939
9309,19837,0,19837,59.6563560962677,0.0008405847965517346
9409,20037,0,20037,60.292248010635376,0.0008341569660013585
9510,20239,0,20239,60.92379283905029,0.0008276910640619939
9610,20439,0,20439,61.55014705657959,0.0008213421525889225
9710,20639,0,20639,62.31665515899658,0.0008150230559175037
9810,20839,0,20839,62.911009073257446,0.0008087508388999406
9910,21039,0,21039,63.513838052749634,0.0008025177898582031
10010,21239,0,21239,64.13097286224365,0.0007963358147768895
10110,21439,0,21439,64.72679400444031,0.0007901961507791906
10210,21639,0,21639,65.32241296768188,0.0007841150761982164
10310,21839,0,21839,65.91669201850891,0.0007780758068359257
10410,22039,0,22039,66.52472400665283,0.0007720959792644743
10511,22241,0,22241,67.17713212966919,0.0007661133807162037
10611,22441,0,22441,67.78945517539978,0.0007602381962508519
10711,22641,0,22641,68.48090076446533,0.0007544339932959039
10811,22841,0,22841,69.11091899871826,0.0007486817152696908
10911,23041,0,23041,69.73817896842957,0.0007429864672240095
11011,23241,0,23241,70.42927098274231,0.0007373467912476561
11111,23441,0,23441,71.06552910804749,0.0007317670519517288
11211,23641,0,23641,71.68601393699646,0.0007262271186072409
11311,23841,0,23841,72.29236507415771,0.0007207458053562501
11411,24041,0,24041,72.92595195770264,0.0007153041910518533
11512,24243,0,24243,73.53457403182983,0.0007098528903494391
11612,24443,0,24443,74.16267585754395,0.0007045043948059424
11712,24643,0,24643,74.78318214416504,0.0006991866902834604
11812,24843,0,24843,75.46767592430115,0.0006939131820039643
11912,25043,0,25043,76.08375287055969,0.0006886686979943295
12012,25243,0,25243,76.69523692131042,0.0006834596379482868
12112,25443,0,25443,77.32318997383118,0.0006782810810842254
12212,25643,0,25643,78.02672100067139,0.000673140277194275
12312,25843,0,25843,78.77969694137573,0.0006680172446606728
12412,26043,0,26043,79.38611793518066,0.000662933542348563
12513,26245,0,26245,79.99329781532288,0.0006578274647383251
12613,26445,0,26445,80.62433791160583,0.000652794812909588
12713,26645,0,26645,81.32913303375244,0.0006478020725564155
12813,26845,0,26845,82.02087187767029,0.0006428315891682619
12913,27045,0,27045,82.64428114891052,0.0006378926848420316
13013,27245,0,27245,83.23762512207031,0.0006329784244122047
13113,27445,0,27445,83.8675229549408,0.0006280947899234017
13213,27645,0,27645,84.46443295478821,0.0006232334516178511
13313,27845,0,27845,85.07261896133423,0.0006184054021369296
13413,28045,0,28045,85.69485807418823,0.0006135939992542019
13514,28247,0,28247,86.30983996391296,0.0006087694716298938
13614,28447,0,28447,86.92777490615845,0.0006040247923667176
13714,28647,0,28647,87.54356002807617,0.0005993051498557232
13814,28847,0,28847,88.17477989196777,0.0005946281900220586
13914,29047,0,29047,88.80349683761597,0.0005899840208390282
14014,29247,0,29247,89.41207098960876,0.000585378590315593
14114,29447,0,29447,90.02428913116455,0.0005808136705156818
14214,29647,0,29647,90.63132500648499,0.0005762942964938985
14314,29847,0,29847,91.3162739276886,0.0005718093606579084
14414,30047,0,30047,92.07652187347412,0.0005673766887800034
14515,30249,0,30249,92.73198795318604,0.00056293813812618
14615,30449,0,30449,93.40262389183044,0.0005585868011223772
14715,30649,0,30649,94.00507497787476,0.0005542857290798216
14815,30849,0,30849,94.6109938621521,0.000550023656887512
14915,31049,0,31049,95.27486681938171,0.0005458078546689329
15015,31249,0,31249,95.9251799583435,0.0005416327920443533
15115,31449,0,31449,96.57166314125061,0.0005375001520164296
15215,31649,0,31649,97.1998028755188,0.0005334065235919501
15315,31849,0,31849,97.79765820503235,0.0005293572486470912
15415,32049,0,32049,98.41478300094604,0.0005253385886448999
15516,32251,0,32251,99.02612209320068,0.0005213237067526812
15616,32451,0,32451,99.63762593269348,0.0005173861963796446
15716,32651,0,32651,100.24147510528564,0.0005134822703219745
15816,32851,0,32851,100.85399985313416,0.0005096197051733007
15916,33051,0,33051,101.46249198913574,0.0005057893169031855
16016,33251,0,33251,102.08565616607666,0.0005019918295248721
16116,33451,0,33451,102.71265888214111,0.0004982251305301748
16216,33651,0,33651,103.32244896888733,0.0004944885121008328
16316,33851,0,33851,103.92506384849548,0.0004907738364088092
16416,34051,0,34051,104.5291359424591,0.0004870877120369311
16517,34253,0,34253,105.15603685379028,0.0004833804984239596
16617,34453,0,34453,105.76220202445984,0.0004797330493777302
16717,34653,0,34653,106.38558197021484,0.00047610690183506405
16817,34853,0,34853,107.0181450843811,0.00047249765018663955
16917,35053,0,35053,107.63880181312561,0.00046891116119504323
17017,35253,0,35253,108.25740599632263,0.0004653437519083225
17117,35453,0,35453,108.8708701133728,0.0004617962528859499
17217,35653,0,35653,109.49806594848633,0.0004582701824303153
17317,35853,0,35853,110.10927200317383,0.0004547687604330165
17417,36053,0,36053,110.71548795700073,0.00045128437346690533
17518,36255,0,36255,111.32962989807129,0.0004477930877810582
17618,36455,0,36455,111.92428708076477,0.0004443591892495973
17718,36655,0,36655,112.51942491531372,0.0004409497955571983
17818,36855,0,36855,113.1193459033966,0.00043757055722700626
17918,37055,0,37055,113.72715997695923,0.0004342176166511042
18018,37255,0,37255,114.32560300827026,0.0004308949137895955
18118,37455,0,37455,114.93120408058167,0.00042760332710377433
18218,37655,0,37655,115.53678894042969,0.00042434238597930545
18318,37855,0,37855,116.15500116348267,0.00042111320081761756
18418,38055,0,38055,116.75652003288269,0.00041791849634199103
18519,38257,0,38257,117.36364793777466,0.0004147187089950228
18619,38457,0,38457,117.97554397583008,0.00041158695939104884
18719,38657,0,38657,118.5896828174591,0.00040848647394878436
18819,38857,0,38857,119.19590187072754,0.0004054158580496927
18919,39057,0,39057,119.81007409095764,0.00040237907853972726
19019,39257,0,39257,120.41503691673279,0.0003993730556905505
19119,39457,0,39457,121.01978802680969,0.00039639367435427065
19219,39657,0,39657,121.63254976272583,0.0003934434677054196
19319,39857,0,39857,122.25486993789673,0.000390520311579414
19419,40057,0,40057,123.06004595756531,0.0003876191080762832
19520,40259,0,40259,124.00348687171936,0.00038471360769292426
19620,40459,0,40459,125.04608678817749,0.00038185600423155724
19720,40659,0,40659,125.7197630405426,0.0003790185753043543
19820,40859,0,40859,126.36906003952026,0.0003761996412252371
19920,41059,0,41059,127.01756119728088,0.00037339614998068137
20020,41259,0,41259,127.63852381706238,0.0003706095186496348
20120,41459,0,41459,128.44525694847107,0.00036783803027635596
20220,41659,0,41659,129.08334493637085,0.0003650780506977404
20320,41859,0,41859,129.73592400550842,0.00036233235838273846
20420,42059,0,42059,130.82493495941162,0.0003595999505905372
20521,42261,0,42261,131.6005699634552,0.00035684891179602193
20621,42461,0,42461,132.5287380218506,0.00035413872752315277
20721,42661,0,42661,133.20463490486145,0.0003514401796663164
20821,42861,0,42861,133.88311386108398,0.0003487530584537215
20921,43061,0,43061,134.52379488945007,0.000346081288205072
21021,43261,0,43261,135.18935203552246,0.00034342336890239445
21121,43461,0,43461,135.89525699615479,0.00034077988080391633
21221,43661,0,43661,136.65432691574097,0.0003381552792047508
21321,43861,0,43861,137.36546206474304,0.0003355467871620267
21421,44061,0,44061,138.07551217079163,0.0003329575301029765
21522,44263,0,44263,138.70357704162598,0.0003303631338765218
21622,44463,0,44463,139.35773015022278,0.00032781345143755296
21722,44663,0,44663,139.9798698425293,0.00032528533403602115
21822,44863,0,44863,140.7370171546936,0.0003227793365833121
21922,45063,0,45063,141.43171310424805,0.0003202933986150201
22022,45263,0,45263,142.08801198005676,0.000317831510223095
22122,45463,0,45463,142.7682821750641,0.00031539237131079754
22222,45663,0,45663,143.39924502372742,0.0003129730274493356
22322,45863,0,45863,144.02545309066772,0.00031057877397405227
22422,46063,0,46063,144.72197794914246,0.0003082062989425342
22523,46265,0,46265,145.39064407348633,0.0003058305658265321
22623,46465,0,46465,146.12807703018188,0.0003035012625069254
22723,46665,0,46665,146.7635350227356,0.0003011931708341892
22823,46865,0,46865,147.68794298171997,0.00029890485815325295
22923,47065,0,47065,148.56560683250427,0.0002966392754110865
23023,47265,0,47265,149.20667695999146,0.00029439297729068104
23123,47465,0,47465,149.8996069431305,0.0002921666178834573
23223,47665,0,47665,150.5553379058838,0.0002899609204899502
23323,47865,0,47865,151.18448686599731,0.00028777152786029403
23423,48065,0,48065,151.7739119529724,0.00028560086598337047
23524,48267,0,48267,152.3808250427246,0.000283425415367278
23624,48467,0,48467,152.98989009857178,0.000281285343596098
23724,48667,0,48667,153.58051991462708,0.0002791592651166682
23824,48867,0,48867,154.1827688217163,0.0002770474455131497
23924,49067,0,49067,154.76696491241455,0.0002749457655943594
24024,49267,0,49267,155.35586786270142,0.00027285720725492697
24124,49467,0,49467,155.94023084640503,0.0002707794414598029
24224,49667,0,49667,156.54836511611938,0.0002687110015026959
24324,49867,0,49867,157.17590594291687,0.0002666549878073356
24424,50067,0,50067,157.80360388755798,0.0002646084946306814
24525,50269,0,50269,158.4638729095459,0.00026255316257905217
24625,50469,0,50469,159.09524393081665,0.00026052936999974456
24725,50669,0,50669,159.7210569381714,0.0002585174985078759
24825,50869,0,50869,160.3486888408661,0.0002565168249625047
24925,51069,0,51069,160.9927899837494,0.0002545306146038231
25025,51269,0,51269,161.66569900512695,0.00025255617540901286
25125,51469,0,51469,162.28719091415405,0.0002505970022365586
25225,51669,0,51669,162.91463804244995,0.0002486523651083687
25325,51869,0,51869,163.51620507240295,0.0002467210610026379
25425,52069,0,52069,164.22326493263245,0.00024480671153083547
25526,52271,0,52271,164.84002995491028,0.0002428889403873808
25626,52471,0,52471,165.44886994361877,0.00024100508276690637
25726,52671,0,52671,166.03661704063416,0.00023913762345952072
25826,52871,0,52871,166.62563395500183,0.00023728854733783952
25926,53071,0,53071,167.22940492630005,0.0002354548191160929
26026,53271,0,53271,167.8174810409546,0.00023364082907492137
26126,53471,0,53471,168.407870054245,0.00023184394983657023
26226,53671,0,53671,169.0115568637848,0.00023006583114829995
26326,53871,0,53871,169.62092685699463,0.00022830774893845568
26426,54071,0,54071,170.21799397468567,0.0002265672500330913
26527,54273,0,54273,170.82471919059753,0.00022483005704650977
26627,54473,0,54473,171.44301295280457,0.0002231283912994526
26727,54673,0,54673,172.0834128856659,0.0002214447442247862
26827,54873,0,54873,172.78787899017334,0.00021977843527910056
26927,55073,0,55073,173.40511107444763,0.0002181304824832683
27027,55273,0,55273,174.017569065094,0.0002164967824813005
27127,55473,0,55473,174.62448596954346,0.00021488007347808178
27227,55673,0,55673,175.2231800556183,0.00021327745909552535
27327,55873,0,55873,175.83118319511414,0.00021168733259085756
27427,56073,0,56073,176.430006980896,0.00021011134181499002
27528,56275,0,56275,177.13954091072083,0.00020853148852802478
27628,56475,0,56475,177.8225531578064,0.00020697657033605182
27728,56675,0,56675,178.44165992736816,0.00020543276352366958
27828,56875,0,56875,179.04805397987366,0.00020389906726857066
27928,57075,0,57075,179.6666579246521,0.00020237301150427867
28028,57275,0,57275,180.32892894744873,0.00020085728865357745
28128,57475,0,57475,180.98265194892883,0.00019934892810812715
28228,57675,0,57675,181.78625893592834,0.0001978494083934189
28328,57875,0,57875,182.4686357975006,0.00019635774952518771
28428,58075,0,58075,183.16277885437012,0.00019487328990784112
28529,58277,0,58277,183.69937586784363,0.00019338311135536077
28629,58477,0,58477,184.4154748916626,0.00019191532079112776
28729,58677,0,58677,185.1088740825653,0.00019045551933789047
28829,58877,0,58877,185.76232290267944,0.00018900433314244754
28929,59077,0,59077,186.46609687805176,0.00018756345769059362
29029,59277,0,59277,187.20150804519653,0.00018613002286098547
29129,59477,0,59477,187.8998510837555,0.00018470874899264813
29229,59677,0,59677,188.77955985069275,0.00018329699709438766
29329,59877,0,59877,189.4547038078308,0.00018189626234066733
29429,60077,0,60077,190.1146490573883,0.0001805079591626119
29530,60279,0,60279,190.98282194137573,0.00017911792327088473
29630,60479,0,60479,191.62425088882446,0.00017775347981368876
29730,60679,0,60679,192.2395088672638,0.0001764021671225788
29830,60879,0,60879,193.16676497459412,0.00017506414447812418
29930,61079,0,61079,193.83730506896973,0.00017373841390050366
30030,61279,0,61279,194.43358898162842,0.0001724277115588337
30130,61479,0,61479,195.04026198387146,0.000171128725403631
30230,61679,0,61679,195.9217610359192,0.0001698440874122675
30330,61879,0,61879,196.54260778427124,0.000168572193476397
30430,62079,0,62079,197.39280009269714,0.0001673121741196704
30531,62281,0,62281,198.16310501098633,0.0001660523094134607
30631,62481,0,62481,198.8099970817566,0.0001648160222200106
30731,62681,0,62681,199.5168640613556,0.00016358943784135465
30831,62881,0,62881,200.25389003753662,0.00016237289954352757
30931,63081,0,63081,201.07305097579956,0.00016116625916700667
31031,63281,0,63281,201.73207998275757,0.00015996645778294533
31131,63481,0,63481,202.53593707084656,0.00015877595923150073
31231,63681,0,63681,203.30050611495972,0.00015759139816969936
31331,63881,0,63881,204.01559400558472,0.0001564142936334903
31431,64081,0,64081,204.6910331249237,0.0001552431025456382
31532,64283,0,64283,205.38644194602966,0.00015406606266292033
31632,64483,0,64483,206.16119813919067,0.00015290577696838527
31732,64683,0,64683,206.8336479663849,0.00015175066717090682
31832,64883,0,64883,207.48850893974304,0.0001506006285510276
31932,65083,0,65083,208.1568660736084,0.00014945552988276822
32032,65283,0,65283,208.81217408180237,0.00014831700517161893
32132,65483,0,65483,209.48066782951355,0.00014718225070919924
32232,65683,0,65683,210.13635087013245,0.00014605507968210675
32332,65883,0,65883,211.01289010047913,0.00014493339219364977
32432,66083,0,66083,212.05531120300293,0.0001438178336584473
32533,66285,0,66285,212.81058502197266,0.00014269831289686962
32633,66485,0,66485,213.45252513885498,0.0001415968044264991
32733,66685,0,66685,214.10069704055786,0.0001405012898246268
32833,66885,0,66885,214.7384729385376,0.00013941327057696726
32933,67085,0,67085,215.3522801399231,0.00013833313920478258
33033,67285,0,67285,216.0153510570526,0.00013725971375036042
33133,67485,0,67485,216.64478588104248,0.00013619581661395767
33233,67685,0,67685,217.26382207870483,0.00013513927122535697
33333,67885,0,67885,217.90499210357666,0.00013409201003752486
33433,68085,0,68085,218.5293607711792,0.00013305408727889813
33534,68287,0,68287,219.17728400230408,0.0001320157740428634
33634,68487,0,68487,219.82823181152344,0.00013099710551960124
33734,68687,0,68687,220.4589581489563,0.00012998883125896088
33834,68887,0,68887,221.08950805664062,0.00012899001029243267
33934,69087,0,69087,221.70202708244324,0.00012800127891324502
34034,69287,0,69287,222.319561958313,0.0001270232414831008
34134,69487,0,69487,222.96285009384155,0.00012605360841796571
34234,69687,0,69687,223.58916878700256,0.00012509486854965992
34334,69887,0,69887,224.19584107398987,0.00012414464919178382
34434,70087,0,70087,224.82733297348022,0.00012320314742889858
34535,70289,0,70289,225.46966886520386,0.00012226112923271603
34635,70489,0,70489,226.1762239933014,0.00012133680648015636
34735,70689,0,70689,226.83656287193298,0.00012041901537431509
34835,70889,0,70889,227.51425004005432,0.00011950850479196048
34935,71089,0,71089,228.1524360179901,0.00011860512871200248
35035,71289,0,71289,228.91786694526672,0.00011770768612362751
35135,71489,0,71489,229.5420789718628,0.00011681771815507912
35235,71689,0,71689,230.23105096817017,0.00011593301479817612
35335,71889,0,71889,231.04729080200195,0.00011505544979761924
35435,72089,0,72089,231.74563097953796,0.00011418384359810981
35536,72291,0,72291,232.54534602165222,0.0001133095489306335
35636,72491,0,72491,233.21299290657043,0.00011244948311060167
35736,72691,0,72691,233.90584087371826,0.00011159541376238941
35836,72891,0,72891,234.55936694145203,0.0001107461648523344
35936,73091,0,73091,235.1596920490265,0.00010990178311003876
36036,73291,0,73291,235.84373879432678,0.0001090631414045197
36136,73491,0,73491,236.52281188964844,0.00010822854079998133
36236,73691,0,73691,237.12053084373474,0.00010739963142051337
36336,73891,0,73891,237.74765801429749,0.00010657504426321588
36436,74091,0,74091,238.374449968338,0.00010575581804849181
36537,74293,0,74293,238.96523809432983,0.00010493379840527903
36637,74493,0,74493,239.59968495368958,0.00010412550051366789
36737,74693,0,74693,240.2002251148224,0.00010332243979409745
36837,74893,0,74893,240.80988788604736,0.00010252545337754673
36937,75093,0,75093,241.39804697036743,0.00010173432290030916
37037,75293,0,75293,242.01562809944153,0.0001009493166840781
37137,75493,0,75493,242.61565494537354,0.00010017200392660194
37237,75693,0,75693,243.22374606132507,9.940053450249466e-05
37337,75893,0,75893,243.85982012748718,9.863714322880651e-05
37437,76093,0,76093,244.49518489837646,9.788101101211603e-05
37538,76295,0,76295,245.11855578422546,9.712488764820541e-05
37638,76495,0,76495,245.7154791355133,9.638388637943132e-05
37738,76695,0,76695,246.32887601852417,9.565107724430238e-05
37838,76895,0,76895,246.92242574691772,9.492526967449331e-05
37938,77095,0,77095,247.50263285636902,9.420701735260339e-05
38038,77295,0,77295,248.08391284942627,9.349657348637701e-05
38138,77495,0,77495,248.67868208885193,9.27929926563787e-05
38238,77695,0,77695,249.25940895080566,9.209739344045966e-05
38338,77895,0,77895,249.88612699508667,9.140795839302996e-05
38438,78095,0,78095,250.56012296676636,9.072596785544364e-05
38539,78297,0,78297,251.21732711791992,9.004364332352874e-05
38639,78497,0,78497,251.81299996376038,8.937434065194356e-05
38739,78697,0,78697,252.43141198158264,8.871057595504296e-05
38839,78897,0,78897,253.07039999961853,8.805266715968323e-05
38939,79097,0,79097,253.6945059299469,8.739938172311207e-05
39039,79297,0,79297,254.31948900222778,8.675059852876052e-05
39139,79497,0,79497,254.92196106910706,8.610691571864104e-05
39239,79697,0,79697,255.5321409702301,8.546657782203729e-05
39339,79897,0,79897,256.195280790329,8.483061418949398e-05
39439,80097,0,80097,256.8293960094452,8.419787432410362e-05
39540,80299,0,80299,257.47469997406006,8.356234376145117e-05
39640,80499,0,80499,258.125501871109,8.293637639645695e-05
39740,80699,0,80699,258.8050570487976,8.231374234293663e-05
39840,80899,0,80899,259.4195258617401,8.169351300950722e-05
39940,81099,0,81099,260.04206705093384,8.107650554352536e-05
40040,81299,0,81299,260.66415309906006,8.046241694219585e-05
40140,81499,0,81499,261.2646269798279,7.98510604664737e-05
40240,81699,0,81699,261.9257950782776,7.924378465520752e-05
40340,81899,0,81899,262.5607581138611,7.863918892009517e-05
40440,82099,0,82099,263.1705138683319,7.803881410523735e-05
40541,82301,0,82301,263.7903528213501,7.743649762678876e-05
40641,82501,0,82501,264.40058279037476,7.68442771565698e-05
40741,82701,0,82701,264.99062395095825,7.625654710508454e-05
40841,82901,0,82901,265.61910700798035,7.56739784998458e-05
40941,83101,0,83101,266.2294268608093,7.509581080976655e-05
41041,83301,0,83301,266.8148009777069,7.452269962300603e-05
41141,83501,0,83501,267.4017128944397,7.395508657068421e-05
41241,83701,0,83701,268.0309760570526,7.339225578271027e-05
41341,83901,0,83901,268.67869997024536,7.283539553671882e-05
41441,84101,0,84101,269.3540539741516,7.228343188734343e-05
41542,84303,0,84303,269.99715209007263,7.173144985901524e-05
41642,84503,0,84503,270.59252095222473,7.119026673264571e-05
41742,84703,0,84703,271.19855213165283,7.065427020085051e-05
41842,84903,0,84903,271.79841685295105,7.012284916203294e-05
41942,85103,0,85103,272.4300081729889,6.95964589360568e-05
42042,85303,0,85303,273.0467550754547,6.907440714732261e-05
42142,85503,0,85503,273.6844160556793,6.855638698617058e-05
42242,85703,0,85703,274.32533288002014,6.80431143177364e-05
42342,85903,0,85903,274.9689657688141,6.753313055557815e-05
42442,86103,0,86103,275.6555781364441,6.70273378896746e-05
42543,86305,0,86305,276.33174085617065,6.652000189465398e-05
42643,86505,0,86505,276.98042702674866,6.602093227357179e-05
42743,86705,0,86705,277.6614999771118,6.552520530361839e-05
42843,86905,0,86905,278.33678579330444,6.503285457849874e-05
42943,87105,0,87105,278.96060013771057,6.454311424559498e-05
43043,87305,0,87305,279.57845306396484,6.405622852978978e-05
43143,87505,0,87505,280.1980059146881,6.357231000006421e-05
43243,87705,0,87705,280.81048488616943,6.30905376468477e-05
43343,87905,0,87905,281.42666387557983,6.261183045847129e-05
43443,88105,0,88105,282.06085777282715,6.213498541749344e-05
43544,88307,0,88307,282.6765968799591,6.165612881598858e-05
43644,88507,0,88507,283.3594660758972,6.118418804801787e-05
43744,88707,0,88707,283.9830777645111,6.071441210752756e-05
43844,88907,0,88907,284.6134331226349,6.0246894393600237e-05
43944,89107,0,89107,285.24489402770996,5.978196655349359e-05
44044,89307,0,89307,285.87508511543274,5.931910077149472e-05
44144,89507,0,89507,286.51080298423767,5.885893744758608e-05
44244,89707,0,89707,287.1990110874176,5.8402172021352594e-05
44344,89907,0,89907,287.83762407302856,5.794768852772707e-05
44444,90107,0,90107,288.53836584091187,5.749721344987527e-05
44545,90309,0,90309,289.262423992157,5.7045629493327914e-05
44645,90509,0,90509,289.8851897716522,5.660194787177847e-05
44745,90709,0,90709,290.50241208076477,5.616229602226952e-05
44845,90909,0,90909,291.0987560749054,5.572664853885232e-05
44945,91109,0,91109,291.7102429866791,5.529468902648988e-05
45045,91309,0,91309,292.3205590248108,5.4866811065071414e-05
45145,91509,0,91509,292.9358232021332,5.4443009773984783e-05
45245,91709,0,91709,293.55915904045105,5.4022748027274466e-05
45345,91909,0,91909,294.15739011764526,5.360716837731729e-05
45445,92109,0,92109,294.79322600364685,5.319489721805407e-05
45546,92311,0,92311,295.43519592285156,5.278286028414498e-05
45646,92511,0,92511,296.0567879676819,5.2379017355885644e-05
45746,92711,0,92711,296.6551458835602,5.197894037279224e-05
45846,92911,0,92911,297.2536828517914,5.1582810622158925e-05
45946,93111,0,93111,297.8995678424835,5.11908045861562e-05
46046,93311,0,93311,298.51045989990234,5.080248123445317e-05
46146,93511,0,93511,299.10808801651,5.0417963484566186e-05
46246,93711,0,93711,299.7077341079712,5.00375611458384e-05
46346,93911,0,93911,300.32214307785034,4.9660322960779094e-05
46446,94111,0,94111,300.92493891716003,4.928711397785531e-05
46547,94313,0,94313,301.5496509075165,4.891326095647499e-05
46647,94513,0,94513,302.1861639022827,4.854621146598419e-05
46747,94713,0,94713,302.86983919143677,4.8182061776829455e-05
46847,94913,0,94913,303.47004103660583,4.782059564788464e-05
46947,95113,0,95113,304.0695197582245,4.746137469564154e-05
47047,95313,0,95313,304.69054889678955,4.7104603874885286e-05
47147,95513,0,95513,305.32476592063904,4.674986780861241e-05
47247,95713,0,95713,305.9562039375305,4.6396996463405836e-05
47347,95913,0,95913,306.5839729309082,4.604667994954013e-05
47447,96113,0,96113,307.2306728363037,4.569773493930747e-05
47548,96315,0,96315,307.89585518836975,4.5347664953674166e-05
47648,96515,0,96515,308.5352210998535,4.5003088292862485e-05
47748,96715,0,96715,309.1831338405609,4.466034906287146e-05
47848,96915,0,96915,309.99512100219727,4.4319712501454125e-05
47948,97115,0,97115,310.65628600120544,4.398129134801827e-05
48048,97315,0,97315,311.27326583862305,4.364476471695583e-05
48148,97515,0,97515,311.8998010158539,4.331041428687018e-05
48248,97715,0,97715,312.5549690723419,4.297856902932587e-05
48348,97915,0,97915,313.21011090278625,4.264866143459578e-05
48448,98115,0,98115,313.82904505729675,4.232188980734421e-05
48549,98317,0,98317,314.4438910484314,4.199404269397213e-05
48649,98517,0,98517,315.0822739601135,4.167231678516772e-05
48749,98717,0,98717,315.7777590751648,4.135353619686628e-05
48849,98917,0,98917,316.4194600582123,4.103765035766239e-05
48949,99117,0,99117,317.07096695899963,4.072460522226543e-05
49049,99317,0,99317,317.8059220314026,4.041472521671458e-05
49149,99517,0,99517,318.4816040992737,4.010799105812023e-05
49249,99717,0,99717,319.095666885376,3.980424415389728e-05
49349,99917,0,99917,319.7405378818512,3.950404639026843e-05
49449,100117,0,100117,320.3455801010132,3.920660413744864e-05
49550,100319,0,100319,320.94023394584656,3.890971781278493e-05
49650,100519,0,100519,321.54556488990784,3.8618810463466516e-05
49750,100719,0,100719,322.34872603416443,3.833077829905268e-05
49850,100919,0,100919,323.21276807785034,3.804564711144888e-05
49950,101119,0,101119,324.30821895599365,3.776331453170784e-05
50050,101319,0,101319,325.0324831008911,3.74833523510667e-05
50150,101519,0,101519,325.7647190093994,3.720584587137094e-05
50250,101719,0,101719,326.41942501068115,3.693062042191386e-05
50350,101919,0,101919,327.32740783691406,3.6657228163448914e-05
50450,102119,0,102119,328.15406799316406,3.638614125525189e-05
50551,102321,0,102321,328.7749660015106,3.611373987522251e-05
50651,102521,0,102521,329.3693277835846,3.5845807319357395e-05
50751,102721,0,102721,329.99326491355896,3.557933648513148e-05
50851,102921,0,102921,330.5853319168091,3.531413109097836e-05
50951,103121,0,103121,331.17602801322937,3.5050145076216006e-05
51051,103321,0,103321,331.76759099960327,3.478745295010657e-05
51151,103521,0,103521,332.3749289512634,3.452575653460189e-05
51251,103721,0,103721,332.983766078949,3.4265168029987166e-05
51351,103921,0,103921,333.6047978401184,3.40060196903115e-05
51451,104121,0,104121,334.2046089172363,3.374763791811429e-05
51552,104323,0,104323,335.0697548389435,3.348840966315586e-05
51652,104523,0,104523,335.6807837486267,3.323298358861103e-05
51752,104723,0,104723,336.28847885131836,3.297895696371409e-05
51852,104923,0,104923,336.89856576919556,3.2726515890778106e-05
51952,105123,0,105123,337.4913430213928,3.2475800655501076e-05
52052,105323,0,105323,338.0805058479309,3.2226532196011374e-05
52152,105523,0,105523,338.67868280410767,3.197916099323629e-05
52252,105723,0,105723,339.2710859775543,3.1733638745644914e-05
52352,105923,0,105923,339.8845360279083,3.148976793595069e-05
52452,106123,0,106123,340.49234890937805,3.1248287381188036e-05
52553,106325,0,106325,341.12679386138916,3.100603446358872e-05
52653,106525,0,106525,341.7794859409332,3.076850288402706e-05
52753,106725,0,106725,342.4600830078125,3.053310549363389e-05
52853,106925,0,106925,343.1286928653717,3.0299879882048615e-05
52953,107125,0,107125,343.75484013557434,3.006870365520377e-05
53053,107325,0,107325,344.3911271095276,2.9839857335849676e-05
53153,107525,0,107525,345.0135941505432,2.96130264010156e-05
53253,107725,0,107725,345.67022705078125,2.9388338746368155e-05
53353,107925,0,107925,346.2984688282013,2.9165943396633036e-05
53453,108125,0,108125,347.0047130584717,2.894542443994101e-05
53554,108327,0,108327,347.67646312713623,2.872511028379031e-05
53654,108527,0,108527,348.3052759170532,2.8508766216073827e-05
53754,108727,0,108727,349.03134989738464,2.829443008010574e-05
53854,108927,0,108927,349.7788710594177,2.808189275915651e-05
53954,109127,0,109127,350.5026822090149,2.7871104825364495e-05
54054,109327,0,109327,351.2570948600769,2.766174664941889e-05
54154,109527,0,109527,351.94405794143677,2.7453971265987298e-05
54254,109727,0,109727,352.67224407196045,2.7247401868772074e-05
54354,109927,0,109927,353.3786470890045,2.7041950610316864e-05
54454,110127,0,110127,354.1697189807892,2.6837934531089925e-05
54555,110329,0,110329,354.8905348777771,2.663257074141629e-05
54655,110529,0,110529,355.7283329963684,2.6430587780569974e-05
54755,110729,0,110729,356.44058299064636,2.6229535317192693e-05
54855,110929,0,110929,357.15073680877686,2.6029552013235097e-05
54955,111129,0,111129,357.88414216041565,2.5830518181817362e-05
55055,111329,0,111329,358.59960985183716,2.5632764911201122e-05
55155,111529,0,111529,359.30150294303894,2.5435883324491686e-05
55255,111729,0,111729,359.9685220718384,2.524017673636083e-05
55355,111929,0,111929,360.7099299430847,2.5045689120942454e-05
55455,112129,0,112129,361.39246582984924,2.4852206539384386e-05
55556,112331,0,112331,362.1593589782715,2.465826036784896e-05
55656,112531,0,112531,362.8707129955292,2.446730537766309e-05
55756,112731,0,112731,363.4994339942932,2.4277777723184916e-05
55856,112931,0,112931,364.1788420677185,2.4089521978280944e-05
55956,113131,0,113131,364.8579430580139,2.3902691575340915e-05
56056,113331,0,113331,365.48497104644775,2.371708484704446e-05
56156,113531,0,113531,366.1555299758911,2.3533050676478333e-05
56256,113731,0,113731,366.83223700523376,2.3350381624040462e-05
56356,113931,0,113931,367.4798810482025,2.3169202588273757e-05
56456,114131,0,114131,368.22042083740234,2.2989720401696376e-05
56557,114333,0,114333,368.92000579833984,2.2809910362262673e-05
56657,114533,0,114533,369.6110751628876,2.263383417133118e-05
56757,114733,0,114733,370.26581597328186,2.2459352328843787e-05
56857,114933,0,114933,370.9637858867645,2.2286755196490683e-05
56957,115133,0,115133,371.5862760543823,2.2115940830902616e-05
57057,115333,0,115333,372.16930413246155,2.1947049590799025e-05
57157,115533,0,115533,372.76252007484436,2.177979208049645e-05
57257,115733,0,115733,373.36372780799866,2.1614417351885568e-05
57357,115933,0,115933,373.9700779914856,2.145071925963538e-05
57457,116133,0,116133,374.5914099216461,2.128859423325382e-05
57558,116335,0,116335,375.20637488365173,2.112667422998877e-05
57658,116535,0,116535,375.85319805145264,2.0967699516192574e-05
57758,116735,0,116735,376.52798891067505,2.0810408758386963e-05
57858,116935,0,116935,377.1757791042328,2.065448158127986e-05
57958,117135,0,117135,377.8636348247528,2.049993181781727e-05
58058,117335,0,117335,378.57864594459534,2.0346614991395484e-05
58158,117535,0,117535,379.2965569496155,2.0194704858145192e-05
58258,117735,0,117735,379.95403504371643,2.0043783640262423e-05
58358,117935,0,117935,380.6011619567871,1.9894032141978684e-05
58458,118135,0,118135,381.24692392349243,1.97454291394858e-05
58559,118337,0,118337,381.8853528499603,1.9596158221805785e-05
58659,118537,0,118537,382.5211970806122,1.9449516101442805e-05
58759,118737,0,118737,383.27076411247253,1.9303652319141874e-05
58859,118937,0,118937,383.9805829524994,1.915872212089755e-05
58959,119137,0,119137,384.7412528991699,1.9014558244743635e-05
59059,119337,0,119337,385.4037010669708,1.887126195748468e-05
59159,119537,0,119537,386.03964400291443,1.872860522796255e-05
59259,119737,0,119737,386.69029784202576,1.8586901452993914e-05
59359,119937,0,119937,387.32730197906494,1.844584041925176e-05
59459,120137,0,120137,387.9417657852173,1.830559611170457e-05
59560,120339,0,120339,388.69621205329895,1.816488629364249e-05
59660,120539,0,120539,389.3617830276489,1.8026267040952264e-05
59760,120739,0,120739,390.0135669708252,1.7888733357865932e-05
59860,120939,0,120939,390.7386939525604,1.775211442151869e-05
59960,121139,0,121139,391.394238948822,1.761658564471472e-05
60060,121339,0,121339,392.0378839969635,1.748204897797837e-05
60160,121539,0,121539,392.74437403678894,1.7348803819419792e-05
60260,121739,0,121739,393.43798875808716,1.7216544850927023e-05
60360,121939,0,121939,394.1121201515198,1.708563634181421e-05
60460,122139,0,122139,394.86521792411804,1.6955945053165952e-05
60561,122341,0,122341,395.5207929611206,1.6826160028791547e-05
60661,122541,0,122541,396.1546711921692,1.669910615911218e-05
60761,122741,0,122741,396.7959179878235,1.6573212706128094e-05
60861,122941,0,122941,397.4983940124512,1.6448708926825412e-05
60961,123141,0,123141,398.19069480895996,1.632541848389529e-05
61061,123341,0,123341,398.87851119041443,1.6203436570302123e-05
61161,123541,0,123541,399.4818859100342,1.6082518029769993e-05
61261,123741,0,123741,400.10635900497437,1.5962891772901577e-05
61361,123941,0,123941,400.8191831111908,1.5844194950537758e-05
61461,124141,0,124141,401.4544150829315,1.5726544734975448e-05
61562,124343,0,124343,402.094398021698,1.5608769900655392e-05
61662,124543,0,124543,402.78393602371216,1.5492878980594764e-05
61762,124743,0,124743,403.46703696250916,1.5377941291400723e-05
61862,124943,0,124943,404.11604404449463,1.5263701389698473e-05
61962,125143,0,125143,404.74460101127625,1.5150199649539458e-05
62062,125343,0,125343,405.46997594833374,1.5037328438538426e-05
62162,125543,0,125543,406.1849138736725,1.4925154827623717e-05
62262,125743,0,125743,406.835618019104,1.4813441117636205e-05
62362,125943,0,125943,407.48988103866577,1.4702409965936642e-05
62462,126143,0,126143,408.08847093582153,1.4591840478928431e-05
62563,126345,0,126345,408.69754791259766,1.4480683365918852e-05
62663,126545,0,126545,409.3220510482788,1.437126738197788e-05
62763,126745,0,126745,409.9333429336548,1.4262276009837356e-05
62863,126945,0,126945,410.53281903266907,1.4153877784041205e-05
62963,127145,0,127145,411.1538031101227,1.4046001156033034e-05
63063,127345,0,127345,411.765949010849,1.3938722739015937e-05
63163,127545,0,127545,412.37078499794006,1.383191018574915e-05
63263,127745,0,127745,412.9565329551697,1.3725779572735748e-05
63363,127945,0,127945,413.54607486724854,1.3620141684758081e-05
63463,128145,0,128145,414.1534368991852,1.3515190282173448e-05
63564,128347,0,128347,414.7744948863983,1.3409850173584944e-05
63664,128547,0,128547,415.39181113243103,1.3306187645815762e-05
63764,128747,0,128747,416.02448987960815,1.3203371994691153e-05
63864,128947,0,128947,416.64029908180237,1.3101283465909305e-05
63964,129147,0,129147,417.2598338127136,1.3000090630357126e-05
64064,129347,0,129347,417.86910581588745,1.2899767113116023e-05
64164,129547,0,129547,418.47745513916016,1.2800416166629442e-05
64264,129747,0,129747,419.0674910545349,1.270190393674691e-05
64364,129947,0,129947,419.6441309452057,1.2604462067721216e-05
64464,130147,0,130147,420.24226999282837,1.2507878208588994e-05
64565,130349,0,130349,420.84535694122314,1.2411269890918923e-05
64665,130549,0,130549,421.42707991600037,1.2316659628862083e-05
64765,130749,0,130749,422.024973154068,1.2222819263759922e-05
64865,130949,0,130949,422.65682888031006,1.2129922600918836e-05
64965,131149,0,131149,423.28590989112854,1.2037853611787515e-05
65065,131349,0,131349,423.9060218334198,1.1946580965315364e-05
65165,131549,0,131549,424.5155670642853,1.1856065136206761e-05
65265,131749,0,131749,425.11040210723877,1.1766353708199098e-05
65365,131949,0,131949,425.72669291496277,1.167724871246685e-05
65465,132149,0,132149,426.32280802726746,1.1588947343439148e-05
65566,132351,0,132351,426.9393699169159,1.1500438385053332e-05
65666,132551,0,132551,427.55221819877625,1.1413423254379055e-05
65766,132751,0,132751,428.14381289482117,1.1327170441942158e-05
65866,132951,0,132951,428.74916100502014,1.1241518259173395e-05
65966,133151,0,133151,429.34031319618225,1.1156506329348e-05
66066,133351,0,133351,429.9369249343872,1.1072097398836292e-05
66166,133551,0,133551,430.5435938835144,1.0988308526350402e-05
66266,133751,0,133751,431.25048184394836,1.0904986088647595e-05
66366,133951,0,133951,432.14616084098816,1.0822277263820602e-05
66466,134151,0,134151,432.98023080825806,1.0739992642320685e-05
66567,134353,0,134353,433.89529180526733,1.0657363612103514e-05
66667,134553,0,134553,434.7601239681244,1.0576102336443649e-05
66767,134753,0,134753,435.61061787605286,1.0495182742941092e-05
66867,134953,0,134953,436.48784494400024,1.0414793228570489e-05
66967,135153,0,135153,437.2382950782776,1.033483385346973e-05
67067,135353,0,135353,438.016685962677,1.0255339052786068e-05
67167,135553,0,135553,438.812735080719,1.0176337895995188e-05
67267,135753,0,135753,439.623899936676,1.0097875100640438e-05
67367,135953,0,135953,440.42767214775085,1.0019865868934044e-05
67467,136153,0,136153,441.2257149219513,9.942464363251308e-06
67568,136355,0,136355,442.0674271583557,9.864838208106528e-06
67668,136555,0,136555,442.8186628818512,9.788552321385637e-06
67768,136755,0,136755,443.45524311065674,9.71298748709938e-06
67868,136955,0,136955,444.15042209625244,9.637984877770238e-06
67968,137155,0,137155,444.8312158584595,9.563667522618277e-06
68068,137355,0,137355,445.4767370223999,9.490071452886143e-06
68168,137555,0,137555,446.1261591911316,9.417143965723027e-06
68268,137755,0,137755,446.8735947608948,9.344881027881366e-06
68368,137955,0,137955,447.5651981830597,9.273424073879207e-06
68468,138155,0,138155,448.29535007476807,9.202581376413858e-06
68569,138357,0,138357,448.9791600704193,9.131791870563843e-06
68669,138557,0,138557,449.65449810028076,9.062507289409087e-06
68769,138757,0,138757,450.3195080757141,8.99387642718576e-06
68869,138957,0,138957,451.04637908935547,8.926021546686734e-06
68969,139157,0,139157,451.65922498703003,8.858878998736708e-06
69069,139357,0,139357,452.3623070716858,8.792442734339651e-06
69169,139557,0,139557,453.01997208595276,8.726668729635766e-06
69269,139757,0,139757,453.6280961036682,8.661604176695646e-06
69369,139957,0,139957,454.29483699798584,8.597111507336238e-06
69469,140157,0,140157,454.9539740085602,8.533243973006507e-06
69570,140359,0,140359,455.69319200515747,8.46926274520164e-06
69670,140559,0,140559,456.34978795051575,8.4064320740932e-06
69770,140759,0,140759,457.05005288124084,8.34413592844067e-06
69870,140959,0,140959,457.71186685562134,8.282209224020744e-06
69970,141159,0,141159,458.3615128993988,8.220716244237576e-06
70070,141359,0,141359,459.0150001049042,8.15960579700872e-06
70170,141559,0,141559,459.7156238555908,8.09882843162136e-06
70270,141759,0,141759,460.3523588180542,8.038352925438101e-06
70370,141959,0,141959,461.07253408432007,7.978231898212134e-06
70470,142159,0,142159,461.7345688343048,7.918350513493208e-06
70571,142361,0,142361,462.36542105674744,7.85816125301329e-06
70671,142561,0,142561,462.99021792411804,7.798913813381822e-06
70771,142761,0,142761,463.58568596839905,7.739923909181886e-06
70871,142961,0,142961,464.1959738731384,7.681304821705222e-06
70971,143161,0,143161,464.78199100494385,7.622960271769597e-06
71071,143361,0,143361,465.41716980934143,7.564964713800656e-06
71171,143561,0,143561,466.07135701179504,7.507363479542707e-06
71271,143761,0,143761,466.72151613235474,7.450142415256025e-06
71371,143961,0,143961,467.3684720993042,7.393285777399734e-06
71471,144161,0,144161,467.9876379966736,7.336921548769119e-06
71572,144363,0,144363,468.75275015830994,7.280381105019782e-06
71672,144563,0,144563,469.4639639854431,7.224857186431219e-06
71772,144763,0,144763,470.1030521392822,7.1698837072445935e-06
71872,144963,0,144963,470.8810999393463,7.115334130268065e-06
71972,145163,0,145163,471.53812289237976,7.06132749647829e-06
72072,145363,0,145363,472.2201430797577,7.007825944211396e-06
72172,145563,0,145563,472.8610529899597,6.954835793758115e-06
72272,145763,0,145763,473.5195698738098,6.902340738013492e-06
72372,145963,0,145963,474.2089421749115,6.850390865927634e-06
72472,146163,0,146163,474.8682041168213,6.798900524696962e-06
72573,146365,0,146365,475.5143837928772,6.74738038507656e-06
72673,146565,0,146565,476.1572799682617,6.69686324770728e-06
72773,146765,0,146765,476.83115100860596,6.646771911011553e-06
72873,146965,0,146965,477.6176450252533,6.59717745652697e-06
72973,147165,0,147165,478.25211811065674,6.547943306296499e-06
73073,147365,0,147365,478.98289585113525,6.499128352094346e-06
73173,147565,0,147565,479.6576318740845,6.450697382032735e-06
73273,147765,0,147765,480.2871301174164,6.402620827333474e-06
73373,147965,0,147965,480.88256192207336,6.354853803882367e-06
73473,148165,0,148165,481.577898979187,6.307454005809182e-06
73574,148367,0,148367,482.31625390052795,6.259831382669664e-06
73674,148567,0,148567,483.3391628265381,6.212946624938324e-06
73774,148767,0,148767,484.07390999794006,6.166366123968573e-06
73874,148967,0,148967,484.69056582450867,6.119968230353549e-06
73974,149167,0,149167,485.3141529560089,6.073843096076162e-06
74074,149367,0,149367,485.92646503448486,6.027884190548463e-06
74174,149567,0,149567,486.52882409095764,5.9821171241385404e-06
74274,149767,0,149767,487.1366078853607,5.936552718669297e-06
74374,149967,0,149967,487.72609305381775,5.891190427785493e-06
74474,150167,0,150167,488.3263759613037,5.845976198538585e-06
74575,150369,0,150369,488.9737629890442,5.800565718091956e-06
74675,150569,0,150569,489.57557702064514,5.7558369132181936e-06
74775,150769,0,150769,490.1651918888092,5.711324993775308e-06
74875,150969,0,150969,490.840900182724,5.667149355843167e-06
74975,151169,0,151169,491.4607789516449,5.623223486844825e-06
75075,151369,0,151369,492.05795884132385,5.579632484490381e-06
75175,151569,0,151569,492.65349102020264,5.536366216019064e-06
75275,151769,0,151769,493.2597119808197,5.493438410783094e-06
75375,151969,0,151969,493.8481459617615,5.450842567026544e-06
75475,152169,0,152169,494.43840193748474,5.408634446041755e-06
75576,152371,0,152371,495.0362501144409,5.366330496517034e-06
75676,152571,0,152571,495.6350929737091,5.324802466985541e-06
75776,152771,0,152771,496.2743270397186,5.28367961591007e-06
75876,152971,0,152971,496.9093029499054,5.242884052922791e-06
75976,153171,0,153171,497.5529668331146,5.2025006269278264e-06
76076,153371,0,153371,498.2955551147461,5.162474070247018e-06
76176,153571,0,153571,499.0639429092407,5.122827011812248e-06
76276,153771,0,153771,499.75546002388,5.083569693792328e-06
76376,153971,0,153971,500.3991689682007,5.044715217185312e-06
76476,154171,0,154171,501.2404658794403,5.006207089397427e-06
76577,154373,0,154373,501.93090415000916,4.967732215366245e-06
76677,154573,0,154573,502.7770380973816,4.9300297651013014e-06
76777,154773,0,154773,503.51630687713623,4.892667429254642e-06
76877,154973,0,154973,504.1841480731964,4.855714931500125e-06
76977,155173,0,155173,504.89077496528625,4.81908439921022e-06
77077,155373,0,155373,505.5897150039673,4.782801293762221e-06
77177,155573,0,155573,506.27947998046875,4.7468190984422e-06
77277,155773,0,155773,507.09723591804504,4.711136634652969e-06
77377,155973,0,155973,508.0875689983368,4.6757064895309695e-06
77477,156173,0,156173,508.8962061405182,4.640550846775455e-06
77578,156375,0,156375,509.8362228870392,4.605259714452819e-06
77678,156575,0,156575,510.79137897491455,4.570538505013441e-06
77778,156775,0,156775,511.4780170917511,4.536058643988779e-06
77878,156975,0,156975,512.1315879821777,4.50176351097292e-06
77978,157175,0,157175,512.7893800735474,4.467706645686447e-06
78078,157375,0,157375,513.5007028579712,4.433828506148469e-06
78178,157575,0,157575,514.1695308685303,4.400166848662369e-06
78278,157775,0,157775,515.1405999660492,4.36670054666082e-06
78378,157975,0,157975,516.1388289928436,4.333439773565808e-06
78478,158175,0,158175,516.914244890213,4.30035366528698e-06
78579,158377,0,158377,517.6172490119934,4.26717338839268e-06
78679,158577,0,158577,518.3363630771637,4.234506444369769e-06
78779,158777,0,158777,519.1833038330078,4.2020341075590146e-06
78879,158977,0,158977,519.8516170978546,4.169817229262236e-06
78979,159177,0,159177,520.5025520324707,4.137784507893257e-06
79079,159377,0,159377,521.1632080078125,4.106001278618e-06
79179,159577,0,159577,522.0002980232239,4.074449252982557e-06
79279,159777,0,159777,522.7276520729065,4.043145921149018e-06
79379,159977,0,159977,523.5685591697693,4.012080752675307e-06
79479,160177,0,160177,524.7420680522919,3.981317666105197e-06
79580,160379,0,160379,525.4439549446106,3.950496040725624e-06
79680,160579,0,160579,526.1651358604431,3.920276808071134e-06
79780,160779,0,160779,526.845675945282,3.890383427832657e-06
79880,160979,0,160979,527.5440559387207,3.8607737059271235e-06
79980,161179,0,161179,528.1611189842224,3.831512068940237e-06
80080,161379,0,161379,528.833398103714,3.8025453023885537e-06
80180,161579,0,161579,529.48384308815,3.7739078379104337e-06
80280,161779,0,161779,530.4195849895477,3.7455753286746114e-06
80380,161979,0,161979,531.1123919487,3.7175551393393335e-06
80480,162179,0,162179,531.7630319595337,3.68980297314952e-06
80581,162381,0,162381,532.4402461051941,3.662076834574067e-06
80681,162581,0,162581,533.0767920017242,3.6348709231321e-06
80781,162781,0,162781,533.6986210346222,3.607906757920782e-06
80881,162981,0,162981,534.315672159195,3.5811925187506002e-06
80981,163181,0,163181,534.914351940155,3.5546783979919598e-06
81081,163381,0,163381,535.5051209926605,3.5283876305968027e-06
81181,163581,0,163581,536.0958080291748,3.5022651556287515e-06
81281,163781,0,163781,536.7111728191376,3.476330539603092e-06
81381,163981,0,163981,537.3039548397064,3.4505516904251232e-06
81481,164181,0,164181,537.8951139450073,3.4249350964786683e-06
81582,164383,0,164383,538.5337378978729,3.399182405427791e-06
81682,164583,0,164583,539.1522009372711,3.3738407379563757e-06
81782,164783,0,164783,539.7673690319061,3.3486130951712232e-06
81882,164983,0,164983,540.3566768169403,3.323494234062731e-06
81982,165183,0,165183,540.9868788719177,3.2985329460532954e-06
82082,165383,0,165383,541.6059498786926,3.2736639603264874e-06
82182,165583,0,165583,542.2150871753693,3.248929878597313e-06
82282,165783,0,165783,542.8452107906342,3.224321037993892e-06
82382,165983,0,165983,543.4570989608765,3.199843142208055e-06
82482,166183,0,166183,544.0671417713165,3.1754777956940448e-06
82583,166385,0,166385,544.6755578517914,3.151042886154563e-06
82683,166585,0,166585,545.286041021347,3.1269674225249115e-06
82783,166785,0,166785,545.8747789859772,3.1030502698863703e-06
82883,166985,0,166985,546.4670519828796,3.0793172371672937e-06
82983,167185,0,167185,547.0766189098358,3.055729893422786e-06
83083,167385,0,167385,547.6598899364471,3.0323502903909136e-06
83183,167585,0,167585,548.2589540481567,3.0091515024766936e-06
83283,167785,0,167785,548.8459329605103,2.986155210052376e-06
83383,167985,0,167985,549.4396591186523,2.963356847060609e-06
83483,168185,0,168185,550.0195660591125,2.9407802042907966e-06
83584,168387,0,168387,550.605908870697,2.918170619569536e-06
83684,168587,0,168587,551.191731929779,2.8960151440899013e-06
83784,168787,0,168787,551.7786328792572,2.874061410343222e-06
83884,168987,0,168987,552.3727450370789,2.85231843241691e-06
83984,169187,0,169187,552.9603190422058,2.8308037674667108e-06
84084,169387,0,169387,553.5554180145264,2.8094754450873076e-06
84184,169587,0,169587,554.1372790336609,2.7883687710220772e-06
84284,169787,0,169787,554.7185111045837,2.767452767990027e-06
84384,169987,0,169987,555.3015899658203,2.7467214645459015e-06
84484,170187,0,170187,555.8983118534088,2.72615933508333e-06
84585,170389,0,170389,556.4948379993439,2.705571511941965e-06
84685,170589,0,170589,557.0769329071045,2.685309433290966e-06
84785,170789,0,170789,557.6723310947418,2.665194921709819e-06
84885,170989,0,170989,558.2541718482971,2.645208115197551e-06
84985,171189,0,171189,558.8372559547424,2.6253184580682564e-06
85085,171389,0,171389,559.4406979084015,2.605566462832908e-06
85185,171589,0,171589,560.0951619148254,2.585904061393184e-06
85285,171789,0,171789,560.7126569747925,2.566345352638161e-06
85385,171989,0,171989,561.3095240592957,2.5468993078231486e-06
85485,172189,0,172189,561.9271218776703,2.5275594877472443e-06
85586,172391,0,172391,562.5450518131256,2.508113175755994e-06
85686,172591,0,172591,563.1670877933502,2.488984446413225e-06
85786,172791,0,172791,563.7580919265747,2.46994892586167e-06
85886,172991,0,172991,564.3616309165955,2.451017548838693e-06
85986,173191,0,173191,564.9477660655975,2.4322055746942683e-06
86086,173391,0,173391,565.5448288917542,2.413491154492168e-06
86186,173591,0,173591,566.1716830730438,2.3948986978617078e-06
86286,173791,0,173791,566.7796580791473,2.3764150333947072e-06
86386,173991,0,173991,567.3714711666107,2.3580481831241218e-06
86486,174191,0,174191,567.9748778343201,2.339794836447996e-06
86587,174393,0,174393,568.5997200012207,2.321495051495372e-06
86687,174593,0,174593,569.2078640460968,2.3034812661446043e-06
86787,174793,0,174793,569.8030829429626,2.2856068311588078e-06
86887,174993,0,174993,570.4031829833984,2.2678613479223647e-06
86987,175193,0,175193,571.0293021202087,2.250253911743942e-06
87087,175393,0,175393,571.629312992096,2.232804458135173e-06
87187,175593,0,175593,572.2268528938293,2.215495589391987e-06
87287,175793,0,175793,572.8286700248718,2.1983557392862455e-06
87387,175993,0,175993,573.4384250640869,2.1813796435135547e-06
87487,176193,0,176193,574.0209710597992,2.1645688755179054e-06
87588,176395,0,176395,574.6137809753418,2.147755829317943e-06
87688,176595,0,176595,575.2253239154816,2.1312924838890866e-06
87788,176795,0,176795,575.8048748970032,2.1149801759977623e-06
87888,176995,0,176995,576.3926179409027,2.0988379535929303e-06
87988,177195,0,177195,576.9907479286194,2.082858702918764e-06
88088,177395,0,177395,577.5803310871124,2.0670354740016958e-06
88188,177595,0,177595,578.197338104248,2.0513756143699444e-06
88288,177795,0,177795,578.7861199378967,2.035858888402486e-06
88388,177995,0,177995,579.3867688179016,2.020494909856002e-06
88488,178195,0,178195,579.9717991352081,2.0052747932716198e-06
88589,178397,0,178397,580.5732569694519,1.9900508459123435e-06
88689,178597,0,178597,581.1855340003967,1.9750985379851917e-06
88789,178797,0,178797,581.7794480323792,1.9602906551972216e-06
88889,178997,0,178997,582.3756411075592,1.945596151435756e-06
88989,179197,0,179197,582.9636399745941,1.9310241467658295e-06
89089,179397,0,179397,583.5594608783722,1.9165712747214978e-06
89189,179597,0,179597,584.2747828960419,1.9022216891742925e-06
89289,179797,0,179797,584.9579257965088,1.887975560370724e-06
89389,179997,0,179997,585.7207617759705,1.8738260539184176e-06
89489,180197,0,180197,586.5515367984772,1.8597684035906994e-06
89590,180399,0,180399,587.3266041278839,1.8456527108642321e-06
89690,180599,0,180599,588.3229150772095,1.8317665243006394e-06
89790,180799,0,180799,589.0684008598328,1.8179468026736838e-06
89890,180999,0,180999,589.6977269649506,1.8042040416748932e-06
89990,181199,0,181199,590.4895720481873,1.7905314581199996e-06
90090,181399,0,181399,591.3753180503845,1.776931842160697e-06
90190,181599,0,181599,592.0639729499817,1.7634158459338296e-06
90290,181799,0,181799,592.8882579803467,1.7499692914795147e-06
90390,181999,0,181999,593.499354839325,1.7366111646817009e-06
90490,182199,0,182199,594.1284260749817,1.7233476500255928e-06
90591,182401,0,182401,594.7257721424103,1.710049434287031e-06
90691,182601,0,182601,595.3474910259247,1.6969704935572674e-06
90791,182801,0,182801,595.9379539489746,1.6840096149626877e-06
90891,183001,0,183001,596.5566971302032,1.6711520777234454e-06
90991,183201,0,183201,597.1538910865784,1.6584066526467182e-06
91091,183401,0,183401,597.7538540363312,1.645783710156191e-06
91191,183601,0,183601,598.3675048351288,1.633280882331549e-06
91291,183801,0,183801,598.9858827590942,1.6209014746470676e-06
91391,184001,0,184001,599.5942988395691,1.6086441137379897e-06
91491,184201,0,184201,600.1933560371399,1.596509742104133e-06
91592,184403,0,184403,600.8179559707642,1.5843787362078483e-06
91692,184603,0,184603,601.425598859787,1.5724946821974035e-06
91792,184803,0,184803,602.0334300994873,1.5607202830781737e-06
91892,185003,0,185003,602.6386139392853,1.5490663500186797e-06
91992,185203,0,185203,603.2656409740448,1.5375209073907825e-06
92092,185403,0,185403,603.8959879875183,1.5260812466214766e-06
92192,185603,0,185603,604.5085701942444,1.5147506325257688e-06
92292,185803,0,185803,605.126219034195,1.5035130687255285e-06
92392,186003,0,186003,605.7266299724579,1.4923692652286187e-06
92492,186203,0,186203,606.3310580253601,1.4813166098323629e-06
92593,186405,0,186405,606.9500200748444,1.4702379345534065e-06
92693,186605,0,186605,607.5604820251465,1.459335993350903e-06
92793,186805,0,186805,608.1909618377686,1.4485156785497143e-06
92893,187005,0,187005,608.811802148819,1.437755459854486e-06
92993,187205,0,187205,609.4189748764038,1.4270543735565689e-06
93093,187405,0,187405,610.0142540931702,1.4164150710628116e-06
93193,187605,0,187605,610.6045770645142,1.4058248629781644e-06
93293,187805,0,187805,611.20228099823,1.395291249509511e-06
93393,188005,0,188005,611.8114049434662,1.3848043912678075e-06
93493,188205,0,188205,612.4165670871735,1.3743634345532688e-06
93594,188407,0,188407,613.0349559783936,1.3638681824790274e-06
93694,188607,0,188607,613.6392419338226,1.3535277450155348e-06
93794,188807,0,188807,614.2417321205139,1.3432236341376245e-06
93894,189007,0,189007,614.8418719768524,1.3329751419255003e-06
93994,189207,0,189207,615.4455499649048,1.3227798818890784e-06
94094,189407,0,189407,616.0512890815735,1.3126353530357905e-06
94194,189607,0,189607,616.6510980129242,1.3025547539576348e-06
94294,189807,0,189807,617.2606341838837,1.2925397849867724e-06
94394,190007,0,190007,617.8822209835052,1.2825915753454641e-06
94494,190207,0,190207,618.4849500656128,1.2727206850032e-06
94595,190409,0,190409,619.0867660045624,1.2628334451157749e-06
94695,190609,0,190609,619.6870319843292,1.2531183974701988e-06
94795,190809,0,190809,620.2983071804047,1.2434959456660206e-06
94895,191009,0,191009,620.9165308475494,1.2339553454112062e-06
94995,191209,0,191209,621.5151998996735,1.2245015662122534e-06
95095,191409,0,191409,622.119304895401,1.2151416319119495e-06
95195,191609,0,191609,622.7104949951172,1.2058636528237055e-06
95295,191809,0,191809,623.2983779907227,1.1966755125647558e-06
95395,192009,0,192009,623.8850340843201,1.1875720422037863e-06
95495,192209,0,192209,624.489984035492,1.178548265083279e-06
95596,192411,0,192411,625.0832901000977,1.1695183919269834e-06
95696,192611,0,192611,625.6753380298615,1.1606571934457763e-06
95796,192811,0,192811,626.2768361568451,1.1518652626813492e-06
95896,193011,0,193011,626.906594991684,1.1431520471685178e-06
95996,193211,0,193211,627.5283739566803,1.1345122821810895e-06
96096,193411,0,193411,628.1312749385834,1.1259423518478545e-06
96196,193611,0,193611,628.7546439170837,1.1174488074276777e-06
96296,193811,0,193811,629.3544399738312,1.109021561821781e-06
96396,194011,0,194011,629.9657537937164,1.1006638273926115e-06
96496,194211,0,194211,630.5774290561676,1.0923722907727755e-06
96597,194413,0,194413,631.1818768978119,1.0840583368099956e-06
96697,194613,0,194613,631.7842519283295,1.075881840308675e-06
96797,194813,0,194813,632.3880798816681,1.0677634112301208e-06
96897,195013,0,195013,633.0047340393066,1.0596883876249186e-06
96997,195213,0,195213,633.5937559604645,1.051663210002239e-06
97097,195413,0,195413,634.185035943985,1.0436860946132034e-06
97197,195613,0,195613,634.7786450386047,1.035747017504654e-06
97297,195813,0,195813,635.3675577640533,1.0278549296860162e-06
97397,196013,0,196013,635.9553279876709,1.0200052089645967e-06
97497,196213,0,196213,636.548975944519,1.0121943544906185e-06
97598,196415,0,196415,637.1539199352264,1.0043523179938854e-06
97698,196615,0,196615,637.7392871379852,9.966326188669086e-07
97798,196815,0,196815,638.3265841007233,9.889522774418954e-07
97898,197015,0,197015,638.9100549221039,9.813222441203943e-07
97998,197215,0,197215,639.5118458271027,9.737394366816385e-07
98098,197415,0,197415,640.1088230609894,9.662046130810569e-07
98198,197615,0,197615,640.7085750102997,9.587290081837911e-07
98298,197815,0,197815,641.3140740394592,9.513035387357513e-07
98398,198015,0,198015,641.9098289012909,9.439384114206126e-07
98498,198215,0,198215,642.5046610832214,9.366322869161767e-07
98599,198417,0,198417,643.1066329479218,9.293146885608845e-07
98699,198617,0,198617,643.7138249874115,9.221294159223128e-07
98799,198817,0,198817,644.3119428157806,9.150099619610875e-07
98899,199017,0,199017,644.9177448749542,9.079534592504279e-07
98999,199217,0,199217,645.5203168392181,9.009640445539038e-07
99099,199417,0,199417,646.1035780906677,8.940445639886966e-07
99199,199617,0,199617,646.6888709068298,8.871930218869844e-07
99299,199817,0,199817,647.27774477005,8.804185973959066e-07
99399,200017,0,200017,647.8891589641571,8.737119264510185e-07
99499,200217,0,200217,648.5291268825531,8.670821048970407e-07
99600,200419,0,200419,649.14275598526,8.604598341583776e-07
99700,200619,0,200619,649.7710380554199,8.539735896117068e-07
99800,200819,0,200819,650.3901538848877,8.475539440632675e-07
99900,201019,0,201019,651.0035009384155,8.41203786902975e-07
100000,201219,0,201219,651.6190719604492,8.349147262165961e-07


==> extragradient/plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0026328563690185547,30.358106049564984
100,306,0,306,14.320288896560669,0.9422502041522252
200,619,0,619,27.078051805496216,0.6454136351145678
300,942,0,942,39.46141576766968,0.5019972146039132
400,1286,0,1286,51.95039200782776,0.43140873841620175
501,1619,0,1619,66.2687919139862,0.30496679106112357
601,1944,0,1944,79.18061375617981,0.18817142900277187
701,2262,0,2262,92.19059681892395,0.15371379297272325
801,2579,0,2579,104.54784774780273,0.12338554112716502
901,2894,0,2894,117.20402669906616,0.08221709423217131
1001,3237,0,3237,130.38253784179688,0.06984434218493957
1101,3561,0,3561,143.53513193130493,0.06010246580473832
1201,3898,0,3898,156.12393069267273,0.047199717744222616
1301,4221,0,4221,168.42241096496582,0.04086055685802822
1401,4544,0,4544,180.83590483665466,0.03746282103789143
1502,4890,0,4890,193.27395677566528,0.03298771243418722
1602,5256,0,5256,205.75885581970215,0.030609032513997284
1702,5608,0,5608,218.09506678581238,0.027487031735449835
1802,5950,0,5950,230.6181778907776,0.020729467353265186
1902,6262,0,6262,244.77308678627014,0.016411253938967335
2002,6566,0,6566,257.7110116481781,0.014535583141738168
2102,6924,0,6924,270.39437794685364,0.013081551052449453
2202,7258,0,7258,283.3077030181885,0.01253580897335412
2302,7616,0,7616,297.29773783683777,0.011474476867663135
2402,8018,0,8018,311.64810490608215,0.011022913812834226
2503,8424,0,8424,323.96124792099,0.010595203571808329
2603,8827,0,8827,336.60743594169617,0.01027737539856765
2703,9203,0,9203,349.1094739437103,0.009619172677001865
2803,9575,0,9575,363.7211458683014,0.009170373933208886
2903,9970,0,9970,377.47912979125977,0.008889484050902249
3003,10350,0,10350,390.5671308040619,0.008616093915275026
3103,10748,0,10748,402.9129958152771,0.008305742516016706
3203,11148,0,11148,415.49212884902954,0.008060462809686189
3303,11548,0,11548,427.90462589263916,0.007827010149757493
3403,11948,0,11948,441.50829577445984,0.007600005517303026
3504,12352,0,12352,454.07040572166443,0.007377068571289519
3604,12721,0,12721,466.48176193237305,0.006934409501450845
3704,13105,0,13105,480.4797348976135,0.006671262425635498
3804,13484,0,13484,493.051894903183,0.0064036368258757834
3904,13887,0,13887,505.90757870674133,0.0062162913644169746
4004,14287,0,14287,519.415755033493,0.0060527692799498874
4104,14688,0,14688,532.2386207580566,0.005888929265942775
4204,15090,0,15090,545.2517008781433,0.005745148820044792
4304,15458,0,15458,557.7466368675232,0.005544341333481691
4404,15859,0,15859,570.2446918487549,0.005401691863294874
4505,16267,0,16267,583.5146317481995,0.005264399318165443
4605,16667,0,16667,596.2369027137756,0.005137824160175279
4705,17055,0,17055,609.0616450309753,0.004967653676811899
4805,17408,0,17408,622.1610238552094,0.004760483722098519
4905,17808,0,17808,635.0699429512024,0.004644044355785966
5005,18180,0,18180,647.6781597137451,0.004533124046759345
5105,18584,0,18584,661.5949869155884,0.004425196115630989
5205,18984,0,18984,674.1957459449768,0.004323504846899951
5305,19386,0,19386,688.3045749664307,0.004218546758477948
5405,19786,0,19786,701.8029727935791,0.004117843277968966
5506,20190,0,20190,715.7630977630615,0.004022398318283946
5606,20606,0,20606,728.1963038444519,0.00393091013479318
5706,21010,0,21010,740.8697829246521,0.0038533633795048007
5806,21365,0,21365,753.4239187240601,0.003726492113100608
5906,21747,0,21747,766.8110547065735,0.003625610447392005
6006,22154,0,22154,779.6448328495026,0.0035434126392202715
6106,22521,0,22521,792.4005868434906,0.0034732136208631805
6206,22922,0,22922,804.9844448566437,0.0034003347687246084
6306,23268,0,23268,817.6081347465515,0.003330482374597922
6406,23668,0,23668,830.8294508457184,0.0032464377800249748
6507,24080,0,24080,844.0932068824768,0.003177920281810571
6607,24483,0,24483,857.4227876663208,0.003114156893866665
6707,24848,0,24848,870.7252368927002,0.0030232935387433262
6807,25237,0,25237,884.1292088031769,0.0029530785144706866
6907,25629,0,25629,897.6164417266846,0.0028837659394432146
7007,25996,0,25996,910.8111429214478,0.0028135980733120704
7107,26340,0,26340,924.1725697517395,0.002779390401043439
7207,26734,0,26734,937.2359910011292,0.0027224226840900155
7307,27130,0,27130,950.429780960083,0.0026730402817795595
7407,27489,0,27489,964.0635948181152,0.0026310161955881654
7508,27845,0,27845,977.4715876579285,0.0025825858740462834
7608,28243,0,28243,990.6157388687134,0.002528906891232298
7708,28647,0,28647,1003.7907519340515,0.0024790644118429985
7808,29034,0,29034,1018.2161557674408,0.0024329172547202602
7908,29415,0,29415,1033.5922708511353,0.0023814944757358397
8008,29815,0,29815,1047.6484627723694,0.002333865148872729
8108,30226,0,30226,1061.5310850143433,0.002286652378843076
8208,30619,0,30619,1075.2793338298798,0.0022533649811338164
8308,31012,0,31012,1089.0825889110565,0.0022152277147825016
8408,31419,0,31419,1101.9019718170166,0.0021729502222565637
8509,31825,0,31825,1115.6117010116577,0.0021345489793878755
8609,32182,0,32182,1129.381561756134,0.0020578318140581004
8709,32520,0,32520,1142.8710677623749,0.002020681228389821
8809,32921,0,32921,1158.062005996704,0.001984076473889116
8909,33321,0,33321,1170.9583506584167,0.0019495324044025732
9009,33714,0,33714,1184.101893901825,0.0019117539977271398
9109,34115,0,34115,1197.4933869838715,0.0018802119638683995
9209,34523,0,34523,1210.7037768363953,0.0018478231295097627
9309,34923,0,34923,1223.86079788208,0.0018151816746560902
9409,35323,0,35323,1236.7886867523193,0.001785075383718616
9510,35693,0,35693,1250.95831990242,0.001750890860639731
9610,36061,0,36061,1264.3509788513184,0.0017260215747920834
9710,36462,0,36462,1277.2281339168549,0.0016970871431886921
9810,36863,0,36863,1290.1840069293976,0.0016687473787766263
9910,37248,0,37248,1302.8961129188538,0.0016387053062096035
10010,37626,0,37626,1315.112049818039,0.0015991861080642167
10110,38030,0,38030,1329.5293889045715,0.001572717378416053
10210,38439,0,38439,1342.9929978847504,0.0015473764092206392
10310,38841,0,38841,1355.0766327381134,0.0015231332080212032
10410,39203,0,39203,1367.1157848834991,0.0014926783972053364
10511,39614,0,39614,1379.3518829345703,0.0014589677200493845
10611,40033,0,40033,1391.9240798950195,0.0014336658423230527
10711,40443,0,40443,1407.3018009662628,0.0014126628104428258
10811,40849,0,40849,1420.2639198303223,0.0013896365840841676
10911,41249,0,41249,1435.9298989772797,0.0013697459903100231
11011,41650,0,41650,1449.1853036880493,0.001351024386897269
11111,42050,0,42050,1462.6232538223267,0.001331738889948267
11211,42440,0,42440,1476.052875995636,0.0013131124619855164
11311,42841,0,42841,1488.8200318813324,0.0012938310456183768
11411,43232,0,43232,1502.3149619102478,0.0012732451084010836
11512,43636,0,43636,1515.7867438793182,0.0012554015228936448
11612,44039,0,44039,1528.7091567516327,0.0012353780352350962
11712,44439,0,44439,1542.1411938667297,0.0012171475796690988
11812,44842,0,44842,1555.3097338676453,0.0012000052203734396
11912,45242,0,45242,1568.1469719409943,0.001182460501693055
12012,45649,0,45649,1581.4098329544067,0.0011663032102492224
12112,46050,0,46050,1594.4399118423462,0.0011494719563772899
12212,46456,0,46456,1609.2976748943329,0.001132723206714369
12312,46856,0,46856,1623.9189157485962,0.0011170926976670154
12412,47259,0,47259,1638.1216268539429,0.0011011919814463591
12513,47663,0,47663,1654.0793499946594,0.0010859361579843802
12613,48065,0,48065,1669.9881646633148,0.0010721755351631563
12713,48465,0,48465,1682.8820819854736,0.0010568730436232136
12813,48865,0,48865,1695.256404876709,0.001041453670032459
12913,49265,0,49265,1705.6983397006989,0.001027166286410131
13013,49665,0,49665,1716.2093250751495,0.0010135892301770537
13113,50067,0,50067,1726.5059387683868,0.0009991442060019596
13213,50467,0,50467,1736.7197387218475,0.0009852861658181111
13313,50867,0,50867,1747.8129708766937,0.0009719468480550609
13413,51267,0,51267,1758.6908700466156,0.0009601337440435346
13514,51675,0,51675,1769.4830548763275,0.000946612122085883
13614,52011,0,52011,1780.5671517848969,0.0009271237410040231
13714,52402,0,52402,1791.445071697235,0.000907199593501205
13814,52802,0,52802,1801.578617811203,0.0008916422030383128
13914,53239,0,53239,1811.9286658763885,0.0008783760194220778
14014,53719,0,53719,1822.5408608913422,0.0008661778610022733
14114,54123,0,54123,1832.587462902069,0.0008539540801192267
14214,54523,0,54523,1842.6651289463043,0.0008418467849681847
14314,54923,0,54923,1852.7770779132843,0.0008299138528635405
14414,55323,0,55323,1862.8224167823792,0.0008156513884347599
14515,55727,0,55727,1873.1323509216309,0.0008032012308447868
14615,56151,0,56151,1883.000331878662,0.000794606684711435
14715,56566,0,56566,1893.0025007724762,0.000783648597672953
14815,56931,0,56931,1903.6007947921753,0.0007718833450045091
14915,57331,0,57331,1913.9983139038086,0.0007593463922832501
15015,57731,0,57731,1924.0168859958649,0.0007390001595945756
15115,58131,0,58131,1933.8897268772125,0.0007204871710550149
15215,58531,0,58531,1943.8463339805603,0.0007098726301379159
15315,58931,0,58931,1953.8134589195251,0.0007006559230223607
15415,59331,0,59331,1966.0064158439636,0.0006900433427787053
15516,59735,0,59735,1976.5860648155212,0.0006814299631436453
15616,60135,0,60135,1986.741266965866,0.00067218983020765
15716,60538,0,60538,1996.8994617462158,0.0006592218163309039
15816,60938,0,60938,2007.127644777298,0.0006494569607892599
15916,61339,0,61339,2017.1052479743958,0.0006393652583115093
16016,61740,0,61740,2027.4574139118195,0.0006314554294007589
16116,62140,0,62140,2038.113273859024,0.0006242061074775746
16216,62540,0,62540,2049.5724079608917,0.0006198007037450807
16316,62943,0,62943,2060.2774288654327,0.0006112244860067309
16416,63343,0,63343,2070.4109008312225,0.0006033667849436786
16517,63752,0,63752,2081.179081916809,0.0005958126018257389
16617,64152,0,64152,2091.878425836563,0.0005884304076770148
16717,64560,0,64560,2103.9045197963715,0.0005807329723163746
16817,64960,0,64960,2114.2978649139404,0.000572434739333991
16917,65360,0,65360,2124.975908756256,0.0005645859132482295
17017,65775,0,65775,2137.437141895294,0.0005550983510809038
17117,66177,0,66177,2149.628495693207,0.0005506704438528659
17217,66577,0,66577,2161.1236548423767,0.0005460777058542842
17317,66997,0,66997,2173.260134935379,0.0005390892578602638
17417,67397,0,67397,2185.1960220336914,0.0005325580499249493
17518,67801,0,67801,2195.550178050995,0.0005256167183984047
17618,68239,0,68239,2205.8031108379364,0.0005163361818477986
17718,68712,0,68712,2215.7998719215393,0.0005059529496340252
17818,69113,0,69113,2225.64341878891,0.0004970593989266672
17918,69513,0,69513,2235.604395866394,0.000490409209747679
18018,69914,0,69914,2246.724880695343,0.00048408129955181676
18118,70314,0,70314,2259.1571867465973,0.0004779228277252532
18218,70711,0,70711,2271.1914498806,0.0004712955836481078
18318,71108,0,71108,2281.9602658748627,0.0004650416142208705
18418,71508,0,71508,2291.9779546260834,0.0004588579804950263
18519,71923,0,71923,2302.2331619262695,0.0004530204673623569
18619,72323,0,72323,2312.353904724121,0.00044759037349184546
18719,72723,0,72723,2322.512184858322,0.0004420890566590109
18819,73128,0,73128,2332.6552879810333,0.0004367747293393769
18919,73485,0,73485,2342.8513708114624,0.00043254697721018426
19019,73889,0,73889,2353.4478499889374,0.00042765332796154573
19119,74289,0,74289,2365.029685020447,0.00042268659756135237
19219,74692,0,74692,2375.327740907669,0.0004181894881244355
19319,75093,0,75093,2385.458564758301,0.00041259586685208526
19419,75493,0,75493,2395.5801708698273,0.00040745441649334043
19520,75914,0,75914,2405.8247170448303,0.0004011222259599184
19620,76314,0,76314,2416.0710949897766,0.0003908954558087201
19720,76714,0,76714,2429.1064398288727,0.00038646913196544954
19820,77114,0,77114,2441.77351975441,0.0003837312889559713
19920,77605,0,77605,2454.6682097911835,0.00037901970647472667
20020,78028,0,78028,2465.947621822357,0.00037337793501585775
20120,78428,0,78428,2477.3179309368134,0.00036709534095047484
20220,78828,0,78828,2488.0166709423065,0.0003592615084853481
20320,79254,0,79254,2498.3813309669495,0.0003540389496825915
20420,79753,0,79753,2508.406221628189,0.00034979435996740707
20521,80245,0,80245,2518.6325948238373,0.0003455421829862938
20621,80645,0,80645,2528.718903064728,0.00034109566144315434
20721,81045,0,81045,2538.859433889389,0.0003370433598572845
20821,81445,0,81445,2549.1613688468933,0.0003328912296929974
20921,81845,0,81845,2559.236934900284,0.00032824005876116324
21021,82245,0,82245,2569.1069428920746,0.0003222839904480631
21121,82645,0,82645,2580.5283436775208,0.0003149735616087853
21221,83045,0,83045,2592.5516879558563,0.0003094166758643336
21321,83445,0,83445,2603.307413816452,0.0003056853573100172
21421,83867,0,83867,2613.49449801445,0.0003035396969177266
21522,84278,0,84278,2623.5829129219055,0.0003002678940075171
21622,84722,0,84722,2633.5474138259888,0.0002972424011706127
21722,85123,0,85123,2643.5911927223206,0.0002927944542119663
21822,85520,0,85520,2653.8582026958466,0.0002886471003959103
21922,85920,0,85920,2663.8333439826965,0.0002842087046260646
22022,86325,0,86325,2674.5096328258514,0.0002801494043541774
22122,86725,0,86725,2684.714166879654,0.0002765273536950806
22222,87127,0,87127,2694.6676077842712,0.00027331854256015955
22322,87527,0,87527,2706.027328014374,0.0002703982739312082
22422,87938,0,87938,2716.852288007736,0.0002671699642845657
22523,88342,0,88342,2727.6057438850403,0.00026393392202295754
22623,88739,0,88739,2737.629264831543,0.00026054968150296783
22723,89083,0,89083,2747.581135749817,0.00025739168438893874
22823,89462,0,89462,2757.754903793335,0.0002546240611557995
22923,89863,0,89863,2767.790071964264,0.00025135567755494404
23023,90278,0,90278,2777.8962817192078,0.0002481322576717506
23123,90678,0,90678,2787.796170949936,0.00024436314245598764
23223,91069,0,91069,2797.9175169467926,0.00023944502471971656
23323,91469,0,91469,2808.1920037269592,0.00023644915138251903
23423,91878,0,91878,2818.3492867946625,0.0002336891765335185
23524,92282,0,92282,2828.6790556907654,0.0002313167001717177
23624,92685,0,92685,2840.067464828491,0.00022747135636723886
23724,93018,0,93018,2851.958416700363,0.00022256793569638532
23824,93415,0,93415,2864.5241808891296,0.0002197736223251733
23924,93874,0,93874,2877.2504897117615,0.00021676343303387948
24024,94281,0,94281,2890.878970861435,0.00021460278266645765
24124,94681,0,94681,2903.4709787368774,0.0002121725598343107
24224,95097,0,95097,2914.8310227394104,0.00020995755189278845
24324,95501,0,95501,2925.0266468524933,0.0002073447719691021
24424,95904,0,95904,2935.1892297267914,0.00020485085406243838
24525,96308,0,96308,2945.5024378299713,0.00020234842124037587
24625,96708,0,96708,2955.6885879039764,0.00019990870849697433
24725,97126,0,97126,2965.9204998016357,0.00019757604451493875
24825,97526,0,97526,2976.485944747925,0.00019519605992010454
24925,97927,0,97927,2987.0093989372253,0.00019278623540830374
25025,98328,0,98328,2997.2754468917847,0.00019027273379862935
25125,98728,0,98728,3007.46142578125,0.00018782146487290562
25225,99136,0,99136,3017.6086568832397,0.00018545885317105474
25325,99536,0,99536,3027.7731597423553,0.00018343074029495042
25425,99936,0,99936,3037.852336883545,0.00018121262467681127
25526,100355,0,100355,3048.353572845459,0.00017885030901587144
25626,100755,0,100755,3058.483521938324,0.00017744250239785196
25726,101155,0,101155,3068.516399860382,0.00017620022457903863
25826,101555,0,101555,3078.8042690753937,0.00017432231954308343
25926,101955,0,101955,3088.941330909729,0.00017235473907902421
26026,102360,0,102360,3099.06387090683,0.0001703375897657138
26126,102760,0,102760,3109.594944000244,0.00016824277805839092
26226,103160,0,103160,3119.785757780075,0.00016613215877260622
26326,103577,0,103577,3129.8505227565765,0.00016417944210684837
26426,103977,0,103977,3140.1339190006256,0.0001621673380239702
26527,104381,0,104381,3150.4823989868164,0.00016014291144940578
26627,104782,0,104782,3161.9972388744354,0.00015807519639960568
26727,105182,0,105182,3172.9561138153076,0.00015596637564836035
26827,105582,0,105582,3184.272752761841,0.00015365815470126724
26927,106003,0,106003,3197.077116727829,0.0001520655123490817
27027,106445,0,106445,3209.068366765976,0.00015073270353364255
27127,106845,0,106845,3221.616997718811,0.00014921545296488274
27227,107251,0,107251,3231.8350188732147,0.00014734865759007267
27327,107658,0,107658,3242.047626018524,0.00014577787942409172
27427,108058,0,108058,3252.392695903778,0.0001442151355241795
27528,108462,0,108462,3262.63801074028,0.00014258573622551632
27628,108862,0,108862,3272.9561710357666,0.00013992986611692052
27728,109262,0,109262,3284.481151819229,0.0001379309281835918
27828,109662,0,109662,3296.6992888450623,0.00013624660496959026
27928,110062,0,110062,3307.9787929058075,0.00013472107999085067
28028,110470,0,110470,3318.666251897812,0.00013307307705188572
28128,110868,0,110868,3328.813841819763,0.00013097885779502112
28228,111268,0,111268,3339.798820734024,0.00012944935322995203
28328,111668,0,111668,3350.0267357826233,0.00012794100022306263
28428,112068,0,112068,3360.3446147441864,0.00012643371187944367
28529,112484,0,112484,3370.85897397995,0.0001251510589176902
28629,112886,0,112886,3381.0274329185486,0.0001237224753678505
28729,113288,0,113288,3391.111303806305,0.00012234700531482272
28829,113688,0,113688,3401.552274942398,0.00012105308878328524
28929,114094,0,114094,3411.7404396533966,0.00011984130612321805
29029,114494,0,114494,3421.843284845352,0.00011831028544112074
29129,114897,0,114897,3432.0412769317627,0.000116863388425639
29229,115297,0,115297,3442.1782598495483,0.0001155090881472452
29329,115697,0,115697,3453.0048887729645,0.00011435749326729027
29429,116104,0,116104,3463.918296813965,0.00011275102387235703
29530,116508,0,116508,3475.3084738254547,0.00011137631688930513
29630,116911,0,116911,3486.5675337314606,0.00010994599303183763
29730,117311,0,117311,3497.7788178920746,0.00010868704086356126
29830,117715,0,117715,3508.458199739456,0.00010749132585568326
29930,118108,0,118108,3518.988511800766,0.00010573523422980514
30030,118470,0,118470,3530.6023547649384,0.00010427149020952374
30130,118902,0,118902,3542.5246357917786,0.00010238439144053656
30230,119328,0,119328,3552.650099992752,0.00010120286543551357
30330,119728,0,119728,3563.0353558063507,0.00010016376256316201
30430,120128,0,120128,3574.745941877365,9.899154154943003e-05
30531,120532,0,120532,3587.2326788902283,9.783412763344362e-05
30631,120932,0,120932,3600.6748719215393,9.670266493882557e-05
30731,121332,0,121332,3611.5405728816986,9.556820637225997e-05
30831,121732,0,121732,3622.702734708786,9.451937675865648e-05
30931,122137,0,122137,3634.2105967998505,9.345792122304126e-05
31031,122537,0,122537,3645.1981859207153,9.224222854676652e-05
31131,122937,0,122937,3657.150510787964,9.089501189611666e-05
31231,123339,0,123339,3671.5934069156647,8.982681197707944e-05
31331,123739,0,123739,3684.3202769756317,8.880867559191539e-05
31431,124139,0,124139,3695.6493859291077,8.782861827264184e-05
31532,124567,0,124567,3707.0144877433777,8.685378806724268e-05
31632,124971,0,124971,3717.607852935791,8.568056820440973e-05
31732,125425,0,125425,3727.92174577713,8.456313465542205e-05
31832,125905,0,125905,3738.064008951187,8.356591233946333e-05
31932,126305,0,126305,3748.341814994812,8.257840044893502e-05
32032,126705,0,126705,3758.713833808899,8.167460515263254e-05
32132,127105,0,127105,3770.195755004883,8.07903865550202e-05
32232,127504,0,127504,3780.9095590114594,7.982945388256612e-05
32332,127904,0,127904,3791.4729838371277,7.887673167716399e-05
32432,128304,0,128304,3801.6878888607025,7.797824808701287e-05
32533,128724,0,128724,3811.8930938243866,7.705514441986566e-05
32633,129124,0,129124,3822.077381849289,7.602862569224201e-05
32733,129524,0,129524,3833.0901918411255,7.517930967801706e-05
32833,129924,0,129924,3844.7061858177185,7.433557134709314e-05
32933,130320,0,130320,3855.539563894272,7.340595561279589e-05
33033,130720,0,130720,3865.6352648735046,7.24778667596786e-05
33133,131120,0,131120,3875.800526857376,7.155545381974582e-05
33233,131537,0,131537,3885.8442759513855,7.078417101927625e-05
33333,131937,0,131937,3896.709077835083,6.999728209802592e-05
33433,132337,0,132337,3907.623962879181,6.93934668221286e-05
33534,132760,0,132760,3917.9817748069763,6.853028539667494e-05
33634,133160,0,133160,3928.254852771759,6.778675541907926e-05
33734,133560,0,133560,3940.9250617027283,6.736134291238419e-05
33834,133966,0,133966,3954.983341693878,6.67157720353266e-05
33934,134366,0,134366,3968.4900019168854,6.602598143685546e-05
34034,134774,0,134774,3980.8073558807373,6.54221366098861e-05
34134,135206,0,135206,3991.9372317790985,6.453727229134149e-05
34234,135617,0,135617,4002.3161787986755,6.396465409845194e-05
34334,136017,0,136017,4013.07923579216,6.320597244996557e-05
34434,136417,0,136417,4025.0460538864136,6.238717770196551e-05
34535,136824,0,136824,4035.7009868621826,6.163485949844837e-05
34635,137224,0,137224,4045.6716380119324,6.091563171089057e-05
34735,137624,0,137624,4055.7392678260803,6.020143165021511e-05
34835,138034,0,138034,4066.73597574234,5.9561336599476496e-05
34935,138434,0,138434,4077.6231570243835,5.892966210536418e-05
35035,138834,0,138834,4087.7863857746124,5.8444390828926566e-05
35135,139234,0,139234,4097.93643283844,5.7903114351401115e-05
35235,139634,0,139634,4108.184392929077,5.714054849741641e-05
35335,140057,0,140057,4119.116251707077,5.6164668673561406e-05
35435,140479,0,140479,4129.350229024887,5.567728491481927e-05
35536,140883,0,140883,4140.04344701767,5.5098798203238274e-05
35636,141283,0,141283,4150.725972890854,5.4577777657216226e-05
35736,141683,0,141683,4161.557512760162,5.393398063107944e-05
35836,142083,0,142083,4172.361981868744,5.328298949773998e-05
35936,142483,0,142483,4182.935382843018,5.2694614917925634e-05
36036,142883,0,142883,4196.078763008118,5.2115032567726434e-05
36136,143283,0,143283,4206.873333930969,5.152686108950694e-05
36236,143683,0,143683,4218.458694934845,5.08969942216297e-05
36336,144083,0,144083,4228.7423667907715,5.0269390135097306e-05
36436,144483,0,144483,4238.797570705414,4.965012760690812e-05
36537,144916,0,144916,4248.8703808784485,4.899587551565599e-05
36637,145316,0,145316,4260.735287904739,4.836202742050014e-05
36737,145732,0,145732,4271.326268911362,4.778087015953832e-05
36837,146193,0,146193,4282.098360776901,4.724512062706605e-05
36937,146655,0,146655,4292.295848846436,4.6840877385218866e-05
37037,147069,0,147069,4302.525901079178,4.639659651361963e-05
37137,147493,0,147493,4312.62343287468,4.588819103869085e-05
37237,147893,0,147893,4322.5288026332855,4.536320075098226e-05
37337,148293,0,148293,4332.695277690887,4.481017225825197e-05
37437,148693,0,148693,4342.5907208919525,4.41078841408741e-05
37538,149097,0,149097,4352.70111489296,4.358566571676771e-05
37638,149497,0,149497,4363.154179811478,4.313335671503863e-05
37738,149919,0,149919,4373.512731790543,4.2716110020942954e-05
37838,150319,0,150319,4383.948361873627,4.2194737723441915e-05
37938,150715,0,150715,4393.886861085892,4.161033947365209e-05
38038,151123,0,151123,4403.9251227378845,4.113552616975659e-05
38138,151523,0,151523,4413.91786980629,4.06857486244519e-05
38238,151923,0,151923,4423.733615875244,4.030817032521562e-05
38338,152330,0,152330,4433.726512908936,3.97464528722631e-05
38438,152738,0,152738,4443.656572818756,3.932924176513749e-05
38539,153145,0,153145,4453.900458812714,3.8934127746041905e-05
38639,153545,0,153545,4463.75693488121,3.839332190384249e-05
38739,153945,0,153945,4474.878427743912,3.784860045309609e-05
38839,154346,0,154346,4486.6213257312775,3.71868576988942e-05
38939,154767,0,154767,4496.968081951141,3.6708971579778275e-05
39039,155171,0,155171,4507.167531013489,3.63115642901297e-05
39139,155571,0,155571,4516.9626569747925,3.5907477202159014e-05
39239,155971,0,155971,4526.734974861145,3.548819613236401e-05
39339,156371,0,156371,4536.79537987709,3.5078287986173454e-05
39439,156789,0,156789,4546.592157840729,3.459846285166222e-05
39540,157193,0,157193,4556.453375816345,3.413088614416957e-05
39640,157593,0,157593,4567.030353784561,3.371303340880087e-05
39740,157993,0,157993,4579.504422903061,3.3268258139279165e-05
39840,158405,0,158405,4589.299461841583,3.271433058919915e-05
39940,158813,0,158813,4599.260725021362,3.2461090072945196e-05
40040,159267,0,159267,4609.4146900177,3.2058850385841914e-05
40140,159667,0,159667,4619.198193788528,3.168800467911144e-05
40240,160071,0,160071,4629.182372808456,3.129020721717123e-05
40340,160471,0,160471,4638.985112667084,3.0928661935873606e-05
40440,160872,0,160872,4649.4882798194885,3.0562911023019355e-05
40541,161276,0,161276,4659.480014801025,3.0187697024666925e-05
40641,161679,0,161679,4669.531934976578,2.9848702079798598e-05
40741,162079,0,162079,4680.510471820831,2.9519568518714734e-05
40841,162479,0,162479,4692.447855710983,2.9175100383889804e-05
40941,162879,0,162879,4703.369692802429,2.882527263320823e-05
41041,163281,0,163281,4714.25435590744,2.851200088929682e-05
41141,163683,0,163683,4725.569247961044,2.8203158722222263e-05
41241,164083,0,164083,4735.730828046799,2.7885697857660244e-05
41341,164490,0,164490,4746.959768772125,2.7575361468084376e-05
41441,164890,0,164890,4758.149640798569,2.729608407853401e-05
41542,165343,0,165343,4769.049248933792,2.706331452754166e-05
41642,165764,0,165764,4780.049454689026,2.6660154793363547e-05
41742,166164,0,166164,4791.22819185257,2.628852459491141e-05
41842,166576,0,166576,4802.465106964111,2.595007146490731e-05
41942,167020,0,167020,4813.324889659882,2.5655526130181784e-05
42042,167420,0,167420,4823.83212685585,2.532965838536584e-05
42142,167820,0,167820,4834.477093696594,2.5031770030239653e-05
42242,168262,0,168262,4845.29097867012,2.4824594205915403e-05
42342,168712,0,168712,4855.489416837692,2.4554693324789405e-05
42442,169112,0,169112,4865.652290821075,2.424994326827886e-05
42543,169516,0,169516,4876.939782857895,2.3946943791369842e-05
42643,169916,0,169916,4887.544286966324,2.368230508305363e-05
42743,170316,0,170316,4897.634063720703,2.3424852048576904e-05
42843,170718,0,170718,4907.549701690674,2.315500117887978e-05
42943,171124,0,171124,4918.015922784805,2.2866906003554736e-05
43043,171524,0,171524,4928.2339408397675,2.261205958635084e-05
43143,171924,0,171924,4939.7607617378235,2.234806716367232e-05
43243,172324,0,172324,4951.0381598472595,2.206940008733229e-05
43343,172752,0,172752,4961.478968858719,2.1830336340416323e-05
43443,173165,0,173165,4972.182922840118,2.156746679860404e-05
43544,173569,0,173569,4982.675860881805,2.1324232292795074e-05
43644,173971,0,173971,4993.014811754227,2.1086319392166087e-05
43744,174371,0,174371,5003.6672167778015,2.0849303813133373e-05
43844,174771,0,174771,5014.8869388103485,2.0618252988014274e-05
43944,175171,0,175171,5025.874874830246,2.0428074471604026e-05
44044,175579,0,175579,5035.892442703247,2.0216628712791705e-05
44144,175979,0,175979,5045.915585041046,2.001200989623607e-05
44244,176379,0,176379,5056.712639808655,1.978816457252913e-05
44344,176780,0,176780,5068.182596683502,1.95670079437613e-05
44444,177180,0,177180,5078.4361798763275,1.9349374272162423e-05
44545,177584,0,177584,5089.130698919296,1.9138829147075982e-05
44645,177989,0,177989,5099.708534955978,1.8971141035306394e-05
44745,178389,0,178389,5111.08406496048,1.8753997904304344e-05
44845,178789,0,178789,5122.096751689911,1.8525506379824143e-05
44945,179186,0,179186,5133.39354968071,1.829022230647906e-05
45045,179587,0,179587,5144.344250679016,1.8091986684099703e-05
45145,179987,0,179987,5154.312718868256,1.7881846006866393e-05
45245,180387,0,180387,5164.798399925232,1.768224702491259e-05
45345,180787,0,180787,5174.792721748352,1.7460532900104204e-05
45445,181187,0,181187,5184.948194742203,1.723242316174815e-05
45546,181591,0,181591,5196.3235738277435,1.7025631880332628e-05
45646,182010,0,182010,5206.863363742828,1.6876316522709253e-05
45746,182451,0,182451,5217.5674369335175,1.6710999324673394e-05
45846,182862,0,182862,5228.484987735748,1.6531766342470556e-05
45946,183262,0,183262,5239.077036857605,1.638838835223355e-05
46046,183662,0,183662,5249.284647941589,1.6250863947252408e-05
46146,184062,0,184062,5259.31104683876,1.611922120852518e-05
46246,184493,0,184493,5269.318282842636,1.5985157267241232e-05
46346,184912,0,184912,5279.40225481987,1.5776588784033497e-05
46446,185394,0,185394,5290.089840888977,1.5569814480015045e-05
46547,185861,0,185861,5300.253712892532,1.530581284839792e-05
46647,186286,0,186286,5310.498909950256,1.50648802651523e-05
46747,186687,0,186687,5320.58917093277,1.4858430871343398e-05
46847,187087,0,187087,5330.54723405838,1.4687276132686402e-05
46947,187487,0,187487,5341.5915858745575,1.4532423666935653e-05
47047,187887,0,187887,5352.701686859131,1.4470956239492378e-05
47147,188287,0,188287,5363.631676912308,1.4238108624375247e-05
47247,188687,0,188687,5374.274030685425,1.3830366697500005e-05
47347,189087,0,189087,5385.685078859329,1.3597156015712433e-05
47447,189487,0,189487,5395.71701669693,1.342528667369465e-05
47548,189892,0,189892,5405.864633798599,1.3258520744842657e-05
47648,190292,0,190292,5416.042627811432,1.3116190288640837e-05
47748,190744,0,190744,5426.035094022751,1.2980172541237682e-05
47848,191194,0,191194,5436.215679883957,1.2788036334922801e-05
47948,191598,0,191598,5448.63534283638,1.2637215632115302e-05
48048,191998,0,191998,5459.430818080902,1.2477754383523048e-05
48148,192398,0,192398,5469.444789886475,1.2299972777150304e-05
48248,192798,0,192798,5479.482694864273,1.2136605585952214e-05
48348,193214,0,193214,5489.866908788681,1.1971081094836657e-05
48448,193614,0,193614,5502.103098869324,1.1844461754963386e-05
48549,194060,0,194060,5512.12437081337,1.171528405790925e-05
48649,194462,0,194462,5522.228287935257,1.1554897354792769e-05
48749,194862,0,194862,5533.769217014313,1.1414597292951774e-05
48849,195265,0,195265,5544.9055688381195,1.125880700614873e-05
48949,195665,0,195665,5555.437716960907,1.1139675995979238e-05
49049,196065,0,196065,5565.4607038497925,1.1020432295072243e-05
49149,196481,0,196481,5575.610279798508,1.0900187352281154e-05
49249,196881,0,196881,5585.649618864059,1.0769889276972745e-05
49349,197281,0,197281,5595.685715913773,1.064627372715248e-05
49449,197681,0,197681,5606.304788827896,1.0525563523899414e-05
49550,198085,0,198085,5616.7632439136505,1.042187113519763e-05
49650,198537,0,198537,5626.851796865463,1.0313348509871162e-05
49750,198943,0,198943,5636.912987709045,1.0186057078732708e-05
49850,199343,0,199343,5647.164335727692,1.0083348773931497e-05
49950,199743,0,199743,5657.734130859375,9.980630424658256e-06
50050,200143,0,200143,5668.735941886902,9.888773482690802e-06
50150,200561,0,200561,5679.965418815613,9.804023609915965e-06
50250,201024,0,201024,5690.150532722473,9.682444694856837e-06
50350,201445,0,201445,5700.1978487968445,9.581215447898793e-06
50450,201845,0,201845,5710.442479848862,9.465698092260571e-06
50551,202311,0,202311,5720.719299793243,9.35394046232098e-06
50651,202736,0,202736,5730.787453889847,9.306934794413667e-06
50751,203147,0,203147,5741.022821903229,9.231362089064466e-06
50851,203551,0,203551,5752.605818748474,9.113591110249482e-06
50951,203951,0,203951,5763.109275817871,9.007051101234301e-06
51051,204351,0,204351,5773.987378835678,8.902272761549182e-06
51151,204753,0,204753,5784.817870855331,8.799943891521851e-06
51251,205153,0,205153,5794.966627836227,8.69876722801585e-06
51351,205553,0,205553,5805.464652061462,8.596302981169532e-06
51451,205955,0,205955,5817.167312860489,8.495105583119697e-06
51552,206359,0,206359,5828.283645868301,8.399346704903733e-06
51652,206769,0,206769,5839.159593820572,8.314394151670704e-06
51752,207188,0,207188,5849.95116186142,8.214676671364452e-06
51852,207616,0,207616,5860.731780767441,8.1229090312935e-06
51952,208016,0,208016,5871.957078933716,8.02623165788817e-06
52052,208416,0,208416,5883.588018894196,7.934131364352607e-06
52152,208820,0,208820,5894.94437289238,7.843330498326725e-06
52252,209220,0,209220,5906.955757856369,7.750954060909387e-06
52352,209620,0,209620,5917.639263868332,7.665023734343951e-06
52452,210035,0,210035,5928.709703922272,7.593378375188449e-06
52553,210441,0,210441,5940.192176818848,7.4942685379516696e-06
52653,210841,0,210841,5951.48242688179,7.40790571840286e-06
52753,211251,0,211251,5963.860898017883,7.33135323530711e-06
52853,211651,0,211651,5975.599026918411,7.244134373062369e-06
52953,212051,0,212051,5987.012977838516,7.168177194264008e-06
53053,212466,0,212466,5998.409687757492,7.113549694973732e-06
53153,212878,0,212878,6009.582151889801,7.026998430259692e-06
53253,213278,0,213278,6020.208327770233,6.9467247210828205e-06
53353,213678,0,213678,6030.79859995842,6.870113439326289e-06
53453,214078,0,214078,6041.498998880386,6.7959071784617575e-06
53554,214484,0,214484,6052.552349805832,6.723883966941916e-06
53654,214884,0,214884,6063.074895858765,6.6492067379089875e-06
53754,215291,0,215291,6073.579252958298,6.5721755472975515e-06
53854,215690,0,215690,6083.956429004669,6.495893647372448e-06
53954,216090,0,216090,6094.240772724152,6.423023420075878e-06
54054,216490,0,216490,6104.384328842163,6.352718985421361e-06
54154,216928,0,216928,6114.748403787613,6.288196511592228e-06
54254,217330,0,217330,6125.165185928345,6.216683548407225e-06
54354,217740,0,217740,6135.669550657272,6.121262803207672e-06
54454,218160,0,218160,6146.052115917206,6.082028683836774e-06
54555,218564,0,218564,6156.599954843521,6.0399517114100855e-06
54655,218964,0,218964,6168.407337903976,5.988628870417393e-06
54755,219398,0,219398,6178.977984905243,5.927141694345715e-06
54855,219816,0,219816,6189.519851922989,5.827774635370873e-06
54955,220216,0,220216,6201.0712077617645,5.737545491409928e-06
55055,220616,0,220616,6211.939050912857,5.6389711550402334e-06
55155,221021,0,221021,6224.002977848053,5.548474276971407e-06
55255,221421,0,221421,6234.610040664673,5.493797967710033e-06
55355,221821,0,221821,6245.74210691452,5.439645830606562e-06
55455,222237,0,222237,6256.538938760757,5.380789089292857e-06
55556,222641,0,222641,6267.344523906708,5.313852258092505e-06
55656,223041,0,223041,6278.137974977493,5.2500186030035825e-06
55756,223441,0,223441,6289.188262939453,5.1881383030339805e-06
55856,223841,0,223841,6299.9364647865295,5.129711487413517e-06
55956,224241,0,224241,6309.912473678589,5.073067050438757e-06
56056,224648,0,224648,6319.856200933456,5.016830084648336e-06
56156,225048,0,225048,6329.745715856552,4.960453306234759e-06
56256,225448,0,225448,6339.912431716919,4.903677984941614e-06
56356,225848,0,225848,6350.583124876022,4.85097982085289e-06
56456,226290,0,226290,6361.1688277721405,4.79741280558138e-06
56557,226709,0,226709,6373.889014005661,4.730011937986839e-06
56657,227126,0,227126,6386.898291826248,4.689971952161236e-06
56757,227526,0,227526,6398.329894781113,4.647048172052899e-06
56857,227926,0,227926,6409.246228933334,4.59694095657292e-06
56957,228326,0,228326,6419.943177938461,4.547556612461091e-06
57057,228726,0,228726,6429.844078779221,4.5128033713149055e-06
57157,229150,0,229150,6439.95091676712,4.4533364064090605e-06
57257,229550,0,229550,6451.639367818832,4.3973023300702936e-06
57357,229950,0,229950,6462.413186073303,4.347810297784083e-06
57457,230373,0,230373,6472.433758974075,4.304443452209902e-06
57558,230777,0,230777,6482.479736089706,4.268014115320721e-06
57658,231200,0,231200,6492.521454811096,4.216705319764031e-06
57758,231600,0,231600,6503.987907648087,4.167996597655336e-06
57858,232000,0,232000,6514.406795978546,4.1226949198811136e-06
57958,232400,0,232400,6524.448867797852,4.078679981304765e-06
58058,232800,0,232800,6534.88875079155,4.035813166370459e-06
58158,233210,0,233210,6545.798992872238,3.992801917373896e-06
58258,233610,0,233610,6557.050982713699,3.943799626549921e-06
58358,234019,0,234019,6567.040434837341,3.897027019152542e-06
58458,234419,0,234419,6578.073345899582,3.855001292252268e-06
58559,234823,0,234823,6589.431523799896,3.8132994025712006e-06
58659,235223,0,235223,6603.872560739517,3.774602791944578e-06
58759,235650,0,235650,6615.565088033676,3.739124529237241e-06
58859,236050,0,236050,6628.239198923111,3.693208533509167e-06
58959,236450,0,236450,6639.196997880936,3.6500253698180134e-06
59059,236855,0,236855,6649.345595836639,3.6092819017486706e-06
59159,237255,0,237255,6659.30327296257,3.5712072976781485e-06
59259,237655,0,237655,6669.114847898483,3.535824461703461e-06
59359,238079,0,238079,6679.057107925415,3.5094123836806934e-06
59459,238486,0,238486,6690.341347694397,3.460350696653848e-06
59560,238890,0,238890,6701.551258802414,3.4172713765374545e-06
59660,239290,0,239290,6711.54962182045,3.3788963853607173e-06
59760,239716,0,239716,6721.513408899307,3.344416751750773e-06
59860,240116,0,240116,6731.665677785873,3.308377530628277e-06
59960,240516,0,240516,6741.886015892029,3.274083711519252e-06
60060,240941,0,240941,6751.941395998001,3.2399277962230358e-06
60160,241341,0,241341,6762.607656955719,3.2022356680261435e-06
60260,241741,0,241741,6774.9292578697205,3.166124679701199e-06
60360,242141,0,242141,6785.641284704208,3.1308050751517447e-06
60460,242544,0,242544,6795.748785734177,3.0978318385399927e-06
60561,242955,0,242955,6806.00492477417,3.061141955773735e-06
60661,243357,0,243357,6815.982434749603,3.026342263944977e-06
60761,243757,0,243757,6826.462989807129,2.993669256996373e-06
60861,244157,0,244157,6836.800254821777,2.9598728633145336e-06
60961,244557,0,244557,6846.862382650375,2.9269927671491856e-06
61061,244971,0,244971,6856.974760770798,2.9008338717312994e-06
61161,245392,0,245392,6867.0651977062225,2.866866387957142e-06
61261,245812,0,245812,6878.759229898453,2.8345821190155197e-06
61361,246263,0,246263,6889.680304765701,2.798538181405236e-06
61461,246720,0,246720,6901.035206794739,2.7749687384301106e-06
61562,247192,0,247192,6912.522010803223,2.7419974410638376e-06
61662,247614,0,247614,6923.924127817154,2.7071891868517793e-06
61762,248014,0,248014,6935.175519943237,2.6747138328648107e-06
61862,248414,0,248414,6946.560245990753,2.64419654839792e-06
61962,248814,0,248814,6956.7614488601685,2.6139010502765676e-06
62062,249214,0,249214,6966.744277954102,2.58320113449307e-06
62162,249614,0,249614,6980.967495918274,2.5623865649745302e-06
62262,250017,0,250017,6991.685698747635,2.5313798309933523e-06
62362,250417,0,250417,7130.561433792114,2.50325161168091e-06
62462,250817,0,250817,7144.060402870178,2.4760799122340626e-06
62563,251221,0,251221,7155.007926940918,2.4505143242134578e-06
62663,251653,0,251653,7165.424834012985,2.4272100381258585e-06
62763,252056,0,252056,7176.063416719437,2.398698182750731e-06
62863,252458,0,252458,7185.893605709076,2.3712131526833173e-06
62963,252859,0,252859,7195.947855710983,2.3486279402466145e-06
63063,253259,0,253259,7206.729133844376,2.3240627763563196e-06
63163,253659,0,253659,7220.108228683472,2.2993386098569537e-06
63263,254060,0,254060,7230.194826841354,2.276323700992765e-06
63363,254543,0,254543,7241.748633861542,2.2529113228515458e-06
63463,254957,0,254957,7253.03680896759,2.232512906693952e-06
63564,255362,0,255362,7266.5976939201355,2.2089413419983377e-06
63664,255778,0,255778,7279.514303922653,2.1873171095272813e-06
63764,256178,0,256178,7290.438591003418,2.1648694720531835e-06
63864,256578,0,256578,7300.657102823257,2.1422366969407022e-06
63964,256978,0,256978,7310.928555011749,2.1170639269188167e-06
64064,257408,0,257408,7320.9234828948975,2.0943110712389345e-06
64164,257808,0,257808,7330.89550280571,2.0726780639948353e-06
64264,258208,0,258208,7340.797921895981,2.04850974175818e-06
64364,258616,0,258616,7350.848154783249,2.024432043531637e-06
64464,259016,0,259016,7364.275927782059,2.0007855480485393e-06
64565,259420,0,259420,7377.339048862457,1.974744178672659e-06
64665,259844,0,259844,7390.293400764465,1.9507496269949372e-06
64765,260244,0,260244,7401.330806970596,1.930336787223596e-06
64865,260644,0,260644,7415.548991918564,1.910082060219956e-06
64965,261044,0,261044,7426.118906736374,1.8904970211509851e-06
65065,261447,0,261447,7437.03723692894,1.876005256229634e-06
65165,261878,0,261878,7447.495055675507,1.8538447316420386e-06
65265,262278,0,262278,7458.0891127586365,1.8336837005698339e-06
65365,262696,0,262696,7468.440954685211,1.8151394535474332e-06
65465,263096,0,263096,7478.9291298389435,1.7971553648884543e-06
65566,263500,0,263500,7489.011496782303,1.7806875709085267e-06
65666,263918,0,263918,7498.96933889389,1.7669135680824723e-06
65766,264331,0,264331,7510.030032873154,1.744163940637864e-06
65866,264731,0,264731,7519.963414907455,1.7237721992891986e-06
65966,265130,0,265130,7530.952185869217,1.7036444515446634e-06
66066,265536,0,265536,7541.562170743942,1.6843442642963872e-06
66166,265949,0,265949,7551.472735881805,1.6668151650154212e-06
66266,266377,0,266377,7561.252680778503,1.6518713371833432e-06
66366,266788,0,266788,7572.763526916504,1.6281155395410053e-06
66466,267188,0,267188,7582.582846879959,1.6075401053360116e-06
66567,267592,0,267592,7593.745565891266,1.5885363300896434e-06
66667,267992,0,267992,7604.767908811569,1.5712863993797225e-06
66767,268393,0,268393,7689.023098707199,1.555194061089775e-06
66867,268793,0,268793,7727.548644781113,1.5396609228738053e-06
66967,269197,0,269197,7765.137663841248,1.5240343036482317e-06
67067,269597,0,269597,7786.671293973923,1.5070412711410389e-06
67167,269997,0,269997,13520.848861932755,1.49084890704183e-06
67267,270397,0,270397,13536.916369915009,1.4754826628343498e-06
67367,270797,0,270797,13553.955519914627,1.4611579781155318e-06
67467,271231,0,271231,13569.34403681755,1.4458233604153994e-06
67568,271700,0,271700,13582.381492853165,1.4287637620475838e-06
67668,272100,0,272100,13593.752383947372,1.4177748333950488e-06
67768,272500,0,272500,13605.308815717697,1.4049215332131361e-06
67868,272900,0,272900,13617.487741947174,1.392096204809855e-06
67968,273300,0,273300,13628.88274884224,1.3790095081733934e-06
68068,273728,0,273728,13642.253819704056,1.3669564816260645e-06
68168,274134,0,274134,13657.66178202629,1.3505213695926098e-06
68268,274534,0,274534,13673.149640798569,1.3342109382112987e-06
68368,274995,0,274995,13688.408628940582,1.3180577277775576e-06
68468,275442,0,275442,13705.88222694397,1.3074120288244478e-06
68569,275851,0,275851,13725.300395965576,1.2999680212634706e-06
68669,276269,0,276269,13744.52787399292,1.2836178587190838e-06
68769,276669,0,276669,13758.534643888474,1.268964885444587e-06
68869,277069,0,277069,13771.22844696045,1.2543004083205812e-06
68969,277469,0,277469,13784.803527832031,1.2398659073653343e-06
69069,277881,0,277881,13797.879735946655,1.2264720414525902e-06
69169,278284,0,278284,13811.065168857574,1.2092716782662362e-06
69269,278703,0,278703,13825.623783826828,1.1974524783488282e-06
69369,279103,0,279103,13838.348809957504,1.184253505406977e-06
69469,279503,0,279503,13851.021616697311,1.1712390022266077e-06
69570,279907,0,279907,13862.672761678696,1.1593639503684127e-06
69670,280345,0,280345,13873.935953855515,1.1487286153379232e-06
69770,280759,0,280759,13885.218297719955,1.1344217395285738e-06
69870,281159,0,281159,13897.184917926788,1.1212149625672243e-06
69970,281559,0,281559,13911.443629741669,1.1080076491003522e-06
70070,281960,0,281960,13926.943417787552,1.0961625287842646e-06
70170,282360,0,282360,13942.243999958038,1.0846008796971656e-06
70270,282760,0,282760,13955.086726903915,1.0746970309398854e-06
70370,283187,0,283187,13967.901709079742,1.0620794082976127e-06
70470,283587,0,283587,13980.773181915283,1.0493442228658675e-06
70571,283991,0,283991,13992.7038667202,1.0375099782643808e-06
70671,284392,0,284392,14005.466857910156,1.0248599846607567e-06
70771,284792,0,284792,14019.3892557621,1.014312930603419e-06
70871,285192,0,285192,14030.500526666641,1.0037112377102884e-06
70971,285610,0,285610,14041.964143753052,9.934929753541923e-07
71071,286010,0,286010,14054.321960926056,9.822915458035683e-07
71171,286410,0,286410,14068.522819757462,9.714335854496573e-07
71271,286810,0,286810,14082.440248012543,9.607674601155528e-07
71371,287210,0,287210,14094.670219898224,9.503172500976728e-07
71471,287610,0,287610,14106.438518047333,9.404897529081387e-07
71572,288014,0,288014,14119.649853944778,9.311205670874974e-07
71672,288414,0,288414,14132.96973490715,9.220211514355736e-07
71772,288814,0,288814,14145.083048820496,9.126129770836336e-07
71872,289214,0,289214,14158.40751695633,9.032076703395716e-07
71972,289614,0,289614,14170.334521770477,8.942279281489675e-07
72072,290015,0,290015,14182.575288057327,8.87471195931216e-07
72172,290515,0,290515,14194.954794883728,8.773176528154345e-07
72272,290947,0,290947,14208.546563863754,8.655670815112437e-07
72372,291428,0,291428,14222.928004741669,8.549343884997848e-07
72472,291849,0,291849,14235.797130823135,8.479533777361922e-07
72573,292253,0,292253,14252.268322706223,8.418179992999328e-07
72673,292698,0,292698,14265.629841804504,8.350570126896555e-07
72773,293117,0,293117,14280.819965839386,8.242434816989671e-07
72873,293514,0,293514,14295.005631923676,8.139683184143849e-07
72973,293914,0,293914,14309.32589006424,8.045617516330923e-07
73073,294314,0,294314,14323.935647964478,7.952322657820172e-07
73173,294714,0,294714,14338.203241825104,7.858214065760654e-07
73273,295114,0,295114,14352.457570075989,7.767373945643967e-07
73373,295514,0,295514,14368.482233762741,7.678185060952507e-07
73473,295914,0,295914,14383.405756950378,7.594382372447948e-07
73574,296318,0,296318,14397.946604013443,7.514702004921488e-07
73674,296718,0,296718,14412.02955698967,7.437714201643554e-07
73774,297138,0,297138,14426.891326904297,7.353525296978136e-07
73874,297541,0,297541,14441.375842809677,7.263531540251491e-07
73974,297969,0,297969,14457.22301697731,7.191228186840203e-07
74074,298369,0,298369,14475.915849924088,7.120889985653659e-07
74174,298769,0,298769,14494.93766093254,7.0553340125369e-07
74274,299169,0,299169,14513.349521875381,7.007026550264617e-07
74374,299624,0,299624,14527.48746085167,6.939705682312843e-07
74474,300031,0,300031,14543.621475696564,6.855232692009365e-07
74575,300435,0,300435,14558.459505796432,6.774329822591194e-07
74675,300837,0,300837,14573.223762750626,6.697861440130672e-07
74775,301237,0,301237,14588.678036928177,6.629175666633251e-07
74875,301637,0,301637,14608.348542928696,6.558758916042579e-07
74975,302041,0,302041,14630.481372833252,6.498660706007343e-07
75075,302462,0,302462,14651.259255886078,6.417244851779826e-07
75175,302862,0,302862,14670.681910037994,6.346398648875173e-07
75275,303262,0,303262,14693.138034820557,6.273273656076201e-07
75375,303662,0,303662,14706.855571985245,6.194985338664273e-07
75475,304064,0,304064,14719.816530942917,6.13419376632122e-07
75576,304496,0,304496,14732.505197763443,6.075625611295174e-07
75676,304901,0,304901,14745.017341852188,6.002225062382942e-07
75776,305301,0,305301,14757.829218626022,5.934851523102857e-07
75876,305701,0,305701,14774.6754758358,5.867866997059162e-07
75976,306101,0,306101,14790.541660785675,5.800908044501054e-07
76076,306501,0,306501,14807.441243886948,5.73919536913779e-07
76176,306950,0,306950,14823.933819770813,5.678116931486469e-07
76276,307434,0,307434,14840.250585794449,5.612638310598383e-07
76376,307865,0,307865,14857.061288833618,5.560733937588856e-07
76476,308265,0,308265,14873.82907485962,5.501119444480241e-07
76577,308669,0,308669,14890.514155864716,5.442978147499882e-07
76677,309069,0,309069,14906.996808767319,5.402596204110269e-07
76777,309518,0,309518,14924.000007867813,5.346879130915806e-07
76877,309926,0,309926,14940.519862890244,5.278699462468655e-07
76977,310326,0,310326,14957.031074047089,5.218951092492117e-07
77077,310726,0,310726,14973.550788879395,5.158469368598607e-07
77177,311130,0,311130,14990.335552930832,5.088374433608189e-07
77277,311541,0,311541,15006.907369852066,5.035118510622414e-07
77377,311945,0,311945,15023.258351802826,4.977021864274098e-07
77477,312345,0,312345,15039.512373924255,4.916639482090588e-07
77578,312749,0,312749,15056.167650699615,4.854509161007306e-07
77678,313149,0,313149,15072.95151591301,4.797117836780916e-07
77778,313549,0,313549,15088.963807821274,4.7428393513668223e-07
77878,313957,0,313957,15105.553271055222,4.6897264606878285e-07
77978,314357,0,314357,15122.103750944138,4.6413865153820304e-07
78078,314770,0,314770,15138.665925741196,4.5914903812422647e-07
78178,315170,0,315170,15154.932953834534,4.5414992110568997e-07
78278,315570,0,315570,15171.452276945114,4.4943835264549854e-07
78378,315988,0,315988,15187.96973991394,4.4499629192246506e-07
78478,316407,0,316407,15204.842444896698,4.3949225538393664e-07
78579,316878,0,316878,15221.982729911804,4.345183240074859e-07
78679,317282,0,317282,15239.508748054504,4.303521129268585e-07
78779,317683,0,317683,15256.003060817719,4.2574616101850916e-07
78879,318083,0,318083,15273.175028800964,4.21505218328016e-07
78979,318483,0,318483,15289.970846891403,4.173612784536854e-07
79079,318892,0,318892,15307.035054683685,4.1443764543620156e-07
79179,319337,0,319337,15323.880649805069,4.094211563940876e-07
79279,319739,0,319739,15340.597425937653,4.038078363650969e-07
79379,320182,0,320182,15357.499654769897,3.9902838209812533e-07
79479,320664,0,320664,15374.752733945847,3.9448349885476335e-07
79580,321102,0,321102,15392.51977968216,3.891285586136519e-07
79680,321507,0,321507,15410.16709971428,3.84089359355555e-07
79780,321907,0,321907,15426.948192834854,3.797560853945233e-07
79880,322307,0,322307,15443.900880813599,3.756121146322568e-07
79980,322707,0,322707,15460.600098848343,3.715657574812282e-07
80080,323107,0,323107,15477.9101998806,3.6767188433199283e-07
80180,323507,0,323507,15494.746936798096,3.6392048599851405e-07
80280,323907,0,323907,15511.463689804077,3.602224026294866e-07
80380,324307,0,324307,15528.675112962723,3.564930832136617e-07
80480,324707,0,324707,15545.68844795227,3.528303165499225e-07
80581,325111,0,325111,15563.515948057175,3.4924023064370487e-07
80681,325524,0,325524,15580.531557798386,3.4636115532735223e-07
80781,325954,0,325954,15597.711624860764,3.422439203479064e-07
80881,326354,0,326354,15614.396297931671,3.3789223370687146e-07
80981,326763,0,326763,15630.945016860962,3.335605072101008e-07
81081,327201,0,327201,15647.489248991013,3.3075578551367555e-07
81181,327601,0,327601,15664.085426807404,3.2838897827818514e-07
81281,328019,0,328019,15681.095537900925,3.2608050332692496e-07
81381,328439,0,328439,15697.12857580185,3.2189219070497296e-07
81481,328839,0,328839,15713.816102743149,3.1807258685682894e-07
81582,329243,0,329243,15730.892192840576,3.14409486510509e-07
81682,329643,0,329643,15747.568557739258,3.1066246421252924e-07
81782,330051,0,330051,15764.288004875183,3.074906172809023e-07
81882,330451,0,330451,15780.870626688004,3.04441798144283e-07
81982,330855,0,330855,15797.601193904877,3.0202495326455546e-07
82082,331279,0,331279,15814.234801769257,2.9846763208428665e-07
82182,331676,0,331676,15831.199179887772,2.94995138107707e-07
82282,332076,0,332076,15848.009873867035,2.918066030655304e-07
82382,332476,0,332476,15864.786816835403,2.8876057885118127e-07
82482,332882,0,332882,15881.775674819946,2.860998905169654e-07
82583,333298,0,333298,15898.745918989182,2.827582593916247e-07
82683,333699,0,333699,15915.604249715805,2.7977353284147384e-07
82783,334099,0,334099,15932.408201932907,2.765792351863162e-07
82883,334499,0,334499,15949.421532869339,2.7360545274271834e-07
82983,334899,0,334899,15966.025629758835,2.7054016602564795e-07
83083,335299,0,335299,15982.772310972214,2.6798631277379294e-07
83183,335757,0,335757,15999.643648862839,2.6523193443771547e-07
83283,336250,0,336250,16016.479781866074,2.621573813908726e-07
83383,336745,0,336745,16033.590453863144,2.590850120427256e-07
83483,337241,0,337241,16050.816306829453,2.562374233320243e-07
83584,337736,0,337736,16068.222395896912,2.53458372030281e-07
83684,338215,0,338215,16085.04884505272,2.506637856501577e-07
83784,338696,0,338696,16101.972738742828,2.4784400479645475e-07
83884,339097,0,339097,16118.709660768509,2.448674848434284e-07
83984,339525,0,339525,16135.287276029587,2.418252576458208e-07
84084,339925,0,339925,16151.915331840515,2.3867454824098213e-07
84184,340325,0,340325,16169.202194929123,2.359511116835448e-07
84284,340734,0,340734,16185.988778829575,2.3328835527590855e-07
84384,341134,0,341134,16202.230846881866,2.3076378069014194e-07
84484,341534,0,341534,16218.659557819366,2.2837747000064633e-07
84585,341938,0,341938,16236.057975053787,2.2591220803122445e-07
84685,342377,0,342377,16252.586108922958,2.2396951318741884e-07
84785,342877,0,342877,16267.785552740097,2.2149524486498983e-07
84885,343380,0,343380,16284.205383777618,2.1899449686308108e-07
84985,343832,0,343832,16300.064196825027,2.1713427169819043e-07
85085,344248,0,344248,16316.123724937439,2.154409562675113e-07
85185,344706,0,344706,16332.763937950134,2.1353890787340823e-07
85285,345200,0,345200,16349.411043643951,2.1114031245006489e-07
85385,345640,0,345640,16366.239155769348,2.0874209721395754e-07
85485,346040,0,346040,16383.222201824188,2.0637902316607376e-07
85586,346444,0,346444,16400.042165994644,2.046094066943201e-07
85686,346859,0,346859,16416.112982034683,2.028735283106159e-07
85786,347264,0,347264,16432.788405895233,2.0103497378850287e-07
85886,347664,0,347664,16449.090122938156,1.9961059726473524e-07
85986,348086,0,348086,16466.05198574066,1.9806146225771726e-07
86086,348505,0,348505,16482.262558937073,1.9561544431576993e-07
86186,348905,0,348905,16499.094829797745,1.930673473588112e-07
86286,349305,0,349305,16516.336216688156,1.9083836136289953e-07
86386,349709,0,349709,16534.15461587906,1.8873195617643762e-07
86486,350109,0,350109,16551.135371923447,1.8710201358036535e-07
86587,350519,0,350519,16568.91496706009,1.8539982823435127e-07
86687,350919,0,350919,16586.203938007355,1.8326534947126e-07
86787,351319,0,351319,16603.823423862457,1.8118767333990246e-07
86887,351719,0,351719,16620.884287834167,1.7917378827190804e-07
86987,352119,0,352119,16638.07405781746,1.7732601758255137e-07
87087,352519,0,352519,16655.144119024277,1.7538805637834614e-07
87187,352985,0,352985,16672.50740671158,1.737603785673645e-07
87287,353440,0,353440,16689.468461036682,1.7221584895567955e-07
87387,353863,0,353863,16706.5229036808,1.707209838437113e-07
87487,354263,0,354263,16723.08661198616,1.6902631863167814e-07
87588,354667,0,354667,16740.323824882507,1.6728170094151757e-07
87688,355067,0,355067,16757.690091848373,1.657573651539669e-07
87788,355514,0,355514,16776.09467983246,1.6427934822956142e-07
87888,355945,0,355945,16793.92746067047,1.627308768062199e-07
87988,356351,0,356351,16811.043840885162,1.6110324294089615e-07
88088,356751,0,356751,16828.059235811234,1.5924636943165983e-07
88188,357151,0,357151,16845.4700217247,1.5731866937904354e-07
88288,357568,0,357568,16862.34520292282,1.5539723384327008e-07
88388,357971,0,357971,16880.007618665695,1.5398715530114612e-07
88488,358371,0,358371,16898.052629947662,1.5217727109014406e-07
88589,358775,0,358775,16915.517234802246,1.5038642783770023e-07
88689,359175,0,359175,16932.700761795044,1.4863392079053175e-07
88789,359575,0,359575,16949.62714290619,1.4709615472948048e-07
88889,359977,0,359977,16966.819042682648,1.455396173100678e-07
88989,360382,0,360382,16984.018115758896,1.439819304890888e-07
89089,360787,0,360787,17001.55196595192,1.4228767331729662e-07
89189,361187,0,361187,17019.219342708588,1.4066312597793106e-07
89289,361587,0,361587,17036.408198833466,1.3916439167062391e-07
89389,361987,0,361987,17054.144582748413,1.379253727489247e-07
89489,362387,0,362387,17071.531824827194,1.368161311848869e-07
89590,362804,0,362804,17088.654189825058,1.353605519336311e-07
89690,363256,0,363256,17105.430329799652,1.3387712132779978e-07
89790,363701,0,363701,17123.17912697792,1.327709024862888e-07
89890,364114,0,364114,17140.46694779396,1.3150209759042126e-07
89990,364532,0,364532,17157.56935596466,1.3032675377304123e-07
90090,364934,0,364934,17174.648664712906,1.29400077243808e-07
90190,365334,0,365334,17192.081341981888,1.279356217571168e-07
90290,365748,0,365748,17209.251225709915,1.2707389063520447e-07
90390,366181,0,366181,17226.056595802307,1.259065728011688e-07
90490,366581,0,366581,17242.819936037064,1.2493621866819186e-07
90591,367002,0,367002,17261.044704914093,1.2399903018416328e-07
90691,367433,0,367433,17278.481316804886,1.2326620963531135e-07
90791,367833,0,367833,17295.92996096611,1.2243363673608862e-07
90891,368238,0,368238,17312.655117750168,1.2102962702048405e-07
90991,368640,0,368640,17329.281161785126,1.1976138359055542e-07
91091,369041,0,369041,17345.455058813095,1.1822056662051088e-07
91191,369443,0,369443,17361.95388174057,1.1689271676808044e-07
91291,369861,0,369861,17379.132032871246,1.1537227964015238e-07
91391,370264,0,370264,17396.153426885605,1.1392061361549021e-07
91491,370684,0,370684,17412.776926994324,1.1264337098703756e-07
91592,371108,0,371108,17429.691930770874,1.1149437938877706e-07
91692,371535,0,371535,17446.73506784439,1.1039117110305343e-07
91792,371944,0,371944,17463.094883680344,1.0890570621879834e-07
91892,372344,0,372344,17479.03117275238,1.0729389654525857e-07
91992,372744,0,372744,17496.186893701553,1.05738724185194e-07
92092,373144,0,373144,17512.594274044037,1.0456754405039415e-07
92192,373544,0,373544,17529.171110868454,1.028736637099955e-07
92292,373960,0,373960,17546.419762849808,1.0163406373658878e-07
92392,374360,0,374360,17564.352607011795,1.0030289196989211e-07
92492,374760,0,374760,17582.7334856987,9.897487515309336e-08
92593,375164,0,375164,17599.372788906097,9.783715943127147e-08
92693,375564,0,375564,17617.12578368187,9.667751589724215e-08
92793,375966,0,375966,17634.536660909653,9.560029585819874e-08
92893,376371,0,376371,17651.800632715225,9.455122189411496e-08
92993,376771,0,376771,17668.337813854218,9.337249570503426e-08
93093,377171,0,377171,17681.81037592888,9.22761964931805e-08
93193,377571,0,377571,17695.392057657242,9.122577444106852e-08
93293,377971,0,377971,17708.77663588524,9.020938987365484e-08
93393,378384,0,378384,17722.003447055817,8.920535041894006e-08
93493,378788,0,378788,17735.109533786774,8.831238772031648e-08
93594,379194,0,379194,17748.75566482544,8.73212530230848e-08
93694,379594,0,379594,17762.190478801727,8.637855423286896e-08
93794,379994,0,379994,17775.79851269722,8.536823367375284e-08
93894,380394,0,380394,17789.278181791306,8.436178907311676e-08
93994,380794,0,380794,17805.15885591507,8.340601180925517e-08
94094,381194,0,381194,17821.749264717102,8.231095117754788e-08
94194,381615,0,381615,17835.33438181877,8.105766452754393e-08
94294,382113,0,382113,17848.44676876068,8.013904983480435e-08
94394,382601,0,382601,17861.709520816803,7.93252911613184e-08
94494,383004,0,383004,17875.14972281456,7.875180334942952e-08
94595,383408,0,383408,17888.945774793625,7.826334029299435e-08
94695,383840,0,383840,17902.4111058712,7.775483079943193e-08
94795,384280,0,384280,17916.2815618515,7.679651502061278e-08
94895,384694,0,384694,17929.83689069748,7.596205631416066e-08
94995,385126,0,385126,17943.207675933838,7.546981869082434e-08
95095,385526,0,385526,17956.707291841507,7.472680046823974e-08
95195,385926,0,385926,17969.968990802765,7.388964166495848e-08
95295,386406,0,386406,17985.697425842285,7.307055152554242e-08
95395,386817,0,386817,17996.419474840164,7.201780177284061e-08
95495,387220,0,387220,18007.262611865997,7.102241643398086e-08
95596,387624,0,387624,18018.515835762024,7.035566402068843e-08
95696,388024,0,388024,18031.36367583275,6.978037938714585e-08
95796,388432,0,388432,18043.81618285179,6.933841058515675e-08
95896,388856,0,388856,18057.566844940186,6.876210875288444e-08
95996,389256,0,389256,18068.235913991928,6.810695865575518e-08
96096,389656,0,389656,18079.848688840866,6.753140383169205e-08
96196,390056,0,390056,18092.22718477249,6.70249430207126e-08
96296,390500,0,390500,18105.638551712036,6.639047896165022e-08
96396,390905,0,390905,18116.820812940598,6.585455484940558e-08
96496,391305,0,391305,18128.1346449852,6.515855170302506e-08
96597,391709,0,391709,18146.03696680069,6.464788551669323e-08
96697,392109,0,392109,18161.011561870575,6.417162443421299e-08
96797,392535,0,392535,18174.816218852997,6.354100933537149e-08
96897,392935,0,392935,18188.594550848007,6.286098475133281e-08
96997,393335,0,393335,18202.861769914627,6.206026187324512e-08
97097,393735,0,393735,18216.9926776886,6.133779357180541e-08
97197,394135,0,394135,18229.39980006218,6.060462598415631e-08
97297,394535,0,394535,18245.975040912628,5.975711297133548e-08
97397,394995,0,394995,18258.029283761978,5.912935533763928e-08
97497,395395,0,395395,18269.730046987534,5.840521111852311e-08
97598,395799,0,395799,18281.18526005745,5.7663745639994564e-08
97698,396199,0,396199,18292.800553798676,5.696699191693378e-08
97798,396599,0,396599,18304.58425593376,5.6319752510952725e-08
97898,396999,0,396999,18316.264544010162,5.5671567286123847e-08
97998,397399,0,397399,18329.473797798157,5.501351813452079e-08
98098,397799,0,397799,18343.167600870132,5.456995590938496e-08
98198,398199,0,398199,18359.76096892357,5.420247371377915e-08
98298,398599,0,398599,18372.703540802002,5.348344135530575e-08
98398,398999,0,398999,18385.13614487648,5.274857482142117e-08
98498,399399,0,399399,18397.37694168091,5.217998129385823e-08
98599,399803,0,399803,18409.859637975693,5.171315126473708e-08
98699,400280,0,400280,18421.979474782944,5.109606705686943e-08
98799,400690,0,400690,18433.848405838013,5.036346200305783e-08
98899,401175,0,401175,18445.617862939835,4.973823201808809e-08
98999,401635,0,401635,18457.574733018875,4.916140360743018e-08
99099,402070,0,402070,18469.481784820557,4.8682400601033e-08
99199,402492,0,402492,18481.356375694275,4.803456827132368e-08
99299,402892,0,402892,18493.98102402687,4.7317108423285936e-08
99399,403292,0,403292,18507.821284770966,4.663701697501625e-08
99499,403692,0,403692,18519.195009946823,4.6120049341829064e-08
99600,404100,0,404100,18532.40629673004,4.547682688458229e-08
99700,404500,0,404500,18543.96808075905,4.489454433830025e-08
99800,404903,0,404903,18557.293793916702,4.4330824546781934e-08
99900,405325,0,405325,18568.5245718956,4.3876470418214795e-08
100000,405740,0,405740,18579.303149700165,4.342412912807868e-08


==> extragradient/plots/Cournot_Nash.tex <==
\begin{figure}[t]
    \centering
    
    %-----------------------------------
    % Subfigure #1
    %-----------------------------------
    \begin{subfigure}[c]{0.49\textwidth}
        \centering
        \caption{\(n=10\) }
        \label{fig:nash:10}
        \begin{tikzpicture}
            \begin{semilogyaxis}[
                width=\textwidth,
                height=0.8\textwidth, % Adjust as needed
                xlabel={Number of operator evaluations},
                ylabel={\(\norm{r^{k}}\)},
                y label style={rotate=-90},
                legend to name=commonLegend,
                legend style={
                    legend columns=6,
                    cells={anchor=west},
                    font=\tiny,
                },
                grid=both,
                grid style={dashed, gray!30},
                ticklabel style={font=\tiny},
                label style={font=\tiny},
                xmin=0,
                xmax=1400,
                ymin=10^(-10),
            ]
            % EG
            \addplot+[
                color=color1,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n10/eg.tex};
            \addlegendentry{\algnamefont EG}

            % GRAAL
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n10/graal.tex};
            \addlegendentry{\algnamefont GRAAL}
            
            % aGRAAL
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n10/agraal.tex};
            \addlegendentry{\algnamefont aGRAAL}

            % EG-AA
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n10/eg-aa.tex};
            \addlegendentry{\algnamefont EG-AA}
            
            % ProxFLEX: AA-I
            \addplot+[
                color=color8,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n10/proxflex-aai.tex};
            \addlegendentry{\algnamefont \ProxFLEX: AA-I}

            % ProxFLEX: AA-II
            \addplot+[
                color=color10,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n10/proxflex-aaii.tex};
            \addlegendentry{\algnamefont \ProxFLEX: AA-II}
            
            \end{semilogyaxis}
        \end{tikzpicture}
    \end{subfigure}
    \hfill
    %-----------------------------------
    % Subfigure #2
    %-----------------------------------
    \begin{subfigure}[c]{0.49\textwidth}
        \centering
        \caption{\(n=100\)}
        \label{fig:nash:100}
        \begin{tikzpicture}
            \begin{semilogyaxis}[
                width=\textwidth,
                height=0.8\textwidth,
                xlabel={Number of operator evaluations},
                %ylabel={\(\norm{r^{k}}\)},
                %y label style={rotate=-90},
                legend to name=commonLegend,
                legend style={
                    legend columns=6,
                    cells={anchor=west},
                    font=\tiny,
                },
                grid=both,
                grid style={dashed, gray!30},
                ticklabel style={font=\tiny},
                label style={font=\tiny},
                xmin=0,
                xmax=4000,
                ymin=10^(-10),
            ]
            % EG
            \addplot+[
                color=color1,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n100/eg.tex};
            \addlegendentry{\algnamefont EG}

            % GRAAL
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n100/graal.tex};
            \addlegendentry{\algnamefont GRAAL}
            
            % aGRAAL
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n100/agraal.tex};
            \addlegendentry{\algnamefont aGRAAL}

            % EG-AA
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n100/eg-aa.tex};
            \addlegendentry{\algnamefont EG-AA}
            
            % ProxFLEX: AA-I
            \addplot+[
                color=color8,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n100/proxflex-aai.tex};
            \addlegendentry{\algnamefont \ProxFLEX: AA-I}

            % ProxFLEX: AA-II
            \addplot+[
                color=color10,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/cournot-nash_equilibrium_problem_n100/proxflex-aaii.tex};
            \addlegendentry{\algnamefont \ProxFLEX: AA-II}

            \end{semilogyaxis}
        \end{tikzpicture}
    \end{subfigure}

    %-----------------------------------
    % Place the single (common) legend below
    %-----------------------------------
    \vspace{1em}
    \centering
    \pgfplotslegendfromname{commonLegend}
    \vspace{0.5em}
    
    \caption{Convergence of algorithms on the Cournot–Nash equilibrium problem where \(r^{k} = R_{1/2L_F}(z^k)\) and \(R\) is the residual mapping in~\eqref{eq:direction:Rgam}. Both {\algnamefont AA-I} and {\algnamefont AA-II} use memory parameter \(m=3\). The number of operator evaluations equals the number of \(F\) and \(\prox_{\gamma g}\) evaluations.}
    \label{fig:nash}
\end{figure}


==> extragradient/plots/bilinear.tex <==
\begin{figure}[t]
    \centering
    %-----------------------------------
    % Subfigure #1
    %-----------------------------------
    \begin{subfigure}[c]{0.49\textwidth}
        \centering
        \caption{\(n=250\)}
        \label{fig:bmg:250}
        \begin{tikzpicture}
            \begin{semilogyaxis}[
                width=\textwidth,
                height=0.8\textwidth,
                xlabel={Number of operator evaluations},
                ylabel={\(\norm{r^{k}}\)},
                y label style={rotate=-90},
                legend to name=commonLegend,
                legend style={
                    legend columns=6,
                    cells={anchor=west},
                    font=\tiny,
                },
                grid=both,
                grid style={dashed, gray!30},
                ticklabel style={font=\tiny},
                label style={font=\tiny},
                xmin=0,
                xmax=4*10^5,
                ymin=10^(-10),
            ]
            % EG
            \addplot+[
                color=color1,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n250/eg.tex};
            \addlegendentry{\algnamefont EG}
    
            % GRAAL
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n250/graal.tex};
            \addlegendentry{\algnamefont GRAAL}
            
            % aGRAAL
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n250/agraal.tex};
            \addlegendentry{\algnamefont aGRAAL}
    
            % EG-AA
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,%
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n250/eg-aa.tex};
            \addlegendentry{\algnamefont EG-AA}
            
            % FLEX: AA-I
            \addplot+[
                color=color8,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n250/proxflex-aai.tex};
            \addlegendentry{\algnamefont \ProxFLEX: AA-I}
    
            % FLEX: AA-II
            \addplot+[
                color=color10,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n250/proxflex-aaii.tex};
            \addlegendentry{\algnamefont \ProxFLEX: AA-II}
            
            \end{semilogyaxis}
        \end{tikzpicture}
    \end{subfigure}
    \hfill
    %-----------------------------------
    % Subfigure #2
    %-----------------------------------
    \begin{subfigure}[c]{0.49\textwidth}
        \centering
        \caption{\(n=500\)}
        \label{fig:bmg:500}
        \begin{tikzpicture}
            \begin{semilogyaxis}[
                width=\textwidth,
                height=0.8\textwidth,
                xlabel={Number of operator evaluations},
                %ylabel={\(\norm{r^{k}}\)},
                y label style={rotate=-90},
                legend to name=commonLegend,
                legend style={
                    legend columns=6,
                    cells={anchor=west},
                    font=\tiny,
                },
                grid=both,
                grid style={dashed, gray!30},
                ticklabel style={font=\tiny},
                label style={font=\tiny},
                xmin=0,
                xmax=4*10^5,
                ymin=10^(-8),
            ]
            % EG
            \addplot+[
                color=color1,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n500/eg.tex};
            \addlegendentry{\algnamefont EG}
    
            % GRAAL
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n500/graal.tex};
            \addlegendentry{\algnamefont GRAAL}
            
            % aGRAAL
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n500/agraal.tex};
            \addlegendentry{\algnamefont aGRAAL}
    
            % EG-AA
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,%
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n500/eg-aa.tex};
            \addlegendentry{\algnamefont EG-AA}
            
            % FLEX: AA-I
            \addplot+[
                color=color8,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n500/proxflex-aai.tex};
            \addlegendentry{\algnamefont \ProxFLEX: AA-I}
    
            % FLEX: AA-II
            \addplot+[
                color=color10,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numoperatorevals,
                y=performance,
                col sep=comma,
            ] {plot_data/bilinear_matrix_game_n500/proxflex-aaii.tex};
            \addlegendentry{\algnamefont \ProxFLEX: AA-II}
            
            \end{semilogyaxis}
        \end{tikzpicture}
    \end{subfigure}

    %-----------------------------------
    % Place the single (common) legend below
    %-----------------------------------
    \vspace{1em}
    \centering
    \pgfplotslegendfromname{commonLegend}
    \vspace{0.5em}
    
    \caption{Convergence of algorithms on the bilinear zero-sum game with simplex constraints~\eqref{eq:bilinear} where \(r^{k} = R_{1/2L_F}(z^k)\) and \(R\) is the residual mapping in~\eqref{eq:direction:Rgam}. Both {\algnamefont AA-I} and {\algnamefont AA-II} use memory parameter \(m=10\) for \Cref{fig:bmg:250} and \(m=20\) for \Cref{fig:bmg:500}. The number of operator evaluations equals the number of \(F\) and \(\prox_{\gamma g}\) evaluations.}
    \label{fig:bmg}
\end{figure}

==> extragradient/plots/quadratic_minimax.tex <==
\begin{figure}[t]
    \centering
    
    %-----------------------------------
    % Subfigure  1x1
    %-----------------------------------
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \caption{\(n=500\) and \(\QuadMinMaxParam = 0\)}
        \begin{tikzpicture}
            \begin{semilogyaxis}[
                width=\textwidth,
                height=0.8\textwidth, 
                %xlabel={Number of \(F\) evaluations},
                ylabel={\(\norm{F\p{z^{k}}}\)},
                legend to name=commonLegend,
                legend style={
                    legend columns=6,        % <-- number of columns
                    cells={anchor=west},
                    font=\tiny,
                },
                grid=both,
                grid style={dashed, gray!30},
                ticklabel style={font=\tiny},
                label style={font=\tiny},
                xmin=0,
                xmax=200000,
                ymin=0.0005,
                ymax=10^(1)
            ]
            % EG
            \addplot+[
                color=color1,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha0/eg.tex};
            \addlegendentry{\algnamefont EG}

            % EAG-C
            \addplot+[
                color=color5,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha0/eag-c.tex};
            \addlegendentry{\algnamefont EAG-C}

            % GRAAL
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha0/graal.tex};
            \addlegendentry{\algnamefont GRAAL}

            % aGRAAL
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha0/agraal.tex};
            \addlegendentry{\algnamefont aGRAAL}

            % EG-AA
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha0/eg-aa.tex};
            \addlegendentry{\algnamefont EG-AA}

            % FLEX: AA-I
            \addplot+[
                color=color8,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha0/flex-aai.tex};
            \addlegendentry{\algnamefont \FLEX: AA-I}

            % FLEX: AA-II
            \addplot+[
                color=color10,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha0/flex-aaii.tex};
            \addlegendentry{\algnamefont \FLEX: AA-II}

            % FLEX: J-sym
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha0/flex-jsym.tex};
            \addlegendentry{\algnamefont \FLEX: J-sym}

            \end{semilogyaxis}
        \end{tikzpicture}
    \end{subfigure}
    \hfill
    %-----------------------------------
    % Subfigure 1 x 2 
    %-----------------------------------
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \caption{\(n=500\) and \(\QuadMinMaxParam = 0.0001\)}
        \begin{tikzpicture}
            \begin{semilogyaxis}[
                width=\textwidth,
                height=0.8\textwidth,
                %xlabel={Number of \(F\) evaluations},
                %ylabel={\(\norm{F\p{z^{k}}}\)},
                legend to name=commonLegend,
                legend style={
                    legend columns=6,
                    cells={anchor=west},
                    font=\tiny,
                },
                grid=both,
                grid style={dashed, gray!30},
                ticklabel style={font=\tiny},
                label style={font=\tiny},
                xmin=0,
                xmax=2*10^5,
                ymin=10^(-7),
                ymax=10^2,
            ]
            % EG
            \addplot+[
                color=color1,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/eg.tex};
            \addlegendentry{\algnamefont EG}

            % EAG-C
            \addplot+[
                color=color5,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/eag-c.tex};
            \addlegendentry{\algnamefont EAG-C}

            % GRAAL
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/graal.tex};
            \addlegendentry{\algnamefont GRAAL}

            % aGRAAL
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/agraal.tex};
            \addlegendentry{\algnamefont aGRAAL}

            % EG-AA
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/eg-aa.tex};
            \addlegendentry{\algnamefont EG-AA}

            % FLEX: AA-I
            \addplot+[
                color=color8,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/flex-aai.tex};
            \addlegendentry{\algnamefont \FLEX: AA-I}

            % FLEX: AA-II
            \addplot+[
                color=color10,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/flex-aaii.tex};
            \addlegendentry{\algnamefont \FLEX: AA-II}

            % FLEX: J-sym
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/flex-jsym.tex};
            \addlegendentry{\algnamefont \FLEX: J-sym}

            % IFLEX: AA-I
            \addplot+[
                color=color5,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-aai.tex};
            \addlegendentry{\algnamefont \IFLEX: AA-I}

            % IFLEX: AA-II
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-aaii.tex};
            \addlegendentry{\algnamefont \IFLEX: AA-II}

            % IFLEX: J-sym
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-jsym.tex};
            \addlegendentry{\algnamefont \IFLEX: J-sym}
            
            \end{semilogyaxis}
        \end{tikzpicture}
    \end{subfigure}

    %-----------------------------------
    % Subfigure  2x1
    %-----------------------------------
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \caption{\(n=20\) and \(\QuadMinMaxParam = 0\)}
        \begin{tikzpicture}
            \begin{semilogyaxis}[
                width=\textwidth,
                height=0.8\textwidth, 
                xlabel={Number of \(F\) evaluations},
                ylabel={\(\norm{F\p{z^{k}}}\)},
                legend to name=commonLegend,
                legend style={
                    legend columns=6,        % <-- number of columns
                    cells={anchor=west},
                    font=\tiny,
                },
                grid=both,
                grid style={dashed, gray!30},
                ticklabel style={font=\tiny},
                label style={font=\tiny},
                xmin=0,
                xmax=50000,
                ymin=10^(-8),
                ymax=10,
            ]
            % EG
            \addplot+[
                color=color1,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha0/eg.tex};
            \addlegendentry{\algnamefont EG}

            % EAG-C
            \addplot+[
                color=color5,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha0/eag-c.tex};
            \addlegendentry{\algnamefont EAG-C}

            % GRAAL
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha0/graal.tex};
            \addlegendentry{\algnamefont GRAAL}

            % aGRAAL
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha0/agraal.tex};
            \addlegendentry{\algnamefont aGRAAL}

            % EG-AA
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha0/eg-aa.tex};
            \addlegendentry{\algnamefont EG-AA}

            % FLEX: AA-I
            \addplot+[
                color=color8,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha0/flex-aai.tex};
            \addlegendentry{\algnamefont \FLEX: AA-I}

            % FLEX: AA-II
            \addplot+[
                color=color10,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha0/flex-aaii.tex};
            \addlegendentry{\algnamefont \FLEX: AA-II}

            % FLEX: J-sym
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha0/flex-jsym.tex};
            \addlegendentry{\algnamefont \FLEX: J-sym}

            \end{semilogyaxis}
        \end{tikzpicture}
    \end{subfigure}
    \hfill
    %-----------------------------------
    % Subfigure 2 x 2 
    %-----------------------------------
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \caption{\(n=20\) and \(\QuadMinMaxParam = 0.0001\)}
        \begin{tikzpicture}
            \begin{semilogyaxis}[
                width=\textwidth,
                height=0.8\textwidth,
                xlabel={Number of \(F\) evaluations},
                %ylabel={\(\norm{F\p{z^{k}}}\)},
                legend to name=commonLegend,
                legend style={
                    legend columns=6,
                    cells={anchor=west},
                    font=\tiny,
                },
                grid=both,
                grid style={dashed, gray!30},
                ticklabel style={font=\tiny},
                label style={font=\tiny},
                xmin=0,
                xmax=50000,
                ymin=10^(-8),
                ymax=10,
            ]
            % EG
            \addplot+[
                color=color1,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/eg.tex};
            \addlegendentry{\algnamefont EG}

            % EAG-C
            \addplot+[
                color=color5,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/eag-c.tex};
            \addlegendentry{\algnamefont EAG-C}

            % GRAAL
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/graal.tex};
            \addlegendentry{\algnamefont GRAAL}

            % aGRAAL
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/agraal.tex};
            \addlegendentry{\algnamefont aGRAAL}

            % EG-AA
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/eg-aa.tex};
            \addlegendentry{\algnamefont EG-AA}

            % FLEX: AA-I
            \addplot+[
                color=color8,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/flex-aai.tex};
            \addlegendentry{\algnamefont \FLEX: AA-I}

            % FLEX: AA-II
            \addplot+[
                color=color10,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/flex-aaii.tex};
            \addlegendentry{\algnamefont \FLEX: AA-II}

            % FLEX: J-sym
            \addplot+[
                color=color3,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/flex-jsym.tex};
            \addlegendentry{\algnamefont \FLEX: J-sym}

            % IFLEX: AA-I
            \addplot+[
                color=color5,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-aai.tex};
            \addlegendentry{\algnamefont \IFLEX: AA-I}

            % IFLEX: AA-II
            \addplot+[
                color=color2,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-aaii.tex};
            \addlegendentry{\algnamefont \IFLEX: AA-II}

            % IFLEX: J-sym
            \addplot+[
                color=color7,
                mark=none,
                line width=1.5pt,
                dashed,
            ] table[
                x=numFevals,
                y=performance,
                col sep=comma,
            ] {plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-jsym.tex};
            \addlegendentry{\algnamefont \IFLEX: J-sym}
            
            \end{semilogyaxis}
        \end{tikzpicture}
    \end{subfigure}


    %-----------------------------------
    % Place the single (common) legend below
    %-----------------------------------
    \vspace{1em}
    \centering
    \pgfplotslegendfromname{commonLegend}
    \vspace{0.5em}

    \caption{Convergence of algorithms on the quadratic minimax problem~\eqref{eq:quadratic_minimax}. Both {\algnamefont AA-I} and {\algnamefont AA-II} use memory parameter \(m=20\). \new{When \(\QuadMinMaxParam = 0\), the operator \(F\) in \eqref{eq:quadratic_minimax:F} is monotone; for \(\QuadMinMaxParam > 0\), it becomes strongly monotone.}}

    \label{fig:qmp}

\end{figure}


==> plot_data/bilinear_matrix_game_n250/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007281303405761719,2.0175302852282635
200,201,200,401,0.0959312915802002,0.04349679025208781
400,401,400,801,0.18608999252319336,0.01463313080366676
601,602,601,1203,0.26926732063293457,0.008383382119091624
801,802,801,1603,0.35022425651550293,0.005308128436778398
1001,1002,1001,2003,0.43725109100341797,0.003611737845149916
1201,1202,1201,2403,0.5174431800842285,0.0024998306769794553
1401,1402,1401,2803,0.5994551181793213,0.0019129109684775767
1602,1603,1602,3205,0.6778171062469482,0.001517403112843079
1802,1803,1802,3605,0.8061790466308594,0.0010801183065014036
2002,2003,2002,4005,0.8882951736450195,0.00084483215213907
2202,2203,2202,4405,0.9704623222351074,0.0006737009382688204
2402,2403,2402,4805,1.0517749786376953,0.0006006934794445092
2603,2604,2603,5207,1.1305081844329834,0.0005524341654471254
2803,2804,2803,5607,1.2131781578063965,0.0005203715067254704
3003,3004,3003,6007,1.2967259883880615,0.0004938357892155201
3203,3204,3203,6407,1.3826229572296143,0.00047381790976371306
3403,3404,3403,6807,1.4719600677490234,0.0004562055350135338
3604,3605,3604,7209,1.5571630001068115,0.0004405816327960734
3804,3805,3804,7609,1.6411750316619873,0.00042684807770256423
4004,4005,4004,8009,1.7317380905151367,0.0004144581307523731
4204,4205,4204,8409,1.8344430923461914,0.00038701197829392155
4404,4405,4404,8809,1.9236962795257568,0.0003589698467677532
4605,4606,4605,9211,2.0135202407836914,0.0003389567700187074
4805,4806,4805,9611,2.0992672443389893,0.00032438123433770473
5005,5006,5005,10011,2.18808913230896,0.00031323731496694224
5205,5206,5205,10411,2.277238130569458,0.00030312153139750776
5405,5406,5405,10811,2.365588426589966,0.0002951313295900683
5606,5607,5606,11213,2.454519033432007,0.0002868730286204068
5806,5807,5806,11613,2.5455241203308105,0.0002796332694694478
6006,6007,6006,12013,2.637850284576416,0.0002726067510085043
6206,6207,6206,12413,2.7258191108703613,0.0002662437298906885
6406,6407,6406,12813,2.817854404449463,0.0002606660196780025
6607,6608,6607,13215,2.907839059829712,0.00025464941279198096
6807,6808,6807,13615,3.000429153442383,0.0002492815683777871
7007,7008,7007,14015,3.0906150341033936,0.00024396338135374693
7207,7208,7207,14415,3.182464122772217,0.0002388132550460753
7407,7408,7407,14815,3.2756950855255127,0.0002338609486167385
7608,7609,7608,15217,3.3696093559265137,0.00022920305099681287
7808,7809,7808,15617,3.4653522968292236,0.0002245584023920893
8008,8009,8008,16017,3.554715156555176,0.00022025811900593448
8208,8209,8208,16417,3.6455612182617188,0.00021579995562336568
8408,8409,8408,16817,3.738467216491699,0.0002117638984231238
8609,8610,8609,17219,3.824047088623047,0.00020765253453355168
8809,8810,8809,17619,3.9229352474212646,0.000203800244734095
9009,9010,9009,18019,4.02763819694519,0.00020007474747131315
9209,9210,9209,18419,4.115026235580444,0.00019642733860085837
9409,9410,9409,18819,4.203932285308838,0.00019277617511714317
9610,9611,9610,19221,4.2919652462005615,0.00018910103929544058
9810,9811,9810,19621,4.380505084991455,0.00018559030195585525
10010,10011,10010,20021,4.470429182052612,0.00018217491027878736
10210,10211,10210,20421,4.5800042152404785,0.00017912284445985077
10410,10411,10410,20821,4.6981422901153564,0.0001760786239302967
10611,10612,10611,21223,4.811402082443237,0.00017298073175407749
10811,10812,10811,21623,4.920499324798584,0.00017016636966793168
11011,11012,11011,22023,5.029935121536255,0.00016737462008611416
11211,11212,11211,22423,5.132140159606934,0.00016464480556627341
11411,11412,11411,22823,5.234155178070068,0.00016197874359082196
11612,11613,11612,23225,5.338236331939697,0.00015923884347311177
11812,11813,11812,23625,5.438040256500244,0.00015662353894798823
12012,12013,12012,24025,5.539370059967041,0.00015415289946156186
12212,12213,12212,24425,5.637982368469238,0.00015162225637175758
12412,12413,12412,24825,5.7329981327056885,0.00014936172321451153
12613,12614,12613,25227,5.82281231880188,0.00014701752975775564
12813,12814,12813,25627,5.909841299057007,0.00014481711209930154
13013,13014,13013,26027,6.0059521198272705,0.00014272320071532593
13213,13214,13213,26427,6.120509386062622,0.0001405836563330132
13413,13414,13413,26827,6.210010290145874,0.00013853138183307168
13614,13615,13614,27229,6.303691148757935,0.00013641277160255833
13814,13815,13814,27629,6.3946921825408936,0.00013437125727317872
14014,14015,14014,28029,6.489281177520752,0.00013243351483812772
14214,14215,14214,28429,6.585764169692993,0.00013061002723731207
14414,14415,14414,28829,6.682311296463013,0.0001288618374643721
14615,14616,14615,29231,6.782353162765503,0.00012700312591845954
14815,14816,14815,29631,6.887568235397339,0.00012533549026164323
15015,15016,15015,30031,6.986952304840088,0.0001237316292711887
15215,15216,15215,30431,7.07727313041687,0.00012210328503496048
15415,15416,15415,30831,7.174143075942993,0.00012051037294022716
15616,15617,15616,31233,7.268860340118408,0.00011892206660066964
15816,15817,15816,31633,7.35948634147644,0.00011735141627086584
16016,16017,16016,32033,7.448448181152344,0.00011582617945084914
16216,16217,16216,32433,7.536229133605957,0.00011438478665953952
16416,16417,16416,32833,7.631782293319702,0.0001130040587119364
16617,16618,16617,33235,7.735324144363403,0.00011159045898095159
16817,16818,16817,33635,7.836766242980957,0.00011027016872333847
17017,17018,17017,34035,7.929502248764038,0.00010901316527982595
17217,17218,17217,34435,8.022398233413696,0.00010772137193150168
17417,17418,17417,34835,8.114703178405762,0.00010648026163911816
17618,17619,17618,35237,8.224632263183594,0.00010520697983787658
17818,17819,17818,35637,8.323623180389404,0.00010399621761891964
18018,18019,18018,36037,8.411773204803467,0.00010284042235574151
18218,18219,18218,36437,8.517847061157227,0.00010170143365575595
18418,18419,18418,36837,8.624557256698608,0.00010056456640249463
18619,18620,18619,37239,8.729220151901245,9.944541358835505e-05
18819,18820,18819,37639,8.836987257003784,9.839306022937163e-05
19019,19020,19019,38039,8.937278985977173,9.738862420113625e-05
19219,19220,19219,38439,9.031203269958496,9.639341303068005e-05
19419,19420,19419,38839,9.12900710105896,9.538202453546805e-05
19620,19621,19620,39241,9.27678918838501,9.4363304220243e-05
19820,19821,19820,39641,9.431886196136475,9.340180684196344e-05
20020,20021,20020,40041,9.564775228500366,9.243656539940447e-05
20220,20221,20220,40441,9.686647176742554,9.15572172742962e-05
20420,20421,20420,40841,9.809267282485962,9.065229658907348e-05
20621,20622,20621,41243,9.929938316345215,8.977120777822201e-05
20821,20822,20821,41643,10.022725105285645,8.892907706479929e-05
21021,21022,21021,42043,10.11018419265747,8.812551845793952e-05
21221,21222,21221,42443,10.196634292602539,8.730915054718582e-05
21421,21422,21421,42843,10.285643100738525,8.649798321388793e-05
21622,21623,21622,43245,10.388175249099731,8.567629477582349e-05
21822,21823,21822,43645,10.483395099639893,8.487925320532365e-05
22022,22023,22022,44045,10.570648193359375,8.40986245948514e-05
22222,22223,22222,44445,10.658637046813965,8.33526239707654e-05
22422,22423,22422,44845,10.74113416671753,8.262284079297658e-05
22623,22624,22623,45247,10.826329231262207,8.187989195743251e-05
22823,22824,22823,45647,10.909593105316162,8.119464191111391e-05
23023,23024,23023,46047,10.994264125823975,8.052384466515087e-05
23223,23224,23223,46447,11.077093124389648,7.984401896895232e-05
23423,23424,23423,46847,11.156476259231567,7.918024523915324e-05
23624,23625,23624,47249,11.239704132080078,7.84837687200331e-05
23824,23825,23824,47649,11.323280334472656,7.782481633673095e-05
24024,24025,24024,48049,11.402717351913452,7.719433726700041e-05
24224,24225,24224,48449,11.494933128356934,7.657328989244122e-05
24424,24425,24424,48849,11.57755708694458,7.594551450031627e-05
24625,24626,24625,49251,11.656225204467773,7.531904821314078e-05
24825,24826,24825,49651,11.73757529258728,7.473586971830085e-05
25025,25026,25025,50051,11.817572116851807,7.416603701640299e-05
25225,25226,25225,50451,11.899257183074951,7.359763946756605e-05
25425,25426,25425,50851,11.98238730430603,7.304486610845149e-05
25626,25627,25626,51253,12.069847106933594,7.245258116200675e-05
25826,25827,25826,51653,12.156044006347656,7.187416202223475e-05
26026,26027,26026,52053,12.236670970916748,7.133977069260418e-05
26226,26227,26226,52453,12.318674325942993,7.081460010485274e-05
26426,26427,26426,52853,12.405185222625732,7.026964256451874e-05
26627,26628,26627,53255,12.508796215057373,6.973241909225221e-05
26827,26828,26827,53655,12.598721027374268,6.923029817992534e-05
27027,27028,27027,54055,12.685818195343018,6.875023710613176e-05
27227,27228,27227,54455,12.777579069137573,6.824743391150301e-05
27427,27428,27427,54855,12.864879131317139,6.774479328299629e-05
27628,27629,27628,55257,12.95504117012024,6.724269230360465e-05
27828,27829,27828,55657,13.043668270111084,6.676429741580756e-05
28028,28029,28028,56057,13.129280090332031,6.63060719300869e-05
28228,28229,28228,56457,13.21379828453064,6.583518619066744e-05
28428,28429,28428,56857,13.30055022239685,6.537685298370303e-05
28629,28630,28629,57259,13.388512134552002,6.491668355074883e-05
28829,28830,28829,57659,13.471657276153564,6.448072388554719e-05
29029,29030,29029,58059,13.560417175292969,6.405672803483145e-05
29229,29230,29229,58459,13.646382093429565,6.361382713284362e-05
29429,29430,29429,58859,13.733050107955933,6.31888947632797e-05
29630,29631,29630,59261,13.818182229995728,6.274900507254005e-05
29830,29831,29830,59661,13.902440309524536,6.232775681204577e-05
30030,30031,30030,60061,13.996052265167236,6.191535312863151e-05
30230,30231,30230,60461,14.081595182418823,6.150523032318522e-05
30430,30431,30430,60861,14.168079137802124,6.109476700765481e-05
30631,30632,30631,61263,14.25273323059082,6.069076591888799e-05
30831,30832,30831,61663,14.33932113647461,6.031392572042342e-05
31031,31032,31031,62063,14.425340175628662,5.9924358648023766e-05
31231,31232,31231,62463,14.511688232421875,5.955666867858864e-05
31431,31432,31431,62863,14.614310264587402,5.9155968409256884e-05
31632,31633,31632,63265,14.710103034973145,5.877554694422264e-05
31832,31833,31832,63665,14.798553228378296,5.839570861606201e-05
32032,32033,32032,64065,14.887530088424683,5.803407125043927e-05
32232,32233,32232,64465,14.981438398361206,5.766553082290742e-05
32432,32433,32432,64865,15.07377004623413,5.728559856767123e-05
32633,32634,32633,65267,15.169085264205933,5.6922519498144956e-05
32833,32834,32833,65667,15.263267278671265,5.657271025306751e-05
33033,33034,33033,66067,15.349680185317993,5.6226674498752885e-05
33233,33234,33233,66467,15.442358016967773,5.5880773115064576e-05
33433,33434,33433,66867,15.530570983886719,5.552197816727787e-05
33634,33635,33634,67269,15.615693092346191,5.516561988359456e-05
33834,33835,33834,67669,15.70409607887268,5.483004777874078e-05
34034,34035,34034,68069,15.792055130004883,5.449542895384602e-05
34234,34235,34234,68469,15.878031253814697,5.414930042640301e-05
34434,34435,34434,68869,15.974096298217773,5.3813721934697497e-05
34635,34636,34635,69271,16.076503038406372,5.3480548749246844e-05
34835,34836,34835,69671,16.167524099349976,5.316271007961268e-05
35035,35036,35035,70071,16.25555920600891,5.284537795893794e-05
35235,35236,35235,70471,16.34127116203308,5.25210258070886e-05
35435,35436,35435,70871,16.443947076797485,5.219307813928155e-05
35636,35637,35636,71273,16.533640384674072,5.187487251807022e-05
35836,35837,35836,71673,16.620553970336914,5.156750595635992e-05
36036,36037,36036,72073,16.715681076049805,5.126633912635567e-05
36236,36237,36236,72473,16.819322109222412,5.0953583616013344e-05
36436,36437,36436,72873,16.905238151550293,5.06364164037916e-05
36637,36638,36637,73275,16.994919300079346,5.033224679889726e-05
36837,36838,36837,73675,17.086060047149658,5.003721734554995e-05
37037,37038,37037,74075,17.178019046783447,4.9741082168717235e-05
37237,37238,37237,74475,17.266119241714478,4.944104546404938e-05
37437,37438,37437,74875,17.352636337280273,4.9139840639682104e-05
37638,37639,37638,75277,17.440890312194824,4.885057992917566e-05
37838,37839,37838,75677,17.526872158050537,4.85575752231326e-05
38038,38039,38038,76077,17.61354923248291,4.827473332435137e-05
38238,38239,38238,76477,17.697108268737793,4.7980470467051044e-05
38438,38439,38438,76877,17.785032272338867,4.7692428596902716e-05
38639,38640,38639,77279,17.87205410003662,4.7408535184029144e-05
38839,38840,38839,77679,17.963057279586792,4.713660351074352e-05
39039,39040,39039,78079,18.04795813560486,4.686073608735103e-05
39239,39240,39239,78479,18.135825157165527,4.6582040221635385e-05
39439,39440,39439,78879,18.219581365585327,4.6300431451159644e-05
39640,39641,39640,79281,18.305496215820312,4.602805926680519e-05
39840,39841,39840,79681,18.393071174621582,4.576611665363842e-05
40040,40041,40040,80081,18.484689235687256,4.55030706163161e-05
40240,40241,40240,80481,18.569539070129395,4.5229626912537586e-05
40440,40441,40440,80881,18.655269145965576,4.495617216004105e-05
40641,40642,40641,81283,18.741225957870483,4.469361414303455e-05
40841,40842,40841,81683,18.832993030548096,4.443907725495218e-05
41041,41042,41041,82083,18.94217610359192,4.418266302272347e-05
41241,41242,41241,82483,19.031660079956055,4.3923346657347656e-05
41441,41442,41441,82883,19.119991064071655,4.3661149519129555e-05
41642,41643,41642,83285,19.205779314041138,4.340203533190099e-05
41842,41843,41842,83685,19.29512619972229,4.315515969837136e-05
42042,42043,42042,84085,19.3821382522583,4.290805443483866e-05
42242,42243,42242,84485,19.476263284683228,4.2654259017404e-05
42442,42443,42442,84885,19.5628080368042,4.240127396810882e-05
42643,42644,42643,85287,19.65214514732361,4.2158107159545125e-05
42843,42844,42843,85687,19.738636016845703,4.1918176335549746e-05
43043,43044,43043,86087,19.826378107070923,4.168443320234073e-05
43243,43244,43243,86487,19.917054414749146,4.1432271363523665e-05
43443,43444,43443,86887,20.00820827484131,4.1189617959602924e-05
43644,43645,43644,87289,20.095766067504883,4.094897669748808e-05
43844,43845,43844,87689,20.181411266326904,4.0722031790799655e-05
44044,44045,44044,88089,20.26870822906494,4.048807391286977e-05
44244,44245,44244,88489,20.353931188583374,4.024834902875708e-05
44444,44445,44444,88889,20.4399151802063,4.002200765569792e-05
44645,44646,44645,89291,20.530725240707397,3.979216703043228e-05
44845,44846,44845,89691,20.617687225341797,3.9573382357795005e-05
45045,45046,45045,90091,20.70560932159424,3.935498479010369e-05
45245,45246,45245,90491,20.79341220855713,3.911584928846526e-05
45445,45446,45445,90891,20.8846652507782,3.8885417425241024e-05
45646,45647,45646,91293,20.984723329544067,3.866250353869032e-05
45846,45847,45846,91693,21.08818221092224,3.84441429876271e-05
46046,46047,46046,92093,21.17937731742859,3.8223162140471584e-05
46246,46247,46246,92493,21.267199993133545,3.800206366730713e-05
46446,46447,46446,92893,21.35773015022278,3.777199618817935e-05
46647,46648,46647,93295,21.44730806350708,3.756278377254041e-05
46847,46848,46847,93695,21.53773522377014,3.7346762305204784e-05
47047,47048,47047,94095,21.62648916244507,3.712812633548001e-05
47247,47248,47247,94495,21.712921142578125,3.690899975869172e-05
47447,47448,47447,94895,21.8012752532959,3.669440941879532e-05
47648,47649,47648,95297,21.886057376861572,3.649059687226073e-05
47848,47849,47848,95697,21.972025156021118,3.629093444915889e-05
48048,48049,48048,96097,22.053450107574463,3.607905216132611e-05
48248,48249,48248,96497,22.133105278015137,3.5866872854294585e-05
48448,48449,48448,96897,22.212169408798218,3.566114855347171e-05
48649,48650,48649,97299,22.29220414161682,3.5464307067232614e-05
48849,48850,48849,97699,22.373934268951416,3.5260934826246345e-05
49049,49050,49049,98099,22.458714246749878,3.5058303816099254e-05
49249,49250,49249,98499,22.54260516166687,3.485677672621492e-05
49449,49450,49449,98899,22.63002109527588,3.465229051577856e-05
49650,49651,49650,99301,22.71369218826294,3.446204642760552e-05
49850,49851,49850,99701,22.797407150268555,3.426979772366392e-05
50050,50051,50050,100101,22.87967324256897,3.407187424216444e-05
50250,50251,50250,100501,22.967891216278076,3.387398383225383e-05
50450,50451,50450,100901,23.051912307739258,3.3679433436960105e-05
50651,50652,50651,101303,23.14886713027954,3.348877979673868e-05
50851,50852,50851,101703,23.241708040237427,3.3297045777433164e-05
51051,51052,51051,102103,23.324677228927612,3.310325505168251e-05
51251,51252,51251,102503,23.409648180007935,3.2908020179998376e-05
51451,51452,51451,102903,23.496121168136597,3.271969423756346e-05
51652,51653,51652,103305,23.581294059753418,3.254145881685616e-05
51852,51853,51852,103705,23.66253638267517,3.2363333636571314e-05
52052,52053,52052,104105,23.743874073028564,3.218078029110317e-05
52252,52253,52252,104505,23.82852029800415,3.199345322738687e-05
52452,52453,52452,104905,23.91178011894226,3.1808958844089716e-05
52653,52654,52653,105307,23.997891187667847,3.16296981168475e-05
52853,52854,52853,105707,24.080198287963867,3.145343828161283e-05
53053,53054,53053,106107,24.161572217941284,3.1272107881341055e-05
53253,53254,53253,106507,24.242918252944946,3.108836469116431e-05
53453,53454,53453,106907,24.322376251220703,3.0909774845599655e-05
53654,53655,53654,107309,24.407057285308838,3.073469595710666e-05
53854,53855,53854,107709,24.492629051208496,3.056027578407177e-05
54054,54055,54054,108109,24.574190139770508,3.038100894217561e-05
54254,54255,54254,108509,24.656105995178223,3.0203118740216653e-05
54454,54455,54454,108909,24.738986015319824,3.0030033428673074e-05
54655,54656,54655,109311,24.8208429813385,2.98647824054099e-05
54855,54856,54855,109711,24.903655290603638,2.9697277166727948e-05
55055,55056,55055,110111,24.992390155792236,2.952720305410415e-05
55255,55256,55255,110511,25.07669234275818,2.9356086829694833e-05
55455,55456,55455,110911,25.162471294403076,2.918587659355347e-05
55656,55657,55656,111313,25.25596809387207,2.902127739964588e-05
55856,55857,55856,111713,25.35647225379944,2.8854875181490635e-05
56056,56057,56056,112113,25.43930721282959,2.8688969036073803e-05
56256,56257,56256,112513,25.52698016166687,2.8519344336321652e-05
56456,56457,56456,112913,25.61405324935913,2.8362085893505203e-05
56657,56658,56657,113315,25.700395107269287,2.8208489059329487e-05
56857,56858,56857,113715,25.785850286483765,2.805028514924895e-05
57057,57058,57057,114115,25.86933922767639,2.789225266345393e-05
57257,57258,57257,114515,25.960916996002197,2.7730269917025014e-05
57457,57458,57457,114915,26.048280239105225,2.7576539585561855e-05
57658,57659,57658,115317,26.13961434364319,2.7422879010784986e-05
57858,57859,57858,115717,26.231770277023315,2.7270934028296223e-05
58058,58059,58058,116117,26.32039499282837,2.71116464066292e-05
58258,58259,58258,116517,26.409600019454956,2.6958623057787118e-05
58458,58459,58458,116917,26.503130197525024,2.6806296062578798e-05
58659,58660,58659,117319,26.591439247131348,2.6654732163003354e-05
58859,58860,58859,117719,26.680423259735107,2.6504644921813096e-05
59059,59060,59059,118119,26.76919412612915,2.6353382897758466e-05
59259,59260,59259,118519,26.857580184936523,2.6209521400123258e-05
59459,59460,59459,118919,26.947571992874146,2.605103973363189e-05
59660,59661,59660,119321,27.044185161590576,2.5908216042562068e-05
59860,59861,59860,119721,27.131198406219482,2.5758696896866847e-05
60060,60061,60060,120121,27.215150117874146,2.5609108228294194e-05
60260,60261,60260,120521,27.301974058151245,2.5458114950506286e-05
60460,60461,60460,120921,27.395907163619995,2.5313059922511282e-05
60661,60662,60661,121323,27.500123262405396,2.5173770542197303e-05
60861,60862,60861,121723,27.58786630630493,2.5031268591886076e-05
61061,61062,61061,122123,27.67835807800293,2.4885463431454354e-05
61261,61262,61261,122523,27.7620952129364,2.47408479227083e-05
61461,61462,61461,122923,27.847088098526,2.4605641264016896e-05
61662,61663,61662,123325,27.93605136871338,2.4468448103554395e-05
61862,61863,61862,123725,28.023831129074097,2.4330026607709257e-05
62062,62063,62062,124125,28.109291076660156,2.4184956760315136e-05
62262,62263,62262,124525,28.193724155426025,2.4047497090560827e-05
62462,62463,62462,124925,28.285835027694702,2.3909342168140502e-05
62663,62664,62663,125327,28.37330937385559,2.3777020478215538e-05
62863,62864,62863,125727,28.460122108459473,2.3642438244826853e-05
63063,63064,63063,126127,28.54674220085144,2.3510426749577215e-05
63263,63264,63263,126527,28.634721040725708,2.3373624985522568e-05
63463,63464,63463,126927,28.71939516067505,2.3241726833500494e-05
63664,63665,63664,127329,28.804619073867798,2.3110620054245152e-05
63864,63865,63864,127729,28.89165425300598,2.2978669536567172e-05
64064,64065,64064,128129,28.980464220046997,2.284442418077898e-05
64264,64265,64264,128529,29.073018312454224,2.2713707140117137e-05
64464,64465,64464,128929,29.156590223312378,2.2584849821385144e-05
64665,64666,64665,129331,29.24294137954712,2.2458991312388633e-05
64865,64866,64865,129731,29.328445196151733,2.2331154158446256e-05
65065,65066,65065,130131,29.414799213409424,2.220309375251141e-05
65265,65266,65265,130531,29.511436223983765,2.2075911381711464e-05
65465,65466,65465,130931,29.620408058166504,2.1948898272173608e-05
65666,65667,65666,131333,29.70530414581299,2.1826364675657413e-05
65866,65867,65866,131733,29.790765047073364,2.170112154996743e-05
66066,66067,66066,132133,29.876289129257202,2.15737448610592e-05
66266,66267,66266,132533,29.965140342712402,2.1449877968642182e-05
66466,66467,66466,132933,30.050936222076416,2.132837537995066e-05
66667,66668,66667,133335,30.135828971862793,2.120706404296143e-05
66867,66868,66867,133735,30.219041109085083,2.1087404115954594e-05
67067,67068,67067,134135,30.30274200439453,2.0967753027169325e-05
67267,67268,67267,134535,30.38755202293396,2.0847117874275213e-05
67467,67468,67467,134935,30.476243257522583,2.073328887901093e-05
67668,67669,67668,135337,30.562254190444946,2.0615851924748196e-05
67868,67869,67868,135737,30.64954113960266,2.049701664325926e-05
68068,68069,68068,136137,30.73502016067505,2.037283772410546e-05
68268,68269,68268,136537,30.819689989089966,2.0254139543673416e-05
68468,68469,68468,136937,30.910118341445923,2.014272231499512e-05
68669,68670,68669,137339,31.000458002090454,2.0032141631323935e-05
68869,68870,68869,137739,31.08446431159973,1.9915547674094848e-05
69069,69070,69069,138139,31.172425270080566,1.980543503806041e-05
69269,69270,69269,138539,31.256185293197632,1.9689311784544486e-05
69469,69470,69469,138939,31.344226121902466,1.957909782685141e-05
69670,69671,69670,139341,31.432355165481567,1.946957057844719e-05
69870,69871,69870,139741,31.52322220802307,1.936034205208686e-05
70070,70071,70070,140141,31.609008312225342,1.9248035024627546e-05
70270,70271,70270,140541,31.71252417564392,1.9137475047250834e-05
70470,70471,70470,140941,31.8079891204834,1.9032495567941314e-05
70671,70672,70671,141343,31.89241123199463,1.8925067225835913e-05
70871,70872,70871,141743,31.979313135147095,1.8816859701573948e-05
71071,71072,71071,142143,32.06584811210632,1.871317163277767e-05
71271,71272,71271,142543,32.150076150894165,1.8602829039216538e-05
71471,71472,71471,142943,32.23574924468994,1.849854790345044e-05
71672,71673,71672,143345,32.321300983428955,1.8393355147318334e-05
71872,71873,71872,143745,32.40733814239502,1.8288877257039196e-05
72072,72073,72072,144145,32.49301505088806,1.8182668416874208e-05
72272,72273,72272,144545,32.57851314544678,1.8078682742004895e-05
72472,72473,72472,144945,32.669490337371826,1.797781604599285e-05
72673,72674,72673,145347,32.75463318824768,1.7877559608407162e-05
72873,72874,72873,145747,32.84002113342285,1.7774621973660255e-05
73073,73074,73073,146147,32.92782020568848,1.7671610821187407e-05
73273,73274,73273,146547,33.015589237213135,1.756973935132372e-05
73473,73474,73473,146947,33.101744174957275,1.747329327111986e-05
73674,73675,73674,147349,33.190232038497925,1.7374525672091756e-05
73874,73875,73874,147749,33.27490711212158,1.7275369901994712e-05
74074,74075,74074,148149,33.3624210357666,1.717358237177867e-05
74274,74275,74274,148549,33.4491183757782,1.7077728116492744e-05
74474,74475,74474,148949,33.53477120399475,1.6984968192025977e-05
74675,74676,74675,149351,33.626697301864624,1.6888433011821516e-05
74875,74876,74875,149751,33.72048997879028,1.6789067229618358e-05
75075,75076,75075,150151,33.82384014129639,1.6694372616519443e-05
75275,75276,75275,150551,33.92210936546326,1.6599683191183772e-05
75475,75476,75475,150951,34.01589608192444,1.6507158233319994e-05
75676,75677,75676,151353,34.1069540977478,1.641388719841217e-05
75876,75877,75876,151753,34.193522214889526,1.6318430792519853e-05
76076,76077,76076,152153,34.28123211860657,1.622664920892012e-05
76276,76277,76276,152553,34.36935019493103,1.613263647306398e-05
76476,76477,76476,152953,34.45884919166565,1.6042642537678262e-05
76677,76678,76677,153355,34.54640531539917,1.595332275702541e-05
76877,76878,76877,153755,34.63629412651062,1.5861364616726558e-05
77077,77078,77077,154155,34.72506618499756,1.5771308142881872e-05
77277,77278,77277,154555,34.8109712600708,1.567945437052457e-05
77477,77478,77477,154955,34.89591908454895,1.5592383651183548e-05
77678,77679,77678,155357,34.987088203430176,1.550500368071316e-05
77878,77879,77878,155757,35.07900619506836,1.541514508955842e-05
78078,78079,78078,156157,35.169002056121826,1.532726187204755e-05
78278,78279,78278,156557,35.25713014602661,1.5239189362436148e-05
78478,78479,78478,156957,35.34570908546448,1.5155070081383821e-05
78679,78680,78679,157359,35.42943525314331,1.5068687944061798e-05
78879,78880,78879,157759,35.51671504974365,1.498359297659093e-05
79079,79080,79079,158159,35.598002195358276,1.4896729783120503e-05
79279,79280,79279,158559,35.68087029457092,1.4813475747881937e-05
79479,79480,79479,158959,35.76240420341492,1.4730560494425782e-05
79680,79681,79680,159361,35.844667196273804,1.4646996890496018e-05
79880,79881,79880,159761,35.93958806991577,1.4560002145798024e-05
80080,80081,80080,160161,36.03884816169739,1.4476186589892849e-05
80280,80281,80280,160561,36.12272310256958,1.4395097411046645e-05
80480,80481,80480,160961,36.206061124801636,1.4315172193088612e-05
80681,80682,80681,161363,36.289852142333984,1.4236856002886425e-05
80881,80882,80881,161763,36.37353825569153,1.4150203928221278e-05
81081,81082,81081,162163,36.46173810958862,1.4067153841413783e-05
81281,81282,81281,162563,36.571128129959106,1.3990612108117471e-05
81481,81482,81481,162963,36.663679122924805,1.3913492084054254e-05
81682,81683,81682,163365,36.74499320983887,1.3833593305324456e-05
81882,81883,81882,163765,36.825958251953125,1.3753436174266995e-05
82082,82083,82082,164165,36.907679080963135,1.3673504656062576e-05
82282,82283,82282,164565,36.99503827095032,1.3597546959275085e-05
82482,82483,82482,164965,37.07935905456543,1.3523344221911589e-05
82683,82684,82683,165367,37.1655490398407,1.3445790494248331e-05
82883,82884,82883,165767,37.24769115447998,1.3366168963109555e-05
83083,83084,83083,166167,37.332786321640015,1.3290207252721693e-05
83283,83284,83283,166567,37.417065382003784,1.3217145131435926e-05
83483,83484,83483,166967,37.503191232681274,1.3144771373967242e-05
83684,83685,83684,167369,37.58613038063049,1.3068561346953922e-05
83884,83885,83884,167769,37.66823410987854,1.2993877510351008e-05
84084,84085,84084,168169,37.76060223579407,1.2918538839732042e-05
84284,84285,84284,168569,37.87095808982849,1.284635403925718e-05
84484,84485,84484,168969,37.977957248687744,1.2775084182800254e-05
84685,84686,84685,169371,38.091347217559814,1.2703089080745518e-05
84885,84886,84885,169771,38.19183111190796,1.2627186356168554e-05
85085,85086,85085,170171,38.28093910217285,1.2553614886837949e-05
85285,85286,85285,170571,38.371111154556274,1.2482807758333311e-05
85485,85486,85485,170971,38.46280813217163,1.2412574522608132e-05
85686,85687,85686,171373,38.55041837692261,1.2341653257175407e-05
85886,85887,85886,171773,38.64422821998596,1.2268011364632383e-05
86086,86087,86086,172173,38.73240613937378,1.2198067277010739e-05
86286,86287,86286,172573,38.822418212890625,1.2130567663723096e-05
86486,86487,86486,172973,38.913533210754395,1.2063519989761432e-05
86687,86688,86687,173375,39.00458025932312,1.1994782350828172e-05
86887,86888,86887,173775,39.09005117416382,1.1926540938979378e-05
87087,87088,87087,174175,39.177168130874634,1.1859056114325685e-05
87287,87288,87287,174575,39.26691937446594,1.1792963164654534e-05
87487,87488,87487,174975,39.36198616027832,1.1728072346173193e-05
87688,87689,87688,175377,39.45076131820679,1.1661055000865613e-05
87888,87889,87888,175777,39.53821015357971,1.1591635581218765e-05
88088,88089,88088,176177,39.625449419021606,1.1524971141301988e-05
88288,88289,88288,176577,39.71242427825928,1.1462061148892754e-05
88488,88489,88488,176977,39.79675912857056,1.1397996884956163e-05
88689,88690,88689,177379,39.90486931800842,1.1331194879032195e-05
88889,88890,88889,177779,40.001904249191284,1.1264734713039969e-05
89089,89090,89089,178179,40.09389901161194,1.1201278905969727e-05
89289,89290,89289,178579,40.19308638572693,1.1138286682471249e-05
89489,89490,89489,178979,40.32176208496094,1.1076275055199093e-05
89690,89691,89690,179381,40.42419219017029,1.1011625595230796e-05
89890,89891,89890,179781,40.51807904243469,1.0946218733063632e-05
90090,90091,90090,180181,40.610016107559204,1.0883652978229117e-05
90290,90291,90290,180581,40.71813416481018,1.082407796913197e-05
90490,90491,90490,180981,40.81458520889282,1.0762841532907455e-05
90691,90692,90691,181383,40.90506720542908,1.069995362685662e-05
90891,90892,90891,181783,40.99842119216919,1.0637989688755233e-05
91091,91092,91091,182183,41.08807325363159,1.0576978793842233e-05
91291,91292,91291,182583,41.17828035354614,1.0519428315203072e-05
91491,91492,91491,182983,41.273818254470825,1.0460205544327225e-05
91692,91693,91692,183385,41.373125314712524,1.0399279010932019e-05
91892,91893,91892,183785,41.46453809738159,1.0338077800684421e-05
92092,92093,92092,184185,41.55148434638977,1.0279236108530647e-05
92292,92293,92292,184585,41.63846826553345,1.0222595426219058e-05
92492,92493,92492,184985,41.729570150375366,1.0165476590759664e-05
92693,92694,92693,185387,41.82087826728821,1.0106965946968143e-05
92893,92894,92893,185787,41.91093301773071,1.0047979093423436e-05
93093,93094,93093,186187,42.01155924797058,9.992029115818428e-06
93293,93294,93293,186587,42.11090421676636,9.936188686266707e-06
93493,93494,93493,186987,42.20409917831421,9.888179843250737e-06
93694,93695,93694,187389,42.29166221618652,9.822220005432028e-06
93894,93895,93894,187789,42.39812135696411,9.766523145870332e-06
94094,94095,94094,188189,42.493778228759766,9.711209007788484e-06
94294,94295,94294,188589,42.592668294906616,9.656566854886302e-06
94494,94495,94494,188989,42.69567322731018,9.601785480860508e-06
94695,94696,94695,189391,42.79308319091797,9.545181432049737e-06
94895,94896,94895,189791,42.883384227752686,9.491006241791224e-06
95095,95096,95095,190191,42.97774839401245,9.437170162256242e-06
95295,95296,95295,190591,43.07686519622803,9.385722909177113e-06
95495,95496,95495,190991,43.17552423477173,9.331982594350384e-06
95696,95697,95696,191393,43.27419710159302,9.276436018378357e-06
95896,95897,95896,191793,43.371798038482666,9.22380359591023e-06
96096,96097,96096,192193,43.46268630027771,9.173311425034029e-06
96296,96297,96296,192593,43.564003229141235,9.12304677342077e-06
96496,96497,96496,192993,43.663639068603516,9.076016934642456e-06
96697,96698,96697,193395,43.76241993904114,9.017977783387326e-06
96897,96898,96897,193795,43.85579538345337,8.964977245746173e-06
97097,97098,97097,194195,43.946585178375244,8.915509818162027e-06
97297,97298,97297,194595,44.03918528556824,8.865499485225698e-06
97497,97498,97497,194995,44.135743141174316,8.815651035134451e-06
97698,97699,97698,195397,44.22439503669739,8.763548882829001e-06
97898,97899,97898,195797,44.31154727935791,8.714078811968866e-06
98098,98099,98098,196197,44.397473096847534,8.664748059073114e-06
98298,98299,98298,196597,44.50200414657593,8.617950007077424e-06
98498,98499,98498,196997,44.602713108062744,8.569490594598892e-06
98699,98700,98699,197399,44.6940233707428,8.519496449041145e-06
98899,98900,98899,197799,44.81284022331238,8.469081446068534e-06
99099,99100,99099,198199,44.91015124320984,8.421919303452898e-06
99299,99300,99299,198599,45.0010712146759,8.375832936988574e-06
99499,99500,99499,198999,45.08664131164551,8.327289277030876e-06
99700,99701,99700,199401,45.17001438140869,8.279740604673074e-06
99900,99901,99900,199801,45.254982233047485,8.232556299703297e-06
100100,100101,100100,200201,45.33551001548767,8.187861662788702e-06
100300,100301,100300,200601,45.4224750995636,8.143090911955738e-06
100501,100502,100501,201003,45.50975012779236,8.096226425652079e-06
100701,100702,100701,201403,45.593329191207886,8.047851563498193e-06
100901,100902,100901,201803,45.67242217063904,8.001506353776e-06
101101,101102,101101,202203,45.753419160842896,7.957957067868442e-06
101301,101302,101301,202603,45.83167314529419,7.914362998011838e-06
101502,101503,101502,203005,45.91275906562805,7.868267750736862e-06
101702,101703,101702,203405,45.99980711936951,7.822778572526234e-06
101902,101903,101902,203805,46.08198928833008,7.777997477156777e-06
102102,102103,102102,204205,46.16177725791931,7.735105682221598e-06
102302,102303,102302,204605,46.242027044296265,7.69140113834208e-06
102503,102504,102503,205007,46.32365012168884,7.647265836262396e-06
102703,102704,102703,205407,46.41679835319519,7.6024128769950155e-06
102903,102904,102903,205807,46.50459027290344,7.558557999868285e-06
103103,103104,103103,206207,46.594165086746216,7.5172329858954946e-06
103303,103304,103303,206607,46.695430278778076,7.475667689075542e-06
103504,103505,103504,207009,46.777791023254395,7.433316207017866e-06
103704,103705,103704,207409,46.86339211463928,7.3904607216209005e-06
103904,103905,103904,207809,46.94918608665466,7.3487793982693055e-06
104104,104105,104104,208209,47.0341522693634,7.308695653046114e-06
104304,104305,104304,208609,47.11628532409668,7.267843087453281e-06
104505,104506,104505,209011,47.19780611991882,7.225187486675726e-06
104705,104706,104705,209411,47.28155517578125,7.1847829705377135e-06
104905,104906,104905,209811,47.360255002975464,7.1425970162026215e-06
105105,105106,105105,210211,47.440399169921875,7.102740645568939e-06
105305,105306,105305,210611,47.52539110183716,7.063664662893853e-06
105506,105507,105506,211013,47.60515522956848,7.022931594858061e-06
105706,105707,105706,211413,47.68693828582764,6.983007970698289e-06
105906,105907,105906,211813,47.76656222343445,6.942851370848088e-06
106106,106107,106106,212213,47.84989905357361,6.904054188906401e-06
106306,106307,106306,212613,47.93008732795715,6.866024858623425e-06
106507,106508,106507,213015,48.01617407798767,6.831161309195722e-06
106707,106708,106707,213415,48.09770917892456,6.786716736019232e-06
106907,106908,106907,213815,48.17917013168335,6.747085679167501e-06
107107,107108,107107,214215,48.259138107299805,6.710457176493548e-06
107307,107308,107307,214615,48.34131622314453,6.673894731775271e-06
107508,107509,107508,215017,48.423524141311646,6.634596728957456e-06
107708,107709,107708,215417,48.51013422012329,6.596333389429583e-06
107908,107909,107908,215817,48.591888189315796,6.55875567330477e-06
108108,108109,108108,216217,48.67230796813965,6.521709778577157e-06
108308,108309,108308,216617,48.768097162246704,6.48475646096923e-06
108509,108510,108509,217019,48.86126637458801,6.446957563705855e-06
108709,108710,108709,217419,48.94289422035217,6.410124675273209e-06
108909,108910,108909,217819,49.02840614318848,6.3735047949777245e-06
109109,109110,109109,218219,49.110273122787476,6.3387100395728065e-06
109309,109310,109309,218619,49.18974804878235,6.303264507839649e-06
109510,109511,109510,219021,49.27346730232239,6.26594156040476e-06
109710,109711,109710,219421,49.356210231781006,6.230114679577024e-06
109910,109911,109910,219821,49.44166707992554,6.195392964836623e-06
110110,110111,110110,220221,49.526987075805664,6.160919111543487e-06
110310,110311,110310,220621,49.612834215164185,6.126547435417245e-06
110511,110512,110511,221023,49.6968731880188,6.090908389723805e-06
110711,110712,110711,221423,49.782581090927124,6.056373075441068e-06
110911,110912,110911,221823,49.86642813682556,6.022046526245351e-06
111111,111112,111111,222223,49.953198194503784,5.989234963475322e-06
111311,111312,111311,222623,50.03725004196167,5.9546821462155175e-06
111512,111513,111512,223025,50.121598958969116,5.919971932242254e-06
111712,111713,111712,223425,50.20906329154968,5.885588224794241e-06
111912,111913,111912,223825,50.29168510437012,5.852521556349666e-06
112112,112113,112112,224225,50.37882423400879,5.819652453995612e-06
112312,112313,112312,224625,50.469651222229004,5.786986589682616e-06
112513,112514,112513,225027,50.55397129058838,5.761303188026167e-06
112713,112714,112713,225427,50.64255905151367,5.7209883144942705e-06
112913,112914,112913,225827,50.72891902923584,5.689392897735931e-06
113113,113114,113113,226227,50.827126026153564,5.658430138208078e-06
113313,113314,113313,226627,50.93534517288208,5.626163438732719e-06
113514,113515,113514,227029,51.0314781665802,5.59329222763666e-06
113714,113715,113714,227429,51.11634111404419,5.560483086520448e-06
113914,113915,113914,227829,51.207160234451294,5.529595917532374e-06
114114,114115,114114,228229,51.29783320426941,5.498878527221582e-06
114314,114315,114314,228629,51.38554120063782,5.467604774574579e-06
114515,114516,114515,229031,51.48664927482605,5.436039426810836e-06
114715,114716,114715,229431,51.57849717140198,5.404885074361433e-06
114915,114916,114915,229831,51.68083620071411,5.37465957030492e-06
115115,115116,115115,230231,51.822256326675415,5.344551722224886e-06
115315,115316,115315,230631,51.924217224121094,5.3139674276703164e-06
115516,115517,115516,231033,52.03352117538452,5.282484136343555e-06
115716,115717,115716,231433,52.12432932853699,5.252167052581579e-06
115916,115917,115916,231833,52.22235631942749,5.2225895859792976e-06
116116,116117,116116,232233,52.31183838844299,5.193619933992208e-06
116316,116317,116316,232633,52.40067410469055,5.163634391351634e-06
116517,116518,116517,233035,52.49454426765442,5.133862547879912e-06
116717,116718,116717,233435,52.586546182632446,5.104173935153621e-06
116917,116918,116917,233835,52.676539182662964,5.075048980562166e-06
117117,117118,117117,234235,52.765629291534424,5.0469882079925365e-06
117317,117318,117317,234635,52.85749316215515,5.018754647973475e-06
117518,117519,117518,235037,52.9489221572876,4.989883322961416e-06
117718,117719,117718,235437,53.052213191986084,4.960454651475315e-06
117918,117919,117918,235837,53.15244126319885,4.9333725433021495e-06
118118,118119,118118,236237,53.239437103271484,4.906215436775493e-06
118318,118319,118318,236637,53.33315300941467,4.878549755850128e-06
118519,118520,118519,237039,53.438016176223755,4.849999058121794e-06
118719,118720,118719,237439,53.53287220001221,4.8222777819013e-06
118919,118920,118919,237839,53.6273992061615,4.795527613240651e-06
119119,119120,119119,238239,53.7214732170105,4.769372596404722e-06
119319,119320,119319,238639,53.81100630760193,4.7420195749754784e-06
119520,119521,119520,239041,53.89844512939453,4.714145423391133e-06
119720,119721,119720,239441,53.993834018707275,4.68744748784577e-06
119920,119921,119920,239841,54.08727812767029,4.661452050644872e-06
120120,120121,120120,240241,54.178460359573364,4.635832608636287e-06
120320,120321,120320,240641,54.26636624336243,4.608816707570432e-06
120521,120522,120521,241043,54.35849714279175,4.582145810216974e-06
120721,120722,120721,241443,54.45196533203125,4.557121301219853e-06
120921,120922,120921,241843,54.54093813896179,4.53207321944241e-06
121121,121122,121121,242243,54.633501291275024,4.506712853053064e-06
121321,121322,121321,242643,54.73170518875122,4.480349117063416e-06
121522,121523,121522,243045,54.828819274902344,4.4554788836808854e-06
121722,121723,121722,243445,54.91991710662842,4.429815612875676e-06
121922,121923,121922,243845,55.01193809509277,4.404986312075987e-06
122122,122123,122122,244245,55.10078001022339,4.3807255256023425e-06
122322,122323,122322,244645,55.21037721633911,4.355918356725533e-06
122523,122524,122523,245047,55.30659317970276,4.330151175773273e-06
122723,122724,122723,245447,55.40895915031433,4.305382257365376e-06
122923,122924,122923,245847,55.4962272644043,4.281954035529351e-06
123123,123124,123123,246247,55.581159353256226,4.258066003107592e-06
123323,123324,123323,246647,55.671040058135986,4.234807829512278e-06
123524,123525,123524,247049,55.755115032196045,4.209306584459531e-06
123724,123725,123724,247449,55.84262228012085,4.1850994300822315e-06
123924,123925,123924,247849,55.9251503944397,4.162027353551061e-06
124124,124125,124124,248249,56.016584396362305,4.138511605945008e-06
124324,124325,124324,248649,56.10177421569824,4.1142411309897794e-06
124525,124526,124525,249051,56.18327021598816,4.090216506405872e-06
124725,124726,124725,249451,56.26347327232361,4.0672064586146996e-06
124925,124926,124925,249851,56.347331047058105,4.044312350661372e-06
125125,125126,125125,250251,56.42869305610657,4.021473262463542e-06
125325,125326,125325,250651,56.51269316673279,3.998615972002192e-06
125526,125527,125526,251053,56.597246408462524,3.974866067594163e-06
125726,125727,125726,251453,56.679646253585815,3.952386089389956e-06
125926,125927,125926,251853,56.75952625274658,3.930279568985189e-06
126126,126127,126126,252253,56.840665102005005,3.908425677116255e-06
126326,126327,126326,252653,56.92083215713501,3.8853745473425175e-06
126527,126528,126527,253055,57.01153206825256,3.862763463840644e-06
126727,126728,126727,253455,57.09730815887451,3.841000728521865e-06
126927,126928,126927,253855,57.17815828323364,3.819576216189526e-06
127127,127128,127127,254255,57.26222324371338,3.798158847496963e-06
127327,127328,127327,254655,57.361873149871826,3.7774076703632913e-06
127528,127529,127528,255057,57.44834518432617,3.75443117023806e-06
127728,127729,127728,255457,57.530511140823364,3.7329396374982485e-06
127928,127929,127928,255857,57.61095333099365,3.7123139046352756e-06
128128,128129,128128,256257,57.692867279052734,3.6913673064958397e-06
128328,128329,128328,256657,57.77237915992737,3.6703484167712795e-06
128529,128530,128529,257059,57.853761196136475,3.64871700757102e-06
128729,128730,128729,257459,57.936909198760986,3.6282191666943833e-06
128929,128930,128929,257859,58.02786922454834,3.608326582631187e-06
129129,129130,129129,258259,58.10923218727112,3.587862519135937e-06
129329,129330,129329,258659,58.188711166381836,3.567497511752732e-06
129530,129531,129530,259061,58.268033027648926,3.5463680175267706e-06
129730,129731,129730,259461,58.35261631011963,3.526806613637431e-06
129930,129931,129930,259861,58.43675112724304,3.507040998849397e-06
130130,130131,130130,260261,58.51893711090088,3.4873589432489304e-06
130330,130331,130330,260661,58.603127241134644,3.467121896273956e-06
130531,130532,130531,261063,58.68762016296387,3.4471028983850092e-06
130731,130732,130731,261463,58.768731117248535,3.4272218749924875e-06
130931,130932,130931,261863,58.849626302719116,3.408373109611838e-06
131131,131132,131131,262263,58.93136429786682,3.3888258036825796e-06
131331,131332,131331,262663,59.019240379333496,3.370022053174968e-06
131532,131533,131532,263065,59.10644721984863,3.349740448428859e-06
131732,131733,131732,263465,59.18827700614929,3.3311533741821176e-06
131932,131933,131932,263865,59.269222259521484,3.3123546732014664e-06
132132,132133,132132,264265,59.35318398475647,3.294216828231353e-06
132332,132333,132332,264665,59.45107936859131,3.2746188997900226e-06
132533,132534,132533,265067,59.544440269470215,3.2564814371836964e-06
132733,132734,132733,265467,59.6243052482605,3.2381577745146836e-06
132933,132934,132933,265867,59.70670533180237,3.2202873466823e-06
133133,133134,133133,266267,59.78807020187378,3.2020437662962715e-06
133333,133334,133333,266667,59.868343114852905,3.1833013017315015e-06
133534,133535,133534,267069,59.95253825187683,3.165538512896137e-06
133734,133735,133734,267469,60.03793931007385,3.147936966649231e-06
133934,133935,133934,267869,60.1218900680542,3.130525836772855e-06
134134,134135,134134,268269,60.20272731781006,3.1128261226792207e-06
134334,134335,134334,268669,60.2862069606781,3.094539206919594e-06
134535,134536,134535,269071,60.368030309677124,3.0764632467627773e-06
134735,134736,134735,269471,60.45102524757385,3.0591994206220575e-06
134935,134936,134935,269871,60.533467292785645,3.042267653097232e-06
135135,135136,135135,270271,60.614479303359985,3.029664901103961e-06
135335,135336,135335,270671,60.69613003730774,3.0071122277653154e-06
135536,135537,135536,271073,60.77813124656677,2.990187523948622e-06
135736,135737,135736,271473,60.859251976013184,2.9733484074857267e-06
135936,135937,135936,271873,60.94271731376648,2.9573306186851967e-06
136136,136137,136136,272273,61.03611636161804,2.9402991867878705e-06
136336,136337,136336,272673,61.12214517593384,2.9232189941024096e-06
136537,136538,136537,273075,61.20425820350647,2.9062591299551176e-06
136737,136738,136737,273475,61.28866934776306,2.8899228612593216e-06
136937,136938,136937,273875,61.37317609786987,2.8740198165689633e-06
137137,137138,137137,274275,61.457863330841064,2.857682139417256e-06
137337,137338,137337,274675,61.55189228057861,2.8414319596705668e-06
137538,137539,137538,275077,61.65402817726135,2.825357813276045e-06
137738,137739,137738,275477,61.73937940597534,2.809807840002144e-06
137938,137939,137938,275877,61.82424330711365,2.794254403054702e-06
138138,138139,138138,276277,61.90872120857239,2.7780723454245834e-06
138338,138339,138338,276677,62.000731229782104,2.7617434256517622e-06
138539,138540,138539,277079,62.087000131607056,2.745888935792973e-06
138739,138740,138739,277479,62.17082333564758,2.7306118650300285e-06
138939,138940,138939,277879,62.254353284835815,2.7152552841518053e-06
139139,139140,139139,278279,62.33811712265015,2.6995980824671166e-06
139339,139340,139339,278679,62.421884298324585,2.683903841784815e-06
139540,139541,139540,279081,62.51154017448425,2.6689224115844418e-06
139740,139741,139740,279481,62.596100091934204,2.6541026301367727e-06
139940,139941,139940,279881,62.684070348739624,2.639522105128327e-06
140140,140141,140140,280281,62.77025008201599,2.624119251892004e-06
140340,140341,140340,280681,62.855215311050415,2.6089059476600566e-06
140541,140542,140541,281083,62.94090914726257,2.593948506390809e-06
140741,140742,140741,281483,63.02745819091797,2.5793133367035224e-06
140941,140942,140941,281883,63.112969398498535,2.564484466064733e-06
141141,141142,141141,282283,63.19780707359314,2.5498298422342615e-06
141341,141342,141341,282683,63.281222343444824,2.5349893659549536e-06
141542,141543,141542,283085,63.36606526374817,2.5205360191464064e-06
141742,141743,141742,283485,63.45773005485535,2.5066106262036886e-06
141942,141943,141942,283885,63.544188261032104,2.492891297211928e-06
142142,142143,142142,284285,63.62878632545471,2.478543662518289e-06
142342,142343,142342,284685,63.73173713684082,2.4642758108044606e-06
142543,142544,142543,285087,63.82488012313843,2.4503111080130504e-06
142743,142744,142743,285487,63.91644024848938,2.436495898988028e-06
142943,142944,142943,285887,64.0080304145813,2.4231776927164623e-06
143143,143144,143143,286287,64.093985080719,2.4090391102364873e-06
143343,143344,143343,286687,64.18219327926636,2.3946855322819923e-06
143544,143545,143544,287089,64.26683211326599,2.3809877820546917e-06
143744,143745,143744,287489,64.35139107704163,2.368134433118297e-06
143944,143945,143944,287889,64.43585419654846,2.3548396166942888e-06
144144,144145,144144,288289,64.52274417877197,2.341095060031355e-06
144344,144345,144344,288689,64.6108672618866,2.3272029171049934e-06
144545,144546,144545,289091,64.71733713150024,2.313839348283859e-06
144745,144746,144745,289491,64.81882810592651,2.3012678548074625e-06
144945,144946,144945,289891,64.91929030418396,2.288486671191682e-06
145145,145146,145145,290291,65.02398729324341,2.275624022035547e-06
145345,145346,145345,290691,65.12602615356445,2.261827355641338e-06
145546,145547,145546,291093,65.22216701507568,2.24938029762909e-06
145746,145747,145746,291493,65.3068790435791,2.236829167762275e-06
145946,145947,145946,291893,65.39177322387695,2.2242327706517435e-06
146146,146147,146146,292293,65.47965908050537,2.2112506418933274e-06
146346,146347,146346,292693,65.57010006904602,2.1985453376863777e-06
146547,146548,146547,293095,65.65482020378113,2.1860274161723088e-06
146747,146748,146747,293495,65.73876023292542,2.1737610464866753e-06
146947,146948,146947,293895,65.83322525024414,2.1616262951522927e-06
147147,147148,147147,294295,65.9346091747284,2.151126929646245e-06
147347,147348,147347,294695,66.024405002594,2.137008947122713e-06
147548,147549,147548,295097,66.11118006706238,2.124881452027083e-06
147748,147749,147748,295497,66.19579124450684,2.113039070017792e-06
147948,147949,147948,295897,66.27935838699341,2.100782219713635e-06
148148,148149,148148,296297,66.36417818069458,2.088748825141724e-06
148348,148349,148348,296697,66.45030307769775,2.076502686374212e-06
148549,148550,148549,297099,66.53940415382385,2.064735336122421e-06
148749,148750,148749,297499,66.62313604354858,2.0534550687387436e-06
148949,148950,148949,297899,66.70881938934326,2.041851633126925e-06
149149,149150,149149,298299,66.79395198822021,2.030002240236783e-06
149349,149350,149349,298699,66.88272428512573,2.018232044194471e-06
149550,149551,149550,299101,66.97243118286133,2.006900430778905e-06
149750,149751,149750,299501,67.05919528007507,1.9955816065548074e-06
149950,149951,149950,299901,67.14407134056091,1.98423750763542e-06
150150,150151,150150,300301,67.22739315032959,1.972789115227807e-06
150350,150351,150350,300701,67.3109622001648,1.961795532936832e-06
150551,150552,150551,301103,67.39764523506165,1.951381433041126e-06
150751,150752,150751,301503,67.48822617530823,1.9401783392959634e-06
150951,150952,150951,301903,67.57386922836304,1.929333276496591e-06
151151,151152,151151,302303,67.65852427482605,1.9178842374624006e-06
151351,151352,151351,302703,67.7481632232666,1.9070490234917765e-06
151552,151553,151552,303105,67.83478808403015,1.896089291746204e-06
151752,151753,151752,303505,67.91557216644287,1.8856985384355935e-06
151952,151953,151952,303905,68.01843619346619,1.8749630877464356e-06
152152,152153,152152,304305,68.10704922676086,1.8641227771494844e-06
152352,152353,152352,304705,68.19049119949341,1.8532767979950097e-06
152553,152554,152553,305107,68.27241921424866,1.8426994246499879e-06
152753,152754,152753,305507,68.3529462814331,1.8322641373658785e-06
152953,152954,152953,305907,68.43296122550964,1.8219125865047145e-06
153153,153154,153153,306307,68.52345323562622,1.8116113653022025e-06
153353,153354,153353,306707,68.6076431274414,1.8008863212770262e-06
153554,153555,153554,307109,68.69192218780518,1.7909098501926035e-06
153754,153755,153754,307509,68.77533912658691,1.7811143640887083e-06
153954,153955,153954,307909,68.85911417007446,1.7706995870076275e-06
154154,154155,154154,308309,68.94375705718994,1.7602966536502565e-06
154354,154355,154354,308709,69.02685213088989,1.750393814074423e-06
154555,154556,154555,309111,69.10880422592163,1.7405935095661445e-06
154755,154756,154755,309511,69.2007691860199,1.7309545365512805e-06
154955,154956,154955,309911,69.2832441329956,1.7207723281600438e-06
155155,155156,155155,310311,69.36306405067444,1.71095335116057e-06
155355,155356,155355,310711,69.4468641281128,1.7012836024144258e-06
155556,155557,155556,311113,69.53017115592957,1.6918905935332747e-06
155756,155757,155756,311513,69.61179637908936,1.6825843005794104e-06
155956,155957,155956,311913,69.69340324401855,1.6729058890094791e-06
156156,156157,156156,312313,69.77425527572632,1.6636194524444971e-06
156356,156357,156356,312713,69.85610604286194,1.653711939253074e-06
156557,156558,156557,313115,69.94010019302368,1.6444939302208409e-06
156757,156758,156757,313515,70.02695322036743,1.6352911800215729e-06
156957,156958,156957,313915,70.12745809555054,1.6258284698317766e-06
157157,157158,157157,314315,70.21875619888306,1.618368740586243e-06
157357,157358,157357,314715,70.30283808708191,1.6067393543857386e-06
157558,157559,157558,315117,70.38761234283447,1.5977250476711676e-06
157758,157759,157758,315517,70.47188830375671,1.5888757827668538e-06
157958,157959,157958,315917,70.55356311798096,1.5795913004581145e-06
158158,158159,158158,316317,70.63537120819092,1.570608810350478e-06
158358,158359,158358,316717,70.71579122543335,1.5617110188569635e-06
158559,158560,158559,317119,70.79988408088684,1.5528794429914128e-06
158759,158760,158759,317519,70.88253021240234,1.5441675464706106e-06
158959,158960,158959,317919,70.96916818618774,1.535305644798588e-06
159159,159160,159159,318319,71.05104613304138,1.5263321360950432e-06
159359,159360,159359,318719,71.13193917274475,1.5177715565740298e-06
159560,159561,159560,319121,71.21447014808655,1.509384229492866e-06
159760,159761,159760,319521,71.29808735847473,1.5008620845155104e-06
159960,159961,159960,319921,71.38238739967346,1.492269599551294e-06
160160,160161,160160,320321,71.46986222267151,1.4834707498540984e-06
160360,160361,160360,320721,71.55293416976929,1.4749946879052687e-06
160561,160562,160561,321123,71.63887310028076,1.4669138871960282e-06
160761,160762,160761,321523,71.72281122207642,1.458729283316187e-06
160961,160962,160961,321923,71.80681419372559,1.4502849325085294e-06
161161,161162,161161,322323,71.88667011260986,1.4417152147817524e-06
161361,161362,161361,322723,71.97321820259094,1.433496262834744e-06
161562,161563,161562,323125,72.05464720726013,1.4253392282509135e-06
161762,161763,161762,323525,72.13727021217346,1.4171773543585026e-06
161962,161963,161962,323925,72.2316381931305,1.4090352163833686e-06
162162,162163,162162,324325,72.3301842212677,1.4007608036353105e-06
162362,162363,162362,324725,72.41723108291626,1.3930191069323943e-06
162563,162564,162563,325127,72.50107622146606,1.385408610647173e-06
162763,162764,162763,325527,72.58217024803162,1.3776391935560298e-06
162963,162964,162963,325927,72.6654942035675,1.3695410927058486e-06
163163,163164,163163,326327,72.74903130531311,1.361705671488435e-06
163363,163364,163363,326727,72.83518123626709,1.3541468337733352e-06
163564,163565,163564,327129,72.92025423049927,1.3466406455584843e-06
163764,163765,163764,327529,73.01315021514893,1.3396506712546759e-06
163964,163965,163964,327929,73.0967812538147,1.3310884658048107e-06
164164,164165,164164,328329,73.18311929702759,1.323705287918419e-06
164364,164365,164364,328729,73.26453232765198,1.3160237064158271e-06
164565,164566,164565,329131,73.35499334335327,1.3087070040440991e-06
164765,164766,164765,329531,73.4385621547699,1.3013563882263244e-06
164965,164966,164965,329931,73.52450513839722,1.293682160063805e-06
165165,165166,165165,330331,73.60887122154236,1.2863540017328635e-06
165365,165366,165365,330731,73.693852186203,1.2790972851853344e-06
165566,165567,165566,331133,73.7794680595398,1.2720229469069562e-06
165766,165767,165766,331533,73.86330604553223,1.2645975261853332e-06
165966,165967,165966,331933,73.9543821811676,1.2574254102904896e-06
166166,166167,166166,332333,74.03971219062805,1.2502970852412562e-06
166366,166367,166366,332733,74.12403321266174,1.243201792165125e-06
166567,166568,166567,333135,74.20994019508362,1.2362991437277558e-06
166767,166768,166767,333535,74.29239821434021,1.229181530098369e-06
166967,166968,166967,333935,74.39245319366455,1.2220104192229843e-06
167167,167168,167167,334335,74.49317717552185,1.215107685643783e-06
167367,167368,167367,334735,74.5774872303009,1.2084285586683026e-06
167568,167569,167568,335137,74.66306209564209,1.2016796159513486e-06
167768,167769,167768,335537,74.7453281879425,1.194753447166928e-06
167968,167969,167968,335937,74.83089828491211,1.1879011243063643e-06
168168,168169,168168,336337,74.9145781993866,1.1811101859234309e-06
168368,168369,168368,336737,75.00385618209839,1.1743978693841215e-06
168569,168570,168569,337139,75.09056997299194,1.1677525890106903e-06
168769,168770,168769,337539,75.17265725135803,1.1609821434926218e-06
168969,168970,168969,337939,75.25789523124695,1.1545172614384433e-06
169169,169170,169169,338339,75.34411597251892,1.1478393542035605e-06
169369,169370,169369,338739,75.4303343296051,1.1413134343205205e-06
169570,169571,169570,339141,75.51909613609314,1.1348085554437323e-06
169770,169771,169770,339541,75.60366916656494,1.1283247118979894e-06
169970,169971,169970,339941,75.68957114219666,1.1216969098350833e-06
170170,170171,170170,340341,75.77269911766052,1.1154101765609897e-06
170370,170371,170370,340741,75.8593909740448,1.1091514981415845e-06
170571,170572,170571,341143,75.95056319236755,1.1030735539157273e-06
170771,170772,170771,341543,76.04130029678345,1.0969246157260208e-06
170971,170972,170971,341943,76.13083910942078,1.0903969783507227e-06
171171,171172,171171,342343,76.22507524490356,1.084074278344191e-06
171371,171372,171371,342743,76.3136613368988,1.0781296401053813e-06
171572,171573,171572,343145,76.41091322898865,1.0721365407258387e-06
171772,171773,171772,343545,76.51547908782959,1.0660123391442508e-06
171972,171973,171972,343945,76.61334133148193,1.0597118778765552e-06
172172,172173,172172,344345,76.69817018508911,1.0537316470694623e-06
172372,172373,172372,344745,76.78634810447693,1.0479812427289459e-06
172573,172574,172573,345147,76.87309622764587,1.0420043751657023e-06
172773,172774,172773,345547,76.96471619606018,1.0359569363089506e-06
172973,172974,172973,345947,77.05447506904602,1.0300347057521302e-06
173173,173174,173173,346347,77.14677715301514,1.0240676695724767e-06
173373,173374,173373,346747,77.23544025421143,1.018367613584667e-06
173574,173575,173574,347149,77.32656121253967,1.0126565989746515e-06
173774,173775,173774,347549,77.41710019111633,1.0069378287980792e-06
173974,173975,173974,347949,77.51365399360657,1.0009584897469769e-06
174174,174175,174174,348349,77.60151505470276,9.9526863722283e-07
174374,174375,174374,348749,77.69118738174438,9.896905560489258e-07
174575,174576,174575,349151,77.7815523147583,9.841965770004544e-07
174775,174776,174775,349551,77.86895632743835,9.785847893980665e-07
174975,174976,174975,349951,77.95851922035217,9.729713271939889e-07
175175,175176,175175,350351,78.04887914657593,9.67434579833167e-07
175375,175376,175375,350751,78.14032530784607,9.621580873898784e-07
175576,175577,175576,351153,78.22319626808167,9.567406696831976e-07
175776,175777,175776,351553,78.30948209762573,9.514092090496734e-07
175976,175977,175976,351953,78.39351320266724,9.458702194952806e-07
176176,176177,176176,352353,78.48345422744751,9.404131409160448e-07
176376,176377,176376,352753,78.56807398796082,9.351040730747422e-07
176577,176578,176577,353155,78.67342615127563,9.297711726256543e-07
176777,176778,176777,353555,78.76823234558105,9.244347252873792e-07
176977,176978,176977,353955,78.85048127174377,9.189835080894896e-07
177177,177178,177177,354355,78.93354225158691,9.137048423938579e-07
177377,177378,177377,354755,79.02119517326355,9.087381221152103e-07
177578,177579,177578,355157,79.10580205917358,9.035499664885918e-07
177778,177779,177778,355557,79.18887519836426,8.988208864982556e-07
177978,177979,177978,355957,79.27180218696594,8.931433401258064e-07
178178,178179,178178,356357,79.35419917106628,8.88217220107514e-07
178378,178379,178378,356757,79.44062328338623,8.833870022013993e-07
178579,178580,178579,357159,79.52743029594421,8.783014637941094e-07
178779,178780,178779,357559,79.61257028579712,8.731778758467085e-07
178979,178980,178979,357959,79.69666814804077,8.682153073103946e-07
179179,179180,179179,358359,79.77777814865112,8.632622826504102e-07
179379,179380,179379,358759,79.85971403121948,8.585086205329206e-07
179580,179581,179580,359161,79.94281721115112,8.535715903474609e-07
179780,179781,179780,359561,80.0290641784668,8.488045755539175e-07
179980,179981,179980,359961,80.11285305023193,8.43735664859004e-07
180180,180181,180180,360361,80.19827508926392,8.390635844414143e-07
180380,180381,180380,360761,80.28178215026855,8.343654711936556e-07
180581,180582,180581,361163,80.3748049736023,8.295917085084299e-07
180781,180782,180781,361563,80.45827031135559,8.247359812657187e-07
180981,180982,180981,361963,80.5426230430603,8.199624027656454e-07
181181,181182,181181,362363,80.63252711296082,8.152774409615655e-07
181381,181382,181381,362763,80.71852707862854,8.10818265342465e-07
181582,181583,181582,363165,80.82114100456238,8.061483218654954e-07
181782,181783,181782,363565,80.90704822540283,8.014186109194501e-07
181982,181983,181982,363965,80.99162697792053,7.966942973198168e-07
182182,182183,182182,364365,81.08420825004578,7.923019482382126e-07
182382,182383,182382,364765,81.1715440750122,7.878994990193921e-07
182583,182584,182583,365167,81.25319719314575,7.833626112886265e-07
182783,182784,182783,365567,81.33611226081848,7.790971272303747e-07
182983,182984,182983,365967,81.41890406608582,7.743870722857946e-07
183183,183184,183183,366367,81.50921130180359,7.700228492843724e-07
183383,183384,183383,366767,81.59558033943176,7.656999658276006e-07
183584,183585,183584,367169,81.68667912483215,7.613295380249383e-07
183784,183785,183784,367569,81.78168320655823,7.568606673573515e-07
183984,183985,183984,367969,81.86837816238403,7.52433361813907e-07
184184,184185,184184,368369,81.9528021812439,7.482265273240532e-07
184384,184385,184384,368769,82.03949809074402,7.440239782120753e-07
184585,184586,184585,369171,82.12498617172241,7.398498631444622e-07
184785,184786,184785,369571,82.210125207901,7.35694108615847e-07
184985,184986,184985,369971,82.29050421714783,7.313266299648924e-07
185185,185186,185185,370371,82.37285304069519,7.272369133182928e-07
185385,185386,185385,370771,82.45696115493774,7.231025316213001e-07
185586,185587,185586,371173,82.54091715812683,7.190787341995408e-07
185786,185787,185786,371573,82.62648010253906,7.148656406098845e-07
185986,185987,185986,371973,82.7092490196228,7.107791952803422e-07
186186,186187,186186,372373,82.79500126838684,7.067740523380568e-07
186386,186387,186386,372773,82.88611721992493,7.028546932199119e-07
186587,186588,186587,373175,82.9913432598114,6.994423345264101e-07
186787,186788,186787,373575,83.07317018508911,6.94835256838561e-07
186987,186988,186987,373975,83.15543341636658,6.90798797463085e-07
187187,187188,187187,374375,83.23738598823547,6.868985106011215e-07
187387,187388,187387,374775,83.31937408447266,6.83150056231658e-07
187588,187589,187588,375177,83.40254521369934,6.791958547894463e-07
187788,187789,187788,375577,83.4896183013916,6.752142021811029e-07
187988,187989,187988,375977,83.57182216644287,6.712707412703946e-07
188188,188189,188188,376377,83.65272331237793,6.676213378443125e-07
188388,188389,188388,376777,83.73511719703674,6.63861842528099e-07
188589,188590,188589,377179,83.81949639320374,6.599675066056163e-07
188789,188790,188789,377579,83.90352511405945,6.561611078041058e-07
188989,188990,188989,377979,83.98798727989197,6.525168518915859e-07
189189,189190,189189,378379,84.07259631156921,6.489438035948672e-07
189389,189390,189389,378779,84.15499210357666,6.452057207741219e-07
189590,189591,189590,379181,84.23464822769165,6.414828022347998e-07
189790,189791,189790,379581,84.31692004203796,6.379218627081438e-07
189990,189991,189990,379981,84.39945030212402,6.341534624299936e-07
190190,190191,190190,380381,84.48668217658997,6.305996198821383e-07
190390,190391,190390,380781,84.5701732635498,6.270795524012682e-07
190591,190592,190591,381183,84.65944814682007,6.235004520639838e-07
190791,190792,190791,381583,84.74176216125488,6.19802914747599e-07
190991,190992,190991,381983,84.82805728912354,6.16311345231977e-07
191191,191192,191191,382383,84.91150307655334,6.12930597550132e-07
191391,191392,191391,382783,85.00691413879395,6.094311973779521e-07
191592,191593,191592,383185,85.11287331581116,6.059591644938298e-07
191792,191793,191792,383585,85.19695115089417,6.023656603796567e-07
191992,191993,191992,383985,85.28079223632812,5.989395263239582e-07
192192,192193,192192,384385,85.36564016342163,5.956833716031137e-07
192392,192393,192392,384785,85.45174407958984,5.924392465923274e-07
192593,192594,192593,385187,85.53754806518555,5.889510172922747e-07
192793,192794,192793,385587,85.62152028083801,5.855765487780605e-07
192993,192994,192993,385987,85.705313205719,5.822954106317591e-07
193193,193194,193193,386387,85.78813004493713,5.791414083868989e-07
193393,193394,193393,386787,85.87448906898499,5.759362043870781e-07
193594,193595,193594,387189,85.96216917037964,5.72539815660154e-07
193794,193795,193794,387589,86.04885125160217,5.693783562355431e-07
193994,193995,193994,387989,86.13573503494263,5.661114582370183e-07
194194,194195,194194,388389,86.22248220443726,5.630425224663886e-07
194394,194395,194394,388789,86.30280923843384,5.599084046997841e-07
194595,194596,194595,389191,86.3889410495758,5.566337895315287e-07
194795,194796,194795,389591,86.4788122177124,5.534270201112066e-07
194995,194996,194995,389991,86.56181716918945,5.503048952815871e-07
195195,195196,195195,390391,86.64605331420898,5.473687590676287e-07
195395,195396,195395,390791,86.72925329208374,5.44254787735938e-07
195596,195597,195596,391193,86.8123242855072,5.410624280695706e-07
195796,195797,195796,391593,86.89521217346191,5.379968787457807e-07
195996,195997,195996,391993,86.9868233203888,5.349279576888236e-07
196196,196197,196196,392393,87.07024931907654,5.319565892269288e-07
196396,196397,196396,392793,87.16988706588745,5.289533801549177e-07
196597,196598,196597,393195,87.27372908592224,5.258412149092268e-07
196797,196798,196797,393595,87.36277914047241,5.228466904680187e-07
196997,196998,196997,393995,87.45530605316162,5.198050756252843e-07
197197,197198,197197,394395,87.54201436042786,5.169894968839095e-07
197397,197398,197397,394795,87.63115429878235,5.14023018605938e-07
197598,197599,197598,395197,87.72147727012634,5.1098066775506e-07
197798,197799,197798,395597,87.80976819992065,5.081093523268522e-07
197998,197999,197998,395997,87.89838719367981,5.052262276137409e-07
198198,198199,198198,396397,87.98861122131348,5.024005016115388e-07
198398,198399,198398,396797,88.07749819755554,4.995611789583819e-07
198599,198600,198599,397199,88.17024111747742,4.965828284980772e-07
198799,198800,198799,397599,88.25665616989136,4.936393280495487e-07
198999,199000,198999,397999,88.34202814102173,4.909466866543911e-07
199199,199200,199199,398399,88.42644810676575,4.881870538851842e-07
199399,199400,199399,398799,88.51781725883484,4.853742564905798e-07
199600,199601,199600,399201,88.60183715820312,4.8251840039751e-07
199800,199801,199800,399601,88.6873950958252,4.797568227500172e-07
200000,200001,200000,400001,88.77694797515869,4.77107858322766e-07


==> plot_data/bilinear_matrix_game_n250/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00047588348388671875,2.0175302852282635
100,201,200,401,0.07272672653198242,0.03870059256068895
200,401,400,801,0.1674938201904297,0.0179642168274124
300,601,600,1201,0.2631378173828125,0.010215612352113134
400,801,800,1601,0.3383307456970215,0.006414884987572114
501,1003,1002,2005,0.401430606842041,0.004292887866686561
601,1203,1202,2405,0.4629027843475342,0.0031981848552840673
701,1403,1402,2805,0.5230207443237305,0.0023495755858960704
801,1603,1602,3205,0.5862510204315186,0.0017642014700653555
901,1803,1802,3605,0.6527140140533447,0.0013107140383380224
1001,2003,2002,4005,0.7124638557434082,0.0010771361342336561
1101,2203,2202,4405,0.773129940032959,0.0008891647471929582
1201,2403,2402,4805,0.8368008136749268,0.0007896238285358858
1301,2603,2602,5205,0.897061824798584,0.0007243730865874144
1401,2803,2802,5605,0.9626357555389404,0.000648621889859143
1502,3005,3004,6009,1.0246357917785645,0.000605342378155228
1602,3205,3204,6409,1.0892417430877686,0.0005733026994351765
1702,3405,3404,6809,1.1666560173034668,0.0005447368428944139
1802,3605,3604,7209,1.2288289070129395,0.00048258186702094223
1902,3805,3804,7609,1.294442892074585,0.00043623502306099424
2002,4005,4004,8009,1.3591816425323486,0.0004039543762459166
2102,4205,4204,8409,1.425360918045044,0.00037891678446560513
2202,4405,4404,8809,1.4932479858398438,0.00035856970156738626
2302,4605,4604,9209,1.5671398639678955,0.00034167885404962273
2402,4805,4804,9609,1.6504325866699219,0.000327471216222133
2503,5007,5006,10013,1.7211709022521973,0.00031528514633575623
2603,5207,5206,10413,1.7851316928863525,0.00030494059155017047
2703,5407,5406,10813,1.8479349613189697,0.0002959793336833732
2803,5607,5606,11213,1.912571907043457,0.0002881403091160926
2903,5807,5806,11613,1.9763097763061523,0.000281214281208699
3003,6007,6006,12013,2.042221784591675,0.0002750331765274161
3103,6207,6206,12413,2.113581657409668,0.00026946189858635845
3203,6407,6406,12813,2.179924964904785,0.00026439183980072673
3303,6607,6606,13213,2.2421817779541016,0.00025973566986274647
3403,6807,6806,13613,2.3085358142852783,0.000255423132572343
3504,7009,7008,14017,2.3710098266601562,0.0002513586896688166
3604,7209,7208,14417,2.4370386600494385,0.0002475768793537788
3704,7409,7408,14817,2.5008208751678467,0.00024399934675541638
3804,7609,7608,15217,2.565274715423584,0.00024059633077260883
3904,7809,7808,15617,2.629607915878296,0.00023734367502605227
4004,8009,8008,16017,2.6918137073516846,0.00023422171215643902
4104,8209,8208,16417,2.756436824798584,0.00023121437386540734
4204,8409,8408,16817,2.8209075927734375,0.00022830848122147552
4304,8609,8608,17217,2.883953809738159,0.0002254931786417318
4404,8809,8808,17617,2.9494547843933105,0.00022275948222810613
4505,9011,9010,18021,3.015483856201172,0.0002200736757568169
4605,9211,9210,18421,3.0785017013549805,0.00021748264631160484
4705,9411,9410,18821,3.148026704788208,0.00021495419299109208
4805,9611,9610,19221,3.212247848510742,0.00021248387115568304
4905,9811,9810,19621,3.2781167030334473,0.0002100678928804713
5005,10011,10010,20021,3.341017723083496,0.00020770300764981782
5105,10211,10210,20421,3.4063117504119873,0.00020538640619713179
5205,10411,10410,20821,3.469348907470703,0.0002031156428412569
5305,10611,10610,21221,3.533604860305786,0.00020088857263204926
5405,10811,10810,21621,3.6030948162078857,0.0001987033003656253
5506,11013,11012,22025,3.6710116863250732,0.00019653688483370254
5606,11213,11212,22425,3.7486836910247803,0.00019443070110695764
5706,11413,11412,22825,3.8196768760681152,0.0001923617375405541
5806,11613,11612,23225,3.8810906410217285,0.0001903287540892684
5906,11813,11812,23625,3.941903829574585,0.00018833061625778637
6006,12013,12012,24025,4.002641916275024,0.00018636627982224012
6106,12213,12212,24425,4.0656418800354,0.00018443477820151422
6206,12413,12412,24825,4.13269567489624,0.00018253521198341002
6306,12613,12612,25225,4.195744752883911,0.00018066674020936473
6406,12813,12812,25625,4.255319833755493,0.00017882857309627258
6507,13015,13014,26029,4.320741891860962,0.0001770020267232668
6607,13215,13214,26429,4.382824897766113,0.00017522255984983156
6707,13415,13414,26829,4.44559383392334,0.0001734712724405494
6807,13615,13614,27229,4.511922836303711,0.0001717475275193629
6907,13815,13814,27629,4.592723846435547,0.00017005071684054419
7007,14015,14014,28029,4.674487829208374,0.00016838025819878897
7107,14215,14214,28429,4.7548627853393555,0.00016673559311093918
7207,14415,14414,28829,4.8321616649627686,0.00016511618481099277
7307,14615,14614,29229,4.9103429317474365,0.000163521516504671
7407,14815,14814,29629,4.985045909881592,0.00016195108984464797
7508,15017,15016,30033,5.062867879867554,0.0001603890753312936
7608,15217,15216,30433,5.1423118114471436,0.0001588659348191652
7708,15417,15416,30833,5.217313766479492,0.00015736563452041881
7808,15617,15616,31233,5.288184881210327,0.00015588773806327232
7908,15817,15816,31633,5.359011888504028,0.00015443182216535014
8008,16017,16016,32033,5.428246021270752,0.0001529974758801278
8108,16217,16216,32433,5.505482912063599,0.00015158429991368803
8208,16417,16416,32833,5.577248811721802,0.00015019190600647155
8308,16617,16616,33233,5.655069828033447,0.00014881991636835176
8408,16817,16816,33633,5.72034478187561,0.00014746796316294591
8509,17019,17018,34037,5.783164978027344,0.00014612246346770548
8609,17219,17218,34437,5.862015962600708,0.00014480970865508907
8709,17419,17418,34837,5.938431978225708,0.0001435159385685191
8809,17619,17618,35237,6.001131057739258,0.00014224082088285596
8909,17819,17818,35637,6.074168682098389,0.0001409840311898774
9009,18019,18018,36037,6.145569801330566,0.00013974525267497582
9109,18219,18218,36437,6.208853006362915,0.00013852417581637554
9209,18419,18418,36837,6.2771687507629395,0.00013732049810336562
9309,18619,18618,37237,6.345607757568359,0.00013613392377165485
9409,18819,18818,37637,6.411422967910767,0.0001349641635563538
9510,19021,19020,38041,6.475384712219238,0.00013379948470752128
9610,19221,19220,38441,6.539919853210449,0.00013266267093725852
9710,19421,19420,38841,6.6088478565216064,0.0001315418375357308
9810,19621,19620,39241,6.679074764251709,0.00013043671908828831
9910,19821,19820,39641,6.750177621841431,0.00012934705563775144
10010,20021,20020,40041,6.822494983673096,0.00012827259250720958
10110,20221,20220,40441,6.901018857955933,0.0001272130801360416
10210,20421,20420,40841,6.977330923080444,0.0001261682739210451
10310,20621,20620,41241,7.046806812286377,0.00012513793406670548
10410,20821,20820,41641,7.117313623428345,0.00012412182544308851
10511,21023,21022,42045,7.181934833526611,0.00012310976630411754
10611,21223,21222,42445,7.253396987915039,0.00012212156935771686
10711,21423,21422,42845,7.322274684906006,0.00012114692271993615
10811,21623,21622,43245,7.386224746704102,0.000120185608667928
10911,21823,21822,43645,7.451824903488159,0.00011923741352364664
11011,22023,22022,44045,7.514302968978882,0.00011830212754717816
11111,22223,22222,44445,7.577594757080078,0.00011737954483300902
11211,22423,22422,44845,7.649980783462524,0.00011646946321229426
11311,22623,22622,45245,7.7232208251953125,0.00011557168415702394
11411,22823,22822,45645,7.80270791053772,0.00011468601269024659
11512,23025,23024,46049,7.872832775115967,0.00011380357928193565
11612,23225,23224,46449,7.945671796798706,0.00011294166817294914
11712,23425,23424,46849,8.025213956832886,0.00011209129834021222
11812,23625,23624,47249,8.10024881362915,0.00011125228820360766
11912,23825,23824,47649,8.164610862731934,0.00011042445932999713
12012,24025,24024,48049,8.229391813278198,0.0001096076363612358
12112,24225,24224,48449,8.295880794525146,0.00010880164694508419
12212,24425,24424,48849,8.371251821517944,0.00010800632166848759
12312,24625,24624,49249,8.445003032684326,0.00010722149399299883
12412,24825,24824,49649,8.50806975364685,0.00010644700019297531
12513,25027,25026,50053,8.574897766113281,0.00010567508692150307
12613,25227,25226,50453,8.651501655578613,0.00010492088000252017
12713,25427,25426,50853,8.729159832000732,0.00010417653052252305
12813,25627,25626,51253,8.804819822311401,0.00010344188545014195
12913,25827,25826,51653,8.875765800476074,0.00010271679428441283
13013,26027,26026,52053,8.959142923355103,0.0001020011090041051
13113,26227,26226,52453,9.0274658203125,0.00010129468401762708
13213,26427,26426,52853,9.090668678283691,0.00010059737611571367
13313,26627,26626,53253,9.155654907226562,9.990904442504029e-05
13413,26827,26826,53653,9.218154907226562,9.922955036211032e-05
13514,27029,27028,54057,9.30608081817627,9.855209314758345e-05
13614,27229,27228,54457,9.400410890579224,9.788995253410103e-05
13714,27429,27428,54857,9.498633861541748,9.723624579831776e-05
13814,27629,27628,55257,9.611552715301514,9.659084311227403e-05
13914,27829,27828,55657,9.701282739639282,9.595361673015083e-05
14014,28029,28028,56057,9.787440776824951,9.532444095068601e-05
14114,28229,28228,56457,9.876288652420044,9.470319207907087e-05
14214,28429,28428,56857,9.96551775932312,9.408974839206253e-05
14314,28629,28628,57257,10.055198907852173,9.348399010080046e-05
14414,28829,28828,57657,10.140354633331299,9.28857993179508e-05
14515,29031,29030,58061,10.21906590461731,9.228918987302865e-05
14615,29231,29230,58461,10.284523725509644,9.170586068479885e-05
14715,29431,29430,58861,10.353298902511597,9.112975530307399e-05
14815,29631,29630,59261,10.420745849609375,9.056076313423452e-05
14915,29831,29830,59661,10.487427711486816,8.99987753263165e-05
15015,30031,30030,60061,10.55381989479065,8.94436847378516e-05
15115,30231,30230,60461,10.626414775848389,8.889538590984509e-05
15215,30431,30430,60861,10.692333698272705,8.835377503693193e-05
15315,30631,30630,61261,10.760651588439941,8.78187499394078e-05
15415,30831,30830,61661,10.825255870819092,8.729021003659379e-05
15516,31033,31032,62065,10.89151382446289,8.676286670204717e-05
15616,31233,31232,62465,10.961732864379883,8.624706410975493e-05
15716,31433,31432,62865,11.02937388420105,8.57374533479452e-05
15816,31633,31632,63265,11.09963870048523,8.523393998619012e-05
15916,31833,31832,63665,11.165775775909424,8.473643106529019e-05
16016,32033,32032,64065,11.232435941696167,8.424483507322058e-05
16116,32233,32232,64465,11.299577713012695,8.375906192201825e-05
16216,32433,32432,64865,11.367831707000732,8.327902292558504e-05
16316,32633,32632,65265,11.430197715759277,8.280463077566314e-05
16416,32833,32832,65665,11.496893882751465,8.233579952114378e-05
16517,33035,33034,66069,11.560484886169434,8.186783836882488e-05
16617,33235,33234,66469,11.631219863891602,8.140992988516565e-05
16717,33435,33434,66869,11.698361873626709,8.095733155701019e-05
16817,33635,33634,67269,11.761122703552246,8.050996266081315e-05
16917,33835,33834,67669,11.822941780090332,8.006774372664463e-05
17017,34035,34034,68069,11.886918783187866,7.963059651706329e-05
17117,34235,34234,68469,11.947406768798828,7.919844400880142e-05
17217,34435,34434,68869,12.009092807769775,7.877121037323326e-05
17317,34635,34634,69269,12.068854808807373,7.834882095884943e-05
17417,34835,34834,69669,12.131845712661743,7.793120227196671e-05
17518,35037,35036,70073,12.191683769226074,7.751417624099244e-05
17618,35237,35236,70473,12.264989852905273,7.710592898752043e-05
17718,35437,35436,70873,12.341523885726929,7.670223805725681e-05
17818,35637,35636,71273,12.400407791137695,7.630303442478913e-05
17918,35837,35836,71673,12.46053671836853,7.590825013610193e-05
18018,36037,36036,72073,12.520835876464844,7.551781829324232e-05
18118,36237,36236,72473,12.58266282081604,7.513167303666393e-05
18218,36437,36436,72873,12.648432731628418,7.474974953090994e-05
18318,36637,36636,73273,12.70765495300293,7.437198394798899e-05
18418,36837,36836,73673,12.769538640975952,7.399831345240632e-05
18519,37039,37038,74077,12.831421852111816,7.362499997502704e-05
18619,37239,37238,74477,12.892984867095947,7.325937446272465e-05
18719,37439,37438,74877,12.952471733093262,7.289766074269952e-05
18819,37639,37638,75277,13.012419700622559,7.253979981131108e-05
18919,37839,37838,75677,13.072731733322144,7.2185733583804e-05
19019,38039,38038,76077,13.133089780807495,7.183540488073206e-05
19119,38239,38238,76477,13.19375491142273,7.148875741550155e-05
19219,38439,38438,76877,13.254408836364746,7.114573577934091e-05
19319,38639,38638,77277,13.314326763153076,7.080628542869801e-05
19419,38839,38838,77677,13.373690843582153,7.047035267272691e-05
19520,39041,39040,78081,13.434013843536377,7.013457729963545e-05
19620,39241,39240,78481,13.494062662124634,6.980555587168995e-05
19720,39441,39440,78881,13.557009935379028,6.947989544303976e-05
19820,39641,39640,79281,13.625906944274902,6.915754561282357e-05
19920,39841,39840,79681,13.685525894165039,6.88384567705233e-05
20020,40041,40040,80081,13.746004819869995,6.852258008345205e-05
20120,40241,40240,80481,13.80783987045288,6.820986748509168e-05
20220,40441,40440,80881,13.87239670753479,6.790027166386641e-05
20320,40641,40640,81281,13.932830810546875,6.759374605147888e-05
20420,40841,40840,81681,13.99358582496643,6.729024481193715e-05
20521,41043,41042,82085,14.0553138256073,6.698673250509319e-05
20621,41243,41242,82485,14.11851692199707,6.668917450416247e-05
20721,41443,41442,82885,14.178155660629272,6.639450721864771e-05
20821,41643,41642,83285,14.23722767829895,6.610268763956923e-05
20921,41843,41842,83685,14.296689748764038,6.581367343690462e-05
21021,42043,42042,84085,14.361608982086182,6.552742294888833e-05
21121,42243,42242,84485,14.437617778778076,6.524389517202788e-05
21221,42443,42442,84885,14.505149841308594,6.496304975121927e-05
21321,42643,42642,85285,14.565720796585083,6.468484696983597e-05
21421,42843,42842,85685,14.633960962295532,6.440924774014854e-05
21522,43045,43044,86089,14.695036888122559,6.41334960777934e-05
21622,43245,43244,86489,14.75614881515503,6.38630142401576e-05
21722,43445,43444,86889,14.817907810211182,6.359502200085604e-05
21822,43645,43644,87289,14.879477739334106,6.332948269971798e-05
21922,43845,43844,87689,14.940345764160156,6.30663602598269e-05
22022,44045,44044,88089,15.00441288948059,6.280561917716129e-05
22122,44245,44244,88489,15.064349889755249,6.254722451316279e-05
22222,44445,44444,88889,15.127297639846802,6.229114188589911e-05
22322,44645,44644,89289,15.188875675201416,6.203733746082567e-05
22422,44845,44844,89689,15.252185821533203,6.17857779432218e-05
22523,45047,45046,90093,15.317328929901123,6.15339481577865e-05
22623,45247,45246,90493,15.376502752304077,6.128680232625892e-05
22723,45447,45446,90893,15.435687780380249,6.104180435902917e-05
22823,45647,45646,91293,15.498583793640137,6.0798923043198106e-05
22923,45847,45846,91693,15.559515953063965,6.0558127666077395e-05
23023,46047,46046,92093,15.623236894607544,6.0319388005680966e-05
23123,46247,46246,92493,15.684305906295776,6.008267432479922e-05
23223,46447,46446,92893,15.744663715362549,5.984795736310033e-05
23323,46647,46646,93293,15.805034875869751,5.96152083296387e-05
23423,46847,46846,93693,15.865962982177734,5.938439889501202e-05
23524,47049,47048,94097,15.927655935287476,5.915322176959705e-05
23624,47249,47248,94497,15.987140893936157,5.892622706563186e-05
23724,47449,47448,94897,16.050443649291992,5.870108940807669e-05
23824,47649,47648,95297,16.11430287361145,5.847778225090531e-05
23924,47849,47848,95697,16.17697787284851,5.825627947499746e-05
24024,48049,48048,96097,16.23909878730774,5.803655538210418e-05
24124,48249,48248,96497,16.299139738082886,5.781858468792967e-05
24224,48449,48448,96897,16.361562728881836,5.760234251642121e-05
24324,48649,48648,97297,16.42176079750061,5.7387804392374776e-05
24424,48849,48848,97697,16.489569664001465,5.717494623594152e-05
24525,49051,49050,98101,16.568176746368408,5.696164062245334e-05
24625,49251,49250,98501,16.648170948028564,5.675208792416326e-05
24725,49451,49450,98901,16.709577798843384,5.6544145035742415e-05
24825,49651,49650,99301,16.771440744400024,5.633778939997808e-05
24925,49851,49850,99701,16.834394693374634,5.613299882503801e-05
25025,50051,50050,100101,16.895659685134888,5.592975147842594e-05
25125,50251,50250,100501,16.956289768218994,5.5728025881110405e-05
25225,50451,50450,100901,17.020992040634155,5.552780090197602e-05
25325,50651,50650,101301,17.083465814590454,5.532905575236193e-05
25425,50851,50850,101701,17.14965581893921,5.5131769980631085e-05
25526,51053,51052,102105,17.211790800094604,5.493397220296787e-05
25626,51253,51252,102505,17.27417278289795,5.473955924971031e-05
25726,51453,51452,102905,17.3357937335968,5.454654609613513e-05
25826,51653,51652,103305,17.396607875823975,5.435491358867113e-05
25926,51853,51852,103705,17.458869695663452,5.416464288595694e-05
26026,52053,52052,104105,17.521105766296387,5.3975715451758205e-05
26126,52253,52252,104505,17.584826707839966,5.378811305171785e-05
26226,52453,52452,104905,17.652232885360718,5.360181774731357e-05
26326,52653,52652,105305,17.714491844177246,5.34168118919679e-05
26426,52853,52852,105705,17.779160737991333,5.323307812581171e-05
26527,53055,53054,106109,17.842590808868408,5.304878086415723e-05
26627,53255,53254,106509,17.90602397918701,5.2867552619982375e-05
26727,53455,53454,106909,17.968557834625244,5.2687545897219964e-05
26827,53655,53654,107309,18.031638622283936,5.250874444120578e-05
26927,53855,53854,107709,18.097718715667725,5.2331132261406814e-05
27027,54055,54054,108109,18.163861989974976,5.215469362782098e-05
27127,54255,54254,108509,18.226041793823242,5.197941306635809e-05
27227,54455,54454,108909,18.288907766342163,5.1805275354476744e-05
27327,54655,54654,109309,18.352965831756592,5.1632265517846414e-05
27427,54855,54854,109709,18.417703866958618,5.1460368825518695e-05
27528,55057,55056,110113,18.48016881942749,5.1287868306265416e-05
27628,55257,55256,110513,18.54567575454712,5.111816543831433e-05
27728,55457,55456,110913,18.618793964385986,5.09495328064174e-05
27828,55657,55656,111313,18.697121620178223,5.078195661803489e-05
27928,55857,55856,111713,18.766775846481323,5.0615423305065665e-05
28028,56057,56056,112113,18.831172704696655,5.0449919519951715e-05
28128,56257,56256,112513,18.895862817764282,5.028543213283578e-05
28228,56457,56456,112913,18.958630800247192,5.012194822687067e-05
28328,56657,56656,113313,19.0207040309906,4.995945509631485e-05
28428,56857,56856,113713,19.084012746810913,4.9797940240634196e-05
28529,57059,57058,114117,19.148635864257812,4.9635790712233653e-05
28629,57259,57258,114517,19.21101689338684,4.947620519613613e-05
28729,57459,57458,114917,19.27271580696106,4.931756154448826e-05
28829,57659,57658,115317,19.338337659835815,4.915984805257059e-05
28929,57859,57858,115717,19.401904821395874,4.9003053205780613e-05
29029,58059,58058,116117,19.466214895248413,4.8847165676960624e-05
29129,58259,58258,116517,19.529254913330078,4.86921743226596e-05
29229,58459,58458,116917,19.593536615371704,4.853806817981771e-05
29329,58659,58658,117317,19.658894777297974,4.838483646400338e-05
29429,58859,58858,117717,19.71975564956665,4.823246856530781e-05
29530,59061,59060,118121,19.789920806884766,4.807944317543942e-05
29630,59261,59260,118521,19.853489875793457,4.7928780146489794e-05
29730,59461,59460,118921,19.91538977622986,4.77789500257163e-05
29830,59661,59660,119321,19.978328704833984,4.762994287589807e-05
29930,59861,59860,119721,20.04066777229309,4.74817489207553e-05
30030,60061,60060,120121,20.110052824020386,4.7334358542261396e-05
30130,60261,60260,120521,20.17225670814514,4.7187762277395645e-05
30230,60461,60460,120921,20.234437704086304,4.704195081676821e-05
30330,60661,60660,121321,20.297086000442505,4.689691500079174e-05
30430,60861,60860,121721,20.35811686515808,4.6752645817759055e-05
30531,61063,61062,122125,20.420567750930786,4.66077030845435e-05
30631,61263,61262,122525,20.48275876045227,4.6464948158740704e-05
30731,61463,61462,122925,20.544649839401245,4.632293360830165e-05
30831,61663,61662,123325,20.60789680480957,4.6181650990126026e-05
30931,61863,61862,123725,20.670949935913086,4.604109199664402e-05
31031,62063,62062,124125,20.736583948135376,4.590124845406999e-05
31131,62263,62262,124525,20.81710171699524,4.576211231931207e-05
31231,62463,62462,124925,20.890580892562866,4.5623675679175676e-05
31331,62663,62662,125325,20.954001903533936,4.5485930746875977e-05
31431,62863,62862,125725,21.016719818115234,4.534886986040284e-05
31532,63065,63064,126129,21.080803871154785,4.521112502764261e-05
31632,63265,63264,126529,21.15177869796753,4.5075416389486785e-05
31732,63465,63464,126929,21.215779781341553,4.494036946647604e-05
31832,63665,63664,127329,21.279448747634888,4.480597707620194e-05
31932,63865,63864,127729,21.34489870071411,4.467223215084162e-05
32032,64065,64064,128129,21.4071307182312,4.453912773524867e-05
32132,64265,64264,128529,21.471852779388428,4.440665698460036e-05
32232,64465,64464,128929,21.53396463394165,4.4274813163455194e-05
32332,64665,64664,129329,21.59962272644043,4.414358964266024e-05
32432,64865,64864,129729,21.666780948638916,4.4012979898811586e-05
32533,65067,65066,130133,21.73043203353882,4.388168053371468e-05
32633,65267,65266,130533,21.795270919799805,4.3752285163802853e-05
32733,65467,65466,130933,21.85829186439514,4.362348455197484e-05
32833,65667,65666,131333,21.92271375656128,4.349527257846508e-05
32933,65867,65866,131733,21.98644185066223,4.336764322057305e-05
33033,66067,66066,132133,22.05093479156494,4.324059055024682e-05
33133,66267,66266,132533,22.12180185317993,4.3114108732870426e-05
33233,66467,66466,132933,22.183629751205444,4.2988192024788874e-05
33333,66667,66666,133333,22.248013734817505,4.286283477379785e-05
33433,66867,66866,133733,22.317211866378784,4.273803141498402e-05
33534,67069,67068,134137,22.380308866500854,4.2612536673078805e-05
33634,67269,67268,134537,22.443177938461304,4.248883015614444e-05
33734,67469,67468,134937,22.50528883934021,4.23656613025213e-05
33834,67669,67668,135337,22.566770792007446,4.224302488806544e-05
33934,67869,67868,135737,22.633603811264038,4.212091576986844e-05
34034,68069,68068,136137,22.697070837020874,4.199932888547904e-05
34134,68269,68268,136537,22.763086795806885,4.187825925009619e-05
34234,68469,68468,136937,22.82633876800537,4.175770195691165e-05
34334,68669,68668,137337,22.897483825683594,4.1637652174587665e-05
34434,68869,68868,137737,22.976841926574707,4.151810514622675e-05
34535,69071,69070,138141,23.04711079597473,4.139786819858964e-05
34635,69271,69270,138541,23.115595817565918,4.1279317611775465e-05
34735,69471,69470,138941,23.181025743484497,4.116125589861157e-05
34835,69671,69670,139341,23.24330496788025,4.104367858893266e-05
34935,69871,69870,139741,23.306303024291992,4.0926581280700996e-05
35035,70071,70070,140141,23.366692781448364,4.080995963938163e-05
35135,70271,70270,140541,23.426178693771362,4.069380939636397e-05
35235,70471,70470,140941,23.486709594726562,4.057812634818032e-05
35335,70671,70670,141341,23.548614740371704,4.0462906354930845e-05
35435,70871,70870,141741,23.609497785568237,4.034814533943403e-05
35536,71073,71072,142145,23.673510789871216,4.023269851009812e-05
35636,71273,71272,142545,23.733162879943848,4.0118847955303736e-05
35736,71473,71472,142945,23.793778896331787,4.0005444474302674e-05
35836,71673,71672,143345,23.85513973236084,3.989248423133194e-05
35936,71873,71872,143745,23.914684772491455,3.977996344779066e-05
36036,72073,72072,144145,23.97638177871704,3.966787840167345e-05
36136,72273,72272,144545,24.03983163833618,3.9556225426652794e-05
36236,72473,72472,144945,24.105119943618774,3.944500091107113e-05
36336,72673,72672,145345,24.16535186767578,3.9334201296940535e-05
36436,72873,72872,145745,24.226430892944336,3.922382307882055e-05
36537,73075,73074,146149,24.285569667816162,3.911276530013233e-05
36637,73275,73274,146549,24.347455978393555,3.9003223693911626e-05
36737,73475,73474,146949,24.40735697746277,3.889409324269979e-05
36837,73675,73674,147349,24.468113899230957,3.878537064403034e-05
36937,73875,73874,147749,24.52676773071289,3.867705264373247e-05
37037,74075,74074,148149,24.587738752365112,3.8569136035575155e-05
37137,74275,74274,148549,24.65071988105774,3.846161765936627e-05
37237,74475,74474,148949,24.708622694015503,3.8354494401890974e-05
37337,74675,74674,149349,24.766830682754517,3.824776319413055e-05
37437,74875,74874,149749,24.83012366294861,3.814142101205568e-05
37538,75077,75076,150153,24.89115285873413,3.803440725340683e-05
37638,75277,75276,150553,24.950530767440796,3.79288380403949e-05
37738,75477,75476,150953,25.012677907943726,3.782364901093012e-05
37838,75677,75676,151353,25.090811729431152,3.7718837310885584e-05
37938,75877,75876,151753,25.161483764648438,3.7614400127851394e-05
38038,76077,76076,152153,25.219861030578613,3.751033468881929e-05
38138,76277,76276,152553,25.280463695526123,3.740663826028056e-05
38238,76477,76476,152953,25.342641830444336,3.730330814739174e-05
38338,76677,76676,153353,25.4044828414917,3.720034169323855e-05
38438,76877,76876,153753,25.465162992477417,3.709773627867321e-05
38539,77079,77078,154157,25.523655891418457,3.699446865294886e-05
38639,77279,77278,154557,25.583855867385864,3.6892581151433304e-05
38739,77479,77478,154957,25.652617931365967,3.679104702434905e-05
38839,77679,77678,155357,25.71157670021057,3.668986379534003e-05
38939,77879,77878,155757,25.771318674087524,3.6589029022979676e-05
39039,78079,78078,156157,25.833792686462402,3.648854029927933e-05
39139,78279,78278,156557,25.896007776260376,3.638839524956265e-05
39239,78479,78478,156957,25.95579481124878,3.6288591531761835e-05
39339,78679,78678,157357,26.01594591140747,3.61891268352783e-05
39439,78879,78878,157757,26.076109647750854,3.608999888182181e-05
39540,79081,79080,158161,26.139468669891357,3.5990219170194606e-05
39640,79281,79280,158561,26.199374675750732,3.589176130081737e-05
39740,79481,79480,158961,26.259541988372803,3.579363349966635e-05
39840,79681,79680,159361,26.320567846298218,3.569583360914854e-05
39940,79881,79880,159761,26.378925800323486,3.559835949977883e-05
40040,80081,80080,160161,26.43829870223999,3.5501209071416535e-05
40140,80281,80280,160561,26.497519731521606,3.5404380251281975e-05
40240,80481,80480,160961,26.556930780410767,3.5307870994029904e-05
40340,80681,80680,161361,26.619699954986572,3.5211679281427e-05
40440,80881,80880,161761,26.679641723632812,3.511580312144049e-05
40541,81083,81082,162165,26.738422632217407,3.5019286499979554e-05
40641,81283,81282,162565,26.800447940826416,3.492403868100052e-05
40741,81483,81482,162965,26.859991788864136,3.4829100574807754e-05
40841,81683,81682,163365,26.92001485824585,3.4734470291890646e-05
40941,81883,81882,163765,26.978901863098145,3.464014596647524e-05
41041,82083,82082,164165,27.039376735687256,3.45461257568566e-05
41141,82283,82282,164565,27.104881763458252,3.445240784510626e-05
41241,82483,82482,164965,27.174027681350708,3.435899043634538e-05
41341,82683,82682,165365,27.250688791275024,3.426587175791585e-05
41441,82883,82882,165765,27.316126823425293,3.4173050060040944e-05
41542,83085,83084,166169,27.377529859542847,3.4079599835957025e-05
41642,83285,83284,166569,27.43725895881653,3.3987369864515485e-05
41742,83485,83484,166969,27.49760890007019,3.3895431737749304e-05
41842,83685,83684,167369,27.557403802871704,3.380378379178892e-05
41942,83885,83884,167769,27.623613834381104,3.3712424383170477e-05
42042,84085,84084,168169,27.6836040019989,3.3621351888860514e-05
42142,84285,84284,168569,27.742475748062134,3.3530564705567713e-05
42242,84485,84484,168969,27.80174684524536,3.344006124921282e-05
42342,84685,84684,169369,27.861262798309326,3.3349839955396146e-05
42442,84885,84884,169769,27.924989938735962,3.325989927833864e-05
42543,85087,85086,170173,27.98733377456665,3.316934247953814e-05
42643,85287,85286,170573,28.050837993621826,3.307996124134588e-05
42743,85487,85486,170973,28.116127014160156,3.2990856078097836e-05
42843,85687,85686,171373,28.180689811706543,3.2902025516997306e-05
42943,85887,85886,171773,28.242631912231445,3.2813468102134975e-05
43043,86087,86086,172173,28.305933713912964,3.2725182394760776e-05
43143,86287,86286,172573,28.370012760162354,3.2637166973119995e-05
43243,86487,86486,172973,28.43040370941162,3.2549420431910284e-05
43343,86687,86686,173373,28.492596864700317,3.246194138205185e-05
43443,86887,86886,173773,28.55423593521118,3.2374728450169683e-05
43544,87089,87088,174177,28.623234748840332,3.2286912129785224e-05
43644,87289,87288,174577,28.686349868774414,3.220023000499881e-05
43744,87489,87488,174977,28.751685857772827,3.211380995897561e-05
43844,87689,87688,175377,28.815334796905518,3.2027650679817884e-05
43944,87889,87888,175777,28.87765884399414,3.194175087097991e-05
44044,88089,88088,176177,28.940574884414673,3.185610924959775e-05
44144,88289,88288,176577,29.00537395477295,3.177072454766679e-05
44244,88489,88488,176977,29.0709388256073,3.1685595510624095e-05
44344,88689,88688,177377,29.138222694396973,3.1600720897995835e-05
44444,88889,88888,177777,29.20726990699768,3.151609948276434e-05
44545,89091,89090,178181,29.27113676071167,3.14308876253352e-05
44645,89291,89290,178581,29.351338863372803,3.134677147855145e-05
44745,89491,89490,178981,29.427680015563965,3.12629049154091e-05
44845,89691,89690,179381,29.49190664291382,3.117928676108141e-05
44945,89891,89890,179781,29.554945707321167,3.109591585283589e-05
45045,90091,90090,180181,29.62382984161377,3.101279104053156e-05
45145,90291,90290,180581,29.688154697418213,3.092991118627236e-05
45245,90491,90490,180981,29.755613803863525,3.0847275163573484e-05
45345,90691,90690,181381,29.82003092765808,3.076488185817855e-05
45445,90891,90890,181781,29.88526678085327,3.068273016674983e-05
45546,91093,91092,182185,29.949141025543213,3.060000109696152e-05
45646,91293,91292,182585,30.014394760131836,3.051833175864916e-05
45746,91493,91492,182985,30.07803964614868,3.0436900781789743e-05
45846,91693,91692,183385,30.14532995223999,3.035570710759452e-05
45946,91893,91892,183785,30.208630800247192,3.0274749687879228e-05
46046,92093,92092,184185,30.27203679084778,3.019402748502417e-05
46146,92293,92292,184585,30.340221881866455,3.0113539471342186e-05
46246,92493,92492,184985,30.40301275253296,3.0033284629731675e-05
46346,92693,92692,185385,30.46654486656189,2.9953261952689638e-05
46446,92893,92892,185785,30.530184984207153,2.9873470442305168e-05
46547,93095,93094,186189,30.596466779708862,2.97931146568962e-05
46647,93295,93294,186589,30.66164994239807,2.9713784813298593e-05
46747,93495,93494,186989,30.72463369369507,2.9634683191163725e-05
46847,93695,93694,187389,30.79154372215271,2.9555808830914836e-05
46947,93895,93894,187789,30.85551166534424,2.947716078132438e-05
47047,94095,94094,188189,30.92010498046875,2.9398738100701532e-05
47147,94295,94294,188589,30.985195636749268,2.9320539855758794e-05
47247,94495,94494,188989,31.048735857009888,2.9242565122036886e-05
47347,94695,94694,189389,31.116156816482544,2.9164812983457692e-05
47447,94895,94894,189789,31.18205690383911,2.9087282532179822e-05
47548,95097,95096,190193,31.24878478050232,2.9009200884041206e-05
47648,95297,95296,190593,31.31783175468445,2.8932113311716377e-05
47748,95497,95496,190993,31.382730960845947,2.8855244743650734e-05
47848,95697,95696,191393,31.462570905685425,2.877859430446245e-05
47948,95897,95896,191793,31.54263401031494,2.8702161126272125e-05
48048,96097,96096,192193,31.60734486579895,2.862594434899295e-05
48148,96297,96296,192593,31.67253088951111,2.8549943120269324e-05
48248,96497,96496,192993,31.73583984375,2.8474156594495263e-05
48348,96697,96696,193393,31.802209615707397,2.8398583933947197e-05
48448,96897,96896,193793,31.865108966827393,2.8323224307540278e-05
48549,97099,97098,194197,31.93009376525879,2.8247326486691827e-05
48649,97299,97298,194597,31.99338388442993,2.817239257455151e-05
48749,97499,97498,194997,32.05857181549072,2.8097669238021834e-05
48849,97699,97698,195397,32.127349615097046,2.8023155674178978e-05
48949,97899,97898,195797,32.19183278083801,2.7948851086527247e-05
49049,98099,98098,196197,32.255483865737915,2.7874754684591886e-05
49149,98299,98298,196597,32.32176470756531,2.780086568570416e-05
49249,98499,98498,196997,32.390267848968506,2.7727183311740008e-05
49349,98699,98698,197397,32.45708680152893,2.7653706792183907e-05
49449,98899,98898,197797,32.52044701576233,2.758043536234747e-05
49550,99101,99100,198201,32.584118604660034,2.7506638621631794e-05
49650,99301,99300,198601,32.653728008270264,2.7433777132734744e-05
49750,99501,99500,199001,32.71680164337158,2.7361118467608967e-05
49850,99701,99700,199401,32.780311822891235,2.7288661885254508e-05
49950,99901,99900,199801,32.8449547290802,2.7216406650517186e-05
50050,100101,100100,200201,32.910966634750366,2.7144352033615213e-05
50150,100301,100300,200601,32.973827838897705,2.7072497310831866e-05
50250,100501,100500,201001,33.040363788604736,2.7000841762909114e-05
50350,100701,100700,201401,33.10841774940491,2.6929384677127086e-05
50450,100901,100900,201801,33.17995285987854,2.6858125345551605e-05
50551,101103,101102,202205,33.24387264251709,2.6786353435153334e-05
50651,101303,101302,202605,33.309685707092285,2.6715489468926942e-05
50751,101503,101502,203005,33.37795686721802,2.664482115731684e-05
50851,101703,101702,203405,33.44026494026184,2.6574347812971902e-05
50951,101903,101902,203805,33.506608724594116,2.6504068753598124e-05
51051,102103,102102,204205,33.58182668685913,2.6433983301478658e-05
51151,102303,102302,204605,33.664233922958374,2.6364090784217187e-05
51251,102503,102502,205005,33.72711396217346,2.6294390533643692e-05
51351,102703,102702,205405,33.78829884529114,2.622488188663606e-05
51451,102903,102902,205805,33.8530969619751,2.615556418426677e-05
51552,103105,103104,206209,33.91295266151428,2.6085746457375544e-05
51652,103305,103304,206609,33.9733829498291,2.6016810580009973e-05
51752,103505,103504,207009,34.03633689880371,2.5948063691814663e-05
51852,103705,103704,207409,34.102829694747925,2.587950515238442e-05
51952,103905,103904,207809,34.16466999053955,2.5811134324963e-05
52052,104105,104104,208209,34.22405481338501,2.5742950577323302e-05
52152,104305,104304,208609,34.28350472450256,2.567495328149912e-05
52252,104505,104504,209009,34.34286880493164,2.560714181311486e-05
52352,104705,104704,209409,34.4020516872406,2.5539515552817387e-05
52452,104905,104904,209809,34.46197462081909,2.5472073884457064e-05
52553,105107,105106,210213,34.5233678817749,2.5404144546321363e-05
52653,105307,105306,210613,34.58318591117859,2.533707206083591e-05
52753,105507,105506,211013,34.647419929504395,2.5270182337160887e-05
52853,105707,105706,211413,34.70920777320862,2.520347477521847e-05
52953,105907,105906,211813,34.76962876319885,2.5136948778363798e-05
53053,106107,106106,212213,34.83373284339905,2.5070603753709034e-05
53153,106307,106306,212613,34.8931667804718,2.500443911217596e-05
53253,106507,106506,213013,34.95272088050842,2.4938454268183675e-05
53353,106707,106706,213413,35.013731718063354,2.48726486398525e-05
53453,106907,106906,213813,35.07195687294006,2.4807021648456734e-05
53554,107109,107108,214217,35.13920783996582,2.4740919127460702e-05
53654,107309,107308,214617,35.199403047561646,2.4675649460674334e-05
53754,107509,107508,215017,35.25947189331055,2.461055671077888e-05
53854,107709,107708,215417,35.31996393203735,2.4545640312633613e-05
53954,107909,107908,215817,35.37937688827515,2.4480899704857497e-05
54054,108109,108108,216217,35.440008878707886,2.441633432916529e-05
54154,108309,108308,216617,35.500051975250244,2.4351943630693313e-05
54254,108509,108508,217017,35.56007981300354,2.4287727057213384e-05
54354,108709,108708,217417,35.62243676185608,2.422368406037015e-05
54454,108909,108908,217817,35.68525290489197,2.4159814094366667e-05
54555,109111,109110,218221,35.7649028301239,2.4095480511209837e-05
54655,109311,109310,218621,35.838013887405396,2.403195669900347e-05
54755,109511,109510,219021,35.89842486381531,2.396860429375416e-05
54855,109711,109710,219421,35.96056389808655,2.390542276187011e-05
54955,109911,109910,219821,36.020386695861816,2.3842411572404317e-05
55055,110111,110110,220221,36.08207368850708,2.377957019812172e-05
55155,110311,110310,220621,36.15934181213379,2.3716898113502782e-05
55255,110511,110510,221021,36.220353841781616,2.3654394796708936e-05
55355,110711,110710,221421,36.28086566925049,2.3592059728499633e-05
55455,110911,110910,221821,36.342429876327515,2.352989239212878e-05
55556,111113,111112,222225,36.403488636016846,2.3467273115073354e-05
55656,111313,111312,222625,36.466869592666626,2.3405441367879728e-05
55756,111513,111512,223025,36.52736282348633,2.3343775813775845e-05
55856,111713,111712,223425,36.590242862701416,2.3282275946711545e-05
55956,111913,111912,223825,36.652925968170166,2.322094126385062e-05
56056,112113,112112,224225,36.71377182006836,2.3159771263642842e-05
56156,112313,112312,224625,36.77490472793579,2.3098765448635443e-05
56256,112513,112512,225025,36.83595871925354,2.3037923322603186e-05
56356,112713,112712,225425,36.90648865699768,2.2977244392556e-05
56456,112913,112912,225825,36.9749538898468,2.2916728167328615e-05
56557,113115,113114,226229,37.04696559906006,2.285577143627992e-05
56657,113315,113314,226629,37.11756086349487,2.2795580773450657e-05
56757,113515,113514,227029,37.19169878959656,2.2735551352643295e-05
56857,113715,113714,227429,37.26145267486572,2.2675682692531344e-05
56957,113915,113914,227829,37.33019495010376,2.2615974314403126e-05
57057,114115,114114,228229,37.40320062637329,2.2556425741619783e-05
57157,114315,114314,228629,37.46857666969299,2.2497036499421136e-05
57257,114515,114514,229029,37.52863788604736,2.2437806115965838e-05
57357,114715,114714,229429,37.5961217880249,2.2378734121140846e-05
57457,114915,114914,229829,37.658761978149414,2.23198200471003e-05
57558,115117,115116,230233,37.7204008102417,2.2260476655638483e-05
57658,115317,115316,230633,37.78886389732361,2.220187859615511e-05
57758,115517,115516,231033,37.859503746032715,2.2143437062694848e-05
57858,115717,115716,231433,37.93786382675171,2.208515159585446e-05
57958,115917,115916,231833,38.00258469581604,2.2027021738412768e-05
58058,116117,116116,232233,38.063939809799194,2.196904703531825e-05
58158,116317,116316,232633,38.12898778915405,2.1911227033862122e-05
58258,116517,116516,233033,38.18970775604248,2.1853561282433104e-05
58358,116717,116716,233433,38.249839782714844,2.179604933237747e-05
58458,116917,116916,233833,38.313055992126465,2.1738690736792868e-05
58559,117119,117118,234237,38.37541079521179,2.1680913764197943e-05
58659,117319,117318,234637,38.43527293205261,2.16238620660385e-05
58759,117519,117518,235037,38.497769832611084,2.1566962388363205e-05
58859,117719,117718,235437,38.56167197227478,2.1510214291852315e-05
58959,117919,117918,235837,38.62746977806091,2.145361733882728e-05
59059,118119,118118,236237,38.68745279312134,2.1397171093987558e-05
59159,118319,118318,236637,38.7475106716156,2.1340875123504925e-05
59259,118519,118518,237037,38.80898380279541,2.1284728995255595e-05
59359,118719,118718,237437,38.871450901031494,2.1228732279424487e-05
59459,118919,118918,237837,38.934820890426636,2.1172884547671173e-05
59560,119121,119120,238241,38.997742891311646,2.1116629130278112e-05
59660,119321,119320,238641,39.058573722839355,2.1061079567991885e-05
59760,119521,119520,239041,39.12334990501404,2.1005677711233096e-05
59860,119721,119720,239441,39.18463587760925,2.0950423138432683e-05
59960,119921,119920,239841,39.247824907302856,2.0895315430546292e-05
60060,120121,120120,240241,39.315417766571045,2.084035416953603e-05
60160,120321,120320,240641,39.383118867874146,2.0785538939042277e-05
60260,120521,120520,241041,39.4451117515564,2.0730869324710094e-05
60360,120721,120720,241441,39.50621175765991,2.0676344913662552e-05
60460,120921,120920,241841,39.56856560707092,2.0621965294468176e-05
60561,121123,121122,242245,39.63962483406067,2.0567188433262498e-05
60661,121323,121322,242645,39.7005558013916,2.051309860880756e-05
60761,121523,121522,243045,39.7645959854126,2.0459152348164386e-05
60861,121723,121722,243445,39.82689881324768,2.040534924679027e-05
60961,121923,121922,243845,39.88857078552246,2.035168890128138e-05
61061,122123,122122,244245,39.95306968688965,2.0298170909973146e-05
61161,122323,122322,244645,40.03318667411804,2.0244794872959396e-05
61261,122523,122522,245045,40.106661796569824,2.0191560391286615e-05
61361,122723,122722,245445,40.16896367073059,2.013846706802766e-05
61461,122923,122922,245845,40.2325656414032,2.0085514507503593e-05
61562,123125,123124,246249,40.294004917144775,2.0032174901477545e-05
61662,123325,123324,246649,40.35611176490784,1.9979504083596258e-05
61762,123525,123524,247049,40.42210268974304,1.9926972846823785e-05
61862,123725,123724,247449,40.48480677604675,1.9874580801212154e-05
61962,123925,123924,247849,40.54647493362427,1.982232755876665e-05
62062,124125,124124,248249,40.613316774368286,1.977021273223869e-05
62162,124325,124324,248649,40.67843770980835,1.9718235937093582e-05
62262,124525,124524,249049,40.73909783363342,1.9666396788647028e-05
62362,124725,124724,249449,40.800609827041626,1.9614694904457984e-05
62462,124925,124924,249849,40.86293077468872,1.9563129903492418e-05
62563,125127,125126,250253,40.927931785583496,1.95111878088456e-05
62663,125327,125326,250653,40.98856782913208,1.9459896795404316e-05
62763,125527,125526,251053,41.05214285850525,1.9408741525726247e-05
62863,125727,125726,251453,41.11838173866272,1.9357721624437273e-05
62963,125927,125926,251853,41.182180881500244,1.9306836717067964e-05
63063,126127,126126,252253,41.24813961982727,1.9256086430376436e-05
63163,126327,126326,252653,41.311903953552246,1.9205470392660153e-05
63263,126527,126526,253053,41.37296485900879,1.9154988233616504e-05
63363,126727,126726,253453,41.43518590927124,1.9104639584039083e-05
63463,126927,126926,253853,41.49732303619385,1.905442407592919e-05
63564,127129,127128,254257,41.56132197380066,1.900384118471068e-05
63664,127329,127328,254657,41.62863492965698,1.8953892183638294e-05
63764,127529,127528,255057,41.69296073913574,1.890407522448166e-05
63864,127729,127728,255457,41.75541877746582,1.8854389944565315e-05
63964,127929,127928,255857,41.818063735961914,1.8804835982245097e-05
64064,128129,128128,256257,41.88010382652283,1.8755412977338632e-05
64164,128329,128328,256657,41.94575476646423,1.8706120570740475e-05
64264,128529,128528,257057,42.010913610458374,1.865695840461242e-05
64364,128729,128728,257457,42.07405376434326,1.860792612203922e-05
64464,128929,128928,257857,42.1563138961792,1.855902336819472e-05
64565,129131,129130,258261,42.23398971557617,1.850976270343003e-05
64665,129331,129330,258661,42.29843783378601,1.8461119230959207e-05
64765,129531,129530,259061,42.3647255897522,1.841260422389944e-05
64865,129731,129730,259461,42.42790198326111,1.836421733186464e-05
64965,129931,129930,259861,42.48987698554993,1.8315958205267807e-05
65065,130131,130130,260261,42.55211877822876,1.8267826495468693e-05
65165,130331,130330,260661,42.62112879753113,1.8219821855713516e-05
65265,130531,130530,261061,42.683899879455566,1.8171943939394313e-05
65365,130731,130730,261461,42.74708366394043,1.8124192401890763e-05
65465,130931,130930,261861,42.81195282936096,1.807656689920891e-05
65566,131133,131132,262265,42.87499499320984,1.802859272401759e-05
65666,131333,131332,262665,42.93743896484375,1.7981219515825615e-05
65766,131533,131532,263065,43.00391888618469,1.7933971314153006e-05
65866,131733,131732,263465,43.0698618888855,1.7886847779718556e-05
65966,131933,131932,263865,43.139283895492554,1.7839848574542793e-05
66066,132133,132132,264265,43.20223879814148,1.7792973360984327e-05
66166,132333,132332,264665,43.26378870010376,1.774622180305548e-05
66266,132533,132532,265065,43.32903504371643,1.7699593565845852e-05
66366,132733,132732,265465,43.391610860824585,1.765308831498967e-05
66466,132933,132932,265865,43.45572090148926,1.7606705718167207e-05
66567,133135,133134,266269,43.51843786239624,1.755998345668219e-05
66667,133335,133334,266669,43.582661867141724,1.7513846390966255e-05
66767,133535,133534,267069,43.64826488494873,1.7467830982985047e-05
66867,133735,133734,267469,43.714876890182495,1.742193690438056e-05
66967,133935,133934,267869,43.78171968460083,1.7376163827261714e-05
67067,134135,134134,268269,43.85039782524109,1.733051142500303e-05
67167,134335,134334,268669,43.9307918548584,1.7284979372039063e-05
67267,134535,134534,269069,44.006051778793335,1.7239567343650374e-05
67367,134735,134734,269469,44.06965184211731,1.7194275015922567e-05
67467,134935,134934,269869,44.13825988769531,1.714910206677827e-05
67568,135137,135136,270273,44.204345703125,1.7103598235798575e-05
67668,135337,135336,270673,44.280171632766724,1.7058664265164614e-05
67768,135537,135536,271073,44.35967183113098,1.7013848707814715e-05
67868,135737,135736,271473,44.42330288887024,1.6969151245040448e-05
67968,135937,135936,271873,44.4865927696228,1.692457155918788e-05
68068,136137,136136,272273,44.55309081077576,1.6880109333620768e-05
68168,136337,136336,272673,44.62365388870239,1.683576425243439e-05
68268,136537,136536,273073,44.68789291381836,1.6791536000936082e-05
68368,136737,136736,273473,44.75003695487976,1.6747424265589038e-05
68468,136937,136936,273873,44.81188893318176,1.670342873304796e-05
68569,137139,137138,274277,44.87170886993408,1.665911087932783e-05
68669,137339,137338,274677,44.93295884132385,1.6615347972363444e-05
68769,137539,137538,275077,44.994489669799805,1.6571700332197553e-05
68869,137739,137738,275477,45.05829358100891,1.6528167649959238e-05
68969,137939,137938,275877,45.121466875076294,1.6484749617580144e-05
69069,138139,138138,276277,45.183440923690796,1.6441445927369382e-05
69169,138339,138338,276677,45.243870973587036,1.639825627356887e-05
69269,138539,138538,277077,45.304391860961914,1.635518035047111e-05
69369,138739,138738,277477,45.36407780647278,1.6312217853410014e-05
69469,138939,138938,277877,45.42367887496948,1.6269368479208947e-05
69570,139141,139140,278281,45.484657764434814,1.6226205128021875e-05
69670,139341,139340,278681,45.545018911361694,1.618358221545783e-05
69770,139541,139540,279081,45.607767820358276,1.6141071517023545e-05
69870,139741,139740,279481,45.66744565963745,1.6098672732901098e-05
69970,139941,139940,279881,45.725178718566895,1.6056385563722527e-05
70070,140141,140140,280281,45.79205584526062,1.601420971158354e-05
70170,140341,140340,280681,45.85235095024109,1.597214487904291e-05
70270,140541,140540,281081,45.914833784103394,1.5930190769403622e-05
70370,140741,140740,281481,45.97655177116394,1.5888347086828253e-05
70470,140941,140940,281881,46.04197669029236,1.5846613537293226e-05
70571,141143,141142,282285,46.11008381843567,1.5804574142821485e-05
70671,141343,141342,282685,46.17034697532654,1.5763061071677336e-05
70771,141543,141542,283085,46.231791734695435,1.572165725098083e-05
70871,141743,141742,283485,46.292701959609985,1.568036238932342e-05
70971,141943,141942,283885,46.35278391838074,1.563917619661719e-05
71071,142143,142142,284285,46.4298198223114,1.5598098383079944e-05
71171,142343,142342,284685,46.50633502006531,1.5557128659879805e-05
71271,142543,142542,285085,46.57215690612793,1.551626673904173e-05
71371,142743,142742,285485,46.6460497379303,1.5475512333340215e-05
71471,142943,142942,285885,46.70930576324463,1.543486515664381e-05
71572,143145,143144,286289,46.7738037109375,1.5393920059972016e-05
71672,143345,143344,286689,46.83751082420349,1.535348755058224e-05
71772,143545,143544,287089,46.89985466003418,1.531316141333044e-05
71872,143745,143744,287489,46.96201181411743,1.5272941365183232e-05
71972,143945,143944,287889,47.022955656051636,1.523282712384033e-05
72072,144145,144144,288289,47.08926177024841,1.5192818407997424e-05
72172,144345,144344,288689,47.15054988861084,1.5152914936847771e-05
72272,144545,144544,289089,47.2124707698822,1.5113116430789984e-05
72372,144745,144744,289489,47.272623777389526,1.5073422610793069e-05
72472,144945,144944,289889,47.33659291267395,1.5033833198687016e-05
72573,145147,145146,290293,47.399831771850586,1.4993953589126237e-05
72673,145347,145346,290693,47.4590117931366,1.4954573198261597e-05
72773,145547,145546,291093,47.52144980430603,1.4915296382650158e-05
72873,145747,145746,291493,47.583388805389404,1.4876122867020013e-05
72973,145947,145946,291893,47.64910697937012,1.4837052377335046e-05
73073,146147,146146,292293,47.7104377746582,1.4798084639996012e-05
73173,146347,146346,292693,47.77579593658447,1.4759219382225475e-05
73273,146547,146546,293093,47.841179847717285,1.4720456332134343e-05
73373,146747,146746,293493,47.90208983421326,1.4681795218396131e-05
73473,146947,146946,293893,47.96236968040466,1.464323577088099e-05
73574,147149,147148,294297,48.027838945388794,1.4604393650022224e-05
73674,147349,147348,294697,48.09632062911987,1.4566037736105774e-05
73774,147549,147548,295097,48.1641149520874,1.4527782678803756e-05
73874,147749,147748,295497,48.22772574424744,1.4489628210470056e-05
73974,147949,147948,295897,48.29231286048889,1.4451574064646674e-05
74074,148149,148148,296297,48.357097864151,1.4413619975729352e-05
74174,148349,148348,296697,48.41983389854431,1.4375765677929323e-05
74274,148549,148548,297097,48.482542753219604,1.4338010907430697e-05
74374,148749,148748,297497,48.56151485443115,1.4300355400015598e-05
74474,148949,148948,297897,48.638797760009766,1.4262798893241198e-05
74575,149151,149150,298301,48.70144987106323,1.4224967044582713e-05
74675,149351,149350,298701,48.76380491256714,1.4187608735879116e-05
74775,149551,149550,299101,48.827343702316284,1.4150348640633926e-05
74875,149751,149750,299501,48.88867783546448,1.411318649859706e-05
74975,149951,149950,299901,48.95222783088684,1.4076122050697859e-05
75075,150151,150150,300301,49.015859842300415,1.4039155038217177e-05
75175,150351,150350,300701,49.07669281959534,1.4002285203044059e-05
75275,150551,150550,301101,49.14351487159729,1.396551228814974e-05
75375,150751,150750,301501,49.203664779663086,1.3928836037334154e-05
75475,150951,150950,301901,49.26411485671997,1.3892256194644411e-05
75576,151153,151152,302305,49.32530999183655,1.3855408152760232e-05
75676,151353,151352,302705,49.39313364028931,1.3819021319724948e-05
75776,151553,151552,303105,49.45714473724365,1.378273012937316e-05
75876,151753,151752,303505,49.52260875701904,1.37465343287313e-05
75976,151953,151952,303905,49.593164682388306,1.3710433665364345e-05
76076,152153,152152,304305,49.662842750549316,1.3674427888222097e-05
76176,152353,152352,304705,49.72659373283386,1.3638516746108737e-05
76276,152553,152552,305105,49.78871488571167,1.3602699989017592e-05
76376,152753,152752,305505,49.855841636657715,1.3566977367307783e-05
76476,152953,152952,305905,49.91856575012207,1.3531348632291498e-05
76577,153155,153154,306309,49.98172879219055,1.3495458657206668e-05
76677,153355,153354,306709,50.04346179962158,1.3460017884723614e-05
76777,153555,153554,307109,50.1093168258667,1.3424670254234672e-05
76877,153755,153754,307509,50.17098069190979,1.3389415520023877e-05
76977,153955,153954,307909,50.23222279548645,1.3354253435917976e-05
77077,154155,154154,308309,50.29608869552612,1.331918375795346e-05
77177,154355,154354,308709,50.35841369628906,1.3284206241693176e-05
77277,154555,154554,309109,50.419339656829834,1.3249320643883574e-05
77377,154755,154754,309509,50.48069787025452,1.321452672189924e-05
77477,154955,154954,309909,50.54465675354004,1.3179824233379296e-05
77578,155157,155156,310313,50.612870931625366,1.3144867284058924e-05
77678,155357,155356,310713,50.68724298477173,1.3110347847813236e-05
77778,155557,155556,311113,50.765379667282104,1.3075919120364645e-05
77878,155757,155756,311513,50.83086895942688,1.3041580862856384e-05
77978,155957,155956,311913,50.89207077026367,1.3007332836114578e-05
78078,156157,156156,312313,50.9590847492218,1.2973174802116794e-05
78178,156357,156356,312713,51.021283864974976,1.2939106523417998e-05
78278,156557,156556,313113,51.087806940078735,1.2905127763163407e-05
78378,156757,156756,313513,51.155457735061646,1.2871238285231564e-05
78478,156957,156956,313913,51.21731781959534,1.2837437853971156e-05
78579,157159,157158,314317,51.28267979621887,1.2803389565780477e-05
78679,157359,157358,314717,51.3445258140564,1.2769767408582331e-05
78779,157559,157558,315117,51.40675091743469,1.2736233592828765e-05
78879,157759,157758,315517,51.46991991996765,1.2702787885569308e-05
78979,157959,157958,315917,51.533527851104736,1.266943005464994e-05
79079,158159,158158,316317,51.59865069389343,1.263615986810437e-05
79179,158359,158358,316717,51.662890911102295,1.2602977095002604e-05
79279,158559,158558,317117,51.72475075721741,1.2569881504720002e-05
79379,158759,158758,317517,51.787813901901245,1.253687286739442e-05
79479,158959,158958,317917,51.852107763290405,1.2503950953878767e-05
79580,159161,159160,318321,51.91646885871887,1.2470787617383913e-05
79680,159361,159360,318721,51.97757887840271,1.2438039327649303e-05
79780,159561,159560,319121,52.04013681411743,1.240537707547421e-05
79880,159761,159760,319521,52.10605072975159,1.237280063375178e-05
79980,159961,159960,319921,52.169761657714844,1.2340309776876111e-05
80080,160161,160160,320321,52.23467183113098,1.2307904278813797e-05
80180,160361,160360,320721,52.30017590522766,1.2275583914711291e-05
80280,160561,160560,321121,52.36604595184326,1.2243348460431628e-05
80380,160761,160760,321521,52.429768800735474,1.221119769218869e-05
80480,160961,160960,321921,52.491896867752075,1.2179131386483536e-05
80581,161163,161162,322325,52.55766677856445,1.2146829925215369e-05
80681,161363,161362,322725,52.62608575820923,1.2114932717436678e-05
80781,161563,161562,323125,52.68730878829956,1.2083119304311862e-05
80881,161763,161762,323525,52.751253843307495,1.205138946520942e-05
80981,161963,161962,323925,52.83150267601013,1.2019742980131977e-05
81081,162163,162162,324325,52.909152030944824,1.1988179629343102e-05
81181,162363,162362,324725,52.97776675224304,1.1956699193857707e-05
81281,162563,162562,325125,53.04440665245056,1.1925301455426336e-05
81381,162763,162762,325525,53.110718965530396,1.1893986196231848e-05
81481,162963,162962,325925,53.173091888427734,1.1862753198888453e-05
81582,163165,163164,326329,53.23634672164917,1.1831291150946348e-05
81682,163365,163364,326729,53.299784898757935,1.1800222845606567e-05
81782,163565,163564,327129,53.36803579330444,1.1769236151740224e-05
81882,163765,163764,327529,53.434117794036865,1.1738330854899474e-05
81982,163965,163964,327929,53.49762678146362,1.1707506740377812e-05
82082,164165,164164,328329,53.560675859451294,1.1676763594383616e-05
82182,164365,164364,328729,53.626788854599,1.1646101204224468e-05
82282,164565,164564,329129,53.69016671180725,1.161551935693326e-05
82382,164765,164764,329529,53.75265574455261,1.1585017840624047e-05
82482,164965,164964,329929,53.815067768096924,1.1554596443897515e-05
82583,165167,165166,330333,53.878150939941406,1.1523951943227812e-05
82683,165367,165366,330733,53.94112181663513,1.1493690949118079e-05
82783,165567,165566,331133,54.004857778549194,1.1463509441390283e-05
82883,165767,165766,331533,54.06805777549744,1.1433407210656454e-05
82983,165967,165966,331933,54.13514280319214,1.1403384048218123e-05
83083,166167,166166,332333,54.19924974441528,1.1373439746596062e-05
83183,166367,166366,332733,54.26348066329956,1.1343574097645675e-05
83283,166567,166566,333133,54.32720375061035,1.131378689441373e-05
83383,166767,166766,333533,54.3893518447876,1.1284077930830338e-05
83483,166967,166966,333933,54.45244789123535,1.1254447000641382e-05
83584,167169,167168,334337,54.51708173751831,1.1224598760195044e-05
83684,167369,167368,334737,54.58513689041138,1.11951240568669e-05
83784,167569,167568,335137,54.654451847076416,1.1165726770648461e-05
83884,167769,167768,335537,54.72075271606445,1.1136406698171625e-05
83984,167969,167968,335937,54.78343391418457,1.1107163635669422e-05
84084,168169,168168,336337,54.845852851867676,1.1077997381037363e-05
84184,168369,168368,336737,54.916547775268555,1.1048907731975638e-05
84284,168569,168568,337137,54.995606660842896,1.1019894487093157e-05
84384,168769,168768,337537,55.06654977798462,1.0990957445159922e-05
84484,168969,168968,337937,55.139970779418945,1.0962096405986309e-05
84585,169171,169170,338341,55.207175970077515,1.0933023699233323e-05
84685,169371,169370,338741,55.27115488052368,1.0904314820877476e-05
84785,169571,169570,339141,55.333653926849365,1.0875681345230212e-05
84885,169771,169770,339541,55.398563861846924,1.0847123073347615e-05
84985,169971,169970,339941,55.46084189414978,1.0818639808014849e-05
85085,170171,170170,340341,55.523459672927856,1.0790231351637085e-05
85185,170371,170370,340741,55.590152978897095,1.0761897507666352e-05
85285,170571,170570,341141,55.65738272666931,1.0733638079534253e-05
85385,170771,170770,341541,55.718788862228394,1.0705452871767683e-05
85485,170971,170970,341941,55.78410482406616,1.067734168925997e-05
85586,171173,171172,342345,55.84885787963867,1.064902433568676e-05
85686,171373,171372,342745,55.91477084159851,1.0621061355043744e-05
85786,171573,171572,343145,55.98222494125366,1.059317181518744e-05
85886,171773,171772,343545,56.044158935546875,1.0565355523073603e-05
85986,171973,171972,343945,56.11265778541565,1.0537612285765303e-05
86086,172173,172172,344345,56.17842483520508,1.0509941911292575e-05
86186,172373,172372,344745,56.24048376083374,1.0482344208128958e-05
86286,172573,172572,345145,56.303576707839966,1.0454818985153182e-05
86386,172773,172772,345545,56.36762595176697,1.0427366051932911e-05
86486,172973,172972,345945,56.43075680732727,1.0399985217957848e-05
86587,173175,173174,346349,56.49749994277954,1.0372403567356618e-05
86687,173375,173374,346749,56.560948848724365,1.0345167080779708e-05
86787,173575,173574,347149,56.62744975090027,1.0318002124323727e-05
86887,173775,173774,347549,56.6940758228302,1.0290908510408078e-05
86987,173975,173974,347949,56.7755069732666,1.0263886051489661e-05
87087,174175,174174,348349,56.83990287780762,1.023693456009163e-05
87187,174375,174374,348749,56.90011692047119,1.0210053849828041e-05
87287,174575,174574,349149,56.96192169189453,1.0183243734818245e-05
87387,174775,174774,349549,57.022228956222534,1.0156504029432973e-05
87487,174975,174974,349949,57.097779989242554,1.0129834548314839e-05
87588,175177,175176,350353,57.172900676727295,1.0102969465708931e-05
87688,175377,175376,350753,57.236249685287476,1.0076440577754233e-05
87788,175577,175576,351153,57.2980580329895,1.0049981359889729e-05
87888,175777,175776,351553,57.35730791091919,1.0023591629317674e-05
87988,175977,175976,351953,57.41666793823242,9.997271203206732e-06
88088,176177,176176,352353,57.477030754089355,9.971019899275373e-06
88188,176377,176376,352753,57.5373158454895,9.944837536108938e-06
88288,176577,176576,353153,57.60360288619995,9.918723932113912e-06
88388,176777,176776,353553,57.66580772399902,9.892678906949668e-06
88488,176977,176976,353953,57.726704835891724,9.86670228002259e-06
88589,177179,177178,354357,57.78657364845276,9.840535131651284e-06
88689,177379,177378,354757,57.85005283355713,9.814695442258035e-06
88789,177579,177578,355157,57.90976881980896,9.788923611639064e-06
88889,177779,177778,355557,57.96827173233032,9.763219461283837e-06
88989,177979,177978,355957,58.032957792282104,9.737582813622028e-06
89089,178179,178178,356357,58.09718465805054,9.71201349078275e-06
89189,178379,178378,356757,58.15884804725647,9.686511316281724e-06
89289,178579,178578,357157,58.219987869262695,9.661076113395552e-06
89389,178779,178778,357557,58.28227376937866,9.635707706140528e-06
89489,178979,178978,357957,58.34099888801575,9.610405919055778e-06
89590,179181,179180,358361,58.40276098251343,9.584918558584647e-06
89690,179381,179380,358761,58.46356773376465,9.559750148907463e-06
89790,179581,179580,359161,58.52334475517273,9.534647833836196e-06
89890,179781,179780,359561,58.58604693412781,9.509611439370758e-06
89990,179981,179980,359961,58.64669179916382,9.484640792811653e-06
90090,180181,180180,360361,58.707385778427124,9.459735720964691e-06
90190,180381,180380,360761,58.76913094520569,9.434896051772496e-06
90290,180581,180580,361161,58.83020877838135,9.41012161331594e-06
90390,180781,180780,361561,58.88839888572693,9.385412234062858e-06
90490,180981,180980,361961,58.94734573364258,9.360767743141195e-06
90591,181183,181182,362365,59.00803780555725,9.335942498442284e-06
90691,181383,181382,362765,59.06842494010925,9.311427917734878e-06
90791,181583,181582,363165,59.13674592971802,9.286977713627531e-06
90891,181783,181782,363565,59.204509973526,9.262591716663786e-06
90991,181983,181982,363965,59.28204584121704,9.238269758334862e-06
91091,182183,182182,364365,59.35250473022461,9.214011670239104e-06
91191,182383,182382,364765,59.414482831954956,9.189817284931266e-06
91291,182583,182582,365165,59.47769284248352,9.165686434584442e-06
91391,182783,182782,365565,59.537710666656494,9.141618952547733e-06
91491,182983,182982,365965,59.607956886291504,9.117614672312289e-06
91592,183185,183184,366369,59.67258286476135,9.093434332876992e-06
91692,183385,183384,366769,59.736228704452515,9.069556586098724e-06
91792,183585,183584,367169,59.807148694992065,9.045741542650036e-06
91892,183785,183784,367569,59.870224714279175,9.021989037697424e-06
91992,183985,183984,367969,59.937676668167114,8.998298906767125e-06
92092,184185,184184,368369,60.00594472885132,8.974670986220466e-06
92192,184385,184384,368769,60.068989992141724,8.951105112489225e-06
92292,184585,184584,369169,60.134809732437134,8.927601122714584e-06
92392,184785,184784,369569,60.20256686210632,8.904158854121014e-06
92492,184985,184984,369969,60.266865968704224,8.880778144547698e-06
92593,185187,185186,370373,60.33127188682556,8.857225948945374e-06
92693,185387,185386,370773,60.3946008682251,8.833968484521094e-06
92793,185587,185586,371173,60.46256685256958,8.810772093657265e-06
92893,185787,185786,371573,60.52518582344055,8.787636616030929e-06
92993,185987,185986,371973,60.586747884750366,8.76456189144025e-06
93093,186187,186186,372373,60.65077090263367,8.74154776047529e-06
93193,186387,186386,372773,60.71414566040039,8.718594063931502e-06
93293,186587,186586,373173,60.774542808532715,8.69570064296409e-06
93393,186787,186786,373573,60.83701181411743,8.672867339118376e-06
93493,186987,186986,373973,60.89744472503662,8.650093994644548e-06
93594,187189,187188,374377,60.95997977256775,8.627153618231377e-06
93694,187389,187388,374777,61.01917290687561,8.604500315880699e-06
93794,187589,187588,375177,61.079434871673584,8.581906500167287e-06
93894,187789,187788,375577,61.143789768218994,8.559372014568675e-06
93994,187989,187988,375977,61.20530080795288,8.536896703382973e-06
94094,188189,188188,376377,61.26762390136719,8.51448041113686e-06
94194,188389,188388,376777,61.3402099609375,8.492122982742851e-06
94294,188589,188588,377177,61.418150901794434,8.469824263595075e-06
94394,188789,188788,377577,61.48151397705078,8.447584099478365e-06
94494,188989,188988,377977,61.541154861450195,8.425402336658989e-06
94595,189191,189190,378381,61.60847282409668,8.403057880107026e-06
94695,189391,189390,378781,61.66924977302551,8.380993040051644e-06
94795,189591,189590,379181,61.729530811309814,8.358986140706932e-06
94895,189791,189790,379581,61.79324173927307,8.337037029693978e-06
94995,189991,189990,379981,61.85584473609924,8.315145555526873e-06
95095,190191,190190,380381,61.918139934539795,8.293311566688538e-06
95195,190391,190390,380781,61.982097864151,8.271534912131095e-06
95295,190591,190590,381181,62.04397487640381,8.249815441257319e-06
95395,190791,190790,381581,62.108863830566406,8.228153003993022e-06
95495,190991,190990,381981,62.1702516078949,8.20654745034469e-06
95596,191193,191192,382385,62.234365940093994,8.18478342861278e-06
95696,191393,191392,382785,62.30076599121094,8.163291759574838e-06
95796,191593,191592,383185,62.3842077255249,8.141856525790952e-06
95896,191793,191792,383585,62.46625280380249,8.120477578772226e-06
95996,191993,191992,383985,62.53123474121094,8.099154771029846e-06
96096,192193,192192,384385,62.60042190551758,8.077887954753892e-06
96196,192393,192392,384785,62.6646249294281,8.056676983023173e-06
96296,192593,192592,385185,62.72741079330444,8.035521709281445e-06
96396,192793,192792,385585,62.790751934051514,8.01442198711689e-06
96496,192993,192992,385985,62.8533399105072,7.993377670530982e-06
96597,193195,193194,386389,62.915512800216675,7.972179002151493e-06
96697,193395,193394,386789,62.979718923568726,7.951245611324585e-06
96797,193595,193594,387189,63.04375076293945,7.930367189221866e-06
96897,193795,193794,387589,63.10781383514404,7.909543591465406e-06
96997,193995,193994,387989,63.17216682434082,7.888774674113965e-06
97097,194195,194194,388389,63.23477387428284,7.868060293792467e-06
97197,194395,194394,388789,63.30028796195984,7.847400306949162e-06
97297,194595,194594,389189,63.36410188674927,7.82679457074163e-06
97397,194795,194794,389589,63.428107023239136,7.806242942921378e-06
97497,194995,194994,389989,63.50613284111023,7.785745281091523e-06
97598,195197,195196,390393,63.584152698516846,7.765097276632814e-06
97698,195397,195396,390793,63.65177869796753,7.744707658473797e-06
97798,195597,195596,391193,63.7145049571991,7.724371580820378e-06
97898,195797,195796,391593,63.77921104431152,7.704088903287185e-06
97998,195997,195996,391993,63.84142279624939,7.683859485397779e-06
98098,196197,196196,392393,63.9047737121582,7.66368318755156e-06
98198,196397,196396,392793,63.96815490722656,7.643559869844438e-06
98298,196597,196596,393193,64.03508567810059,7.623489393519238e-06
98398,196797,196796,393593,64.10143899917603,7.603471619576296e-06
98498,196997,196996,393993,64.16545176506042,7.583506409682425e-06
98599,197199,197198,394397,64.22760677337646,7.563394762203865e-06
98699,197399,197398,394797,64.29047298431396,7.543534788658607e-06
98799,197599,197598,395197,64.35208988189697,7.5237269649544795e-06
98899,197799,197798,395597,64.41716885566711,7.5039711537993115e-06
98999,197999,197998,395997,64.48248672485352,7.484267218548834e-06
99099,198199,198198,396397,64.54431176185608,7.464615023158375e-06
99199,198399,198398,396797,64.60906767845154,7.445014431702537e-06
99299,198599,198598,397197,64.67135286331177,7.425465308523278e-06
99399,198799,198798,397597,64.73917484283447,7.405967518857829e-06
99499,198999,198998,397997,64.80042481422424,7.386520927231448e-06
99600,199201,199200,398401,64.86484575271606,7.366931701973265e-06
99700,199401,199400,398801,64.92686080932617,7.3475876126997645e-06
99800,199601,199600,399201,64.99025583267212,7.3282943183382445e-06
99900,199801,199800,399601,65.05600571632385,7.309051685286365e-06
100000,200001,200000,400001,65.12728381156921,7.289859580783329e-06


==> plot_data/bilinear_matrix_game_n250/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00047588348388671875,2.0175302852282635
100,201,200,401,0.07343316078186035,0.03870059256068895
200,401,400,801,0.1350259780883789,0.0179642168274124
300,601,600,1201,0.21738910675048828,0.010215612352113134
400,801,800,1601,0.3028271198272705,0.006414884987572114
501,1003,1002,2005,0.38286495208740234,0.004292887866686561
601,1203,1202,2405,0.4563760757446289,0.0031981848552840673
701,1403,1402,2805,0.5311760902404785,0.0023495755858960704
801,1603,1602,3205,0.606680154800415,0.0017642014700653555
901,1803,1802,3605,0.6794161796569824,0.0013107140383380224
1001,2003,2002,4005,0.754554033279419,0.0010771361342336561
1101,2203,2202,4405,0.821796178817749,0.0008891647471929582
1201,2403,2402,4805,0.8943130970001221,0.0007896238285358858
1301,2603,2602,5205,0.9764370918273926,0.0007243730865874144
1401,2803,2802,5605,1.0550200939178467,0.000648621889859143
1502,3005,3004,6009,1.1196181774139404,0.000605342378155228
1602,3205,3204,6409,1.1941471099853516,0.0005733026994351765
1702,3405,3404,6809,1.2673139572143555,0.0005447368428944139
1802,3605,3604,7209,1.4162800312042236,0.00048258186702094223
1902,3805,3804,7609,1.5148448944091797,0.00043623502306099424
2002,4005,4004,8009,1.5982789993286133,0.0004039543762459166
2102,4205,4204,8409,1.6816120147705078,0.00037891678446560513
2202,4405,4404,8809,1.7489171028137207,0.00035856970156738626
2302,4605,4604,9209,1.8173861503601074,0.00034167885404962273
2402,4805,4804,9609,1.8881070613861084,0.000327471216222133
2503,5007,5006,10013,1.9650418758392334,0.00031528514633575623
2603,5207,5206,10413,2.035529136657715,0.00030494059155017047
2703,5407,5406,10813,2.1040210723876953,0.0002959793336833732
2803,5607,5606,11213,2.1681830883026123,0.0002881403091160926
2903,5807,5806,11613,2.231938123703003,0.000281214281208699
3003,6007,6006,12013,2.3091230392456055,0.0002750331765274161
3103,6207,6206,12413,2.400527238845825,0.00026946189858635845
3203,6407,6406,12813,2.4808499813079834,0.00026439183980072673
3303,6607,6606,13213,2.547389030456543,0.00025973566986274647
3403,6807,6806,13613,2.618852138519287,0.000255423132572343
3504,7009,7008,14017,2.7045681476593018,0.0002513586896688166
3604,7209,7208,14417,2.79475998878479,0.0002475768793537788
3704,7409,7408,14817,2.8882720470428467,0.00024399934675541638
3804,7609,7608,15217,2.964362144470215,0.00024059633077260883
3904,7809,7808,15617,3.0376369953155518,0.00023734367502605227
4004,8009,8008,16017,3.1161391735076904,0.00023422171215643902
4104,8209,8208,16417,3.2095940113067627,0.00023121437386540734
4204,8409,8408,16817,3.2963531017303467,0.00022830848122147552
4304,8609,8608,17217,3.383721113204956,0.0002254931786417318
4404,8809,8808,17617,3.479944944381714,0.00022275948222810613
4505,9011,9010,18021,3.5598201751708984,0.0002200736757568169
4605,9211,9210,18421,3.6319000720977783,0.00021748264631160484
4705,9411,9410,18821,3.698601007461548,0.00021495419299109208
4805,9611,9610,19221,3.777956962585449,0.00021248387115568304
4905,9811,9810,19621,3.870835065841675,0.0002100678928804713
5005,10011,10010,20021,3.968748092651367,0.00020770300764981782
5105,10211,10210,20421,4.083566188812256,0.00020538640619713179
5205,10411,10410,20821,4.1821582317352295,0.0002031156428412569
5305,10611,10610,21221,4.277889013290405,0.00020088857263204926
5405,10811,10810,21621,4.38100004196167,0.0001987033003656253
5506,11013,11012,22025,4.483083009719849,0.00019653688483370254
5606,11213,11212,22425,4.592471122741699,0.00019443070110695764
5706,11413,11412,22825,4.675595045089722,0.0001923617375405541
5806,11613,11612,23225,4.754606246948242,0.0001903287540892684
5906,11813,11812,23625,4.830786228179932,0.00018833061625778637
6006,12013,12012,24025,4.916647911071777,0.00018636627982224012
6106,12213,12212,24425,4.998574256896973,0.00018443477820151422
6206,12413,12412,24825,5.078344106674194,0.00018253521198341002
6306,12613,12612,25225,5.151682138442993,0.00018066674020936473
6406,12813,12812,25625,5.2225470542907715,0.00017882857309627258
6507,13015,13014,26029,5.29066014289856,0.0001770020267232668
6607,13215,13214,26429,5.359029054641724,0.00017522255984983156
6707,13415,13414,26829,5.423156023025513,0.0001734712724405494
6807,13615,13614,27229,5.489932060241699,0.0001717475275193629
6907,13815,13814,27629,5.555908918380737,0.00017005071684054419
7007,14015,14014,28029,5.621159076690674,0.00016838025819878897
7107,14215,14214,28429,5.6914591789245605,0.00016673559311093918
7207,14415,14414,28829,5.75805401802063,0.00016511618481099277
7307,14615,14614,29229,5.82707405090332,0.000163521516504671
7407,14815,14814,29629,5.896754026412964,0.00016195108984464797
7508,15017,15016,30033,5.963438987731934,0.0001603890753312936
7608,15217,15216,30433,6.033016204833984,0.0001588659348191652
7708,15417,15416,30833,6.100348949432373,0.00015736563452041881
7808,15617,15616,31233,6.168921947479248,0.00015588773806327232
7908,15817,15816,31633,6.249572992324829,0.00015443182216535014
8008,16017,16016,32033,6.3154072761535645,0.0001529974758801278
8108,16217,16216,32433,6.382838010787964,0.00015158429991368803
8208,16417,16416,32833,6.450484037399292,0.00015019190600647155
8308,16617,16616,33233,6.524154901504517,0.00014881991636835176
8408,16817,16816,33633,6.586607933044434,0.00014746796316294591
8509,17019,17018,34037,6.660737037658691,0.00014612246346770548
8609,17219,17218,34437,6.739203214645386,0.00014480970865508907
8709,17419,17418,34837,6.804547071456909,0.0001435159385685191
8809,17619,17618,35237,6.870097875595093,0.00014224082088285596
8909,17819,17818,35637,6.935740947723389,0.0001409840311898774
9009,18019,18018,36037,7.002842903137207,0.00013974525267497582
9109,18219,18218,36437,7.070187091827393,0.00013852417581637554
9209,18419,18418,36837,7.132735013961792,0.00013732049810336562
9309,18619,18618,37237,7.197118043899536,0.00013613392377165485
9409,18819,18818,37637,7.25817084312439,0.0001349641635563538
9510,19021,19020,38041,7.323210000991821,0.00013379948470752128
9610,19221,19220,38441,7.3848700523376465,0.00013266267093725852
9710,19421,19420,38841,7.4489359855651855,0.0001315418375357308
9810,19621,19620,39241,7.516002178192139,0.00013043671908828831
9910,19821,19820,39641,7.577508211135864,0.00012934705563775144
10010,20021,20020,40041,7.645086050033569,0.00012827259250720958
10110,20221,20220,40441,7.711074113845825,0.0001272130801360416
10210,20421,20420,40841,7.773271083831787,0.0001261682739210451
10310,20621,20620,41241,7.833543062210083,0.00012513793406670548
10410,20821,20820,41641,7.892524003982544,0.00012412182544308851
10511,21023,21022,42045,7.955588102340698,0.00012310976630411754
10611,21223,21222,42445,8.026118993759155,0.00012212156935771686
10711,21423,21422,42845,8.090049028396606,0.00012114692271993615
10811,21623,21622,43245,8.15012001991272,0.000120185608667928
10911,21823,21822,43645,8.209603071212769,0.00011923741352364664
11011,22023,22022,44045,8.270666122436523,0.00011830212754717816
11111,22223,22222,44445,8.33216905593872,0.00011737954483300902
11211,22423,22422,44845,8.391311168670654,0.00011646946321229426
11311,22623,22622,45245,8.456070899963379,0.00011557168415702394
11411,22823,22822,45645,8.524376153945923,0.00011468601269024659
11512,23025,23024,46049,8.585857152938843,0.00011380357928193565
11612,23225,23224,46449,8.646278858184814,0.00011294166817294914
11712,23425,23424,46849,8.706762075424194,0.00011209129834021222
11812,23625,23624,47249,8.773117065429688,0.00011125228820360766
11912,23825,23824,47649,8.849900007247925,0.00011042445932999713
12012,24025,24024,48049,8.920488119125366,0.0001096076363612358
12112,24225,24224,48449,8.986858129501343,0.00010880164694508419
12212,24425,24424,48849,9.055395126342773,0.00010800632166848759
12312,24625,24624,49249,9.124843120574951,0.00010722149399299883
12412,24825,24824,49649,9.190991163253784,0.00010644700019297531
12513,25027,25026,50053,9.255736112594604,0.00010567508692150307
12613,25227,25226,50453,9.323813915252686,0.00010492088000252017
12713,25427,25426,50853,9.412030935287476,0.00010417653052252305
12813,25627,25626,51253,9.493982076644897,0.00010344188545014195
12913,25827,25826,51653,9.562824010848999,0.00010271679428441283
13013,26027,26026,52053,9.630218982696533,0.0001020011090041051
13113,26227,26226,52453,9.693585872650146,0.00010129468401762708
13213,26427,26426,52853,9.75853705406189,0.00010059737611571367
13313,26627,26626,53253,9.822446823120117,9.990904442504029e-05
13413,26827,26826,53653,9.884482145309448,9.922955036211032e-05
13514,27029,27028,54057,9.974233865737915,9.855209314758345e-05
13614,27229,27228,54457,10.076505184173584,9.788995253410103e-05
13714,27429,27428,54857,10.16294813156128,9.723624579831776e-05
13814,27629,27628,55257,10.247828006744385,9.659084311227403e-05
13914,27829,27828,55657,10.311815977096558,9.595361673015083e-05
14014,28029,28028,56057,10.372221946716309,9.532444095068601e-05
14114,28229,28228,56457,10.435741901397705,9.470319207907087e-05
14214,28429,28428,56857,10.50788402557373,9.408974839206253e-05
14314,28629,28628,57257,10.57536792755127,9.348399010080046e-05
14414,28829,28828,57657,10.641330003738403,9.28857993179508e-05
14515,29031,29030,58061,10.701415061950684,9.228918987302865e-05
14615,29231,29230,58461,10.76329493522644,9.170586068479885e-05
14715,29431,29430,58861,10.823459148406982,9.112975530307399e-05
14815,29631,29630,59261,10.883630990982056,9.056076313423452e-05
14915,29831,29830,59661,10.959683179855347,8.99987753263165e-05
15015,30031,30030,60061,11.034543991088867,8.94436847378516e-05
15115,30231,30230,60461,11.09489893913269,8.889538590984509e-05
15215,30431,30430,60861,11.153671026229858,8.835377503693193e-05
15315,30631,30630,61261,11.215556144714355,8.78187499394078e-05
15415,30831,30830,61661,11.278244256973267,8.729021003659379e-05
15516,31033,31032,62065,11.340703010559082,8.676286670204717e-05
15616,31233,31232,62465,11.506344079971313,8.624706410975493e-05
15716,31433,31432,62865,11.588660955429077,8.57374533479452e-05
15816,31633,31632,63265,11.669956922531128,8.523393998619012e-05
15916,31833,31832,63665,11.739082098007202,8.473643106529019e-05
16016,32033,32032,64065,11.800426959991455,8.424483507322058e-05
16116,32233,32232,64465,11.860701084136963,8.375906192201825e-05
16216,32433,32432,64865,11.92795205116272,8.327902292558504e-05
16316,32633,32632,65265,11.994153022766113,8.280463077566314e-05
16416,32833,32832,65665,12.056287050247192,8.233579952114378e-05
16517,33035,33034,66069,12.11782193183899,8.186783836882488e-05
16617,33235,33234,66469,12.177124977111816,8.140992988516565e-05
16717,33435,33434,66869,12.23940896987915,8.095733155701019e-05
16817,33635,33634,67269,12.299065828323364,8.050996266081315e-05
16917,33835,33834,67669,12.358952045440674,8.006774372664463e-05
17017,34035,34034,68069,12.4217050075531,7.963059651706329e-05
17117,34235,34234,68469,12.485789060592651,7.919844400880142e-05
17217,34435,34434,68869,12.548320055007935,7.877121037323326e-05
17317,34635,34634,69269,12.608582973480225,7.834882095884943e-05
17417,34835,34834,69669,12.668835163116455,7.793120227196671e-05
17518,35037,35036,70073,12.734426975250244,7.751417624099244e-05
17618,35237,35236,70473,12.794718980789185,7.710592898752043e-05
17718,35437,35436,70873,12.854438066482544,7.670223805725681e-05
17818,35637,35636,71273,12.914785146713257,7.630303442478913e-05
17918,35837,35836,71673,12.976360082626343,7.590825013610193e-05
18018,36037,36036,72073,13.05699110031128,7.551781829324232e-05
18118,36237,36236,72473,13.134474039077759,7.513167303666393e-05
18218,36437,36436,72873,13.20080304145813,7.474974953090994e-05
18318,36637,36636,73273,13.26089096069336,7.437198394798899e-05
18418,36837,36836,73673,13.322571039199829,7.399831345240632e-05
18519,37039,37038,74077,13.383954048156738,7.362499997502704e-05
18619,37239,37238,74477,13.44687795639038,7.325937446272465e-05
18719,37439,37438,74877,13.512434959411621,7.289766074269952e-05
18819,37639,37638,75277,13.576700925827026,7.253979981131108e-05
18919,37839,37838,75677,13.637963056564331,7.2185733583804e-05
19019,38039,38038,76077,13.702265977859497,7.183540488073206e-05
19119,38239,38238,76477,13.763113975524902,7.148875741550155e-05
19219,38439,38438,76877,13.826855897903442,7.114573577934091e-05
19319,38639,38638,77277,13.88791823387146,7.080628542869801e-05
19419,38839,38838,77677,13.95231008529663,7.047035267272691e-05
19520,39041,39040,78081,14.019391059875488,7.013457729963545e-05
19620,39241,39240,78481,14.080207824707031,6.980555587168995e-05
19720,39441,39440,78881,14.144328117370605,6.947989544303976e-05
19820,39641,39640,79281,14.210116147994995,6.915754561282357e-05
19920,39841,39840,79681,14.271610975265503,6.88384567705233e-05
20020,40041,40040,80081,14.336351156234741,6.852258008345205e-05
20120,40241,40240,80481,14.401312112808228,6.820986748509168e-05
20220,40441,40440,80881,14.462592124938965,6.790027166386641e-05
20320,40641,40640,81281,14.52526307106018,6.759374605147888e-05
20420,40841,40840,81681,14.586520195007324,6.729024481193715e-05
20521,41043,41042,82085,14.650897026062012,6.698673250509319e-05
20621,41243,41242,82485,14.712496995925903,6.668917450416247e-05
20721,41443,41442,82885,14.774214029312134,6.639450721864771e-05
20821,41643,41642,83285,14.837050914764404,6.610268763956923e-05
20921,41843,41842,83685,14.89735198020935,6.581367343690462e-05
21021,42043,42042,84085,14.960206031799316,6.552742294888833e-05
21121,42243,42242,84485,15.031552076339722,6.524389517202788e-05
21221,42443,42442,84885,15.10669493675232,6.496304975121927e-05
21321,42643,42642,85285,15.180561065673828,6.468484696983597e-05
21421,42843,42842,85685,15.26571798324585,6.440924774014854e-05
21522,43045,43044,86089,15.338438987731934,6.41334960777934e-05
21622,43245,43244,86489,15.401171922683716,6.38630142401576e-05
21722,43445,43444,86889,15.4708731174469,6.359502200085604e-05
21822,43645,43644,87289,15.554537057876587,6.332948269971798e-05
21922,43845,43844,87689,15.656753063201904,6.30663602598269e-05
22022,44045,44044,88089,15.742815971374512,6.280561917716129e-05
22122,44245,44244,88489,15.826184034347534,6.254722451316279e-05
22222,44445,44444,88889,15.896483182907104,6.229114188589911e-05
22322,44645,44644,89289,15.959712982177734,6.203733746082567e-05
22422,44845,44844,89689,16.028170108795166,6.17857779432218e-05
22523,45047,45046,90093,16.095652103424072,6.15339481577865e-05
22623,45247,45246,90493,16.16066598892212,6.128680232625892e-05
22723,45447,45446,90893,16.22472906112671,6.104180435902917e-05
22823,45647,45646,91293,16.28817892074585,6.0798923043198106e-05
22923,45847,45846,91693,16.352083921432495,6.0558127666077395e-05
23023,46047,46046,92093,16.4148428440094,6.0319388005680966e-05
23123,46247,46246,92493,16.48942494392395,6.008267432479922e-05
23223,46447,46446,92893,16.576825857162476,5.984795736310033e-05
23323,46647,46646,93293,16.654251098632812,5.96152083296387e-05
23423,46847,46846,93693,16.726219177246094,5.938439889501202e-05
23524,47049,47048,94097,16.797863006591797,5.915322176959705e-05
23624,47249,47248,94497,16.86500310897827,5.892622706563186e-05
23724,47449,47448,94897,16.93070697784424,5.870108940807669e-05
23824,47649,47648,95297,17.00060200691223,5.847778225090531e-05
23924,47849,47848,95697,17.07359004020691,5.825627947499746e-05
24024,48049,48048,96097,17.14391803741455,5.803655538210418e-05
24124,48249,48248,96497,17.209400177001953,5.781858468792967e-05
24224,48449,48448,96897,17.28093385696411,5.760234251642121e-05
24324,48649,48648,97297,17.36248517036438,5.7387804392374776e-05
24424,48849,48848,97697,17.436079025268555,5.717494623594152e-05
24525,49051,49050,98101,17.50133991241455,5.696164062245334e-05
24625,49251,49250,98501,17.566242218017578,5.675208792416326e-05
24725,49451,49450,98901,17.626689195632935,5.6544145035742415e-05
24825,49651,49650,99301,17.687072038650513,5.633778939997808e-05
24925,49851,49850,99701,17.747967958450317,5.613299882503801e-05
25025,50051,50050,100101,17.808813095092773,5.592975147842594e-05
25125,50251,50250,100501,17.87018609046936,5.5728025881110405e-05
25225,50451,50450,100901,17.93022894859314,5.552780090197602e-05
25325,50651,50650,101301,17.997947931289673,5.532905575236193e-05
25425,50851,50850,101701,18.058608055114746,5.5131769980631085e-05
25526,51053,51052,102105,18.122747898101807,5.493397220296787e-05
25626,51253,51252,102505,18.184081077575684,5.473955924971031e-05
25726,51453,51452,102905,18.246819019317627,5.454654609613513e-05
25826,51653,51652,103305,18.30887198448181,5.435491358867113e-05
25926,51853,51852,103705,18.368821144104004,5.416464288595694e-05
26026,52053,52052,104105,18.427808046340942,5.3975715451758205e-05
26126,52253,52252,104505,18.489118099212646,5.378811305171785e-05
26226,52453,52452,104905,18.554276943206787,5.360181774731357e-05
26326,52653,52652,105305,18.61440896987915,5.34168118919679e-05
26426,52853,52852,105705,18.673380851745605,5.323307812581171e-05
26527,53055,53054,106109,18.73564600944519,5.304878086415723e-05
26627,53255,53254,106509,18.80081009864807,5.2867552619982375e-05
26727,53455,53454,106909,18.86258316040039,5.2687545897219964e-05
26827,53655,53654,107309,18.923017024993896,5.250874444120578e-05
26927,53855,53854,107709,18.986143112182617,5.2331132261406814e-05
27027,54055,54054,108109,19.048579216003418,5.215469362782098e-05
27127,54255,54254,108509,19.109400033950806,5.197941306635809e-05
27227,54455,54454,108909,19.17191195487976,5.1805275354476744e-05
27327,54655,54654,109309,19.232340097427368,5.1632265517846414e-05
27427,54855,54854,109709,19.29310703277588,5.1460368825518695e-05
27528,55057,55056,110113,19.356661081314087,5.1287868306265416e-05
27628,55257,55256,110513,19.416484832763672,5.111816543831433e-05
27728,55457,55456,110913,19.494091033935547,5.09495328064174e-05
27828,55657,55656,111313,19.570528984069824,5.078195661803489e-05
27928,55857,55856,111713,19.63014006614685,5.0615423305065665e-05
28028,56057,56056,112113,19.69282102584839,5.0449919519951715e-05
28128,56257,56256,112513,19.75321912765503,5.028543213283578e-05
28228,56457,56456,112913,19.812342166900635,5.012194822687067e-05
28328,56657,56656,113313,19.871321201324463,4.995945509631485e-05
28428,56857,56856,113713,19.93083119392395,4.9797940240634196e-05
28529,57059,57058,114117,19.995983839035034,4.9635790712233653e-05
28629,57259,57258,114517,20.057284116744995,4.947620519613613e-05
28729,57459,57458,114917,20.119473934173584,4.931756154448826e-05
28829,57659,57658,115317,20.179906129837036,4.915984805257059e-05
28929,57859,57858,115717,20.241369247436523,4.9003053205780613e-05
29029,58059,58058,116117,20.30073094367981,4.8847165676960624e-05
29129,58259,58258,116517,20.361204147338867,4.86921743226596e-05
29229,58459,58458,116917,20.42389416694641,4.853806817981771e-05
29329,58659,58658,117317,20.489437103271484,4.838483646400338e-05
29429,58859,58858,117717,20.552964210510254,4.823246856530781e-05
29530,59061,59060,118121,20.614126205444336,4.807944317543942e-05
29630,59261,59260,118521,20.675737142562866,4.7928780146489794e-05
29730,59461,59460,118921,20.734943151474,4.77789500257163e-05
29830,59661,59660,119321,20.793910026550293,4.762994287589807e-05
29930,59861,59860,119721,20.86021399497986,4.74817489207553e-05
30030,60061,60060,120121,20.92821192741394,4.7334358542261396e-05
30130,60261,60260,120521,21.000325918197632,4.7187762277395645e-05
30230,60461,60460,120921,21.059906005859375,4.704195081676821e-05
30330,60661,60660,121321,21.11972212791443,4.689691500079174e-05
30430,60861,60860,121721,21.179396152496338,4.6752645817759055e-05
30531,61063,61062,122125,21.240628957748413,4.66077030845435e-05
30631,61263,61262,122525,21.300339937210083,4.6464948158740704e-05
30731,61463,61462,122925,21.360275983810425,4.632293360830165e-05
30831,61663,61662,123325,21.4247989654541,4.6181650990126026e-05
30931,61863,61862,123725,21.489184141159058,4.604109199664402e-05
31031,62063,62062,124125,21.549930095672607,4.590124845406999e-05
31131,62263,62262,124525,21.626277923583984,4.576211231931207e-05
31231,62463,62462,124925,21.70211410522461,4.5623675679175676e-05
31331,62663,62662,125325,21.764585971832275,4.5485930746875977e-05
31431,62863,62862,125725,21.823428869247437,4.534886986040284e-05
31532,63065,63064,126129,21.884209871292114,4.521112502764261e-05
31632,63265,63264,126529,21.945003032684326,4.5075416389486785e-05
31732,63465,63464,126929,22.009697198867798,4.494036946647604e-05
31832,63665,63664,127329,22.07280993461609,4.480597707620194e-05
31932,63865,63864,127729,22.133182048797607,4.467223215084162e-05
32032,64065,64064,128129,22.196921825408936,4.453912773524867e-05
32132,64265,64264,128529,22.25826406478882,4.440665698460036e-05
32232,64465,64464,128929,22.318892002105713,4.4274813163455194e-05
32332,64665,64664,129329,22.382190227508545,4.414358964266024e-05
32432,64865,64864,129729,22.442739963531494,4.4012979898811586e-05
32533,65067,65066,130133,22.507764101028442,4.388168053371468e-05
32633,65267,65266,130533,22.56766390800476,4.3752285163802853e-05
32733,65467,65466,130933,22.62724208831787,4.362348455197484e-05
32833,65667,65666,131333,22.68734383583069,4.349527257846508e-05
32933,65867,65866,131733,22.754194974899292,4.336764322057305e-05
33033,66067,66066,132133,22.817228078842163,4.324059055024682e-05
33133,66267,66266,132533,22.87998390197754,4.3114108732870426e-05
33233,66467,66466,132933,22.941440105438232,4.2988192024788874e-05
33333,66667,66666,133333,23.004770040512085,4.286283477379785e-05
33433,66867,66866,133733,23.065598011016846,4.273803141498402e-05
33534,67069,67068,134137,23.12633204460144,4.2612536673078805e-05
33634,67269,67268,134537,23.187089920043945,4.248883015614444e-05
33734,67469,67468,134937,23.24946117401123,4.23656613025213e-05
33834,67669,67668,135337,23.315654039382935,4.224302488806544e-05
33934,67869,67868,135737,23.375306129455566,4.212091576986844e-05
34034,68069,68068,136137,23.435209035873413,4.199932888547904e-05
34134,68269,68268,136537,23.501359939575195,4.187825925009619e-05
34234,68469,68468,136937,23.561525106430054,4.175770195691165e-05
34334,68669,68668,137337,23.62149405479431,4.1637652174587665e-05
34434,68869,68868,137737,23.685164213180542,4.151810514622675e-05
34535,69071,69070,138141,23.762242078781128,4.139786819858964e-05
34635,69271,69270,138541,23.837980031967163,4.1279317611775465e-05
34735,69471,69470,138941,23.900025129318237,4.116125589861157e-05
34835,69671,69670,139341,23.96117091178894,4.104367858893266e-05
34935,69871,69870,139741,24.024566173553467,4.0926581280700996e-05
35035,70071,70070,140141,24.086927890777588,4.080995963938163e-05
35135,70271,70270,140541,24.1510910987854,4.069380939636397e-05
35235,70471,70470,140941,24.21554684638977,4.057812634818032e-05
35335,70671,70670,141341,24.275197982788086,4.0462906354930845e-05
35435,70871,70870,141741,24.336708068847656,4.034814533943403e-05
35536,71073,71072,142145,24.400001049041748,4.023269851009812e-05
35636,71273,71272,142545,24.465681076049805,4.0118847955303736e-05
35736,71473,71472,142945,24.529128074645996,4.0005444474302674e-05
35836,71673,71672,143345,24.591012239456177,3.989248423133194e-05
35936,71873,71872,143745,24.650862216949463,3.977996344779066e-05
36036,72073,72072,144145,24.710915088653564,3.966787840167345e-05
36136,72273,72272,144545,24.771440982818604,3.9556225426652794e-05
36236,72473,72472,144945,24.835297107696533,3.944500091107113e-05
36336,72673,72672,145345,24.898639917373657,3.9334201296940535e-05
36436,72873,72872,145745,24.958641052246094,3.922382307882055e-05
36537,73075,73074,146149,25.02669405937195,3.911276530013233e-05
36637,73275,73274,146549,25.086930990219116,3.9003223693911626e-05
36737,73475,73474,146949,25.146661043167114,3.889409324269979e-05
36837,73675,73674,147349,25.20660400390625,3.878537064403034e-05
36937,73875,73874,147749,25.265960931777954,3.867705264373247e-05
37037,74075,74074,148149,25.326695919036865,3.8569136035575155e-05
37137,74275,74274,148549,25.386808156967163,3.846161765936627e-05
37237,74475,74474,148949,25.448529958724976,3.8354494401890974e-05
37337,74675,74674,149349,25.516902923583984,3.824776319413055e-05
37437,74875,74874,149749,25.578537940979004,3.814142101205568e-05
37538,75077,75076,150153,25.640088081359863,3.803440725340683e-05
37638,75277,75276,150553,25.70636010169983,3.79288380403949e-05
37738,75477,75476,150953,25.768594980239868,3.782364901093012e-05
37838,75677,75676,151353,25.829385995864868,3.7718837310885584e-05
37938,75877,75876,151753,25.906239986419678,3.7614400127851394e-05
38038,76077,76076,152153,25.98167395591736,3.751033468881929e-05
38138,76277,76276,152553,26.044738054275513,3.740663826028056e-05
38238,76477,76476,152953,26.108609199523926,3.730330814739174e-05
38338,76677,76676,153353,26.169402837753296,3.720034169323855e-05
38438,76877,76876,153753,26.23012113571167,3.709773627867321e-05
38539,77079,77078,154157,26.29254984855652,3.699446865294886e-05
38639,77279,77278,154557,26.356276988983154,3.6892581151433304e-05
38739,77479,77478,154957,26.419641971588135,3.679104702434905e-05
38839,77679,77678,155357,26.486824989318848,3.668986379534003e-05
38939,77879,77878,155757,26.550708055496216,3.6589029022979676e-05
39039,78079,78078,156157,26.614723205566406,3.648854029927933e-05
39139,78279,78278,156557,26.678500175476074,3.638839524956265e-05
39239,78479,78478,156957,26.741147994995117,3.6288591531761835e-05
39339,78679,78678,157357,26.805557012557983,3.61891268352783e-05
39439,78879,78878,157757,26.86624312400818,3.608999888182181e-05
39540,79081,79080,158161,26.925209045410156,3.5990219170194606e-05
39640,79281,79280,158561,26.988821983337402,3.589176130081737e-05
39740,79481,79480,158961,27.054599046707153,3.579363349966635e-05
39840,79681,79680,159361,27.11619806289673,3.569583360914854e-05
39940,79881,79880,159761,27.176886081695557,3.559835949977883e-05
40040,80081,80080,160161,27.23843216896057,3.5501209071416535e-05
40140,80281,80280,160561,27.30005717277527,3.5404380251281975e-05
40240,80481,80480,160961,27.359698057174683,3.5307870994029904e-05
40340,80681,80680,161361,27.425312042236328,3.5211679281427e-05
40440,80881,80880,161761,27.490803003311157,3.511580312144049e-05
40541,81083,81082,162165,27.553033113479614,3.5019286499979554e-05
40641,81283,81282,162565,27.611776113510132,3.492403868100052e-05
40741,81483,81482,162965,27.671313047409058,3.4829100574807754e-05
40841,81683,81682,163365,27.733587980270386,3.4734470291890646e-05
40941,81883,81882,163765,27.796478033065796,3.464014596647524e-05
41041,82083,82082,164165,27.85707402229309,3.45461257568566e-05
41141,82283,82282,164565,27.919551134109497,3.445240784510626e-05
41241,82483,82482,164965,27.98361301422119,3.435899043634538e-05
41341,82683,82682,165365,28.064504146575928,3.426587175791585e-05
41441,82883,82882,165765,28.13604211807251,3.4173050060040944e-05
41542,83085,83084,166169,28.19820809364319,3.4079599835957025e-05
41642,83285,83284,166569,28.258728981018066,3.3987369864515485e-05
41742,83485,83484,166969,28.32262396812439,3.3895431737749304e-05
41842,83685,83684,167369,28.3836190700531,3.380378379178892e-05
41942,83885,83884,167769,28.447817087173462,3.3712424383170477e-05
42042,84085,84084,168169,28.51190710067749,3.3621351888860514e-05
42142,84285,84284,168569,28.572402000427246,3.3530564705567713e-05
42242,84485,84484,168969,28.634758949279785,3.344006124921282e-05
42342,84685,84684,169369,28.69732689857483,3.3349839955396146e-05
42442,84885,84884,169769,28.757309913635254,3.325989927833864e-05
42543,85087,85086,170173,28.817710161209106,3.316934247953814e-05
42643,85287,85286,170573,28.878966093063354,3.307996124134588e-05
42743,85487,85486,170973,28.938889026641846,3.2990856078097836e-05
42843,85687,85686,171373,29.004228115081787,3.2902025516997306e-05
42943,85887,85886,171773,29.067846059799194,3.2813468102134975e-05
43043,86087,86086,172173,29.12875008583069,3.2725182394760776e-05
43143,86287,86286,172573,29.189945936203003,3.2637166973119995e-05
43243,86487,86486,172973,29.249550104141235,3.2549420431910284e-05
43343,86687,86686,173373,29.314621925354004,3.246194138205185e-05
43443,86887,86886,173773,29.374917030334473,3.2374728450169683e-05
43544,87089,87088,174177,29.437520027160645,3.2286912129785224e-05
43644,87289,87288,174577,29.502690076828003,3.220023000499881e-05
43744,87489,87488,174977,29.564358949661255,3.211380995897561e-05
43844,87689,87688,175377,29.625138998031616,3.2027650679817884e-05
43944,87889,87888,175777,29.687814950942993,3.194175087097991e-05
44044,88089,88088,176177,29.748260974884033,3.185610924959775e-05
44144,88289,88288,176577,29.81150507926941,3.177072454766679e-05
44244,88489,88488,176977,29.87224292755127,3.1685595510624095e-05
44344,88689,88688,177377,29.935152053833008,3.1600720897995835e-05
44444,88889,88888,177777,29.99995493888855,3.151609948276434e-05
44545,89091,89090,178181,30.06231999397278,3.14308876253352e-05
44645,89291,89290,178581,30.127152919769287,3.134677147855145e-05
44745,89491,89490,178981,30.206428050994873,3.12629049154091e-05
44845,89691,89690,179381,30.277119159698486,3.117928676108141e-05
44945,89891,89890,179781,30.33815884590149,3.109591585283589e-05
45045,90091,90090,180181,30.40171194076538,3.101279104053156e-05
45145,90291,90290,180581,30.463276147842407,3.092991118627236e-05
45245,90491,90490,180981,30.52742099761963,3.0847275163573484e-05
45345,90691,90690,181381,30.586591958999634,3.076488185817855e-05
45445,90891,90890,181781,30.64703893661499,3.068273016674983e-05
45546,91093,91092,182185,30.70935821533203,3.060000109696152e-05
45646,91293,91292,182585,30.769718170166016,3.051833175864916e-05
45746,91493,91492,182985,30.830543994903564,3.0436900781789743e-05
45846,91693,91692,183385,30.889766931533813,3.035570710759452e-05
45946,91893,91892,183785,30.949860095977783,3.0274749687879228e-05
46046,92093,92092,184185,31.014179229736328,3.019402748502417e-05
46146,92293,92292,184585,31.07537317276001,3.0113539471342186e-05
46246,92493,92492,184985,31.134984970092773,3.0033284629731675e-05
46346,92693,92692,185385,31.194934129714966,2.9953261952689638e-05
46446,92893,92892,185785,31.253893852233887,2.9873470442305168e-05
46547,93095,93094,186189,31.315081119537354,2.97931146568962e-05
46647,93295,93294,186589,31.37522602081299,2.9713784813298593e-05
46747,93495,93494,186989,31.437015056610107,2.9634683191163725e-05
46847,93695,93694,187389,31.504925966262817,2.9555808830914836e-05
46947,93895,93894,187789,31.565916061401367,2.947716078132438e-05
47047,94095,94094,188189,31.626742124557495,2.9398738100701532e-05
47147,94295,94294,188589,31.6867778301239,2.9320539855758794e-05
47247,94495,94494,188989,31.74597716331482,2.9242565122036886e-05
47347,94695,94694,189389,31.80498504638672,2.9164812983457692e-05
47447,94895,94894,189789,31.866416931152344,2.9087282532179822e-05
47548,95097,95096,190193,31.926162004470825,2.9009200884041206e-05
47648,95297,95296,190593,31.98571491241455,2.8932113311716377e-05
47748,95497,95496,190993,32.046512842178345,2.8855244743650734e-05
47848,95697,95696,191393,32.10714411735535,2.877859430446245e-05
47948,95897,95896,191793,32.16607904434204,2.8702161126272125e-05
48048,96097,96096,192193,32.227293968200684,2.862594434899295e-05
48148,96297,96296,192593,32.29750108718872,2.8549943120269324e-05
48248,96497,96496,192993,32.37343215942383,2.8474156594495263e-05
48348,96697,96696,193393,32.435569047927856,2.8398583933947197e-05
48448,96897,96896,193793,32.50310516357422,2.8323224307540278e-05
48549,97099,97098,194197,32.56303906440735,2.8247326486691827e-05
48649,97299,97298,194597,32.622446060180664,2.817239257455151e-05
48749,97499,97498,194997,32.68220806121826,2.8097669238021834e-05
48849,97699,97698,195397,32.742225885391235,2.8023155674178978e-05
48949,97899,97898,195797,32.79985809326172,2.7948851086527247e-05
49049,98099,98098,196197,32.86019992828369,2.7874754684591886e-05
49149,98299,98298,196597,32.91786289215088,2.780086568570416e-05
49249,98499,98498,196997,32.97821593284607,2.7727183311740008e-05
49349,98699,98698,197397,33.04173707962036,2.7653706792183907e-05
49449,98899,98898,197797,33.1019721031189,2.758043536234747e-05
49550,99101,99100,198201,33.16315698623657,2.7506638621631794e-05
49650,99301,99300,198601,33.226613998413086,2.7433777132734744e-05
49750,99501,99500,199001,33.28790092468262,2.7361118467608967e-05
49850,99701,99700,199401,33.34882211685181,2.7288661885254508e-05
49950,99901,99900,199801,33.41244912147522,2.7216406650517186e-05
50050,100101,100100,200201,33.474843978881836,2.7144352033615213e-05
50150,100301,100300,200601,33.53719210624695,2.7072497310831866e-05
50250,100501,100500,201001,33.598244190216064,2.7000841762909114e-05
50350,100701,100700,201401,33.658616065979004,2.6929384677127086e-05
50450,100901,100900,201801,33.718199014663696,2.6858125345551605e-05
50551,101103,101102,202205,33.77887010574341,2.6786353435153334e-05
50651,101303,101302,202605,33.83878207206726,2.6715489468926942e-05
50751,101503,101502,203005,33.90007305145264,2.664482115731684e-05
50851,101703,101702,203405,33.96159315109253,2.6574347812971902e-05
50951,101903,101902,203805,34.026583194732666,2.6504068753598124e-05
51051,102103,102102,204205,34.08673691749573,2.6433983301478658e-05
51151,102303,102302,204605,34.145323038101196,2.6364090784217187e-05
51251,102503,102502,205005,34.20225787162781,2.6294390533643692e-05
51351,102703,102702,205405,34.25861096382141,2.622488188663606e-05
51451,102903,102902,205805,34.31529092788696,2.615556418426677e-05
51552,103105,103104,206209,34.37206411361694,2.6085746457375544e-05
51652,103305,103304,206609,34.444064140319824,2.6016810580009973e-05
51752,103505,103504,207009,34.51768708229065,2.5948063691814663e-05
51852,103705,103704,207409,34.57418608665466,2.587950515238442e-05
51952,103905,103904,207809,34.631526947021484,2.5811134324963e-05
52052,104105,104104,208209,34.691428899765015,2.5742950577323302e-05
52152,104305,104304,208609,34.75179195404053,2.567495328149912e-05
52252,104505,104504,209009,34.81348204612732,2.560714181311486e-05
52352,104705,104704,209409,34.87326002120972,2.5539515552817387e-05
52452,104905,104904,209809,34.933434009552,2.5472073884457064e-05
52553,105107,105106,210213,34.99685883522034,2.5404144546321363e-05
52653,105307,105306,210613,35.05789017677307,2.533707206083591e-05
52753,105507,105506,211013,35.116515159606934,2.5270182337160887e-05
52853,105707,105706,211413,35.176865100860596,2.520347477521847e-05
52953,105907,105906,211813,35.23504996299744,2.5136948778363798e-05
53053,106107,106106,212213,35.294333934783936,2.5070603753709034e-05
53153,106307,106306,212613,35.35459303855896,2.500443911217596e-05
53253,106507,106506,213013,35.41207003593445,2.4938454268183675e-05
53353,106707,106706,213413,35.46925902366638,2.48726486398525e-05
53453,106907,106906,213813,35.530752182006836,2.4807021648456734e-05
53554,107109,107108,214217,35.589913845062256,2.4740919127460702e-05
53654,107309,107308,214617,35.64864420890808,2.4675649460674334e-05
53754,107509,107508,215017,35.71019005775452,2.461055671077888e-05
53854,107709,107708,215417,35.76896905899048,2.4545640312633613e-05
53954,107909,107908,215817,35.82634496688843,2.4480899704857497e-05
54054,108109,108108,216217,35.884624004364014,2.441633432916529e-05
54154,108309,108308,216617,35.94183611869812,2.4351943630693313e-05
54254,108509,108508,217017,36.004230976104736,2.4287727057213384e-05
54354,108709,108708,217417,36.06269598007202,2.422368406037015e-05
54454,108909,108908,217817,36.1186089515686,2.4159814094366667e-05
54555,109111,109110,218221,36.17714786529541,2.4095480511209837e-05
54655,109311,109310,218621,36.234050035476685,2.403195669900347e-05
54755,109511,109510,219021,36.291516065597534,2.396860429375416e-05
54855,109711,109710,219421,36.34851789474487,2.390542276187011e-05
54955,109911,109910,219821,36.409252882003784,2.3842411572404317e-05
55055,110111,110110,220221,36.468438148498535,2.377957019812172e-05
55155,110311,110310,220621,36.53349995613098,2.3716898113502782e-05
55255,110511,110510,221021,36.60826921463013,2.3654394796708936e-05
55355,110711,110710,221421,36.678497076034546,2.3592059728499633e-05
55455,110911,110910,221821,36.736088037490845,2.352989239212878e-05
55556,111113,111112,222225,36.79369306564331,2.3467273115073354e-05
55656,111313,111312,222625,36.85337495803833,2.3405441367879728e-05
55756,111513,111512,223025,36.911197900772095,2.3343775813775845e-05
55856,111713,111712,223425,36.97515797615051,2.3282275946711545e-05
55956,111913,111912,223825,37.048951148986816,2.322094126385062e-05
56056,112113,112112,224225,37.11321187019348,2.3159771263642842e-05
56156,112313,112312,224625,37.1738440990448,2.3098765448635443e-05
56256,112513,112512,225025,37.234411001205444,2.3037923322603186e-05
56356,112713,112712,225425,37.2939510345459,2.2977244392556e-05
56456,112913,112912,225825,37.354856967926025,2.2916728167328615e-05
56557,113115,113114,226229,37.41774106025696,2.285577143627992e-05
56657,113315,113314,226629,37.47979497909546,2.2795580773450657e-05
56757,113515,113514,227029,37.541768074035645,2.2735551352643295e-05
56857,113715,113714,227429,37.60663414001465,2.2675682692531344e-05
56957,113915,113914,227829,37.66718506813049,2.2615974314403126e-05
57057,114115,114114,228229,37.72553300857544,2.2556425741619783e-05
57157,114315,114314,228629,37.784953117370605,2.2497036499421136e-05
57257,114515,114514,229029,37.844940185546875,2.2437806115965838e-05
57357,114715,114714,229429,37.90478014945984,2.2378734121140846e-05
57457,114915,114914,229829,37.96525812149048,2.23198200471003e-05
57558,115117,115116,230233,38.030476093292236,2.2260476655638483e-05
57658,115317,115316,230633,38.09724187850952,2.220187859615511e-05
57758,115517,115516,231033,38.17395806312561,2.2143437062694848e-05
57858,115717,115716,231433,38.27467393875122,2.208515159585446e-05
57958,115917,115916,231833,38.37975811958313,2.2027021738412768e-05
58058,116117,116116,232233,38.45366406440735,2.196904703531825e-05
58158,116317,116316,232633,38.53201413154602,2.1911227033862122e-05
58258,116517,116516,233033,38.603452920913696,2.1853561282433104e-05
58358,116717,116716,233433,38.67583203315735,2.179604933237747e-05
58458,116917,116916,233833,38.814563035964966,2.1738690736792868e-05
58559,117119,117118,234237,38.91707706451416,2.1680913764197943e-05
58659,117319,117318,234637,38.99020600318909,2.16238620660385e-05
58759,117519,117518,235037,39.05570101737976,2.1566962388363205e-05
58859,117719,117718,235437,39.121212005615234,2.1510214291852315e-05
58959,117919,117918,235837,39.194600105285645,2.145361733882728e-05
59059,118119,118118,236237,39.26524019241333,2.1397171093987558e-05
59159,118319,118318,236637,39.33371710777283,2.1340875123504925e-05
59259,118519,118518,237037,39.40707993507385,2.1284728995255595e-05
59359,118719,118718,237437,39.47681403160095,2.1228732279424487e-05
59459,118919,118918,237837,39.5463330745697,2.1172884547671173e-05
59560,119121,119120,238241,39.622212171554565,2.1116629130278112e-05
59660,119321,119320,238641,39.70764708518982,2.1061079567991885e-05
59760,119521,119520,239041,39.79366207122803,2.1005677711233096e-05
59860,119721,119720,239441,39.86970496177673,2.0950423138432683e-05
59960,119921,119920,239841,39.944485902786255,2.0895315430546292e-05
60060,120121,120120,240241,40.02109217643738,2.084035416953603e-05
60160,120321,120320,240641,40.085602045059204,2.0785538939042277e-05
60260,120521,120520,241041,40.154300928115845,2.0730869324710094e-05
60360,120721,120720,241441,40.22001004219055,2.0676344913662552e-05
60460,120921,120920,241841,40.28709411621094,2.0621965294468176e-05
60561,121123,121122,242245,40.36570596694946,2.0567188433262498e-05
60661,121323,121322,242645,40.46163892745972,2.051309860880756e-05
60761,121523,121522,243045,40.59351086616516,2.0459152348164386e-05
60861,121723,121722,243445,40.68087100982666,2.040534924679027e-05
60961,121923,121922,243845,40.761879205703735,2.035168890128138e-05
61061,122123,122122,244245,40.84949994087219,2.0298170909973146e-05
61161,122323,122322,244645,40.93617010116577,2.0244794872959396e-05
61261,122523,122522,245045,41.00992488861084,2.0191560391286615e-05
61361,122723,122722,245445,41.075340032577515,2.013846706802766e-05
61461,122923,122922,245845,41.140610218048096,2.0085514507503593e-05
61562,123125,123124,246249,41.20603799819946,2.0032174901477545e-05
61662,123325,123324,246649,41.26913905143738,1.9979504083596258e-05
61762,123525,123524,247049,41.33357501029968,1.9926972846823785e-05
61862,123725,123724,247449,41.4020721912384,1.9874580801212154e-05
61962,123925,123924,247849,41.46933722496033,1.982232755876665e-05
62062,124125,124124,248249,41.53588318824768,1.977021273223869e-05
62162,124325,124324,248649,41.61472797393799,1.9718235937093582e-05
62262,124525,124524,249049,41.67889213562012,1.9666396788647028e-05
62362,124725,124724,249449,41.74444603919983,1.9614694904457984e-05
62462,124925,124924,249849,41.81407904624939,1.9563129903492418e-05
62563,125127,125126,250253,41.897539138793945,1.95111878088456e-05
62663,125327,125326,250653,41.971031188964844,1.9459896795404316e-05
62763,125527,125526,251053,42.052191972732544,1.9408741525726247e-05
62863,125727,125726,251453,42.143413066864014,1.9357721624437273e-05
62963,125927,125926,251853,42.214234828948975,1.9306836717067964e-05
63063,126127,126126,252253,42.283514976501465,1.9256086430376436e-05
63163,126327,126326,252653,42.355140924453735,1.9205470392660153e-05
63263,126527,126526,253053,42.424036264419556,1.9154988233616504e-05
63363,126727,126726,253453,42.49950385093689,1.9104639584039083e-05
63463,126927,126926,253853,42.571844816207886,1.905442407592919e-05
63564,127129,127128,254257,42.65924406051636,1.900384118471068e-05
63664,127329,127328,254657,42.73374700546265,1.8953892183638294e-05
63764,127529,127528,255057,42.80725407600403,1.890407522448166e-05
63864,127729,127728,255457,42.8773980140686,1.8854389944565315e-05
63964,127929,127928,255857,42.94754910469055,1.8804835982245097e-05
64064,128129,128128,256257,43.02516007423401,1.8755412977338632e-05
64164,128329,128328,256657,43.12477898597717,1.8706120570740475e-05
64264,128529,128528,257057,43.20882201194763,1.865695840461242e-05
64364,128729,128728,257457,43.28218102455139,1.860792612203922e-05
64464,128929,128928,257857,43.35149693489075,1.855902336819472e-05
64565,129131,129130,258261,43.43532919883728,1.850976270343003e-05
64665,129331,129330,258661,43.55033206939697,1.8461119230959207e-05
64765,129531,129530,259061,43.64145112037659,1.841260422389944e-05
64865,129731,129730,259461,43.72235608100891,1.836421733186464e-05
64965,129931,129930,259861,43.79960107803345,1.8315958205267807e-05
65065,130131,130130,260261,43.8638129234314,1.8267826495468693e-05
65165,130331,130330,260661,43.93085598945618,1.8219821855713516e-05
65265,130531,130530,261061,44.007577896118164,1.8171943939394313e-05
65365,130731,130730,261461,44.07643914222717,1.8124192401890763e-05
65465,130931,130930,261861,44.15638709068298,1.807656689920891e-05
65566,131133,131132,262265,44.2262659072876,1.802859272401759e-05
65666,131333,131332,262665,44.30878806114197,1.7981219515825615e-05
65766,131533,131532,263065,44.37558102607727,1.7933971314153006e-05
65866,131733,131732,263465,44.44200921058655,1.7886847779718556e-05
65966,131933,131932,263865,44.508220911026,1.7839848574542793e-05
66066,132133,132132,264265,44.57316207885742,1.7792973360984327e-05
66166,132333,132332,264665,44.645423889160156,1.774622180305548e-05
66266,132533,132532,265065,44.71285796165466,1.7699593565845852e-05
66366,132733,132732,265465,44.77874422073364,1.765308831498967e-05
66466,132933,132932,265865,44.85220503807068,1.7606705718167207e-05
66567,133135,133134,266269,44.921720027923584,1.755998345668219e-05
66667,133335,133334,266669,45.00990700721741,1.7513846390966255e-05
66767,133535,133534,267069,45.08195114135742,1.7467830982985047e-05
66867,133735,133734,267469,45.165651082992554,1.742193690438056e-05
66967,133935,133934,267869,45.24304413795471,1.7376163827261714e-05
67067,134135,134134,268269,45.30722403526306,1.733051142500303e-05
67167,134335,134334,268669,45.37396216392517,1.7284979372039063e-05
67267,134535,134534,269069,45.43927884101868,1.7239567343650374e-05
67367,134735,134734,269469,45.51144599914551,1.7194275015922567e-05
67467,134935,134934,269869,45.58039402961731,1.714910206677827e-05
67568,135137,135136,270273,45.65519309043884,1.7103598235798575e-05
67668,135337,135336,270673,45.72137808799744,1.7058664265164614e-05
67768,135537,135536,271073,45.786109924316406,1.7013848707814715e-05
67868,135737,135736,271473,45.849003076553345,1.6969151245040448e-05
67968,135937,135936,271873,45.91118907928467,1.692457155918788e-05
68068,136137,136136,272273,45.98314094543457,1.6880109333620768e-05
68168,136337,136336,272673,46.06321406364441,1.683576425243439e-05
68268,136537,136536,273073,46.1374249458313,1.6791536000936082e-05
68368,136737,136736,273473,46.21761894226074,1.6747424265589038e-05
68468,136937,136936,273873,46.28481411933899,1.670342873304796e-05
68569,137139,137138,274277,46.350478172302246,1.665911087932783e-05
68669,137339,137338,274677,46.42668604850769,1.6615347972363444e-05
68769,137539,137538,275077,46.54464912414551,1.6571700332197553e-05
68869,137739,137738,275477,46.623708963394165,1.6528167649959238e-05
68969,137939,137938,275877,46.70111894607544,1.6484749617580144e-05
69069,138139,138138,276277,46.76961803436279,1.6441445927369382e-05
69169,138339,138338,276677,46.8310170173645,1.639825627356887e-05
69269,138539,138538,277077,46.89963912963867,1.635518035047111e-05
69369,138739,138738,277477,46.9647171497345,1.6312217853410014e-05
69469,138939,138938,277877,47.034991979599,1.6269368479208947e-05
69570,139141,139140,278281,47.09899187088013,1.6226205128021875e-05
69670,139341,139340,278681,47.15993595123291,1.618358221545783e-05
69770,139541,139540,279081,47.22236394882202,1.6141071517023545e-05
69870,139741,139740,279481,47.29422116279602,1.6098672732901098e-05
69970,139941,139940,279881,47.36868095397949,1.6056385563722527e-05
70070,140141,140140,280281,47.42943000793457,1.601420971158354e-05
70170,140341,140340,280681,47.491909980773926,1.597214487904291e-05
70270,140541,140540,281081,47.55337405204773,1.5930190769403622e-05
70370,140741,140740,281481,47.61780309677124,1.5888347086828253e-05
70470,140941,140940,281881,47.67964005470276,1.5846613537293226e-05
70571,141143,141142,282285,47.73950386047363,1.5804574142821485e-05
70671,141343,141342,282685,47.80331087112427,1.5763061071677336e-05
70771,141543,141542,283085,47.86467003822327,1.572165725098083e-05
70871,141743,141742,283485,47.92683506011963,1.568036238932342e-05
70971,141943,141942,283885,47.99285316467285,1.563917619661719e-05
71071,142143,142142,284285,48.0574312210083,1.5598098383079944e-05
71171,142343,142342,284685,48.122058153152466,1.5557128659879805e-05
71271,142543,142542,285085,48.182312965393066,1.551626673904173e-05
71371,142743,142742,285485,48.2444748878479,1.5475512333340215e-05
71471,142943,142942,285885,48.302847146987915,1.543486515664381e-05
71572,143145,143144,286289,48.36166191101074,1.5393920059972016e-05
71672,143345,143344,286689,48.421552896499634,1.535348755058224e-05
71772,143545,143544,287089,48.483402967453,1.531316141333044e-05
71872,143745,143744,287489,48.544431924819946,1.5272941365183232e-05
71972,143945,143944,287889,48.60335898399353,1.523282712384033e-05
72072,144145,144144,288289,48.66177201271057,1.5192818407997424e-05
72172,144345,144344,288689,48.721412897109985,1.5152914936847771e-05
72272,144545,144544,289089,48.7825448513031,1.5113116430789984e-05
72372,144745,144744,289489,48.84299612045288,1.5073422610793069e-05
72472,144945,144944,289889,48.904239892959595,1.5033833198687016e-05
72573,145147,145146,290293,48.96405792236328,1.4993953589126237e-05
72673,145347,145346,290693,49.02584910392761,1.4954573198261597e-05
72773,145547,145546,291093,49.08558106422424,1.4915296382650158e-05
72873,145747,145746,291493,49.143707036972046,1.4876122867020013e-05
72973,145947,145946,291893,49.2022762298584,1.4837052377335046e-05
73073,146147,146146,292293,49.26285696029663,1.4798084639996012e-05
73173,146347,146346,292693,49.32313299179077,1.4759219382225475e-05
73273,146547,146546,293093,49.387080907821655,1.4720456332134343e-05
73373,146747,146746,293493,49.462162017822266,1.4681795218396131e-05
73473,146947,146946,293893,49.531558990478516,1.464323577088099e-05
73574,147149,147148,294297,49.59518003463745,1.4604393650022224e-05
73674,147349,147348,294697,49.65400719642639,1.4566037736105774e-05
73774,147549,147548,295097,49.712162017822266,1.4527782678803756e-05
73874,147749,147748,295497,49.77154207229614,1.4489628210470056e-05
73974,147949,147948,295897,49.829899072647095,1.4451574064646674e-05
74074,148149,148148,296297,49.89012002944946,1.4413619975729352e-05
74174,148349,148348,296697,49.950109004974365,1.4375765677929323e-05
74274,148549,148548,297097,50.01958990097046,1.4338010907430697e-05
74374,148749,148748,297497,50.09098696708679,1.4300355400015598e-05
74474,148949,148948,297897,50.16384792327881,1.4262798893241198e-05
74575,149151,149150,298301,50.23714208602905,1.4224967044582713e-05
74675,149351,149350,298701,50.3080689907074,1.4187608735879116e-05
74775,149551,149550,299101,50.38009190559387,1.4150348640633926e-05
74875,149751,149750,299501,50.453068017959595,1.411318649859706e-05
74975,149951,149950,299901,50.526692152023315,1.4076122050697859e-05
75075,150151,150150,300301,50.59930920600891,1.4039155038217177e-05
75175,150351,150350,300701,50.67139005661011,1.4002285203044059e-05
75275,150551,150550,301101,50.742648124694824,1.396551228814974e-05
75375,150751,150750,301501,50.813210010528564,1.3928836037334154e-05
75475,150951,150950,301901,50.88388800621033,1.3892256194644411e-05
75576,151153,151152,302305,50.96641707420349,1.3855408152760232e-05
75676,151353,151352,302705,51.04253387451172,1.3819021319724948e-05
75776,151553,151552,303105,51.10890293121338,1.378273012937316e-05
75876,151753,151752,303505,51.17459297180176,1.37465343287313e-05
75976,151953,151952,303905,51.23417091369629,1.3710433665364345e-05
76076,152153,152152,304305,51.29582214355469,1.3674427888222097e-05
76176,152353,152352,304705,51.357146978378296,1.3638516746108737e-05
76276,152553,152552,305105,51.41727590560913,1.3602699989017592e-05
76376,152753,152752,305505,51.47824311256409,1.3566977367307783e-05
76476,152953,152952,305905,51.549875020980835,1.3531348632291498e-05
76577,153155,153154,306309,51.62541699409485,1.3495458657206668e-05
76677,153355,153354,306709,51.6894690990448,1.3460017884723614e-05
76777,153555,153554,307109,51.75234889984131,1.3424670254234672e-05
76877,153755,153754,307509,51.810774087905884,1.3389415520023877e-05
76977,153955,153954,307909,51.87255883216858,1.3354253435917976e-05
77077,154155,154154,308309,51.93256616592407,1.331918375795346e-05
77177,154355,154354,308709,51.999232053756714,1.3284206241693176e-05
77277,154555,154554,309109,52.061965227127075,1.3249320643883574e-05
77377,154755,154754,309509,52.121992111206055,1.321452672189924e-05
77477,154955,154954,309909,52.18409514427185,1.3179824233379296e-05
77578,155157,155156,310313,52.26201510429382,1.3144867284058924e-05
77678,155357,155356,310713,52.364274978637695,1.3110347847813236e-05
77778,155557,155556,311113,52.434406995773315,1.3075919120364645e-05
77878,155757,155756,311513,52.49760699272156,1.3041580862856384e-05
77978,155957,155956,311913,52.56014704704285,1.3007332836114578e-05
78078,156157,156156,312313,52.61971092224121,1.2973174802116794e-05
78178,156357,156356,312713,52.681859254837036,1.2939106523417998e-05
78278,156557,156556,313113,52.743342876434326,1.2905127763163407e-05
78378,156757,156756,313513,52.804682970047,1.2871238285231564e-05
78478,156957,156956,313913,52.872211933135986,1.2837437853971156e-05
78579,157159,157158,314317,52.945780992507935,1.2803389565780477e-05
78679,157359,157358,314717,53.015170097351074,1.2769767408582331e-05
78779,157559,157558,315117,53.07935118675232,1.2736233592828765e-05
78879,157759,157758,315517,53.14018702507019,1.2702787885569308e-05
78979,157959,157958,315917,53.2009539604187,1.266943005464994e-05
79079,158159,158158,316317,53.26300406455994,1.263615986810437e-05
79179,158359,158358,316717,53.32847499847412,1.2602977095002604e-05
79279,158559,158558,317117,53.39084506034851,1.2569881504720002e-05
79379,158759,158758,317517,53.450828075408936,1.253687286739442e-05
79479,158959,158958,317917,53.516319036483765,1.2503950953878767e-05
79580,159161,159160,318321,53.57790017127991,1.2470787617383913e-05
79680,159361,159360,318721,53.63758587837219,1.2438039327649303e-05
79780,159561,159560,319121,53.71590518951416,1.240537707547421e-05
79880,159761,159760,319521,53.788382053375244,1.237280063375178e-05
79980,159961,159960,319921,53.84899401664734,1.2340309776876111e-05
80080,160161,160160,320321,53.90836715698242,1.2307904278813797e-05
80180,160361,160360,320721,53.97010803222656,1.2275583914711291e-05
80280,160561,160560,321121,54.036465883255005,1.2243348460431628e-05
80380,160761,160760,321521,54.10026407241821,1.221119769218869e-05
80480,160961,160960,321921,54.16195511817932,1.2179131386483536e-05
80581,161163,161162,322325,54.222883224487305,1.2146829925215369e-05
80681,161363,161362,322725,54.28583908081055,1.2114932717436678e-05
80781,161563,161562,323125,54.34552812576294,1.2083119304311862e-05
80881,161763,161762,323525,54.40606498718262,1.205138946520942e-05
80981,161963,161962,323925,54.46708297729492,1.2019742980131977e-05
81081,162163,162162,324325,54.53352499008179,1.1988179629343102e-05
81181,162363,162362,324725,54.5942862033844,1.1956699193857707e-05
81281,162563,162562,325125,54.6559271812439,1.1925301455426336e-05
81381,162763,162762,325525,54.71763205528259,1.1893986196231848e-05
81481,162963,162962,325925,54.78127121925354,1.1862753198888453e-05
81582,163165,163164,326329,54.843661069869995,1.1831291150946348e-05
81682,163365,163364,326729,54.90649700164795,1.1800222845606567e-05
81782,163565,163564,327129,54.97090697288513,1.1769236151740224e-05
81882,163765,163764,327529,55.03459620475769,1.1738330854899474e-05
81982,163965,163964,327929,55.098690032958984,1.1707506740377812e-05
82082,164165,164164,328329,55.16075611114502,1.1676763594383616e-05
82182,164365,164364,328729,55.22142791748047,1.1646101204224468e-05
82282,164565,164564,329129,55.284862995147705,1.161551935693326e-05
82382,164765,164764,329529,55.34860706329346,1.1585017840624047e-05
82482,164965,164964,329929,55.410505056381226,1.1554596443897515e-05
82583,165167,165166,330333,55.477620124816895,1.1523951943227812e-05
82683,165367,165366,330733,55.539631843566895,1.1493690949118079e-05
82783,165567,165566,331133,55.60016894340515,1.1463509441390283e-05
82883,165767,165766,331533,55.66121697425842,1.1433407210656454e-05
82983,165967,165966,331933,55.733959913253784,1.1403384048218123e-05
83083,166167,166166,332333,55.81354594230652,1.1373439746596062e-05
83183,166367,166366,332733,55.90067195892334,1.1343574097645675e-05
83283,166567,166566,333133,55.971961975097656,1.131378689441373e-05
83383,166767,166766,333533,56.06272220611572,1.1284077930830338e-05
83483,166967,166966,333933,56.13110399246216,1.1254447000641382e-05
83584,167169,167168,334337,56.2074408531189,1.1224598760195044e-05
83684,167369,167368,334737,56.27086400985718,1.11951240568669e-05
83784,167569,167568,335137,56.33277606964111,1.1165726770648461e-05
83884,167769,167768,335537,56.398136138916016,1.1136406698171625e-05
83984,167969,167968,335937,56.46111798286438,1.1107163635669422e-05
84084,168169,168168,336337,56.52499008178711,1.1077997381037363e-05
84184,168369,168368,336737,56.592005014419556,1.1048907731975638e-05
84284,168569,168568,337137,56.6559739112854,1.1019894487093157e-05
84384,168769,168768,337537,56.71983313560486,1.0990957445159922e-05
84484,168969,168968,337937,56.782668113708496,1.0962096405986309e-05
84585,169171,169170,338341,56.85440015792847,1.0933023699233323e-05
84685,169371,169370,338741,56.918915033340454,1.0904314820877476e-05
84785,169571,169570,339141,56.98477816581726,1.0875681345230212e-05
84885,169771,169770,339541,57.054137229919434,1.0847123073347615e-05
84985,169971,169970,339941,57.12385416030884,1.0818639808014849e-05
85085,170171,170170,340341,57.223886251449585,1.0790231351637085e-05
85185,170371,170370,340741,57.34209203720093,1.0761897507666352e-05
85285,170571,170570,341141,57.41559982299805,1.0733638079534253e-05
85385,170771,170770,341541,57.48238706588745,1.0705452871767683e-05
85485,170971,170970,341941,57.55517601966858,1.067734168925997e-05
85586,171173,171172,342345,57.6290819644928,1.064902433568676e-05
85686,171373,171372,342745,57.70120406150818,1.0621061355043744e-05
85786,171573,171572,343145,57.76696705818176,1.059317181518744e-05
85886,171773,171772,343545,57.834681034088135,1.0565355523073603e-05
85986,171973,171972,343945,57.9016489982605,1.0537612285765303e-05
86086,172173,172172,344345,57.98109221458435,1.0509941911292575e-05
86186,172373,172372,344745,58.06200194358826,1.0482344208128958e-05
86286,172573,172572,345145,58.12554097175598,1.0454818985153182e-05
86386,172773,172772,345545,58.19473910331726,1.0427366051932911e-05
86486,172973,172972,345945,58.25661110877991,1.0399985217957848e-05
86587,173175,173174,346349,58.321529150009155,1.0372403567356618e-05
86687,173375,173374,346749,58.383257150650024,1.0345167080779708e-05
86787,173575,173574,347149,58.453930139541626,1.0318002124323727e-05
86887,173775,173774,347549,58.52028799057007,1.0290908510408078e-05
86987,173975,173974,347949,58.58262896537781,1.0263886051489661e-05
87087,174175,174174,348349,58.654279947280884,1.023693456009163e-05
87187,174375,174374,348749,58.74740719795227,1.0210053849828041e-05
87287,174575,174574,349149,58.82279706001282,1.0183243734818245e-05
87387,174775,174774,349549,58.886335134506226,1.0156504029432973e-05
87487,174975,174974,349949,58.95944809913635,1.0129834548314839e-05
87588,175177,175176,350353,59.03487801551819,1.0102969465708931e-05
87688,175377,175376,350753,59.10231614112854,1.0076440577754233e-05
87788,175577,175576,351153,59.17583394050598,1.0049981359889729e-05
87888,175777,175776,351553,59.27949905395508,1.0023591629317674e-05
87988,175977,175976,351953,59.38219404220581,9.997271203206732e-06
88088,176177,176176,352353,59.46260905265808,9.971019899275373e-06
88188,176377,176376,352753,59.52503991127014,9.944837536108938e-06
88288,176577,176576,353153,59.58541393280029,9.918723932113912e-06
88388,176777,176776,353553,59.66006088256836,9.892678906949668e-06
88488,176977,176976,353953,59.72267198562622,9.86670228002259e-06
88589,177179,177178,354357,59.80564522743225,9.840535131651284e-06
88689,177379,177378,354757,59.895848989486694,9.814695442258035e-06
88789,177579,177578,355157,59.965404987335205,9.788923611639064e-06
88889,177779,177778,355557,60.02500295639038,9.763219461283837e-06
88989,177979,177978,355957,60.09770917892456,9.737582813622028e-06
89089,178179,178178,356357,60.169198989868164,9.71201349078275e-06
89189,178379,178378,356757,60.22980213165283,9.686511316281724e-06
89289,178579,178578,357157,60.28949785232544,9.661076113395552e-06
89389,178779,178778,357557,60.346922159194946,9.635707706140528e-06
89489,178979,178978,357957,60.40296912193298,9.610405919055778e-06
89590,179181,179180,358361,60.463566064834595,9.584918558584647e-06
89690,179381,179380,358761,60.52304410934448,9.559750148907463e-06
89790,179581,179580,359161,60.58046913146973,9.534647833836196e-06
89890,179781,179780,359561,60.64058709144592,9.509611439370758e-06
89990,179981,179980,359961,60.69972801208496,9.484640792811653e-06
90090,180181,180180,360361,60.7566180229187,9.459735720964691e-06
90190,180381,180380,360761,60.81454014778137,9.434896051772496e-06
90290,180581,180580,361161,60.871915102005005,9.41012161331594e-06
90390,180781,180780,361561,60.92906904220581,9.385412234062858e-06
90490,180981,180980,361961,60.991580963134766,9.360767743141195e-06
90591,181183,181182,362365,61.05205798149109,9.335942498442284e-06
90691,181383,181382,362765,61.10981798171997,9.311427917734878e-06
90791,181583,181582,363165,61.173251152038574,9.286977713627531e-06
90891,181783,181782,363565,61.23197293281555,9.262591716663786e-06
90991,181983,181982,363965,61.291651248931885,9.238269758334862e-06
91091,182183,182182,364365,61.34740400314331,9.214011670239104e-06
91191,182383,182382,364765,61.40494108200073,9.189817284931266e-06
91291,182583,182582,365165,61.46318221092224,9.165686434584442e-06
91391,182783,182782,365565,61.51978397369385,9.141618952547733e-06
91491,182983,182982,365965,61.57594299316406,9.117614672312289e-06
91592,183185,183184,366369,61.63368511199951,9.093434332876992e-06
91692,183385,183384,366769,61.69197392463684,9.069556586098724e-06
91792,183585,183584,367169,61.749796867370605,9.045741542650036e-06
91892,183785,183784,367569,61.80956697463989,9.021989037697424e-06
91992,183985,183984,367969,61.867374897003174,8.998298906767125e-06
92092,184185,184184,368369,61.92514705657959,8.974670986220466e-06
92192,184385,184384,368769,61.98847484588623,8.951105112489225e-06
92292,184585,184584,369169,62.04955816268921,8.927601122714584e-06
92392,184785,184784,369569,62.1106071472168,8.904158854121014e-06
92492,184985,184984,369969,62.172420263290405,8.880778144547698e-06
92593,185187,185186,370373,62.249412059783936,8.857225948945374e-06
92693,185387,185386,370773,62.32385206222534,8.833968484521094e-06
92793,185587,185586,371173,62.38503408432007,8.810772093657265e-06
92893,185787,185786,371573,62.44967818260193,8.787636616030929e-06
92993,185987,185986,371973,62.51503801345825,8.76456189144025e-06
93093,186187,186186,372373,62.57600688934326,8.74154776047529e-06
93193,186387,186386,372773,62.63807392120361,8.718594063931502e-06
93293,186587,186586,373173,62.70024085044861,8.69570064296409e-06
93393,186787,186786,373573,62.75999402999878,8.672867339118376e-06
93493,186987,186986,373973,62.82198190689087,8.650093994644548e-06
93594,187189,187188,374377,62.88219404220581,8.627153618231377e-06
93694,187389,187388,374777,62.94294619560242,8.604500315880699e-06
93794,187589,187588,375177,63.007352113723755,8.581906500167287e-06
93894,187789,187788,375577,63.068793058395386,8.559372014568675e-06
93994,187989,187988,375977,63.129430055618286,8.536896703382973e-06
94094,188189,188188,376377,63.192564964294434,8.51448041113686e-06
94194,188389,188388,376777,63.253337144851685,8.492122982742851e-06
94294,188589,188588,377177,63.3152379989624,8.469824263595075e-06
94394,188789,188788,377577,63.3754780292511,8.447584099478365e-06
94494,188989,188988,377977,63.43884015083313,8.425402336658989e-06
94595,189191,189190,378381,63.50341987609863,8.403057880107026e-06
94695,189391,189390,378781,63.567315101623535,8.380993040051644e-06
94795,189591,189590,379181,63.629010915756226,8.358986140706932e-06
94895,189791,189790,379581,63.68923592567444,8.337037029693978e-06
94995,189991,189990,379981,63.75510501861572,8.315145555526873e-06
95095,190191,190190,380381,63.816511154174805,8.293311566688538e-06
95195,190391,190390,380781,63.87701416015625,8.271534912131095e-06
95295,190591,190590,381181,63.93740105628967,8.249815441257319e-06
95395,190791,190790,381581,64.00578308105469,8.228153003993022e-06
95495,190991,190990,381981,64.07020401954651,8.20654745034469e-06
95596,191193,191192,382385,64.1295530796051,8.18478342861278e-06
95696,191393,191392,382785,64.20947313308716,8.163291759574838e-06
95796,191593,191592,383185,64.30380201339722,8.141856525790952e-06
95896,191793,191792,383585,64.38137602806091,8.120477578772226e-06
95996,191993,191992,383985,64.45665216445923,8.099154771029846e-06
96096,192193,192192,384385,64.52126121520996,8.077887954753892e-06
96196,192393,192392,384785,64.58236289024353,8.056676983023173e-06
96296,192593,192592,385185,64.64344310760498,8.035521709281445e-06
96396,192793,192792,385585,64.70583295822144,8.01442198711689e-06
96496,192993,192992,385985,64.77690815925598,7.993377670530982e-06
96597,193195,193194,386389,64.87492203712463,7.972179002151493e-06
96697,193395,193394,386789,64.9681601524353,7.951245611324585e-06
96797,193595,193594,387189,65.0380539894104,7.930367189221866e-06
96897,193795,193794,387589,65.10066103935242,7.909543591465406e-06
96997,193995,193994,387989,65.16144490242004,7.888774674113965e-06
97097,194195,194194,388389,65.22143006324768,7.868060293792467e-06
97197,194395,194394,388789,65.28319811820984,7.847400306949162e-06
97297,194595,194594,389189,65.34560585021973,7.82679457074163e-06
97397,194795,194794,389589,65.43794202804565,7.806242942921378e-06
97497,194995,194994,389989,65.53986597061157,7.785745281091523e-06
97598,195197,195196,390393,65.61782884597778,7.765097276632814e-06
97698,195397,195396,390793,65.68192100524902,7.744707658473797e-06
97798,195597,195596,391193,65.74933505058289,7.724371580820378e-06
97898,195797,195796,391593,65.81123518943787,7.704088903287185e-06
97998,195997,195996,391993,65.87289309501648,7.683859485397779e-06
98098,196197,196196,392393,65.93844103813171,7.66368318755156e-06
98198,196397,196396,392793,66.00352120399475,7.643559869844438e-06
98298,196597,196596,393193,66.06980109214783,7.623489393519238e-06
98398,196797,196796,393593,66.16812109947205,7.603471619576296e-06
98498,196997,196996,393993,66.2714250087738,7.583506409682425e-06
98599,197199,197198,394397,66.34382605552673,7.563394762203865e-06
98699,197399,197398,394797,66.40471720695496,7.543534788658607e-06
98799,197599,197598,395197,66.47266888618469,7.5237269649544795e-06
98899,197799,197798,395597,66.54924607276917,7.5039711537993115e-06
98999,197999,197998,395997,66.6159610748291,7.484267218548834e-06
99099,198199,198198,396397,66.71374607086182,7.464615023158375e-06
99199,198399,198398,396797,66.81213283538818,7.445014431702537e-06
99299,198599,198598,397197,66.90341520309448,7.425465308523278e-06
99399,198799,198798,397597,66.97349214553833,7.405967518857829e-06
99499,198999,198998,397997,67.04444599151611,7.386520927231448e-06
99600,199201,199200,398401,67.10474300384521,7.366931701973265e-06
99700,199401,199400,398801,67.16728806495667,7.3475876126997645e-06
99800,199601,199600,399201,67.23281407356262,7.3282943183382445e-06
99900,199801,199800,399601,67.32581615447998,7.309051685286365e-06
100000,200001,200000,400001,67.43154215812683,7.289859580783329e-06


==> plot_data/bilinear_matrix_game_n250/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0008831024169921875,2.0175302852282635
200,201,200,401,0.12049603462219238,0.04478652689802895
400,401,400,801,0.20284509658813477,0.01876849959713967
601,602,601,1203,0.2959010601043701,0.010727747668166946
801,802,801,1603,0.4237070083618164,0.006834670046924187
1001,1002,1001,2003,0.5958869457244873,0.0046996607619437004
1201,1202,1201,2403,0.750946044921875,0.003564882185873673
1401,1402,1401,2803,0.876762866973877,0.0027081890851968246
1602,1603,1602,3205,0.9743978977203369,0.001855631651017109
1802,1803,1802,3605,1.0715441703796387,0.0014061223319154967
2002,2003,2002,4005,1.1632349491119385,0.0010943812851285626
2202,2203,2202,4405,1.2528870105743408,0.0009419078130188925
2402,2403,2402,4805,1.3943300247192383,0.0008516517817800815
2603,2604,2603,5207,1.5030009746551514,0.0007836220906947915
2803,2804,2803,5607,1.5856258869171143,0.0007337162996024967
3003,3004,3003,6007,1.6683039665222168,0.0006843837934935394
3203,3204,3203,6407,1.7451019287109375,0.000621430620659287
3403,3404,3403,6807,1.8288710117340088,0.0005738291089869442
3604,3605,3604,7209,1.9163148403167725,0.0005386157069433298
3804,3805,3804,7609,1.9980790615081787,0.0005102432591415502
4004,4005,4004,8009,2.08270001411438,0.0004859931252849459
4204,4205,4204,8409,2.16211199760437,0.0004647943297305488
4404,4405,4404,8809,2.245716094970703,0.0004460128472459026
4605,4606,4605,9211,2.378455877304077,0.0004291432956780943
4805,4806,4805,9611,2.500087022781372,0.00041404377633446406
5005,5006,5005,10011,2.6060659885406494,0.0004003897550704579
5205,5206,5205,10411,2.692835807800293,0.00038799322043170777
5405,5406,5405,10811,2.7805190086364746,0.0003766997750865513
5606,5607,5606,11213,2.877800941467285,0.0003663304164950251
5806,5807,5806,11613,2.9619860649108887,0.00035687721271075555
6006,6007,6006,12013,3.075845956802368,0.0003481906656339682
6206,6207,6206,12413,3.183511972427368,0.00034018745892135376
6406,6407,6406,12813,3.3075931072235107,0.0003327945029156792
6607,6608,6607,13215,3.4310169219970703,0.000325914425714135
6807,6808,6807,13615,3.5302951335906982,0.00031955852168277804
7007,7008,7007,14015,3.611382007598877,0.00031364081882276855
7207,7208,7207,14415,3.6889679431915283,0.0003081165565063809
7407,7408,7407,14815,3.7686169147491455,0.00030294595791825675
7608,7609,7608,15217,3.8599209785461426,0.0002980701275253528
7808,7809,7808,15617,4.004011154174805,0.0002935059691853229
8008,8009,8008,16017,4.111639976501465,0.0002892004304440692
8208,8209,8208,16417,4.216598987579346,0.0002851285393824211
8408,8409,8408,16817,4.307560920715332,0.00028126803576462617
8609,8610,8609,17219,4.39081883430481,0.00027758117322436584
8809,8810,8809,17619,4.529435873031616,0.00027408685490339953
9009,9010,9009,18019,4.703139781951904,0.0002707504714707638
9209,9210,9209,18419,4.801892995834351,0.0002675579071072609
9409,9410,9409,18819,4.908695936203003,0.0002644965460433607
9610,9611,9610,19221,5.035598993301392,0.00026154068254627383
9810,9811,9810,19621,5.14483904838562,0.0002587095917783479
10010,10011,10010,20021,5.2472779750823975,0.0002559792390777811
10210,10211,10210,20421,5.417272090911865,0.00025334152331706045
10410,10411,10410,20821,5.535682201385498,0.00025078917689414995
10611,10612,10611,21223,5.65929388999939,0.00024830349446085443
10811,10812,10811,21623,5.764245986938477,0.000245903320786389
11011,11012,11011,22023,5.841943025588989,0.00024357082283191648
11211,11212,11211,22423,5.921584844589233,0.0002413012497644246
11411,11412,11411,22823,6.005275011062622,0.0002390903176070361
11612,11613,11612,23225,6.084932804107666,0.00023692350957163374
11812,11813,11812,23625,6.163479804992676,0.000234818876188913
12012,12013,12012,24025,6.274410009384155,0.00023276234079066868
12212,12213,12212,24425,6.4124720096588135,0.00023075103695135703
12412,12413,12412,24825,6.522176027297974,0.0002287823631151437
12613,12614,12613,25227,6.597858190536499,0.0002268444101240626
12813,12814,12813,25627,6.675458192825317,0.0002249543001830085
13013,13014,13013,26027,6.750562906265259,0.00022310033153375412
13213,13214,13213,26427,6.829948902130127,0.00022128071310333408
13413,13414,13413,26827,6.919861078262329,0.00021949380670303125
13614,13615,13614,27229,7.059284925460815,0.00021772940904341104
13814,13815,13814,27629,7.1755030155181885,0.00021600369343878668
14014,14015,14014,28029,7.25197696685791,0.00021430653915116896
14214,14215,14214,28429,7.325778007507324,0.00021263678034784885
14414,14415,14414,28829,7.399510145187378,0.0002109933413399964
14615,14616,14615,29231,7.494488954544067,0.00020936719927568728
14815,14816,14815,29631,7.605759143829346,0.0002077736101569283
15015,15016,15015,30031,7.699090003967285,0.00020620356714784883
15215,15216,15215,30431,7.777405023574829,0.00020465627632769098
15415,15416,15415,30831,7.859264135360718,0.000203130998293746
15616,15617,15616,31233,7.940685987472534,0.00020161957581777
15816,15817,15816,31633,8.017739057540894,0.0002001364003753276
16016,16017,16016,32033,8.092456102371216,0.00019867329583096713
16216,16217,16216,32433,8.171181917190552,0.00019722969554983585
16416,16417,16416,32833,8.246679782867432,0.00019580506686676602
16617,16618,16617,33235,8.324879884719849,0.00019439192294999017
16817,16818,16817,33635,8.399815082550049,0.00019300384976726458
17017,17018,17017,34035,8.475190162658691,0.00019163332384738367
17217,17218,17217,34435,8.548149108886719,0.00019027992188536436
17417,17418,17417,34835,8.625688791275024,0.00018894324247093898
17618,17619,17618,35237,8.706074953079224,0.00018761634308815523
17818,17819,17818,35637,8.780152797698975,0.00018631206254184643
18018,18019,18018,36037,8.854882001876831,0.00018502341330576148
18218,18219,18218,36437,8.931019067764282,0.00018375006570833902
18418,18419,18418,36837,9.01211404800415,0.0001824917047254518
18619,18620,18619,37239,9.085239171981812,0.00018124184694090495
18819,18820,18819,37639,9.161256074905396,0.00018001263874275233
19019,19020,19019,38039,9.255383968353271,0.00017879754841943784
19219,19220,19219,38439,9.339904069900513,0.00017759630984320028
19419,19420,19419,38839,9.418071031570435,0.0001764086670745427
19620,19621,19620,39241,9.497464895248413,0.000175228535364549
19820,19821,19820,39641,9.573375940322876,0.00017406741883776853
20020,20021,20020,40041,9.648216962814331,0.00017291918390125387
20220,20221,20220,40441,9.722985982894897,0.00017178360927004832
20420,20421,20420,40841,9.802890062332153,0.00017066048102396057
20621,20622,20621,41243,9.882990837097168,0.00016954406814495123
20821,20822,20821,41643,9.968230962753296,0.00016844527794923606
21021,21022,21021,42043,10.049038887023926,0.0001673583314685384
21221,21222,21221,42443,10.12700605392456,0.0001662830402869128
21421,21422,21421,42843,10.208755016326904,0.00016521922150953457
21622,21623,21622,43245,10.288034915924072,0.0001641614629402783
21822,21823,21822,43645,10.36751389503479,0.00016312011613611507
22022,22023,22022,44045,10.44872498512268,0.0001620897225734824
22222,22223,22222,44445,10.536749839782715,0.0001610701187869821
22422,22423,22422,44845,10.643959999084473,0.00016006114558607382
22623,22624,22623,45247,10.781828880310059,0.000159057681431108
22823,22824,22823,45647,10.911773920059204,0.00015806955919467862
23023,23024,23023,46047,11.035829067230225,0.00015709161296936859
23223,23224,23223,46447,11.120351076126099,0.00015612369882119328
23423,23424,23423,46847,11.200459003448486,0.00015516567621955306
23624,23625,23624,47249,11.281244039535522,0.00015421269083493608
23824,23825,23824,47649,11.383264064788818,0.00015327409041627737
24024,24025,24024,48049,11.531846046447754,0.00015234497834770155
24224,24225,24224,48449,11.663513898849487,0.00015142522639086814
24424,24425,24424,48849,11.76941180229187,0.00015051470908089608
24625,24626,24625,49251,11.883808135986328,0.00014960881928547922
24825,24826,24825,49651,11.997035026550293,0.0001487164501126954
25025,25026,25025,50051,12.10321307182312,0.00014783295423499924
25225,25226,25225,50451,12.23271894454956,0.00014695821630477903
25425,25426,25425,50851,12.340255975723267,0.00014609212327915575
25626,25627,25626,51253,12.47423005104065,0.00014523029780489532
25826,25827,25826,51653,12.601628065109253,0.000144381206144761
26026,26027,26026,52053,12.728004932403564,0.0001435404327899102
26226,26227,26226,52453,12.882900953292847,0.00014270787317310877
26426,26427,26426,52853,13.02777099609375,0.00014188342467383932
26627,26628,26627,53255,13.160400867462158,0.00014106292432481763
26827,26828,26827,53655,13.296576976776123,0.00014025443699057426
27027,27028,27027,54055,13.437337875366211,0.0001394537635074081
27227,27228,27227,54455,13.55974793434143,0.00013866080846049175
27427,27428,27427,54855,13.649142980575562,0.00013787547810154065
27628,27629,27628,55257,13.728205919265747,0.00013709381008254016
27828,27829,27828,55657,13.807626962661743,0.00013632349125976612
28028,28029,28028,56057,13.890321016311646,0.000135560524954989
28228,28229,28228,56457,13.9719979763031,0.00013480482362331078
28428,28429,28428,56857,14.054435968399048,0.00013405630116166174
28629,28630,28629,57259,14.142336130142212,0.0001333111834121381
28829,28830,28829,57659,14.246279954910278,0.00013257680080252073
29029,29030,29029,58059,14.329503059387207,0.00013184934661522748
29229,29230,29229,58459,14.40976595878601,0.00013112874014536353
29429,29430,29429,58859,14.491132974624634,0.00013041490194906852
29630,29631,29630,59261,14.573677062988281,0.00012970423474908816
29830,29831,29830,59661,14.65652585029602,0.00012900373252629438
30030,30031,30030,60061,14.736051082611084,0.00012830976712002569
30230,30231,30230,60461,14.820665836334229,0.0001276222638275209
30430,30431,30430,60861,14.94722318649292,0.00012694114905889648
30631,30632,30631,61263,15.037583827972412,0.0001262629920642769
30831,30832,30831,61663,15.115169048309326,0.00012559446893549512
31031,31032,31031,62063,15.189738035202026,0.00012493211962466455
31231,31232,31231,62463,15.269076108932495,0.0001242758747413995
31431,31432,31431,62863,15.352334976196289,0.00012362566588363646
31632,31633,31632,63265,15.43562388420105,0.00012297821930005854
31832,31833,31832,63665,15.508949995040894,0.00012233991048153504
32032,32033,32032,64065,15.584118127822876,0.00012170743787703473
32232,32233,32232,64465,15.673862934112549,0.00012108073683266719
32432,32433,32432,64865,15.760732889175415,0.00012045974358089348
32633,32634,32633,65267,15.837193965911865,0.00011984133255828426
32833,32834,32833,65667,15.947982788085938,0.00011923159480041812
33033,33034,33033,66067,16.086374044418335,0.0001186273783612972
33233,33234,33233,66467,16.216865062713623,0.00011802862284136297
33433,33434,33433,66867,16.30769109725952,0.00011743526863959277
33634,33635,33634,67269,16.38527202606201,0.00011684433020463652
33834,33835,33834,67669,16.457973957061768,0.00011626162923078444
34034,34035,34034,68069,16.535773038864136,0.0001156841551247771
34234,34235,34234,68469,16.628818035125732,0.00011511185133113707
34434,34435,34434,68869,16.72135901451111,0.00011454466201889047
34635,34636,34635,69271,16.80422306060791,0.00011397973403805185
34835,34836,34835,69671,16.889918088912964,0.00011342263391541219
35035,35036,35035,70071,16.9703209400177,0.0001128704847270032
35235,35236,35235,70471,17.05233907699585,0.00011232323341223033
35435,35436,35435,70871,17.128280878067017,0.00011178082757014295
35636,35637,35636,71273,17.21573519706726,0.0001112405393460803
35836,35837,35836,71673,17.3018000125885,0.00011070769341683268
36036,36037,36036,72073,17.381528854370117,0.00011017953935532546
36236,36237,36236,72473,17.4526150226593,0.00010965602729298843
36436,36437,36436,72873,17.52601718902588,0.0001091371079663427
36637,36638,36637,73275,17.598998069763184,0.00010862017216672441
36837,36838,36837,73675,17.674810886383057,0.00010811031525171424
37037,37038,37037,74075,17.751288175582886,0.00010760490657805096
37237,37238,37237,74475,17.84167981147766,0.0001071038992072625
37437,37438,37437,74875,17.920642137527466,0.00010660724675889057
37638,37639,37638,75277,17.997591972351074,0.00010611245243394272
37838,37839,37838,75677,18.082210779190063,0.00010562439407843234
38038,38039,38038,76077,18.179426908493042,0.00010514055453646331
38238,38239,38238,76477,18.318520069122314,0.00010466088957114157
38438,38439,38438,76877,18.444578170776367,0.00010418535546241655
38639,38640,38639,77279,18.544833183288574,0.00010371156196181448
38839,38840,38839,77679,18.635758876800537,0.00010324418054166516
39039,39040,39039,78079,18.77023482322693,0.0001027808016175643
39239,39240,39239,78479,18.931095123291016,0.00010232138345445304
39439,39440,39439,78879,19.039772987365723,0.00010186588479476518
39640,39641,39640,79281,19.141204118728638,0.00010141201642939574
39840,39841,39840,79681,19.23035192489624,0.00010096425397197347
40040,40041,40040,80081,19.32494282722473,0.00010052028984418028
40240,40241,40240,80481,19.42292594909668,0.00010008008463429918
40440,40441,40440,80881,19.532476902008057,9.964359937337433e-05
40641,40642,40641,81283,19.62502098083496,9.920864069779614e-05
40841,40842,40841,81683,19.717000007629395,9.877949829929947e-05
41041,41042,41041,82083,19.809156894683838,9.835396136279923e-05
41241,41242,41241,82483,19.903674840927124,9.793199263978274e-05
41441,41442,41441,82883,20.00769805908203,9.751355529516753e-05
41642,41643,41642,83285,20.098005056381226,9.709654691218016e-05
41842,41843,41842,83685,20.181541919708252,9.668508065671065e-05
42042,42043,42042,84085,20.263671159744263,9.62770375316916e-05
42242,42243,42242,84485,20.343008041381836,9.587238230831156e-05
42442,42443,42442,84885,20.420871019363403,9.547108014633218e-05
42643,42644,42643,85287,20.507550954818726,9.507111494994549e-05
42843,42844,42843,85687,20.58618402481079,9.46764322514415e-05
43043,43044,43043,86087,20.666361808776855,9.428500020119824e-05
43243,43244,43243,86487,20.747601985931396,9.389678546250573e-05
43443,43444,43443,86887,20.82712411880493,9.351175506177486e-05
43644,43645,43644,87289,20.906795978546143,9.312797485581297e-05
43844,43845,43844,87689,20.99163508415222,9.274923115939283e-05
44044,44045,44044,88089,21.075260877609253,9.237357485832367e-05
44244,44245,44244,88489,21.155706882476807,9.200097439029355e-05
44444,44445,44444,88889,21.239439964294434,9.163139853442863e-05
44645,44646,44645,89291,21.327847003936768,9.126299096701417e-05
44845,44846,44845,89691,21.409576892852783,9.089938675815504e-05
45045,45046,45045,90091,21.49201798439026,9.053871535572686e-05
45245,45246,45245,90491,21.570523023605347,9.018094686580128e-05
45445,45446,45445,90891,21.64850115776062,8.982605171536e-05
45646,45647,45646,91293,21.72933316230774,8.947224748965964e-05
45846,45847,45846,91693,21.810827016830444,8.912302556724162e-05
46046,46047,46046,92093,21.890777826309204,8.877659001126892e-05
46246,46247,46246,92493,21.97556781768799,8.843291249752094e-05
46446,46447,46446,92893,22.06977391242981,8.809196500370597e-05
46647,46648,46647,93295,22.163414001464844,8.775203532486355e-05
46847,46848,46847,93695,22.249400854110718,8.741647830476478e-05
47047,47048,47047,94095,22.331507921218872,8.708356888522966e-05
47247,47248,47247,94495,22.41346788406372,8.67532802213865e-05
47447,47448,47447,94895,22.494573831558228,8.642558575382821e-05
47648,47649,47648,95297,22.57612180709839,8.609883998114885e-05
47848,47849,47848,95697,22.658337116241455,8.577626799914256e-05
48048,48049,48048,96097,22.739909887313843,8.545621208802587e-05
48248,48249,48248,96497,22.822602033615112,8.513864679971089e-05
48448,48449,48448,96897,22.902847051620483,8.482354695528796e-05
48649,48650,48649,97299,22.98941707611084,8.450933043627853e-05
48849,48850,48849,97699,23.069077014923096,8.419909902464256e-05
49049,49050,49049,98099,23.149054050445557,8.389125898630491e-05
49249,49250,49249,98499,23.228686809539795,8.358578619249559e-05
49449,49450,49449,98899,23.312968015670776,8.328265676829103e-05
49650,49651,49650,99301,23.395845890045166,8.298034883202131e-05
49850,49851,49850,99701,23.480364084243774,8.26818469527207e-05
50050,50051,50050,100101,23.560869932174683,8.238561820525842e-05
50250,50251,50250,100501,23.643989086151123,8.209163970748663e-05
50450,50451,50450,100901,23.723180055618286,8.179988881806894e-05
50651,50652,50651,101303,23.800158977508545,8.150890090921825e-05
50851,50852,50851,101703,23.89248275756836,8.122154912387039e-05
51051,51052,51051,102103,23.986531972885132,8.093635833399582e-05
51251,51252,51251,102503,24.07516598701477,8.065330683722813e-05
51451,51452,51451,102903,24.162660837173462,8.037237315940119e-05
51652,51653,51652,103305,24.267250061035156,8.009214709870085e-05
51852,51853,51852,103705,24.351770877838135,7.98153958614352e-05
52052,52053,52052,104105,24.435747861862183,7.954069926096685e-05
52252,52253,52252,104505,24.52430009841919,7.92680367120229e-05
52452,52453,52452,104905,24.603420972824097,7.899738784538442e-05
52653,52654,52653,105307,24.6835720539093,7.872739420379245e-05
52853,52854,52853,105707,24.76341676712036,7.846072226447492e-05
53053,53054,53053,106107,24.846208095550537,7.819600407440881e-05
53253,53254,53253,106507,24.92695188522339,7.793322010616023e-05
53453,53454,53453,106907,25.012013912200928,7.767235103745557e-05
53654,53655,53654,107309,25.093711853027344,7.741208761281565e-05
53854,53855,53854,107709,25.173446893692017,7.715500052003898e-05
54054,54055,54054,108109,25.254040956497192,7.689977147197986e-05
54254,54255,54254,108509,25.334940910339355,7.664638194434872e-05
54454,54455,54454,108909,25.41624093055725,7.639481360610304e-05
54655,54656,54655,109311,25.503758907318115,7.61438039924113e-05
54855,54856,54855,109711,25.582852840423584,7.589583268786947e-05
55055,55056,55055,110111,25.663201093673706,7.564962863625688e-05
55255,55256,55255,110511,25.74322009086609,7.540517426344573e-05
55455,55456,55455,110911,25.821986198425293,7.516245217910972e-05
55656,55657,55656,111313,25.902826070785522,7.492024442034343e-05
55856,55857,55856,111713,25.99095392227173,7.468094391609287e-05
56056,56057,56056,112113,26.071812868118286,7.444332453028067e-05
56256,56257,56256,112513,26.152323961257935,7.42073695898061e-05
56456,56457,56456,112913,26.233736038208008,7.397306259647093e-05
56657,56658,56657,113315,26.324461221694946,7.373922791978346e-05
56857,56858,56857,113715,26.418071031570435,7.350817605088851e-05
57057,57058,57057,114115,26.498764038085938,7.327872358259517e-05
57257,57258,57257,114515,26.577029943466187,7.305085469714894e-05
57457,57458,57457,114915,26.65278697013855,7.282455374198466e-05
57658,57659,57658,115317,26.73037815093994,7.25986853602794e-05
57858,57859,57858,115717,26.807143926620483,7.237548160855203e-05
58058,58059,58058,116117,26.884843111038208,7.215379972950237e-05
58258,58259,58258,116517,26.963917016983032,7.193362471635184e-05
58458,58459,58458,116917,27.04108190536499,7.171494171926677e-05
58659,58660,58659,117319,27.11909008026123,7.149665370228072e-05
58859,58860,58859,117719,27.1958270072937,7.12809180841927e-05
59059,59060,59059,118119,27.271045923233032,7.106663078614305e-05
59259,59260,59259,118519,27.35154414176941,7.085377757066214e-05
59459,59460,59459,118919,27.43084192276001,7.064234434913386e-05
59660,59661,59660,119321,27.50988507270813,7.04312705540779e-05
59860,59861,59860,119721,27.586936950683594,7.022264257005662e-05
60060,60061,60060,120121,27.664318084716797,7.001539312474726e-05
60260,60261,60260,120521,27.740385055541992,6.980950871115826e-05
60460,60461,60460,120921,27.82063388824463,6.960497596325298e-05
60661,60662,60661,121323,27.899882078170776,6.940076902442114e-05
60861,60862,60861,121723,27.9793758392334,6.91989066624089e-05
61061,61062,61061,122123,28.055932998657227,6.899835663758004e-05
61261,61262,61261,122523,28.13402509689331,6.879910613550458e-05
61461,61462,61461,122923,28.209588050842285,6.860114247641028e-05
61662,61663,61662,123325,28.289003133773804,6.840347284622901e-05
61862,61863,61862,123725,28.368034839630127,6.820805164001644e-05
62062,62063,62062,124125,28.454330921173096,6.801387996602056e-05
62262,62263,62262,124525,28.54748797416687,6.782094566770763e-05
62462,62463,62462,124925,28.624649047851562,6.762923671586997e-05
62663,62664,62663,125327,28.703840970993042,6.743779175831863e-05
62863,62864,62863,125727,28.781768083572388,6.72485038930965e-05
63063,63064,63063,126127,28.856557846069336,6.706040597897114e-05
63263,63264,63263,126527,28.932852029800415,6.687348648372273e-05
63463,63464,63463,126927,29.01355504989624,6.668773399591672e-05
63664,63665,63664,127329,29.091745138168335,6.650221712455504e-05
63864,63865,63864,127729,29.168794870376587,6.631877058890159e-05
64064,64065,64064,128129,29.24690318107605,6.61364574834492e-05
64264,64265,64264,128529,29.324352025985718,6.59552668681437e-05
64464,64465,64464,128929,29.40546488761902,6.577518791799872e-05
64665,64666,64665,129331,29.486733198165894,6.559531777946051e-05
64865,64866,64865,129731,29.565805912017822,6.54174355616983e-05
65065,65066,65065,130131,29.645183086395264,6.524063315732268e-05
65265,65266,65265,130531,29.72502899169922,6.506490018873243e-05
65465,65466,65465,130931,29.79925799369812,6.489022638686707e-05
65666,65667,65666,131333,29.877559185028076,6.471573608532318e-05
65866,65867,65866,131733,29.954976081848145,6.454315541007359e-05
66066,66067,66066,132133,30.03234100341797,6.437160368764693e-05
66266,66267,66266,132533,30.107356071472168,6.420107107375229e-05
66466,66467,66466,132933,30.186134099960327,6.403154782756372e-05
66667,66668,66667,133335,30.264997005462646,6.386218418921362e-05
66867,66868,66867,133735,30.342664003372192,6.369465579189391e-05
67067,67068,67067,134135,30.42068576812744,6.35281081026798e-05
67267,67268,67267,134535,30.503714084625244,6.336253178358987e-05
67467,67468,67467,134935,30.593995094299316,6.319791759543655e-05
67668,67669,67668,135337,30.68472719192505,6.303344046842269e-05
67868,67869,67868,135737,30.761645078659058,6.287072790733236e-05
68068,68069,68068,136137,30.837589979171753,6.27089502918304e-05
68268,68269,68268,136537,30.913481950759888,6.254809876510694e-05
68468,68469,68468,136937,30.99388098716736,6.238816456301334e-05
68669,68670,68669,137339,31.074273109436035,6.222834615446276e-05
68869,68870,68869,137739,31.15427303314209,6.207022515635127e-05
69069,69070,69069,138139,31.2361159324646,6.191299569727916e-05
69269,69270,69269,138539,31.31629180908203,6.175664937664303e-05
69469,69470,69469,138939,31.394287824630737,6.16011778815979e-05
69670,69671,69670,139341,31.478402853012085,6.144580212597409e-05
69870,69871,69870,139741,31.55917501449585,6.129205996493087e-05
70070,70071,70070,140141,31.638890027999878,6.113916817214204e-05
70270,70271,70270,140541,31.71678900718689,6.098711877923536e-05
70470,70471,70470,140941,31.798381805419922,6.083590390207905e-05
70671,70672,70671,141343,31.87745213508606,6.0684765862157374e-05
70871,70872,70871,141743,31.964252948760986,6.053520076929896e-05
71071,71072,71071,142143,32.04550886154175,6.038644699480457e-05
71271,71272,71271,142543,32.12396192550659,6.023849698105509e-05
71471,71472,71471,142943,32.20651698112488,6.0091343249464345e-05
71672,71673,71672,143345,32.28747200965881,5.994424854685157e-05
71872,71873,71872,143745,32.36630892753601,5.979866914962293e-05
72072,72073,72072,144145,32.44901990890503,5.965386403302622e-05
72272,72273,72272,144545,32.532268047332764,5.950982602909717e-05
72472,72473,72472,144945,32.61255192756653,5.9366548045045374e-05
72673,72674,72673,145347,32.69681215286255,5.922331231836823e-05
72873,72874,72873,145747,32.79669785499573,5.90815371070149e-05
73073,73074,73073,146147,32.880292892456055,5.8940501047744434e-05
73273,73274,73273,146547,32.96521306037903,5.880019734245497e-05
73473,73474,73473,146947,33.05357599258423,5.866061926368029e-05
73674,73675,73674,147349,33.134254932403564,5.852106765516473e-05
73874,73875,73874,147749,33.21486496925354,5.8382924476626055e-05
74074,74075,74074,148149,33.29492783546448,5.8245487132798064e-05
74274,74275,74274,148549,33.37486290931702,5.810874917559272e-05
74474,74475,74474,148949,33.45612287521362,5.7972704225169004e-05
74675,74676,74675,149351,33.5372748374939,5.783667089169477e-05
74875,74876,74875,149751,33.61662006378174,5.770199646834424e-05
75075,75076,75075,150151,33.6955509185791,5.7567996279863634e-05
75275,75276,75275,150551,33.77832102775574,5.743466421089161e-05
75475,75476,75475,150951,33.8564031124115,5.73019942102215e-05
75676,75677,75676,151353,33.936882972717285,5.716932185897792e-05
75876,75877,75876,151753,34.020718812942505,5.7037961330809366e-05
76076,76077,76076,152153,34.0984411239624,5.690724506755854e-05
76276,76277,76276,152553,34.17979979515076,5.677716726815116e-05
76476,76477,76476,152953,34.25961709022522,5.664772219367532e-05
76677,76678,76677,153355,34.340604066848755,5.6518261641105676e-05
76877,76878,76877,153755,34.424769163131714,5.63900681324997e-05
77077,77078,77077,154155,34.509692907333374,5.626249046277443e-05
77277,77278,77277,154555,34.59125900268555,5.613552313081021e-05
77477,77478,77477,154955,34.673171043395996,5.600916069291289e-05
77678,77679,77678,155357,34.75337100028992,5.588277044546666e-05
77878,77879,77878,155757,34.84217596054077,5.575760465119703e-05
78078,78079,78078,156157,34.94300198554993,5.563302773534676e-05
78278,78279,78278,156557,35.03144598007202,5.550903448005872e-05
78478,78479,78478,156957,35.11827802658081,5.538561972235338e-05
78679,78680,78679,157359,35.19811701774597,5.526216557873743e-05
78879,78880,78879,157759,35.279863119125366,5.513989537255256e-05
79079,79080,79079,158159,35.36023187637329,5.5018188473490145e-05
79279,79280,79279,158559,35.445720911026,5.489703993204642e-05
79479,79480,79479,158959,35.528383016586304,5.477644485141013e-05
79680,79681,79680,159361,35.614418029785156,5.465579952392235e-05
79880,79881,79880,159761,35.70518898963928,5.453629958596505e-05
80080,80081,80080,160161,35.78712821006775,5.441733870051712e-05
80280,80281,80280,160561,35.86912202835083,5.429891217312706e-05
80480,80481,80480,160961,35.950814962387085,5.418101535887664e-05
80681,80682,80681,161363,36.03790903091431,5.4063058114779584e-05
80881,80882,80881,161763,36.11598181724548,5.394620957790516e-05
81081,81082,81081,162163,36.19698476791382,5.382987708743884e-05
81281,81282,81281,162563,36.27899408340454,5.3714056190593805e-05
81481,81482,81481,162963,36.35883402824402,5.359874248125065e-05
81682,81683,81682,163365,36.44224691390991,5.3483358801464176e-05
81882,81883,81882,163765,36.52805209159851,5.336904891532779e-05
82082,82083,82082,164165,36.60699915885925,5.325523325306986e-05
82282,82283,82282,164565,36.687411069869995,5.314190759032265e-05
82482,82483,82482,164965,36.76889610290527,5.302906774833565e-05
82683,82684,82683,165367,36.84950518608093,5.291614900333781e-05
82883,82884,82883,165767,36.93309020996094,5.2804270815807494e-05
83083,83084,83083,166167,37.03491401672363,5.269286615101121e-05
83283,83284,83283,166567,37.12440204620361,5.2581931001994976e-05
83483,83484,83483,166967,37.204638957977295,5.247146140387234e-05
83684,83685,83684,167369,37.282936811447144,5.2360904546793865e-05
83884,83885,83884,167769,37.36454510688782,5.225135660081314e-05
84084,84085,84084,168169,37.44671106338501,5.2142262539445014e-05
84284,84285,84284,168569,37.53071999549866,5.203361856143172e-05
84484,84485,84484,168969,37.6095609664917,5.192542090537031e-05
84685,84686,84685,169371,37.69192099571228,5.181712817989302e-05
84885,84886,84885,169771,37.771737813949585,5.1709814226058195e-05
85085,85086,85085,170171,37.852418184280396,5.1602935526182555e-05
85285,85286,85285,170571,37.93754601478577,5.149648847405787e-05
85485,85486,85485,170971,38.03316402435303,5.1390469500802935e-05
85686,85687,85686,171373,38.110337018966675,5.128434816386314e-05
85886,85887,85886,171773,38.187089920043945,5.117917688809456e-05
86086,86087,86086,172173,38.26246190071106,5.1074423190192124e-05
86286,86287,86286,172573,38.33917188644409,5.097008364846747e-05
86486,86487,86486,172973,38.413886070251465,5.08661548770032e-05
86687,86688,86687,173375,38.49755096435547,5.0762116936507874e-05
86887,86888,86887,173775,38.57399606704712,5.0659001700684e-05
87087,87088,87087,174175,38.65196919441223,5.0556287271015e-05
87287,87288,87287,174575,38.72747182846069,5.045397040122372e-05
87487,87488,87487,174975,38.804770946502686,5.0352047877948285e-05
87688,87689,87688,175377,38.88428020477295,5.0250009842411725e-05
87888,87889,87888,175777,38.96459603309631,5.014886843963249e-05
88088,88089,88088,176177,39.043445110321045,5.00481119280004e-05
88288,88289,88288,176577,39.133360862731934,4.994773722723566e-05
88488,88489,88488,176977,39.22648000717163,4.9847741287811807e-05
88689,88690,88689,177379,39.30248188972473,4.974762393134118e-05
88889,88890,88889,177779,39.378626108169556,4.964837835114046e-05
89089,89090,89089,178179,39.46527600288391,4.954950255986683e-05
89289,89290,89289,178579,39.541452169418335,4.945099363336175e-05
89489,89490,89489,178979,39.61946988105774,4.935284867797949e-05
89690,89691,89690,179381,39.69503593444824,4.925457681335154e-05
89890,89891,89890,179781,39.77126097679138,4.9157153023239795e-05
90090,90091,90090,180181,39.846813917160034,4.906008468798891e-05
90290,90291,90290,180581,39.921870946884155,4.896336903265644e-05
90490,90491,90490,180981,40.00406312942505,4.886700331024598e-05
90691,90692,90691,181383,40.08094000816345,4.877050557829593e-05
90891,90892,90891,181783,40.161118030548096,4.8674833311830626e-05
91091,91092,91091,182183,40.244093894958496,4.857950289529335e-05
91291,91292,91291,182583,40.32598614692688,4.848451169400805e-05
91491,91492,91491,182983,40.40557599067688,4.8389857100470086e-05
91692,91693,91692,183385,40.4888379573822,4.829506576708527e-05
91892,91893,91892,183785,40.57007098197937,4.820107832665457e-05
92092,92093,92092,184185,40.6472430229187,4.810741982061989e-05
92292,92293,92292,184585,40.72266602516174,4.8014087747849376e-05
92492,92493,92492,184985,40.79735517501831,4.7921079633238715e-05
92693,92694,92693,185387,40.87606501579285,4.78279303978405e-05
92893,92894,92893,185787,40.95604419708252,4.773556446505198e-05
93093,93094,93093,186187,41.03342604637146,4.764351520490155e-05
93293,93294,93293,186587,41.115866899490356,4.755178024267786e-05
93493,93494,93493,186987,41.19392800331116,4.746035722810253e-05
93694,93695,93694,187389,41.29188895225525,4.736878904256728e-05
93894,93895,93894,187789,41.38224911689758,4.7277984500203896e-05
94094,94095,94094,188189,41.466525077819824,4.718748498762865e-05
94294,94295,94294,188589,41.544636964797974,4.709728824991651e-05
94494,94495,94494,188989,41.621017932891846,4.700739205520845e-05
94695,94696,94695,189391,41.69918608665466,4.6917346951021994e-05
94895,94896,94895,189791,41.774725914001465,4.682804671365096e-05
95095,95096,95095,190191,41.851755142211914,4.6739040449231476e-05
95295,95296,95295,190591,41.93176507949829,4.6650326016469764e-05
95495,95496,95495,190991,42.01332902908325,4.65619012955308e-05
95696,95697,95696,191393,42.09184908866882,4.647332422196686e-05
95896,95897,95896,191793,42.17249393463135,4.638547407461628e-05
96096,96097,96096,192193,42.25408601760864,4.62979073989207e-05
96296,96297,96296,192593,42.32894492149353,4.6210622160562225e-05
96496,96497,96496,192993,42.40735220909119,4.6123616346403906e-05
96697,96698,96697,193395,42.492279052734375,4.603645501466148e-05
96897,96898,96897,193795,42.56978988647461,4.595000346169595e-05
97097,97098,97097,194195,42.65055012702942,4.5863825404706794e-05
97297,97298,97297,194595,42.728776931762695,4.5777918910961394e-05
97497,97498,97497,194995,42.81455993652344,4.569228206742184e-05
97698,97699,97698,195397,42.90494894981384,4.5606486804786894e-05
97898,97899,97898,195797,42.99353504180908,4.552138492516394e-05
98098,98099,98098,196197,43.07409596443176,4.5436547063727276e-05
98298,98299,98298,196597,43.15143084526062,4.535197138353022e-05
98498,98499,98498,196997,43.230798959732056,4.526765606715384e-05
98699,98700,98699,197399,43.31730580329895,4.518317967796968e-05
98899,98900,98899,197799,43.40867495536804,4.509938098880208e-05
99099,99100,99099,198199,43.50590896606445,4.501583731072681e-05
99299,99300,99299,198599,43.58467888832092,4.4932546898934345e-05
99499,99500,99499,198999,43.668943881988525,4.4849508025442464e-05
99700,99701,99700,199401,43.74657201766968,4.476630565986469e-05
99900,99901,99900,199801,43.82656788825989,4.468376598651652e-05
100100,100101,100100,200201,43.91165804862976,4.460147276404328e-05
100300,100301,100300,200601,43.99417304992676,4.4519424333958804e-05
100501,100502,100501,201003,44.074317932128906,4.4437210635475236e-05
100701,100702,100701,201403,44.15537214279175,4.4355648082676674e-05
100901,100902,100901,201803,44.23448896408081,4.427432543655744e-05
101101,101102,101101,202203,44.31381893157959,4.4193241104020573e-05
101301,101302,101301,202603,44.39270997047424,4.411239350782217e-05
101502,101503,101502,203005,44.478676080703735,4.403137861250175e-05
101702,101703,101702,203405,44.557607889175415,4.3951000984366675e-05
101902,101903,101902,203805,44.63611078262329,4.387085544702319e-05
102102,102103,102102,204205,44.71394395828247,4.379094048596792e-05
102302,102303,102302,204605,44.79495882987976,4.371125460109813e-05
102503,102504,102503,205007,44.87564396858215,4.363139958517778e-05
102703,102704,102703,205407,44.95785713195801,4.355216853968124e-05
102903,102904,102903,205807,45.04213881492615,4.347316215269364e-05
103103,103104,103103,206207,45.121954917907715,4.339437898297778e-05
103303,103304,103303,206607,45.20370101928711,4.3315817604432367e-05
103504,103505,103504,207009,45.28641319274902,4.3237085450637275e-05
103704,103705,103704,207409,45.36842393875122,4.31589645219411e-05
103904,103905,103904,207809,45.45476698875427,4.308106118189421e-05
104104,104105,104104,208209,45.54423999786377,4.300337405977073e-05
104304,104305,104304,208609,45.64161705970764,4.292590179788452e-05
104505,104506,104505,209011,45.72373700141907,4.284825729345846e-05
104705,104706,104705,209411,45.803914070129395,4.2771211792207505e-05
104905,104906,104905,209811,45.8831729888916,4.2694377153060974e-05
105105,105106,105105,210211,45.96348690986633,4.2617752071961553e-05
105305,105306,105305,210611,46.04665184020996,4.2541335256941415e-05
105506,105507,105506,211013,46.13040113449097,4.246474489785581e-05
105706,105707,105706,211413,46.212258100509644,4.238874181677754e-05
105906,105907,105906,211813,46.293575048446655,4.23129431963783e-05
106106,106107,106106,212213,46.37206196784973,4.223734779535781e-05
106306,106307,106306,212613,46.45710492134094,4.21619543842812e-05
106507,106508,106507,213015,46.538617849349976,4.208638628516038e-05
106707,106708,106707,213415,46.61709499359131,4.2011394208758133e-05
106907,106908,106907,213815,46.695218086242676,4.193660049983342e-05
107107,107108,107107,214215,46.775821924209595,4.186200397677679e-05
107307,107308,107307,214615,46.85411477088928,4.178760346839654e-05
107508,107509,107508,215017,46.93628191947937,4.171302727544776e-05
107708,107709,107708,215417,47.01962184906006,4.163901629685916e-05
107908,107909,107908,215817,47.09853005409241,4.1565197883957355e-05
108108,108109,108108,216217,47.181257009506226,4.1491570911192283e-05
108308,108309,108308,216617,47.264363050460815,4.141813426371686e-05
108509,108510,108509,217019,47.34454679489136,4.134452107380839e-05
108709,108710,108709,217419,47.42446494102478,4.127146271369822e-05
108909,108910,108909,217819,47.509562969207764,4.119859139323062e-05
109109,109110,109109,218219,47.59292697906494,4.112590604067391e-05
109309,109310,109309,218619,47.686015129089355,4.105340559358115e-05
109510,109511,109510,219021,47.78118681907654,4.098072787766297e-05
109710,109711,109710,219421,47.86658596992493,4.090859500833572e-05
109910,109911,109910,219821,47.949278116226196,4.08366439143689e-05
110110,110111,110110,220221,48.03438115119934,4.076487357428793e-05
110310,110311,110310,220621,48.11350393295288,4.069328297583729e-05
110511,110512,110511,221023,48.19527792930603,4.06215145052255e-05
110711,110712,110711,221423,48.27540111541748,4.0550281279324136e-05
110911,110912,110911,221823,48.35679388046265,4.047922481193626e-05
111111,111112,111111,222223,48.43810200691223,4.0408344129327434e-05
111311,111312,111311,222623,48.51961088180542,4.033763826678008e-05
111512,111513,111512,223025,48.60093283653259,4.026675404407288e-05
111712,111713,111712,223425,48.68097376823425,4.0196395826437246e-05
111912,111913,111912,223825,48.76327395439148,4.012620958492055e-05
112112,112113,112112,224225,48.846166133880615,4.005619439092852e-05
112312,112313,112312,224625,48.92725205421448,3.9986349324519967e-05
112513,112514,112513,225027,49.01716685295105,3.991632551894718e-05
112713,112714,112713,225427,49.09960889816284,3.984681882233775e-05
112913,112914,112913,225827,49.1836371421814,3.977747954114498e-05
113113,113114,113113,226227,49.26512002944946,3.9708306789901046e-05
113313,113314,113313,226627,49.350492000579834,3.963929969087814e-05
113514,113515,113514,227029,49.43362498283386,3.957011357645754e-05
113714,113715,113714,227429,49.515828132629395,3.950143600047526e-05
113914,113915,113914,227829,49.59797692298889,3.943292148971854e-05
114114,114115,114114,228229,49.679116010665894,3.936456919881085e-05
114314,114315,114314,228629,49.76152205467224,3.929637829092299e-05
114515,114516,114515,229031,49.862327098846436,3.922800818680446e-05
114715,114716,114715,229431,49.94787001609802,3.91601383607746e-05
114915,114916,114915,229831,50.03011417388916,3.909242744835706e-05
115115,115116,115115,230231,50.1070830821991,3.902487464335613e-05
115315,115316,115315,230631,50.1849639415741,3.895747914627273e-05
115516,115517,115516,231033,50.26413917541504,3.888990436266954e-05
115716,115717,115716,231433,50.34012293815613,3.8822821890638963e-05
115916,115917,115916,231833,50.421066999435425,3.8755894369682186e-05
116116,116117,116116,232233,50.503714084625244,3.8689121029266045e-05
116316,116317,116316,232633,50.581632137298584,3.8622501106821576e-05
116517,116518,116517,233035,50.65706396102905,3.8555701891965155e-05
116717,116718,116717,233435,50.73379111289978,3.8489387301604596e-05
116917,116918,116917,233835,50.80900597572327,3.842322387769995e-05
117117,117118,117117,234235,50.88679003715515,3.8357210885008294e-05
117317,117318,117317,234635,50.96498107910156,3.829134759437342e-05
117518,117519,117518,235037,51.044734954833984,3.822530508543405e-05
117718,117719,117718,235437,51.12202596664429,3.815973977851581e-05
117918,117919,117918,235837,51.203428983688354,3.8094322023284365e-05
118118,118119,118118,236237,51.284037828445435,3.8029051116542725e-05
118318,118319,118318,236637,51.36483311653137,3.7963926362210494e-05
118519,118520,118519,237039,51.4428391456604,3.789862253742803e-05
118719,118720,118719,237439,51.526309967041016,3.783378874488906e-05
118919,118920,118919,237839,51.60740399360657,3.7769099048986214e-05
119119,119120,119119,238239,51.68603181838989,3.770455277765697e-05
119319,119320,119319,238639,51.766318798065186,3.764014926536829e-05
119520,119521,119520,239041,51.84431791305542,3.7575566900848915e-05
119720,119721,119720,239441,51.92880582809448,3.751144763786003e-05
119920,119921,119920,239841,52.026668071746826,3.744746916831129e-05
120120,120121,120120,240241,52.109638929367065,3.738363084998344e-05
120320,120321,120320,240641,52.18917798995972,3.7319932045600794e-05
120521,120522,120521,241043,52.26630902290344,3.7256054672370245e-05
120721,120722,120721,241443,52.34456515312195,3.71926336979702e-05
120921,120922,120921,241843,52.420315980911255,3.712935035773095e-05
121121,121122,121121,242243,52.4990758895874,3.706620403679001e-05
121321,121322,121321,242643,52.57432413101196,3.7003194126042957e-05
121522,121523,121522,243045,52.65137696266174,3.694000599102525e-05
121722,121723,121722,243445,52.72774600982666,3.687726776829454e-05
121922,121923,121922,243845,52.803921937942505,3.681466415666744e-05
122122,122123,122122,244245,52.88351106643677,3.675219456746879e-05
122322,122323,122322,244645,52.96416997909546,3.668985841792255e-05
122523,122524,122523,245047,53.04464602470398,3.662734444588582e-05
122723,122724,122723,245447,53.12048602104187,3.656527410556934e-05
122923,122924,122923,245847,53.19624400138855,3.650333548221747e-05
123123,123124,123123,246247,53.273268938064575,3.644152801252862e-05
123323,123324,123323,246647,53.34997296333313,3.637985113779499e-05
123524,123525,123524,247049,53.42550086975098,3.631799689617622e-05
123724,123725,123724,247449,53.5063259601593,3.6256580201276516e-05
123924,123925,123924,247849,53.58531308174133,3.6195292451558116e-05
124124,124125,124124,248249,53.664392948150635,3.61341331075647e-05
124324,124325,124324,248649,53.74486780166626,3.6073101634029336e-05
124525,124526,124525,249051,53.820728063583374,3.601189329879468e-05
124725,124726,124725,249451,53.89958691596985,3.595111661170688e-05
124925,124926,124925,249851,53.982946157455444,3.589046621418496e-05
125125,125126,125125,250251,54.07029414176941,3.582994158898002e-05
125325,125326,125325,250651,54.16751503944397,3.576954222295726e-05
125526,125527,125526,251053,54.24735903739929,3.5708966547326677e-05
125726,125727,125726,251453,54.32513689994812,3.5648816798425745e-05
125926,125927,125926,251853,54.405335903167725,3.5588790793452624e-05
126126,126127,126126,252253,54.491832971572876,3.552888803582781e-05
126326,126327,126326,252653,54.57054805755615,3.546910803420644e-05
126527,126528,126527,253055,54.65074801445007,3.54091523182087e-05
126727,126728,126727,253455,54.73316502571106,3.534961697648097e-05
126927,126928,126927,253855,54.81295585632324,3.529020293667073e-05
127127,127128,127127,254255,54.89159393310547,3.5230909723080626e-05
127327,127328,127327,254655,54.97502112388611,3.517173686366934e-05
127528,127529,127528,255057,55.05451703071594,3.5112388926087264e-05
127728,127729,127728,255457,55.13575291633606,3.5053455970777626e-05
127928,127929,127928,255857,55.21449613571167,3.499464197430056e-05
128128,128129,128128,256257,55.29251194000244,3.493594648039009e-05
128328,128329,128328,256657,55.372421979904175,3.4877369035759516e-05
128529,128530,128529,257059,55.45490217208862,3.481861718652739e-05
128729,128730,128729,257459,55.53842496871948,3.476027508052361e-05
128929,128930,128929,257859,55.61725187301636,3.470204968447367e-05
129129,129130,129129,258259,55.69550704956055,3.464394055939638e-05
129329,129330,129329,258659,55.776094913482666,3.458594727052638e-05
129530,129531,129530,259061,55.858604192733765,3.452778028585888e-05
129730,129731,129730,259461,55.93754696846008,3.447001795149704e-05
129930,129931,129930,259861,56.02201199531555,3.441237016624485e-05
130130,130131,130130,260261,56.10311198234558,3.4354836508896e-05
130330,130331,130330,260661,56.18953204154968,3.429741656130051e-05
130531,130532,130531,261063,56.28816604614258,3.4239823659516414e-05
130731,130732,130731,261463,56.36943006515503,3.418263045364034e-05
130931,130932,130931,261863,56.450993061065674,3.412554972080765e-05
131131,131132,131131,262263,56.533968925476074,3.406858105580677e-05
131331,131332,131331,262663,56.61682891845703,3.401172405665122e-05
131532,131533,131532,263065,56.6952760219574,3.395469487482563e-05
131732,131733,131732,263465,56.77333998680115,3.3898060567339216e-05
131932,131933,131932,263865,56.85051202774048,3.3841536736675074e-05
132132,132133,132132,264265,56.929431200027466,3.3785122992633076e-05
132332,132333,132332,264665,57.01650905609131,3.3728818948922185e-05
132533,132534,132533,265067,57.09825801849365,3.3672343522096916e-05
132733,132734,132733,265467,57.179256200790405,3.361625827438868e-05
132933,132934,132933,265867,57.26089596748352,3.3560281582751796e-05
133133,133134,133133,266267,57.34064602851868,3.3504413071810436e-05
133333,133334,133333,266667,57.41987490653992,3.3448652369900155e-05
133534,133535,133534,267069,57.50400900840759,3.339272111034821e-05
133734,133735,133734,267469,57.58537411689758,3.333717545501748e-05
133934,133935,133934,267869,57.6638867855072,3.328173650691955e-05
134134,134135,134134,268269,57.74568510055542,3.3226403905068906e-05
134334,134335,134334,268669,57.823628187179565,3.317117729093063e-05
134535,134536,134535,269071,57.90759992599487,3.311578096867486e-05
134735,134736,134735,269471,57.99188780784607,3.306076579105177e-05
134935,134936,134935,269871,58.07089376449585,3.300585554015017e-05
135135,135136,135135,270271,58.15035605430603,3.29510498680178e-05
135335,135336,135335,270671,58.22900581359863,3.289634842950437e-05
135536,135537,135536,271073,58.31248688697815,3.284147815433303e-05
135736,135737,135736,271473,58.413609981536865,3.2786984673873046e-05
135936,135937,135936,271873,58.5001118183136,3.273259440441426e-05
136136,136137,136136,272273,58.583348989486694,3.26783070105449e-05
136336,136337,136336,272673,58.66291785240173,3.262412215948365e-05
136537,136538,136537,273075,58.74141812324524,3.256976936384509e-05
136737,136738,136737,273475,58.82089805603027,3.251578911756609e-05
136937,136938,136937,273875,58.90895104408264,3.246191042815115e-05
137137,137138,137137,274275,58.996533155441284,3.2408132972123315e-05
137337,137338,137337,274675,59.12900400161743,3.2354456428208e-05
137538,137539,137538,275077,59.23639106750488,3.2300612849941055e-05
137738,137739,137738,275477,59.32491707801819,3.2247137676755736e-05
137938,137939,137938,275877,59.41680097579956,3.219376246431049e-05
138138,138139,138138,276277,59.512840032577515,3.21404869005079e-05
138338,138339,138338,276677,59.650712966918945,3.2087310675677356e-05
138539,138540,138539,277079,59.75735402107239,3.2033968343968456e-05
138739,138740,138739,277479,59.840436935424805,3.198099036833098e-05
138939,138940,138939,277879,59.924654960632324,3.1928110813003945e-05
139139,139140,139139,278279,60.02080798149109,3.187532937664559e-05
139339,139340,139339,278679,60.11024498939514,3.182264576006815e-05
139540,139541,139540,279081,60.2020947933197,3.176979697987561e-05
139740,139741,139740,279481,60.287895917892456,3.171730859837285e-05
139940,139941,139940,279881,60.37164902687073,3.166491714939388e-05
140140,140141,140140,280281,60.47385811805725,3.1612622341890724e-05
140340,140341,140340,280681,60.63343286514282,3.156042388655909e-05
140541,140542,140541,281083,60.75730800628662,3.1508061225090445e-05
140741,140742,140741,281483,60.853440046310425,3.1456055092394756e-05
140941,140942,140941,281883,60.9466598033905,3.140414445468293e-05
141141,141142,141141,282283,61.115293979644775,3.1352329030188275e-05
141341,141342,141341,282683,61.22227907180786,3.130060853944777e-05
141542,141543,141542,283085,61.30240797996521,3.124872481293569e-05
141742,141743,141742,283485,61.39384698867798,3.119719382931265e-05
141942,141943,141942,283885,61.48024106025696,3.114575695049307e-05
142142,142143,142142,284285,61.56629204750061,3.109441390386984e-05
142342,142343,142342,284685,61.64851093292236,3.104316441907263e-05
142543,142544,142543,285087,61.72599720954895,3.0991752680304946e-05
142743,142744,142743,285487,61.80568194389343,3.094068997928876e-05
142943,142944,142943,285887,61.881242990493774,3.088972003759656e-05
143143,143144,143143,286287,61.96367120742798,3.0838842592008134e-05
143343,143344,143343,286687,62.0442099571228,3.078805738069055e-05
143544,143545,143544,287089,62.12278985977173,3.0737110907847793e-05
143744,143745,143744,287489,62.20016598701477,3.0686509843999976e-05
143944,143945,143944,287889,62.279021978378296,3.063600023778612e-05
144144,144145,144144,288289,62.357348918914795,3.0585581833750395e-05
144344,144345,144344,288689,62.43450307846069,3.0535254378489374e-05
144545,144546,144545,289091,62.51990604400635,3.0484766663359365e-05
144745,144746,144745,289491,62.606056928634644,3.043462080276711e-05
144945,144946,144945,289891,62.7058482170105,3.0384565138386286e-05
145145,145146,145145,290291,62.799638986587524,3.0334599422977208e-05
145345,145346,145345,290691,62.88571500778198,3.0284723410669133e-05
145546,145547,145546,291093,62.97048997879028,3.0234688149085694e-05
145746,145747,145746,291493,63.050812005996704,3.0184991257592242e-05
145946,145947,145946,291893,63.142739057540894,3.013538334007429e-05
146146,146147,146146,292293,63.260359048843384,3.008586415646252e-05
146346,146347,146346,292693,63.37720823287964,3.003643346912084e-05
146547,146548,146547,293095,63.46417307853699,2.9986844549692967e-05
146747,146748,146747,293495,63.544156074523926,2.993759058442196e-05
146947,146948,146947,293895,63.620667934417725,2.9888424407463857e-05
147147,147148,147147,294295,63.699203968048096,2.9839345786595368e-05
147347,147348,147347,294695,63.77456998825073,2.97903544902232e-05
147548,147549,147548,295097,63.851314067840576,2.9741205986444744e-05
147748,147749,147748,295497,63.93123197555542,2.9692389085414498e-05
147948,147949,147948,295897,64.01650595664978,2.9643658822735838e-05
148148,148149,148148,296297,64.09740710258484,2.9595014972604923e-05
148348,148349,148348,296697,64.17262601852417,2.9546457310445976e-05
148549,148550,148549,297099,64.25500702857971,2.94977434705667e-05
148749,148750,148749,297499,64.33599400520325,2.944935794508017e-05
148949,148950,148949,297899,64.42420792579651,2.9401057940915373e-05
149149,149150,149149,298299,64.51295900344849,2.9352843239262764e-05
149349,149350,149349,298699,64.60090494155884,2.9304713621886748e-05
149550,149551,149550,299101,64.68781805038452,2.9256428861240055e-05
149750,149751,149750,299501,64.78203392028809,2.9208469186524026e-05
149950,149951,149950,299901,64.88598608970642,2.9160593948292362e-05
150150,150151,150150,300301,64.97136211395264,2.9112802934132927e-05
150350,150351,150350,300701,65.05492901802063,2.9065095931660782e-05
150551,150552,150551,301103,65.13524794578552,2.9017234824598267e-05
150751,150752,150751,301503,65.21284508705139,2.8969695632407664e-05
150951,150952,150951,301903,65.29227089881897,2.8922239822920026e-05
151151,151152,151151,302303,65.37263488769531,2.8874867188456232e-05
151351,151352,151351,302703,65.45100402832031,2.8827577523143312e-05
151552,151553,151552,303105,65.53881812095642,2.8780134795310163e-05
151752,151753,151752,303505,65.62929010391235,2.873301086728754e-05
151952,151953,151952,303905,65.71251201629639,2.8685969296261616e-05
152152,152153,152152,304305,65.7923309803009,2.863900988055603e-05
152352,152353,152352,304705,65.87299799919128,2.8592132419901223e-05
152553,152554,152553,305107,65.95416498184204,2.854510294121894e-05
152753,152754,152753,305507,66.03378009796143,2.8498389200783686e-05
152953,152954,152953,305907,66.11412310600281,2.8451756819195488e-05
153153,153154,153153,306307,66.19321608543396,2.8405205600672602e-05
153353,153354,153353,306707,66.27086901664734,2.835873534986366e-05
153554,153555,153554,307109,66.34968495368958,2.8312114127950125e-05
153754,153755,153754,307509,66.43026995658875,2.8265805633858505e-05
153954,153955,153954,307909,66.51378893852234,2.8219577527341483e-05
154154,154155,154154,308309,66.59417200088501,2.8173429617296937e-05
154354,154355,154354,308709,66.67005181312561,2.8127361713733652e-05
154555,154556,154555,309111,66.74963998794556,2.808114388731143e-05
154755,154756,154755,309511,66.82511115074158,2.8035235827740164e-05
154955,154956,154955,309911,66.90601086616516,2.798940720963267e-05
155155,155156,155155,310311,67.00175595283508,2.7943657846335562e-05
155355,155356,155355,310711,67.08723592758179,2.7897987552790368e-05
155556,155557,155556,311113,67.16258311271667,2.7852168385338706e-05
155756,155757,155756,311513,67.24588298797607,2.7806656072274796e-05
155956,155957,155956,311913,67.32316493988037,2.776122227784372e-05
156156,156157,156156,312313,67.4009428024292,2.7715866820602497e-05
156356,156357,156356,312713,67.48641300201416,2.767058951975651e-05
156557,156558,156557,313115,67.56510901451111,2.7625164394857523e-05
156757,156758,156757,313515,67.64877009391785,2.7580043257270633e-05
156957,156958,156957,313915,67.72689580917358,2.7534999738770038e-05
157157,157158,157157,314315,67.80661988258362,2.7490033662440043e-05
157357,157358,157357,314715,67.8848888874054,2.744514485171511e-05
157558,157559,157558,315117,67.97049307823181,2.7400109266054946e-05
157758,157759,157758,315517,68.05316090583801,2.73553748458076e-05
157958,157959,157958,315917,68.13464403152466,2.7310717166699878e-05
158158,158159,158158,316317,68.21304821968079,2.726613605625704e-05
158358,158359,158358,316717,68.29418182373047,2.7221631342149742e-05
158559,158560,158559,317119,68.37260293960571,2.7176980902198065e-05
158759,158760,158759,317519,68.45442485809326,2.7132628848051296e-05
158959,158960,158959,317919,68.53934597969055,2.7088352678290366e-05
159159,159160,159159,318319,68.62397599220276,2.7044152224168055e-05
159359,159360,159359,318719,68.70588397979736,2.700002731772764e-05
159560,159561,159560,319121,68.78680300712585,2.695575773311357e-05
159760,159761,159760,319521,68.86467599868774,2.6911783796723035e-05
159960,159961,159960,319921,68.94763708114624,2.6867884907825417e-05
160160,160161,160160,320321,69.0287868976593,2.6824060901366357e-05
160360,160361,160360,320721,69.12804698944092,2.6780311613273723e-05
160561,160562,160561,321123,69.2211651802063,2.6736418693567236e-05
160761,160762,160761,321523,69.2997100353241,2.669281872431606e-05
160961,160962,160961,321923,69.38189387321472,2.6649292984668876e-05
161161,161162,161161,322323,69.46844911575317,2.6605841313346673e-05
161361,161362,161361,322723,69.54917788505554,2.656246354986753e-05
161562,161563,161562,323125,69.63123989105225,2.6518943199524403e-05
161762,161763,161762,323525,69.7119529247284,2.6475713140751926e-05
161962,161963,161962,323925,69.79346489906311,2.643255651172769e-05
162162,162163,162162,324325,69.874342918396,2.6389473155239724e-05
162362,162363,162362,324725,69.96125912666321,2.6346462913894484e-05
162563,162564,162563,325127,70.04554605484009,2.6303311128111402e-05
162763,162764,162763,325527,70.12514686584473,2.626044701272213e-05
162963,162964,162963,325927,70.20838403701782,2.6217655545066073e-05
163163,163164,163163,326327,70.29753708839417,2.6174936570835707e-05
163363,163364,163363,326727,70.37494993209839,2.613228993624304e-05
163564,163565,163564,327129,70.46351385116577,2.6089502797447043e-05
163764,163765,163764,327529,70.54457807540894,2.60470007442656e-05
163964,163965,163964,327929,70.62369203567505,2.6004570573183797e-05
164164,164165,164164,328329,70.70361185073853,2.59622121331005e-05
164364,164365,164364,328729,70.78573703765869,2.591992527400661e-05
164565,164566,164565,329131,70.86762809753418,2.5877498948005026e-05
164765,164766,164765,329531,70.95184707641602,2.583535515765484e-05
164965,164966,164965,329931,71.03708386421204,2.579328250024782e-05
165165,165166,165165,330331,71.12117791175842,2.575128082717377e-05
165365,165366,165365,330731,71.20958280563354,2.5709349991992775e-05
165566,165567,165566,331133,71.31035089492798,2.566728072405003e-05
165766,165767,165766,331533,71.39327907562256,2.5625491476525075e-05
165966,165967,165966,331933,71.47820591926575,2.5583772627428496e-05
166166,166167,166166,332333,71.55819511413574,2.5542124031821056e-05
166366,166367,166366,332733,71.64023494720459,2.5500545545581572e-05
166567,166568,166567,333135,71.72308588027954,2.5458829657697984e-05
166767,166768,166767,333535,71.80168795585632,2.5417391307826607e-05
166967,166968,166967,333935,71.88214778900146,2.5376022637118338e-05
167167,167168,167167,334335,71.96519613265991,2.533472350322284e-05
167367,167368,167367,334735,72.04813814163208,2.5293493764724562e-05
167568,167569,167568,335137,72.12994694709778,2.5252127652204736e-05
167768,167769,167768,335537,72.23067498207092,2.5211036627615562e-05
167968,167969,167968,335937,72.37901020050049,2.517001457651908e-05
168168,168169,168168,336337,72.48583984375,2.5129061359817475e-05
168368,168369,168368,336737,72.58683395385742,2.5088176838883764e-05
168569,168570,168569,337139,72.67611908912659,2.504715696707863e-05
168769,168770,168769,337539,72.75958895683289,2.5006409764613043e-05
168969,168970,168969,337939,72.85273098945618,2.4965730843957197e-05
169169,169170,169169,338339,72.95363688468933,2.492512006818308e-05
169369,169370,169369,338739,73.03515601158142,2.4884577301458747e-05
169570,169571,169570,339141,73.11619687080383,2.4843900203789654e-05
169770,169771,169770,339541,73.19726014137268,2.4803493386753263e-05
169970,169971,169970,339941,73.27739191055298,2.476315417274965e-05
170170,170171,170170,340341,73.37172198295593,2.4722882427436343e-05
170370,170371,170370,340741,73.4651780128479,2.4682678017042692e-05
170571,170572,170571,341143,73.5430281162262,2.464234029133234e-05
170771,170772,170771,341543,73.61900281906128,2.4602270487442722e-05
170971,170972,170971,341943,73.69428300857544,2.4562267619795407e-05
171171,171172,171171,342343,73.77080702781677,2.4522331557166596e-05
171371,171372,171371,342743,73.8505449295044,2.44824621681199e-05
171572,171573,171572,343145,73.93052387237549,2.444246047446521e-05
171772,171773,171772,343545,74.01479005813599,2.440272437249855e-05
171972,171973,171972,343945,74.10432291030884,2.4363054552510238e-05
172172,172173,172172,344345,74.18094301223755,2.432345088527498e-05
172372,172373,172372,344745,74.25656199455261,2.4283913241877487e-05
172573,172574,172573,345147,74.33667588233948,2.424424430063261e-05
172773,172774,172773,345547,74.41180300712585,2.4204838648445188e-05
172973,172974,172973,345947,74.49563908576965,2.416549863573101e-05
173173,173174,173173,346347,74.57271194458008,2.4126224135012666e-05
173373,173374,173373,346747,74.64954996109009,2.408701501978019e-05
173574,173575,173574,347149,74.72903776168823,2.4047675608390944e-05
173774,173775,173774,347549,74.80734300613403,2.4008597211097718e-05
173974,173975,173974,347949,74.8836760520935,2.3969583821460713e-05
174174,174175,174174,348349,74.96640276908875,2.393063531418105e-05
174374,174375,174374,348749,75.04356002807617,2.3891751565157153e-05
174575,174576,174575,349151,75.12446188926697,2.3852738516664782e-05
174775,174776,174775,349551,75.20208096504211,2.381398423381695e-05
174975,174976,174975,349951,75.27801990509033,2.377529433750164e-05
175175,175176,175175,350351,75.35660600662231,2.3736668704880963e-05
175375,175376,175375,350751,75.43533897399902,2.369810721313198e-05
175576,175577,175576,351153,75.5359570980072,2.365941741395211e-05
175776,175777,175776,351553,75.62187504768372,2.362098415806257e-05
175976,175977,175976,351953,75.69964504241943,2.358261467762799e-05
176176,176177,176176,352353,75.77583694458008,2.3544308852217578e-05
176376,176377,176376,352753,75.85486698150635,2.3506066560952518e-05
176577,176578,176577,353155,75.9324791431427,2.346769694891448e-05
176777,176778,176777,353555,76.01628589630127,2.3429581682828507e-05
176977,176978,176977,353955,76.09648394584656,2.3391529591373932e-05
177177,177178,177177,354355,76.17445302009583,2.335354055597404e-05
177377,177378,177377,354755,76.2517352104187,2.331561445777261e-05
177578,177579,177578,355157,76.33051705360413,2.327756202008536e-05
177778,177779,177778,355557,76.4132969379425,2.3239761755813876e-05
177978,177979,177978,355957,76.49679112434387,2.3202024074966632e-05
178178,178179,178178,356357,76.57534003257751,2.3164348860408362e-05
178378,178379,178378,356757,76.65414619445801,2.3126735995848277e-05
178579,178580,178579,357159,76.73327112197876,2.30889977676818e-05
178779,178780,178779,357559,76.81040287017822,2.3051509564292444e-05
178979,178980,178979,357959,76.88769316673279,2.3014083362342935e-05
179179,179180,179179,358359,76.96696710586548,2.2976719046527596e-05
179379,179380,179379,358759,77.04788517951965,2.2939416502165614e-05
179580,179581,179580,359161,77.12526178359985,2.290198956470806e-05
179780,179781,179780,359561,77.20362901687622,2.2864810527063875e-05
179980,179981,179980,359961,77.28173398971558,2.2827692917542094e-05
180180,180181,180180,360361,77.3619978427887,2.279063662294794e-05
180380,180381,180380,360761,77.43956112861633,2.275364152996231e-05
180581,180582,180581,361163,77.52642703056335,2.2716523009035234e-05
180781,180782,180781,361563,77.61226916313171,2.2679650285878982e-05
180981,180982,180981,361963,77.70938086509705,2.2642838426256483e-05
181181,181182,181181,362363,77.78803992271423,2.2606087318521188e-05
181381,181382,181381,362763,77.8656358718872,2.2569396851381405e-05
181582,181583,181582,363165,77.94710087776184,2.2532583915660897e-05
181782,181783,181782,363565,78.03105688095093,2.2496014698016048e-05
181982,181983,181982,363965,78.10898113250732,2.2459505787817227e-05
182182,182183,182182,364365,78.18795084953308,2.2423057074984687e-05
182382,182383,182382,364765,78.27460503578186,2.238666844956508e-05
182583,182584,182583,365167,78.35239887237549,2.23501583093598e-05
182783,182784,182783,365567,78.43050694465637,2.231388982964097e-05
182983,182984,182983,365967,78.51196599006653,2.2277681109248998e-05
183183,183184,183183,366367,78.59074378013611,2.2241532039375165e-05
183383,183384,183383,366767,78.66966104507446,2.2205442512081338e-05
183584,183585,183584,367169,78.75222206115723,2.216923241788285e-05
183784,183785,183784,367569,78.8373351097107,2.213326194814222e-05
183984,183985,183984,367969,78.91518998146057,2.209735069722583e-05
184184,184185,184184,368369,78.9989321231842,2.206149855818492e-05
184384,184385,184384,368769,79.08092093467712,2.2025705424122853e-05
184585,184586,184585,369171,79.16448378562927,2.1989792665458342e-05
184785,184786,184785,369571,79.24175596237183,2.195411751612526e-05
184985,184986,184985,369971,79.32132697105408,2.1918501052878556e-05
185185,185186,185185,370371,79.40154099464417,2.188294317003418e-05
185385,185386,185385,370771,79.48456192016602,2.184744376233669e-05
185586,185587,185586,371173,79.56626415252686,2.1811825666163558e-05
185786,185787,185786,371573,79.65042686462402,2.1776443184989083e-05
185986,185987,185986,371973,79.7382800579071,2.1741118864522782e-05
186186,186187,186186,372373,79.83636212348938,2.170585260020651e-05
186386,186387,186386,372773,79.91850090026855,2.1670644288367613e-05
186587,186588,186587,373175,80.00304794311523,2.1635318218169804e-05
186787,186788,186787,373575,80.0810980796814,2.1600225789428827e-05
186987,186988,186987,373975,80.16105389595032,2.156519100240126e-05
187187,187188,187187,374375,80.24417901039124,2.1530213754814547e-05
187387,187388,187387,374775,80.32584500312805,2.1495293943770525e-05
187588,187589,187588,375177,80.40543293952942,2.146025729886453e-05
187788,187789,187788,375577,80.4919319152832,2.142545234100725e-05
187988,187989,187988,375977,80.5713460445404,2.139070451345724e-05
188188,188189,188188,376377,80.65219497680664,2.1356013714720305e-05
188388,188389,188388,376777,80.73476696014404,2.1321379844114263e-05
188589,188590,188589,377179,80.81750798225403,2.1286630057780718e-05
188789,188790,188789,377579,80.89874005317688,2.1252110023521814e-05
188989,188990,188989,377979,80.98782396316528,2.1217646614955024e-05
189189,189190,189189,378379,81.07085180282593,2.1183239731677537e-05
189389,189390,189389,378779,81.15163707733154,2.1148889273751914e-05
189590,189591,189590,379181,81.22996520996094,2.1114423812671987e-05
189790,189791,189790,379581,81.31006908416748,2.108018618819083e-05
189990,189991,189990,379981,81.39129877090454,2.1046004690758173e-05
190190,190191,190190,380381,81.47272086143494,2.1011879221415873e-05
190390,190391,190390,380781,81.555184841156,2.0977809681550047e-05
190591,190592,190591,381183,81.63444900512695,2.0943626044549757e-05
190791,190792,190791,381583,81.7119870185852,2.0909668347591e-05
190991,190992,190991,381983,81.7903881072998,2.08757662853754e-05
191191,191192,191191,382383,81.87673091888428,2.0841919760578568e-05
191391,191392,191391,382783,81.97823810577393,2.0808128675370656e-05
191592,191593,191592,383185,82.05850601196289,2.0774224393076465e-05
191792,191793,191792,383585,82.13778114318848,2.0740544172617413e-05
191992,191993,191992,383985,82.21685791015625,2.0706919100714405e-05
192192,192193,192192,384385,82.2965259552002,2.067334908140701e-05
192392,192393,192392,384785,82.37558507919312,2.0639834017932536e-05
192593,192594,192593,385187,82.46506190299988,2.0606206651676476e-05
192793,192794,192793,385587,82.54411196708679,2.0572801486660452e-05
192993,192994,192993,385987,82.623281955719,2.053945099044336e-05
193193,193194,193193,386387,82.70281982421875,2.0506155067475658e-05
193393,193394,193393,386787,82.7836549282074,2.0472913622900712e-05
193594,193595,193594,387189,82.8673779964447,2.0439560763288755e-05
193794,193795,193794,387589,82.95098805427551,2.0406428262576952e-05
193994,193995,193994,387989,83.03341388702393,2.0373349956217545e-05
194194,194195,194194,388389,83.11208987236023,2.034032575001734e-05
194394,194395,194394,388789,83.19315481185913,2.030735555027573e-05
194595,194596,194595,389191,83.27531385421753,2.0274274816786687e-05
194795,194796,194795,389591,83.35463309288025,2.0241412617790692e-05
194995,194996,194995,389991,83.43343806266785,2.0208604144447255e-05
195195,195196,195195,390391,83.51981496810913,2.0175849303462362e-05
195395,195396,195395,390791,83.59795475006104,2.0143148002623625e-05
195596,195597,195596,391193,83.68014597892761,2.0110337043753115e-05
195796,195797,195796,391593,83.7615418434143,2.0077742811394474e-05
195996,195997,195996,391993,83.84008002281189,2.004520184155823e-05
196196,196197,196196,392393,83.92409801483154,2.0012714042127814e-05
196396,196397,196396,392793,84.01330304145813,1.9980279321454077e-05
196597,196598,196597,393195,84.11510515213013,1.9947735812606565e-05
196797,196798,196797,393595,84.19420099258423,1.991540723970521e-05
196997,196998,196997,393995,84.27405500411987,1.9883131471160428e-05
197197,197198,197197,394395,84.35312390327454,1.9850908416439607e-05
197397,197398,197397,394795,84.43261075019836,1.981873798463001e-05
197598,197599,197598,395197,84.51691603660583,1.9786459627906017e-05
197798,197799,197798,395597,84.59809112548828,1.975439443307053e-05
197998,197999,197998,395997,84.67818999290466,1.972238159024842e-05
198198,198199,198198,396397,84.75963807106018,1.9690421009510514e-05
198398,198399,198398,396797,84.84417009353638,1.9658512601123204e-05
198599,198600,198599,397199,84.92877507209778,1.9626497124947146e-05
198799,198800,198799,397599,85.0115659236908,1.959469305310981e-05
198999,199000,198999,397999,85.09134292602539,1.9562940885766075e-05
199199,199200,199199,398399,85.16927599906921,1.9531240534026683e-05
199399,199400,199399,398799,85.2428948879242,1.9499591909158424e-05
199600,199601,199600,399201,85.3191339969635,1.9467837067431413e-05
199800,199801,199800,399601,85.39420914649963,1.9436291888846276e-05
200000,200001,200000,400001,85.47471189498901,1.940479817205344e-05


==> plot_data/bilinear_matrix_game_n250/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0022521018981933594,2.0175302852282635
27,140,140,280,0.11786293983459473,0.13386604132059543
53,324,324,648,0.23158597946166992,0.05239901804132782
80,524,524,1048,0.321026086807251,0.025483537201023237
106,722,722,1444,0.4019429683685303,0.014797314834664448
133,926,926,1852,0.4670898914337158,0.010422851966899497
159,1128,1128,2256,0.5397119522094727,0.00823981414556747
186,1334,1334,2668,0.6062941551208496,0.005949829350939559
212,1538,1538,3076,0.6630330085754395,0.004895687120914551
239,1748,1748,3496,0.7195460796356201,0.0039387324137672795
265,1948,1948,3896,0.7773702144622803,0.0031334824091006626
292,2150,2150,4300,0.8646221160888672,0.002151612155160017
318,2354,2354,4708,0.9531641006469727,0.0018311447514661934
345,2570,2570,5140,1.022481918334961,0.0018042080287622372
371,2778,2778,5556,1.1024482250213623,0.00179021331690119
398,2994,2994,5988,1.206083059310913,0.0017788398911990659
425,3210,3210,6420,1.2930150032043457,0.0017437804703963203
451,3412,3412,6824,1.371291160583496,0.0014807552790521632
478,3628,3628,7256,1.4577879905700684,0.0014119864217351996
504,3836,3836,7672,1.5337810516357422,0.0014024814049348523
531,4042,4042,8084,1.6428380012512207,0.001070835919770597
557,4244,4244,8488,1.7207098007202148,0.0008657670844045979
584,4456,4456,8912,1.7912940979003906,0.0007541440144498692
610,4664,4664,9328,1.8709361553192139,0.0007214237513235053
637,4878,4878,9756,1.964846134185791,0.0006679622953102352
663,5082,5082,10164,2.063000202178955,0.0005805290268225688
690,5298,5298,10596,2.2186429500579834,0.0005699182526091067
716,5506,5506,11012,2.3672990798950195,0.0005591325622961148
743,5720,5720,11440,2.6216681003570557,0.0005519075003482119
769,5926,5926,11852,2.7312090396881104,0.0004844202086686495
796,6140,6140,12280,2.821415901184082,0.0004508791766902869
822,6348,6348,12696,2.920520067214966,0.00043709173602084396
849,6550,6550,13100,3.0005390644073486,0.00030231464991499723
876,6766,6766,13532,3.066215991973877,0.00028836861154595797
902,6974,6974,13948,3.1498939990997314,0.00028429351895218924
929,7190,7190,14380,3.2088701725006104,0.0002812130174537038
955,7398,7398,14796,3.2707982063293457,0.00027728577118186153
982,7612,7612,15224,3.3387489318847656,0.00027441835396858287
1008,7812,7812,15624,3.4027981758117676,0.0002135443685586855
1035,8028,8028,16056,3.4842381477355957,0.00020930359686738954
1061,8236,8236,16472,3.6295440196990967,0.00020747106041227239
1088,8452,8452,16904,3.6934080123901367,0.00020601837043941735
1114,8660,8660,17320,3.746070146560669,0.0002048442213182238
1141,8870,8870,17740,3.7994518280029297,0.0001711968704143183
1167,9078,9078,18156,3.8500568866729736,0.00016787962445776085
1194,9294,9294,18588,3.9119009971618652,0.00016685197067492708
1220,9502,9502,19004,3.9665799140930176,0.00016608140305148398
1247,9718,9718,19436,4.0265491008758545,0.00016540632347586423
1274,9924,9924,19848,4.094965934753418,0.00015505071678485066
1300,10132,10132,20264,4.150645971298218,0.00015163264462378788
1327,10348,10348,20696,4.201340913772583,0.0001505610595880387
1353,10556,10556,21112,4.252288103103638,0.00014991846436712182
1380,10772,10772,21544,4.302511215209961,0.00014938322943022553
1406,10980,10980,21960,4.364464998245239,0.0001489416491123278
1433,11196,11196,22392,4.43955397605896,0.00014853780425029808
1459,11404,11404,22808,4.515912055969238,0.0001481893063254073
1486,11620,11620,23240,4.590045928955078,0.00014786032917005562
1512,11826,11826,23652,4.654447078704834,0.000141631966840428
1539,12042,12042,24084,4.753337144851685,0.00013795986233394698
1565,12250,12250,24500,4.890406847000122,0.00013662932758002464
1592,12466,12466,24932,5.016093969345093,0.00013583443566834609
1618,12674,12674,25348,5.083708047866821,0.00013530970582852612
1645,12890,12890,25780,5.151303052902222,0.00013490204202589863
1671,13098,13098,26196,5.254472017288208,0.0001345911142012028
1698,13312,13312,26624,5.361530065536499,0.00013279247106082716
1725,13526,13526,27052,5.45979118347168,0.0001214775156834342
1751,13734,13734,27468,5.518681049346924,0.00011860912868665622
1778,13950,13950,27900,5.5772950649261475,0.0001169647997291521
1804,14158,14158,28316,5.628485202789307,0.00011593111834342874
1831,14368,14368,28736,5.679145097732544,0.00011516660359808975
1857,14576,14576,29152,5.732731103897095,0.00011461444399115416
1884,14792,14792,29584,5.786726951599121,0.00011416722114314834
1910,15000,15000,30000,5.843304872512817,0.00011382098870405677
1937,15216,15216,30432,5.905013084411621,0.00011352414149890013
1963,15424,15424,30848,5.968358993530273,0.00011328275836235257
1990,15638,15638,31276,6.059362173080444,0.0001084823543773074
2016,15846,15846,31692,6.166356086730957,0.00010561959785485005
2043,16062,16062,32124,6.251826047897339,0.00010450006180903445
2069,16270,16270,32540,6.311590909957886,0.00010395809268762762
2096,16486,16486,32972,6.374425172805786,0.00010360430410391714
2123,16702,16702,33404,6.451365232467651,0.0001033515789537631
2149,16906,16906,33812,6.598901033401489,9.371785491371214e-05
2176,17122,17122,34244,6.707133054733276,9.068926478384993e-05
2202,17330,17330,34660,6.796364068984985,8.931322542185274e-05
2229,17546,17546,35092,6.867257118225098,8.848928190346306e-05
2255,17754,17754,35508,6.924974203109741,8.797005645963781e-05
2282,17970,17970,35940,7.000967979431152,8.758228905676102e-05
2308,18178,18178,36356,7.133243083953857,8.729446211838591e-05
2335,18394,18394,36788,7.213040113449097,8.705094863479934e-05
2361,18602,18602,37204,7.279374122619629,8.685171389426975e-05
2388,18816,18816,37632,7.350128889083862,8.499979333457976e-05
2414,19024,19024,38048,7.4133710861206055,8.241750845332826e-05
2441,19240,19240,38480,7.467947006225586,8.139918447999447e-05
2467,19448,19448,38896,7.524602174758911,8.085605297882907e-05
2494,19664,19664,39328,7.584980010986328,8.046589846610135e-05
2520,19872,19872,39744,7.650965929031372,8.017867258280167e-05
2547,20088,20088,40176,7.711814880371094,7.993825011628805e-05
2574,20302,20302,40604,7.777748107910156,7.830088300152179e-05
2600,20510,20510,41020,7.8478310108184814,7.532593076527558e-05
2627,20726,20726,41452,7.928389072418213,7.421244247688861e-05
2653,20934,20934,41868,7.99311900138855,7.3672105715229e-05
2680,21144,21144,42288,8.063168048858643,7.33175064950595e-05
2706,21352,21352,42704,8.125668048858643,7.307387538284401e-05
2733,21568,21568,43136,8.191911935806274,7.287968218194353e-05
2759,21776,21776,43552,8.249104976654053,7.27292381899256e-05
2786,21990,21990,43980,8.309134006500244,6.885302509422136e-05
2812,22198,22198,44396,8.369533061981201,6.765233804292725e-05
2839,22408,22408,44816,8.425894975662231,6.711511825580034e-05
2865,22616,22616,45232,8.489995002746582,6.681415240167379e-05
2892,22832,22832,45664,8.554644107818604,6.65996395543345e-05
2918,23034,23034,46068,8.60841703414917,6.644485180737433e-05
2945,23250,23250,46500,8.665284156799316,6.631702726622706e-05
2972,23466,23466,46932,8.722867012023926,6.621114171973429e-05
2998,23666,23666,47332,8.771969079971313,6.493623635808064e-05
3025,23882,23882,47764,8.82278823852539,6.167459296993791e-05
3051,24090,24090,48180,8.884504079818726,6.09284669044297e-05
3078,24306,24306,48612,8.948414087295532,6.0638890985231244e-05
3104,24514,24514,49028,9.007719039916992,6.048030200274136e-05
3131,24722,24722,49444,9.128625869750977,5.784700683514006e-05
3157,24930,24930,49860,9.20567512512207,5.6444100339231787e-05
3184,25146,25146,50292,9.278661251068115,5.59664365878355e-05
3210,25354,25354,50708,9.34933614730835,5.5725894259415703e-05
3237,25570,25570,51140,9.426176071166992,5.555623134898498e-05
3263,25778,25778,51556,9.489758968353271,5.5431253877137254e-05
3290,25994,25994,51988,9.560914039611816,5.5325091267556734e-05
3316,26196,26196,52392,9.623784065246582,5.523774797174259e-05
3343,26412,26412,52824,9.692344188690186,5.515769194501938e-05
3370,26622,26622,53244,9.768681049346924,5.5085423533469376e-05
3396,26824,26824,53648,9.817859172821045,4.77378914207915e-05
3423,27040,27040,54080,9.86974310874939,4.587565317309067e-05
3449,27248,27248,54496,9.920037269592285,4.481493991377205e-05
3476,27464,27464,54928,9.969804048538208,4.4087665282734094e-05
3502,27672,27672,55344,10.021512031555176,4.359386612887478e-05
3529,27888,27888,55776,10.073235988616943,4.32123476541333e-05
3555,28090,28090,56180,10.11982011795044,4.292730302694882e-05
3582,28304,28304,56608,10.169533014297485,4.188928992277808e-05
3608,28512,28512,57024,10.219257116317749,4.155762719988694e-05
3635,28728,28728,57456,10.27060604095459,4.132716867357425e-05
3661,28928,28928,57856,10.318481922149658,3.99200863214391e-05
3688,29144,29144,58288,10.373099088668823,3.883659594322249e-05
3714,29352,29352,58704,10.422804117202759,3.844886526348497e-05
3741,29568,29568,59136,10.474486112594604,3.823961130631038e-05
3767,29776,29776,59552,10.523056268692017,3.8109007228984274e-05
3794,29992,29992,59984,10.573950052261353,3.800889598681757e-05
3821,30208,30208,60416,10.62541913986206,3.792945648535132e-05
3847,30416,30416,60832,10.674789190292358,3.786523955975681e-05
3874,30632,30632,61264,10.726577997207642,3.7807064376290335e-05
3900,30840,30840,61680,10.781315088272095,3.775676618346048e-05
3927,31056,31056,62112,10.837064981460571,3.770879755003675e-05
3953,31264,31264,62528,10.885648250579834,3.766564847956498e-05
3980,31478,31478,62956,10.941834926605225,3.565839830206878e-05
4006,31686,31686,63372,10.991253137588501,3.490356320384085e-05
4033,31902,31902,63804,11.04212999343872,3.455567826805344e-05
4059,32110,32110,64220,11.090188026428223,3.437115130505264e-05
4086,32326,32326,64652,11.14206600189209,3.4248044691080096e-05
4112,32534,32534,65068,11.191554069519043,3.416417852874644e-05
4139,32748,32748,65496,11.242393016815186,3.2376515824540745e-05
4165,32956,32956,65912,11.29013991355896,3.173951492471495e-05
4192,33172,33172,66344,11.340918064117432,3.1520683885889836e-05
4219,33388,33388,66776,11.39651107788086,3.1414201525974064e-05
4245,33596,33596,67192,11.445641040802002,3.134651026886788e-05
4272,33812,33812,67624,11.495362997055054,3.129216955226211e-05
4298,34020,34020,68040,11.545071125030518,3.1248263894868376e-05
4325,34236,34236,68472,11.595269918441772,3.120805880591474e-05
4351,34444,34444,68888,11.6429922580719,3.117280971466993e-05
4378,34658,34658,69316,11.694154024124146,2.9362450330697884e-05
4404,34866,34866,69732,11.742655992507935,2.8933755483151436e-05
4431,35082,35082,70164,11.793884038925171,2.8748797062197033e-05
4457,35290,35290,70580,11.842998027801514,2.8647936584784465e-05
4484,35506,35506,71012,11.892839908599854,2.8576082075314087e-05
4510,35712,35712,71424,11.939726114273071,2.8568455042885183e-05
4537,35928,35928,71856,11.990597248077393,2.715819267937776e-05
4563,36136,36136,72272,12.038399934768677,2.670528045573686e-05
4590,36352,36352,72704,12.089936971664429,2.6473089793050608e-05
4616,36560,36560,73120,12.138375997543335,2.63387849570088e-05
4643,36776,36776,73552,12.196505069732666,2.6243867578324844e-05
4670,36992,36992,73984,12.24733591079712,2.6174070523914213e-05
4696,37200,37200,74400,12.300095081329346,2.6121169946479188e-05
4723,37416,37416,74832,12.35162901878357,2.607574838686311e-05
4749,37622,37622,75244,12.404536008834839,2.5574920831748935e-05
4776,37838,37838,75676,12.45529294013977,2.457924163327967e-05
4802,38046,38046,76092,12.509525060653687,2.4290358135247928e-05
4829,38262,38262,76524,12.561557054519653,2.4146412692876718e-05
4855,38470,38470,76940,12.613218069076538,2.4058879542196876e-05
4882,38680,38680,77360,12.664427042007446,2.399323040849407e-05
4908,38882,38882,77764,12.714942932128906,2.3944248149366882e-05
4935,39096,39096,78192,12.771934986114502,2.286871783005853e-05
4961,39304,39304,78608,12.824717044830322,2.2396852967113035e-05
4988,39520,39520,79040,12.886391162872314,2.2207487795219564e-05
5014,39728,39728,79456,12.93936800956726,2.211009749324525e-05
5041,39944,39944,79888,12.989595890045166,2.2043070382135523e-05
5068,40154,40154,80308,13.03895616531372,2.19930901749752e-05
5094,40362,40362,80724,13.088166236877441,2.1954199869933548e-05
5121,40578,40578,81156,13.137755155563354,2.1919912084014755e-05
5147,40786,40786,81572,13.192728042602539,2.1890896399747784e-05
5174,41000,41000,82000,13.243595123291016,2.113632699190753e-05
5200,41208,41208,82416,13.29367208480835,2.065579783253509e-05
5227,41424,41424,82848,13.344955205917358,2.0478518890918242e-05
5253,41632,41632,83264,13.395933866500854,2.0388961644178854e-05
5280,41848,41848,83696,13.447001218795776,2.0328052613951203e-05
5306,42056,42056,84112,13.496336936950684,2.0284809415658133e-05
5333,42272,42272,84544,13.547231912612915,2.024914636759447e-05
5359,42478,42478,84956,13.596578121185303,1.9164465123797088e-05
5386,42694,42694,85388,13.646286010742188,1.886180952885167e-05
5412,42902,42902,85804,13.694293022155762,1.8746056849765743e-05
5439,43118,43118,86236,13.746047019958496,1.8676226845042725e-05
5465,43320,43320,86640,13.798388957977295,1.8628755979689576e-05
5492,43536,43536,87072,13.848267078399658,1.8590259759957193e-05
5519,43752,43752,87504,13.904207229614258,1.8558483609209513e-05
5545,43960,43960,87920,13.953518152236938,1.8532081433165425e-05
5572,44174,44174,88348,14.003972053527832,1.767721978794513e-05
5598,44382,44382,88764,14.055486917495728,1.7389935439783714e-05
5625,44598,44598,89196,14.105928897857666,1.7276129137474404e-05
5651,44806,44806,89612,14.154624938964844,1.7213037357547875e-05
5678,45022,45022,90044,14.204571962356567,1.716696847020796e-05
5704,45228,45228,90456,14.253201961517334,1.6186359514089838e-05
5731,45444,45444,90888,14.303974866867065,1.5982886028568674e-05
5757,45652,45652,91304,14.352151155471802,1.589167484100302e-05
5784,45868,45868,91736,14.404288053512573,1.583112628223609e-05
5810,46076,46076,92152,14.452955961227417,1.5788194825316296e-05
5837,46292,46292,92584,14.50324296951294,1.5752546291371434e-05
5863,46500,46500,93000,14.552881002426147,1.5723608572896556e-05
5890,46716,46716,93432,14.602864265441895,1.5697301367058494e-05
5917,46932,46932,93864,14.652223110198975,1.567368645439576e-05
5943,47140,47140,94280,14.701200246810913,1.5652818882483105e-05
5970,47356,47356,94712,14.75200891494751,1.5632632524878597e-05
5996,47564,47564,95128,14.800342082977295,1.561432099992208e-05
6023,47778,47778,95556,14.851035833358765,1.4833382146013845e-05
6049,47986,47986,95972,14.904275894165039,1.4740859336284681e-05
6076,48202,48202,96404,14.962889909744263,1.4690054270272048e-05
6102,48410,48410,96820,15.023020029067993,1.4657230486153633e-05
6129,48626,48626,97252,15.078128814697266,1.4631399466933933e-05
6155,48834,48834,97668,15.129851818084717,1.4611021257114592e-05
6182,49050,49050,98100,15.185184955596924,1.4592725805484992e-05
6208,49256,49256,98512,15.238086938858032,1.385770588114784e-05
6235,49472,49472,98944,15.29203724861145,1.3573134293083075e-05
6261,49680,49680,99360,15.342271089553833,1.3476653544717966e-05
6288,49896,49896,99792,15.396870851516724,1.3422781397062628e-05
6315,50112,50112,100224,15.451764106750488,1.3386889368457435e-05
6341,50320,50320,100640,15.500114917755127,1.3360765867466923e-05
6368,50534,50534,101068,15.550987958908081,1.2698403827586001e-05
6394,50742,50742,101484,15.599744081497192,1.2521258501181357e-05
6421,50958,50958,101916,15.64988112449646,1.2450217423193459e-05
6447,51166,51166,102332,15.698907136917114,1.240840802423431e-05
6474,51382,51382,102764,15.749876976013184,1.2376396963969564e-05
6500,51590,51590,103180,15.798398971557617,1.2351684303538062e-05
6527,51806,51806,103612,15.848531007766724,1.2330029388741112e-05
6553,52014,52014,104028,15.901179075241089,1.231180578199364e-05
6580,52230,52230,104460,15.950672149658203,1.2294817618689408e-05
6606,52438,52438,104876,15.998822927474976,1.2279832288967316e-05
6633,52654,52654,105308,16.052660942077637,1.2265347795433905e-05
6659,52862,52862,105724,16.100779056549072,1.2252205896324105e-05
6686,53078,53078,106156,16.15157723426819,1.2239222188055422e-05
6712,53286,53286,106572,16.200420141220093,1.2227238107172625e-05
6739,53502,53502,107004,16.250648021697998,1.2215237525064696e-05
6766,53718,53718,107436,16.30125594139099,1.2203616917566838e-05
6792,53926,53926,107852,16.350656032562256,1.2192732465262935e-05
6819,54120,54120,108240,16.39771604537964,6.482293554408768e-06
6845,54314,54314,108628,16.44376802444458,3.3639300084132412e-06
6872,54518,54518,109036,16.49209713935852,2.270950508417078e-06
6898,54726,54726,109452,16.541006088256836,2.2116137144652923e-06
6925,54942,54942,109884,16.59039306640625,2.186084970010495e-06
6951,55150,55150,110300,16.64016318321228,2.168025181538764e-06
6978,55366,55366,110732,16.689915895462036,2.1524448853865892e-06
7004,55574,55574,111148,16.738728046417236,2.139294690385555e-06
7031,55790,55790,111580,16.789462089538574,2.1269952429169403e-06
7057,55998,55998,111996,16.836831092834473,2.1161749091863977e-06
7084,56214,56214,112428,16.89032816886902,2.1058222042766963e-06
7110,56414,56414,112828,16.94182300567627,1.98294391508423e-06
7137,56630,56630,113260,16.991131067276,1.9792618539584646e-06
7164,56846,56846,113692,17.047528982162476,1.9762809987192465e-06
7190,57046,57046,114092,17.10164713859558,1.9087559147450525e-06
7217,57262,57262,114524,17.15247893333435,1.8643889327961766e-06
7243,57470,57470,114940,17.201712131500244,1.8458751871396735e-06
7270,57686,57686,115372,17.252121210098267,1.8356146779659014e-06
7296,57894,57894,115788,17.301172018051147,1.8293256503856762e-06
7323,58110,58110,116220,17.35158920288086,1.8245883139306753e-06
7349,58318,58318,116636,17.402512073516846,1.8209902102157538e-06
7376,58534,58534,117068,17.452580213546753,1.817868278983619e-06
7402,58742,58742,117484,17.500495195388794,1.8152533241548102e-06
7429,58958,58958,117916,17.549904108047485,1.8128177782991241e-06
7455,59166,59166,118332,17.59753108024597,1.8106655668664043e-06
7482,59382,59382,118764,17.64752507209778,1.8085778966767408e-06
7508,59590,59590,119180,17.695736169815063,1.8066750183025746e-06
7535,59806,59806,119612,17.746268033981323,1.8047854498155256e-06
7561,60014,60014,120028,17.794738054275513,1.8030322804317549e-06
7588,60230,60230,120460,17.844583988189697,1.801267860115637e-06
7615,60446,60446,120892,17.896639108657837,1.7995511348484285e-06
7641,60654,60654,121308,17.944512128829956,1.7979363100339613e-06
7668,60870,60870,121740,17.995028972625732,1.7962938086400112e-06
7694,61078,61078,122156,18.04370903968811,1.7947413116437452e-06
7721,61270,61270,122540,18.089659214019775,9.801651153810561e-07
7747,61470,61470,122940,18.1358060836792,7.781729287710595e-07
7774,61686,61686,123372,18.186150074005127,7.503228693316351e-07
7800,61894,61894,123788,18.234426259994507,7.418855873121678e-07
7827,62110,62110,124220,18.284271240234375,7.365605839453741e-07
7853,62318,62318,124636,18.332539081573486,7.328164468601248e-07
7880,62534,62534,125068,18.38431215286255,7.29654143769554e-07
7906,62742,62742,125484,18.431912899017334,7.270154935204601e-07
7933,62958,62958,125916,18.48183012008667,7.245492044228381e-07
7959,63166,63166,126332,18.530248880386353,7.223636358777695e-07
7986,63382,63382,126764,18.580140113830566,7.20245787112376e-07
8013,63598,63598,127196,18.63086485862732,7.182543787362395e-07
8039,63806,63806,127612,18.67930507659912,7.164385431988053e-07
8066,64022,64022,128044,18.729897022247314,7.146456933932975e-07
8092,64230,64230,128460,18.777682065963745,7.129994931471628e-07
8119,64446,64446,128892,18.827536821365356,7.113657977680619e-07
8145,64654,64654,129308,18.87870502471924,7.098598008838166e-07
8172,64870,64870,129740,18.92972207069397,7.083604933061446e-07
8198,65076,65076,130152,18.97933006286621,6.756001307624728e-07
8225,65292,65292,130584,19.029873847961426,6.729801542818347e-07
8251,65500,65500,131000,19.079803228378296,6.714996219268264e-07
8278,65716,65716,131432,19.13465189933777,6.702772168642425e-07
8304,65924,65924,131848,19.19125199317932,6.692491455597113e-07
8331,66140,66140,132280,19.242733001708984,6.682719202926963e-07
8357,66348,66348,132696,19.290716886520386,6.673892975390276e-07
8384,66564,66564,133128,19.342061042785645,6.66517638233652e-07
8410,66772,66772,133544,19.3908851146698,6.657128630435071e-07
8437,66988,66988,133976,19.442065000534058,6.649072711239891e-07
8464,67204,67204,134408,19.49208402633667,6.641282907642649e-07
8490,67412,67412,134824,19.540704011917114,6.634004194547181e-07
8517,67628,67628,135256,19.59184217453003,6.626652972668231e-07
8543,67836,67836,135672,19.639536142349243,6.619755233032762e-07
8570,68052,68052,136104,19.689499139785767,6.612763863520846e-07
8596,68258,68258,136516,19.73823595046997,6.286452096010413e-07
8623,68474,68474,136948,19.78730010986328,6.251089808166837e-07
8649,68682,68682,137364,19.835302114486694,6.230268121186324e-07
8676,68898,68898,137796,19.889683961868286,6.215168058506068e-07
8702,69106,69106,138212,19.939322233200073,6.203976927035464e-07
8729,69322,69322,138644,19.989410161972046,6.194328866853801e-07
8755,69530,69530,139060,20.037353992462158,6.186206863532935e-07
8782,69746,69746,139492,20.08672523498535,6.178571688906542e-07
8808,69954,69954,139908,20.13473892211914,6.171764181573655e-07
8835,70170,70170,140340,20.184968948364258,6.165116706574259e-07
8862,70386,70386,140772,20.234918117523193,6.158803963944961e-07
8888,70594,70594,141188,20.281707048416138,6.152979172811688e-07
8915,70810,70810,141620,20.33037304878235,6.147147281486978e-07
8941,71018,71018,142036,20.378523111343384,6.141706301989394e-07
8968,71234,71234,142468,20.433488130569458,6.136209648111344e-07
8994,71442,71442,142884,20.488720178604126,6.1310430710107e-07
9021,71654,71654,143308,20.549326181411743,5.620021354457368e-07
9047,71848,71848,143696,20.60204315185547,3.723914763882819e-07
9074,72050,72050,144100,20.658984899520874,2.4833383964094253e-07
9100,72248,72248,144496,20.717812061309814,1.8466403470263716e-07
9127,72464,72464,144928,20.779590845108032,1.7420796618528976e-07
9153,72672,72672,145344,20.835480213165283,1.7292155133234222e-07
9180,72888,72888,145776,20.89610505104065,1.7207727437454413e-07
9206,73096,73096,146192,20.950842142105103,1.7140184167528777e-07
9233,73312,73312,146624,21.005342960357666,1.707717564810728e-07
9260,73528,73528,147056,21.059011220932007,1.701886737779958e-07
9286,73736,73736,147472,21.111257076263428,1.6966064848449172e-07
9313,73946,73946,147892,21.16248917579651,1.69141043085831e-07
9339,74152,74152,148304,21.217949867248535,1.5947512978053335e-07
9366,74368,74368,148736,21.27544403076172,1.5919279360662965e-07
9392,74576,74576,149152,21.324481964111328,1.5898597842920977e-07
9419,74792,74792,149584,21.37867283821106,1.5880803491966152e-07
9445,75000,75000,150000,21.430424213409424,1.5865685862431035e-07
9472,75216,75216,150432,21.482807159423828,1.585121223568774e-07
9498,75424,75424,150848,21.532416105270386,1.5837994682162644e-07
9525,75630,75630,151260,21.581794023513794,1.1965190799828172e-07
9551,75836,75836,151672,21.630789041519165,1.0592199434159446e-07
9578,76052,76052,152104,21.68128514289856,1.0449529241836949e-07
9604,76260,76260,152520,21.73021411895752,1.0354478427472251e-07
9631,76476,76476,152952,21.78104019165039,1.0276150971058099e-07
9657,76676,76676,153352,21.827311038970947,9.86717853306269e-08
9684,76892,76892,153784,21.877404928207397,9.780045947312819e-08
9711,77108,77108,154216,21.927419185638428,9.724207223556604e-08
9737,77316,77316,154632,21.977187156677246,9.68623231874329e-08
9764,77532,77532,155064,22.02715492248535,9.656059279363799e-08
9790,77740,77740,155480,22.075666904449463,9.632317302782461e-08
9817,77956,77956,155912,22.1256160736084,9.611076050759287e-08
9843,78164,78164,156328,22.17411994934082,9.59276015170029e-08
9870,78380,78380,156760,22.22452211380005,9.575243317811626e-08
9896,78588,78588,157176,22.272881984710693,9.559405765308704e-08
9923,78802,78802,157604,22.324765920639038,9.227767550154768e-08
9949,79010,79010,158020,22.38255214691162,9.200554586484151e-08
9976,79226,79226,158452,22.43379306793213,9.181538367428163e-08
10002,79434,79434,158868,22.482731103897095,9.166570102827042e-08
10029,79650,79650,159300,22.532649993896484,9.153007157506743e-08
10055,79858,79858,159716,22.581478118896484,9.14116503851238e-08
10082,80074,80074,160148,22.632692098617554,9.129713068686918e-08
10109,80290,80290,160580,22.68545627593994,9.118858925198865e-08
10135,80498,80498,160996,22.733687162399292,9.108811488150926e-08
10162,80712,80712,161424,22.789479970932007,8.667864439282008e-08
10188,80920,80920,161840,22.8406081199646,8.642929024252174e-08
10215,81136,81136,162272,22.89767813682556,8.629158749435724e-08
10241,81344,81344,162688,22.948019981384277,8.618882748105997e-08
10268,81560,81560,163120,22.998101949691772,8.609557781321453e-08
10294,81768,81768,163536,23.047685861587524,8.601268011064987e-08
10321,81984,81984,163968,23.098492860794067,8.593082352599343e-08
10347,82192,82192,164384,23.14786195755005,8.585461479682454e-08
10374,82408,82408,164816,23.200469970703125,8.577731566606505e-08
10400,82614,82614,165228,23.25110101699829,8.17988332361502e-08
10427,82830,82830,165660,23.305029153823853,8.157275877362854e-08
10453,83038,83038,166076,23.364810943603516,8.146733951408776e-08
10480,83254,83254,166508,23.419806957244873,8.137651748780843e-08
10506,83462,83462,166924,23.468239068984985,8.129732007146897e-08
10533,83678,83678,167356,23.518683195114136,8.122024007359589e-08
10560,83894,83894,167788,23.570927143096924,8.114670475157896e-08
10586,84100,84100,168200,23.62405300140381,7.833127836595647e-08
10613,84316,84316,168632,23.676099061965942,7.764364776059635e-08
10639,84524,84524,169048,23.725605249404907,7.745628663066036e-08
10666,84740,84740,169480,23.778044939041138,7.733738485397787e-08
10692,84948,84948,169896,23.831854104995728,7.724683071272162e-08
10719,85164,85164,170328,23.886877059936523,7.716440351294449e-08
10745,85372,85372,170744,23.935550928115845,7.709154477897092e-08
10772,85588,85588,171176,23.986334085464478,7.702030129864721e-08
10798,85796,85796,171592,24.03543496131897,7.695469488341327e-08
10825,86004,86004,172008,24.084764003753662,6.316672723335424e-08
10851,86212,86212,172424,24.134387016296387,5.813363702737362e-08
10878,86428,86428,172856,24.184941053390503,5.618370974052356e-08
10904,86636,86636,173272,24.23318910598755,5.518371329034335e-08
10931,86852,86852,173704,24.283013820648193,5.454329638168174e-08
10958,87068,87068,174136,24.332093000411987,5.4115837639667745e-08
10984,87276,87276,174552,24.383673191070557,5.3821811535306644e-08
11011,87492,87492,174984,24.44175910949707,5.3592728675997555e-08
11037,87700,87700,175400,24.491987943649292,5.342022788966661e-08
11064,87916,87916,175832,24.542477130889893,5.3274701286936864e-08
11090,88124,88124,176248,24.592432260513306,5.3157070179074445e-08
11117,88340,88340,176680,24.64319109916687,5.305152701628783e-08
11143,88548,88548,177096,24.692174196243286,5.296160751452458e-08
11170,88764,88764,177528,24.743088245391846,5.2877327217727946e-08
11196,88970,88970,177940,24.79142189025879,4.9783385491705415e-08
11223,89186,89186,178372,24.840841054916382,4.945330673917523e-08
11249,89394,89394,178788,24.890552043914795,4.9271480786476946e-08
11276,89610,89610,179220,24.940301179885864,4.914475998891065e-08
11302,89818,89818,179636,24.990463972091675,4.905379858482024e-08
11329,90034,90034,180068,25.040336847305298,4.897759757382978e-08
11355,90242,90242,180484,25.090471982955933,4.891505234113249e-08
11382,90458,90458,180916,25.14059591293335,4.885744841418883e-08
11409,90674,90674,181348,25.190388917922974,4.8804993642807103e-08
11435,90882,90882,181764,25.238043069839478,4.875796069146215e-08
11462,91096,91096,182192,25.288090229034424,4.575166839789606e-08
11488,91304,91304,182608,25.336988925933838,4.55688873928656e-08
11515,91520,91520,183040,25.39331889152527,4.5458319221530755e-08
11541,91728,91728,183456,25.450122117996216,4.538090126222209e-08
11568,91944,91944,183888,25.504317045211792,4.5316655701045794e-08
11594,92152,92152,184304,25.552917003631592,4.52641516814563e-08
11621,92368,92368,184736,25.603116989135742,4.521582090614254e-08
11647,92576,92576,185152,25.653565883636475,4.5173269128871444e-08
11674,92792,92792,185584,25.704499006271362,4.513192945893812e-08
11700,92998,92998,185996,25.753700017929077,4.163714744965339e-08
11727,93214,93214,186428,25.803696155548096,4.144332863243436e-08
11753,93422,93422,186844,25.851476907730103,4.134266753725041e-08
11780,93638,93638,187276,25.907927989959717,4.127226566162487e-08
11807,93854,93854,187708,25.958820104599,4.1217338384369516e-08
11833,94062,94062,188124,26.008170127868652,4.117186465101644e-08
11860,94278,94278,188556,26.058440923690796,4.1129090114746646e-08
11886,94486,94486,188972,26.106034994125366,4.109066062612021e-08
11913,94702,94702,189404,26.156266927719116,4.105273767226845e-08
11939,94910,94910,189820,26.204665184020996,4.1017621737603926e-08
11966,95126,95126,190252,26.2553391456604,4.098226375312266e-08
11992,95332,95332,190664,26.305809020996094,3.83847210881023e-08
12019,95548,95548,191096,26.362330198287964,3.8051233488664596e-08
12045,95756,95756,191512,26.416726112365723,3.791001716447089e-08
12072,95972,95972,191944,26.469808101654053,3.7829467808583773e-08
12098,96180,96180,192360,26.517718076705933,3.777775298966859e-08
12125,96396,96396,192792,26.569414854049683,3.7735703347069324e-08
12151,96604,96604,193208,26.62083888053894,3.770062140112706e-08
12178,96818,96818,193636,26.674744129180908,3.4902535742452574e-08
12205,97034,97034,194068,26.72801685333252,3.465925042674646e-08
12231,97242,97242,194484,26.77686309814453,3.454366353881045e-08
12258,97458,97458,194916,26.827497005462646,3.446773901955822e-08
12284,97666,97666,195332,26.876457929611206,3.441327483601478e-08
12311,97882,97882,195764,26.926454067230225,3.436641193091832e-08
12337,98090,98090,196180,26.975163221359253,3.432662959794648e-08
12364,98306,98306,196612,27.02936816215515,3.4288814981487295e-08
12390,98514,98514,197028,27.08163809776306,3.425470944099852e-08
12417,98730,98730,197460,27.146308183670044,3.422102724832726e-08
12443,98938,98938,197876,27.204560041427612,3.418986217681712e-08
12470,99154,99154,198308,27.261170864105225,3.4158532898019955e-08
12496,99362,99362,198724,27.314191102981567,3.412917072387689e-08
12523,99576,99576,199152,27.370328187942505,3.194309532705665e-08
12549,99784,99784,199568,27.42475700378418,3.1315165970127556e-08
12576,100000,100000,200000,27.4806489944458,3.1044566147961335e-08
12602,100208,100208,200416,27.543943881988525,3.090317425505134e-08
12629,100424,100424,200848,27.604400873184204,3.081174422222816e-08
12656,100640,100640,201280,27.6634361743927,3.074823991389183e-08
12682,100848,100848,201696,27.715656042099,3.070120081788147e-08
12709,101064,101064,202128,27.771205186843872,3.066082275194959e-08
12735,101272,101272,202544,27.823642253875732,3.062702181098593e-08
12762,101486,101486,202972,27.880073070526123,2.9307676128613264e-08
12788,101694,101694,203388,27.934751987457275,2.9096734719838536e-08
12815,101910,101910,203820,27.994017124176025,2.898005122135084e-08
12841,102118,102118,204236,28.047703981399536,2.8902928859335093e-08
12868,102334,102334,204668,28.103469133377075,2.8842142406016128e-08
12894,102542,102542,205084,28.155792236328125,2.8795023281197162e-08
12921,102758,102758,205516,28.20711922645569,2.8753917271565133e-08
12947,102966,102966,205932,28.273011922836304,2.8719556187250218e-08
12974,103182,103182,206364,28.357230186462402,2.86877131792045e-08
13000,103390,103390,206780,28.418761014938354,2.8659724584423115e-08
13027,103604,103604,207208,28.474779844284058,2.659026505587146e-08
13054,103820,103820,207640,28.53519105911255,2.636255937348481e-08
13080,104028,104028,208056,28.585851907730103,2.6256863352299592e-08
13107,104244,104244,208488,28.63621997833252,2.6190476352213853e-08
13133,104452,104452,208904,28.68430495262146,2.6144825070483548e-08
13160,104668,104668,209336,28.734463930130005,2.6107006968988892e-08
13186,104876,104876,209752,28.783596992492676,2.6075972671658692e-08
13213,105092,105092,210184,28.833627939224243,2.6047317571927962e-08
13239,105300,105300,210600,28.882442951202393,2.6022079397370064e-08
13266,105514,105514,211028,28.933040142059326,2.497332232133732e-08
13292,105722,105722,211444,28.981913089752197,2.4859480227465657e-08
13319,105938,105938,211876,29.032305002212524,2.4790877569155815e-08
13345,106146,106146,212292,29.080727100372314,2.4743813792967105e-08
13372,106362,106362,212724,29.130887985229492,2.470558568156012e-08
13398,106570,106570,213140,29.181886911392212,2.4675066808632903e-08
13425,106778,106778,213556,29.232605934143066,2.1045778916679627e-08
13451,106976,106976,213952,29.2795672416687,1.4553750854105837e-08
13478,107188,107188,214376,29.32932209968567,1.236392872331942e-08
13505,107404,107404,214808,29.383002042770386,1.2247491512100302e-08
13531,107612,107612,215224,29.431856870651245,1.2179613449260736e-08
13558,107828,107828,215656,29.482610940933228,1.2123073861701939e-08
13584,108036,108036,216072,29.537065982818604,1.2076613183021443e-08
13611,108252,108252,216504,29.5905442237854,1.2034137452234584e-08
13637,108460,108460,216920,29.645643949508667,1.1997461293452776e-08
13664,108676,108676,217352,29.6995689868927,1.196287106476073e-08
13690,108884,108884,217768,29.747686862945557,1.1932340287563358e-08
13717,109100,109100,218200,29.798168182373047,1.190306446652295e-08
13743,109308,109308,218616,29.847097158432007,1.1876880233006802e-08
13770,109524,109524,219048,29.897136211395264,1.18514976923426e-08
13796,109732,109732,219464,29.945804119110107,1.182858446365172e-08
13823,109948,109948,219896,29.996986150741577,1.180619397618999e-08
13849,110156,110156,220312,30.04659104347229,1.1785837205279528e-08
13876,110372,110372,220744,30.097466230392456,1.176581678821107e-08
13903,110588,110588,221176,30.146849155426025,1.1746821356667623e-08
13929,110796,110796,221592,30.19627022743225,1.172940310007071e-08
13956,111012,111012,222024,30.246073007583618,1.1712135716461398e-08
13982,111220,111220,222440,30.294625997543335,1.1696225662091161e-08
14009,111436,111436,222872,30.344796895980835,1.1680381510232621e-08
14035,111644,111644,223288,30.39616584777832,1.1665719284864168e-08
14062,111860,111860,223720,30.44754195213318,1.1651056692459972e-08
14088,112068,112068,224136,30.49672293663025,1.163743376032991e-08
14115,112284,112284,224568,30.54746389389038,1.1623758594755423e-08
14141,112492,112492,224984,30.59538197517395,1.1611006123656809e-08
14168,112708,112708,225416,30.645906925201416,1.159815956643294e-08
14194,112916,112916,225832,30.695049047470093,1.1586139538087852e-08
14221,113132,113132,226264,30.74705195426941,1.1573991347201891e-08
14247,113340,113340,226680,30.79545497894287,1.1562589571373698e-08
14274,113556,113556,227112,30.852461099624634,1.155103199665218e-08
14300,113762,113762,227524,30.90613293647766,1.0982508411257378e-08
14327,113978,113978,227956,30.959094047546387,1.090987165721981e-08
14354,114194,114194,228388,31.01079821586609,1.088336695132162e-08
14380,114402,114402,228804,31.05874514579773,1.0863512732264081e-08
14407,114618,114618,229236,31.108379125595093,1.0845882574431997e-08
14433,114826,114826,229652,31.158926010131836,1.0830851153903378e-08
14460,115042,115042,230084,31.21569514274597,1.0816724192029043e-08
14486,115250,115250,230500,31.26387310028076,1.080421660512175e-08
14513,115466,115466,230932,31.313596963882446,1.0792120988216546e-08
14539,115674,115674,231348,31.366277933120728,1.0781161809274484e-08
14566,115890,115890,231780,31.4201819896698,1.0770360356367054e-08
14592,116098,116098,232196,31.472080945968628,1.0760416493944473e-08
14619,116314,116314,232628,31.525202989578247,1.0750483415794483e-08
14645,116522,116522,233044,31.576033115386963,1.0741234573542822e-08
14672,116738,116738,233476,31.63325595855713,1.0731905754956147e-08
14698,116946,116946,233892,31.689652919769287,1.0723147314237343e-08
14725,117160,117160,234320,31.751626014709473,1.0374589811499138e-08
14752,117374,117374,234748,31.80627202987671,9.320273746872426e-09
14778,117582,117582,235164,31.85559606552124,9.260128457516207e-09
14805,117798,117798,235596,31.91099214553833,9.215131147704734e-09
14831,118006,118006,236012,31.96307611465454,9.181827817177534e-09
14858,118222,118222,236444,32.01792788505554,9.154425713617178e-09
14884,118430,118430,236860,32.0681049823761,9.133005829606647e-09
14911,118646,118646,237292,32.12005805969238,9.114513777369648e-09
14937,118854,118854,237708,32.18181920051575,9.099373503176047e-09
14964,119070,119070,238140,32.266319036483765,9.085705376534355e-09
14990,119278,119278,238556,32.32625699043274,9.074028506686815e-09
15017,119494,119494,238988,32.39094090461731,9.063064704379459e-09
15043,119702,119702,239404,32.447272062301636,9.053360651992557e-09
15070,119918,119918,239836,32.49844813346863,9.043962507617825e-09
15096,120126,120126,240252,32.54803800582886,9.03541975109878e-09
15123,120342,120342,240684,32.59802508354187,9.026959939626707e-09
15150,120558,120558,241116,32.6484010219574,9.018830723275011e-09
15176,120766,120766,241532,32.69691014289856,9.011251569502171e-09
15203,120982,120982,241964,32.747188091278076,9.003588985830203e-09
15229,121190,121190,242380,32.79479908943176,8.996374215236541e-09
15256,121404,121404,242808,32.84459710121155,8.715461560364205e-09
15282,121612,121612,243224,32.89502215385437,8.610825268513496e-09
15309,121828,121828,243656,32.94524598121643,8.59607336829992e-09
15335,122036,122036,244072,32.99638605117798,8.586479355359625e-09
15362,122252,122252,244504,33.054309129714966,8.577900022289505e-09
15388,122460,122460,244920,33.10907793045044,8.570296918568652e-09
15415,122676,122676,245352,33.16472911834717,8.562816165330635e-09
15441,122884,122884,245768,33.218985080718994,8.555884437056221e-09
15468,123100,123100,246200,33.279412031173706,8.548889867276195e-09
15494,123306,123306,246612,33.33303189277649,8.233370725752458e-09
15521,123522,123522,247044,33.38973808288574,8.211566194343423e-09
15547,123730,123730,247460,33.44302487373352,8.198681646946204e-09
15574,123946,123946,247892,33.494619846343994,8.188283438579382e-09
15601,124162,124162,248324,33.5453839302063,8.179475718755337e-09
15627,124370,124370,248740,33.59361791610718,8.17190438034602e-09
15654,124580,124580,249160,33.67481303215027,7.195085328884555e-09
15680,124784,124784,249568,33.73996901512146,5.925531959866341e-09
15707,125000,125000,250000,33.80896306037903,5.691676408991624e-09
15733,125208,125208,250416,33.874415159225464,5.5560109956803855e-09
15760,125424,125424,250848,33.930258989334106,5.4592591957152336e-09
15786,125632,125632,251264,33.98092317581177,5.391567091981272e-09
15813,125848,125848,251696,34.033231019973755,5.3385185938728485e-09
15839,126056,126056,252112,34.082342863082886,5.298886310054247e-09
15866,126272,126272,252544,34.13430094718933,5.266179172146452e-09
15892,126480,126480,252960,34.18434715270996,5.2406463343738636e-09
15919,126696,126696,253392,34.23627710342407,5.218754435385755e-09
15945,126904,126904,253808,34.28565311431885,5.201072979909106e-09
15972,127120,127120,254240,34.3376669883728,5.185443091330974e-09
15999,127336,127336,254672,34.393638134002686,5.171997311307352e-09
16025,127544,127544,255088,34.44420409202576,5.160689319570114e-09
16052,127760,127760,255520,34.493520975112915,5.1503127437608225e-09
16078,127968,127968,255936,34.54524326324463,5.1413886712758564e-09
16105,128184,128184,256368,34.60092115402222,5.133026363909419e-09
16131,128392,128392,256784,34.65673494338989,5.125691344672317e-09
16158,128608,128608,257216,34.71256184577942,5.118689537511902e-09
16184,128816,128816,257632,34.767301082611084,5.1124402862707104e-09
16211,129032,129032,258064,34.822365045547485,5.106377769025786e-09
16237,129240,129240,258480,34.87619090080261,5.1008850375156776e-09
16264,129456,129456,258912,34.93346619606018,5.095482561902372e-09
16290,129664,129664,259328,34.98952388763428,5.090525392073564e-09
16317,129880,129880,259760,35.048032999038696,5.08559331970645e-09
16343,130084,130084,260168,35.09870791435242,4.618778577597207e-09
16370,130300,130300,260600,35.149214029312134,4.554179139759402e-09
16396,130508,130508,261016,35.19755005836487,4.521653940727291e-09
16423,130724,130724,261448,35.24903607368469,4.497917475463576e-09
16450,130940,130940,261880,35.29940986633301,4.4799388424928055e-09
16476,131148,131148,262296,35.34702801704407,4.466201780216034e-09
16503,131364,131364,262728,35.40149188041687,4.454545987175855e-09
16529,131572,131572,263144,35.45062208175659,4.445156950781284e-09
16556,131788,131788,263576,35.591886043548584,4.436821940854117e-09
16582,131996,131996,263992,35.646016120910645,4.42982591298641e-09
16609,132212,132212,264424,35.70308804512024,4.42337660043316e-09
16635,132420,132420,264840,35.76995396614075,4.417773109351732e-09
16662,132636,132636,265272,35.8276801109314,4.4124441200368086e-09
16688,132844,132844,265688,35.88564109802246,4.407683415478625e-09
16715,133060,133060,266120,35.94725823402405,4.403044677890086e-09
16741,133268,133268,266536,36.00890898704529,4.398812521389773e-09
16768,133484,133484,266968,36.0633909702301,4.394613678109437e-09
16794,133692,133692,267384,36.11515402793884,4.390724021084872e-09
16821,133908,133908,267816,36.1669659614563,4.3868152453647095e-09
16848,134124,134124,268248,36.21695899963379,4.383015999669431e-09
16874,134332,134332,268664,36.26975417137146,4.379443491810952e-09
16901,134548,134548,269096,36.32217502593994,4.375808526586297e-09
16927,134756,134756,269512,36.374449014663696,4.372369220312512e-09
16954,134972,134972,269944,36.42697501182556,4.368851517729395e-09
16980,135180,135180,270360,36.479249000549316,4.365508707869389e-09
17007,135396,135396,270792,36.532305002212524,4.36207736293431e-09
17033,135604,135604,271208,36.58330702781677,4.358806734886172e-09
17060,135820,135820,271640,36.636688232421875,4.355440800389815e-09
17086,136022,136022,272044,36.68683218955994,3.9408908228585145e-09
17113,136236,136236,272472,36.73975706100464,3.3767703592315993e-09
17139,136444,136444,272888,36.79060506820679,3.3286268534980642e-09
17166,136660,136660,273320,36.842817068099976,3.294793623118673e-09
17192,136868,136868,273736,36.894779205322266,3.2693279413006996e-09
17219,137084,137084,274168,36.948055028915405,3.24788356801964e-09
17245,137292,137292,274584,36.99920415878296,3.2307504188389805e-09
17272,137508,137508,275016,37.05271291732788,3.215700319554067e-09
17299,137724,137724,275448,37.10410404205322,3.202792623548526e-09
17325,137932,137932,275864,37.15147590637207,3.191939876005199e-09
17352,138148,138148,276296,37.20134615898132,3.1819628701729116e-09
17378,138356,138356,276712,37.24997806549072,3.1733533191032393e-09
17405,138572,138572,277144,37.299586057662964,3.165250856427533e-09
17431,138780,138780,277560,37.34944701194763,3.158109884443869e-09
17458,138996,138996,277992,37.40211796760559,3.151261752483314e-09
17484,139204,139204,278408,37.45095205307007,3.1451252913683666e-09
17511,139420,139420,278840,37.50161623954773,3.1391535714073467e-09
17537,139628,139628,279256,37.54983305931091,3.1337332640965935e-09
17564,139844,139844,279688,37.59930491447449,3.128399474120118e-09
17590,140052,140052,280104,37.647162199020386,3.123510293729514e-09
17617,140268,140268,280536,37.697954177856445,3.118658431715808e-09
17643,140476,140476,280952,37.7463219165802,3.1141779322513166e-09
17670,140692,140692,281384,37.796600103378296,3.1097024640190265e-09
17697,140908,140908,281816,37.84666705131531,3.1053890385944543e-09
17723,141116,141116,282232,37.89457416534424,3.1013734504982132e-09
17750,141332,141332,282664,37.94523811340332,3.0973338166260963e-09
17776,141540,141540,283080,37.99736499786377,3.093558130701936e-09
17803,141756,141756,283512,38.05302405357361,3.089746298581286e-09
17829,141964,141964,283928,38.108344078063965,3.0861723338235445e-09
17856,142180,142180,284360,38.15922784805298,3.082553401273512e-09
17882,142388,142388,284776,38.20794701576233,3.079151361544254e-09
17909,142604,142604,285208,38.25897693634033,3.0756980568011367e-09
17935,142812,142812,285624,38.306660175323486,3.072444263803485e-09
17962,143028,143028,286056,38.35919523239136,3.069134768265108e-09
17988,143236,143236,286472,38.413970947265625,3.0660104697680355e-09
18015,143452,143452,286904,38.46690106391907,3.0628264067277634e-09
18041,143660,143660,287320,38.51557922363281,3.059815441631472e-09
18068,143876,143876,287752,38.566279888153076,3.0567421645807584e-09
18095,144092,144092,288184,38.61624717712402,3.0537202160345224e-09
18121,144300,144300,288600,38.66462802886963,3.0508558870224063e-09
18148,144516,144516,289032,38.71491503715515,3.047926053028114e-09
18174,144724,144724,289448,38.76386094093323,3.0451454077027916e-09
18201,144940,144940,289880,38.81441617012024,3.0422975550416937e-09
18227,145148,145148,290296,38.863539934158325,3.0395913072104352e-09
18254,145364,145364,290728,38.91473412513733,3.036816638105382e-09
18280,145572,145572,291144,38.96329712867737,3.0341770284884322e-09
18307,145788,145788,291576,39.01370286941528,3.0314679338448213e-09
18333,145994,145994,291988,39.062337160110474,2.754252837536229e-09
18360,146202,146202,292404,39.11026406288147,2.0385898557429877e-09
18386,146410,146410,292820,39.16187810897827,1.994119999287948e-09
18413,146626,146626,293252,39.21202611923218,1.9689333183023516e-09
18439,146834,146834,293668,39.26063513755798,1.94946048619299e-09
18466,147050,147050,294100,39.310267210006714,1.9320310663570594e-09
18492,147258,147258,294516,39.35938620567322,1.9172353792188698e-09
18519,147474,147474,294948,39.41061997413635,1.903546985391276e-09
18546,147690,147690,295380,39.461026191711426,1.8912952474175665e-09
18572,147898,147898,295796,39.50906801223755,1.880657267277363e-09
18599,148114,148114,296228,39.56003212928772,1.87064784046831e-09
18625,148322,148322,296644,39.60789394378662,1.8618766874425667e-09
18652,148538,148538,297076,39.65808320045471,1.8535526557777876e-09
18678,148746,148746,297492,39.70688199996948,1.8461984424988483e-09
18705,148962,148962,297924,39.75739502906799,1.8391645374626117e-09
18731,149170,149170,298340,39.805976152420044,1.8329036073810948e-09
18758,149386,149386,298772,39.85540294647217,1.8268727248974085e-09
18784,149594,149594,299188,39.90574502944946,1.8214680092133865e-09
18811,149810,149810,299620,39.95647597312927,1.816227898930003e-09
18837,150018,150018,300036,40.00419521331787,1.811502758740886e-09
18864,150234,150234,300468,40.05579900741577,1.8068944865605773e-09
18890,150442,150442,300884,40.11220622062683,1.8027157062273497e-09
18917,150658,150658,301316,40.16665697097778,1.798618323113457e-09
18944,150874,150874,301748,40.21639704704285,1.7947438998676322e-09
18970,151082,151082,302164,40.26375412940979,1.791203560375327e-09
18997,151298,151298,302596,40.31379508972168,1.787706818681249e-09
19023,151506,151506,303012,40.363829135894775,1.7844972644032896e-09
19050,151722,151722,303444,40.41533017158508,1.7813138038489333e-09
19076,151930,151930,303860,40.4635808467865,1.7783793946203e-09
19103,152146,152146,304292,40.51330900192261,1.7754569847436415e-09
19129,152354,152354,304708,40.56448006629944,1.7727529949171123e-09
19156,152570,152570,305140,40.61795711517334,1.7700502400856208e-09
19182,152778,152778,305556,40.67138886451721,1.7675404771983607e-09
19209,152994,152994,305988,40.72121286392212,1.7650234207386447e-09
19235,153202,153202,306404,40.769288063049316,1.7626784918939504e-09
19262,153418,153418,306836,40.81903409957886,1.760318991122382e-09
19288,153626,153626,307252,40.86920094490051,1.7581142619101856e-09
19315,153842,153842,307684,40.91988205909729,1.755889456913624e-09
19341,154050,154050,308100,40.968666076660156,1.7538050795431167e-09
19368,154266,154266,308532,41.01831603050232,1.7516958916735193e-09
19395,154482,154482,308964,41.068275928497314,1.749639227652956e-09
19421,154690,154690,309380,41.11373710632324,1.7477050430222987e-09
19448,154906,154906,309812,41.16303992271423,1.7457409079203432e-09
19474,155114,155114,310228,41.211714029312134,1.7438894927433297e-09
19501,155330,155330,310660,41.262624979019165,1.7420053845551068e-09
19527,155538,155538,311076,41.31103706359863,1.7402259108605262e-09
19554,155754,155754,311508,41.3635950088501,1.7384114851983098e-09
19580,155962,155962,311924,41.413496017456055,1.7366943934731455e-09
19607,156178,156178,312356,41.46401619911194,1.7349409196723484e-09
19633,156382,156382,312764,41.511337995529175,1.5271291634042704e-09
19660,156598,156598,313196,41.56156015396118,1.5107854313440196e-09
19686,156806,156806,313612,41.61032700538635,1.5063144709264903e-09
19713,157022,157022,314044,41.66008400917053,1.5023580174463173e-09
19739,157230,157230,314460,41.70968294143677,1.4989523914854085e-09
19766,157446,157446,314892,41.760266065597534,1.495739571395177e-09
19793,157662,157662,315324,41.80885910987854,1.4927953241883967e-09
19819,157870,157870,315740,41.85632300376892,1.4901728782336183e-09
19846,158086,158086,316172,41.906113147735596,1.4876374188690583e-09
19872,158294,158294,316588,41.953927993774414,1.48535196312125e-09
19899,158510,158510,317020,42.003265142440796,1.4831195738439229e-09
19925,158718,158718,317436,42.050785064697266,1.4810882622377115e-09
19952,158934,158934,317868,42.10026693344116,1.4790869402255657e-09
19978,159142,159142,318284,42.148316860198975,1.4772517546337678e-09
20005,159358,159358,318716,42.20439600944519,1.4754301305217451e-09
20031,159566,159566,319132,42.25797986984253,1.4737483298424897e-09
20058,159782,159782,319564,42.30746603012085,1.4720683691759985e-09
20084,159990,159990,319980,42.35733604431152,1.4705078418469971e-09
20111,160206,160206,320412,42.41067290306091,1.4689407973703804e-09
20137,160414,160414,320828,42.459264039993286,1.4674777571693796e-09
20164,160630,160630,321260,42.508147954940796,1.4660012941902235e-09
20190,160838,160838,321676,42.55618405342102,1.4646166261070144e-09
20217,161054,161054,322108,42.6059730052948,1.4632135678752492e-09
20244,161270,161270,322540,42.65536093711853,1.4618425866091364e-09
20270,161478,161478,322956,42.7034649848938,1.4605498275857863e-09
20297,161694,161694,323388,42.751118183135986,1.459232956523294e-09
20323,161902,161902,323804,42.799540996551514,1.4579876885932895e-09
20350,162118,162118,324236,42.849205017089844,1.4567156565489237e-09
20376,162326,162326,324652,42.89849591255188,1.455509666668491e-09
20403,162538,162538,325076,42.947962045669556,1.179102050742756e-09
20429,162746,162746,325492,42.99640512466431,1.1390709678442723e-09
20456,162962,162962,325924,43.04764795303345,1.1257066842355735e-09
20482,163170,163170,326340,43.095707178115845,1.1155812259139533e-09
20509,163386,163386,326772,43.14640998840332,1.1067823363195112e-09
20535,163594,163594,327188,43.1945641040802,1.099579377230038e-09
20562,163810,163810,327620,43.24473714828491,1.0931606629145279e-09
20588,164018,164018,328036,43.29170513153076,1.087818871216318e-09
20615,164234,164234,328468,43.34189224243164,1.0829922457087006e-09
20642,164450,164450,328900,43.395617961883545,1.0787757260483052e-09
20668,164658,164658,329316,43.44254803657532,1.0751966132634088e-09
20695,164874,164874,329748,43.491848945617676,1.071897836376734e-09
20721,165082,165082,330164,43.53982424736023,1.069060172424087e-09
20748,165298,165298,330596,43.59014916419983,1.0664094919796405e-09
20774,165506,165506,331012,43.63978815078735,1.0640979707329833e-09
20801,165722,165722,331444,43.688326835632324,1.0619089266474604e-09
20827,165930,165930,331860,43.73467493057251,1.0599741079869308e-09
20854,166146,166146,332292,43.78403997421265,1.058117451883689e-09
20880,166354,166354,332708,43.8307580947876,1.0564548056545894e-09
20907,166570,166570,333140,43.880250215530396,1.0548398821956905e-09
20933,166778,166778,333556,43.92948603630066,1.0533766202824056e-09
20960,166994,166994,333988,43.97951102256775,1.0519391929385193e-09
20986,167202,167202,334404,44.02803301811218,1.0506230640110168e-09
21013,167418,167418,334836,44.07764196395874,1.0493173293545792e-09
21040,167634,167634,335268,44.12799787521362,1.0480657591650542e-09
21066,167842,167842,335684,44.176109075546265,1.0469049775528515e-09
21093,168058,168058,336116,44.22671604156494,1.0457394618823047e-09
21119,168266,168266,336532,44.27908396720886,1.0446512508308197e-09
21146,168482,168482,336964,44.335633993148804,1.0435521564261377e-09
21172,168690,168690,337380,44.386996030807495,1.042519945284346e-09
21199,168906,168906,337812,44.437451124191284,1.041472344239033e-09
21225,169114,169114,338228,44.485151052474976,1.0404840467892877e-09
21252,169330,169330,338660,44.53593111038208,1.0394771214630908e-09
21278,169536,169536,339072,44.58394813537598,9.85951547272177e-10
21305,169752,169752,339504,44.63376212120056,9.806214212964366e-10
21331,169960,169960,339920,44.682072162628174,9.791686172317546e-10
21358,170176,170176,340352,44.73316311836243,9.779500594461906e-10
21384,170384,170384,340768,44.78151297569275,9.76897393553761e-10
21411,170600,170600,341200,44.83208918571472,9.758840346599972e-10
21437,170808,170808,341616,44.88229513168335,9.749646569216198e-10
21464,171024,171024,342048,44.93991804122925,9.740556010145501e-10
21491,171240,171240,342480,44.99752402305603,9.73183896046032e-10
21517,171448,171448,342896,45.04885506629944,9.723729775214853e-10
21544,171664,171664,343328,45.098711013793945,9.715550831735025e-10
21570,171872,171872,343744,45.14943528175354,9.707867863540409e-10
21597,172082,172082,344164,45.2012140750885,8.144034550928322e-10
21623,172274,172274,344548,45.25033402442932,4.91373409501672e-10
21650,172486,172486,344972,45.303022146224976,4.151602240871747e-10
21676,172694,172694,345388,45.36006712913513,4.089318433278169e-10
21703,172910,172910,345820,45.41794991493225,4.0424539430372127e-10
21729,173118,173118,346236,45.4698600769043,4.0051025587859924e-10
21756,173334,173334,346668,45.52254009246826,3.9716101279593727e-10
21782,173542,173542,347084,45.57394504547119,3.9429861477611267e-10
21809,173758,173758,347516,45.62411904335022,3.9160602463260497e-10
21835,173966,173966,347932,45.672693967819214,3.8922170833469605e-10
21862,174182,174182,348364,45.72289681434631,3.8691812204300453e-10
21889,174398,174398,348796,45.773431062698364,3.847578417165901e-10
21915,174606,174606,349212,45.82149291038513,3.8279057883641406e-10
21942,174822,174822,349644,45.87265992164612,3.808474253846863e-10
21968,175030,175030,350060,45.92610216140747,3.7905935832982983e-10
21995,175246,175246,350492,45.97993016242981,3.772780742340626e-10
22021,175454,175454,350908,46.0289421081543,3.756274153721434e-10
22048,175670,175670,351340,46.08059000968933,3.739729566793404e-10
22074,175878,175878,351756,46.13281202316284,3.7243241030792595e-10
22101,176094,176094,352188,46.201526165008545,3.708817024726051e-10
22127,176302,176302,352604,46.433205127716064,3.694322765200313e-10
22154,176518,176518,353036,46.5122811794281,3.679686797219304e-10
22180,176726,176726,353452,46.57299995422363,3.665967902204963e-10
22207,176942,176942,353884,46.634032249450684,3.6520840678293177e-10
22233,177150,177150,354300,46.688392877578735,3.6390427245535956e-10
22260,177366,177366,354732,46.742916107177734,3.62581831325577e-10
22286,177574,177574,355148,46.79462003707886,3.613375323508887e-10
22313,177790,177790,355580,46.85002112388611,3.600742922086493e-10
22340,178006,178006,356012,46.91052603721619,3.588385583389832e-10
22366,178214,178214,356428,46.96736216545105,3.57673780904062e-10
22393,178430,178430,356860,47.02373194694519,3.564891261163934e-10
22419,178638,178638,357276,47.08161401748657,3.553710791742343e-10
22446,178854,178854,357708,47.14038705825806,3.5423326766026594e-10
22472,179062,179062,358124,47.19464302062988,3.531585623849731e-10
22499,179278,179278,358556,47.250508069992065,3.520639728326588e-10
22525,179486,179486,358972,47.305821895599365,3.510296692180383e-10
22552,179702,179702,359404,47.36448788642883,3.499754408001583e-10
22578,179910,179910,359820,47.41852807998657,3.489786885579964e-10
22605,180126,180126,360252,47.47511291503906,3.479621882505795e-10
22631,180332,180332,360664,47.531249046325684,3.372985312260888e-10
22658,180548,180548,361096,47.58519506454468,3.349943576993715e-10
22684,180756,180756,361512,47.63615584373474,3.340261717232244e-10
22711,180972,180972,361944,47.68972206115723,3.331545820719997e-10
22738,181188,181188,362376,47.741945028305054,3.3233303359875036e-10
22764,181396,181396,362792,47.79337406158447,3.3157035223510595e-10
22791,181612,181612,363224,47.8465940952301,3.3080094617036596e-10
22817,181820,181820,363640,48.01314997673035,3.300783797116761e-10
22844,182036,182036,364072,48.10572385787964,3.293448168522896e-10
22870,182244,182244,364488,48.167989015579224,3.286532540158866e-10
22897,182460,182460,364920,48.224138021469116,3.2794961160922876e-10
22923,182668,182668,365336,48.27978301048279,3.2728451747842774e-10
22950,182884,182884,365768,48.337449073791504,3.2660672519701e-10
22976,183092,183092,366184,48.39833402633667,3.259654950650672e-10
23003,183308,183308,366616,48.46144199371338,3.2531099937784675e-10
23029,183516,183516,367032,48.53028702735901,3.2469142870405665e-10
23056,183732,183732,367464,48.5925509929657,3.240582797929899e-10
23082,183940,183940,367880,48.646435022354126,3.2345846325716325e-10
23109,184156,184156,368312,48.70228099822998,3.228452382641829e-10
23135,184364,184364,368728,48.75724005699158,3.2226393113846105e-10
23162,184580,184580,369160,48.8148980140686,3.216691830649567e-10
23189,184796,184796,369592,48.872533082962036,3.210835517590475e-10
23215,185004,185004,370008,48.95948791503906,3.2052789224622424e-10
23242,185220,185220,370440,49.04325819015503,3.1995905758328193e-10
23268,185428,185428,370856,49.10331392288208,3.1941904058920797e-10
23295,185644,185644,371288,49.159088134765625,3.1886624561335006e-10
23321,185852,185852,371704,49.21566414833069,3.183412055992943e-10
23348,186068,186068,372136,49.27568507194519,3.178034182194054e-10
23374,186276,186276,372552,49.32619595527649,3.1729240962248493e-10
23401,186490,186490,372980,49.3791720867157,3.0530152661866424e-10
23427,186698,186698,373396,49.428208112716675,3.026541214832442e-10
23454,186914,186914,373828,49.477944135665894,3.015588263408091e-10
23480,187122,187122,374244,49.52731800079346,3.0068046583234935e-10
23507,187338,187338,374676,49.57732820510864,2.99858525945102e-10
23533,187546,187546,375092,49.626708984375,2.9913065675582827e-10
23560,187762,187762,375524,49.676762104034424,2.984288771599595e-10
23587,187978,187978,375956,49.72454810142517,2.977730559748071e-10
23613,188186,188186,376372,49.77243208885193,2.971789807749287e-10
23640,188402,188402,376804,49.82179307937622,2.965954522969727e-10
23666,188610,188610,377220,49.87063026428223,2.960615318807665e-10
23693,188826,188826,377652,49.921021938323975,2.95532623334152e-10
23719,189034,189034,378068,49.96988105773926,2.950450356696166e-10
23746,189250,189250,378500,50.01989817619324,2.9455880112838426e-10
23772,189458,189458,378916,50.0680410861969,2.9410769399342475e-10
23799,189674,189674,379348,50.117936849594116,2.936551390984652e-10
23825,189882,189882,379764,50.16493105888367,2.9323287124275506e-10
23852,190098,190098,380196,50.213963985443115,2.9280733656749874e-10
23878,190306,190306,380612,50.261582136154175,2.9240884040700086e-10
23905,190522,190522,381044,50.31189513206482,2.920054985676106e-10
23931,190728,190728,381456,50.36308002471924,2.764757535985974e-10
23958,190944,190944,381888,50.424888134002686,2.75019409149424e-10
23985,191160,191160,382320,50.48118805885315,2.742673918304457e-10
24011,191368,191368,382736,50.53324913978577,2.736733691457546e-10
24038,191584,191584,383168,50.589115142822266,2.7313598421803856e-10
24064,191792,191792,383584,50.65294599533081,2.72675247316346e-10
24091,192008,192008,384016,50.7140531539917,2.72242663789203e-10
24117,192216,192216,384432,50.7633159160614,2.7186190157023346e-10
24144,192432,192432,384864,50.81506299972534,2.7149633099463814e-10
24170,192640,192640,385280,50.86906385421753,2.711683434603649e-10
24197,192856,192856,385712,50.92184090614319,2.7084816479115085e-10
24223,193064,193064,386128,50.974138259887695,2.705563842312856e-10
24250,193280,193280,386560,51.02688694000244,2.7026776109276255e-10
24276,193488,193488,386976,51.076475858688354,2.7000171108317374e-10
24303,193704,193704,387408,51.12950801849365,2.697355919207224e-10
24329,193910,193910,387820,51.1793270111084,2.51197061008475e-10
24356,194126,194126,388252,51.22966814041138,2.4948526649906596e-10
24382,194334,194334,388668,51.28073811531067,2.4856049268641e-10
24409,194550,194550,389100,51.329750061035156,2.478319107630578e-10
24436,194766,194766,389532,51.46214509010315,2.472559942439297e-10
24462,194974,194974,389948,51.557279109954834,2.4680272610039083e-10
24489,195190,195190,390380,51.62726187705994,2.464078164441183e-10
24515,195398,195398,390796,51.68726706504822,2.4608061948413327e-10
24542,195614,195614,391228,51.742311000823975,2.457816392280499e-10
24568,195822,195822,391644,51.79316210746765,2.455227221292621e-10
24595,196038,196038,392076,51.848499059677124,2.452761209437787e-10
24621,196246,196246,392492,51.91196322441101,2.450548226777264e-10
24648,196460,196460,392920,51.977618932724,2.3184524360877893e-10
24674,196668,196668,393336,52.03176712989807,2.3071528818318698e-10
24701,196884,196884,393768,52.08821511268616,2.3018514060955262e-10
24727,197092,197092,394184,52.145694971084595,2.297981789716863e-10
24754,197308,197308,394616,52.20365905761719,2.2947042395000194e-10
24780,197516,197516,395032,52.262699127197266,2.292018815455303e-10
24807,197732,197732,395464,52.3239848613739,2.2895626521423914e-10
24834,197948,197948,395896,52.38589596748352,2.287340467471147e-10
24860,198156,198156,396312,52.441981077194214,2.2853573522102568e-10
24887,198372,198372,396744,52.49801707267761,2.2834120983843012e-10
24913,198580,198580,397160,52.560901165008545,2.281620402062767e-10
24940,198788,198788,397576,52.62107706069946,1.8664037791155965e-10
24966,198994,198994,397988,52.67828416824341,1.6921718553620175e-10
24993,199210,199210,398420,52.746273040771484,1.6745932904801618e-10
25019,199418,199418,398836,52.80449104309082,1.6615345443744904e-10
25046,199634,199634,399268,52.861563205718994,1.6501616591359448e-10
25072,199842,199842,399684,52.917208194732666,1.6408808246868233e-10
25099,200058,200058,400116,52.97368025779724,1.6326450791424247e-10
25125,200266,200266,400532,53.02777695655823,1.6258164390160714e-10
25152,200482,200482,400964,53.08713698387146,1.6196647090713364e-10
25178,200690,200690,401380,53.13739490509033,1.614490443734176e-10
25205,200906,200906,401812,53.188210010528564,1.609760618625813e-10
25231,201114,201114,402228,53.23671007156372,1.6057249504759005e-10
25258,201330,201330,402660,53.28749704360962,1.60198429283347e-10
25285,201546,201546,403092,53.33724308013916,1.5986280665855122e-10
25311,201754,201754,403508,53.391940116882324,1.5957012248533634e-10
25338,201970,201970,403940,53.44289684295654,1.5929328771591507e-10
25364,202178,202178,404356,53.49325895309448,1.5904832705736028e-10
25391,202394,202394,404788,53.54532814025879,1.588132855664465e-10
25417,202602,202602,405204,53.594155073165894,1.5860284566900567e-10
25444,202818,202818,405636,53.64402413368225,1.5839806351008877e-10
25470,203026,203026,406052,53.692129135131836,1.5821261464190592e-10
25497,203242,203242,406484,53.74271583557129,1.5803028341640335e-10
25523,203450,203450,406900,53.79029202461243,1.578631701083756e-10
25550,203666,203666,407332,53.84007811546326,1.5769728480112235e-10
25576,203870,203870,407740,53.89224910736084,1.5245853057992653e-10
25603,204086,204086,408172,53.94326615333557,1.4092609366995786e-10
25629,204294,204294,408588,53.99314093589783,1.3979883411964305e-10
25656,204510,204510,409020,54.04377198219299,1.3902037013007854e-10
25683,204726,204726,409452,54.09384799003601,1.383980737874464e-10
25709,204934,204934,409868,54.14091897010803,1.378964560781229e-10
25736,205150,205150,410300,54.1910080909729,1.3745180089560851e-10
25762,205358,205358,410716,54.238534927368164,1.3708114222350224e-10
25789,205574,205574,411148,54.29546117782593,1.3674394292109498e-10
25815,205782,205782,411564,54.343636989593506,1.3645627157082882e-10
25842,205998,205998,411996,54.39477825164795,1.361889049236478e-10
25868,206206,206206,412412,54.44349122047424,1.3595599102728846e-10
25895,206422,206422,412844,54.49519896507263,1.3573536424741303e-10
25921,206628,206628,413256,54.542702198028564,1.31872879804505e-10
25948,206844,206844,413688,54.599608182907104,1.3111476100081764e-10
25974,207052,207052,414104,54.65060091018677,1.3084286963275665e-10
26001,207268,207268,414536,54.701329946517944,1.3063601127100293e-10
26027,207476,207476,414952,54.74926996231079,1.3047123891059795e-10
26054,207692,207692,415384,54.80565309524536,1.3032222727162313e-10
26080,207900,207900,415800,54.86499094963074,1.3019299785447032e-10
26107,208116,208116,416232,54.9215202331543,1.3006923690540625e-10
26134,208332,208332,416664,54.982614040374756,1.2995326136556266e-10
26160,208540,208540,417080,55.03372001647949,1.2984691878187716e-10
26187,208756,208756,417512,55.08434987068176,1.2974053495429668e-10
26213,208962,208962,417924,55.13338112831116,1.2352845442102827e-10
26240,209178,209178,418356,55.18900108337402,1.2302212162922477e-10
26266,209386,209386,418772,55.237189054489136,1.2282604295118663e-10
26293,209602,209602,419204,55.28784704208374,1.226691835073487e-10
26319,209810,209810,419620,55.33585524559021,1.2254077163732595e-10
26346,210026,210026,420052,55.387797117233276,1.2242140618741984e-10
26372,210234,210234,420468,55.43795418739319,1.2231523737579488e-10
26399,210450,210450,420900,55.49569606781006,1.2221100473591906e-10
26425,210658,210658,421316,55.546751976013184,1.221149796028102e-10
26452,210874,210874,421748,55.597557067871094,1.220184615135572e-10
26478,211082,211082,422164,55.64609408378601,1.2192764039242257e-10
26505,211288,211288,422576,55.69403910636902,9.941933474411593e-11


==> plot_data/bilinear_matrix_game_n250/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0003790855407714844,2.0175302852282635
19,40,40,80,0.026957035064697266,0.3228983898673162
38,80,80,160,0.050685882568359375,0.1498185508703752
57,130,130,260,0.0745401382446289,0.07567792005333666
77,188,188,376,0.0974888801574707,0.047935423211501516
96,244,244,488,0.1203761100769043,0.03468826647884769
115,306,306,612,0.14422607421875,0.021315318614970064
134,362,362,724,0.16945195198059082,0.012393377357513611
153,422,422,844,0.1971898078918457,0.00904687651286605
172,488,488,976,0.22531986236572266,0.00790227561050279
191,552,552,1104,0.25109410285949707,0.006616396449975184
211,622,622,1244,0.28113317489624023,0.005758668913051867
230,696,696,1392,0.30570507049560547,0.0052543449605302476
249,770,770,1540,0.3308119773864746,0.004877799310625684
268,844,844,1688,0.356564998626709,0.004563773813828424
287,920,920,1840,0.381619930267334,0.004350350316512475
306,994,994,1988,0.40740299224853516,0.003920567854838844
325,1056,1056,2112,0.43190813064575195,0.0032199106975918123
344,1124,1124,2248,0.4560708999633789,0.00277529093157287
364,1188,1188,2376,0.4808781147003174,0.002247813917176663
383,1250,1250,2500,0.5061471462249756,0.0018446853257633592
402,1310,1310,2620,0.5354061126708984,0.0015033045682312609
421,1378,1378,2756,0.5662579536437988,0.0013371149219795504
440,1454,1454,2908,0.596473217010498,0.001275307295872697
459,1530,1530,3060,0.6321010589599609,0.0012343664472471046
478,1606,1606,3212,0.6614789962768555,0.0011965732408387435
498,1686,1686,3372,0.6949372291564941,0.0011281633539907418
517,1762,1762,3524,0.7263100147247314,0.001085102855492376
536,1838,1838,3676,0.7521259784698486,0.0010496653714075828
555,1906,1906,3812,0.7785861492156982,0.0009437854330096502
574,1974,1974,3948,0.8033668994903564,0.0008243170722245169
593,2050,2050,4100,0.8307540416717529,0.0007869330262073819
612,2124,2124,4248,0.8547570705413818,0.0007277305486597394
632,2204,2204,4408,0.8813331127166748,0.0006980571443961036
651,2280,2280,4560,0.9120020866394043,0.0006758961171027778
670,2356,2356,4712,0.9408042430877686,0.0006319804069390513
689,2424,2424,4848,0.9664700031280518,0.0005719965397465796
708,2498,2498,4996,0.9931230545043945,0.0005221820932372291
727,2574,2574,5148,1.0192110538482666,0.0004944556593075173
746,2650,2650,5300,1.0456230640411377,0.00047183985509187984
766,2730,2730,5460,1.0771620273590088,0.00044586596650082966
785,2806,2806,5612,1.1154282093048096,0.0004266742517845743
804,2882,2882,5764,1.1542441844940186,0.0004158061867951996
823,2958,2958,5916,1.1803710460662842,0.00040502523948225065
842,3034,3034,6068,1.2049989700317383,0.0003902062946982429
861,3110,3110,6220,1.229449987411499,0.0003798301666891546
880,3186,3186,6372,1.2550389766693115,0.00037213346826118614
899,3262,3262,6524,1.2804019451141357,0.0003616023883668246
919,3342,3342,6684,1.3086190223693848,0.00034995879904334656
938,3418,3418,6836,1.3338391780853271,0.00034359202544205367
957,3494,3494,6988,1.3584380149841309,0.0003362633431563166
976,3570,3570,7140,1.38466215133667,0.00032460583203786943
995,3646,3646,7292,1.4108669757843018,0.0003175934433178128
1014,3722,3722,7444,1.4354429244995117,0.0003132409457599409
1033,3798,3798,7596,1.4623780250549316,0.0003058335334654909
1053,3878,3878,7756,1.488158941268921,0.00029763316389054003
1072,3954,3954,7908,1.5122339725494385,0.0002929620516876683
1091,4030,4030,8060,1.5373451709747314,0.00028820108926604754
1110,4106,4106,8212,1.5630221366882324,0.0002824243588623943
1129,4182,4182,8364,1.5890181064605713,0.0002748999519585629
1148,4258,4258,8516,1.6145339012145996,0.00026629110443704684
1167,4334,4334,8668,1.639772891998291,0.0002577173337108483
1187,4414,4414,8828,1.6664190292358398,0.00025064183733689623
1206,4490,4490,8980,1.6908988952636719,0.0002442832836223381
1225,4566,4566,9132,1.7172322273254395,0.00024075221396476922
1244,4642,4642,9284,1.7433719635009766,0.0002382113555391448
1263,4718,4718,9436,1.7682318687438965,0.0002340770507126394
1282,4794,4794,9588,1.7925629615783691,0.0002299217961040375
1301,4870,4870,9740,1.817093849182129,0.00022694855707144438
1321,4950,4950,9900,1.8433499336242676,0.0002229478616984248
1340,5026,5026,10052,1.8678889274597168,0.00021624442529538077
1359,5102,5102,10204,1.894714117050171,0.00021017667813369816
1378,5178,5178,10356,1.9212191104888916,0.00020712358713058005
1397,5254,5254,10508,1.9479460716247559,0.0002039336518822789
1416,5330,5330,10660,1.9723079204559326,0.00020003928831681554
1435,5406,5406,10812,1.9978089332580566,0.0001968146653664996
1454,5482,5482,10964,2.0233700275421143,0.00019450209352442693
1474,5562,5562,11124,2.0520241260528564,0.0001915093835953259
1493,5638,5638,11276,2.0796642303466797,0.0001886627954276121
1512,5714,5714,11428,2.1064939498901367,0.0001867693905431896
1531,5790,5790,11580,2.131575107574463,0.00018435148693195903
1550,5866,5866,11732,2.156757116317749,0.00018102213408817945
1569,5942,5942,11884,2.1828019618988037,0.0001791548917834186
1588,6018,6018,12036,2.207545042037964,0.0001771828615709225
1608,6098,6098,12196,2.2339892387390137,0.00017382644742640097
1627,6174,6174,12348,2.2588090896606445,0.00017049842908553126
1646,6250,6250,12500,2.284738063812256,0.00016840930460057052
1665,6326,6326,12652,2.3118221759796143,0.0001660527419139597
1684,6402,6402,12804,2.3400540351867676,0.0001645412092055474
1703,6478,6478,12956,2.3681750297546387,0.00015896536239880964
1722,6554,6554,13108,2.3966519832611084,0.00015605039238803057
1742,6634,6634,13268,2.4287731647491455,0.0001513606131050411
1761,6710,6710,13420,2.4548869132995605,0.00014834515177159025
1780,6786,6786,13572,2.4814419746398926,0.000146467621824141
1799,6862,6862,13724,2.5074081420898438,0.00014509283641646513
1818,6938,6938,13876,2.5346081256866455,0.00014351646571388347
1837,7014,7014,14028,2.5647361278533936,0.000142128756557581
1856,7090,7090,14180,2.5928120613098145,0.00014071508702683344
1876,7170,7170,14340,2.620434045791626,0.00013911691550149983
1895,7246,7246,14492,2.646843910217285,0.00013793153627629149
1914,7322,7322,14644,2.6730899810791016,0.00013662023472092545
1933,7398,7398,14796,2.6989340782165527,0.00013496877550316365
1952,7474,7474,14948,2.7248129844665527,0.0001335604483672822
1971,7550,7550,15100,2.752716064453125,0.00013273541653023525
1990,7626,7626,15252,2.7784690856933594,0.00013132430460411642
2010,7706,7706,15412,2.805528163909912,0.000129257945327756
2029,7782,7782,15564,2.831674098968506,0.00012814285438100532
2048,7858,7858,15716,2.859205961227417,0.0001271577424605461
2067,7934,7934,15868,2.890321969985962,0.00012604024060895497
2086,8010,8010,16020,2.9204559326171875,0.0001243859699381058
2105,8086,8086,16172,2.9502971172332764,0.00012330640981205346
2124,8162,8162,16324,2.979663133621216,0.00012233795103569554
2143,8238,8238,16476,3.008358955383301,0.00012106127321824741
2163,8318,8318,16636,3.03757381439209,0.00012010498381069365
2182,8394,8394,16788,3.0647380352020264,0.0001192938040322467
2201,8470,8470,16940,3.092024087905884,0.00011831396432527017
2220,8546,8546,17092,3.118865966796875,0.00011586356343898263
2239,8622,8622,17244,3.149451971054077,0.00011351976544594829
2258,8698,8698,17396,3.1854000091552734,0.00011255385794139954
2277,8774,8774,17548,3.225482940673828,0.00011184627726385472
2297,8854,8854,17708,3.3193259239196777,0.00011086266829920093
2316,8930,8930,17860,3.347707986831665,0.00010963648056806331
2335,9006,9006,18012,3.3766069412231445,0.00010868888633007279
2354,9082,9082,18164,3.4061460494995117,0.00010715105335647734
2373,9158,9158,18316,3.439253091812134,0.00010561337277398657
2392,9234,9234,18468,3.468890905380249,0.00010403891235306137
2411,9310,9310,18620,3.498802900314331,0.00010261846495541443
2431,9390,9390,18780,3.5289950370788574,0.00010020972137794654
2450,9466,9466,18932,3.5609710216522217,9.786547645216975e-05
2469,9542,9542,19084,3.589478015899658,9.638504899789277e-05
2488,9618,9618,19236,3.616136074066162,9.56012120210361e-05
2507,9694,9694,19388,3.642595052719116,9.481236407775397e-05
2526,9770,9770,19540,3.669398069381714,9.383340913667569e-05
2545,9846,9846,19692,3.6958820819854736,9.296829058552138e-05
2565,9926,9926,19852,3.72444486618042,9.212571885911171e-05
2584,10002,10002,20004,3.752812147140503,9.128349320076944e-05
2603,10078,10078,20156,3.7814579010009766,9.055274668584026e-05
2622,10154,10154,20308,3.810621976852417,8.980703370628129e-05
2641,10230,10230,20460,3.842036008834839,8.891076954627032e-05
2660,10306,10306,20612,3.8751020431518555,8.811408259271204e-05
2679,10382,10382,20764,3.9101200103759766,8.755511650838224e-05
2698,10458,10458,20916,3.946599006652832,8.690116982072477e-05
2718,10538,10538,21076,3.987758159637451,8.582519026426493e-05
2737,10614,10614,21228,4.036738157272339,8.503863403446941e-05
2756,10690,10690,21380,4.0894951820373535,8.457992914014676e-05
2775,10766,10766,21532,4.145998001098633,8.356271687918801e-05
2794,10842,10842,21684,4.1949639320373535,8.135291665542812e-05
2813,10918,10918,21836,4.229257106781006,8.005579998767833e-05
2832,10994,10994,21988,4.268249034881592,7.952411845655962e-05
2852,11074,11074,22148,4.306529998779297,7.79474844626115e-05
2871,11150,11150,22300,4.341532945632935,7.643533687821026e-05
2890,11226,11226,22452,4.381439924240112,7.553307757988387e-05
2909,11302,11302,22604,4.425256967544556,7.488076913396961e-05
2928,11378,11378,22756,4.469105958938599,7.421578130876301e-05
2947,11454,11454,22908,4.5150909423828125,7.355911107631924e-05
2966,11530,11530,23060,4.558912992477417,7.288728433894157e-05
2986,11610,11610,23220,4.603184223175049,7.22609762145224e-05
3005,11686,11686,23372,4.645240068435669,7.161870269669543e-05
3024,11762,11762,23524,4.698071002960205,7.106684155981786e-05
3043,11838,11838,23676,4.7502851486206055,7.033588252684922e-05
3062,11914,11914,23828,4.791490077972412,6.937888236506033e-05
3081,11990,11990,23980,4.82598614692688,6.893494493967078e-05
3100,12066,12066,24132,4.856105089187622,6.804722355891129e-05
3120,12146,12146,24292,4.88659405708313,6.578440682041257e-05
3139,12222,12222,24444,4.916157960891724,6.307723235721876e-05
3158,12296,12296,24592,4.945683002471924,6.021205552201465e-05
3177,12372,12372,24744,4.9755470752716064,5.795120851422954e-05
3196,12448,12448,24896,5.0049920082092285,5.732128475736447e-05
3215,12524,12524,25048,5.034170150756836,5.590741606836574e-05
3234,12600,12600,25200,5.063931941986084,5.400223795973229e-05
3253,12676,12676,25352,5.093800067901611,5.165025904912568e-05
3273,12756,12756,25512,5.123060941696167,4.9570595262097536e-05
3292,12832,12832,25664,5.153572082519531,4.8194689693770004e-05
3311,12908,12908,25816,5.182197093963623,4.741321118979061e-05
3330,12984,12984,25968,5.2109949588775635,4.692610422824808e-05
3349,13060,13060,26120,5.242654085159302,4.644564256145297e-05
3368,13136,13136,26272,5.271162033081055,4.606318914889834e-05
3387,13212,13212,26424,5.299745082855225,4.5742581835810526e-05
3407,13292,13292,26584,5.3291709423065186,4.527591880127348e-05
3426,13368,13368,26736,5.361296892166138,4.488139912671564e-05
3445,13444,13444,26888,5.393439054489136,4.457390962479894e-05
3464,13520,13520,27040,5.424391984939575,4.423927000811646e-05
3483,13596,13596,27192,5.4509499073028564,4.375773407595282e-05
3502,13672,13672,27344,5.47686505317688,4.330183136405989e-05
3521,13748,13748,27496,5.503280878067017,4.302709776070579e-05
3541,13828,13828,27656,5.531553030014038,4.268599074368539e-05
3560,13904,13904,27808,5.558804035186768,4.229938237535625e-05
3579,13980,13980,27960,5.586022853851318,4.2006623713820904e-05
3598,14056,14056,28112,5.617470979690552,4.176970224883301e-05
3617,14132,14132,28264,5.651376247406006,4.141619672053851e-05
3636,14208,14208,28416,5.680170059204102,4.1084677141792353e-05
3655,14284,14284,28568,5.709174156188965,4.081822563690908e-05
3675,14364,14364,28728,5.751659154891968,4.047901297456077e-05
3694,14440,14440,28880,5.799084186553955,4.019118274025782e-05
3713,14516,14516,29032,5.841543912887573,3.9684358005713136e-05
3732,14592,14592,29184,5.879024982452393,3.879144950608753e-05
3751,14668,14668,29336,5.916637897491455,3.808316819036218e-05
3770,14744,14744,29488,5.955078840255737,3.757838963198868e-05
3789,14820,14820,29640,5.993396043777466,3.7022674368797836e-05
3808,14896,14896,29792,6.026766061782837,3.658984833942952e-05
3828,14976,14976,29952,6.06911301612854,3.627441390342288e-05
3847,15052,15052,30104,6.097218036651611,3.5952312007025993e-05
3866,15128,15128,30256,6.127371072769165,3.560526780103887e-05
3885,15204,15204,30408,6.1633570194244385,3.528676011310906e-05
3904,15280,15280,30560,6.194199085235596,3.499545593781946e-05
3923,15356,15356,30712,6.220769166946411,3.462461205094376e-05
3942,15432,15432,30864,6.248703956604004,3.4327965018842924e-05
3962,15512,15512,31024,6.278416872024536,3.4057005602285226e-05
3981,15588,15588,31176,6.306085824966431,3.3674403375194456e-05
4000,15664,15664,31328,6.334196090698242,3.319528994498697e-05
4019,15740,15740,31480,6.3617260456085205,3.292224144872073e-05
4038,15816,15816,31632,6.389644145965576,3.191643996136267e-05
4057,15892,15892,31784,6.417590141296387,3.0491031214857217e-05
4076,15968,15968,31936,6.484866142272949,2.9268930051656906e-05
4096,16048,16048,32096,6.519949197769165,2.882013242207161e-05
4115,16124,16124,32248,6.546706914901733,2.8581032195988534e-05
4134,16200,16200,32400,6.574974060058594,2.8268107550317493e-05
4153,16276,16276,32552,6.6014180183410645,2.7978660640506512e-05
4172,16352,16352,32704,6.62758207321167,2.7689649212646687e-05
4191,16428,16428,32856,6.653665065765381,2.7396542755456227e-05
4210,16504,16504,33008,6.682292938232422,2.712474391712649e-05
4230,16584,16584,33168,6.710263013839722,2.6877003112486187e-05
4249,16660,16660,33320,6.736721992492676,2.6636678750493646e-05
4268,16736,16736,33472,6.766211032867432,2.6365956948824394e-05
4287,16812,16812,33624,6.812191963195801,2.6166705001180993e-05
4306,16888,16888,33776,6.852997064590454,2.5919221553792704e-05
4325,16964,16964,33928,6.887853145599365,2.5541522428796416e-05
4344,17040,17040,34080,6.918400049209595,2.5379146186538e-05
4363,17116,17116,34232,6.947848081588745,2.4794957761500124e-05
4383,17196,17196,34392,6.978410959243774,2.3718837800267234e-05
4402,17270,17270,34540,7.006395101547241,2.2032440966393797e-05
4421,17332,17332,34664,7.0346879959106445,1.8882627820101763e-05
4440,17396,17396,34792,7.067112922668457,1.5774138095846622e-05
4459,17466,17466,34932,7.096421957015991,1.4623852273810803e-05
4478,17542,17542,35084,7.1235949993133545,1.4443365509139972e-05
4497,17618,17618,35236,7.150317192077637,1.4217279523931072e-05
4517,17698,17698,35396,7.178293943405151,1.39558276029802e-05
4536,17774,17774,35548,7.205086946487427,1.3787816119299687e-05
4555,17850,17850,35700,7.231328010559082,1.3635817303894182e-05
4574,17926,17926,35852,7.257399082183838,1.3418305818083003e-05
4593,18002,18002,36004,7.283522129058838,1.2933618636456774e-05
4612,18078,18078,36156,7.312929153442383,1.2678758115919515e-05
4631,18154,18154,36308,7.340739011764526,1.2487083240216316e-05
4651,18234,18234,36468,7.368335247039795,1.2371561556111374e-05
4670,18310,18310,36620,7.394979000091553,1.2172122804113603e-05
4689,18386,18386,36772,7.421003103256226,1.1795182363995153e-05
4708,18462,18462,36924,7.450648069381714,1.1585080779926392e-05
4727,18538,18538,37076,7.478063106536865,1.1428128858104445e-05
4746,18614,18614,37228,7.506853103637695,1.1205827103580563e-05
4765,18690,18690,37380,7.535181045532227,1.1030039059068808e-05
4785,18770,18770,37540,7.566465139389038,1.0867004863850638e-05
4804,18846,18846,37692,7.593012094497681,1.0711690929714693e-05
4823,18922,18922,37844,7.61938214302063,1.0524350147417501e-05
4842,18998,18998,37996,7.646093130111694,1.0233908031212052e-05
4861,19074,19074,38148,7.671919107437134,1.0029140664952466e-05
4880,19150,19150,38300,7.697947978973389,9.955455756736647e-06
4899,19226,19226,38452,7.72607421875,9.87731326430738e-06
4919,19306,19306,38612,7.755829095840454,9.767042139018196e-06
4938,19382,19382,38764,7.785372972488403,9.6691718152243e-06
4957,19458,19458,38916,7.814738035202026,9.562124346426962e-06
4976,19534,19534,39068,7.8462138175964355,9.480276981256454e-06
4995,19610,19610,39220,7.878848075866699,9.413521195767384e-06
5014,19686,19686,39372,7.911349058151245,9.317608318871124e-06
5033,19762,19762,39524,7.943127155303955,9.199527535808796e-06
5052,19838,19838,39676,7.972332000732422,9.131233783016483e-06
5072,19918,19918,39836,8.005044937133789,9.057482673364713e-06
5091,19994,19994,39988,8.036698818206787,8.911471537343377e-06
5110,20070,20070,40140,8.068739175796509,8.783893046852182e-06
5129,20146,20146,40292,8.097573041915894,8.732868946907649e-06
5148,20222,20222,40444,8.12598991394043,8.651224804525217e-06
5167,20298,20298,40596,8.15427303314209,8.534454089388488e-06
5186,20374,20374,40748,8.182738065719604,8.419684360601436e-06
5206,20454,20454,40908,8.216098070144653,8.35201198511418e-06
5225,20530,20530,41060,8.246889114379883,8.248815870551312e-06
5244,20606,20606,41212,8.27763295173645,8.138664822136965e-06
5263,20682,20682,41364,8.307248830795288,8.076509540604217e-06
5282,20758,20758,41516,8.337262153625488,8.001420659445664e-06
5301,20834,20834,41668,8.366353988647461,7.931461754421474e-06
5320,20910,20910,41820,8.395130157470703,7.850103710170154e-06
5340,20990,20990,41980,8.426184892654419,7.795291669885273e-06
5359,21066,21066,42132,8.455661058425903,7.734642487373119e-06
5378,21142,21142,42284,8.48528504371643,7.638071438165847e-06
5397,21218,21218,42436,8.51448917388916,7.583591776029057e-06
5416,21294,21294,42588,8.544440031051636,7.533178204119876e-06
5435,21370,21370,42740,8.573814153671265,7.490145543716813e-06
5454,21446,21446,42892,8.602313995361328,7.397027384516808e-06
5474,21526,21526,43052,8.631715059280396,7.246735189879488e-06
5493,21602,21602,43204,8.658172845840454,7.185079328607147e-06
5512,21678,21678,43356,8.684613227844238,7.109307967846526e-06
5531,21754,21754,43508,8.710710048675537,6.956408714921932e-06
5550,21830,21830,43660,8.737122058868408,6.7021809875714556e-06
5569,21906,21906,43812,8.763216257095337,6.317604564395027e-06
5588,21982,21982,43964,8.791587114334106,5.959115454395556e-06
5607,22058,22058,44116,8.818197011947632,5.693638047240866e-06
5627,22138,22138,44276,8.8454110622406,5.576854392857891e-06
5646,22214,22214,44428,8.871029138565063,5.5225787205363135e-06
5665,22290,22290,44580,8.89635705947876,5.481763998446739e-06
5684,22366,22366,44732,8.921659231185913,5.444859340701007e-06
5703,22442,22442,44884,8.94754409790039,5.402164237758666e-06
5722,22518,22518,45036,8.97198486328125,5.351635124742235e-06
5741,22594,22594,45188,8.997323989868164,5.301801599208546e-06
5761,22674,22674,45348,9.023997068405151,5.263026681270247e-06
5780,22750,22750,45500,9.05042314529419,5.221597769256241e-06
5799,22826,22826,45652,9.076350927352905,5.167609611285496e-06
5818,22902,22902,45804,9.101033926010132,5.132317022212822e-06
5837,22978,22978,45956,9.125395059585571,5.096642730999931e-06
5856,23054,23054,46108,9.150218963623047,5.037207850083691e-06
5875,23130,23130,46260,9.174800872802734,4.977997987051101e-06
5895,23210,23210,46420,9.20045018196106,4.9417707696311285e-06
5914,23286,23286,46572,9.224855184555054,4.905580382367852e-06
5933,23362,23362,46724,9.249639987945557,4.840735199854986e-06
5952,23438,23438,46876,9.274018049240112,4.7866609678381914e-06
5971,23514,23514,47028,9.298496007919312,4.755882592923055e-06
5990,23590,23590,47180,9.322615146636963,4.723709543582555e-06
6009,23666,23666,47332,9.347473859786987,4.67261982746689e-06
6029,23746,23746,47492,9.373452186584473,4.589726027762183e-06
6048,23822,23822,47644,9.397841930389404,4.543996124419403e-06
6067,23898,23898,47796,9.422840118408203,4.498670936917222e-06
6086,23974,23974,47948,9.448178052902222,4.439266949294305e-06
6105,24050,24050,48100,9.472994089126587,4.355922186869912e-06
6124,24126,24126,48252,9.49767804145813,4.283160033115196e-06
6143,24202,24202,48404,9.522348165512085,4.254599731543941e-06
6162,24278,24278,48556,9.550740003585815,4.221380838975599e-06
6182,24358,24358,48716,9.581774234771729,4.187034811156217e-06
6201,24434,24434,48868,9.61033296585083,4.011753799927059e-06
6220,24510,24510,49020,9.636044025421143,3.8055816356736127e-06
6239,24586,24586,49172,9.660312175750732,3.6771641326223698e-06
6258,24662,24662,49324,9.684700965881348,3.603485630677282e-06
6277,24738,24738,49476,9.70939016342163,3.526942985030453e-06
6296,24814,24814,49628,9.733482122421265,3.483765775429887e-06
6316,24894,24894,49788,9.758648157119751,3.453918498708187e-06
6335,24970,24970,49940,9.782518148422241,3.4118112868932765e-06
6354,25046,25046,50092,9.806745052337646,3.3842179509393666e-06
6373,25122,25122,50244,9.831516027450562,3.3599560762845403e-06
6392,25198,25198,50396,9.856032133102417,3.3319203279805948e-06
6411,25274,25274,50548,9.880819082260132,3.304103833517798e-06
6430,25350,25350,50700,9.904863119125366,3.241404276123197e-06
6450,25430,25430,50860,9.930340051651001,3.1517705515953465e-06
6469,25506,25506,51012,9.954345941543579,3.1268214608582474e-06
6488,25582,25582,51164,9.978240013122559,3.0919917200668193e-06
6507,25658,25658,51316,10.002202987670898,3.035157515303282e-06
6526,25734,25734,51468,10.026133060455322,2.9236935085843403e-06
6545,25810,25810,51620,10.051343202590942,2.8315219154830204e-06
6564,25886,25886,51772,10.08141803741455,2.7885504081731686e-06
6584,25966,25966,51932,10.107025861740112,2.7594825026002794e-06
6603,26042,26042,52084,10.1318359375,2.7342947650547863e-06
6622,26118,26118,52236,10.156451225280762,2.707066941993117e-06
6641,26194,26194,52388,10.181274175643921,2.665822075985095e-06
6660,26270,26270,52540,10.205770015716553,2.6407470912791272e-06
6679,26346,26346,52692,10.23079800605774,2.6220070212616786e-06
6698,26422,26422,52844,10.255729913711548,2.593138226963386e-06
6717,26498,26498,52996,10.280765056610107,2.569152620315324e-06
6737,26578,26578,53156,10.30739712715149,2.5500116604193708e-06
6756,26654,26654,53308,10.333456993103027,2.5276724732056612e-06
6775,26730,26730,53460,10.358617067337036,2.508272315734266e-06
6794,26806,26806,53612,10.383882999420166,2.4895636525010773e-06
6813,26882,26882,53764,10.408481121063232,2.470578191057554e-06
6832,26958,26958,53916,10.432662010192871,2.4520064853922513e-06
6851,27034,27034,54068,10.457028150558472,2.433916969986658e-06
6871,27114,27114,54228,10.483246088027954,2.4134602006838295e-06
6890,27190,27190,54380,10.50813913345337,2.362317917931276e-06
6909,27266,27266,54532,10.53307294845581,2.2949093412734173e-06
6928,27342,27342,54684,10.560023069381714,2.207313618484793e-06
6947,27418,27418,54836,10.585673093795776,2.1692325092001153e-06
6966,27494,27494,54988,10.610832929611206,2.1560010234056612e-06
6985,27570,27570,55140,10.636698246002197,2.1343048462727146e-06
7005,27650,27650,55300,10.662121057510376,2.1117182901250213e-06
7024,27726,27726,55452,10.687103033065796,2.077438273309809e-06
7043,27802,27802,55604,10.711971044540405,2.0158281541566885e-06
7062,27878,27878,55756,10.736912250518799,1.999632441443173e-06
7081,27954,27954,55908,10.76433515548706,1.981933422381867e-06
7100,28030,28030,56060,10.789093971252441,1.95445923682678e-06
7119,28106,28106,56212,10.813328981399536,1.935950674172215e-06
7139,28186,28186,56372,10.839141130447388,1.8935752595571038e-06
7158,28262,28262,56524,10.864253997802734,1.831519343380959e-06
7177,28338,28338,56676,10.88936710357666,1.7450026183774698e-06
7196,28414,28414,56828,10.913105964660645,1.6110154119972297e-06
7215,28490,28490,56980,10.937128067016602,1.5585673289733337e-06
7234,28566,28566,57132,10.960785865783691,1.5290605926164126e-06
7253,28642,28642,57284,10.985352993011475,1.5117507251575947e-06
7272,28718,28718,57436,11.009511947631836,1.500249720445125e-06
7292,28798,28798,57596,11.034367084503174,1.4779482119705333e-06
7311,28874,28874,57748,11.058810234069824,1.440333671925266e-06
7330,28950,28950,57900,11.083434104919434,1.4175347855775186e-06
7349,29026,29026,58052,11.10721206665039,1.4080680947557514e-06
7368,29102,29102,58204,11.131974935531616,1.3931998426297632e-06
7387,29178,29178,58356,11.155387163162231,1.3790529066834568e-06
7406,29254,29254,58508,11.179323196411133,1.368205270582583e-06
7426,29334,29334,58668,11.208964109420776,1.3552788545740731e-06
7445,29410,29410,58820,11.235111951828003,1.3423661905752576e-06
7464,29486,29486,58972,11.265936851501465,1.3333464719288878e-06
7483,29562,29562,59124,11.296030044555664,1.3157528319071315e-06
7502,29638,29638,59276,11.322327136993408,1.2897957035246862e-06
7521,29714,29714,59428,11.34875226020813,1.2740536580779728e-06
7540,29790,29790,59580,11.375422954559326,1.2530287573315032e-06
7560,29870,29870,59740,11.402992963790894,1.2050424514845937e-06
7579,29946,29946,59892,11.429331064224243,1.1778794734178375e-06
7598,30022,30022,60044,11.456024169921875,1.1676046174544041e-06
7617,30098,30098,60196,11.48409390449524,1.151347567282193e-06
7636,30174,30174,60348,11.509093046188354,1.1123234275409094e-06
7655,30250,30250,60500,11.534292936325073,1.0841338456171113e-06
7674,30326,30326,60652,11.560685157775879,1.0751897112760152e-06
7694,30406,30406,60812,11.588526010513306,1.0556826316110598e-06
7713,30482,30482,60964,11.615571975708008,1.0352007908785669e-06
7732,30558,30558,61116,11.645836114883423,1.0244207170074395e-06
7751,30634,30634,61268,11.674925088882446,1.0136184370027393e-06
7770,30710,30710,61420,11.70596718788147,9.973701546178073e-07
7789,30786,30786,61572,11.734520196914673,9.813954344970281e-07
7808,30862,30862,61724,11.760701894760132,9.726207871547228e-07
7827,30938,30938,61876,11.786956071853638,9.600410227689745e-07
7847,31018,31018,62036,11.81591510772705,9.434895835779149e-07
7866,31094,31094,62188,11.842435121536255,9.355706998631097e-07
7885,31170,31170,62340,11.86868405342102,9.274837619349303e-07
7904,31246,31246,62492,11.893836975097656,9.122220229543149e-07
7923,31322,31322,62644,11.91868281364441,8.940976588099979e-07
7942,31398,31398,62796,11.9441499710083,8.811070195231093e-07
7961,31474,31474,62948,11.9689199924469,8.718049136884984e-07
7981,31554,31554,63108,11.99581503868103,8.56215153610875e-07
8000,31630,31630,63260,12.022788047790527,8.260926986246417e-07
8019,31706,31706,63412,12.054189205169678,7.989490343047128e-07
8038,31782,31782,63564,12.082665920257568,7.862950556563411e-07
8057,31858,31858,63716,12.108533143997192,7.802668614680248e-07
8076,31934,31934,63868,12.133764028549194,7.710721036334104e-07
8095,32010,32010,64020,12.158136129379272,7.59329831878912e-07
8115,32090,32090,64180,12.182712078094482,7.524358267928398e-07
8134,32166,32166,64332,12.207520961761475,7.43355612549941e-07
8153,32242,32242,64484,12.232397079467773,7.212732013206015e-07
8172,32318,32318,64636,12.257026195526123,7.03799256084607e-07
8191,32394,32394,64788,12.281772136688232,6.939583780735346e-07
8210,32470,32470,64940,12.306210041046143,6.825770338642899e-07
8229,32546,32546,65092,12.33043098449707,6.602711568446025e-07
8249,32626,32626,65252,12.358731985092163,6.209605318886539e-07
8268,32702,32702,65404,12.385037183761597,6.080455307022952e-07
8287,32778,32778,65556,12.410980224609375,6.027204149838272e-07
8306,32854,32854,65708,12.436062097549438,5.97625470141118e-07
8325,32930,32930,65860,12.461453199386597,5.913449063784614e-07
8344,33006,33006,66012,12.485249996185303,5.847655762485115e-07
8363,33082,33082,66164,12.509046077728271,5.793653526715182e-07
8383,33162,33162,66324,12.534357070922852,5.741525244382481e-07
8402,33238,33238,66476,12.561439990997314,5.69965893918156e-07
8421,33314,33314,66628,12.611098051071167,5.651154677480464e-07
8440,33390,33390,66780,12.766846895217896,5.598689013297229e-07
8459,33466,33466,66932,12.809402227401733,5.559138992655764e-07
8478,33542,33542,67084,12.846740007400513,5.516813107003708e-07
8497,33618,33618,67236,12.879951238632202,5.453449050040802e-07
8516,33694,33694,67388,12.923732995986938,5.411422034416186e-07
8536,33774,33774,67548,12.962069988250732,5.376564890975951e-07
8555,33850,33850,67700,12.997495174407959,5.302425697114291e-07
8574,33926,33926,67852,13.026316165924072,5.174899715505873e-07
8593,34002,34002,68004,13.054663896560669,5.099102581790435e-07
8612,34078,34078,68156,13.084453105926514,5.06574691094215e-07
8631,34154,34154,68308,13.11216115951538,5.018648040399332e-07
8650,34230,34230,68460,13.13844108581543,4.974503536995299e-07
8670,34310,34310,68620,13.167108058929443,4.935036004837861e-07
8689,34386,34386,68772,13.195137023925781,4.881754228071711e-07
8708,34462,34462,68924,13.222979068756104,4.7451310661866373e-07
8727,34538,34538,69076,13.25071096420288,4.6783534847266625e-07
8746,34614,34614,69228,13.276937007904053,4.6287318352817366e-07
8765,34690,34690,69380,13.300904989242554,4.55750170739361e-07
8784,34766,34766,69532,13.326061010360718,4.5302208268773146e-07
8804,34846,34846,69692,13.352832078933716,4.4711290781700213e-07
8823,34922,34922,69844,13.37833023071289,4.3429766642223075e-07
8842,34998,34998,69996,13.403923988342285,4.1611046082325325e-07
8861,35074,35074,70148,13.431636095046997,3.9741735258566415e-07
8880,35150,35150,70300,13.458368062973022,3.9194543150725093e-07
8899,35226,35226,70452,13.48373818397522,3.889991449630418e-07
8918,35302,35302,70604,13.509011030197144,3.785311884956437e-07
8938,35382,35382,70764,13.535524129867554,3.6378378745650414e-07
8957,35458,35458,70916,13.568986177444458,3.5123649034412205e-07
8976,35534,35534,71068,13.605443000793457,3.447947189620574e-07
8995,35610,35610,71220,13.692230939865112,3.4061186525849e-07
9014,35686,35686,71372,13.72465205192566,3.375161045442387e-07
9033,35762,35762,71524,13.752233028411865,3.346435269070403e-07
9052,35838,35838,71676,13.778929948806763,3.3175799537398096e-07
9071,35914,35914,71828,13.805958986282349,3.292196894357558e-07
9091,35994,35994,71988,13.831500053405762,3.265503667055457e-07
9110,36070,36070,72140,13.85689401626587,3.2389345647333023e-07
9129,36146,36146,72292,13.884162187576294,3.205981632226604e-07
9148,36222,36222,72444,13.912928104400635,3.179494506344113e-07
9167,36298,36298,72596,13.941829204559326,3.1573575429152433e-07
9186,36374,36374,72748,13.968487024307251,3.1213442619960426e-07
9205,36450,36450,72900,13.994053840637207,3.093915023410332e-07
9225,36530,36530,73060,14.022724151611328,3.0740607341750224e-07
9244,36606,36606,73212,14.050166130065918,3.0483754452877795e-07
9263,36682,36682,73364,14.077791929244995,3.0237868666657844e-07
9282,36758,36758,73516,14.102512836456299,3.00303660443521e-07
9301,36834,36834,73668,14.130005121231079,2.981581620705105e-07
9320,36910,36910,73820,14.15619707107544,2.9548313926399296e-07
9339,36986,36986,73972,14.181957960128784,2.929178950361286e-07
9359,37066,37066,74132,14.209655046463013,2.9067845831274635e-07
9378,37142,37142,74284,14.235656023025513,2.88347557575493e-07
9397,37218,37218,74436,14.262666940689087,2.8607971378914433e-07
9416,37294,37294,74588,14.291990041732788,2.8396924080150304e-07
9435,37370,37370,74740,14.319348096847534,2.821087068396243e-07
9454,37446,37446,74892,14.349593162536621,2.7985492532826463e-07
9473,37522,37522,75044,14.378445148468018,2.779958466811596e-07
9493,37602,37602,75204,14.40720510482788,2.755694139110002e-07
9512,37678,37678,75356,14.432760000228882,2.7243764552870145e-07
9531,37754,37754,75508,14.459985971450806,2.705532798123168e-07
9550,37830,37830,75660,14.48703408241272,2.683375913377821e-07
9569,37906,37906,75812,14.514256954193115,2.652100968778569e-07
9588,37982,37982,75964,14.54234504699707,2.6093421602270614e-07
9607,38058,38058,76116,14.575109243392944,2.568822990932386e-07
9626,38134,38134,76268,14.60202693939209,2.5430118976032596e-07
9646,38214,38214,76428,14.631672143936157,2.499206723462347e-07
9665,38290,38290,76580,14.662761926651001,2.477328396629314e-07
9684,38366,38366,76732,14.690956115722656,2.447502672990802e-07
9703,38442,38442,76884,14.716705083847046,2.4057305458779137e-07
9722,38518,38518,77036,14.743281841278076,2.3643615699498853e-07
9741,38594,38594,77188,14.768900156021118,2.3381307774859543e-07
9760,38670,38670,77340,14.796441078186035,2.32033568111576e-07
9780,38750,38750,77500,14.82541012763977,2.3011507673275918e-07
9799,38826,38826,77652,14.855026006698608,2.2835015234850787e-07
9818,38902,38902,77804,14.890378952026367,2.2457544676555165e-07
9837,38978,38978,77956,14.93654203414917,2.2223952001638764e-07
9856,39054,39054,78108,15.052608966827393,2.2047633931829834e-07
9875,39130,39130,78260,15.096871852874756,2.171301512132511e-07
9894,39206,39206,78412,15.131529092788696,2.1314495527086599e-07
9914,39286,39286,78572,15.165858030319214,2.0582183418004533e-07
9933,39362,39362,78724,15.199959993362427,2.0334770718352096e-07
9952,39438,39438,78876,15.22857403755188,2.0037930564110314e-07
9971,39514,39514,79028,15.25667405128479,1.9554135210614035e-07
9990,39590,39590,79180,15.284349918365479,1.903937399746747e-07
10009,39666,39666,79332,15.311885118484497,1.8714323745317418e-07
10028,39742,39742,79484,15.339740991592407,1.8543294327779848e-07
10048,39822,39822,79644,15.367172241210938,1.834821960125647e-07
10067,39898,39898,79796,15.393383979797363,1.8146789663677985e-07
10086,39974,39974,79948,15.418936014175415,1.798810029473968e-07
10105,40050,40050,80100,15.447163105010986,1.783224731646988e-07
10124,40126,40126,80252,15.474684953689575,1.765459484861123e-07
10143,40202,40202,80404,15.50234603881836,1.7527730147138863e-07
10162,40278,40278,80556,15.529587984085083,1.7400996434055474e-07
10181,40354,40354,80708,15.55888319015503,1.7193746932483943e-07
10201,40434,40434,80868,15.586235284805298,1.703124938203353e-07
10220,40510,40510,81020,15.612246990203857,1.6922004922507634e-07
10239,40586,40586,81172,15.638092041015625,1.6716758895756044e-07
10258,40662,40662,81324,15.663267135620117,1.6541146231430715e-07
10277,40738,40738,81476,15.689232110977173,1.6433640565858102e-07
10296,40814,40814,81628,15.714364051818848,1.626092871699249e-07
10315,40890,40890,81780,15.740207195281982,1.6156809542811833e-07
10335,40970,40970,81940,15.766525030136108,1.5932896225627154e-07
10354,41046,41046,82092,15.792968034744263,1.5602263087513647e-07
10373,41122,41122,82244,15.822848081588745,1.5036045595095985e-07
10392,41198,41198,82396,15.851722002029419,1.490616425297635e-07
10411,41274,41274,82548,15.879408121109009,1.467604041308098e-07
10430,41350,41350,82700,15.907189130783081,1.452898381852695e-07
10449,41426,41426,82852,15.935664892196655,1.4248040571390264e-07
10469,41506,41506,83012,15.96613097190857,1.3906813821127356e-07
10488,41582,41582,83164,15.993690967559814,1.3734712334356317e-07
10507,41658,41658,83316,16.0206139087677,1.3643125585341458e-07
10526,41734,41734,83468,16.047213077545166,1.353919987452578e-07
10545,41810,41810,83620,16.072776079177856,1.342552438397828e-07
10564,41886,41886,83772,16.097162008285522,1.333793980341655e-07
10583,41962,41962,83924,16.121732234954834,1.3248853645048653e-07
10603,42042,42042,84084,16.14785408973694,1.3136770745709364e-07
10622,42118,42118,84236,16.174192905426025,1.3078583677589325e-07
10641,42194,42194,84388,16.203289031982422,1.294836779665041e-07
10660,42270,42270,84540,16.23114800453186,1.2765406813883796e-07
10679,42346,42346,84692,16.256903886795044,1.2661200773217276e-07
10698,42422,42422,84844,16.28210997581482,1.2451857269641833e-07
10717,42498,42498,84996,16.30671000480652,1.228787309051713e-07
10736,42574,42574,85148,16.331077098846436,1.1941211370582445e-07
10756,42654,42654,85308,16.35714626312256,1.1539681273720418e-07
10775,42730,42730,85460,16.38165807723999,1.1319466207637223e-07
10794,42806,42806,85612,16.405846118927002,1.1206918815042183e-07
10813,42882,42882,85764,16.432907104492188,1.1116315576231877e-07
10832,42958,42958,85916,16.457698106765747,1.1007449486322114e-07
10851,43034,43034,86068,16.48449683189392,1.0863532497829951e-07
10870,43110,43110,86220,16.51062822341919,1.0710833728671388e-07
10890,43190,43190,86380,16.537646055221558,1.0636661997475458e-07
10909,43266,43266,86532,16.566116094589233,1.04378423078976e-07
10928,43342,43342,86684,16.594385862350464,1.0230941643384394e-07
10947,43418,43418,86836,16.619384050369263,1.0077586975164321e-07
10966,43494,43494,86988,16.644987106323242,9.922996548361543e-08
10985,43570,43570,87140,16.670547008514404,9.80504474497917e-08
11004,43646,43646,87292,16.69814705848694,9.639680917186724e-08
11024,43726,43726,87452,16.725208044052124,9.525863962656455e-08
11043,43802,43802,87604,16.750366926193237,9.437903930934381e-08
11062,43878,43878,87756,16.77602195739746,9.152921853629519e-08
11081,43954,43954,87908,16.801659107208252,8.613133070435472e-08
11100,44030,44030,88060,16.827577114105225,8.28887606167079e-08
11119,44106,44106,88212,16.85318088531494,8.220020341728871e-08
11138,44182,44182,88364,16.878688097000122,8.14266951748913e-08
11158,44262,44262,88524,16.905583143234253,8.03004470565211e-08
11177,44338,44338,88676,16.932199954986572,7.926527328491887e-08
11196,44414,44414,88828,16.9580659866333,7.87347906903955e-08
11215,44490,44490,88980,16.98328399658203,7.804371736830008e-08
11234,44566,44566,89132,17.00841498374939,7.718987120182144e-08
11253,44642,44642,89284,17.035311222076416,7.663572500721359e-08
11272,44718,44718,89436,17.062573194503784,7.613700357286634e-08
11292,44798,44798,89596,17.08958911895752,7.55220256494139e-08
11311,44874,44874,89748,17.115426063537598,7.485840157545957e-08
11330,44950,44950,89900,17.141327142715454,7.429261349684688e-08
11349,45026,45026,90052,17.178310871124268,7.352446497136087e-08
11368,45102,45102,90204,17.22393798828125,7.261232550234918e-08
11387,45178,45178,90356,17.254556894302368,7.203394487918418e-08
11406,45254,45254,90508,17.283421993255615,7.153128227189651e-08
11425,45330,45330,90660,17.311129093170166,7.082453843694383e-08
11445,45410,45410,90820,17.34017515182495,7.008463788670893e-08
11464,45486,45486,90972,17.370420932769775,6.960561459622244e-08
11483,45562,45562,91124,17.400132179260254,6.826978265575268e-08
11502,45638,45638,91276,17.446876049041748,6.708180482131434e-08
11521,45714,45714,91428,17.480773210525513,6.623140740594348e-08
11540,45790,45790,91580,17.511696100234985,6.514612542690798e-08
11559,45866,45866,91732,17.542321920394897,6.429618758320467e-08
11579,45946,45946,91892,17.571887254714966,6.292442753367921e-08
11598,46022,46022,92044,17.598891973495483,6.237467574885127e-08
11617,46098,46098,92196,17.628303050994873,6.203994998861795e-08
11636,46174,46174,92348,17.65620994567871,6.06723844649361e-08
11655,46250,46250,92500,17.68679189682007,5.962044658678671e-08
11674,46326,46326,92652,17.71674919128418,5.756481246918268e-08
11693,46402,46402,92804,17.744165182113647,5.5269100723158e-08
11713,46482,46482,92964,17.776113986968994,5.435300333938948e-08
11732,46558,46558,93116,17.817289113998413,5.385426686415536e-08
11751,46634,46634,93268,17.851790189743042,5.3005970913211766e-08
11770,46710,46710,93420,17.887528896331787,5.2012999063250154e-08
11789,46786,46786,93572,17.92059302330017,5.14757802967535e-08
11808,46862,46862,93724,17.95544695854187,5.092183268325296e-08
11827,46938,46938,93876,17.99309206008911,5.0164443983467764e-08
11847,47018,47018,94036,18.025179862976074,4.956040758386796e-08
11866,47094,47094,94188,18.053953170776367,4.905158275055611e-08
11885,47170,47170,94340,18.084779024124146,4.834703563188641e-08
11904,47246,47246,94492,18.110996961593628,4.782384268889288e-08
11923,47322,47322,94644,18.136863946914673,4.746382679774443e-08
11942,47398,47398,94796,18.163305044174194,4.690189574102989e-08
11961,47474,47474,94948,18.188519954681396,4.6108059009858624e-08
11980,47550,47550,95100,18.21442198753357,4.577148427257149e-08
12000,47630,47630,95260,18.2417049407959,4.521576711649911e-08
12019,47706,47706,95412,18.267162084579468,4.4303786385103095e-08
12038,47782,47782,95564,18.29547905921936,4.3742201009727945e-08
12057,47858,47858,95716,18.324143171310425,4.3340960985999195e-08
12076,47934,47934,95868,18.35058307647705,4.285208349278467e-08
12095,48010,48010,96020,18.381335020065308,4.2273113439207584e-08
12114,48086,48086,96172,18.408878087997437,4.136451415018338e-08
12134,48166,48166,96332,18.44019603729248,4.0834046989516206e-08
12153,48242,48242,96484,18.465620040893555,4.05533244421094e-08
12172,48318,48318,96636,18.49207615852356,4.0188707911261066e-08
12191,48394,48394,96788,18.51746106147766,3.9771194148525164e-08
12210,48470,48470,96940,18.544207096099854,3.9430902927330194e-08
12229,48546,48546,97092,18.571299076080322,3.908226144672192e-08
12248,48622,48622,97244,18.596714973449707,3.872825483203991e-08
12268,48702,48702,97404,18.62300395965576,3.842332567917799e-08
12287,48778,48778,97556,18.648802042007446,3.802273466070255e-08
12306,48854,48854,97708,18.674302101135254,3.742358778201812e-08
12325,48930,48930,97860,18.699306964874268,3.712112396059052e-08
12344,49006,49006,98012,18.72503399848938,3.680728988205042e-08
12363,49082,49082,98164,18.750949144363403,3.6508233472414696e-08
12382,49158,49158,98316,18.77713418006897,3.609026520610402e-08
12402,49238,49238,98476,18.807897090911865,3.5646950405196314e-08
12421,49314,49314,98628,18.837902069091797,3.5087763004437536e-08
12440,49390,49390,98780,18.86698293685913,3.419738698491668e-08
12459,49466,49466,98932,18.898840188980103,3.293617564021175e-08
12478,49542,49542,99084,18.92722201347351,3.220088758119591e-08
12497,49618,49618,99236,18.954775094985962,3.198535670093827e-08
12516,49694,49694,99388,18.980458974838257,3.174425905521725e-08
12535,49770,49770,99540,19.00676417350769,3.1278323900449814e-08
12555,49850,49850,99700,19.038851022720337,3.094713634239555e-08
12574,49926,49926,99852,19.069332122802734,3.0656984719254595e-08
12593,50002,50002,100004,19.100543975830078,3.0370965049691386e-08
12612,50078,50078,100156,19.1286940574646,2.9931745842312414e-08
12631,50154,50154,100308,19.156656980514526,2.9567151872611242e-08
12650,50230,50230,100460,19.189263105392456,2.9338065875312828e-08
12669,50306,50306,100612,19.220784187316895,2.910833443667019e-08
12689,50386,50386,100772,19.24981713294983,2.8809562254474463e-08
12708,50462,50462,100924,19.276596069335938,2.8544346781246448e-08
12727,50538,50538,101076,19.302640914916992,2.8329820922438343e-08
12746,50614,50614,101228,19.32818603515625,2.8108058712547013e-08
12765,50690,50690,101380,19.356178998947144,2.781172820706738e-08
12784,50766,50766,101532,19.381484985351562,2.7569268962602605e-08
12803,50842,50842,101684,19.40780997276306,2.7403705072005963e-08
12823,50922,50922,101844,19.43644690513611,2.7102183362925178e-08
12842,50998,50998,101996,19.46336603164673,2.6617674759643852e-08
12861,51074,51074,102148,19.490128993988037,2.635827089888049e-08
12880,51150,51150,102300,19.515534162521362,2.6052127278680988e-08
12899,51226,51226,102452,19.542320251464844,2.521645020054392e-08
12918,51302,51302,102604,19.57611107826233,2.4480762863674434e-08
12937,51378,51378,102756,19.604961156845093,2.3875240811483564e-08
12957,51458,51458,102916,19.638500213623047,2.3461218626185518e-08
12976,51534,51534,103068,19.66926407814026,2.32511191018955e-08
12995,51610,51610,103220,19.699434995651245,2.305189348008416e-08
13014,51686,51686,103372,19.7344331741333,2.2819765008412288e-08
13033,51762,51762,103524,19.769891023635864,2.2620316126344e-08
13052,51838,51838,103676,19.80080795288086,2.2478643849878555e-08
13071,51914,51914,103828,19.837918043136597,2.224002044059171e-08
13090,51990,51990,103980,19.875622034072876,2.1872775304893167e-08
13110,52070,52070,104140,19.914303064346313,2.1598785722460005e-08
13129,52146,52146,104292,19.952255964279175,2.145199344823116e-08
13148,52222,52222,104444,19.983999967575073,2.128200393051849e-08
13167,52298,52298,104596,20.014212131500244,2.1073799194517552e-08
13186,52374,52374,104748,20.054739952087402,2.0883053847765038e-08
13205,52450,52450,104900,20.091917037963867,2.0539680978449223e-08
13224,52526,52526,105052,20.133827209472656,2.0353937993944897e-08
13244,52606,52606,105212,20.166420936584473,1.9974214919746477e-08
13263,52682,52682,105364,20.202155113220215,1.9532123022011546e-08
13282,52758,52758,105516,20.240148067474365,1.9205504996158316e-08
13301,52834,52834,105668,20.27207088470459,1.8996476217379524e-08
13320,52910,52910,105820,20.303479194641113,1.884026084702916e-08
13339,52986,52986,105972,20.337518215179443,1.862664286725609e-08
13358,53062,53062,106124,20.369264841079712,1.8313526235750087e-08
13378,53142,53142,106284,20.39704918861389,1.8172453217176777e-08
13397,53218,53218,106436,20.42494010925293,1.7889372206632495e-08
13416,53294,53294,106588,20.451431035995483,1.710811678949239e-08
13435,53370,53370,106740,20.477365016937256,1.59626433781478e-08
13454,53446,53446,106892,20.503448009490967,1.5023434987331274e-08
13473,53522,53522,107044,20.530899047851562,1.460127761690278e-08
13492,53598,53598,107196,20.557648181915283,1.4376273853425856e-08
13512,53678,53678,107356,20.586645126342773,1.4265809362926662e-08
13531,53754,53754,107508,20.61333703994751,1.4136164020827228e-08
13550,53830,53830,107660,20.638476133346558,1.3906536239601473e-08
13569,53906,53906,107812,20.66358208656311,1.3714372958383737e-08
13588,53982,53982,107964,20.690030097961426,1.3625767822016242e-08
13607,54058,54058,108116,20.714564085006714,1.3502674711396301e-08
13626,54134,54134,108268,20.740104913711548,1.336708558087578e-08
13645,54210,54210,108420,20.76555299758911,1.3256282100844254e-08
13665,54290,54290,108580,20.792160034179688,1.3011817718915725e-08
13684,54366,54366,108732,20.818401098251343,1.2743801754883238e-08
13703,54442,54442,108884,20.844671964645386,1.2409518352877433e-08
13722,54518,54518,109036,20.86987018585205,1.2048252820271863e-08
13741,54594,54594,109188,20.895036935806274,1.186939263102265e-08
13760,54670,54670,109340,20.921975135803223,1.1765067033988007e-08
13779,54746,54746,109492,20.947720050811768,1.1668938178209883e-08
13799,54826,54826,109652,20.974747896194458,1.1578595563725505e-08
13818,54902,54902,109804,20.9998459815979,1.147224408656984e-08
13837,54978,54978,109956,21.024891138076782,1.130777189511324e-08
13856,55054,55054,110108,21.052191972732544,1.1196421390651567e-08
13875,55130,55130,110260,21.078976154327393,1.1102222454630661e-08
13894,55206,55206,110412,21.104248046875,1.1001089189905664e-08
13913,55282,55282,110564,21.129817008972168,1.0924119455184525e-08
13933,55362,55362,110724,21.15647315979004,1.0710802230565706e-08
13952,55438,55438,110876,21.18314814567566,9.953948563288455e-09
13971,55510,55510,111020,21.207717895507812,9.046966807312428e-09
13990,55586,55586,111172,21.233038187026978,8.807033689508296e-09
14009,55662,55662,111324,21.258736848831177,8.732002360333906e-09
14028,55738,55738,111476,21.28340196609497,8.661324625413237e-09
14047,55814,55814,111628,21.308868169784546,8.489329710600225e-09
14067,55894,55894,111788,21.338631868362427,8.225255285686635e-09
14086,55970,55970,111940,21.36849617958069,7.957833505337916e-09
14105,56046,56046,112092,21.39926505088806,7.77237852315203e-09
14124,56122,56122,112244,21.429857969284058,7.698747615675068e-09
14143,56198,56198,112396,21.45979118347168,7.629789592456136e-09
14162,56274,56274,112548,21.487033128738403,7.554411510311557e-09
14181,56350,56350,112700,21.51193404197693,7.494573993600703e-09
14200,56426,56426,112852,21.53653311729431,7.429759150543498e-09
14220,56506,56506,113012,21.564496994018555,7.358662724805082e-09
14239,56582,56582,113164,21.589723825454712,7.31441431397731e-09
14258,56658,56658,113316,21.614251136779785,7.2465251889643505e-09
14277,56734,56734,113468,21.639193058013916,7.143396894992209e-09
14296,56810,56810,113620,21.66386318206787,7.081438150058934e-09
14315,56886,56886,113772,21.68853497505188,7.035803280073274e-09
14334,56962,56962,113924,21.713171005249023,6.971033167183084e-09
14354,57042,57042,114084,21.739301204681396,6.827824795945569e-09
14373,57118,57118,114236,21.763997077941895,6.779724566281315e-09
14392,57194,57194,114388,21.788469076156616,6.710962759521894e-09
14411,57270,57270,114540,21.81301712989807,6.607702686012319e-09
14430,57346,57346,114692,21.837477207183838,6.41563006374133e-09
14449,57422,57422,114844,21.861430168151855,6.2751906978431865e-09
14468,57498,57498,114996,21.886117935180664,6.218471493041952e-09
14488,57578,57578,115156,21.91265892982483,6.173585089602788e-09
14507,57654,57654,115308,21.938267946243286,6.116244663357851e-09
14526,57730,57730,115460,21.9632089138031,6.056513087598996e-09
14545,57806,57806,115612,21.987877130508423,6.0047031933896634e-09
14564,57882,57882,115764,22.012383937835693,5.947467025964566e-09
14583,57958,57958,115916,22.036932229995728,5.899674751282645e-09
14602,58034,58034,116068,22.062705039978027,5.857347979369291e-09
14622,58114,58114,116228,22.08937406539917,5.796594372437242e-09
14641,58190,58190,116380,22.11614418029785,5.723993675963049e-09
14660,58266,58266,116532,22.14287495613098,5.687236605615658e-09
14679,58342,58342,116684,22.175206899642944,5.632594036877115e-09
14698,58418,58418,116836,22.20447301864624,5.58485209553809e-09
14717,58494,58494,116988,22.23661494255066,5.456684723445231e-09
14736,58570,58570,117140,22.266350030899048,5.3352255127176995e-09
14756,58650,58650,117300,22.299707889556885,5.265558175385488e-09
14775,58726,58726,117452,22.331329107284546,5.21471524041096e-09
14794,58802,58802,117604,22.35961604118347,5.178613136046546e-09
14813,58878,58878,117756,22.387087106704712,5.126938084640616e-09
14832,58954,58954,117908,22.414546966552734,5.079386971614159e-09
14851,59030,59030,118060,22.442858934402466,5.032279233620644e-09
14870,59106,59106,118212,22.475855112075806,4.994117079540176e-09
14889,59182,59182,118364,22.511600971221924,4.957440670392196e-09
14909,59262,59262,118524,22.546441078186035,4.9162165379768474e-09
14928,59338,59338,118676,22.579818964004517,4.871066336175836e-09
14947,59414,59414,118828,22.610738039016724,4.834691213783057e-09
14966,59490,59490,118980,22.63909912109375,4.794398269408208e-09
14985,59566,59566,119132,22.665178060531616,4.750295543892221e-09
15004,59642,59642,119284,22.69313406944275,4.717535766502281e-09
15023,59718,59718,119436,22.720208883285522,4.679684128428746e-09
15043,59798,59798,119596,22.74909496307373,4.62683593131303e-09
15062,59874,59874,119748,22.775799989700317,4.585855019417694e-09
15081,59950,59950,119900,22.802706956863403,4.559409181859359e-09
15100,60026,60026,120052,22.829843044281006,4.504520856841202e-09
15119,60102,60102,120204,22.85798406600952,4.447791119540012e-09
15138,60178,60178,120356,22.88503098487854,4.419731292548446e-09
15157,60254,60254,120508,22.913203954696655,4.392908876626748e-09
15177,60334,60334,120668,22.94500708580017,4.328456640129379e-09
15196,60410,60410,120820,22.973496198654175,4.241293823541063e-09
15215,60486,60486,120972,23.004456043243408,4.184262728050918e-09
15234,60562,60562,121124,23.0329270362854,4.1477104332184e-09
15253,60638,60638,121276,23.06614398956299,4.118635810244612e-09
15272,60714,60714,121428,23.098018169403076,4.085550326278136e-09
15291,60790,60790,121580,23.12842607498169,4.060752972149538e-09
15311,60870,60870,121740,23.158611059188843,4.024140777674009e-09
15330,60946,60946,121892,23.187745094299316,3.984110707636406e-09
15349,61022,61022,122044,23.2174870967865,3.928976205680765e-09
15368,61098,61098,122196,23.246134042739868,3.886319404566696e-09
15387,61174,61174,122348,23.273933172225952,3.733897158465928e-09
15406,61244,61244,122488,23.299370050430298,3.3483812511925777e-09
15425,61310,61310,122620,23.32446002960205,2.9213246302534777e-09
15444,61378,61378,122756,23.349406957626343,2.5810472852808924e-09
15464,61452,61452,122904,23.375810146331787,2.275707589626283e-09
15483,61528,61528,123056,23.399932861328125,2.223720824270411e-09
15502,61604,61604,123208,23.42788815498352,2.1982644128753292e-09
15521,61680,61680,123360,23.454318046569824,2.170412395040682e-09
15540,61756,61756,123512,23.480674028396606,2.1466320215925137e-09
15559,61832,61832,123664,23.50648593902588,2.1228344806090236e-09
15578,61908,61908,123816,23.531836986541748,2.1022461436760196e-09
15598,61988,61988,123976,23.562047958374023,2.085318189085071e-09
15617,62064,62064,124128,23.58856511116028,2.0634587143495304e-09
15636,62140,62140,124280,23.61261796951294,2.0341360437134478e-09
15655,62216,62216,124432,23.63728094100952,2.0192576203252032e-09
15674,62292,62292,124584,23.661618947982788,2.0035396580267694e-09
15693,62368,62368,124736,23.6856791973114,1.973795726678738e-09
15712,62444,62444,124888,23.71014404296875,1.9551951197469996e-09
15732,62524,62524,125048,23.7361159324646,1.935857558870567e-09
15751,62600,62600,125200,23.762032985687256,1.902752774981094e-09
15770,62676,62676,125352,23.78807306289673,1.8680085565059616e-09
15789,62752,62752,125504,23.813552856445312,1.8238775237025082e-09
15808,62828,62828,125656,23.84126114845276,1.8001931727876243e-09
15827,62904,62904,125808,23.86847686767578,1.7855701551765708e-09
15846,62980,62980,125960,23.89510703086853,1.7711919323540194e-09
15866,63060,63060,126120,23.92740511894226,1.7511952873461403e-09
15885,63136,63136,126272,23.95202112197876,1.7353567788081513e-09
15904,63212,63212,126424,23.97657012939453,1.7073502716006043e-09
15923,63288,63288,126576,24.001206159591675,1.6857148497623019e-09
15942,63364,63364,126728,24.027429819107056,1.6723384027898227e-09
15961,63440,63440,126880,24.05290389060974,1.6583424916635487e-09
15980,63516,63516,127032,24.077797889709473,1.6363000624760596e-09
15999,63592,63592,127184,24.10322618484497,1.6098418618316493e-09
16019,63672,63672,127344,24.128662109375,1.5869368786853441e-09
16038,63748,63748,127496,24.153409004211426,1.5709884472125336e-09
16057,63824,63824,127648,24.17794418334961,1.5589515371929474e-09
16076,63900,63900,127800,24.20340394973755,1.545006620068925e-09
16095,63976,63976,127952,24.230334043502808,1.5319774725545616e-09
16114,64052,64052,128104,24.258990049362183,1.5210883404948956e-09
16133,64128,64128,128256,24.287755012512207,1.5081337720631577e-09
16153,64208,64208,128416,24.317482948303223,1.4920488649088993e-09
16172,64284,64284,128568,24.343717098236084,1.481311294386571e-09
16191,64360,64360,128720,24.368292093276978,1.4719675012336963e-09
16210,64436,64436,128872,24.39462399482727,1.4532175690441475e-09
16229,64512,64512,129024,24.421308040618896,1.4318254608261732e-09
16248,64588,64588,129176,24.449968814849854,1.4225303927854775e-09
16267,64664,64664,129328,24.476052045822144,1.4073100822321958e-09
16287,64744,64744,129488,24.503509998321533,1.3868273462771134e-09
16306,64820,64820,129640,24.531996965408325,1.3652255572961767e-09
16325,64896,64896,129792,24.5622341632843,1.3530869408444316e-09
16344,64972,64972,129944,24.589495182037354,1.3396075148202928e-09
16363,65048,65048,130096,24.614530086517334,1.3139059516622554e-09
16382,65124,65124,130248,24.63958191871643,1.2963475527986686e-09
16401,65200,65200,130400,24.66420006752014,1.28764056764663e-09
16421,65280,65280,130560,24.690353870391846,1.2762497654164924e-09
16440,65356,65356,130712,24.715497970581055,1.262761382903009e-09
16459,65432,65432,130864,24.740423917770386,1.2515352637381206e-09
16478,65508,65508,131016,24.766206979751587,1.241614235412984e-09
16497,65584,65584,131168,24.79283905029297,1.229212928420058e-09
16516,65660,65660,131320,24.81837797164917,1.218120783311026e-09
16535,65736,65736,131472,24.843941926956177,1.2078757470815185e-09
16554,65812,65812,131624,24.8694109916687,1.197117922511142e-09
16574,65892,65892,131784,24.898255109786987,1.1881228961333235e-09
16593,65968,65968,131936,24.92452621459961,1.1799127666144108e-09
16612,66044,66044,132088,24.94835901260376,1.16756972590051e-09
16631,66120,66120,132240,24.971972227096558,1.1569508947677734e-09
16650,66196,66196,132392,24.99577021598816,1.1505589278484708e-09
16669,66272,66272,132544,25.019239902496338,1.1398355732043759e-09
16688,66348,66348,132696,25.043873071670532,1.1264046715669374e-09
16708,66428,66428,132856,25.071117162704468,1.1176053879273786e-09
16727,66504,66504,133008,25.095194101333618,1.1039203955447988e-09
16746,66580,66580,133160,25.119140148162842,1.0938900975326181e-09
16765,66656,66656,133312,25.142646074295044,1.0611769999889544e-09
16784,66732,66732,133464,25.167458057403564,1.0194796603254013e-09
16803,66808,66808,133616,25.19381809234619,9.877263144647557e-10
16822,66884,66884,133768,25.219995975494385,9.752369374436238e-10
16842,66964,66964,133928,25.24647307395935,9.66801154249689e-10
16861,67040,67040,134080,25.272258043289185,9.573342694336994e-10
16880,67116,67116,134232,25.297441005706787,9.48837818496589e-10
16899,67192,67192,134384,25.32215404510498,9.413270922720891e-10
16918,67268,67268,134536,25.34718418121338,9.307755481330474e-10
16937,67344,67344,134688,25.37030005455017,9.212440554438018e-10
16956,67420,67420,134840,25.39429497718811,9.158193687675185e-10
16976,67500,67500,135000,25.419332027435303,9.051490282818979e-10
16995,67576,67576,135152,25.442479133605957,8.887680768021845e-10
17014,67652,67652,135304,25.465861082077026,8.76106652433935e-10
17033,67728,67728,135456,25.489616870880127,8.701036779796625e-10
17052,67804,67804,135608,25.513070106506348,8.574267028403075e-10
17071,67880,67880,135760,25.536871910095215,8.416678963185764e-10
17090,67956,67956,135912,25.56094002723694,8.179859417401469e-10
17109,68032,68032,136064,25.58483624458313,8.052911780635141e-10
17129,68112,68112,136224,25.60987114906311,7.928851577860093e-10
17148,68188,68188,136376,25.633785009384155,7.838534724515638e-10
17167,68264,68264,136528,25.65716314315796,7.75296007586155e-10
17186,68340,68340,136680,25.680902004241943,7.643403922332503e-10
17205,68416,68416,136832,25.704787015914917,7.58752830876068e-10
17224,68492,68492,136984,25.728559255599976,7.518518381676017e-10
17243,68568,68568,137136,25.75176501274109,7.380297171955318e-10
17263,68648,68648,137296,25.77695107460022,7.320604649370911e-10
17282,68724,68724,137448,25.800689935684204,7.227062470863463e-10
17301,68800,68800,137600,25.824765920639038,7.105280014395129e-10
17320,68876,68876,137752,25.848124027252197,7.049475824515699e-10
17339,68952,68952,137904,25.872055053710938,6.969587585366719e-10
17358,69028,69028,138056,25.895820140838623,6.91612373159959e-10
17377,69104,69104,138208,25.92080807685852,6.838518990841614e-10
17397,69184,69184,138368,25.94605588912964,6.766796652273205e-10
17416,69260,69260,138520,25.969949960708618,6.663102842676656e-10
17435,69336,69336,138672,25.99382495880127,6.561007648853108e-10
17454,69412,69412,138824,26.0175359249115,6.504014490438953e-10
17473,69488,69488,138976,26.04222011566162,6.448250342260688e-10
17492,69564,69564,139128,26.069313049316406,6.370950253945585e-10
17511,69640,69640,139280,26.09277606010437,6.306104803075918e-10
17531,69720,69720,139440,26.117543935775757,6.259115795761608e-10
17550,69796,69796,139592,26.141451120376587,6.196689823480773e-10
17569,69872,69872,139744,26.16507387161255,6.128522100662818e-10
17588,69948,69948,139896,26.1885929107666,6.079587127589242e-10
17607,70024,70024,140048,26.212785005569458,6.026753195768273e-10
17626,70100,70100,140200,26.236598014831543,5.962004441002043e-10
17645,70176,70176,140352,26.26033902168274,5.901400529783045e-10
17665,70256,70256,140512,26.285095930099487,5.845259625933176e-10
17684,70332,70332,140664,26.30851101875305,5.798120617504628e-10
17703,70408,70408,140816,26.332787036895752,5.761370410063161e-10
17722,70484,70484,140968,26.359230041503906,5.696000080992084e-10
17741,70560,70560,141120,26.385215997695923,5.592921094640386e-10
17760,70636,70636,141272,26.411333084106445,5.524250575626027e-10
17779,70712,70712,141424,26.43647313117981,5.490640869662535e-10
17798,70788,70788,141576,26.45988416671753,5.442377683075396e-10
17818,70868,70868,141736,26.484950065612793,5.369573413789578e-10
17837,70944,70944,141888,26.50940704345703,5.249036268647372e-10
17856,71020,71020,142040,26.533493995666504,5.197879922076542e-10
17875,71096,71096,142192,26.564078092575073,5.132242635708938e-10
17894,71172,71172,142344,26.588722944259644,5.079003912039374e-10
17913,71248,71248,142496,26.614331245422363,4.986674861073562e-10
17932,71324,71324,142648,26.639650106430054,4.866442160356789e-10
17952,71404,71404,142808,26.66384792327881,4.747814302098987e-10
17971,71480,71480,142960,26.68720507621765,4.699420616178839e-10
17990,71556,71556,143112,26.711788177490234,4.661195528920667e-10
18009,71632,71632,143264,26.737231254577637,4.630115157649221e-10
18028,71708,71708,143416,26.76443910598755,4.5915036786552945e-10
18047,71784,71784,143568,26.79813003540039,4.55982292121083e-10
18066,71860,71860,143720,26.849870204925537,4.506809700951012e-10
18086,71940,71940,143880,26.912731885910034,4.431081927447979e-10
18105,72016,72016,144032,26.961239099502563,4.376850221335132e-10
18124,72092,72092,144184,26.997541904449463,4.320434053336853e-10
18143,72168,72168,144336,27.030189037322998,4.29070678969461e-10
18162,72244,72244,144488,27.063432931900024,4.251792086886737e-10
18181,72320,72320,144640,27.091354846954346,4.1800194579248575e-10
18200,72396,72396,144792,27.12053608894348,4.091192732573801e-10
18220,72476,72476,144952,27.15315294265747,3.95401452302434e-10
18239,72552,72552,145104,27.181907892227173,3.844910906608798e-10
18258,72628,72628,145256,27.208603858947754,3.801957904114449e-10
18277,72704,72704,145408,27.237773180007935,3.7666058893890575e-10
18296,72780,72780,145560,27.266159057617188,3.7278539210155233e-10
18315,72856,72856,145712,27.291892051696777,3.689679735102998e-10
18334,72932,72932,145864,27.325093269348145,3.6517758603199857e-10
18353,73008,73008,146016,27.387096166610718,3.619719029481995e-10
18373,73088,73088,146176,27.43195104598999,3.590060192817644e-10
18392,73164,73164,146328,27.465683937072754,3.5530660140719954e-10
18411,73240,73240,146480,27.50155210494995,3.522429304826888e-10
18430,73316,73316,146632,27.530094146728516,3.4981409921987823e-10
18449,73392,73392,146784,27.559324026107788,3.4532714904418516e-10
18468,73468,73468,146936,27.590464115142822,3.411843834227715e-10
18487,73544,73544,147088,27.615143060684204,3.3906315271995637e-10
18507,73624,73624,147248,27.642755031585693,3.348959868880364e-10
18526,73700,73700,147400,27.667388916015625,3.280892048665021e-10
18545,73776,73776,147552,27.696571826934814,3.2529178891575464e-10
18564,73852,73852,147704,27.724413871765137,3.2248877001579904e-10
18583,73928,73928,147856,27.75141191482544,3.185247349460129e-10
18602,74004,74004,148008,27.776385068893433,3.1233384234389396e-10
18621,74080,74080,148160,27.80099606513977,3.029792203954347e-10
18641,74160,74160,148320,27.827747106552124,2.9625503774718513e-10
18660,74236,74236,148472,27.853914976119995,2.9302102302452344e-10
18679,74312,74312,148624,27.88144588470459,2.9072008718383656e-10
18698,74388,74388,148776,27.90752100944519,2.8853838051364027e-10
18717,74464,74464,148928,27.935101985931396,2.8616435820479453e-10
18736,74540,74540,149080,27.959824085235596,2.832716654650673e-10
18755,74616,74616,149232,27.988905906677246,2.8015206236480673e-10
18775,74696,74696,149392,28.020753860473633,2.7615049324464034e-10
18794,74772,74772,149544,28.060487985610962,2.726038611167965e-10
18813,74848,74848,149696,28.09604811668396,2.706533853401499e-10
18832,74922,74922,149844,28.12948989868164,2.6128484250726064e-10
18851,74998,74998,149996,28.163044214248657,2.4912643758534363e-10
18870,75074,75074,150148,28.193723917007446,2.4039648052014673e-10
18889,75150,75150,150300,28.221823930740356,2.3243961237380164e-10
18908,75226,75226,150452,28.250991106033325,2.2698172966114265e-10
18928,75306,75306,150612,28.2793869972229,2.2446775824877319e-10
18947,75382,75382,150764,28.31003499031067,2.2045462848712608e-10
18966,75458,75458,150916,28.341698169708252,2.160167347342216e-10
18985,75534,75534,151068,28.370162963867188,2.1302009395340623e-10
19004,75610,75610,151220,28.396483182907104,2.1131947092692786e-10
19023,75686,75686,151372,28.42569088935852,2.0855921304135283e-10
19042,75762,75762,151524,28.45758318901062,2.035279097064256e-10
19062,75842,75842,151684,28.492834091186523,1.9545620023190134e-10
19081,75906,75906,151812,28.564209938049316,1.7057430094828486e-10
19100,75966,75966,151932,28.609542846679688,1.2679405409216228e-10
19119,76028,76028,152056,28.653594970703125,9.938571835454203e-11


==> plot_data/bilinear_matrix_game_n500/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0006918907165527344,2.018959020339561
200,201,200,401,0.1296858787536621,0.04076116011065535
400,401,400,801,0.26802611351013184,0.013980634384136865
601,602,601,1203,0.3660888671875,0.007478912404918883
801,802,801,1603,0.4648020267486572,0.004753673888981912
1001,1002,1001,2003,0.5659382343292236,0.0034486820656248356
1201,1202,1201,2403,0.6663830280303955,0.002503810172570822
1401,1402,1401,2803,0.7686519622802734,0.001967307432897608
1602,1603,1602,3205,0.8746190071105957,0.0016086456926083137
1802,1803,1802,3605,0.9693329334259033,0.001346028185622625
2002,2003,2002,4005,1.0699031352996826,0.0011547644415371076
2202,2203,2202,4405,1.1716101169586182,0.0010113283795863633
2402,2403,2402,4805,1.2654519081115723,0.0008764012526336981
2603,2604,2603,5207,1.3598101139068604,0.0007885591955443794
2803,2804,2803,5607,1.452869176864624,0.0007122684974326582
3003,3004,3003,6007,1.5454058647155762,0.0006497270049117522
3203,3204,3203,6407,1.6400229930877686,0.0005899921784646016
3403,3404,3403,6807,1.7330100536346436,0.0005401320849306003
3604,3605,3604,7209,1.8269810676574707,0.00048778459359689
3804,3805,3804,7609,1.9202721118927002,0.0004349041072029605
4004,4005,4004,8009,2.0117061138153076,0.00038847113218683465
4204,4205,4204,8409,2.1071619987487793,0.00034649996662180084
4404,4405,4404,8809,2.201352834701538,0.0003201086977566544
4605,4606,4605,9211,2.29284405708313,0.0002976451494178679
4805,4806,4805,9611,2.388306140899658,0.0002787488048750214
5005,5006,5005,10011,2.4809839725494385,0.0002616834252635549
5205,5206,5205,10411,2.573606014251709,0.00024784174446748375
5405,5406,5405,10811,2.673776149749756,0.0002358932581286411
5606,5607,5606,11213,2.7657270431518555,0.00022222057465141908
5806,5807,5806,11613,2.8600728511810303,0.00021096911391128278
6006,6007,6006,12013,2.958130121231079,0.00020129223980205993
6206,6207,6206,12413,3.0504298210144043,0.00019273585909174623
6406,6407,6406,12813,3.1431519985198975,0.00018480935625377168
6607,6608,6607,13215,3.2350680828094482,0.00017803357936582126
6807,6808,6807,13615,3.3298280239105225,0.0001711143671780811
7007,7008,7007,14015,3.4230520725250244,0.00016481564381359934
7207,7208,7207,14415,3.5168471336364746,0.00015805629373417124
7407,7408,7407,14815,3.611877202987671,0.00015149638458837136
7608,7609,7608,15217,3.7040019035339355,0.0001457797693524913
7808,7809,7808,15617,3.7940468788146973,0.00014069619698805783
8008,8009,8008,16017,3.8849031925201416,0.0001359878556802032
8208,8209,8208,16417,3.98093581199646,0.0001315320310631447
8408,8409,8408,16817,4.078026056289673,0.00012704728798727748
8609,8610,8609,17219,4.177298069000244,0.0001228685672485282
8809,8810,8809,17619,4.2906410694122314,0.00011888091126387573
9009,9010,9009,18019,4.400728940963745,0.00011504608407371523
9209,9210,9209,18419,4.506505012512207,0.00011138986323499458
9409,9410,9409,18819,4.624882936477661,0.00010790003027536749
9610,9611,9610,19221,4.739508867263794,0.00010454200480419918
9810,9811,9810,19621,4.8490800857543945,0.00010140520053005085
10010,10011,10010,20021,4.967380046844482,9.822756870887653e-05
10210,10211,10210,20421,5.2764060497283936,9.541139505465662e-05
10410,10411,10410,20821,5.399012088775635,9.248817336717906e-05
10611,10612,10611,21223,5.503271818161011,8.995358236946512e-05
10811,10812,10811,21623,5.6055450439453125,8.734485968815005e-05
11011,11012,11011,22023,5.704674959182739,8.48791956616179e-05
11211,11212,11211,22423,5.800329923629761,8.245861582703645e-05
11411,11412,11411,22823,5.894937038421631,8.010144426179838e-05
11612,11613,11612,23225,5.998507976531982,7.797391654826677e-05
11812,11813,11812,23625,6.112811088562012,7.583731772200379e-05
12012,12013,12012,24025,6.217639207839966,7.386174880433945e-05
12212,12213,12212,24425,6.31752610206604,7.20418939795912e-05
12412,12413,12412,24825,6.4215521812438965,7.028027063577944e-05
12613,12614,12613,25227,6.525040149688721,6.85981658108995e-05
12813,12814,12813,25627,6.628347158432007,6.659217145937226e-05
13013,13014,13013,26027,6.736782073974609,6.470267677953778e-05
13213,13214,13213,26427,6.8364951610565186,6.310141366150047e-05
13413,13414,13413,26827,6.937504053115845,6.161135450139276e-05
13614,13615,13614,27229,7.043515205383301,6.020157899221332e-05
13814,13815,13814,27629,7.149831056594849,5.8815072055932136e-05
14014,14015,14014,28029,7.265031814575195,5.7547747299027675e-05
14214,14215,14214,28429,7.367095947265625,5.614420156885427e-05
14414,14415,14414,28829,7.471224069595337,5.486335234982929e-05
14615,14616,14615,29231,7.578567028045654,5.322820019981047e-05
14815,14816,14815,29631,7.691308975219727,5.202449048620488e-05
15015,15016,15015,30031,7.799606084823608,5.086413902761968e-05
15215,15216,15215,30431,7.904677152633667,4.982837480104092e-05
15415,15416,15415,30831,8.005128860473633,4.890273196719915e-05
15616,15617,15616,31233,8.114667892456055,4.79454249621053e-05
15816,15817,15816,31633,8.21501898765564,4.706167708545054e-05
16016,16017,16016,32033,8.313063144683838,4.62281166999516e-05
16216,16217,16216,32433,8.41104793548584,4.538942964559918e-05
16416,16417,16416,32833,8.514524221420288,4.4590360490614544e-05
16617,16618,16617,33235,8.61496901512146,4.353209502387373e-05
16817,16818,16817,33635,8.714219093322754,4.263773141728704e-05
17017,17018,17017,34035,8.814344882965088,4.183191531420544e-05
17217,17218,17217,34435,8.912204027175903,4.1101143869169994e-05
17417,17418,17417,34835,9.015105962753296,4.0360256985905896e-05
17618,17619,17618,35237,9.113395929336548,3.906652236937047e-05
17818,17819,17818,35637,9.207871913909912,3.790749927061513e-05
18018,18019,18018,36037,9.30925989151001,3.69682448243175e-05
18218,18219,18218,36437,9.41080117225647,3.565240984025893e-05
18418,18419,18418,36837,9.50629711151123,3.464829804257318e-05
18619,18620,18619,37239,9.603679895401001,3.3696335798690846e-05
18819,18820,18819,37639,9.699116945266724,3.283983530912163e-05
19019,19020,19019,38039,9.795572996139526,3.207373520938785e-05
19219,19220,19219,38439,9.896644115447998,3.137846258035208e-05
19419,19420,19419,38839,9.992188215255737,3.071992072208155e-05
19620,19621,19620,39241,10.087995052337646,3.0082033730808437e-05
19820,19821,19820,39641,10.183105945587158,2.9510012025143946e-05
20020,20021,20020,40041,10.27529501914978,2.896615470596412e-05
20220,20221,20220,40441,10.368828058242798,2.8434583872974098e-05
20420,20421,20420,40841,10.469096899032593,2.793860337033127e-05
20621,20622,20621,41243,10.569383144378662,2.7490957086516356e-05
20821,20822,20821,41643,10.672912120819092,2.703876168167222e-05
21021,21022,21021,42043,10.766280889511108,2.658779938271546e-05
21221,21222,21221,42443,10.859131097793579,2.615450272457967e-05
21421,21422,21421,42843,10.954699993133545,2.5738748388132668e-05
21622,21623,21622,43245,11.060182094573975,2.5334905800384553e-05
21822,21823,21822,43645,11.20461893081665,2.4959294441267445e-05
22022,22023,22022,44045,11.353259086608887,2.459701794802076e-05
22222,22223,22222,44445,11.491460084915161,2.426120923799731e-05
22422,22423,22422,44845,11.610867023468018,2.3922797641951904e-05
22623,22624,22623,45247,11.737671136856079,2.358720458996452e-05
22823,22824,22823,45647,11.854620218276978,2.3275211369388992e-05
23023,23024,23023,46047,11.9806649684906,2.2973512579643727e-05
23223,23224,23223,46447,12.074445009231567,2.2665489990414793e-05
23423,23424,23423,46847,12.167971134185791,2.2368521492252474e-05
23624,23625,23624,47249,12.264154195785522,2.2072263160185305e-05
23824,23825,23824,47649,12.360112190246582,2.1792185038854662e-05
24024,24025,24024,48049,12.45248293876648,2.1525360890788575e-05
24224,24225,24224,48449,12.544377088546753,2.125398993827494e-05
24424,24425,24424,48849,12.639373064041138,2.0998476168699493e-05
24625,24626,24625,49251,12.73472785949707,2.0753234444392037e-05
24825,24826,24825,49651,12.83138394355774,2.050499326246106e-05
25025,25026,25025,50051,12.928743124008179,2.0263779114669623e-05
25225,25226,25225,50451,13.023812055587769,2.002763713607128e-05
25425,25426,25425,50851,13.118359088897705,1.9805233570316335e-05
25626,25627,25626,51253,13.215132236480713,1.957580440117947e-05
25826,25827,25826,51653,13.314393043518066,1.9354726886901396e-05
26026,26027,26026,52053,13.412336111068726,1.9139851551286825e-05
26226,26227,26226,52453,13.516237020492554,1.892443046324196e-05
26426,26427,26426,52853,13.614874124526978,1.870746277251029e-05
26627,26628,26627,53255,13.711395025253296,1.849366920421552e-05
26827,26828,26827,53655,13.806719064712524,1.82954772494338e-05
27027,27028,27027,54055,13.901834964752197,1.80982210178185e-05
27227,27228,27227,54455,13.99579405784607,1.7894585600168836e-05
27427,27428,27427,54855,14.091858148574829,1.7709397908678323e-05
27628,27629,27628,55257,14.186588048934937,1.7515650693615462e-05
27828,27829,27828,55657,14.28153395652771,1.732427641359571e-05
28028,28029,28028,56057,14.376243829727173,1.7147237054429712e-05
28228,28229,28228,56457,14.473362922668457,1.6972500600055034e-05
28428,28429,28428,56857,14.56869387626648,1.679195799284979e-05
28629,28630,28629,57259,14.669846057891846,1.6607256050936346e-05
28829,28830,28829,57659,14.76469087600708,1.642869071927071e-05
29029,29030,29029,58059,14.86123013496399,1.6231257726122935e-05
29229,29230,29229,58459,14.956342935562134,1.6024972866530433e-05
29429,29430,29429,58859,15.051623106002808,1.5853808018765536e-05
29630,29631,29630,59261,15.148389101028442,1.569204420032237e-05
29830,29831,29830,59661,15.244492053985596,1.5532286416476243e-05
30030,30031,30030,60061,15.339235067367554,1.5368048729864727e-05
30230,30231,30230,60461,15.433658123016357,1.52144092700436e-05
30430,30431,30430,60861,15.528075933456421,1.5064718214837631e-05
30631,30632,30631,61263,15.634865045547485,1.4918452637393357e-05
30831,30832,30831,61663,15.731381893157959,1.4761723748896858e-05
31031,31032,31031,62063,15.825240135192871,1.4608026991756164e-05
31231,31232,31231,62463,15.918967962265015,1.445938620784927e-05
31431,31432,31431,62863,16.019155025482178,1.4309819524528183e-05
31632,31633,31632,63265,16.11668610572815,1.4165565403782295e-05
31832,31833,31832,63665,16.211090087890625,1.4026286746972872e-05
32032,32033,32032,64065,16.307175874710083,1.3891845552646173e-05
32232,32233,32232,64465,16.4012930393219,1.3759353011761771e-05
32432,32433,32432,64865,16.49498200416565,1.3627393518862995e-05
32633,32634,32633,65267,16.590874195098877,1.3493330216095803e-05
32833,32834,32833,65667,16.686962127685547,1.336472730427581e-05
33033,33034,33033,66067,16.783434867858887,1.3237456413725868e-05
33233,33234,33233,66467,16.877807140350342,1.3104077921619519e-05
33433,33434,33433,66867,16.972100019454956,1.2971952307878424e-05
33634,33635,33634,67269,17.06850004196167,1.2849211294540985e-05
33834,33835,33834,67669,17.16551113128662,1.27304845762743e-05
34034,34035,34034,68069,17.261146068572998,1.2610698323242823e-05
34234,34235,34234,68469,17.356317043304443,1.2494558653915198e-05
34434,34435,34434,68869,17.45000696182251,1.2380092999855784e-05
34635,34636,34635,69271,17.545637130737305,1.2261217945080221e-05
34835,34836,34835,69671,17.646136045455933,1.2139834880251609e-05
35035,35036,35035,70071,17.746479988098145,1.2026607430768636e-05
35235,35236,35235,70471,17.839752912521362,1.191297555905526e-05
35435,35436,35435,70871,17.933840036392212,1.1802104176124104e-05
35636,35637,35636,71273,18.02974510192871,1.1697859209508473e-05
35836,35837,35836,71673,18.127595901489258,1.1593350938515641e-05
36036,36037,36036,72073,18.222767114639282,1.1484846965917414e-05
36236,36237,36236,72473,18.316753149032593,1.137616652938302e-05
36436,36437,36436,72873,18.41055679321289,1.1274540752686246e-05
36637,36638,36637,73275,18.505696058273315,1.1169779568499476e-05
36837,36838,36837,73675,18.60184383392334,1.1065977902943369e-05
37037,37038,37037,74075,18.697523832321167,1.0964628542114361e-05
37237,37238,37237,74475,18.79206609725952,1.0865536874384976e-05
37437,37438,37437,74875,18.886479139328003,1.076698146593839e-05
37638,37639,37638,75277,18.980812072753906,1.0669147761633347e-05
37838,37839,37838,75677,19.08000612258911,1.0577326056653098e-05
38038,38039,38038,76077,19.175289154052734,1.0489528596715121e-05
38238,38239,38238,76477,19.269999980926514,1.039699018425426e-05
38438,38439,38438,76877,19.366328954696655,1.0300859837930527e-05
38639,38640,38639,77279,19.462563037872314,1.0206423717576803e-05
38839,38840,38839,77679,19.558115005493164,1.01168692783896e-05
39039,39040,39039,78079,19.65616202354431,1.0027431114998991e-05
39239,39240,39239,78479,19.756765842437744,9.936632068242417e-06
39439,39440,39439,78879,19.85674500465393,9.849268237464279e-06
39640,39641,39640,79281,19.95108389854431,9.764672465319682e-06
39840,39841,39840,79681,20.042896032333374,9.681609859551707e-06
40040,40041,40040,80081,20.13780403137207,9.597575790342973e-06
40240,40241,40240,80481,20.230418920516968,9.518647301155423e-06
40440,40441,40440,80881,20.32302212715149,9.4410621490745e-06
40641,40642,40641,81283,20.416075944900513,9.363718544451202e-06
40841,40842,40841,81683,20.507107973098755,9.280907336570204e-06
41041,41042,41041,82083,20.600291967391968,9.199697595519134e-06
41241,41242,41241,82483,20.719552040100098,9.121410873527956e-06
41441,41442,41441,82883,20.832530975341797,9.045341672050303e-06
41642,41643,41642,83285,20.940994024276733,8.972881324353301e-06
41842,41843,41842,83685,21.04140591621399,8.90221492046207e-06
42042,42043,42042,84085,21.14841914176941,8.83213764554076e-06
42242,42243,42242,84485,21.24477791786194,8.760057655293868e-06
42442,42443,42442,84885,21.343119144439697,8.685254751873719e-06
42643,42644,42643,85287,21.441895246505737,8.61612623864594e-06
42843,42844,42843,85687,21.538846969604492,8.545982217779857e-06
43043,43044,43043,86087,21.638636112213135,8.474467565874431e-06
43243,43244,43243,86487,21.738508939743042,8.403897586724643e-06
43443,43444,43443,86887,21.84026002883911,8.336935516667862e-06
43644,43645,43644,87289,21.943989992141724,8.27007569037697e-06
43844,43845,43844,87689,22.042582035064697,8.206592746369263e-06
44044,44045,44044,88089,22.143998861312866,8.146718725239161e-06
44244,44245,44244,88489,22.241874933242798,8.084758748804204e-06
44444,44445,44444,88889,22.33720111846924,8.019859794305835e-06
44645,44646,44645,89291,22.437224864959717,7.954726309405252e-06
44845,44846,44845,89691,22.53642201423645,7.891127928376821e-06
45045,45046,45045,90091,22.635721921920776,7.830402212055003e-06
45245,45246,45245,90491,22.73248600959778,7.770226660958626e-06
45445,45446,45445,90891,22.829209089279175,7.713394005620631e-06
45646,45647,45646,91293,22.929249048233032,7.656807957493565e-06
45846,45847,45846,91693,23.032167196273804,7.597628530126564e-06
46046,46047,46046,92093,23.136861085891724,7.5399833159383375e-06
46246,46247,46246,92493,23.242263078689575,7.484794376567849e-06
46446,46447,46446,92893,23.343194007873535,7.431001207166474e-06
46647,46648,46647,93295,23.446534156799316,7.375298460765313e-06
46847,46848,46847,93695,23.54470920562744,7.3179891854175204e-06
47047,47048,47047,94095,23.6479651927948,7.2643933610587996e-06
47247,47248,47247,94495,23.751644134521484,7.210976018832241e-06
47447,47448,47447,94895,23.85156512260437,7.157167250338387e-06
47648,47649,47648,95297,23.960018157958984,7.106481508665893e-06
47848,47849,47848,95697,24.065216064453125,7.058426206645073e-06
48048,48049,48048,96097,24.169049978256226,7.011757297099145e-06
48248,48249,48248,96497,24.271368980407715,6.96287273060307e-06
48448,48449,48448,96897,24.37349009513855,6.914040790896323e-06
48649,48650,48649,97299,24.47553515434265,6.864688381152165e-06
48849,48850,48849,97699,24.57674217224121,6.817333096090463e-06
49049,49050,49049,98099,24.680713891983032,6.76971622479867e-06
49249,49250,49249,98499,24.782012224197388,6.722371397200465e-06
49449,49450,49449,98899,24.883830070495605,6.676677912066424e-06
49650,49651,49650,99301,24.98781704902649,6.633045644389544e-06
49850,49851,49850,99701,25.09436798095703,6.590913145902961e-06
50050,50051,50050,100101,25.196091175079346,6.549847249049841e-06
50250,50251,50250,100501,25.29758310317993,6.509289614765456e-06
50450,50451,50450,100901,25.397894144058228,6.467316660525181e-06
50651,50652,50651,101303,25.49740695953369,6.423400223265311e-06
50851,50852,50851,101703,25.599399089813232,6.38011207953982e-06
51051,51052,51051,102103,25.698559999465942,6.339115387005411e-06
51251,51252,51251,102503,25.79839515686035,6.299527201620974e-06
51451,51452,51451,102903,25.89651393890381,6.261892104954493e-06
51652,51653,51652,103305,25.997303009033203,6.2254929303293284e-06
51852,51853,51852,103705,26.106410026550293,6.188056806975595e-06
52052,52053,52052,104105,26.20594882965088,6.149521534613314e-06
52252,52253,52252,104505,26.30411696434021,6.112217875909116e-06
52452,52453,52452,104905,26.40741205215454,6.0755667616829965e-06
52653,52654,52653,105307,26.51087212562561,6.037966831298695e-06
52853,52854,52853,105707,26.613919019699097,6.000595396202917e-06
53053,53054,53053,106107,26.721017122268677,5.964719897248612e-06
53253,53254,53253,106507,26.824865102767944,5.929290757505344e-06
53453,53454,53453,106907,26.929698944091797,5.8930219972410895e-06
53654,53655,53654,107309,27.03413200378418,5.860179437535335e-06
53854,53855,53854,107709,27.14177107810974,5.82905388092337e-06
54054,54055,54054,108109,27.248713970184326,5.797622797539256e-06
54254,54255,54254,108509,27.354344844818115,5.764513518132299e-06
54454,54455,54454,108909,27.460352897644043,5.73207691718837e-06
54655,54656,54655,109311,27.565953969955444,5.700153188091916e-06
54855,54856,54855,109711,27.68617606163025,5.669208311318425e-06
55055,55056,55055,110111,27.789266109466553,5.636970540443322e-06
55255,55256,55255,110511,27.892818927764893,5.606782221634632e-06
55455,55456,55455,110911,27.995154857635498,5.576470004151609e-06
55656,55657,55656,111313,28.105796098709106,5.547153176124909e-06
55856,55857,55856,111713,28.2175190448761,5.518532269959701e-06
56056,56057,56056,112113,28.337097883224487,5.490115285505996e-06
56256,56257,56256,112513,28.438060998916626,5.4635662726641095e-06
56456,56457,56456,112913,28.540628910064697,5.436879659221792e-06
56657,56658,56657,113315,28.643023014068604,5.408584772660401e-06
56857,56858,56857,113715,28.74557113647461,5.380623637182365e-06
57057,57058,57057,114115,28.84782886505127,5.352979434197074e-06
57257,57258,57257,114515,28.951789140701294,5.3267180316268536e-06
57457,57458,57457,114915,29.05465292930603,5.301241596314342e-06
57658,57659,57658,115317,29.15745997428894,5.27710711255904e-06
57858,57859,57858,115717,29.25677514076233,5.254068373673773e-06
58058,58059,58058,116117,29.354795932769775,5.230000029364922e-06
58258,58259,58258,116517,29.45415186882019,5.205039121357084e-06
58458,58459,58458,116917,29.553133964538574,5.180943469472777e-06
58659,58660,58659,117319,29.656657218933105,5.157011645011207e-06
58859,58860,58859,117719,29.753202199935913,5.132910296991532e-06
59059,59060,59059,118119,29.8489990234375,5.109750031148203e-06
59259,59260,59259,118519,29.94454288482666,5.087007908396386e-06
59459,59460,59459,118919,30.039232969284058,5.0648453998596624e-06
59660,59661,59660,119321,30.13569712638855,5.0433900557700875e-06
59860,59861,59860,119721,30.234748125076294,5.023202304706336e-06
60060,60061,60060,120121,30.333423137664795,5.003052869498259e-06
60260,60261,60260,120521,30.428997039794922,4.9825495787796475e-06
60460,60461,60460,120921,30.524867057800293,4.960494591596389e-06
60661,60662,60661,121323,30.621906995773315,4.9393012891353374e-06
60861,60862,60861,121723,30.717531204223633,4.918420123380644e-06
61061,61062,61061,122123,30.81237506866455,4.8985283671483695e-06
61261,61262,61261,122523,30.9104220867157,4.879252320801058e-06
61461,61462,61461,122923,31.00460410118103,4.860985096003401e-06
61662,61663,61662,123325,31.102582931518555,4.84254485608748e-06
61862,61863,61862,123725,31.19775414466858,4.823939417995177e-06
62062,62063,62062,124125,31.292733907699585,4.805359624821139e-06
62262,62263,62262,124525,31.387348890304565,4.7876716781659345e-06
62462,62463,62462,124925,31.47947096824646,4.770333724815941e-06
62663,62664,62663,125327,31.573507070541382,4.751917075696197e-06
62863,62864,62863,125727,31.665882110595703,4.734497071727218e-06
63063,63064,63063,126127,31.75905990600586,4.716981144593251e-06
63263,63264,63263,126527,31.850483894348145,4.699738393525728e-06
63463,63464,63463,126927,31.942511081695557,4.68302970087913e-06
63664,63665,63664,127329,32.03462290763855,4.667474086693693e-06
63864,63865,63864,127729,32.13322901725769,4.652468759595238e-06
64064,64065,64064,128129,32.26862621307373,4.6374707246470715e-06
64264,64265,64264,128529,32.45208120346069,4.622366835618746e-06
64464,64465,64464,128929,32.56269598007202,4.607134866975447e-06
64665,64666,64665,129331,32.671852111816406,4.591599882665121e-06
64865,64866,64865,129731,32.8482460975647,4.576496106197752e-06
65065,65066,65065,130131,33.010972023010254,4.561101505619987e-06
65265,65266,65265,130531,33.107089042663574,4.546860134347892e-06
65465,65466,65465,130931,33.20658802986145,4.532842824405755e-06
65666,65667,65666,131333,33.30677604675293,4.519075480989607e-06
65866,65867,65866,131733,33.40000891685486,4.505964376744404e-06
66066,66067,66066,132133,33.4933500289917,4.493110169566521e-06
66266,66267,66266,132533,33.58946204185486,4.480415647204266e-06
66466,66467,66466,132933,33.68166899681091,4.467205847928215e-06
66667,66668,66667,133335,33.77987289428711,4.4536148780169356e-06
66867,66868,66867,133735,33.8745059967041,4.440545853833456e-06
67067,67068,67067,134135,33.968589067459106,4.4281484209915045e-06
67267,67268,67267,134535,34.06047010421753,4.415453849927751e-06
67467,67468,67467,134935,34.158344984054565,4.4037673371999596e-06
67668,67669,67668,135337,34.25226402282715,4.39236225021195e-06
67868,67869,67868,135737,34.351333141326904,4.3810901735621005e-06
68068,68069,68068,136137,34.45274591445923,4.369691234486843e-06
68268,68269,68268,136537,34.551236152648926,4.358164543030429e-06
68468,68469,68468,136937,34.65007710456848,4.346713176592339e-06
68669,68670,68669,137339,34.74675393104553,4.335463344571485e-06
68869,68870,68869,137739,34.84600281715393,4.324737368158083e-06
69069,69070,69069,138139,34.94595503807068,4.313903768047646e-06
69269,69270,69269,138539,35.04680109024048,4.30313423285168e-06
69469,69470,69469,138939,35.14942502975464,4.292781123240539e-06
69670,69671,69670,139341,35.248818159103394,4.282688677953163e-06
69870,69871,69870,139741,35.348260164260864,4.273067794852501e-06
70070,70071,70070,140141,35.44508695602417,4.2636157067140405e-06
70270,70271,70270,140541,35.541301012039185,4.253838947828608e-06
70470,70471,70470,140941,35.640661001205444,4.243846625576968e-06
70671,70672,70671,141343,35.73720908164978,4.234177267318673e-06
70871,70872,70871,141743,35.83641505241394,4.224645396643351e-06
71071,71072,71071,142143,35.92889213562012,4.215049202222403e-06
71271,71272,71271,142543,36.021042823791504,4.205948448742238e-06
71471,71472,71471,142943,36.111812114715576,4.197279939738672e-06
71672,71673,71672,143345,36.205511808395386,4.188786196939538e-06
71872,71873,71872,143745,36.30340600013733,4.180408358976297e-06
72072,72073,72072,144145,36.45951294898987,4.17190893009907e-06
72272,72273,72272,144545,36.554157972335815,4.163786463602608e-06
72472,72473,72472,144945,36.64809322357178,4.155652908468142e-06
72673,72674,72673,145347,36.73644804954529,4.147242216025874e-06
72873,72874,72873,145747,36.83294987678528,4.139013513304246e-06
73073,73074,73073,146147,36.92401099205017,4.130919640312966e-06
73273,73274,73273,146547,37.01356792449951,4.123127015327734e-06
73473,73474,73473,146947,37.10783791542053,4.115585418812253e-06
73674,73675,73674,147349,37.1999568939209,4.108381735321472e-06
73874,73875,73874,147749,37.29207491874695,4.1012675465273464e-06
74074,74075,74074,148149,37.38387393951416,4.094248224277239e-06
74274,74275,74274,148549,37.47462606430054,4.0870923060152975e-06
74474,74475,74474,148949,37.56565713882446,4.079693746196919e-06
74675,74676,74675,149351,37.65762400627136,4.0727133283119276e-06
74875,74876,74875,149751,37.74791121482849,4.065826301944098e-06
75075,75076,75075,150151,37.84222412109375,4.059006507320213e-06
75275,75276,75275,150551,37.93434500694275,4.0521906697351686e-06
75475,75476,75475,150951,38.02464509010315,4.045674576685878e-06
75676,75677,75676,151353,38.11622405052185,4.0393336016755366e-06
75876,75877,75876,151753,38.20697498321533,4.033333273628305e-06
76076,76077,76076,152153,38.3018901348114,4.027298543636594e-06
76276,76277,76276,152553,38.39377999305725,4.021193192440547e-06
76476,76477,76476,152953,38.4865038394928,4.0149576661416324e-06
76677,76678,76677,153355,38.58054804801941,4.008895581939894e-06
76877,76878,76877,153755,38.67763710021973,4.002774638468063e-06
77077,77078,77077,154155,38.77093696594238,3.9969923587777165e-06
77277,77278,77277,154555,38.86297011375427,3.991401466563471e-06
77477,77478,77477,154955,38.95234704017639,3.985886879839035e-06
77678,77679,77678,155357,39.04276204109192,3.980451839208984e-06
77878,77879,77878,155757,39.13620901107788,3.975126866825627e-06
78078,78079,78078,156157,39.228610038757324,3.969799667592655e-06
78278,78279,78278,156557,39.321882009506226,3.964469089178127e-06
78478,78479,78478,156957,39.41318917274475,3.959272054995678e-06
78679,78680,78679,157359,39.504117012023926,3.954077470783236e-06
78879,78880,78879,157759,39.595104932785034,3.94898050721214e-06
79079,79080,79079,158159,39.68644189834595,3.943673356239752e-06
79279,79280,79279,158559,39.78028416633606,3.9386541712250405e-06
79479,79480,79479,158959,39.8751380443573,3.933803650520798e-06
79680,79681,79680,159361,39.96749401092529,3.929140761824007e-06
79880,79881,79880,159761,40.057514905929565,3.924539350390322e-06
80080,80081,80080,160161,40.14920496940613,3.920094688821877e-06
80280,80281,80280,160561,40.24252796173096,3.915453915360784e-06
80480,80481,80480,160961,40.33435797691345,3.910767291848993e-06
80681,80682,80681,161363,40.43546199798584,3.906111333251841e-06
80881,80882,80881,161763,40.62334418296814,3.901714516713664e-06
81081,81082,81081,162163,40.71922993659973,3.897214431136008e-06
81281,81282,81281,162563,40.83222699165344,3.892946791404614e-06
81481,81482,81481,162963,41.02259802818298,3.888896912543337e-06
81682,81683,81682,163365,41.13066101074219,3.884563437801456e-06
81882,81883,81882,163765,41.303099155426025,3.8805551465020765e-06
82082,82083,82082,164165,41.424992084503174,3.876599629082436e-06
82282,82283,82282,164565,41.53570914268494,3.872625858505034e-06
82482,82483,82482,164965,41.64863991737366,3.868763556883427e-06
82683,82684,82683,165367,41.75031113624573,3.864558697265752e-06
82883,82884,82883,165767,41.84966707229614,3.860634353469451e-06
83083,83084,83083,166167,41.94989013671875,3.85684809239632e-06
83283,83284,83283,166567,42.05026412010193,3.85308683509126e-06
83483,83484,83483,166967,42.150813817977905,3.849526720554424e-06
83684,83685,83684,167369,42.25664710998535,3.846000914369786e-06
83884,83885,83884,167769,42.35644602775574,3.842559418722024e-06
84084,84085,84084,168169,42.455684185028076,3.839121728038319e-06
84284,84285,84284,168569,42.55196785926819,3.8356570707362545e-06
84484,84485,84484,168969,42.65697407722473,3.8321670359823925e-06
84685,84686,84685,169371,42.762418031692505,3.8287586140416584e-06
84885,84886,84885,169771,42.873571157455444,3.825344477799412e-06
85085,85086,85085,170171,42.996302127838135,3.822200867033416e-06
85285,85286,85285,170571,43.1283860206604,3.818747085077099e-06
85485,85486,85485,170971,43.2457070350647,3.815519354451327e-06
85686,85687,85686,171373,43.356924057006836,3.8124183993943223e-06
85886,85887,85886,171773,43.452800035476685,3.8094628980598518e-06
86086,86087,86086,172173,43.55099701881409,3.806435672493939e-06
86286,86287,86286,172573,43.65881705284119,3.8034591493704346e-06
86486,86487,86486,172973,43.75982093811035,3.800325027549511e-06
86687,86688,86687,173375,43.863672971725464,3.7973266881858254e-06
86887,86888,86887,173775,43.96985220909119,3.7945347980899444e-06
87087,87088,87087,174175,44.08529615402222,3.791435936185064e-06
87287,87288,87287,174575,44.195558071136475,3.7886118597548922e-06
87487,87488,87487,174975,44.33368802070618,3.785796509879588e-06
87688,87689,87688,175377,44.5316321849823,3.78303453246106e-06
87888,87889,87888,175777,44.64543414115906,3.780385938384853e-06
88088,88089,88088,176177,44.74361205101013,3.777667771943591e-06
88288,88289,88288,176577,44.83990406990051,3.7750884264033755e-06
88488,88489,88488,176977,44.94275999069214,3.772397819825494e-06
88689,88690,88689,177379,45.06967115402222,3.769863306207296e-06
88889,88890,88889,177779,45.2270929813385,3.7671615873099728e-06
89089,89090,89089,178179,45.36690878868103,3.7645308834472864e-06
89289,89290,89289,178579,45.49857711791992,3.7620974500934466e-06
89489,89490,89489,178979,45.61096501350403,3.759614833835517e-06
89690,89691,89690,179381,45.83793807029724,3.7572130715827153e-06
89890,89891,89890,179781,46.02369499206543,3.754864221432682e-06
90090,90091,90090,180181,46.139047145843506,3.7525294408557296e-06
90290,90291,90290,180581,46.24462699890137,3.7501803552079395e-06
90490,90491,90490,180981,46.388453006744385,3.7477842998475575e-06
90691,90692,90691,181383,46.526610136032104,3.7454945656799693e-06
90891,90892,90891,181783,46.64155912399292,3.7432000227649795e-06
91091,91092,91091,182183,46.73408102989197,3.7409134530419383e-06
91291,91292,91291,182583,46.8275671005249,3.738683795275269e-06
91491,91492,91491,182983,46.92595195770264,3.7365222446340325e-06
91692,91693,91692,183385,47.04710078239441,3.7343767569591324e-06
91892,91893,91892,183785,47.149458169937134,3.7323154290629394e-06
92092,92093,92092,184185,47.239197969436646,3.7301716297545393e-06
92292,92293,92292,184585,47.32997918128967,3.7281863854228945e-06
92492,92493,92492,184985,47.420137882232666,3.726067592104909e-06
92693,92694,92693,185387,47.508331060409546,3.724183839862485e-06
92893,92894,92893,185787,47.59714984893799,3.721825316935096e-06
93093,93094,93093,186187,47.684956073760986,3.71972810444048e-06
93293,93294,93293,186587,47.7758629322052,3.7177701170806563e-06
93493,93494,93493,186987,47.86515808105469,3.7158223947371162e-06
93694,93695,93694,187389,47.95587921142578,3.7138827485621074e-06
93894,93895,93894,187789,48.04366993904114,3.712019497988328e-06
94094,94095,94094,188189,48.13531684875488,3.710109732879412e-06
94294,94295,94294,188589,48.225646018981934,3.70820806248976e-06
94494,94495,94494,188989,48.319069147109985,3.706328687912312e-06
94695,94696,94695,189391,48.409878969192505,3.7048368386704402e-06
94895,94896,94895,189791,48.50325083732605,3.702601561340612e-06
95095,95096,95095,190191,48.61845302581787,3.700848325617244e-06
95295,95296,95295,190591,48.70965504646301,3.6990599923859866e-06
95495,95496,95495,190991,48.80339980125427,3.6972888686868124e-06
95696,95697,95696,191393,48.89261507987976,3.6955438880176505e-06
95896,95897,95896,191793,49.001646995544434,3.6938752363480025e-06
96096,96097,96096,192193,49.1314799785614,3.6923681691613874e-06
96296,96297,96296,192593,49.231239795684814,3.6906668149503246e-06
96496,96497,96496,192993,49.3258171081543,3.6888131307535134e-06
96697,96698,96697,193395,49.42498707771301,3.6871557762478547e-06
96897,96898,96897,193795,49.53670287132263,3.6856869824557805e-06
97097,97098,97097,194195,49.63691997528076,3.684000212393828e-06
97297,97298,97297,194595,49.73324489593506,3.6821924860130233e-06
97497,97498,97497,194995,49.82456398010254,3.680807010521433e-06
97698,97699,97698,195397,49.91615414619446,3.6790336353535507e-06
97898,97899,97898,195797,50.01034998893738,3.677536949066528e-06
98098,98099,98098,196197,50.10253691673279,3.675993762552712e-06
98298,98299,98298,196597,50.195690870285034,3.674504717919146e-06
98498,98499,98498,196997,50.29033899307251,3.6729623017245877e-06
98699,98700,98699,197399,50.38551998138428,3.6714088305943873e-06
98899,98900,98899,197799,50.47486686706543,3.6698918742390845e-06
99099,99100,99099,198199,50.56640601158142,3.6684024894023545e-06
99299,99300,99299,198599,50.65923309326172,3.6669233787449315e-06
99499,99500,99499,198999,50.75168299674988,3.665470817937386e-06
99700,99701,99700,199401,50.850322246551514,3.6640486061728827e-06
99900,99901,99900,199801,50.952394008636475,3.6625962913386964e-06
100100,100101,100100,200201,51.04625415802002,3.661321063926394e-06
100300,100301,100300,200601,51.14597702026367,3.659934498220359e-06
100501,100502,100501,201003,51.2496280670166,3.6583940046432007e-06
100701,100702,100701,201403,51.34889483451843,3.6570459840609714e-06
100901,100902,100901,201803,51.4476420879364,3.6555778345557384e-06
101101,101102,101101,202203,51.53963899612427,3.65425530159682e-06
101301,101302,101301,202603,51.63260793685913,3.6529769183013395e-06
101502,101503,101502,203005,51.72717595100403,3.651588252692143e-06
101702,101703,101702,203405,51.82353615760803,3.650338155017774e-06
101902,101903,101902,203805,51.91591691970825,3.6490016715319337e-06
102102,102103,102102,204205,52.010631799697876,3.6476743822881173e-06
102302,102303,102302,204605,52.11590003967285,3.6464075866002488e-06
102503,102504,102503,205007,52.2110378742218,3.645163129078619e-06
102703,102704,102703,205407,52.30600595474243,3.643813897321237e-06
102903,102904,102903,205807,52.39948797225952,3.6425627628613955e-06
103103,103104,103103,206207,52.49227809906006,3.6412924832709977e-06
103303,103304,103303,206607,52.58258509635925,3.6400597933845685e-06
103504,103505,103504,207009,52.68566703796387,3.6389025693785554e-06
103704,103705,103704,207409,52.77837896347046,3.637688045649134e-06
103904,103905,103904,207809,52.86756086349487,3.636410691344211e-06
104104,104105,104104,208209,52.95899319648743,3.6351880889918814e-06
104304,104305,104304,208609,53.04885292053223,3.63400220949961e-06
104505,104506,104505,209011,53.14626502990723,3.632792721563805e-06
104705,104706,104705,209411,53.2363121509552,3.631566200796507e-06
104905,104906,104905,209811,53.333500146865845,3.6304514597641224e-06
105105,105106,105105,210211,53.427687883377075,3.6292143445833866e-06
105305,105306,105305,210611,53.5181941986084,3.6280599779825227e-06
105506,105507,105506,211013,53.6130211353302,3.626989157960634e-06
105706,105707,105706,211413,53.70371413230896,3.6258268346509264e-06
105906,105907,105906,211813,53.795125007629395,3.6246556145840978e-06
106106,106107,106106,212213,53.88651490211487,3.623549306803784e-06
106306,106307,106306,212613,53.980369091033936,3.622456921551003e-06
106507,106508,106507,213015,54.074939012527466,3.6213720110268776e-06
106707,106708,106707,213415,54.16955900192261,3.62016283014433e-06
106907,106908,106907,213815,54.26261806488037,3.6190779435693513e-06
107107,107108,107107,214215,54.359132051467896,3.6180257979024736e-06
107307,107308,107307,214615,54.45151901245117,3.6169510374423863e-06
107508,107509,107508,215017,54.54325008392334,3.615847792170557e-06
107708,107709,107708,215417,54.634669065475464,3.614804081416602e-06
107908,107909,107908,215817,54.72487497329712,3.613776195877722e-06
108108,108109,108108,216217,54.82055115699768,3.6127350462912375e-06
108308,108309,108308,216617,54.913492918014526,3.6116533175993466e-06
108509,108510,108509,217019,55.00493407249451,3.61066190820256e-06
108709,108710,108709,217419,55.10102605819702,3.60959283690523e-06
108909,108910,108909,217819,55.19363808631897,3.6085558839492688e-06
109109,109110,109109,218219,55.289167165756226,3.6074692116373004e-06
109309,109310,109309,218619,55.385814905166626,3.6064728761455927e-06
109510,109511,109510,219021,55.487919092178345,3.605416999944293e-06
109710,109711,109710,219421,55.579545974731445,3.604413560242234e-06
109910,109911,109910,219821,55.67207908630371,3.603418617273633e-06
110110,110111,110110,220221,55.76504397392273,3.602393225901843e-06
110310,110311,110310,220621,55.856667041778564,3.6014218381734103e-06
110511,110512,110511,221023,55.94851303100586,3.600700056428718e-06
110711,110712,110711,221423,56.04057812690735,3.5993842837907464e-06
110911,110912,110911,221823,56.13319110870361,3.5984143936985385e-06
111111,111112,111111,222223,56.22398400306702,3.5974722266238937e-06
111311,111312,111311,222623,56.31700086593628,3.5967595894486207e-06
111512,111513,111512,223025,56.40873384475708,3.5955721846205844e-06
111712,111713,111712,223425,56.499176025390625,3.5945584812528503e-06
111912,111913,111912,223825,56.59226584434509,3.5936665258617684e-06
112112,112113,112112,224225,56.6836211681366,3.592655565972945e-06
112312,112313,112312,224625,56.777273178100586,3.591718297376623e-06
112513,112514,112513,225027,56.8686408996582,3.590736554979234e-06
112713,112714,112713,225427,56.96247601509094,3.5898088141995905e-06
112913,112914,112913,225827,57.05435585975647,3.5888654697869555e-06
113113,113114,113113,226227,57.148947954177856,3.5879380170002856e-06
113313,113314,113313,226627,57.24056100845337,3.5870165408366276e-06
113514,113515,113514,227029,57.333438873291016,3.586075454086718e-06
113714,113715,113714,227429,57.42562818527222,3.5851665726852584e-06
113914,113915,113914,227829,57.524746894836426,3.584284045528196e-06
114114,114115,114114,228229,57.61766600608826,3.5834424465347335e-06
114314,114315,114314,228629,57.71021509170532,3.582460661770281e-06
114515,114516,114515,229031,57.80681586265564,3.581598190738723e-06
114715,114716,114715,229431,57.89836597442627,3.580646366523325e-06
114915,114916,114915,229831,57.99176383018494,3.5797398065941318e-06
115115,115116,115115,230231,58.08562707901001,3.578802918227916e-06
115315,115316,115315,230631,58.177494049072266,3.5780069642737337e-06
115516,115517,115516,231033,58.26969790458679,3.5770515803358267e-06
115716,115717,115716,231433,58.36274003982544,3.5761837770838292e-06
115916,115917,115916,231833,58.453558921813965,3.5753204374720326e-06
116116,116117,116116,232233,58.544723987579346,3.5744395190576685e-06
116316,116317,116316,232633,58.63681888580322,3.5735904507546236e-06
116517,116518,116517,233035,58.7299702167511,3.5727045747248425e-06
116717,116718,116717,233435,58.822696924209595,3.571820613667159e-06
116917,116918,116917,233835,58.915359020233154,3.5710219655410136e-06
117117,117118,117117,234235,59.007988929748535,3.570291537889936e-06
117317,117318,117317,234635,59.10262703895569,3.5693396183529e-06
117518,117519,117518,235037,59.19489097595215,3.5684107862366385e-06
117718,117719,117718,235437,59.288946866989136,3.5676647279645713e-06
117918,117919,117918,235837,59.38119912147522,3.566792582555437e-06
118118,118119,118118,236237,59.473016023635864,3.5659263881836753e-06
118318,118319,118318,236637,59.56638312339783,3.5650234293002642e-06
118519,118520,118519,237039,59.667826890945435,3.5641751314567284e-06
118719,118720,118719,237439,59.76055121421814,3.563336753411786e-06
118919,118920,118919,237839,59.85114502906799,3.5624700222558714e-06
119119,119120,119119,238239,59.94211983680725,3.561674513359251e-06
119319,119320,119319,238639,60.032907009124756,3.5608745990155976e-06
119520,119521,119520,239041,60.12494897842407,3.560022096479922e-06
119720,119721,119720,239441,60.218767166137695,3.5593898354947857e-06
119920,119921,119920,239841,60.31383800506592,3.5584745937809444e-06
120120,120121,120120,240241,60.40705609321594,3.557593676248367e-06
120320,120321,120320,240641,60.4993531703949,3.5567668282299495e-06
120521,120522,120521,241043,60.59048104286194,3.555901939431318e-06
120721,120722,120721,241443,60.679245948791504,3.555086751142809e-06
120921,120922,120921,241843,60.77135109901428,3.5542912867220536e-06
121121,121122,121121,242243,60.86029505729675,3.5535031376142156e-06
121321,121322,121321,242643,60.947548151016235,3.5526661675162146e-06
121522,121523,121522,243045,61.03523087501526,3.551905502602422e-06
121722,121723,121722,243445,61.12284207344055,3.551087652116537e-06
121922,121923,121922,243845,61.21103096008301,3.5503198156791884e-06
122122,122123,122122,244245,61.30056691169739,3.5495609295052415e-06
122322,122323,122322,244645,61.39022612571716,3.5488026772929757e-06
122523,122524,122523,245047,61.478424072265625,3.5480119796001534e-06
122723,122724,122723,245447,61.565768003463745,3.547192604328507e-06
122923,122924,122923,245847,61.6547429561615,3.546387736032759e-06
123123,123124,123123,246247,61.74920916557312,3.5456493717712528e-06
123323,123324,123323,246647,61.838299036026,3.5448293149937176e-06
123524,123525,123524,247049,61.92569708824158,3.5440487908477966e-06
123724,123725,123724,247449,62.014272928237915,3.543368191925474e-06
123924,123925,123924,247849,62.102782011032104,3.542509218553008e-06
124124,124125,124124,248249,62.18991994857788,3.541721528580885e-06
124324,124325,124324,248649,62.27818489074707,3.541039301986417e-06
124525,124526,124525,249051,62.36692190170288,3.54014850858092e-06
124725,124726,124725,249451,62.45385003089905,3.5394631372012827e-06
124925,124926,124925,249851,62.541561126708984,3.5386925317015138e-06
125125,125126,125125,250251,62.63221096992493,3.5378831737959678e-06
125325,125326,125325,250651,62.720191955566406,3.537152504250966e-06
125526,125527,125526,251053,62.81426191329956,3.5362994818281e-06
125726,125727,125726,251453,62.904847145080566,3.535572000413214e-06
125926,125927,125926,251853,62.99170804023743,3.5347763929844403e-06
126126,126127,126126,252253,63.07954406738281,3.5340457596137737e-06
126326,126327,126326,252653,63.16828894615173,3.5332964728934487e-06
126527,126528,126527,253055,63.256393909454346,3.5326429391150837e-06
126727,126728,126727,253455,63.34591197967529,3.531792719119011e-06
126927,126928,126927,253855,63.43310904502869,3.5309849233837294e-06
127127,127128,127127,254255,63.52011322975159,3.530228588921692e-06
127327,127328,127327,254655,63.60719895362854,3.529431473946044e-06
127528,127529,127528,255057,63.695026874542236,3.5287003386970187e-06
127728,127729,127728,255457,63.79266715049744,3.5280125268634974e-06
127928,127929,127928,255857,63.885565996170044,3.5272725083081323e-06
128128,128129,128128,256257,63.97267508506775,3.526477265727934e-06
128328,128329,128328,256657,64.06014204025269,3.525748812844922e-06
128529,128530,128529,257059,64.15022110939026,3.5250033809509174e-06
128729,128730,128729,257459,64.23729300498962,3.524285184961569e-06
128929,128930,128929,257859,64.32784509658813,3.5238308557443216e-06
129129,129130,129129,258259,64.41509699821472,3.522803299949979e-06
129329,129330,129329,258659,64.50192999839783,3.522017013481699e-06
129530,129531,129530,259061,64.59017014503479,3.521299064603755e-06
129730,129731,129730,259461,64.67738914489746,3.5205674263314605e-06
129930,129931,129930,259861,64.76944303512573,3.5199178235738453e-06
130130,130131,130130,260261,64.86010789871216,3.5190710069940486e-06
130330,130331,130330,260661,64.95252394676208,3.5183700257661206e-06
130531,130532,130531,261063,65.04340291023254,3.5176945673851214e-06
130731,130732,130731,261463,65.13491106033325,3.5168878186808805e-06
130931,130932,130931,261863,65.22514986991882,3.5161579184222357e-06
131131,131132,131131,262263,65.31656503677368,3.5153908100359487e-06
131331,131332,131331,262663,65.4070680141449,3.514866690626913e-06
131532,131533,131532,263065,65.49560284614563,3.5139532039472525e-06
131732,131733,131732,263465,65.5883309841156,3.513289123403636e-06
131932,131933,131932,263865,65.67851209640503,3.5126876714394535e-06
132132,132133,132132,264265,65.77021598815918,3.5117701315830934e-06
132332,132333,132332,264665,65.86473202705383,3.511095852865735e-06
132533,132534,132533,265067,65.96084094047546,3.5103706977963687e-06
132733,132734,132733,265467,66.05109596252441,3.5096067222499512e-06
132933,132934,132933,265867,66.1447081565857,3.5088774444739407e-06
133133,133134,133133,266267,66.23631715774536,3.5081648227961693e-06
133333,133334,133333,266667,66.32828307151794,3.5075501746365935e-06
133534,133535,133534,267069,66.41893005371094,3.5067376452936556e-06
133734,133735,133734,267469,66.50920915603638,3.5060937908496315e-06
133934,133935,133934,267869,66.59984517097473,3.505328131593079e-06
134134,134135,134134,268269,66.69040608406067,3.504697321649805e-06
134334,134335,134334,268669,66.78409218788147,3.503972505804664e-06
134535,134536,134535,269071,66.87404799461365,3.503345646086937e-06
134735,134736,134735,269471,66.96305823326111,3.5024778995242773e-06
134935,134936,134935,269871,67.05193996429443,3.5019223167713573e-06
135135,135136,135135,270271,67.14177203178406,3.501066388453343e-06
135335,135336,135335,270671,67.23007202148438,3.500394387875641e-06
135536,135537,135536,271073,67.32238793373108,3.499689949140648e-06
135736,135737,135736,271473,67.41466212272644,3.4989808787122177e-06
135936,135937,135936,271873,67.505117893219,3.4981894468716895e-06
136136,136137,136136,272273,67.59568786621094,3.4974832107236417e-06
136336,136337,136336,272673,67.68640995025635,3.4967907541811196e-06
136537,136538,136537,273075,67.77853107452393,3.4960577457299842e-06
136737,136738,136737,273475,67.86736416816711,3.495398869756492e-06
136937,136938,136937,273875,67.96443486213684,3.494647282419294e-06
137137,137138,137137,274275,68.06065106391907,3.493932986909508e-06
137337,137338,137337,274675,68.15153503417969,3.493244886974424e-06
137538,137539,137538,275077,68.24282789230347,3.4925112060764606e-06
137738,137739,137738,275477,68.33789896965027,3.49191744435819e-06
137938,137939,137938,275877,68.4299430847168,3.4911165184422223e-06
138138,138139,138138,276277,68.52151393890381,3.490540132402268e-06
138338,138339,138338,276677,68.61695504188538,3.4897026097470855e-06
138539,138540,138539,277079,68.71215987205505,3.4890305090634606e-06
138739,138740,138739,277479,68.80822610855103,3.4883105292270884e-06
138939,138940,138939,277879,68.98308491706848,3.4876273836291153e-06
139139,139140,139139,278279,69.12741494178772,3.486919837310448e-06
139339,139340,139339,278679,69.23948216438293,3.4861955815432036e-06
139540,139541,139540,279081,69.3427619934082,3.4854673297202553e-06
139740,139741,139740,279481,69.50762391090393,3.48484303689197e-06
139940,139941,139940,279881,69.63860297203064,3.4840711036439993e-06
140140,140141,140140,280281,69.73347091674805,3.483416872278094e-06
140340,140341,140340,280681,69.82700300216675,3.4826981322866945e-06
140541,140542,140541,281083,69.92115497589111,3.4819924884594537e-06
140741,140742,140741,281483,70.01010990142822,3.4816334047995833e-06
140941,140942,140941,281883,70.11327004432678,3.4805962912100866e-06
141141,141142,141141,282283,70.20310711860657,3.479925762186245e-06
141341,141342,141341,282683,70.29368495941162,3.479219174555366e-06
141542,141543,141542,283085,70.38299584388733,3.4785308432079906e-06
141742,141743,141742,283485,70.47344994544983,3.477831626322073e-06
141942,141943,141942,283885,70.5667769908905,3.4771412674857387e-06
142142,142143,142142,284285,70.65889811515808,3.4764415266969835e-06
142342,142343,142342,284685,70.74912405014038,3.4758578626966332e-06
142543,142544,142543,285087,70.83870315551758,3.4751026507959646e-06
142743,142744,142743,285487,70.93199706077576,3.4743682537944623e-06
142943,142944,142943,285887,71.02158904075623,3.4737682532478783e-06
143143,143144,143143,286287,71.11590099334717,3.473027417084298e-06
143343,143344,143343,286687,71.2061722278595,3.472318797698662e-06
143544,143545,143544,287089,71.29559588432312,3.471789361445389e-06
143744,143745,143744,287489,71.38512706756592,3.470935760410887e-06
143944,143945,143944,287889,71.47452807426453,3.4703682123404705e-06
144144,144145,144144,288289,71.56584000587463,3.469566040773638e-06
144344,144345,144344,288689,71.65932703018188,3.4689274390683853e-06
144545,144546,144545,289091,71.74756813049316,3.46819572027044e-06
144745,144746,144745,289491,71.83584499359131,3.467510667838851e-06
144945,144946,144945,289891,71.92568492889404,3.46697663083158e-06
145145,145146,145145,290291,72.01532316207886,3.4661892726735403e-06
145345,145346,145345,290691,72.10860705375671,3.46546081689497e-06
145546,145547,145546,291093,72.20680212974548,3.464950685002346e-06
145746,145747,145746,291493,72.29694414138794,3.464207398085972e-06
145946,145947,145946,291893,72.38726902008057,3.463449659072743e-06
146146,146147,146146,292293,72.47705221176147,3.462777777466818e-06
146346,146347,146346,292693,72.56691408157349,3.462106263862404e-06
146547,146548,146547,293095,72.65774011611938,3.4614232802677062e-06
146747,146748,146747,293495,72.7487359046936,3.46078491646456e-06
146947,146948,146947,293895,72.83910298347473,3.4600821704532618e-06
147147,147148,147147,294295,72.9296510219574,3.4593711530446307e-06
147347,147348,147347,294695,73.02011799812317,3.4588003775604815e-06
147548,147549,147548,295097,73.11458921432495,3.458024191135792e-06
147748,147749,147748,295497,73.20909786224365,3.457344878006345e-06
147948,147949,147948,295897,73.30163288116455,3.4566604769453155e-06
148148,148149,148148,296297,73.45096015930176,3.455988225477692e-06
148348,148349,148348,296697,73.58246397972107,3.4553322855737114e-06
148549,148550,148549,297099,73.68294405937195,3.454642903832826e-06
148749,148750,148749,297499,73.78631496429443,3.4539444481618764e-06
148949,148950,148949,297899,73.88309097290039,3.453271672964887e-06
149149,149150,149149,298299,74.05168890953064,3.452575770284382e-06
149349,149350,149349,298699,74.15095114707947,3.451926121333366e-06
149550,149551,149550,299101,74.25214004516602,3.451228768828515e-06
149750,149751,149750,299501,74.3514051437378,3.4506536374759687e-06
149950,149951,149950,299901,74.44615125656128,3.450097155564441e-06
150150,150151,150150,300301,74.54742193222046,3.44924778743016e-06
150350,150351,150350,300701,74.65680718421936,3.448705982265692e-06
150551,150552,150551,301103,74.76267600059509,3.448076620390334e-06
150751,150752,150751,301503,74.85411405563354,3.4471931590768103e-06
150951,150952,150951,301903,74.94694089889526,3.446629173176605e-06
151151,151152,151151,302303,75.03963899612427,3.4458867574480568e-06
151351,151352,151351,302703,75.13047122955322,3.4454103991922682e-06
151552,151553,151552,303105,75.22581815719604,3.444519252877284e-06
151752,151753,151752,303505,75.31673288345337,3.4439563862612033e-06
151952,151953,151952,303905,75.40548920631409,3.4431652800843435e-06
152152,152153,152152,304305,75.4962990283966,3.442520922807105e-06
152352,152353,152352,304705,75.5882978439331,3.4420042070252237e-06
152553,152554,152553,305107,75.75744724273682,3.4411280171572528e-06
152753,152754,152753,305507,75.89748811721802,3.440526233403317e-06
152953,152954,152953,305907,76.01344299316406,3.4397724821426077e-06
153153,153154,153153,306307,76.1408360004425,3.439178079967985e-06
153353,153354,153353,306707,76.24802994728088,3.438604152072623e-06
153554,153555,153554,307109,76.37207913398743,3.4378544233462346e-06
153754,153755,153754,307509,76.50334405899048,3.437129355774005e-06
153954,153955,153954,307909,76.7069640159607,3.436441927624496e-06
154154,154155,154154,308309,76.87808513641357,3.435817628689162e-06
154354,154355,154354,308709,77.00418210029602,3.4351241098725588e-06
154555,154556,154555,309111,77.11921715736389,3.4344584106569338e-06
154755,154756,154755,309511,77.23233103752136,3.4337817002090034e-06
154955,154956,154955,309911,77.40522313117981,3.43322308805101e-06
155155,155156,155155,310311,77.50960993766785,3.4324670872371094e-06
155355,155356,155355,310711,77.63313412666321,3.4319358885620312e-06
155556,155557,155556,311113,77.74723196029663,3.431184867085261e-06
155756,155757,155756,311513,77.87779402732849,3.4304567587841552e-06
155956,155957,155956,311913,78.00778484344482,3.429770336676518e-06
156156,156157,156156,312313,78.20791602134705,3.429166330153163e-06
156356,156357,156356,312713,78.31961107254028,3.428443927604507e-06
156557,156558,156557,313115,78.4688229560852,3.4278053905641005e-06
156757,156758,156757,313515,78.56340098381042,3.4271514408267063e-06
156957,156958,156957,313915,78.67934679985046,3.4264759326647524e-06
157157,157158,157157,314315,78.77258801460266,3.4257553646262294e-06
157357,157358,157357,314715,78.86126399040222,3.425140726683123e-06
157558,157559,157558,315117,79.29195404052734,3.424503995448006e-06
157758,157759,157758,315517,79.41204810142517,3.4237592836184784e-06
157958,157959,157958,315917,79.56829309463501,3.4232632918188655e-06
158158,158159,158158,316317,79.73529601097107,3.4224184305079447e-06
158358,158359,158358,316717,79.86795592308044,3.4217951124150534e-06
158559,158560,158559,317119,79.96277713775635,3.4211278757330945e-06
158759,158760,158759,317519,80.11604714393616,3.4205666996138646e-06
158959,158960,158959,317919,80.26785516738892,3.419816390514421e-06
159159,159160,159159,318319,80.43250513076782,3.4192576775609206e-06
159359,159360,159359,318719,80.63040208816528,3.4185710765626936e-06
159560,159561,159560,319121,80.7477879524231,3.417930451283167e-06
159760,159761,159760,319521,80.86276412010193,3.4171622995098387e-06
159960,159961,159960,319921,81.0679018497467,3.4165339290644833e-06
160160,160161,160160,320321,81.21168613433838,3.4159499058822118e-06
160360,160361,160360,320721,81.31885099411011,3.415184119116376e-06
160561,160562,160561,321123,81.4782178401947,3.414617612269566e-06
160761,160762,160761,321523,81.58495092391968,3.413897615677291e-06
160961,160962,160961,321923,81.67347979545593,3.4132468791163803e-06
161161,161162,161161,322323,81.76309490203857,3.412644737022177e-06
161361,161362,161361,322723,81.92263507843018,3.4119157942788337e-06
161562,161563,161562,323125,82.04798197746277,3.4112562859757845e-06
161762,161763,161762,323525,82.14724087715149,3.4106295803551933e-06
161962,161963,161962,323925,82.24423384666443,3.409976142059682e-06
162162,162163,162162,324325,82.35847592353821,3.409303331091664e-06
162362,162363,162362,324725,82.50785899162292,3.408683645185493e-06
162563,162564,162563,325127,82.59557914733887,3.408024208394193e-06
162763,162764,162763,325527,82.68590688705444,3.4073412021995734e-06
162963,162964,162963,325927,82.78439283370972,3.4066787874865304e-06
163163,163164,163163,326327,82.88073015213013,3.4060242750313874e-06
163363,163364,163363,326727,83.01500415802002,3.4054648573308787e-06
163564,163565,163564,327129,83.13153982162476,3.4047021201642704e-06
163764,163765,163764,327529,83.24413204193115,3.404092126762162e-06
163964,163965,163964,327929,83.34336304664612,3.4034196099975267e-06
164164,164165,164164,328329,83.45004200935364,3.4027616254540074e-06
164364,164365,164364,328729,83.59796500205994,3.4021199457661598e-06
164565,164566,164565,329131,83.68722414970398,3.401434743711699e-06
164765,164766,164765,329531,83.78665208816528,3.400796263594804e-06
164965,164966,164965,329931,83.91025304794312,3.4002003638651694e-06
165165,165166,165165,330331,84.00670504570007,3.39944032626465e-06
165365,165366,165365,330731,84.10822701454163,3.3987961480092597e-06
165566,165567,165566,331133,84.2057409286499,3.3981523763085232e-06
165766,165767,165766,331533,84.31247901916504,3.397519158592078e-06
165966,165967,165966,331933,84.52383303642273,3.3969279719757815e-06
166166,166167,166166,332333,84.61318612098694,3.396430521283752e-06
166366,166367,166366,332733,84.70151591300964,3.395568324944846e-06
166567,166568,166567,333135,84.79836702346802,3.394907248876583e-06
166767,166768,166767,333535,84.89627599716187,3.3942424082397956e-06
166967,166968,166967,333935,84.98455500602722,3.3936537878528283e-06
167167,167168,167167,334335,85.06939911842346,3.392969036862157e-06
167367,167368,167367,334735,85.15993595123291,3.392276909574587e-06
167568,167569,167568,335137,85.24653697013855,3.3916397940340583e-06
167768,167769,167768,335537,85.33594393730164,3.390953520046819e-06
167968,167969,167968,335937,85.42914915084839,3.3903391600834536e-06
168168,168169,168168,336337,85.51950097084045,3.3896361395323865e-06
168368,168369,168368,336737,85.68872594833374,3.389047473624733e-06
168569,168570,168569,337139,85.82596611976624,3.388346064336822e-06
168769,168770,168769,337539,85.9300971031189,3.387695292678486e-06
168969,168970,168969,337939,86.02599596977234,3.3870536001885914e-06
169169,169170,169169,338339,86.18377590179443,3.3864051699603985e-06
169369,169370,169369,338739,86.31375789642334,3.3858812051130585e-06
169570,169571,169570,339141,86.40387296676636,3.385137217178538e-06
169770,169771,169770,339541,86.49593806266785,3.384422155807015e-06
169970,169971,169970,339941,86.58613395690918,3.3838229293431887e-06
170170,170171,170170,340341,86.70032620429993,3.3831706604989417e-06
170370,170371,170370,340741,86.79628586769104,3.3825618317817883e-06
170571,170572,170571,341143,86.89981698989868,3.3818671842808877e-06
170771,170772,170771,341543,87.03592300415039,3.381204478871493e-06
170971,170972,170971,341943,87.14048886299133,3.3806274435162043e-06
171171,171172,171171,342343,87.25238800048828,3.379989852001807e-06
171371,171372,171371,342743,87.36700797080994,3.3793206599910786e-06
171572,171573,171572,343145,87.54483914375305,3.3786743658935063e-06
171772,171773,171772,343545,87.65336894989014,3.3779683176251157e-06
171972,171973,171972,343945,87.74472904205322,3.3773347349614195e-06
172172,172173,172172,344345,87.83460307121277,3.376685123170381e-06
172372,172373,172372,344745,87.9234230518341,3.3760701628044765e-06
172573,172574,172573,345147,88.01237916946411,3.3754093398700396e-06
172773,172774,172773,345547,88.12131714820862,3.3747875571274564e-06
172973,172974,172973,345947,88.21407103538513,3.374100107905853e-06
173173,173174,173173,346347,88.3344419002533,3.37352526932218e-06
173373,173374,173373,346747,88.46120500564575,3.372819970962153e-06
173574,173575,173574,347149,88.5717089176178,3.3721750902713298e-06
173774,173775,173774,347549,88.68049001693726,3.3714706506108707e-06
173974,173975,173974,347949,88.83451104164124,3.370860532882936e-06
174174,174175,174174,348349,88.95465016365051,3.370212253199084e-06
174374,174375,174374,348749,89.08841109275818,3.3695445575166e-06
174575,174576,174575,349151,89.19369006156921,3.368887968672079e-06
174775,174776,174775,349551,89.30470490455627,3.3682047008774316e-06
174975,174976,174975,349951,89.42561411857605,3.367564154279671e-06
175175,175176,175175,350351,89.56946396827698,3.3669485454626686e-06
175375,175376,175375,350751,89.72860789299011,3.366281638626052e-06
175576,175577,175576,351153,89.83069801330566,3.3656151729741273e-06
175776,175777,175776,351553,89.92696905136108,3.3650546492546464e-06
175976,175977,175976,351953,90.01978492736816,3.3643535442588354e-06
176176,176177,176176,352353,90.11235809326172,3.3637086342624873e-06
176376,176377,176376,352753,90.22169017791748,3.363109537758372e-06
176577,176578,176577,353155,90.31638693809509,3.3624978655769054e-06
176777,176778,176777,353555,90.41806197166443,3.3617900914369723e-06
176977,176978,176977,353955,90.51583504676819,3.3611699055292966e-06
177177,177178,177177,354355,90.61724996566772,3.360552755127972e-06
177377,177378,177377,354755,90.74362111091614,3.3599091827120814e-06
177578,177579,177578,355157,90.87839317321777,3.3592230072068913e-06
177778,177779,177778,355557,91.01897311210632,3.358540831131648e-06
177978,177979,177978,355957,91.15695786476135,3.3579036857553855e-06
178178,178179,178178,356357,91.2556369304657,3.357255515194151e-06
178378,178379,178378,356757,91.36409997940063,3.3565629603326405e-06
178579,178580,178579,357159,91.50692820549011,3.356044927325285e-06
178779,178780,178779,357559,91.65913605690002,3.3552906279575177e-06
178979,178980,178979,357959,91.7627329826355,3.354654590387562e-06
179179,179180,179179,358359,91.86067199707031,3.3540145671172687e-06
179379,179380,179379,358759,91.9573540687561,3.3534061305991415e-06
179580,179581,179580,359161,92.05357098579407,3.3527393655184977e-06
179780,179781,179780,359561,92.15118622779846,3.3521298543957716e-06
179980,179981,179980,359961,92.24879884719849,3.3515517004098762e-06
180180,180181,180180,360361,92.34737706184387,3.350844153883206e-06
180380,180381,180380,360761,92.44541907310486,3.350250965202778e-06
180581,180582,180581,361163,92.6175742149353,3.349539123676289e-06
180781,180782,180781,361563,92.79039883613586,3.3488541884208035e-06
180981,180982,180981,361963,93.02943992614746,3.348261176514396e-06
181181,181182,181181,362363,93.25762104988098,3.347579497542345e-06
181381,181382,181381,362763,93.46082305908203,3.3469339322649455e-06
181582,181583,181582,363165,93.68392491340637,3.346320720681804e-06
181782,181783,181782,363565,93.88377499580383,3.345695141641126e-06
181982,181983,181982,363965,94.10338187217712,3.345031785873872e-06
182182,182183,182182,364365,94.26099300384521,3.3444012427202306e-06
182382,182383,182382,364765,94.47114586830139,3.3437329965697242e-06
182583,182584,182583,365167,94.63372302055359,3.3432315057821984e-06
182783,182784,182783,365567,94.7783579826355,3.3424697200203775e-06
182983,182984,182983,365967,94.91957712173462,3.3418072335729596e-06
183183,183184,183183,366367,95.0609860420227,3.3412012115310623e-06
183383,183384,183383,366767,95.19886517524719,3.340525883947471e-06
183584,183585,183584,367169,95.3376088142395,3.3399139620384896e-06
183784,183785,183784,367569,95.48006916046143,3.339290543959559e-06
183984,183985,183984,367969,95.6169068813324,3.3386055654649744e-06
184184,184185,184184,368369,95.75215601921082,3.3380268300804425e-06
184384,184385,184384,368769,95.88416719436646,3.3373190201738643e-06
184585,184586,184585,369171,96.0176329612732,3.336809403604226e-06
184785,184786,184785,369571,96.15019488334656,3.3360265989773456e-06
184985,184986,184985,369971,96.28283905982971,3.3354472901500613e-06
185185,185186,185185,370371,96.41452598571777,3.3347707424439878e-06
185385,185386,185385,370771,96.54717206954956,3.334286188686744e-06
185586,185587,185586,371173,96.67994117736816,3.3336551860262184e-06
185786,185787,185786,371573,96.81164479255676,3.332894296914425e-06
185986,185987,185986,371973,96.94526696205139,3.332280134855741e-06
186186,186187,186186,372373,97.07758402824402,3.3315978112037023e-06
186386,186387,186386,372773,97.20597815513611,3.330934864024138e-06
186587,186588,186587,373175,97.33349084854126,3.3302963769696974e-06
186787,186788,186787,373575,97.46547102928162,3.329680423230011e-06
186987,186988,186987,373975,97.6000440120697,3.3290100396817725e-06
187187,187188,187187,374375,97.72885394096375,3.3284266386005066e-06
187387,187388,187387,374775,97.85769319534302,3.3277224848510946e-06
187588,187589,187588,375177,97.98953914642334,3.327182233113577e-06
187788,187789,187788,375577,98.11994218826294,3.32649268491151e-06
187988,187989,187988,375977,98.2512149810791,3.3258127152538236e-06
188188,188189,188188,376377,98.3833909034729,3.325171560250952e-06
188388,188389,188388,376777,98.51320290565491,3.3246988841601044e-06
188589,188590,188589,377179,98.64458012580872,3.3239022829689867e-06
188789,188790,188789,377579,98.77505898475647,3.3233112026639262e-06
188989,188990,188989,377979,98.90650606155396,3.3226153634903792e-06
189189,189190,189189,378379,99.03715395927429,3.3219782722871176e-06
189389,189390,189389,378779,99.1705892086029,3.3215512432829327e-06
189590,189591,189590,379181,99.30200815200806,3.3207039505051247e-06
189790,189791,189790,379581,99.43993282318115,3.320065171092034e-06
189990,189991,189990,379981,99.5920250415802,3.319457993469332e-06
190190,190191,190190,380381,99.73626112937927,3.318869819007809e-06
190390,190391,190390,380781,99.88042211532593,3.3181900806196383e-06
190591,190592,190591,381183,100.0255401134491,3.3175315945672974e-06
190791,190792,190791,381583,100.2519862651825,3.3168980669266286e-06
190991,190992,190991,381983,100.47894501686096,3.3162627023978704e-06
191191,191192,191191,382383,100.64531302452087,3.3156389721718295e-06
191391,191392,191391,382783,100.8662462234497,3.3150104793049094e-06
191592,191593,191592,383185,101.01458716392517,3.314355621055969e-06
191792,191793,191792,383585,101.17182612419128,3.3137832187968524e-06
191992,191993,191992,383985,101.33043909072876,3.3131101559246675e-06
192192,192193,192192,384385,101.47556805610657,3.3124726124379095e-06
192392,192393,192392,384785,101.6245949268341,3.3118468889391635e-06
192593,192594,192593,385187,101.77484583854675,3.3112598741459983e-06
192793,192794,192793,385587,101.91741418838501,3.310589778153652e-06
192993,192994,192993,385987,102.06255602836609,3.3099617171187286e-06
193193,193194,193193,386387,102.2122311592102,3.309325277507578e-06
193393,193394,193393,386787,102.35639119148254,3.308688425381222e-06
193594,193595,193594,387189,102.50137710571289,3.3081905701703216e-06
193794,193795,193794,387589,102.64424705505371,3.307494560084455e-06
193994,193995,193994,387989,102.78581094741821,3.3068319216605577e-06
194194,194195,194194,388389,102.92579102516174,3.3061964692855746e-06
194394,194395,194394,388789,103.06817102432251,3.3055793426945365e-06
194595,194596,194595,389191,103.21387100219727,3.3050041782001423e-06
194795,194796,194795,389591,103.3535668849945,3.3042669867422242e-06
194995,194996,194995,389991,103.49243688583374,3.303642429415485e-06
195195,195196,195195,390391,103.62884092330933,3.3029945056986474e-06
195395,195396,195395,390791,103.7712790966034,3.3023578143166874e-06
195596,195597,195596,391193,103.90990614891052,3.301709350255027e-06
195796,195797,195796,391593,104.04524993896484,3.301125447554811e-06
195996,195997,195996,391993,104.18705296516418,3.300442308385055e-06
196196,196197,196196,392393,104.32571482658386,3.2998402298932846e-06
196396,196397,196396,392793,104.4634599685669,3.2992563449047137e-06
196597,196598,196597,393195,104.60139584541321,3.2986100697137956e-06
196797,196798,196797,393595,104.73679614067078,3.2979295409922413e-06
196997,196998,196997,393995,104.87557291984558,3.297295796262986e-06
197197,197198,197197,394395,105.02048707008362,3.296665564859316e-06
197397,197398,197397,394795,105.15401315689087,3.296059796886112e-06
197598,197599,197598,395197,105.29481792449951,3.295385729088287e-06
197798,197799,197798,395597,105.43347597122192,3.2947669303936944e-06
197998,197999,197998,395997,105.58395481109619,3.2941387721313485e-06
198198,198199,198198,396397,105.71854400634766,3.293536489326479e-06
198398,198399,198398,396797,105.8626868724823,3.2929934109579766e-06
198599,198600,198599,397199,106.00780010223389,3.2923666886425277e-06
198799,198800,198799,397599,106.14717888832092,3.2916220904989886e-06
198999,199000,198999,397999,106.28946495056152,3.2909945986226353e-06
199199,199200,199199,398399,106.42613387107849,3.2903488078438487e-06
199399,199400,199399,398799,106.56055402755737,3.289723177103505e-06
199600,199601,199600,399201,106.74682593345642,3.2890853061528397e-06
199800,199801,199800,399601,107.0596330165863,3.288488741848778e-06
200000,200001,200000,400001,107.24130702018738,3.287916130847992e-06


==> plot_data/bilinear_matrix_game_n500/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.001096963882446289,2.018959020339561
100,201,200,401,0.12761402130126953,0.04084193889187754
200,401,400,801,0.24407100677490234,0.01555572904704933
300,601,600,1201,0.3618738651275635,0.008941559671892264
400,801,800,1601,0.5734660625457764,0.005957710393872965
501,1003,1002,2005,0.7021570205688477,0.004080388626738635
601,1203,1202,2405,0.8251359462738037,0.003044183482286378
701,1403,1402,2805,0.9428930282592773,0.00247078219342337
801,1603,1602,3205,1.071336030960083,0.002022425653118514
901,1803,1802,3605,1.2060868740081787,0.0017090990324214828
1001,2003,2002,4005,1.3234241008758545,0.0014375084752964995
1101,2203,2202,4405,1.4424350261688232,0.0012047380988628406
1201,2403,2402,4805,1.5759758949279785,0.001000692926912849
1301,2603,2602,5205,1.6909470558166504,0.0008161398070111659
1401,2803,2802,5605,1.817399024963379,0.0007105240339073027
1502,3005,3004,6009,1.9883739948272705,0.0006406047458752685
1602,3205,3204,6409,2.113914966583252,0.0005873580809235912
1702,3405,3404,6809,2.2286458015441895,0.0005382536666146199
1802,3605,3604,7209,2.34254789352417,0.0004953501567577407
1902,3805,3804,7609,2.462355852127075,0.00046283265676205554
2002,4005,4004,8009,2.5771610736846924,0.0004308549629022895
2102,4205,4204,8409,2.6892149448394775,0.0003999154365291184
2202,4405,4404,8809,2.8060190677642822,0.00037725255875169743
2302,4605,4604,9209,2.9175941944122314,0.0003527435669886361
2402,4805,4804,9609,3.033135175704956,0.0003335273689751663
2503,5007,5006,10013,3.145364999771118,0.00031945940005734464
2603,5207,5206,10413,3.2616031169891357,0.00030878973556726564
2703,5407,5406,10813,3.381549119949341,0.0003000156905100278
2803,5607,5606,11213,3.507230043411255,0.00029252572517975546
2903,5807,5806,11613,3.635338068008423,0.00028541420036607454
3003,6007,6006,12013,3.7633018493652344,0.0002780152490870146
3103,6207,6206,12413,3.8923110961914062,0.00027195002345469855
3203,6407,6406,12813,4.032411813735962,0.00026673775102073016
3303,6607,6606,13213,4.160904884338379,0.00026209269718888097
3403,6807,6806,13613,4.288547992706299,0.00025787167822761395
3504,7009,7008,14017,4.412109136581421,0.00025394578198297755
3604,7209,7208,14417,4.537891149520874,0.00025011718889721537
3704,7409,7408,14817,4.669328927993774,0.0002467056013739032
3804,7609,7608,15217,4.807438135147095,0.00024351263461413038
3904,7809,7808,15617,4.935776948928833,0.00024048591179458707
4004,8009,8008,16017,5.0740790367126465,0.00023752401694437778
4104,8209,8208,16417,5.213096857070923,0.00023457721923087589
4204,8409,8408,16817,5.316133975982666,0.00023189293501112748
4304,8609,8608,17217,5.406888961791992,0.00022910798042041975
4404,8809,8808,17617,5.49542498588562,0.00022619918421695374
4505,9011,9010,18021,5.580489873886108,0.0002230343272817675
4605,9211,9210,18421,5.669863939285278,0.00022034767502957447
4705,9411,9410,18821,5.756553888320923,0.0002178537931555071
4805,9611,9610,19221,5.8356359004974365,0.00021549280886485868
4905,9811,9810,19621,5.918337106704712,0.00021323705999951907
5005,10011,10010,20021,6.002753973007202,0.00021107038667084828
5105,10211,10210,20421,6.103009939193726,0.00020898191834835915
5205,10411,10410,20821,6.193850994110107,0.0002069636366998869
5305,10611,10610,21221,6.277092933654785,0.00020500924417355266
5405,10811,10810,21621,6.358474016189575,0.00020311357261230275
5506,11013,11012,22025,6.441426992416382,0.00020125409421659746
5606,11213,11212,22425,6.52184796333313,0.000199463812585603
5706,11413,11412,22825,6.608471155166626,0.00019772072266799426
5806,11613,11612,23225,6.698142051696777,0.00019602185970323322
5906,11813,11812,23625,6.781621932983398,0.00019436456045111267
6006,12013,12012,24025,6.869600057601929,0.00019226895881548032
6106,12213,12212,24425,6.955971002578735,0.00018981336384564818
6206,12413,12412,24825,7.039137125015259,0.00018778452212550104
6306,12613,12612,25225,7.1226561069488525,0.00018589168393157325
6406,12813,12812,25625,7.205045938491821,0.00018405691086032967
6507,13015,13014,26029,7.289658784866333,0.00018229450115027232
6607,13215,13214,26429,7.376216173171997,0.00018061323138483316
6707,13415,13414,26829,7.46609902381897,0.00017896837070119164
6807,13615,13614,27229,7.558402061462402,0.00017670539366986823
6907,13815,13814,27629,7.649850845336914,0.00017394478665026857
7007,14015,14014,28029,7.731376886367798,0.00017182380289514751
7107,14215,14214,28429,7.814044952392578,0.00016995140199686445
7207,14415,14414,28829,7.89528489112854,0.00016822996598922252
7307,14615,14614,29229,7.977820873260498,0.00016600502050577174
7407,14815,14814,29629,8.066671133041382,0.00016417365369737495
7508,15017,15016,30033,8.16715383529663,0.00016248289306673215
7608,15217,15216,30433,8.261332988739014,0.00016090886540011637
7708,15417,15416,30833,8.347661972045898,0.0001588388697985169
7808,15617,15616,31233,8.440347909927368,0.00015716504752308173
7908,15817,15816,31633,8.525253057479858,0.00015560807575707016
8008,16017,16016,32033,8.60353398323059,0.0001528670951392979
8108,16217,16216,32433,8.677960872650146,0.0001508824226984641
8208,16417,16416,32833,8.75490403175354,0.00014869762396062543
8308,16617,16616,33233,8.831784963607788,0.00014660531424563205
8408,16817,16816,33633,8.907333850860596,0.00014472799576799907
8509,17019,17018,34037,8.987329006195068,0.00014295922339428892
8609,17219,17218,34437,9.066649198532104,0.0001412736273534982
8709,17419,17418,34837,9.146150827407837,0.0001396714101891978
8809,17619,17618,35237,9.220611095428467,0.00013813795600318
8909,17819,17818,35637,9.300578117370605,0.00013538373808574897
9009,18019,18018,36037,9.381643056869507,0.00013331524081584936
9109,18219,18218,36437,9.46270203590393,0.0001315176266269928
9209,18419,18418,36837,9.53578805923462,0.00012838146992159456
9309,18619,18618,37237,9.61345100402832,0.0001260062401086033
9409,18819,18818,37637,9.691370964050293,0.000123989736577564
9510,19021,19020,38041,9.76991319656372,0.0001221400303066318
9610,19221,19220,38441,9.845095872879028,0.0001204386966298002
9710,19421,19420,38841,9.917457818984985,0.00011847239407814625
9810,19621,19620,39241,9.993470907211304,0.00011669918825553777
9910,19821,19820,39641,10.07895302772522,0.00011274641903217324
10010,20021,20020,40041,10.155710935592651,0.00011039424919270669
10110,20221,20220,40441,10.230703830718994,0.00010842101331861896
10210,20421,20420,40841,10.312434911727905,0.0001056460432049642
10310,20621,20620,41241,10.391633987426758,0.0001034347785040179
10410,20821,20820,41641,10.471705198287964,0.00010121426707386297
10511,21023,21022,42045,10.551375150680542,9.88379844340756e-05
10611,21223,21222,42445,10.623746156692505,9.691614316935306e-05
10711,21423,21422,42845,10.695191144943237,9.51729702356169e-05
10811,21623,21622,43245,10.768929958343506,9.355874460556968e-05
10911,21823,21822,43645,10.838359117507935,9.195903659656644e-05
11011,22023,22022,44045,10.9112389087677,9.044062572871737e-05
11111,22223,22222,44445,10.9878249168396,8.760072395653058e-05
11211,22423,22422,44845,11.063947916030884,8.501766878337613e-05
11311,22623,22622,45245,11.14454197883606,8.292729869838731e-05
11411,22823,22822,45645,11.220165967941284,8.10564411007725e-05
11512,23025,23024,46049,11.293896913528442,7.89596690741875e-05
11612,23225,23224,46449,11.370150804519653,7.709389597231927e-05
11712,23425,23424,46849,11.45893406867981,7.544918173016605e-05
11812,23625,23624,47249,11.55593490600586,7.397387281337675e-05
11912,23825,23824,47649,11.664345026016235,7.25963281164493e-05
12012,24025,24024,48049,11.774802923202515,7.129342706426366e-05
12112,24225,24224,48449,11.88359808921814,6.997551128540555e-05
12212,24425,24424,48849,11.99154782295227,6.870086322848533e-05
12312,24625,24624,49249,12.089431047439575,6.749927088782142e-05
12412,24825,24824,49649,12.19192910194397,6.532043439414624e-05
12513,25027,25026,50053,12.31520700454712,6.377417764162247e-05
12613,25227,25226,50453,12.4426429271698,6.241931681348971e-05
12713,25427,25426,50853,12.590233087539673,6.117000796872597e-05
12813,25627,25626,51253,12.708111763000488,5.9999357950401774e-05
12913,25827,25826,51653,12.784279108047485,5.8892075906161434e-05
13013,26027,26026,52053,12.860136985778809,5.783806989101728e-05
13113,26227,26226,52453,12.934285163879395,5.683013725086848e-05
13213,26427,26426,52853,13.010757207870483,5.586287849136061e-05
13313,26627,26626,53253,13.08290410041809,5.493210368684028e-05
13413,26827,26826,53653,13.154614925384521,5.40344745752552e-05
13514,27029,27028,54057,13.226295948028564,5.315874701548238e-05
13614,27229,27228,54457,13.297316789627075,5.231999088587542e-05
13714,27429,27428,54857,13.367642164230347,5.150748953360285e-05
13814,27629,27628,55257,13.440670013427734,5.071961773190266e-05
13914,27829,27828,55657,13.511812210083008,4.9954964822641746e-05
14014,28029,28028,56057,13.587191104888916,4.9212291176279406e-05
14114,28229,28228,56457,13.666639804840088,4.8490495271269185e-05
14214,28429,28428,56857,13.87378191947937,4.778858852014829e-05
14314,28629,28628,57257,13.972169876098633,4.710567581298244e-05
14414,28829,28828,57657,14.052112817764282,4.6440940328542634e-05
14515,29031,29030,58061,14.130964994430542,4.5787244079736674e-05
14615,29231,29230,58461,14.214099884033203,4.515683226577822e-05
14715,29431,29430,58861,14.293139934539795,4.454250253990974e-05
14815,29631,29630,59261,14.368993997573853,4.394365350429401e-05
14915,29831,29830,59661,14.445281028747559,4.335972145555563e-05
15015,30031,30030,60061,14.53045392036438,4.279017615475833e-05
15115,30231,30230,60461,14.612350940704346,4.2234517292302766e-05
15215,30431,30430,60861,14.690605163574219,4.169227150309635e-05
15315,30631,30630,61261,14.767595052719116,4.116298982875498e-05
15415,30831,30830,61661,14.84438705444336,4.064624553921866e-05
15516,31033,31032,62065,14.920983076095581,4.013664605096901e-05
15616,31233,31232,62465,14.998863935470581,3.96438916138613e-05
15716,31433,31432,62865,15.075066089630127,3.916250645932755e-05
15816,31633,31632,63265,15.149865865707397,3.8692136325430465e-05
15916,31833,31832,63665,15.223530054092407,3.823244181240052e-05
16016,32033,32032,64065,15.296606063842773,3.778309738033774e-05
16116,32233,32232,64465,15.370474100112915,3.7343790450688504e-05
16216,32433,32432,64865,15.449031829833984,3.69142205982145e-05
16316,32633,32632,65265,15.528342008590698,3.6494098819374294e-05
16416,32833,32832,65665,15.601690769195557,3.6083146870131576e-05
16517,33035,33034,66069,15.675189971923828,3.5677120231280035e-05
16617,33235,33234,66469,15.749475002288818,3.528379843960052e-05
16717,33435,33434,66869,15.828022003173828,3.4898868073149153e-05
16817,33635,33634,67269,15.908409118652344,3.452208846989514e-05
16917,33835,33834,67669,16.004122972488403,3.4153227173809356e-05
17017,34035,34034,68069,16.09199094772339,3.379205954143965e-05
17117,34235,34234,68469,16.17581009864807,3.3438368377594996e-05
17217,34435,34434,68869,16.25357484817505,3.309194359746961e-05
17317,34635,34634,69269,16.334832906723022,3.2752581913295634e-05
17417,34835,34834,69669,16.415905952453613,3.242008654192568e-05
17518,35037,35036,70073,16.49494194984436,3.2091041818962486e-05
17618,35237,35236,70473,16.572021007537842,3.177177739504206e-05
17718,35437,35436,70873,16.65629482269287,3.145882356187534e-05
17818,35637,35636,71273,16.733814001083374,3.115200705127862e-05
17918,35837,35836,71673,16.807672023773193,3.085115989694329e-05
18018,36037,36036,72073,16.882555961608887,3.055611923573243e-05
18118,36237,36236,72473,16.95915198326111,3.0266727121420946e-05
18218,36437,36436,72873,17.033157110214233,2.998283034703666e-05
18318,36637,36636,73273,17.106882095336914,2.9704280278715254e-05
18418,36837,36836,73673,17.18053889274597,2.9430932697111267e-05
18519,37039,37038,74077,17.252413034439087,2.9159989898597117e-05
18619,37239,37238,74477,17.325382947921753,2.8896680138948832e-05
18719,37439,37438,74877,17.397274017333984,2.8638163927325157e-05
18819,37639,37638,75277,17.469266891479492,2.838431330815558e-05
18919,37839,37838,75677,17.54068088531494,2.8135004055142335e-05
19019,38039,38038,76077,17.610975980758667,2.7890115554991762e-05
19119,38239,38238,76477,17.68160104751587,2.7649530692710136e-05
19219,38439,38438,76877,17.756972074508667,2.7413135744249717e-05
19319,38639,38638,77277,17.82768201828003,2.7180820271181197e-05
19419,38839,38838,77677,17.89791488647461,2.6952477022695076e-05
19520,39041,39040,78081,17.97134304046631,2.6725776274959876e-05
19620,39241,39240,78481,18.043089866638184,2.6505105158808064e-05
19720,39441,39440,78881,18.113878965377808,2.6288101721943395e-05
19820,39641,39640,79281,18.189677000045776,2.60746705615014e-05
19920,39841,39840,79681,18.27058696746826,2.5864719015414138e-05
20020,40041,40040,80081,18.34655213356018,2.5658157080510214e-05
20120,40241,40240,80481,18.43445611000061,2.5454897336755517e-05
20220,40441,40440,80881,18.519476890563965,2.5254854872420898e-05
20320,40641,40640,81281,18.604310035705566,2.5057947211617455e-05
20420,40841,40840,81681,18.6878559589386,2.4864094243831293e-05
20521,41043,41042,82085,18.77606511116028,2.4671324172818473e-05
20621,41243,41242,82485,18.850317001342773,2.4483378027808908e-05
20721,41443,41442,82885,18.923684120178223,2.429825905215031e-05
20821,41643,41642,83285,18.999311208724976,2.411589596343249e-05
20921,41843,41842,83685,19.072793006896973,2.3936219526962322e-05
21021,42043,42042,84085,19.146358966827393,2.375916249582231e-05
21121,42243,42242,84485,19.221683979034424,2.358465955640318e-05
21221,42443,42442,84885,19.295365810394287,2.3412647271865886e-05
21321,42643,42642,85285,19.36719012260437,2.3243064029661924e-05
21421,42843,42842,85685,19.43897294998169,2.307584999029077e-05
21522,43045,43044,86089,19.511658906936646,2.290930948446167e-05
21622,43245,43244,86489,19.583112001419067,2.274668343669633e-05
21722,43445,43444,86889,19.65372586250305,2.2586256669867326e-05
21822,43645,43644,87289,19.725353956222534,2.2427975960148327e-05
21922,43845,43844,87689,19.79776406288147,2.2271789617417764e-05
22022,44045,44044,88089,19.86985492706299,2.2117647441859577e-05
22122,44245,44244,88489,19.95303511619568,2.1965500681564148e-05
22222,44445,44444,88889,20.042757987976074,2.1815301990555972e-05
22322,44645,44644,89289,20.14317488670349,2.1667005389170224e-05
22422,44845,44844,89689,20.22169589996338,2.1520566223945708e-05
22523,45047,45046,90093,20.298234939575195,2.137450389743613e-05
22623,45247,45246,90493,20.37393307685852,2.1231668274742093e-05
22723,45447,45446,90893,20.450881004333496,2.109056331098932e-05
22823,45647,45646,91293,20.523797035217285,2.095114930112278e-05
22923,45847,45846,91693,20.59470009803772,2.0813387685584392e-05
23023,46047,46046,92093,20.666278839111328,2.067724101748545e-05
23123,46247,46246,92493,20.739521026611328,2.054267293063988e-05
23223,46447,46446,92893,20.835583925247192,2.040964810749064e-05
23323,46647,46646,93293,20.90951919555664,2.0278132248572443e-05
23423,46847,46846,93693,20.9794180393219,2.014809204346726e-05
23524,47049,47048,94097,21.048605918884277,2.0018216353502114e-05
23624,47249,47248,94497,21.117487907409668,1.989104529704416e-05
23724,47449,47448,94897,21.187855005264282,1.9765255307275363e-05
23824,47649,47648,95297,21.256896018981934,1.9640816754702152e-05
23924,47849,47848,95697,21.323410034179688,1.9517700861296387e-05
24024,48049,48048,96097,21.393530130386353,1.9395879674889236e-05
24124,48249,48248,96497,21.478386878967285,1.9275326045535996e-05
24224,48449,48448,96897,21.5487859249115,1.9156013600908175e-05
24324,48649,48648,97297,21.618031978607178,1.9037916723550638e-05
24424,48849,48848,97697,21.68618607521057,1.8921010528517207e-05
24525,49051,49050,98101,21.755781888961792,1.8804119255199948e-05
24625,49251,49250,98501,21.82394003868103,1.8689533904571334e-05
24725,49451,49450,98901,21.892395973205566,1.857606853538815e-05
24825,49651,49650,99301,21.964552879333496,1.846370098658152e-05
24925,49851,49850,99701,22.032359838485718,1.835240972575939e-05
25025,50051,50050,100101,22.100332021713257,1.8242173830892025e-05
25125,50251,50250,100501,22.16816997528076,1.8132972971845767e-05
25225,50451,50450,100901,22.235920906066895,1.8024787392688152e-05
25325,50651,50650,101301,22.304487943649292,1.791759789366019e-05
25425,50851,50850,101701,22.378192901611328,1.7811385815375412e-05
25526,51053,51052,102105,22.466506958007812,1.7705085278162808e-05
25626,51253,51252,102505,22.541590929031372,1.7600783470369335e-05
25726,51453,51452,102905,22.61687183380127,1.749740601403757e-05
25826,51653,51652,103305,22.688760995864868,1.7394936255609e-05
25926,51853,51852,103705,22.7609920501709,1.729335800409566e-05
26026,52053,52052,104105,22.83814287185669,1.7192655517201312e-05
26126,52253,52252,104505,22.915133953094482,1.7092813487563866e-05
26226,52453,52452,104905,22.989957094192505,1.6993817030214183e-05
26326,52653,52652,105305,23.05929398536682,1.68956516684544e-05
26426,52853,52852,105705,23.127636909484863,1.6798303322708575e-05
26527,53055,53054,106109,23.200187921524048,1.670079685866953e-05
26627,53255,53254,106509,23.271903038024902,1.660504966524333e-05
26727,53455,53454,106909,23.34390878677368,1.6510079380238825e-05
26827,53655,53654,107309,23.415092945098877,1.641587339620174e-05
26927,53855,53854,107709,23.488311052322388,1.6322419444874413e-05
27027,54055,54054,108109,23.559279203414917,1.622970558720964e-05
27127,54255,54254,108509,23.6304829120636,1.6137720202917003e-05
27227,54455,54454,108909,23.709583044052124,1.604645198133419e-05
27327,54655,54654,109309,23.786777019500732,1.5955889911033592e-05
27427,54855,54854,109709,23.861466884613037,1.5866023271890535e-05
27528,55057,55056,110113,23.934846878051758,1.5775953233158783e-05
27628,55257,55256,110513,24.008338928222656,1.568745311075853e-05
27728,55457,55456,110913,24.08047890663147,1.559961781625362e-05
27828,55657,55656,111313,24.150479793548584,1.5512437707874757e-05
27928,55857,55856,111713,24.221068143844604,1.5425903392593543e-05
28028,56057,56056,112113,24.29201102256775,1.5340005718320964e-05
28128,56257,56256,112513,24.362289905548096,1.525473576666453e-05
28228,56457,56456,112913,24.433223962783813,1.5170084845910363e-05
28328,56657,56656,113313,24.503427028656006,1.5086044483851001e-05
28428,56857,56856,113713,24.575226068496704,1.5002606421231444e-05
28529,57059,57058,114117,24.64724612236023,1.4918937141126023e-05
28629,57259,57258,114517,24.717171907424927,1.4836685543758747e-05
28729,57459,57458,114917,24.786906003952026,1.4755012605720003e-05
28829,57659,57658,115317,24.861464023590088,1.4673910858305012e-05
28929,57859,57858,115717,24.93104314804077,1.4593373014588697e-05
29029,58059,58058,116117,25.00850796699524,1.4513391965261338e-05
29129,58259,58258,116517,25.08350110054016,1.4433960771370196e-05
29229,58459,58458,116917,25.153981924057007,1.4355072660792616e-05
29329,58659,58658,117317,25.224217176437378,1.4276721022064467e-05
29429,58859,58858,117717,25.29456901550293,1.4198899400570339e-05
29530,59061,59060,118121,25.36618185043335,1.412083113709544e-05
29630,59261,59260,118521,25.438392162322998,1.4044055930350786e-05
29730,59461,59460,118921,25.508455991744995,1.3967792206863045e-05
29830,59661,59660,119321,25.57916808128357,1.3892034091469082e-05
29930,59861,59860,119721,25.667461156845093,1.3816775843772175e-05
30030,60061,60060,120121,25.825155019760132,1.3742011852258061e-05
30130,60261,60260,120521,25.90750479698181,1.3667736632245829e-05
30230,60461,60460,120921,25.981377124786377,1.3593944821175885e-05
30330,60661,60660,121321,26.053498029708862,1.3520631174841028e-05
30430,60861,60860,121721,26.123279809951782,1.3447790563785466e-05
30531,61063,61062,122125,26.195186853408813,1.3374696591499395e-05
30631,61263,61262,122525,26.26737403869629,1.3302791713261758e-05
30731,61463,61462,122925,26.338029146194458,1.323134509156123e-05
30831,61663,61662,123325,26.409916877746582,1.3160352024723339e-05
30931,61863,61862,123725,26.48111891746521,1.3089807910219068e-05
31031,62063,62062,124125,26.55295491218567,1.3019708241126746e-05
31131,62263,62262,124525,26.62286901473999,1.2950048603807798e-05
31231,62463,62462,124925,26.693433046340942,1.2880824674895394e-05
31331,62663,62662,125325,26.7625789642334,1.2812032218859102e-05
31431,62863,62862,125725,26.834033966064453,1.2743667084967246e-05
31532,63065,63064,126129,26.909325122833252,1.2675047910385669e-05
31632,63265,63264,126529,26.98162293434143,1.2607529470036943e-05
31732,63465,63464,126929,27.05293107032776,1.2540426347793953e-05
31832,63665,63664,127329,27.141531944274902,1.2473734709913572e-05
31932,63865,63864,127729,27.22516393661499,1.2407450796598108e-05
32032,64065,64064,128129,27.30821704864502,1.2341570918836015e-05
32132,64265,64264,128529,27.383866786956787,1.2276091457306583e-05
32232,64465,64464,128929,27.455891847610474,1.2211008859601882e-05
32332,64665,64664,129329,27.52599287033081,1.2146319638728943e-05
32432,64865,64864,129729,27.59622097015381,1.2082020371446252e-05
32533,65067,65066,130133,27.667299032211304,1.2017470510092746e-05
32633,65267,65266,130533,27.7378990650177,1.1953944940703191e-05
32733,65467,65466,130933,27.82461380958557,1.1890799385439199e-05
32833,65667,65666,131333,27.971014976501465,1.1828030657689164e-05
32933,65867,65866,131733,28.041895866394043,1.1765635626103807e-05
33033,66067,66066,132133,28.11245322227478,1.1703611212723357e-05
33133,66267,66266,132533,28.194426774978638,1.1641954391581306e-05
33233,66467,66466,132933,28.26665997505188,1.1580662187235834e-05
33333,66667,66666,133333,28.337690830230713,1.151973167320635e-05
33433,66867,66866,133733,28.40821409225464,1.145915997127233e-05
33534,67069,67068,134137,28.481445789337158,1.1398343880375843e-05
33634,67269,67268,134537,28.561541080474854,1.1338484869761771e-05
33734,67469,67468,134937,28.650254011154175,1.1278976282498303e-05
33834,67669,67668,135337,28.730575799942017,1.1219815419291802e-05
33934,67869,67868,135737,28.803237915039062,1.1160999622212621e-05
34034,68069,68068,136137,28.886374950408936,1.1102526274125163e-05
34134,68269,68268,136537,28.958348989486694,1.1044392797122087e-05
34234,68469,68468,136937,29.02831196784973,1.0986596652116044e-05
34334,68669,68668,137337,29.108270168304443,1.092913533714529e-05
34434,68869,68868,137737,29.214366912841797,1.087200638689396e-05
34535,69071,69070,138141,29.353482007980347,1.0814641039152443e-05
34635,69271,69270,138541,29.424020051956177,1.0758172826412265e-05
34735,69471,69470,138941,29.4968159198761,1.0702029768192477e-05
34835,69671,69670,139341,29.566255807876587,1.0646209535832354e-05
34935,69871,69870,139741,29.634788751602173,1.0590709832984052e-05
35035,70071,70070,140141,29.70313596725464,1.0535528394461525e-05
35135,70271,70270,140541,29.77219796180725,1.0480662985438994e-05
35235,70471,70470,140941,29.851051092147827,1.0426111400662178e-05
35335,70671,70670,141341,29.928076028823853,1.0371871463733768e-05
35435,70871,70870,141741,29.99859881401062,1.0317941026897855e-05
35536,71073,71072,142145,30.068323135375977,1.0263783283944533e-05
35636,71273,71272,142545,30.13632297515869,1.0210468554471236e-05
35736,71473,71472,142945,30.205604791641235,1.0157457022502795e-05
35836,71673,71672,143345,30.27677011489868,1.0104746646564005e-05
35936,71873,71872,143745,30.34517812728882,1.0052335410015979e-05
36036,72073,72072,144145,30.41482186317444,1.0000221320252732e-05
36136,72273,72272,144545,30.49792790412903,9.948402408870986e-06
36236,72473,72472,144945,30.566853046417236,9.896876730314829e-06
36336,72673,72672,145345,30.633946180343628,9.845642362438357e-06
36436,72873,72872,145745,30.714571952819824,9.794697404628907e-06
36537,73075,73074,146149,30.785908937454224,9.74353484946901e-06
36637,73275,73274,146549,30.854099988937378,9.693165944138935e-06
36737,73475,73474,146949,30.922213792800903,9.643080857668941e-06
36837,73675,73674,147349,30.99303102493286,9.593277773582359e-06
36937,73875,73874,147749,31.06166100502014,9.543754895089129e-06
37037,74075,74074,148149,31.129328966140747,9.494510445563372e-06
37137,74275,74274,148549,31.197998046875,9.445542666678655e-06
37237,74475,74474,148949,31.26694917678833,9.39684981854373e-06
37337,74675,74674,149349,31.338430881500244,9.348430179943802e-06
37437,74875,74874,149749,31.41509509086609,9.300282047109628e-06
37538,75077,75076,150153,31.485002040863037,9.251926307497324e-06
37638,75277,75276,150553,31.553173065185547,9.204318817428131e-06
37738,75477,75476,150953,31.632922887802124,9.156977808712949e-06
37838,75677,75676,151353,31.708256006240845,9.109901645389194e-06
37938,75877,75876,151753,31.77719497680664,9.06308870710001e-06
38038,76077,76076,152153,31.846298933029175,9.016537389877662e-06
38138,76277,76276,152553,31.914397954940796,8.97024610490771e-06
38238,76477,76476,152953,31.986521005630493,8.924213278269528e-06
38338,76677,76676,153353,32.05594491958618,8.878437350907728e-06
38438,76877,76876,153753,32.12362194061279,8.83291677849829e-06
38539,77079,77078,154157,32.19227194786072,8.787198639970328e-06
38639,77279,77278,154557,32.266266107559204,8.742186716186681e-06
38739,77479,77478,154957,32.3398699760437,8.69742558348526e-06
38839,77679,77678,155357,32.41372108459473,8.652913752906591e-06
38939,77879,77878,155757,32.48853302001953,8.608649748757887e-06
39039,78079,78078,156157,32.55872988700867,8.564632108607513e-06
39139,78279,78278,156557,32.62793493270874,8.520859381960493e-06
39239,78479,78478,156957,32.6964647769928,8.477330131968392e-06
39339,78679,78678,157357,32.76560401916504,8.434042933128069e-06
39439,78879,78878,157757,32.83546280860901,8.390996372740759e-06
39540,79081,79080,158161,32.90314078330994,8.347762179717916e-06
39640,79281,79280,158561,32.97943902015686,8.305195075779838e-06
39740,79481,79480,158961,33.05616998672485,8.262864427904646e-06
39840,79681,79680,159361,33.13908410072327,8.220768869818147e-06
39940,79881,79880,159761,33.2110059261322,8.178907046014787e-06
40040,80081,80080,160161,33.28960990905762,8.13727761196053e-06
40140,80281,80280,160561,33.38313603401184,8.095879234201466e-06
40240,80481,80480,160961,33.48282599449158,8.054710589422994e-06
40340,80681,80680,161361,33.560083866119385,8.013770365173272e-06
40440,80881,80880,161761,33.632901191711426,7.973057259006582e-06
40541,81083,81082,162165,33.71219778060913,7.93216624198212e-06
40641,81283,81282,162565,33.78965997695923,7.891905744237378e-06
40741,81483,81482,162965,33.863577127456665,7.85186850499992e-06
40841,81683,81682,163365,33.938737869262695,7.812053261607058e-06
40941,81883,81882,163765,34.01409196853638,7.772458760678725e-06
41041,82083,82082,164165,34.107768058776855,7.733083758506741e-06
41141,82283,82282,164565,34.30961585044861,7.693927020716855e-06
41241,82483,82482,164965,34.41290998458862,7.654987321654853e-06
41341,82683,82682,165365,34.49614906311035,7.616263445389694e-06
41441,82883,82882,165765,34.57344889640808,7.577754183968579e-06
41542,83085,83084,166169,34.6516637802124,7.539076454204235e-06
41642,83285,83284,166569,34.72819209098816,7.500994951635613e-06
41742,83485,83484,166969,34.87647008895874,7.4631244818936705e-06
41842,83685,83684,167369,34.98021101951599,7.425463871914123e-06
41942,83885,83884,167769,35.063727140426636,7.388011956974788e-06
42042,84085,84084,168169,35.13854908943176,7.35076758060331e-06
42142,84285,84284,168569,35.211276054382324,7.313729594061847e-06
42242,84485,84484,168969,35.283100843429565,7.2768968571314685e-06
42342,84685,84684,169369,35.35355806350708,7.24026823721206e-06
42442,84885,84884,169769,35.42340087890625,7.203842609448843e-06
42543,85087,85086,170173,35.49665594100952,7.16725763496288e-06
42643,85287,85286,170573,35.57561492919922,7.131236650136116e-06
42743,85487,85486,170973,35.6498339176178,7.095415318007942e-06
42843,85687,85686,171373,35.729480028152466,7.059792544354096e-06
42943,85887,85886,171773,35.80146312713623,7.0243672419622075e-06
43043,86087,86086,172173,35.87255907058716,6.989138331090712e-06
43143,86287,86286,172573,35.94755506515503,6.954104739154548e-06
43243,86487,86486,172973,36.017701864242554,6.9192654006023495e-06
43343,86687,86686,173373,36.08926701545715,6.884619256872231e-06
43443,86887,86886,173773,36.15984010696411,6.850165256685627e-06
43544,87089,87088,174177,36.23258399963379,6.815560687752278e-06
43644,87289,87288,174577,36.31043982505798,6.781489742640136e-06
43744,87489,87488,174977,36.38764500617981,6.747607816964063e-06
43844,87689,87688,175377,36.45941877365112,6.7139138864022474e-06
43944,87889,87888,175777,36.53039312362671,6.680406933143287e-06
44044,88089,88088,176177,36.60039496421814,6.647085946019172e-06
44144,88289,88288,176577,36.67127299308777,6.613949920010182e-06
44244,88489,88488,176977,36.74121022224426,6.58099785674499e-06
44344,88689,88688,177377,36.812865018844604,6.5482287641530055e-06
44444,88889,88888,177777,36.885605812072754,6.515641656444835e-06
44545,89091,89090,178181,36.95863199234009,6.482912403623686e-06
44645,89291,89290,178581,37.029573917388916,6.450688128178052e-06
44745,89491,89490,178981,37.0997200012207,6.4186429074786614e-06
44845,89691,89690,179381,37.17013502120972,6.386775780018332e-06
44945,89891,89890,179781,37.239691972732544,6.355085790635725e-06
45045,90091,90090,180181,37.309996128082275,6.323571989721938e-06
45145,90291,90290,180581,37.380481004714966,6.292233433956981e-06
45245,90491,90490,180981,37.46369791030884,6.261069185429767e-06
45345,90691,90690,181381,37.54446887969971,6.230078312059861e-06
45445,90891,90890,181781,37.6224639415741,6.199259887835986e-06
45546,91093,91092,182185,37.701570987701416,6.168307385898487e-06
45646,91293,91292,182585,37.77109885215759,6.137832804711906e-06
45746,91493,91492,182985,37.842074155807495,6.1075279183302e-06
45846,91693,91692,183385,37.91293692588806,6.077391822975231e-06
45946,91893,91892,183785,37.983055114746094,6.047423619766005e-06
46046,92093,92092,184185,38.05249905586243,6.017622416051659e-06
46146,92293,92292,184585,38.125706911087036,5.987987324065617e-06
46246,92493,92492,184985,38.201038122177124,5.958517461319691e-06
46346,92693,92692,185385,38.27179789543152,5.929211950894008e-06
46446,92893,92892,185785,38.34473180770874,5.900069920885861e-06
46547,93095,93094,186189,38.41503405570984,5.870801528813013e-06
46647,93295,93294,186589,38.490373849868774,5.841985478237522e-06
46747,93495,93494,186989,38.56064987182617,5.813330314928808e-06
46847,93695,93694,187389,38.63480186462402,5.784835187868471e-06
46947,93895,93894,187789,38.703763008117676,5.756499250526048e-06
47047,94095,94094,188189,38.77419400215149,5.7283216620927856e-06
47147,94295,94294,188589,38.844074964523315,5.7003015858583396e-06
47247,94495,94494,188989,38.9144549369812,5.672438190651915e-06
47347,94695,94694,189389,38.98704481124878,5.6447306499422615e-06
47447,94895,94894,189789,39.05746793746948,5.61717814195004e-06
47548,95097,95096,190193,39.12756395339966,5.589506643035452e-06
47648,95297,95296,190593,39.19454908370972,5.562263284700671e-06
47748,95497,95496,190993,39.26336193084717,5.535172514797879e-06
47848,95697,95696,191393,39.33214497566223,5.50823353060782e-06
47948,95897,95896,191793,39.400306940078735,5.48144553394883e-06
48048,96097,96096,192193,39.46723985671997,5.454807731632171e-06
48148,96297,96296,192593,39.53531789779663,5.428319334839365e-06
48248,96497,96496,192993,39.60313391685486,5.401979559216118e-06
48348,96697,96696,193393,39.66940116882324,5.375787625232161e-06
48448,96897,96896,193793,39.744767904281616,5.349742757503943e-06
48549,97099,97098,194197,39.816986083984375,5.323585935685384e-06
48649,97299,97298,194597,39.88421392440796,5.297834343902858e-06
48749,97499,97498,194997,39.95539712905884,5.272227511842524e-06
48849,97699,97698,195397,40.02338004112244,5.246764681542395e-06
48949,97899,97898,195797,40.09161901473999,5.22144510013245e-06
49049,98099,98098,196197,40.16041088104248,5.196268018480843e-06
49149,98299,98298,196597,40.22707200050354,5.171232691703259e-06
49249,98499,98498,196997,40.294589042663574,5.146338379849339e-06
49349,98699,98698,197397,40.364161014556885,5.121584346210965e-06
49449,98899,98898,197797,40.434096813201904,5.096969858858035e-06
49550,99101,99100,198201,40.50340509414673,5.072250131919366e-06
49650,99301,99300,198601,40.57938003540039,5.047913935088097e-06
49750,99501,99500,199001,40.65838003158569,5.023715105716969e-06
49850,99701,99700,199401,40.74133086204529,4.999652928508329e-06
49950,99901,99900,199801,40.81439208984375,4.975726691870215e-06
50050,100101,100100,200201,40.88902807235718,4.951935688293543e-06
50150,100301,100300,200601,40.96863794326782,4.928279214059409e-06
50250,100501,100500,201001,41.06242513656616,4.904756569533034e-06
50350,100701,100700,201401,41.1516318321228,4.881367059087401e-06
50450,100901,100900,201801,41.22422194480896,4.858109990902602e-06
50551,101103,101102,202205,41.302666902542114,4.834754087025463e-06
50651,101303,101302,202605,41.379855155944824,4.811761150684866e-06
50751,101503,101502,203005,41.45747518539429,4.788898597468498e-06
50851,101703,101702,203405,41.531347036361694,4.7661657510782e-06
50951,101903,101902,203805,41.602821826934814,4.7435619388122915e-06
51051,102103,102102,204205,41.67313885688782,4.721086491744434e-06
51151,102303,102302,204605,41.74377083778381,4.698738744567397e-06
51251,102503,102502,205005,41.821946144104004,4.67651803588588e-06
51351,102703,102702,205405,41.8944251537323,4.65442370798411e-06
51451,102903,102902,205805,41.964563846588135,4.632455106646605e-06
51552,103105,103104,206209,42.03250503540039,4.6103937754140965e-06
51652,103305,103304,206609,42.101747035980225,4.588675919869479e-06
51752,103505,103504,207009,42.16954493522644,4.56708184364518e-06
51852,103705,103704,207409,42.238028049468994,4.5456109068755234e-06
51952,103905,103904,207809,42.30637502670288,4.524262473038207e-06
52052,104105,104104,208209,42.377718925476074,4.50303590985631e-06
52152,104305,104304,208609,42.46031212806702,4.481930587629535e-06
52252,104505,104504,209009,42.5433669090271,4.4609458807438155e-06
52352,104705,104704,209409,42.617496967315674,4.44008116686596e-06
52452,104905,104904,209809,42.687257051467896,4.419335826924423e-06
52553,105107,105106,210213,42.759377002716064,4.398503576999496e-06
52653,105307,105306,210613,42.830195903778076,4.377996319994162e-06
52753,105507,105506,211013,42.9013090133667,4.357606594234406e-06
52853,105707,105706,211413,42.97286081314087,4.337333794270907e-06
52953,105907,105906,211813,43.043484926223755,4.317177317871906e-06
53053,106107,106106,212213,43.115062952041626,4.297136566234023e-06
53153,106307,106306,212613,43.1864697933197,4.277210943642991e-06
53253,106507,106506,213013,43.25796604156494,4.257399857657006e-06
53353,106707,106706,213413,43.32678198814392,4.237702719258374e-06
53453,106907,106906,213813,43.39454197883606,4.218118942136207e-06
53554,107109,107108,214217,43.469626903533936,4.198453801489868e-06
53654,107309,107308,214617,43.54593801498413,4.1790961215606555e-06
53754,107509,107508,215017,43.63023400306702,4.159850058205327e-06
53854,107709,107708,215417,43.70662498474121,4.140715038374712e-06
53954,107909,107908,215817,43.78087592124939,4.12169049185086e-06
54054,108109,108108,216217,43.85509991645813,4.102775851226692e-06
54154,108309,108308,216617,43.9396858215332,4.083970552582838e-06
54254,108509,108508,217017,44.01490783691406,4.065274034718134e-06
54354,108709,108708,217417,44.086764097213745,4.046685739693659e-06
54454,108909,108908,217817,44.15858197212219,4.028205112167068e-06
54555,109111,109110,218221,44.234851121902466,4.009648404477159e-06
54655,109311,109310,218621,44.31241488456726,3.991382522047146e-06
54755,109511,109510,219021,44.3857479095459,3.9732226543964645e-06
54855,109711,109710,219421,44.45734190940857,3.95516825846744e-06
54955,109911,109910,219821,44.52795100212097,3.937218793731326e-06
55055,110111,110110,220221,44.59768080711365,3.9193737228706324e-06
55155,110311,110310,220621,44.6673641204834,3.901632511197682e-06
55255,110511,110510,221021,44.74003195762634,3.883994627014341e-06
55355,110711,110710,221421,44.81431698799133,3.866459541242284e-06
55455,110911,110910,221821,44.88526201248169,3.849026727987626e-06
55556,111113,111112,222225,44.963114976882935,3.831522865416961e-06
55656,111313,111312,222625,45.033313035964966,3.814294039421805e-06
55756,111513,111512,223025,45.104944944381714,3.7971659193340194e-06
55856,111713,111712,223425,45.17578196525574,3.7801379897162253e-06
55956,111913,111912,223825,45.24748706817627,3.7632097383087628e-06
56056,112113,112112,224225,45.322311878204346,3.746380655818998e-06
56156,112313,112312,224625,45.39608097076416,3.7296502350543283e-06
56256,112513,112512,225025,45.47146916389465,3.7130179717656068e-06
56356,112713,112712,225425,45.54185199737549,3.6964833643197807e-06
56456,112913,112912,225825,45.610896825790405,3.680045913899004e-06
56557,113115,113114,226229,45.684041023254395,3.6635422025605246e-06
56657,113315,113314,226629,45.76325297355652,3.6472985387737856e-06
56757,113515,113514,227029,45.8371148109436,3.631150545658939e-06
56857,113715,113714,227429,45.90832996368408,3.6150977346360793e-06
56957,113915,113914,227829,45.98531794548035,3.5991396197010377e-06
57057,114115,114114,228229,46.06306004524231,3.5832757172888128e-06
57157,114315,114314,228629,46.13350987434387,3.5675055463678695e-06
57257,114515,114514,229029,46.20726704597473,3.5518286286233473e-06
57357,114715,114714,229429,46.27881097793579,3.5362444877194963e-06
57457,114915,114914,229829,46.35221290588379,3.520752650323909e-06
57558,115117,115116,230233,46.42676091194153,3.5051991071690087e-06
57658,115317,115316,230633,46.498636960983276,3.4898913768323703e-06
57758,115517,115516,231033,46.57248902320862,3.474674539149808e-06
57858,115717,115716,231433,46.64836883544922,3.4595481300296076e-06
57958,115917,115916,231833,46.72419309616089,3.444511688451795e-06
58058,116117,116116,232233,46.80020093917847,3.4295647549437967e-06
58158,116317,116316,232633,46.87156105041504,3.414706872755212e-06
58258,116517,116516,233033,46.94558596611023,3.3999375876989694e-06
58358,116717,116716,233433,47.02105712890625,3.3852564473989437e-06
58458,116917,116916,233833,47.09240913391113,3.370663002187943e-06
58559,117119,117118,234237,47.163968086242676,3.3560121814881122e-06
58659,117319,117318,234637,47.233680963516235,3.341593651901923e-06
58759,117519,117518,235037,47.30398201942444,3.327261477001474e-06
58859,117719,117718,235437,47.373003005981445,3.313015216356852e-06
58959,117919,117918,235837,47.445063829422,3.29885443130374e-06
59059,118119,118118,236237,47.51489782333374,3.2847786855520033e-06
59159,118319,118318,236637,47.587085008621216,3.270787545082869e-06
59259,118519,118518,237037,47.65963006019592,3.2568805777448162e-06
59359,118719,118718,237437,47.7319438457489,3.243057354221872e-06
59459,118919,118918,237837,47.80570101737976,3.229317446507438e-06
59560,119121,119120,238241,47.8811981678009,3.2155242764601247e-06
59660,119321,119320,238641,47.95652890205383,3.2019505491993925e-06
59760,119521,119520,239041,48.046530961990356,3.188458863532566e-06
59860,119721,119720,239441,48.14667892456055,3.1750488005229006e-06
59960,119921,119920,239841,48.22349214553833,3.1617199431699828e-06
60060,120121,120120,240241,48.29840898513794,3.148471876535181e-06
60160,120321,120320,240641,48.37248206138611,3.1353041875904403e-06
60260,120521,120520,241041,48.44804787635803,3.12221646560781e-06
60360,120721,120720,241441,48.522977113723755,3.109208301734977e-06
60460,120921,120920,241841,48.59606981277466,3.096279288879458e-06
60561,121123,121122,242245,48.673168897628784,3.0833009160880306e-06
60661,121323,121322,242645,48.74701905250549,3.0705297745346636e-06
60761,121523,121522,243045,48.82254481315613,3.057836571767367e-06
60861,121723,121722,243445,48.89572191238403,3.0452209085410903e-06
60961,121923,121922,243845,48.969276905059814,3.0326823878801493e-06
61061,122123,122122,244245,49.04455089569092,3.0202206151558014e-06
61161,122323,122322,244645,49.11736607551575,3.0078351968175384e-06
61261,122523,122522,245045,49.188942193984985,2.995525741793433e-06
61361,122723,122722,245445,49.260936975479126,2.983291860656169e-06
61461,122923,122922,245845,49.33193492889404,2.9711331660294383e-06
61562,123125,123124,246249,49.40277719497681,2.9589288098924783e-06
61662,123325,123324,246649,49.472355127334595,2.9469200756642875e-06
61762,123525,123524,247049,49.54762005805969,2.934985372665422e-06
61862,123725,123724,247449,49.62604284286499,2.9231243211627506e-06
61962,123925,123924,247849,49.698084115982056,2.9113365428115323e-06
62062,124125,124124,248249,49.77164912223816,2.8996216609782116e-06
62162,124325,124324,248649,49.84279918670654,2.8879793009363483e-06
62262,124525,124524,249049,49.91619396209717,2.876409090102088e-06
62362,124725,124724,249449,49.99341702461243,2.864910657114372e-06
62462,124925,124924,249849,50.06777501106262,2.853483632643486e-06
62563,125127,125126,250253,50.143357038497925,2.8420144466557163e-06
62663,125327,125326,250653,50.23497009277344,2.830729842905204e-06
62763,125527,125526,251053,50.3152859210968,2.819515546092488e-06
62863,125727,125726,251453,50.39330196380615,2.8083711939183947e-06
62963,125927,125926,251853,50.46758818626404,2.797296425574582e-06
63063,126127,126126,252253,50.53906512260437,2.7862908817192455e-06
63163,126327,126326,252653,50.6185040473938,2.775354205192744e-06
63263,126527,126526,253053,50.694839000701904,2.7644860399032016e-06
63363,126727,126726,253453,50.76990795135498,2.7536860318430737e-06
63463,126927,126926,253853,50.8443489074707,2.7429538284824577e-06
63564,127129,127128,254257,50.91617679595947,2.7321827708355152e-06
63664,127329,127328,254657,50.990731954574585,2.721585794767247e-06
63764,127529,127528,255057,51.062554121017456,2.711055572255011e-06
63864,127729,127728,255457,51.13549304008484,2.700591756681407e-06
63964,127929,127928,255857,51.206661224365234,2.6901940038882488e-06
64064,128129,128128,256257,51.2767870426178,2.6798619706745087e-06
64164,128329,128328,256657,51.347057819366455,2.6695953156258623e-06
64264,128529,128528,257057,51.41762614250183,2.659393699021787e-06
64364,128729,128728,257457,51.48976492881775,2.649256782559759e-06
64464,128929,128928,257857,51.55862307548523,2.639184229190856e-06
64565,129131,129130,258261,51.62944412231445,2.6290759409266197e-06
64665,129331,129330,258661,51.70014309883118,2.6191317449486765e-06
64765,129531,129530,259061,51.768963098526,2.6092509074161096e-06
64865,129731,129730,259461,51.83746790885925,2.5994330977607984e-06
64965,129931,129930,259861,51.906309843063354,2.589677986323251e-06
65065,130131,130130,260261,51.97751593589783,2.5799852454567913e-06
65165,130331,130330,260661,52.04592299461365,2.5703545484942893e-06
65265,130531,130530,261061,52.11480402946472,2.5607855706475568e-06
65365,130731,130730,261461,52.18163204193115,2.5512779882598767e-06
65465,130931,130930,261861,52.24852395057678,2.5418314792641497e-06
65566,131133,131132,262265,52.32625985145569,2.5323521709510194e-06
65666,131333,131332,262665,52.3963258266449,2.523027450649723e-06
65766,131533,131532,263065,52.47155785560608,2.5137628423610064e-06
65866,131733,131732,263465,52.54235100746155,2.5045580298119715e-06
65966,131933,131932,263865,52.62768793106079,2.4954126978385856e-06
66066,132133,132132,264265,52.70843505859375,2.4863265324961008e-06
66166,132333,132332,264665,52.78497314453125,2.4772992213185746e-06
66266,132533,132532,265065,52.87507104873657,2.468330453227136e-06
66366,132733,132732,265465,52.97519493103027,2.4594199184772105e-06
66466,132933,132932,265865,53.04699397087097,2.4505673088944696e-06
66567,133135,133134,266269,53.1208930015564,2.4416846569844214e-06
66667,133335,133334,266669,53.19413495063782,2.4329475486101967e-06
66767,133535,133534,267069,53.26772499084473,2.424267444997775e-06
66867,133735,133734,267469,53.339343786239624,2.415644042512235e-06
66967,133935,133934,267869,53.41228103637695,2.407077039411883e-06
67067,134135,134134,268269,53.4872100353241,2.398566135092775e-06
67167,134335,134334,268669,53.56065106391907,2.3901110302742894e-06
67267,134535,134534,269069,53.63433909416199,2.3817114267139655e-06
67367,134735,134734,269469,53.707239866256714,2.373367027660072e-06
67467,134935,134934,269869,53.78173804283142,2.3650775374344425e-06
67568,135137,135136,270273,53.853919982910156,2.3567605878678364e-06
67668,135337,135336,270673,53.925498962402344,2.3485805752968476e-06
67768,135537,135536,271073,53.998778104782104,2.3404545891950986e-06
67868,135737,135736,271473,54.07103991508484,2.3323823390859886e-06
67968,135937,135936,271873,54.1431097984314,2.324363535425193e-06
68068,136137,136136,272273,54.2176718711853,2.3163978898000402e-06
68168,136337,136336,272673,54.28940391540527,2.3084851152131723e-06
68268,136537,136536,273073,54.36292886734009,2.3006249257527494e-06
68368,136737,136736,273473,54.4419219493866,2.292817036715171e-06
68468,136937,136936,273873,54.51297307014465,2.28506116463904e-06
68569,137139,137138,274277,54.58465313911438,2.277280245826642e-06
68669,137339,137338,274677,54.65662217140198,2.269628074550235e-06
68769,137539,137538,275077,54.72842288017273,2.262027073533906e-06
68869,137739,137738,275477,54.79981207847595,2.2544769639386698e-06
68969,137939,137938,275877,54.86952090263367,2.246977468094862e-06
69069,138139,138138,276277,54.94379186630249,2.239528309248918e-06
69169,138339,138338,276677,55.01922607421875,2.232129211675099e-06
69269,138539,138538,277077,55.09207201004028,2.224779901255263e-06
69369,138739,138738,277477,55.16268587112427,2.217480104439679e-06
69469,138939,138938,277877,55.23352909088135,2.210229549177222e-06
69570,139141,139140,278281,55.30650281906128,2.2029561950037375e-06
69670,139341,139340,278681,55.37718892097473,2.195803796210658e-06
69770,139541,139540,279081,55.4523389339447,2.188699826214872e-06
69870,139741,139740,279481,55.526089906692505,2.1816440171058295e-06
69970,139941,139940,279881,55.60014486312866,2.1746361021918227e-06
70070,140141,140140,280281,55.67289400100708,2.1676758158810486e-06
70170,140341,140340,280681,55.74444603919983,2.160762893294456e-06
70270,140541,140540,281081,55.81593704223633,2.153897071094307e-06
70370,140741,140740,281481,55.88795495033264,2.1470780865682e-06
70470,140941,140940,281881,55.96220588684082,2.1403056783586055e-06
70571,141143,141142,282285,56.036673069000244,2.1335125582210985e-06
70671,141343,141342,282685,56.11044406890869,2.126832981776931e-06
70771,141543,141542,283085,56.18540000915527,2.1201992007846804e-06
70871,141743,141742,283485,56.26055288314819,2.1136109580559547e-06
70971,141943,141942,283885,56.33446979522705,2.1070679973443883e-06
71071,142143,142142,284285,56.4070200920105,2.100570063260819e-06
71171,142343,142342,284685,56.48858118057251,2.094116901446059e-06
71271,142543,142542,285085,56.567424058914185,2.087708259066037e-06
71371,142743,142742,285485,56.647247076034546,2.0813438834648194e-06
71471,142943,142942,285885,56.72894597053528,2.0750235232705427e-06
71572,143145,143144,286289,56.81772708892822,2.0686843828919825e-06
71672,143345,143344,286689,56.969274044036865,2.0624517383600515e-06
71772,143545,143544,287089,57.16792917251587,2.056262359115471e-06
71872,143745,143744,287489,57.25225496292114,2.050115997800982e-06
71972,143945,143944,287889,57.33186888694763,2.0440124083681556e-06
72072,144145,144144,288289,57.44246816635132,2.0379513453490074e-06
72172,144345,144344,288689,57.55598211288452,2.0319325641643383e-06
72272,144545,144544,289089,57.65483283996582,2.0259558216145032e-06
72372,144745,144744,289489,57.759860038757324,2.0200208753586987e-06
72472,144945,144944,289889,57.8575119972229,2.0141274837413022e-06
72573,145147,145146,290293,57.986648082733154,2.008217093332123e-06
72673,145347,145346,290693,58.10359811782837,2.002406499793463e-06
72773,145547,145546,291093,58.220020055770874,1.996636739963973e-06
72873,145747,145746,291493,58.37285304069519,1.9909075760700736e-06
72973,145947,145946,291893,58.51882004737854,1.985218771099692e-06
73073,146147,146146,292293,58.616738080978394,1.979570089524111e-06
73173,146347,146346,292693,58.70088601112366,1.9739612963998257e-06
73273,146547,146546,293093,58.78315997123718,1.9683921578082133e-06
73373,146747,146746,293493,58.86001801490784,1.9628624408575366e-06
73473,146947,146946,293893,58.945537090301514,1.9573719130255463e-06
73574,147149,147148,294297,59.03167009353638,1.951866023886824e-06
73674,147349,147348,294697,59.11124515533447,1.946453568571144e-06
73774,147549,147548,295097,59.18671989440918,1.9410796095815656e-06
73874,147749,147748,295497,59.26131296157837,1.9357439186554453e-06
73974,147949,147948,295897,59.33521509170532,1.930446268220333e-06
74074,148149,148148,296297,59.41333293914795,1.9251864315266883e-06
74174,148349,148348,296697,59.493890047073364,1.919964183130938e-06
74274,148549,148548,297097,59.56971192359924,1.9147792981028865e-06
74374,148749,148748,297497,59.65098285675049,1.9096315527452103e-06
74474,148949,148948,297897,59.733636140823364,1.904520723824285e-06
74575,149151,149150,298301,59.81791400909424,1.8993960326464324e-06
74675,149351,149350,298701,59.8901948928833,1.8943587350300446e-06
74775,149551,149550,299101,59.96285581588745,1.8893576883488883e-06
74875,149751,149750,299501,60.03399085998535,1.884392672963078e-06
74975,149951,149950,299901,60.10562610626221,1.879463470399839e-06
75075,150151,150150,300301,60.18236494064331,1.8745698629375028e-06
75175,150351,150350,300701,60.254727840423584,1.8697116340249785e-06
75275,150551,150550,301101,60.32468104362488,1.8648885677041297e-06
75375,150751,150750,301501,60.39591693878174,1.860100448892799e-06
75475,150951,150950,301901,60.4701669216156,1.8553470635185739e-06
75576,151153,151152,302305,60.57488203048706,1.850581183229221e-06
75676,151353,151352,302705,60.65757203102112,1.8458969680701343e-06
75776,151553,151552,303105,60.73555088043213,1.841246847050018e-06
75876,151753,151752,303505,60.80660700798035,1.836630609614162e-06
75976,151953,151952,303905,60.88055396080017,1.832048046098284e-06
76076,152153,152152,304305,60.956743001937866,1.8274989473565958e-06
76176,152353,152352,304705,61.035258769989014,1.8229831058025645e-06
76276,152553,152552,305105,61.12924909591675,1.818500313879528e-06
76376,152753,152752,305505,61.21458196640015,1.8140503654104226e-06
76476,152953,152952,305905,61.29322600364685,1.8096330548917877e-06
76577,153155,153154,306309,61.367249965667725,1.8052044924095253e-06
76677,153355,153354,306709,61.441890001297,1.8008521664431159e-06
76777,153555,153554,307109,61.514612913131714,1.7965318653049106e-06
76877,153755,153754,307509,61.5899920463562,1.7922433870349087e-06
76977,153955,153954,307909,61.66326093673706,1.7879865303773963e-06
77077,154155,154154,308309,61.73578596115112,1.7837610951737734e-06
77177,154355,154354,308709,61.80779194831848,1.7795668817952114e-06
77277,154555,154554,309109,61.88446807861328,1.775403691839618e-06
77377,154755,154754,309509,61.961199045181274,1.7712713274828856e-06
77477,154955,154954,309909,62.03153419494629,1.7671695917911344e-06
77578,155157,155156,310313,62.11247801780701,1.763057728629924e-06
77678,155357,155356,310713,62.19210076332092,1.759016964202382e-06
77778,155557,155556,311113,62.271831035614014,1.755006240998e-06
77878,155757,155756,311513,62.3539559841156,1.7510253653561124e-06
77978,155957,155956,311913,62.455573081970215,1.7470741444808845e-06
78078,156157,156156,312313,62.53610014915466,1.7431523867505794e-06
78178,156357,156356,312713,62.61177396774292,1.739259901037415e-06
78278,156557,156556,313113,62.685948848724365,1.7353964971853342e-06
78378,156757,156756,313513,62.76630091667175,1.7315619860625706e-06
78478,156957,156956,313913,62.84904599189758,1.7277561789569766e-06
78579,157159,157158,314317,62.924530029296875,1.7239412587906194e-06
78679,157359,157358,314717,63.00164198875427,1.7201925799825884e-06
78779,157559,157558,315117,63.07585692405701,1.7164720431074261e-06
78879,157759,157758,315517,63.1503050327301,1.7127794629624441e-06
78979,157959,157958,315917,63.22413396835327,1.7091146549861194e-06
79079,158159,158158,316317,63.29810094833374,1.7054774360387703e-06
79179,158359,158358,316717,63.37608814239502,1.7018676233897183e-06
79279,158559,158558,317117,63.45469284057617,1.698285035077022e-06
79379,158759,158758,317517,63.53827500343323,1.6947294902313227e-06
79479,158959,158958,317917,63.61941885948181,1.6912008087318635e-06
79580,159161,159160,318321,63.698418855667114,1.6876639254544311e-06
79680,159361,159360,318721,63.77352595329285,1.684188697519512e-06
79780,159561,159560,319121,63.85061717033386,1.6807397956576483e-06
79880,159761,159760,319521,63.92747902870178,1.6773170429601805e-06
79980,159961,159960,319921,64.00474905967712,1.6739202634554277e-06
80080,160161,160160,320321,64.08145999908447,1.6705492819888668e-06
80180,160361,160360,320721,64.1577820777893,1.6672039242535504e-06
80280,160561,160560,321121,64.2343499660492,1.6638840163777806e-06
80380,160761,160760,321521,64.31194996833801,1.660589385918047e-06
80480,160961,160960,321921,64.38817310333252,1.6573198610569068e-06
80581,161163,161162,322325,64.46783900260925,1.6540429497962114e-06
80681,161363,161362,322725,64.54290199279785,1.6508233700928283e-06
80781,161563,161562,323125,64.61773014068604,1.6476283833373464e-06
80881,161763,161762,323525,64.69210290908813,1.6444578209271493e-06
80981,161963,161962,323925,64.76538014411926,1.6413115151153036e-06
81081,162163,162162,324325,64.84190702438354,1.6381892988558482e-06
81181,162363,162362,324725,64.92215490341187,1.6350910059707293e-06
81281,162563,162562,325125,65.01429986953735,1.6320164711392937e-06
81381,162763,162762,325525,65.10189008712769,1.6289655296477216e-06
81481,162963,162962,325925,65.19637989997864,1.6259380180947523e-06
81582,163165,163164,326329,65.34731698036194,1.6229038476649173e-06
81682,163365,163364,326729,65.45349407196045,1.619922937826256e-06
81782,163565,163564,327129,65.53290486335754,1.6169649696847463e-06
81882,163765,163764,327529,65.60747385025024,1.614029782964095e-06
81982,163965,163964,327929,65.690425157547,1.6111172178562461e-06
82082,164165,164164,328329,65.77483010292053,1.608227115614968e-06
82182,164365,164364,328729,65.8751540184021,1.6053593179189702e-06
82282,164565,164564,329129,65.9681568145752,1.6025136679114424e-06
82382,164765,164764,329529,66.05261206626892,1.599690008754685e-06
82482,164965,164964,329929,66.15925288200378,1.5968881850724742e-06
82583,165167,165166,330333,66.28485822677612,1.594080349363094e-06
82683,165367,165366,330733,66.40743613243103,1.5913219471252603e-06
82783,165567,165566,331133,66.49222803115845,1.588584916599724e-06
82883,165767,165766,331533,66.57049489021301,1.5858691054244984e-06
82983,165967,165966,331933,66.65568399429321,1.5831743617700876e-06
83083,166167,166166,332333,66.73676204681396,1.5805005350361195e-06
83183,166367,166366,332733,66.81768703460693,1.5778474748757486e-06
83283,166567,166566,333133,66.96390199661255,1.5752150326098378e-06
83383,166767,166766,333533,67.04806613922119,1.572603059155467e-06
83483,166967,166966,333933,67.12381601333618,1.5700114072136505e-06
83584,167169,167168,334337,67.19931101799011,1.5674143163533773e-06
83684,167369,167368,334737,67.2751739025116,1.5648630669727027e-06
83784,167569,167568,335137,67.34995102882385,1.5623316993091795e-06
83884,167769,167768,335537,67.43186616897583,1.5598200690349098e-06
83984,167969,167968,335937,67.5145320892334,1.5573280321679621e-06
84084,168169,168168,336337,67.5947048664093,1.5548554459424362e-06
84184,168369,168368,336737,67.67700409889221,1.5524021681994328e-06
84284,168569,168568,337137,67.74986505508423,1.5499680578256143e-06
84384,168769,168768,337537,67.81996011734009,1.5475529739526512e-06
84484,168969,168968,337937,67.88930606842041,1.5451567769376212e-06
84585,169171,169170,338341,67.96084785461426,1.5427556474698198e-06
84685,169371,169370,338741,68.0351140499115,1.5403969933505532e-06
84785,169571,169570,339141,68.11504197120667,1.5380568098468841e-06
84885,169771,169770,339541,68.18636202812195,1.535734960562266e-06
84985,169971,169970,339941,68.26095199584961,1.5334313094921342e-06
85085,170171,170170,340341,68.33754396438599,1.5311457214689604e-06
85185,170371,170370,340741,68.41568517684937,1.5288780623743324e-06
85285,170571,170570,341141,68.4911060333252,1.526628198387049e-06
85385,170771,170770,341541,68.5607259273529,1.5243959968526471e-06
85485,170971,170970,341941,68.63015508651733,1.5221813256097273e-06
85586,171173,171172,342345,68.70061302185059,1.5199621680827842e-06
85686,171373,171372,342745,68.77140784263611,1.5177823365159705e-06
85786,171573,171572,343145,68.84421896934509,1.5156196423009276e-06
85886,171773,171772,343545,68.92285895347595,1.5134739568266023e-06
85986,171973,171972,343945,68.99951887130737,1.5113451514983241e-06
86086,172173,172172,344345,69.08006811141968,1.5092330991083433e-06
86186,172373,172372,344745,69.1626181602478,1.5071376727685602e-06
86286,172573,172572,345145,69.24062299728394,1.5050587465666602e-06
86386,172773,172772,345545,69.32267808914185,1.502996195389828e-06
86486,172973,172972,345945,69.40260195732117,1.5009498945678348e-06
86587,173175,173174,346349,69.48088812828064,1.4988994999018596e-06
86687,173375,173374,346749,69.55895400047302,1.4968854890651688e-06
86787,173575,173574,347149,69.63507509231567,1.494887358749664e-06
86887,173775,173774,347549,69.7116129398346,1.4929049870984796e-06
86987,173975,173974,347949,69.78380489349365,1.4909382537904246e-06
87087,174175,174174,348349,69.88013696670532,1.4889870386305271e-06
87187,174375,174374,348749,69.96298289299011,1.4870512223823873e-06
87287,174575,174574,349149,70.04795002937317,1.4851306864376108e-06
87387,174775,174774,349549,70.13316893577576,1.4832253130428921e-06
87487,174975,174974,349949,70.21263003349304,1.4813349852828165e-06
87588,175177,175176,350353,70.29317998886108,1.479440907684181e-06
87688,175377,175376,350753,70.3679449558258,1.4775804702262628e-06
87788,175577,175576,351153,70.44201588630676,1.4757347303277195e-06
87888,175777,175776,351553,70.51570892333984,1.4739035738584341e-06
87988,175977,175976,351953,70.59650206565857,1.472086887270369e-06
88088,176177,176176,352353,70.67098999023438,1.4702845579719397e-06
88188,176377,176376,352753,70.74478888511658,1.4684964739474555e-06
88288,176577,176576,353153,70.8189160823822,1.4667225239311733e-06
88388,176777,176776,353553,70.89260387420654,1.4649625973142203e-06
88488,176977,176976,353953,70.96290612220764,1.4632165841767938e-06
88589,177179,177178,354357,71.03498077392578,1.4614671226851623e-06
88689,177379,177378,354757,71.10689210891724,1.4597487462110185e-06
88789,177579,177578,355157,71.18229699134827,1.4580439569882368e-06
88889,177779,177778,355557,71.25433015823364,1.4563526476187764e-06
88989,177979,177978,355957,71.32851600646973,1.4546747120474548e-06
89089,178179,178178,356357,71.40420603752136,1.4530100443197464e-06
89189,178379,178378,356757,71.47553586959839,1.4513585399173698e-06
89289,178579,178578,357157,71.58033680915833,1.449720094158862e-06
89389,178779,178778,357557,71.65662479400635,1.4480946036842707e-06
89489,178979,178978,357957,71.72971606254578,1.4464819654288502e-06
89590,179181,179180,358361,71.82574200630188,1.4448661425046581e-06
89690,179381,179380,358761,71.9017128944397,1.443279028929558e-06
89790,179581,179580,359161,71.99795293807983,1.4417044619077524e-06
89890,179781,179780,359561,72.07052493095398,1.4401423414844319e-06
89990,179981,179980,359961,72.16034412384033,1.4385925681442626e-06
90090,180181,180180,360361,72.23221611976624,1.437055042820718e-06
90190,180381,180380,360761,72.30706691741943,1.4355296675786023e-06
90290,180581,180580,361161,72.38331484794617,1.4340163447196163e-06
90390,180781,180780,361561,72.45414900779724,1.432514977630394e-06
90490,180981,180980,361961,72.52265000343323,1.4310254699660522e-06
90591,181183,181182,362365,72.59627485275269,1.4295330079215403e-06
90691,181383,181382,362765,72.6646101474762,1.4280670495519363e-06
90791,181583,181582,363165,72.73372602462769,1.4266126651034025e-06
90891,181783,181782,363565,72.80232501029968,1.4251697609257057e-06
90991,181983,181982,363965,72.87524890899658,1.4237382443122814e-06
91091,182183,182182,364365,72.94749116897583,1.4223180227652558e-06
91191,182383,182382,364765,73.01836585998535,1.4209090048431104e-06
91291,182583,182582,365165,73.09382700920105,1.4195110994672459e-06
91391,182783,182782,365565,73.16676712036133,1.4181242161469805e-06
91491,182983,182982,365965,73.238028049469,1.4167482654553145e-06
91592,183185,183184,366369,73.3213198184967,1.4153695613472516e-06
91692,183385,183384,366769,73.4268319606781,1.4140153160225222e-06
91792,183585,183584,367169,73.51969695091248,1.4126717368033945e-06
91892,183785,183784,367569,73.60921597480774,1.4113387365096943e-06
91992,183985,183984,367969,73.68926692008972,1.4100162286344663e-06
92092,184185,184184,368369,73.76327300071716,1.4087041271765727e-06
92192,184385,184384,368769,73.83497405052185,1.4074023466679913e-06
92292,184585,184584,369169,73.90830993652344,1.4061108024713637e-06
92392,184785,184784,369569,74.02981805801392,1.4048294103705945e-06
92492,184985,184984,369969,74.10685110092163,1.4035580868439076e-06
92593,185187,185186,370373,74.17940306663513,1.402284185577777e-06
92693,185387,185386,370773,74.25293016433716,1.4010328495400257e-06
92793,185587,185586,371173,74.32350492477417,1.3997913341642846e-06
92893,185787,185786,371573,74.39193487167358,1.3985595584414396e-06
92993,185987,185986,371973,74.47486209869385,1.3973374416603614e-06
93093,186187,186186,372373,74.5578920841217,1.3961249039379972e-06
93193,186387,186386,372773,74.62818789482117,1.3949218657123098e-06
93293,186587,186586,373173,74.69855093955994,1.3937282484210587e-06
93393,186787,186786,373573,74.7751259803772,1.3925439736077279e-06
93493,186987,186986,373973,74.8539628982544,1.3913689637980936e-06
93594,187189,187188,374377,74.92611193656921,1.3901915296867567e-06
93694,187389,187388,374777,75.00283288955688,1.3890349098432154e-06
93794,187589,187588,375177,75.07335186004639,1.3878873246357019e-06
93894,187789,187788,375577,75.14713597297668,1.3867486985945261e-06
93994,187989,187988,375977,75.21955108642578,1.3856189570908606e-06
94094,188189,188188,376377,75.30344700813293,1.38449802570958e-06
94194,188389,188388,376777,75.3826801776886,1.3833858307656064e-06
94294,188589,188588,377177,75.46144318580627,1.3822822991316638e-06
94394,188789,188788,377577,75.53371381759644,1.3811873582845045e-06
94494,188989,188988,377977,75.60540008544922,1.380100935891496e-06
94595,189191,189190,378381,75.67790102958679,1.3790122236024353e-06
94695,189391,189390,378781,75.75213599205017,1.3779427080479144e-06
94795,189591,189590,379181,75.83418488502502,1.376881497565118e-06
94895,189791,189790,379581,75.90955400466919,1.3758285222432733e-06
94995,189991,189990,379981,75.984610080719,1.374783712646331e-06
95095,190191,190190,380381,76.06032800674438,1.3737469999185782e-06
95195,190391,190390,380781,76.13598012924194,1.3727183158601186e-06
95295,190591,190590,381181,76.21611905097961,1.3716975926498783e-06
95395,190791,190790,381581,76.29199314117432,1.3706847629116834e-06
95495,190991,190990,381981,76.37700986862183,1.3696797599346017e-06
95596,191193,191192,382385,76.46512579917908,1.368672584022339e-06
95696,191393,191392,382785,76.55124187469482,1.367683112962588e-06
95796,191593,191592,383185,76.6246588230133,1.3667012708478613e-06
95896,191793,191792,383585,76.70560884475708,1.3657269930463281e-06
95996,191993,191992,383985,76.78116297721863,1.3647602150997397e-06
96096,192193,192192,384385,76.85214376449585,1.3638008733392518e-06
96196,192393,192392,384785,76.93126702308655,1.3628489047718675e-06
96296,192593,192592,385185,77.05319499969482,1.3619042464747929e-06
96396,192793,192792,385585,77.16177988052368,1.3609668361281709e-06
96496,192993,192992,385985,77.28858184814453,1.360036612080165e-06
96597,193195,193194,386389,77.3745129108429,1.3591043179385103e-06
96697,193395,193394,386789,77.48634696006775,1.358188353514031e-06
96797,193595,193594,387189,77.61352705955505,1.3572793923773275e-06
96897,193795,193794,387589,77.69308996200562,1.3563773748001648e-06
96997,193995,193994,387989,77.78841018676758,1.3554822410965038e-06
97097,194195,194194,388389,77.89498901367188,1.35459393284761e-06
97197,194395,194394,388789,77.97774004936218,1.3537123913264018e-06
97297,194595,194594,389189,78.07344198226929,1.3528375585785545e-06
97397,194795,194794,389589,78.15262579917908,1.3519693771399977e-06
97497,194995,194994,389989,78.23534202575684,1.351107789933584e-06
97598,195197,195196,390393,78.3273069858551,1.3502442227272008e-06
97698,195397,195396,390793,78.46989583969116,1.349395719271456e-06
97798,195597,195596,391193,78.57799196243286,1.348553640899381e-06
97898,195797,195796,391593,78.65797305107117,1.3477179327329728e-06
97998,195997,195996,391993,78.74201011657715,1.3468885396055964e-06
98098,196197,196196,392393,78.84986186027527,1.3460654073491742e-06
98198,196397,196396,392793,78.93418097496033,1.3452484819625905e-06
98298,196597,196596,393193,79.0104410648346,1.3444377100831858e-06
98398,196797,196796,393593,79.14340090751648,1.3436330384876309e-06
98498,196997,196996,393993,79.22752094268799,1.3428344145000124e-06
98599,197199,197198,394397,79.30831694602966,1.3420338897748264e-06
98699,197399,197398,394797,79.38493204116821,1.3412472640671224e-06
98799,197599,197598,395197,79.46774101257324,1.3404665303278835e-06
98899,197799,197798,395597,79.56147503852844,1.3396916374270527e-06
98999,197999,197998,395997,79.65011501312256,1.338922534672346e-06
99099,198199,198198,396397,79.72694897651672,1.3381591725322445e-06
99199,198399,198398,396797,79.81008577346802,1.3374015005807464e-06
99299,198599,198598,397197,79.88635015487671,1.3366494697956206e-06
99399,198799,198798,397597,79.96523690223694,1.335903031252909e-06
99499,198999,198998,397997,80.04846477508545,1.3351621364456628e-06
99600,199201,199200,398401,80.13039588928223,1.3344194110065009e-06
99700,199401,199400,398801,80.20455503463745,1.3336895139686216e-06
99800,199601,199600,399201,80.27845811843872,1.3329650172670143e-06
99900,199801,199800,399601,80.35852789878845,1.332245873735849e-06
100000,200001,200000,400001,80.44037985801697,1.3315320367501845e-06


==> plot_data/bilinear_matrix_game_n500/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0009160041809082031,2.018959020339561
100,201,200,401,0.07715821266174316,0.04084193889187754
200,401,400,801,0.16120600700378418,0.01555572904704933
300,601,600,1201,0.24944210052490234,0.008941559671892264
400,801,800,1601,0.3368391990661621,0.005957710393872965
501,1003,1002,2005,0.46764707565307617,0.004080388626738635
601,1203,1202,2405,0.5416932106018066,0.003044183482286378
701,1403,1402,2805,0.621251106262207,0.00247078219342337
801,1603,1602,3205,0.7011713981628418,0.002022425653118514
901,1803,1802,3605,0.7767093181610107,0.0017090990324214828
1001,2003,2002,4005,0.8524861335754395,0.0014375084752964995
1101,2203,2202,4405,0.9366452693939209,0.0012047380988628406
1201,2403,2402,4805,1.019376277923584,0.001000692926912849
1301,2603,2602,5205,1.1019251346588135,0.0008161398070111659
1401,2803,2802,5605,1.1924023628234863,0.0007105240339073027
1502,3005,3004,6009,1.2840192317962646,0.0006406047458752685
1602,3205,3204,6409,1.3672723770141602,0.0005873580809235912
1702,3405,3404,6809,1.4364511966705322,0.0005382536666146199
1802,3605,3604,7209,1.510073184967041,0.0004953501567577407
1902,3805,3804,7609,1.5858969688415527,0.00046283265676205554
2002,4005,4004,8009,1.7175931930541992,0.0004308549629022895
2102,4205,4204,8409,1.8151521682739258,0.0003999154365291184
2202,4405,4404,8809,1.9494280815124512,0.00037725255875169743
2302,4605,4604,9209,2.157297134399414,0.0003527435669886361
2402,4805,4804,9609,2.242280960083008,0.0003335273689751663
2503,5007,5006,10013,2.4526331424713135,0.00031945940005734464
2603,5207,5206,10413,2.590062141418457,0.00030878973556726564
2703,5407,5406,10813,2.7304251194000244,0.0003000156905100278
2803,5607,5606,11213,2.823237180709839,0.00029252572517975546
2903,5807,5806,11613,2.897221326828003,0.00028541420036607454
3003,6007,6006,12013,2.973459005355835,0.0002780152490870146
3103,6207,6206,12413,3.0520529747009277,0.00027195002345469855
3203,6407,6406,12813,3.1366500854492188,0.00026673775102073016
3303,6607,6606,13213,3.2105050086975098,0.00026209269718888097
3403,6807,6806,13613,3.284858226776123,0.00025787167822761395
3504,7009,7008,14017,3.3663980960845947,0.00025394578198297755
3604,7209,7208,14417,3.44762921333313,0.00025011718889721537
3704,7409,7408,14817,3.5469560623168945,0.0002467056013739032
3804,7609,7608,15217,3.635627031326294,0.00024351263461413038
3904,7809,7808,15617,3.7246532440185547,0.00024048591179458707
4004,8009,8008,16017,3.8213601112365723,0.00023752401694437778
4104,8209,8208,16417,3.9039900302886963,0.00023457721923087589
4204,8409,8408,16817,3.9846279621124268,0.00023189293501112748
4304,8609,8608,17217,4.058801174163818,0.00022910798042041975
4404,8809,8808,17617,4.136341094970703,0.00022619918421695374
4505,9011,9010,18021,4.219438076019287,0.0002230343272817675
4605,9211,9210,18421,4.296112298965454,0.00022034767502957447
4705,9411,9410,18821,4.372629165649414,0.0002178537931555071
4805,9611,9610,19221,4.449649333953857,0.00021549280886485868
4905,9811,9810,19621,4.52517032623291,0.00021323705999951907
5005,10011,10010,20021,4.602029085159302,0.00021107038667084828
5105,10211,10210,20421,4.686842203140259,0.00020898191834835915
5205,10411,10410,20821,4.759340047836304,0.0002069636366998869
5305,10611,10610,21221,4.832656145095825,0.00020500924417355266
5405,10811,10810,21621,4.916287183761597,0.00020311357261230275
5506,11013,11012,22025,5.001103162765503,0.00020125409421659746
5606,11213,11212,22425,5.0937652587890625,0.000199463812585603
5706,11413,11412,22825,5.196096181869507,0.00019772072266799426
5806,11613,11612,23225,5.292882919311523,0.00019602185970323322
5906,11813,11812,23625,5.397942066192627,0.00019436456045111267
6006,12013,12012,24025,5.526998043060303,0.00019226895881548032
6106,12213,12212,24425,5.664118051528931,0.00018981336384564818
6206,12413,12412,24825,5.77864408493042,0.00018778452212550104
6306,12613,12612,25225,5.865795135498047,0.00018589168393157325
6406,12813,12812,25625,5.958546161651611,0.00018405691086032967
6507,13015,13014,26029,6.034569978713989,0.00018229450115027232
6607,13215,13214,26429,6.1109912395477295,0.00018061323138483316
6707,13415,13414,26829,6.1928770542144775,0.00017896837070119164
6807,13615,13614,27229,6.32046103477478,0.00017670539366986823
6907,13815,13814,27629,6.4215381145477295,0.00017394478665026857
7007,14015,14014,28029,6.527940273284912,0.00017182380289514751
7107,14215,14214,28429,6.661684989929199,0.00016995140199686445
7207,14415,14414,28829,6.759672164916992,0.00016822996598922252
7307,14615,14614,29229,6.865925312042236,0.00016600502050577174
7407,14815,14814,29629,6.957630157470703,0.00016417365369737495
7508,15017,15016,30033,7.026482343673706,0.00016248289306673215
7608,15217,15216,30433,7.097146272659302,0.00016090886540011637
7708,15417,15416,30833,7.173899173736572,0.0001588388697985169
7808,15617,15616,31233,7.319712162017822,0.00015716504752308173
7908,15817,15816,31633,7.410336017608643,0.00015560807575707016
8008,16017,16016,32033,7.489384174346924,0.0001528670951392979
8108,16217,16216,32433,7.6832640171051025,0.0001508824226984641
8208,16417,16416,32833,7.777975082397461,0.00014869762396062543
8308,16617,16616,33233,7.868849277496338,0.00014660531424563205
8408,16817,16816,33633,7.978354215621948,0.00014472799576799907
8509,17019,17018,34037,8.067054271697998,0.00014295922339428892
8609,17219,17218,34437,8.14896011352539,0.0001412736273534982
8709,17419,17418,34837,8.225372314453125,0.0001396714101891978
8809,17619,17618,35237,8.297926187515259,0.00013813795600318
8909,17819,17818,35637,8.376390218734741,0.00013538373808574897
9009,18019,18018,36037,8.449045181274414,0.00013331524081584936
9109,18219,18218,36437,8.540098190307617,0.0001315176266269928
9209,18419,18418,36837,8.61720609664917,0.00012838146992159456
9309,18619,18618,37237,8.692612171173096,0.0001260062401086033
9409,18819,18818,37637,8.776901245117188,0.000123989736577564
9510,19021,19020,38041,8.883724212646484,0.0001221400303066318
9610,19221,19220,38441,8.994230031967163,0.0001204386966298002
9710,19421,19420,38841,9.079511165618896,0.00011847239407814625
9810,19621,19620,39241,9.16598916053772,0.00011669918825553777
9910,19821,19820,39641,9.239830017089844,0.00011274641903217324
10010,20021,20020,40041,9.312960147857666,0.00011039424919270669
10110,20221,20220,40441,9.384573221206665,0.00010842101331861896
10210,20421,20420,40841,9.455811262130737,0.0001056460432049642
10310,20621,20620,41241,9.530109167098999,0.0001034347785040179
10410,20821,20820,41641,9.606977224349976,0.00010121426707386297
10511,21023,21022,42045,9.682388067245483,9.88379844340756e-05
10611,21223,21222,42445,9.77069902420044,9.691614316935306e-05
10711,21423,21422,42845,9.861533164978027,9.51729702356169e-05
10811,21623,21622,43245,9.959519147872925,9.355874460556968e-05
10911,21823,21822,43645,10.04480528831482,9.195903659656644e-05
11011,22023,22022,44045,10.126850128173828,9.044062572871737e-05
11111,22223,22222,44445,10.207280158996582,8.760072395653058e-05
11211,22423,22422,44845,10.281220197677612,8.501766878337613e-05
11311,22623,22622,45245,10.35869812965393,8.292729869838731e-05
11411,22823,22822,45645,10.43043303489685,8.10564411007725e-05
11512,23025,23024,46049,10.50618028640747,7.89596690741875e-05
11612,23225,23224,46449,10.581852197647095,7.709389597231927e-05
11712,23425,23424,46849,10.666245222091675,7.544918173016605e-05
11812,23625,23624,47249,10.742191076278687,7.397387281337675e-05
11912,23825,23824,47649,10.818507194519043,7.25963281164493e-05
12012,24025,24024,48049,10.893757343292236,7.129342706426366e-05
12112,24225,24224,48449,10.969269037246704,6.997551128540555e-05
12212,24425,24424,48849,11.04262924194336,6.870086322848533e-05
12312,24625,24624,49249,11.118250131607056,6.749927088782142e-05
12412,24825,24824,49649,11.193716049194336,6.532043439414624e-05
12513,25027,25026,50053,11.27043104171753,6.377417764162247e-05
12613,25227,25226,50453,11.342777252197266,6.241931681348971e-05
12713,25427,25426,50853,11.416340112686157,6.117000796872597e-05
12813,25627,25626,51253,11.490470170974731,5.9999357950401774e-05
12913,25827,25826,51653,11.563889265060425,5.8892075906161434e-05
13013,26027,26026,52053,11.642538070678711,5.783806989101728e-05
13113,26227,26226,52453,11.718331336975098,5.683013725086848e-05
13213,26427,26426,52853,11.796934127807617,5.586287849136061e-05
13313,26627,26626,53253,11.879348039627075,5.493210368684028e-05
13413,26827,26826,53653,11.960280179977417,5.40344745752552e-05
13514,27029,27028,54057,12.07690715789795,5.315874701548238e-05
13614,27229,27228,54457,12.19296407699585,5.231999088587542e-05
13714,27429,27428,54857,12.297738075256348,5.150748953360285e-05
13814,27629,27628,55257,12.398382186889648,5.071961773190266e-05
13914,27829,27828,55657,12.518952369689941,4.9954964822641746e-05
14014,28029,28028,56057,12.624227046966553,4.9212291176279406e-05
14114,28229,28228,56457,12.736079216003418,4.8490495271269185e-05
14214,28429,28428,56857,12.840842008590698,4.778858852014829e-05
14314,28629,28628,57257,12.95626711845398,4.710567581298244e-05
14414,28829,28828,57657,13.069595336914062,4.6440940328542634e-05
14515,29031,29030,58061,13.185526132583618,4.5787244079736674e-05
14615,29231,29230,58461,13.307294130325317,4.515683226577822e-05
14715,29431,29430,58861,13.416558265686035,4.454250253990974e-05
14815,29631,29630,59261,13.522042274475098,4.394365350429401e-05
14915,29831,29830,59661,13.626391172409058,4.335972145555563e-05
15015,30031,30030,60061,13.739590167999268,4.279017615475833e-05
15115,30231,30230,60461,13.847413063049316,4.2234517292302766e-05
15215,30431,30430,60861,13.967111349105835,4.169227150309635e-05
15315,30631,30630,61261,14.086551189422607,4.116298982875498e-05
15415,30831,30830,61661,14.20417833328247,4.064624553921866e-05
15516,31033,31032,62065,14.321059226989746,4.013664605096901e-05
15616,31233,31232,62465,14.437446117401123,3.96438916138613e-05
15716,31433,31432,62865,14.556769132614136,3.916250645932755e-05
15816,31633,31632,63265,14.66842007637024,3.8692136325430465e-05
15916,31833,31832,63665,14.771836280822754,3.823244181240052e-05
16016,32033,32032,64065,14.90726613998413,3.778309738033774e-05
16116,32233,32232,64465,15.068897008895874,3.7343790450688504e-05
16216,32433,32432,64865,15.21175503730774,3.69142205982145e-05
16316,32633,32632,65265,15.357553243637085,3.6494098819374294e-05
16416,32833,32832,65665,15.496569156646729,3.6083146870131576e-05
16517,33035,33034,66069,15.640648365020752,3.5677120231280035e-05
16617,33235,33234,66469,15.748964071273804,3.528379843960052e-05
16717,33435,33434,66869,15.851580142974854,3.4898868073149153e-05
16817,33635,33634,67269,15.959979057312012,3.452208846989514e-05
16917,33835,33834,67669,16.06515622138977,3.4153227173809356e-05
17017,34035,34034,68069,16.18707013130188,3.379205954143965e-05
17117,34235,34234,68469,16.288823127746582,3.3438368377594996e-05
17217,34435,34434,68869,16.3892822265625,3.309194359746961e-05
17317,34635,34634,69269,16.490548133850098,3.2752581913295634e-05
17417,34835,34834,69669,16.594680070877075,3.242008654192568e-05
17518,35037,35036,70073,16.75674605369568,3.2091041818962486e-05
17618,35237,35236,70473,16.855870008468628,3.177177739504206e-05
17718,35437,35436,70873,16.956817150115967,3.145882356187534e-05
17818,35637,35636,71273,17.06025719642639,3.115200705127862e-05
17918,35837,35836,71673,17.17358112335205,3.085115989694329e-05
18018,36037,36036,72073,17.276860237121582,3.055611923573243e-05
18118,36237,36236,72473,17.426112174987793,3.0266727121420946e-05
18218,36437,36436,72873,17.526703119277954,2.998283034703666e-05
18318,36637,36636,73273,17.63402223587036,2.9704280278715254e-05
18418,36837,36836,73673,17.74004626274109,2.9430932697111267e-05
18519,37039,37038,74077,17.84474015235901,2.9159989898597117e-05
18619,37239,37238,74477,17.944088220596313,2.8896680138948832e-05
18719,37439,37438,74877,18.045551300048828,2.8638163927325157e-05
18819,37639,37638,75277,18.148414134979248,2.838431330815558e-05
18919,37839,37838,75677,18.264541387557983,2.8135004055142335e-05
19019,38039,38038,76077,18.376450061798096,2.7890115554991762e-05
19119,38239,38238,76477,18.478642225265503,2.7649530692710136e-05
19219,38439,38438,76877,18.584816217422485,2.7413135744249717e-05
19319,38639,38638,77277,18.69430136680603,2.7180820271181197e-05
19419,38839,38838,77677,18.798993349075317,2.6952477022695076e-05
19520,39041,39040,78081,18.90667223930359,2.6725776274959876e-05
19620,39241,39240,78481,19.028571128845215,2.6505105158808064e-05
19720,39441,39440,78881,19.135950088500977,2.6288101721943395e-05
19820,39641,39640,79281,19.242622137069702,2.60746705615014e-05
19920,39841,39840,79681,19.34536123275757,2.5864719015414138e-05
20020,40041,40040,80081,19.4580180644989,2.5658157080510214e-05
20120,40241,40240,80481,19.56177306175232,2.5454897336755517e-05
20220,40441,40440,80881,19.683651208877563,2.5254854872420898e-05
20320,40641,40640,81281,19.793426990509033,2.5057947211617455e-05
20420,40841,40840,81681,19.899259328842163,2.4864094243831293e-05
20521,41043,41042,82085,19.999800205230713,2.4671324172818473e-05
20621,41243,41242,82485,20.10373306274414,2.4483378027808908e-05
20721,41443,41442,82885,20.209615230560303,2.429825905215031e-05
20821,41643,41642,83285,20.310593128204346,2.411589596343249e-05
20921,41843,41842,83685,20.426883220672607,2.3936219526962322e-05
21021,42043,42042,84085,20.528851985931396,2.375916249582231e-05
21121,42243,42242,84485,20.627896070480347,2.358465955640318e-05
21221,42443,42442,84885,20.735274076461792,2.3412647271865886e-05
21321,42643,42642,85285,20.842782974243164,2.3243064029661924e-05
21421,42843,42842,85685,20.9623122215271,2.307584999029077e-05
21522,43045,43044,86089,21.10989212989807,2.290930948446167e-05
21622,43245,43244,86489,21.254266262054443,2.274668343669633e-05
21722,43445,43444,86889,21.404250144958496,2.2586256669867326e-05
21822,43645,43644,87289,21.612995147705078,2.2427975960148327e-05
21922,43845,43844,87689,21.752506256103516,2.2271789617417764e-05
22022,44045,44044,88089,21.870522260665894,2.2117647441859577e-05
22122,44245,44244,88489,21.99016499519348,2.1965500681564148e-05
22222,44445,44444,88889,22.099338054656982,2.1815301990555972e-05
22322,44645,44644,89289,22.232834100723267,2.1667005389170224e-05
22422,44845,44844,89689,22.351218223571777,2.1520566223945708e-05
22523,45047,45046,90093,22.45926308631897,2.137450389743613e-05
22623,45247,45246,90493,22.58220911026001,2.1231668274742093e-05
22723,45447,45446,90893,22.70063328742981,2.109056331098932e-05
22823,45647,45646,91293,22.825556993484497,2.095114930112278e-05
22923,45847,45846,91693,22.93882131576538,2.0813387685584392e-05
23023,46047,46046,92093,23.06244206428528,2.067724101748545e-05
23123,46247,46246,92493,23.180089235305786,2.054267293063988e-05
23223,46447,46446,92893,23.283591270446777,2.040964810749064e-05
23323,46647,46646,93293,23.387843132019043,2.0278132248572443e-05
23423,46847,46846,93693,23.48790192604065,2.014809204346726e-05
23524,47049,47048,94097,23.593610048294067,2.0018216353502114e-05
23624,47249,47248,94497,23.701472997665405,1.989104529704416e-05
23724,47449,47448,94897,23.80323100090027,1.9765255307275363e-05
23824,47649,47648,95297,23.90330219268799,1.9640816754702152e-05
23924,47849,47848,95697,24.00944995880127,1.9517700861296387e-05
24024,48049,48048,96097,24.110535144805908,1.9395879674889236e-05
24124,48249,48248,96497,24.214813947677612,1.9275326045535996e-05
24224,48449,48448,96897,24.31739115715027,1.9156013600908175e-05
24324,48649,48648,97297,24.41633105278015,1.9037916723550638e-05
24424,48849,48848,97697,24.51978325843811,1.8921010528517207e-05
24525,49051,49050,98101,24.63312005996704,1.8804119255199948e-05
24625,49251,49250,98501,24.75270915031433,1.8689533904571334e-05
24725,49451,49450,98901,24.853676080703735,1.857606853538815e-05
24825,49651,49650,99301,24.95366621017456,1.846370098658152e-05
24925,49851,49850,99701,25.052947998046875,1.835240972575939e-05
25025,50051,50050,100101,25.156164169311523,1.8242173830892025e-05
25125,50251,50250,100501,25.25630807876587,1.8132972971845767e-05
25225,50451,50450,100901,25.359933376312256,1.8024787392688152e-05
25325,50651,50650,101301,25.460934162139893,1.791759789366019e-05
25425,50851,50850,101701,25.564114332199097,1.7811385815375412e-05
25526,51053,51052,102105,25.66991114616394,1.7705085278162808e-05
25626,51253,51252,102505,25.769639253616333,1.7600783470369335e-05
25726,51453,51452,102905,25.86827325820923,1.749740601403757e-05
25826,51653,51652,103305,25.968862056732178,1.7394936255609e-05
25926,51853,51852,103705,26.070621967315674,1.729335800409566e-05
26026,52053,52052,104105,26.172730207443237,1.7192655517201312e-05
26126,52253,52252,104505,26.277496099472046,1.7092813487563866e-05
26226,52453,52452,104905,26.377682209014893,1.6993817030214183e-05
26326,52653,52652,105305,26.4779691696167,1.68956516684544e-05
26426,52853,52852,105705,26.580912113189697,1.6798303322708575e-05
26527,53055,53054,106109,26.68442440032959,1.670079685866953e-05
26627,53255,53254,106509,26.79988932609558,1.660504966524333e-05
26727,53455,53454,106909,26.91183614730835,1.6510079380238825e-05
26827,53655,53654,107309,27.014228105545044,1.641587339620174e-05
26927,53855,53854,107709,27.118714094161987,1.6322419444874413e-05
27027,54055,54054,108109,27.22154211997986,1.622970558720964e-05
27127,54255,54254,108509,27.327182054519653,1.6137720202917003e-05
27227,54455,54454,108909,27.424816131591797,1.604645198133419e-05
27327,54655,54654,109309,27.529564142227173,1.5955889911033592e-05
27427,54855,54854,109709,27.635689973831177,1.5866023271890535e-05
27528,55057,55056,110113,27.735810041427612,1.5775953233158783e-05
27628,55257,55256,110513,27.837635278701782,1.568745311075853e-05
27728,55457,55456,110913,27.940760135650635,1.559961781625362e-05
27828,55657,55656,111313,28.044401168823242,1.5512437707874757e-05
27928,55857,55856,111713,28.152737140655518,1.5425903392593543e-05
28028,56057,56056,112113,28.252470016479492,1.5340005718320964e-05
28128,56257,56256,112513,28.35704016685486,1.525473576666453e-05
28228,56457,56456,112913,28.45846128463745,1.5170084845910363e-05
28328,56657,56656,113313,28.562904119491577,1.5086044483851001e-05
28428,56857,56856,113713,28.66449522972107,1.5002606421231444e-05
28529,57059,57058,114117,28.765266180038452,1.4918937141126023e-05
28629,57259,57258,114517,28.870808124542236,1.4836685543758747e-05
28729,57459,57458,114917,28.98716115951538,1.4755012605720003e-05
28829,57659,57658,115317,29.086259365081787,1.4673910858305012e-05
28929,57859,57858,115717,29.187304258346558,1.4593373014588697e-05
29029,58059,58058,116117,29.29400396347046,1.4513391965261338e-05
29129,58259,58258,116517,29.396027326583862,1.4433960771370196e-05
29229,58459,58458,116917,29.49954628944397,1.4355072660792616e-05
29329,58659,58658,117317,29.605151176452637,1.4276721022064467e-05
29429,58859,58858,117717,29.713823080062866,1.4198899400570339e-05
29530,59061,59060,118121,29.822351217269897,1.412083113709544e-05
29630,59261,59260,118521,29.924923181533813,1.4044055930350786e-05
29730,59461,59460,118921,30.027302265167236,1.3967792206863045e-05
29830,59661,59660,119321,30.133381128311157,1.3892034091469082e-05
29930,59861,59860,119721,30.239591360092163,1.3816775843772175e-05
30030,60061,60060,120121,30.347352266311646,1.3742011852258061e-05
30130,60261,60260,120521,30.450016021728516,1.3667736632245829e-05
30230,60461,60460,120921,30.550556182861328,1.3593944821175885e-05
30330,60661,60660,121321,30.653573274612427,1.3520631174841028e-05
30430,60861,60860,121721,30.753499269485474,1.3447790563785466e-05
30531,61063,61062,122125,30.85486912727356,1.3374696591499395e-05
30631,61263,61262,122525,30.95430612564087,1.3302791713261758e-05
30731,61463,61462,122925,31.06964421272278,1.323134509156123e-05
30831,61663,61662,123325,31.182352304458618,1.3160352024723339e-05
30931,61863,61862,123725,31.292527198791504,1.3089807910219068e-05
31031,62063,62062,124125,31.405327081680298,1.3019708241126746e-05
31131,62263,62262,124525,31.507395267486572,1.2950048603807798e-05
31231,62463,62462,124925,31.612488985061646,1.2880824674895394e-05
31331,62663,62662,125325,31.71368908882141,1.2812032218859102e-05
31431,62863,62862,125725,31.817703247070312,1.2743667084967246e-05
31532,63065,63064,126129,31.92434310913086,1.2675047910385669e-05
31632,63265,63264,126529,32.03887724876404,1.2607529470036943e-05
31732,63465,63464,126929,32.144713163375854,1.2540426347793953e-05
31832,63665,63664,127329,32.246196031570435,1.2473734709913572e-05
31932,63865,63864,127729,32.34967613220215,1.2407450796598108e-05
32032,64065,64064,128129,32.449201345443726,1.2341570918836015e-05
32132,64265,64264,128529,32.54858422279358,1.2276091457306583e-05
32232,64465,64464,128929,32.66675114631653,1.2211008859601882e-05
32332,64665,64664,129329,32.76741623878479,1.2146319638728943e-05
32432,64865,64864,129729,32.869649171829224,1.2082020371446252e-05
32533,65067,65066,130133,32.97638416290283,1.2017470510092746e-05
32633,65267,65266,130533,33.07767915725708,1.1953944940703191e-05
32733,65467,65466,130933,33.189101219177246,1.1890799385439199e-05
32833,65667,65666,131333,33.30017113685608,1.1828030657689164e-05
32933,65867,65866,131733,33.40964412689209,1.1765635626103807e-05
33033,66067,66066,132133,33.51306223869324,1.1703611212723357e-05
33133,66267,66266,132533,33.611897230148315,1.1641954391581306e-05
33233,66467,66466,132933,33.713993072509766,1.1580662187235834e-05
33333,66667,66666,133333,33.81589722633362,1.151973167320635e-05
33433,66867,66866,133733,33.91670513153076,1.145915997127233e-05
33534,67069,67068,134137,34.020872354507446,1.1398343880375843e-05
33634,67269,67268,134537,34.122106313705444,1.1338484869761771e-05
33734,67469,67468,134937,34.225759983062744,1.1278976282498303e-05
33834,67669,67668,135337,34.32770323753357,1.1219815419291802e-05
33934,67869,67868,135737,34.430339097976685,1.1160999622212621e-05
34034,68069,68068,136137,34.527913093566895,1.1102526274125163e-05
34134,68269,68268,136537,34.62800312042236,1.1044392797122087e-05
34234,68469,68468,136937,34.73245811462402,1.0986596652116044e-05
34334,68669,68668,137337,34.83179211616516,1.092913533714529e-05
34434,68869,68868,137737,34.93324613571167,1.087200638689396e-05
34535,69071,69070,138141,35.04060912132263,1.0814641039152443e-05
34635,69271,69270,138541,35.1400990486145,1.0758172826412265e-05
34735,69471,69470,138941,35.239885091781616,1.0702029768192477e-05
34835,69671,69670,139341,35.35705494880676,1.0646209535832354e-05
34935,69871,69870,139741,35.463709354400635,1.0590709832984052e-05
35035,70071,70070,140141,35.56255531311035,1.0535528394461525e-05
35135,70271,70270,140541,35.66658616065979,1.0480662985438994e-05
35235,70471,70470,140941,35.76502823829651,1.0426111400662178e-05
35335,70671,70670,141341,35.86672019958496,1.0371871463733768e-05
35435,70871,70870,141741,35.96499824523926,1.0317941026897855e-05
35536,71073,71072,142145,36.0654993057251,1.0263783283944533e-05
35636,71273,71272,142545,36.166359186172485,1.0210468554471236e-05
35736,71473,71472,142945,36.26771521568298,1.0157457022502795e-05
35836,71673,71672,143345,36.368667125701904,1.0104746646564005e-05
35936,71873,71872,143745,36.46716594696045,1.0052335410015979e-05
36036,72073,72072,144145,36.5653293132782,1.0000221320252732e-05
36136,72273,72272,144545,36.67101693153381,9.948402408870986e-06
36236,72473,72472,144945,36.7737090587616,9.896876730314829e-06
36336,72673,72672,145345,36.873839139938354,9.845642362438357e-06
36436,72873,72872,145745,36.977638244628906,9.794697404628907e-06
36537,73075,73074,146149,37.083521127700806,9.74353484946901e-06
36637,73275,73274,146549,37.21228313446045,9.693165944138935e-06
36737,73475,73474,146949,37.33172607421875,9.643080857668941e-06
36837,73675,73674,147349,37.44846320152283,9.593277773582359e-06
36937,73875,73874,147749,37.56352210044861,9.543754895089129e-06
37037,74075,74074,148149,37.67926502227783,9.494510445563372e-06
37137,74275,74274,148549,37.78353214263916,9.445542666678655e-06
37237,74475,74474,148949,37.890079975128174,9.39684981854373e-06
37337,74675,74674,149349,37.9896981716156,9.348430179943802e-06
37437,74875,74874,149749,38.0910861492157,9.300282047109628e-06
37538,75077,75076,150153,38.19508934020996,9.251926307497324e-06
37638,75277,75276,150553,38.2969172000885,9.204318817428131e-06
37738,75477,75476,150953,38.398585081100464,9.156977808712949e-06
37838,75677,75676,151353,38.50137495994568,9.109901645389194e-06
37938,75877,75876,151753,38.60097098350525,9.06308870710001e-06
38038,76077,76076,152153,38.71761107444763,9.016537389877662e-06
38138,76277,76276,152553,38.85112714767456,8.97024610490771e-06
38238,76477,76476,152953,39.005346059799194,8.924213278269528e-06
38338,76677,76676,153353,39.14303421974182,8.878437350907728e-06
38438,76877,76876,153753,39.25026822090149,8.83291677849829e-06
38539,77079,77078,154157,39.354480266571045,8.787198639970328e-06
38639,77279,77278,154557,39.4545202255249,8.742186716186681e-06
38739,77479,77478,154957,39.564836263656616,8.69742558348526e-06
38839,77679,77678,155357,39.68078327178955,8.652913752906591e-06
38939,77879,77878,155757,39.82592225074768,8.608649748757887e-06
39039,78079,78078,156157,39.98680233955383,8.564632108607513e-06
39139,78279,78278,156557,40.163650035858154,8.520859381960493e-06
39239,78479,78478,156957,40.37507104873657,8.477330131968392e-06
39339,78679,78678,157357,40.47745203971863,8.434042933128069e-06
39439,78879,78878,157757,40.65609407424927,8.390996372740759e-06
39540,79081,79080,158161,40.874149322509766,8.347762179717916e-06
39640,79281,79280,158561,40.982991218566895,8.305195075779838e-06
39740,79481,79480,158961,41.08484625816345,8.262864427904646e-06
39840,79681,79680,159361,41.19215226173401,8.220768869818147e-06
39940,79881,79880,159761,41.301215171813965,8.178907046014787e-06
40040,80081,80080,160161,41.40928411483765,8.13727761196053e-06
40140,80281,80280,160561,41.5113160610199,8.095879234201466e-06
40240,80481,80480,160961,41.620946168899536,8.054710589422994e-06
40340,80681,80680,161361,41.83861303329468,8.013770365173272e-06
40440,80881,80880,161761,42.017919063568115,7.973057259006582e-06
40541,81083,81082,162165,42.247716188430786,7.93216624198212e-06
40641,81283,81282,162565,42.44263505935669,7.891905744237378e-06
40741,81483,81482,162965,42.543612241744995,7.85186850499992e-06
40841,81683,81682,163365,42.72900724411011,7.812053261607058e-06
40941,81883,81882,163765,42.85758018493652,7.772458760678725e-06
41041,82083,82082,164165,42.96165204048157,7.733083758506741e-06
41141,82283,82282,164565,43.06507706642151,7.693927020716855e-06
41241,82483,82482,164965,43.169800996780396,7.654987321654853e-06
41341,82683,82682,165365,43.275665283203125,7.616263445389694e-06
41441,82883,82882,165765,43.38475704193115,7.577754183968579e-06
41542,83085,83084,166169,43.490100145339966,7.539076454204235e-06
41642,83285,83284,166569,43.599133253097534,7.500994951635613e-06
41742,83485,83484,166969,43.70434927940369,7.4631244818936705e-06
41842,83685,83684,167369,43.80776500701904,7.425463871914123e-06
41942,83885,83884,167769,43.99910521507263,7.388011956974788e-06
42042,84085,84084,168169,44.17692232131958,7.35076758060331e-06
42142,84285,84284,168569,44.37733316421509,7.313729594061847e-06
42242,84485,84484,168969,44.48134207725525,7.2768968571314685e-06
42342,84685,84684,169369,44.584593296051025,7.24026823721206e-06
42442,84885,84884,169769,44.69068717956543,7.203842609448843e-06
42543,85087,85086,170173,44.79387331008911,7.16725763496288e-06
42643,85287,85286,170573,44.90286898612976,7.131236650136116e-06
42743,85487,85486,170973,45.002530097961426,7.095415318007942e-06
42843,85687,85686,171373,45.10636019706726,7.059792544354096e-06
42943,85887,85886,171773,45.21059727668762,7.0243672419622075e-06
43043,86087,86086,172173,45.312313079833984,6.989138331090712e-06
43143,86287,86286,172573,45.41354322433472,6.954104739154548e-06
43243,86487,86486,172973,45.52088499069214,6.9192654006023495e-06
43343,86687,86686,173373,45.622828006744385,6.884619256872231e-06
43443,86887,86886,173773,45.73828101158142,6.850165256685627e-06
43544,87089,87088,174177,45.94174528121948,6.815560687752278e-06
43644,87289,87288,174577,46.110809087753296,6.781489742640136e-06
43744,87489,87488,174977,46.27103328704834,6.747607816964063e-06
43844,87689,87688,175377,46.37400221824646,6.7139138864022474e-06
43944,87889,87888,175777,46.47498607635498,6.680406933143287e-06
44044,88089,88088,176177,46.58612608909607,6.647085946019172e-06
44144,88289,88288,176577,46.703660011291504,6.613949920010182e-06
44244,88489,88488,176977,46.819880962371826,6.58099785674499e-06
44344,88689,88688,177377,46.99234628677368,6.5482287641530055e-06
44444,88889,88888,177777,47.22457814216614,6.515641656444835e-06
44545,89091,89090,178181,47.43951916694641,6.482912403623686e-06
44645,89291,89290,178581,47.60617804527283,6.450688128178052e-06
44745,89491,89490,178981,47.70934724807739,6.4186429074786614e-06
44845,89691,89690,179381,47.83062124252319,6.386775780018332e-06
44945,89891,89890,179781,48.031583070755005,6.355085790635725e-06
45045,90091,90090,180181,48.13915801048279,6.323571989721938e-06
45145,90291,90290,180581,48.253451108932495,6.292233433956981e-06
45245,90491,90490,180981,48.365581035614014,6.261069185429767e-06
45345,90691,90690,181381,48.46831226348877,6.230078312059861e-06
45445,90891,90890,181781,48.56904220581055,6.199259887835986e-06
45546,91093,91092,182185,48.67323613166809,6.168307385898487e-06
45646,91293,91292,182585,48.777981996536255,6.137832804711906e-06
45746,91493,91492,182985,48.8846001625061,6.1075279183302e-06
45846,91693,91692,183385,48.9891562461853,6.077391822975231e-06
45946,91893,91892,183785,49.09219717979431,6.047423619766005e-06
46046,92093,92092,184185,49.194677114486694,6.017622416051659e-06
46146,92293,92292,184585,49.29855513572693,5.987987324065617e-06
46246,92493,92492,184985,49.40027904510498,5.958517461319691e-06
46346,92693,92692,185385,49.501004219055176,5.929211950894008e-06
46446,92893,92892,185785,49.60478734970093,5.900069920885861e-06
46547,93095,93094,186189,49.71181321144104,5.870801528813013e-06
46647,93295,93294,186589,49.814640283584595,5.841985478237522e-06
46747,93495,93494,186989,49.915300130844116,5.813330314928808e-06
46847,93695,93694,187389,50.0175621509552,5.784835187868471e-06
46947,93895,93894,187789,50.11969304084778,5.756499250526048e-06
47047,94095,94094,188189,50.22571611404419,5.7283216620927856e-06
47147,94295,94294,188589,50.32874417304993,5.7003015858583396e-06
47247,94495,94494,188989,50.447163343429565,5.672438190651915e-06
47347,94695,94694,189389,50.54650115966797,5.6447306499422615e-06
47447,94895,94894,189789,50.6466600894928,5.61717814195004e-06
47548,95097,95096,190193,50.74992823600769,5.589506643035452e-06
47648,95297,95296,190593,50.84984016418457,5.562263284700671e-06
47748,95497,95496,190993,50.94977521896362,5.535172514797879e-06
47848,95697,95696,191393,51.05258226394653,5.50823353060782e-06
47948,95897,95896,191793,51.15896224975586,5.48144553394883e-06
48048,96097,96096,192193,51.26131510734558,5.454807731632171e-06
48148,96297,96296,192593,51.3629412651062,5.428319334839365e-06
48248,96497,96496,192993,51.46465826034546,5.401979559216118e-06
48348,96697,96696,193393,51.5663480758667,5.375787625232161e-06
48448,96897,96896,193793,51.67214918136597,5.349742757503943e-06
48549,97099,97098,194197,51.77845025062561,5.323585935685384e-06
48649,97299,97298,194597,51.88401818275452,5.297834343902858e-06
48749,97499,97498,194997,51.986568212509155,5.272227511842524e-06
48849,97699,97698,195397,52.08934807777405,5.246764681542395e-06
48949,97899,97898,195797,52.19312834739685,5.22144510013245e-06
49049,98099,98098,196197,52.29562711715698,5.196268018480843e-06
49149,98299,98298,196597,52.39695429801941,5.171232691703259e-06
49249,98499,98498,196997,52.51057410240173,5.146338379849339e-06
49349,98699,98698,197397,52.62275409698486,5.121584346210965e-06
49449,98899,98898,197797,52.73303031921387,5.096969858858035e-06
49550,99101,99100,198201,52.837470054626465,5.072250131919366e-06
49650,99301,99300,198601,52.940104246139526,5.047913935088097e-06
49750,99501,99500,199001,53.04196810722351,5.023715105716969e-06
49850,99701,99700,199401,53.14535713195801,4.999652928508329e-06
49950,99901,99900,199801,53.2530403137207,4.975726691870215e-06
50050,100101,100100,200201,53.3644642829895,4.951935688293543e-06
50150,100301,100300,200601,53.468767166137695,4.928279214059409e-06
50250,100501,100500,201001,53.56981825828552,4.904756569533034e-06
50350,100701,100700,201401,53.6709303855896,4.881367059087401e-06
50450,100901,100900,201801,53.77235007286072,4.858109990902602e-06
50551,101103,101102,202205,53.87683415412903,4.834754087025463e-06
50651,101303,101302,202605,53.9776291847229,4.811761150684866e-06
50751,101503,101502,203005,54.0791802406311,4.788898597468498e-06
50851,101703,101702,203405,54.18799901008606,4.7661657510782e-06
50951,101903,101902,203805,54.287660121917725,4.7435619388122915e-06
51051,102103,102102,204205,54.386139154434204,4.721086491744434e-06
51151,102303,102302,204605,54.48935413360596,4.698738744567397e-06
51251,102503,102502,205005,54.595059394836426,4.67651803588588e-06
51351,102703,102702,205405,54.716997146606445,4.65442370798411e-06
51451,102903,102902,205805,54.820436000823975,4.632455106646605e-06
51552,103105,103104,206209,54.92305827140808,4.6103937754140965e-06
51652,103305,103304,206609,55.0226571559906,4.588675919869479e-06
51752,103505,103504,207009,55.12048530578613,4.56708184364518e-06
51852,103705,103704,207409,55.239176988601685,4.5456109068755234e-06
51952,103905,103904,207809,55.37847924232483,4.524262473038207e-06
52052,104105,104104,208209,55.533244132995605,4.50303590985631e-06
52152,104305,104304,208609,55.633039236068726,4.481930587629535e-06
52252,104505,104504,209009,55.73797917366028,4.4609458807438155e-06
52352,104705,104704,209409,55.84005403518677,4.44008116686596e-06
52452,104905,104904,209809,55.94533133506775,4.419335826924423e-06
52553,105107,105106,210213,56.04826331138611,4.398503576999496e-06
52653,105307,105306,210613,56.153748989105225,4.377996319994162e-06
52753,105507,105506,211013,56.277130126953125,4.357606594234406e-06
52853,105707,105706,211413,56.44590210914612,4.337333794270907e-06
52953,105907,105906,211813,56.58954215049744,4.317177317871906e-06
53053,106107,106106,212213,56.71138405799866,4.297136566234023e-06
53153,106307,106306,212613,56.828797340393066,4.277210943642991e-06
53253,106507,106506,213013,56.93524932861328,4.257399857657006e-06
53353,106707,106706,213413,57.03900218009949,4.237702719258374e-06
53453,106907,106906,213813,57.14194631576538,4.218118942136207e-06
53554,107109,107108,214217,57.245851278305054,4.198453801489868e-06
53654,107309,107308,214617,57.34871220588684,4.1790961215606555e-06
53754,107509,107508,215017,57.448331117630005,4.159850058205327e-06
53854,107709,107708,215417,57.547160148620605,4.140715038374712e-06
53954,107909,107908,215817,57.64982724189758,4.12169049185086e-06
54054,108109,108108,216217,57.78003215789795,4.102775851226692e-06
54154,108309,108308,216617,57.95662808418274,4.083970552582838e-06
54254,108509,108508,217017,58.08343815803528,4.065274034718134e-06
54354,108709,108708,217417,58.232728242874146,4.046685739693659e-06
54454,108909,108908,217817,58.34463906288147,4.028205112167068e-06
54555,109111,109110,218221,58.444677114486694,4.009648404477159e-06
54655,109311,109310,218621,58.543519020080566,3.991382522047146e-06
54755,109511,109510,219021,58.64771914482117,3.9732226543964645e-06
54855,109711,109710,219421,58.74995517730713,3.95516825846744e-06
54955,109911,109910,219821,58.85095024108887,3.937218793731326e-06
55055,110111,110110,220221,58.97096014022827,3.9193737228706324e-06
55155,110311,110310,220621,59.07712531089783,3.901632511197682e-06
55255,110511,110510,221021,59.17912030220032,3.883994627014341e-06
55355,110711,110710,221421,59.27898812294006,3.866459541242284e-06
55455,110911,110910,221821,59.38111615180969,3.849026727987626e-06
55556,111113,111112,222225,59.48685121536255,3.831522865416961e-06
55656,111313,111312,222625,59.5897159576416,3.814294039421805e-06
55756,111513,111512,223025,59.69114923477173,3.7971659193340194e-06
55856,111713,111712,223425,59.78925323486328,3.7801379897162253e-06
55956,111913,111912,223825,59.88989210128784,3.7632097383087628e-06
56056,112113,112112,224225,59.98958420753479,3.746380655818998e-06
56156,112313,112312,224625,60.11167120933533,3.7296502350543283e-06
56256,112513,112512,225025,60.23150014877319,3.7130179717656068e-06
56356,112713,112712,225425,60.34554719924927,3.6964833643197807e-06
56456,112913,112912,225825,60.458627223968506,3.680045913899004e-06
56557,113115,113114,226229,60.573596239089966,3.6635422025605246e-06
56657,113315,113314,226629,60.68550205230713,3.6472985387737856e-06
56757,113515,113514,227029,60.8016791343689,3.631150545658939e-06
56857,113715,113714,227429,60.91537308692932,3.6150977346360793e-06
56957,113915,113914,227829,61.0342321395874,3.5991396197010377e-06
57057,114115,114114,228229,61.15578317642212,3.5832757172888128e-06
57157,114315,114314,228629,61.26014423370361,3.5675055463678695e-06
57257,114515,114514,229029,61.36601495742798,3.5518286286233473e-06
57357,114715,114714,229429,61.47215914726257,3.5362444877194963e-06
57457,114915,114914,229829,61.579395055770874,3.520752650323909e-06
57558,115117,115116,230233,61.68844699859619,3.5051991071690087e-06
57658,115317,115316,230633,61.791574001312256,3.4898913768323703e-06
57758,115517,115516,231033,61.896756172180176,3.474674539149808e-06
57858,115717,115716,231433,62.00423717498779,3.4595481300296076e-06
57958,115917,115916,231833,62.112807273864746,3.444511688451795e-06
58058,116117,116116,232233,62.22048830986023,3.4295647549437967e-06
58158,116317,116316,232633,62.33106517791748,3.414706872755212e-06
58258,116517,116516,233033,62.43858623504639,3.3999375876989694e-06
58358,116717,116716,233433,62.54180097579956,3.3852564473989437e-06
58458,116917,116916,233833,62.65843725204468,3.370663002187943e-06
58559,117119,117118,234237,62.778656005859375,3.3560121814881122e-06
58659,117319,117318,234637,62.89924216270447,3.341593651901923e-06
58759,117519,117518,235037,63.00933623313904,3.327261477001474e-06
58859,117719,117718,235437,63.11628603935242,3.313015216356852e-06
58959,117919,117918,235837,63.283374071121216,3.29885443130374e-06
59059,118119,118118,236237,63.44907808303833,3.2847786855520033e-06
59159,118319,118318,236637,63.60206317901611,3.270787545082869e-06
59259,118519,118518,237037,63.73354434967041,3.2568805777448162e-06
59359,118719,118718,237437,63.90878915786743,3.243057354221872e-06
59459,118919,118918,237837,64.10689115524292,3.229317446507438e-06
59560,119121,119120,238241,64.28118515014648,3.2155242764601247e-06
59660,119321,119320,238641,64.62930727005005,3.2019505491993925e-06
59760,119521,119520,239041,64.84549927711487,3.188458863532566e-06
59860,119721,119720,239441,65.09259128570557,3.1750488005229006e-06
59960,119921,119920,239841,65.29561805725098,3.1617199431699828e-06
60060,120121,120120,240241,65.45650815963745,3.148471876535181e-06
60160,120321,120320,240641,65.764484167099,3.1353041875904403e-06
60260,120521,120520,241041,65.94493699073792,3.12221646560781e-06
60360,120721,120720,241441,66.07479119300842,3.109208301734977e-06
60460,120921,120920,241841,66.19477415084839,3.096279288879458e-06
60561,121123,121122,242245,66.30953598022461,3.0833009160880306e-06
60661,121323,121322,242645,66.42448616027832,3.0705297745346636e-06
60761,121523,121522,243045,66.54067516326904,3.057836571767367e-06
60861,121723,121722,243445,66.65636825561523,3.0452209085410903e-06
60961,121923,121922,243845,66.77815818786621,3.0326823878801493e-06
61061,122123,122122,244245,66.8913562297821,3.0202206151558014e-06
61161,122323,122322,244645,67.00161409378052,3.0078351968175384e-06
61261,122523,122522,245045,67.11826729774475,2.995525741793433e-06
61361,122723,122722,245445,67.2259521484375,2.983291860656169e-06
61461,122923,122922,245845,67.33637809753418,2.9711331660294383e-06
61562,123125,123124,246249,67.44893908500671,2.9589288098924783e-06
61662,123325,123324,246649,67.5767571926117,2.9469200756642875e-06
61762,123525,123524,247049,67.6853392124176,2.934985372665422e-06
61862,123725,123724,247449,67.79008316993713,2.9231243211627506e-06
61962,123925,123924,247849,67.89725518226624,2.9113365428115323e-06
62062,124125,124124,248249,68.01188921928406,2.8996216609782116e-06
62162,124325,124324,248649,68.15599918365479,2.8879793009363483e-06
62262,124525,124524,249049,68.30095219612122,2.876409090102088e-06
62362,124725,124724,249449,68.40800213813782,2.864910657114372e-06
62462,124925,124924,249849,68.50756025314331,2.853483632643486e-06
62563,125127,125126,250253,68.60940313339233,2.8420144466557163e-06
62663,125327,125326,250653,68.70946717262268,2.830729842905204e-06
62763,125527,125526,251053,68.80888605117798,2.819515546092488e-06
62863,125727,125726,251453,68.90914916992188,2.8083711939183947e-06
62963,125927,125926,251853,69.01304602622986,2.797296425574582e-06
63063,126127,126126,252253,69.11284303665161,2.7862908817192455e-06
63163,126327,126326,252653,69.21514010429382,2.775354205192744e-06
63263,126527,126526,253053,69.31524419784546,2.7644860399032016e-06
63363,126727,126726,253453,69.41325807571411,2.7536860318430737e-06
63463,126927,126926,253853,69.5091462135315,2.7429538284824577e-06
63564,127129,127128,254257,69.61159706115723,2.7321827708355152e-06
63664,127329,127328,254657,69.72320103645325,2.721585794767247e-06
63764,127529,127528,255057,69.8349711894989,2.711055572255011e-06
63864,127729,127728,255457,70.00159811973572,2.700591756681407e-06
63964,127929,127928,255857,70.1339361667633,2.6901940038882488e-06
64064,128129,128128,256257,70.23588299751282,2.6798619706745087e-06
64164,128329,128328,256657,70.33814716339111,2.6695953156258623e-06
64264,128529,128528,257057,70.46089816093445,2.659393699021787e-06
64364,128729,128728,257457,70.62414693832397,2.649256782559759e-06
64464,128929,128928,257857,70.77940917015076,2.639184229190856e-06
64565,129131,129130,258261,70.89299511909485,2.6290759409266197e-06
64665,129331,129330,258661,70.9902720451355,2.6191317449486765e-06
64765,129531,129530,259061,71.10234498977661,2.6092509074161096e-06
64865,129731,129730,259461,71.22846531867981,2.5994330977607984e-06
64965,129931,129930,259861,71.33300924301147,2.589677986323251e-06
65065,130131,130130,260261,71.4307131767273,2.5799852454567913e-06
65165,130331,130330,260661,71.52759623527527,2.5703545484942893e-06
65265,130531,130530,261061,71.62449836730957,2.5607855706475568e-06
65365,130731,130730,261461,71.72826218605042,2.5512779882598767e-06
65465,130931,130930,261861,71.84188532829285,2.5418314792641497e-06
65566,131133,131132,262265,71.94398427009583,2.5323521709510194e-06
65666,131333,131332,262665,72.04446816444397,2.523027450649723e-06
65766,131533,131532,263065,72.143470287323,2.5137628423610064e-06
65866,131733,131732,263465,72.24342608451843,2.5045580298119715e-06
65966,131933,131932,263865,72.3437283039093,2.4954126978385856e-06
66066,132133,132132,264265,72.44011116027832,2.4863265324961008e-06
66166,132333,132332,264665,72.53612613677979,2.4772992213185746e-06
66266,132533,132532,265065,72.63615322113037,2.468330453227136e-06
66366,132733,132732,265465,72.73270034790039,2.4594199184772105e-06
66466,132933,132932,265865,72.82887411117554,2.4505673088944696e-06
66567,133135,133134,266269,72.92542719841003,2.4416846569844214e-06
66667,133335,133334,266669,73.02438521385193,2.4329475486101967e-06
66767,133535,133534,267069,73.12055611610413,2.424267444997775e-06
66867,133735,133734,267469,73.2204282283783,2.415644042512235e-06
66967,133935,133934,267869,73.32311725616455,2.407077039411883e-06
67067,134135,134134,268269,73.42170596122742,2.398566135092775e-06
67167,134335,134334,268669,73.52293038368225,2.3901110302742894e-06
67267,134535,134534,269069,73.61944723129272,2.3817114267139655e-06
67367,134735,134734,269469,73.71494507789612,2.373367027660072e-06
67467,134935,134934,269869,73.81232523918152,2.3650775374344425e-06
67568,135137,135136,270273,73.9314432144165,2.3567605878678364e-06
67668,135337,135336,270673,74.03434324264526,2.3485805752968476e-06
67768,135537,135536,271073,74.13284730911255,2.3404545891950986e-06
67868,135737,135736,271473,74.22797012329102,2.3323823390859886e-06
67968,135937,135936,271873,74.32362914085388,2.324363535425193e-06
68068,136137,136136,272273,74.41878724098206,2.3163978898000402e-06
68168,136337,136336,272673,74.51795625686646,2.3084851152131723e-06
68268,136537,136536,273073,74.61405110359192,2.3006249257527494e-06
68368,136737,136736,273473,74.7115273475647,2.292817036715171e-06
68468,136937,136936,273873,74.80643010139465,2.28506116463904e-06
68569,137139,137138,274277,74.90263414382935,2.277280245826642e-06
68669,137339,137338,274677,75.00094103813171,2.269628074550235e-06
68769,137539,137538,275077,75.09928226470947,2.262027073533906e-06
68869,137739,137738,275477,75.2052092552185,2.2544769639386698e-06
68969,137939,137938,275877,75.31380105018616,2.246977468094862e-06
69069,138139,138138,276277,75.41963124275208,2.239528309248918e-06
69169,138339,138338,276677,75.51684021949768,2.232129211675099e-06
69269,138539,138538,277077,75.61428713798523,2.224779901255263e-06
69369,138739,138738,277477,75.71352410316467,2.217480104439679e-06
69469,138939,138938,277877,75.81177926063538,2.210229549177222e-06
69570,139141,139140,278281,75.91126132011414,2.2029561950037375e-06
69670,139341,139340,278681,76.02415418624878,2.195803796210658e-06
69770,139541,139540,279081,76.136057138443,2.188699826214872e-06
69870,139741,139740,279481,76.23487734794617,2.1816440171058295e-06
69970,139941,139940,279881,76.33326816558838,2.1746361021918227e-06
70070,140141,140140,280281,76.43243217468262,2.1676758158810486e-06
70170,140341,140340,280681,76.5362823009491,2.160762893294456e-06
70270,140541,140540,281081,76.63513922691345,2.153897071094307e-06
70370,140741,140740,281481,76.7354941368103,2.1470780865682e-06
70470,140941,140940,281881,76.83453917503357,2.1403056783586055e-06
70571,141143,141142,282285,76.93393421173096,2.1335125582210985e-06
70671,141343,141342,282685,77.0343542098999,2.126832981776931e-06
70771,141543,141542,283085,77.13158822059631,2.1201992007846804e-06
70871,141743,141742,283485,77.23248624801636,2.1136109580559547e-06
70971,141943,141942,283885,77.33168816566467,2.1070679973443883e-06
71071,142143,142142,284285,77.43060302734375,2.100570063260819e-06
71171,142343,142342,284685,77.52851915359497,2.094116901446059e-06
71271,142543,142542,285085,77.62760019302368,2.087708259066037e-06
71371,142743,142742,285485,77.72929000854492,2.0813438834648194e-06
71471,142943,142942,285885,77.82766222953796,2.0750235232705427e-06
71572,143145,143144,286289,77.9301540851593,2.0686843828919825e-06
71672,143345,143344,286689,78.02818727493286,2.0624517383600515e-06
71772,143545,143544,287089,78.14102911949158,2.056262359115471e-06
71872,143745,143744,287489,78.25385928153992,2.050115997800982e-06
71972,143945,143944,287889,78.3537962436676,2.0440124083681556e-06
72072,144145,144144,288289,78.4560010433197,2.0379513453490074e-06
72172,144345,144344,288689,78.55420231819153,2.0319325641643383e-06
72272,144545,144544,289089,78.66750812530518,2.0259558216145032e-06
72372,144745,144744,289489,78.88346028327942,2.0200208753586987e-06
72472,144945,144944,289889,79.01966214179993,2.0141274837413022e-06
72573,145147,145146,290293,79.14887714385986,2.008217093332123e-06
72673,145347,145346,290693,79.30927801132202,2.002406499793463e-06
72773,145547,145546,291093,79.42158794403076,1.996636739963973e-06
72873,145747,145746,291493,79.55884003639221,1.9909075760700736e-06
72973,145947,145946,291893,79.71916913986206,1.985218771099692e-06
73073,146147,146146,292293,79.86513113975525,1.979570089524111e-06
73173,146347,146346,292693,79.9888813495636,1.9739612963998257e-06
73273,146547,146546,293093,80.1880111694336,1.9683921578082133e-06
73373,146747,146746,293493,80.33305597305298,1.9628624408575366e-06
73473,146947,146946,293893,80.45786499977112,1.9573719130255463e-06
73574,147149,147148,294297,80.58053922653198,1.951866023886824e-06
73674,147349,147348,294697,80.71064019203186,1.946453568571144e-06
73774,147549,147548,295097,80.85702419281006,1.9410796095815656e-06
73874,147749,147748,295497,80.98993015289307,1.9357439186554453e-06
73974,147949,147948,295897,81.133798122406,1.930446268220333e-06
74074,148149,148148,296297,81.2742862701416,1.9251864315266883e-06
74174,148349,148348,296697,81.39790916442871,1.919964183130938e-06
74274,148549,148548,297097,81.51293802261353,1.9147792981028865e-06
74374,148749,148748,297497,81.6778461933136,1.9096315527452103e-06
74474,148949,148948,297897,81.82833409309387,1.904520723824285e-06
74575,149151,149150,298301,81.96236538887024,1.8993960326464324e-06
74675,149351,149350,298701,82.07087731361389,1.8943587350300446e-06
74775,149551,149550,299101,82.18559908866882,1.8893576883488883e-06
74875,149751,149750,299501,82.29206013679504,1.884392672963078e-06
74975,149951,149950,299901,82.41211700439453,1.879463470399839e-06
75075,150151,150150,300301,82.5331220626831,1.8745698629375028e-06
75175,150351,150350,300701,82.64353895187378,1.8697116340249785e-06
75275,150551,150550,301101,82.79541301727295,1.8648885677041297e-06
75375,150751,150750,301501,82.9594361782074,1.860100448892799e-06
75475,150951,150950,301901,83.09409427642822,1.8553470635185739e-06
75576,151153,151152,302305,83.23633933067322,1.850581183229221e-06
75676,151353,151352,302705,83.44004416465759,1.8458969680701343e-06
75776,151553,151552,303105,83.59899497032166,1.841246847050018e-06
75876,151753,151752,303505,83.74046897888184,1.836630609614162e-06
75976,151953,151952,303905,83.87303519248962,1.832048046098284e-06
76076,152153,152152,304305,84.02393126487732,1.8274989473565958e-06
76176,152353,152352,304705,84.22670221328735,1.8229831058025645e-06
76276,152553,152552,305105,84.40283608436584,1.818500313879528e-06
76376,152753,152752,305505,84.54468512535095,1.8140503654104226e-06
76476,152953,152952,305905,84.73232007026672,1.8096330548917877e-06
76577,153155,153154,306309,84.87966799736023,1.8052044924095253e-06
76677,153355,153354,306709,85.05643320083618,1.8008521664431159e-06
76777,153555,153554,307109,85.27463126182556,1.7965318653049106e-06
76877,153755,153754,307509,85.39880013465881,1.7922433870349087e-06
76977,153955,153954,307909,85.51560616493225,1.7879865303773963e-06
77077,154155,154154,308309,85.62580418586731,1.7837610951737734e-06
77177,154355,154354,308709,85.75929403305054,1.7795668817952114e-06
77277,154555,154554,309109,85.87474822998047,1.775403691839618e-06
77377,154755,154754,309509,85.98389029502869,1.7712713274828856e-06
77477,154955,154954,309909,86.08848309516907,1.7671695917911344e-06
77578,155157,155156,310313,86.20611214637756,1.763057728629924e-06
77678,155357,155356,310713,86.35916423797607,1.759016964202382e-06
77778,155557,155556,311113,86.51732611656189,1.755006240998e-06
77878,155757,155756,311513,86.73001909255981,1.7510253653561124e-06
77978,155957,155956,311913,86.87972521781921,1.7470741444808845e-06
78078,156157,156156,312313,87.0017831325531,1.7431523867505794e-06
78178,156357,156356,312713,87.17805218696594,1.739259901037415e-06
78278,156557,156556,313113,87.32341194152832,1.7353964971853342e-06
78378,156757,156756,313513,87.43999528884888,1.7315619860625706e-06
78478,156957,156956,313913,87.5625159740448,1.7277561789569766e-06
78579,157159,157158,314317,87.68316221237183,1.7239412587906194e-06
78679,157359,157358,314717,87.80998826026917,1.7201925799825884e-06
78779,157559,157558,315117,87.92280602455139,1.7164720431074261e-06
78879,157759,157758,315517,88.03131127357483,1.7127794629624441e-06
78979,157959,157958,315917,88.13860416412354,1.7091146549861194e-06
79079,158159,158158,316317,88.26107335090637,1.7054774360387703e-06
79179,158359,158358,316717,88.4091432094574,1.7018676233897183e-06
79279,158559,158558,317117,88.51409316062927,1.698285035077022e-06
79379,158759,158758,317517,88.61962914466858,1.6947294902313227e-06
79479,158959,158958,317917,88.72694420814514,1.6912008087318635e-06
79580,159161,159160,318321,88.85969734191895,1.6876639254544311e-06
79680,159361,159360,318721,88.97842311859131,1.684188697519512e-06
79780,159561,159560,319121,89.07598423957825,1.6807397956576483e-06
79880,159761,159760,319521,89.18444609642029,1.6773170429601805e-06
79980,159961,159960,319921,89.30364608764648,1.6739202634554277e-06
80080,160161,160160,320321,89.40490818023682,1.6705492819888668e-06
80180,160361,160360,320721,89.55618715286255,1.6672039242535504e-06
80280,160561,160560,321121,89.71426820755005,1.6638840163777806e-06
80380,160761,160760,321521,89.835764169693,1.660589385918047e-06
80480,160961,160960,321921,89.97450232505798,1.6573198610569068e-06
80581,161163,161162,322325,90.09926724433899,1.6540429497962114e-06
80681,161363,161362,322725,90.2290141582489,1.6508233700928283e-06
80781,161563,161562,323125,90.36642217636108,1.6476283833373464e-06
80881,161763,161762,323525,90.60947513580322,1.6444578209271493e-06
80981,161963,161962,323925,90.72151613235474,1.6413115151153036e-06
81081,162163,162162,324325,90.83162808418274,1.6381892988558482e-06
81181,162363,162362,324725,90.94294810295105,1.6350910059707293e-06
81281,162563,162562,325125,91.0874490737915,1.6320164711392937e-06
81381,162763,162762,325525,91.20136022567749,1.6289655296477216e-06
81481,162963,162962,325925,91.30678820610046,1.6259380180947523e-06
81582,163165,163164,326329,91.41367721557617,1.6229038476649173e-06
81682,163365,163364,326729,91.51982116699219,1.619922937826256e-06
81782,163565,163564,327129,91.62342619895935,1.6169649696847463e-06
81882,163765,163764,327529,91.73388123512268,1.614029782964095e-06
81982,163965,163964,327929,91.86147713661194,1.6111172178562461e-06
82082,164165,164164,328329,91.98789715766907,1.608227115614968e-06
82182,164365,164364,328729,92.09929704666138,1.6053593179189702e-06
82282,164565,164564,329129,92.20586705207825,1.6025136679114424e-06
82382,164765,164764,329529,92.30565214157104,1.599690008754685e-06
82482,164965,164964,329929,92.41766500473022,1.5968881850724742e-06
82583,165167,165166,330333,92.53006410598755,1.594080349363094e-06
82683,165367,165366,330733,92.9722511768341,1.5913219471252603e-06
82783,165567,165566,331133,93.081866979599,1.588584916599724e-06
82883,165767,165766,331533,93.19315934181213,1.5858691054244984e-06
82983,165967,165966,331933,93.29824829101562,1.5831743617700876e-06
83083,166167,166166,332333,93.41257500648499,1.5805005350361195e-06
83183,166367,166366,332733,93.52518200874329,1.5778474748757486e-06
83283,166567,166566,333133,93.64514517784119,1.5752150326098378e-06
83383,166767,166766,333533,93.75449514389038,1.572603059155467e-06
83483,166967,166966,333933,93.86165809631348,1.5700114072136505e-06
83584,167169,167168,334337,93.97964024543762,1.5674143163533773e-06
83684,167369,167368,334737,94.10658717155457,1.5648630669727027e-06
83784,167569,167568,335137,94.21281838417053,1.5623316993091795e-06
83884,167769,167768,335537,94.32114720344543,1.5598200690349098e-06
83984,167969,167968,335937,94.43762516975403,1.5573280321679621e-06
84084,168169,168168,336337,94.56369614601135,1.5548554459424362e-06
84184,168369,168368,336737,94.68600010871887,1.5524021681994328e-06
84284,168569,168568,337137,94.79502415657043,1.5499680578256143e-06
84384,168769,168768,337537,94.9050281047821,1.5475529739526512e-06
84484,168969,168968,337937,95.00996112823486,1.5451567769376212e-06
84585,169171,169170,338341,95.11934113502502,1.5427556474698198e-06
84685,169371,169370,338741,95.2494101524353,1.5403969933505532e-06
84785,169571,169570,339141,95.35683917999268,1.5380568098468841e-06
84885,169771,169770,339541,95.45274424552917,1.535734960562266e-06
84985,169971,169970,339941,95.55066227912903,1.5334313094921342e-06
85085,170171,170170,340341,95.64839720726013,1.5311457214689604e-06
85185,170371,170370,340741,95.74668216705322,1.5288780623743324e-06
85285,170571,170570,341141,95.86059904098511,1.526628198387049e-06
85385,170771,170770,341541,95.98376607894897,1.5243959968526471e-06
85485,170971,170970,341941,96.11770820617676,1.5221813256097273e-06
85586,171173,171172,342345,96.23578596115112,1.5199621680827842e-06
85686,171373,171372,342745,96.33239030838013,1.5177823365159705e-06
85786,171573,171572,343145,96.43331933021545,1.5156196423009276e-06
85886,171773,171772,343545,96.5825469493866,1.5134739568266023e-06
85986,171973,171972,343945,96.75318717956543,1.5113451514983241e-06
86086,172173,172172,344345,96.85284924507141,1.5092330991083433e-06
86186,172373,172372,344745,96.9531421661377,1.5071376727685602e-06
86286,172573,172572,345145,97.05555629730225,1.5050587465666602e-06
86386,172773,172772,345545,97.15552735328674,1.502996195389828e-06
86486,172973,172972,345945,97.27389025688171,1.5009498945678348e-06
86587,173175,173174,346349,97.48162627220154,1.4988994999018596e-06
86687,173375,173374,346749,97.59139513969421,1.4968854890651688e-06
86787,173575,173574,347149,97.72366714477539,1.494887358749664e-06
86887,173775,173774,347549,97.83290123939514,1.4929049870984796e-06
86987,173975,173974,347949,97.93794107437134,1.4909382537904246e-06
87087,174175,174174,348349,98.0398530960083,1.4889870386305271e-06
87187,174375,174374,348749,98.14783310890198,1.4870512223823873e-06
87287,174575,174574,349149,98.24815917015076,1.4851306864376108e-06
87387,174775,174774,349549,98.35274600982666,1.4832253130428921e-06
87487,174975,174974,349949,98.45888113975525,1.4813349852828165e-06
87588,175177,175176,350353,98.5620322227478,1.479440907684181e-06
87688,175377,175376,350753,98.66804313659668,1.4775804702262628e-06
87788,175577,175576,351153,98.78160119056702,1.4757347303277195e-06
87888,175777,175776,351553,98.97549104690552,1.4739035738584341e-06
87988,175977,175976,351953,99.13419532775879,1.472086887270369e-06
88088,176177,176176,352353,99.27405118942261,1.4702845579719397e-06
88188,176377,176376,352753,99.43142294883728,1.4684964739474555e-06
88288,176577,176576,353153,99.57987403869629,1.4667225239311733e-06
88388,176777,176776,353553,99.78443312644958,1.4649625973142203e-06
88488,176977,176976,353953,99.91965126991272,1.4632165841767938e-06
88589,177179,177178,354357,100.0458812713623,1.4614671226851623e-06
88689,177379,177378,354757,100.19044423103333,1.4597487462110185e-06
88789,177579,177578,355157,100.35189199447632,1.4580439569882368e-06
88889,177779,177778,355557,100.48634505271912,1.4563526476187764e-06
88989,177979,177978,355957,100.61389803886414,1.4546747120474548e-06
89089,178179,178178,356357,100.73774313926697,1.4530100443197464e-06
89189,178379,178378,356757,100.85363411903381,1.4513585399173698e-06
89289,178579,178578,357157,100.96205425262451,1.449720094158862e-06
89389,178779,178778,357557,101.06928014755249,1.4480946036842707e-06
89489,178979,178978,357957,101.17774105072021,1.4464819654288502e-06
89590,179181,179180,358361,101.30249333381653,1.4448661425046581e-06
89690,179381,179380,358761,101.42164301872253,1.443279028929558e-06
89790,179581,179580,359161,101.53781723976135,1.4417044619077524e-06
89890,179781,179780,359561,101.65390801429749,1.4401423414844319e-06
89990,179981,179980,359961,101.77976608276367,1.4385925681442626e-06
90090,180181,180180,360361,101.8983039855957,1.437055042820718e-06
90190,180381,180380,360761,102.01084613800049,1.4355296675786023e-06
90290,180581,180580,361161,102.12431526184082,1.4340163447196163e-06
90390,180781,180780,361561,102.23787522315979,1.432514977630394e-06
90490,180981,180980,361961,102.34231519699097,1.4310254699660522e-06
90591,181183,181182,362365,102.46240615844727,1.4295330079215403e-06
90691,181383,181382,362765,102.57666826248169,1.4280670495519363e-06
90791,181583,181582,363165,102.69147515296936,1.4266126651034025e-06
90891,181783,181782,363565,102.79964113235474,1.4251697609257057e-06
90991,181983,181982,363965,102.90350413322449,1.4237382443122814e-06
91091,182183,182182,364365,103.03303408622742,1.4223180227652558e-06
91191,182383,182382,364765,103.20101809501648,1.4209090048431104e-06
91291,182583,182582,365165,103.31295204162598,1.4195110994672459e-06
91391,182783,182782,365565,103.42662715911865,1.4181242161469805e-06
91491,182983,182982,365965,103.5311541557312,1.4167482654553145e-06
91592,183185,183184,366369,103.64447736740112,1.4153695613472516e-06
91692,183385,183384,366769,103.80086016654968,1.4140153160225222e-06
91792,183585,183584,367169,103.94320893287659,1.4126717368033945e-06
91892,183785,183784,367569,104.08269119262695,1.4113387365096943e-06
91992,183985,183984,367969,104.25820112228394,1.4100162286344663e-06
92092,184185,184184,368369,104.42326617240906,1.4087041271765727e-06
92192,184385,184384,368769,104.56827807426453,1.4074023466679913e-06
92292,184585,184584,369169,104.82582521438599,1.4061108024713637e-06
92392,184785,184784,369569,105.03728222846985,1.4048294103705945e-06
92492,184985,184984,369969,105.26979303359985,1.4035580868439076e-06
92593,185187,185186,370373,105.52982926368713,1.402284185577777e-06
92693,185387,185386,370773,105.74928307533264,1.4010328495400257e-06
92793,185587,185586,371173,105.93291902542114,1.3997913341642846e-06
92893,185787,185786,371573,106.14074420928955,1.3985595584414396e-06
92993,185987,185986,371973,106.31491422653198,1.3973374416603614e-06
93093,186187,186186,372373,106.42064619064331,1.3961249039379972e-06
93193,186387,186386,372773,106.55228114128113,1.3949218657123098e-06
93293,186587,186586,373173,106.73558306694031,1.3937282484210587e-06
93393,186787,186786,373573,106.87419509887695,1.3925439736077279e-06
93493,186987,186986,373973,106.98887228965759,1.3913689637980936e-06
93594,187189,187188,374377,107.1040723323822,1.3901915296867567e-06
93694,187389,187388,374777,107.26602506637573,1.3890349098432154e-06
93794,187589,187588,375177,107.45153522491455,1.3878873246357019e-06
93894,187789,187788,375577,107.5809690952301,1.3867486985945261e-06
93994,187989,187988,375977,107.6941351890564,1.3856189570908606e-06
94094,188189,188188,376377,107.84236311912537,1.38449802570958e-06
94194,188389,188388,376777,108.03728818893433,1.3833858307656064e-06
94294,188589,188588,377177,108.15611219406128,1.3822822991316638e-06
94394,188789,188788,377577,108.28355002403259,1.3811873582845045e-06
94494,188989,188988,377977,108.39712715148926,1.380100935891496e-06
94595,189191,189190,378381,108.50991415977478,1.3790122236024353e-06
94695,189391,189390,378781,108.650071144104,1.3779427080479144e-06
94795,189591,189590,379181,108.81130337715149,1.376881497565118e-06
94895,189791,189790,379581,109.03955721855164,1.3758285222432733e-06
94995,189991,189990,379981,109.2151780128479,1.374783712646331e-06
95095,190191,190190,380381,109.3678891658783,1.3737469999185782e-06
95195,190391,190390,380781,109.56848621368408,1.3727183158601186e-06
95295,190591,190590,381181,109.86159110069275,1.3716975926498783e-06
95395,190791,190790,381581,110.04809403419495,1.3706847629116834e-06
95495,190991,190990,381981,110.25134801864624,1.3696797599346017e-06
95596,191193,191192,382385,110.38564419746399,1.368672584022339e-06
95696,191393,191392,382785,110.58093118667603,1.367683112962588e-06
95796,191593,191592,383185,110.73061513900757,1.3667012708478613e-06
95896,191793,191792,383585,110.82876229286194,1.3657269930463281e-06
95996,191993,191992,383985,110.9324791431427,1.3647602150997397e-06
96096,192193,192192,384385,111.0347592830658,1.3638008733392518e-06
96196,192393,192392,384785,111.13786911964417,1.3628489047718675e-06
96296,192593,192592,385185,111.23613429069519,1.3619042464747929e-06
96396,192793,192792,385585,111.3360960483551,1.3609668361281709e-06
96496,192993,192992,385985,111.44344401359558,1.360036612080165e-06
96597,193195,193194,386389,111.54480528831482,1.3591043179385103e-06
96697,193395,193394,386789,111.66218709945679,1.358188353514031e-06
96797,193595,193594,387189,111.78188800811768,1.3572793923773275e-06
96897,193795,193794,387589,111.89626812934875,1.3563773748001648e-06
96997,193995,193994,387989,112.03595519065857,1.3554822410965038e-06
97097,194195,194194,388389,112.14686799049377,1.35459393284761e-06
97197,194395,194394,388789,112.29300832748413,1.3537123913264018e-06
97297,194595,194594,389189,112.4224591255188,1.3528375585785545e-06
97397,194795,194794,389589,112.55034232139587,1.3519693771399977e-06
97497,194995,194994,389989,112.65154314041138,1.351107789933584e-06
97598,195197,195196,390393,112.86236333847046,1.3502442227272008e-06
97698,195397,195396,390793,113.00616216659546,1.349395719271456e-06
97798,195597,195596,391193,113.11509108543396,1.348553640899381e-06
97898,195797,195796,391593,113.2205183506012,1.3477179327329728e-06
97998,195997,195996,391993,113.3239471912384,1.3468885396055964e-06
98098,196197,196196,392393,113.46361708641052,1.3460654073491742e-06
98198,196397,196396,392793,113.58850312232971,1.3452484819625905e-06
98298,196597,196596,393193,113.73002600669861,1.3444377100831858e-06
98398,196797,196796,393593,113.86904120445251,1.3436330384876309e-06
98498,196997,196996,393993,114.04113006591797,1.3428344145000124e-06
98599,197199,197198,394397,114.27629709243774,1.3420338897748264e-06
98699,197399,197398,394797,114.46716022491455,1.3412472640671224e-06
98799,197599,197598,395197,114.59969997406006,1.3404665303278835e-06
98899,197799,197798,395597,114.73124814033508,1.3396916374270527e-06
98999,197999,197998,395997,114.84335613250732,1.338922534672346e-06
99099,198199,198198,396397,114.95711421966553,1.3381591725322445e-06
99199,198399,198398,396797,115.08629727363586,1.3374015005807464e-06
99299,198599,198598,397197,115.19669818878174,1.3366494697956206e-06
99399,198799,198798,397597,115.30324411392212,1.335903031252909e-06
99499,198999,198998,397997,115.41541409492493,1.3351621364456628e-06
99600,199201,199200,398401,115.55123710632324,1.3344194110065009e-06
99700,199401,199400,398801,115.67147922515869,1.3336895139686216e-06
99800,199601,199600,399201,115.78401732444763,1.3329650172670143e-06
99900,199801,199800,399601,115.89904737472534,1.332245873735849e-06
100000,200001,200000,400001,116.01496505737305,1.3315320367501845e-06


==> plot_data/bilinear_matrix_game_n500/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012600421905517578,2.018959020339561
200,201,200,401,0.14514613151550293,0.046482251948234084
400,401,400,801,0.2978670597076416,0.01712120879549692
601,602,601,1203,0.43784022331237793,0.010238352144301867
801,802,801,1603,0.5829730033874512,0.006553442772398745
1001,1002,1001,2003,0.7231240272521973,0.004385682950619011
1201,1202,1201,2403,0.8626072406768799,0.003197778950946866
1401,1402,1401,2803,1.0024261474609375,0.002496321008503863
1602,1603,1602,3205,1.163182258605957,0.002144660757615812
1802,1803,1802,3605,1.29364013671875,0.001762637810262336
2002,2003,2002,4005,1.4332520961761475,0.0015091980552559801
2202,2203,2202,4405,1.6063041687011719,0.0012087647514370439
2402,2403,2402,4805,1.7513999938964844,0.0010289858283729944
2603,2604,2603,5207,1.8973362445831299,0.0008925435566486958
2803,2804,2803,5607,2.0444180965423584,0.0008015520107389197
3003,3004,3003,6007,2.1909031867980957,0.0007289576997704426
3203,3204,3203,6407,2.3724770545959473,0.0006617447243810016
3403,3404,3403,6807,2.5353879928588867,0.0006131100527668779
3604,3605,3604,7209,2.6904311180114746,0.0005680655402142006
3804,3805,3804,7609,2.863551139831543,0.00048022264511595044
4004,4005,4004,8009,3.0355851650238037,0.00043212050886599706
4204,4205,4204,8409,3.1889290809631348,0.000393116042656765
4404,4405,4404,8809,3.331102132797241,0.0003666199428392579
4605,4606,4605,9211,3.4773762226104736,0.0003451532971075256
4805,4806,4805,9611,3.6228091716766357,0.00032846386195348946
5005,5006,5005,10011,3.7640531063079834,0.0003145392112841674
5205,5206,5205,10411,3.9029722213745117,0.00030251142235609215
5405,5406,5405,10811,4.054957151412964,0.00028821983850401523
5606,5607,5606,11213,4.198130130767822,0.0002738558083393277
5806,5807,5806,11613,4.33680534362793,0.0002636576222328156
6006,6007,6006,12013,4.494132995605469,0.0002550453263141989
6206,6207,6206,12413,4.657612085342407,0.0002475459908481011
6406,6407,6406,12813,4.796328067779541,0.0002409047627142882
6607,6608,6607,13215,4.9418933391571045,0.0002346104783932992
6807,6808,6807,13615,5.152656316757202,0.00022923018703085668
7007,7008,7007,14015,5.427306175231934,0.0002243568267627466
7207,7208,7207,14415,5.687941312789917,0.00021990372138149208
7407,7408,7407,14815,5.9810802936553955,0.0002158119315476405
7608,7609,7608,15217,6.259033203125,0.00021201712334363766
7808,7809,7808,15617,6.506990194320679,0.00020810533579128433
8008,8009,8008,16017,6.742325067520142,0.00020462043559535262
8208,8209,8208,16417,6.897526025772095,0.00019918143092702428
8408,8409,8408,16817,7.043233156204224,0.0001953078143870299
8609,8610,8609,17219,7.217888116836548,0.00019186561505209513
8809,8810,8809,17619,7.3665242195129395,0.00018874806386831746
9009,9010,9009,18019,7.521957159042358,0.0001858670233743703
9209,9210,9209,18419,7.663906097412109,0.000183179331511306
9409,9410,9409,18819,7.807445049285889,0.00018065534051514326
9610,9611,9610,19221,7.941411256790161,0.00017826164346721222
9810,9811,9810,19621,8.074471950531006,0.000176005145036593
10010,10011,10010,20021,8.223432064056396,0.00017194113344987783
10210,10211,10210,20421,8.354803085327148,0.00016743146783829504
10410,10411,10410,20821,8.486855030059814,0.00016424816011725076
10611,10612,10611,21223,8.630044937133789,0.0001615453071910808
10811,10812,10811,21623,8.790509223937988,0.00015915931460213953
11011,11012,11011,22023,8.933178186416626,0.000156494203539692
11211,11212,11211,22423,9.059962272644043,0.00015407193762690633
11411,11412,11411,22823,9.192383050918579,0.00015197881750619153
11612,11613,11612,23225,9.324392080307007,0.00014998039132118108
11812,11813,11812,23625,9.46609902381897,0.0001482286014210995
12012,12013,12012,24025,9.60834002494812,0.00014662753605077162
12212,12213,12212,24425,9.78330397605896,0.00014349315766923722
12412,12413,12412,24825,10.010026216506958,0.00014067479182094144
12613,12614,12613,25227,10.209289073944092,0.0001383935801344753
12813,12814,12813,25627,10.541073322296143,0.00013641820828361962
13013,13014,13013,26027,10.813481092453003,0.00013463503462371373
13213,13214,13213,26427,11.136569261550903,0.00013267099402021105
13413,13414,13413,26827,11.356925010681152,0.00013066436936772606
13614,13615,13614,27229,11.572815179824829,0.0001289509776855378
13814,13815,13814,27629,11.770438194274902,0.00012695764619518967
14014,14015,14014,28029,11.959854125976562,0.00012553852777686178
14214,14215,14214,28429,12.176806926727295,0.0001242966564725052
14414,14415,14414,28829,12.374903202056885,0.0001226691610167531
14615,14616,14615,29231,12.560961246490479,0.00012114326492845113
14815,14816,14815,29631,12.694914102554321,0.00011992373667054951
15015,15016,15015,30031,12.829683065414429,0.00011883437251330645
15215,15216,15215,30431,12.961914300918579,0.00011746116004514385
15415,15416,15415,30831,13.122225999832153,0.00011627365810361616
15616,15617,15616,31233,13.292293310165405,0.00011494202133355959
15816,15817,15816,31633,13.423165082931519,0.00011380136928453277
16016,16017,16016,32033,13.563583135604858,0.00011278886354251818
16216,16217,16216,32433,13.70481014251709,0.0001108625525811567
16416,16417,16416,32833,13.840825319290161,0.00010936533325807899
16617,16618,16617,33235,13.976957082748413,0.0001078360624225857
16817,16818,16817,33635,14.1309072971344,0.00010646863722811088
17017,17018,17017,34035,14.272335290908813,0.0001052815822331466
17217,17218,17217,34435,14.402703285217285,0.00010419081065635188
17417,17418,17417,34835,14.537955284118652,0.00010304917243215209
17618,17619,17618,35237,14.67287302017212,0.00010196966675974209
17818,17819,17818,35637,14.809681177139282,9.993263786335589e-05
18018,18019,18018,36037,14.946874141693115,9.778462010637506e-05
18218,18219,18218,36437,15.08458399772644,9.622565445469146e-05
18418,18419,18418,36837,15.223376274108887,9.48686193257932e-05
18619,18620,18619,37239,15.368772268295288,9.290515410830554e-05
18819,18820,18819,37639,15.516224145889282,9.132968286909853e-05
19019,19020,19019,38039,15.65610408782959,8.998369516507806e-05
19219,19220,19219,38439,15.795960187911987,8.879849428756358e-05
19419,19420,19419,38839,15.933882236480713,8.771036141256288e-05
19620,19621,19620,39241,16.092019081115723,8.668888609940676e-05
19820,19821,19820,39641,16.228254079818726,8.547475690231487e-05
20020,20021,20020,40041,16.363744020462036,8.443869200609595e-05
20220,20221,20220,40441,16.506999254226685,8.246313013584528e-05
20420,20421,20420,40841,16.655288219451904,8.11581658930375e-05
20621,20622,20621,41243,16.80072522163391,7.999595753313809e-05
20821,20822,20821,41643,16.938998222351074,7.892685657496265e-05
21021,21022,21021,42043,17.082861185073853,7.792137960650144e-05
21221,21222,21221,42443,17.223963260650635,7.696662023583319e-05
21421,21422,21421,42843,17.37539529800415,7.6054167456929e-05
21622,21623,21622,43245,17.538817167282104,7.517372130089341e-05
21822,21823,21822,43645,17.681883335113525,7.43294998575266e-05
22022,22023,22022,44045,17.825006246566772,7.351349938882748e-05
22222,22223,22222,44445,17.9719340801239,7.272287927894987e-05
22422,22423,22422,44845,18.120655298233032,7.195531307062059e-05
22623,22624,22623,45247,18.259881019592285,7.120518396725883e-05
22823,22824,22823,45647,18.400633096694946,7.04783205571956e-05
23023,23024,23023,46047,18.558226108551025,6.97695541350563e-05
23223,23224,23223,46447,18.69919228553772,6.907769470916285e-05
23423,23424,23423,46847,18.839216232299805,6.840171157892528e-05
23624,23625,23624,47249,18.989493131637573,6.77374363123991e-05
23824,23825,23824,47649,19.1439311504364,6.709068453065306e-05
24024,24025,24024,48049,19.28413414955139,6.645741470020184e-05
24224,24225,24224,48449,19.42569136619568,6.583700291778728e-05
24424,24425,24424,48849,19.593454122543335,6.522888947237478e-05
24625,24626,24625,49251,19.745521306991577,6.46296163617347e-05
24825,24826,24825,49651,19.88302230834961,6.404468590260554e-05
25025,25026,25025,50051,20.03135323524475,6.347066876523294e-05
25225,25226,25225,50451,20.177649974822998,6.290718042680914e-05
25425,25426,25425,50851,20.325681924819946,6.235386603456538e-05
25626,25627,25626,51253,20.46769618988037,6.180770341956507e-05
25826,25827,25826,51653,20.617171049118042,6.127381936011798e-05
26026,26027,26026,52053,20.756291151046753,6.074918578479355e-05
26226,26227,26226,52453,20.90580916404724,6.023353373562771e-05
26426,26427,26426,52853,21.05268931388855,5.972660983966785e-05
26627,26628,26627,53255,21.197460174560547,5.9225703408486985e-05
26827,26828,26827,53655,21.338621139526367,5.8735570708512064e-05
27027,27028,27027,54055,21.492202043533325,5.825348300766713e-05
27227,27228,27227,54455,21.64440131187439,5.7779234883752995e-05
27427,27428,27427,54855,21.804235219955444,5.731263021530778e-05
27628,27629,27628,55257,21.950355052947998,5.6851204073482e-05
27828,27829,27828,55657,22.103323221206665,5.6399367235227945e-05
28028,28029,28028,56057,22.234316110610962,5.595463301104026e-05
28228,28229,28228,56457,22.347458124160767,5.551683552126061e-05
28428,28429,28428,56857,22.469223022460938,5.508581508604093e-05
28629,28630,28629,57259,22.602074146270752,5.465931220875329e-05
28829,28830,28829,57659,22.71276617050171,5.424142159615184e-05
29029,29030,29029,58059,22.820433378219604,5.38298615098952e-05
29229,29230,29229,58459,22.934701204299927,5.342449331001834e-05
29429,29430,29429,58859,23.04284906387329,5.302518284603325e-05
29630,29631,29630,59261,23.206806182861328,5.262984797572304e-05
29830,29831,29830,59661,23.372571229934692,5.2242295969390406e-05
30030,30031,30030,60061,23.492276191711426,5.186042320499224e-05
30230,30231,30230,60461,23.63127613067627,5.148411122937319e-05
30430,30431,30430,60861,23.90234112739563,5.111324503012289e-05
30631,30632,30631,61263,24.00805926322937,5.074589843226193e-05
30831,30832,30831,61663,24.123696327209473,5.038561757739843e-05
31031,31032,31031,62063,24.248091220855713,5.0030456031216506e-05
31231,31232,31231,62463,24.356842041015625,4.968031105798552e-05
31431,31432,31431,62863,24.454406261444092,4.9335082662645556e-05
31632,31633,31632,63265,24.554129362106323,4.899298337974067e-05
31832,31833,31832,63665,24.673924207687378,4.865732194860279e-05
32032,32033,32032,64065,24.783249378204346,4.832629200612741e-05
32232,32233,32232,64465,24.87970519065857,4.799980347295473e-05
32432,32433,32432,64865,24.974018096923828,4.767776851191872e-05
32633,32634,32633,65267,25.064289093017578,4.7358523943857555e-05
32833,32834,32833,65667,25.15842914581299,4.704516239229665e-05
33033,33034,33033,66067,25.248825311660767,4.673600315045491e-05
33233,33234,33233,66467,25.34378218650818,4.643096657848961e-05
33433,33434,33433,66867,25.44339418411255,4.612997490931848e-05
33634,33635,33634,67269,25.54515314102173,4.5831476917467705e-05
33834,33835,33834,67669,25.647933959960938,4.5538368218799185e-05
34034,34035,34034,68069,25.759108304977417,4.5249081382821374e-05
34234,34235,34234,68469,25.88338613510132,4.496354554183562e-05
34434,34435,34434,68869,25.992146015167236,4.468169141584407e-05
34635,34636,34635,69271,26.090628147125244,4.440206903210665e-05
34835,34836,34835,69671,26.18622326850891,4.412739418180952e-05
35035,35036,35035,70071,26.28350591659546,4.385620193721823e-05
35235,35236,35235,70471,26.38726305961609,4.3588428910829274e-05
35435,35436,35435,70871,26.50752329826355,4.33240130799537e-05
35636,35637,35636,71273,26.63034224510193,4.306159633349643e-05
35836,35837,35836,71673,26.740304231643677,4.280373013053059e-05
36036,36037,36036,72073,26.858155012130737,4.254904257590863e-05
36236,36237,36236,72473,26.99963116645813,4.2297476739904984e-05
36436,36437,36436,72873,27.164287090301514,4.204897687910038e-05
36637,36638,36637,73275,27.37017822265625,4.18022684376533e-05
36837,36838,36837,73675,27.54705309867859,4.155975254162307e-05
37037,37038,37037,74075,27.69939613342285,4.1320141939070216e-05
37237,37238,37237,74475,27.874901056289673,4.108338533348318e-05
37437,37438,37437,74875,28.05324125289917,4.084943246946974e-05
37638,37639,37638,75277,28.23068404197693,4.0617084952938246e-05
37838,37839,37838,75677,28.356577157974243,4.038860624924723e-05
38038,38039,38038,76077,28.490979194641113,4.0162786274017004e-05
38238,38239,38238,76477,28.60239315032959,3.9939578688379176e-05
38438,38439,38438,76877,28.707544088363647,3.971893807343628e-05
38639,38640,38639,77279,29.145904302597046,3.94997355814331e-05
38839,38840,38839,77679,29.340537309646606,3.928410850827424e-05
39039,39040,39039,78079,29.51750421524048,3.907091724329487e-05
39239,39240,39239,78479,29.645483016967773,3.886011984195347e-05
39439,39440,39439,78879,29.75278902053833,3.865167517799471e-05
39640,39641,39640,79281,29.842135190963745,3.844451800765205e-05
39840,39841,39840,79681,29.93302822113037,3.824066988993605e-05
40040,40041,40040,80081,30.01878809928894,3.8039055670061645e-05
40240,40241,40240,80481,30.120408296585083,3.783963732244478e-05
40440,40441,40440,80881,30.256263971328735,3.764237755311526e-05
40641,40642,40641,81283,30.374924182891846,3.744626936738244e-05
40841,40842,40841,81683,30.48551034927368,3.7253228066234705e-05
41041,41042,41041,82083,30.592182159423828,3.706223752687029e-05
41241,41242,41241,82483,30.696604013442993,3.687326323452506e-05
41441,41442,41441,82883,30.798938274383545,3.66862713328702e-05
41642,41643,41642,83285,30.902891159057617,3.650030823855181e-05
41842,41843,41842,83685,31.006432056427002,3.631719161467735e-05
42042,42043,42042,84085,31.119814157485962,3.613595946621684e-05
42242,42243,42242,84485,31.21942710876465,3.595658043798982e-05
42442,42443,42442,84885,31.324332237243652,3.57790237678335e-05
42643,42644,42643,85287,31.431270360946655,3.560238490501452e-05
42843,42844,42843,85687,31.52005624771118,3.542839171642989e-05
43043,43044,43043,86087,31.6076340675354,3.525613189535699e-05
43243,43244,43243,86487,31.69571304321289,3.508557693744426e-05
43443,43444,43443,86887,31.78084421157837,3.491669887425543e-05
43644,43645,43644,87289,31.869376182556152,3.474863821856932e-05
43844,43845,43844,87689,31.954997062683105,3.458304017664543e-05
44044,44045,44044,88089,32.042142152786255,3.441903810443876e-05
44244,44245,44244,88489,32.12962627410889,3.425660607625741e-05
44444,44445,44444,88889,32.215885162353516,3.409571865172703e-05
44645,44646,44645,89291,32.30864691734314,3.393555780413881e-05
44845,44846,44845,89691,32.399174213409424,3.377769257492962e-05
45045,45046,45045,90091,32.48354911804199,3.36212983279557e-05
45245,45246,45245,90491,32.57027220726013,3.346635147388814e-05
45445,45446,45445,90891,32.66498613357544,3.33128288637691e-05
45646,45647,45646,91293,32.75137114524841,3.315995065859952e-05
45846,45847,45846,91693,32.837600231170654,3.300921564869888e-05
46046,46047,46046,92093,32.92296314239502,3.285983788453062e-05
46246,46247,46246,92493,33.00935411453247,3.271179589688412e-05
46446,46447,46446,92893,33.09670829772949,3.25650686163105e-05
46647,46648,46647,93295,33.18457913398743,3.24189114156641e-05
46847,46848,46847,93695,33.27504205703735,3.2274758218588145e-05
47047,47048,47047,94095,33.37079930305481,3.213185874309639e-05
47247,47248,47247,94495,33.45638918876648,3.199019344500518e-05
47447,47448,47447,94895,33.53927707672119,3.184974314316998e-05
47648,47649,47648,95297,33.62557816505432,3.1709795716324703e-05
47848,47849,47848,95697,33.71322822570801,3.157172512443075e-05
48048,48049,48048,96097,33.79749321937561,3.1434814005624235e-05
48248,48249,48248,96497,33.8827862739563,3.129904456531931e-05
48448,48449,48448,96897,33.973188161849976,3.1164399338385454e-05
48649,48650,48649,97299,34.059046268463135,3.103019624625016e-05
48849,48850,48849,97699,34.14633131027222,3.089775374975954e-05
49049,49050,49049,98099,34.236040115356445,3.07663849082937e-05
49249,49250,49249,98499,34.32284331321716,3.063607351682905e-05
49449,49450,49449,98899,34.44578719139099,3.0506803670608126e-05
49650,49651,49650,99301,34.55240201950073,3.0377921091134972e-05
49850,49851,49850,99701,34.648935079574585,3.0250692807107405e-05
50050,50051,50050,100101,34.75107407569885,3.012446002254187e-05
50250,50251,50250,100501,34.84409499168396,2.9999207978304106e-05
50450,50451,50450,100901,34.935460329055786,2.9874922187545127e-05
50651,50652,50651,101303,35.02441716194153,2.9750974131023067e-05
50851,50852,50851,101703,35.11425423622131,2.96285831081996e-05
51051,51052,51051,102103,35.20168399810791,2.9507116396292626e-05
51251,51252,51251,102503,35.28807616233826,2.938656055009835e-05
51451,51452,51451,102903,35.367393255233765,2.926690237216241e-05
51652,51653,51652,103305,35.44815015792847,2.914753724253906e-05
51852,51853,51852,103705,35.53099012374878,2.902964010587454e-05
52052,52053,52052,104105,35.625288009643555,2.8912602424620825e-05
52252,52253,52252,104505,35.72148013114929,2.8796411948261192e-05
52452,52453,52452,104905,35.81532025337219,2.86810566513841e-05
52653,52654,52653,105307,35.90273904800415,2.8565954119412308e-05
52853,52854,52853,105707,35.9942672252655,2.845223801586405e-05
53053,53054,53053,106107,36.086045026779175,2.833932226940535e-05
53253,53254,53253,106507,36.194252252578735,2.8227195714919036e-05
53453,53454,53453,106907,36.30929112434387,2.811584739238264e-05
53654,53655,53654,107309,36.44191002845764,2.800471554887439e-05
53854,53855,53854,107709,36.55337309837341,2.7894895368070214e-05
54054,54055,54054,108109,36.65229320526123,2.7785821677693187e-05
54254,54255,54254,108509,36.74607229232788,2.7677484299499778e-05
54454,54455,54454,108909,36.831539154052734,2.7569873241230218e-05
54655,54656,54655,109311,36.91353917121887,2.7462446004623772e-05
54855,54856,54855,109711,36.99459910392761,2.7356261846727034e-05
55055,55056,55055,110111,37.07502818107605,2.725077506653154e-05
55255,55256,55255,110511,37.15795111656189,2.714597638234907e-05
55455,55456,55455,110911,37.23895215988159,2.704185668086908e-05
55656,55657,55656,111313,37.32210731506348,2.6937891435424704e-05
55856,55857,55856,111713,37.40258717536926,2.6835106305327283e-05
56056,56057,56056,112113,37.482553243637085,2.6732973758590242e-05
56256,56257,56256,112513,37.563844203948975,2.663148532741533e-05
56456,56457,56456,112913,37.646361112594604,2.6530632697336934e-05
56657,56658,56657,113315,37.726529121398926,2.6429908142948734e-05
56857,56858,56857,113715,37.80669903755188,2.633030584940144e-05
57057,57058,57057,114115,37.887105226516724,2.623131526670404e-05
57257,57258,57257,114515,37.967199087142944,2.613292866583915e-05
57457,57458,57457,114915,38.048078298568726,2.6035138457738e-05
57658,57659,57658,115317,38.13300323486328,2.593745265072798e-05
57858,57859,57858,115717,38.2145631313324,2.584083589395524e-05
58058,58059,58058,116117,38.295165061950684,2.5744793535738902e-05
58258,58259,58258,116517,38.37734627723694,2.5649318518629235e-05
58458,58459,58458,116917,38.45971202850342,2.5554403911189596e-05
58659,58660,58659,117319,38.54290318489075,2.5459572481065633e-05
58859,58860,58859,117719,38.63540005683899,2.5365761111430925e-05
59059,59060,59059,118119,38.71957302093506,2.5272490060190403e-05
59259,59260,59259,118519,38.801727056503296,2.517975287871068e-05
59459,59460,59459,118919,38.884151220321655,2.5087543233125403e-05
59660,59661,59660,119321,38.97304606437683,2.4995397759972512e-05
59860,59861,59860,119721,39.055641174316406,2.490422719334325e-05
60060,60061,60060,120121,39.1409752368927,2.4813565798024234e-05
60260,60261,60260,120521,39.22315716743469,2.4723407677749496e-05
60460,60461,60460,120921,39.309699296951294,2.4633747040773896e-05
60661,60662,60661,121323,39.392553091049194,2.4544133578804296e-05
60861,60862,60861,121723,39.475656032562256,2.445545335596371e-05
61061,61062,61061,122123,39.56047606468201,2.4367253818083246e-05
61261,61262,61261,122523,39.64517617225647,2.4279529570473223e-05
61461,61462,61461,122923,39.72691893577576,2.419227531280689e-05
61662,61663,61662,123325,39.80868220329285,2.4105053049282856e-05
61862,61863,61862,123725,39.89128136634827,2.4018725524974882e-05
62062,62063,62062,124125,39.97302317619324,2.393285261366525e-05
62262,62263,62262,124525,40.05393314361572,2.3847429375221576e-05
62462,62463,62462,124925,40.13815212249756,2.3762450955219734e-05
62663,62664,62663,125327,40.22333908081055,2.367749098917859e-05
62863,62864,62863,125727,40.30549216270447,2.3593390142712952e-05
63063,63064,63063,126127,40.38931107521057,2.3509720026446284e-05
63263,63264,63263,126527,40.4712290763855,2.3426476112930486e-05
63463,63464,63463,126927,40.552550315856934,2.3343653952199534e-05
63664,63665,63664,127329,40.640188217163086,2.3260838188049547e-05
63864,63865,63864,127729,40.73017716407776,2.3178848541311665e-05
64064,64065,64064,128129,40.81672191619873,2.3097267727812514e-05
64264,64265,64264,128529,40.90213918685913,2.301609159425178e-05
64464,64465,64464,128929,40.98490905761719,2.2935316057600474e-05
64665,64666,64665,129331,41.0671010017395,2.285453619857201e-05
64865,64866,64865,129731,41.15092992782593,2.2774551834489358e-05
65065,65066,65065,130131,41.23350214958191,2.2694956207966895e-05
65265,65266,65265,130531,41.316845178604126,2.261574550445783e-05
65465,65466,65465,130931,41.39958715438843,2.2536915973737697e-05
65666,65667,65666,131333,41.48357915878296,2.2458072609819874e-05
65866,65867,65866,131733,41.56598615646362,2.2379996282607706e-05
66066,66067,66066,132133,41.64959001541138,2.2302290230041918e-05
66266,66267,66266,132533,41.732869148254395,2.2224950945359918e-05
66466,66467,66466,132933,41.81506896018982,2.214797497965102e-05
66667,66668,66667,133335,41.89903020858765,2.2070976759758464e-05
66867,66868,66867,133735,41.98053002357483,2.1994719086430073e-05
67067,67068,67067,134135,42.063552141189575,2.1918814706062988e-05
67267,67268,67267,134535,42.150269985198975,2.184326039062006e-05
67467,67468,67467,134935,42.23257613182068,2.176805296494671e-05
67668,67669,67668,135337,42.31943917274475,2.1692815845554933e-05
67868,67869,67868,135737,42.40129208564758,2.1618294574471988e-05
68068,68069,68068,136137,42.48292112350464,2.1544110957735844e-05
68268,68269,68268,136537,42.567588329315186,2.1470262020018156e-05
68468,68469,68468,136937,42.64931011199951,2.1396744834767492e-05
68669,68670,68669,137339,42.73258399963379,2.1323191401157828e-05
68869,68870,68869,137739,42.82264018058777,2.1250330747897147e-05
69069,69070,69069,138139,42.907435178756714,2.117779332844724e-05
69269,69270,69269,138539,42.99036502838135,2.1105576397422385e-05
69469,69470,69469,138939,43.07250213623047,2.103367725270873e-05
69670,69671,69670,139341,43.158547163009644,2.0961736101926563e-05
69870,69871,69870,139741,43.240233182907104,2.0890466148643186e-05
70070,70071,70070,140141,43.322426319122314,2.081950611376842e-05
70270,70271,70270,140541,43.405068159103394,2.0748853460282683e-05
70470,70471,70470,140941,43.48699927330017,2.067850569045603e-05
70671,70672,70671,141343,43.57007908821106,2.0608110873715858e-05
70871,70872,70871,141743,43.653810024261475,2.0538367024535718e-05
71071,71072,71071,142143,43.735849142074585,2.0468920781284533e-05
71271,71272,71271,142543,43.819966077804565,2.039976979595512e-05
71471,71472,71471,142943,43.903003215789795,2.0330911755908095e-05
71672,71673,71672,143345,43.98634219169617,2.0262002273157513e-05
71872,71873,71872,143745,44.06945514678955,2.019372476173676e-05
72072,72073,72072,144145,44.15385293960571,2.0125733453889435e-05
72272,72273,72272,144545,44.23960828781128,2.0058026172939623e-05
72472,72473,72472,144945,44.325000047683716,1.9990600774481392e-05
72673,72674,72673,145347,44.40813326835632,1.9923120117651816e-05
72873,72874,72873,145747,44.48855018615723,1.985625356098274e-05
73073,73074,73073,146147,44.570730209350586,1.9789662631901633e-05
73273,73274,73273,146547,44.65583515167236,1.972334530909264e-05
73473,73474,73473,146947,44.73605728149414,1.965729960122765e-05
73674,73675,73674,147349,44.815953969955444,1.9591195339295265e-05
73874,73875,73874,147749,44.90125107765198,1.9525688334960787e-05
74074,74075,74074,148149,44.98626732826233,1.9460447131892794e-05
74274,74275,74274,148549,45.06622815132141,1.9395469850748335e-05
74474,74475,74474,148949,45.14847421646118,1.9330754638791675e-05
74675,74676,74675,149351,45.22895908355713,1.9265978045387693e-05
74875,74876,74875,149751,45.307910203933716,1.9201782805228185e-05
75075,75076,75075,150151,45.38691735267639,1.913784422237462e-05
75275,75276,75275,150551,45.467788219451904,1.9074160545524843e-05
75475,75476,75475,150951,45.54771304130554,1.9010730048309565e-05
75676,75677,75676,151353,45.63355112075806,1.8947235761531615e-05
75876,75877,75876,151753,45.714914083480835,1.8884307782907123e-05
76076,76077,76076,152153,45.794103145599365,1.882162793661646e-05
76276,76277,76276,152553,45.873279094696045,1.8759194588663902e-05
76476,76477,76476,152953,45.95307397842407,1.869700612725142e-05
76677,76678,76677,153355,46.03263211250305,1.8634751844596676e-05
76877,76878,76877,153755,46.11339616775513,1.857304961089388e-05
77077,77078,77077,154155,46.19196128845215,1.851158754835832e-05
77277,77278,77277,154555,46.27171325683594,1.8450364129109865e-05
77477,77478,77477,154955,46.35158610343933,1.8389377845871568e-05
77678,77679,77678,155357,46.432382106781006,1.832832404689695e-05
77878,77879,77878,155757,46.511687994003296,1.826780875814684e-05
78078,78079,78078,156157,46.59302020072937,1.820752619194463e-05
78278,78279,78278,156557,46.675095081329346,1.814747491725869e-05
78478,78479,78478,156957,46.754526138305664,1.8087653521743525e-05
78679,78680,78679,157359,46.834689140319824,1.8027763217743672e-05
78879,78880,78879,157759,46.91481018066406,1.7968398546087996e-05
79079,79080,79079,158159,47.002111196517944,1.790925961531048e-05
79279,79280,79279,158559,47.086590051651,1.7850345082594146e-05
79479,79480,79479,158959,47.16901922225952,1.77916536220726e-05
79680,79681,79680,159361,47.24979901313782,1.7732892130257014e-05
79880,79881,79880,159761,47.33171200752258,1.767464399981772e-05
80080,80081,80080,160161,47.411569356918335,1.7616615053687694e-05
80280,80281,80280,160561,47.49116921424866,1.7558804029918216e-05
80480,80481,80480,160961,47.57131505012512,1.7501209680881247e-05
80681,80682,80681,161363,47.65248227119446,1.7443544419424363e-05
80881,80882,80881,161763,47.73202204704285,1.7386380806455728e-05
81081,81082,81081,162163,47.810752153396606,1.732943020950099e-05
81281,81282,81281,162563,47.891120195388794,1.727269143931636e-05
81481,81482,81481,162963,47.97016930580139,1.721616332099927e-05
81682,81683,81682,163365,48.04989314079285,1.7159563624247025e-05
81882,81883,81882,163765,48.130043268203735,1.7103454376987176e-05
82082,82083,82082,164165,48.20962309837341,1.704755233113992e-05
82282,82283,82282,164565,48.290152072906494,1.6991856364663583e-05
82482,82483,82482,164965,48.37482023239136,1.6936365368107678e-05
82683,82684,82683,165367,48.45788908004761,1.6880802319181295e-05
82883,82884,82883,165767,48.539708375930786,1.68257189948937e-05
83083,83084,83083,166167,48.625216007232666,1.6770837380892027e-05
83283,83284,83283,166567,48.707961320877075,1.671615641601582e-05
83483,83484,83483,166967,48.79037117958069,1.6661675051111054e-05
83684,83685,83684,167369,48.87225127220154,1.660712133124954e-05
83884,83885,83884,167769,48.95408320426941,1.6553037048599732e-05
84084,84085,84084,168169,49.03753709793091,1.6499149280554046e-05
84284,84285,84284,168569,49.12951421737671,1.6445457022070205e-05
84484,84485,84484,168969,49.21263313293457,1.639195927880118e-05
84685,84686,84685,169371,49.295525312423706,1.6338389030361827e-05
84885,84886,84885,169771,49.37850022315979,1.6285278336546473e-05
85085,85086,85085,170171,49.46029496192932,1.6232359232065325e-05
85285,85286,85285,170571,49.542994022369385,1.617963076332526e-05
85485,85486,85485,170971,49.62920022010803,1.6127091986225298e-05
85686,85687,85686,171373,49.712876081466675,1.607448068914669e-05
85886,85887,85886,171773,49.79535698890686,1.6022319438823913e-05
86086,86087,86086,172173,49.87778615951538,1.5970345100562545e-05
86286,86287,86286,172573,49.95950698852539,1.59185567678154e-05
86486,86487,86486,172973,50.03991198539734,1.5866953542714857e-05
86687,86688,86687,173375,50.12251925468445,1.5815277902837814e-05
86887,86888,86887,173775,50.20437526702881,1.5764043149488323e-05
87087,87088,87087,174175,50.28575801849365,1.5712990858523172e-05
87287,87288,87287,174575,50.36725211143494,1.5662120166279346e-05
87487,87488,87487,174975,50.448121309280396,1.561143021732443e-05
87688,87689,87688,175377,50.53107404708862,1.556066806512898e-05
87888,87889,87888,175777,50.617125272750854,1.551033796261631e-05
88088,88089,88088,176177,50.70149827003479,1.546018608140113e-05
88288,88289,88288,176577,50.783332109451294,1.541021159757741e-05
88488,88489,88488,176977,50.865468978881836,1.5360413694842413e-05
88689,88690,88689,177379,50.948644161224365,1.5310543893950142e-05
88889,88890,88889,177779,51.03002905845642,1.5261097607059525e-05
89089,89090,89089,178179,51.11573624610901,1.5211825492432295e-05
89289,89290,89289,178579,51.207757234573364,1.5162726762667496e-05
89489,89490,89489,178979,51.28935623168945,1.5113800637662409e-05
89690,89691,89690,179381,51.371663331985474,1.5064803002550323e-05
89890,89891,89890,179781,51.45304298400879,1.5016220626173443e-05
90090,90091,90090,180181,51.536499977111816,1.496780854995849e-05
90290,90291,90290,180581,51.622777223587036,1.4919566020356012e-05
90490,90491,90490,180981,51.70666027069092,1.4871492290022668e-05
90691,90692,90691,181383,51.7896683216095,1.482334751064452e-05
90891,90892,90891,181783,51.87171411514282,1.4775609996959472e-05
91091,91092,91091,182183,51.954761028289795,1.4728039074650312e-05
91291,91292,91291,182583,52.03614592552185,1.4680634020818699e-05
91491,91492,91491,182983,52.11994218826294,1.4633394119198879e-05
91692,91693,91692,183385,52.20252513885498,1.4586083693257845e-05
91892,91893,91892,183785,52.302470207214355,1.4539172785598242e-05
92092,92093,92092,184185,52.38480615615845,1.449242491083937e-05
92292,92293,92292,184585,52.46718430519104,1.4445839375256317e-05
92492,92493,92492,184985,52.549750089645386,1.4399415490292629e-05
92693,92694,92693,185387,52.63514018058777,1.4352921661750194e-05
92893,92894,92893,185787,52.718037128448486,1.4306819834244368e-05
93093,93094,93093,186187,52.80059504508972,1.4260877620885504e-05
93293,93294,93293,186587,52.88272523880005,1.421509435426674e-05
93493,93494,93493,186987,52.983479261398315,1.416946937231629e-05
93694,93695,93694,187389,53.065057039260864,1.4123775075896307e-05
93894,93895,93894,187789,53.14977431297302,1.407846547956422e-05
94094,94095,94094,188189,53.23535108566284,1.403331220762613e-05
94294,94295,94294,188589,53.32433223724365,1.3988314617509197e-05
94494,94495,94494,188989,53.406904220581055,1.3943472071226609e-05
94695,94696,94695,189391,53.490148305892944,1.3898560881576206e-05
94895,94896,94895,189791,53.57285928726196,1.3854027294927159e-05
95095,95096,95095,190191,53.65824913978577,1.3809646862917044e-05
95295,95296,95295,190591,53.739262104034424,1.37654189656538e-05
95495,95496,95495,190991,53.82012605667114,1.3721342987907271e-05
95696,95697,95696,191393,53.90365123748779,1.3677199074409121e-05
95896,95897,95896,191793,53.984935998916626,1.3633425858836057e-05
96096,96097,96096,192193,54.067047119140625,1.3589802739206199e-05
96296,96297,96296,192593,54.1490421295166,1.35463291176933e-05
96496,96497,96496,192993,54.23257303237915,1.3503004399434766e-05
96697,96698,96697,193395,54.3149311542511,1.3459612484043863e-05
96897,96898,96897,193795,54.39736604690552,1.3416584543123717e-05
97097,97098,97097,194195,54.479088306427,1.3373703743705375e-05
97297,97298,97297,194595,54.56222701072693,1.3330969507415631e-05
97497,97498,97497,194995,54.64604115486145,1.3288381259472336e-05
97698,97699,97698,195397,54.729719161987305,1.3245726579234039e-05
97898,97899,97898,195797,54.81182813644409,1.3203429321934942e-05
98098,98099,98098,196197,54.89386224746704,1.3161276348606287e-05
98298,98299,98298,196597,54.97547507286072,1.311926709916427e-05
98498,98499,98498,196997,55.05808901786804,1.3077401017313403e-05
98699,98700,98699,197399,55.14601135253906,1.3035469290422872e-05
98899,98900,98899,197799,55.23300099372864,1.2993888597849217e-05
99099,99100,99099,198199,55.319483280181885,1.295244942193559e-05
99299,99300,99299,198599,55.40947914123535,1.2911151220506686e-05
99499,99500,99499,198999,55.49622297286987,1.286999345406011e-05
99700,99701,99700,199401,55.58433532714844,1.2828770847985822e-05
99900,99901,99900,199801,55.671189069747925,1.2787893042801397e-05
100100,100101,100100,200201,55.759101152420044,1.2747154072082138e-05
100300,100301,100300,200601,55.847018003463745,1.2706553409680154e-05
100501,100502,100501,201003,55.93038320541382,1.2665888563453976e-05
100701,100702,100701,201403,56.01234722137451,1.2625563636433892e-05
100901,100902,100901,201803,56.09601902961731,1.2585375455221049e-05
101101,101102,101101,202203,56.17913818359375,1.2545323505865218e-05
101301,101302,101301,202603,56.261112213134766,1.2505407277379385e-05
101502,101503,101502,203005,56.34305214881897,1.246542769567226e-05
101702,101703,101702,203405,56.425682067871094,1.242578206043349e-05
101902,101903,101902,203805,56.50773620605469,1.2386270628372378e-05
102102,102103,102102,204205,56.592748165130615,1.2346892900642486e-05
102302,102303,102302,204605,56.677401304244995,1.2307648380173032e-05
102503,102504,102503,205007,56.760523080825806,1.226834134718589e-05
102703,102704,102703,205407,56.843353271484375,1.2229362423342488e-05
102903,102904,102903,205807,56.92632818222046,1.21905152316598e-05
103103,103104,103103,206207,57.00939130783081,1.2151799286759989e-05
103303,103304,103303,206607,57.090880155563354,1.211321410573703e-05
103504,103505,103504,207009,57.17375707626343,1.2074567260251462e-05
103704,103705,103704,207409,57.25677013397217,1.2036242816293373e-05
103904,103905,103904,207809,57.339313983917236,1.1998047700984065e-05
104104,104105,104104,208209,57.42503523826599,1.1959981441548137e-05
104304,104305,104304,208609,57.51032614707947,1.1922043567960165e-05
104505,104506,104505,209011,57.59447622299194,1.1884044883636587e-05
104705,104706,104705,209411,57.68574333190918,1.1846363017727352e-05
104905,104906,104905,209811,57.7726571559906,1.1808808140174205e-05
105105,105106,105105,210211,57.860472202301025,1.1771379790578626e-05
105305,105306,105305,210611,57.94793915748596,1.173407751130435e-05
105506,105507,105506,211013,58.034064292907715,1.1696715278194096e-05
105706,105707,105706,211413,58.12151503562927,1.1659664399754602e-05
105906,105907,105906,211813,58.20805311203003,1.1622738229691517e-05
106106,106107,106106,212213,58.295690059661865,1.1585936319549328e-05
106306,106307,106306,212613,58.37905216217041,1.1549258222760815e-05
106507,106508,106507,213015,58.46277832984924,1.1512521031012849e-05
106707,106708,106707,213415,58.545199155807495,1.1476089844787305e-05
106907,106908,106907,213815,58.629393339157104,1.1439781144320975e-05
107107,107108,107107,214215,58.71263527870178,1.1403594491893309e-05
107307,107308,107307,214615,58.795422077178955,1.1367529452242465e-05
107508,107509,107508,215017,58.88515520095825,1.1331406176650323e-05
107708,107709,107708,215417,58.9714560508728,1.129558366783659e-05
107908,107909,107908,215817,59.05280113220215,1.1259881476273338e-05
108108,108109,108108,216217,59.133827209472656,1.1224299174926978e-05
108308,108309,108308,216617,59.21881604194641,1.118883633898473e-05
108509,108510,108509,217019,59.30098819732666,1.115331612505416e-05
108709,108710,108709,217419,59.382495164871216,1.1118091545471364e-05
108909,108910,108909,217819,59.46509122848511,1.1082985166328097e-05
109109,109110,109109,218219,59.55757212638855,1.1047996571136456e-05
109309,109310,109309,218619,59.64228415489197,1.101312534450629e-05
109510,109511,109510,219021,59.724966287612915,1.0978197595520242e-05
109710,109711,109710,219421,59.80658006668091,1.0943560450911147e-05
109910,109911,109910,219821,59.886285066604614,1.0909039439771724e-05
110110,110111,110110,220221,59.97186613082886,1.0874634154690197e-05
110310,110311,110310,220621,60.05821418762207,1.0840344190103891e-05
110511,110512,110511,221023,60.1472430229187,1.0805998555340542e-05
110711,110712,110711,221423,60.23111605644226,1.0771938594496827e-05
110911,110912,110911,221823,60.31340718269348,1.0737992747055034e-05
111111,111112,111111,222223,60.39606523513794,1.0704160614568677e-05
111311,111312,111311,222623,60.47836494445801,1.067044180086801e-05
111512,111513,111512,223025,60.56355834007263,1.063666816496293e-05
111712,111713,111712,223425,60.652015209198,1.060317536842048e-05
111912,111913,111912,223825,60.73712420463562,1.0569794710229288e-05
112112,112113,112112,224225,60.82260012626648,1.0536525800915557e-05
112312,112313,112312,224625,60.90695810317993,1.0503368252932648e-05
112513,112514,112513,225027,60.990076303482056,1.0470156725601657e-05
112713,112714,112713,225427,61.074737310409546,1.0437221296023998e-05
112913,112914,112913,225827,61.157536029815674,1.0404396073128646e-05
113113,113114,113113,226227,61.241475105285645,1.037168067598162e-05
113313,113314,113313,226627,61.322914123535156,1.0339074725084136e-05
113514,113515,113514,227029,61.40246105194092,1.0306415632052334e-05
113714,113715,113714,227429,61.481754302978516,1.0274027985320975e-05
113914,113915,113914,227829,61.56212306022644,1.0241748655058571e-05
114114,114115,114114,228229,61.65098714828491,1.0209577268509251e-05
114314,114315,114314,228629,61.7320830821991,1.0177513454397468e-05
114515,114516,114515,229031,61.81203818321228,1.0145397328777266e-05
114715,114716,114715,229431,61.89190196990967,1.0113548085397391e-05
114915,114916,114915,229831,61.969919204711914,1.0081805308292804e-05
115115,115116,115115,230231,62.04933309555054,1.0050168632586782e-05
115315,115316,115315,230631,62.13101506233215,1.0018637694797622e-05
115516,115517,115516,231033,62.21102333068848,9.987055269208646e-06
115716,115717,115716,231433,62.29133319854736,9.955735246800352e-06
115916,115917,115916,231833,62.3699471950531,9.92451987894531e-06
116116,116117,116116,232233,62.448580265045166,9.893408808518569e-06
116316,116317,116316,232633,62.528685092926025,9.862401678996708e-06
116517,116518,116517,233035,62.611998081207275,9.831343878126327e-06
116717,116718,116717,233435,62.69117498397827,9.800544084108416e-06
116917,116918,116917,233835,62.77099132537842,9.769847170287656e-06
117117,117118,117117,234235,62.851256132125854,9.739252786091199e-06
117317,117318,117317,234635,62.93094515800476,9.708760583111614e-06
117518,117519,117518,235037,63.011595010757446,9.678218517043588e-06
117718,117719,117718,235437,63.09220814704895,9.64793014194564e-06
117918,117919,117918,235837,63.171974182128906,9.617742908107303e-06
118118,118119,118118,236237,63.25153613090515,9.587656472445572e-06
118318,118319,118318,236637,63.33178114891052,9.557670492909305e-06
118519,118520,118519,237039,63.4126501083374,9.52763545108183e-06
118719,118720,118719,237439,63.49139904975891,9.497849862176717e-06
118919,118920,118919,237839,63.572394132614136,9.468163710447886e-06
119119,119120,119119,238239,63.65534424781799,9.438576659636312e-06
119319,119320,119319,238639,63.74105715751648,9.409088374268713e-06
119520,119521,119520,239041,63.820749282836914,9.379551818509335e-06
119720,119721,119720,239441,63.89986205101013,9.350260554350756e-06
119920,119921,119920,239841,63.9797682762146,9.321067056833196e-06
120120,120121,120120,240241,64.05941200256348,9.29197099608622e-06
120320,120321,120320,240641,64.14099621772766,9.262972043598616e-06
120521,120522,120521,241043,64.22175526618958,9.233925603618453e-06
120721,120722,120721,241443,64.30166506767273,9.205120368296e-06
120921,120922,120921,241843,64.38187336921692,9.17641126156657e-06
121121,121122,121121,242243,64.46089029312134,9.147797959813484e-06
121321,121322,121321,242643,64.54038405418396,9.119280140789257e-06
121522,121523,121522,243045,64.6213493347168,9.090715608890595e-06
121722,121723,121722,243445,64.70330023765564,9.062388267207441e-06
121922,121923,121922,243845,64.78582620620728,9.034155447263861e-06
122122,122123,122122,244245,64.86826825141907,9.006016832067756e-06
122322,122323,122322,244645,64.95072412490845,8.977972105350256e-06
122523,122524,122523,245047,65.03344321250916,8.949881431041437e-06
122723,122724,122723,245447,65.11611318588257,8.922024003229597e-06
122923,122924,122923,245847,65.19912624359131,8.894259521458041e-06
123123,123124,123123,246247,65.28164720535278,8.866587673950486e-06
123323,123324,123323,246647,65.36757731437683,8.83900815125399e-06
123524,123525,123524,247049,65.44757413864136,8.811383437088735e-06
123724,123725,123724,247449,65.52745127677917,8.783988095040832e-06
123924,123925,123924,247849,65.61439514160156,8.756684152684236e-06
124124,124125,124124,248249,65.69609212875366,8.729471304443888e-06
124324,124325,124324,248649,65.7847352027893,8.702349245869233e-06
124525,124526,124525,249051,65.87060403823853,8.675182742870968e-06
124725,124726,124725,249451,65.95205521583557,8.648241805597124e-06
124925,124926,124925,249851,66.03696322441101,8.62139075050072e-06
125125,125126,125125,250251,66.1193060874939,8.594629277698607e-06
125325,125326,125325,250651,66.20284223556519,8.567957088477786e-06
125526,125527,125526,251053,66.28498315811157,8.54124119258651e-06
125726,125727,125726,251453,66.3669912815094,8.514747121879422e-06
125926,125927,125926,251853,66.44849634170532,8.48834144398622e-06
126126,126127,126126,252253,66.53056621551514,8.462023864807587e-06
126326,126327,126326,252653,66.61522316932678,8.435794090847101e-06
126527,126528,126527,253055,66.69977498054504,8.409521338462826e-06
126727,126728,126727,253455,66.7852771282196,8.38346673558935e-06
126927,126928,126927,253855,66.86958599090576,8.357499063731341e-06
127127,127128,127127,254255,66.95108723640442,8.331618033921907e-06
127327,127328,127327,254655,67.03261613845825,8.30582335838185e-06
127528,127529,127528,255057,67.11662006378174,8.279986422925265e-06
127728,127729,127728,255457,67.19920706748962,8.254364025002071e-06
127928,127929,127928,255857,67.28080105781555,8.228827122700622e-06
128128,128129,128128,256257,67.36298704147339,8.203375432618442e-06
128328,128329,128328,256657,67.44664025306702,8.178008672136299e-06
128529,128530,128529,257059,67.52905201911926,8.15260036121952e-06
128729,128730,128729,257459,67.61581707000732,8.127403037376114e-06
128929,128930,128929,257859,67.69750714302063,8.102289800305277e-06
129129,129130,129129,258259,67.7787721157074,8.077260371112561e-06
129329,129330,129329,258659,67.86357307434082,8.05231447263009e-06
129530,129531,129530,259061,67.95147013664246,8.027327724085965e-06
129730,129731,129730,259461,68.03400135040283,8.002548472907759e-06
129930,129931,129930,259861,68.11838817596436,7.977851924540117e-06
130130,130131,130130,260261,68.20078611373901,7.953237805721846e-06
130330,130331,130330,260661,68.28298807144165,7.928705843924688e-06
130531,130532,130531,261063,68.36508917808533,7.904133722467289e-06
130731,130732,130731,261463,68.44769716262817,7.879765668388104e-06
130931,130932,130931,261863,68.52838516235352,7.855478958332093e-06
131131,131132,131131,262263,68.61180329322815,7.831273323906519e-06
131331,131332,131331,262663,68.69618320465088,7.80714849714627e-06
131532,131533,131532,263065,68.77891421318054,7.782984192247002e-06
131732,131733,131732,263465,68.86512327194214,7.759020582952624e-06
131932,131933,131932,263865,68.9474949836731,7.735136983153761e-06
132132,132133,132132,264265,69.0284571647644,7.711333128961429e-06
132332,132333,132332,264665,69.11035132408142,7.687608757569467e-06
132533,132534,132533,265067,69.19677710533142,7.663845579966502e-06
132733,132734,132733,265467,69.28165936470032,7.64027978354873e-06
132933,132934,132933,265867,69.37582325935364,7.616792685465662e-06
133133,133134,133133,266267,69.65532493591309,7.59338402694937e-06
133333,133334,133333,266667,70.18477129936218,7.570053549732815e-06
133534,133535,133534,267069,70.39662003517151,7.546684928873255e-06
133734,133735,133734,267469,70.49111104011536,7.5235104308046415e-06
133934,133935,133934,267869,70.5857002735138,7.500413343511995e-06
134134,134135,134134,268269,70.67993307113647,7.477393412523349e-06
134334,134335,134334,268669,70.78225111961365,7.454450384212125e-06
134535,134536,134535,269071,70.8787100315094,7.431469865915137e-06
134735,134736,134735,269471,70.97583413124084,7.408680266896116e-06
134935,134936,134935,269871,71.06534814834595,7.385966813593818e-06
135135,135136,135135,270271,71.15178918838501,7.3633292561568134e-06
135335,135336,135335,270671,71.23639297485352,7.340767345116454e-06
135536,135537,135536,271073,71.31830525398254,7.3181685889755275e-06
135736,135737,135736,271473,71.40337324142456,7.295757602098325e-06
135936,135937,135936,271873,71.49139618873596,7.2734215183694e-06
136136,136137,136136,272273,71.5752022266388,7.251160091890145e-06
136336,136337,136336,272673,71.65918326377869,7.228973077821536e-06
136537,136538,136537,273075,71.74149823188782,7.206749854210524e-06
136737,136738,136737,273475,71.82965421676636,7.184711303109882e-06
136937,136938,136937,273875,71.92425417900085,7.162746434143544e-06
137137,137138,137137,274275,72.00585198402405,7.140855005631626e-06
137337,137338,137337,274675,72.0938241481781,7.119036777113917e-06
137538,137539,137538,275077,72.19051599502563,7.097182965459542e-06
137738,137739,137738,275477,72.28550100326538,7.0755107816114285e-06
137938,137939,137938,275877,72.37241315841675,7.0539110800218686e-06
138138,138139,138138,276277,72.45609927177429,7.032383623238822e-06
138338,138339,138338,276677,72.5475401878357,7.010928175214588e-06
138539,138540,138539,277079,72.64508390426636,6.989437761847133e-06
138739,138740,138739,277479,72.72696208953857,6.968125982219415e-06
138939,138940,138939,277879,72.80712914466858,6.94688550594555e-06
139139,139140,139139,278279,72.89026713371277,6.9257160998572495e-06
139339,139340,139339,278679,72.97753405570984,6.9046175317472975e-06
139540,139541,139540,279081,73.07275414466858,6.883484607254361e-06
139740,139741,139740,279481,73.16079211235046,6.862527372744858e-06
139940,139941,139940,279881,73.24163913726807,6.8416402829467025e-06
140140,140141,140140,280281,73.32342100143433,6.820823108963178e-06
140340,140341,140340,280681,73.40516304969788,6.800075622496457e-06
140541,140542,140541,281083,73.48748111724854,6.779294380109529e-06
140741,140742,140741,281483,73.57267308235168,6.75868593274596e-06
140941,140942,140941,281883,73.66525602340698,6.738146491706433e-06
141141,141142,141141,282283,73.75500321388245,6.717675832176795e-06
141341,141342,141341,282683,73.84777617454529,6.697273729440451e-06
141542,141543,141542,283085,73.9300811290741,6.676838462741711e-06
141742,141743,141742,283485,74.01140999794006,6.656573144298918e-06
141942,141943,141942,283885,74.09667015075684,6.636375713416838e-06
142142,142143,142142,284285,74.18892502784729,6.616245948960334e-06
142342,142343,142342,284685,74.29210233688354,6.596183630459056e-06
142543,142544,142543,285087,74.38144207000732,6.576088731472025e-06
142743,142744,142743,285487,74.46471214294434,6.556160981244117e-06
142943,142944,142943,285887,74.55007004737854,6.536300019031881e-06
143143,143144,143143,286287,74.64809012413025,6.516505627667735e-06
143343,143344,143343,286687,74.74036407470703,6.496777590244595e-06
143544,143545,143544,287089,74.82950711250305,6.477017547417035e-06
143744,143745,143744,287489,74.91263628005981,6.457421900283139e-06
143944,143945,143944,287889,74.99823522567749,6.437891960801721e-06
144144,144145,144144,288289,75.0924642086029,6.4184275151688715e-06
144344,144345,144344,288689,75.18819522857666,6.399028350372062e-06
144545,144546,144545,289091,75.28292608261108,6.379597746888274e-06
144745,144746,144745,289491,75.37040424346924,6.36032883183998e-06
144945,144946,144945,289891,75.45894622802734,6.341124562219437e-06
145145,145146,145145,290291,75.54470920562744,6.321984728138481e-06
145345,145346,145345,290691,75.62730813026428,6.302909120228026e-06
145546,145547,145546,291093,75.71021604537964,6.2838026324741395e-06
145746,145747,145746,291493,75.79186820983887,6.264855170358031e-06
145946,145947,145946,291893,75.87667512893677,6.245971309952342e-06
146146,146147,146146,292293,75.96036005020142,6.227150844507652e-06
146346,146347,146346,292693,76.04610514640808,6.208393568735078e-06
146547,146548,146547,293095,76.13376808166504,6.189605963924979e-06
146747,146748,146747,293495,76.21604323387146,6.170974766069455e-06
146947,146948,146947,293895,76.30161619186401,6.152406143804706e-06
147147,147148,147147,294295,76.39349412918091,6.133899894440153e-06
147347,147348,147347,294695,76.47602820396423,6.115455815292239e-06
147548,147549,147548,295097,76.5607750415802,6.096981950148837e-06
147748,147749,147748,295497,76.64663910865784,6.0786619166569175e-06
147948,147949,147948,295897,76.73002123832703,6.060403450161269e-06
148148,148149,148148,296297,76.8124611377716,6.0422063514438506e-06
148348,148349,148348,296697,76.89551019668579,6.024070421392554e-06
148549,148550,148549,297099,76.97915410995483,6.005905240359498e-06
148749,148750,148749,297499,77.06420612335205,5.9878913581281e-06
148949,148950,148949,297899,77.14962720870972,5.969938051646227e-06
149149,149150,149149,298299,77.23365521430969,5.952045124915494e-06
149349,149350,149349,298699,77.317312002182,5.934212382477478e-06
149550,149551,149550,299101,77.4003803730011,5.916350916448263e-06
149750,149751,149750,299501,77.48380398750305,5.898638257874787e-06
149950,149951,149950,299901,77.56787109375,5.880985200618706e-06
150150,150151,150150,300301,77.65407705307007,5.863391552095641e-06
150350,150351,150350,300701,77.73729515075684,5.845857120064781e-06
150551,150552,150551,301103,77.8217101097107,5.8282944842517344e-06
150751,150752,150751,301503,77.9050931930542,5.810878205637926e-06
150951,150952,150951,301903,77.98876404762268,5.793520570547523e-06
151151,151152,151151,302303,78.07310128211975,5.776221389484622e-06
151351,151352,151351,302703,78.15638518333435,5.758980473760684e-06
151552,151553,151552,303105,78.24030208587646,5.7417118665296125e-06
151752,151753,151752,303505,78.32296299934387,5.7245872065216314e-06
151952,151953,151952,303905,78.41066217422485,5.707520248421549e-06
152152,152153,152152,304305,78.50056719779968,5.690510806009137e-06
152352,152353,152352,304705,78.5856761932373,5.673558693701847e-06
152553,152554,152553,305107,78.67054414749146,5.656579395014361e-06
152753,152754,152753,305507,78.75332307815552,5.6397416732233425e-06
152953,152954,152953,305907,78.83580327033997,5.622960727485643e-06
153153,153154,153153,306307,78.91842103004456,5.60623637512853e-06
153353,153354,153353,306707,79.00165915489197,5.589568433535449e-06
153554,153555,153554,307109,79.08798432350159,5.572873803292435e-06
153754,153755,153754,307509,79.17192816734314,5.556318418328363e-06
153954,153955,153954,307909,79.25389814376831,5.53981889963583e-06
154154,154155,154154,308309,79.33682107925415,5.523375067476945e-06
154354,154355,154354,308709,79.42008829116821,5.506986742267757e-06
154555,154556,154555,309111,79.50329613685608,5.490572219075588e-06
154755,154756,154755,309511,79.59057116508484,5.474294647870861e-06
154955,154956,154955,309911,79.6765022277832,5.458072048367161e-06
155155,155156,155155,310311,79.75979328155518,5.441904243861847e-06
155355,155356,155355,310711,79.84225797653198,5.425791057964205e-06
155556,155557,155556,311113,79.92532205581665,5.409652157798915e-06
155756,155757,155756,311513,80.00808024406433,5.393647953517257e-06
155956,155957,155956,311913,80.09406614303589,5.377697841658157e-06
156156,156157,156156,312313,80.17740511894226,5.361801648365874e-06
156356,156357,156356,312713,80.26141428947449,5.345959200183234e-06
156557,156558,156557,313115,80.3458480834961,5.330091514488206e-06
156757,156758,156757,313515,80.42912697792053,5.314356305722761e-06
156957,156958,156957,313915,80.5181040763855,5.298674324951923e-06
157157,157158,157157,314315,80.60876226425171,5.283045401037381e-06
157357,157358,157357,314715,80.6929280757904,5.267469363605866e-06
157558,157559,157558,315117,80.77761626243591,5.251868558504785e-06
157758,157759,157758,315517,80.86196303367615,5.236398047709231e-06
157958,157959,157958,315917,80.9455292224884,5.220979914787411e-06
158158,158159,158158,316317,81.02847123146057,5.20561399170804e-06
158358,158359,158358,316717,81.11386227607727,5.190300110980987e-06
158559,158560,158559,317119,81.1976752281189,5.17496192570724e-06
158759,158760,158759,317519,81.28125214576721,5.159751887560836e-06
158959,158960,158959,317919,81.36353898048401,5.144593391857393e-06
159159,159160,159159,318319,81.44860219955444,5.12948627310576e-06
159359,159360,159359,318719,81.53195714950562,5.114430366742394e-06
159560,159561,159560,319121,81.61807608604431,5.099350612312682e-06
159760,159761,159760,319521,81.70053720474243,5.084396892996728e-06
159960,159961,159960,319921,81.78380703926086,5.069493894353015e-06
160160,160161,160160,320321,81.86683392524719,5.054641454197632e-06
160360,160361,160360,320721,81.94985604286194,5.039839410504112e-06
160561,160562,160561,321123,82.03676128387451,5.0250139685924725e-06
160761,160762,160761,321523,82.12274217605591,5.010312483961548e-06
160961,160962,160961,321923,82.20556426048279,4.995660912460998e-06
161161,161162,161161,322323,82.28741002082825,4.981059094358693e-06
161361,161362,161361,322723,82.3715672492981,4.966506870434838e-06
161562,161563,161562,323125,82.45309805870056,4.951931691979661e-06
161762,161763,161762,323525,82.53753519058228,4.937478426846193e-06
161962,161963,161962,323925,82.63427114486694,4.923074280748261e-06
162162,162163,162162,324325,82.71947121620178,4.908719096604075e-06
162362,162363,162362,324725,82.8032820224762,4.8944127178173414e-06
162563,162564,162563,325127,82.88685917854309,4.880083821849876e-06
162763,162764,162763,325527,82.96958422660828,4.865874828457729e-06
162963,162964,162963,325927,83.05414032936096,4.85171417324227e-06
163163,163164,163163,326327,83.13734722137451,4.837601701773514e-06
163363,163364,163363,326727,83.22019004821777,4.823537260273935e-06
163564,163565,163564,327129,83.30385899543762,4.809450732482969e-06
163764,163765,163764,327529,83.38437724113464,4.795482129261541e-06
163964,163965,163964,327929,83.46392297744751,4.7815610965890805e-06
164164,164165,164164,328329,83.54588413238525,4.767687482577345e-06
164364,164365,164364,328729,83.6284191608429,4.753861135957325e-06
164565,164566,164565,329131,83.70778298377991,4.7400131277851735e-06
164765,164766,164765,329531,83.78936123847961,4.7262810984038405e-06
164965,164966,164965,329931,83.87116599082947,4.712595884574897e-06
165165,165166,165165,330331,83.95205116271973,4.698957337224422e-06
165365,165366,165365,330731,84.03083395957947,4.685365307538176e-06
165566,165567,165566,331133,84.11362409591675,4.671752035158019e-06
165766,165767,165766,331533,84.19334197044373,4.658252826979034e-06
165966,165967,165966,331933,84.27852606773376,4.644799692376063e-06
166166,166167,166166,332333,84.35987210273743,4.631392484494098e-06
166366,166367,166366,332733,84.44255113601685,4.618031056900356e-06
166567,166568,166567,333135,84.5227541923523,4.604648799540899e-06
166767,166768,166767,333535,84.60620617866516,4.591378723030828e-06
166967,166968,166967,333935,84.69136810302734,4.5781539903311905e-06
167167,167168,167167,334335,84.77600693702698,4.564974456861088e-06
167367,167368,167367,334735,84.85540103912354,4.5518399790590344e-06
167568,167569,167568,335137,84.93938732147217,4.538685078197147e-06
167768,167769,167768,335537,85.04242515563965,4.525640505249132e-06
167968,167969,167968,335937,85.22534823417664,4.512640558597665e-06
168168,168169,168168,336337,85.35312700271606,4.499685096210891e-06
168368,168369,168368,336737,85.46996927261353,4.486773976566787e-06
168569,168570,168569,337139,85.62969517707825,4.473842834837155e-06
168769,168770,168769,337539,85.7568621635437,4.461020198219809e-06
168969,168970,168969,337939,85.85062408447266,4.448241482146131e-06
169169,169170,169169,338339,85.94550609588623,4.435506547144565e-06
169369,169370,169369,338739,86.03550601005554,4.422815253946041e-06
169570,169571,169570,339141,86.12473607063293,4.410104334204606e-06
169770,169771,169770,339541,86.21001601219177,4.397500125925452e-06
169970,169971,169970,339941,86.29458904266357,4.384939144325197e-06
170170,170171,170170,340341,86.39054322242737,4.3724212521793095e-06
170370,170371,170370,340741,86.47238612174988,4.35994631292614e-06
170571,170572,170571,341143,86.5525860786438,4.347452136560655e-06
170771,170772,170771,341543,86.63819599151611,4.335062907228532e-06
170971,170972,170971,341943,86.73045992851257,4.322716222189959e-06
171171,171172,171171,342343,86.83357119560242,4.310411946732527e-06
171371,171372,171371,342743,86.91714906692505,4.298149946170563e-06
171572,171573,171572,343145,87.00003099441528,4.285869092836647e-06
171772,171773,171772,343545,87.08158016204834,4.273691450262132e-06
171972,171973,171972,343945,87.16664028167725,4.261555681150889e-06
172172,172173,172172,344345,87.24870920181274,4.249461652809163e-06
172372,172373,172372,344745,87.33037424087524,4.2374092329218775e-06
172573,172574,172573,345147,87.41122102737427,4.225338339002142e-06
172773,172774,172773,345547,87.49238419532776,4.213368947507302e-06
172973,172974,172973,345947,87.57524108886719,4.201440769678948e-06
173173,173174,173173,346347,87.66237020492554,4.189553674950268e-06
173373,173374,173373,346747,87.74525022506714,4.177707533306873e-06
173574,173575,173574,347149,87.83526039123535,4.1658432907343624e-06
173774,173775,173774,347549,87.95246815681458,4.154078869982883e-06
173974,173975,173974,347949,88.06980514526367,4.142355013982203e-06
174174,174175,174174,348349,88.1721441745758,4.130671594444888e-06
174374,174375,174374,348749,88.27610397338867,4.119028483341975e-06
174575,174576,174575,349151,88.38093423843384,4.107367639356372e-06
174775,174776,174775,349551,88.55289220809937,4.095804963243175e-06
174975,174976,174975,349951,88.67004704475403,4.08428221362813e-06
175175,175176,175175,350351,88.75565695762634,4.07279926471679e-06
175375,175376,175375,350751,88.87589526176453,4.061355990216689e-06
175576,175577,175576,351153,89.08825612068176,4.049895345413593e-06
175776,175777,175776,351553,89.21320033073425,4.038531241383466e-06
175976,175977,175976,351953,89.31206822395325,4.027206436351518e-06
176176,176177,176176,352353,89.45635509490967,4.0159208061340195e-06
176376,176377,176376,352753,89.54749417304993,4.004674227189648e-06
176577,176578,176577,353155,89.63443422317505,3.993410635410604e-06
176777,176778,176777,353555,89.72042918205261,3.982241982920431e-06
176977,176978,176977,353955,89.80315232276917,3.971112012351288e-06
177177,177178,177177,354355,89.89599919319153,3.960020601547578e-06
177377,177378,177377,354755,89.99499011039734,3.948967628741191e-06
177578,177579,177578,355157,90.08924126625061,3.93789799552895e-06
177778,177779,177778,355557,90.18333697319031,3.926921725920134e-06
177978,177979,177978,355957,90.27276110649109,3.915983531108525e-06
178178,178179,178178,356357,90.35851216316223,3.905083291013593e-06
178378,178379,178378,356757,90.44582319259644,3.894220885888012e-06
178579,178580,178579,357159,90.53684210777283,3.883342167592487e-06
178779,178780,178779,357559,90.6274561882019,3.8725552626467974e-06
178979,178980,178979,357959,90.71124625205994,3.861805835294575e-06
179179,179180,179179,358359,90.79846811294556,3.851093767523302e-06
179379,179380,179379,358759,90.88042497634888,3.840418941583324e-06
179580,179581,179580,359161,90.97934126853943,3.829728144689203e-06
179780,179781,179780,359561,91.07939314842224,3.819127635572895e-06
179980,179981,179980,359961,91.16667222976685,3.8085640167242036e-06
180180,180181,180180,360361,91.25168704986572,3.798037172209107e-06
180380,180381,180380,360761,91.33764004707336,3.78754698582098e-06
180581,180582,180581,361163,91.43054604530334,3.7770411660805533e-06
180781,180782,180781,361563,91.51832413673401,3.766624132485261e-06
180981,180982,180981,361963,91.61066222190857,3.7562434117344197e-06
181181,181182,181181,362363,91.69976925849915,3.7458988894226225e-06
181381,181382,181381,362763,91.7863712310791,3.735590451487756e-06
181582,181583,181582,363165,91.87139511108398,3.725266712420481e-06
181782,181783,181782,363565,91.95488810539246,3.7150302823397906e-06
181982,181983,181982,363965,92.03960704803467,3.7048295966063823e-06
182182,182183,182182,364365,92.12823295593262,3.694664543184869e-06
182382,182383,182382,364765,92.21705722808838,3.6845350093777956e-06
182583,182584,182583,365167,92.30245923995972,3.674390502331316e-06
182783,182784,182783,365567,92.44869303703308,3.6643318500779676e-06
182983,182984,182983,365967,92.55951428413391,3.6543083833884026e-06
183183,183184,183183,366367,92.66052412986755,3.6443199917770276e-06
183383,183384,183383,366767,92.75522303581238,3.6343665645754896e-06
183584,183585,183584,367169,92.84922122955322,3.6243984866895515e-06
183784,183785,183784,367569,92.94401621818542,3.6145148331475004e-06
183984,183985,183984,367969,93.03875517845154,3.604665815118484e-06
184184,184185,184184,368369,93.13649106025696,3.594851323842784e-06
184384,184385,184384,368769,93.23334503173828,3.585071251068171e-06
184585,184586,184585,369171,93.32234311103821,3.5752768455795214e-06
184785,184786,184785,369571,93.43902111053467,3.5655654562939783e-06
184985,184986,184985,369971,93.54184913635254,3.555888161526495e-06
185185,185186,185185,370371,93.64711213111877,3.546244854486385e-06
185385,185386,185385,370771,93.74704813957214,3.5366354282192133e-06
185586,185587,185586,371173,93.84707713127136,3.5270119830807915e-06
185786,185787,185786,371573,93.94477319717407,3.5174701681373214e-06
185986,185987,185986,371973,94.04428720474243,3.5079619156391466e-06
186186,186187,186186,372373,94.14524602890015,3.4984871202307283e-06
186386,186387,186386,372773,94.24584603309631,3.489045676859773e-06
186587,186588,186587,373175,94.33968114852905,3.4795905234501075e-06
186787,186788,186787,373575,94.47994804382324,3.4702156363848467e-06
186987,186988,186987,373975,94.60863423347473,3.4608737880986954e-06
187187,187188,187187,374375,94.71200919151306,3.4515648749836343e-06
187387,187388,187387,374775,94.80528903007507,3.442288793944027e-06
187588,187589,187588,375177,94.90378499031067,3.432999306950669e-06
187788,187789,187788,375577,95.00267910957336,3.4237887440570193e-06
187988,187989,187988,375977,95.10134410858154,3.4146107047527672e-06
188188,188189,188188,376377,95.2101731300354,3.4054650870217814e-06
188388,188389,188388,376777,95.31319308280945,3.3963517894367473e-06
188589,188590,188589,377179,95.40930509567261,3.3872253859145233e-06
188789,188790,188789,377579,95.51400399208069,3.378176585100577e-06
188989,188990,188989,377979,95.61129713058472,3.3691598010748837e-06
189189,189190,189189,378379,95.71116232872009,3.360174933378381e-06
189389,189390,189389,378779,95.80019903182983,3.3512218820301922e-06
189590,189591,189590,379181,95.89053010940552,3.3422560202512777e-06
189790,189791,189790,379581,95.98109126091003,3.333366460839072e-06
189990,189991,189990,379981,96.0824122428894,3.3245084193059867e-06
190190,190191,190190,380381,96.1750180721283,3.3156817968977727e-06
190390,190391,190390,380781,96.2740581035614,3.3068864953261105e-06
190591,190592,190591,381183,96.36535811424255,3.2980786741537125e-06
190791,190792,190791,381583,96.4585211277008,3.2893458755720514e-06
190991,190992,190991,381983,96.55125403404236,3.2806441039922677e-06
191191,191192,191191,382383,96.64191317558289,3.271973262189206e-06
191391,191392,191391,382783,96.7356550693512,3.2633332534198247e-06
191592,191593,191592,383185,96.82852506637573,3.2546810119418195e-06
191792,191793,191792,383585,96.91915822029114,3.246102533030569e-06
191992,191993,191992,383985,97.02435898780823,3.2375545979473857e-06
192192,192193,192192,384385,97.1788592338562,3.229037111300812e-06
192392,192393,192392,384785,97.28403425216675,3.2205499777021097e-06
192593,192594,192593,385187,97.40208530426025,3.2120508937044906e-06
192793,192794,192793,385587,97.51149010658264,3.203624332187115e-06
192993,192994,192993,385987,97.68711829185486,3.1952278391694564e-06
193193,193194,193193,386387,97.82531714439392,3.18686132047068e-06
193393,193394,193393,386787,97.93581318855286,3.1785246828576896e-06
193594,193595,193594,387189,98.04452323913574,3.1701763724487542e-06
193794,193795,193794,387589,98.15052008628845,3.161899364064116e-06
193994,193995,193994,387989,98.2971830368042,3.153651956277848e-06
194194,194195,194194,388389,98.41300320625305,3.1454340564722e-06
194394,194395,194394,388789,98.52772212028503,3.1372455723753427e-06
194595,194596,194595,389191,98.6321370601654,3.1290456898217e-06
194795,194796,194795,389591,98.73207712173462,3.120915907429245e-06
194995,194996,194995,389991,98.83217430114746,3.1128152649873918e-06
195195,195196,195195,390391,98.93304705619812,3.1047436716530736e-06
195395,195396,195395,390791,99.04259729385376,3.096701036413431e-06
195596,195597,195596,391193,99.14281702041626,3.0886472721443106e-06
195796,195797,195796,391593,99.24699020385742,3.0806624253621303e-06
195996,195997,195996,391993,99.3459861278534,3.0727062652486203e-06
196196,196197,196196,392393,99.456707239151,3.0647787021755737e-06
196396,196397,196396,392793,99.63131618499756,3.0568796467545124e-06
196597,196598,196597,393195,99.73147392272949,3.0489697279017453e-06
196797,196798,196797,393595,99.82690906524658,3.041127561739402e-06
196997,196998,196997,393995,99.92197608947754,3.0333136362707805e-06
197197,197198,197197,394395,100.08301210403442,3.0255278630411608e-06
197397,197398,197397,394795,100.22543597221375,3.0177701539259605e-06
197598,197599,197598,395197,100.33053421974182,3.0100018425907908e-06
197798,197799,197798,395597,100.42784023284912,3.0023001379631036e-06
197998,197999,197998,395997,100.57458305358887,2.99462623443086e-06
198198,198199,198198,396397,100.73203611373901,2.9869800453218034e-06
198398,198399,198398,396797,100.84103512763977,2.9793614836000283e-06
198599,198600,198599,397199,100.95713806152344,2.9717325770115906e-06
198799,198800,198799,397599,101.0737202167511,2.964169148538521e-06
198999,199000,198999,397999,101.19772219657898,2.9566330888374547e-06
199199,199200,199199,398399,101.36313724517822,2.9491243120777195e-06
199399,199400,199399,398799,101.4587972164154,2.9416427331583467e-06
199600,199601,199600,399201,101.6027102470398,2.934151062541536e-06
199800,199801,199800,399601,101.77419400215149,2.926723758749551e-06
200000,200001,200000,400001,101.9226770401001,2.9193233981248053e-06


==> plot_data/bilinear_matrix_game_n500/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0008990764617919922,2.018959020339561
100,630,630,1260,0.7926907539367676,0.016955538903785962
200,1408,1408,2816,1.9575417041778564,0.00509124984935892
300,2194,2194,4388,2.821923017501831,0.0029190791169841366
400,2988,2988,5976,3.999485731124878,0.0019769291918388643
501,3788,3788,7576,4.753366947174072,0.001386850821596553
601,4578,4578,9156,5.501091003417969,0.0009261398725110851
701,5368,5368,10736,6.4988720417022705,0.0006371851507888394
801,6160,6160,12320,7.2532737255096436,0.00045484893904930196
901,6960,6960,13920,8.152987718582153,0.0004287061386675959
1001,7758,7758,15516,8.962201833724976,0.0003616089715194565
1101,8552,8552,17104,9.955989837646484,0.00028162733682044773
1201,9348,9348,18696,10.838840007781982,0.00024026955667390244
1301,10148,10148,20296,11.558543682098389,0.00023407537823526932
1401,10940,10940,21880,12.324745893478394,0.00017539558177249575
1502,11748,11748,23496,13.085269927978516,0.00017056819096984547
1602,12544,12544,25088,13.846674919128418,0.00014760133033107917
1702,13344,13344,26688,14.746678829193115,0.00014341869917563582
1802,14140,14140,28280,15.644820928573608,0.0001210621447322439
1902,14936,14936,29872,16.603880882263184,0.00010682822637046061
2002,15736,15736,31472,17.556581735610962,0.0001009986259508994
2102,16532,16532,33064,18.52286982536316,9.02976930312845e-05
2202,17332,17332,34664,19.873430967330933,8.448992177688343e-05
2302,18114,18114,36228,20.83201289176941,4.646700913824585e-05
2402,18914,18914,37828,21.978569984436035,4.22413395307836e-05
2503,19722,19722,39444,23.02886986732483,4.148860509170336e-05
2603,20522,20522,41044,24.078049898147583,4.1000273598608064e-05
2703,21316,21316,42632,25.140458822250366,3.239542001884659e-05
2803,22110,22110,44220,26.042916774749756,2.6661849554904908e-05
2903,22900,22900,45800,27.07267665863037,1.7326274576708128e-05
3003,23700,23700,47400,28.019145965576172,1.713009128439785e-05
3103,24496,24496,48992,29.041709899902344,1.4906355248503622e-05
3203,25296,25296,50592,30.39768075942993,1.4668108882325533e-05
3303,26096,26096,52192,31.57872772216797,1.4605272127657383e-05
3403,26896,26896,53792,32.56172490119934,1.4550957029235648e-05
3504,27694,27694,55388,33.59352087974548,1.0517257699384487e-05
3604,28494,28494,56988,34.594701051712036,1.0276429266699877e-05
3704,29294,29294,58588,35.55801177024841,1.0165989403438173e-05
3804,30094,30094,60188,36.523990869522095,1.0094068642342995e-05
3904,30894,30894,61788,37.59448170661926,1.0042615494573434e-05
4004,31692,31692,63384,38.588966846466064,9.662160914747742e-06
4104,32488,32488,64976,39.558127880096436,8.297329399426618e-06
4204,33288,33288,66576,40.49451684951782,8.167730381531815e-06
4304,34088,34088,68176,41.78272294998169,8.081141659904289e-06
4404,34888,34888,69776,42.905396938323975,8.01243396686031e-06
4505,35696,35696,71392,44.094162940979004,7.954645482219052e-06
4605,36496,36496,72992,45.21505689620972,7.905875249941169e-06
4705,37296,37296,74592,46.378437757492065,7.863640478012805e-06
4805,38096,38096,76192,47.41506886482239,7.826650289335817e-06
4905,38896,38896,77792,48.41278672218323,7.793952952282462e-06
5005,39696,39696,79392,49.449824810028076,7.764819611501512e-06
5105,40494,40494,80988,50.34048366546631,7.166402662396179e-06
5205,41294,41294,82588,51.24671196937561,7.047236425733933e-06
5305,42094,42094,84188,52.107511043548584,6.990741772512877e-06
5405,42894,42894,85788,52.984118938446045,6.9537677374474735e-06
5506,43702,43702,87404,53.8645658493042,6.925716947904835e-06
5606,44502,44502,89004,54.91956400871277,6.903215712920718e-06
5706,45302,45302,90604,55.76042985916138,6.884226767241571e-06
5806,46098,46098,92196,56.637136697769165,6.327974417755719e-06
5906,46898,46898,93796,57.5794198513031,6.208366959417366e-06
6006,47698,47698,95396,58.43850064277649,6.136007466258612e-06
6106,48498,48498,96996,59.393412828445435,6.084044217559392e-06
6206,49298,49298,98596,60.231329917907715,6.044335784100266e-06
6306,50098,50098,100196,61.10032367706299,6.01283857894685e-06
6406,50898,50898,101796,61.9570198059082,5.987261697908394e-06
6507,51706,51706,103412,62.80311870574951,5.965972732795764e-06
6607,52506,52506,105012,63.81721901893616,5.9484040330547516e-06
6707,53306,53306,106612,64.66270089149475,5.933614986659097e-06
6807,54106,54106,108212,65.51485896110535,5.92106982596861e-06
6907,54906,54906,109812,66.34856796264648,5.910352400037816e-06
7007,55706,55706,111412,67.19943881034851,5.901133338181961e-06
7107,56506,56506,113012,68.11392188072205,5.893148619359206e-06
7207,57306,57306,114612,69.03902983665466,5.886184733560652e-06
7307,58106,58106,116212,69.89641070365906,5.880067919030899e-06
7407,58906,58906,117812,70.80985498428345,5.874656086411362e-06
7508,59714,59714,119428,71.67700600624084,5.869787002670731e-06
7608,60514,60514,121028,72.55386996269226,5.8654603424681444e-06
7708,61314,61314,122628,73.49285769462585,5.861546002901846e-06
7808,62114,62114,124228,74.4341549873352,5.857978493310768e-06
7908,62914,62914,125828,75.3052008152008,5.854703492354356e-06
8008,63714,63714,127428,76.2234480381012,5.8516758491434274e-06
8108,64514,64514,129028,77.18024802207947,5.8488579589917724e-06
8208,65314,65314,130628,78.14422082901001,5.8462184416253495e-06
8308,66114,66114,132228,79.00415897369385,5.843731060338492e-06
8408,66914,66914,133828,79.85006284713745,5.841373837443945e-06
8509,67722,67722,135444,80.70301675796509,5.839106382327398e-06
8609,68522,68522,137044,81.70879673957825,5.836957968985265e-06
8709,69322,69322,138644,82.74072289466858,5.809443370042186e-06
8809,70122,70122,140244,83.72970986366272,5.793271603385568e-06
8909,70922,70922,141844,84.81722593307495,5.780556087621354e-06
9009,71722,71722,143444,86.0396568775177,5.769409677235646e-06
9109,72522,72522,145044,87.08651781082153,5.759252189389179e-06
9209,73322,73322,146644,88.03691792488098,5.749798073419194e-06
9309,74122,74122,148244,88.96929478645325,5.74087728462336e-06
9409,74922,74922,149844,89.91716074943542,5.7323778165870145e-06
9510,75730,75730,151460,90.85673475265503,5.724141135486942e-06
9610,76530,76530,153060,91.81113696098328,5.716272632508954e-06
9710,77330,77330,154660,92.76479887962341,5.708646194882714e-06
9810,78130,78130,156260,93.71330285072327,5.701228817024818e-06
9910,78930,78930,157860,94.63588285446167,5.693994694010253e-06
10010,79730,79730,159460,95.58167791366577,5.686923346424502e-06
10110,80530,80530,161060,96.505441904068,5.679998300698835e-06
10210,81330,81330,162660,97.44689989089966,5.67320613726925e-06
10310,82130,82130,164260,98.38244771957397,5.666535794335813e-06
10410,82930,82930,165860,99.29994988441467,5.659978047952543e-06
10511,83738,83738,167476,100.24005079269409,5.653461099630956e-06
10611,84538,84538,169076,101.17765402793884,5.6471073237840765e-06
10711,85338,85338,170676,102.33229184150696,5.640845993031622e-06
10811,86138,86138,172276,103.40878486633301,5.634672163954087e-06
10911,86938,86938,173876,104.35806894302368,5.628581503665035e-06
11011,87738,87738,175476,105.30638003349304,5.6225701828768e-06
11111,88538,88538,177076,106.22948884963989,5.616634791473215e-06
11211,89338,89338,178676,107.16312170028687,5.610772270460315e-06
11311,90136,90136,180272,108.18980884552002,5.433366258963905e-06
11411,90936,90936,181872,109.23143482208252,5.403292853218072e-06
11512,91744,91744,183488,110.34522795677185,5.389959419218816e-06
11612,92544,92544,185088,111.36492681503296,5.379030745130811e-06
11712,93344,93344,186688,112.28995084762573,5.369638516264796e-06
11812,94144,94144,188288,113.20416188240051,5.361383657521053e-06
11912,94944,94944,189888,114.07621598243713,5.353992105512874e-06
12012,95744,95744,191488,114.94809079170227,5.347266919615798e-06
12112,96544,96544,193088,115.91251301765442,5.341064042036829e-06
12212,97344,97344,194688,116.83648586273193,5.335276896750111e-06
12312,98144,98144,196288,117.82964181900024,5.329825866342663e-06
12412,98944,98944,197888,118.68134498596191,5.324650900786245e-06
12513,99752,99752,199504,119.56882405281067,5.319657845143588e-06
12613,100552,100552,201104,120.44012999534607,5.31491010416988e-06
12713,101352,101352,202704,121.35282683372498,5.310329810370406e-06
12813,102152,102152,204304,122.31796383857727,5.30589542210023e-06
12913,102944,102944,205888,123.26762580871582,5.192621568150064e-06
13013,103744,103744,207488,124.133535861969,5.16479772963822e-06
13113,104544,104544,209088,124.99061870574951,5.142004920835586e-06
13213,105344,105344,210688,125.85401701927185,5.1231099305234735e-06
13313,106144,106144,212288,126.704833984375,5.107257847446768e-06
13413,106944,106944,213888,127.56999182701111,5.093801173906834e-06
13514,107752,107752,215504,128.430490732193,5.082139849072233e-06
13614,108552,108552,217104,129.28515577316284,5.072124986796357e-06
13714,109352,109352,218704,130.1589138507843,5.063342636365345e-06
13814,110152,110152,220304,131.01790380477905,5.055568101051718e-06
13914,110952,110952,221904,131.8923008441925,5.048625788082972e-06
14014,111752,111752,223504,132.75447988510132,5.04237737357884e-06
14114,112552,112552,225104,133.61401176452637,5.036712972719286e-06
14214,113352,113352,226704,134.48756885528564,5.031544529553057e-06
14314,114152,114152,228304,135.33707070350647,5.02680085013945e-06
14414,114952,114952,229904,136.2086319923401,5.022423855243657e-06
14515,115760,115760,231520,137.06181693077087,5.018326629130713e-06
14615,116560,116560,233120,137.8997449874878,5.014550312422205e-06
14715,117360,117360,234720,138.75052285194397,5.011019631983871e-06
14815,118160,118160,236320,139.58890986442566,5.0077065643186775e-06
14915,118960,118960,237920,140.42978978157043,5.004587261485966e-06
15015,119760,119760,239520,141.2569169998169,5.001641279663504e-06
15115,120560,120560,241120,142.07784700393677,4.998850972807352e-06
15215,121360,121360,242720,142.91890573501587,4.9962010146302325e-06
15315,122160,122160,244320,143.7598798274994,4.993678014896531e-06
15415,122960,122960,245920,144.8801829814911,4.991270213706705e-06
15516,123768,123768,247536,145.85919785499573,4.9889447000698655e-06
15616,124568,124568,249136,146.90839290618896,4.986738253236554e-06
15716,125368,125368,250736,147.82764101028442,4.984619163624402e-06
15816,126168,126168,252336,148.81653380393982,4.982580128397618e-06
15916,126968,126968,253936,149.85489296913147,4.980614604300355e-06
16016,127768,127768,255536,150.78765177726746,4.978716710934794e-06
16116,128568,128568,257136,151.72352981567383,4.97688115084674e-06
16216,129368,129368,258736,152.71759796142578,4.975103139092488e-06
16316,130168,130168,260336,153.5848367214203,4.9733783446441515e-06
16416,130968,130968,261936,154.42488169670105,4.971702839861684e-06
16517,131776,131776,263552,155.25937390327454,4.970056977581966e-06
16617,132576,132576,265152,156.12090182304382,4.96847007503903e-06
16717,133376,133376,266752,157.02502870559692,4.966922655717912e-06
16817,134176,134176,268352,157.87944173812866,4.965412018782064e-06
16917,134976,134976,269952,158.77211785316467,4.963935695571115e-06
17017,135776,135776,271552,159.64168286323547,4.962491425940999e-06
17117,136576,136576,273152,160.4925618171692,4.9610771391968174e-06
17217,137376,137376,274752,161.3494598865509,4.95969093471717e-06
17317,138176,138176,276352,162.27296996116638,4.958331067236122e-06
17417,138976,138976,277952,163.24627780914307,4.956995931715843e-06
17518,139784,139784,279568,164.17522287368774,4.955671044840833e-06
17618,140584,140584,281168,165.15838384628296,4.954381269944263e-06
17718,141384,141384,282768,166.15204977989197,4.953112120964265e-06
17818,142184,142184,284368,166.96804976463318,4.951862440025244e-06
17918,142984,142984,285968,167.77408289909363,4.950631157126128e-06
18018,143784,143784,287568,168.63221979141235,4.9494172823507566e-06
18118,144584,144584,289168,169.48170065879822,4.948219899866434e-06
18218,145384,145384,290768,170.4063549041748,4.947038160690222e-06
18318,146184,146184,292368,171.40724086761475,4.945871277590534e-06
18418,146984,146984,293968,172.41504979133606,4.944718520160994e-06
18519,147792,147792,295584,173.5036427974701,4.943567881934315e-06
18619,148592,148592,297184,174.54851388931274,4.9424415120070085e-06
18719,149392,149392,298784,175.63830399513245,4.941327364929787e-06
18819,150192,150192,300384,176.61627578735352,4.9402248938552925e-06
18919,150992,150992,301984,177.6413698196411,4.9391335893815905e-06
19019,151792,151792,303584,178.7753746509552,4.93805297615081e-06
19119,152592,152592,305184,179.894122838974,4.9369826100609116e-06
19219,153392,153392,306784,180.8796968460083,4.935922076426304e-06
19319,154192,154192,308384,181.86896467208862,4.93487098702412e-06
19419,154992,154992,309984,182.68357181549072,4.93382897844952e-06
19520,155800,155800,311600,183.52358388900757,4.932785420841633e-06
19620,156600,156600,313200,184.35950994491577,4.931760656522194e-06
19720,157400,157400,314800,185.56887292861938,4.930744011056225e-06
19820,158200,158200,316400,186.87751483917236,4.929735202655005e-06
19920,159000,159000,318000,188.01257181167603,4.928733967078879e-06
20020,159800,159800,319600,188.9733808040619,4.927740055307313e-06
20120,160600,160600,321200,189.8329257965088,4.926753232761681e-06
20220,161400,161400,322800,190.85738372802734,4.9257732787178775e-06
20320,162200,162200,324400,191.68229293823242,4.924799984467828e-06
20420,163000,163000,326000,192.81600689888,4.923833153096547e-06
20521,163808,163808,327616,193.80948185920715,4.922863024241698e-06
20621,164608,164608,329216,194.69390892982483,4.92190863091457e-06
20721,165408,165408,330816,195.55455470085144,4.920960170058639e-06
20821,166208,166208,332416,196.43030071258545,4.920017484250153e-06
20921,167008,167008,334016,197.29114484786987,4.919080423562327e-06
21021,167808,167808,335616,198.19066286087036,4.918148846148426e-06
21121,168608,168608,337216,199.06382083892822,4.917222617117805e-06
21221,169408,169408,338816,199.9280970096588,4.9163016082130124e-06
21321,170208,170208,340416,200.77890586853027,4.915385697379111e-06
21421,171008,171008,342016,201.60491490364075,4.914474768486693e-06
21522,171816,171816,343632,202.45354390144348,4.9135596743875945e-06
21622,172616,172616,345232,203.27708888053894,4.912658429265875e-06
21722,173416,173416,346832,204.10430002212524,4.91176184803219e-06
21822,174216,174216,348432,204.9461328983307,4.91086983405129e-06
21922,175016,175016,350032,205.7898817062378,4.909982295532316e-06
22022,175816,175816,351632,206.6513638496399,4.909099144396792e-06
22122,176616,176616,353232,207.5239598751068,4.90822029600857e-06
22222,177416,177416,354832,208.38232278823853,4.907345669585487e-06
22322,178216,178216,356432,209.26846885681152,4.906475187651591e-06
22422,179016,179016,358032,210.15039777755737,4.905608775775045e-06
22523,179824,179824,359648,211.0474009513855,4.904737758157217e-06
22623,180624,180624,361248,211.9204399585724,4.9038793132754394e-06
22723,181424,181424,362848,212.74619269371033,4.903024731245771e-06
22823,182224,182224,364448,213.59569191932678,4.90217394848497e-06
22923,183024,183024,366048,214.43516492843628,4.901326903363302e-06
23023,183824,183824,367648,215.28404784202576,4.900483537009076e-06
23123,184624,184624,369248,216.12264966964722,4.899643792292679e-06
23223,185424,185424,370848,216.98411178588867,4.898807613953216e-06
23323,186224,186224,372448,217.85246896743774,4.897974948929928e-06
23423,187024,187024,374048,218.69842386245728,4.8971457455601415e-06
23524,187832,187832,375664,219.5846288204193,4.896311713132123e-06
23624,188632,188632,377264,220.4475588798523,4.895489318677397e-06
23724,189432,189432,378864,221.30826377868652,4.894670240703785e-06
23824,190232,190232,380464,222.19872570037842,4.893854433838033e-06
23924,191032,191032,382064,223.0712399482727,4.893041854262482e-06
24024,191832,191832,383664,223.95579481124878,4.892232459248288e-06
24124,192632,192632,385264,224.77918887138367,4.891426207524228e-06
24224,193432,193432,386864,225.61920475959778,4.89062305875853e-06
24324,194232,194232,388464,226.46440482139587,4.889822973762024e-06
24424,195032,195032,390064,227.29020380973816,4.88902591476898e-06
24525,195840,195840,391680,228.15982484817505,4.8882239186026426e-06
24625,196640,196640,393280,229.01238870620728,4.887432830315789e-06
24725,197440,197440,394880,229.85817885398865,4.886644659212072e-06
24825,198240,198240,396480,230.72473978996277,4.8858593709398355e-06
24925,199040,199040,398080,231.57987189292908,4.885076932184582e-06
25025,199840,199840,399680,232.45204281806946,4.884297310261742e-06
25125,200640,200640,401280,233.4643907546997,4.883520473427146e-06
25225,201440,201440,402880,234.43414187431335,4.882746390446844e-06
25325,202240,202240,404480,235.5612998008728,4.8819750311302345e-06
25425,203040,203040,406080,236.3941798210144,4.881206365401439e-06
25526,203848,203848,407696,237.3497438430786,4.880432717790807e-06
25626,204648,204648,409296,238.19102096557617,4.879669379365874e-06
25726,205448,205448,410896,239.10012078285217,4.87890864907179e-06
25826,206248,206248,412496,239.95978474617004,4.878150499676639e-06
25926,207048,207048,414096,240.79580283164978,4.877394904184224e-06
26026,207848,207848,415696,241.65496683120728,4.87664183694365e-06
26126,208648,208648,417296,242.5050618648529,4.875891271896491e-06
26226,209448,209448,418896,243.37648487091064,4.875143183836067e-06
26326,210248,210248,420496,244.2464439868927,4.87439754818149e-06
26426,211048,211048,422096,245.1106469631195,4.873654340754695e-06
26527,211856,211856,423712,245.99679374694824,4.872906141619082e-06
26627,212656,212656,425312,246.96126985549927,4.8721677430374195e-06
26727,213456,213456,426912,247.80768465995789,4.871431702217687e-06
26827,214256,214256,428512,248.65327262878418,4.870697996449882e-06
26927,215056,215056,430112,249.50585079193115,4.869966603788587e-06
27027,215856,215856,431712,250.34847784042358,4.8692375022141085e-06
27127,216656,216656,433312,251.19623804092407,4.868510670209844e-06
27227,217456,217456,434912,252.06609892845154,4.867786086722743e-06
27327,218256,218256,436512,252.92696595191956,4.867063731033386e-06
27427,219056,219056,438112,253.79932594299316,4.86634358252248e-06
27528,219864,219864,439728,254.66587591171265,4.865618452514604e-06
27628,220664,220664,441328,255.52389979362488,4.8649026800900085e-06
27728,221464,221464,442928,256.39035391807556,4.864189055061051e-06
27828,222264,222264,444528,257.2500698566437,4.863477558393832e-06
27928,223064,223064,446128,258.12548780441284,4.8627681710635504e-06
28028,223864,223864,447728,258.98813104629517,4.86206087405649e-06
28128,224664,224664,449328,259.77605867385864,4.861355649380006e-06
28228,225464,225464,450928,260.52522373199463,4.86065247879821e-06
28328,226264,226264,452528,261.3929898738861,4.8599513439297705e-06
28428,227064,227064,454128,262.2297878265381,4.859252227516353e-06
28529,227872,227872,455744,263.0964767932892,4.858548150552324e-06
28629,228672,228672,457344,263.96510791778564,4.857853038265656e-06
28729,229472,229472,458944,264.83814883232117,4.85715989229644e-06
28829,230272,230272,460544,265.8015468120575,4.8564686957794885e-06
28929,231072,231072,462144,266.72592186927795,4.8557794322898615e-06
29029,231872,231872,463744,267.651154756546,4.855092085696993e-06
29129,232672,232672,465344,268.5532920360565,4.854406639361983e-06
29229,233472,233472,466944,269.5044207572937,4.8537230774488914e-06
29329,234272,234272,468544,270.5796809196472,4.853041384257598e-06
29429,235072,235072,470144,271.42698884010315,4.852361544207562e-06
29530,235880,235880,471760,272.24646973609924,4.851676770874589e-06
29630,236680,236680,473360,273.0845878124237,4.851000608963806e-06
29730,237480,237480,474960,273.9310188293457,4.850326254433214e-06
29830,238280,238280,476560,274.7721838951111,4.84965369204159e-06
29930,239080,239080,478160,275.64069867134094,4.848982907298591e-06
30030,239880,239880,479760,276.5107419490814,4.848313885627249e-06
30130,240680,240680,481360,277.39399695396423,4.847646612664651e-06
30230,241480,241480,482960,278.25378465652466,4.846981074000991e-06
30330,242280,242280,484560,279.1093487739563,4.846317255722349e-06
30430,243080,243080,486160,279.9962718486786,4.845655143855417e-06
30531,243888,243888,487776,280.86738872528076,4.84498812887101e-06
30631,244688,244688,489376,281.756728887558,4.844329405283994e-06
30731,245488,245488,490976,282.604291677475,4.843672347167358e-06
30831,246288,246288,492576,283.4243607521057,4.8430169409837094e-06
30931,247088,247088,494176,284.2591378688812,4.842363173538502e-06
31031,247888,247888,495776,285.07599091529846,4.841711031847414e-06
31131,248688,248688,497376,285.9197928905487,4.841060502887077e-06
31231,249488,249488,498976,286.7690348625183,4.840411573964157e-06
31331,250288,250288,500576,287.63460969924927,4.8397642321744656e-06
31431,251088,251088,502176,288.50277280807495,4.839118465207043e-06
31532,251896,251896,503792,289.3569269180298,4.838467826234232e-06
31632,252696,252696,505392,290.22660279273987,4.837825186795306e-06
31732,253496,253496,506992,291.07087087631226,4.837184085069309e-06
31832,254296,254296,508592,291.922376871109,4.8365445087957174e-06
31932,255096,255096,510192,292.7827777862549,4.835906446201516e-06
32032,255896,255896,511792,293.6375789642334,4.835269885319518e-06
32132,256696,256696,513392,294.52702379226685,4.834634814306966e-06
32232,257496,257496,514992,295.3943347930908,4.834001221924884e-06
32332,258296,258296,516592,296.2365906238556,4.8333690963550625e-06
32432,259096,259096,518192,297.09894585609436,4.832738426052974e-06
32533,259904,259904,519808,297.92349100112915,4.8321029151325255e-06
32633,260702,260702,521404,298.8180968761444,4.604629833097849e-06
32733,261502,261502,523004,299.67667508125305,4.600136419406604e-06
32833,262302,262302,524604,300.5567948818207,4.598995723804767e-06
32933,263102,263102,526204,301.49195075035095,4.59799024382155e-06
33033,263902,263902,527804,302.3635907173157,4.597029172412958e-06
33133,264702,264702,529404,303.28103399276733,4.596095111804067e-06
33233,265502,265502,531004,304.20198702812195,4.595182097446971e-06
33333,266302,266302,532604,305.0831227302551,4.594287307279866e-06
33433,267102,267102,534204,305.93928694725037,4.593409070575173e-06
33534,267910,267910,535820,306.75472378730774,4.592537672199313e-06
33634,268710,268710,537420,307.597305059433,4.59168945930272e-06
33734,269510,269510,539020,308.41223192214966,4.590854978280289e-06
33834,270310,270310,540620,309.2356929779053,4.590033572718997e-06
33934,271110,271110,542220,310.05858993530273,4.589224651523402e-06
34034,271910,271910,543820,310.88651275634766,4.588427672530782e-06
34134,272710,272710,545420,311.75761580467224,4.587642131591869e-06
34234,273510,273510,547020,312.6985809803009,4.586867556622695e-06
34334,274310,274310,548620,313.58072900772095,4.586103502595802e-06
34434,275110,275110,550220,314.4611887931824,4.585349548543548e-06
34535,275918,275918,551836,315.3573157787323,4.5845979001196075e-06
34635,276718,276718,553436,316.23239183425903,4.5838630585919506e-06
34735,277518,277518,555036,317.05743384361267,4.583137172192717e-06
34835,278318,278318,556636,317.8846950531006,4.582419896216173e-06
34935,279118,279118,558236,318.6962339878082,4.581710901786448e-06
35035,279918,279918,559836,319.5149998664856,4.581009874293144e-06
35135,280718,280718,561436,320.33840894699097,4.5803165133171275e-06
35235,281518,281518,563036,321.157292842865,4.579630531523523e-06
35335,282318,282318,564636,321.9951958656311,4.578951654450081e-06
35435,283118,283118,566236,322.8395128250122,4.5782796186758716e-06
35536,283926,283926,567852,323.6903610229492,4.577607550395796e-06
35636,284726,284726,569452,324.55676794052124,4.576948515006481e-06
35736,285526,285526,571052,325.43005895614624,4.576295594823995e-06
35836,286326,286326,572652,326.2960648536682,4.575648568793212e-06
35936,287126,287126,574252,327.15095591545105,4.5750072249533764e-06
36036,287926,287926,575852,328.0015528202057,4.574371360133256e-06
36136,288726,288726,577452,328.8373968601227,4.5737407795328165e-06
36236,289526,289526,579052,329.66507482528687,4.573115296510676e-06
36336,290326,290326,580652,330.4839859008789,4.5724947319996e-06
36436,291126,291126,582252,331.3189299106598,4.571878914236683e-06
36537,291934,291934,583868,332.14726185798645,4.5712615887379586e-06
36637,292734,292734,585468,332.98975467681885,4.57065482034825e-06
36737,293534,293534,587068,333.8265359401703,4.570052322558124e-06
36837,294334,294334,588668,334.661732673645,4.569453950245414e-06
36937,295134,295134,590268,335.51571774482727,4.568859563422218e-06
37037,295934,295934,591868,336.3485789299011,4.568269027976445e-06
37137,296734,296734,593468,337.2322108745575,4.56768221532667e-06
37237,297534,297534,595068,338.102303981781,4.567099001671959e-06
37337,298334,298334,596668,338.95053005218506,4.566519268536585e-06
37437,299134,299134,598268,339.79618096351624,4.565942901704047e-06
37538,299942,299942,599884,340.627445936203,4.565364076659206e-06
37638,300742,300742,601484,341.4716627597809,4.564794149082148e-06
37738,301542,301542,603084,342.3094928264618,4.564227270937175e-06
37838,302342,302342,604684,343.1310279369354,4.563663345093994e-06
37938,303142,303142,606284,343.97211170196533,4.563102278070568e-06
38038,303942,303942,607884,344.79497170448303,4.56254398018525e-06
38138,304742,304742,609484,345.64529395103455,4.561988365077883e-06
38238,305542,305542,611084,346.47989988327026,4.561435349716041e-06
38338,306342,306342,612684,347.31504583358765,4.560884854448118e-06
38438,307142,307142,614284,348.1879677772522,4.560336802368728e-06
38539,307950,307950,615900,349.05001974105835,4.559785674774761e-06
38639,308750,308750,617500,349.83297181129456,4.559242313078218e-06
38739,309550,309550,619100,350.66041898727417,4.558701181016537e-06
38839,310350,310350,620700,351.49822998046875,4.558162212476368e-06
38939,311150,311150,622300,352.38021874427795,4.557625344458531e-06
39039,311950,311950,623900,353.2207820415497,4.557090515972697e-06
39139,312750,312750,625500,354.0847599506378,4.556557668357964e-06
39239,313550,313550,627100,354.9390697479248,4.556026745130521e-06
39339,314350,314350,628700,355.8520188331604,4.555497692130276e-06
39439,315150,315150,630300,356.7360818386078,4.554970456821213e-06
39540,315958,315958,631916,357.642187833786,4.554439743033921e-06
39640,316758,316758,633516,358.53472995758057,4.553916011005039e-06
39740,317558,317558,635116,359.4381899833679,4.553393950338097e-06
39840,318358,318358,636716,360.4898109436035,4.552873516300069e-06
39940,319158,319158,638316,361.3630976676941,4.552354665307639e-06
40040,319958,319958,639916,362.2273428440094,4.5518373554659675e-06
40140,320758,320758,641516,363.0611128807068,4.5513215464001764e-06
40240,321558,321558,643116,363.873242855072,4.55080719921714e-06
40340,322358,322358,644716,364.7028238773346,4.550294276369271e-06
40440,323158,323158,646316,365.5385158061981,4.54978274179864e-06
40541,323966,323966,647932,366.36861276626587,4.549267465265683e-06
40641,324766,324766,649532,367.22014689445496,4.548758616499264e-06
40741,325566,325566,651132,368.0564568042755,4.5482510545093114e-06
40841,326366,326366,652732,368.9077949523926,4.547744747803345e-06
40941,327166,327166,654332,369.75778889656067,4.54723966626595e-06
41041,327966,327966,655932,370.6086540222168,4.5467357806738975e-06
41141,328766,328766,657532,371.4674518108368,4.546233062714463e-06
41241,329566,329566,659132,372.3226318359375,4.545731485207718e-06
41341,330366,330366,660732,373.1804118156433,4.545231021870882e-06
41441,331166,331166,662332,374.0215017795563,4.544731647151984e-06
41542,331974,331974,663948,374.84240889549255,4.5442283589715e-06
41642,332774,332774,665548,375.67625188827515,4.543731099118786e-06
41742,333574,333574,667148,376.49810671806335,4.5432348566189585e-06
41842,334374,334374,668748,377.31036901474,4.5427396090496e-06
41942,335174,335174,670348,378.1477608680725,4.542245335391556e-06
42042,335974,335974,671948,378.98577976226807,4.541752014398165e-06
42142,336774,336774,673548,379.85609579086304,4.541259626222222e-06
42242,337574,337574,675148,380.71719694137573,4.540768151683778e-06
42342,338374,338374,676748,381.5789318084717,4.540277571861651e-06
42442,339174,339174,678348,382.46274304389954,4.539787868449689e-06
42543,339982,339982,679964,383.33225178718567,4.539294139877735e-06
42643,340782,340782,681564,384.2068946361542,4.538806145685264e-06
42743,341582,341582,683164,385.025554895401,4.538318976774654e-06
42843,342382,342382,684764,385.84014987945557,4.537832617328752e-06
42943,343182,343182,686364,386.6870319843292,4.53734705160405e-06
43043,343982,343982,687964,387.53700590133667,4.536862264731915e-06
43143,344782,344782,689564,388.39708375930786,4.5363782423431245e-06
43243,345582,345582,691164,389.22591185569763,4.535894970212356e-06
43343,346382,346382,692764,390.07443499565125,4.535412434593025e-06
43443,347182,347182,694364,390.9308090209961,4.534930622547914e-06
43544,347990,347990,695980,391.7805030345917,4.534444713558768e-06
43644,348790,348790,697580,392.6474578380585,4.5339643170998035e-06
43744,349590,349590,699180,393.4966628551483,4.533484606584482e-06
43844,350390,350390,700780,394.3668968677521,4.533005570160431e-06
43944,351190,351190,702380,395.23564887046814,4.532527196600475e-06
44044,351990,351990,703980,396.0571939945221,4.5320494746626894e-06
44144,352790,352790,705580,396.90811800956726,4.5315723940323325e-06
44244,353590,353590,707180,397.7412328720093,4.531095943725527e-06
44344,354390,354390,708780,398.5853097438812,4.530620114090053e-06
44444,355190,355190,710380,399.4412217140198,4.5301448948582016e-06
44545,355998,355998,711996,400.2950849533081,4.529665533662585e-06
44645,356798,356798,713596,401.1493937969208,4.529191513137263e-06
44745,357598,357598,715196,401.9968638420105,4.528718075395577e-06
44845,358398,358398,716796,402.8418688774109,4.528245211329192e-06
44945,359198,359198,718396,403.72151279449463,4.527772912432723e-06
45045,359998,359998,719996,404.5745527744293,4.52730117057756e-06
45145,360798,360798,721596,405.44981598854065,4.52682997727656e-06
45245,361598,361598,723196,406.3095679283142,4.526359324958034e-06
45345,362398,362398,724796,407.16922998428345,4.52588920584027e-06
45445,363198,363198,726396,408.00772285461426,4.52541961235316e-06
45546,364006,364006,728012,408.83425283432007,4.524945849087261e-06
45646,364806,364806,729612,409.67748403549194,4.524477290261283e-06
45746,365606,365606,731212,410.52584171295166,4.5240092356034084e-06
45846,366406,366406,732812,411.35876870155334,4.5235416785357625e-06
45946,367206,367206,734412,412.20716166496277,4.523074612339908e-06
46046,368006,368006,736012,413.07431292533875,4.522608030567709e-06
46146,368806,368806,737612,413.9371078014374,4.5221419268933725e-06
46246,369606,369606,739212,414.7819848060608,4.521676295078724e-06
46346,370406,370406,740812,415.62191891670227,4.521211129534075e-06
46446,371206,371206,742412,416.4683289527893,4.52074642407511e-06
46547,372014,372014,744028,417.3904798030853,4.520277532753709e-06
46647,372814,372814,745628,418.19849276542664,4.519813735035613e-06
46747,373614,373614,747228,419.0173718929291,4.519350380793215e-06
46847,374414,374414,748828,419.9220037460327,4.518887464482064e-06
46947,375214,375214,750428,420.74579882621765,4.51842498115821e-06
47047,376014,376014,752028,421.6141617298126,4.517962925485357e-06
47147,376814,376814,753628,422.57165575027466,4.517501292560722e-06
47247,377614,377614,755228,423.3883128166199,4.517040077442627e-06
47347,378414,378414,756828,424.2993037700653,4.516579275538917e-06
47447,379214,379214,758428,425.1042637825012,4.516118882064248e-06
47548,380022,380022,760044,425.83719182014465,4.51565429453464e-06
47648,380822,380822,761644,426.69406270980835,4.515194708315209e-06
47748,381622,381622,763244,427.41465067863464,4.514735516961886e-06
47848,382422,382422,764844,428.09939670562744,4.514276716357121e-06
47948,383222,383222,766444,428.78592681884766,4.513818302267018e-06
48048,384022,384022,768044,429.4677770137787,4.513360270517133e-06
48148,384822,384822,769644,430.1439788341522,4.512902616914464e-06
48248,385622,385622,771244,430.82603788375854,4.512445337807345e-06
48348,386422,386422,772844,431.49393582344055,4.511988429012249e-06
48448,387222,387222,774444,432.17587876319885,4.5115318870023404e-06
48549,388030,388030,776060,432.86178183555603,4.511071147794614e-06
48649,388830,388830,777660,433.54260301589966,4.5106153314006604e-06
48749,389630,389630,779260,434.21233892440796,4.510159870537256e-06
48849,390430,390430,780860,434.88283681869507,4.509704761707304e-06
48949,391230,391230,782460,435.56576466560364,4.50925000149336e-06
49049,392030,392030,784060,436.2403109073639,4.5087955863804175e-06
49149,392830,392830,785660,436.91282391548157,4.5083415130721365e-06
49249,393628,393628,787256,437.60137271881104,4.2811613440091574e-06
49349,394428,394428,788856,438.26620388031006,4.279149905351285e-06
49449,395228,395228,790456,438.9322507381439,4.278267991906017e-06
49550,396036,396036,792072,439.62207794189453,4.277519405663049e-06
49650,396836,396836,793672,440.28833293914795,4.276827588954259e-06
49750,397636,397636,795272,440.9682049751282,4.276162249322784e-06
49850,398436,398436,796872,441.65726590156555,4.275514965707856e-06
49950,399236,399236,798472,442.3254859447479,4.274881706666361e-06
50050,400036,400036,800072,442.9983060359955,4.274260203280592e-06
50150,400836,400836,801672,443.70089173316956,4.273649020894579e-06
50250,401636,401636,803272,444.3693606853485,4.273047168815719e-06
50350,402436,402436,804872,445.0388159751892,4.272453911465919e-06
50450,403236,403236,806472,445.71952295303345,4.271868670512469e-06
50551,404044,404044,808088,446.39727878570557,4.271285229989237e-06
50651,404844,404844,809688,447.0629949569702,4.270714733140953e-06
50751,405644,405644,811288,447.7454209327698,4.270151009671269e-06
50851,406444,406444,812888,448.4210548400879,4.269593739421163e-06
50951,407244,407244,814488,449.09549379348755,4.269042629839699e-06
51051,408044,408044,816088,449.7794077396393,4.268497410972689e-06
51151,408840,408840,817680,450.44807171821594,3.8296867042511715e-06
51251,409638,409638,819276,451.12031292915344,3.594426338129996e-06
51351,410438,410438,820876,451.8029806613922,3.5400606683056335e-06
51451,411238,411238,822476,452.4754078388214,3.4962482928613617e-06
51552,412046,412046,824092,453.1487259864807,3.4593219659608056e-06
51652,412846,412846,825692,453.81065797805786,3.428055334031666e-06
51752,413646,413646,827292,454.4929008483887,3.4007800747659677e-06
51852,414446,414446,828892,455.15683674812317,3.3766250114890736e-06
51952,415246,415246,830492,455.82266902923584,3.3549720768525768e-06
52052,416046,416046,832092,456.50462889671326,3.335369500092996e-06
52152,416846,416846,833692,457.1861927509308,3.317478200766124e-06
52252,417646,417646,835292,457.8527789115906,3.3010376297035518e-06
52352,418446,418446,836892,458.5350978374481,3.285843392858299e-06
52452,419246,419246,838492,459.20307874679565,3.271732211555962e-06
52553,420054,420054,840108,459.87815380096436,3.2584443747405506e-06
52653,420854,420854,841708,460.572518825531,3.246133138568061e-06
52753,421654,421654,843308,461.2467758655548,3.234571703561925e-06
52853,422454,422454,844908,461.9201228618622,3.223683699355742e-06
52953,423254,423254,846508,462.6046619415283,3.2134041934287082e-06
53053,424054,424054,848108,463.2747230529785,3.203677498013672e-06
53153,424854,424854,849708,463.94705295562744,3.1944554787905707e-06
53253,425654,425654,851308,464.6268730163574,3.1856962281394353e-06
53353,426454,426454,852908,465.2961657047272,3.177363015772136e-06
53453,427254,427254,854508,465.969518661499,3.1694234475433375e-06
53554,428062,428062,856124,466.6589608192444,3.1617747942098056e-06
53654,428862,428862,857724,467.3267467021942,3.15454268305767e-06
53754,429662,429662,859324,468.010470867157,3.1476266510940117e-06
53854,430462,430462,860924,468.69107484817505,3.141006018186456e-06
53954,431262,431262,862524,469.35880279541016,3.1346620686029022e-06
54054,432062,432062,864124,470.02805495262146,3.128577792921577e-06
54154,432862,432862,865724,470.707722902298,3.1227376717756032e-06
54254,433662,433662,867324,471.37081599235535,3.1171274923839448e-06
54354,434462,434462,868924,472.04375171661377,3.1117341942388632e-06
54454,435262,435262,870524,472.7148768901825,3.106545738264017e-06
54555,436070,436070,872140,473.4052426815033,3.10150198951808e-06
54655,436870,436870,873740,474.07576179504395,3.096692423690446e-06
54755,437670,437670,875340,474.7402718067169,3.0920565710570304e-06
54855,438470,438470,876940,475.42448377609253,3.0875855075343113e-06
54955,439270,439270,878540,476.09077763557434,3.0832709038194283e-06
55055,440070,440070,880140,476.7721858024597,3.0791049711801535e-06
55155,440870,440870,881740,477.46339082717896,3.0750804141059163e-06
55255,441670,441670,883340,478.13604402542114,3.0711903879618465e-06
55355,442470,442470,884940,478.8070378303528,3.0674284619536607e-06
55455,443270,443270,886540,479.4933376312256,3.063788585996164e-06
55556,444078,444078,888156,480.1699357032776,3.060230395912923e-06
55656,444878,444878,889756,480.8388600349426,3.0568189344217648e-06
55756,445678,445678,891356,481.5193657875061,3.0535133313634625e-06
55856,446478,446478,892956,482.18526887893677,3.0503087978621714e-06
55956,447278,447278,894556,482.8539698123932,3.0472008067919614e-06
56056,448078,448078,896156,483.5408387184143,3.044185073557163e-06
56156,448878,448878,897756,484.21158480644226,3.0412575413533305e-06
56256,449678,449678,899356,484.87315678596497,3.0384143657726303e-06
56356,450478,450478,900956,485.5613868236542,3.0356519018993244e-06
56456,451278,451278,902556,486.22636103630066,3.0329666918226397e-06
56557,452086,452086,904172,486.91212797164917,3.0303297036470373e-06
56657,452886,452886,905772,487.60012102127075,3.0277900125222558e-06
56757,453686,453686,907372,488.28559279441833,3.025318185206183e-06
56857,454486,454486,908972,488.95743894577026,3.02291140759902e-06
56957,455286,455286,910572,489.6366708278656,3.0205670040805893e-06
57057,456086,456086,912172,490.3051257133484,3.0182824288827885e-06
57157,456886,456886,913772,490.9790768623352,3.0160552594641874e-06
57257,457686,457686,915372,491.6585199832916,3.013883189110839e-06
57357,458486,458486,916972,492.34930396080017,3.0117640211152345e-06
57457,459286,459286,918572,493.0219178199768,3.009695662729058e-06
57558,460094,460094,920188,493.7238540649414,3.0076561639078337e-06
57658,460894,460894,921788,494.40843892097473,3.005683993832743e-06
57758,461694,461694,923388,495.09333395957947,3.003756906387314e-06
57858,462494,462494,924988,495.76148676872253,3.0018731726158045e-06
57958,463294,463294,926588,496.4451148509979,3.00003114289077e-06
58058,464094,464094,928188,497.11572885513306,2.998229242748675e-06
58158,464894,464894,929788,497.7797968387604,2.996465968691238e-06
58258,465694,465694,931388,498.47498178482056,2.994739885189447e-06
58358,466494,466494,932988,499.1389207839966,2.993049620767382e-06
58458,467294,467294,934588,499.80557894706726,2.991393865316744e-06
58559,468102,468102,936204,500.5006399154663,2.9897553051065526e-06
58659,468902,468902,937804,501.1678977012634,2.988165179810929e-06
58759,469702,469702,939404,501.8319869041443,2.986605957584267e-06
58859,470502,470502,941004,502.5187876224518,2.985076543775712e-06
58959,471302,471302,942604,503.186648607254,2.9835758910367955e-06
59059,472102,472102,944204,503.85169887542725,2.9821029971465337e-06
59159,472902,472902,945804,504.54421281814575,2.980656902952329e-06
59259,473702,473702,947404,505.21136569976807,2.979236689973586e-06
59359,474502,474502,949004,505.8802638053894,2.9778414785071957e-06
59459,475302,475302,950604,506.56580877304077,2.9764704259930004e-06
59560,476110,476110,952220,507.31065583229065,2.9751093633191848e-06
59660,476910,476910,953820,507.99156403541565,2.9737844625574785e-06
59760,477710,477710,955420,508.67243480682373,2.9724813908355116e-06
59860,478510,478510,957020,509.339017868042,2.9711994373042187e-06
59960,479310,479310,958620,510.02536964416504,2.969937920523273e-06
60060,480110,480110,960220,510.7052619457245,2.9686961863873088e-06
60160,480910,480910,961820,511.3688817024231,2.9674736075422786e-06
60260,481710,481710,963420,512.0385589599609,2.9662695821089224e-06
60360,482510,482510,965020,512.7590148448944,2.965083531695628e-06
60460,483310,483310,966620,513.4714798927307,2.9639149017198834e-06
60561,484118,484118,968236,514.2134399414062,2.962751725059652e-06
60661,484918,484918,969836,514.9803018569946,2.9616165189122123e-06
60761,485718,485718,971436,515.7646749019623,2.96049719136962e-06
60861,486518,486518,973036,516.5173900127411,2.9593932700832103e-06
60961,487318,487318,974636,517.3245558738708,2.958304300782077e-06
61061,488118,488118,976236,518.0714728832245,2.957229846753192e-06
61161,488918,488918,977836,518.810311794281,2.956169487886017e-06
61261,489718,489718,979436,519.5679898262024,2.9551228206443893e-06
61361,490518,490518,981036,520.2526657581329,2.9540894559243118e-06
61461,491318,491318,982636,520.9511768817902,2.953069020197556e-06
61562,492126,492126,984252,521.6486468315125,2.952051136827488e-06
61662,492926,492926,985852,522.4032158851624,2.9510556125353734e-06
61762,493726,493726,987452,523.1403987407684,2.95007197362184e-06
61862,494526,494526,989052,523.8690679073334,2.9490998986244802e-06
61962,495326,495326,990652,524.6602597236633,2.9481390780948523e-06
62062,496126,496126,992252,525.516964673996,2.947189213597877e-06
62162,496926,496926,993852,526.2331328392029,2.946250017843603e-06
62262,497726,497726,995452,526.9244518280029,2.945321213603686e-06
62362,498526,498526,997052,527.6266407966614,2.944402533601126e-06
62462,499326,499326,998652,528.3122689723969,2.9434937200268073e-06
62563,500134,500134,1000268,529.0055060386658,2.942585580497354e-06
62663,500934,500934,1001868,529.697723865509,2.9416958555402648e-06
62763,501734,501734,1003468,530.3712570667267,2.9408152748852574e-06
62863,502534,502534,1005068,531.046238899231,2.9399436150952077e-06
62963,503334,503334,1006668,531.7250118255615,2.9390806602068955e-06
63063,504134,504134,1008268,532.4059519767761,2.938226202123167e-06
63163,504934,504934,1009868,533.0853607654572,2.9373800398117144e-06
63263,505734,505734,1011468,533.7651238441467,2.9365419784550657e-06
63363,506534,506534,1013068,534.4495129585266,2.9357118303654914e-06
63463,507334,507334,1014668,535.1362369060516,2.934889413792746e-06
63564,508142,508142,1016284,535.8077807426453,2.934066442312875e-06
63664,508942,508942,1017884,536.5007197856903,2.9332590410282095e-06
63764,509742,509742,1019484,537.1723036766052,2.9324588599722797e-06
63864,510542,510542,1021084,537.8418936729431,2.9316657405452123e-06
63964,511342,511342,1022684,538.5348908901215,2.9308795289117798e-06
64064,512142,512142,1024284,539.2033967971802,2.9301000762843337e-06
64164,512942,512942,1025884,539.8869078159332,2.929327238592095e-06
64264,513742,513742,1027484,540.6350839138031,2.928560876409481e-06
64364,514542,514542,1029084,541.3351306915283,2.927800854649138e-06
64464,515342,515342,1030684,542.0370597839355,2.9270470422338568e-06
64565,516150,516150,1032300,542.7601778507233,2.9262918656652888e-06
64665,516950,516950,1033900,543.4439578056335,2.92555015492639e-06
64765,517750,517750,1035500,544.1430988311768,2.9248142836554267e-06
64865,518550,518550,1037100,544.9131319522858,2.924084136143028e-06
64965,519350,519350,1038700,545.6813716888428,2.9233596006910872e-06
65065,520150,520150,1040300,546.3615937232971,2.9226405685864254e-06
65165,520950,520950,1041900,547.2141468524933,2.9219269343045795e-06
65265,521750,521750,1043500,548.0584697723389,2.9212185952195724e-06
65365,522550,522550,1045100,548.9060096740723,2.9205154524925916e-06
65465,523350,523350,1046700,549.6302709579468,2.919817409361015e-06
65566,524158,524158,1048316,550.4923257827759,2.9191174669293076e-06
65666,524958,524958,1049916,551.2982437610626,2.918429393469752e-06
65766,525758,525758,1051516,552.0069680213928,2.91774614568516e-06
65866,526558,526558,1053116,552.6878399848938,2.9170676378018503e-06
65966,527358,527358,1054716,553.4771230220795,2.9163937860604526e-06
66066,528158,528158,1056316,554.4352607727051,2.9157245093946404e-06
66166,528958,528958,1057916,555.1487908363342,2.9150597288120766e-06
66266,529758,529758,1059516,555.8469569683075,2.914399367587968e-06
66366,530558,530558,1061116,556.5233888626099,2.913743350928279e-06
66466,531358,531358,1062716,557.2139177322388,2.913091606074145e-06
66567,532166,532166,1064332,557.9248998165131,2.9124376076917646e-06
66667,532966,532966,1065932,558.6539378166199,2.9117942369550335e-06
66767,533766,533766,1067532,559.3536858558655,2.9111549304722505e-06
66867,534566,534566,1069132,560.1714890003204,2.9105196229565096e-06
66967,535366,535366,1070732,561.0698747634888,2.9098882507583323e-06
67067,536166,536166,1072332,561.7897357940674,2.9092607517101413e-06
67167,536966,536966,1073932,562.6272509098053,2.9086370653503617e-06
67267,537766,537766,1075532,563.5146877765656,2.908017132708817e-06
67367,538566,538566,1077132,564.199296951294,2.9074008964337946e-06
67467,539366,539366,1078732,564.9133598804474,2.9067883002566414e-06
67568,540174,540174,1080348,565.7529017925262,2.906173217266398e-06
67668,540974,540974,1081948,566.6313889026642,2.90556777355081e-06
67768,541774,541774,1083548,567.3412709236145,2.9049658093251557e-06
67868,542574,542574,1085148,568.1627378463745,2.9043672734759396e-06
67968,543374,543374,1086748,568.8508908748627,2.9037721166996506e-06
68068,544174,544174,1088348,569.7204208374023,2.9031802901989522e-06
68168,544974,544974,1089948,570.5598359107971,2.9025917468035987e-06
68268,545774,545774,1091548,571.478414773941,2.902006439960015e-06
68368,546574,546574,1093148,572.2174227237701,2.9014243247184597e-06
68468,547374,547374,1094748,572.9942028522491,2.900845356684095e-06
68569,548182,548182,1096364,573.7513718605042,2.9002637495677396e-06
68669,548982,548982,1097964,574.4517149925232,2.8996909776024024e-06
68769,549782,549782,1099564,575.2334866523743,2.8991212258834847e-06
68869,550582,550582,1101164,575.9715728759766,2.8985544534478898e-06
68969,551382,551382,1102764,576.7608449459076,2.897990621001346e-06
69069,552182,552182,1104364,577.4762270450592,2.8974296899253598e-06
69169,552982,552982,1105964,578.4549028873444,2.89687162215954e-06
69269,553782,553782,1107564,579.2529747486115,2.896316380457682e-06
69369,554582,554582,1109164,579.997181892395,2.895763928836362e-06
69469,555382,555382,1110764,580.7337188720703,2.89521423124002e-06
69570,556190,556190,1112380,581.5034277439117,2.8946617969840946e-06
69670,556990,556990,1113980,582.218181848526,2.8941175307301477e-06
69770,557790,557790,1115580,582.9819986820221,2.89357591587038e-06
69870,558590,558590,1117180,583.7158398628235,2.8930369194781428e-06
69970,559390,559390,1118780,584.490984916687,2.8925005095248943e-06
70070,560190,560190,1120380,585.2173597812653,2.8919666544727722e-06
70170,560990,560990,1121980,585.9113199710846,2.891435323148363e-06
70270,561790,561790,1123580,586.8215680122375,2.890906485282822e-06
70370,562590,562590,1125180,587.5543489456177,2.8903801111814377e-06
70470,563390,563390,1126780,588.2777190208435,2.889856171578342e-06
70571,564198,564198,1128396,588.9853386878967,2.889329434441934e-06
70671,564998,564998,1129996,589.6625978946686,2.8888103018158572e-06
70771,565798,565798,1131596,590.3398289680481,2.8882935188326295e-06
70871,566598,566598,1133196,591.0995230674744,2.887779058558327e-06
70971,567398,567398,1134796,591.8450269699097,2.8872668939943078e-06
71071,568198,568198,1136396,592.60537981987,2.8867569992831195e-06
71171,568998,568998,1137996,593.4254767894745,2.886249348357193e-06
71271,569798,569798,1139596,594.2983357906342,2.8857439159902005e-06
71371,570598,570598,1141196,595.2593579292297,2.8852406776476782e-06
71471,571398,571398,1142796,596.1781418323517,2.8847396085589496e-06
71572,572206,572206,1144412,596.9398949146271,2.884235706267738e-06
71672,573006,573006,1146012,597.6548488140106,2.883738925441429e-06
71772,573806,573806,1147612,598.3639197349548,2.8832442428053864e-06
71872,574606,574606,1149212,599.0947878360748,2.8827516355318564e-06
71972,575406,575406,1150812,599.853385925293,2.8822610811801873e-06
72072,576206,576206,1152412,600.6041898727417,2.88177255780339e-06
72172,577006,577006,1154012,601.3446877002716,2.881286043493232e-06
72272,577806,577806,1155612,602.2446010112762,2.8808015168742723e-06
72372,578606,578606,1157212,603.0779666900635,2.8803189568551275e-06
72472,579406,579406,1158812,603.881020784378,2.879838342624194e-06
72573,580214,580214,1160428,604.6405317783356,2.8793548766974055e-06
72673,581014,581014,1162028,605.3827557563782,2.8788781123840116e-06
72773,581814,581814,1163628,606.222339630127,2.8784032332004224e-06
72873,582614,582614,1165228,606.9742619991302,2.8779302200295254e-06
72973,583414,583414,1166828,607.7180557250977,2.877459053312639e-06
73073,584214,584214,1168428,608.4433326721191,2.876989714421222e-06
73173,585014,585014,1170028,609.1324830055237,2.8765221844264746e-06
73273,585814,585814,1171628,609.8438897132874,2.8760564452214853e-06
73373,586614,586614,1173228,610.6410918235779,2.8755924783199295e-06
73473,587414,587414,1174828,611.4380300045013,2.875130266299295e-06
73574,588222,588222,1176444,612.1531980037689,2.874665195384081e-06
73674,589022,589022,1178044,612.8449399471283,2.8742064571913053e-06
73774,589822,589822,1179644,613.557461977005,2.8737494215904376e-06
73874,590622,590622,1181244,614.2450108528137,2.8732940715233087e-06
73974,591422,591422,1182844,615.0319197177887,2.8728403903480505e-06
74074,592222,592222,1184444,615.7361488342285,2.8723883618085965e-06
74174,593022,593022,1186044,616.5306589603424,2.8719379694967657e-06
74274,593822,593822,1187644,617.5640408992767,2.8714891975613406e-06
74374,594622,594622,1189244,618.7295069694519,2.8710420303725093e-06
74474,595422,595422,1190844,619.6775989532471,2.8705964519866795e-06
74575,596230,596230,1192460,620.4913237094879,2.8701480154403196e-06
74675,597030,597030,1194060,621.2748956680298,2.8697055851213536e-06
74775,597830,597830,1195660,622.0670049190521,2.8692646981434317e-06
74875,598630,598630,1197260,622.8427209854126,2.868825340046429e-06
74975,599430,599430,1198860,623.6071479320526,2.8683874959933058e-06
75075,600230,600230,1200460,624.3430438041687,2.867951151838202e-06
75175,601030,601030,1202060,625.1543617248535,2.8675162932444827e-06
75275,601830,601830,1203660,625.9554669857025,2.867082906236852e-06
75375,602630,602630,1205260,626.6909687519073,2.866650977014385e-06
75475,603430,603430,1206860,627.4162917137146,2.8662204918888074e-06
75576,604238,604238,1208476,628.1211929321289,2.865787153793261e-06
75676,605038,605038,1210076,628.8096780776978,2.865359530628952e-06
75776,605838,605838,1211676,629.5241379737854,2.8649333112457506e-06
75876,606638,606638,1213276,630.2510018348694,2.8645084827177676e-06
75976,607438,607438,1214876,630.9990079402924,2.864085032424788e-06
76076,608238,608238,1216476,631.8362927436829,2.863662947290726e-06
76176,609038,609038,1218076,632.6128067970276,2.8632422149361798e-06
76276,609838,609838,1219676,633.4355597496033,2.862822823182281e-06
76376,610638,610638,1221276,634.2152497768402,2.86240475939841e-06
76476,611438,611438,1222876,634.9518840312958,2.861988011517387e-06
76577,612246,612246,1224492,635.7265667915344,2.8615684199980443e-06
76677,613046,613046,1226092,636.5504078865051,2.8611542812141984e-06
76777,613846,613846,1227692,637.5144996643066,2.8607414229509894e-06
76877,614646,614646,1229292,638.3691809177399,2.8603298333983283e-06
76977,615446,615446,1230892,639.1147499084473,2.859919501170031e-06
77077,616246,616246,1232492,639.8638348579407,2.859510414876835e-06
77177,617046,617046,1234092,640.5867550373077,2.859102563674912e-06
77277,617846,617846,1235692,641.3439748287201,2.8586959362073663e-06
77377,618646,618646,1237292,642.0746438503265,2.858290521499398e-06
77477,619446,619446,1238892,642.8280267715454,2.857886308848064e-06
77578,620254,620254,1240508,643.6258747577667,2.8574792633967367e-06
77678,621054,621054,1242108,644.3396427631378,2.857077434611679e-06
77778,621854,621854,1243708,645.0668389797211,2.8566767760787513e-06
77878,622654,622654,1245308,645.7955567836761,2.8562772774391283e-06
77978,623454,623454,1246908,646.5009078979492,2.855878928424108e-06
78078,624254,624254,1248508,647.267648935318,2.855481718828137e-06
78178,625054,625054,1250108,648.0180258750916,2.8550856388486374e-06
78278,625854,625854,1251708,648.9096350669861,2.854690678352222e-06
78378,626654,626654,1253308,649.6533010005951,2.854296827619749e-06
78478,627454,627454,1254908,650.4377799034119,2.853904076888813e-06
78579,628262,628262,1256524,651.1730690002441,2.8535085054752085e-06
78679,629062,629062,1258124,651.9188787937164,2.8531179369388997e-06
78779,629862,629862,1259724,652.6656997203827,2.8527284399116782e-06
78879,630662,630662,1261324,653.4400587081909,2.8523400050405004e-06
78979,631462,631462,1262924,654.165168762207,2.8519526230481265e-06
79079,632262,632262,1264524,654.9542577266693,2.851566284954542e-06
79179,633062,633062,1266124,655.6902267932892,2.8511809816865446e-06
79279,633862,633862,1267724,656.4171948432922,2.8507967042330423e-06
79379,634662,634662,1269324,657.1575307846069,2.850413443895712e-06
79479,635462,635462,1270924,657.9115138053894,2.850031191863992e-06
79580,636270,636270,1272540,658.7540168762207,2.849646131973673e-06
79680,637070,637070,1274140,659.4741020202637,2.8492658805666505e-06
79780,637870,637870,1275740,660.1773548126221,2.8488866117992126e-06
79880,638670,638670,1277340,660.9110310077667,2.84850831701559e-06
79980,639470,639470,1278940,661.6395697593689,2.8481309880313585e-06
80080,640270,640270,1280540,662.3733539581299,2.8477546167321712e-06
80180,641070,641070,1282140,663.1838278770447,2.84737919494369e-06
80280,641870,641870,1283740,663.9272239208221,2.8470047142951295e-06
80380,642670,642670,1285340,664.650224685669,2.8466311672393983e-06
80480,643470,643470,1286940,665.3621068000793,2.846258545607762e-06
80581,644278,644278,1288556,666.0661797523499,2.8458831291162136e-06
80681,645078,645078,1290156,666.8592779636383,2.845512344127753e-06
80781,645878,645878,1291756,667.5980107784271,2.8451424611563655e-06
80881,646678,646678,1293356,668.2852838039398,2.8447734727909193e-06
80981,647478,647478,1294956,669.0046818256378,2.844405371390117e-06
81081,648278,648278,1296556,669.6934509277344,2.84403814948359e-06
81181,649078,649078,1298156,670.4012138843536,2.8436717998762537e-06
81281,649878,649878,1299756,671.137776851654,2.843306314962009e-06
81381,650678,650678,1301356,671.8618927001953,2.842941687812606e-06
81481,651478,651478,1302956,672.5801410675049,2.842577911025031e-06
81582,652286,652286,1304572,673.3494489192963,2.8422113524603126e-06
81682,653086,653086,1306172,674.0840308666229,2.8418492636808655e-06
81782,653886,653886,1307772,674.7926859855652,2.8414880039348673e-06
81882,654686,654686,1309372,675.5370209217072,2.8411275667399744e-06
81982,655486,655486,1310972,676.2552587985992,2.840767945013052e-06
82082,656286,656286,1312572,676.9734647274017,2.8404091319954134e-06
82182,657086,657086,1314172,677.7308838367462,2.8400511209472664e-06
82282,657882,657882,1315764,678.4827938079834,2.6696365363294956e-06
82382,658682,658682,1317364,679.2169289588928,2.5053501642031878e-06
82482,659482,659482,1318964,679.9618747234344,2.502927881588802e-06
82583,660290,660290,1320580,680.6927769184113,2.501557135865115e-06
82683,661090,661090,1322180,681.4285619258881,2.500449358946527e-06
82783,661890,661890,1323780,682.1464729309082,2.4994471985923827e-06
82883,662690,662690,1325380,682.8791396617889,2.4985050556157355e-06
82983,663490,663490,1326980,683.5722508430481,2.4976037579784827e-06
83083,664290,664290,1328580,684.3574566841125,2.496733766361495e-06
83183,665090,665090,1330180,685.1130838394165,2.4958897111035144e-06
83283,665890,665890,1331780,685.8449966907501,2.4950682642161413e-06
83383,666690,666690,1333380,686.5869796276093,2.494267194377935e-06
83483,667490,667490,1334980,687.6244609355927,2.4934849004726865e-06
83584,668298,668298,1336596,688.4793207645416,2.4927126028031258e-06
83684,669098,669098,1338196,689.2053937911987,2.491964614230565e-06
83784,669898,669898,1339796,690.1056838035583,2.49123239189559e-06
83884,670698,670698,1341396,690.9097199440002,2.490515237158229e-06
83984,671498,671498,1342996,691.6665599346161,2.4898125308593876e-06
84084,672298,672298,1344596,692.6850717067719,2.4891237127763426e-06
84184,673098,673098,1346196,693.6342687606812,2.4884482682441877e-06
84284,673898,673898,1347796,694.3967819213867,2.487785719215878e-06
84384,674698,674698,1349396,695.2548108100891,2.487135616452342e-06
84484,675498,675498,1350996,696.0147678852081,2.486497536644431e-06
84585,676306,676306,1352612,696.7610607147217,2.4858648702828104e-06
84685,677106,677106,1354212,697.7124118804932,2.485249759460896e-06
84785,677906,677906,1355812,698.7723438739777,2.4846455168004023e-06
84885,678706,678706,1357412,699.8133509159088,2.484051792003605e-06
84985,679506,679506,1359012,700.824052810669,2.48346824883876e-06
85085,680306,680306,1360612,701.5957727432251,2.4828945645140907e-06
85185,681106,681106,1362212,702.402126789093,2.4823304282461234e-06
85285,681906,681906,1363812,703.1939718723297,2.4817755410413613e-06
85385,682706,682706,1365412,703.9404196739197,2.481229614628232e-06
85485,683506,683506,1367012,704.9779489040375,2.4806923713410694e-06
85586,684314,684314,1368628,706.0195198059082,2.4801582960285153e-06
85686,685114,685114,1370228,706.8577568531036,2.4796377037050406e-06
85786,685914,685914,1371828,707.6713428497314,2.4791250153054506e-06
85886,686714,686714,1373428,708.4431507587433,2.478619989729279e-06
85986,687514,687514,1375028,709.3725697994232,2.4781223934338455e-06
86086,688314,688314,1376628,710.4430248737335,2.477632001610339e-06
86186,689114,689114,1378228,711.4967248439789,2.477148596284174e-06
86286,689914,689914,1379828,712.4419617652893,2.476671967280305e-06
86386,690714,690714,1381428,713.4205968379974,2.476201910971237e-06
86486,691514,691514,1383028,714.2103910446167,2.4757382305087198e-06
86587,692322,692322,1384644,714.9909288883209,2.4752761911365823e-06
86687,693122,693122,1386244,715.748851776123,2.4748247564322964e-06
86787,693922,693922,1387844,716.5121939182281,2.4743791430714254e-06
86887,694722,694722,1389444,717.2908279895782,2.4739391787733442e-06
86987,695522,695522,1391044,718.074914932251,2.4735046964764097e-06
87087,696322,696322,1392644,718.7930917739868,2.47307553489816e-06
87187,697122,697122,1394244,719.5193059444427,2.472651537676676e-06
87287,697922,697922,1395844,720.3069477081299,2.4722325537229206e-06
87387,698722,698722,1397444,721.1342678070068,2.4718184361451795e-06
87487,699522,699522,1399044,721.8933317661285,2.471409043791398e-06
87588,700330,700330,1400660,722.611958026886,2.471000213556827e-06
87688,701130,701130,1402260,723.5188558101654,2.470599907176825e-06
87788,701930,701930,1403860,724.4162828922272,2.470203925344366e-06
87888,702730,702730,1405460,725.2061839103699,2.4698121435975124e-06
87988,703530,703530,1407060,725.8963928222656,2.469424441190212e-06
88088,704330,704330,1408660,726.6152029037476,2.4690407009374874e-06
88188,705130,705130,1410260,727.3274717330933,2.468660809705565e-06
88288,705930,705930,1411860,728.0054528713226,2.4682846579052773e-06
88388,706730,706730,1413460,728.8870198726654,2.4679121390404405e-06
88488,707530,707530,1415060,729.6742236614227,2.467543150124458e-06
88589,708338,708338,1416676,730.4026718139648,2.467173952767229e-06
88689,709138,709138,1418276,731.1116578578949,2.4668117604321792e-06
88789,709938,709938,1419876,731.8385148048401,2.466452806890863e-06
88889,710738,710738,1421476,732.6477317810059,2.466097001230313e-06
88989,711538,711538,1423076,733.3781669139862,2.4657442558258326e-06
89089,712338,712338,1424676,734.1011147499084,2.465394484886586e-06
89189,713138,713138,1426276,734.8975958824158,2.465047606149379e-06
89289,713938,713938,1427876,735.66539478302,2.4647035391703118e-06
89389,714738,714738,1429476,736.369295835495,2.4643622064436e-06
89489,715538,715538,1431076,737.1060059070587,2.4640235325302645e-06
89590,716346,716346,1432692,737.9119186401367,2.463684096484332e-06
89690,717146,717146,1434292,738.6838607788086,2.463350548206746e-06
89790,717946,717946,1435892,739.4467778205872,2.463019445653458e-06
89890,718746,718746,1437492,740.2506139278412,2.462690722080573e-06
89990,719546,719546,1439092,741.0319259166718,2.4623643130765014e-06
90090,720346,720346,1440692,741.809506893158,2.4620401561332373e-06
90190,721146,721146,1442292,742.6863470077515,2.4617181903205653e-06
90290,721946,721946,1443892,743.4035408496857,2.461398356740772e-06
90390,722746,722746,1445492,744.0939557552338,2.4610805981589044e-06
90490,723546,723546,1447092,745.0860779285431,2.4607648594095344e-06
90591,724354,724354,1448708,745.905957698822,2.4604479585540247e-06
90691,725154,725154,1450308,746.78364777565,2.460136118403859e-06
90791,725954,725954,1451908,747.6555099487305,2.4598261407808925e-06
90891,726754,726754,1453508,748.6399397850037,2.4595179766256964e-06
90991,727554,727554,1455108,749.4466338157654,2.4592115783775153e-06
91091,728354,728354,1456708,750.2854399681091,2.4589068996365686e-06
91191,729154,729154,1458308,751.0973470211029,2.4586038956606212e-06
91291,729954,729954,1459908,751.9377210140228,2.458302522705414e-06
91391,730754,730754,1461508,752.7262089252472,2.458002738703992e-06
91491,731554,731554,1463108,753.6606860160828,2.4577045024928565e-06
91592,732362,732362,1464724,754.6925098896027,2.4574048143427572e-06
91692,733162,733162,1466324,755.5247218608856,2.457109569741691e-06
91792,733962,733962,1467924,756.5274789333344,2.4568157564811167e-06
91892,734762,734762,1469524,757.3046677112579,2.456523338006819e-06
91992,735562,735562,1471124,758.1284987926483,2.4562322789324794e-06
92092,736362,736362,1472724,758.9097399711609,2.4559425449602976e-06
92192,737162,737162,1474324,759.6886878013611,2.4556541025568143e-06
92292,737962,737962,1475924,760.4833068847656,2.455366919545123e-06
92392,738762,738762,1477524,761.2223479747772,2.455080964270256e-06
92492,739562,739562,1479124,761.9700808525085,2.4547962058597536e-06
92593,740370,740370,1480740,762.7620317935944,2.4545097849848536e-06
92693,741170,741170,1482340,763.587201833725,2.4542273439816544e-06
92793,741970,741970,1483940,764.3615946769714,2.453946013169236e-06
92893,742770,742770,1485540,765.1277680397034,2.4536657653843456e-06
92993,743570,743570,1487140,765.8657939434052,2.453386573969768e-06
93093,744370,744370,1488740,766.7436809539795,2.453108413306136e-06
93193,745170,745170,1490340,767.7725818157196,2.452831258535445e-06
93293,745970,745970,1491940,768.5303149223328,2.452555085201648e-06
93393,746770,746770,1493540,769.2617106437683,2.4522798696370975e-06
93493,747570,747570,1495140,770.2267980575562,2.4520055889639992e-06
93594,748378,748378,1496756,771.0958209037781,2.45172949182061e-06
93694,749178,749178,1498356,771.9127616882324,2.451457023515838e-06
93794,749978,749978,1499956,772.7075986862183,2.4511854247672446e-06
93894,750778,750778,1501556,773.5196838378906,2.4509146751418336e-06
93994,751578,751578,1503156,774.4879946708679,2.4506447547974703e-06
94094,752378,752378,1504756,775.3301119804382,2.4503756441579967e-06
94194,753178,753178,1506356,776.2807078361511,2.450107324587916e-06
94294,753978,753978,1507956,777.1377589702606,2.449839777469841e-06
94394,754778,754778,1509556,777.9457619190216,2.4495729853290045e-06
94494,755578,755578,1511156,778.71013879776,2.4493069307876995e-06
94595,756386,756386,1512772,779.520260810852,2.449038946880224e-06
94695,757186,757186,1514372,780.4009499549866,2.4487743240427474e-06
94795,757986,757986,1515972,781.2757349014282,2.4485103892798324e-06
94895,758786,758786,1517572,782.1712996959686,2.448247127130375e-06
94995,759586,759586,1519172,782.9732048511505,2.4479845224712253e-06
95095,760386,760386,1520772,783.7086117267609,2.4477225605570355e-06
95195,761186,761186,1522372,784.4869067668915,2.4474612271806865e-06
95295,761986,761986,1523972,785.2645797729492,2.4472005084152543e-06
95395,762786,762786,1525572,786.0413780212402,2.446940390737576e-06
95495,763586,763586,1527172,786.7428269386292,2.4466808608699895e-06
95596,764394,764394,1528788,787.5186049938202,2.446419319462807e-06
95696,765194,765194,1530388,788.2580318450928,2.4461609327631493e-06
95796,765994,765994,1531988,788.9765598773956,2.4459030962686958e-06
95896,766794,766794,1533588,789.7217628955841,2.44564579827973e-06
95996,767594,767594,1535188,790.4604148864746,2.4453890271895707e-06
96096,768394,768394,1536788,791.2090878486633,2.445132771731149e-06
96196,769194,769194,1538388,792.0081059932709,2.44487702115304e-06
96296,769990,769990,1539980,792.769437789917,2.1807758698646533e-06
96396,770790,770790,1541580,793.5521547794342,2.172208876737374e-06
96496,771590,771590,1543180,794.3026437759399,2.1697395186380027e-06
96597,772398,772398,1544796,795.0778028964996,2.167904543934975e-06
96697,773198,773198,1546396,795.8579399585724,2.1663250974519596e-06
96797,773998,773998,1547996,796.5591788291931,2.1648670450341448e-06
96897,774798,774798,1549596,797.2388818264008,2.1634878708964602e-06
96997,775598,775598,1551196,797.9767308235168,2.1621682547995077e-06
97097,776398,776398,1552796,798.7308719158173,2.1608977925509792e-06
97197,777198,777198,1554396,799.5073268413544,2.1596700633130174e-06
97297,777998,777998,1555996,800.2979938983917,2.1584806801938324e-06
97397,778798,778798,1557596,801.0999050140381,2.1573264154086306e-06
97497,779598,779598,1559196,801.8526027202606,2.156204759271425e-06
97598,780406,780406,1560812,802.615327835083,2.1551029115697347e-06
97698,781206,781206,1562412,803.3625347614288,2.15404096664431e-06
97798,782006,782006,1564012,804.1248488426208,2.1530063894022536e-06
97898,782806,782806,1565612,804.848494052887,2.1519978771108077e-06
97998,783606,783606,1567212,805.5328989028931,2.1510142583410236e-06
98098,784406,784406,1568812,806.2726047039032,2.1500544656582067e-06
98198,785206,785206,1570412,807.048773765564,2.1491175150663405e-06
98298,786006,786006,1572012,807.765213727951,2.1482024916979503e-06
98398,786806,786806,1573612,808.5166010856628,2.147308538934553e-06
98498,787606,787606,1575212,809.2770717144012,2.146434850245368e-06
98599,788414,788414,1576828,810.0141470432281,2.1455722175132488e-06
98699,789214,789214,1578428,810.7475838661194,2.1447369935990473e-06
98799,790014,790014,1580028,811.4443566799164,2.143919853689865e-06
98899,790814,790814,1581628,812.185546875,2.1431201423103506e-06
98999,791614,791614,1583228,812.863452911377,2.1423372338419767e-06
99099,792414,792414,1584828,813.5719900131226,2.1415705299991436e-06
99199,793214,793214,1586428,814.3212189674377,2.1408194578780535e-06
99299,794014,794014,1588028,815.086639881134,2.1400834685005416e-06
99399,794814,794814,1589628,815.8800737857819,2.139362035979933e-06
99499,795614,795614,1591228,816.6726830005646,2.1386546551080843e-06
99600,796422,796422,1592844,817.3951368331909,2.1379539699894763e-06
99700,797222,797222,1594444,818.0839989185333,2.1372733860115384e-06
99800,798022,798022,1596044,818.846364736557,2.136605451859056e-06
99900,798822,798822,1597644,819.6157579421997,2.1359497372988015e-06
100000,799622,799622,1599244,820.2989549636841,2.1353058295195124e-06


==> plot_data/bilinear_matrix_game_n500/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.004578828811645508,2.018959020339561
69,162,162,324,0.5456399917602539,0.059786073230173785
138,362,362,724,1.0914397239685059,0.01507175353552151
207,606,606,1212,1.6178748607635498,0.006802968350301351
276,854,854,1708,2.2067418098449707,0.003444646449262009
345,1124,1124,2248,2.8194258213043213,0.0028073235526150354
413,1390,1390,2780,3.3963279724121094,0.0021475962551178577
482,1656,1656,3312,4.299939870834351,0.0015811463673860975
551,1928,1928,3856,4.858036994934082,0.0013172553409269178
620,2198,2198,4396,5.475833892822266,0.0010024683676113034
689,2474,2474,4948,5.9514429569244385,0.0008031365805358339
758,2750,2750,5500,6.4927427768707275,0.0006681776194095929
827,3020,3020,6040,7.0113348960876465,0.0005085639104525426
896,3290,3290,6580,7.496543884277344,0.0004035657261022955
965,3566,3566,7132,7.974887847900391,0.0003585004704135169
1034,3842,3842,7684,8.452881813049316,0.0003329619936725249
1102,4114,4114,8228,8.92270278930664,0.0002713694035712921
1171,4390,4390,8780,9.42782974243164,0.00023184231104492845
1240,4666,4666,9332,9.914666891098022,0.00020626155997945992
1309,4942,4942,9884,10.395846843719482,0.00018590285321652873
1378,5218,5218,10436,10.879998922348022,0.00015901636808948527
1447,5486,5486,10972,11.363213777542114,0.00011797622395897509
1516,5762,5762,11524,11.851638793945312,0.00010116404468617912
1585,6038,6038,12076,12.335442781448364,8.929153885947352e-05
1654,6314,6314,12628,12.823810815811157,7.338889446726718e-05
1723,6590,6590,13180,13.300436019897461,6.50943815530093e-05
1792,6866,6866,13732,13.78229570388794,5.961726407905162e-05
1860,7138,7138,14276,14.247904777526855,5.676209587709056e-05
1929,7414,7414,14828,14.719422817230225,5.449163988795128e-05
1998,7690,7690,15380,15.192276000976562,5.170103272576408e-05
2067,7966,7966,15932,15.675442934036255,5.064870630975057e-05
2136,8242,8242,16484,16.14820885658264,4.988391862133933e-05
2205,8518,8518,17036,16.619136810302734,4.94680950431296e-05
2274,8794,8794,17588,17.19023060798645,4.907274356430394e-05
2343,9070,9070,18140,17.76914691925049,4.862028825735144e-05
2412,9346,9346,18692,18.38659381866455,4.836182259874062e-05
2481,9622,9622,19244,18.967670679092407,4.7838961380909206e-05
2549,9894,9894,19788,19.519465923309326,4.740810021484917e-05
2618,10170,10170,20340,20.10663676261902,4.708209595837559e-05
2687,10446,10446,20892,20.62573480606079,4.685625831742085e-05
2756,10722,10722,21444,21.330275774002075,4.643259057843834e-05
2825,10998,10998,21996,21.90008783340454,4.5912453744244845e-05
2894,11274,11274,22548,22.42951464653015,4.5151777475619436e-05
2963,11550,11550,23100,23.01525092124939,4.478454227214779e-05
3032,11826,11826,23652,23.63002872467041,4.448468329324223e-05
3101,12124,12124,24248,24.13505268096924,3.620353059135834e-05
3170,12400,12400,24800,24.663233757019043,3.251915887215331e-05
3238,12672,12672,25344,25.13606572151184,2.8239348201756584e-05
3307,12948,12948,25896,25.6695077419281,2.4409104790933668e-05
3376,13224,13224,26448,26.472150802612305,2.068078503720382e-05
3445,13500,13500,27000,27.128644704818726,1.7031458943989376e-05
3514,13776,13776,27552,28.02178692817688,1.4639992711182283e-05
3583,14052,14052,28104,28.580612897872925,1.3744720038568658e-05
3652,14328,14328,28656,29.467164754867554,1.2894622738995196e-05
3721,14604,14604,29208,30.031800746917725,1.1391260677440633e-05
3790,14880,14880,29760,30.71770668029785,1.0840637113303256e-05
3859,15156,15156,30312,31.465824604034424,9.567314571383638e-06
3928,15432,15432,30864,31.965258598327637,8.440378370343375e-06
3996,15704,15704,31408,32.45776581764221,8.00883928781533e-06
4065,15980,15980,31960,33.03022789955139,7.603169096266994e-06
4134,16256,16256,32512,33.67987680435181,7.249099309669078e-06
4203,16532,16532,33064,34.65804171562195,6.98605537064377e-06
4272,16808,16808,33616,35.156808853149414,6.813677447981931e-06
4341,17084,17084,34168,35.82108783721924,6.633958009424428e-06
4410,17360,17360,34720,36.315247774124146,6.511536951408726e-06
4479,17636,17636,35272,36.995630741119385,6.4024524244725075e-06
4548,17912,17912,35824,37.63811683654785,6.2423795468798714e-06
4617,18188,18188,36376,38.18744874000549,5.97454015020185e-06
4685,18460,18460,36920,38.662723779678345,5.776198361899567e-06
4754,18736,18736,37472,39.1594660282135,5.7066415871047025e-06
4823,19012,19012,38024,39.63657283782959,5.662363600606621e-06
4892,19288,19288,38576,40.118484020233154,5.608157874705812e-06
4961,19564,19564,39128,40.78804874420166,5.586862087440221e-06
5030,19840,19840,39680,41.674314737319946,5.555281483380804e-06
5099,20116,20116,40232,42.369223833084106,5.513130160111171e-06
5168,20392,20392,40784,42.86113882064819,5.492686441001222e-06
5237,20668,20668,41336,43.36520981788635,5.475088713179951e-06
5306,20944,20944,41888,44.03134799003601,5.46705334450441e-06
5375,21220,21220,42440,44.65252470970154,5.460848121567388e-06
5443,21492,21492,42984,45.22128367424011,5.453818894016797e-06
5512,21768,21768,43536,45.712486743927,5.447236580205579e-06
5581,22044,22044,44088,46.20673990249634,5.4387630950359455e-06
5650,22320,22320,44640,46.68996977806091,5.431394897585033e-06
5719,22596,22596,45192,47.194124698638916,5.427704849361499e-06
5788,22872,22872,45744,47.713292837142944,5.425989605747568e-06
5857,23148,23148,46296,48.2057158946991,5.424711908319121e-06
5926,23424,23424,46848,48.69077682495117,5.422924850565926e-06
5995,23700,23700,47400,49.167961835861206,5.4217238251780764e-06
6064,23976,23976,47952,49.65929865837097,5.420935028426244e-06
6132,24248,24248,48496,50.141685009002686,5.42040717169227e-06
6201,24524,24524,49048,50.62200880050659,5.4200651945350095e-06
6270,24800,24800,49600,51.12325978279114,5.419478662225166e-06
6339,25076,25076,50152,51.636194705963135,5.419085779662984e-06
6408,25352,25352,50704,52.12013483047485,5.41893747747273e-06
6477,25628,25628,51256,52.596930742263794,5.418821159457836e-06
6546,25904,25904,51808,53.07664895057678,5.418645145651468e-06
6615,26180,26180,52360,53.56790471076965,5.418487041407756e-06
6684,26456,26456,52912,54.056307792663574,5.418434387219458e-06
6753,26732,26732,53464,54.54692363739014,5.418414317821249e-06
6821,27004,27004,54008,55.019720792770386,5.418393387514571e-06
6890,27280,27280,54560,55.499666929244995,5.418368128302607e-06
6959,27556,27556,55112,55.991543769836426,5.4183457009122965e-06
7028,27832,27832,55664,56.46899080276489,5.418328923610278e-06
7097,28108,28108,56216,56.94961094856262,5.4183139780970555e-06
7166,28384,28384,56768,57.43232274055481,5.418305937423661e-06
7235,28660,28660,57320,57.92724680900574,5.418300152453088e-06
7304,28936,28936,57872,58.40895986557007,5.418288053802376e-06
7373,29212,29212,58424,58.88772201538086,5.4182801979015144e-06
7442,29488,29488,58976,59.36830472946167,5.4182743004584945e-06
7511,29764,29764,59528,59.84884190559387,5.418269572197874e-06
7579,30036,30036,60072,60.332435846328735,5.418263446889721e-06
7648,30312,30312,60624,60.85203981399536,5.418262281929102e-06
7717,30588,30588,61176,61.41766881942749,5.418261723282967e-06
7786,30864,30864,61728,61.9419846534729,5.418259716728734e-06
7855,31140,31140,62280,62.504610776901245,5.4182577139139575e-06
7924,31416,31416,62832,63.0895779132843,5.4182572722007674e-06
7993,31692,31692,63384,63.606979846954346,5.418256883295804e-06
8062,31976,31976,63952,64.13519167900085,5.418256216359825e-06
8131,32252,32252,64504,64.65218472480774,5.418255872450233e-06
8200,32538,32538,65076,65.1442518234253,5.418255674035442e-06
8268,32838,32838,65676,65.64438986778259,5.418255571075618e-06
8337,33152,33152,66304,66.22209072113037,5.418255502354908e-06
8406,33436,33436,66872,66.79581904411316,5.41825523066635e-06
8475,33714,33714,67428,67.38300490379333,5.418255126419933e-06
8544,34018,34018,68036,67.95306277275085,5.418255049628186e-06
8613,34422,34422,68844,68.5252468585968,5.418255021982535e-06
8682,34974,34974,69948,69.12334275245667,5.41825502005996e-06
8751,35526,35526,71052,69.70276474952698,5.418255018671845e-06
8820,36078,36078,72156,70.28041887283325,5.4182550174083004e-06
8889,36630,36630,73260,70.86144781112671,5.418255016345616e-06
8958,37182,37182,74364,71.43410086631775,5.41825501537391e-06
9026,37726,37726,75452,72.08378076553345,5.418255014386167e-06
9095,38278,38278,76556,72.75474786758423,5.418255013473212e-06
9164,38830,38830,77660,73.36643195152283,5.418255012718085e-06
9233,39382,39382,78764,73.92911171913147,5.418255011796792e-06
9302,39934,39934,79868,74.49487900733948,5.4182550111414e-06
9371,40486,40486,80972,75.08050680160522,5.418255010361636e-06
9440,41038,41038,82076,75.68770790100098,5.418255009653609e-06
9509,41590,41590,83180,76.3066029548645,5.418255009010715e-06
9578,42142,42142,84284,76.89820384979248,5.418255008396674e-06
9647,42694,42694,85388,77.5326600074768,5.4182550077918015e-06
9715,43238,43238,86476,78.10458970069885,5.418255007182623e-06
9784,43790,43790,87580,78.72326993942261,5.4182550065124455e-06
9853,44342,44342,88684,79.34092688560486,5.418255005972505e-06
9922,44894,44894,89788,79.90126085281372,5.41825500537467e-06
9991,45446,45446,90892,80.46528387069702,5.418255004875147e-06
10060,45998,45998,91996,81.02905988693237,5.418255004388995e-06
10129,46550,46550,93100,81.60380387306213,5.418255003793285e-06
10198,47102,47102,94204,82.17937588691711,5.418255003188061e-06
10267,47654,47654,95308,82.78198575973511,5.418255002686026e-06
10336,48206,48206,96412,83.50581479072571,5.418255002221748e-06
10404,48750,48750,97500,84.16928482055664,5.418255001808962e-06
10473,49302,49302,98604,84.79986095428467,5.4182550012904755e-06
10542,49854,49854,99708,85.47574090957642,5.418255000729741e-06
10611,50406,50406,100812,86.07367992401123,5.418255000343454e-06
10680,50958,50958,101916,86.68417882919312,5.41825499986559e-06
10749,51510,51510,103020,87.34366393089294,5.418254999425903e-06
10818,52062,52062,104124,88.02355480194092,5.418254999020172e-06
10887,52614,52614,105228,88.78230404853821,5.418254998486678e-06
10956,53166,53166,106332,89.38490080833435,5.418254998049228e-06
11025,53526,53526,107052,89.90795493125916,5.379547401755516e-06
11094,53802,53802,107604,90.40278887748718,5.3426670713357725e-06
11162,54074,54074,108148,90.88102459907532,5.309576309987809e-06
11231,54350,54350,108700,91.362637758255,5.228618145228647e-06
11300,54626,54626,109252,91.85619282722473,5.1381711934584415e-06
11369,54902,54902,109804,92.33656668663025,5.062428016607756e-06
11438,55178,55178,110356,92.8174238204956,4.969859668291807e-06
11507,55454,55454,110908,93.30003476142883,4.86847663901688e-06
11576,55730,55730,111460,93.79546594619751,4.755987280676342e-06
11645,56006,56006,112012,94.27767491340637,4.644532227667598e-06
11714,56282,56282,112564,94.758957862854,4.563349586281484e-06
11783,56558,56558,113116,95.23718786239624,4.533739135253155e-06
11851,56830,56830,113660,95.7141649723053,4.5210874601977395e-06
11920,57106,57106,114212,96.20344090461731,4.508520254346753e-06
11989,57382,57382,114764,96.6818368434906,4.484287019303792e-06
12058,57658,57658,115316,97.16001486778259,4.4630354275369e-06
12127,57934,57934,115868,97.64086771011353,4.443563763235381e-06
12196,58210,58210,116420,98.1308479309082,4.406499784912793e-06
12265,58486,58486,116972,98.60904383659363,4.332028206850215e-06
12334,58762,58762,117524,99.08745288848877,4.179523878315869e-06
12403,59038,59038,118076,99.57094669342041,4.101358422251185e-06
12472,59314,59314,118628,100.05453372001648,4.066338157524443e-06
12541,59590,59590,119180,100.54263663291931,4.042072198776329e-06
12609,59862,59862,119724,101.01864194869995,4.018938734216345e-06
12678,60138,60138,120276,101.49686789512634,4.000887569001475e-06
12747,60414,60414,120828,101.97273588180542,3.9733525362892284e-06
12816,60690,60690,121380,102.46234393119812,3.9342055477318715e-06
12885,60966,60966,121932,102.94093179702759,3.8650482095291755e-06
12954,61242,61242,122484,103.42078971862793,3.8109340206641276e-06
13023,61518,61518,123036,103.90232181549072,3.7649103833791135e-06
13092,61794,61794,123588,104.39420175552368,3.696113990085636e-06
13161,62070,62070,124140,104.87279891967773,3.6055238752519567e-06
13230,62346,62346,124692,105.35035276412964,3.5524983195185987e-06
13298,62618,62618,125236,105.82279872894287,3.5065767386028974e-06
13367,62894,62894,125788,106.30136680603027,3.446093724195037e-06
13436,63170,63170,126340,106.79411888122559,3.3855570258591333e-06
13505,63446,63446,126892,107.27620792388916,3.33406273000387e-06
13574,63722,63722,127444,107.7551896572113,3.309015222826138e-06
13643,63998,63998,127996,108.23607778549194,3.2908416674441734e-06
13712,64274,64274,128548,108.7286467552185,3.2785321132046944e-06
13781,64550,64550,129100,109.21156883239746,3.265927737613496e-06
13850,64826,64826,129652,109.68989372253418,3.2493750907092485e-06
13919,65102,65102,130204,110.16170597076416,3.227451908685225e-06
13987,65374,65374,130748,110.6427857875824,3.1953320519373076e-06
14056,65650,65650,131300,111.12254786491394,3.1590658898290943e-06
14125,65926,65926,131852,111.60080981254578,3.146278309381513e-06
14194,66202,66202,132404,112.07815980911255,3.122832000338217e-06
14263,66478,66478,132956,112.5546886920929,3.09471414007653e-06
14332,66754,66754,133508,113.04385995864868,3.0735605749670397e-06
14401,67030,67030,134060,113.52760767936707,3.0624759573872955e-06
14470,67306,67306,134612,114.00836086273193,3.054884208510233e-06
14539,67582,67582,135164,114.48928785324097,3.03930903352301e-06
14608,67858,67858,135716,114.97990465164185,3.0263525617670096e-06
14677,68134,68134,136268,115.46103501319885,2.9920327126437077e-06
14745,68406,68406,136812,115.93091773986816,2.9295877158557433e-06
14814,68682,68682,137364,116.4104425907135,2.874816925018769e-06
14883,68958,68958,137916,116.90064787864685,2.830029493067806e-06
14952,69234,69234,138468,117.38359093666077,2.779916292566648e-06
15021,69510,69510,139020,117.86635184288025,2.7339584903750026e-06
15090,69786,69786,139572,118.34165787696838,2.695673817906832e-06
15159,70062,70062,140124,118.81935286521912,2.6698145911623207e-06
15228,70338,70338,140676,119.31217885017395,2.654228314266887e-06
15297,70614,70614,141228,119.78511166572571,2.6391625276232674e-06
15366,70890,70890,141780,120.26530385017395,2.606295359743482e-06
15434,71162,71162,142324,120.73939776420593,2.583233934499561e-06
15503,71438,71438,142876,121.23155999183655,2.5664358154462755e-06
15572,71714,71714,143428,121.7150206565857,2.5519621579815e-06
15641,71990,71990,143980,122.1929087638855,2.531931294151587e-06
15710,72266,72266,144532,122.67445373535156,2.503489255404376e-06
15779,72542,72542,145084,123.1540858745575,2.466982805767326e-06
15848,72818,72818,145636,123.73884391784668,2.4314317719930634e-06
15917,73094,73094,146188,124.43646478652954,2.4091318040744467e-06
15986,73370,73370,146740,125.00150179862976,2.3904339999841636e-06
16055,73646,73646,147292,125.60482096672058,2.376863791655242e-06
16124,73922,73922,147844,126.32121086120605,2.359634565643593e-06
16192,74194,74194,148388,126.96366286277771,2.333418903938666e-06
16261,74470,74470,148940,127.65596270561218,2.3086168708927725e-06
16330,74746,74746,149492,128.18821573257446,2.2730733817043784e-06
16399,75022,75022,150044,128.76531791687012,2.2365216269952053e-06
16468,75298,75298,150596,129.3210108280182,2.2187470113601148e-06
16537,75574,75574,151148,129.95412182807922,2.199845508405292e-06
16606,75850,75850,151700,130.5681037902832,2.1814330684542478e-06
16675,76126,76126,152252,131.18356275558472,2.172503808892014e-06
16744,76402,76402,152804,131.7752640247345,2.16625852929633e-06
16813,76678,76678,153356,132.40534090995789,2.1516443758307487e-06
16881,76950,76950,153900,133.0773618221283,2.126511890966414e-06
16950,77226,77226,154452,133.66180086135864,2.116538043107509e-06
17019,77502,77502,155004,134.3171808719635,2.1077464725182797e-06
17088,77778,77778,155556,134.88161063194275,2.0923809873870935e-06
17157,78054,78054,156108,135.48418879508972,2.0465776339539337e-06
17226,78330,78330,156660,136.0952398777008,2.0064223858974566e-06
17295,78606,78606,157212,136.7511248588562,1.9882665420288513e-06
17364,78882,78882,157764,137.37223982810974,1.9726226475808127e-06
17433,79158,79158,158316,137.9405529499054,1.949843429886953e-06
17502,79434,79434,158868,138.48915886878967,1.898575797035018e-06
17570,79706,79706,159412,139.01702880859375,1.825812240710027e-06
17639,79982,79982,159964,139.77199387550354,1.7670667087923431e-06
17708,80258,80258,160516,140.36450672149658,1.695356879005043e-06
17777,80534,80534,161068,140.95298171043396,1.6624449907969114e-06
17846,80810,80810,161620,141.46453380584717,1.6519312959117966e-06
17915,81086,81086,162172,142.04820275306702,1.6441434431695751e-06
17984,81362,81362,162724,142.62411499023438,1.630399252387567e-06
18053,81638,81638,163276,143.12631583213806,1.6143139010391927e-06
18122,81914,81914,163828,143.62419366836548,1.6033632476360622e-06
18191,82190,82190,164380,144.12284183502197,1.5947452591192024e-06
18260,82466,82466,164932,144.6396119594574,1.5776860349530363e-06
18328,82738,82738,165476,145.13236260414124,1.5646476321530133e-06
18397,83014,83014,166028,145.62970781326294,1.5477648298014243e-06
18466,83290,83290,166580,146.13220977783203,1.5286419766736564e-06
18535,83566,83566,167132,146.71902799606323,1.5223604238744888e-06
18604,83842,83842,167684,147.26508378982544,1.5166957568915914e-06
18673,84118,84118,168236,147.79954886436462,1.513282337267129e-06
18742,84394,84394,168788,148.3522880077362,1.5086975197298485e-06
18811,84670,84670,169340,148.87463474273682,1.5011823137560756e-06
18880,84946,84946,169892,149.3893687725067,1.4924237302927829e-06
18949,85222,85222,170444,149.88780975341797,1.4784491511895857e-06
19017,85494,85494,170988,150.38222074508667,1.461681303758386e-06
19086,85770,85770,171540,150.89545679092407,1.4445150531194183e-06
19155,86046,86046,172092,151.4021918773651,1.4199759165226276e-06
19224,86322,86322,172644,151.90009093284607,1.4027188241343778e-06
19293,86598,86598,173196,152.3926568031311,1.3980436795145816e-06
19362,86874,86874,173748,152.90250706672668,1.3923136339774182e-06
19431,87150,87150,174300,153.40311574935913,1.3805372028031636e-06
19500,87426,87426,174852,153.90194368362427,1.3662198790610016e-06
19569,87702,87702,175404,154.40004467964172,1.3490319419563382e-06
19638,87978,87978,175956,154.89802479743958,1.3281318485553294e-06
19707,88254,88254,176508,155.40235376358032,1.3186388513945672e-06
19775,88526,88526,177052,155.8922939300537,1.3099714601188582e-06
19844,88802,88802,177604,156.39035868644714,1.303953012246928e-06
19913,89078,89078,178156,156.8865737915039,1.298735559702936e-06
19982,89354,89354,178708,157.3945438861847,1.2910084705819036e-06
20051,89630,89630,179260,157.89169883728027,1.2873215006626254e-06
20120,89906,89906,179812,158.5357849597931,1.2817563060710208e-06
20189,90182,90182,180364,159.2645399570465,1.2716255372986975e-06
20258,90458,90458,180916,159.81633687019348,1.2532575070518929e-06
20327,90734,90734,181468,160.30382585525513,1.1473436953976021e-06
20396,91010,91010,182020,160.79677963256836,1.0851608329482079e-06
20464,91282,91282,182564,161.28470396995544,1.0584566246509227e-06
20533,91558,91558,183116,161.8676779270172,1.0434514902594282e-06
20602,91834,91834,183668,162.48167085647583,1.0359026980603957e-06
20671,92110,92110,184220,163.00680661201477,1.0254069764230329e-06
20740,92386,92386,184772,163.58061289787292,1.0203345441734503e-06
20809,92662,92662,185324,164.0960488319397,1.0154704957168949e-06
20878,92938,92938,185876,164.59131979942322,1.00971258309033e-06
20947,93214,93214,186428,165.07269287109375,1.0021022460935357e-06
21016,93490,93490,186980,165.5636658668518,9.906048423369248e-07
21085,93766,93766,187532,166.05083394050598,9.699213117371869e-07
21153,94038,94038,188076,166.54242372512817,9.400182634328307e-07
21222,94314,94314,188628,167.0457637310028,9.151938773094182e-07
21291,94590,94590,189180,167.57129383087158,8.984040867255151e-07
21360,94866,94866,189732,168.1079728603363,8.840788182356527e-07
21429,95142,95142,190284,168.64778184890747,8.733381640492883e-07
21498,95418,95418,190836,169.17987275123596,8.658876642915251e-07
21567,95694,95694,191388,169.6691448688507,8.592701391158319e-07
21636,95970,95970,191940,170.198588848114,8.443412367382944e-07
21705,96246,96246,192492,170.72593784332275,8.25012109361403e-07
21774,96522,96522,193044,171.2292377948761,8.126607912454637e-07
21843,96798,96798,193596,171.79760575294495,8.073059474274276e-07
21911,97070,97070,194140,172.424222946167,8.01959418662202e-07
21980,97346,97346,194692,172.94713878631592,7.984426879752806e-07
22049,97622,97622,195244,173.43403482437134,7.939919817434364e-07
22118,97898,97898,195796,173.92277359962463,7.8087203001552e-07
22187,98174,98174,196348,174.44212889671326,7.603204120233894e-07
22256,98450,98450,196900,174.9587857723236,7.421182678033652e-07
22325,98726,98726,197452,175.44470977783203,7.318314211332239e-07
22394,99002,99002,198004,175.9348337650299,7.230773834374872e-07
22463,99278,99278,198556,176.45981287956238,7.093826863918587e-07
22532,99554,99554,199108,176.94859170913696,6.98171304938684e-07
22600,99826,99826,199652,177.42905187606812,6.945361157339042e-07
22669,100102,100102,200204,177.92191076278687,6.921058132271046e-07
22738,100378,100378,200756,178.41727685928345,6.885784789664433e-07
22807,100654,100654,201308,178.97648787498474,6.820300902537438e-07
22876,100930,100930,201860,179.53876090049744,6.769494496959827e-07
22945,101206,101206,202412,180.05971789360046,6.738213138870547e-07
23014,101482,101482,202964,180.5999937057495,6.71483172413822e-07
23083,101758,101758,203516,181.12906289100647,6.697619336209671e-07
23152,102034,102034,204068,181.62410187721252,6.656121919536343e-07
23221,102310,102310,204620,182.3446238040924,6.594194519797e-07
23290,102586,102586,205172,182.9580807685852,6.565239623791896e-07
23358,102858,102858,205716,183.59112882614136,6.522469162379786e-07
23427,103134,103134,206268,184.2047917842865,6.482124897592562e-07
23496,103410,103410,206820,184.76584577560425,6.449968407295649e-07
23565,103686,103686,207372,185.27368664741516,6.418520534121865e-07
23634,103962,103962,207924,185.788067817688,6.363629007049928e-07
23703,104238,104238,208476,186.28840279579163,6.287779424455271e-07
23772,104514,104514,209028,186.90825390815735,6.191427324205314e-07
23841,104790,104790,209580,187.48864483833313,6.065189961471137e-07
23910,105066,105066,210132,188.20597577095032,5.904301809218356e-07
23979,105342,105342,210684,188.88677978515625,5.694476783045236e-07
24047,105614,105614,211228,189.44515371322632,5.525427749368964e-07
24116,105890,105890,211780,190.0699667930603,5.357153146269196e-07
24185,106166,106166,212332,190.7250418663025,5.174091663324174e-07
24254,106442,106442,212884,191.26396870613098,4.969855731860432e-07
24323,106718,106718,213436,191.79122471809387,4.867648006982636e-07
24392,106994,106994,213988,192.37824487686157,4.7421732873092195e-07
24461,107270,107270,214540,193.0177538394928,4.691237399806547e-07
24530,107546,107546,215092,193.7070369720459,4.6385720330441294e-07
24599,107822,107822,215644,194.37032079696655,4.504870795197237e-07
24668,108098,108098,216196,195.01179766654968,4.3939604700883184e-07
24737,108374,108374,216748,195.65669679641724,4.2584430356560884e-07
24805,108646,108646,217292,196.28931093215942,4.226221376562356e-07
24874,108922,108922,217844,196.93034601211548,4.193931065169757e-07
24943,109198,109198,218396,197.57167792320251,4.158762988963848e-07
25012,109474,109474,218948,198.45741963386536,4.14186759828887e-07
25081,109750,109750,219500,199.14776873588562,4.1174728026577517e-07
25150,110026,110026,220052,199.8340549468994,4.0753415783939937e-07
25219,110302,110302,220604,200.4778037071228,4.0140628309749583e-07
25288,110578,110578,221156,201.12299704551697,3.904923196235539e-07
25357,110854,110854,221708,201.77380776405334,3.8222460850907154e-07
25426,111130,111130,222260,202.41849088668823,3.736825101400761e-07
25494,111402,111402,222804,203.05621099472046,3.6604533627855266e-07
25563,111678,111678,223356,203.72605276107788,3.6189190697284677e-07
25632,111954,111954,223908,204.51335096359253,3.604440624720314e-07
25701,112230,112230,224460,205.19433665275574,3.5906430110827535e-07
25770,112506,112506,225012,205.90044498443604,3.572780241508375e-07
25839,112782,112782,225564,206.5789430141449,3.5572242970569193e-07
25908,113058,113058,226116,207.31769680976868,3.5396727934222414e-07
25977,113334,113334,226668,208.00306677818298,3.5130967778377487e-07
26046,113610,113610,227220,208.66326189041138,3.491582075076855e-07
26115,113886,113886,227772,209.3343858718872,3.480960718397233e-07
26183,114158,114158,228316,209.9871768951416,3.467779826184963e-07
26252,114434,114434,228868,210.64050102233887,3.4554493264282956e-07
26321,114710,114710,229420,211.3166058063507,3.4395078401953363e-07
26390,114986,114986,229972,211.96480894088745,3.41296122736764e-07
26459,115262,115262,230524,212.62562775611877,3.3755422437841316e-07
26528,115538,115538,231076,213.35346484184265,3.3376826120619847e-07
26597,115814,115814,231628,214.04836893081665,3.2964236521976967e-07
26666,116090,116090,232180,214.79706597328186,3.2358601890400513e-07
26735,116366,116366,232732,215.4765908718109,3.161005719347034e-07
26804,116642,116642,233284,216.1779408454895,3.1133643243180285e-07
26873,116918,116918,233836,216.8323757648468,3.085086365463688e-07
26941,117190,117190,234380,217.4780149459839,3.0628621412350836e-07
27010,117466,117466,234932,218.14209985733032,3.028116180685083e-07
27079,117742,117742,235484,218.85747265815735,3.0021703904444676e-07
27148,118018,118018,236036,219.50494170188904,2.977368275002452e-07
27217,118294,118294,236588,220.15312004089355,2.941835517438351e-07
27286,118570,118570,237140,220.80410075187683,2.9071655681229157e-07
27355,118846,118846,237692,221.4570598602295,2.8979741943857235e-07
27424,119122,119122,238244,222.11467695236206,2.8911918115620434e-07
27493,119398,119398,238796,222.76910591125488,2.876853903431476e-07
27562,119674,119674,239348,223.42443776130676,2.8486909316030424e-07
27630,119946,119946,239892,224.06174898147583,2.8212475715809413e-07
27699,120222,120222,240444,224.70781898498535,2.790019380769651e-07
27768,120498,120498,240996,225.35825777053833,2.766207391723426e-07
27837,120774,120774,241548,225.99882984161377,2.7515489762164966e-07
27906,121050,121050,242100,226.67181873321533,2.7424820777028363e-07
27975,121326,121326,242652,227.35774683952332,2.7299159281630986e-07
28044,121602,121602,243204,228.05729484558105,2.7178798793784285e-07
28113,121878,121878,243756,228.73596858978271,2.697920312556463e-07
28182,122154,122154,244308,229.41913485527039,2.6477965818522863e-07
28251,122430,122430,244860,230.16819882392883,2.6024610813203045e-07
28320,122706,122706,245412,230.84040570259094,2.5617488911482987e-07
28388,122978,122978,245956,231.47265672683716,2.533229357772704e-07
28457,123254,123254,246508,232.1348967552185,2.496465631360814e-07
28526,123530,123530,247060,232.78393983840942,2.46789230091113e-07
28595,123806,123806,247612,233.4238748550415,2.4583526113063445e-07
28664,124082,124082,248164,234.0754566192627,2.44487981637092e-07
28733,124358,124358,248716,234.72709465026855,2.4272290450073585e-07
28802,124634,124634,249268,235.3767786026001,2.3956571896642965e-07
28871,124910,124910,249820,236.0384497642517,2.3315566270277283e-07
28940,125186,125186,250372,236.68685865402222,2.2883658732484045e-07
29009,125462,125462,250924,237.32569193840027,2.2567294809410412e-07
29077,125734,125734,251468,237.96625685691833,2.2392417651845067e-07
29146,126010,126010,252020,238.62996196746826,2.2273818222902288e-07
29215,126286,126286,252572,239.273521900177,2.2212666203007682e-07
29284,126562,126562,253124,239.91052293777466,2.2110603538175724e-07
29353,126838,126838,253676,240.55987977981567,2.1845132477990954e-07
29422,127114,127114,254228,241.203430891037,2.160027505960292e-07
29491,127390,127390,254780,241.84379172325134,2.1480538289272548e-07
29560,127666,127666,255332,242.4903507232666,2.1370895833494108e-07
29629,127942,127942,255884,243.13119888305664,2.1288053061217554e-07
29698,128218,128218,256436,243.7752227783203,2.1181875736117828e-07
29766,128490,128490,256980,244.4064269065857,2.1059939449617577e-07
29835,128766,128766,257532,245.05514478683472,2.0891634556288388e-07
29904,129042,129042,258084,245.69463562965393,2.0706120532770302e-07
29973,129318,129318,258636,246.3295476436615,2.0221842238583562e-07
30042,129594,129594,259188,246.97644066810608,1.9545145029553934e-07
30111,129870,129870,259740,247.61255884170532,1.8921106300299956e-07
30180,130146,130146,260292,248.2477309703827,1.8350255514487614e-07
30249,130422,130422,260844,248.89169001579285,1.7982156837081027e-07
30318,130698,130698,261396,249.52943897247314,1.7815860757490988e-07
30387,130974,130974,261948,250.16625380516052,1.7601310962337625e-07
30456,131250,131250,262500,250.80623579025269,1.715064809279877e-07
30524,131522,131522,263044,251.4348816871643,1.664861088791907e-07
30593,131798,131798,263596,252.06886887550354,1.6371368452323642e-07
30662,132074,132074,264148,252.71198081970215,1.5853168000553902e-07
30731,132350,132350,264700,253.37865591049194,1.5432128239490236e-07
30800,132626,132626,265252,254.04853987693787,1.5295707590396073e-07
30869,132902,132902,265804,254.72963571548462,1.5176413698610226e-07
30938,133178,133178,266356,255.4235348701477,1.5039967641636483e-07
31007,133454,133454,266908,256.10738372802734,1.495239342875822e-07
31076,133730,133730,267460,256.8021788597107,1.480012795564731e-07
31145,134006,134006,268012,257.5050427913666,1.4687677282874137e-07
31213,134278,134278,268556,258.1926968097687,1.4604284196718903e-07
31282,134554,134554,269108,258.85950899124146,1.4558705225831947e-07
31351,134830,134830,269660,259.53318667411804,1.4491048651426383e-07
31420,135106,135106,270212,260.1881170272827,1.4336938719654986e-07
31489,135382,135382,270764,260.8432557582855,1.4286191505661095e-07
31558,135658,135658,271316,261.4997498989105,1.4229411479175603e-07
31627,135934,135934,271868,262.1406726837158,1.407070653240422e-07
31696,136210,136210,272420,262.78220081329346,1.377832811094919e-07
31765,136486,136486,272972,263.4113817214966,1.353540122080494e-07
31834,136762,136762,273524,264.0613429546356,1.318679619038856e-07
31903,137038,137038,274076,264.7114658355713,1.2826107566339736e-07
31971,137308,137308,274616,265.34703278541565,1.171928960003993e-07
32040,137584,137584,275168,266.01116275787354,1.0132417749435293e-07
32109,137860,137860,275720,266.6687738895416,9.650243263749317e-08
32178,138136,138136,276272,267.33119082450867,9.43169996843555e-08
32247,138412,138412,276824,267.9954698085785,9.331792737875765e-08
32316,138688,138688,277376,268.6592288017273,9.264063588882561e-08
32385,138964,138964,277928,269.3211188316345,9.212432019597905e-08
32454,139240,139240,278480,269.9795117378235,9.176588640971987e-08
32523,139516,139516,279032,270.6572518348694,9.139952021059324e-08
32592,139792,139792,279584,271.3302128314972,9.087626009741395e-08
32660,140064,140064,280128,271.98853874206543,8.967201816813838e-08
32729,140340,140340,280680,272.6710617542267,8.836217372058603e-08
32798,140616,140616,281232,273.3497648239136,8.782883348378235e-08
32867,140892,140892,281784,274.00649070739746,8.756704903899811e-08
32936,141168,141168,282336,274.6531536579132,8.725012488511617e-08
33005,141444,141444,282888,275.29378271102905,8.66773924310983e-08
33074,141720,141720,283440,275.9339249134064,8.597079784935756e-08
33143,141996,141996,283992,276.58721470832825,8.563822453302807e-08
33212,142272,142272,284544,277.2322578430176,8.527511212740912e-08
33281,142548,142548,285096,277.8711757659912,8.4698734485662e-08
33349,142820,142820,285640,278.4963777065277,8.378761323805962e-08
33418,143096,143096,286192,279.13953280448914,8.362196681417924e-08
33487,143372,143372,286744,279.77154779434204,8.337397639506041e-08
33556,143648,143648,287296,280.4639256000519,8.283835279240032e-08
33625,143924,143924,287848,281.1617286205292,8.199480047054082e-08
33694,144200,144200,288400,281.84865164756775,8.093339114288381e-08
33763,144476,144476,288952,282.53495502471924,7.934371705683026e-08
33832,144752,144752,289504,283.2183287143707,7.808568637215932e-08
33901,145028,145028,290056,283.8971438407898,7.703089350830445e-08
33970,145304,145304,290608,284.65860199928284,7.651263278264364e-08
34039,145580,145580,291160,285.38020300865173,7.629183536683357e-08
34107,145852,145852,291704,286.0350296497345,7.59673693136612e-08
34176,146128,146128,292256,286.6893229484558,7.530684656913268e-08
34245,146404,146404,292808,287.35250878334045,7.480446304591012e-08
34314,146680,146680,293360,288.0057158470154,7.410970722169751e-08
34383,146956,146956,293912,288.75623297691345,7.326631062819864e-08
34452,147232,147232,294464,289.4334318637848,7.27193753063976e-08
34521,147508,147508,295016,290.15724873542786,7.245272023878989e-08
34590,147784,147784,295568,290.8470118045807,7.17252063146894e-08
34659,148060,148060,296120,291.5293457508087,7.10803535777876e-08
34728,148336,148336,296672,292.2022488117218,7.06294931258012e-08
34796,148608,148608,297216,292.85228180885315,7.03249274607657e-08
34865,148884,148884,297768,293.50874185562134,6.991528381434786e-08
34934,149160,149160,298320,294.1971278190613,6.938715860557984e-08
35003,149436,149436,298872,294.8630928993225,6.906329778356431e-08
35072,149712,149712,299424,295.50174283981323,6.877939140210791e-08
35141,149988,149988,299976,296.15096783638,6.836522673050149e-08
35210,150264,150264,300528,296.84655690193176,6.719074799508175e-08
35279,150540,150540,301080,297.48795080184937,6.611533697066439e-08
35348,150816,150816,301632,298.17958092689514,6.523090180646529e-08
35417,151092,151092,302184,298.8244049549103,6.479434965145409e-08
35486,151368,151368,302736,299.51485896110535,6.374411826001546e-08
35554,151640,151640,303280,300.1954996585846,6.296379456387648e-08
35623,151916,151916,303832,301.05082082748413,6.245135491003757e-08
35692,152192,152192,304384,301.7575888633728,6.213939287679705e-08
35761,152468,152468,304936,302.4301428794861,6.168659357225229e-08
35830,152744,152744,305488,303.0847339630127,6.137800717762748e-08
35899,153020,153020,306040,303.75619888305664,6.117526998383412e-08
35968,153296,153296,306592,304.42027282714844,6.098291219658838e-08
36037,153572,153572,307144,305.0764636993408,6.049508147852142e-08
36106,153848,153848,307696,305.74141693115234,6.000884080687201e-08
36175,154124,154124,308248,306.4669678211212,5.978675901893143e-08
36243,154396,154396,308792,307.1674346923828,5.956260456147538e-08
36312,154672,154672,309344,307.8939609527588,5.891665410713299e-08
36381,154948,154948,309896,308.5717329978943,5.846147565112455e-08
36450,155224,155224,310448,309.27128076553345,5.803098683807715e-08
36519,155500,155500,311000,309.92412185668945,5.760114291429521e-08
36588,155776,155776,311552,310.55934596061707,5.719733501432382e-08
36657,156052,156052,312104,311.24150562286377,5.6653620058837056e-08
36726,156328,156328,312656,312.080463886261,5.603753622351761e-08
36795,156604,156604,313208,312.7679109573364,5.566658600211047e-08
36864,156880,156880,313760,313.4206657409668,5.552303539918677e-08
36932,157152,157152,314304,314.0600326061249,5.541027937292887e-08
37001,157428,157428,314856,314.7267208099365,5.524794219093595e-08
37070,157704,157704,315408,315.4166567325592,5.504316639183883e-08
37139,157980,157980,315960,316.1104428768158,5.4818952409480265e-08
37208,158256,158256,316512,316.83944392204285,5.4543699654833795e-08
37277,158532,158532,317064,317.522176027298,5.393853292004666e-08
37346,158808,158808,317616,318.27353978157043,5.336001239452197e-08
37415,159084,159084,318168,318.98832988739014,5.2949140734512487e-08
37484,159360,159360,318720,319.66468572616577,5.199594474389038e-08
37553,159636,159636,319272,320.32919573783875,5.1053899173300757e-08
37622,159912,159912,319824,320.98120188713074,4.989683084712992e-08
37690,160184,160184,320368,321.62967562675476,4.865686035102206e-08
37759,160460,160460,320920,322.2804927825928,4.733327371898263e-08
37828,160736,160736,321472,322.95098781585693,4.5782538225368195e-08
37897,161012,161012,322024,323.6392488479614,4.323141394361311e-08
37966,161288,161288,322576,324.21842670440674,4.025843090267798e-08
38035,161564,161564,323128,324.78037190437317,3.887447883811857e-08
38104,161840,161840,323680,325.3633577823639,3.8211015974264216e-08
38173,162116,162116,324232,325.9757046699524,3.683301121112338e-08
38242,162392,162392,324784,326.5171809196472,3.646293309529641e-08
38311,162668,162668,325336,327.10060477256775,3.616874990233188e-08
38379,162940,162940,325880,327.7188799381256,3.574991690454122e-08
38448,163216,163216,326432,328.34158968925476,3.490118807184019e-08
38517,163492,163492,326984,329.02814388275146,3.418871709467111e-08
38586,163768,163768,327536,329.67919182777405,3.36042471374257e-08
38655,164044,164044,328088,330.38970398902893,3.3380988425129425e-08
38724,164320,164320,328640,331.00402784347534,3.324678469187364e-08
38793,164596,164596,329192,331.57908272743225,3.309484413960848e-08
38862,164872,164872,329744,332.10897278785706,3.274080966023562e-08
38931,165148,165148,330296,332.6475558280945,3.2426456447699345e-08
39000,165424,165424,330848,333.24768590927124,3.2273530783533174e-08
39069,165700,165700,331400,333.7359449863434,3.2103452369594196e-08
39137,165972,165972,331944,334.21406388282776,3.198741770676236e-08
39206,166248,166248,332496,334.72843170166016,3.189942510231858e-08
39275,166524,166524,333048,335.2157347202301,3.1669622378626716e-08
39344,166800,166800,333600,335.7026598453522,3.116418256158964e-08
39413,167076,167076,334152,336.17347264289856,2.9581404959419772e-08
39482,167352,167352,334704,336.67703080177307,2.8124716727284565e-08
39551,167628,167628,335256,337.161239862442,2.734010282874724e-08
39620,167904,167904,335808,337.6412229537964,2.718541223673838e-08
39689,168180,168180,336360,338.12448287010193,2.6977845908482417e-08
39758,168456,168456,336912,338.62051367759705,2.6742366551078775e-08
39826,168728,168728,337456,339.09021496772766,2.6284919573105782e-08
39895,169004,169004,338008,339.56635761260986,2.5617638033437815e-08
39964,169280,169280,338560,340.04421973228455,2.5394570686772807e-08
40033,169556,169556,339112,340.54634976387024,2.5295009783784887e-08
40102,169832,169832,339664,341.0632178783417,2.509741812885375e-08
40171,170108,170108,340216,341.54733872413635,2.4512805032040537e-08
40240,170384,170384,340768,342.02766966819763,2.429589312713311e-08
40309,170660,170660,341320,342.50435996055603,2.4177213255511873e-08
40378,170936,170936,341872,342.99747467041016,2.4091421697957917e-08
40447,171212,171212,342424,343.47495579719543,2.402329159802836e-08
40515,171484,171484,342968,343.94392681121826,2.3545493958117555e-08
40584,171760,171760,343520,344.41981172561646,2.303747183382659e-08
40653,172036,172036,344072,344.9082486629486,2.2561588041989718e-08
40722,172312,172312,344624,345.3904597759247,2.2078526278597626e-08
40791,172588,172588,345176,345.87769985198975,2.17913102265046e-08
40860,172864,172864,345728,346.35388684272766,2.161001804878353e-08
40929,173140,173140,346280,346.8334767818451,2.1293994530429697e-08
40998,173416,173416,346832,347.35002970695496,2.0943434008074683e-08
41067,173692,173692,347384,347.8476617336273,2.084000942874622e-08
41136,173968,173968,347936,348.34973788261414,2.077248749443322e-08
41205,174244,174244,348488,348.8436748981476,2.068724493080108e-08
41273,174516,174516,349032,349.3445818424225,2.0524849780940728e-08
41342,174792,174792,349584,349.85069489479065,2.0457112211350664e-08
41411,175068,175068,350136,350.34317803382874,2.0329897106409392e-08
41480,175344,175344,350688,350.8178708553314,2.022894959844226e-08
41549,175620,175620,351240,351.3001937866211,2.014214369051683e-08
41618,175896,175896,351792,351.77512979507446,1.99733745399545e-08
41687,176172,176172,352344,352.25613594055176,1.9794910349051174e-08
41756,176448,176448,352896,352.7922627925873,1.9577051213679814e-08
41825,176724,176724,353448,353.3258776664734,1.9439572929981147e-08
41894,177000,177000,354000,353.8826518058777,1.9301377690262157e-08
41962,177272,177272,354544,354.4010548591614,1.9234179562677915e-08
42031,177548,177548,355096,354.9055349826813,1.917107327187677e-08
42100,177824,177824,355648,355.3992006778717,1.9055565599172018e-08
42169,178100,178100,356200,355.8777937889099,1.8966599583791368e-08
42238,178376,178376,356752,356.35800075531006,1.889518515394689e-08
42307,178652,178652,357304,356.8611147403717,1.878286299157154e-08
42376,178928,178928,357856,357.3429298400879,1.8708034150103402e-08
42445,179204,179204,358408,357.9163568019867,1.8607228393260128e-08
42514,179480,179480,358960,358.4307358264923,1.8400460837927416e-08
42583,179756,179756,359512,358.950199842453,1.8159282963334205e-08
42652,180032,180032,360064,359.4471786022186,1.7955611969020902e-08
42720,180304,180304,360608,360.00181674957275,1.777905212863198e-08
42789,180580,180580,361160,360.52773880958557,1.7608190241520244e-08
42858,180856,180856,361712,361.1785228252411,1.73583200100653e-08
42927,181132,181132,362264,361.6801288127899,1.7053645442832836e-08
42996,181408,181408,362816,362.19471168518066,1.6925875988396743e-08
43065,181684,181684,363368,362.68168663978577,1.6872398358332787e-08
43134,181960,181960,363920,363.2916359901428,1.6770829680530976e-08
43203,182236,182236,364472,363.8091866970062,1.6601018281398506e-08
43272,182512,182512,365024,364.32421875,1.6414761119238676e-08
43341,182788,182788,365576,364.805392742157,1.6309574691491078e-08
43409,183060,183060,366120,365.2835838794708,1.6142398438558668e-08
43478,183336,183336,366672,365.7607398033142,1.6034279348782667e-08
43547,183612,183612,367224,366.2501440048218,1.5949146983948047e-08
43616,183888,183888,367776,366.7288398742676,1.586934298590346e-08
43685,184164,184164,368328,367.2061257362366,1.5807309838901874e-08
43754,184440,184440,368880,367.6799030303955,1.574366119908707e-08
43823,184716,184716,369432,368.18590688705444,1.5659979362749393e-08
43892,184992,184992,369984,368.6639087200165,1.5531526358519117e-08
43961,185268,185268,370536,369.1376929283142,1.5485223619875414e-08
44030,185544,185544,371088,369.6113398075104,1.5406139855185226e-08
44098,185816,185816,371632,370.07950472831726,1.5327015732567238e-08
44167,186092,186092,372184,370.56775283813477,1.526627322737932e-08
44236,186368,186368,372736,371.0422477722168,1.5164866127681813e-08
44305,186644,186644,373288,371.51371598243713,1.4895653297465927e-08
44374,186920,186920,373840,371.99114966392517,1.4783132638589661e-08
44443,187196,187196,374392,372.49057483673096,1.4700178261095942e-08
44512,187472,187472,374944,372.9672567844391,1.464081258703361e-08
44581,187748,187748,375496,373.4436078071594,1.457072184376416e-08
44650,188024,188024,376048,373.9204828739166,1.4448983035405149e-08
44719,188300,188300,376600,374.4041347503662,1.4400121024460208e-08
44788,188576,188576,377152,374.8864107131958,1.4365513859689097e-08
44856,188848,188848,377696,375.3533308506012,1.4296883362324932e-08
44925,189124,189124,378248,375.8280668258667,1.4195049916950638e-08
44994,189400,189400,378800,376.30389380455017,1.41222855480377e-08
45063,189676,189676,379352,376.7939918041229,1.4067449724420574e-08
45132,189952,189952,379904,377.2731018066406,1.3958838543700092e-08
45201,190228,190228,380456,377.7444038391113,1.3858254461930909e-08
45270,190504,190504,381008,378.2207918167114,1.3779557740568337e-08
45339,190780,190780,381560,378.7070438861847,1.3640193823380357e-08
45408,191056,191056,382112,379.1817977428436,1.3294849179345518e-08
45477,191332,191332,382664,379.6586208343506,1.3048054912118135e-08
45545,191604,191604,383208,380.19900703430176,1.296633419594049e-08
45614,191880,191880,383760,380.7521216869354,1.2920184461903211e-08
45683,192156,192156,384312,381.3169598579407,1.2835967816792208e-08
45752,192432,192432,384864,381.8391606807709,1.2635374063836347e-08
45821,192708,192708,385416,382.35349893569946,1.2268381107259145e-08
45890,192984,192984,385968,382.8474168777466,1.1251056291509347e-08
45959,193260,193260,386520,383.3540987968445,1.0655140987036657e-08
46028,193536,193536,387072,383.9781677722931,1.0282882476913885e-08
46097,193812,193812,387624,384.5168068408966,1.0137218135343047e-08
46166,194088,194088,388176,385.050550699234,1.0079348263221941e-08
46235,194364,194364,388728,385.58105087280273,1.0020515276001762e-08
46303,194636,194636,389272,386.1579577922821,9.990432463921724e-09
46372,194912,194912,389824,386.65403866767883,9.953134420979108e-09
46441,195188,195188,390376,387.14723896980286,9.916787171293523e-09
46510,195464,195464,390928,387.6568739414215,9.77220772434774e-09
46579,195740,195740,391480,388.1452338695526,9.685682371202764e-09
46648,196016,196016,392032,388.69078397750854,9.626878130161697e-09
46717,196292,196292,392584,389.2382278442383,9.521347256630837e-09
46786,196568,196568,393136,389.7477607727051,9.350486866134259e-09
46855,196844,196844,393688,390.25181579589844,9.058346851406907e-09
46924,197120,197120,394240,390.7405126094818,8.980620824167765e-09
46992,197392,197392,394784,391.2474477291107,8.913816126085181e-09
47061,197668,197668,395336,391.7372977733612,8.883720640832215e-09
47130,197944,197944,395888,392.2149178981781,8.834838241282082e-09
47199,198220,198220,396440,392.69472789764404,8.80717884057288e-09
47268,198496,198496,396992,393.1832377910614,8.76959077079573e-09
47337,198772,198772,397544,393.6761920452118,8.396559820535782e-09
47406,199048,199048,398096,394.1472358703613,7.697257444737086e-09
47475,199324,199324,398648,394.61879086494446,7.1879491194523704e-09
47544,199600,199600,399200,395.0909128189087,6.879690368770713e-09
47613,199876,199876,399752,395.57858085632324,6.651807322929095e-09
47682,200152,200152,400304,396.05532789230347,6.577756432901497e-09
47750,200424,200424,400848,396.5331027507782,6.4639847859304e-09
47819,200700,200700,401400,397.01554894447327,6.382253833026478e-09
47888,200976,200976,401952,397.4875919818878,6.3466599460061094e-09
47957,201252,201252,402504,398.05284571647644,6.321390368371481e-09
48026,201528,201528,403056,398.59196186065674,6.300697561686111e-09
48095,201804,201804,403608,399.12306690216064,6.27713806947328e-09
48164,202080,202080,404160,399.6855869293213,6.245453856939552e-09
48233,202356,202356,404712,400.2020049095154,6.194431107750746e-09
48302,202632,202632,405264,400.7430908679962,6.141611811039899e-09
48371,202908,202908,405816,401.30093693733215,6.0987899585010706e-09
48439,203180,203180,406360,401.83267092704773,6.061387114364413e-09
48508,203456,203456,406912,402.3458659648895,6.041132649005496e-09
48577,203732,203732,407464,402.8602776527405,6.012330061279831e-09
48646,204008,204008,408016,403.3982207775116,5.960149013165854e-09
48715,204284,204284,408568,404.1110887527466,5.943761754704202e-09
48784,204560,204560,409120,404.6865029335022,5.905116658312808e-09
48853,204836,204836,409672,405.33615899086,5.850398427986864e-09
48922,205112,205112,410224,405.8239486217499,5.824944870516106e-09
48991,205388,205388,410776,406.3220307826996,5.8052466304908995e-09
49060,205664,205664,411328,406.8220057487488,5.623871372257996e-09
49128,205936,205936,411872,407.30626678466797,5.1950209052941185e-09
49197,206212,206212,412424,407.7838237285614,4.5569015584789734e-09
49266,206488,206488,412976,408.31470584869385,4.4344995480608055e-09
49335,206764,206764,413528,408.8048529624939,4.35398838096287e-09
49404,207040,207040,414080,409.2810230255127,4.308420337132631e-09
49473,207316,207316,414632,409.75422167778015,4.269509467643095e-09
49542,207592,207592,415184,410.2357337474823,4.245218354680386e-09
49611,207868,207868,415736,410.7236957550049,4.211266519152842e-09
49680,208144,208144,416288,411.2348418235779,4.1762690440796006e-09
49749,208420,208420,416840,411.77395272254944,4.16050130949354e-09
49818,208696,208696,417392,412.3603856563568,4.145684578862457e-09
49886,208968,208968,417936,412.8803608417511,4.110247057512067e-09
49955,209244,209244,418488,413.39886474609375,4.049030241792203e-09
50024,209520,209520,419040,413.9005446434021,3.9357215603834355e-09
50093,209796,209796,419592,414.3935878276825,3.842768826812378e-09
50162,210072,210072,420144,414.8926947116852,3.819280656353185e-09
50231,210348,210348,420696,415.38057494163513,3.7879807092814795e-09
50300,210624,210624,421248,415.9393558502197,3.757417929079265e-09
50369,210900,210900,421800,416.45882987976074,3.735801774751609e-09
50438,211176,211176,422352,416.95729994773865,3.6950604747787495e-09
50507,211452,211452,422904,417.44596576690674,3.647564224736588e-09
50575,211724,211724,423448,417.9171736240387,3.5497098215738283e-09
50644,212000,212000,424000,418.3939347267151,3.4249449408725987e-09
50713,212276,212276,424552,418.87975096702576,3.3696260826169682e-09
50782,212552,212552,425104,419.35761880874634,3.3517040602094667e-09
50851,212828,212828,425656,419.8318510055542,3.3181082103516687e-09
50920,213104,213104,426208,420.30975890159607,3.290760446592035e-09
50989,213380,213380,426760,420.78755259513855,3.2350858639959197e-09
51058,213656,213656,427312,421.2766079902649,3.1901595921619057e-09
51127,213932,213932,427864,421.748982667923,3.1636094928587122e-09
51196,214208,214208,428416,422.2713689804077,3.1460277769951864e-09
51265,214484,214484,428968,422.78849482536316,3.1127703068175617e-09
51333,214756,214756,429512,423.306697845459,3.0871637877536724e-09
51402,215032,215032,430064,423.82774567604065,3.0584803187848747e-09
51471,215308,215308,430616,424.3418958187103,3.028341836284192e-09
51540,215584,215584,431168,424.85498881340027,2.9794455381733032e-09
51609,215860,215860,431720,425.3814957141876,2.9277597762108842e-09
51678,216136,216136,432272,425.8888318538666,2.9148358767368383e-09
51747,216412,216412,432824,426.4118158817291,2.8933239988879873e-09
51816,216688,216688,433376,426.9154257774353,2.878282921076666e-09
51885,216964,216964,433928,427.4749827384949,2.870102131058246e-09
51954,217240,217240,434480,428.0511507987976,2.8522446484670953e-09
52022,217512,217512,435024,428.5260407924652,2.8295998004661735e-09
52091,217788,217788,435576,429.00607681274414,2.822336564092519e-09
52160,218064,218064,436128,429.4997887611389,2.8078287180295076e-09
52229,218340,218340,436680,429.978551864624,2.7416271247039067e-09
52298,218616,218616,437232,430.45946073532104,2.6401724505977955e-09
52367,218892,218892,437784,430.93876361846924,2.457781308096212e-09
52436,219168,219168,438336,431.4251039028168,2.3751228470725177e-09
52505,219444,219444,438888,431.9069256782532,2.348258629901946e-09
52574,219720,219720,439440,432.387247800827,2.325631313868198e-09
52643,219996,219996,439992,432.8700969219208,2.3068077653752593e-09
52711,220268,220268,440536,433.36318373680115,2.2863140120358693e-09
52780,220544,220544,441088,433.85587191581726,2.2488127962117253e-09
52849,220820,220820,441640,434.4555928707123,2.2335890405516453e-09
52918,221096,221096,442192,434.96755194664,2.2245026199162873e-09
52987,221372,221372,442744,435.48082876205444,2.2094453615701704e-09
53056,221648,221648,443296,435.9915289878845,2.1956268249099064e-09
53125,221924,221924,443848,436.4737186431885,2.1808678856906877e-09
53194,222200,222200,444400,437.0761127471924,2.1569413107965688e-09
53263,222476,222476,444952,437.62628984451294,2.133473612466227e-09
53332,222752,222752,445504,438.147962808609,2.110115989871607e-09
53401,223028,223028,446056,438.6540858745575,2.0817059322994783e-09
53469,223300,223300,446600,439.19912481307983,2.0729633183188693e-09
53538,223576,223576,447152,439.72119092941284,2.062360247995324e-09
53607,223852,223852,447704,440.2203719615936,2.0543765905478996e-09
53676,224128,224128,448256,440.70250391960144,2.0333344550227096e-09
53745,224404,224404,448808,441.23166584968567,2.0162842299797854e-09
53814,224680,224680,449360,441.7659797668457,2.0064317737002327e-09
53883,224956,224956,449912,442.3088607788086,2.0002907984069454e-09
53952,225232,225232,450464,442.82453870773315,1.990982394717192e-09
54021,225508,225508,451016,443.31033086776733,1.9654918616000283e-09
54090,225784,225784,451568,443.89754581451416,1.953512502379722e-09
54158,226056,226056,452112,444.4168047904968,1.9410854989180417e-09
54227,226332,226332,452664,444.99092197418213,1.9347407238642083e-09
54296,226608,226608,453216,445.50373888015747,1.918317244611672e-09
54365,226884,226884,453768,446.0019438266754,1.8762375151407468e-09
54434,227160,227160,454320,446.5005588531494,1.838625519901394e-09
54503,227436,227436,454872,446.98861479759216,1.8223207056310332e-09
54572,227712,227712,455424,447.4724009037018,1.8081826706384006e-09
54641,227988,227988,455976,447.9542098045349,1.7974920990590113e-09
54710,228264,228264,456528,448.4942636489868,1.7861597172963949e-09
54779,228540,228540,457080,448.99636578559875,1.779741520393808e-09
54848,228816,228816,457632,449.5643746852875,1.76054284124284e-09
54916,229088,229088,458176,450.0652480125427,1.7272635773660054e-09
54985,229364,229364,458728,450.58923172950745,1.683448825600747e-09
55054,229640,229640,459280,451.0712068080902,1.6656943465194279e-09
55123,229916,229916,459832,451.5625648498535,1.6561825994001457e-09
55192,230192,230192,460384,452.04622888565063,1.650047141757345e-09
55261,230468,230468,460936,452.54358673095703,1.63603835046073e-09
55330,230744,230744,461488,453.02367186546326,1.6173012926335166e-09
55399,231020,231020,462040,453.501966714859,1.6056888805898053e-09
55468,231296,231296,462592,453.9765827655792,1.597752390433735e-09
55537,231572,231572,463144,454.453177690506,1.590453249433691e-09
55605,231844,231844,463688,454.9353096485138,1.5829850714672603e-09
55674,232120,232120,464240,455.4127869606018,1.5356057262021622e-09
55743,232396,232396,464792,455.8892867565155,1.4317017288187108e-09
55812,232672,232672,465344,456.3647298812866,1.304646609390832e-09
55881,232948,232948,465896,456.85492181777954,1.1780111838632805e-09
55950,233224,233224,466448,457.3392038345337,1.0682479452866582e-09
56019,233500,233500,467000,457.82509183883667,1.0270785063982181e-09
56088,233776,233776,467552,458.3135597705841,1.0066313637536928e-09
56157,234052,234052,468104,458.8647608757019,9.977432069366327e-10
56226,234328,234328,468656,459.35002398490906,9.865302017253653e-10
56294,234600,234600,469200,459.83343482017517,9.772548067613208e-10
56363,234876,234876,469752,460.31178879737854,9.651332492714114e-10
56432,235152,235152,470304,460.79155683517456,9.510833142698576e-10
56501,235428,235428,470856,461.2826247215271,9.435766775372483e-10
56570,235704,235704,471408,461.7572648525238,9.391447443295818e-10
56639,235980,235980,471960,462.23590874671936,9.216072473410704e-10
56708,236256,236256,472512,462.7122309207916,8.906911659557822e-10
56777,236532,236532,473064,463.20326566696167,8.750427785402999e-10
56846,236808,236808,473616,463.67874097824097,8.600868795331737e-10
56915,237084,237084,474168,464.1593017578125,8.546704874436489e-10
56984,237360,237360,474720,464.636088848114,8.503308026511166e-10
57052,237632,237632,475264,465.1159257888794,8.465086136507355e-10
57121,237908,237908,475816,465.59401679039,8.446288059075626e-10
57190,238184,238184,476368,466.07412981987,8.402862755447936e-10
57259,238460,238460,476920,466.5511407852173,8.317934401491716e-10
57328,238736,238736,477472,467.0298240184784,8.254957847335968e-10
57397,239012,239012,478024,467.5242030620575,7.998583663591589e-10
57466,239288,239288,478576,468.0046169757843,7.541586868695745e-10
57535,239564,239564,479128,468.48600482940674,7.19464717138544e-10
57604,239840,239840,479680,468.96535992622375,7.136943892550313e-10
57673,240116,240116,480232,469.44515895843506,7.108255148554479e-10
57741,240388,240388,480776,469.91805696487427,7.064388980588756e-10
57810,240664,240664,481328,470.3970558643341,7.031242718372024e-10
57879,240940,240940,481880,470.87483978271484,7.001973477719222e-10
57948,241216,241216,482432,471.3526887893677,6.933680251214118e-10
58017,241492,241492,482984,471.8382217884064,6.394342611504823e-10
58086,241768,241768,483536,472.31149077415466,5.786360493521619e-10
58155,242044,242044,484088,472.791298866272,5.611051189403305e-10
58224,242320,242320,484640,473.2658660411835,5.550181324237399e-10
58293,242596,242596,485192,473.7518699169159,5.513870567818612e-10
58362,242872,242872,485744,474.2298996448517,5.477361131055751e-10
58431,243148,243148,486296,474.7173328399658,5.462183482721908e-10
58499,243420,243420,486840,475.1957287788391,5.432613186015048e-10
58568,243696,243696,487392,475.69083070755005,5.411004199176294e-10
58637,243972,243972,487944,476.16540789604187,5.36241165996271e-10
58706,244248,244248,488496,476.6482229232788,5.337082201831936e-10
58775,244524,244524,489048,477.12703371047974,5.318409732037425e-10
58844,244800,244800,489600,477.60350489616394,5.286733399142967e-10
58913,245076,245076,490152,478.09300780296326,5.199007844736455e-10
58982,245352,245352,490704,478.5694646835327,5.091314996023779e-10
59051,245628,245628,491256,479.0492277145386,5.062824328560362e-10
59120,245904,245904,491808,479.52586483955383,5.027733232569621e-10
59188,246176,246176,492352,480.00602173805237,5.015349093610229e-10
59257,246452,246452,492904,480.4874486923218,4.969080652330707e-10
59326,246728,246728,493456,480.9647047519684,4.689934437936e-10
59395,247004,247004,494008,481.4386887550354,4.5996397546798535e-10
59464,247280,247280,494560,481.9193286895752,4.563181738760873e-10
59533,247556,247556,495112,482.39988470077515,4.491002402885118e-10
59602,247832,247832,495664,482.8776078224182,4.4496044561224936e-10
59671,248108,248108,496216,483.3548307418823,4.41403186913556e-10
59740,248384,248384,496768,483.8286609649658,4.3884455431015565e-10
59809,248660,248660,497320,484.3178927898407,4.3721778598119293e-10
59877,248932,248932,497864,484.7874298095703,4.3513891926179973e-10
59946,249208,249208,498416,485.260018825531,4.3215381082997955e-10
60015,249484,249484,498968,485.731675863266,4.2986428668878534e-10
60084,249760,249760,499520,486.226655960083,4.215795308951113e-10
60153,250036,250036,500072,486.7015266418457,4.147537646123436e-10
60222,250312,250312,500624,487.17402482032776,4.129593772402108e-10
60291,250588,250588,501176,487.65276288986206,4.1163538886123826e-10
60360,250864,250864,501728,488.1304018497467,4.100940710695433e-10
60429,251140,251140,502280,488.61781191825867,4.017170007790655e-10
60498,251416,251416,502832,489.0971736907959,3.715517204651431e-10
60567,251692,251692,503384,489.5862138271332,3.4567665577333703e-10
60635,251964,251964,503928,490.060950756073,3.404772362473657e-10
60704,252240,252240,504480,490.55983901023865,3.3772565158503376e-10
60773,252516,252516,505032,491.0431938171387,3.3543300249273077e-10
60842,252792,252792,505584,491.53103280067444,3.34080195492148e-10
60911,253068,253068,506136,492.0428276062012,3.3164114833137674e-10
60980,253344,253344,506688,492.54049587249756,3.2797581429597196e-10
61049,253620,253620,507240,493.0433306694031,3.245656845621023e-10
61118,253896,253896,507792,493.5284585952759,3.2281506217124017e-10
61187,254172,254172,508344,494.01967573165894,3.220310093254724e-10
61256,254448,254448,508896,494.5144658088684,3.1884197138576544e-10
61324,254720,254720,509440,495.0015916824341,3.042496595896231e-10
61393,254996,254996,509992,495.49003767967224,2.927004177103194e-10
61462,255272,255272,510544,495.96612191200256,2.8274654535614354e-10
61531,255548,255548,511096,496.44346594810486,2.804031382962144e-10
61600,255824,255824,511648,496.93802070617676,2.7844219216384224e-10
61669,256100,256100,512200,497.4132149219513,2.769490876510157e-10
61738,256376,256376,512752,497.89046478271484,2.747621104548797e-10
61807,256652,256652,513304,498.38600873947144,2.729666385995145e-10
61876,256928,256928,513856,498.9699957370758,2.7016002141516247e-10
61945,257204,257204,514408,499.51196789741516,2.69227656832365e-10
62014,257480,257480,514960,500.0541708469391,2.6744046264434876e-10
62082,257752,257752,515504,500.80252385139465,2.6523191133971087e-10
62151,258028,258028,516056,501.7229688167572,2.6393112484655907e-10
62220,258304,258304,516608,502.47943663597107,2.5856504310634584e-10
62289,258580,258580,517160,503.22122287750244,2.537248183091794e-10
62358,258856,258856,517712,503.9189577102661,2.522494676317861e-10
62427,259132,259132,518264,504.69376277923584,2.5060146744524133e-10
62496,259408,259408,518816,505.524778842926,2.498404678682855e-10
62565,259684,259684,519368,506.0643389225006,2.488462635754402e-10
62634,259960,259960,519920,506.58583974838257,2.482948550664054e-10
62703,260236,260236,520472,507.14372301101685,2.4709904688209097e-10
62771,260508,260508,521016,507.65938997268677,2.4444524403324717e-10
62840,260784,260784,521568,508.1775028705597,2.4326808496734935e-10
62909,261066,261066,522132,508.6686007976532,2.425466558035443e-10
62978,261342,261342,522684,509.18668961524963,2.419505876936139e-10
63047,261618,261618,523236,509.6890687942505,2.3575229578570296e-10
63116,261894,261894,523788,510.17324686050415,2.1461180573021576e-10
63185,262170,262170,524340,510.756306886673,1.9304151199180117e-10
63254,262446,262446,524892,511.2682387828827,1.8088437156679454e-10
63323,262722,262722,525444,511.82204389572144,1.766901030847456e-10
63392,262998,262998,525996,512.3725688457489,1.741684346087916e-10
63460,263270,263270,526540,513.0307159423828,1.7231710035008167e-10
63529,263546,263546,527092,513.9497380256653,1.7179520100026706e-10
63598,263822,263822,527644,514.6980049610138,1.7101877979551166e-10
63667,264098,264098,528196,515.7242388725281,1.698854197321954e-10
63736,264374,264374,528748,516.3172118663788,1.690932236114274e-10
63805,264650,264650,529300,517.022935628891,1.6764941772676888e-10
63874,264926,264926,529852,517.5816698074341,1.6648122795054715e-10
63943,265202,265202,530404,518.1180427074432,1.6586327169393982e-10
64012,265478,265478,530956,518.6717267036438,1.653875516155829e-10
64081,265754,265754,531508,519.2091069221497,1.649361154940856e-10
64150,266030,266030,532060,519.6864326000214,1.6388943812181412e-10
64218,266302,266302,532604,520.1945128440857,1.6218259622741124e-10
64287,266578,266578,533156,520.7325546741486,1.6066443294340131e-10
64356,266860,266860,533720,521.2358138561249,1.5973169087759508e-10
64425,267136,267136,534272,521.7176818847656,1.589954583034215e-10
64494,267412,267412,534824,522.1926369667053,1.5833787228047472e-10
64563,267688,267688,535376,522.671924829483,1.5795621412644305e-10
64632,267964,267964,535928,523.1444900035858,1.5719342798120898e-10
64701,268240,268240,536480,523.6125688552856,1.5633984281397136e-10
64770,268516,268516,537032,524.0828688144684,1.5522308553145977e-10
64839,268792,268792,537584,524.5660598278046,1.5469470707214966e-10
64907,269064,269064,538128,525.0229017734528,1.520161726644774e-10
64976,269340,269340,538680,525.486359834671,1.50005655663295e-10
65045,269616,269616,539232,525.9544577598572,1.4878544838797851e-10
65114,269892,269892,539784,526.4184367656708,1.481324805534563e-10
65183,270168,270168,540336,526.8961689472198,1.4755017464257888e-10
65252,270444,270444,540888,527.3645639419556,1.4405700325441007e-10
65321,270720,270720,541440,527.8314018249512,1.4275413649421134e-10
65390,270996,270996,541992,528.2984838485718,1.4164171865121527e-10
65459,271272,271272,542544,528.7766499519348,1.4105748384033124e-10
65528,271548,271548,543096,529.2443447113037,1.3988642888721074e-10
65597,271824,271824,543648,529.7288167476654,1.3824004372225948e-10
65665,272096,272096,544192,530.1909618377686,1.3731836850350162e-10
65734,272372,272372,544744,530.6639575958252,1.3673878494525755e-10
65803,272648,272648,545296,531.1515200138092,1.3606897763888546e-10
65872,272924,272924,545848,531.6213598251343,1.3513833417353897e-10
65941,273200,273200,546400,532.1270477771759,1.3322453019151397e-10
66010,273476,273476,546952,532.5967717170715,1.324318620142513e-10
66079,273752,273752,547504,533.1554276943207,1.3167491503280417e-10
66148,274028,274028,548056,533.619256734848,1.3035256045626918e-10
66217,274304,274304,548608,534.0892457962036,1.2933991242322576e-10
66286,274584,274584,549168,534.5723190307617,1.2799011261741937e-10
66354,274856,274856,549712,535.0435497760773,1.2728112888312506e-10
66423,275136,275136,550272,535.5105228424072,1.269776531755683e-10
66492,275412,275412,550824,535.9746487140656,1.26421145656976e-10
66561,275692,275692,551384,536.4405319690704,1.2597204988395968e-10
66630,275968,275968,551936,536.9031617641449,1.2477907905988092e-10
66699,276244,276244,552488,537.3748910427094,1.2399733989265328e-10
66768,276526,276526,553052,537.83846783638,1.2338983220697375e-10
66837,276802,276802,553604,538.2951807975769,1.2197201198055995e-10
66906,277078,277078,554156,538.7535009384155,1.2038260833667676e-10
66975,277354,277354,554708,539.2265067100525,1.195087325645255e-10
67043,277626,277626,555252,539.6795477867126,1.1915446856584062e-10
67112,277906,277906,555812,540.1367428302765,1.187741625905155e-10
67181,278182,278182,556364,540.596314907074,1.1723731729754077e-10
67250,278458,278458,556916,541.0698897838593,1.154999271588429e-10
67319,278734,278734,557468,541.5575108528137,1.1472042723373715e-10
67388,279016,279016,558032,542.0201337337494,1.1428445457592594e-10
67457,279292,279292,558584,542.4806237220764,1.1331242104288649e-10
67526,279568,279568,559136,542.9377846717834,1.1289743507052338e-10
67595,279844,279844,559688,543.4648127555847,1.1171704892953853e-10
67664,280120,280120,560240,544.0069987773895,1.111684592854643e-10
67733,280402,280402,560804,544.4764888286591,1.1096222191644483e-10
67801,280674,280674,561348,544.9431238174438,1.1039537777245288e-10
67870,280950,280950,561900,545.4117226600647,1.0924609982447427e-10
67939,281226,281226,562452,545.887631893158,1.0858180731402792e-10
68008,281502,281502,563004,546.3442566394806,1.0822547397224536e-10
68077,281778,281778,563556,546.8071618080139,1.079871319874029e-10
68146,282054,282054,564108,547.2682816982269,1.0730173332750318e-10
68215,282330,282330,564660,547.747410774231,1.0624507559378357e-10
68284,282606,282606,565212,548.2082996368408,1.055458783174553e-10
68353,282882,282882,565764,548.6656148433685,1.0470220597095206e-10
68422,283160,283160,566320,549.1204307079315,1.0442834161857392e-10
68490,283432,283432,566864,549.5773546695709,1.040471683544823e-10
68559,283708,283708,567416,550.050568819046,1.031774351678362e-10
68628,283984,283984,567968,550.5103828907013,1.0278969528089088e-10
68697,284260,284260,568520,550.9760746955872,1.022504065337219e-10
68766,284536,284536,569072,551.4327816963196,1.0146044244333267e-10
68835,284812,284812,569624,551.9037749767303,9.999176189053676e-11


==> plot_data/cournot-nash_equilibrium_problem_n10/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00010609626770019531,542.5060889379029
1,2,1,3,0.0001800060272216797,1666.8595157418215
2,3,2,5,0.0002791881561279297,212.04506609322962
3,4,3,7,0.0003669261932373047,208.02515743800268
4,5,4,9,0.0004439353942871094,207.7222062763633
5,6,5,11,0.0005209445953369141,207.34277179873342
6,7,6,13,0.0005981922149658203,206.84290521249017
7,8,7,15,0.0006742477416992188,206.1892319518037
8,9,8,17,0.0007488727569580078,205.33901138860733
9,10,9,19,0.0008420944213867188,204.23758412764963
10,11,10,21,0.0009171962738037109,202.81140143857675
11,12,11,23,0.0009911060333251953,200.95450579700974
12,13,12,25,0.0010790824890136719,190.5833072731874
13,14,13,27,0.0011670589447021484,173.72377418324155
14,15,14,29,0.001260995864868164,136.19078373965837
15,16,15,31,0.0013451576232910156,118.81474962300322
16,17,16,33,0.0014200210571289062,109.35756653363543
17,18,17,35,0.0014920234680175781,101.88990671760939
18,19,18,37,0.00156402587890625,83.77465309915809
19,20,19,39,0.001634836196899414,64.42534268294193
20,21,20,41,0.0017139911651611328,104.37222934765423
21,22,21,43,0.0017931461334228516,101.36976725742844
22,23,22,45,0.001867055892944336,99.99904759544981
23,24,23,47,0.0019421577453613281,96.28131709773105
24,25,24,49,0.0020182132720947266,87.22735280279764
25,26,25,51,0.002095937728881836,74.55422130888289
26,27,26,53,0.002179861068725586,67.86856403317122
27,28,27,55,0.002254962921142578,62.615958866200494
28,29,28,57,0.002334117889404297,57.66956515369755
29,30,29,59,0.0024149417877197266,32.90945641911591
30,31,30,61,0.0024971961975097656,23.454309436355246
31,32,31,63,0.0025739669799804688,20.437308297240886
32,33,32,65,0.0026519298553466797,57.448985024460804
33,34,33,67,0.0027370452880859375,54.613111909715435
34,35,34,69,0.003016948699951172,46.25721483909821
35,36,35,71,0.0031561851501464844,31.223228971632597
36,37,36,73,0.0032410621643066406,22.77614557805692
37,38,37,75,0.003332853317260742,21.114003593365613
38,39,38,77,0.003422975540161133,20.333008467508023
39,40,39,79,0.0035080909729003906,18.545482068492177
40,41,40,81,0.003583192825317383,19.205731691748937
41,42,41,83,0.0036780834197998047,21.800668450989452
42,43,42,85,0.003756999969482422,20.59523896400334
43,44,43,87,0.0038559436798095703,20.27162333362212
44,45,44,89,0.003936052322387695,19.87235261102326
45,46,45,91,0.0040090084075927734,19.36479376411522
46,47,46,93,0.0040819644927978516,18.726909025896465
47,48,47,95,0.0041501522064208984,17.9278866294255
48,49,48,97,0.004216909408569336,16.93171534501472
49,50,49,99,0.004287004470825195,15.701470612309878
50,51,50,101,0.004355907440185547,14.211645468360668
51,52,51,103,0.004431962966918945,12.465460593844128
52,53,52,105,0.00450587272644043,10.511389352088857
53,54,53,107,0.0045871734619140625,1.7211274189739494
54,55,54,109,0.004663228988647461,13.409862321788362
55,56,55,111,0.004744052886962891,13.261033243488574
56,57,56,113,0.004832029342651367,13.101052378815252
57,58,57,115,0.004915952682495117,12.893022357079781
58,59,58,117,0.004987001419067383,12.621522133724758
59,60,59,119,0.00506901741027832,12.26981008562788
60,61,60,121,0.005136966705322266,11.817341880620468
61,62,61,123,0.005208015441894531,11.240697323316205
62,63,62,125,0.005282163619995117,10.516038812929267
63,64,63,127,0.005349874496459961,3.7552435128580517
64,65,64,129,0.005421876907348633,5.57147963843948
65,66,65,131,0.0055179595947265625,10.96018639854843
66,67,66,133,0.005594015121459961,10.840636348115629
67,68,67,135,0.005667924880981445,10.695918238775139
68,69,68,137,0.005740165710449219,10.504936917837286
69,70,69,139,0.005813121795654297,7.199799799741188
70,71,70,141,0.005911111831665039,4.487726592521903
71,72,71,143,0.00598907470703125,3.688164992125455
72,73,72,145,0.006069183349609375,4.320356014092189
73,74,73,147,0.006140947341918945,4.360248496573518
74,75,74,149,0.006208181381225586,3.8968584235025916
75,76,75,151,0.006273031234741211,3.468219253691397
76,77,76,153,0.006340980529785156,2.990009095731937
77,78,77,155,0.006418943405151367,2.962873458996724
78,79,78,157,0.006487131118774414,2.3753487940119666
79,80,79,159,0.006557941436767578,2.865995402235806
80,81,80,161,0.006628990173339844,2.866574414279671
81,82,81,163,0.006696939468383789,2.619809814425414
82,83,82,165,0.006767988204956055,2.383789273815374
83,84,83,167,0.0068361759185791016,2.1230130384215866
84,85,84,169,0.0069119930267333984,1.8667149821866529
85,86,85,171,0.006989955902099609,1.751478605161731
86,87,86,173,0.007061004638671875,1.4579937912974015
87,88,87,175,0.007130861282348633,1.7616632136774035
88,89,88,177,0.0072021484375,1.837179899096737
89,90,89,179,0.007277011871337891,1.7291257191052187
90,91,90,181,0.007361173629760742,1.6280666626242182
91,92,91,183,0.0074310302734375,1.5112045357337265
92,93,92,185,0.007500886917114258,1.3883647028450417
93,94,93,187,0.007590055465698242,1.2599593870423642
94,95,94,189,0.007659196853637695,1.1274955695667603
95,96,95,191,0.007739067077636719,0.9880639853401243
96,97,96,193,0.007822990417480469,0.8413783323350533
97,98,97,195,0.007910966873168945,0.687962221332964
98,99,98,197,0.007999181747436523,0.5395601916345821
99,100,99,199,0.008083105087280273,0.4625369651120378
100,101,100,201,0.008170127868652344,0.7269251982224049
101,102,101,203,0.008257150650024414,0.664492000806044
102,103,102,205,0.008345842361450195,0.7577753109921761
103,104,103,207,0.008428096771240234,0.7415084039049615
104,105,104,209,0.008580923080444336,0.7277222846502204
105,106,105,211,0.008759021759033203,0.7093116539132149
106,107,106,213,0.008855104446411133,0.686179362531918
107,108,107,215,0.008945941925048828,0.6572566916786748
108,109,108,217,0.009020090103149414,0.6216007993481891
109,110,109,219,0.009109020233154297,0.5782186904318322
110,111,110,221,0.009183168411254883,0.526348092122027
111,112,111,223,0.00925302505493164,0.4658336157007213
112,113,112,225,0.009322166442871094,0.39778457548894974
113,114,113,227,0.009398221969604492,0.3250762814288778
114,115,114,229,0.009472131729125977,0.25253927821215855
115,116,115,231,0.009544134140014648,0.24041401841370916
116,117,116,233,0.009612798690795898,0.2863212880977248
117,118,117,235,0.00968313217163086,0.2165316446378098
118,119,118,237,0.009756088256835938,0.17979442894387035
119,120,119,239,0.00982522964477539,0.16351842298707808
120,121,120,241,0.009896039962768555,0.2479137578322988
121,122,121,243,0.009985923767089844,0.22470004887022174
122,123,122,245,0.010079145431518555,0.21040072385079667
123,124,123,247,0.010159015655517578,0.18838602562963638
124,125,124,249,0.010239124298095703,0.168426596033924
125,126,125,251,0.010316133499145508,0.17145306047624642
126,127,126,253,0.010389089584350586,0.20131516537925237
127,128,127,255,0.010464191436767578,0.19881260928861033
128,129,128,257,0.010538101196289062,0.19629156814808013
129,130,129,259,0.010629892349243164,0.19291485516129822
130,131,130,261,0.010701894760131836,0.18847694705905652
131,132,131,263,0.010773181915283203,0.18268460709196543
132,133,132,265,0.010843992233276367,0.17520883353197814
133,134,133,267,0.010917901992797852,0.16570092871565592
134,135,134,269,0.010992050170898438,0.15384454883457147
135,136,135,271,0.011063098907470703,0.13944263927869235
136,137,136,273,0.011135101318359375,0.12254826985949148
137,138,137,275,0.011205911636352539,0.10361831645411673
138,139,138,277,0.011277914047241211,0.0836296964069761
139,140,139,279,0.01135706901550293,0.06403008568008774
140,141,140,281,0.011451005935668945,0.07062433944522667
141,142,141,283,0.011530160903930664,0.06836576364699194
142,143,142,285,0.011600971221923828,0.05929383906538298
143,144,143,287,0.011673927307128906,0.0460330027563537
144,145,144,289,0.011766195297241211,0.05125827638724003
145,146,145,291,0.011867046356201172,0.07037767842949123
146,147,146,293,0.011938810348510742,0.06999007477387297
147,148,147,295,0.01201009750366211,0.06957186347885545
148,149,148,297,0.012076139450073242,0.06901552860894748
149,150,149,299,0.012153863906860352,0.06827464754107815
150,151,150,301,0.012225151062011719,0.06729228745111673
151,152,151,303,0.012300968170166016,0.06599665559635107
152,153,152,305,0.01237797737121582,0.06429985545818902
153,154,153,307,0.012454032897949219,0.062098195782455866
154,155,154,309,0.01252603530883789,0.05927615507416558
155,156,155,311,0.012600898742675781,0.05571680148863984
156,157,156,313,0.012673139572143555,0.051322490230029494
157,158,157,315,0.012750864028930664,0.04604963931845398
158,159,158,317,0.01282811164855957,0.039957876797503684
159,160,159,319,0.012903928756713867,0.03326288292512263
160,161,160,321,0.01298379898071289,0.026363155428263205
161,162,161,323,0.013064146041870117,0.021086785067088335
162,163,162,325,0.013138055801391602,0.024851665154871378
163,164,163,327,0.013224124908447266,0.02271142048029854
164,165,164,329,0.013309001922607422,0.0171468959459445
165,166,165,331,0.013392925262451172,0.014752841015747685
166,167,166,333,0.01347208023071289,0.019733236772055608
167,168,167,335,0.013555049896240234,0.01930569211686666
168,169,168,337,0.013635873794555664,0.022597443252298063
169,170,169,339,0.013717174530029297,0.022462986386180425
170,171,170,341,0.013788938522338867,0.022323373805563432
171,172,171,343,0.01386404037475586,0.022135892842769678
172,173,172,345,0.013936996459960938,0.021886121626525347
173,174,173,347,0.014019012451171875,0.021554587423748415
174,175,174,349,0.01409006118774414,0.021116844687140167
175,176,175,351,0.014158964157104492,0.020542964490837003
176,177,176,353,0.014230012893676758,0.019797797392129658
177,178,177,355,0.014301061630249023,0.018842669208736083
178,179,178,357,0.014371871948242188,0.01763958448477015
179,180,179,359,0.01444697380065918,0.01615922353689769
180,181,180,361,0.014519214630126953,0.01439368318303452
181,182,181,363,0.01459503173828125,0.012373229811791933
182,183,182,365,0.01466822624206543,0.010182366541901296
183,184,183,367,0.014741182327270508,0.007964192748299327
184,185,184,369,0.014814138412475586,0.007382265803966273
185,186,185,371,0.014887094497680664,0.007816810335025627
186,187,186,373,0.014956235885620117,0.006841316673029504
187,188,187,375,0.015043020248413086,0.005147661044628372
188,189,188,377,0.015127182006835938,0.005426660908576986
189,190,189,379,0.015214920043945312,0.007882892643287159
190,191,190,381,0.015304088592529297,0.0076619617344173396
191,192,191,383,0.015382051467895508,0.007473741322714033
192,193,192,385,0.015456199645996094,0.007222047148729345
193,194,193,387,0.015533924102783203,0.00689946497721021
194,195,194,389,0.015614986419677734,0.006490237746161834
195,196,195,391,0.01569390296936035,0.005983487638855283
196,197,196,393,0.01577305793762207,0.005372844074292427
197,198,197,395,0.0158538818359375,0.0046661423407632265
198,199,198,397,0.01593780517578125,0.0038859038494895863
199,200,199,399,0.016019105911254883,0.003085935477811096
200,201,200,401,0.016103029251098633,0.002591964705444328
201,202,201,403,0.016185998916625977,0.0031526820098663807
202,203,202,405,0.01625800132751465,0.003758116022331218
203,204,203,407,0.016332149505615234,0.0034987043294671346
204,205,204,409,0.016405105590820312,0.003185740193549921
205,206,205,411,0.016482830047607422,0.002919467514590297
206,207,206,413,0.016561031341552734,0.002966160174863141
207,208,207,415,0.016640186309814453,0.003337094630019871
208,209,208,417,0.016723155975341797,0.003282451287028511
209,210,209,419,0.016798973083496094,0.003225468601615311
210,211,210,421,0.016885042190551758,0.0031492863271203827
211,212,211,423,0.01696610450744629,0.003050104826039938
212,213,212,425,0.017045021057128906,0.0029220392828241165
213,214,213,427,0.017121076583862305,0.002759277765343828
214,215,214,429,0.01720404624938965,0.0025564950270562815
215,216,215,431,0.01727914810180664,0.0023106481638622677
216,217,216,433,0.01735520362854004,0.0020230727295785455
217,218,217,435,0.01743006706237793,0.0017023599483190484
218,219,218,437,0.017504215240478516,0.001365684601311561
219,220,219,439,0.017575979232788086,0.0010392881823125175
220,221,220,441,0.017650127410888672,0.0012283550337118029
221,222,221,443,0.017724037170410156,0.0012237679098390476
222,223,222,445,0.01779317855834961,0.0015988968799219663
223,224,223,447,0.017863988876342773,0.0015847346362420991
224,225,224,449,0.01793694496154785,0.0015701939522313703
225,226,225,451,0.01800990104675293,0.0015508160537717342
226,227,226,453,0.018085956573486328,0.0015251379772172286
227,228,227,455,0.018156051635742188,0.0014913127518086692
228,229,228,457,0.018234968185424805,0.0014471023890910845
229,230,229,459,0.018306970596313477,0.001389923341716876
230,231,230,461,0.018398046493530273,0.001317008090359222
231,232,231,463,0.018477916717529297,0.001225768972332609
232,233,232,465,0.018629074096679688,0.0011144548171447295
233,234,233,467,0.018732070922851562,0.000983152444820352
234,235,234,469,0.01881718635559082,0.0008350249759892974
235,236,235,471,0.018900156021118164,0.000677331301625878
236,237,236,473,0.01898193359375,0.0005212974684618184
237,238,237,475,0.019067049026489258,0.0005589212132141582
238,239,238,477,0.019150972366333008,0.0005459505598027518
239,240,239,479,0.019234180450439453,0.00044763544556626427
240,241,240,481,0.019318103790283203,0.0003547760984369796
241,242,241,483,0.019401073455810547,0.0003667649691736517
242,243,242,485,0.01947617530822754,0.000549058616030713
243,244,243,487,0.01955413818359375,0.0005444289216806876
244,245,244,489,0.019633054733276367,0.0005400340524011891
245,246,245,491,0.019717931747436523,0.0005341719868895568
246,247,246,493,0.01980304718017578,0.0005263900135027435
247,248,247,495,0.019877910614013672,0.0005161144207033198
248,249,248,497,0.019952058792114258,0.0005026396642898976
249,250,249,499,0.020032167434692383,0.0004851329476626917
250,251,250,501,0.020115137100219727,0.0004626681207309647
251,252,251,503,0.02018904685974121,0.00043431478963227134
252,253,252,505,0.02025890350341797,0.0003993131005613359
253,254,253,507,0.020334959030151367,0.0003573622686260982
254,255,254,509,0.020419836044311523,0.0003090186130530489
255,256,255,511,0.020503997802734375,0.00025610915276333423
256,257,256,513,0.020588159561157227,0.0002019132926007696
257,258,257,515,0.02068305015563965,0.00017450694568841186
258,259,258,517,0.020773887634277344,0.00019436813560974925
259,260,259,519,0.020860910415649414,0.00017604355145553246
260,261,260,521,0.020940065383911133,0.0001335294456189907
261,262,261,523,0.021021127700805664,0.00011398072412582067
262,263,262,525,0.021095991134643555,0.0001644532914452953
263,264,263,527,0.021168947219848633,0.0001489811224609695
264,265,264,529,0.021240949630737305,0.00015677161528193623
265,266,265,531,0.021320104598999023,0.00016405516917176557
266,267,266,533,0.021400928497314453,0.00015675169416871383
267,268,267,535,0.021494150161743164,0.00014952884451548338
268,269,268,537,0.021574020385742188,0.00013963200366948195
269,270,269,539,0.021663188934326172,0.000128095014206235
270,271,270,541,0.0217440128326416,0.00011362725173365497
271,272,271,543,0.021837949752807617,9.8410865403169e-05
272,273,272,545,0.0219271183013916,7.987083376213825e-05
273,274,273,547,0.02202296257019043,0.00010222847510153164
274,275,274,549,0.02211904525756836,0.00010700553941139655
275,276,275,551,0.022207021713256836,0.00010688143675687707
276,277,276,553,0.022296905517578125,0.00010493296313880637
277,278,277,555,0.02237701416015625,0.00010142895960917406
278,279,278,557,0.02245306968688965,9.681389132894115e-05
279,280,279,559,0.02252984046936035,9.106882193263568e-05
280,281,280,561,0.02260899543762207,8.389244888001287e-05
281,282,281,563,0.022684097290039062,7.533544311373369e-05
282,283,282,565,0.022754192352294922,6.532271703403199e-05
283,284,283,567,0.022821903228759766,5.4552639106991297e-05
284,285,284,569,0.022890090942382812,4.282568974293239e-05
285,286,285,571,0.02295994758605957,4.7055893780206465e-05
286,287,286,573,0.023029088973999023,6.39266005227027e-05
287,288,287,575,0.02309703826904297,6.370754650793207e-05
288,289,288,577,0.023164987564086914,6.345640450467803e-05
289,290,289,579,0.023234844207763672,6.31215172638044e-05
290,291,290,581,0.023308992385864258,6.267399039722037e-05
291,292,291,583,0.02338385581970215,6.207773816515656e-05
292,293,292,585,0.023463010787963867,6.128629183457477e-05
293,294,293,587,0.023543119430541992,6.024088991138827e-05
294,295,294,589,0.02362203598022461,5.8868857026007636e-05
295,296,295,591,0.0236968994140625,5.708308143613754e-05
296,297,296,593,0.02376413345336914,5.4783846627794496e-05
297,298,297,595,0.02383708953857422,5.1865074575106045e-05
298,299,298,597,0.023906230926513672,4.82280528850719e-05
299,300,299,599,0.02397608757019043,4.3806507880524136e-05
300,301,300,601,0.02404308319091797,3.8605772019052284e-05
301,302,301,603,0.024108171463012695,3.275218925397876e-05
302,303,302,605,0.024178028106689453,2.6533584141225033e-05
303,304,303,607,0.024253129959106445,2.039366703711251e-05
304,305,304,609,0.024321794509887695,2.2109622842606254e-05
305,306,305,611,0.024389028549194336,2.1096923104176122e-05
306,307,306,613,0.024466991424560547,2.0586026768461124e-05
307,308,307,615,0.024543046951293945,2.634409054155125e-05
308,309,308,617,0.024621963500976562,2.5026196672696643e-05
309,310,309,619,0.024738073348999023,2.3759712628610043e-05
310,311,310,621,0.02482008934020996,2.2176657077480136e-05
311,312,311,623,0.024903059005737305,2.0210057683450215e-05
312,313,312,625,0.024983882904052734,1.7921974835530702e-05
313,314,313,627,0.025070905685424805,1.5253337074545635e-05
314,315,314,629,0.025175809860229492,1.2606707196632908e-05
315,316,315,631,0.02526712417602539,1.2332092437718158e-05
316,317,316,633,0.025345802307128906,1.722337405938138e-05
317,318,317,635,0.02544999122619629,1.713165138502278e-05
318,319,318,637,0.02556300163269043,1.7049672927066865e-05
319,320,319,639,0.025668859481811523,1.693930211329276e-05
320,321,320,641,0.02577996253967285,1.6791832595320148e-05
321,322,321,643,0.025880813598632812,1.6595336238261327e-05
322,323,322,645,0.02596902847290039,1.6334548615953898e-05
323,324,323,647,0.026058197021484375,1.5990281433908304e-05
324,325,324,649,0.026135921478271484,1.5539101364583402e-05
325,326,325,651,0.026211977005004883,1.4953610446405971e-05
326,327,326,653,0.02628302574157715,1.4203937486792851e-05
327,328,327,655,0.0263519287109375,1.3261313344338953e-05
328,329,328,657,0.026441097259521484,1.2104733532399194e-05
329,330,329,659,0.026517152786254883,1.0731306455729167e-05
330,331,330,661,0.026588916778564453,9.169373058883452e-06
331,332,331,663,0.026660919189453125,7.490231938856399e-06
332,333,332,665,0.026731014251708984,5.8092393565527265e-06
333,334,333,667,0.026803970336914062,5.889851101478503e-06
334,335,334,669,0.02688288688659668,6.4361928364806016e-06
335,336,335,671,0.026955127716064453,4.785509397114417e-06
336,337,336,673,0.02702808380126953,3.961371894218908e-06
337,338,337,675,0.02709794044494629,5.096463217136462e-06
338,339,338,677,0.027174949645996094,5.578598244009184e-06
339,340,339,679,0.02724480628967285,5.852375065008761e-06
340,341,340,681,0.027313947677612305,5.687510238724106e-06
341,342,341,683,0.027383089065551758,5.468490344797307e-06
342,343,342,685,0.027476072311401367,5.200009309982704e-06
343,344,343,687,0.027565956115722656,4.855150496010245e-06
344,345,344,689,0.027659177780151367,4.438363823713637e-06
345,346,345,691,0.02774214744567871,3.935427149315263e-06
346,347,346,693,0.027816057205200195,3.3765662399994337e-06
347,348,347,695,0.027888059616088867,2.74344554252618e-06
348,349,348,697,0.027956008911132812,2.3207120960021382e-06
349,350,349,699,0.02803206443786621,3.45257823852768e-06
350,351,350,701,0.02810811996459961,3.229726353593783e-06
351,352,351,703,0.028181076049804688,2.974636945381511e-06
352,353,352,705,0.028250932693481445,2.7624786820855548e-06
353,354,353,707,0.028358936309814453,2.5055054551571225e-06
354,355,354,709,0.0284271240234375,2.844857549735781e-06
355,356,355,711,0.02849602699279785,2.621395517242284e-06
356,357,356,713,0.028649091720581055,2.463361431063036e-06
357,358,357,715,0.02873396873474121,2.2001654750612353e-06
358,359,358,717,0.028812885284423828,1.9992413594752266e-06
359,360,359,719,0.028936147689819336,2.195593647176598e-06
360,361,360,721,0.02903294563293457,2.2478609177920356e-06
361,362,361,723,0.0291290283203125,2.321982450097876e-06
362,363,362,725,0.029228925704956055,2.2844723528792943e-06
363,364,363,727,0.02931499481201172,2.2355914461851397e-06
364,365,364,729,0.029397010803222656,2.1721205557707293e-06
365,366,365,731,0.029475927352905273,2.089756162630882e-06
366,367,366,733,0.02955913543701172,1.9845790481919176e-06
367,368,367,735,0.02963113784790039,1.8525525007429005e-06
368,369,368,737,0.029695987701416016,1.6908557834962112e-06
369,370,369,739,0.029764890670776367,1.4990177877442895e-06
370,371,370,741,0.0298309326171875,1.2810491079634126e-06
371,372,371,743,0.029900074005126953,1.046572344601988e-06
372,373,372,745,0.029968976974487305,8.12461790515587e-07
373,374,373,747,0.030035018920898438,8.264169336341189e-07
374,375,374,749,0.030102014541625977,1.1847776694199893e-06
375,376,375,751,0.030167818069458008,1.0912427654542998e-06
376,377,376,753,0.030236005783081055,1.0193820679509448e-06
377,378,377,755,0.0303041934967041,9.245568683160205e-07
378,379,378,757,0.03037095069885254,8.170688706794758e-07
379,380,379,759,0.030440092086791992,6.893147063596336e-07
380,381,380,761,0.030508041381835938,5.776930418620683e-07
381,382,381,763,0.03057694435119629,7.316230671012965e-07
382,383,382,765,0.030668020248413086,7.544259296603818e-07
383,384,383,767,0.03075098991394043,8.005587310871629e-07
384,385,384,769,0.030828237533569336,7.930980269044938e-07
385,386,385,771,0.03097701072692871,7.832714799190624e-07
386,387,386,773,0.031095027923583984,7.70339032055037e-07
387,388,387,775,0.031211137771606445,7.532906677296758e-07
388,389,388,777,0.03131818771362305,7.310147496375663e-07
389,390,389,779,0.03142213821411133,7.022071462504639e-07
390,391,390,781,0.03153800964355469,6.654742080229828e-07
391,392,391,783,0.031655073165893555,6.195073144393044e-07
392,393,392,785,0.03175997734069824,5.634137052141592e-07
393,394,393,787,0.031854867935180664,4.972180192010728e-07
394,395,394,789,0.031941890716552734,4.224918815823644e-07
395,396,395,791,0.0320279598236084,3.4287166762537767e-07
396,397,396,793,0.03210711479187012,2.6402109947696565e-07
397,398,397,795,0.03217506408691406,2.8369072228559563e-07
398,399,398,797,0.032243967056274414,2.769966028396949e-07
399,400,399,799,0.032328128814697266,2.257160510630308e-07
400,401,400,801,0.03240203857421875,1.79390289502608e-07
401,402,401,803,0.03253507614135742,1.8701649900054167e-07
402,403,402,805,0.03260922431945801,2.7242205637549266e-07
403,404,403,807,0.032752037048339844,2.636201755363454e-07
404,405,404,809,0.03284788131713867,2.5556026232912507e-07
405,406,405,811,0.032930850982666016,2.451331086077341e-07
406,407,406,813,0.033010005950927734,2.3181185997220735e-07
407,408,407,815,0.03308916091918945,2.152311162426964e-07
408,409,408,817,0.03316903114318848,1.9503753365301479e-07
409,410,409,819,0.03324294090270996,1.7138156099914433e-07
410,411,410,821,0.033316850662231445,1.447541937792651e-07
411,412,411,823,0.03339195251464844,1.1692359740969683e-07
412,413,412,825,0.0334780216217041,8.86915409874495e-08
413,414,413,827,0.03355002403259277,1.0862881574639176e-07
414,415,414,829,0.03362107276916504,1.421035774799367e-07
415,416,415,831,0.033689022064208984,1.380360444917253e-07
416,417,416,833,0.03375816345214844,1.3339631238941687e-07
417,418,417,835,0.03382682800292969,1.2776216384478133e-07
418,419,418,837,0.03389406204223633,1.204427491933262e-07
419,420,419,839,0.03396320343017578,1.1148471667684191e-07
420,421,420,841,0.034034013748168945,1.0053750886971714e-07
421,422,421,843,0.0341038703918457,8.795079485227783e-08
422,423,422,845,0.03418087959289551,7.360962396267747e-08
423,424,423,847,0.034253835678100586,5.985606753354997e-08
424,425,424,849,0.03432798385620117,6.714087736621095e-08
425,426,425,851,0.03440594673156738,8.489666430933948e-08
426,427,426,853,0.034484148025512695,8.189915813514593e-08
427,428,427,855,0.03456282615661621,7.942319159233574e-08
428,429,428,857,0.03463315963745117,7.600180725535225e-08
429,430,429,859,0.03470182418823242,7.17478210456023e-08
430,431,430,861,0.034770965576171875,6.638737699617803e-08
431,432,431,863,0.03483986854553223,5.995706838785387e-08
432,433,432,865,0.034912109375,5.2355689216707066e-08
433,434,433,867,0.034986019134521484,4.409191473267053e-08
434,435,434,869,0.03506302833557129,3.4968821775496634e-08
435,436,435,871,0.0351409912109375,3.435488109330986e-08
436,437,436,873,0.03521585464477539,4.957058915868285e-08
437,438,437,875,0.03528904914855957,4.892424705507414e-08
438,439,438,877,0.03535914421081543,4.8213208102145275e-08
439,440,439,879,0.03542804718017578,4.729591487503236e-08
440,441,440,881,0.03550004959106445,4.6090550299828674e-08
441,442,441,883,0.0355830192565918,4.452799364823933e-08
442,443,442,885,0.035661935806274414,4.2524817605431294e-08
443,444,443,887,0.03574204444885254,3.999784216814137e-08
444,445,444,889,0.03582191467285156,3.6875438166605635e-08
445,446,445,891,0.03589892387390137,3.3123524173485615e-08
446,447,446,893,0.03597903251647949,2.8779528689903044e-08
447,448,447,895,0.036054134368896484,2.3992806852752408e-08
448,449,448,897,0.0361180305480957,1.9043206981874968e-08
449,450,449,899,0.036202192306518555,1.5365137676366465e-08
450,451,450,901,0.03627204895019531,1.8045725150593875e-08
451,452,451,903,0.03635096549987793,1.6783975465686262e-08
452,453,452,905,0.0364229679107666,1.4844414065158843e-08
453,454,453,907,0.036496877670288086,1.2113289553451002e-08
454,455,454,909,0.036570072174072266,1.656605077343612e-08
455,456,455,911,0.036643028259277344,1.626423773586727e-08
456,457,456,913,0.03671622276306152,1.7262547308387873e-08
457,458,457,915,0.036812782287597656,1.6927151416820445e-08
458,459,458,917,0.03688406944274902,1.647746000456257e-08
459,460,459,919,0.03695487976074219,1.5908847568206828e-08
460,461,460,921,0.037023067474365234,1.5173614541431305e-08
461,462,461,923,0.03709816932678223,1.424924188867324e-08
462,463,462,925,0.03720712661743164,1.3105873740899538e-08
463,464,463,927,0.03730607032775879,1.1737704577291375e-08
464,465,464,929,0.03738093376159668,1.0155798935548254e-08
465,466,465,931,0.03747892379760742,8.43158995282325e-09
466,467,466,933,0.03761601448059082,6.634532699740784e-09
467,468,467,935,0.03771805763244629,5.613964814693456e-09
468,469,468,937,0.03781318664550781,8.612929793321277e-09
469,470,469,939,0.037919044494628906,7.486632225590422e-09
470,471,470,941,0.0380251407623291,6.530364639418519e-09
471,472,471,943,0.038178205490112305,7.937071236417938e-09
472,473,472,945,0.0383760929107666,7.38646905831857e-09
473,474,473,947,0.03846406936645508,7.034562008968805e-09
474,475,474,949,0.03854084014892578,6.448150693565756e-09
475,476,475,951,0.03873491287231445,5.88911818397361e-09
476,477,476,953,0.03883719444274902,5.053678089990798e-09
477,478,477,955,0.03894209861755371,5.458840237413302e-09
478,479,478,957,0.03902101516723633,6.234186309794356e-09
479,480,479,959,0.039093017578125,6.183821799953213e-09
480,481,480,961,0.03917288780212402,6.118635078102181e-09
481,482,481,963,0.039244890213012695,6.032941275172608e-09
482,483,482,965,0.039314985275268555,5.919741553276812e-09
483,484,483,967,0.03939008712768555,5.771079600367884e-09
484,485,484,969,0.039457082748413086,5.57778589643932e-09
485,486,485,971,0.03952503204345703,5.3294811877229e-09
486,487,486,973,0.03959512710571289,5.015369293724071e-09
487,488,487,975,0.039662837982177734,4.6263599613798745e-09
488,489,488,977,0.039733171463012695,4.15804599637651e-09
489,490,489,979,0.03979992866516113,3.6149758464461275e-09
490,491,490,981,0.03986692428588867,3.015682847893983e-09
491,492,491,983,0.03993105888366699,2.3955204506006946e-09
492,493,492,985,0.03999590873718262,1.9294805038623023e-09
493,494,493,987,0.04006004333496094,2.2523969795889677e-09
494,495,494,989,0.040125131607055664,2.0494148728259296e-09
495,496,495,991,0.040193796157836914,1.5556632936622797e-09
496,497,496,993,0.04026198387145996,1.528356713059957e-09
497,498,497,995,0.04032588005065918,2.3128210870254084e-09
498,499,498,997,0.04041004180908203,2.3023176304331676e-09
499,500,499,999,0.04047703742980957,2.293298209049469e-09
500,501,500,1001,0.04054403305053711,2.280948736198089e-09
501,502,501,1003,0.04061102867126465,2.264571149235163e-09
502,503,502,1005,0.04067707061767578,2.242597126470766e-09
503,504,503,1007,0.040740013122558594,2.2135082092616518e-09
504,505,504,1009,0.04081106185913086,2.174832475906895e-09
505,506,505,1011,0.04087686538696289,2.1239257176940385e-09
506,507,506,1013,0.040946006774902344,2.0575197179438285e-09
507,508,507,1015,0.04102301597595215,1.9716793218240915e-09
508,509,508,1017,0.041097164154052734,1.8623987259289231e-09
509,510,509,1019,0.04117012023925781,1.7261217840117508e-09
510,511,510,1021,0.041236162185668945,1.5605590888249127e-09
511,512,511,1023,0.04130697250366211,1.366837803567545e-09
512,513,512,1025,0.04137396812438965,1.1504472480059875e-09
513,514,513,1027,0.041442155838012695,9.234773737215119e-10
514,515,514,1029,0.041506052017211914,7.017111196639038e-10
515,516,515,1031,0.04157614707946777,8.239718845634621e-10
516,517,516,1033,0.041654109954833984,7.656643308531208e-10
517,518,517,1035,0.04172992706298828,9.989066288617897e-10
518,519,518,1037,0.04180479049682617,9.155920296240036e-10
519,520,519,1039,0.04187512397766113,8.54103465877821e-10
520,521,520,1041,0.041970014572143555,7.648832740097262e-10
521,522,521,1043,0.04206490516662598,6.795719942436703e-10
522,523,522,1045,0.04213404655456543,6.139722293149492e-10
523,524,523,1047,0.04220294952392578,7.817061952699347e-10
524,525,524,1049,0.04227113723754883,7.486708726516493e-10
525,526,525,1051,0.04234004020690918,7.221798936971286e-10
526,527,526,1053,0.04241013526916504,6.850284036624972e-10
527,528,527,1055,0.04249405860900879,6.400468715448851e-10
528,529,528,1057,0.04257798194885254,5.834176030921633e-10
529,530,529,1059,0.04264998435974121,5.180526342009666e-10
530,531,530,1061,0.04273390769958496,4.40664577633904e-10
531,532,531,1063,0.04281306266784668,3.675633171781986e-10
532,533,532,1065,0.042945146560668945,4.203877259719344e-10
533,534,533,1067,0.043035030364990234,4.947163003891985e-10
534,535,534,1069,0.043109893798828125,4.733008917502649e-10
535,536,535,1071,0.04318094253540039,4.552046455132722e-10
536,537,536,1073,0.0432741641998291,4.2978978370695876e-10
537,538,537,1075,0.0433502197265625,3.9949435451408675e-10
538,539,538,1077,0.04342317581176758,3.611701283332229e-10
539,540,539,1079,0.043496131896972656,3.1830433647107326e-10
540,541,540,1081,0.04357504844665527,2.664770467686392e-10
541,542,541,1083,0.043660879135131836,2.294269537083464e-10
542,543,542,1085,0.043734073638916016,3.1220610842998927e-10
543,544,543,1087,0.04380512237548828,2.909540995603016e-10
544,545,544,1089,0.043879032135009766,2.641238861997499e-10
545,546,545,1091,0.04395914077758789,2.578145532115048e-10
546,547,546,1093,0.04404497146606445,2.8292842106717354e-10
547,548,547,1095,0.044129133224487305,2.749477395597132e-10
548,549,548,1097,0.04420113563537598,2.647713716412269e-10
549,550,549,1099,0.044445037841796875,2.522782038657e-10
550,551,550,1101,0.044548988342285156,2.3622875426061366e-10
551,552,551,1103,0.04463005065917969,2.167500697898633e-10
552,553,552,1105,0.044708967208862305,1.9311400696944083e-10
553,554,553,1107,0.044786930084228516,1.6661820849717503e-10
554,555,554,1109,0.044862985610961914,1.3662290704227962e-10
555,556,555,1111,0.044931888580322266,1.1255252923000918e-10
556,557,556,1113,0.045004844665527344,1.6111117245439242e-10
557,558,557,1115,0.04507613182067871,1.5149321385370566e-10
558,559,558,1117,0.04514789581298828,1.5219391262085882e-10
559,560,559,1119,0.04521894454956055,1.604437358230849e-10
560,561,560,1121,0.04528999328613281,1.565684615178189e-10
561,562,561,1123,0.04535794258117676,1.524624852662434e-10
562,563,562,1125,0.045456886291503906,1.4686183209281416e-10
563,564,563,1127,0.04553103446960449,1.3977480334307464e-10
564,565,564,1129,0.04561209678649902,1.308201379789687e-10
565,566,565,1131,0.0456850528717041,1.1982586473070732e-10
566,567,566,1133,0.04575181007385254,1.0673744502651324e-10
567,568,567,1135,0.04582095146179199,9.168593581113906e-11


==> plot_data/cournot-nash_equilibrium_problem_n10/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0001227855682373047,542.5060889379029
1,3,2,5,0.000308990478515625,409.6353395028631
2,5,4,9,0.0004279613494873047,294.6291701407307
3,7,6,13,0.0005319118499755859,197.24353095956113
4,9,8,17,0.0006310939788818359,131.75231590331154
5,11,10,21,0.0007450580596923828,85.91880628167098
6,13,12,25,0.0008530616760253906,65.03254300872524
7,15,14,29,0.0009658336639404297,41.285630953207175
8,17,16,33,0.001065969467163086,708.9286288511969
9,19,18,37,0.0016109943389892578,90.74981504690473
10,21,20,41,0.0017349720001220703,343.97713763941863
11,23,22,45,0.0018351078033447266,67.42351124787656
12,25,24,49,0.001920938491821289,2.926531869696776
13,27,26,53,0.002023935317993164,0.8458899526752867
14,29,28,57,0.002123117446899414,0.40033047553612555
15,31,30,61,0.0022368431091308594,0.23949100905408657
16,33,32,65,0.0023500919342041016,0.14267893333496387
17,35,34,69,0.0024640560150146484,0.08989523195733685
18,37,36,73,0.0025641918182373047,0.05019054962887102
19,39,38,77,0.0026607513427734375,0.033796314602463365
20,41,40,81,0.002763032913208008,0.012232801326463252
21,43,42,85,0.00286102294921875,0.00794360602484813
22,45,44,89,0.002958059310913086,0.004516048899076068
23,47,46,93,0.0030570030212402344,0.0028958014185372794
24,49,48,97,0.0031528472900390625,0.0038183401737358455
25,51,50,101,0.0032520294189453125,0.00368636533871323
26,53,52,105,0.0033311843872070312,0.0011457816367236226
27,55,54,109,0.003429889678955078,0.0006711793933413259
28,57,56,113,0.0035278797149658203,0.0004963280231576432
29,59,58,117,0.003760814666748047,0.00017160827918518928
30,61,60,121,0.0038788318634033203,0.00011406481495617977
31,63,62,125,0.004155874252319336,7.366308278459671e-05
32,65,64,129,0.004277944564819336,4.6293139937841126e-05
33,67,66,133,0.004394054412841797,3.0629956288868006e-05
34,69,68,137,0.0045299530029296875,1.92000904765276e-05
35,71,70,141,0.0046541690826416016,1.7787308873988487e-05
36,73,72,145,0.004758119583129883,4.0746577426772744e-05
37,75,74,149,0.004904985427856445,1.52698950794787e-05
38,77,76,153,0.005007028579711914,2.984659097657674e-05
39,79,78,157,0.005110025405883789,1.617973584199071e-05
40,81,80,161,0.0052258968353271484,1.2504439878285665e-05
41,83,82,165,0.0053730010986328125,2.8141597023106934e-05
42,85,84,169,0.005499839782714844,9.474317229480118e-06
43,87,86,173,0.005630970001220703,1.7468965446954278e-05
44,89,88,177,0.005836009979248047,1.0642520285212278e-05
45,91,90,181,0.00595402717590332,7.185910828408354e-06
46,93,92,185,0.006062030792236328,1.9668811091630222e-05
47,95,94,189,0.006180763244628906,6.668482856264436e-06
48,97,96,193,0.006283998489379883,7.54654828190053e-06
49,99,98,197,0.006384849548339844,9.826472179159455e-06
50,101,100,201,0.0064928531646728516,3.269104228819362e-06
51,103,102,205,0.0065920352935791016,1.4301033558340755e-05
52,105,104,209,0.006700992584228516,2.6335771760111477e-06
53,107,106,213,0.006829977035522461,1.4939626893556758e-06
54,109,108,217,0.007004976272583008,1.123455257947926e-06
55,111,110,221,0.007113933563232422,2.6469106951997896e-06
56,113,112,225,0.007215023040771484,8.904794723025736e-07
57,115,114,229,0.007312774658203125,1.4595479215346358e-06
58,117,116,233,0.007415056228637695,1.0828099531956602e-06
59,119,118,237,0.007523059844970703,5.510888223406352e-07
60,121,120,241,0.007631778717041016,2.2079135782737187e-06
61,123,122,245,0.007759809494018555,7.457191667324768e-07
62,125,124,249,0.007866144180297852,3.0037919219575125e-07
63,127,126,253,0.007967948913574219,1.2630523651797249e-06
64,129,128,257,0.008070945739746094,3.9423083706593603e-07
65,131,130,261,0.008178949356079102,1.324683964430944e-07
66,133,132,265,0.008276939392089844,2.2807799632852549e-07
67,135,134,269,0.008383989334106445,1.5634237135822493e-07
68,137,136,273,0.008485794067382812,8.848841478844611e-08
69,139,138,277,0.008599042892456055,3.1016277999440296e-07
70,141,140,281,0.008711814880371094,1.0583239011307027e-07
71,143,142,285,0.00880885124206543,6.058055551810527e-08
72,145,144,289,0.008932113647460938,2.091656142180143e-07
73,147,146,293,0.009054899215698242,7.140351966636998e-08
74,149,148,297,0.00917506217956543,4.2605894667862044e-08
75,151,150,301,0.009284019470214844,1.3905252300018056e-07
76,153,152,305,0.009387016296386719,4.7507209729943315e-08
77,155,154,309,0.009511947631835938,3.310365856786001e-08
78,157,156,313,0.009613990783691406,8.696510610582679e-08
79,159,158,317,0.009720087051391602,2.9504378381331194e-08
80,161,160,321,0.009817123413085938,3.662608199786493e-08
81,163,162,325,0.009914875030517578,4.171053964235848e-08
82,165,164,329,0.010015010833740234,1.4489362122527584e-08
83,167,166,333,0.010120868682861328,2.3089712122960386e-08
84,169,168,337,0.010452032089233398,5.00561583775111e-09
85,171,170,341,0.010764122009277344,6.855330156277213e-10
86,173,172,345,0.010889053344726562,2.454316844316619e-09
87,175,174,349,0.011236190795898438,7.434604907140231e-10
88,177,176,353,0.01137399673461914,2.514862597678451e-10
89,179,178,357,0.011487007141113281,2.5989020731145174e-10
90,181,180,361,0.01164698600769043,3.8729857812688484e-10
91,183,182,365,0.011807918548583984,1.2641235914026003e-10
92,185,184,369,0.01194906234741211,5.647297242013917e-10
93,187,186,373,0.012091875076293945,7.733581872838501e-11


==> plot_data/cournot-nash_equilibrium_problem_n10/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00012922286987304688,542.5060889379029
1,3,2,5,0.00023126602172851562,437.43651362206106
2,5,4,9,0.00031113624572753906,346.892909191993
3,7,6,13,0.00037932395935058594,272.4410508043172
4,9,8,17,0.00044536590576171875,212.0408052814726
5,11,10,21,0.0005252361297607422,166.69432451752004
6,13,12,25,0.0005900859832763672,133.3304668212217
7,15,14,29,0.0006620883941650391,107.35953271733689
8,17,16,33,0.0007352828979492188,88.87089053936654
9,19,18,37,0.000797271728515625,76.1398167426833
10,21,20,41,0.0008602142333984375,67.44790329122274
11,23,22,45,0.0009200572967529297,61.45455630670913
12,25,24,49,0.0009961128234863281,57.180289873746716
13,27,26,53,0.0010633468627929688,32.92216846413252
14,29,28,57,0.0011262893676757812,31.518443218527352
15,31,30,61,0.0012001991271972656,24.72720172827196
16,33,32,65,0.0012621879577636719,23.33459462064131
17,35,34,69,0.001329183578491211,22.151841447159534
18,37,36,73,0.0013911724090576172,21.11384989663433
19,39,38,77,0.0014531612396240234,20.177799263942465
20,41,40,81,0.0015223026275634766,19.315904047119957
21,43,42,85,0.0015861988067626953,18.51028419655607
22,45,44,89,0.0016529560089111328,17.749467052294484
23,47,46,93,0.0017333030700683594,17.02606537440799
24,49,48,97,0.001814126968383789,16.33526544552545
25,51,50,101,0.0018973350524902344,15.673856844393542
26,53,52,105,0.0019762516021728516,15.03961723765496
27,55,54,109,0.0020542144775390625,14.43092656652283
28,57,56,113,0.0021212100982666016,13.846527844572298
29,59,58,117,0.0021843910217285156,13.285380784392757
30,61,60,121,0.0022492408752441406,12.746573668322059
31,63,62,125,0.0023102760314941406,12.229271402786075
32,65,64,129,0.0023822784423828125,11.73268578584889
33,67,66,133,0.002452373504638672,11.256059205387718
34,69,68,137,0.0025212764739990234,10.798656292137993
35,71,70,141,0.002582073211669922,8.39592091400955
36,73,72,145,0.0026421546936035156,4.807180204852864
37,75,74,149,0.002704143524169922,4.023356988760287
38,77,76,153,0.0027642250061035156,3.393523621498062
39,79,78,157,0.0028252601623535156,2.8887254847740422
40,81,80,161,0.002887248992919922,2.4851131696304947
41,83,82,165,0.0029761791229248047,2.162965654776843
42,85,84,169,0.003045320510864258,1.9059427008094105
43,87,86,173,0.003117084503173828,1.7005272660684978
44,89,88,177,0.0031921863555908203,1.5356101471635766
45,91,90,181,0.0032732486724853516,1.4021649940177654
46,93,92,185,0.003337383270263672,1.29296885196626
47,95,94,189,0.0034041404724121094,1.2023402684526479
48,97,96,193,0.0034711360931396484,1.125886017566264
49,99,98,197,0.0035352706909179688,1.0602608170370167
50,101,100,201,0.003608226776123047,1.0029492168279008
51,103,102,205,0.0036783218383789062,0.952077184145346
52,105,104,209,0.0037581920623779297,0.9062565711432994
53,107,106,213,0.0038530826568603516,0.8644615135804111
54,109,108,217,0.00400996208190918,0.8259331238963948
55,111,110,221,0.004088163375854492,0.7901076806078755
56,113,112,225,0.0041620731353759766,0.7565634428527174
57,115,114,229,0.004229307174682617,0.724981742874848
58,117,116,233,0.0043010711669921875,0.6951187638521601
59,119,118,237,0.004373073577880859,0.6667851784912998
60,121,120,241,0.0044362545013427734,0.6398315013212134
61,123,122,245,0.00449824333190918,0.6141375602228843
62,125,124,249,0.004557132720947266,0.5896049221526096
63,127,126,253,0.004615306854248047,0.5661514312745007
64,129,128,257,0.004672050476074219,0.5437072558799938
65,131,130,261,0.004740238189697266,0.5222120133509649
66,133,132,265,0.004802227020263672,0.5016126666547746
67,135,134,269,0.00487518310546875,0.48186197451157853
68,137,136,273,0.004937410354614258,0.4629173403621552
69,139,138,277,0.0050013065338134766,0.4447399499004458
70,141,140,281,0.005068063735961914,0.4272941185270261
71,143,142,285,0.005132198333740234,0.4105467924451946
72,145,144,289,0.005208253860473633,0.3944671629681253
73,147,146,293,0.005277156829833984,0.37902636485747954
74,149,148,297,0.005341291427612305,0.36419723752005984
75,151,150,301,0.005403280258178711,0.3499541336139532
76,153,152,305,0.005469322204589844,0.3362727637166878
77,155,154,309,0.005563259124755859,0.3231300686668245
78,157,156,313,0.005631208419799805,0.31050411332950506
79,159,158,317,0.005700111389160156,0.29837399710317286
80,161,160,321,0.005767345428466797,0.2867197776221733
81,163,162,325,0.005837202072143555,0.2755224049618734
82,165,164,329,0.0058972835540771484,0.264763664273821
83,167,166,333,0.0059583187103271484,0.25442612525509783
84,169,168,337,0.006021261215209961,0.24449309720447854
85,171,170,341,0.006083250045776367,0.23494858868975627
86,173,172,345,0.006145000457763672,0.22577727105662584
87,175,174,349,0.0062122344970703125,0.2169644451648659
88,177,176,353,0.006274223327636719,0.2084960108641294
89,179,178,357,0.0063402652740478516,0.20035843881217194
90,181,180,361,0.006415128707885742,0.19253874431826218
91,183,182,365,0.00648808479309082,0.18502446295078648
92,185,184,369,0.006554126739501953,0.17780362769415875
93,187,186,373,0.006646156311035156,0.17086474748029595
94,189,188,377,0.00670623779296875,0.16419678694729425
95,191,190,381,0.00676727294921875,0.15778914730273347
96,193,192,385,0.006832122802734375,0.15163164818787586
97,195,194,389,0.006898164749145508,0.14571451045692685
98,197,196,393,0.006965160369873047,0.14002833979499105
99,199,198,397,0.007026195526123047,0.13456411111017286
100,201,200,401,0.0070841312408447266,0.1293131536454797
101,203,202,405,0.00714421272277832,0.1242671367610666
102,205,204,409,0.00720524787902832,0.119418056342969
103,207,206,413,0.0072650909423828125,0.11475822180171974
104,209,208,417,0.00732421875,0.11028024362626516
105,211,210,421,0.00738525390625,0.10597702146181512
106,213,212,425,0.007445096969604492,0.10184173268567166
107,215,214,429,0.007512092590332031,0.097867821453361
108,217,216,433,0.007573127746582031,0.0940489881945397
109,219,218,437,0.007643222808837891,0.09037917953473365
110,221,220,441,0.007708311080932617,0.08685257862487926
111,223,222,445,0.0077800750732421875,0.08346359585967973
112,225,224,449,0.00785207748413086,0.08020685996693115
113,227,226,453,0.007914066314697266,0.07707720945282427
114,229,228,457,0.00797724723815918,0.07406968438644278
115,231,230,461,0.008037090301513672,0.07117951851053991
116,233,232,465,0.008097171783447266,0.06840213166422236
117,235,234,469,0.008156299591064453,0.0657331225042708
118,237,236,473,0.008216142654418945,0.06316826151363833
119,239,238,477,0.008276224136352539,0.060703484285325494
120,241,240,481,0.008334159851074219,0.05833488506937798
121,243,242,485,0.008395195007324219,0.056058710573958004
122,245,244,489,0.008459091186523438,0.05387135400948592
123,247,246,493,0.008524179458618164,0.0517693493660266
124,249,248,497,0.008585214614868164,0.04974936591458566
125,251,250,501,0.008649349212646484,0.04780820292483645
126,253,252,505,0.008709192276000977,0.04594278458801918
127,255,254,509,0.008773088455200195,0.044150155139731764
128,257,256,513,0.008842229843139648,0.04242747417265084
129,259,258,517,0.008916378021240234,0.04077201213318525
130,261,260,521,0.009057044982910156,0.03918114599335533
131,263,262,525,0.009133100509643555,0.03765235509293629
132,265,264,529,0.009198188781738281,0.036183217142472676
133,267,266,533,0.009261131286621094,0.0347714043841882
134,269,268,537,0.009325027465820312,0.03341467990172313
135,271,270,541,0.009395360946655273,0.032110894074000244
136,273,272,545,0.009464263916015625,0.030857981168538454
137,275,274,549,0.00953817367553711,0.029653956066670706
138,277,276,553,0.009604215621948242,0.02849691111747005
139,279,278,557,0.009670257568359375,0.027385013113885876
140,281,280,561,0.009810209274291992,0.026316500387274358
141,283,282,565,0.009885311126708984,0.025289680015730745
142,285,284,569,0.009949207305908203,0.024302925140422784
143,287,286,573,0.010012149810791016,0.02335467238769415
144,289,288,577,0.010073184967041016,0.022443419391185677
145,291,290,581,0.01015019416809082,0.021567722411174058
146,293,292,585,0.010310173034667969,0.0207261940460586
147,295,294,589,0.010491132736206055,0.01991750103434357
148,297,296,593,0.010570287704467773,0.019140362140932815
149,299,298,597,0.010652303695678711,0.01839354612757884
150,301,300,601,0.01071929931640625,0.017675869801107177
151,303,302,605,0.010787248611450195,0.016986196138833374
152,305,304,609,0.010856389999389648,0.016323432486491395
153,307,306,613,0.010925054550170898,0.01568652882699357
154,309,308,617,0.010991096496582031,0.015074476116181014
155,311,310,621,0.011060237884521484,0.014486304684300722
156,313,312,625,0.01112818717956543,0.0139210826991567
157,315,314,629,0.011193275451660156,0.013377914689659789
158,317,316,633,0.011263370513916016,0.012855940126829165
159,319,318,637,0.01133418083190918,0.012354332060096231
160,321,320,641,0.01140141487121582,0.011872295807441974
161,323,322,645,0.011466264724731445,0.011409067695363307
162,325,324,649,0.011536121368408203,0.01096391384973048
163,327,326,653,0.011602163314819336,0.010536129032149278
164,329,328,657,0.011678218841552734,0.010125035523190344
165,331,330,661,0.011758089065551758,0.009729982047777334
166,333,332,665,0.011837244033813477,0.009350342743906918
167,335,334,669,0.011919260025024414,0.008985516170928926
168,337,336,673,0.012005090713500977,0.008634924355919307
169,339,338,677,0.012279033660888672,0.008298011878808914
170,341,340,681,0.01238703727722168,0.007974244991635111
171,343,342,685,0.012484073638916016,0.007663110773239533
172,345,344,689,0.012548208236694336,0.007364116316489199
173,347,346,693,0.012629985809326172,0.007076787947184648
174,349,348,697,0.012703418731689453,0.006800670473723784
175,351,350,701,0.012992143630981445,0.006535326465692955
176,353,352,705,0.013074159622192383,0.0062803355611051595
177,355,354,709,0.013147115707397461,0.006035293800050675
178,357,356,713,0.013219118118286133,0.005799812984792163
179,359,358,717,0.013290166854858398,0.0055735200649312385
180,361,360,721,0.01350712776184082,0.005356056546015208
181,363,362,725,0.013598203659057617,0.005147077921546557
182,365,364,729,0.013665199279785156,0.0049462531276114555
183,367,366,733,0.013733148574829102,0.0047532640178327154
184,369,368,737,0.013798236846923828,0.004567804859592573
185,371,370,741,0.013865232467651367,0.004389581849685407
186,373,372,745,0.013933181762695312,0.004218312648510509
187,375,374,749,0.014000177383422852,0.004053725933287791
188,377,376,753,0.014069080352783203,0.0038955609675745536
189,379,378,757,0.014136075973510742,0.0037435671886148487
190,381,380,761,0.014205217361450195,0.0035975038103751057
191,383,382,765,0.014281272888183594,0.003457139441701459
192,385,384,769,0.014349222183227539,0.0033222517201560242
193,387,386,773,0.014419317245483398,0.003192626959459821
194,389,388,777,0.014489173889160156,0.003068059810943388
195,391,390,781,0.014561176300048828,0.0029483529382753463
196,393,392,785,0.0146331787109375,0.002833316705001248
197,395,394,789,0.014721155166625977,0.002722768873867421
198,397,396,793,0.014796018600463867,0.0026165343181881627
199,399,398,797,0.01487112045288086,0.0025144447443065506
200,401,400,801,0.014945030212402344,0.0024163384253150194
201,403,402,805,0.015025138854980469,0.0023220599442951534
202,405,404,809,0.015099287033081055,0.0022314599485026955
203,407,406,813,0.015172243118286133,0.0021443949125897585
204,409,408,817,0.015248298645019531,0.0020607269114610726
205,411,410,821,0.01532125473022461,0.0019803234014133327
206,413,412,825,0.015394210815429688,0.0019030570103310742
207,415,414,829,0.015469074249267578,0.0018288053358947493
208,417,416,833,0.01554417610168457,0.001757450751668465
209,419,418,837,0.015610218048095703,0.0016888802207537842
210,421,420,841,0.01567220687866211,0.0016229851166448882
211,423,422,845,0.015735149383544922,0.0015596610514120451
212,425,424,849,0.015807390213012695,0.0014988077097954973
213,427,426,853,0.015882253646850586,0.0014403286907647504
214,429,428,857,0.015955209732055664,0.0013841313547355385
215,431,430,861,0.016028165817260742,0.0013301266764229728
216,433,432,865,0.016100168228149414,0.0012782291043898716
217,435,434,869,0.016172170639038086,0.0012283564250635051
218,437,436,873,0.01624441146850586,0.0011804296325674715
219,439,438,877,0.016318321228027344,0.0011343728039809155
220,441,440,881,0.016393184661865234,0.0010901129782634996
221,443,442,885,0.016468286514282227,0.001047580041340157
222,445,444,889,0.01656818389892578,0.001006706614968704
223,447,446,893,0.016646146774291992,0.0009674279495677968
224,449,448,897,0.01671910285949707,0.0009296818220983381
225,451,450,901,0.016793251037597656,0.0008934084372555575
226,453,452,905,0.016866207122802734,0.0008585503326549087
227,455,454,909,0.01694011688232422,0.0008250522881398469
228,457,456,913,0.017013072967529297,0.0007928612381221467
229,459,458,917,0.017089128494262695,0.0007619261873273383
230,461,460,921,0.01716303825378418,0.0007321981301929986
231,463,462,925,0.01723623275756836,0.0007036299733131437
232,465,464,929,0.017312049865722656,0.0006761764609298715
233,467,466,933,0.017400264739990234,0.0006497941025223991
234,469,468,937,0.017475128173828125,0.0006244411049403347
235,471,470,941,0.017550230026245117,0.0006000773054399955
236,473,472,945,0.017626285552978516,0.0005766641085249237
237,475,474,949,0.01770329475402832,0.0005541644241753831
238,477,476,953,0.01777815818786621,0.0005325426100877916
239,479,478,957,0.017853260040283203,0.0005117644141278338
240,481,480,961,0.017927169799804688,0.000491796920929384
241,483,482,965,0.01800227165222168,0.0004726084992122925
242,485,484,969,0.018077373504638672,0.0004541687519210449
243,487,486,973,0.01815319061279297,0.00043644846782421614
244,489,488,977,0.01822519302368164,0.00041941957578599904
245,491,490,981,0.018287181854248047,0.00040305509962813016
246,493,492,985,0.01834416389465332,0.0003873291159777035
247,495,494,989,0.018429279327392578,0.0003722167125160981
248,497,496,993,0.0185091495513916,0.0003576939493652657
249,499,498,997,0.01857924461364746,0.0003437378204199749
250,501,500,1001,0.018657207489013672,0.0003303262172771757
251,503,502,1005,0.01872730255126953,0.0003174378941979059
252,505,504,1009,0.01879119873046875,0.00030505243439892996
253,507,506,1013,0.018854141235351562,0.00029315021766018116
254,509,508,1017,0.018917083740234375,0.0002817123892437782
255,511,510,1021,0.018985271453857422,0.0002707208301286335
256,513,512,1025,0.019054174423217773,0.00026015812823353623
257,515,514,1029,0.019118070602416992,0.00025000755084199377
258,517,516,1033,0.019181251525878906,0.00024025301804221868
259,519,518,1037,0.019242048263549805,0.00023087907751694528
260,521,520,1041,0.01930522918701172,0.00022187087956473953
261,523,522,1045,0.019365310668945312,0.00021321415400175287
262,525,524,1049,0.019497394561767578,0.00020489518750305984
263,527,526,1053,0.01956915855407715,0.00019690080172976877
264,529,528,1057,0.01963329315185547,0.00018921833255674273
265,531,530,1061,0.019697189331054688,0.00018183560990394035
266,533,532,1065,0.019774198532104492,0.00017474093854457978
267,535,534,1069,0.019843101501464844,0.00016792307960275093
268,537,536,1073,0.01991724967956543,0.00016137123277423145
269,539,538,1077,0.01998734474182129,0.00015507501893295106
270,541,540,1081,0.020072221755981445,0.00014902446417375872
271,543,542,1085,0.02014017105102539,0.00014320998362964382
272,545,544,1089,0.020203113555908203,0.00013762236625912378
273,547,546,1093,0.020269155502319336,0.0001322527607170798
274,549,548,1097,0.02033519744873047,0.00012709266082525737
275,551,550,1101,0.020403385162353516,0.00012213389222079615
276,553,552,1105,0.020473241806030273,0.00011736859970032754
277,555,554,1109,0.02054119110107422,0.00011278923428642776
278,557,556,1113,0.020611047744750977,0.0001083885417104131
279,559,558,1117,0.020679235458374023,0.00010415955074536173
280,561,560,1121,0.020740270614624023,0.00010009556196515134
281,563,562,1125,0.0208132266998291,9.619013775718002e-05
282,565,564,1129,0.020876169204711914,9.24370912856949e-05
283,567,566,1133,0.02094101905822754,8.883047712913854e-05
284,569,568,1137,0.021007299423217773,8.536458207691356e-05
285,571,570,1141,0.021069049835205078,8.203391565899023e-05
286,573,572,1145,0.021128177642822266,7.88332016849376e-05
287,575,574,1149,0.021190166473388672,7.575736984077025e-05
288,577,576,1153,0.021254301071166992,7.280154756302927e-05
289,579,578,1157,0.021320343017578125,6.996105236090507e-05
290,581,580,1161,0.02138519287109375,6.723138462409784e-05
291,583,582,1165,0.0214540958404541,6.460822027175152e-05
292,585,584,1169,0.021555185317993164,6.208740369563189e-05
293,587,586,1173,0.02161717414855957,5.9664941725685195e-05
294,589,588,1177,0.021677255630493164,5.733699684196163e-05
295,591,590,1181,0.021737337112426758,5.509988125370876e-05
296,593,592,1185,0.021796226501464844,5.2950051109475524e-05
297,595,594,1189,0.021856069564819336,5.088410071673632e-05
298,597,596,1193,0.02191615104675293,4.889875750964775e-05
299,599,598,1197,0.021975040435791016,4.699087623684391e-05
300,601,600,1201,0.02203536033630371,4.5157434751187295e-05
301,603,602,1205,0.02209615707397461,4.339552855336934e-05
302,605,604,1209,0.02215719223022461,4.17023664608714e-05
303,607,606,1213,0.022220134735107422,4.0075266494943766e-05
304,609,608,1217,0.022286176681518555,3.8511651036839826e-05
305,611,610,1221,0.022345304489135742,3.700904304467993e-05
306,613,612,1225,0.022413253784179688,3.556506218770733e-05
307,615,614,1229,0.02247333526611328,3.417742112603628e-05
308,617,616,1233,0.022539138793945312,3.284392159346263e-05
309,619,618,1237,0.022607088088989258,3.156245114667204e-05
310,621,620,1241,0.022681236267089844,3.033097975973181e-05
311,623,622,1245,0.022736310958862305,2.9147556675579586e-05
312,625,624,1249,0.022792339324951172,2.8010307145211304e-05
313,627,626,1253,0.022863149642944336,2.691742963252594e-05
314,629,628,1257,0.022925138473510742,2.5867192861570113e-05
315,631,630,1261,0.02298903465270996,2.485793314001625e-05
316,633,632,1265,0.0230562686920166,2.3888051739747515e-05
317,635,634,1269,0.023122310638427734,2.295601205309767e-05
318,637,636,1273,0.02318739891052246,2.206033783225679e-05
319,639,638,1277,0.0232541561126709,2.1199610009351152e-05
320,641,640,1281,0.023324251174926758,2.037246517637046e-05
321,643,642,1285,0.023391246795654297,1.9577593039723553e-05
322,645,644,1289,0.023449182510375977,1.881373447127672e-05
323,647,646,1293,0.023513078689575195,1.807967922259979e-05
324,649,648,1297,0.023572206497192383,1.737426464706643e-05
325,651,650,1301,0.02363109588623047,1.6696373192604184e-05
326,653,652,1305,0.02369213104248047,1.6044931056640427e-05
327,655,654,1309,0.0237581729888916,1.5418906167735643e-05
328,657,656,1313,0.02382636070251465,1.4817306902354164e-05
329,659,658,1317,0.02390122413635254,1.423918016854675e-05
330,661,660,1321,0.023967266082763672,1.3683610235753103e-05
331,663,662,1325,0.024031400680541992,1.3149717032309135e-05
332,665,664,1329,0.024096012115478516,1.2636654581721193e-05
333,667,666,1333,0.024160146713256836,1.2143610401392343e-05
334,669,668,1337,0.024239301681518555,1.1669803155498594e-05
335,671,670,1341,0.024306297302246094,1.1214482524565392e-05
336,673,672,1345,0.02437615394592285,1.0776927185484824e-05
337,675,674,1349,0.02444911003112793,1.0356443885939597e-05
338,677,676,1353,0.024520158767700195,9.952366541121925e-06
339,679,678,1357,0.02459120750427246,9.564055112007646e-06
340,681,680,1361,0.02466726303100586,9.190894419656837e-06
341,683,682,1365,0.024735212326049805,8.832293240746775e-06
342,685,684,1369,0.02480316162109375,8.487683660061348e-06
343,687,686,1373,0.02487325668334961,8.15651979393122e-06
344,689,688,1377,0.024944305419921875,7.838276833193686e-06
345,691,690,1381,0.025008201599121094,7.5324507338155735e-06
346,693,692,1385,0.025069236755371094,7.238557185738857e-06
347,695,694,1389,0.025132179260253906,6.95613038904859e-06
348,697,696,1393,0.02519512176513672,6.684722993034641e-06
349,699,698,1397,0.025265216827392578,6.423905085704579e-06
350,701,700,1401,0.025336027145385742,6.173263596810279e-06
351,703,702,1405,0.025403261184692383,5.932401341219535e-06
352,705,704,1409,0.025471210479736328,5.700936845786831e-06
353,707,706,1413,0.025544166564941406,5.478503338642731e-06
354,709,708,1417,0.025606155395507812,5.264748568292871e-06
355,711,710,1421,0.02567911148071289,5.059333834531598e-06
356,713,712,1425,0.02574896812438965,4.861933754187416e-06
357,715,714,1429,0.025809288024902344,4.672235656337158e-06
358,717,716,1433,0.025870084762573242,4.489938928445738e-06
359,719,718,1437,0.02593207359313965,4.314755015406312e-06
360,721,720,1441,0.02599811553955078,4.1464061853515565e-06
361,723,722,1445,0.026064157485961914,3.984625725606023e-06
362,725,724,1449,0.026143312454223633,3.829157607719305e-06
363,727,726,1453,0.026240110397338867,3.679755344339546e-06
364,729,728,1457,0.02632617950439453,3.536182242741062e-06
365,731,730,1461,0.026407241821289062,3.3982109706382505e-06
366,733,732,1465,0.02649521827697754,3.2656229015866322e-06
367,735,734,1469,0.0265653133392334,3.1382080761556143e-06
368,737,736,1473,0.026642322540283203,3.0157645658837727e-06
369,739,738,1477,0.026731014251708984,2.8980984585155546e-06
370,741,740,1481,0.02681708335876465,2.785023277418465e-06
371,743,742,1485,0.0269010066986084,2.6763599658872474e-06
372,745,744,1489,0.027021169662475586,2.5719363879908382e-06
373,747,746,1493,0.02718520164489746,2.4715871344671204e-06
374,749,748,1497,0.027300119400024414,2.3751531427249943e-06
375,751,750,1501,0.02742624282836914,2.282481754367066e-06
376,753,752,1505,0.02753305435180664,2.1934260789694313e-06
377,755,754,1509,0.02770829200744629,2.1078451232280347e-06
378,757,756,1513,0.02783203125,2.02560329466403e-06
379,759,758,1517,0.027938127517700195,1.946570311442325e-06
380,761,760,1521,0.028028249740600586,1.870620925400814e-06
381,763,762,1525,0.02811717987060547,1.797634912380939e-06
382,765,764,1529,0.028180360794067383,1.727496533290736e-06
383,767,766,1533,0.028257131576538086,1.6600946971764276e-06
384,769,768,1537,0.028331995010375977,1.5953227233555441e-06
385,771,770,1541,0.028409242630004883,1.533078015006749e-06
386,773,772,1545,0.0284731388092041,1.4732618591773384e-06
387,775,774,1549,0.02854132652282715,1.4157796074242164e-06
388,777,776,1553,0.028614282608032227,1.3605400483330717e-06
389,779,778,1557,0.028695106506347656,1.3074558261597286e-06
390,781,780,1561,0.028783082962036133,1.2564428407111703e-06
391,783,782,1565,0.028872251510620117,1.2074201014662186e-06
392,785,784,1569,0.02899622917175293,1.1603102328314388e-06
393,787,786,1573,0.029078006744384766,1.1150383794015295e-06
394,789,788,1577,0.029146194458007812,1.071532881101824e-06
395,791,790,1581,0.029212236404418945,1.0297248175264282e-06
396,793,792,1585,0.029279232025146484,9.895480275183042e-07
397,795,794,1589,0.029348134994506836,9.509387963885513e-07
398,797,796,1593,0.0294952392578125,9.138359743289207e-07
399,799,798,1597,0.029577255249023438,8.781807706531322e-07
400,801,800,1601,0.029671192169189453,8.439167391227624e-07
401,803,802,1605,0.029770374298095703,8.109896565583979e-07
402,805,804,1609,0.029858112335205078,7.793472169709408e-07
403,807,806,1613,0.02994513511657715,7.489394277567106e-07
404,809,808,1617,0.03002333641052246,7.197180338116877e-07
405,811,810,1621,0.030091047286987305,6.916367787312482e-07
406,813,812,1625,0.03015613555908203,6.646511436101068e-07
407,815,814,1629,0.03021836280822754,6.387184082220201e-07
408,817,816,1633,0.030280351638793945,6.137975421983264e-07
409,819,818,1637,0.030344247817993164,5.898489574442705e-07
410,821,820,1641,0.03040623664855957,5.668347926299798e-07
411,823,822,1645,0.030476093292236328,5.447186626595682e-07
412,825,824,1649,0.030559301376342773,5.234652944780737e-07
413,827,826,1653,0.030643224716186523,5.030412389383088e-07
414,829,828,1657,0.03072834014892578,4.834140404312521e-07
415,831,830,1661,0.030810117721557617,4.645526457478158e-07
416,833,832,1665,0.030879974365234375,4.4642719628741204e-07
417,835,834,1669,0.030950307846069336,4.290089561459663e-07
418,837,836,1673,0.031022071838378906,4.1227022083558453e-07
419,839,838,1677,0.03110027313232422,3.9618474264776e-07
420,841,840,1681,0.03116631507873535,3.8072678864824034e-07
421,843,842,1685,0.031235218048095703,3.658719467096191e-07
422,845,844,1689,0.0312960147857666,3.515966448210108e-07
423,847,846,1693,0.0313572883605957,3.378784530737118e-07
424,849,848,1697,0.0314180850982666,3.2469539706482245e-07
425,851,850,1701,0.0314791202545166,3.1202676204288107e-07
426,853,852,1705,0.031539201736450195,2.998523557813865e-07
427,855,854,1709,0.031606197357177734,2.8815301742548464e-07
428,857,856,1713,0.03168010711669922,2.7691016790896364e-07
429,859,858,1717,0.03174138069152832,2.6610590895013917e-07
430,861,860,1721,0.03180432319641113,2.5572330378450633e-07
431,863,862,1725,0.031867265701293945,2.457457419435445e-07
432,865,864,1729,0.03193020820617676,2.3615740742846477e-07
433,867,866,1733,0.03199410438537598,2.269432864331384e-07
434,869,868,1737,0.0320591926574707,2.1808861280632527e-07
435,871,870,1741,0.032125234603881836,2.095794167965561e-07
436,873,872,1745,0.03218722343444824,2.0140227058579363e-07
437,875,874,1749,0.03225421905517578,1.9354415811040682e-07
438,877,876,1753,0.03232526779174805,1.859925975104904e-07
439,879,878,1757,0.0323944091796875,1.7873569060827695e-07
440,881,880,1761,0.032479286193847656,1.7176198205531542e-07
441,883,882,1765,0.032546043395996094,1.6506037396324237e-07
442,885,884,1769,0.032616376876831055,1.5862015106099078e-07
443,887,886,1773,0.03267717361450195,1.52431279859872e-07
444,889,888,1777,0.03273439407348633,1.4648391433177982e-07
445,891,890,1781,0.03279829025268555,1.4076855224087703e-07
446,893,892,1785,0.03286337852478027,1.352761332558194e-07
447,895,894,1789,0.032923221588134766,1.2999801368305085e-07
448,897,896,1793,0.03298306465148926,1.249259499642107e-07
449,899,898,1797,0.033042192459106445,1.20051683983753e-07
450,901,900,1801,0.033106327056884766,1.1536767629439138e-07
451,903,902,1805,0.0331723690032959,1.1086635251225883e-07
452,905,904,1809,0.03323221206665039,1.0654063159871462e-07
453,907,906,1813,0.03329610824584961,1.0238375788116406e-07
454,909,908,1817,0.03335714340209961,9.838900482199322e-08
455,911,910,1821,0.033419132232666016,9.455014605144168e-08
456,913,912,1825,0.033480167388916016,9.086109699860813e-08
457,915,914,1829,0.033550262451171875,8.731592264543317e-08
458,917,916,1833,0.033614158630371094,8.390911336722207e-08
459,919,918,1837,0.0336911678314209,8.063529745986107e-08
460,921,920,1841,0.03375840187072754,7.748910028430733e-08
461,923,922,1845,0.033820152282714844,7.446572314357436e-08
462,925,924,1849,0.03391122817993164,7.156025661712576e-08
463,927,926,1853,0.03398013114929199,6.87682370631272e-08
464,929,928,1857,0.03404426574707031,6.60851279979245e-08
465,931,930,1861,0.034110307693481445,6.350660951679668e-08
466,933,932,1865,0.0341792106628418,6.102883955984016e-08
467,935,934,1869,0.03424215316772461,5.864764971484541e-08
468,937,936,1873,0.03430604934692383,5.6359352343640924e-08
469,939,938,1877,0.03437209129333496,5.4160442384920695e-08
470,941,940,1881,0.03443717956542969,5.2047205948678984e-08
471,943,942,1885,0.03450131416320801,5.001645557045838e-08
472,945,944,1889,0.03456521034240723,4.806497947765475e-08
473,947,946,1893,0.03462815284729004,4.618968148958354e-08
474,949,948,1897,0.034690141677856445,4.438748774473138e-08
475,951,950,1901,0.034754037857055664,4.265562255584387e-08
476,953,952,1905,0.034815311431884766,4.0991250009575674e-08
477,955,954,1909,0.03493523597717285,3.939196542573217e-08
478,957,956,1913,0.03502917289733887,3.785497853193851e-08
479,959,958,1917,0.03510332107543945,3.6377972045425875e-08
480,961,960,1921,0.035178184509277344,3.495862479622804e-08
481,963,962,1925,0.0352482795715332,3.359464863394367e-08
482,965,964,1929,0.0353243350982666,3.2283868071071885e-08
483,967,966,1933,0.03541302680969238,3.1024295056238936e-08
484,969,968,1937,0.03548431396484375,2.9813797799304854e-08
485,971,970,1941,0.03555417060852051,2.8650599008075007e-08
486,973,972,1945,0.035627126693725586,2.7532696065330435e-08
487,975,974,1949,0.0357050895690918,2.6458401017310786e-08
488,977,976,1953,0.0357823371887207,2.542609487603269e-08
489,979,978,1957,0.03586411476135254,2.4434018805912255e-08
490,981,980,1961,0.03594017028808594,2.3480670342750388e-08
491,983,982,1965,0.03601717948913574,2.2564545106884706e-08
492,985,984,1969,0.036092281341552734,2.1684196980468794e-08
493,987,986,1973,0.03618025779724121,2.0838141955157397e-08
494,989,988,1977,0.03625130653381348,2.0025017444979148e-08
495,991,990,1981,0.03632211685180664,1.924366481044195e-08
496,993,992,1985,0.0363922119140625,1.8492938030535024e-08
497,995,994,1989,0.03646421432495117,1.777139293419102e-08
498,997,996,1993,0.036547183990478516,1.707794175976507e-08
499,999,998,1997,0.03662896156311035,1.6411624010131193e-08
500,1001,1000,2001,0.03670334815979004,1.577133930604825e-08
501,1003,1002,2005,0.03678321838378906,1.5155956190354236e-08
502,1005,1004,2009,0.03686404228210449,1.4564588938736502e-08
503,1007,1006,2013,0.03694319725036621,1.399636249613316e-08
504,1009,1008,2017,0.03703498840332031,1.3450291093053104e-08
505,1011,1010,2021,0.0371091365814209,1.2925485109457703e-08
506,1013,1012,2025,0.037194252014160156,1.24211316447961e-08
507,1015,1014,2029,0.0372772216796875,1.193648481882728e-08
508,1017,1016,2033,0.03735709190368652,1.1470786135546793e-08
509,1019,1018,2037,0.037450313568115234,1.1023235310339514e-08
510,1021,1020,2041,0.03753542900085449,1.0593117540697083e-08
511,1023,1022,2045,0.03762626647949219,1.0179785044135552e-08
512,1025,1024,2049,0.037722110748291016,9.782679373521822e-09
513,1027,1026,2053,0.037827253341674805,9.400991527337729e-09
514,1029,1028,2057,0.03790736198425293,9.034128081207756e-09
515,1031,1030,2061,0.03799033164978027,8.681634534648964e-09
516,1033,1032,2065,0.03807520866394043,8.342952440457601e-09
517,1035,1034,2069,0.038161277770996094,8.017363096199573e-09
518,1037,1036,2073,0.03825116157531738,7.704555743067209e-09
519,1039,1038,2077,0.03833818435668945,7.40398259711187e-09
520,1041,1040,2081,0.038433074951171875,7.115061933032515e-09
521,1043,1042,2085,0.03854632377624512,6.837487805341884e-09
522,1045,1044,2089,0.038616180419921875,6.570705666804301e-09
523,1047,1046,2093,0.03869009017944336,6.314413472409368e-09
524,1049,1048,2097,0.038767099380493164,6.06794011150924e-09
525,1051,1050,2101,0.03885841369628906,5.831212765055339e-09
526,1053,1052,2105,0.038938283920288086,5.603702112567803e-09
527,1055,1054,2109,0.0390012264251709,5.385093496176269e-09
528,1057,1056,2113,0.03906726837158203,5.174970256656906e-09
529,1059,1058,2117,0.03913712501525879,4.9730614270077926e-09
530,1061,1060,2121,0.0391993522644043,4.7789562028090585e-09
531,1063,1062,2125,0.039260149002075195,4.592546783755809e-09
532,1065,1064,2129,0.0393221378326416,4.413351442767816e-09
533,1067,1066,2133,0.03938722610473633,4.241180796371008e-09
534,1069,1068,2137,0.03944826126098633,4.0756696821957895e-09
535,1071,1070,2141,0.039527177810668945,3.9166248135357444e-09
536,1073,1072,2145,0.03959226608276367,3.763877226134218e-09
537,1075,1074,2149,0.0396573543548584,3.617010260529515e-09
538,1077,1076,2153,0.039716243743896484,3.4758442336779236e-09
539,1079,1078,2157,0.03977608680725098,3.340227655652756e-09
540,1081,1080,2161,0.039838314056396484,3.2099206387757545e-09
541,1083,1082,2165,0.0399012565612793,3.0846648264341577e-09
542,1085,1084,2169,0.039965152740478516,2.9643058204763465e-09
543,1087,1086,2173,0.040038108825683594,2.8486668459707524e-09
544,1089,1088,2177,0.04010319709777832,2.737509969956892e-09
545,1091,1090,2181,0.04016995429992676,2.630756516096193e-09
546,1093,1092,2185,0.040246009826660156,2.528085015405078e-09
547,1095,1094,2189,0.04032611846923828,2.429451777746748e-09
548,1097,1096,2193,0.04040336608886719,2.3346654662762753e-09
549,1099,1098,2197,0.04049515724182129,2.2435988562506917e-09
550,1101,1100,2201,0.04057908058166504,2.156026622328697e-09
551,1103,1102,2205,0.04066920280456543,2.0719196391533604e-09
552,1105,1104,2209,0.040763139724731445,1.991086568919414e-09
553,1107,1106,2213,0.04087018966674805,1.9134021406329454e-09
554,1109,1108,2217,0.040972232818603516,1.838670155185329e-09
555,1111,1110,2221,0.041056156158447266,1.7670100888673113e-09
556,1113,1112,2225,0.041129350662231445,1.6980004192799094e-09
557,1115,1114,2229,0.04120612144470215,1.6318227825473021e-09
558,1117,1116,2233,0.04127836227416992,1.5681226747702866e-09
559,1119,1118,2237,0.041355133056640625,1.5069000973037925e-09
560,1121,1120,2241,0.041419029235839844,1.448078324440392e-09
561,1123,1122,2245,0.0414881706237793,1.391659312925431e-09
562,1125,1124,2249,0.04155921936035156,1.3373196394658402e-09
563,1127,1126,2253,0.0416262149810791,1.285140886812653e-09
564,1129,1128,2257,0.04168820381164551,1.2350482843514632e-09
565,1131,1130,2261,0.041749000549316406,1.186860198545145e-09
566,1133,1132,2265,0.04181241989135742,1.140562065305281e-09
567,1135,1134,2269,0.041889190673828125,1.0960120978663005e-09
568,1137,1136,2273,0.04198813438415527,1.0532773156274416e-09
569,1139,1138,2277,0.04205012321472168,1.012159564631889e-09
570,1141,1140,2281,0.04211306571960449,9.726336316793775e-10
571,1143,1142,2285,0.042174339294433594,9.347626212499833e-10
572,1145,1144,2289,0.042240142822265625,8.982541932178419e-10
573,1147,1146,2293,0.04230237007141113,8.631918859737313e-10
574,1149,1148,2297,0.042368173599243164,8.295300533129466e-10
575,1151,1150,2301,0.04243206977844238,7.971560353247145e-10
576,1153,1152,2305,0.0424952507019043,7.660863494472152e-10
577,1155,1154,2309,0.04255819320678711,7.361752984059729e-10
578,1157,1156,2313,0.04262518882751465,7.074228817547586e-10
579,1159,1158,2317,0.04270315170288086,6.798019300741735e-10
580,1161,1160,2321,0.04277229309082031,6.533396127571754e-10
581,1163,1162,2325,0.04283618927001953,6.278795815104037e-10
582,1165,1164,2329,0.042899370193481445,6.033072171939017e-10
583,1167,1166,2333,0.042960166931152344,5.798187207352479e-10
584,1169,1168,2337,0.04302525520324707,5.571528271737344e-10
585,1171,1170,2341,0.04308724403381348,5.354124949142537e-10
586,1173,1172,2345,0.04324030876159668,5.145598302218189e-10
587,1175,1174,2349,0.04334115982055664,4.944384855414559e-10
588,1177,1176,2353,0.043410301208496094,4.751446025467098e-10
589,1179,1178,2357,0.043498992919921875,4.566131195353897e-10
590,1181,1180,2361,0.04355931282043457,4.387944811541427e-10
591,1183,1182,2365,0.043618202209472656,4.216634721420272e-10
592,1185,1184,2369,0.04367828369140625,4.0524726590565135e-10
593,1187,1186,2373,0.04375123977661133,3.894331971593097e-10
594,1189,1188,2377,0.043810129165649414,3.742067053234979e-10
595,1191,1190,2381,0.04387402534484863,3.5968045142699826e-10
596,1193,1192,2385,0.04393315315246582,3.45598031231814e-10
597,1195,1194,2389,0.0439910888671875,3.320886269620184e-10
598,1197,1196,2393,0.04405021667480469,3.1913571380833226e-10
599,1199,1198,2397,0.04411435127258301,3.067412557407374e-10
600,1201,1200,2401,0.04417610168457031,2.9470709670712815e-10
601,1203,1202,2405,0.04424905776977539,2.832003042321964e-10
602,1205,1204,2409,0.04431724548339844,2.722208797596574e-10
603,1207,1206,2413,0.04438614845275879,2.615871920555191e-10
604,1209,1208,2417,0.044448137283325195,2.51368215579273e-10
605,1211,1210,2421,0.04450821876525879,2.4157851173879045e-10
606,1213,1212,2425,0.04456806182861328,2.321054124285886e-10
607,1215,1214,2429,0.04462838172912598,2.2304702707899018e-10
608,1217,1216,2433,0.04468822479248047,2.144013935168305e-10
609,1219,1218,2437,0.04474902153015137,2.059597071422997e-10
610,1221,1220,2441,0.044830322265625,1.9801431036403613e-10
611,1223,1222,2445,0.044898033142089844,1.902437383534575e-10
612,1225,1224,2449,0.044970035552978516,1.8278781644674094e-10
613,1227,1226,2453,0.04503226280212402,1.757174850509383e-10
614,1229,1228,2457,0.0451052188873291,1.6883457724969176e-10
615,1231,1230,2461,0.04516720771789551,1.622372015955831e-10
616,1233,1232,2465,0.04523324966430664,1.5589622810134068e-10
617,1235,1234,2469,0.04529619216918945,1.4984274272880135e-10
618,1237,1236,2473,0.04536128044128418,1.4396016573236969e-10
619,1239,1238,2477,0.04543113708496094,1.3835051116178982e-10
620,1241,1240,2481,0.04550504684448242,1.330118267240005e-10
621,1243,1242,2485,0.04557228088378906,1.2774792185090235e-10
622,1245,1244,2489,0.045632123947143555,1.2280740999601188e-10
623,1247,1246,2493,0.04569435119628906,1.1805630151211657e-10
624,1249,1248,2497,0.04575514793395996,1.133488813466001e-10
625,1251,1250,2501,0.04582023620605469,1.0899792158560653e-10
626,1253,1252,2505,0.0458831787109375,1.0471976771979524e-10
627,1255,1254,2509,0.04594612121582031,1.0065237283999396e-10
628,1257,1256,2513,0.04600811004638672,9.66617062249053e-11


==> plot_data/cournot-nash_equilibrium_problem_n10/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0001709461212158203,542.5060889379029
1,2,1,3,0.0003020763397216797,207.98870940431505
2,3,2,5,0.00037407875061035156,274.0655574126137
3,4,3,7,0.0004291534423828125,175.81646225201428
4,5,4,9,0.0004961490631103516,164.98414436485226
6,7,6,13,0.0006132125854492188,120.69035731832143
7,8,7,15,0.0006670951843261719,110.05724136292307
8,9,8,17,0.0007190704345703125,100.9817631078583
9,10,9,19,0.0007741451263427734,93.9040070272565
10,11,10,21,0.0008270740509033203,89.6901587930119
11,12,11,23,0.0008780956268310547,86.48087704332885
12,13,12,25,0.0009322166442871094,83.90363237471003
13,14,13,27,0.00098419189453125,70.3354823560248
15,16,15,31,0.0010859966278076172,64.13835866777424
16,17,16,33,0.0011401176452636719,62.0248062633654
17,18,17,35,0.0012023448944091797,60.26569227733142
18,19,18,37,0.0012581348419189453,58.7275169303602
19,20,19,39,0.0013120174407958984,57.33681249756586
20,21,20,41,0.001373291015625,56.0428339377457
21,22,21,43,0.0014252662658691406,41.17109166754773
22,23,22,45,0.0014801025390625,35.56400995834689
24,25,24,49,0.0016040802001953125,32.90551431967733
25,26,25,51,0.0016751289367675781,31.80962744205267
26,27,26,53,0.0017271041870117188,23.98320898693349
27,28,27,55,0.0017800331115722656,23.14887668222036
28,29,28,57,0.0018301010131835938,22.570890908767296
29,30,29,59,0.0018811225891113281,22.021963668656266
30,31,30,61,0.0019309520721435547,21.496568136886992
31,32,31,63,0.001980304718017578,20.990871046760084
32,33,32,65,0.002031087875366211,20.501999198134996
34,35,34,69,0.002134084701538086,19.566765906681205
35,36,35,71,0.0021851062774658203,19.11764758580096
36,37,36,73,0.0022361278533935547,18.679588339189444
37,38,37,75,0.002286195755004883,18.251922413304875
38,39,38,77,0.002340078353881836,17.834139723805023
39,40,39,79,0.0023920536041259766,17.425841988121515
40,41,40,81,0.0024461746215820312,17.026710567443025
41,42,41,83,0.002504110336303711,16.63648302350121
43,44,43,87,0.0026140213012695312,15.881873716776415
44,45,44,89,0.0026760101318359375,15.517117886513235
45,46,45,91,0.002730131149291992,15.160502994707883
46,47,46,93,0.0027840137481689453,14.811871363214015
47,48,47,95,0.0028412342071533203,14.4710704082417
48,49,48,97,0.0029091835021972656,14.137950734300818
49,50,49,99,0.002973318099975586,13.812364922223416
50,51,50,101,0.0030410289764404297,13.494166805130115
51,52,51,103,0.0031092166900634766,13.183211082056683
53,54,53,107,0.0032472610473632812,12.582449148328152
54,55,54,109,0.003304004669189453,12.292355942812474
55,56,55,111,0.0033600330352783203,12.008931371424364
56,57,56,113,0.0034110546112060547,11.732034363102503
57,58,57,115,0.0034601688385009766,11.46152512782343
58,59,58,117,0.0035161972045898438,11.197265333420109
59,60,59,119,0.003576040267944336,10.939118271714221
60,61,60,121,0.0036270618438720703,10.686949009389792
62,63,62,125,0.003735065460205078,5.402158040438191
63,64,63,127,0.0038640499114990234,4.761358153405375
64,65,64,129,0.0039370059967041016,4.271520432759425
65,66,65,131,0.0040073394775390625,3.8370636416417843
66,67,66,133,0.004060268402099609,3.4587693629219842
67,68,67,135,0.004113197326660156,3.1287530232702094
68,69,68,137,0.004166126251220703,2.841345039817945
69,70,69,139,0.0042171478271484375,2.5912940307989034
71,72,71,143,0.004353046417236328,2.1851658209445826
72,73,72,145,0.0044422149658203125,2.02123160829976
73,74,73,147,0.00449824333190918,1.8788457522323445
74,75,74,149,0.00455021858215332,1.7550696464366484
75,76,75,151,0.0046041011810302734,1.6472985678540493
76,77,76,153,0.004658222198486328,1.5532350458182878
77,78,77,155,0.004719257354736328,1.4708646705912216
78,79,78,157,0.004770040512084961,1.3984330391989461
79,80,79,159,0.004820108413696289,1.3344230355887088
81,82,81,163,0.004918098449707031,1.2266497932218043
82,83,82,165,0.004965066909790039,1.1808352966214721
83,84,83,167,0.005029201507568359,1.1392964157497862
84,85,84,169,0.005095958709716797,1.101369362909225
85,86,85,171,0.005151987075805664,1.0665003323495321
86,87,86,173,0.0052149295806884766,1.0342288512086701
87,88,87,175,0.005275249481201172,1.0041730294632891
88,89,88,177,0.00533604621887207,0.9760166961785682
90,91,90,181,0.005448102951049805,0.9244016515855726
91,92,91,183,0.0054972171783447266,0.9005476780862695
92,93,92,185,0.005544900894165039,0.877788108339413
93,94,93,187,0.0055999755859375,0.8559998119210516
94,95,94,189,0.005647182464599609,0.8350802849518479
95,96,95,191,0.005693912506103516,0.814943911957379
96,97,96,193,0.005742073059082031,0.7955189020455389
97,98,97,195,0.005800008773803711,0.7767447841921623
98,99,98,197,0.005856037139892578,0.7585703634515314
100,101,100,201,0.005949974060058594,0.7238525299329535
101,102,101,203,0.005999088287353516,0.7072396070643435
102,103,102,205,0.006049156188964844,0.691085358165437
103,104,103,207,0.00609898567199707,0.6753653737326968
104,105,104,209,0.00614619255065918,0.6600581665352444
105,106,105,211,0.0061931610107421875,0.6451446845043806
106,107,106,213,0.006240129470825195,0.6306079126336457
107,108,107,215,0.006287097930908203,0.6164325470766233
109,110,109,219,0.0063931941986083984,0.5891118190180266
110,111,110,221,0.006442070007324219,0.5759422277900494
111,112,111,223,0.006500244140625,0.5630852547792591
112,113,112,225,0.0065572261810302734,0.5505309701534934
113,114,113,227,0.0066111087799072266,0.538270110635148
114,115,114,229,0.006667137145996094,0.5262939936488858
115,116,115,231,0.006724119186401367,0.5145944455065404
116,117,116,233,0.006781101226806641,0.5031637411246458
118,119,118,237,0.006887197494506836,0.48107990942512513
119,120,119,239,0.006942033767700195,0.4704131556739638
120,121,120,241,0.0069980621337890625,0.4599879252508989
121,122,121,243,0.007055044174194336,0.4497981121029822
122,123,122,245,0.007110118865966797,0.4398378479728607
123,124,123,247,0.0071659088134765625,0.4301014826454164
124,125,124,249,0.0072231292724609375,0.42058356681882325
125,126,125,251,0.0072782039642333984,0.41127883718828107
126,127,126,253,0.007333278656005859,0.4021822033978906
128,129,128,257,0.00745391845703125,0.38459365922365873
129,130,129,259,0.007521152496337891,0.3760923362355759
130,131,130,261,0.0075740814208984375,0.36778026692780263
131,132,131,263,0.007628202438354492,0.35965307789183115
132,133,132,265,0.007678031921386719,0.3517065165833811
133,134,133,267,0.007727146148681641,0.3439364455380017
134,135,134,269,0.007778167724609375,0.33633883713214574
135,136,135,271,0.007827043533325195,0.3289097688161205
137,138,137,275,0.007928133010864258,0.3145420618700312
138,139,138,277,0.007980108261108398,0.30759606609568313
139,140,139,279,0.008033037185668945,0.3008038890515508
140,141,140,281,0.008085012435913086,0.2941620748583548
141,142,141,283,0.008134126663208008,0.2876672512125353
142,143,142,285,0.008185148239135742,0.28131612664851496
143,144,143,287,0.008234024047851562,0.27510548797251766
144,145,144,289,0.008285284042358398,0.26903219785114363
145,146,145,291,0.008336067199707031,0.2630931925380429
147,148,147,295,0.008433103561401367,0.2516061365047946
148,149,148,297,0.008479118347167969,0.24605230743601103
149,150,149,299,0.008530139923095703,0.24062120269996232
150,151,150,301,0.008579015731811523,0.23531009634082653
151,152,151,303,0.008630990982055664,0.23011632458353506
152,153,152,305,0.008680105209350586,0.22503728422129732
153,154,153,307,0.008727073669433594,0.22007043106751703
154,155,154,309,0.008774280548095703,0.21521327846855828
156,157,156,313,0.008871316909790039,0.20581840743547744
157,158,157,315,0.008914947509765625,0.201275990713055
158,159,158,317,0.00896000862121582,0.19683387534527286
159,160,159,319,0.009008169174194336,0.19248984182186837
160,161,160,321,0.009057044982910156,0.18824172027180214
161,162,161,323,0.00910806655883789,0.1840873892908794
162,163,162,325,0.009163141250610352,0.1800247748063447
163,164,163,327,0.009213924407958984,0.17605184897228987
165,166,165,331,0.00931406021118164,0.16836717660636932
166,167,166,333,0.009371280670166016,0.16465159601749974
167,168,167,335,0.009427070617675781,0.16101803396446696
168,169,168,337,0.009484052658081055,0.15746467823137011
169,170,169,339,0.00953817367553711,0.15398975681713237
170,171,170,341,0.00959014892578125,0.15059153702358727
171,172,171,343,0.009639263153076172,0.14726832456674457
172,173,172,345,0.009767293930053711,0.14401846270960697
173,174,173,347,0.009890079498291016,0.14084033141634011
175,176,175,351,0.010036945343017578,0.1346929589560412
176,177,176,353,0.01010894775390625,0.131720653898841
177,178,177,355,0.010181188583374023,0.12881395007280683
178,179,178,357,0.010254144668579102,0.12597139896381346
179,180,179,359,0.01032400131225586,0.12319158409624681
180,181,180,361,0.010394096374511719,0.12047312031849117
181,182,181,363,0.010459184646606445,0.11781465310495985
182,183,182,365,0.010524272918701172,0.11521485787481088
184,185,184,369,0.010664939880371094,0.11018613078373568
185,186,185,371,0.010736227035522461,0.10775469356653737
186,187,186,373,0.010809183120727539,0.10537691636283472
187,188,187,375,0.01087808609008789,0.10305161462491585
188,189,188,377,0.010946035385131836,0.10077762997501194
189,190,189,379,0.011015892028808594,0.0985538296252799
190,191,190,381,0.011100292205810547,0.09637910581075006
191,192,191,383,0.011171102523803711,0.09425237523486613
192,193,192,385,0.011244058609008789,0.09217257852812377
194,195,194,389,0.01138615608215332,0.08814966570997212
195,196,195,391,0.011451244354248047,0.08620454578469486
196,197,196,393,0.011516332626342773,0.08430235109901553
197,198,197,395,0.011589288711547852,0.08244213420435499
198,199,198,397,0.011660099029541016,0.08062296857295405
199,200,199,399,0.011736154556274414,0.07884394813547066
200,201,200,401,0.011809110641479492,0.07710418682835267
201,202,201,403,0.011869192123413086,0.07540281815192632
203,204,203,407,0.011996269226074219,0.07211188792544311
204,205,204,409,0.012077093124389648,0.07052068735046704
205,206,205,411,0.012150049209594727,0.06896460053822821
206,207,206,413,0.012229204177856445,0.06744285251014266
207,208,207,415,0.012304067611694336,0.06595468539614385
208,209,208,417,0.01236104965209961,0.06449935805709435
209,210,209,419,0.012414932250976562,0.06307614571531585
210,211,210,421,0.012464284896850586,0.06168433959305711
212,213,212,425,0.012563943862915039,0.058992188781904396
213,214,213,427,0.012613058090209961,0.05769050339498308
214,215,214,429,0.012663125991821289,0.05641754216277564
215,216,215,431,0.012710094451904297,0.05517267115944222
216,217,216,433,0.012761116027832031,0.05395527045225669
217,218,217,435,0.012809991836547852,0.05276473379298964
218,219,218,437,0.012858152389526367,0.05160046831518218
219,220,219,439,0.012907028198242188,0.05046189423929462
220,221,220,441,0.012959957122802734,0.04934844458301679
222,223,222,445,0.013065099716186523,0.04719471289912895
223,224,223,447,0.013120174407958984,0.0461533583829401
224,225,224,449,0.013171911239624023,0.04513498277453306
225,226,225,451,0.013226032257080078,0.04413907896361874
226,227,226,453,0.013280153274536133,0.04316515103291216
227,228,227,455,0.013336181640625,0.04221271401114191
228,229,228,457,0.013392210006713867,0.04128129363107912
229,230,229,459,0.01345515251159668,0.040370426093512844
231,232,231,463,0.013586282730102539,0.03860854530644086
232,233,232,465,0.01377415657043457,0.03775665474323018
233,234,233,467,0.013926267623901367,0.036923561957991666
234,235,234,469,0.014014005661010742,0.036108852124683885
235,236,235,471,0.014101982116699219,0.035312119572801046
236,237,236,473,0.014246225357055664,0.034532967585366815
237,238,237,475,0.01439809799194336,0.033771008201202914
238,239,238,477,0.014467239379882812,0.033025862021703864
239,240,239,479,0.0145721435546875,0.032297158021608444
241,242,241,483,0.014898300170898438,0.03088763322196539
242,243,242,485,0.014952898025512695,0.030206110596187205
243,244,243,487,0.015007972717285156,0.029539626148107893
244,245,244,489,0.015061140060424805,0.028887848027625455
245,246,245,491,0.015115022659301758,0.02825045170848493
246,247,246,493,0.015166997909545898,0.027627119826772937
247,248,247,495,0.01521611213684082,0.027017542022629678
248,249,248,497,0.015267133712768555,0.02642141478560048
250,251,250,501,0.01536417007446289,0.02526833131510024
251,252,251,503,0.015410900115966797,0.024710800964211733
252,253,252,505,0.015461206436157227,0.024165572659698077
253,254,253,507,0.015510082244873047,0.023632374936395133
254,255,254,509,0.015559196472167969,0.02311094232001147
255,256,255,511,0.015614032745361328,0.022601015195210426
256,257,256,513,0.01566624641418457,0.022102339675920284
257,258,257,515,0.015716075897216797,0.0216146674790305
259,260,259,519,0.01581430435180664,0.020671367195368023
260,261,260,521,0.015864133834838867,0.020215269457740617
261,262,261,523,0.015916109085083008,0.019769235506674053
262,263,262,525,0.015965938568115234,0.01933304327246174
263,264,263,527,0.016016244888305664,0.018906475586043664
264,265,264,529,0.016068220138549805,0.018489320070924155
265,266,265,531,0.016117095947265625,0.01808136903730789
266,267,266,533,0.01616525650024414,0.01768241937871636
267,268,267,535,0.01621413230895996,0.01729227247087854
269,270,269,539,0.016316890716552734,0.016537614229555447
270,271,270,541,0.01636505126953125,0.016172727178671784
271,272,271,543,0.016413211822509766,0.01581589125677646
272,273,272,545,0.01646113395690918,0.015466928809089973
273,274,273,547,0.016510009765625,0.015125666101765278
274,275,274,549,0.016560077667236328,0.014791933234339825
275,276,275,551,0.01660919189453125,0.014465564056030411
276,277,276,553,0.01666092872619629,0.014146396082273438
278,279,278,557,0.016762256622314453,0.01352903165947384
279,280,279,559,0.016813039779663086,0.013230527854608152
280,281,280,561,0.01687312126159668,0.012938610389819786
281,282,281,563,0.016924142837524414,0.012653133934415074
282,283,282,565,0.016972064971923828,0.012373956364916703
283,284,283,567,0.01702404022216797,0.012100938693985177
284,285,284,569,0.01707601547241211,0.011833945001345908
285,286,285,571,0.01712512969970703,0.011572842365990538
286,287,286,573,0.01717519760131836,0.011317500800081029
288,289,288,577,0.017281055450439453,0.010823595204038973
289,290,289,579,0.017332077026367188,0.010584785288449066
290,291,290,581,0.017383337020874023,0.010351244548926114
291,292,291,583,0.017431020736694336,0.01012285672050335
292,293,292,585,0.017484188079833984,0.009899508103722574
293,294,293,587,0.01753711700439453,0.009681087508084397
294,295,294,589,0.017588138580322266,0.009467486196500128
295,296,295,591,0.01763916015625,0.009258597831661665
297,298,297,595,0.017742156982421875,0.008854546272220152
298,299,298,597,0.017797231674194336,0.008659181928993355
299,300,299,599,0.017856121063232422,0.008468128134932047
300,301,300,601,0.01790618896484375,0.008281289778366261
301,302,301,603,0.017956256866455078,0.008098573846115066
302,303,302,605,0.0180051326751709,0.007919889377944769
303,304,303,607,0.018053293228149414,0.007745147420329634
304,305,304,609,0.018100976943969727,0.007574260982682762
306,307,306,613,0.018198013305664062,0.007243716260558522
307,308,307,615,0.018246173858642578,0.0070838934240057124
308,309,308,617,0.0182950496673584,0.00692759692165988
309,310,309,619,0.01835799217224121,0.006774748945944709
310,311,310,621,0.018407106399536133,0.006625273406645923
311,312,311,623,0.018455028533935547,0.0064790958923083885
312,313,312,625,0.0185091495513916,0.006336143633428738
313,314,313,627,0.01856207847595215,0.006196345466146585
314,315,314,629,0.018620967864990234,0.0060596317969214735
316,317,316,633,0.01883411407470703,0.005795187222800078
317,318,317,635,0.01890110969543457,0.005667324674212056
318,319,318,637,0.01896500587463379,0.005542283270418612
319,320,319,639,0.019024133682250977,0.0054200007646637485
320,321,320,641,0.01908397674560547,0.005300416283589236
321,322,321,643,0.01914215087890625,0.005183470296844416
322,323,322,645,0.019204139709472656,0.00506910458764676
323,324,323,647,0.019260168075561523,0.004957262224031962
325,326,325,651,0.019360065460205078,0.004740926058266062
326,327,326,653,0.0194091796875,0.004636324562670909
327,328,327,655,0.019459009170532227,0.00453403097209422
328,329,328,657,0.01950693130493164,0.004433994364295724
329,330,329,659,0.019556045532226562,0.004336164940756072
330,331,330,661,0.01960611343383789,0.0042404940016833705
331,332,331,663,0.019654273986816406,0.004146933921796279
332,333,332,665,0.019704103469848633,0.004055438126812003
333,334,333,667,0.01975393295288086,0.003965961069901882
335,336,335,671,0.01986098289489746,0.0037928859863058315
336,337,336,673,0.01991415023803711,0.003709201802807134
337,338,337,675,0.019964218139648438,0.0036273640010897447
338,339,338,677,0.020017147064208984,0.003547331842487434
339,340,339,679,0.0200650691986084,0.003469065486941077
340,341,340,681,0.020113229751586914,0.0033925259738433505
341,342,341,683,0.020169973373413086,0.003317675202018212
342,343,342,685,0.020229101181030273,0.0032444759110702307
344,345,344,689,0.020355224609375,0.0031028868225573786
345,346,345,691,0.02040410041809082,0.0030344265425757007
346,347,346,693,0.020457983016967773,0.0029674767437474956
347,348,347,695,0.020509958267211914,0.0029020040988726337
348,349,348,697,0.020562171936035156,0.0028379760159543406
349,350,349,699,0.020617008209228516,0.0027753606224816493
350,351,350,701,0.020676136016845703,0.0027141267488115226
351,352,351,703,0.020731210708618164,0.0026542439133317355
353,354,353,707,0.02086019515991211,0.002538412777898195
354,355,354,709,0.020919084548950195,0.0024824068182858323
355,356,355,711,0.02108597755432129,0.0024276365488350377
356,357,356,713,0.021146059036254883,0.0023740747054084564
357,358,357,715,0.021206140518188477,0.0023216946254579246
358,359,358,717,0.02126312255859375,0.002270470234856464
359,360,359,719,0.02131819725036621,0.002220376034630402
360,361,360,721,0.02137303352355957,0.0021713870884986332
361,362,361,723,0.02142620086669922,0.0021234790104403267
363,364,363,727,0.021529197692871094,0.0020308105923713066
364,365,364,729,0.021602153778076172,0.0019860041232063115
365,366,365,731,0.0216519832611084,0.0019421862408806278
366,367,366,733,0.02171611785888672,0.0018993351335563834
367,368,367,735,0.021783113479614258,0.0018574294703631086
368,369,368,737,0.02184605598449707,0.0018164483915243427
369,370,369,739,0.021906137466430664,0.0017763714970246193
370,371,370,741,0.021959304809570312,0.001737178837425108
372,373,372,745,0.02207207679748535,0.0016613686151898824
373,374,373,747,0.022127151489257812,0.0016247133155114992
374,375,374,749,0.02218008041381836,0.0015888667577107253
375,376,375,751,0.022234201431274414,0.0015538110979405233
376,377,376,753,0.02228522300720215,0.0015195288861689546
377,378,377,755,0.022335052490234375,0.0014860030572434733
378,379,378,757,0.02238321304321289,0.0014532169226734687
379,380,379,759,0.02243208885192871,0.0014211541621291632
381,382,381,763,0.022533178329467773,0.001359135274173557
382,383,382,765,0.022584199905395508,0.0013291482749761734
383,384,383,767,0.022633075714111328,0.0012998228907309397
384,385,384,769,0.022683143615722656,0.0012711445239768399
385,386,385,771,0.022755146026611328,0.0012430988990539266
386,387,386,773,0.02281808853149414,0.0012156720554441448
387,388,387,775,0.022869110107421875,0.001188850340711998
388,389,388,777,0.022918224334716797,0.0011626204035876506
389,390,389,779,0.02297806739807129,0.0011369691871740788
391,392,391,783,0.02308821678161621,0.0010873521240182607
392,393,392,785,0.02313709259033203,0.0010633615790484763
393,394,393,787,0.023186206817626953,0.0010399003459303292
394,395,394,789,0.023234128952026367,0.0010169567463381558
395,396,395,791,0.023283958435058594,0.0009945193593081172
396,397,396,793,0.023333072662353516,0.0009725770161415304
397,398,397,795,0.023382186889648438,0.0009511187942865064
398,399,398,797,0.02343010902404785,0.0009301340125132091
400,401,400,801,0.023529052734375,0.0008895432165369584
401,402,401,803,0.023586034774780273,0.0008699169972282329
402,403,402,805,0.023637056350708008,0.0008507237975506286
403,404,403,807,0.023687124252319336,0.0008319540636327136
404,405,404,809,0.023736238479614258,0.0008135984524119996
405,406,405,811,0.023785114288330078,0.0007956478267911205
406,407,406,813,0.023835182189941406,0.0007780932514565319
407,408,407,815,0.023897171020507812,0.0007609259882423864
408,409,408,817,0.023946046829223633,0.0007441374915818346
410,411,410,821,0.02404308319091797,0.0007116635550997141
411,412,411,823,0.024091243743896484,0.0006959619504981624
412,413,412,825,0.024140119552612305,0.0006806067750341397
413,414,413,827,0.02418828010559082,0.00066559038542363
414,415,414,829,0.02423715591430664,0.0006509053066785315
415,416,415,831,0.024285316467285156,0.0006365442292159629
416,417,416,833,0.024334192276000977,0.0006225000043531535
417,418,417,835,0.02438211441040039,0.0006087656412060647
419,420,419,839,0.02448105812072754,0.0005821993045239375
420,421,420,841,0.02454400062561035,0.0005693541070361438
421,422,421,843,0.02459430694580078,0.000556792316733283
422,423,422,845,0.0246431827545166,0.000544507680675588
423,424,423,847,0.024693012237548828,0.0005324940838787319
424,425,424,849,0.02474212646484375,0.0005207455462751963
425,426,425,851,0.024796247482299805,0.0005092562198128969
426,427,426,853,0.024845123291015625,0.0004980203854446273
428,429,428,857,0.02495408058166504,0.0004762869448231322
429,430,429,859,0.025004148483276367,0.00046577852031052386
430,431,430,861,0.02505326271057129,0.00045550194583977
431,432,431,863,0.025103092193603516,0.00044545210604646397
432,433,432,865,0.025151968002319336,0.0004356239985420073
433,434,433,867,0.02520132064819336,0.00042601273098715083
434,435,434,869,0.02525019645690918,0.0004166135193066767
435,436,435,871,0.025303125381469727,0.0004074216846904455
436,437,436,873,0.025355100631713867,0.0003984326519324887
438,439,438,877,0.02546405792236328,0.00038104519235047235
439,440,439,879,0.025519132614135742,0.00037263811061508486
440,441,440,881,0.025577068328857422,0.0003644165163252031
441,442,441,883,0.025630950927734375,0.00035637631700843935
442,443,442,885,0.025686979293823242,0.0003485135106554684
443,444,443,887,0.02573704719543457,0.00034082418331530276
444,445,444,889,0.0257871150970459,0.00033330450730031225
445,446,445,891,0.02583599090576172,0.0003259507397382472
447,448,447,895,0.02592611312866211,0.0003117263686212227
448,449,448,897,0.0259702205657959,0.0003048486845830723
449,450,449,899,0.02602410316467285,0.0002981227444833437
450,451,450,901,0.026069164276123047,0.0002915452002944949
451,452,451,903,0.02611517906188965,0.0002851127780188185
452,453,452,905,0.026159048080444336,0.0002788222757495641
453,454,453,907,0.02620410919189453,0.00027267056219192786
454,455,454,909,0.026248931884765625,0.0002666545753837897
455,456,455,911,0.026293039321899414,0.0002607713206044924
457,458,457,915,0.02639007568359375,0.00024939135781170443
458,459,458,917,0.026435136795043945,0.0002438889851708443
459,460,459,919,0.026479244232177734,0.00023850801279715913
460,461,460,921,0.026523113250732422,0.00023324576178378092
461,462,461,923,0.02656722068786621,0.0002280996130182831
462,463,462,925,0.0266110897064209,0.00022306700489038345
463,464,463,927,0.026654958724975586,0.00021814543226725947
464,465,464,929,0.026699066162109375,0.00021333244544563738
466,467,466,933,0.02678704261779785,0.0002040226986784891
467,468,467,935,0.0268402099609375,0.00019952130472560386
468,469,468,937,0.02690410614013672,0.00019511922594162056
469,470,469,939,0.0269622802734375,0.00019081427110839326
470,471,470,941,0.02701711654663086,0.00018660429744396553
471,472,471,943,0.027081966400146484,0.00018248720943802313
472,473,472,945,0.02714705467224121,0.00017846095745648687
473,474,473,947,0.02721714973449707,0.00017452353756411317
475,476,475,951,0.027337074279785156,0.0001669073975079821
476,477,476,953,0.027390003204345703,0.00016322488627652334
477,478,477,955,0.02744007110595703,0.00015962362298147802
478,479,478,957,0.027492046356201172,0.0001561018151307343
479,480,479,959,0.027543067932128906,0.00015265770960735177
480,481,480,961,0.027595043182373047,0.00014928959219188886
481,482,481,963,0.027644872665405273,0.00014599578618782507
482,483,482,965,0.02769613265991211,0.00014277465197764383
483,484,483,967,0.02774500846862793,0.00013962458644032594
485,486,485,971,0.027848005294799805,0.00013353142362952175
486,487,486,973,0.027900218963623047,0.00013058529327932353
487,488,487,975,0.02794814109802246,0.0001277041640419485
488,489,488,977,0.027997970581054688,0.00012488660164821264
489,490,489,979,0.028050899505615234,0.00012213120382541706
490,491,490,981,0.028103113174438477,0.00011943659879708779
491,492,491,983,0.02815413475036621,0.00011680144544541835
492,493,492,985,0.02822089195251465,0.00011422443197714823
494,495,494,989,0.028335094451904297,0.00010923972211164034
495,496,495,991,0.028388261795043945,0.0001068295445142591
496,497,496,993,0.028437137603759766,0.00010447254305295783
497,498,497,995,0.028487205505371094,0.00010216754466810359
498,499,498,997,0.02853703498840332,9.991340187399322e-05
499,500,499,999,0.02858901023864746,9.770899270171721e-05
500,501,500,1001,0.028757095336914062,9.555321981155082e-05
501,502,501,1003,0.028810977935791016,9.344501013330934e-05
502,503,502,1005,0.02886509895324707,9.138331437774592e-05
504,505,504,1009,0.0290071964263916,8.73953820104558e-05
505,506,505,1011,0.029067039489746094,8.546716040661085e-05
506,507,506,1013,0.029125213623046875,8.35814814251813e-05
507,508,507,1015,0.029177188873291016,8.173740667065195e-05
508,509,508,1017,0.029226064682006836,7.993401804793474e-05
509,510,509,1019,0.029275178909301758,7.817041790931796e-05
510,511,510,1021,0.029325008392333984,7.64457284195039e-05
511,512,511,1023,0.029374122619628906,7.475909115153156e-05
513,514,513,1027,0.02948927879333496,7.149663337774589e-05
514,515,514,1029,0.0295412540435791,6.99191888711393e-05
515,516,515,1031,0.029588937759399414,6.837654789916817e-05
516,517,516,1033,0.02963709831237793,6.686794247241582e-05
517,518,517,1035,0.029688119888305664,6.53926217593597e-05
518,519,518,1037,0.029736042022705078,6.394985139440869e-05
519,520,519,1039,0.029801130294799805,6.253891304463458e-05
520,521,520,1041,0.029868125915527344,6.115910453853819e-05
522,523,522,1045,0.029986143112182617,5.849014476254239e-05
523,524,523,1047,0.03003716468811035,5.719966501464566e-05
524,525,524,1049,0.03009510040283203,5.593765734506459e-05
525,526,525,1051,0.03014516830444336,5.470349362255527e-05
526,527,526,1053,0.030222177505493164,5.3496559460289176e-05
527,528,527,1055,0.03032231330871582,5.231625413029969e-05
528,529,528,1057,0.03038620948791504,5.116199016487273e-05
529,530,529,1059,0.030440092086791992,5.00331928456284e-05
530,531,530,1061,0.030504941940307617,4.892930052189755e-05
532,533,532,1065,0.030620098114013672,4.6794044599315275e-05
533,534,533,1067,0.030678987503051758,4.576161808577329e-05
534,535,534,1069,0.03075408935546875,4.475197034333764e-05
535,536,535,1071,0.030820131301879883,4.376459861479928e-05
536,537,536,1073,0.03088212013244629,4.279901135879732e-05
537,538,537,1075,0.030935049057006836,4.1854728105493055e-05
538,539,538,1077,0.030994892120361328,4.09312788140013e-05
539,540,539,1079,0.031057119369506836,4.002820380574834e-05
541,542,541,1083,0.03125715255737305,3.8281388102905975e-05
542,543,542,1085,0.03132009506225586,3.743677814035546e-05
543,544,543,1087,0.03137516975402832,3.6610802887881596e-05
544,545,544,1089,0.03142714500427246,3.5803051288177883e-05
545,546,545,1091,0.03147602081298828,3.501312131179703e-05
546,547,546,1093,0.0315251350402832,3.424061961152563e-05
547,548,547,1095,0.03157925605773926,3.348516187301133e-05
548,549,548,1097,0.03163433074951172,3.2746371961816424e-05
549,550,549,1099,0.03168630599975586,3.202388201827929e-05
551,552,551,1103,0.03179121017456055,3.062637190340981e-05
552,553,552,1105,0.031852006912231445,2.995065596274533e-05
553,554,553,1107,0.03191113471984863,2.9289848460117702e-05
554,555,554,1109,0.0319669246673584,2.8643620547034954e-05
555,556,555,1111,0.03201723098754883,2.8011650476893378e-05
556,557,556,1113,0.03208303451538086,2.739362370577914e-05
557,558,557,1115,0.032241106033325195,2.6789232533047214e-05
558,559,558,1117,0.03232622146606445,2.619817618477594e-05
560,561,560,1121,0.03247809410095215,2.5054897491730444e-05
561,562,561,1123,0.03255200386047363,2.4502106111425138e-05
562,563,562,1125,0.032636165618896484,2.3961511063870686e-05
563,564,563,1127,0.03271293640136719,2.3432843326983816e-05
564,565,564,1129,0.03278803825378418,2.2915839643044647e-05
565,566,565,1131,0.032861948013305664,2.2410242742690288e-05
566,567,566,1133,0.032935142517089844,2.1915800878648077e-05
567,568,567,1135,0.03301715850830078,2.1432267966289655e-05
569,570,569,1139,0.03316926956176758,2.0496971741710957e-05
570,571,570,1141,0.03324317932128906,2.0044742782821493e-05
571,572,571,1143,0.03331303596496582,1.960249140877116e-05
572,573,572,1145,0.03337812423706055,1.9169997497325298e-05
573,574,573,1147,0.03344106674194336,1.8747045915038646e-05
574,575,574,1149,0.03350019454956055,1.8333425847695867e-05
575,576,575,1151,0.03355813026428223,1.7928931614885288e-05
576,577,576,1153,0.033618927001953125,1.7533361831711555e-05
577,578,577,1155,0.03369712829589844,1.714651961487854e-05
579,580,579,1159,0.0338139533996582,1.6398251726976647e-05
580,581,580,1161,0.033872127532958984,1.6036453657002352e-05
581,582,581,1163,0.03392624855041504,1.5682637960461056e-05
582,583,582,1165,0.03397512435913086,1.533662861764422e-05
583,584,583,1167,0.03402113914489746,1.4998253370522472e-05
584,585,584,1169,0.03406810760498047,1.466734371549774e-05
585,586,585,1171,0.03411412239074707,1.4343735006879948e-05
586,587,586,1173,0.03416013717651367,1.4027266095202094e-05
588,589,588,1177,0.03425097465515137,1.3415121257379603e-05
589,590,589,1179,0.03429722785949707,1.3119140561632764e-05
590,591,590,1181,0.03434324264526367,1.2829690172369761e-05
591,592,591,1183,0.034388065338134766,1.2546626056621504e-05
592,593,592,1185,0.03443312644958496,1.2269807099142835e-05
593,594,593,1187,0.03449821472167969,1.1999095756601988e-05
594,595,594,1189,0.034545183181762695,1.1734357125613668e-05
595,596,595,1191,0.034590959548950195,1.147545951841564e-05
596,597,596,1193,0.03463602066040039,1.1222273899534506e-05
598,599,598,1197,0.03473615646362305,1.073253790096571e-05
599,600,599,1199,0.03478193283081055,1.0495743556390904e-05
600,601,600,1201,0.03482818603515625,1.026417380226636e-05
601,602,601,1203,0.034873247146606445,1.0037713114797126e-05
602,603,602,1205,0.0349271297454834,9.816248798092387e-06
603,604,603,1207,0.03499007225036621,9.5996707806142e-06
604,605,604,1209,0.03504514694213867,9.387871140007273e-06
605,606,605,1211,0.03510403633117676,9.180744572332782e-06
607,608,607,1215,0.035218238830566406,8.780100079731466e-06
608,609,608,1217,0.03527712821960449,8.586382819728773e-06
609,610,609,1219,0.03533315658569336,8.396939553760424e-06
610,611,610,1221,0.0353851318359375,8.211676086458847e-06
611,612,611,1223,0.03544116020202637,8.03050010004875e-06
612,613,612,1225,0.03549814224243164,7.853321381183909e-06
613,614,613,1227,0.03555417060852051,7.680051879319413e-06
614,615,614,1229,0.03561115264892578,7.510605193323619e-06
616,617,616,1233,0.03573107719421387,7.1828450088324e-06
617,618,617,1235,0.03578329086303711,7.0243683255315075e-06
618,619,618,1237,0.03583526611328125,6.869388050636138e-06
619,620,619,1239,0.03590106964111328,6.717827241530595e-06
620,621,620,1241,0.035954952239990234,6.569610333463776e-06
621,622,621,1243,0.03600788116455078,6.424663659676869e-06
622,623,622,1245,0.03605914115905762,6.282914856783892e-06
623,624,623,1247,0.03611111640930176,6.144293487035874e-06
624,625,624,1249,0.03616619110107422,6.008730613422601e-06
626,627,626,1253,0.03627419471740723,5.746511639084111e-06
627,628,627,1255,0.03632712364196777,5.619725042337856e-06
628,629,628,1257,0.03638195991516113,5.4957358112185855e-06
629,630,629,1259,0.03643488883972168,5.3744821955023395e-06
630,631,630,1261,0.03648996353149414,5.2559037911301126e-06
631,632,631,1263,0.03654813766479492,5.139941609107002e-06
632,633,632,1265,0.03660702705383301,5.026537915327715e-06
633,634,633,1267,0.03666520118713379,4.915636345795654e-06
635,636,635,1271,0.036787986755371094,4.701119595481944e-06
636,637,636,1273,0.03684520721435547,4.597397743313911e-06
637,638,637,1275,0.03690505027770996,4.495964367146191e-06
638,639,638,1277,0.036962032318115234,4.39676883429937e-06
639,640,639,1279,0.03701925277709961,4.2997619852263335e-06
640,641,640,1281,0.037075042724609375,4.204895308450411e-06
641,642,641,1283,0.03714609146118164,4.112121776189699e-06
642,643,642,1285,0.03720211982727051,4.021395121394591e-06
643,644,643,1287,0.03726005554199219,3.9326701829827235e-06
645,646,645,1291,0.037371158599853516,3.7610497503306316e-06
646,647,646,1293,0.03742408752441406,3.678068793978288e-06
647,648,647,1295,0.03748202323913574,3.5969187349361283e-06
648,649,648,1297,0.03753399848937988,3.5175591468015492e-06
649,650,649,1299,0.037592172622680664,3.4399504725355412e-06
650,651,650,1301,0.037644147872924805,3.3640540630372703e-06
651,652,651,1303,0.03769397735595703,3.2898321764271736e-06
652,653,652,1305,0.03775620460510254,3.21724781858177e-06
654,655,654,1309,0.03786802291870117,3.076848169588334e-06
655,656,655,1311,0.0379180908203125,3.0089629848484995e-06
656,657,656,1313,0.03796815872192383,2.9425755814350398e-06
657,658,657,1315,0.038021087646484375,2.877652863714514e-06
658,659,658,1317,0.0380711555480957,2.814162513898904e-06
659,660,659,1319,0.03812098503112793,2.7520730329928966e-06
660,661,660,1321,0.03817009925842285,2.6913533677408062e-06
661,662,661,1323,0.03821897506713867,2.631973423397246e-06
663,664,663,1327,0.038329124450683594,2.5171150248078965e-06
664,665,664,1329,0.03838205337524414,2.4615792462423223e-06
665,666,665,1331,0.038436174392700195,2.407268895559149e-06
666,667,666,1333,0.03848600387573242,2.354156759653852e-06
667,668,667,1335,0.038535118103027344,2.302216447023986e-06
668,669,668,1337,0.03858828544616699,2.2514221810142497e-06
669,670,669,1339,0.03864288330078125,2.2017484510185646e-06
670,671,670,1341,0.038695335388183594,2.153170739027289e-06
671,672,671,1343,0.03875303268432617,2.105664858217672e-06
673,674,673,1347,0.03886008262634277,2.013774382500487e-06
674,675,674,1349,0.038908958435058594,1.969343968177682e-06
675,676,675,1351,0.038958072662353516,1.925893863786272e-06
676,677,676,1353,0.03900599479675293,1.8834024075715177e-06
677,678,677,1355,0.03905510902404785,1.841848446763889e-06
678,679,678,1357,0.039103031158447266,1.801211357843122e-06
679,680,679,1359,0.039153099060058594,1.7614707630764573e-06
680,681,680,1361,0.03920722007751465,1.7226070849480532e-06
682,683,682,1365,0.03931593894958496,1.6474330689307458e-06
683,684,683,1367,0.03937506675720215,1.6110853533109158e-06
684,685,684,1369,0.0394282341003418,1.5755395911326025e-06
685,686,685,1371,0.03948330879211426,1.5407780802643647e-06
686,687,686,1373,0.039541006088256836,1.506783562425623e-06
687,688,687,1375,0.03959918022155762,1.4735389978565335e-06
688,689,688,1377,0.0396580696105957,1.4410280063072856e-06
689,690,689,1379,0.03971409797668457,1.409234248255263e-06
690,691,690,1381,0.03977012634277344,1.378142026099197e-06
692,693,692,1385,0.03988504409790039,1.3180002755368412e-06
693,694,693,1387,0.03994107246398926,1.2889209379654233e-06
694,695,694,1389,0.039999961853027344,1.2604831577851149e-06
695,696,695,1391,0.04006505012512207,1.2326728215292235e-06
696,697,696,1393,0.04012918472290039,1.205476038054604e-06
697,698,697,1395,0.040183067321777344,1.178879350396357e-06
698,699,698,1397,0.040242910385131836,1.1528695055305866e-06
699,700,699,1399,0.040299177169799805,1.1274334165044736e-06
701,702,701,1403,0.04041910171508789,1.0782326142834613e-06
702,703,702,1405,0.04047513008117676,1.0544432433239328e-06
703,704,703,1407,0.04052925109863281,1.0311788650790242e-06
704,705,704,1409,0.040592193603515625,1.008427745528241e-06
705,706,705,1411,0.04064321517944336,9.861785216098412e-07
706,707,706,1413,0.04069209098815918,9.644202303777127e-07
707,708,707,1415,0.04074215888977051,9.431420652827042e-07
708,709,708,1417,0.04079413414001465,9.223332964752158e-07
710,711,710,1421,0.0408940315246582,8.820829368095245e-07
711,712,711,1423,0.04094409942626953,8.626212848196172e-07
712,713,712,1425,0.040995121002197266,8.43589082594216e-07
713,714,713,1427,0.041047096252441406,8.249767900084509e-07
714,715,714,1429,0.04109907150268555,8.067751408965151e-07
715,716,715,1431,0.04115724563598633,7.889750263116452e-07
716,717,716,1433,0.04120802879333496,7.715676966880661e-07
717,718,717,1435,0.041262149810791016,7.545444083162037e-07
718,719,718,1437,0.041322946548461914,7.378967214263209e-07
720,721,720,1441,0.041439056396484375,7.056951138074819e-07
721,722,721,1443,0.041494131088256836,6.901251915563995e-07
722,723,722,1445,0.04155111312866211,6.748988152946452e-07
723,724,723,1447,0.0416109561920166,6.600083922058918e-07
724,725,724,1449,0.041676998138427734,6.454464139400006e-07
725,726,725,1451,0.04173111915588379,6.312057537515734e-07
726,727,726,1453,0.04179501533508301,6.172793685234022e-07
727,728,727,1455,0.04184913635253906,6.036601335365658e-07
729,730,729,1459,0.04196619987487793,5.773165605838908e-07
730,731,730,1461,0.04202008247375488,5.645791424772669e-07
731,732,731,1463,0.04207205772399902,5.521226851784786e-07
732,733,732,1465,0.042124032974243164,5.399410730473839e-07
733,734,733,1467,0.04218006134033203,5.280281874634792e-07
734,735,734,1469,0.042236328125,5.163781983293458e-07
735,736,735,1471,0.042292118072509766,5.049852395870402e-07
736,737,736,1473,0.0423431396484375,4.938436345467465e-07
737,738,737,1475,0.042391061782836914,4.829478075865091e-07
739,740,739,1479,0.04250025749206543,4.6187206694494e-07
740,741,740,1481,0.04255104064941406,4.5168176141041903e-07
741,742,741,1483,0.04260396957397461,4.417161433208081e-07
742,743,742,1485,0.04267311096191406,4.319704450601988e-07
743,744,743,1487,0.04273724555969238,4.224397756114437e-07
744,745,744,1489,0.04278826713562012,4.131193965069388e-07
745,746,745,1491,0.04283905029296875,4.0400458577039963e-07
746,747,746,1493,0.042893171310424805,3.9509096325499146e-07
748,749,748,1497,0.043015241622924805,3.77849339046309e-07
749,750,749,1499,0.04306817054748535,3.6951276067188404e-07
750,751,750,1501,0.04312396049499512,3.61360088952392e-07
751,752,751,1503,0.043203115463256836,3.533873216133514e-07
752,753,752,1505,0.0432581901550293,3.455904553298304e-07
753,754,753,1507,0.04331207275390625,3.379655936787451e-07
754,755,754,1509,0.04336404800415039,3.30509051863949e-07
755,756,755,1511,0.04341411590576172,3.232169188894218e-07
757,758,757,1515,0.04351210594177246,3.091117659809256e-07
758,759,758,1517,0.043560028076171875,3.022918048535821e-07
759,760,759,1519,0.04360818862915039,2.956222157933265e-07
760,761,760,1521,0.043656110763549805,2.8909984433605273e-07
761,762,761,1523,0.04373311996459961,2.8272136216876104e-07
762,763,762,1525,0.04378318786621094,2.7648364397246845e-07
763,764,763,1527,0.043836116790771484,2.7038347409746545e-07
764,765,764,1529,0.0438840389251709,2.644180292598069e-07
765,766,765,1531,0.04393506050109863,2.5858406466584117e-07
767,768,767,1535,0.04403996467590332,2.472995094144579e-07
768,769,768,1537,0.04409909248352051,2.41843263453762e-07
769,770,769,1539,0.04415106773376465,2.3650740564686016e-07
770,771,770,1541,0.04419994354248047,2.3128932930127086e-07
771,772,771,1543,0.04425406455993652,2.261863480547186e-07
772,773,772,1545,0.04430413246154785,2.2119596595229156e-07
773,774,773,1547,0.04435300827026367,2.163156238664275e-07
774,775,774,1549,0.04440116882324219,2.115430190658377e-07
776,777,776,1553,0.04449892044067383,2.0231137149454668e-07
777,778,777,1555,0.044547080993652344,1.9784769026655788e-07
778,779,778,1557,0.04459500312805176,1.934825441925951e-07
779,780,779,1559,0.044646263122558594,1.8921365775728508e-07
780,781,780,1561,0.04469704627990723,1.8503896812809455e-07
781,782,781,1563,0.04474902153015137,1.8095642704366183e-07
782,783,782,1565,0.04479622840881348,1.7696396293197097e-07
783,784,783,1567,0.0448451042175293,1.730595294596731e-07
785,786,785,1571,0.04494619369506836,1.6550723638749725e-07
786,787,786,1573,0.044997215270996094,1.6185564251320335e-07
787,788,787,1575,0.045046091079711914,1.5828459230159952e-07
788,789,788,1577,0.04509711265563965,1.5479224143548598e-07
789,790,789,1579,0.04515719413757324,1.5137708358770283e-07
790,791,790,1581,0.04520606994628906,1.4803719284836342e-07
791,792,791,1583,0.045255184173583984,1.447710298904865e-07
792,793,792,1585,0.0453031063079834,1.4157695820163265e-07
793,794,793,1587,0.045352935791015625,1.3845325490815582e-07
795,796,795,1591,0.04545712471008301,1.3241117093449674e-07
796,797,796,1593,0.04551196098327637,1.294898018593051e-07
797,798,797,1595,0.04557204246520996,1.2663276417752112e-07
798,799,798,1597,0.04562997817993164,1.238388225291177e-07
799,800,799,1599,0.04568123817443848,1.2110659293946272e-07
800,801,800,1601,0.045736074447631836,1.184345982212447e-07
801,802,801,1603,0.045786142349243164,1.1582158163289262e-07
802,803,802,1605,0.04583406448364258,1.1326612619698239e-07
804,805,804,1609,0.045931100845336914,1.0832320398074545e-07
805,806,805,1611,0.04597926139831543,1.0593327423842855e-07
806,807,806,1613,0.046035051345825195,1.0359599622572091e-07
807,808,807,1615,0.04609107971191406,1.0131035502986396e-07
808,809,808,1617,0.0461421012878418,9.907515899904498e-08
809,810,809,1619,0.04620003700256348,9.68892116020239e-08
810,811,810,1621,0.046253204345703125,9.47515484461297e-08
811,812,811,1623,0.04631400108337402,9.26609564973877e-08
812,813,812,1625,0.046372175216674805,9.061661896596692e-08
814,815,814,1629,0.04647111892700195,8.666208717900616e-08
815,816,815,1631,0.046520233154296875,8.475008649181929e-08
816,817,816,1633,0.046569108963012695,8.28802330205764e-08
817,818,817,1635,0.04662013053894043,8.105157206387547e-08
818,819,818,1637,0.046671152114868164,7.926328102977443e-08
819,820,819,1639,0.046720027923583984,7.751451594486375e-08
820,821,820,1641,0.046772003173828125,7.580430753950502e-08
821,822,821,1643,0.04682612419128418,7.413180990485593e-08
823,824,823,1647,0.04692816734313965,7.089668563869345e-08
824,825,824,1649,0.04697704315185547,6.933248178719568e-08
825,826,825,1651,0.0470280647277832,6.780276916786294e-08
826,827,826,1653,0.047077178955078125,6.630687474330182e-08
827,828,827,1655,0.04712820053100586,6.484389626683674e-08
828,829,828,1657,0.047181129455566406,6.341330637283197e-08
829,830,829,1659,0.04723715782165527,6.201410084642774e-08
830,831,830,1661,0.047289133071899414,6.06458921759559e-08
832,833,832,1665,0.04739999771118164,5.79993119021972e-08
833,834,833,1667,0.04744911193847656,5.6719704939520123e-08
834,835,834,1669,0.047495126724243164,5.5468323017518135e-08
835,836,835,1671,0.047541141510009766,5.4244418319341976e-08
836,837,836,1673,0.04758715629577637,5.304766160685583e-08
837,838,837,1675,0.04763317108154297,5.187723804131085e-08
838,839,838,1677,0.04768514633178711,5.073260568866374e-08
839,840,839,1679,0.04775118827819824,4.961335859650853e-08
840,841,840,1681,0.0478060245513916,4.851871299936514e-08
842,843,842,1685,0.047942161560058594,4.640138391409565e-08
843,844,843,1687,0.04799914360046387,4.537756897807567e-08
844,845,844,1689,0.048052072525024414,4.4376407311604886e-08
845,846,845,1691,0.048104047775268555,4.3397286081131866e-08
846,847,846,1693,0.0481572151184082,4.2439859543538944e-08
847,848,847,1695,0.04820704460144043,4.1503458534923824e-08
848,849,848,1697,0.048258066177368164,4.058774994009136e-08
849,850,849,1699,0.04830813407897949,3.969229186058963e-08
851,852,851,1703,0.04840803146362305,3.7960141130944464e-08
852,853,852,1705,0.048461198806762695,3.712256274467641e-08
853,854,853,1707,0.048528194427490234,3.630359743787117e-08
854,855,854,1709,0.04858708381652832,3.5502554666803064e-08
855,856,855,1711,0.04864096641540527,3.471928488101185e-08
856,857,856,1713,0.0486910343170166,3.395320631848644e-08
857,858,857,1715,0.04874396324157715,3.320416942878849e-08
858,859,858,1717,0.048799991607666016,3.247156331590995e-08
859,860,859,1719,0.04885506629943848,3.1755154900523255e-08
861,862,861,1723,0.0491330623626709,3.0369327681157295e-08
862,863,862,1725,0.049202919006347656,2.9699277601940575e-08
863,864,863,1727,0.04925894737243652,2.9044039310921153e-08
864,865,864,1729,0.049329280853271484,2.8403183536860323e-08
865,866,865,1731,0.04938912391662598,2.7776568484012757e-08
866,867,866,1733,0.04944014549255371,2.7163733806255592e-08
867,868,867,1735,0.04949307441711426,2.6564423103106056e-08
868,869,868,1737,0.049543142318725586,2.597825274483951e-08
870,871,870,1741,0.049642086029052734,2.4844537673663018e-08
871,872,871,1743,0.04969334602355957,2.4296434518171103e-08
872,873,872,1745,0.04974532127380371,2.3760409219380607e-08
873,874,873,1747,0.04979419708251953,2.323616362093626e-08
874,875,874,1749,0.04985308647155762,2.2723497643857263e-08
875,876,875,1751,0.049900054931640625,2.2222119945107167e-08
876,877,876,1753,0.04994916915893555,2.173183627514593e-08
877,878,877,1755,0.049996137619018555,2.1252373723919184e-08
879,880,879,1759,0.05009317398071289,2.0324899999935675e-08
880,881,880,1761,0.05014300346374512,1.9876545030387486e-08
881,882,881,1763,0.05019211769104004,1.943795644356426e-08
882,883,882,1765,0.05023908615112305,1.9009082789223923e-08
883,884,883,1767,0.05028414726257324,1.8589696798087862e-08
884,885,884,1769,0.050330162048339844,1.817952750319496e-08
885,886,885,1771,0.050379037857055664,1.7778418544572487e-08
886,887,886,1773,0.050428152084350586,1.7386211618231685e-08
887,888,887,1775,0.05047607421875,1.700254833670357e-08
889,890,889,1779,0.0505681037902832,1.6260596359590516e-08
890,891,890,1781,0.0506131649017334,1.590185993762055e-08
891,892,891,1783,0.05065798759460449,1.555097081173522e-08
892,893,892,1785,0.0507051944732666,1.5207854209232705e-08
893,894,893,1787,0.0507509708404541,1.4872318803928916e-08
894,895,894,1789,0.05079817771911621,1.454423931323791e-08
895,896,895,1791,0.05084419250488281,1.4223275804343702e-08
896,897,896,1793,0.0509030818939209,1.3909549698451643e-08
898,899,898,1797,0.051004886627197266,1.330251211650884e-08
899,900,899,1799,0.05106210708618164,1.3009013205402411e-08
900,901,900,1801,0.051115989685058594,1.272203494847914e-08
901,902,901,1803,0.05116415023803711,1.2441328695625799e-08
902,903,902,1805,0.05121207237243652,1.216679054415826e-08
903,904,903,1807,0.051258087158203125,1.189840592894953e-08
904,905,904,1809,0.05130410194396973,1.1635849481458407e-08
905,906,905,1811,0.05135011672973633,1.137912801501069e-08
906,907,906,1813,0.05139613151550293,1.1128032716487084e-08
908,909,908,1817,0.051490068435668945,1.0642469088124688e-08
909,910,909,1819,0.051538944244384766,1.0407631694104922e-08
910,911,910,1821,0.05158519744873047,1.0177958172862686e-08
911,912,911,1823,0.05163121223449707,9.953437853389963e-09
912,913,912,1825,0.0516819953918457,9.733826951883057e-09
913,914,913,1827,0.051737070083618164,9.519096338482348e-09
914,915,914,1829,0.051792144775390625,9.30903330581499e-09
915,916,915,1831,0.051841020584106445,9.103648562193014e-09
917,918,917,1835,0.05194211006164551,8.706417612681972e-09
918,919,918,1837,0.051989078521728516,8.514283927011023e-09
919,920,919,1839,0.05203604698181152,8.326459466482152e-09
920,921,920,1841,0.05209016799926758,8.142685881233245e-09
921,922,921,1843,0.052146196365356445,7.9630467039615e-09
922,923,922,1845,0.052201032638549805,7.787429272598547e-09
923,924,923,1847,0.05225706100463867,7.615575236619038e-09
924,925,924,1849,0.05231213569641113,7.4475700775195894e-09
926,927,926,1853,0.05242013931274414,7.122555693849646e-09
927,928,927,1855,0.05246996879577637,6.965371652081703e-09
928,929,928,1857,0.052520036697387695,6.811667422647136e-09
929,930,929,1859,0.05257010459899902,6.661382798928771e-09
930,931,930,1861,0.05261516571044922,6.5144847545374474e-09
931,932,931,1863,0.05266404151916504,6.37071397085743e-09
932,933,932,1865,0.05271291732788086,6.23018797539801e-09
933,934,933,1867,0.05276012420654297,6.092696007706481e-09
934,935,934,1869,0.052805185317993164,5.958240016795014e-09
936,937,936,1873,0.052900075912475586,5.698242684981142e-09
937,938,937,1875,0.052947044372558594,5.572513910701756e-09
938,939,938,1877,0.05300402641296387,5.449579275351016e-09
939,940,939,1879,0.0530550479888916,5.329347494177657e-09
940,941,940,1881,0.05311012268066406,5.211818567311198e-09
941,942,941,1883,0.05315995216369629,5.096783683843895e-09
942,943,942,1885,0.0532071590423584,4.984324428417944e-09
943,944,943,1887,0.053255319595336914,4.874311624532917e-09
945,946,945,1891,0.053353071212768555,4.661627321287278e-09
946,947,946,1893,0.05340433120727539,4.558768388871017e-09
947,948,947,1895,0.0534520149230957,4.458228681887887e-09
948,949,948,1897,0.05350923538208008,4.359866409490801e-09
949,950,949,1899,0.0535731315612793,4.263665057883329e-09
950,951,950,1901,0.05363011360168457,4.169608112503921e-09
951,952,951,1903,0.05368924140930176,4.0775868118967275e-09
952,953,952,1905,0.05376005172729492,3.987666225528707e-09
953,954,953,1907,0.05382823944091797,3.8996482061967075e-09
955,956,955,1911,0.05392718315124512,3.729513205083479e-09
956,957,956,1913,0.053993940353393555,3.6471359191195203e-09
957,958,957,1915,0.054061174392700195,3.5667195081898446e-09
958,959,958,1917,0.054137229919433594,3.4880473594726533e-09
959,960,959,1919,0.0542299747467041,3.411108810674986e-09
960,961,960,1921,0.054305076599121094,3.3357746851690782e-09
961,962,961,1923,0.05437588691711426,3.262155693946089e-09
962,963,962,1925,0.05444502830505371,3.1902246601904834e-09
964,965,964,1929,0.05457305908203125,3.0510156069014238e-09
965,966,965,1931,0.05463123321533203,2.9837084595287415e-09
966,967,966,1933,0.054685354232788086,2.9178328672099618e-09
967,968,967,1935,0.05474209785461426,2.8535141047446713e-09
968,969,968,1937,0.0547940731048584,2.790528798118725e-09
969,970,969,1939,0.054842233657836914,2.7289896098874458e-09
970,971,970,1941,0.05488729476928711,2.6687547510363847e-09
971,972,971,1943,0.05493617057800293,2.609903853508794e-09
973,974,973,1947,0.05509305000305176,2.496013043956323e-09
974,975,974,1949,0.05514216423034668,2.44094205308474e-09
975,976,975,1951,0.055190086364746094,2.3870316509579367e-09
976,977,976,1953,0.05523824691772461,2.3343779835650525e-09
977,978,977,1955,0.05528402328491211,2.2828994682634745e-09
978,979,978,1957,0.055329084396362305,2.2325358992514584e-09
979,980,979,1959,0.055376291275024414,2.183249383256065e-09
980,981,980,1961,0.05542302131652832,2.1350612973345927e-09
981,982,981,1963,0.055477142333984375,2.0880027214375662e-09
983,984,983,1967,0.05557608604431152,1.9968545277996118e-09
984,985,984,1969,0.05562901496887207,1.9528154147945898e-09
985,986,985,1971,0.0556790828704834,1.9097115655982388e-09
986,987,986,1973,0.055730342864990234,1.8675624055989155e-09
987,988,987,1975,0.05578494071960449,1.8264174825199972e-09
988,989,988,1977,0.055834054946899414,1.7860310504165187e-09
989,990,989,1979,0.05589032173156738,1.7466158229990396e-09
990,991,990,1981,0.055938005447387695,1.708104781823992e-09
992,993,992,1985,0.056034088134765625,1.633583556513318e-09
993,994,993,1987,0.05608224868774414,1.5975209194049836e-09
994,995,994,1989,0.05612802505493164,1.5622692261776297e-09
995,996,995,1991,0.056176185607910156,1.527863466720342e-09
996,997,996,1993,0.05622291564941406,1.4940889731269788e-09
997,998,997,1995,0.056272268295288086,1.4611730227905125e-09
998,999,998,1997,0.056333065032958984,1.4289116668519644e-09
999,1000,999,1999,0.0563809871673584,1.39742727138252e-09
1000,1001,1000,2001,0.056429147720336914,1.3665139358918396e-09
1002,1003,1002,2005,0.05653190612792969,1.306962800229682e-09
1003,1004,1003,2007,0.0565800666809082,1.2780851138064408e-09
1004,1005,1004,2009,0.05662703514099121,1.2498891937498846e-09
1005,1006,1005,2011,0.05667400360107422,1.222282804159646e-09
1006,1007,1006,2013,0.05672311782836914,1.1953620897183009e-09
1007,1008,1007,2015,0.056767940521240234,1.1689288986667797e-09
1008,1009,1008,2017,0.05681419372558594,1.143166819589182e-09
1009,1010,1009,2019,0.05686497688293457,1.1179777540193763e-09
1011,1012,1011,2023,0.05698204040527344,1.0691205093271425e-09
1012,1013,1012,2025,0.057032108306884766,1.0455339133553966e-09
1013,1014,1013,2027,0.05708003044128418,1.0225222842478952e-09
1014,1015,1014,2029,0.05713200569152832,9.999379722375662e-10
1015,1016,1015,2031,0.05718517303466797,9.7791015743433e-10
1016,1017,1016,2033,0.05723428726196289,9.56342693225679e-10
1017,1018,1017,2035,0.0572810173034668,9.35204500487646e-10
1018,1019,1018,2037,0.057328224182128906,9.146393204366102e-10
1020,1021,1020,2041,0.05742311477661133,8.746530339066248e-10
1021,1022,1021,2043,0.05747103691101074,8.553902313279615e-10
1022,1023,1022,2045,0.05751919746398926,8.365256216531091e-10
1023,1024,1023,2047,0.057581186294555664,8.180232616760408e-10
1024,1025,1024,2049,0.057639122009277344,8.000026315114943e-10
1025,1026,1025,2051,0.05769801139831543,7.823442516717082e-10
1026,1027,1026,2053,0.05775904655456543,7.650840642271085e-10
1027,1028,1027,2055,0.05781722068786621,7.482385860736119e-10
1028,1029,1028,2057,0.05787491798400879,7.317242791843302e-10
1030,1031,1030,2061,0.05805706977844238,6.997795330236593e-10
1031,1032,1031,2063,0.05810999870300293,6.842820746519306e-10
1032,1033,1032,2065,0.05816221237182617,6.691828070489472e-10
1033,1034,1033,2067,0.05821514129638672,6.544836846885814e-10
1034,1035,1034,2069,0.05826616287231445,6.399865569653082e-10
1035,1036,1035,2071,0.05831503868103027,6.258750103902056e-10
1036,1037,1036,2073,0.058364152908325195,6.120800752748308e-10
1037,1038,1037,2075,0.058413028717041016,5.985395877898194e-10
1039,1040,1039,2079,0.058512210845947266,5.725065421427065e-10
1040,1041,1040,2081,0.05856204032897949,5.598556783223397e-10
1041,1042,1041,2083,0.05861020088195801,5.474903437361277e-10
1042,1043,1042,2085,0.05865907669067383,5.353959767434023e-10
1043,1044,1043,2087,0.05870699882507324,5.236036556816871e-10
1044,1045,1044,2089,0.058767080307006836,5.119842018621766e-10
1045,1046,1045,2091,0.058817148208618164,5.007483766505677e-10
1046,1047,1046,2093,0.05886697769165039,4.896854195281439e-10
1047,1048,1047,2095,0.05891609191894531,4.788953832972055e-10
1049,1050,1049,2099,0.05903005599975586,4.5801359683230384e-10
1050,1051,1050,2101,0.059087276458740234,4.478548242971066e-10
1051,1052,1051,2103,0.059144020080566406,4.3805055537893107e-10
1052,1053,1052,2105,0.059203147888183594,4.2828997376952316e-10
1053,1054,1053,2107,0.05927014350891113,4.1891497660075774e-10
1054,1055,1054,2109,0.059333086013793945,4.0960018715114647e-10
1055,1056,1055,2111,0.059388160705566406,4.0063794248832777e-10
1056,1057,1056,2113,0.059446096420288086,3.9175242124167735e-10
1058,1059,1058,2117,0.05959916114807129,3.746505393790235e-10
1059,1060,1059,2119,0.05967307090759277,3.664196137380893e-10
1060,1061,1060,2121,0.05975031852722168,3.583615565179284e-10
1061,1062,1061,2123,0.05982208251953125,3.5044724159302875e-10
1062,1063,1062,2125,0.0598909854888916,3.427057916794146e-10
1063,1064,1063,2127,0.059963226318359375,3.350770057795157e-10
1064,1065,1064,2129,0.060027122497558594,3.27750266125666e-10
1065,1066,1065,2131,0.06008601188659668,3.204380912833417e-10
1067,1068,1067,2135,0.060212135314941406,3.0645376899779945e-10
1068,1069,1068,2137,0.060272216796875,2.997146062684642e-10
1069,1070,1069,2139,0.06032729148864746,2.931026676484333e-10
1070,1071,1070,2141,0.06038403511047363,2.866179532803119e-10
1071,1072,1071,2143,0.060445308685302734,2.8030806205042515e-10
1072,1073,1072,2145,0.06050825119018555,2.741108315519524e-10
1073,1074,1073,2147,0.060572147369384766,2.680864708488592e-10
1074,1075,1074,2149,0.06063413619995117,2.621747682088018e-10
1075,1076,1075,2151,0.06069302558898926,2.5640681088465204e-10
1077,1078,1077,2155,0.060797929763793945,2.452311946412798e-10
1078,1079,1078,2157,0.06084609031677246,2.398614244647381e-10
1079,1080,1079,2159,0.06089615821838379,2.3453730077056327e-10
1080,1081,1080,2161,0.06094622611999512,2.293714793280497e-10
1081,1082,1081,2163,0.06099510192871094,2.243183257661177e-10
1082,1083,1082,2165,0.061044931411743164,2.19310806265918e-10
1083,1084,1083,2167,0.06109428405761719,2.144470383865247e-10
1084,1085,1084,2169,0.061144113540649414,2.098231484713792e-10
1086,1087,1086,2173,0.061244964599609375,2.0061906585764275e-10
1087,1088,1087,2175,0.06131720542907715,1.961699993914908e-10
1088,1089,1088,2177,0.06136822700500488,1.9184816221596238e-10
1089,1090,1089,2179,0.06144213676452637,1.8766810746188453e-10
1090,1091,1090,2181,0.06150102615356445,1.835045768196647e-10
1091,1092,1091,2183,0.06155800819396973,1.794682673554787e-10
1092,1093,1092,2185,0.061611175537109375,1.7546107804648654e-10
1093,1094,1093,2187,0.06166195869445801,1.715830741570755e-10
1094,1095,1094,2189,0.06171917915344238,1.6783229087103904e-10
1096,1097,1096,2193,0.06181812286376953,1.6049099156186033e-10
1097,1098,1097,2195,0.061866044998168945,1.5691307661382847e-10
1098,1099,1098,2197,0.06191515922546387,1.5346434350948917e-10
1099,1100,1099,2199,0.06196403503417969,1.5012827041115134e-10
1100,1101,1100,2201,0.06201291084289551,1.4679220930592685e-10
1101,1102,1101,2203,0.06209731101989746,1.435308945628077e-10
1102,1103,1102,2205,0.06215023994445801,1.4036964889450278e-10
1103,1104,1103,2207,0.062200069427490234,1.3731910488071225e-10
1105,1106,1105,2211,0.06230616569519043,1.3130930160015377e-10
1106,1107,1106,2213,0.06235694885253906,1.2843358458174707e-10
1107,1108,1107,2215,0.0624089241027832,1.2555590579833495e-10
1108,1109,1108,2217,0.06247305870056152,1.2280740999601188e-10
1109,1110,1109,2219,0.06252503395080566,1.2007347797270158e-10
1110,1111,1110,2221,0.0625762939453125,1.1746872890468555e-10
1111,1112,1111,2223,0.06262826919555664,1.1489309549807627e-10
1112,1113,1112,2225,0.06267595291137695,1.1231746528912807e-10
1114,1115,1114,2229,0.06277298927307129,1.0743717706238036e-10
1115,1116,1115,2231,0.0628211498260498,1.050888412949793e-10
1116,1117,1116,2233,0.06286811828613281,1.0270063080882094e-10
1117,1118,1117,2235,0.06291508674621582,1.0039596965017854e-10
1118,1119,1118,2237,0.06296300888061523,9.822048273450043e-11


==> plot_data/cournot-nash_equilibrium_problem_n10/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00016832351684570312,542.5060889379029
1,4,4,8,0.0003509521484375,437.43651362206106
2,6,6,12,0.0006814002990722656,500.9910455002406
3,8,8,16,0.0009562969207763672,283.995165641375
4,10,10,20,0.0011751651763916016,98.73967534940398
5,12,12,24,0.001379251480102539,48.64250305757986
6,14,14,28,0.0016331672668457031,45.98157682107862
7,16,16,32,0.0019252300262451172,30.634562708932165
8,18,18,36,0.0021822452545166016,25.34876679456932
9,24,24,48,0.0026361942291259766,20.946461685948265
10,28,28,56,0.002978086471557617,13.77872492523781
11,34,34,68,0.0033431053161621094,11.82937972302457
12,42,42,84,0.0038611888885498047,11.188307611800841
13,50,50,100,0.0043561458587646484,7.050555831482018
14,58,58,116,0.004944324493408203,5.800979760574122
15,66,66,132,0.005384922027587891,4.802213879133725
16,68,68,136,0.005591154098510742,7.601934771224064
17,70,70,140,0.005851268768310547,0.05058893989745001
18,72,72,144,0.006077289581298828,0.0479459468159699
19,74,74,148,0.006344318389892578,0.0022762552666861233
20,76,76,152,0.006565093994140625,0.0009311500991786255
21,78,78,156,0.006801128387451172,4.960706692318229e-12


==> plot_data/cournot-nash_equilibrium_problem_n10/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.081031799316406e-05,542.5060889379029
1,4,4,8,0.00020694732666015625,437.43651362206106
2,6,6,12,0.0004699230194091797,250.68522250518726
3,8,8,16,0.0007090568542480469,193.07695757789975
4,10,10,20,0.0009720325469970703,116.59292642060402
5,12,12,24,0.0011758804321289062,68.21186468102738
6,14,14,28,0.0014159679412841797,70.84898259738459
7,16,16,32,0.0016329288482666016,32.22718672548579
8,18,18,36,0.0019979476928710938,26.64452123526115
9,22,22,44,0.002329111099243164,24.606731282542263
10,26,26,52,0.002650022506713867,22.21388258074964
11,28,28,56,0.0029039382934570312,19.072857774546346
12,30,30,60,0.003159046173095703,12.412742376047396
13,36,36,72,0.003551959991455078,13.107095737336845
14,44,44,88,0.00400090217590332,5.7849392509685185
15,50,50,100,0.004400730133056641,4.9118785196109975
16,58,58,116,0.004823923110961914,3.5486959483862526
17,60,60,120,0.0050809383392333984,0.17347250016548185
18,62,62,124,0.005343914031982422,0.16450650845181203
19,64,64,128,0.0056018829345703125,0.02271219525515278
20,66,66,132,0.005810976028442383,5.1160245900507605e-12


==> plot_data/cournot-nash_equilibrium_problem_n100/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0001659393310546875,1624.447741208611
1,2,1,3,0.0003619194030761719,66480.312266118
2,3,2,5,0.0008180141448974609,14341.46814081151
3,4,3,7,0.0015728473663330078,14461.317840003707
4,5,4,9,0.0019469261169433594,14433.618717844925
5,6,5,11,0.0022039413452148438,14396.852887404397
6,7,6,13,0.0024399757385253906,14347.479192894445
7,8,7,15,0.002574920654296875,14281.255685788452
8,9,8,17,0.002716064453125,14192.575556676999
9,10,9,19,0.002907991409301758,14074.08233854318
10,11,10,21,0.003062009811401367,13916.218043252082
11,12,11,23,0.0032148361206054688,13706.733207527326
12,13,12,25,0.003401041030883789,13430.230862591334
13,14,13,27,0.0035867691040039062,13067.895133560034
14,15,14,29,0.0037698745727539062,12596.264706656275
15,16,15,31,0.004019021987915039,11955.95988615279
16,17,16,33,0.004194974899291992,11113.464924978862
17,18,17,35,0.004385948181152344,10048.982070197228
18,19,18,37,0.004560947418212891,8727.81879293032
19,20,19,39,0.004756927490234375,7180.805058867846
20,21,20,41,0.0049359798431396484,5584.378706764449
21,22,21,43,0.0052509307861328125,4202.480134190401
22,23,22,45,0.0055429935455322266,2999.138954000196
23,24,23,47,0.006330013275146484,3264.889341797864
24,25,24,49,0.006636857986450195,3412.343153645238
25,26,25,51,0.006834983825683594,2352.8850025209904
26,27,26,53,0.007047891616821289,1809.5747538939772
27,28,27,55,0.00724482536315918,1595.3048090201014
28,29,28,57,0.007501840591430664,1500.3146609901853
29,30,29,59,0.007652997970581055,1328.880560238683
30,31,30,61,0.007832765579223633,1207.6473496388983
31,32,31,63,0.008026838302612305,1001.1475342960471
32,33,32,65,0.008206844329833984,903.9535897388365
33,34,33,67,0.009765863418579102,694.6687185977336
34,35,34,69,0.01005697250366211,777.3117430420552
35,36,35,71,0.010441064834594727,810.3792926385242
36,37,36,73,0.010597944259643555,704.604802111637
37,38,37,75,0.010798931121826172,593.9726965086217
38,39,38,77,0.011052131652832031,488.45320765521217
39,40,39,79,0.011219024658203125,397.2831966338014
40,41,40,81,0.011361837387084961,288.44388149739746
41,42,41,83,0.011511087417602539,253.13674828935748
42,43,42,85,0.01164388656616211,211.99678386519972
43,44,43,87,0.012024879455566406,209.53369989489195
44,45,44,89,0.01227712631225586,179.04104446788813
45,46,45,91,0.012687921524047852,152.31559956315436
46,47,46,93,0.012848854064941406,171.15729466784816
47,48,47,95,0.01321101188659668,211.03276379821358
48,49,48,97,0.013535022735595703,208.37154346651172
49,50,49,99,0.013754844665527344,196.80024225903858
50,51,50,101,0.013961076736450195,177.82040656391362
51,52,51,103,0.014284133911132812,161.24486217707576
52,53,52,105,0.014627933502197266,153.38882020210585
53,54,53,107,0.016881942749023438,150.61097993265344
54,55,54,109,0.01787877082824707,135.76958053430312
55,56,55,111,0.018178939819335938,126.77788355928496
56,57,56,113,0.01838397979736328,141.84718278535036
57,58,57,115,0.019345998764038086,149.854735822487
58,59,58,117,0.01966381072998047,149.29759713698084
59,60,59,119,0.01989889144897461,148.61262535949174
60,61,60,121,0.020103931427001953,134.1097655197761
61,62,61,123,0.02034783363342285,129.61821999020552
62,63,62,125,0.02063584327697754,127.44058854786189
63,64,63,127,0.020817041397094727,125.28596557763727
64,65,64,129,0.021062850952148438,116.19280308703794
65,66,65,131,0.02126908302307129,113.38147538850397
66,67,66,133,0.021423816680908203,124.91022290460728
67,68,67,135,0.021804094314575195,117.12726507032242
68,69,68,137,0.022009849548339844,112.56254792581356
69,70,69,139,0.022497177124023438,102.83719623968022
70,71,70,141,0.022738933563232422,104.21770518435213
71,72,71,143,0.02295207977294922,118.63945735860626
72,73,72,145,0.02317190170288086,115.98516499429263
73,74,73,147,0.02336597442626953,115.65319338797408
74,75,74,149,0.02351999282836914,111.19439878400193
75,76,75,151,0.02371692657470703,104.39076960191902
76,77,76,153,0.02399587631225586,103.0696248671041
77,78,77,155,0.024293899536132812,101.60264780782458
78,79,78,157,0.024452924728393555,100.02040175527613
79,80,79,159,0.024662017822265625,98.37340684616927
80,81,80,161,0.024971961975097656,96.66423208494595
81,82,81,163,0.025355100631713867,94.80755318932252
82,83,82,165,0.02564692497253418,92.61929085812723
83,84,83,167,0.025935888290405273,82.20467883091727
84,85,84,169,0.026123046875,82.2276336179846
85,86,85,171,0.026276826858520508,93.41373837132049
86,87,86,173,0.026408910751342773,93.1517319305314
87,88,87,175,0.026525020599365234,92.85377700988873
88,89,88,177,0.02682805061340332,92.46553789833177
89,90,89,179,0.02739095687866211,91.96342646834663
90,91,90,181,0.027637004852294922,91.31221138337814
91,92,91,183,0.027830123901367188,87.36978006174586
92,93,92,185,0.027949810028076172,81.52768846267267
93,94,93,187,0.028123855590820312,79.97762508017738
94,95,94,189,0.028279781341552734,73.99020181783855
95,96,95,191,0.028472900390625,76.4313072728746
96,97,96,193,0.028609037399291992,85.59622610405714
97,98,97,195,0.030334949493408203,80.53924771322855
98,99,98,197,0.030627965927124023,80.139048829788
99,100,99,199,0.03119802474975586,79.6378129219736
100,101,100,201,0.031538963317871094,75.24638490190657
101,102,101,203,0.03183698654174805,74.22609156241481
102,103,102,205,0.03207993507385254,73.0635167267425
103,104,103,207,0.032257080078125,67.04428064270962
104,105,104,209,0.0324249267578125,65.31825182865164
105,106,105,211,0.032594919204711914,66.05070641356507
106,107,106,213,0.032788991928100586,72.53922026942206
107,108,107,215,0.03298783302307129,72.404081980174
108,109,108,217,0.03342080116271973,72.24099241556611
109,110,109,219,0.03365302085876465,72.02584820554755
110,111,110,221,0.033822059631347656,71.7441842010779
111,112,111,223,0.03401303291320801,66.68664534216039
112,113,112,225,0.034208059310913086,66.03907776918946
113,114,113,227,0.036170005798339844,65.27496863149007
114,115,114,229,0.03638195991516113,64.36291090607604
115,116,115,231,0.03656196594238281,63.26695724899916
116,117,116,233,0.036769866943359375,41.053399654700996
117,118,117,235,0.0369570255279541,39.75806275852081
118,119,118,237,0.03709602355957031,37.99046284633607
119,120,119,239,0.03723907470703125,36.091526421798235
120,121,120,241,0.037377119064331055,26.286419950819667
121,122,121,243,0.03751206398010254,38.203566208014486
122,123,122,245,0.03769874572753906,37.6464158733411
123,124,123,247,0.037867069244384766,37.30231938233656
124,125,124,249,0.03802299499511719,36.7792516252911
125,126,125,251,0.03816986083984375,36.1252312788008
126,127,126,253,0.03832507133483887,35.268352756834226
127,128,127,255,0.03855013847351074,27.64634537526409
128,129,128,257,0.038800954818725586,26.011098170455444
129,130,129,259,0.038977861404418945,28.14626413478884
130,131,130,261,0.03923988342285156,34.945132292472316
131,132,131,263,0.03950381278991699,34.8115637631556
132,133,132,265,0.039659976959228516,34.62359070489218
133,134,133,267,0.04034996032714844,34.37439158674657
134,135,134,269,0.04072403907775879,27.516130462820737
135,136,135,271,0.04139995574951172,26.89648792414325
136,137,136,273,0.04179096221923828,26.214114204686044
137,138,137,275,0.042085886001586914,25.424876388576987
138,139,138,277,0.04224801063537598,21.595524657869593
139,140,139,279,0.04251885414123535,20.763485350549875
140,141,140,281,0.04281187057495117,20.493499462689265
141,142,141,283,0.04311990737915039,21.238159792348153
142,143,142,285,0.0434267520904541,20.825768927194044
143,144,143,287,0.04367995262145996,20.339039472400103
144,145,144,289,0.04384589195251465,18.763839534692664
145,146,145,291,0.04401588439941406,17.982728372662297
146,147,146,293,0.04439997673034668,18.521217584717395
147,148,147,295,0.044754981994628906,20.045268367213325
148,149,148,297,0.04491901397705078,19.943585971892702
149,150,149,299,0.045194149017333984,19.813130208921198
150,151,150,301,0.04588913917541504,18.689135647777793
151,152,151,303,0.04620099067687988,18.425282899092124
152,153,152,305,0.04644489288330078,18.099639831993226
153,154,153,307,0.04657602310180664,17.689022860468814
154,155,154,309,0.0467379093170166,17.173316720234435
155,156,155,311,0.04688000679016113,16.522933105404036
156,157,156,313,0.047020912170410156,15.70311606888202
157,158,157,315,0.0471649169921875,7.269409531819816
158,159,158,317,0.04764080047607422,16.048535296917258
159,160,159,319,0.048219919204711914,15.61419732633783
160,161,160,321,0.0488588809967041,15.110883046675127
161,162,161,323,0.04908609390258789,6.86175600860245
162,163,162,325,0.04934096336364746,15.714283837481105
163,164,163,327,0.04964590072631836,15.678307557616668
164,165,164,329,0.049813032150268555,15.631355260104748
165,166,165,331,0.05016493797302246,15.568708547941736
166,167,166,333,0.05036807060241699,15.485211722410574
167,168,167,335,0.0514528751373291,15.37424259059334
168,169,168,337,0.05182194709777832,15.227228241040335
169,170,169,339,0.052014827728271484,15.033137715199583
170,171,170,341,0.05226707458496094,7.350017934603584
171,172,171,343,0.052461862564086914,15.061350801723588
172,173,172,345,0.052659034729003906,7.587286659508479
173,174,173,347,0.052906036376953125,7.320275997611698
174,175,174,349,0.05303192138671875,7.474882960645439
175,176,175,351,0.05484795570373535,7.546397717422357
176,177,176,353,0.05500602722167969,7.434545006098061
177,178,177,355,0.05516386032104492,7.302824442244538
178,179,178,357,0.05533909797668457,7.139599053889025
179,180,179,359,0.05551004409790039,6.943436996632568
180,181,180,361,0.05566287040710449,6.916189089907064
181,182,181,363,0.055809736251831055,6.698122211635634
182,183,182,365,0.05597281455993652,6.791050001269135
183,184,183,367,0.056169986724853516,6.89462583261384
184,185,184,369,0.05629897117614746,6.815839045334052
185,186,185,371,0.05641984939575195,6.723950038753889
186,187,186,373,0.056550025939941406,6.608597361855441
187,188,187,375,0.05668997764587402,5.081719251988298
188,189,188,377,0.056819915771484375,4.929845463484044
189,190,189,379,0.05697798728942871,4.822533982388492
190,191,190,381,0.057127952575683594,4.684962999078752
191,192,191,383,0.0572659969329834,4.508856446867718
192,193,192,385,0.05744194984436035,4.286011416172168
193,194,193,387,0.057598114013671875,4.007687467672218
194,195,194,389,0.05777096748352051,3.6670938598022187
195,196,195,391,0.05792117118835449,3.2621763397137156
196,197,196,393,0.05806398391723633,2.227088972392815
197,198,197,395,0.05822396278381348,3.7751892218765275
198,199,198,397,0.05840492248535156,3.746635164515441
199,200,199,399,0.058537960052490234,3.715697817111954
200,201,200,401,0.05865979194641113,3.6747394306870143
201,202,201,403,0.05878400802612305,3.6206080164915715
202,203,202,405,0.05894899368286133,3.549485752861317
203,204,203,407,0.05926799774169922,3.4566645370454605
204,205,204,409,0.059419870376586914,3.3365577515925615
205,206,205,411,0.059600830078125,3.1828734960920295
206,207,206,413,0.0597379207611084,2.4317659921488683
207,208,207,415,0.05989193916320801,3.1335629842218222
208,209,208,417,0.060025930404663086,3.2537054811488444
209,210,209,419,0.0601811408996582,3.2179695358006914
210,211,210,421,0.060324907302856445,3.173862240638381
211,212,211,423,0.06046700477600098,3.115485339250638
212,213,212,425,0.060647010803222656,2.4894356912774347
213,214,213,427,0.06082010269165039,2.376549439522118
214,215,214,429,0.06099200248718262,2.492022594955385
215,216,215,431,0.061192989349365234,3.068263882841167
216,217,216,433,0.061363935470581055,2.479923303639887
217,218,217,435,0.06149792671203613,2.4381509405375152
218,219,218,437,0.06164407730102539,2.3867723658766415
219,220,219,439,0.0617828369140625,2.3224421005865112
220,221,220,441,0.061921119689941406,2.2433067586912516
221,222,221,443,0.06368684768676758,2.2053444349065034
222,223,222,445,0.0640568733215332,2.105153573439436
223,224,223,447,0.06422901153564453,2.154027655358992
224,225,224,449,0.06441593170166016,2.220281745812093
225,226,225,451,0.06459975242614746,2.196200913203472
226,227,226,453,0.06477499008178711,2.1673253795168876
227,228,227,455,0.06492090225219727,2.1297730359195284
228,229,228,457,0.06508803367614746,2.0816213906801138
229,230,229,459,0.06525492668151855,2.020442755191433
230,231,230,461,0.06538891792297363,1.9434707565791276
231,232,231,463,0.06554508209228516,1.8475661810403092
232,233,232,465,0.06570100784301758,1.7293833048258431
233,234,233,467,0.06585192680358887,1.5859537293404178
234,235,234,469,0.06598687171936035,0.7252404474179305
235,236,235,471,0.06610584259033203,0.4185407753917853
236,237,236,473,0.0662529468536377,1.6861037474464389
237,238,237,475,0.06642484664916992,1.6851731962603582
238,239,238,477,0.06659698486328125,1.6838876296067853
239,240,239,479,0.0667579174041748,1.6821604390877678
240,241,240,481,0.06699395179748535,1.6798397517717565
241,242,241,483,0.06717801094055176,1.6767247051100043
242,243,242,485,0.06753396987915039,1.6725488238756219
243,244,243,487,0.06771373748779297,1.6669604060452743
244,245,244,489,0.06795907020568848,1.6594983303733066
245,246,245,491,0.0685579776763916,1.6495631116794278
246,247,246,493,0.06878018379211426,1.6363836015535016
247,248,247,495,0.0689401626586914,1.6189805567170612
248,249,248,497,0.06923079490661621,1.5961291977613332
249,250,249,499,0.06946492195129395,1.566323603870103
250,251,250,501,0.06972384452819824,1.5277466686869614
251,252,251,503,0.06987977027893066,1.4782532994147433
252,253,252,505,0.07003092765808105,0.6933876125098047
253,254,253,507,0.07031106948852539,0.5607530606607608
254,255,254,509,0.07051491737365723,1.5055914443206322
255,256,255,511,0.07135009765625,1.5033236175095301
256,257,256,513,0.07222294807434082,1.5002603057120256
257,258,257,515,0.07238507270812988,1.4961562912875006
258,259,258,517,0.0725870132446289,1.4906623869671758
259,260,259,519,0.07276487350463867,1.483323697708481
260,261,260,521,0.07294702529907227,1.4735477859328214
261,262,261,523,0.07320499420166016,1.4605709741864152
262,263,262,525,0.07335996627807617,1.4434210310118207
263,264,263,527,0.0736091136932373,0.6754406617502472
264,265,264,529,0.07378888130187988,0.6277636745228365
265,266,265,531,0.07434892654418945,1.4422581781464605
266,267,266,533,0.07482409477233887,1.4360715297418858
267,268,267,535,0.07499098777770996,1.42777315645342
268,269,268,537,0.0751340389251709,0.6574764542520731
269,270,269,539,0.07527899742126465,0.6355755144404837
270,271,270,541,0.075408935546875,0.6427907563601136
271,272,271,543,0.07572698593139648,0.6464244305576664
272,273,272,545,0.07615399360656738,0.633954580791477
273,274,273,547,0.07648587226867676,0.6184643195280267
274,275,274,549,0.07663393020629883,0.604570789429221
275,276,275,551,0.07676506042480469,0.6049178820156943
276,277,276,553,0.0768887996673584,0.5990756580792297
277,278,277,555,0.0770120620727539,0.5893732761327974
278,279,278,557,0.07716894149780273,0.579435510874912
279,280,279,559,0.07758593559265137,0.5741490630150198
280,281,280,561,0.07773399353027344,0.5677590605258795
281,282,281,563,0.07789182662963867,0.5607880363032088
282,283,282,565,0.07802295684814453,0.5531399782517495
283,284,283,567,0.07816672325134277,0.5464671624069432
284,285,284,569,0.07834196090698242,0.5401551739129268
285,286,285,571,0.07847309112548828,0.5336742686743067
286,287,286,573,0.07860302925109863,0.5270580758382414
287,288,287,575,0.07872891426086426,0.5206563987044027
288,289,288,577,0.07887697219848633,0.5144761230218802
289,290,289,579,0.07906699180603027,0.5083618961183305
290,291,290,581,0.07939314842224121,0.5022747317852584
291,292,291,583,0.07975602149963379,0.49627613459559883
292,293,292,585,0.08001899719238281,0.4903963920125888
293,294,293,587,0.0801858901977539,0.48461107049557867
294,295,294,589,0.08104205131530762,0.47889932601475277
295,296,295,591,0.08119988441467285,0.4732639079019063
296,297,296,593,0.08133101463317871,0.4677129689753158
297,298,297,595,0.08146214485168457,0.4622450798330764
298,299,298,597,0.08159995079040527,0.45685433315588975
299,300,299,599,0.08179378509521484,0.45153723640456706
300,301,300,601,0.0820009708404541,0.4462931658854212
301,302,301,603,0.08213472366333008,0.4411211375219804
302,303,302,605,0.08229899406433105,0.43601899583580056
303,304,303,607,0.08243680000305176,0.4309841543727129
304,305,304,609,0.08256101608276367,0.42601444486943063
305,306,305,611,0.08269691467285156,0.42110786808353495
306,307,306,613,0.0828409194946289,0.41626237449869935
307,308,307,615,0.0830228328704834,0.4114756715961943
308,309,308,617,0.08319902420043945,0.4067454266354768
309,310,309,619,0.08350896835327148,0.40206922367491715
310,311,310,621,0.08368897438049316,0.39744465601128653
311,312,311,623,0.08388781547546387,0.39286916771464037
312,313,312,625,0.08413290977478027,0.38834016150134976
313,314,313,627,0.08429694175720215,0.38385485356959975
314,315,314,629,0.0847010612487793,0.3794104340867314
315,316,315,631,0.08497095108032227,0.375003860656432
316,317,316,633,0.08514690399169922,0.3706320770779545
317,318,317,635,0.08536601066589355,0.366291700642812
318,319,318,637,0.08572506904602051,0.36197938260565715
319,320,319,639,0.08606910705566406,0.35769128856384447
320,321,320,641,0.0862119197845459,0.35342375386332686
321,322,321,643,0.0863649845123291,0.3491723100481855
322,323,322,645,0.08651089668273926,0.34493301434731355
323,324,323,647,0.0866551399230957,0.34070040645839084
324,325,324,649,0.0867919921875,0.33647052311427805
325,326,325,651,0.08691596984863281,0.3322360733724812
326,327,326,653,0.08705806732177734,0.327994089515171
327,328,327,655,0.08719396591186523,0.32373307623613956
328,329,328,657,0.08748793601989746,0.31945482946226317
329,330,329,659,0.08835315704345703,0.31513572265391865
330,331,330,661,0.0893259048461914,0.31079695412052627
331,332,331,663,0.08954286575317383,0.3063721583304791
332,333,332,665,0.08971500396728516,0.3019641309360552
333,334,333,667,0.08998298645019531,0.29732827977106996
334,335,334,669,0.09018301963806152,0.29294379045103136
335,336,335,671,0.09034395217895508,0.2876931398230988
336,337,336,673,0.09051203727722168,0.2839946668274124
337,338,337,675,0.09068083763122559,0.2751994427239268
338,339,338,677,0.09090209007263184,0.27581382947717054
339,340,339,679,0.0910789966583252,0.2874353214570422
340,341,340,681,0.09123110771179199,0.28675778167149324
341,342,341,683,0.09139680862426758,0.28591633058948807
342,343,342,685,0.09154701232910156,0.28479097085675087
343,344,343,687,0.09168481826782227,0.2832907448475324
344,345,344,689,0.09182095527648926,0.28129753475184355
345,346,345,691,0.09195184707641602,0.27866073860531393
346,347,346,693,0.09209394454956055,0.2751912519506226
347,348,347,695,0.0922708511352539,0.2706558395583119
348,349,348,697,0.09253311157226562,0.26477244649104614
349,350,349,699,0.09270691871643066,0.2572069387652933
350,351,350,701,0.09299898147583008,0.24757238411670957
351,352,351,703,0.09322094917297363,0.23940397849652206
352,353,352,705,0.09338998794555664,0.22708883533723045
353,354,353,707,0.0936899185180664,0.22997432777483937
354,355,354,709,0.09387707710266113,0.2435799041288883
355,356,355,711,0.0940408706665039,0.24166224705512868
356,357,356,713,0.09421086311340332,0.2393259815255683
357,358,357,715,0.09452390670776367,0.23622848485600617
358,359,358,717,0.09485697746276855,0.23214874598737864
359,360,359,719,0.09511899948120117,0.22680959355575184
360,361,360,721,0.0955960750579834,0.2198780957871772
361,362,361,723,0.09573101997375488,0.21096943677590774
362,363,362,725,0.09587216377258301,0.1996673207246075
363,364,363,727,0.09600496292114258,0.18557645348345495
364,365,364,729,0.09612298011779785,0.16842759533702387
365,366,365,731,0.09625887870788574,0.15586211684774778
366,367,366,733,0.09639310836791992,0.13371926250563898
367,368,367,735,0.09654402732849121,0.15868584916771908
368,369,368,737,0.09669780731201172,0.1639024141753832
369,370,369,739,0.09685492515563965,0.158137941973668
370,371,370,741,0.09699010848999023,0.15130547362875005
371,372,371,743,0.09714579582214355,0.1425918441238957
372,373,372,745,0.09829998016357422,0.13176974241445527
373,374,373,747,0.09887003898620605,0.11868406573582256
374,375,374,749,0.09904193878173828,0.10345677206635708
375,376,375,751,0.0991818904876709,0.08657182812786593
376,377,376,753,0.09936809539794922,0.08309196629068981
377,378,377,755,0.09951281547546387,0.06184898445277676
378,379,378,757,0.09965801239013672,0.09067995131694434
379,380,379,759,0.09981179237365723,0.09003785905406819
380,381,380,761,0.099945068359375,0.09657899138279351
381,382,381,763,0.10007405281066895,0.09636943979264737
382,383,382,765,0.1002039909362793,0.09611044293984768
383,384,383,767,0.10033893585205078,0.09576262143142342
384,385,384,769,0.10048389434814453,0.09529616762041856
385,386,385,771,0.10063600540161133,0.09467166282948808
386,387,386,773,0.10076403617858887,0.09383743256591973
387,388,387,775,0.10088205337524414,0.09272642005888754
388,389,388,777,0.10100698471069336,0.0912528331907601
389,390,389,779,0.10112905502319336,0.08930910057299095
390,391,390,781,0.10129380226135254,0.0867642396787898
391,392,391,783,0.10143184661865234,0.08346565705502312
392,393,392,785,0.10155701637268066,0.07924771252400852
393,394,393,787,0.1016850471496582,0.07395186902141064
394,395,394,789,0.10182881355285645,0.06746400700463402
395,396,395,791,0.10200095176696777,0.059772294680576016
396,397,396,793,0.10212898254394531,0.051040170755676954
397,398,397,795,0.1022958755493164,0.04166999937218997
398,399,398,797,0.10244297981262207,0.042642479311263484
399,400,399,799,0.10260796546936035,0.05247441558349193
400,401,400,801,0.10278582572937012,0.04737590623729484
401,402,401,803,0.10321593284606934,0.04309184718360677
402,403,402,805,0.10336112976074219,0.03779164810756731
403,404,403,807,0.10353589057922363,0.031891866022615054
404,405,404,809,0.10367298126220703,0.025734294791687134
405,406,405,811,0.10381197929382324,0.035365363556073615
406,407,406,813,0.10396695137023926,0.03388204234975861
407,408,407,815,0.10416388511657715,0.03546534490296981
408,409,408,817,0.10443902015686035,0.03396070816580271
409,410,409,819,0.1047508716583252,0.03222060901357562
410,411,410,821,0.10488390922546387,0.030033553725426675
411,412,411,823,0.1055459976196289,0.02735517223244065
412,413,412,825,0.10582590103149414,0.024194157154443174
413,414,413,827,0.10607600212097168,0.020606595763428496
414,415,414,829,0.10623908042907715,0.016792629769318324
415,416,415,831,0.10635805130004883,0.01993152484789297
416,417,416,833,0.10654807090759277,0.02136560926801935
417,418,417,835,0.10669898986816406,0.019405198242474483
418,419,418,837,0.10685396194458008,0.017526590322728495
419,420,419,839,0.10700201988220215,0.015356597832480404
420,421,420,841,0.10712003707885742,0.012917796411882456
421,422,421,843,0.10726785659790039,0.017305163791660937
422,423,422,845,0.1074368953704834,0.016306625647765548
423,424,423,847,0.10768795013427734,0.015411293115797422
424,425,424,849,0.10781192779541016,0.014281904532111658
425,426,425,851,0.10794711112976074,0.01290230312380845
426,427,426,853,0.10807991027832031,0.01130614845289011
427,428,427,855,0.1082310676574707,0.00949884564669223
428,429,428,857,0.10847997665405273,0.007682698721166698
429,430,429,859,0.1086721420288086,0.011626636502727453
430,431,430,861,0.10880112648010254,0.011115873558436233
431,432,431,863,0.10906195640563965,0.010679024274575847
432,433,432,865,0.10922408103942871,0.010114597756234984
433,434,433,867,0.10941195487976074,0.009407116455711045
434,435,434,869,0.10958194732666016,0.00854709918452284
435,436,435,871,0.10976195335388184,0.007531877604113676
436,437,436,873,0.10988497734069824,0.006392308240390558
437,438,437,875,0.11002874374389648,0.0051738658288600576
438,439,438,877,0.11016082763671875,0.004001686655688144
439,440,439,879,0.11034202575683594,0.0067299690865775565
440,441,440,881,0.11050987243652344,0.006284350466575288
441,442,441,883,0.11066985130310059,0.005945876602569633
442,443,442,885,0.11086297035217285,0.005511245461313119
443,444,443,887,0.11103010177612305,0.004981512321792579
444,445,444,889,0.11118602752685547,0.004367339484182401
445,446,445,891,0.11131715774536133,0.003672638763999776
446,447,446,893,0.11144495010375977,0.0029692991553993495
447,448,447,895,0.1115880012512207,0.004452364887128656
448,449,448,897,0.11171388626098633,0.004212897730160423
449,450,449,899,0.11182808876037598,0.004012159814168028
450,451,450,901,0.11197495460510254,0.003754970568891069
451,452,451,903,0.1125340461730957,0.003437453654834296
452,453,452,905,0.11292910575866699,0.003061182840691994
453,454,453,907,0.11357688903808594,0.0026281779614489497
454,455,454,909,0.11374807357788086,0.00216526238045758
455,456,455,911,0.11389708518981934,0.0027106960356530563
456,457,456,913,0.11405491828918457,0.0026995323283796582
457,458,457,915,0.11427783966064453,0.002996080494517269
458,459,458,917,0.1144568920135498,0.0029923538782303757
459,460,459,919,0.11461997032165527,0.0029879108248709943
460,461,460,921,0.11480498313903809,0.0029819347301472303
461,462,461,923,0.11496615409851074,0.002973903572404851
462,463,462,925,0.11509203910827637,0.00296312079918788
463,464,463,927,0.11525201797485352,0.002948661983885584
464,465,464,929,0.11541986465454102,0.0029293069441653306
465,466,465,931,0.11561083793640137,0.0029034571101197388
466,467,466,933,0.11575102806091309,0.0028690396929579335
467,468,467,935,0.11589574813842773,0.0028234054351714555
468,469,468,937,0.11603903770446777,0.002763236620510449
469,470,469,939,0.11617588996887207,0.0026844992054962068
470,471,470,941,0.1163017749786377,0.002582500334238168
471,472,471,943,0.1164398193359375,0.0024521512259875243
472,473,472,945,0.1165778636932373,0.0022885795608290154
473,474,473,947,0.11670684814453125,0.002088260322903461
474,475,474,949,0.1168220043182373,0.0018507771451557458
475,476,475,951,0.11695384979248047,0.0015810707771260633
476,477,476,953,0.1170969009399414,0.0012914424256939671
477,478,477,955,0.11722087860107422,0.0012005200329122038
478,479,478,957,0.11738204956054688,0.001258156964737714
479,480,479,959,0.11759185791015625,0.0011966516394558166
480,481,480,961,0.11778998374938965,0.0009981900187846858
481,482,481,963,0.11824584007263184,0.0008024446155144538
482,483,482,965,0.11840295791625977,0.0009752394641062047
483,484,483,967,0.11864709854125977,0.0010294865881905518
484,485,484,969,0.118804931640625,0.000936317461871704
485,486,485,971,0.11895084381103516,0.0008343803818475235
486,487,486,973,0.11926412582397461,0.00082971530163067
487,488,487,975,0.11957001686096191,0.000991840012350993
488,489,488,977,0.11978816986083984,0.0009912154757695901
489,490,489,979,0.11995983123779297,0.0009905262226936442
490,491,490,981,0.12009191513061523,0.000989598148559697
491,492,491,983,0.1204829216003418,0.000988349116820461
492,493,492,985,0.1215360164642334,0.0009866688631312223
493,494,493,987,0.12186813354492188,0.000984409839924737
494,495,494,989,0.12233495712280273,0.0009813750951310053
495,496,495,991,0.12246894836425781,0.000977302607535606
496,497,496,993,0.12261414527893066,0.0009718453762401469
497,498,497,995,0.12275099754333496,0.0009645467234961954
498,499,498,997,0.12290215492248535,0.000954810772917975
499,500,499,999,0.12313985824584961,0.0009418692515501208
500,501,500,1001,0.12341690063476562,0.0009247480896094653
501,502,501,1003,0.12366604804992676,0.0009022415782224391
502,503,502,1005,0.12391209602355957,0.0008729089983857786
503,504,503,1007,0.12452197074890137,0.0008351195589911302
504,505,504,1009,0.12479591369628906,0.0007871857288478566
505,506,505,1011,0.12520289421081543,0.0007276384148419363
506,507,506,1013,0.12554597854614258,0.0006556965536956321
507,508,507,1015,0.1258080005645752,0.0005719399046091268
508,509,508,1017,0.12605500221252441,0.00047906262924275327
509,510,509,1019,0.12621498107910156,0.0003823383261407503
510,511,510,1021,0.12634706497192383,0.00041556358051771835
511,512,511,1023,0.1264820098876953,0.0004169568902919952
512,513,512,1025,0.12663602828979492,0.00032995576403393887
513,514,513,1027,0.12679696083068848,0.00026959124522608213
514,515,514,1029,0.12722301483154297,0.00030959551862262116
515,516,515,1031,0.12747907638549805,0.00032720868477436265
516,517,516,1033,0.12766075134277344,0.00027663499729495955
517,518,517,1035,0.1278519630432129,0.00023632644302929416
518,519,518,1037,0.1280210018157959,0.0002871406614598096
519,520,519,1039,0.12816905975341797,0.0002811566762363627
520,521,520,1041,0.12832379341125488,0.0003046054221826435
521,522,521,1043,0.12853789329528809,0.0003001219973994963
522,523,522,1045,0.1288127899169922,0.00029480289516907134
523,524,523,1047,0.12897014617919922,0.0002877949446927499
524,525,524,1049,0.1292281150817871,0.0002786544810136465
525,526,525,1051,0.1307690143585205,0.00026686683042748095
526,527,526,1053,0.1317288875579834,0.00025189384711078695
527,528,527,1055,0.13201212882995605,0.00023325780523991986
528,529,528,1057,0.13222694396972656,0.00021068471707688167
529,530,529,1059,0.13316798210144043,0.0001843140682198331
530,531,530,1061,0.13340091705322266,0.00015493964377480792
531,532,531,1063,0.1335277557373047,0.0001241728762558038
532,533,532,1065,0.13367676734924316,0.0001294236591350424
533,534,533,1067,0.13391399383544922,0.00013188830848727214
534,535,534,1069,0.13421082496643066,0.0001078705274006648
535,536,535,1071,0.13439583778381348,8.71860011532785e-05
536,537,536,1073,0.13456106185913086,9.072923122134982e-05
537,538,537,1075,0.13469910621643066,7.329844959848635e-05
538,539,538,1077,0.13485383987426758,7.105034623301897e-05
539,540,539,1079,0.1350400447845459,0.00010348042431342327
540,541,540,1081,0.13527512550354004,0.00010247668319204456
541,542,541,1083,0.13556480407714844,0.000101535748941473
542,543,542,1085,0.1357588768005371,0.00010027899024394303
543,544,543,1087,0.1359550952911377,9.861378756462133e-05
544,545,544,1089,0.13613295555114746,9.642017635942056e-05
545,546,545,1091,0.13630390167236328,9.35530665034017e-05
546,547,546,1093,0.1366128921508789,8.98450138304448e-05
547,548,547,1095,0.13686585426330566,8.511686408534255e-05
548,549,548,1097,0.13701105117797852,7.920153336141747e-05
549,550,549,1099,0.13721203804016113,7.198683035416737e-05
550,551,550,1101,0.137376070022583,6.348051791586758e-05
551,552,551,1103,0.13753700256347656,5.389037033844798e-05
552,553,552,1105,0.1377098560333252,4.368940923620456e-05
553,554,553,1107,0.13786602020263672,4.129569447186343e-05
554,555,554,1109,0.13800787925720215,4.2728178823504556e-05
555,556,555,1111,0.13817501068115234,4.042699156976906e-05
556,557,556,1113,0.13834095001220703,3.29368437143913e-05
557,558,557,1115,0.13849878311157227,2.6299549837492763e-05
558,559,558,1117,0.13869094848632812,3.3353446700785706e-05
559,560,559,1119,0.13902902603149414,3.4244309568797964e-05
560,561,560,1121,0.13963985443115234,3.805335608129186e-05
561,562,561,1123,0.14063191413879395,3.721914669492418e-05
562,563,562,1125,0.1408400535583496,3.627245266597335e-05
563,564,563,1127,0.1412067413330078,3.5036313777584835e-05
564,565,564,1129,0.14150190353393555,3.344732722032278e-05
565,566,565,1131,0.1418769359588623,3.143794556600345e-05
566,567,566,1133,0.14215302467346191,2.8951606639151776e-05
567,568,567,1135,0.14231085777282715,2.5963709857897576e-05
568,569,568,1137,0.14261579513549805,2.2509305908073128e-05
569,570,569,1139,0.1428391933441162,1.87137962919938e-05
570,571,570,1141,0.14298605918884277,1.4806416105023654e-05
571,572,571,1143,0.1431901454925537,1.6363670817535298e-05
572,573,572,1145,0.14336705207824707,1.557734809205703e-05
573,574,573,1147,0.14356589317321777,1.2074101735323335e-05
574,575,574,1149,0.143812894821167,1.2900799864178555e-05
575,576,575,1151,0.14405298233032227,1.6568937007998404e-05
576,577,576,1153,0.14419007301330566,1.582709966371723e-05
577,578,577,1155,0.14434599876403809,1.5136227918251953e-05
578,579,578,1157,0.14449286460876465,1.4242372160316145e-05
579,580,579,1159,0.1446831226348877,1.3137353127513472e-05
580,581,580,1161,0.14485883712768555,1.180478718064724e-05
581,582,581,1163,0.1450350284576416,1.0261205667636852e-05
582,583,582,1165,0.1453239917755127,8.55536766520754e-06
583,584,583,1167,0.14572978019714355,6.799198994519411e-06
584,585,584,1169,0.14586997032165527,8.727218363257263e-06
585,586,585,1171,0.14601898193359375,8.983972744395711e-06
586,587,586,1173,0.14627313613891602,9.85753993508241e-06
587,588,587,1175,0.14642000198364258,9.674728657730781e-06
588,589,588,1177,0.1465599536895752,9.462655100954662e-06
589,590,589,1179,0.1466808319091797,9.184645474541015e-06
590,591,590,1181,0.1468219757080078,8.824861977735817e-06
591,592,591,1183,0.14698195457458496,8.36575872716566e-06
592,593,592,1185,0.14711785316467285,7.79078925939884e-06
593,594,593,1187,0.14752912521362305,7.0886147253272005e-06
594,595,594,1189,0.14779186248779297,6.259342106892222e-06
595,596,595,1191,0.14801692962646484,5.322428106872912e-06
596,597,596,1193,0.14815282821655273,4.323153158979861e-06
597,598,597,1195,0.14846086502075195,3.925549814518708e-06
598,599,598,1197,0.14878296852111816,4.17390228920901e-06
599,600,599,1199,0.14896106719970703,3.958603014378573e-06
600,601,600,1201,0.14909601211547852,3.3658050275692063e-06
601,602,601,1203,0.1492319107055664,2.6764191149119246e-06
602,603,602,1205,0.14936399459838867,3.2041886826868785e-06
603,604,603,1207,0.14950990676879883,3.5258200678099158e-06
604,605,604,1209,0.14967775344848633,3.173202477305132e-06
605,606,605,1211,0.14980411529541016,2.8528725962364416e-06
606,607,606,1213,0.15001392364501953,2.7422471801055516e-06
607,608,607,1215,0.1501908302307129,3.2313842859497985e-06
608,609,608,1217,0.15032410621643066,3.14446859271509e-06
609,610,609,1219,0.15044593811035156,3.053376179171684e-06
610,611,610,1221,0.15057682991027832,2.934367493264713e-06
611,612,611,1223,0.15082812309265137,2.7825635597345354e-06
612,613,612,1225,0.15120792388916016,2.5923145576574554e-06
613,614,613,1227,0.1514897346496582,2.3598550372601762e-06
614,615,614,1229,0.1517629623413086,2.0850731112294224e-06
615,616,615,1231,0.15192890167236328,1.7743573426002236e-06
616,617,616,1233,0.15211987495422363,1.442451504230832e-06
617,618,617,1235,0.15230798721313477,1.2634160125774093e-06
618,619,618,1237,0.15254592895507812,1.4791781399802375e-06
619,620,619,1239,0.15271306037902832,1.444043687203794e-06
620,621,620,1241,0.15285491943359375,1.6785716267665588e-06
621,622,621,1243,0.15303611755371094,1.6107031432957775e-06
622,623,622,1245,0.15314793586730957,1.5404354173955313e-06
623,624,623,1247,0.1532609462738037,1.4504114104220994e-06
624,625,624,1249,0.15337896347045898,1.338761647608497e-06
625,626,625,1251,0.15348482131958008,1.2041742637638083e-06
626,627,626,1253,0.1536860466003418,1.04780755161703e-06
627,628,627,1255,0.15386509895324707,8.751315733401114e-07
628,629,628,1257,0.15404295921325684,6.957450133353293e-07
629,630,629,1259,0.1541907787322998,6.455517865926803e-07
630,631,630,1261,0.15433406829833984,9.733680388533302e-07
631,632,631,1263,0.15448498725891113,9.27822875991075e-07
632,633,632,1265,0.15468287467956543,8.896409529192661e-07
633,634,633,1267,0.1548309326171875,8.399958991408978e-07
634,635,634,1269,0.15507197380065918,7.781960290358588e-07
635,636,635,1271,0.15529203414916992,7.033289640052263e-07
636,637,636,1273,0.15554094314575195,6.157051460064349e-07
637,638,637,1275,0.1557159423828125,5.180962905278567e-07
638,639,638,1277,0.1558690071105957,4.1540044415629854e-07
639,640,639,1279,0.15602684020996094,3.2808037924456743e-07
640,641,640,1281,0.15618109703063965,5.372344206121017e-07
641,642,641,1283,0.15630197525024414,4.790173925290075e-07
642,643,642,1285,0.15642881393432617,4.3927255125929794e-07
643,644,643,1287,0.15671515464782715,3.890152565995853e-07
644,645,644,1289,0.15701580047607422,4.086740437147313e-07
645,646,645,1291,0.1571640968322754,4.5894902563734044e-07
646,647,646,1293,0.1574258804321289,4.496969674851456e-07
647,648,647,1295,0.1576390266418457,4.39367046801127e-07
648,649,648,1297,0.15777802467346191,4.2580729667718877e-07
649,650,649,1299,0.15792012214660645,4.0830327408119805e-07
650,651,650,1301,0.1581110954284668,3.860260960060049e-07
651,652,651,1303,0.1582798957824707,3.5823257276292523e-07
652,653,652,1305,0.1584310531616211,3.244569566218033e-07
653,654,653,1307,0.15870904922485352,2.8483245238894333e-07
654,655,654,1309,0.15895414352416992,2.4045030643586215e-07
655,656,655,1311,0.15911507606506348,1.936467563690439e-07
656,657,656,1313,0.15926575660705566,1.836298701387651e-07
657,658,657,1315,0.15941405296325684,1.7810678671087662e-07
658,659,658,1317,0.15955901145935059,2.065531276053515e-07
659,660,659,1319,0.15978693962097168,1.7052684072467039e-07
660,661,660,1321,0.1600170135498047,1.4587275827296616e-07
661,662,661,1323,0.1602308750152588,1.156219899244643e-07
662,663,662,1325,0.16037988662719727,1.6384115706480607e-07
663,664,663,1327,0.16051101684570312,1.5414805324655072e-07
664,665,664,1329,0.16066598892211914,1.587383136188264e-07
665,666,665,1331,0.1608278751373291,1.5760678625243878e-07
666,667,666,1333,0.16095495223999023,1.5817756151800056e-07
667,668,667,1335,0.16111397743225098,1.5289671037279424e-07
668,669,668,1337,0.16130995750427246,1.4635406110626415e-07
669,670,669,1339,0.1615278720855713,1.380360353712995e-07
670,671,670,1341,0.16167306900024414,1.2769217013664072e-07
671,672,671,1343,0.16181087493896484,1.1518059257981035e-07
672,673,672,1345,0.1619420051574707,1.0058820099912389e-07
673,674,673,1347,0.1622300148010254,8.43757575462795e-08
674,675,674,1349,0.16237807273864746,6.743950143586681e-08
675,676,675,1351,0.1625349521636963,6.445704877605943e-08
676,677,676,1353,0.1626598834991455,8.667910629137427e-08
677,678,677,1355,0.16285490989685059,7.565575244041326e-08
678,679,678,1357,0.1630868911743164,6.776502457035718e-08
679,680,679,1359,0.16381502151489258,5.786273806846621e-08
680,681,680,1361,0.16492486000061035,5.298820145662533e-08
681,682,681,1363,0.1651301383972168,6.549837770462968e-08
682,683,682,1365,0.16529583930969238,5.9075367355829924e-08
683,684,683,1367,0.1655287742614746,5.38383504996078e-08
684,685,684,1369,0.16569781303405762,5.176148012542374e-08
685,686,685,1371,0.16583895683288574,5.9214036712708214e-08
686,687,686,1373,0.16612005233764648,5.730232121641318e-08
687,688,687,1375,0.1664741039276123,5.5268414674592546e-08
688,689,688,1377,0.16694879531860352,5.263262739424685e-08
689,690,689,1379,0.16710495948791504,4.931436020556364e-08
690,691,690,1381,0.1672511100769043,4.522423242556543e-08
691,692,691,1383,0.16748404502868652,4.0339066463981715e-08
692,693,692,1385,0.16767382621765137,3.473288579565445e-08
693,694,693,1387,0.16780805587768555,2.8640315161612707e-08
694,695,694,1389,0.16798710823059082,2.3140610397070877e-08
695,696,695,1391,0.16814494132995605,2.1612744973770494e-08
696,697,696,1393,0.16827392578125,3.325764520049203e-08
697,698,697,1395,0.16842198371887207,3.236832717466414e-08
698,699,698,1397,0.16861391067504883,3.1594055666870164e-08
699,700,699,1399,0.16882801055908203,3.0572589264540734e-08
700,701,700,1401,0.16903305053710938,2.9256224804849478e-08
701,702,701,1403,0.16917681694030762,2.7585951151947223e-08
702,703,702,1405,0.16936087608337402,2.550986819904457e-08
703,704,703,1407,0.16960692405700684,2.300011754247135e-08
704,705,704,1409,0.1698770523071289,2.0074656169758468e-08
705,706,705,1411,0.17002606391906738,1.682702494396246e-08
706,707,706,1413,0.1701669692993164,1.3438747951297046e-08
707,708,707,1415,0.17030096054077148,1.312305225806213e-08
708,709,708,1417,0.17044401168823242,1.5715007998173292e-08
709,710,709,1419,0.1705780029296875,1.2524741801304135e-08
710,711,710,1421,0.17072701454162598,1.0640553318087468e-08
711,712,711,1423,0.17087101936340332,8.18213798994825e-09
712,713,712,1425,0.17102384567260742,1.25511686798817e-08
713,714,713,1427,0.17122483253479004,1.1557778105689238e-08
714,715,714,1429,0.17136788368225098,1.103344446769077e-08
715,716,715,1431,0.17149710655212402,1.0884120066273268e-08
716,717,716,1433,0.17163705825805664,1.2015484026586467e-08
717,718,717,1435,0.17199087142944336,1.1887527498351184e-08
718,719,718,1437,0.17342901229858398,1.1737141353263696e-08
719,720,719,1439,0.17367887496948242,1.1538295314361068e-08
720,721,720,1441,0.17388391494750977,1.1275875118379231e-08
721,722,721,1443,0.17403292655944824,1.0933681120633532e-08
722,723,722,1445,0.1742081642150879,1.0491179205010649e-08
723,724,723,1447,0.17446589469909668,9.927531444514891e-09
724,725,724,1449,0.17479205131530762,9.223442932930333e-09
725,726,725,1451,0.1750028133392334,8.366369698367098e-09
726,727,726,1453,0.1751859188079834,7.358537549567513e-09
727,728,727,1455,0.17536187171936035,6.22662915428347e-09
728,729,728,1457,0.17550396919250488,5.028430126529233e-09
729,730,729,1459,0.17583489418029785,4.507598536168781e-09
730,731,730,1461,0.17602896690368652,4.7453449666157106e-09
731,732,731,1463,0.17622780799865723,4.067042104891707e-09
732,733,732,1465,0.17650318145751953,3.253093265665017e-09
733,734,733,1467,0.17671775817871094,4.114124465574654e-09
734,735,734,1469,0.1768798828125,4.256327519955027e-09
735,736,735,1471,0.17706704139709473,4.684631754573519e-09
736,737,736,1473,0.17721891403198242,4.579155051405645e-09
737,738,737,1475,0.17736411094665527,4.458574313807946e-09
738,739,738,1477,0.17749881744384766,4.301241546644073e-09
739,740,739,1479,0.17764592170715332,4.099667822718583e-09
740,741,740,1481,0.1778559684753418,3.8447966504252275e-09
741,742,741,1483,0.17800307273864746,3.530759061051434e-09
742,743,742,1485,0.17818093299865723,3.1546921189815532e-09
743,744,743,1487,0.17861294746398926,2.722215299387753e-09
744,745,744,1489,0.1787729263305664,2.250279169041266e-09
745,746,745,1491,0.17892098426818848,1.7685541252749223e-09
746,747,746,1493,0.1790931224822998,1.919832622534006e-09
747,748,747,1495,0.17927002906799316,1.769178714748502e-09
748,749,748,1497,0.179426908493042,1.3258814423051768e-09
749,750,749,1499,0.17956781387329102,1.7082243634066616e-09
750,751,750,1501,0.179732084274292,1.839970450554488e-09
751,752,751,1503,0.1799459457397461,1.8113510478932405e-09
752,753,752,1505,0.18019580841064453,1.924482873754195e-09
753,754,753,1507,0.18154597282409668,1.8876331318272975e-09
754,755,754,1509,0.18199992179870605,1.844237321645057e-09
755,756,755,1511,0.18214797973632812,1.7872049860726878e-09
756,757,756,1513,0.18232297897338867,1.713602398276652e-09
757,758,757,1515,0.18247199058532715,1.620170988501321e-09
758,759,758,1517,0.18262004852294922,1.5033261334328239e-09
759,760,759,1519,0.18275213241577148,1.3615021753688169e-09
760,761,760,1521,0.18290376663208008,1.195136039686332e-09
761,762,761,1523,0.18319177627563477,1.0087060452378568e-09
762,763,762,1525,0.18345999717712402,8.118445428176673e-10
763,764,763,1527,0.18359613418579102,7.434451202046483e-10
764,765,764,1529,0.18375396728515625,7.550875188815826e-10
765,766,765,1531,0.18391990661621094,6.814509636722767e-10
766,767,766,1533,0.18411707878112793,5.13818759064102e-10
767,768,767,1535,0.18426084518432617,7.022188787285602e-10
768,769,768,1537,0.18444299697875977,7.169792396109498e-10
769,770,769,1539,0.18456697463989258,7.918232727521341e-10
770,771,770,1541,0.18470096588134766,7.877596239072175e-10
771,772,771,1543,0.18481898307800293,7.830857872078105e-10
772,773,772,1545,0.18497586250305176,7.768041999989225e-10
773,774,773,1547,0.18508505821228027,7.688707070841052e-10
774,775,774,1549,0.1852130889892578,7.577809064616734e-10
775,776,775,1551,0.1853489875793457,7.43103107492323e-10
776,777,776,1553,0.18549489974975586,7.244520802403217e-10
777,778,777,1555,0.18579316139221191,6.996230502084038e-10
778,779,778,1557,0.18594598770141602,6.679030883966877e-10
779,780,779,1559,0.18615412712097168,6.27817061447573e-10
780,781,780,1561,0.18633604049682617,5.781603032693598e-10
781,782,781,1563,0.1868429183959961,5.18156873267592e-10
782,783,782,1565,0.18698596954345703,4.4904617376106024e-10
783,784,783,1567,0.18712496757507324,3.734164128521621e-10
784,785,784,1569,0.18728303909301758,2.9523997555338796e-10
785,786,785,1571,0.18742895126342773,3.092551179127568e-10
786,787,786,1573,0.1875600814819336,3.357862847333176e-10
787,788,787,1575,0.1877131462097168,2.6136149498077654e-10
788,789,788,1577,0.18793892860412598,2.1718001913278755e-10
789,790,789,1579,0.18865013122558594,2.8738689902785875e-10
790,791,790,1581,0.18940496444702148,2.776475218444594e-10
791,792,791,1583,0.18958401679992676,3.0841189727513084e-10
792,793,792,1585,0.1897568702697754,3.0212846689533487e-10
793,794,793,1587,0.18997693061828613,2.9537053160426424e-10
794,795,794,1589,0.190216064453125,2.8617082110354423e-10
795,796,795,1591,0.19038605690002441,2.7440999983140667e-10
796,797,796,1593,0.19058489799499512,2.5949561424335095e-10
797,798,797,1595,0.19076108932495117,2.408463508906231e-10
798,799,798,1597,0.19091105461120605,2.182383075653145e-10
799,800,799,1599,0.19106101989746094,1.9156359618803722e-10
800,801,800,1601,0.19120287895202637,1.6186552285535254e-10
801,802,801,1603,0.1914520263671875,1.302853533651303e-10
802,803,802,1605,0.19161081314086914,1.221625941182863e-10
803,804,803,1607,0.19189095497131348,1.0024650271294336e-10
804,805,804,1609,0.19203686714172363,1.4697070366712391e-10
805,806,805,1611,0.19234108924865723,1.2762084884901287e-10
806,807,806,1613,0.19251680374145508,1.1460837964211863e-10
807,808,807,1615,0.1926579475402832,1.0169017687819955e-10
808,809,808,1617,0.19300198554992676,1.2820954600271274e-10
809,810,809,1619,0.19329214096069336,1.237646494196996e-10
810,811,810,1621,0.19344687461853027,1.1899734297065564e-10
811,812,811,1623,0.1936049461364746,1.1294972281488796e-10
812,813,812,1625,0.19382572174072266,1.0525664521643934e-10
813,814,813,1627,0.19442486763000488,9.618530403259426e-11


==> plot_data/cournot-nash_equilibrium_problem_n100/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00016617774963378906,1624.447741208611
1,3,2,5,0.00046324729919433594,1272.8713625173957
2,5,4,9,0.0006520748138427734,961.6137427304949
3,7,6,13,0.0009510517120361328,698.4469064029521
4,9,8,17,0.0011839866638183594,497.92827037651625
5,11,10,21,0.0014050006866455078,385.1543340115312
6,13,12,25,0.0016498565673828125,334.70183338220033
7,15,14,29,0.0019240379333496094,316.76841860359195
8,17,16,33,0.0022020339965820312,327.92081477771296
9,19,18,37,0.003567218780517578,272.49749970969134
10,21,20,41,0.003902912139892578,580.6881017547407
11,23,22,45,0.004102230072021484,220.37726852264976
12,25,24,49,0.00448298454284668,224.8553449936177
13,27,26,53,0.004815101623535156,266.8895204854363
14,29,28,57,0.0050280094146728516,193.4461392124149
15,31,30,61,0.005266904830932617,834.3068414059894
16,33,32,65,0.0055811405181884766,239.0170517910166
17,35,34,69,0.005856990814208984,3407.7137433560315
18,37,36,73,0.00609898567199707,1248.784258972877
19,39,38,77,0.006293058395385742,139.41341914046623
20,41,40,81,0.0064928531646728516,21594.00614835975
21,43,42,85,0.006669044494628906,194.57039389801992
22,45,44,89,0.00693511962890625,350.2600749481253
23,47,46,93,0.007136106491088867,33.07326526419472
24,49,48,97,0.007324934005737305,2234.706125432987
25,51,50,101,0.007554054260253906,33.941357938318475
26,53,52,105,0.007800102233886719,14592.08385644159
27,55,54,109,0.008140087127685547,8.535298976600176
28,57,56,113,0.008419036865234375,1.9797757421528643
29,59,58,117,0.008686065673828125,708.1251614479401
30,61,60,121,0.008901119232177734,3.0406105836254578
31,63,62,125,0.009112119674682617,0.05033558955791663
32,65,64,129,0.009371280670166016,0.013555356108673694
33,67,66,133,0.009653091430664062,0.0016659262350161277
34,69,68,137,0.010061025619506836,0.0007543427002068241
35,71,70,141,0.010424137115478516,0.05669953626123291
36,73,72,145,0.010940074920654297,0.005812801321401162
37,75,74,149,0.011173248291015625,0.00027999462185209867
38,77,76,153,0.011576175689697266,5.531443138224024e-05
39,79,78,157,0.011789083480834961,1.8223553300803196e-05
40,81,80,161,0.011990070343017578,1.458594488182131e-05
41,83,82,165,0.012211084365844727,6.378948061889272e-05
42,85,84,169,0.016657114028930664,4.858754591547119e-07
43,87,86,173,0.017135143280029297,2.866684788390133e-07
44,89,88,177,0.01743793487548828,1.9825944825746362e-07
45,91,90,181,0.01818108558654785,6.766214604747112e-07
46,93,92,185,0.018453121185302734,1.972787088051743e-05
47,95,94,189,0.018705129623413086,1.0200175100283561e-07
48,97,96,193,0.018964052200317383,6.692561059923934e-08
49,99,98,197,0.019346952438354492,3.9603857126417814e-08
50,101,100,201,0.020010948181152344,5.604264415329674e-07
51,103,102,205,0.020631074905395508,2.7120724455841196e-08
52,105,104,209,0.021033048629760742,1.6431127223134333e-08
53,107,106,213,0.021338224411010742,1.8854614096691566e-08
54,109,108,217,0.02155590057373047,4.591250674012719e-06
55,111,110,221,0.021790027618408203,1.4128208926879017e-08
56,113,112,225,0.02392125129699707,5.224481012986719e-10
57,115,114,229,0.02492213249206543,8.689190939431684e-09
58,117,116,233,0.026108264923095703,7.738129801392896e-09
59,119,118,237,0.02697920799255371,3.588271974240823e-10
60,121,120,241,0.02750706672668457,3.7388744250579685e-10
61,123,122,245,0.027802228927612305,1.7566317819302195e-08
62,125,124,249,0.028042078018188477,5.05560233900088e-11


==> plot_data/cournot-nash_equilibrium_problem_n100/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.000225067138671875,1624.447741208611
2,5,4,9,0.003520965576171875,1074.9762595826073
4,9,8,17,0.004966020584106445,681.7815756458663
6,13,12,25,0.006433010101318359,463.5938329857111
8,17,16,33,0.007317066192626953,363.2997632560372
10,21,20,41,0.007950067520141602,310.1010433484549
12,25,24,49,0.009347915649414062,283.49492238268476
14,29,28,57,0.010691165924072266,265.63648716184593
16,33,32,65,0.011513233184814453,241.06426178394614
18,37,36,73,0.012611865997314453,234.03537577243546
20,41,40,81,0.013212919235229492,222.06145980842268
22,45,44,89,0.014168024063110352,209.41498544964557
24,49,48,97,0.017071008682250977,200.74033555129807
26,53,52,105,0.017852067947387695,188.64132703666422
28,57,56,113,0.018288850784301758,182.51331059309462
30,61,60,121,0.01868605613708496,168.09934603253112
32,65,64,129,0.01901698112487793,159.15802793415068
34,69,68,137,0.019357919692993164,155.30835317425192
36,73,72,145,0.020015954971313477,141.46198810810452
38,77,76,153,0.02047586441040039,137.66123385619966
40,81,80,161,0.02094292640686035,129.27776825774362
42,85,84,169,0.021355152130126953,124.0900664223253
44,89,88,177,0.022518157958984375,121.41934420331066
46,93,92,185,0.022849082946777344,119.39983820708568
48,97,96,193,0.02316904067993164,117.84080097273029
50,101,100,201,0.023467063903808594,110.73658910025752
52,105,104,209,0.02392411231994629,109.22864914657332
54,109,108,217,0.02424907684326172,108.0180346297841
56,113,112,225,0.024569034576416016,107.0175767838781
58,117,116,233,0.024879932403564453,106.1635655391015
60,121,120,241,0.025189876556396484,105.40999711959633
62,125,124,249,0.025495052337646484,104.72403047594116
64,129,128,257,0.02604389190673828,98.1301559079027
66,133,132,265,0.026340007781982422,97.31347085260819
68,137,136,273,0.026670217514038086,96.59119460505664
70,141,140,281,0.026973962783813477,92.55492770562087
72,145,144,289,0.027347087860107422,91.81415086375299
74,149,148,297,0.02764606475830078,91.15157004344363
76,153,152,305,0.028046846389770508,90.54478419572912
78,157,156,313,0.02846384048461914,89.97722019224601
80,161,160,321,0.028859853744506836,89.43673019546448
82,165,164,329,0.029223918914794922,88.9145019880561
84,169,168,337,0.029534101486206055,88.404220719104
86,173,172,345,0.03036022186279297,87.90142906828191
88,177,176,353,0.031110048294067383,87.40304197617908
90,181,180,361,0.031816959381103516,86.90698061718919
92,185,184,369,0.03248119354248047,86.41189768592928
94,189,188,377,0.03296303749084473,85.91697220576324
96,193,192,385,0.033358097076416016,85.42175701960993
98,197,196,393,0.033946990966796875,80.56034730897348
100,201,200,401,0.03435015678405762,77.06956513918219
102,205,204,409,0.034783124923706055,76.10163691707787
104,209,208,417,0.03700113296508789,71.18794986306793
106,213,212,425,0.037420034408569336,70.26576633337868
108,217,216,433,0.03819394111633301,69.59564888314954
110,221,220,441,0.03857111930847168,68.99149991945642
112,225,224,449,0.03893780708312988,68.44001081917901
114,229,228,457,0.03939104080200195,67.93040857110837
116,233,232,465,0.039888858795166016,67.4540121696671
118,237,236,473,0.04052090644836426,67.00385642644123
120,241,240,481,0.041259050369262695,66.57437630119239
122,245,244,489,0.04166007041931152,66.16114427000407
124,249,248,497,0.04217982292175293,65.76065333636919
126,253,252,505,0.04264187812805176,65.37013877664205
128,257,256,513,0.043107032775878906,64.98743240048361
130,261,260,521,0.04350590705871582,64.61084387208813
132,265,264,529,0.04388618469238281,64.2390643994702
134,269,268,537,0.04433584213256836,63.87108881159765
136,273,272,545,0.04477500915527344,63.506152684169386
138,277,276,553,0.04539012908935547,63.14368173617925
140,281,280,561,0.04583406448364258,43.05362782494803
142,285,284,569,0.04729509353637695,42.49177885828477
144,289,288,577,0.047883033752441406,41.97646035793068
146,293,292,585,0.0482790470123291,41.50087891390307
148,297,296,593,0.04870796203613281,41.05926500301267
150,301,300,601,0.04907083511352539,40.6467261325363
152,305,304,609,0.04962897300720215,40.25911810719962
154,309,308,617,0.05180001258850098,39.89293312135577
156,313,312,625,0.05258607864379883,39.54520315479662
158,317,316,633,0.05324292182922363,39.21341706390604
160,321,320,641,0.05377316474914551,38.8954497699031
162,325,324,649,0.05441117286682129,38.58950202001386
164,329,328,657,0.054901123046875,38.29404931010172
166,333,332,665,0.05537700653076172,38.00779868995192
168,337,336,673,0.05611395835876465,37.72965231183932
170,341,340,681,0.05653882026672363,37.458676720469455
172,345,344,689,0.057102203369140625,37.19407701239037
174,349,348,697,0.05766701698303223,36.93517511239121
176,353,352,705,0.05820918083190918,36.68139152184006
178,357,356,713,0.058873891830444336,36.432229989057426
180,361,360,721,0.059674978256225586,36.187264634941215
182,365,364,729,0.06016206741333008,30.02031504499176
184,369,368,737,0.06063389778137207,29.631314775608438
186,373,372,745,0.06339001655578613,29.273270353781925
188,377,376,753,0.06522202491760254,28.94200475222541
190,381,380,761,0.06553983688354492,28.633918140413318
192,385,384,769,0.06590795516967773,28.345912995016274
194,389,388,777,0.0663299560546875,28.07532725105172
196,393,392,785,0.06668710708618164,27.819875120361758
198,397,396,793,0.06727099418640137,27.57759506446527
200,401,400,801,0.06848001480102539,27.346804328604833
202,405,404,809,0.06883907318115234,25.56256956546132
204,409,408,817,0.06920003890991211,25.356983395907815
206,413,412,825,0.06952881813049316,25.20844320928263
208,417,416,833,0.06997203826904297,25.060801692928614
210,421,420,841,0.07030606269836426,24.914053652086505
212,425,424,849,0.07066082954406738,24.768193883119785
214,429,428,857,0.07106804847717285,24.62321717699849
216,433,432,865,0.07147598266601562,24.479118322480815
218,437,436,873,0.0719609260559082,24.335892109042256
220,441,440,881,0.07249116897583008,24.193533329555816
222,445,444,889,0.07291603088378906,24.052036782746818
224,449,448,897,0.07326698303222656,23.911397275437746
226,453,452,905,0.07367205619812012,23.771609624603638
228,457,456,913,0.07405400276184082,23.632668659248747
230,461,460,921,0.07441902160644531,23.494569222110368
232,465,464,929,0.07480502128601074,23.357306171222906
234,469,468,937,0.07525897026062012,23.220874381335484
236,473,472,945,0.07590603828430176,23.08526874519954
238,477,476,953,0.07644200325012207,21.631613847525454
240,481,480,961,0.07710504531860352,21.50167467099822
242,485,484,969,0.07744002342224121,21.37422272208519
244,489,488,977,0.0777890682220459,21.248963913561923
246,493,492,985,0.07815814018249512,21.12564544312637
248,497,496,993,0.07854223251342773,21.004050305339188
250,501,500,1001,0.07892990112304688,20.88399249652149
252,505,504,1009,0.0792999267578125,20.765312830886362
254,509,508,1017,0.07967591285705566,20.647875294596968
256,513,512,1025,0.08009719848632812,20.53156387221639
258,517,516,1033,0.08110594749450684,20.416279787334407
260,521,520,1041,0.0823509693145752,20.301939105709835
262,525,524,1049,0.08302903175354004,20.18847065529818
264,529,528,1057,0.08342885971069336,20.075814222946814
266,533,532,1065,0.0840461254119873,19.96391899234228
268,537,536,1073,0.08452105522155762,19.8527421921584
270,541,540,1081,0.08485102653503418,19.742247927161223
272,545,544,1089,0.08526897430419922,19.632406168419053
274,549,548,1097,0.08579111099243164,19.523191881788904
276,553,552,1105,0.08617496490478516,19.414584276466492
278,557,556,1113,0.08731389045715332,19.306566157729467
280,561,560,1121,0.08790302276611328,19.199123370011726
282,565,564,1129,0.08860015869140625,19.092244318280216
284,569,568,1137,0.08949518203735352,18.985919557189884
286,573,572,1145,0.09032821655273438,18.880141438918187
288,577,576,1153,0.09125399589538574,18.774903811719277
290,581,580,1161,0.09430885314941406,17.588038190234478
292,585,584,1169,0.09699797630310059,17.47575474085659
294,589,588,1177,0.09757494926452637,17.3662687083676
296,593,592,1185,0.09865593910217285,17.25930109930783
298,597,596,1193,0.10191106796264648,17.15460434053991
300,601,600,1201,0.10544490814208984,17.05195888954582
302,605,604,1209,0.10633993148803711,16.95117018621938
304,609,608,1217,0.1091458797454834,16.852065916132258
306,613,612,1225,0.11037397384643555,16.75449355701555
308,617,616,1233,0.1114649772644043,16.658318182024995
310,621,620,1241,0.11260390281677246,16.563420495222818
312,625,624,1249,0.11407995223999023,16.469695076611735
314,629,628,1257,0.11520099639892578,16.377048815898192
316,633,632,1265,0.11572504043579102,16.285399515922496
318,637,636,1273,0.1163029670715332,16.194674648392375
320,641,640,1281,0.1185150146484375,16.104810246137145
322,645,644,1289,0.1192011833190918,16.01574991759451
324,649,648,1297,0.11988997459411621,15.92744397061115
326,653,652,1305,0.12042903900146484,15.839848633897864
328,657,656,1313,0.12081694602966309,15.75292536566621
330,661,660,1321,0.12127208709716797,15.66664024000397
332,665,664,1329,0.12166309356689453,15.580963402558352
334,669,668,1337,0.12207221984863281,15.495868587925122
336,673,672,1345,0.12257099151611328,15.411332691986484
338,677,676,1353,0.12292313575744629,15.327335393100128
340,681,680,1361,0.12363600730895996,14.609550428198386
342,685,684,1369,0.12484502792358398,14.357452875413028
344,689,688,1377,0.12540078163146973,14.26640945131788
346,693,692,1385,0.12572693824768066,14.177386692201623
348,697,696,1393,0.12617921829223633,14.09020974241247
350,701,700,1401,0.126694917678833,14.004721077280868
352,705,704,1409,0.1271061897277832,13.920778867515148
354,709,708,1417,0.12757205963134766,13.838255485926483
356,713,712,1425,0.1280231475830078,5.810373159582504
358,717,716,1433,0.12838006019592285,5.693732568137597
360,721,720,1441,0.12874603271484375,5.583637709398936
362,725,724,1449,0.12906908988952637,5.479680806454381
364,729,728,1457,0.12972283363342285,5.381474035126806
366,733,732,1465,0.13018202781677246,5.288649113834686
368,737,736,1473,0.13060522079467773,5.200856863994831
370,741,740,1481,0.13098907470703125,5.11776673905473
372,745,744,1489,0.13144207000732422,5.039066321765213
374,749,748,1497,0.13300299644470215,4.9644607906049085
376,753,752,1505,0.13350296020507812,4.893672357422983
378,757,756,1513,0.1339409351348877,4.826439679279338
380,761,760,1521,0.13429617881774902,4.762517248160752
382,765,764,1529,0.1348729133605957,4.701674762769176
384,769,768,1537,0.13550996780395508,4.643696486854773
386,773,772,1545,0.13622403144836426,4.588380598705006
388,777,776,1553,0.13724589347839355,4.5355385363599865
390,781,780,1561,0.1379399299621582,4.484994342985319
392,785,784,1569,0.13839006423950195,4.436584016546761
394,789,788,1577,0.13882184028625488,4.390154867620876
396,793,792,1585,0.13926982879638672,4.345564888770336
398,797,796,1593,0.1413719654083252,4.302682138510012
400,801,800,1601,0.14204812049865723,4.261384142432892
402,805,804,1609,0.14263701438903809,4.221557313653099
404,809,808,1617,0.14322590827941895,4.183096394290559
406,813,812,1625,0.1437070369720459,4.145903919336139
408,817,816,1633,0.1442708969116211,4.109889703841717
410,821,820,1641,0.14476919174194336,4.074970354086526
412,825,824,1649,0.14556002616882324,4.041068803017976
414,829,828,1657,0.14605712890625,4.008113870045274
416,833,832,1665,0.14656400680541992,3.9760398450187053
418,837,836,1673,0.1469881534576416,3.944786096015071
420,841,840,1681,0.1474919319152832,3.914296700427439
422,845,844,1689,0.15047192573547363,3.8845200986917576
424,849,848,1697,0.15106201171875,3.855408769894528
426,853,852,1705,0.15198898315429688,3.826918928426905
428,857,856,1713,0.15272998809814453,3.7990102407845647
430,861,860,1721,0.1533060073852539,3.771645561588121
432,865,864,1729,0.15375113487243652,3.744790687857948
434,869,868,1737,0.15461111068725586,3.718414130584398
436,873,872,1745,0.15520596504211426,3.6924869026369658
438,877,876,1753,0.155897855758667,3.6669823220445776
440,881,880,1761,0.1563568115234375,3.6418758297451865
442,885,884,1769,0.158250093460083,3.617144820878758
444,889,888,1777,0.15868496894836426,3.5927684887617826
446,893,892,1785,0.1592390537261963,3.5687276807095496
448,897,896,1793,0.15981388092041016,3.5450047648984806
450,901,900,1801,0.16023802757263184,3.521583507508764
452,905,904,1809,0.1607990264892578,3.498448959430378
454,909,908,1817,0.16124200820922852,3.4755873518418574
456,913,912,1825,0.1616039276123047,3.4529860000209607
458,917,916,1833,0.16202092170715332,3.4306332147845793
460,921,920,1841,0.16236114501953125,3.4085182209834834
462,925,924,1849,0.16280293464660645,3.386631082528008
464,929,928,1857,0.16326498985290527,3.3649626334477682
466,933,932,1865,0.16362905502319336,3.3435044145136423
468,937,936,1873,0.16564202308654785,3.322248615001327
470,941,940,1881,0.16606998443603516,3.3011880191935914
472,945,944,1889,0.16650915145874023,3.280315957248566
474,949,948,1897,0.16696596145629883,3.2596262600836328
476,953,952,1905,0.16733002662658691,3.2391132179691486
478,957,956,1913,0.16773414611816406,3.218771542520649
480,961,960,1921,0.1681990623474121,3.1985963318289636
482,965,964,1929,0.1688530445098877,3.178583038468979
484,969,968,1937,0.16929411888122559,3.1587274401560896
486,973,972,1945,0.16958999633789062,3.1390256128309875
488,977,976,1953,0.17001104354858398,3.1194739059898047
490,981,980,1961,0.170928955078125,3.1000689200495843
492,985,984,1969,0.17136597633361816,3.080807485614032
494,989,988,1977,0.17186784744262695,3.0616866444551283
496,993,992,1985,0.17246007919311523,3.0427036320869765
498,997,996,1993,0.17282485961914062,3.023855861796521
501,1003,1002,2005,0.17332005500793457,2.9958325249577022
503,1007,1006,2013,0.1737380027770996,2.977312580827103
505,1011,1010,2021,0.17537212371826172,2.9589200246796143
507,1015,1014,2029,0.17584490776062012,2.940652905426399
509,1019,1018,2037,0.17623615264892578,2.9225093830032827
511,1023,1022,2045,0.17673206329345703,2.904487719328001
513,1027,1026,2053,0.1771390438079834,2.886586270013712
515,1031,1030,2061,0.17747783660888672,2.8688034767753545
517,1035,1034,2069,0.17783880233764648,2.54383724396991
519,1039,1038,2077,0.1782090663909912,2.2462688397207744
521,1043,1042,2085,0.17856907844543457,2.2244301293955133
523,1047,1046,2093,0.17898917198181152,2.2032664005568745
525,1051,1050,2101,0.17949390411376953,2.1827394327886718
527,1055,1054,2109,0.18024516105651855,2.1628132193131706
529,1059,1058,2117,0.18059301376342773,2.143453857558478
531,1063,1062,2125,0.18102407455444336,2.1246294428965906
533,1067,1066,2133,0.18282508850097656,2.1063099657194613
535,1071,1070,2141,0.18340682983398438,2.0884672119756655
537,1075,1074,2149,0.18398118019104004,2.07107466728716
539,1079,1078,2157,0.18441295623779297,2.054107424678921
541,1083,1082,2165,0.18480491638183594,2.037542095985451
543,1087,1086,2173,0.1853179931640625,2.021356726942106
545,1091,1090,2181,0.18572115898132324,2.005530715945752
547,1095,1094,2189,0.18644499778747559,1.9900447364546785
549,1099,1098,2197,0.18680906295776367,1.9748806629982953
551,1103,1102,2205,0.18727397918701172,1.9600215007004924
553,1107,1106,2213,0.18786311149597168,1.945451318281197
555,1111,1110,2221,0.18819522857666016,1.9311551844154973
557,1115,1114,2229,0.18851590156555176,1.91711910737687
559,1119,1118,2237,0.1888749599456787,1.903329977846354
561,1123,1122,2245,0.18938398361206055,1.8897755147991022
563,1127,1126,2253,0.1897890567779541,1.8764442143328828
565,1131,1130,2261,0.19082307815551758,1.8633253013399855
567,1135,1134,2269,0.19136595726013184,1.8504086839085918
569,1139,1138,2277,0.19173789024353027,1.8376849103109403
571,1143,1142,2285,0.192094087600708,1.8251451285062816
573,1147,1146,2293,0.19247698783874512,1.8127810479912534
575,1151,1150,2301,0.19282317161560059,1.8005849039269368
577,1155,1154,2309,0.19319510459899902,1.7885494234047583
579,1159,1158,2317,0.19353508949279785,1.7766677937563093
581,1163,1162,2325,0.1938610076904297,1.7649336327877898
583,1167,1166,2333,0.19417405128479004,1.7533409608563602
585,1171,1170,2341,0.1946859359741211,1.7418841746604061
587,1175,1174,2349,0.19506216049194336,1.73055802268021
589,1179,1178,2357,0.19541406631469727,1.7193575821515827
591,1183,1182,2365,0.19579386711120605,1.708278237501198
593,1187,1186,2373,0.1974179744720459,1.697315660145018
595,1191,1190,2381,0.19784998893737793,1.6864657895873274
597,1195,1194,2389,0.19838213920593262,1.67572481572394
599,1199,1198,2397,0.1988060474395752,1.665089162293896
601,1203,1202,2405,0.19912981986999512,1.654555471402307
603,1207,1206,2413,0.1996018886566162,1.644120589046107
605,1211,1210,2421,0.2000257968902588,1.633781551591254
607,1215,1214,2429,0.20039987564086914,1.6235355731298342
609,1219,1218,2437,0.20096111297607422,1.6133800336729485
611,1223,1222,2445,0.2016589641571045,1.6033124681188393
613,1227,1226,2453,0.20205283164978027,1.593330555952846
615,1231,1230,2461,0.2024080753326416,1.5834321116262295
617,1235,1234,2469,0.20295500755310059,1.573615075579938
619,1239,1238,2477,0.20334696769714355,1.5638775058630316
621,1243,1242,2485,0.20500397682189941,1.5542175703056431
623,1247,1246,2493,0.20614314079284668,1.5446335392247685
625,1251,1250,2501,0.20661616325378418,1.5351237786102467
627,1255,1254,2509,0.2071230411529541,1.5256867437720054
629,1259,1258,2517,0.2074439525604248,1.5163209734129157
631,1263,1262,2525,0.20783400535583496,1.5070250840987007
633,1267,1266,2533,0.2082200050354004,1.497797765103021
635,1271,1270,2541,0.2086038589477539,1.394753143914549
637,1275,1274,2549,0.20899319648742676,0.8261046481012412
639,1279,1278,2557,0.20940494537353516,0.811076510358488
641,1283,1282,2565,0.2097470760345459,0.7965868128058646
643,1287,1286,2573,0.2103288173675537,0.7826160111468873
645,1291,1290,2581,0.21070289611816406,0.769145092459996
647,1295,1294,2589,0.21111512184143066,0.7561555668413322
649,1299,1298,2597,0.21314477920532227,0.7436294594731283
651,1303,1302,2605,0.21365618705749512,0.7315493030501927
653,1307,1306,2613,0.21411585807800293,0.7198981304924273
655,1311,1310,2621,0.21456003189086914,0.7086594678848158
657,1315,1314,2629,0.21491694450378418,0.6978173275846542
659,1319,1318,2637,0.2154090404510498,0.6873562014328006
661,1323,1322,2645,0.215897798538208,0.6772610540244453
663,1327,1326,2653,0.2162470817565918,0.6675173159824528
665,1331,1330,2661,0.21663689613342285,0.6581108771967061
667,1335,1334,2669,0.21719813346862793,0.6490280799873468
669,1339,1338,2677,0.21766996383666992,0.640255712159642
671,1343,1342,2685,0.21838903427124023,0.6317809999224492
673,1347,1346,2693,0.21874094009399414,0.6235916006515233
675,1351,1350,2701,0.2190861701965332,0.6156755954740067
677,1355,1354,2709,0.21956896781921387,0.6080214816709898
679,1359,1358,2717,0.2202129364013672,0.600618164882785
681,1363,1362,2725,0.22163009643554688,0.5934549511217052
683,1367,1366,2733,0.2221660614013672,0.5865215385907163
685,1371,1370,2741,0.22257423400878906,0.5798080093155138
687,1375,1374,2749,0.22298192977905273,0.5733048205976252
689,1379,1378,2757,0.22335004806518555,0.5670027963054397
691,1383,1382,2765,0.22366905212402344,0.5608931180131841
693,1387,1386,2773,0.22406601905822754,0.5549673160087187
695,1391,1390,2781,0.22441601753234863,0.5492172601883055
697,1395,1394,2789,0.2247779369354248,0.5436351508594324
699,1399,1398,2797,0.22517800331115723,0.5382135094728443
701,1403,1402,2805,0.2256460189819336,0.532945169306036
703,1407,1406,2813,0.22601699829101562,0.5278232661190703
705,1411,1410,2821,0.22637391090393066,0.5228412288092734
707,1415,1414,2829,0.22689485549926758,0.5179927700819199
709,1419,1418,2837,0.2274320125579834,0.5132718771610238
711,1423,1422,2845,0.22780704498291016,0.5086728025598879
713,1427,1426,2853,0.228438138961792,0.5041900549313257
715,1431,1430,2861,0.2288651466369629,0.4998183900180182
717,1435,1434,2869,0.22919201850891113,0.49555280171556
719,1439,1438,2877,0.2295241355895996,0.49138851326877736
721,1443,1442,2885,0.22985291481018066,0.48732096861466
723,1447,1446,2893,0.23020124435424805,0.48334582388298336
725,1451,1450,2901,0.2304990291595459,0.47945893907032555
727,1455,1454,2909,0.2308349609375,0.4756563698954312
729,1459,1458,2917,0.23128604888916016,0.47193435984350507
731,1463,1462,2925,0.23172521591186523,0.46828933241174386
733,1467,1466,2933,0.23215007781982422,0.46471788355766813
735,1471,1470,2941,0.23322391510009766,0.46121677435935376
737,1475,1474,2949,0.2338418960571289,0.45778292388874303
739,1479,1478,2957,0.23582792282104492,0.4544134023010585
741,1483,1482,2965,0.23627090454101562,0.4511054241456127
743,1487,1486,2973,0.23666906356811523,0.4478563418939622
745,1491,1490,2981,0.23706293106079102,0.44466363968839523
747,1495,1494,2989,0.23747992515563965,0.4415249273106379
749,1499,1498,2997,0.2380070686340332,0.4384379343654403
751,1503,1502,3005,0.23839592933654785,0.43540050468129604
753,1507,1506,3013,0.23885393142700195,0.4324105909221864
755,1511,1510,3021,0.23932909965515137,0.42946624941056416
757,1515,1514,3029,0.23981809616088867,0.4265656351519966
759,1519,1518,3037,0.24057292938232422,0.423706997064041
761,1523,1522,3045,0.2410120964050293,0.42088867339995395
763,1527,1526,3053,0.24143385887145996,0.41810908736554214
765,1531,1530,3061,0.2421860694885254,0.4153667429209886
767,1535,1534,3069,0.24498510360717773,0.4126602207659163
769,1539,1538,3077,0.24567103385925293,0.4099881744994406
771,1543,1542,3085,0.2464299201965332,0.40734932695232345
773,1547,1546,3093,0.24733591079711914,0.4047424666835572
775,1551,1550,3101,0.2479538917541504,0.40216644463578316
777,1555,1554,3109,0.24845290184020996,0.399620170947167
779,1559,1558,3117,0.24941706657409668,0.39710261190953244
781,1563,1562,3125,0.24982190132141113,0.39461278707232467
783,1567,1566,3133,0.2501840591430664,0.39214976648003586
785,1571,1570,3141,0.250622034072876,0.3897126680470164
787,1575,1574,3149,0.2513909339904785,0.387300655055574
789,1579,1578,3157,0.25281786918640137,0.38491293377701913
791,1583,1582,3165,0.253216028213501,0.3825487512103434
793,1587,1586,3173,0.25365519523620605,0.38020739293082106
795,1591,1590,3181,0.25411105155944824,0.37788818104912153
797,1595,1594,3189,0.2545301914215088,0.3755904722669179
799,1599,1598,3197,0.25495290756225586,0.37331365603764066
801,1603,1602,3205,0.2552671432495117,0.3710571528144266
803,1607,1606,3213,0.2556149959564209,0.3688204123908952
805,1611,1610,3221,0.25609922409057617,0.36660291232434383
807,1615,1614,3229,0.25661301612854004,0.36440415644415847
809,1619,1618,3237,0.2569999694824219,0.36222367343101125
811,1623,1622,3245,0.2573409080505371,0.36006101547774194
813,1627,1626,3253,0.2588028907775879,0.3579157570125408
815,1631,1630,3261,0.25945186614990234,0.3557874934946165
817,1635,1634,3269,0.2599921226501465,0.3536758402698938
819,1639,1638,3277,0.2605729103088379,0.3515804314885204
821,1643,1642,3285,0.2610499858856201,0.34950091908011
823,1647,1646,3293,0.26163196563720703,0.34743697178113087
825,1651,1650,3301,0.26214599609375,0.3453882742173195
827,1655,1654,3309,0.26257801055908203,0.3433545260326307
829,1659,1658,3317,0.26303791999816895,0.3413354410674124
831,1663,1662,3325,0.26347804069519043,0.33933074657604406
833,1667,1666,3333,0.2638568878173828,0.3373401824933018
835,1671,1670,3341,0.26421093940734863,0.33536350073577964
837,1675,1674,3349,0.26456499099731445,0.3334004645421132
839,1679,1678,3357,0.2649059295654297,0.33145084784867457
841,1683,1682,3365,0.26542019844055176,0.32951443470219743
843,1687,1686,3373,0.2659170627593994,0.32759101870003426
845,1691,1690,3381,0.26625585556030273,0.3256804024644863
847,1695,1694,3389,0.266726016998291,0.32378239714383933
849,1699,1698,3397,0.26705479621887207,0.3218968219422105
851,1703,1702,3405,0.2673921585083008,0.3200235036745559
853,1707,1706,3413,0.26772212982177734,0.3181622763462518
855,1711,1710,3421,0.2680661678314209,0.316312980755314
857,1715,1714,3429,0.268420934677124,0.3144754641187991
859,1719,1718,3437,0.268751859664917,0.31264957971726204
861,1723,1722,3445,0.26912498474121094,0.3108351865599634
863,1727,1726,3453,0.26941394805908203,0.30903214906981935
865,1731,1730,3461,0.2697110176086426,0.30724033678353774
867,1735,1734,3469,0.2699930667877197,0.30545962407137006
869,1739,1738,3477,0.2704031467437744,0.30368988987017365
871,1743,1742,3485,0.2708089351654053,0.30193101743135875
873,1747,1746,3493,0.27118492126464844,0.30018289408568666
875,1751,1750,3501,0.27216482162475586,0.2984454110182448
877,1755,1754,3509,0.2724781036376953,0.2967184630575109
879,1759,1758,3517,0.2727780342102051,0.2950019484754627
881,1763,1762,3525,0.27309703826904297,0.2932957688011875
883,1767,1766,3533,0.2734510898590088,0.2915998286411093
885,1771,1770,3541,0.27376794815063477,0.2899140355133697
887,1775,1774,3549,0.2741100788116455,0.28823829968902215
889,1779,1778,3557,0.2744169235229492,0.2865725340426965
891,1783,1782,3565,0.27475595474243164,0.28491665391301724
893,1787,1786,3573,0.2751009464263916,0.283270576969813
895,1791,1790,3581,0.27538013458251953,0.2816342230873632
897,1795,1794,3589,0.27579283714294434,0.2800075142293881
899,1799,1798,3597,0.276080846786499,0.278390374336408
901,1803,1802,3605,0.2763631343841553,0.2767827292197999
903,1807,1806,3613,0.2766530513763428,0.2751845064648523
905,1811,1810,3621,0.27707600593566895,0.2735956353363521
907,1815,1814,3629,0.27750396728515625,0.27201604669185375
909,1819,1818,3637,0.2783019542694092,0.27044567289753263
911,1823,1822,3645,0.27879881858825684,0.2688844477521294
913,1827,1826,3653,0.2790868282318115,0.2673323064102096
915,1831,1830,3661,0.27942705154418945,0.2657891853165776
917,1835,1834,3669,0.2797820568084717,0.26425502213820357
919,1839,1838,3677,0.28011393547058105,0.2627297557042913
921,1843,1842,3685,0.28040289878845215,0.26121332594696356
923,1847,1846,3693,0.2808060646057129,0.25970567384872095
925,1851,1850,3701,0.28110218048095703,0.25820674138823535
927,1855,1854,3709,0.28145599365234375,0.2567164714947125
929,1859,1858,3717,0.28182291984558105,0.2552348079994717
931,1863,1862,3725,0.2821378707885742,0.25376169559588346
933,1867,1866,3733,0.28249406814575195,0.25229707979575916
935,1871,1870,3741,0.28286004066467285,0.2508409068942327
937,1875,1874,3749,0.2831850051879883,0.24939312393197405
939,1879,1878,3757,0.283627986907959,0.24795367866212886
941,1883,1882,3765,0.28423309326171875,0.24652251951728454
943,1887,1886,3773,0.2850508689880371,0.24509959558233635
945,1891,1890,3781,0.28560400009155273,0.24368485656261468
947,1895,1894,3789,0.28613710403442383,0.24227825276018136
949,1899,1898,3797,0.28647518157958984,0.2408797350479571
951,1903,1902,3805,0.2868940830230713,0.23948925484577652
953,1907,1906,3813,0.287229061126709,0.23810676409837825
955,1911,1910,3821,0.2875959873199463,0.236732215254979
957,1915,1914,3829,0.2881741523742676,0.23536556125015465
959,1919,1918,3837,0.2885429859161377,0.23400675548321362
961,1923,1922,3845,0.28890299797058105,0.23265575180395862
963,1927,1926,3853,0.28931212425231934,0.23131250449387575
965,1931,1930,3861,0.2896420955657959,0.22997696825154718
967,1935,1934,3869,0.29003024101257324,0.22864909817815962
969,1939,1938,3877,0.2903571128845215,0.22732884976535578
971,1943,1942,3885,0.29086804389953613,0.226016178879455
973,1947,1946,3893,0.29232096672058105,0.22471104175127232
975,1951,1950,3901,0.2928588390350342,0.2234133949656081
977,1955,1954,3909,0.29320812225341797,0.2221231954486789
979,1959,1958,3917,0.29364895820617676,0.2208404004591429
981,1963,1962,3925,0.2940511703491211,0.21956496757842248
983,1967,1966,3933,0.2943460941314697,0.21829685470156296
985,1971,1970,3941,0.29473304748535156,0.21703602002992062
987,1975,1974,3949,0.29506492614746094,0.2157824220613281
989,1979,1978,3957,0.29537487030029297,0.21453601958516336
991,1983,1982,3965,0.29579710960388184,0.21329677167323305
993,1987,1986,3973,0.2962069511413574,0.21206463767427286
995,1991,1990,3981,0.29685211181640625,0.210839577207624
997,1995,1994,3989,0.29717206954956055,0.20962155015696896
999,1999,1998,3997,0.29756903648376465,0.20841051666520555
1001,2003,2002,4005,0.29883813858032227,0.2072064371305031
1003,2007,2006,4013,0.29918909072875977,0.20600927219805187
1005,2011,2010,4021,0.29966115951538086,0.20481898275953545
1007,2015,2014,4029,0.30023813247680664,0.20363552994507003
1009,2019,2018,4037,0.30058813095092773,0.20245887512290592
1011,2023,2022,4045,0.30104494094848633,0.20128897989180133
1013,2027,2026,4053,0.3015260696411133,0.2001258060801959
1015,2031,2030,4061,0.30187296867370605,0.1989693157410637
1017,2035,2034,4069,0.30259108543395996,0.19781947114968026
1019,2039,2038,4077,0.30347704887390137,0.19667623480027116
1021,2043,2042,4085,0.30391407012939453,0.19553956940288594
1023,2047,2046,4093,0.3043079376220703,0.19440943788016746
1025,2051,2050,4101,0.3048369884490967,0.19328580336643822
1027,2055,2054,4109,0.3053300380706787,0.192168629203726
1029,2059,2058,4117,0.3077099323272705,0.19105787893934414
1031,2063,2062,4125,0.3084428310394287,0.18995351632475455
1033,2067,2066,4133,0.30883097648620605,0.18885550531233453
1035,2071,2070,4141,0.30928587913513184,0.18776381005453432
1037,2075,2074,4149,0.3097660541534424,0.18667839490102564
1039,2079,2078,4157,0.31009793281555176,0.18559922439632118
1041,2083,2082,4165,0.3105459213256836,0.18452626328044644
1043,2087,2086,4173,0.3109598159790039,0.18345947648487315
1045,2091,2090,4181,0.31132006645202637,0.18239882913155603
1047,2095,2094,4189,0.3118479251861572,0.18134428653260598
1049,2099,2098,4197,0.31255197525024414,0.1802958141865738
1051,2103,2102,4205,0.312974214553833,0.1792533777797251
1053,2107,2106,4213,0.31362199783325195,0.17821694318224007
1055,2111,2110,4221,0.3147909641265869,0.17718647644824287
1057,2115,2114,4229,0.31516003608703613,0.1761619438156307
1059,2119,2118,4237,0.31557297706604004,0.17514331170164965
1061,2123,2122,4245,0.31589603424072266,0.17413054670521633
1063,2127,2126,4253,0.316237211227417,0.17312361560335313
1065,2131,2130,4261,0.31657981872558594,0.17212248535204286
1067,2135,2134,4269,0.31693124771118164,0.17112712308316097
1069,2139,2138,4277,0.3172738552093506,0.17013749610517512
1071,2143,2142,4285,0.3176290988922119,0.169153571901508
1073,2147,2146,4293,0.3179929256439209,0.16817531812917286
1075,2151,2150,4301,0.3185911178588867,0.16720270261814404
1077,2155,2154,4309,0.3189680576324463,0.16623569337192265
1079,2159,2158,4317,0.3192861080169678,0.16527425856340308
1081,2163,2162,4325,0.31966280937194824,0.16431836653679366
1083,2167,2166,4333,0.32186293601989746,0.16336798580581846
1085,2171,2170,4341,0.3223130702972412,0.16242308505300404
1087,2175,2174,4349,0.32265806198120117,0.16148363312874686
1089,2179,2178,4357,0.3231821060180664,0.16054959904970817
1091,2183,2182,4365,0.3237619400024414,0.15962095200027188
1093,2187,2186,4373,0.32410597801208496,0.15869766132905516
1095,2191,2190,4381,0.3245048522949219,0.1577796965505485
1097,2195,2194,4389,0.3249499797821045,0.1568670273421225
1099,2199,2198,4397,0.32536911964416504,0.1559596235451076
1101,2203,2202,4405,0.3257730007171631,0.15505745516324587
1103,2207,2206,4413,0.3260691165924072,0.15416049236149987
1105,2211,2210,4421,0.32642602920532227,0.15326870546641563
1107,2215,2214,4429,0.3268868923187256,0.152382064964841
1109,2219,2218,4437,0.3272368907928467,0.15150054150285036
1111,2223,2222,4445,0.32764697074890137,0.15062410588561792
1113,2227,2226,4453,0.3280160427093506,0.14975272907661086
1115,2231,2230,4461,0.32833218574523926,0.14888638219640254
1117,2235,2234,4469,0.32871103286743164,0.14802503652277227
1119,2239,2238,4477,0.3293440341949463,0.14716866348897997
1121,2243,2242,4485,0.3297159671783447,0.14631723468435098
1123,2247,2246,4493,0.33044886589050293,0.14547072185196436
1125,2251,2250,4501,0.33083391189575195,0.14462909689021558
1127,2255,2254,4509,0.33115100860595703,0.14379233184980145
1129,2259,2258,4517,0.33144307136535645,0.14296039893405058
1131,2263,2262,4525,0.33177995681762695,0.1421332704992242
1133,2267,2266,4533,0.3320939540863037,0.14131091905172227
1135,2271,2270,4541,0.3323640823364258,0.14049331724917102
1137,2275,2274,4549,0.33266520500183105,0.13968043789926698
1139,2279,2278,4557,0.3330860137939453,0.13887225395803132
1141,2283,2282,4565,0.33343005180358887,0.13806873853161647
1143,2287,2286,4573,0.3338499069213867,0.13726986487223775
1145,2291,2290,4581,0.3342888355255127,0.13647560638128278
1147,2295,2294,4589,0.33515501022338867,0.13568593660525985
1149,2299,2298,4597,0.3355278968811035,0.13490082923701482
1151,2303,2302,4605,0.33605003356933594,0.13412025811529324
1153,2307,2306,4613,0.33941006660461426,0.13334419722181456
1155,2311,2310,4621,0.3398759365081787,0.13257262068396877
1157,2315,2314,4629,0.34040403366088867,0.13180550277187558
1159,2319,2318,4637,0.3408091068267822,0.1310428178974365
1161,2323,2322,4645,0.3411600589752197,0.1302845406153865
1163,2327,2326,4653,0.3415801525115967,0.12953064562104
1165,2331,2330,4661,0.3420240879058838,0.12878110775117962
1167,2335,2334,4669,0.3424389362335205,0.12803590198167103
1169,2339,2338,4677,0.34287381172180176,0.12729500342756062
1171,2343,2342,4685,0.3432741165161133,0.12655838734348454
1173,2347,2346,4693,0.3437530994415283,0.12582602912157204
1175,2351,2350,4701,0.34427714347839355,0.12509790429064002
1177,2355,2354,4709,0.3446929454803467,0.12437398851684903
1179,2359,2358,4717,0.345073938369751,0.12365425760175791
1181,2363,2362,4725,0.3454930782318115,0.12293868748325054
1183,2367,2366,4733,0.3462200164794922,0.12222725423262108
1185,2371,2370,4741,0.3476870059967041,0.12151993405593248
1187,2375,2374,4749,0.3480699062347412,0.12081670329247982
1189,2379,2378,4757,0.3484780788421631,0.12011753841435283
1191,2383,2382,4765,0.34893107414245605,0.1194224160254811
1193,2387,2386,4773,0.34929323196411133,0.11873131286065428
1195,2391,2390,4781,0.34963512420654297,0.1180442057868564
1197,2395,2394,4789,0.3500349521636963,0.1173610717997915
1199,2399,2398,4797,0.3503570556640625,0.11668188802554587
1201,2403,2402,4805,0.350783109664917,0.11600663171853123
1203,2407,2406,4813,0.35119104385375977,0.11533528026096407
1205,2411,2410,4821,0.35179710388183594,0.11466781116336343
1207,2415,2414,4829,0.35222411155700684,0.11400420206297161
1209,2419,2418,4837,0.35263705253601074,0.11334443072284187
1211,2423,2422,4845,0.35515713691711426,0.11268847503127606
1213,2427,2426,4853,0.35570788383483887,0.11203631300334642
1215,2431,2430,4861,0.3562331199645996,0.11138792277563259
1217,2435,2434,4869,0.35671401023864746,0.11074328261124088
1219,2439,2438,4877,0.35709500312805176,0.11010237089438656
1221,2443,2442,4885,0.3576059341430664,0.10946516613251696
1223,2447,2446,4893,0.35811519622802734,0.10883164695448108
1225,2451,2450,4901,0.35862088203430176,0.10820179211049885
1227,2455,2454,4909,0.35905909538269043,0.10757558047129247
1229,2459,2458,4917,0.3595468997955322,0.10695299102722423
1231,2463,2462,4925,0.3603529930114746,0.10633400288886548
1233,2467,2466,4933,0.36084794998168945,0.10571859528330428
1235,2471,2470,4941,0.36123013496398926,0.10510674755844646
1237,2475,2474,4949,0.36174607276916504,0.10449843917789986
1239,2479,2478,4957,0.36223602294921875,0.1038936497222941
1241,2483,2482,4965,0.3639349937438965,0.10329235888773945
1243,2487,2486,4973,0.364285945892334,0.10269454648784815
1245,2491,2490,4981,0.3646731376647949,0.10210019244911492
1247,2495,2494,4989,0.3650660514831543,0.10150927681376617
1249,2499,2498,4997,0.3653581142425537,0.10092177973722477
1251,2503,2502,5005,0.3656651973724365,0.10033768148744551
1253,2507,2506,5013,0.36595702171325684,0.09975696244616604
1255,2511,2510,5021,0.3663160800933838,0.09917960310615484
1257,2515,2514,5029,0.3667750358581543,0.0986055840715988
1259,2519,2518,5037,0.36708688735961914,0.0980348860579293
1261,2523,2522,5045,0.36742401123046875,0.09746748989012173
1263,2527,2526,5053,0.36782288551330566,0.09690337650244495
1265,2531,2530,5061,0.3681149482727051,0.0963425269391685
1267,2535,2534,5069,0.3684208393096924,0.0957849223518735
1269,2539,2538,5077,0.3687717914581299,0.09523054400033609
1271,2543,2542,5085,0.36944103240966797,0.09467937325112455
1273,2547,2546,5093,0.36997103691101074,0.09413139157839251
1275,2551,2550,5101,0.37035608291625977,0.09358658056155256
1277,2555,2554,5109,0.37071800231933594,0.0930449218850925
1279,2559,2558,5117,0.37119007110595703,0.09250639733903072
1281,2563,2562,5125,0.3715982437133789,0.09197098881799173
1283,2567,2566,5133,0.372006893157959,0.09143867831908412
1285,2571,2570,5141,0.37236499786376953,0.09090944794400567
1287,2575,2574,5149,0.3727607727050781,0.09038327989557608
1289,2579,2578,5157,0.37310004234313965,0.08986015648033822
1291,2583,2582,5165,0.37344908714294434,0.08934006010458785
1293,2587,2586,5173,0.37378478050231934,0.08882297327630624
1295,2591,2590,5181,0.37430500984191895,0.08830887860459023
1297,2595,2594,5189,0.3747270107269287,0.08779775879633653
1299,2599,2598,5197,0.3750569820404053,0.08728959666000823
1301,2603,2602,5205,0.37540197372436523,0.08678437510088664
1303,2607,2606,5213,0.37576985359191895,0.08628207712403117
1305,2611,2610,5221,0.37648892402648926,0.08578268583032754
1307,2615,2614,5229,0.37735414505004883,0.08528618441899323
1309,2619,2618,5237,0.3778839111328125,0.08479255618550097
1311,2623,2622,5245,0.37833404541015625,0.08430178452122435
1313,2627,2626,5253,0.3786790370941162,0.08381385291268142
1315,2631,2630,5261,0.3791959285736084,0.08332874494178778
1317,2635,2634,5269,0.37969112396240234,0.08284644428508274
1319,2639,2638,5277,0.3801591396331787,0.08236693471208818
1321,2643,2642,5285,0.3810131549835205,0.08189020008587228
1323,2647,2646,5293,0.3824341297149658,0.08141622436322762
1325,2651,2650,5301,0.3833470344543457,0.08094499159192053
1327,2655,2654,5309,0.38379502296447754,0.08047648591275991
1329,2659,2658,5317,0.38434696197509766,0.08001069155698881
1331,2663,2662,5325,0.3847789764404297,0.07954759284648201
1333,2667,2666,5333,0.3857741355895996,0.07908717419441844
1335,2671,2670,5341,0.3875248432159424,0.07862942010228534
1337,2675,2674,5349,0.38814282417297363,0.07817431516240578
1339,2679,2678,5357,0.3886301517486572,0.07772184405405337
1341,2683,2682,5365,0.38913488388061523,0.07727199154597991
1343,2687,2686,5373,0.38951611518859863,0.07682474249451232
1345,2691,2690,5381,0.38996005058288574,0.07638008184248717
1347,2695,2694,5389,0.3905320167541504,0.07593799462113024
1349,2699,2698,5397,0.39121007919311523,0.07549846594543538
1351,2703,2702,5405,0.39229607582092285,0.07506148101842487
1353,2707,2706,5413,0.3928380012512207,0.07462702512723628
1355,2711,2710,5421,0.39505791664123535,0.07419508364395708
1357,2715,2714,5429,0.39543890953063965,0.07376564202559302
1359,2719,2718,5437,0.39591407775878906,0.07333868581209743
1361,2723,2722,5445,0.3964049816131592,0.07291420062778305
1363,2727,2726,5453,0.39679908752441406,0.07249217217846272
1365,2731,2730,5461,0.39733099937438965,0.0720725862540304
1367,2735,2734,5469,0.3979761600494385,0.07165542872501013
1369,2739,2738,5477,0.3984670639038086,0.07124068554468159
1371,2743,2742,5485,0.3991730213165283,0.0708283427454418
1373,2747,2746,5493,0.39973902702331543,0.07041838644246795
1375,2751,2750,5501,0.40022778511047363,0.07001080282933801
1377,2755,2754,5509,0.40082406997680664,0.06960557818061765
1379,2759,2758,5517,0.4012291431427002,0.06920269884898034
1381,2763,2762,5525,0.40161991119384766,0.06880215126609682
1383,2767,2766,5533,0.4020400047302246,0.06840392194292835
1385,2771,2770,5541,0.40296101570129395,0.0680079974668031
1387,2775,2774,5549,0.4070260524749756,0.06761436450364208
1389,2779,2778,5557,0.40774106979370117,0.06722300979536261
1391,2783,2782,5565,0.4083709716796875,0.06683392016129094
1393,2787,2786,5573,0.4089200496673584,0.06644708249608859
1395,2791,2790,5581,0.4093310832977295,0.06606248377109873
1397,2795,2794,5589,0.40979695320129395,0.06568011103150727
1399,2799,2798,5597,0.4104771614074707,0.06529995139864096
1401,2803,2802,5605,0.41092419624328613,0.06492199206770745
1403,2807,2806,5613,0.41156888008117676,0.06454622030745694
1405,2811,2810,5621,0.41196703910827637,0.06417262346057899
1407,2815,2814,5629,0.4123690128326416,0.06380118894255843
1409,2819,2818,5637,0.4127938747406006,0.0634319042422694
1411,2823,2822,5645,0.41484498977661133,0.06306475692024537
1413,2827,2826,5653,0.4157130718231201,0.0626997346082699
1415,2831,2830,5661,0.41608309745788574,0.06233682501145439
1417,2835,2834,5669,0.4164140224456787,0.061976015904011666
1419,2839,2838,5677,0.416748046875,0.06161729513174757
1421,2843,2842,5685,0.4173450469970703,0.06126065061096072
1423,2847,2846,5693,0.4178040027618408,0.060906070326798754
1425,2851,2850,5701,0.4183471202850342,0.06055354233480747
1427,2855,2854,5709,0.4186840057373047,0.060203054758545246
1429,2859,2858,5717,0.4189920425415039,0.059854595790993684
1431,2863,2862,5725,0.41931915283203125,0.059508153693730914
1433,2867,2866,5733,0.4198009967803955,0.05916371679477375
1435,2871,2870,5741,0.4202849864959717,0.05882127349078263
1437,2875,2874,5749,0.42070603370666504,0.05848081224539339
1439,2879,2878,5757,0.42125391960144043,0.05814232158834848
1441,2883,2882,5765,0.4217848777770996,0.05780579011577348
1443,2887,2886,5773,0.42219018936157227,0.05747120649060815
1445,2891,2890,5781,0.42281198501586914,0.057138559439867634
1447,2895,2894,5789,0.42316603660583496,0.05680783775668174
1449,2899,2898,5797,0.42349910736083984,0.056479030299518146
1451,2903,2902,5805,0.4242110252380371,0.05615212598964411
1453,2907,2906,5813,0.4246399402618408,0.055827113813764324
1455,2911,2910,5821,0.4250361919403076,0.05550398282175064
1457,2915,2914,5829,0.4255349636077881,0.055182722126550746
1459,2919,2918,5837,0.42587900161743164,0.054863320904816645
1461,2923,2922,5845,0.42620086669921875,0.05454576839449595
1463,2927,2926,5853,0.4265620708465576,0.054230053897207725
1465,2931,2930,5861,0.42691898345947266,0.05391616677565851
1467,2935,2934,5869,0.427325963973999,0.05360409645416237
1469,2939,2938,5877,0.42776989936828613,0.053293832417923036
1471,2943,2942,5885,0.4282829761505127,0.05298536421337362
1473,2947,2946,5893,0.42872095108032227,0.05267868144772399
1475,2951,2950,5901,0.4290938377380371,0.052373773786827345
1477,2955,2954,5909,0.429426908493042,0.052070630958486075
1479,2959,2958,5917,0.4299349784851074,0.051769242748079355
1481,2963,2962,5925,0.4307420253753662,0.051469599000557587
1483,2967,2966,5933,0.4310920238494873,0.05117168962031887
1485,2971,2970,5941,0.4314389228820801,0.0508755045692796
1487,2975,2974,5949,0.4320390224456787,0.050581033867550626
1489,2979,2978,5957,0.43250584602355957,0.05028826759310672
1491,2983,2982,5965,0.432811975479126,0.04999719588197883
1493,2987,2986,5973,0.43343496322631836,0.04970780892604105
1495,2991,2990,5981,0.4337649345397949,0.04942009697490287
1497,2995,2994,5989,0.43409204483032227,0.049134050333649114
1499,2999,2998,5997,0.4344210624694824,0.0488496593643428
1502,3005,3004,6009,0.434967041015625,0.04842615634812345
1504,3009,3008,6017,0.4352760314941406,0.04814586275555157
1506,3013,3012,6025,0.4356701374053955,0.04786719153792814
1508,3017,3016,6033,0.436053991317749,0.047590133304834234
1510,3021,3020,6041,0.43648695945739746,0.047314678721154114
1512,3025,3024,6049,0.4369070529937744,0.047040818504639814
1514,3029,3028,6057,0.43740296363830566,0.04676854342757756
1516,3033,3032,6065,0.438230037689209,0.04649784431540898
1518,3037,3036,6073,0.43859195709228516,0.04622871204706478
1520,3041,3040,6081,0.43891215324401855,0.045961137553644206
1522,3045,3044,6089,0.4395751953125,0.04569511181871307
1524,3049,3048,6097,0.43993091583251953,0.045430625878718135
1526,3053,3052,6105,0.44043803215026855,0.04516767082055246
1528,3057,3056,6113,0.4409160614013672,0.04490623778445991
1530,3061,3060,6121,0.44129300117492676,0.04464631796093654
1532,3065,3064,6129,0.4416179656982422,0.0443879025912342
1534,3069,3068,6137,0.4420318603515625,0.04413098296798166
1536,3073,3072,6145,0.44240808486938477,0.04387555043347391
1538,3077,3076,6153,0.4427919387817383,0.04362159638117561
1540,3081,3080,6161,0.4431419372558594,0.04336911225318421
1542,3085,3084,6169,0.44357800483703613,0.04311808954132091
1544,3089,3088,6177,0.4439089298248291,0.04286851978723343
1546,3093,3092,6185,0.44419312477111816,0.04262039458138637
1548,3097,3096,6193,0.44455814361572266,0.04237370556234907
1550,3101,3100,6201,0.44488096237182617,0.042128444417599234
1552,3105,3104,6209,0.44531702995300293,0.04188460288230641
1554,3109,3108,6217,0.4456489086151123,0.041642172740123544
1556,3113,3112,6225,0.44601988792419434,0.0414011458214659
1558,3117,3116,6233,0.4467611312866211,0.04116151400480712
1560,3121,3120,6241,0.44714903831481934,0.04092326921447629
1562,3125,3124,6249,0.4475421905517578,0.04068640342327444
1564,3129,3128,6257,0.447890043258667,0.04045090864818179
1566,3133,3132,6265,0.4482738971710205,0.04021677695468506
1568,3137,3136,6273,0.44858598709106445,0.03998400045275991
1570,3141,3140,6281,0.4488980770111084,0.03975257129804201
1572,3145,3144,6289,0.44922399520874023,0.03952248169280242
1574,3149,3148,6297,0.4495508670806885,0.03929372388282557
1576,3153,3152,6305,0.44991326332092285,0.03906629015962443
1578,3157,3156,6313,0.4502449035644531,0.038840172859327164
1580,3161,3160,6321,0.4505600929260254,0.03861536436260856
1582,3165,3164,6329,0.45089006423950195,0.03839185709332355
1584,3169,3168,6337,0.45117807388305664,0.03816964352007991
1586,3173,3172,6345,0.45160508155822754,0.03794871615506781
1588,3177,3176,6353,0.4519460201263428,0.037729067553106566
1590,3181,3180,6361,0.4522559642791748,0.03751069031268962
1592,3185,3184,6369,0.4527151584625244,0.03729357707425086
1594,3189,3188,6377,0.4545018672943115,0.03707772052277053
1596,3193,3192,6385,0.45494794845581055,0.036863113383700054
1598,3197,3196,6393,0.45537590980529785,0.03664974842501734
1600,3201,3200,6401,0.45581603050231934,0.036437618457398256
1602,3205,3204,6409,0.4561269283294678,0.03622671633177147
1604,3209,3208,6417,0.4564940929412842,0.03601703494143174
1606,3213,3212,6425,0.4569549560546875,0.03580856722051206
1608,3217,3216,6433,0.45731306076049805,0.03560130614414468
1610,3221,3220,6441,0.45764684677124023,0.03539524472777244
1612,3225,3224,6449,0.45804286003112793,0.035190376027688396
1614,3229,3228,6457,0.4584920406341553,0.03498669314065735
1616,3233,3232,6465,0.45885705947875977,0.03478418920211227
1618,3237,3236,6473,0.4592020511627197,0.03458285738861258
1620,3241,3240,6481,0.45995402336120605,0.03438269091531742
1622,3245,3244,6489,0.4603121280670166,0.03418368303703128
1624,3249,3248,6497,0.46073102951049805,0.03398582704788138
1626,3253,3252,6505,0.4611079692840576,0.03378911628036608
1628,3257,3256,6513,0.46163201332092285,0.03359354410541188
1630,3261,3260,6521,0.4624168872833252,0.033399103932614145
1632,3265,3264,6529,0.4629518985748291,0.033205789209766724
1634,3269,3268,6537,0.4633190631866455,0.033013593422724294
1636,3273,3272,6545,0.4638090133666992,0.03282251009434652
1638,3277,3276,6553,0.4641869068145752,0.03263253278598907
1640,3281,3280,6561,0.464536190032959,0.032443655095290944
1642,3285,3284,6569,0.4649968147277832,0.03225587065782325
1644,3289,3288,6577,0.4653499126434326,0.03206917314530284
1646,3293,3292,6585,0.4656970500946045,0.03188355626641617
1648,3297,3296,6593,0.466001033782959,0.03169901376574045
1650,3301,3300,6601,0.46630406379699707,0.031515539425431754
1652,3305,3304,6609,0.4666318893432617,0.031333127061678866
1654,3309,3308,6617,0.4669661521911621,0.03115177052846618
1656,3313,3312,6625,0.46739697456359863,0.03097146371391286
1658,3317,3316,6633,0.4677901268005371,0.030792200541743975
1660,3321,3320,6641,0.46906089782714844,0.03061397497158509
1662,3325,3324,6649,0.46950793266296387,0.03043678099693437
1664,3329,3328,6657,0.47024106979370117,0.030260612647009185
1666,3333,3332,6665,0.47066593170166016,0.030085463985814725
1668,3337,3336,6673,0.4710547924041748,0.029911329109725132
1670,3341,3340,6681,0.47153496742248535,0.029738202152301725
1672,3345,3344,6689,0.4721710681915283,0.02956607727811981
1674,3349,3348,6697,0.47251105308532715,0.029394948687219792
1676,3353,3352,6705,0.4730062484741211,0.02922481061311198
1678,3357,3356,6713,0.47351598739624023,0.02905565732254712
1680,3361,3360,6721,0.4739370346069336,0.028887483114963003
1682,3365,3364,6729,0.47460412979125977,0.028720282323429207
1684,3369,3368,6737,0.4749939441680908,0.028554049313197924
1686,3373,3372,6745,0.4754040241241455,0.028388778483254707
1688,3377,3376,6753,0.4758448600769043,0.02822446426297787
1690,3381,3380,6761,0.4766349792480469,0.028061101116708002
1692,3385,3384,6769,0.47744202613830566,0.027898683537949425
1694,3389,3388,6777,0.47774386405944824,0.027737206054653112
1696,3393,3392,6785,0.4780712127685547,0.027576663224964798
1698,3397,3396,6793,0.47838497161865234,0.02741704963834547
1700,3401,3400,6801,0.47873497009277344,0.02725835991691794
1702,3405,3404,6809,0.47903895378112793,0.027100588712168687
1704,3409,3408,6817,0.4794430732727051,0.026943730708396615
1706,3413,3412,6825,0.4797670841217041,0.02678778061937461
1708,3417,3416,6833,0.48009300231933594,0.0266327331896507
1710,3421,3420,6841,0.4804549217224121,0.026478583194277837
1712,3425,3424,6849,0.4807710647583008,0.02632532543919655
1714,3429,3428,6857,0.48110389709472656,0.026172954759524157
1716,3433,3432,6865,0.481781005859375,0.02602146602081521
1718,3437,3436,6873,0.48213696479797363,0.025870854118237665
1720,3441,3440,6881,0.48248982429504395,0.02572111397608007
1722,3445,3444,6889,0.48286008834838867,0.02557224054850518
1724,3449,3448,6897,0.48398280143737793,0.02542422881864532
1726,3453,3452,6905,0.4843001365661621,0.025277073799086378
1728,3457,3456,6913,0.4846630096435547,0.025130770530521367
1730,3461,3460,6921,0.4851348400115967,0.024985314083256594
1732,3465,3464,6929,0.48557019233703613,0.024840699555052886
1734,3469,3468,6937,0.4859600067138672,0.024696922073477536
1736,3473,3472,6945,0.4863901138305664,0.02455397679288855
1738,3477,3476,6953,0.4867551326751709,0.02441185889626872
1740,3481,3480,6961,0.4871549606323242,0.02427056359460391
1742,3485,3484,6969,0.48755502700805664,0.02413008612687749
1744,3489,3488,6977,0.48797178268432617,0.023990421758583347
1746,3493,3492,6985,0.4886128902435303,0.023851565784002434
1748,3497,3496,6993,0.48899102210998535,0.02371351352313938
1750,3501,3500,7001,0.4893620014190674,0.023576260324435595
1752,3505,3504,7009,0.48979997634887695,0.023439801562596643
1754,3509,3508,7017,0.49021124839782715,0.023304132639300458
1756,3513,3512,7025,0.4907231330871582,0.023169248982723864
1758,3517,3516,7033,0.4922010898590088,0.023035146047022406
1760,3521,3520,7041,0.49269795417785645,0.022901819313583958
1762,3525,3524,7049,0.493074893951416,0.02276926429003511
1764,3529,3528,7057,0.49350500106811523,0.022637476508955815
1766,3533,3532,7065,0.4938671588897705,0.022506451529368865
1768,3537,3536,7073,0.49428892135620117,0.022376184936065142
1770,3541,3540,7081,0.49464988708496094,0.0222466723393408
1772,3545,3544,7089,0.49497294425964355,0.022117909374760793
1774,3549,3548,7097,0.4952688217163086,0.02198989170317996
1776,3553,3552,7105,0.49559879302978516,0.02186261501104412
1778,3557,3556,7113,0.4958930015563965,0.021736075009088984
1780,3561,3560,7121,0.49617910385131836,0.0216102674328408
1782,3565,3564,7129,0.49659085273742676,0.021485188043797714
1784,3569,3568,7137,0.4968750476837158,0.021360832626173925
1786,3573,3572,7145,0.49718785285949707,0.0212371969894221
1788,3577,3576,7153,0.4978492259979248,0.02111427696770715
1790,3581,3580,7161,0.4982438087463379,0.020992068418710222
1792,3585,3584,7169,0.49854016304016113,0.0208705672244321
1794,3589,3588,7177,0.49884796142578125,0.020749769290130414
1796,3593,3592,7185,0.49930286407470703,0.02062967054528968
1798,3597,3596,7193,0.49968910217285156,0.020510266942855022
1800,3601,3600,7201,0.49998998641967773,0.020391554459483454
1802,3605,3604,7209,0.5004820823669434,0.020273529094466565
1804,3609,3608,7217,0.5008959770202637,0.020156186870452474
1806,3613,3612,7225,0.5012218952178955,0.02003952383366418
1808,3617,3616,7233,0.5015602111816406,0.01992353605233685
1810,3621,3620,7241,0.5019810199737549,0.019808219618754685
1812,3625,3624,7249,0.5023150444030762,0.019693570645983996
1814,3629,3628,7257,0.5027370452880859,0.019579585271081223
1816,3633,3632,7265,0.503727912902832,0.019466259652932784
1818,3637,3636,7273,0.504356861114502,0.01935358997280368
1820,3641,3640,7281,0.5049550533294678,0.019241572433919166
1822,3645,3644,7289,0.5063638687133789,0.01913020326134575
1824,3649,3648,7297,0.5076239109039307,0.019019478702353973
1826,3653,3652,7305,0.5082900524139404,0.01890939502565997
1828,3657,3656,7313,0.5086860656738281,0.018799948521957856
1830,3661,3660,7321,0.5091469287872314,0.018691135503046023
1832,3665,3664,7329,0.5096211433410645,0.01858295230153458
1834,3669,3668,7337,0.5099380016326904,0.018475395272930406
1836,3673,3672,7345,0.5102968215942383,0.018368460792181285
1838,3677,3676,7353,0.5107159614562988,0.018262145255817572
1840,3681,3680,7361,0.5110621452331543,0.01815644508157272
1842,3685,3684,7369,0.511430025100708,0.018051356707192472
1844,3689,3688,7377,0.5118989944458008,0.01794687659194823
1846,3693,3692,7385,0.5122640132904053,0.0178430012147307
1848,3697,3696,7393,0.512969970703125,0.017739727074767665
1850,3701,3700,7401,0.513530969619751,0.017637050693046094
1852,3705,3704,7409,0.5138278007507324,0.017534968608734814
1854,3709,3708,7417,0.5142059326171875,0.017433477382258592
1856,3713,3712,7425,0.5147490501403809,0.017332573593405155
1858,3717,3716,7433,0.5151481628417969,0.017232253841932724
1860,3721,3720,7441,0.5155239105224609,0.01713251474755865
1862,3725,3724,7449,0.516024112701416,0.017033352949452123
1864,3729,3728,7457,0.5164120197296143,0.01693476510525302
1866,3733,3732,7465,0.5167779922485352,0.016836747893993743
1868,3737,3736,7473,0.5171310901641846,0.01673929801152137
1870,3741,3740,7481,0.5174589157104492,0.016642412174845682
1872,3745,3744,7489,0.5178382396697998,0.016546087119228756
1874,3749,3748,7497,0.5182070732116699,0.01645031959778739
1876,3753,3752,7505,0.5185389518737793,0.01635510638442757
1878,3757,3756,7513,0.5189390182495117,0.01626044427032508
1880,3761,3760,7521,0.519362211227417,0.01616633006529007
1882,3765,3764,7529,0.5199408531188965,0.01607276059873741
1884,3769,3768,7537,0.5203139781951904,0.015979732716584115
1886,3773,3772,7545,0.5206730365753174,0.015887243284449376
1888,3777,3776,7553,0.5210671424865723,0.01579528918598623
1890,3781,3780,7561,0.5217499732971191,0.01570386732214945
1892,3785,3784,7569,0.5223381519317627,0.015612974612391655
1894,3789,3788,7577,0.522935152053833,0.015522607993926671
1896,3793,3792,7585,0.5232930183410645,0.01543276442162451
1898,3797,3796,7593,0.5236349105834961,0.015343440868186828
1900,3801,3800,7601,0.5239920616149902,0.015254634323075042
1902,3805,3804,7609,0.5244560241699219,0.015166341794194137
1904,3809,3808,7617,0.5248169898986816,0.015078560305979143
1906,3813,3812,7625,0.5251321792602539,0.014991286900899044
1908,3817,3816,7633,0.5255041122436523,0.014904518637914175
1910,3821,3820,7641,0.5257940292358398,0.014818252592678731
1912,3825,3824,7649,0.5261421203613281,0.014732485858787545
1914,3829,3828,7657,0.5265090465545654,0.01464721554619025
1916,3833,3832,7665,0.5268759727478027,0.014562438781191274
1918,3837,3836,7673,0.5274450778961182,0.014478152706991352
1920,3841,3840,7681,0.5279140472412109,0.014394354483637446
1922,3845,3844,7689,0.5282120704650879,0.014311041287340264
1924,3849,3848,7697,0.5285651683807373,0.014228210310555767
1926,3853,3852,7705,0.5290069580078125,0.014145858762044992
1928,3857,3856,7713,0.5295271873474121,0.014063983867355755
1930,3861,3860,7721,0.5298471450805664,0.013982582866454632
1932,3865,3864,7729,0.5301520824432373,0.013901653017357655
1934,3869,3868,7737,0.5305039882659912,0.013821191592363172
1936,3873,3872,7745,0.5308430194854736,0.013741195880397065
1938,3877,3876,7753,0.531135082244873,0.013661663185317972
1940,3881,3880,7761,0.5315232276916504,0.01358259082801722
1942,3885,3884,7769,0.5318658351898193,0.013503976143536083
1944,3889,3888,7777,0.5321869850158691,0.013425816482631392
1946,3893,3892,7785,0.5325498580932617,0.013348109211756798
1948,3897,3896,7793,0.5328869819641113,0.013270851712119305
1950,3901,3900,7801,0.533257007598877,0.01319404138078172
1952,3905,3904,7809,0.5336101055145264,0.013117675629214303
1954,3909,3908,7817,0.5339651107788086,0.013041751884049857
1956,3913,3912,7825,0.5343930721282959,0.012966267586962356
1958,3917,3916,7833,0.5347089767456055,0.012891220194520806
1960,3921,3920,7841,0.5350751876831055,0.01281660717748162
1962,3925,3924,7849,0.535646915435791,0.012742426021643948
1964,3929,3928,7857,0.5359230041503906,0.012668674227700327
1966,3933,3932,7865,0.5362539291381836,0.012595349310356645
1968,3937,3936,7873,0.5367507934570312,0.012522448798371503
1970,3941,3940,7881,0.5373151302337646,0.012449970235626627
1972,3945,3944,7889,0.5377700328826904,0.012377911179409779
1974,3949,3948,7897,0.5381360054016113,0.012306269202318795
1976,3953,3952,7905,0.5387270450592041,0.012235041889176979
1978,3957,3956,7913,0.5391139984130859,0.012164226840963547
1980,3961,3960,7921,0.5396161079406738,0.012093821670162267
1982,3965,3964,7929,0.5399508476257324,0.012023824005736181
1984,3969,3968,7937,0.5403831005096436,0.011954231487735938
1986,3973,3972,7945,0.5408949851989746,0.011885041771729388
1988,3977,3976,7953,0.541262149810791,0.011816252526171082
1990,3981,3980,7961,0.5419621467590332,0.01174786143315135
1992,3985,3984,7969,0.5423581600189209,0.011679866188123849
1994,3989,3988,7977,0.5438499450683594,0.011612264499335306
1996,3993,3992,7985,0.5449340343475342,0.011545054089493963
1998,3997,3996,7993,0.5459010601043701,0.011478232693533517
2000,4001,4000,8001,0.5463180541992188,0.011411798059870162


==> plot_data/cournot-nash_equilibrium_problem_n100/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00020194053649902344,1624.447741208611
4,5,4,9,0.0008759498596191406,544.0363924486542
8,9,8,17,0.0013208389282226562,401.36173086288113
12,13,12,25,0.001981019973754883,357.6362406908207
16,17,16,33,0.002579927444458008,304.7035721234219
20,21,20,41,0.0031027793884277344,282.5429398756775
24,25,24,49,0.003531932830810547,263.545386602969
28,29,28,57,0.004087924957275391,237.93843605665717
32,33,32,65,0.004586935043334961,232.74209504525268
36,37,36,73,0.005198955535888672,220.62732228780956
40,41,40,81,0.005733013153076172,206.6600819236898
44,45,44,89,0.006302833557128906,195.8071309227584
48,49,48,97,0.006731986999511719,185.98499736100567
52,53,52,105,0.007124900817871094,176.4249801671244
56,57,56,113,0.0076639652252197266,160.99673438238366
60,61,60,121,0.008116960525512695,155.074669878236
64,65,64,129,0.008572101593017578,140.68248881187407
68,69,68,137,0.009264945983886719,136.7436112633426
72,73,72,145,0.010180950164794922,126.13555406669731
76,77,76,153,0.010729789733886719,122.6271767498189
80,81,80,161,0.01119089126586914,120.1033131263988
84,85,84,169,0.012272119522094727,118.24307803399842
88,89,88,177,0.013134002685546875,111.03160848755374
92,93,92,185,0.013734102249145508,109.3209356466436
96,97,96,193,0.014208793640136719,107.9916479742846
100,101,100,201,0.014654874801635742,106.91733970853818
104,105,104,209,0.015380859375,106.01145651130207
108,109,108,217,0.016025066375732422,105.21442637828665
112,113,112,225,0.016675949096679688,104.48584861162735
116,117,116,233,0.01816701889038086,97.67474138373207
120,121,120,241,0.019238948822021484,96.84624281394237
124,125,124,249,0.01974010467529297,92.74771647581538
128,129,128,257,0.02053380012512207,91.91509966615192
132,133,132,265,0.021397829055786133,91.18224271567236
136,137,136,273,0.022439956665039062,90.51735649943699
140,141,140,281,0.023251056671142578,89.89785040541214
144,145,144,289,0.024168014526367188,89.30787727274557
148,149,148,297,0.02477097511291504,88.73647502499213
152,153,152,305,0.025660991668701172,88.17619040764093
156,157,156,313,0.026256084442138672,87.62206905106336
160,161,160,321,0.028964996337890625,87.07091988800155
164,165,164,329,0.02959609031677246,86.52078289621288
168,169,168,337,0.030236005783081055,85.97054634171977
172,173,172,345,0.031232833862304688,85.41967326824538
176,177,176,353,0.031828880310058594,80.48713944352677
180,181,180,361,0.03242897987365723,76.51439549094081
184,185,184,369,0.03319692611694336,75.89004502747424
188,189,188,377,0.034355878829956055,70.61728750362394
192,193,192,385,0.035459041595458984,69.83631139639554
196,197,196,393,0.03595900535583496,69.14499527167709
200,201,200,401,0.037843942642211914,68.52331642120069
204,205,204,409,0.0386967658996582,67.95546289645084
208,209,208,417,0.0392909049987793,67.42903078438667
212,213,212,425,0.03988909721374512,66.93434279160262
216,217,216,433,0.04048895835876465,66.46388913799011
220,221,220,441,0.04096078872680664,66.01187365771331
224,225,224,449,0.041525840759277344,65.57384841501334
228,229,228,457,0.042059898376464844,65.14642156904569
232,233,232,465,0.04266095161437988,64.72702509833591
236,237,236,473,0.04343390464782715,64.31373097304711
240,241,240,481,0.045243024826049805,63.90510624540377
244,245,244,489,0.04606890678405762,63.50009921859921
248,249,248,497,0.04659914970397949,63.097950316462374
252,253,252,505,0.04706978797912598,42.928681601131835
256,257,256,513,0.04754805564880371,42.31386496047765
260,261,260,521,0.048104047775268555,41.75511564194155
264,265,264,529,0.04870104789733887,41.243319637147486
268,269,268,537,0.04923582077026367,40.77090063718943
272,273,272,545,0.04976201057434082,40.33156954690536
276,277,276,553,0.050779104232788086,39.920111580527845
280,281,280,561,0.05128788948059082,39.53220534107694
284,285,284,569,0.051841020584106445,39.1642702706694
288,289,288,577,0.05273103713989258,38.813338833140236
292,293,292,585,0.053900957107543945,38.47694996361897
296,297,296,593,0.054566144943237305,38.15306060715899
300,301,300,601,0.055130958557128906,37.83997251045455
304,305,304,609,0.05572700500488281,37.53627178625901
308,309,308,617,0.05624890327453613,37.24077911442421
312,313,312,625,0.056715965270996094,36.952508761712366
316,317,316,633,0.05713391304016113,36.67063488781365
320,321,320,641,0.05757880210876465,36.394463854972344
324,325,324,649,0.05818295478820801,36.12341147412815
328,329,328,657,0.05860280990600586,29.865925543727368
332,333,332,665,0.05952882766723633,29.44784519348868
336,337,336,673,0.06109309196472168,29.06593245041313
340,341,340,681,0.06172800064086914,28.714757557990858
344,345,344,689,0.06225299835205078,28.389732415638928
348,349,348,697,0.06268787384033203,28.08698598009602
352,353,352,705,0.0631258487701416,27.803256108071604
356,357,356,713,0.06362485885620117,27.535795888509604
360,361,360,721,0.06407690048217773,27.282293138009276
364,365,364,729,0.06450915336608887,25.450190182078607
368,369,368,737,0.06510496139526367,25.28488829886332
372,373,372,745,0.06610798835754395,25.1206770110684
376,377,376,753,0.07094383239746094,24.957548230065413
380,381,380,761,0.07262706756591797,24.795496788854646
384,385,384,769,0.07330608367919922,24.634517344435352
388,389,388,777,0.07378077507019043,24.474604396685685
392,393,392,785,0.0743410587310791,24.3157523058087
396,397,396,793,0.07500886917114258,24.157955308388512
400,401,400,801,0.07596611976623535,24.001207532169683
404,405,404,809,0.07655477523803711,23.845503009641643
408,409,408,817,0.07723498344421387,23.690835690487255
412,413,412,825,0.0785069465637207,23.53719945301423
416,417,416,833,0.08077406883239746,23.384588114610608
420,421,420,841,0.08258199691772461,23.23299544130487
424,425,424,849,0.08413410186767578,23.082415156513356
428,429,428,857,0.08503103256225586,21.615457079608014
432,433,432,865,0.08555102348327637,21.47159438434253
436,437,436,873,0.08709096908569336,21.330744227379853
440,441,440,881,0.08784890174865723,21.192511919558825
444,445,444,889,0.09101605415344238,21.056564123663524
448,449,448,897,0.09402108192443848,20.922620145173763
452,453,452,905,0.09514999389648438,20.79044406821151
456,457,456,913,0.09605908393859863,20.659838011098987
460,461,460,921,0.09940505027770996,20.530636350795973
464,465,464,929,0.10022377967834473,20.40270078376111
468,469,468,937,0.10082793235778809,20.275916107488808
472,473,472,945,0.10131692886352539,20.150186621901526
476,477,476,953,0.10183215141296387,20.025433063048073
480,481,480,961,0.10286092758178711,19.901589993317494
484,485,484,969,0.10356283187866211,19.778603582684593
488,489,488,977,0.10423898696899414,19.65642972452914
492,493,492,985,0.10490989685058594,19.535032437437053
496,497,496,993,0.10547804832458496,19.41438251120289
501,502,501,1003,0.1060950756072998,19.264585605582983
505,506,505,1011,0.10655879974365234,19.145538025655593
509,510,509,1019,0.10696578025817871,19.027176953741304
513,514,513,1027,0.10769295692443848,18.909491149954025
517,518,517,1035,0.1083838939666748,18.792471818905863
521,522,521,1043,0.10926103591918945,17.593531374547773
525,526,525,1051,0.10973095893859863,17.468789168505587
529,530,529,1059,0.11039090156555176,17.34754628684548
533,534,533,1067,0.11083197593688965,17.229370822407297
537,538,537,1075,0.11137509346008301,17.113928110593758
541,542,541,1083,0.1118917465209961,17.000925663288168
545,546,545,1091,0.11245393753051758,16.89010805708794
549,550,549,1099,0.11291313171386719,16.78125240562571
553,554,553,1107,0.11348795890808105,16.674164356111977
557,558,557,1115,0.11393499374389648,16.568674554878626
561,562,561,1123,0.11435794830322266,16.46463553119361
565,566,565,1131,0.11484003067016602,16.361918953300126
569,570,569,1139,0.11815786361694336,16.260413214866336
573,574,573,1147,0.12055587768554688,16.160021314213047
577,578,577,1155,0.12176203727722168,16.06065899252718
581,582,581,1163,0.12252187728881836,15.962253100820071
585,586,585,1171,0.12323689460754395,15.86474016864462
589,590,589,1179,0.12375998497009277,15.768065150595534
593,594,593,1187,0.1243281364440918,15.672180329231544
597,598,597,1195,0.12486004829406738,15.577044355596275
601,602,601,1203,0.12532591819763184,15.482621410560496
605,606,605,1211,0.12752389907836914,15.388880472279665
609,610,609,1219,0.12835383415222168,15.29579467672093
613,614,613,1227,0.1288619041442871,14.40395859398114
617,618,617,1235,0.12962603569030762,14.301780376941366
621,622,621,1243,0.13014793395996094,14.202197274772644
625,626,625,1251,0.13071298599243164,14.104958629311172
629,630,629,1259,0.1313319206237793,14.009840930872933
633,634,633,1267,0.1318509578704834,13.916645399881343
637,638,637,1275,0.13251709938049316,12.598575013848881
641,642,641,1283,0.13425302505493164,5.782445343921283
645,646,645,1291,0.1347799301147461,5.6544576030634826
649,650,649,1299,0.1354978084564209,5.534454775684021
653,654,653,1307,0.1360948085784912,5.421880387553471
657,658,657,1315,0.13713979721069336,5.316208659390859
661,662,661,1323,0.13832306861877441,5.216943774893515
665,666,665,1331,0.1397998332977295,5.123619087963474
669,670,669,1339,0.14033913612365723,5.035796268137652
673,674,673,1347,0.14081406593322754,4.953064385470764
677,678,677,1355,0.14142298698425293,4.875038938973531
681,682,681,1363,0.14196014404296875,4.801360834987081
685,686,685,1371,0.1424710750579834,4.7316953235630494
689,690,689,1379,0.1449570655822754,4.665730902071809
693,694,693,1387,0.14560294151306152,4.603178195854054
697,698,697,1395,0.14802193641662598,4.543768825909008
701,702,701,1403,0.14864492416381836,4.487254273366698
705,706,705,1411,0.1495358943939209,4.4334047499642635
709,710,709,1419,0.15008091926574707,4.382008082988144
713,714,713,1427,0.15060901641845703,4.332868622215
717,718,717,1435,0.1511549949645996,4.285806175373983
721,722,721,1443,0.15267491340637207,4.240654977616675
725,726,725,1451,0.1533200740814209,4.197262699420698
729,730,729,1459,0.15424489974975586,4.155489496357391
733,734,733,1467,0.15486598014831543,4.115207103236635
737,738,737,1475,0.15552878379821777,4.076297974259821
741,742,741,1483,0.15630602836608887,4.038654470088903
745,746,745,1491,0.15685105323791504,4.002178092046624
749,750,749,1499,0.15749192237854004,3.9667787631347764
753,754,753,1507,0.15839815139770508,3.9323741550506397
757,758,757,1515,0.15887999534606934,3.898889060034813
761,762,761,1523,0.1593928337097168,3.866254806059838
765,766,765,1531,0.16135597229003906,3.8344087136450655
769,770,769,1539,0.1619129180908203,3.8032935924216917
773,774,773,1547,0.16254711151123047,3.772857275457154
777,778,777,1555,0.16299891471862793,3.7430521892680515
781,782,781,1563,0.16350412368774414,3.713834957461397
785,786,785,1571,0.163970947265625,3.6851660359000893
789,790,789,1579,0.16450190544128418,3.6570093773595915
793,794,793,1587,0.16498303413391113,3.62933212368159
797,798,797,1595,0.1656968593597412,3.6021043234762016
801,802,801,1603,0.16650891304016113,3.575298673552952
805,806,805,1611,0.1672511100769043,3.5488902822780957
809,810,809,1619,0.16994190216064453,3.522856453218773
813,814,813,1627,0.17064905166625977,3.497176487474093
817,818,817,1635,0.17223286628723145,3.471831503218151
821,822,821,1643,0.1737661361694336,3.4468042710618434
825,826,825,1651,0.17563581466674805,3.4220790639448944
829,830,829,1659,0.17716288566589355,3.3976415203426207
833,834,833,1667,0.1780109405517578,3.3734785196759947
837,838,837,1675,0.17870616912841797,3.3495780688869683
841,842,841,1683,0.17930006980895996,3.3259291992179185
845,846,845,1691,0.1799020767211914,3.3025218723214715
849,850,849,1699,0.18188095092773438,3.2793468948794304
853,854,853,1707,0.1824181079864502,3.25639584098783
857,858,857,1715,0.18320989608764648,3.2336609816215685
861,862,861,1723,0.18374991416931152,3.2111352205496346
865,866,865,1731,0.18462085723876953,3.188812036126301
869,870,869,1739,0.1852269172668457,3.1666854284284787
873,874,873,1747,0.1858210563659668,3.1447498712589637
877,878,877,1755,0.18886995315551758,3.1230002685783123
881,882,881,1763,0.18964385986328125,3.1014319149566507
885,886,885,1771,0.19016003608703613,3.080040459688916
889,890,889,1779,0.1907508373260498,3.0588218742266586
893,894,893,1787,0.1913299560546875,3.037772422635141
897,898,897,1795,0.19181203842163086,3.01688863479086
901,902,901,1803,0.192518949508667,2.9961672820696954
905,906,905,1811,0.19302892684936523,2.975605355297039
909,910,909,1819,0.19400691986083984,2.95520004474309
913,914,913,1827,0.1946089267730713,2.934948721992712
917,918,917,1835,0.19525909423828125,2.91484892349093
921,922,921,1843,0.19584083557128906,2.8948983356372175
925,926,925,1851,0.19702696800231934,2.8750947812544174
929,930,929,1859,0.19822406768798828,2.8554362073293813
933,934,933,1867,0.19966983795166016,2.2495048218023213
937,938,937,1875,0.2002239227294922,2.225129297906036
941,942,941,1883,0.20083403587341309,2.2015948125247875
945,946,945,1891,0.20135998725891113,2.178848380795309
949,950,949,1899,0.2018437385559082,2.156840433128436
953,954,953,1907,0.2022838592529297,2.1355246252098774
957,958,957,1915,0.2027120590209961,2.114857656039003
961,962,961,1923,0.20311284065246582,2.094799092454854
965,966,965,1931,0.20416879653930664,2.0753112004131657
969,970,969,1939,0.20534992218017578,2.0563587831844834
973,974,973,1947,0.2059187889099121,2.0379090265876023
977,978,977,1955,0.20720195770263672,2.019931351299467
981,982,981,1963,0.20774388313293457,2.0023972722312
985,986,985,1971,0.20836997032165527,1.9852802649181345
989,990,989,1979,0.20887374877929688,1.9685556388145433
993,994,993,1987,0.20931291580200195,1.9522004173528398
997,998,997,1995,0.20994281768798828,1.9361932246110767
1001,1002,1001,2003,0.2105109691619873,1.9205141783802298
1005,1006,1005,2011,0.21105694770812988,1.9051447894289122
1009,1010,1009,2019,0.21177315711975098,1.890067866735804
1013,1014,1013,2027,0.21224212646484375,1.8752674284560393
1017,1018,1017,2035,0.21291685104370117,1.860728618358714
1021,1022,1021,2043,0.21352314949035645,1.8464376275109253
1025,1026,1025,2051,0.21421408653259277,1.8323816209387997
1029,1030,1029,2059,0.2146449089050293,1.8185486690234594
1033,1034,1033,2067,0.21507906913757324,1.8049276833790497
1037,1038,1037,2075,0.2157909870147705,1.7915083569840533
1041,1042,1041,2083,0.21660780906677246,1.7782811083031167
1045,1046,1045,2091,0.21730709075927734,1.7652370292013286
1049,1050,1049,2099,0.21810388565063477,1.7523678364039468
1053,1054,1053,2107,0.21915698051452637,1.739665826298046
1057,1058,1057,2115,0.22142696380615234,1.7271238328720435
1061,1062,1061,2123,0.22205781936645508,1.71473518859239
1065,1066,1065,2131,0.22285676002502441,1.702493688032251
1069,1070,1069,2139,0.22336101531982422,1.6903935540809036
1073,1074,1073,2147,0.22399306297302246,1.6784294065473315
1077,1078,1077,2155,0.22443675994873047,1.666596233026288
1081,1082,1081,2163,0.22499489784240723,1.6548893618455922
1085,1086,1085,2171,0.22585201263427734,1.6433044369784833
1089,1090,1089,2179,0.22690391540527344,1.6318373947725497
1093,1094,1093,2187,0.22748780250549316,1.6204844423694857
1097,1098,1097,2195,0.22818589210510254,1.609242037710629
1101,1102,1101,2203,0.22864389419555664,1.5981068710020723
1105,1106,1105,2211,0.230604887008667,1.5870758475453062
1109,1110,1109,2219,0.23119592666625977,1.5761460718322375
1113,1114,1113,2227,0.231964111328125,1.5653148328206459
1117,1118,1117,2235,0.2325611114501953,1.554579590294459
1121,1122,1121,2243,0.23334217071533203,1.543937962241531
1125,1126,1125,2251,0.2338268756866455,1.5333877131672007
1129,1130,1129,2259,0.23444080352783203,1.5229267432862112
1133,1134,1133,2267,0.23502779006958008,1.5125530785087418
1137,1138,1137,2275,0.2355518341064453,1.502264861186468
1141,1142,1141,2283,0.2360069751739502,1.4920603415456681
1145,1146,1145,2291,0.2377159595489502,0.8304834359113775
1149,1150,1149,2299,0.2384810447692871,0.8136089404653333
1153,1154,1153,2307,0.23935198783874512,0.7974069942858905
1157,1158,1157,2315,0.24022793769836426,0.7818505446205847
1161,1162,1161,2323,0.2411518096923828,0.7669132957504431
1165,1166,1165,2331,0.2418510913848877,0.7525697565568208
1169,1170,1169,2339,0.24290704727172852,0.7387952270322665
1173,1174,1173,2347,0.24358487129211426,0.7255657854466626
1177,1178,1177,2355,0.2443699836730957,0.712858276035837
1181,1182,1181,2363,0.24484491348266602,0.7006502970733024
1185,1186,1185,2371,0.24547505378723145,0.688920189201595
1189,1190,1189,2379,0.24604105949401855,0.6776470239038594
1193,1194,1193,2387,0.24688196182250977,0.666810592009419
1197,1198,1197,2395,0.24859881401062012,0.6563913921415775
1201,1202,1201,2403,0.24909305572509766,0.6463706190179203
1205,1206,1205,2411,0.24954795837402344,0.6367301515399042
1209,1210,1209,2419,0.25005412101745605,0.6274525406099924
1213,1214,1213,2427,0.2505369186401367,0.6185209966326219
1217,1218,1217,2435,0.2510371208190918,0.6099193766700071
1221,1222,1221,2443,0.2514641284942627,0.601632171226784
1225,1226,1225,2451,0.25199103355407715,0.5936444906630177
1229,1230,1229,2459,0.25345396995544434,0.5859420512305273
1233,1234,1233,2467,0.2539801597595215,0.578511160746579
1237,1238,1237,2475,0.2544889450073242,0.5713387039290884
1241,1242,1241,2483,0.2551441192626953,0.5644121274113506
1245,1246,1245,2491,0.25568604469299316,0.5577194244799988
1249,1250,1249,2499,0.25643205642700195,0.5512491195682615
1253,1254,1253,2507,0.25689196586608887,0.5449902525475029
1257,1258,1257,2515,0.2575390338897705,0.5389323628643411
1261,1262,1261,2523,0.2585489749908447,0.5330654735699204
1265,1266,1265,2531,0.25936198234558105,0.5273800752869996
1269,1270,1269,2539,0.2600250244140625,0.5218671101657764
1273,1274,1273,2547,0.2606649398803711,0.5165179558709114
1277,1278,1277,2555,0.261077880859375,0.5113244096518587
1281,1282,1281,2563,0.26153993606567383,0.5062786725342693
1285,1286,1285,2571,0.2619490623474121,0.501373333676657
1289,1290,1289,2579,0.2626228332519531,0.49660135492982216
1293,1294,1293,2587,0.2641267776489258,0.49195605563738903
1297,1298,1297,2595,0.2646949291229248,0.4874310977036176
1301,1302,1301,2603,0.2651839256286621,0.4830204709664045
1305,1306,1305,2611,0.2659449577331543,0.47871847889089947
1309,1310,1309,2619,0.2664909362792969,0.4745197246177038
1313,1314,1313,2627,0.26935696601867676,0.47041909737103255
1317,1318,1317,2635,0.26995182037353516,0.4664117592579236
1321,1322,1321,2643,0.2713019847869873,0.46249313245751145
1325,1326,1325,2651,0.27193474769592285,0.45865888681976386
1329,1330,1329,2659,0.2733888626098633,0.4549049278760385
1333,1334,1333,2667,0.277385950088501,0.4512273852688535
1337,1338,1337,2675,0.27861595153808594,0.4476226015994192
1341,1342,1341,2683,0.2792038917541504,0.4440871216992089
1345,1346,1345,2691,0.28005003929138184,0.44061768231650983
1349,1350,1349,2699,0.2808659076690674,0.43721120222103776
1353,1354,1353,2707,0.282088041305542,0.4338647727176026
1357,1358,1357,2715,0.28339505195617676,0.43057564856281866
1361,1362,1361,2723,0.28517889976501465,0.42734123927899603
1365,1366,1365,2731,0.2861759662628174,0.4241591008568908
1369,1370,1369,2739,0.2869999408721924,0.4210269278338884
1373,1374,1373,2747,0.2888941764831543,0.41794254574341877
1377,1378,1377,2755,0.2893648147583008,0.41490390391999965
1381,1382,1381,2763,0.28999805450439453,0.41190906865149624
1385,1386,1385,2771,0.29054999351501465,0.40895621666663623
1389,1390,1389,2779,0.29110288619995117,0.4060436289448085
1393,1394,1393,2787,0.2921891212463379,0.40316968484050336
1397,1398,1397,2795,0.29273104667663574,0.4003328565015572
1401,1402,1401,2803,0.2937638759613037,0.3975317035835102
1405,1406,1405,2811,0.294266939163208,0.3947648682317937
1409,1410,1409,2819,0.29475998878479004,0.39203107033511375
1413,1414,1413,2827,0.29544901847839355,0.38932910302686624
1417,1418,1417,2835,0.2959861755371094,0.3866578284320578
1421,1422,1421,2843,0.2965400218963623,0.38401617364291923
1425,1426,1425,2851,0.2971959114074707,0.3814031269161988
1429,1430,1429,2859,0.2979397773742676,0.37881773407694336
1433,1434,1433,2867,0.29848313331604004,0.3762590951256464
1437,1438,1437,2875,0.29894399642944336,0.3737263610341928
1441,1442,1441,2883,0.29936814308166504,0.37121873071927014
1445,1446,1445,2891,0.2998690605163574,0.36873544819078463
1449,1450,1449,2899,0.30036187171936035,0.3662757998611856
1453,1454,1453,2907,0.3013029098510742,0.36383911200709895
1457,1458,1457,2915,0.30173206329345703,0.36142474838092686
1461,1462,1461,2923,0.302152156829834,0.3590321079557587
1465,1466,1465,2931,0.3025698661804199,0.3566606228054295
1469,1470,1469,2939,0.3029599189758301,0.3543097561062665
1473,1474,1473,2947,0.3033158779144287,0.3519790002560917
1477,1478,1477,2955,0.30370497703552246,0.3496678751036569
1481,1482,1481,2963,0.3041250705718994,0.3473759262820464
1485,1486,1485,2971,0.3045229911804199,0.3451027236440108
1489,1490,1489,2979,0.3049740791320801,0.3428478597858858
1493,1494,1493,2987,0.3053920269012451,0.3406109486613887
1497,1498,1497,2995,0.30608391761779785,0.3383916242811402
1502,1503,1502,3005,0.30660390853881836,0.3356416729852381
1506,1507,1506,3013,0.30703306198120117,0.3334606763003361
1510,1511,1510,3021,0.30744099617004395,0.3312962010827291
1514,1515,1514,3029,0.30785703659057617,0.32914795377159106
1518,1519,1518,3037,0.3083679676055908,0.32701565520190395
1522,1523,1522,3045,0.30887794494628906,0.3248990397221639
1526,1527,1526,3053,0.30942201614379883,0.32279785436459285
1530,1531,1530,3061,0.30994701385498047,0.32071185806818014
1534,1535,1534,3069,0.31067514419555664,0.31864082094651247
1538,1539,1538,3077,0.31122803688049316,0.3165845236024685
1542,1543,1542,3085,0.3118579387664795,0.31454275648494334
1546,1547,1546,3093,0.31232595443725586,0.312515319283273
1550,1551,1550,3101,0.31282901763916016,0.31050202036258084
1554,1555,1554,3109,0.31327390670776367,0.3085026762299642
1558,1559,1558,3117,0.31375885009765625,0.30651711103640483
1562,1563,1562,3125,0.3142850399017334,0.3045451561091146
1566,1567,1566,3133,0.3167269229888916,0.3025866495118356
1570,1571,1570,3141,0.31722211837768555,0.3006414356346439
1574,1575,1574,3149,0.3176109790802002,0.2987093648062779
1578,1579,1578,3157,0.31804800033569336,0.2967902929332278
1582,1583,1582,3165,0.31848907470703125,0.29488408116180076
1586,1587,1586,3173,0.3190019130706787,0.2929905955573933
1590,1591,1590,3181,0.31946802139282227,0.2911097068087943
1594,1595,1594,3189,0.31993579864501953,0.28924128994786535
1598,1599,1598,3197,0.3204519748687744,0.2873852240889178
1602,1603,1602,3205,0.3214409351348877,0.28554139218104574
1606,1607,1606,3213,0.3220489025115967,0.2837096807819017
1610,1611,1610,3221,0.3227040767669678,0.28188997983937847
1614,1615,1614,3229,0.32337284088134766,0.2800821824917321
1618,1619,1618,3237,0.3239269256591797,0.2782861848781429
1622,1623,1622,3245,0.3244037628173828,0.2765018859619645
1626,1627,1626,3253,0.32503485679626465,0.2747291873651564
1630,1631,1630,3261,0.32566118240356445,0.2729679932134051
1634,1635,1634,3269,0.3262648582458496,0.2712182099914898
1638,1639,1638,3277,0.32666993141174316,0.2694797464051123
1642,1643,1642,3285,0.32719874382019043,0.2677525132563789
1646,1647,1646,3293,0.3278040885925293,0.26603642332341587
1650,1651,1650,3301,0.32843685150146484,0.26433139124966226
1654,1655,1654,3309,0.3302009105682373,0.26263733343782447
1658,1659,1658,3317,0.3306751251220703,0.26095416795543935
1662,1663,1662,3325,0.33110594749450684,0.25928181443968146
1666,1667,1666,3333,0.33150410652160645,0.25762019401499325
1670,1671,1670,3341,0.3319358825683594,0.2559692292127202
1674,1675,1674,3349,0.33245086669921875,0.254328843895258
1678,1679,1678,3357,0.3329341411590576,0.25269896318624735
1682,1683,1682,3365,0.3333399295806885,0.2510795134063772
1686,1687,1686,3373,0.3338310718536377,0.2494704220110485
1690,1691,1690,3381,0.3347928524017334,0.24787161753513767
1694,1695,1694,3389,0.3354480266571045,0.2462830295356894
1698,1699,1698,3397,0.3360569477081299,0.24470458854734342
1702,1703,1702,3405,0.3367750644683838,0.24313622603089824
1706,1707,1706,3413,0.33844709396362305,0.24157787433152117
1710,1711,1710,3421,0.33950185775756836,0.24002946663852884
1714,1715,1714,3429,0.34039998054504395,0.23849093694663498
1718,1719,1718,3437,0.34132909774780273,0.23696222001989195
1722,1723,1722,3445,0.3430299758911133,0.23544325135971833
1726,1727,1726,3453,0.34398603439331055,0.23393396717204468
1730,1731,1730,3461,0.3447299003601074,0.2324343043389616
1734,1735,1734,3469,0.3453538417816162,0.23094420039277883
1738,1739,1738,3477,0.3490898609161377,0.22946359348913323
1742,1743,1742,3485,0.3514058589935303,0.22799242238228737
1746,1747,1746,3493,0.35190296173095703,0.22653062640654165
1750,1751,1750,3501,0.3523728847503662,0.22507814545187088
1754,1755,1754,3509,0.3528721332550049,0.22363491994645804
1758,1759,1758,3517,0.35390305519104004,0.22220089083895964
1762,1763,1762,3525,0.3545799255371094,0.22077599957955477
1766,1767,1766,3533,0.3554558753967285,0.21936018810666394
1770,1771,1770,3541,0.3562040328979492,0.21795339883037854
1774,1775,1774,3549,0.3568379878997803,0.2165555746197254
1778,1779,1778,3557,0.35745906829833984,0.21516665878888755
1782,1783,1782,3565,0.3581089973449707,0.2137865950866935
1786,1787,1786,3573,0.3588130474090576,0.21241532768308144
1790,1791,1790,3581,0.35973286628723145,0.21105280116068337
1794,1795,1794,3589,0.3605830669403076,0.20969896050392267
1798,1799,1798,3597,0.3614010810852051,0.20835375109008858
1802,1803,1802,3605,0.3619821071624756,0.20701711868079578
1806,1807,1806,3613,0.36399292945861816,0.20568900941287416
1810,1811,1810,3621,0.36446189880371094,0.204369369792877
1814,1815,1814,3629,0.3649630546569824,0.20305814668829522
1818,1819,1818,3637,0.3657100200653076,0.20175528732134657
1822,1823,1822,3645,0.36736202239990234,0.2004607392627841
1826,1827,1826,3653,0.36904096603393555,0.19917445042697848
1830,1831,1830,3661,0.3713860511779785,0.19789636906444638
1834,1835,1834,3669,0.37293195724487305,0.19662644375806182
1838,1839,1838,3677,0.37378978729248047,0.1953646234194421
1842,1843,1842,3685,0.37432003021240234,0.19411085728101227
1846,1847,1846,3693,0.37482786178588867,0.19286509489494866
1850,1851,1850,3701,0.3759629726409912,0.1916272861272068
1854,1855,1854,3709,0.3771491050720215,0.19039738115495025
1858,1859,1858,3717,0.3780341148376465,0.18917533046189783
1862,1863,1862,3725,0.37868309020996094,0.187961084835882
1866,1867,1866,3733,0.37943482398986816,0.1867545953650554
1870,1871,1870,3741,0.3802018165588379,0.18555581343442398
1874,1875,1874,3749,0.3821909427642822,0.18436469072484013
1878,1879,1878,3757,0.3830399513244629,0.18318117920739976
1882,1883,1882,3765,0.3835740089416504,0.18200523114327088
1886,1887,1886,3773,0.38660693168640137,0.1808367990805792
1890,1891,1890,3781,0.3893918991088867,0.1796758358506431
1894,1895,1894,3789,0.3903629779815674,0.17852229456838398
1898,1899,1898,3797,0.39112210273742676,0.17737612862696442
1902,1903,1902,3805,0.3922419548034668,0.1762372916990448
1906,1907,1906,3813,0.3932168483734131,0.1751057377316911
1910,1911,1910,3821,0.394212007522583,0.17398142094710808
1914,1915,1914,3829,0.395035982131958,0.17286429583876922
1918,1919,1918,3837,0.39570093154907227,0.17175431717130882
1922,1923,1922,3845,0.39647889137268066,0.17065143997650695
1926,1927,1926,3853,0.3972609043121338,0.16955561955469067
1930,1931,1930,3861,0.39795899391174316,0.1684668114707269
1934,1935,1934,3869,0.3985929489135742,0.16738497155335463
1938,1939,1938,3877,0.40048885345458984,0.1663100558935925
1942,1943,1942,3885,0.40108203887939453,0.16524202084291245
1946,1947,1946,3893,0.40157508850097656,0.1641808230125297
1950,1951,1950,3901,0.4042348861694336,0.1631264192711898
1954,1955,1954,3909,0.4049408435821533,0.1620787667444469
1958,1959,1958,3917,0.405925989151001,0.16103782281293652
1962,1963,1962,3925,0.40648698806762695,0.16000354511118164
1966,1967,1966,3933,0.40700793266296387,0.15897589152512326
1970,1971,1970,3941,0.40753984451293945,0.1579548201936105
1974,1975,1974,3949,0.4081587791442871,0.1569402895038741
1978,1979,1978,3957,0.40901899337768555,0.15593225809320505
1982,1983,1982,3965,0.40958404541015625,0.15493068484442515
1986,1987,1986,3973,0.41016101837158203,0.15393552888869297
1990,1991,1990,3981,0.4108140468597412,0.15294674960008933
1994,1995,1994,3989,0.4114859104156494,0.15196430659765484
1998,1999,1998,3997,0.4120359420776367,0.15098815974326202
2002,2003,2002,4005,0.4126420021057129,0.15001826913856944
2006,2007,2006,4013,0.4130830764770508,0.14905459512680289
2010,2011,2010,4021,0.4144108295440674,0.1480970982893223
2014,2015,2014,4029,0.41656494140625,0.14714573944569345
2018,2019,2018,4037,0.41716694831848145,0.14620047965255906
2022,2023,2022,4045,0.41860294342041016,0.14526128020061538
2026,2027,2026,4053,0.41951513290405273,0.14432810261700776
2030,2031,2030,4061,0.42206287384033203,0.1434009086595875
2034,2035,2034,4069,0.42290592193603516,0.14247966032026865
2038,2039,2038,4077,0.4237940311431885,0.14156431982110032
2042,2043,2042,4085,0.4242820739746094,0.1406548496134976
2046,2047,2046,4093,0.4250028133392334,0.1397512123777541
2050,2051,2050,4101,0.42560815811157227,0.13885337102196652
2054,2055,2054,4109,0.42656707763671875,0.13796128868035998
2058,2059,2058,4117,0.42772698402404785,0.1370749287118399
2062,2063,2062,4125,0.4285099506378174,0.13619425470037239
2066,2067,2066,4133,0.4292418956756592,0.13531923045168096
2070,2071,2070,4141,0.4298851490020752,0.134449819994342
2074,2075,2074,4149,0.43170976638793945,0.13358598757720713
2078,2079,2078,4157,0.432811975479126,0.13272769766822884
2082,2083,2082,4165,0.433596134185791,0.13187491495486833
2086,2087,2086,4173,0.4342508316040039,0.13102760434073518
2090,2091,2090,4181,0.43488597869873047,0.1301857309465068
2094,2095,2094,4189,0.43559694290161133,0.1293492601066908
2098,2099,2098,4197,0.4366590976715088,0.12851815737178057
2102,2103,2102,4205,0.4378509521484375,0.12769238850348363
2106,2107,2106,4213,0.43848586082458496,0.12687191947524565
2110,2111,2110,4221,0.43999290466308594,0.1260567164719452
2114,2115,2114,4229,0.4406120777130127,0.12524674588741183
2118,2119,2118,4237,0.4412698745727539,0.12444197432355229
2122,2123,2122,4245,0.4417870044708252,0.12364236859037966
2126,2127,2126,4253,0.4422750473022461,0.12284789570337942
2130,2131,2130,4261,0.44275403022766113,0.12205852288325895
2134,2135,2134,4269,0.4432528018951416,0.12127421755430087
2138,2139,2138,4277,0.44379591941833496,0.12049494734428673
2142,2143,2142,4285,0.4443490505218506,0.11972068008244575
2146,2147,2146,4293,0.44525694847106934,0.11895138379829265
2150,2151,2150,4301,0.44576597213745117,0.11818702672126884
2154,2155,2154,4309,0.44632577896118164,0.11742757727877677
2158,2159,2158,4317,0.44845104217529297,0.11667300409556132
2162,2163,2162,4325,0.4490480422973633,0.11592327599358612
2166,2167,2166,4333,0.4495887756347656,0.11517836198828098
2170,2171,2170,4341,0.45004892349243164,0.11443823129064833
2174,2175,2174,4349,0.45049595832824707,0.11370285330382658
2178,2179,2178,4357,0.45094990730285645,0.11297219762254944
2182,2183,2182,4365,0.45137977600097656,0.11224623403337082
2186,2187,2186,4373,0.4518239498138428,0.1115249325111409
2190,2191,2190,4381,0.45235395431518555,0.11080826322059237
2194,2195,2194,4389,0.453110933303833,0.11009619651384053
2198,2199,2198,4397,0.4536721706390381,0.10938870292798213
2202,2203,2202,4405,0.45505404472351074,0.10868575318786862
2206,2207,2206,4413,0.4578239917755127,0.1079873182003694
2210,2211,2210,4421,0.45859289169311523,0.10729336905736525
2214,2215,2214,4429,0.45915985107421875,0.10660387703263383
2218,2219,2218,4437,0.4597890377044678,0.10591881358030551
2222,2223,2222,4445,0.4602987766265869,0.10523815033492712
2226,2227,2226,4453,0.4607689380645752,0.10456185911055337
2230,2231,2230,4461,0.46143198013305664,0.10388991189909129
2234,2235,2234,4469,0.46188998222351074,0.10322228086945487
2238,2239,2238,4477,0.46269893646240234,0.10255893836534329
2242,2243,2242,4485,0.46321988105773926,0.10189985690736096
2246,2247,2246,4493,0.46367597579956055,0.1012450091884132
2250,2251,2250,4501,0.46422791481018066,0.10059436807493395
2254,2255,2254,4509,0.4676520824432373,0.09994790660542789
2258,2259,2258,4517,0.470761775970459,0.09930559798760026
2262,2263,2262,4525,0.4753129482269287,0.09866741560121706
2266,2267,2266,4533,0.47766685485839844,0.09803333299300138
2270,2271,2270,4541,0.4788808822631836,0.09740332387822757
2274,2275,2274,4549,0.4804048538208008,0.09677736213876373
2278,2279,2278,4557,0.4823038578033447,0.0961554218225594
2282,2283,2282,4565,0.4842410087585449,0.09553747714170734
2286,2287,2286,4573,0.48531389236450195,0.09492350247202247
2290,2291,2290,4581,0.491225004196167,0.0943134723533625
2294,2295,2294,4589,0.49323415756225586,0.09370736148537931
2298,2299,2298,4597,0.4948880672454834,0.09310514473045498
2302,2303,2302,4605,0.4956240653991699,0.09250679710920602
2306,2307,2306,4613,0.4962730407714844,0.09191229380214622
2310,2311,2310,4621,0.4969758987426758,0.09132161014754012
2314,2315,2314,4629,0.49794507026672363,0.09073472164020316
2318,2319,2318,4637,0.49857592582702637,0.09015160393159118
2322,2323,2322,4645,0.4993860721588135,0.08957223282709839
2326,2327,2326,4653,0.4999070167541504,0.08899658428754491
2330,2331,2330,4661,0.5003819465637207,0.08842463442547563
2334,2335,2334,4669,0.500856876373291,0.08785635950726849
2338,2339,2338,4677,0.5013899803161621,0.08729173594888498
2342,2343,2342,4685,0.5032470226287842,0.08673074031776826
2346,2347,2346,4693,0.5039777755737305,0.08617334933073968
2350,2351,2350,4701,0.5044231414794922,0.08561953985232738
2354,2355,2354,4709,0.5049350261688232,0.08506928889522258
2358,2359,2358,4717,0.5054299831390381,0.08452257361835604
2362,2363,2362,4725,0.5059170722961426,0.08397937132705799
2366,2367,2366,4733,0.5063860416412354,0.08343965947144688
2370,2371,2370,4741,0.5068888664245605,0.08290341564523672
2374,2375,2374,4749,0.5073609352111816,0.08237061758460362
2378,2379,2378,4757,0.5079059600830078,0.08184124316903285
2382,2383,2382,4765,0.509958028793335,0.0813152704191796
2386,2387,2386,4773,0.5105850696563721,0.08079267749561077
2390,2391,2390,4781,0.5111219882965088,0.08027344269847105
2394,2395,2394,4789,0.5116598606109619,0.07975754446682569
2398,2399,2398,4797,0.5121550559997559,0.07924496137745278
2402,2403,2402,4805,0.5127608776092529,0.07873567214441106
2406,2407,2406,4813,0.5132420063018799,0.07822965561691857
2410,2411,2410,4821,0.5137529373168945,0.07772689078044429
2414,2415,2414,4829,0.5143280029296875,0.07722735675460618
2418,2419,2418,4837,0.514826774597168,0.0767310327916241
2422,2423,2422,4845,0.5153241157531738,0.07623789827820189
2426,2427,2426,4853,0.5158817768096924,0.0757479327319588
2430,2431,2430,4861,0.5164980888366699,0.07526111580066158
2434,2435,2434,4869,0.5170688629150391,0.07477742726414573
2438,2439,2438,4877,0.5191121101379395,0.07429684703057766
2442,2443,2442,4885,0.5198090076446533,0.07381935513682207
2446,2447,2446,4893,0.5210490226745605,0.07334493174752646
2450,2451,2450,4901,0.5228121280670166,0.07287355715427982
2454,2455,2454,4909,0.5234649181365967,0.07240521177531445
2458,2459,2458,4917,0.5243649482727051,0.07193987615422008
2462,2463,2462,4925,0.5250759124755859,0.07147753095881654
2466,2467,2466,4933,0.5257000923156738,0.07101815698061509
2470,2471,2470,4941,0.5264737606048584,0.0705617351345886
2474,2475,2474,4949,0.529433012008667,0.070108246458183
2478,2479,2478,4957,0.5306239128112793,0.06965767210914796
2482,2483,2482,4965,0.5312018394470215,0.06920999336746454
2486,2487,2486,4973,0.5320439338684082,0.0687651916323492
2490,2491,2490,4981,0.5326859951019287,0.068323248422401
2494,2495,2494,4989,0.5335378646850586,0.06788414537415684
2498,2499,2498,4997,0.5340840816497803,0.06744786424224093
2503,2504,2503,5007,0.5350749492645264,0.06690645354116886
2507,2508,2507,5015,0.5355818271636963,0.06647645561647983
2511,2512,2511,5023,0.5377969741821289,0.06604922111438438
2515,2516,2515,5031,0.5384328365325928,0.06562473228212844
2519,2520,2519,5039,0.5395071506500244,0.06520297147997187
2523,2524,2523,5047,0.5400490760803223,0.06478392118093909
2527,2528,2527,5055,0.5408380031585693,0.06436756397147202
2531,2532,2531,5063,0.5414609909057617,0.06395388254896409
2535,2536,2535,5071,0.5425469875335693,0.06354285972207524
2539,2540,2539,5079,0.5431079864501953,0.06313447841008506
2543,2544,2543,5087,0.5437428951263428,0.06272872164060224
2547,2548,2547,5095,0.5446319580078125,0.062325572551096234
2551,2552,2551,5103,0.5453190803527832,0.06192501438757186
2555,2556,2555,5111,0.5458409786224365,0.06152703050253078
2559,2560,2559,5119,0.546950101852417,0.06113160435587208
2563,2564,2563,5127,0.5480349063873291,0.06073871951328228
2567,2568,2567,5135,0.5485098361968994,0.06034835964644191
2571,2572,2571,5143,0.5491559505462646,0.05996050853105337
2575,2576,2575,5151,0.549656867980957,0.059575150047559575
2579,2580,2579,5159,0.5502228736877441,0.05919226817995475
2583,2584,2583,5167,0.5506429672241211,0.05881184701379559
2587,2588,2587,5175,0.5511348247528076,0.05843387073850857
2591,2592,2591,5183,0.5515601634979248,0.05805832364400515
2595,2596,2595,5191,0.552191972732544,0.05768519012085101
2599,2600,2599,5199,0.5527300834655762,0.05731445466023477
2603,2604,2603,5207,0.5532469749450684,0.05694610185299025
2607,2608,2607,5215,0.554002046585083,0.056580116388344814
2611,2612,2611,5223,0.554542064666748,0.056216483054771595
2615,2616,2615,5231,0.5552408695220947,0.055855186736827045
2619,2620,2619,5239,0.5557301044464111,0.055496212418130804
2623,2624,2623,5247,0.5561890602111816,0.055139545176424394
2627,2628,2627,5255,0.5566449165344238,0.054785170187407854
2631,2632,2631,5263,0.5571281909942627,0.05443307272035289
2635,2636,2635,5271,0.5575978755950928,0.05408323814067652
2639,2640,2639,5279,0.5579988956451416,0.05373565190564457
2643,2644,2643,5287,0.5584690570831299,0.05339029956762315
2647,2648,2647,5295,0.5589230060577393,0.053047166771540616
2651,2652,2651,5303,0.5594568252563477,0.05270623925353253
2655,2656,2655,5311,0.560621976852417,0.052367502842893494
2659,2660,2659,5319,0.5617749691009521,0.05203094345832344
2663,2664,2663,5327,0.56227707862854,0.05169654710978734
2667,2668,2667,5335,0.562856912612915,0.05136429989680391
2671,2672,2671,5343,0.5632610321044922,0.051034188008792045
2675,2676,2675,5351,0.563784122467041,0.05070619772285227
2679,2680,2679,5359,0.5641829967498779,0.050380315404790876
2683,2684,2683,5367,0.5645890235900879,0.0500565275085795
2687,2688,2687,5375,0.5650510787963867,0.04973482057392071
2691,2692,2691,5383,0.5657439231872559,0.049415181227776286
2695,2696,2695,5391,0.5664448738098145,0.04909759618287368
2699,2700,2699,5399,0.5674099922180176,0.048782052237201314
2703,2704,2703,5407,0.568317174911499,0.0484685362735265
2707,2708,2707,5415,0.5691177845001221,0.04815703525910831
2711,2712,2711,5423,0.5696721076965332,0.04784753624435417
2715,2716,2715,5431,0.5700960159301758,0.047540026364038215
2719,2720,2719,5439,0.5708639621734619,0.04723449283394639
2723,2724,2723,5447,0.5714578628540039,0.04693092295354268
2727,2728,2727,5455,0.5721209049224854,0.046629304102730265
2731,2732,2731,5463,0.5731790065765381,0.04632962374290723
2735,2736,2735,5471,0.5737528800964355,0.0460318694164518
2739,2740,2739,5479,0.574321985244751,0.04573602874445909
2743,2744,2743,5487,0.5749459266662598,0.045442089429233466
2747,2748,2747,5495,0.5755171775817871,0.0451500392513484
2751,2752,2751,5503,0.5778720378875732,0.04485986606959038
2755,2756,2755,5511,0.5783870220184326,0.044571557820671494
2759,2760,2759,5519,0.5789580345153809,0.04428510251991772
2763,2764,2763,5527,0.5796248912811279,0.04400048825823924
2767,2768,2767,5535,0.5802018642425537,0.043717703203816884
2771,2772,2771,5543,0.5807111263275146,0.04343673560046185
2775,2776,2775,5551,0.581183910369873,0.04315757376807334
2779,2780,2779,5559,0.5819261074066162,0.04288020610165274
2783,2784,2783,5567,0.5839929580688477,0.042604621069695904
2787,2788,2787,5575,0.5846388339996338,0.04233080721607541
2791,2792,2791,5583,0.5850729942321777,0.042058753157068314
2795,2796,2795,5591,0.5856280326843262,0.041788447583054174
2799,2800,2799,5599,0.586061954498291,0.04151987925711527
2803,2804,2803,5607,0.5869410037994385,0.04125303701321092
2807,2808,2807,5615,0.5875470638275146,0.0409879097591279
2811,2812,2811,5623,0.588148832321167,0.040724486472290725
2815,2816,2815,5631,0.5893499851226807,0.040462756201448416
2819,2820,2819,5639,0.5899240970611572,0.040202708065401126
2823,2824,2823,5647,0.5908818244934082,0.03994433125380305
2827,2828,2827,5655,0.5919249057769775,0.039687615024603023
2831,2832,2831,5663,0.5939130783081055,0.03943254870611054
2835,2836,2835,5671,0.5952529907226562,0.0391791216934485
2839,2840,2839,5679,0.5962221622467041,0.038927323451618645
2843,2844,2843,5687,0.5979049205780029,0.03867714351231007
2847,2848,2847,5695,0.5986490249633789,0.03842857147498952
2851,2852,2851,5703,0.5992469787597656,0.038181597005524474
2855,2856,2855,5711,0.5998177528381348,0.037936209836125105
2859,2860,2859,5719,0.6002829074859619,0.03769239976539099
2863,2864,2863,5727,0.6007001399993896,0.03745015665797693
2867,2868,2867,5735,0.6020798683166504,0.03720947044174804
2871,2872,2871,5743,0.6027910709381104,0.03697033111189857
2875,2876,2875,5751,0.6032359600067139,0.0367327287255243
2879,2880,2879,5759,0.6037158966064453,0.0364966534053401
2883,2884,2883,5767,0.6041970252990723,0.036262095336248995
2887,2888,2887,5775,0.604701042175293,0.036029044767878195
2891,2892,2891,5783,0.6051549911499023,0.035797492010091546
2895,2896,2895,5791,0.6056721210479736,0.03556742743790119
2899,2900,2899,5799,0.6062109470367432,0.035338841485442876
2903,2904,2903,5807,0.6071667671203613,0.035111724650290825
2907,2908,2907,5815,0.6076469421386719,0.03488606748993428
2911,2912,2911,5823,0.6091780662536621,0.03466186062364821
2915,2916,2915,5831,0.610090970993042,0.034439094729508506
2919,2920,2919,5839,0.6107089519500732,0.03421776054660845
2923,2924,2923,5847,0.6113471984863281,0.03399784887382974
2927,2928,2927,5855,0.6119449138641357,0.033779350567914
2931,2932,2931,5863,0.6125190258026123,0.03356225654492072
2935,2936,2935,5871,0.6129469871520996,0.03334655778029662
2939,2940,2939,5879,0.6134328842163086,0.03313224530599332
2943,2944,2943,5887,0.6139109134674072,0.032919310212305
2947,2948,2947,5895,0.614569902420044,0.032707743646961426
2951,2952,2951,5903,0.6149909496307373,0.032497536814036894
2955,2956,2955,5911,0.6171848773956299,0.03228868097444443
2959,2960,2959,5919,0.6176609992980957,0.03208116744516638
2963,2964,2963,5927,0.6183860301971436,0.03187498759939177
2967,2968,2967,5935,0.618959903717041,0.03167013286556535
2971,2972,2971,5943,0.6194729804992676,0.031466594726454876
2975,2976,2975,5951,0.6199541091918945,0.03126436472076119
2979,2980,2979,5959,0.6207478046417236,0.03106343444088875
2983,2984,2983,5967,0.6217589378356934,0.03086379553292434
2987,2988,2987,5975,0.6225178241729736,0.030665439697670282
2991,2992,2991,5983,0.6231169700622559,0.030468358688576485
2995,2996,2995,5991,0.6236450672149658,0.030272544312178396
2999,3000,2999,5999,0.6244378089904785,0.03007798842722398
3003,3004,3003,6007,0.6255037784576416,0.029884682946028605
3007,3008,3007,6015,0.6260771751403809,0.029692619831879753
3011,3012,3011,6023,0.6266500949859619,0.029501791099887636
3015,3016,3015,6031,0.6271500587463379,0.029312188816285008
3019,3020,3019,6039,0.6277270317077637,0.029123805099251457
3023,3024,3023,6047,0.6282138824462891,0.028936632116472374
3027,3028,3027,6055,0.6287598609924316,0.028750662086294475
3031,3032,3031,6063,0.6291928291320801,0.028565887277522555
3035,3036,3035,6071,0.6299710273742676,0.028382300008508353
3039,3040,3039,6079,0.632314920425415,0.028199892646168383
3043,3044,3043,6087,0.632796049118042,0.028018657607587105
3047,3048,3047,6095,0.6333439350128174,0.02783858735817077
3051,3052,3051,6103,0.6338951587677002,0.027659674411922065
3055,3056,3055,6111,0.6344280242919922,0.02748191132973143
3059,3060,3059,6119,0.6350040435791016,0.02730529072280552
3063,3064,3063,6127,0.6356220245361328,0.027129805246703914
3067,3068,3067,6135,0.6361339092254639,0.026955447607347235
3071,3072,3071,6143,0.636652946472168,0.02678221055480195
3075,3076,3075,6151,0.6375110149383545,0.0266100868877643
3079,3080,3079,6159,0.6382489204406738,0.02643906944987764
3083,3084,3083,6167,0.6390807628631592,0.026269151131499406
3087,3088,3087,6175,0.6397778987884521,0.026100324868645282
3091,3092,3091,6183,0.6409168243408203,0.02593258364212947
3095,3096,3095,6191,0.642064094543457,0.025765920478698832
3099,3100,3099,6199,0.6425659656524658,0.025600328449551554
3103,3104,3103,6207,0.6433048248291016,0.025435800669815826
3107,3108,3107,6215,0.6439309120178223,0.025272330300364944
3111,3112,3111,6223,0.6447179317474365,0.025109910544599243
3115,3116,3115,6231,0.645845890045166,0.024948534649947333
3119,3120,3119,6239,0.6464889049530029,0.024788195907532652
3123,3124,3123,6247,0.6473848819732666,0.024628887651658157
3127,3128,3127,6255,0.6479299068450928,0.024470603259128584
3131,3132,3131,6263,0.6492359638214111,0.024313336149639847
3135,3136,3135,6271,0.6497268676757812,0.02415707978491894
3139,3140,3139,6279,0.6500940322875977,0.024001827668771864
3143,3144,3143,6287,0.6505889892578125,0.023847573346884497
3147,3148,3147,6295,0.6510100364685059,0.02369431040602178
3151,3152,3151,6303,0.6514301300048828,0.02354203247513928
3155,3156,3155,6311,0.6518309116363525,0.023390733222700667
3159,3160,3159,6319,0.6522419452667236,0.023240406359360158
3163,3164,3163,6327,0.6526648998260498,0.023091045634739456
3167,3168,3167,6335,0.6531538963317871,0.02294264484004006
3171,3172,3171,6343,0.6535539627075195,0.02279519780537801
3175,3176,3175,6351,0.6539490222930908,0.022648698400634305
3179,3180,3179,6359,0.6544759273529053,0.02250314053609398
3183,3184,3183,6367,0.6555459499359131,0.022358518159583944
3187,3188,3187,6375,0.6567349433898926,0.022214825259149886
3191,3192,3191,6383,0.6572320461273193,0.022072055860160873
3195,3196,3195,6391,0.6576318740844727,0.021930204028582687
3199,3200,3199,6399,0.658052921295166,0.02178926386583703
3203,3204,3203,6407,0.6585168838500977,0.021649229513020403
3207,3208,3207,6415,0.6589829921722412,0.021510095148855393
3211,3212,3211,6423,0.6594557762145996,0.021371854988457683
3215,3216,3215,6431,0.6599390506744385,0.021234503284420787
3219,3220,3219,6439,0.660689115524292,0.021098034327645905
3223,3224,3223,6447,0.6611208915710449,0.020962442443445594
3227,3228,3227,6455,0.6616799831390381,0.020827721995698892
3231,3232,3231,6463,0.6622538566589355,0.020693867383322066
3235,3236,3235,6471,0.6628341674804688,0.020560873041642194
3239,3240,3239,6479,0.6633551120758057,0.020428733441023465
3243,3244,3243,6487,0.6638062000274658,0.020297443088674205
3247,3248,3247,6495,0.6642000675201416,0.020166996525961767
3251,3252,3251,6503,0.6646559238433838,0.02003738833017532
3255,3256,3255,6511,0.6651418209075928,0.01990861311299273
3259,3260,3259,6519,0.6657488346099854,0.019780665520809638
3263,3264,3263,6527,0.6662890911102295,0.01965354023373255
3267,3268,3267,6535,0.6667947769165039,0.019527231967778225
3271,3272,3271,6543,0.6675307750701904,0.01940173547141502
3275,3276,3275,6551,0.6679999828338623,0.019277045527069575
3279,3280,3279,6559,0.6700019836425781,0.019153156951382637
3283,3284,3283,6567,0.671022891998291,0.019030064594086828
3287,3288,3287,6575,0.671666145324707,0.018907763337028795
3291,3292,3291,6583,0.6721539497375488,0.01878624809637969
3295,3296,3295,6591,0.6727759838104248,0.018665513820695794
3299,3300,3299,6599,0.6732268333435059,0.018545555489905323
3303,3304,3303,6607,0.6738300323486328,0.018426368117514143
3307,3308,3307,6615,0.674278974533081,0.018307946748278278
3311,3312,3311,6623,0.6750590801239014,0.01819028645870106
3315,3316,3315,6631,0.6755490303039551,0.018073382357973247
3319,3320,3319,6639,0.6761131286621094,0.017957229585572793
3323,3324,3323,6647,0.6767899990081787,0.017841823312740205
3327,3328,3327,6655,0.6784417629241943,0.017727158742102584
3331,3332,3331,6663,0.6788730621337891,0.017613231105934168
3335,3336,3335,6671,0.6796159744262695,0.017500035668522602
3339,3340,3339,6679,0.6802568435668945,0.017387567723924
3343,3344,3343,6687,0.6808819770812988,0.017275822596037358
3347,3348,3347,6695,0.6812949180603027,0.017164795639956276
3351,3352,3351,6703,0.6817519664764404,0.017054482239288155
3355,3356,3355,6711,0.6825368404388428,0.016944877808715095
3359,3360,3359,6719,0.6831448078155518,0.01683597779092987
3363,3364,3363,6727,0.6836230754852295,0.016727777659048728
3367,3368,3367,6735,0.686161994934082,0.016620272915029936
3371,3372,3371,6743,0.6869080066680908,0.016513459088974846
3375,3376,3375,6751,0.6900119781494141,0.01640733174103471
3379,3380,3379,6759,0.6909878253936768,0.016301886458880754
3383,3384,3383,6767,0.6915419101715088,0.016197118858445644
3387,3388,3387,6775,0.6921019554138184,0.016093024584877207
3391,3392,3391,6783,0.6926708221435547,0.015989599310551623
3395,3396,3395,6791,0.6931791305541992,0.015886838735642533
3399,3400,3399,6799,0.6936941146850586,0.015784738587995718
3403,3404,3403,6807,0.6942451000213623,0.015683294623472784
3407,3408,3407,6815,0.694861888885498,0.015582502624403907
3411,3412,3411,6823,0.6963968276977539,0.0154823584003159
3415,3416,3415,6831,0.6969079971313477,0.01538285778860801
3419,3420,3419,6839,0.697627067565918,0.015283996652110384
3423,3424,3423,6847,0.6981539726257324,0.015185770881564293
3427,3428,3427,6855,0.6987481117248535,0.01508817639285073
3431,3432,3431,6863,0.6992087364196777,0.014991209129188348
3435,3436,3435,6871,0.7012038230895996,0.014894865059181247
3439,3440,3439,6879,0.7017130851745605,0.014799140177223905
3443,3444,3443,6887,0.7021548748016357,0.014704030504834618
3447,3448,3447,6895,0.7026100158691406,0.01460953208666446
3451,3452,3451,6903,0.7032380104064941,0.014515640995193785
3455,3456,3455,6911,0.703711986541748,0.014422353326456416
3459,3460,3459,6919,0.7049829959869385,0.014329665202740897
3463,3464,3463,6927,0.7055509090423584,0.014237572770654025
3467,3468,3467,6935,0.7060787677764893,0.014146072201400796
3471,3472,3471,6943,0.7066619396209717,0.014055159691614427
3475,3476,3475,6951,0.7070958614349365,0.01396483146126848
3479,3480,3479,6959,0.7075691223144531,0.013875083755168636
3483,3484,3483,6967,0.7080228328704834,0.013785912842843825
3487,3488,3487,6975,0.7085118293762207,0.013697315017190072
3491,3492,3491,6983,0.7089860439300537,0.013609286594541185
3495,3496,3495,6991,0.7105848789215088,0.013521823915505946
3499,3500,3499,6999,0.7111551761627197,0.01343492334396674
3504,3505,3504,7009,0.7119128704071045,0.013327082592135234
3508,3509,3508,7017,0.7124509811401367,0.013241433589411999
3512,3513,3512,7025,0.7129108905792236,0.013156335037610585
3516,3517,3516,7033,0.7133510112762451,0.013071783399396493
3520,3521,3520,7041,0.7138779163360596,0.01298777515962672
3524,3525,3524,7049,0.7144670486450195,0.01290430682575357
3528,3529,3528,7057,0.7161300182342529,0.0128213749276769
3532,3533,3532,7065,0.7165710926055908,0.01273897601784292
3536,3537,3536,7073,0.717033863067627,0.012657106671222187
3540,3541,3540,7081,0.7177808284759521,0.012575763483597843
3544,3545,3544,7089,0.7184679508209229,0.012494943073796463
3548,3549,3548,7097,0.7197248935699463,0.012414642081698414
3552,3553,3552,7105,0.7206919193267822,0.012334857169007405
3556,3557,3556,7113,0.7213249206542969,0.012255585019213122
3560,3561,3560,7121,0.7221038341522217,0.01217682233677683
3564,3565,3564,7129,0.7229108810424805,0.012098565846944256
3568,3569,3568,7137,0.7235438823699951,0.012020812296659312
3572,3573,3572,7145,0.7242698669433594,0.011943558453519588
3576,3577,3576,7153,0.7248349189758301,0.011866801106023356
3580,3581,3580,7161,0.7253289222717285,0.011790537063112802
3584,3585,3584,7169,0.727341890335083,0.011714763154446169
3588,3589,3588,7177,0.7281241416931152,0.011639476229813404
3592,3593,3592,7185,0.7287662029266357,0.011564673159178586
3596,3597,3596,7193,0.7292490005493164,0.011490350832977933
3600,3601,3600,7201,0.7299680709838867,0.011416506161994855
3604,3605,3604,7209,0.7322380542755127,0.011343136075926945
3608,3609,3608,7217,0.7327959537506104,0.011270237524470053
3612,3613,3612,7225,0.7335889339447021,0.011197807477196165
3616,3617,3616,7233,0.734529972076416,0.01112584292325243
3620,3621,3620,7241,0.7351100444793701,0.011054340870728657
3624,3625,3624,7249,0.7356340885162354,0.010983298347454522
3628,3629,3628,7257,0.7365238666534424,0.010912712399348086
3632,3633,3632,7265,0.7371959686279297,0.010842580093029066
3636,3637,3636,7273,0.7381389141082764,0.010772898511971427
3640,3641,3640,7281,0.738853931427002,0.010703664759797275
3644,3645,3644,7289,0.7395150661468506,0.010634875958824189
3648,3649,3648,7297,0.7401609420776367,0.010566529248524964
3652,3653,3652,7305,0.7406740188598633,0.010498621788208139
3656,3657,3656,7313,0.7426700592041016,0.010431150754632367
3660,3661,3660,7321,0.7433550357818604,0.010364113342698203
3664,3665,3664,7329,0.7442779541015625,0.010297506765842844
3668,3669,3668,7337,0.7449090480804443,0.010231328255089716
3672,3673,3672,7345,0.7455258369445801,0.010165575059197879
3676,3677,3676,7353,0.7461569309234619,0.010100244444623999
3680,3681,3680,7361,0.7485458850860596,0.010035333695489162
3684,3685,3684,7369,0.7492649555206299,0.009970840113560458
3688,3689,3688,7377,0.7499759197235107,0.009906761017566419
3692,3693,3692,7385,0.7505021095275879,0.009843093743498057
3696,3697,3696,7393,0.7511188983917236,0.00977983564474486
3700,3701,3700,7401,0.7515549659729004,0.009716984091728876
3704,3705,3704,7409,0.7520408630371094,0.009654536471385065
3708,3709,3708,7417,0.7525439262390137,0.009592490187593434
3712,3713,3712,7425,0.7531759738922119,0.00953084266107071
3716,3717,3716,7433,0.7536699771881104,0.00946959132943168
3720,3721,3720,7441,0.7542591094970703,0.009408733645494273
3724,3725,3724,7449,0.7548210620880127,0.009348267080141803
3728,3729,3728,7457,0.7555711269378662,0.009288189119172412
3732,3733,3732,7465,0.7561159133911133,0.009228497265499293
3736,3737,3736,7473,0.7569839954376221,0.009169189037729343
3740,3741,3740,7481,0.7580358982086182,0.009110261969207587
3744,3745,3744,7489,0.7585630416870117,0.009051713611686194
3748,3749,3748,7497,0.7590789794921875,0.008993541529732267
3752,3753,3752,7505,0.7595088481903076,0.008935743306803795
3756,3757,3756,7513,0.7600197792053223,0.008878316538772638
3760,3761,3760,7521,0.7605648040771484,0.008821258838932663
3764,3765,3764,7529,0.761091947555542,0.008764567835068604
3768,3769,3768,7537,0.761512041091919,0.00870824117081753
3772,3773,3772,7545,0.7628319263458252,0.008652276504112584
3776,3777,3776,7553,0.7641189098358154,0.00859667150863377
3780,3781,3780,7561,0.7647089958190918,0.008541423872763793
3784,3785,3784,7569,0.7652449607849121,0.008486531299953788
3788,3789,3788,7577,0.765841007232666,0.008431991508293112
3792,3793,3792,7585,0.7663819789886475,0.008377802230095667
3796,3797,3796,7593,0.7681918144226074,0.008323961213127798
3800,3801,3800,7601,0.7694239616394043,0.008270466218584413
3804,3805,3804,7609,0.7716331481933594,0.008217315023094543
3808,3809,3808,7617,0.7724928855895996,0.008164505417070103
3812,3813,3812,7625,0.7732677459716797,0.008112035205259873
3816,3817,3816,7633,0.7738111019134521,0.008059902205682654
3820,3821,3820,7641,0.7744290828704834,0.008008104251572721
3824,3825,3824,7649,0.7753100395202637,0.007956639189853003
3828,3829,3828,7657,0.7769310474395752,0.007905504880851818
3832,3833,3832,7665,0.7784779071807861,0.007854699199204828
3836,3837,3836,7673,0.7800118923187256,0.007804220031991777
3840,3841,3840,7681,0.7807090282440186,0.00775406528145514
3844,3845,3844,7689,0.7812650203704834,0.007704232862523071
3848,3849,3848,7697,0.7839980125427246,0.007654720703623676
3852,3853,3852,7705,0.7845289707183838,0.007605526745976502
3856,3857,3856,7713,0.7852001190185547,0.007556648945126575
3860,3861,3860,7721,0.7859060764312744,0.007508085269063343
3864,3865,3864,7729,0.7882997989654541,0.007459833698578979
3868,3869,3868,7737,0.7891759872436523,0.007411892228319841
3872,3873,3872,7745,0.7898459434509277,0.007364258864886764
3876,3877,3876,7753,0.7903027534484863,0.007316931628308851
3880,3881,3880,7761,0.7910709381103516,0.007269908551165236
3884,3885,3884,7769,0.7918910980224609,0.007223187678916693
3888,3889,3888,7777,0.7950990200042725,0.007176767068469503
3892,3893,3892,7785,0.7962448596954346,0.007130644791356951
3896,3897,3896,7793,0.7968831062316895,0.007084818929144193
3900,3901,3900,7801,0.7989940643310547,0.007039287577013009
3904,3905,3904,7809,0.7994248867034912,0.006994048842453964
3908,3909,3908,7817,0.7999138832092285,0.00694910084471216
3912,3913,3912,7825,0.8003509044647217,0.006904441715593747
3916,3917,3916,7833,0.8008780479431152,0.006860069598086546
3920,3921,3920,7841,0.801367998123169,0.006815982647528443
3924,3925,3924,7849,0.8018548488616943,0.006772179031765711
3928,3929,3928,7857,0.8024020195007324,0.006728656929584978
3932,3933,3932,7865,0.8028628826141357,0.006685414531643812
3936,3937,3936,7873,0.8034100532531738,0.006642450040260595
3940,3941,3940,7881,0.8039331436157227,0.006599761669990163
3944,3945,3944,7889,0.804405927658081,0.006557347645148018
3948,3949,3948,7897,0.8049619197845459,0.006515206203413191
3952,3953,3952,7905,0.8055860996246338,0.006473335592256027
3956,3957,3956,7913,0.8061738014221191,0.006431734071895598
3960,3961,3960,7921,0.8068158626556396,0.006390399912153385
3964,3965,3964,7929,0.8073649406433105,0.006349331395672245
3968,3969,3968,7937,0.8079419136047363,0.006308526814406099
3972,3973,3972,7945,0.8085780143737793,0.006267984472169173
3976,3977,3976,7953,0.8091728687286377,0.0062277026837764616
3980,3981,3980,7961,0.8097398281097412,0.0061876797745790335
3984,3985,3984,7969,0.8102009296417236,0.006147914081388676
3988,3989,3988,7977,0.8107030391693115,0.006108403950004827
3992,3993,3992,7985,0.8123149871826172,0.0060691477384105475
3996,3997,3996,7993,0.8130199909210205,0.006030143815382422
4000,4001,4000,8001,0.8135027885437012,0.005991390558725566


==> plot_data/cournot-nash_equilibrium_problem_n100/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00021386146545410156,1624.447741208611
1,4,4,8,0.0006029605865478516,1332.3408024303455
2,8,8,16,0.0016217231750488281,946.088855039766
3,12,12,24,0.0023679733276367188,1048.4445827706136
4,14,14,28,0.0027930736541748047,700.8173612812878
5,18,18,36,0.0035610198974609375,374.0520303968597
6,20,20,40,0.0040547847747802734,363.80259197800035
7,26,26,52,0.005124807357788086,268.3075638288215
8,30,30,60,0.005939006805419922,254.22324001709478
9,36,36,72,0.006865978240966797,238.01529429042202
10,42,42,84,0.007664918899536133,209.92580578584443
11,50,50,100,0.008615970611572266,185.20198181997657
12,58,58,116,0.011673927307128906,184.68000690015896
13,66,66,132,0.01262974739074707,180.15955022740363
14,74,74,148,0.013566970825195312,175.92814377228046
15,82,82,164,0.014426946640014648,161.5227899951169
16,90,90,180,0.015360116958618164,159.6240688022446
17,96,96,192,0.01619577407836914,172.05406464160546
18,102,102,204,0.016971826553344727,156.9859077757749
19,110,110,220,0.018186092376708984,136.68764642330362
20,118,118,236,0.019320964813232422,135.42950475530338
21,126,126,252,0.02074289321899414,134.3453868940889
22,134,134,268,0.0220949649810791,125.23053712345713
23,142,142,284,0.02314591407775879,123.6218509878528
24,150,150,300,0.026421785354614258,122.3053119060085
25,158,158,316,0.027647972106933594,121.16241464860279
26,166,166,332,0.028783798217773438,120.16601216249201
27,174,174,348,0.030184030532836914,119.29269567003288
28,182,182,364,0.031610965728759766,118.52238313899163
29,190,190,380,0.03269696235656738,117.83792649180641
30,198,198,396,0.034149885177612305,117.22474500544486
31,206,206,412,0.03567910194396973,110.74853334384088
32,214,214,428,0.03830289840698242,109.97759630554185
33,222,222,444,0.039758920669555664,109.28987583764722
34,230,230,460,0.04269289970397949,108.67238186157404
35,238,238,476,0.04396867752075195,108.11395150423476
36,246,246,492,0.044943809509277344,107.60502473099753
37,254,254,508,0.045886993408203125,107.1374402288755
38,262,262,524,0.04764080047607422,106.70425172116786
39,270,270,540,0.04916787147521973,106.29956416908547
40,278,278,556,0.05014204978942871,105.91838882463065
41,286,286,572,0.05122494697570801,105.5565157951386
42,294,294,588,0.05233287811279297,105.21040261936378
43,302,302,604,0.05371689796447754,104.87707729971883
44,310,310,620,0.054892778396606445,104.55405425373888
45,318,318,636,0.056114912033081055,102.23428262310215
46,326,326,652,0.05926680564880371,97.85112401895425
47,334,334,668,0.060440778732299805,97.45519979669801
48,342,342,684,0.061548709869384766,97.08290543723847
49,350,350,700,0.062486886978149414,96.73050757860472
50,358,358,716,0.06377100944519043,93.21567618825011
51,366,366,732,0.06463384628295898,92.70678973892663
52,374,374,748,0.06580996513366699,92.32081952456242
53,382,382,764,0.06677103042602539,91.95833157814324
54,390,390,780,0.06774783134460449,91.61578097635804
55,398,398,796,0.06878399848937988,91.29010483392668
56,406,406,812,0.06981301307678223,90.97866254017157
57,414,414,828,0.07374787330627441,90.67918256321833
58,422,422,844,0.07482099533081055,90.38971528145184
59,430,430,860,0.07585787773132324,90.10859129899255
60,438,438,876,0.07684683799743652,89.83438471528343
61,446,446,892,0.07786774635314941,89.56588084316704
62,454,454,908,0.07880496978759766,89.30204790120438
63,462,462,924,0.08016586303710938,89.04201224119419
64,470,470,940,0.08130478858947754,88.78503670876194
65,478,478,956,0.0824117660522461,88.53050177187912
66,486,486,972,0.08352375030517578,88.27788908804094
67,494,494,988,0.08450698852539062,88.0267672149437
68,502,502,1004,0.0889427661895752,87.77677920136175
69,510,510,1020,0.08992290496826172,87.52763182429098
70,518,518,1036,0.0908968448638916,87.27908626526333
71,526,526,1052,0.09190201759338379,87.03095004297649
72,534,534,1068,0.09295082092285156,86.7830700412778
73,542,542,1084,0.09395289421081543,86.53532649103141
74,550,550,1100,0.09501194953918457,86.28762778178728
75,558,558,1116,0.09595775604248047,86.03990599464616
76,566,566,1132,0.09701299667358398,85.79211306128495
77,574,574,1148,0.09802079200744629,85.54421746620257
78,582,582,1164,0.09932804107666016,81.61868393807545
79,590,590,1180,0.10084271430969238,80.67673255421042
80,598,598,1196,0.10206079483032227,80.42974323347462
81,606,606,1212,0.10344195365905762,80.18723339704606
82,614,614,1228,0.10445380210876465,76.51970647608681
83,622,622,1244,0.10542488098144531,76.23100554867823
84,630,630,1260,0.10632205009460449,75.95398453689943
85,638,638,1276,0.10727787017822266,75.687155082936
86,646,646,1292,0.1082918643951416,70.80381930479876
87,654,654,1308,0.10928583145141602,70.42952135489813
88,662,662,1324,0.11028003692626953,70.07673564499059
89,668,668,1336,0.11113572120666504,63.470895566119786
90,676,676,1352,0.11206889152526855,56.15538941258864
91,684,684,1368,0.11428189277648926,40.663914927846946
92,692,692,1384,0.11569786071777344,40.538488590865356
93,700,700,1400,0.11683988571166992,40.4134105483917
94,706,706,1412,0.11791491508483887,36.671129081323635
95,714,714,1428,0.11887288093566895,36.560038629947364
96,722,722,1444,0.11977577209472656,36.44919563530819
97,730,730,1460,0.12091302871704102,36.33860206176196
98,738,738,1476,0.12218189239501953,36.22825996199132
99,746,746,1492,0.12328100204467773,36.11817145069235
100,754,754,1508,0.12441611289978027,36.00833868161398
101,762,762,1524,0.12558293342590332,35.898763827561915
102,770,770,1540,0.12816286087036133,31.904821760967362
103,778,778,1556,0.12942290306091309,29.407113843660866
104,786,786,1572,0.1304337978363037,29.247468350489108
105,794,794,1588,0.13149094581604004,29.09331527544887
106,802,802,1604,0.13263583183288574,28.944275274016324
107,810,810,1620,0.13396000862121582,28.799996675279427
108,818,818,1636,0.13477492332458496,28.660153541506467
109,826,826,1652,0.136185884475708,28.524443845986042
110,834,834,1668,0.13741803169250488,28.392587764777122
111,842,842,1684,0.13862204551696777,28.264326077731372
112,850,850,1700,0.1398627758026123,28.139418673911596
113,858,858,1716,0.14254093170166016,28.017643156417325
114,866,866,1732,0.1444697380065918,27.898793541570505
115,874,874,1748,0.14556598663330078,27.782679047391927
116,882,882,1764,0.14654183387756348,27.669122966404338
117,890,890,1780,0.1476140022277832,27.55796161785389
118,898,898,1796,0.14864683151245117,27.449043374553664
119,906,906,1812,0.14955496788024902,27.342227759759172
120,914,914,1828,0.15057587623596191,27.23738460961745
121,922,922,1844,0.1515820026397705,27.134393296910126
122,930,930,1860,0.1524968147277832,26.543020684393106
123,938,938,1876,0.1535639762878418,25.397633339919985
124,946,946,1892,0.15552806854248047,25.324827743720622
125,954,954,1908,0.15741491317749023,25.252188383582858
126,960,960,1920,0.15827679634094238,22.533039587678186
127,968,968,1936,0.15924286842346191,21.60176690056621
128,976,976,1952,0.16016483306884766,21.53333302406177
129,984,984,1968,0.1618208885192871,21.46582382585808
130,990,990,1980,0.1624767780303955,19.474369846681316
131,998,998,1996,0.16360688209533691,19.41451990043444
132,1006,1006,2012,0.16463279724121094,19.355361743953548
133,1014,1014,2028,0.16561174392700195,19.29685151762185
134,1022,1022,2044,0.1666257381439209,19.238948494712307
135,1030,1030,2060,0.16760683059692383,19.18161487018163
136,1038,1038,2076,0.17075276374816895,19.12481556287217
137,1046,1046,2092,0.17194199562072754,19.06851803023941
138,1054,1054,2108,0.17287468910217285,19.01269209499636
139,1062,1062,2124,0.17378902435302734,18.957309782882465
140,1070,1070,2140,0.17468690872192383,18.902345170983924
141,1078,1078,2156,0.1759018898010254,18.847774245906496
142,1086,1086,2172,0.17685198783874512,18.79357477125626
143,1094,1094,2188,0.17791295051574707,18.739726163832096
144,1102,1102,2204,0.17894983291625977,17.766839325614892
145,1110,1110,2220,0.17995786666870117,17.700204933700064
146,1118,1118,2236,0.18105387687683105,17.634913329941103
147,1124,1124,2248,0.181898832321167,15.989688636010285
148,1132,1132,2264,0.1848609447479248,15.932528680624022
149,1140,1140,2280,0.18578577041625977,15.876404825945297
150,1148,1148,2296,0.18705081939697266,15.82126159580744
151,1156,1156,2312,0.1882917881011963,15.767046618202734
152,1164,1164,2328,0.18975186347961426,15.713710463477582
153,1172,1172,2344,0.19078993797302246,15.66120648981694
154,1180,1180,2360,0.19178295135498047,15.609490695852445
155,1188,1188,2376,0.19282889366149902,15.558521580154824
156,1196,1196,2392,0.1942129135131836,15.244753744132487
157,1204,1204,2408,0.19568586349487305,14.858313134310988
158,1212,1212,2424,0.19683384895324707,14.794897180790398
159,1220,1220,2440,0.19951391220092773,14.732901497917437
160,1228,1228,2456,0.20061492919921875,14.6722595674365
161,1236,1236,2472,0.20145702362060547,14.612907930399308
162,1244,1244,2488,0.2023320198059082,14.554786064888798
163,1252,1252,2504,0.20360994338989258,14.49783626704941
164,1260,1260,2520,0.20463895797729492,14.442003535516818
165,1268,1268,2536,0.2056899070739746,14.387235459241605
166,1276,1276,2552,0.20665884017944336,14.333482108759128
167,1284,1284,2568,0.20777201652526855,14.2806959308985
168,1292,1292,2584,0.2087419033050537,14.228831646925356
169,1300,1300,2600,0.2096998691558838,14.17784615410652
170,1308,1308,2616,0.21294689178466797,14.127698430647307
171,1316,1316,2632,0.21385407447814941,14.078349444014824
172,1324,1324,2648,0.21467876434326172,14.02976206253219
173,1332,1332,2664,0.21554279327392578,13.981900970249065
174,1340,1340,2680,0.21689605712890625,13.934732585002626
175,1348,1348,2696,0.21789073944091797,13.888224979616997
176,1356,1356,2712,0.218919038772583,5.437464608419467
177,1364,1364,2728,0.22005295753479004,5.392753021209952
178,1372,1372,2744,0.22152090072631836,5.349253479943514
179,1376,1376,2752,0.2223367691040039,3.714983969073515
180,1382,1382,2764,0.22327303886413574,3.3543789734725236
181,1390,1390,2780,0.226456880569458,3.3288197083214026
182,1398,1398,2796,0.22766685485839844,3.3039336718739065
183,1406,1406,2812,0.2286369800567627,3.2796976570921528
184,1414,1414,2828,0.22968673706054688,3.256089147544076
185,1422,1422,2844,0.23085498809814453,3.2330863050680736
186,1430,1430,2860,0.2316598892211914,3.210667957221446
187,1438,1438,2876,0.23255085945129395,3.1888135845131336
188,1446,1446,2892,0.23352670669555664,3.1675033074614922
189,1454,1454,2908,0.23459100723266602,3.146717873488265
190,1462,1462,2924,0.23572897911071777,3.126438643674987
191,1470,1470,2940,0.23702573776245117,3.106647579413797
192,1478,1478,2956,0.24006390571594238,3.087327228963184
193,1486,1486,2972,0.24122285842895508,3.068460713941889
194,1494,1494,2988,0.24216890335083008,3.0500317157858996
195,1502,1502,3004,0.24313783645629883,3.032024462182306
196,1510,1510,3020,0.2445969581604004,3.014423713511689
197,1518,1518,3036,0.24541592597961426,2.9972147493187213
198,1526,1526,3052,0.24643182754516602,2.9803833548283967
199,1534,1534,3068,0.24734187126159668,2.963915807532271
200,1542,1542,3084,0.24834585189819336,2.9477988638615127
201,1550,1550,3100,0.24938082695007324,2.9320197459657855
202,1558,1558,3116,0.2503387928009033,2.847828029209055
203,1566,1566,3132,0.2535848617553711,2.0434278844766616
204,1574,1574,3148,0.25474095344543457,2.0372702912400027
205,1580,1580,3160,0.25556492805480957,2.152216264074068
206,1586,1586,3172,0.25632786750793457,1.6770096355540969
207,1592,1592,3184,0.2570807933807373,1.5215889967271905
208,1600,1600,3200,0.2581768035888672,1.5170080756141235
209,1608,1608,3216,0.25912976264953613,1.5124411481929645
210,1616,1616,3232,0.26004791259765625,1.507888166609641
211,1624,1624,3248,0.26097989082336426,1.5033490833540804
212,1632,1632,3264,0.26186084747314453,1.4988238512573613
213,1640,1640,3280,0.2627279758453369,1.4943124234796301
214,1648,1648,3296,0.26528072357177734,0.8990544807698934
215,1656,1656,3312,0.26650404930114746,0.8898702227110277
216,1664,1664,3328,0.26733875274658203,0.8808510195718355
217,1666,1666,3332,0.26769590377807617,0.0033170330226337088
218,1668,1668,3336,0.2680659294128418,3.1422033963378556e-05
219,1670,1670,3340,0.2684199810028076,3.1422033963378556e-12


==> plot_data/cournot-nash_equilibrium_problem_n100/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00014495849609375,1624.447741208611
1,4,4,8,0.0005040168762207031,1332.3408024303455
2,6,6,12,0.0011529922485351562,713.8531607135735
3,8,8,16,0.0016009807586669922,580.7956376294903
4,10,10,20,0.0020999908447265625,472.9563599805472
5,12,12,24,0.0025238990783691406,345.1253851566417
6,14,14,28,0.0029449462890625,296.18461714048766
7,16,16,32,0.003381967544555664,286.75853000995244
8,18,18,36,0.003888845443725586,271.0587803845099
9,20,20,40,0.0043277740478515625,272.01279104591094
10,22,22,44,0.004740715026855469,261.96009757850805
11,26,26,52,0.0070667266845703125,267.08261112874806
12,30,30,60,0.007916927337646484,239.37750354060705
13,32,32,64,0.008332014083862305,227.78929663502146
14,36,36,72,0.008916854858398438,223.43164777229262
15,38,38,76,0.00931692123413086,211.12579165307358
16,42,42,84,0.009906768798828125,204.72315180456658
17,44,44,88,0.010340690612792969,203.83061653575888
18,48,48,96,0.01089787483215332,207.06792554388173
19,52,52,104,0.011629104614257812,193.5604859578759
20,56,56,112,0.012386798858642578,182.3675935801982
21,60,60,120,0.01297307014465332,181.22747019150304
22,62,62,124,0.01354074478149414,178.4466408944507
23,64,64,128,0.014073848724365234,169.08748702938055
24,68,68,136,0.015002727508544922,141.23441710762054
25,74,74,148,0.016119956970214844,139.72880791237182
26,78,78,156,0.016873836517333984,135.68485137827224
27,84,84,168,0.017760038375854492,137.2493434272932
28,90,90,180,0.018580913543701172,132.2932287474023
29,96,96,192,0.02175593376159668,121.78411857856216
30,100,100,200,0.022783994674682617,117.08921062562699
31,108,108,216,0.023813724517822266,116.64547294961959
32,116,116,232,0.024866104125976562,109.68431251541442
33,124,124,248,0.02578878402709961,109.10149458161898
34,132,132,264,0.026677846908569336,108.5718387388363
35,140,140,280,0.02766275405883789,108.08663828298728
36,148,148,296,0.028599023818969727,107.63847485916313
37,156,156,312,0.029561758041381836,107.221046328338
38,164,164,328,0.030426740646362305,106.82901404553975
39,172,172,344,0.03135991096496582,106.4578682913725
40,180,180,360,0.032472848892211914,106.10381038979901
41,188,188,376,0.0334169864654541,105.76364995521601
42,196,196,392,0.0366368293762207,105.43471570688006
43,204,204,408,0.03758096694946289,105.11477834144542
44,212,212,424,0.03854179382324219,104.80198404367745
45,220,220,440,0.039502859115600586,104.49479732562725
46,228,228,456,0.04122805595397949,99.41303150256806
47,236,236,472,0.04205894470214844,97.61152377086131
48,244,244,488,0.04306483268737793,97.24826593326785
49,252,252,504,0.043962717056274414,96.90331476916404
50,260,260,520,0.044882774353027344,96.57370224287219
51,268,268,536,0.04585981369018555,92.88463722710284
52,276,276,552,0.04675889015197754,92.4998202727144
53,284,284,568,0.04999971389770508,92.13823293375128
54,292,292,584,0.051030874252319336,91.79636353775416
55,300,300,600,0.05201101303100586,91.47117846770927
56,308,308,616,0.05297589302062988,91.16006281198537
57,316,316,632,0.0538177490234375,90.86076755390683
58,324,324,648,0.054718971252441406,90.57136275834229
59,332,332,664,0.0555877685546875,90.29019621141042
60,340,340,680,0.05664777755737305,90.01585698377365
61,348,348,696,0.05767488479614258,89.74714341307543
62,356,356,712,0.05870485305786133,89.48303503291612
63,364,364,728,0.0598149299621582,89.22266801124472
64,372,372,744,0.06085991859436035,88.96531369815962
65,380,380,760,0.06462287902832031,88.71035992004633
66,388,388,776,0.06578469276428223,88.45729469288023
67,396,396,792,0.06694769859313965,88.20569206151536
68,404,404,808,0.06808590888977051,87.95519980352847
69,412,412,824,0.0694427490234375,87.7055287653946
70,420,420,840,0.07068181037902832,87.45644362548921
71,428,428,856,0.07199478149414062,87.20775490250672
72,436,436,872,0.07329583168029785,86.95931204960348
73,444,444,888,0.07441878318786621,86.71099749396791
74,452,452,904,0.07546496391296387,86.46272149877137
75,460,460,920,0.07814288139343262,86.21441773979113
76,468,468,936,0.07940101623535156,85.96603950251263
77,476,476,952,0.08030104637145996,85.71755641745646
78,484,484,968,0.08118772506713867,85.46895166197719
79,492,492,984,0.08209681510925293,80.8368079825627
80,500,500,1000,0.08301496505737305,80.5875082096376
81,508,508,1016,0.0839238166809082,80.34301931997655
82,516,516,1032,0.0851137638092041,77.6499160931704
83,524,524,1048,0.08618807792663574,76.40787490213843
84,532,532,1064,0.08715295791625977,76.12476490288904
85,540,540,1080,0.08823609352111816,75.85261587916605
86,548,548,1096,0.08927273750305176,71.73352556344149
87,556,556,1112,0.0931546688079834,70.65490064540349
88,564,564,1128,0.09436488151550293,70.29007432445832
89,572,572,1144,0.0953378677368164,69.94577275450258
90,578,578,1156,0.09614896774291992,63.438762653579275
91,586,586,1172,0.09713482856750488,59.46024281122072
92,594,594,1188,0.09794998168945312,40.708254753766724
93,602,602,1204,0.09905385971069336,40.58110258355566
94,608,608,1216,0.09996175765991211,39.91816310167587
95,616,616,1232,0.10110187530517578,36.7459896035863
96,624,624,1248,0.10206794738769531,36.63211734074269
97,632,632,1264,0.10304784774780273,36.51860170012257
98,640,640,1280,0.10594677925109863,36.40544186988257
99,648,648,1296,0.10727882385253906,36.29263702362454
100,656,656,1312,0.10834407806396484,36.180186321245856
101,664,664,1328,0.10940694808959961,36.068088909759254
102,672,672,1344,0.11026573181152344,35.9563439240612
103,680,680,1360,0.11111187934875488,30.978291652014498
104,688,688,1376,0.11194705963134766,29.542917657600896
105,696,696,1392,0.11286282539367676,29.3748577477875
106,704,704,1408,0.11386275291442871,29.212903153186158
107,712,712,1424,0.1150357723236084,29.0566297942741
108,720,720,1440,0.11631178855895996,28.905644359247834
109,728,728,1456,0.11735773086547852,28.75958218267534
110,736,736,1472,0.11834979057312012,28.618105247774853
111,744,744,1488,0.12122964859008789,28.48090030869356
112,752,752,1504,0.12230086326599121,28.347677128658788
113,760,760,1520,0.12338590621948242,28.218166829512505
114,768,768,1536,0.12426495552062988,28.092120347885235
115,776,776,1552,0.12512469291687012,27.96930699306927
116,784,784,1568,0.12594985961914062,27.849513101616424
117,792,792,1584,0.12677502632141113,27.732540783591404
118,800,800,1600,0.12761378288269043,27.618206755474603
119,808,808,1616,0.12854504585266113,27.506341254793153
120,816,816,1632,0.1295018196105957,27.396787031621002
121,824,824,1648,0.1304187774658203,27.28939841230653
122,832,832,1664,0.13130807876586914,27.18404043084
123,840,840,1680,0.13421392440795898,25.51872476467503
124,848,848,1696,0.13526201248168945,25.4358332541519
125,856,856,1712,0.136124849319458,25.36243784545523
126,862,862,1724,0.1367969512939453,26.66623928642606
127,870,870,1740,0.13768386840820312,21.70555709986321
128,878,878,1756,0.13864970207214355,21.63877079167312
129,886,886,1772,0.13949179649353027,21.572754026080112
130,892,892,1784,0.14021086692810059,19.593935732281786
131,900,900,1800,0.14110898971557617,19.53520235606641
132,908,908,1816,0.14206290245056152,19.4770423335768
133,916,916,1832,0.14301085472106934,19.41942039450476
134,924,924,1848,0.1439647674560547,19.362303822287352
135,932,932,1864,0.14478111267089844,19.30566227959125
136,940,940,1880,0.1478438377380371,19.249467645052697
137,948,948,1896,0.14878582954406738,19.19369386061461
138,956,956,1912,0.14974594116210938,19.138316788813214
139,964,964,1928,0.1506187915802002,19.083314079410176
140,972,972,1944,0.15192699432373047,19.028665044811667
141,980,980,1960,0.15284490585327148,18.97435054373976
142,988,988,1976,0.15368986129760742,18.920352872604397
143,996,996,1992,0.15462994575500488,18.866655664153818
144,1004,1004,2008,0.15548181533813477,18.813243792896202
145,1012,1012,2024,0.15636682510375977,18.13613492823198
146,1020,1020,2040,0.15721869468688965,17.754992347750786
147,1028,1028,2056,0.16012072563171387,17.69112587124343
148,1036,1036,2072,0.16113877296447754,17.62843332503099
149,1042,1042,2084,0.16187691688537598,15.989494600257544
150,1050,1050,2100,0.16269373893737793,15.934424566054227
151,1058,1058,2116,0.16384387016296387,15.880260296466659
152,1066,1066,2132,0.16460394859313965,15.82695365488675
153,1074,1074,2148,0.1656198501586914,15.77445922595541
154,1082,1082,2164,0.1666579246520996,15.722734171093464
155,1090,1090,2180,0.1676008701324463,15.671738090856987
156,1098,1098,2196,0.1685628890991211,15.621432893847173
157,1106,1106,2212,0.16958093643188477,15.571782671967021
158,1114,1114,2228,0.17239093780517578,15.522753581783501
159,1122,1122,2244,0.17357277870178223,15.47431373174751
160,1130,1130,2260,0.1744828224182129,14.803440647435467
161,1138,1138,2276,0.1753687858581543,14.742600306767724
162,1146,1146,2292,0.17625093460083008,14.683051696305899
163,1154,1154,2308,0.17728281021118164,14.624734223092688
164,1162,1162,2324,0.17814874649047852,14.567590116949127
165,1170,1170,2340,0.1790318489074707,14.511564314598488
166,1178,1178,2356,0.17998003959655762,14.456604347190034
167,1186,1186,2372,0.18105483055114746,14.402660231307172
168,1194,1194,2388,0.18198680877685547,14.349684363411825
169,1202,1202,2404,0.1829240322113037,14.297631417748935
170,1210,1210,2420,0.18568181991577148,14.246458247691615
171,1218,1218,2436,0.18658876419067383,14.1961237904757
172,1226,1226,2452,0.18739986419677734,14.146588975316254
173,1234,1234,2468,0.18819308280944824,14.097816634831128
174,1242,1242,2484,0.18909382820129395,14.049771419732998
175,1250,1250,2500,0.1900317668914795,14.002419716746106
176,1258,1258,2516,0.1908280849456787,13.955729569636015
177,1266,1266,2532,0.1916790008544922,13.90967060334317
178,1274,1274,2548,0.1925487518310547,13.757841323475837
179,1282,1282,2564,0.19343996047973633,5.473275180549204
180,1290,1290,2580,0.19427990913391113,5.426734523640236
181,1298,1298,2596,0.19516897201538086,5.3814695541161175
182,1302,1302,2604,0.19806170463562012,3.7370558806611074
183,1308,1308,2616,0.19887375831604004,3.373421906000708
184,1316,1316,2632,0.1997509002685547,3.3468576003285033
185,1324,1324,2648,0.2005786895751953,3.3210025692849774
186,1332,1332,2664,0.20135784149169922,3.2958325774071136
187,1340,1340,2680,0.20276093482971191,3.271324094985925
188,1348,1348,2696,0.20365595817565918,3.2474542862688374
189,1356,1356,2712,0.20460176467895508,3.2242009973996955
190,1364,1364,2728,0.20545578002929688,3.2015427441223867
191,1372,1372,2744,0.20645594596862793,3.17945869926108
192,1380,1380,2760,0.207413911819458,3.1579286800051034
193,1388,1388,2776,0.20830988883972168,3.1369331350164176
194,1396,1396,2792,0.2114109992980957,3.116453131389013
195,1404,1404,2808,0.21222400665283203,3.096470341473579
196,1412,1412,2824,0.21297693252563477,3.076967029601341
197,1420,1420,2840,0.21384596824645996,3.0579260387288283
198,1428,1428,2856,0.21483492851257324,3.039330777020514
199,1436,1436,2872,0.21562480926513672,3.02116520440053
200,1444,1444,2888,0.21650481224060059,3.0034138190949027
201,1452,1452,2904,0.21746397018432617,2.9860616441816035
202,1460,1460,2920,0.21856379508972168,2.9690942141764527
203,1468,1468,2936,0.21956396102905273,2.952497561669348
204,1476,1476,2952,0.22048473358154297,2.9362582040381207
205,1484,1484,2968,0.22143101692199707,2.0517737196816634
206,1492,1492,2984,0.2245008945465088,2.0392196306491015
207,1500,1500,3000,0.22542285919189453,2.033063273813949
208,1508,1508,3016,0.22626471519470215,2.02692611541341
209,1514,1514,3028,0.22694993019104004,1.8393627654299343
210,1520,1520,3040,0.2282397747039795,1.6687717838988827
211,1526,1526,3052,0.2291889190673828,1.5140026391506165
212,1534,1534,3068,0.23032808303833008,1.5094361032287131
213,1542,1542,3084,0.2312939167022705,1.5048837522719285
214,1550,1550,3100,0.23224186897277832,1.5003455294015655
215,1558,1558,3116,0.23310089111328125,1.4958213784182588
216,1566,1566,3132,0.2339777946472168,1.0263082211184575
217,1574,1574,3148,0.2371828556060791,0.8986612295500099
218,1582,1582,3164,0.23815488815307617,0.8893968483222792
219,1590,1590,3180,0.2391507625579834,0.8802987156344021
220,1592,1592,3184,0.23961091041564941,0.003972305643875937
221,1594,1594,3188,0.24010896682739258,2.679901527966293e-05
222,1596,1596,3192,0.24056792259216309,3.1422033963378556e-12


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.006479978561401367,7526.915480382486
1001,2004,1002,3006,3.5441129207611084,16.607310482411776
2002,4006,2003,6009,6.740976810455322,8.44604186183642
3003,6008,3004,9012,10.131140947341919,5.384187945803205
4004,8010,4005,12015,13.564121961593628,3.953212580012405
5005,10012,5006,15018,16.912140130996704,3.1670385358302156
6006,12014,6007,18021,20.323441982269287,2.6660191487208067
7007,14016,7008,21024,24.03473997116089,2.322857366572862
8008,16018,8009,24027,27.344194173812866,2.0735852000416344
9009,18020,9010,27030,30.581588983535767,1.8774693972100067
10010,20022,10011,30033,33.7753050327301,1.7188494503752736
11011,22024,11012,33036,37.083268880844116,1.582673018288915
12012,24026,12013,36039,40.37950587272644,1.471707319997222
13013,26028,13014,39042,43.583324909210205,1.3744369879677834
14014,28030,14015,42045,46.76132893562317,1.2886299983183562
15015,30032,15016,45048,49.984355211257935,1.2140860543386225
16016,32034,16017,48051,53.22905397415161,1.1476694552820845
17017,34036,17018,51054,56.370681047439575,1.088071876201866
18018,36038,18019,54057,59.64098405838013,1.0332849611713755
19019,38040,19020,57060,62.88238787651062,0.9833981326173671
20020,40042,20021,60063,66.11721611022949,0.939032640593723
21021,42044,21022,63066,69.34110999107361,0.8974108840684494
22022,44046,22023,66069,72.53726387023926,0.8600530857729609
23023,46048,23024,69072,75.76485824584961,0.8258471587159875
24024,48050,24025,72075,79.35508894920349,0.7934561818037764
25025,50052,25026,75078,82.54595994949341,0.7642925602212927
26026,52054,26027,78081,85.69618797302246,0.7367598122000345
27027,54056,27028,81084,88.8949499130249,0.7111625554553029
28028,56058,28029,84087,92.06171607971191,0.6871552191914816
29029,58060,29030,87090,95.23148393630981,0.6645381343878398
30030,60062,30031,90093,98.5493950843811,0.6432413014699705
31031,62064,31032,93096,101.71502685546875,0.6238021842946182
32032,64066,32033,96099,104.91014289855957,0.605301730125575
33033,66068,33034,99102,108.10603904724121,0.5878315822774312
34034,68070,34035,102105,111.3280041217804,0.571435268062487
35035,70072,35036,105108,114.57196593284607,0.5557054523924307
36036,72074,36037,108111,117.90704202651978,0.5408851722713734
37037,74076,37038,111114,121.14691686630249,0.5269430078697042
38038,76078,38039,114117,124.3833589553833,0.5132465510723705
39039,78080,39040,117120,127.63018488883972,0.5003511031427479
40040,80082,40041,120123,130.8636269569397,0.48800866575220425
41041,82084,41042,123126,134.1103868484497,0.4766423442415544
42042,84086,42043,126129,137.3918080329895,0.4654066780785797
43043,86088,43044,129132,140.55379104614258,0.4548106745551195
44044,88090,44045,132135,144.5558421611786,0.4446414657140849
45045,90092,45046,135138,148.3430380821228,0.4348921094715479
46046,92094,46047,138141,151.7042691707611,0.425505028826592
47047,94096,47048,141144,155.1401391029358,0.4165199768503953
48048,96098,48049,144147,158.46228504180908,0.4079241794333939
49049,98100,49050,147150,161.7031590938568,0.39948473689764796
50050,100102,50051,150153,165.0432939529419,0.39134187462150294
51051,102104,51052,153156,168.34076809883118,0.3836366670020652
52052,104106,52053,156159,171.66346406936646,0.3764342811409733
53053,106108,53054,159162,175.01661014556885,0.36919396650773706
54054,108110,54055,162165,178.28645205497742,0.36230758592137136
55055,110112,55056,165168,181.50732588768005,0.3556901604988525
56056,112114,56057,168171,184.76968097686768,0.3492317360396555
57057,114116,57058,171174,188.0262668132782,0.34296508188526786
58058,116118,58059,174177,191.27908205986023,0.33697372967253614
59059,118120,59060,177180,194.50817584991455,0.3313018955868756
60060,120122,60061,180183,197.73727703094482,0.3256641824846156
61061,122124,61062,183186,200.96349906921387,0.32019864118410624
62062,124126,62063,186189,204.2221441268921,0.3148136218151194
63063,126128,63064,189192,207.53573894500732,0.30967236786091235
64064,128130,64065,192195,210.956472158432,0.3046702432202437
65065,130132,65066,195198,214.305321931839,0.2998149078212009
66066,132134,66067,198201,217.58343291282654,0.29516451411655
67067,134136,67068,201204,220.82792711257935,0.29064668407045247
68068,136138,68069,204207,224.07446718215942,0.28621519477565016
69069,138140,69070,207210,227.49353289604187,0.2819115918082389
70070,140142,70071,210213,230.83379006385803,0.27779908519005403
71071,142144,71072,213216,234.12945580482483,0.27384245153007214
72072,144146,72073,216219,237.40497207641602,0.26989217328082304
73073,146148,73074,219222,240.65365505218506,0.2660547712475818
74074,148150,74075,222225,245.24590301513672,0.262335357894699
75075,150152,75076,225228,249.40277409553528,0.25864909180018003
76076,152154,76077,228231,252.74715280532837,0.2550970652282558
77077,154156,77078,231234,257.4114010334015,0.2516935070234467
78078,156158,78079,234237,263.5583050251007,0.24833497777217417
79079,158160,79080,237240,268.9645400047302,0.2451368044330593
80080,160162,80081,240243,273.8991701602936,0.24199128226064204
81081,162164,81082,243246,279.00500416755676,0.23894381176251045
82082,164166,82083,246249,283.99812293052673,0.23594794828204613
83083,166168,83084,249252,288.9537580013275,0.23296090906842437
84084,168170,84085,252255,294.17182993888855,0.23004385963031382
85085,170172,85086,255258,299.3436770439148,0.2272559894117876
86086,172174,86087,258261,304.46783423423767,0.22452971490747586
87087,174176,87088,261264,309.3200240135193,0.22186004084687738
88088,176178,88089,264267,313.90145993232727,0.21924445435251982
89089,178180,89090,267270,318.95341396331787,0.21668076603782538
90090,180182,90091,270273,324.4294159412384,0.21416691177546454
91091,182184,91092,273276,329.07114696502686,0.21166160795291944
92092,184186,92093,276279,334.1726059913635,0.20914881158751086
93093,186188,93094,279282,339.33644914627075,0.20667534263156995
94094,188190,94095,282285,345.2051479816437,0.20424204975097382
95095,190192,95096,285288,350.3596920967102,0.20184840537331183
96096,192194,96097,288291,355.2950921058655,0.19949390214969753
97097,194196,97098,291294,361.2078421115875,0.19717854433110915
98098,196198,98099,294297,366.43927001953125,0.19494487212250533
99099,198200,99100,297300,371.0514039993286,0.1927948216034565
100100,200202,100101,300303,375.6520059108734,0.19065856019915373
101101,202204,101102,303306,380.68790197372437,0.18859509082176373
102102,204206,102103,306309,385.72709703445435,0.18659051755639666
103103,206208,103104,309312,391.30790305137634,0.18460732131643454
104104,208210,104105,312315,395.605299949646,0.18260361287866544
105105,210212,105106,315318,400.6962938308716,0.18068051412956265
106106,212214,106107,318321,405.32034516334534,0.17880895168309507
107107,214216,107108,321324,409.469938993454,0.17694370840217744
108108,216218,108109,324327,414.1092028617859,0.17512045776493324
109109,218220,109110,327330,418.7154178619385,0.17335131644176727
110110,220222,110111,330333,423.14688205718994,0.17159818137224647
111111,222224,111112,333336,427.8711919784546,0.16987975322990678
112112,224226,112113,336339,433.5740427970886,0.16822902301464637
113113,226228,113114,339342,438.4849100112915,0.16659121578049962
114114,228230,114115,342345,442.56773495674133,0.1650106808192504
115115,230232,115116,345348,446.56058287620544,0.16341408167863847
116116,232234,116117,348351,451.53994703292847,0.16187666171208548
117117,234236,117118,351354,456.75928497314453,0.1603578229460254
118118,236238,118119,354357,461.74205589294434,0.15886139585563797
119119,238240,119120,357360,466.11524415016174,0.15735733398105367
120120,240242,120121,360363,470.6618571281433,0.15587040044556488
121121,242244,121122,363366,475.3424069881439,0.1544428653724026
122122,244246,122123,366369,479.8399109840393,0.15301780183472147
123123,246248,123124,369372,484.2531490325928,0.1516400990931288
124124,248250,124125,372375,487.92694306373596,0.15025963716652768
125125,250252,125126,375378,491.560574054718,0.1489112307990581
126126,252254,126127,378381,495.66027188301086,0.14761421217917814
127127,254256,127128,381384,499.3764638900757,0.14631680492857413
128128,256258,128129,384387,503.1838059425354,0.1450752294385893
129129,258260,129130,387390,506.76850986480713,0.14381988993591222
130130,260262,130131,390393,510.5091321468353,0.14257792303396855
131131,262264,131132,393396,514.2886819839478,0.14136632160807494
132132,264266,132133,396399,517.8366301059723,0.14019431189080933
133133,266268,133134,399402,522.9184319972992,0.13901773133693496
134134,268270,134135,402405,527.3423249721527,0.13785333586383786
135135,270272,135136,405408,531.458701133728,0.13669293777275016
136136,272274,136137,408411,535.7159569263458,0.13559269618235703
137137,274276,137138,411414,540.0425250530243,0.13449485313685727
138138,276278,138139,414417,544.9074518680573,0.13338498170378443
139139,278280,139140,417420,550.2467231750488,0.13231213131803088
140140,280282,140141,420423,555.8437299728394,0.13124558982963208
141141,282284,141142,423426,561.0479009151459,0.13023391386195726
142142,284286,142143,426429,565.546816110611,0.1292165988470515
143143,286288,143144,429432,569.4098098278046,0.12819196858436044
144144,288290,144145,432435,573.4714970588684,0.12716854414975387
145145,290292,145146,435438,578.2710769176483,0.12620230870015803
146146,292294,146147,438441,582.5513129234314,0.12526358662398707
147147,294296,147148,441444,586.7244758605957,0.12434501083589566
148148,296298,148149,444447,590.9844501018524,0.123400823391421
149149,298300,149150,447450,595.2063500881195,0.12249096163759532
150150,300302,150151,450453,599.4106910228729,0.12158502898273582
151151,302304,151152,453456,603.5037441253662,0.12070627397224598
152152,304306,152153,456459,607.5897841453552,0.11984584042693314
153153,306308,153154,459462,611.9162650108337,0.11897642279836873
154154,308310,154155,462465,616.8101971149445,0.11810693065308442
155155,310312,155156,465468,621.1397597789764,0.11726718153477123
156156,312314,156157,468471,625.7284700870514,0.11642346645749058
157157,314316,157158,471474,630.0109748840332,0.11561519744282123
158158,316318,158159,474477,634.327791929245,0.11479682040771877
159159,318320,159160,477480,638.878338098526,0.11399117269502312
160160,320322,160161,480483,643.7178289890289,0.11320039781276137
161161,322324,161162,483486,648.250862121582,0.11240221921434568
162162,324326,162163,486489,652.5657229423523,0.11164483547690907
163163,326328,163164,489492,656.7928121089935,0.1108815559600771
164164,328330,164165,492495,661.0727119445801,0.11011743099516025
165165,330332,165166,495498,665.2357289791107,0.10937031366302108
166166,332334,166167,498501,669.4791309833527,0.10862555021776643
167167,334336,167168,501504,673.8401222229004,0.10790561618887295
168168,336338,168169,504507,678.2316060066223,0.10718855160666863
169169,338340,169170,507510,682.6850008964539,0.10646122358775756
170170,340342,170171,510513,687.0982069969177,0.10577157904663181
171171,342344,171172,513516,691.341481924057,0.10505977850880299
172172,344346,172173,516519,695.6489100456238,0.10437878124685085
173173,346348,173174,519522,699.729532957077,0.10370472200884251
174174,348350,174175,522525,704.4017758369446,0.10302122304165096
175175,350352,175176,525528,709.2964150905609,0.10237048447015695
176176,352354,176177,528531,713.5630369186401,0.10173174938063312
177177,354356,177178,531534,717.8149580955505,0.10108055990531284
178178,356358,178179,534537,722.3299300670624,0.10044570981153811
179179,358360,179180,537540,726.4267590045929,0.09981958184835094
180180,360362,180181,540543,731.2850840091705,0.09919241784336918
181181,362364,181182,543546,736.0189590454102,0.09858298464496329
182182,364366,182183,546549,740.6452720165253,0.09796748981716519
183183,366368,183184,549552,745.1168930530548,0.09736162174885976
184184,368370,184185,552555,749.3616809844971,0.09675337709813903
185185,370372,185186,555558,753.6861639022827,0.09616819443908753
186186,372374,186187,558561,758.9634029865265,0.09559156182695006
187187,374376,187188,561564,763.4359469413757,0.09501270678447327
188188,376378,188189,564567,767.8466548919678,0.09443522115543601
189189,378380,189190,567570,772.1993019580841,0.09386824761713797
190190,380382,190191,570573,776.6636869907379,0.09331787455812446
191191,382384,191192,573576,781.1524701118469,0.09276613868132699
192192,384386,192193,576579,785.6537630558014,0.09221484820773185
193193,386388,193194,579582,790.0265390872955,0.091677767199144
194194,388390,194195,582585,794.383159160614,0.0911399445758434
195195,390392,195196,585588,798.7441279888153,0.09062665188139363
196196,392394,196197,588591,803.1104259490967,0.09010046880030131
197197,394396,197198,591594,807.3738648891449,0.08958799116408045
198198,396398,198199,594597,811.627259016037,0.08907978457500576
199199,398400,199200,597600,815.9751529693604,0.08856669398119266
200200,400402,200201,600603,820.2421870231628,0.0880655324071995
201201,402404,201202,603606,824.5262529850006,0.08756885958973726
202202,404406,202203,606609,828.955323934555,0.08707849906750198
203203,406408,203204,609612,833.4505050182343,0.08660245967075753
204204,408410,204205,612615,837.8961520195007,0.086111599144715
205205,410412,205206,615618,842.23770403862,0.08565389002433221
206206,412414,206207,618621,846.6163311004639,0.08518198994170234
207207,414416,207208,621624,850.9905190467834,0.08473386992227461
208208,416418,208209,624627,855.407151222229,0.08427084970026044
209209,418420,209210,627630,859.7565879821777,0.0838338905468845
210210,420422,210211,630633,863.9814341068268,0.08338153458862507
211211,422424,211212,633636,868.3440451622009,0.08293659274204401
212212,424426,212213,636639,872.7082340717316,0.082500408132546
213213,426428,213214,639642,877.0785768032074,0.08207298989509582
214214,428430,214215,642645,881.4167170524597,0.08165115026713465
215215,430432,215216,645648,885.8426110744476,0.08122702955188288
216216,432434,216217,648651,890.1791560649872,0.08082239213581488
217217,434436,217218,651654,894.5441091060638,0.08042151403606113
218218,436438,218219,654657,898.82963514328,0.08000549956886971
219219,438440,219220,657660,903.0747220516205,0.07959238119838119
220220,440442,220221,660663,907.5196630954742,0.07919900827982929
221221,442444,221222,663666,911.8981690406799,0.07880747086710471
222222,444446,222223,666669,916.0751240253448,0.07841909605122055
223223,446448,223224,669672,920.2910521030426,0.07802783463739615
224224,448450,224225,672675,924.6232478618622,0.07763058551790891
225225,450452,225226,675678,928.7265322208405,0.07724427419452695
226226,452454,226227,678681,932.9298710823059,0.07685819561447715
227227,454456,227228,681684,937.143541097641,0.07648496453293774
228228,456458,228229,684687,941.3715209960938,0.07611063340118562
229229,458460,229230,687690,945.8224101066589,0.0757255789667397
230230,460462,230231,690693,950.2664940357208,0.07536120260192547
231231,462464,231232,693696,954.7544620037079,0.07499600686605845
232232,464466,232233,696699,959.2349970340729,0.07464385523053352
233233,466468,233234,699702,963.5875442028046,0.07427229031418392
234234,468470,234235,702705,967.9414489269257,0.07391028472557082
235235,470472,235236,705708,972.2568209171295,0.07355090622331772
236236,472474,236237,708711,976.6209149360657,0.07320209811950917
237237,474476,237238,711714,980.9468328952789,0.07286511062193313
238238,476478,238239,714717,985.2770659923553,0.07250273810677754
239239,478480,239240,717720,989.7086260318756,0.07216610703108017
240240,480482,240241,720723,994.1199131011963,0.07183349221122626
241241,482484,241242,723726,998.4430961608887,0.0714962379552162
242242,484486,242243,726729,1002.5176770687103,0.0711534223810304
243243,486488,243244,729732,1006.76953291893,0.07082581918075448
244244,488490,244245,732735,1011.0284831523895,0.0704867765725794
245245,490492,245246,735738,1015.3633949756622,0.0701750759526476
246246,492494,246247,738741,1019.6918761730194,0.06985486609846703
247247,494496,247248,741744,1023.9797840118408,0.0695395885304606
248248,496498,248249,744747,1028.3045120239258,0.06921285118005471
249249,498500,249250,747750,1032.649866104126,0.06889476538162853
250250,500502,250251,750753,1036.933357000351,0.06857697793930129
251251,502504,251252,753756,1041.4226381778717,0.06827420561967301
252252,504506,252253,756759,1045.8927989006042,0.06796137230776367
253253,506508,253254,759762,1050.2440881729126,0.06765711242769612
254254,508510,254255,762765,1054.5330739021301,0.06734790730115492
255255,510512,255256,765768,1058.8238849639893,0.06704151672602165
256256,512514,256257,768771,1062.9980511665344,0.06675027380879328
257257,514516,257258,771774,1067.4260959625244,0.06644428369327215
258258,516518,258259,774777,1071.8809430599213,0.06615332470391877
259259,518520,259260,777780,1076.140769958496,0.0658577934573259
260260,520522,260261,780783,1080.3904540538788,0.06556909136452305
261261,522524,261262,783786,1084.9063308238983,0.06528670097213762
262262,524526,262263,786789,1089.3435850143433,0.06500484663047246
263263,526528,263264,789792,1093.660549879074,0.06472449207285536
264264,528530,264265,792795,1098.012680053711,0.06444293089407438
265265,530532,265266,795798,1102.285768032074,0.0641603163585387
266266,532534,266267,798801,1106.7277569770813,0.0638921062436566
267267,534536,267268,801804,1110.9907488822937,0.06361693733924767
268268,536538,268269,804807,1115.130713224411,0.06334646259711008
269269,538540,269270,807810,1119.2814090251923,0.06307743637808017
270270,540542,270271,810813,1123.36580991745,0.06281655627208238
271271,542544,271272,813816,1127.607300043106,0.06255138261076354
272272,544546,272273,816819,1131.8722620010376,0.06229056183474313
273273,546548,273274,819822,1136.1376781463623,0.06202264130115509
274274,548550,274275,822825,1140.481891155243,0.06176848407085345
275275,550552,275276,825828,1144.830134153366,0.06151886341467616
276276,552554,276277,828831,1149.1673369407654,0.06125758933558245
277277,554556,277278,831834,1153.5398840904236,0.06100141256865754
278278,556558,278279,834837,1157.6964468955994,0.06074882749999233
279279,558560,279280,837840,1161.817885875702,0.06050732125368086
280280,560562,280281,840843,1166.0080881118774,0.06025894721642544
281281,562564,281282,843846,1170.5618550777435,0.060008233436747105
282282,564566,282283,846849,1174.7093970775604,0.05976371100769029
283283,566568,283284,849852,1178.960186958313,0.05951964972882706
284284,568570,284285,852855,1183.2018010616302,0.059283695760314004
285285,570572,285286,855858,1187.9271161556244,0.059045855810836656
286286,572574,286287,858861,1192.4553060531616,0.058808509493246675
287287,574576,287288,861864,1196.8752131462097,0.05857745984576468
288288,576578,288289,864867,1201.3813440799713,0.05834453810894047
289289,578580,289290,867870,1205.8487710952759,0.05812028709624428
290290,580582,290291,870873,1210.2644119262695,0.057891811560693895
291291,582584,291292,873876,1214.7429950237274,0.05766478814257425
292292,584586,292293,876879,1218.6215710639954,0.05743860463735473
293293,586588,293294,879882,1222.8418271541595,0.057215856439142954
294294,588590,294295,882885,1227.3284060955048,0.056989711987625924
295295,590592,295296,885888,1231.665533065796,0.05676464362477418
296296,592594,296297,888891,1235.9234869480133,0.05654486270759662
297297,594596,297298,891894,1240.2741661071777,0.05632711717044003
298298,596598,298299,894897,1244.8976891040802,0.056105868134181947
299299,598600,299300,897900,1249.5075788497925,0.055890497900691116
300300,600602,300301,900903,1253.9100008010864,0.05567845566656615
301301,602604,301302,903906,1258.1922810077667,0.05546463220161968
302302,604606,302303,906909,1262.680517911911,0.05525064425455639
303303,606608,303304,909912,1267.1205041408539,0.055037134274243726
304304,608610,304305,912915,1271.5624310970306,0.05482591118561686
305305,610612,305306,915918,1275.9306800365448,0.05461271436797688
306306,612614,306307,918921,1280.308053970337,0.05440817330236314
307307,614616,307308,921924,1284.4897820949554,0.05420153496561397
308308,616618,308309,924927,1288.6366121768951,0.05399002982812817
309309,618620,309310,927930,1292.8736708164215,0.053787573904628516
310310,620622,310311,930933,1297.2203562259674,0.05359131342447654
311311,622624,311312,933936,1301.411076784134,0.05339077615644783
312312,624626,312313,936939,1305.6430988311768,0.05319426237110747
313313,626628,313314,939942,1310.0357229709625,0.05299681124415656
314314,628630,314315,942945,1314.4505400657654,0.052803079031946254
315315,630632,315316,945948,1318.7736330032349,0.05260463263766724
316316,632634,316317,948951,1322.9787549972534,0.05241148790628358
317317,634636,317318,951954,1327.245577096939,0.05222041825072665
318318,636638,318319,954957,1331.582582950592,0.05203339199943002
319319,638640,319320,957960,1335.8252229690552,0.05184671259485185
320320,640642,320321,960963,1340.0114409923553,0.051660822366102366
321321,642644,321322,963966,1344.2498669624329,0.05147211063376744
322322,644646,322323,966969,1347.9698469638824,0.05128980839799624
323323,646648,323324,969972,1352.112231016159,0.051108065294101834
324324,648650,324325,972975,1356.4153809547424,0.05092636479639623
325325,650652,325326,975978,1360.7814168930054,0.050745644883136265
326326,652654,326327,978981,1364.9910998344421,0.05056677149332245
327327,654656,327328,981984,1369.3719749450684,0.05038340997998603
328328,656658,328329,984987,1373.7319340705872,0.050206687843456166
329329,658660,329330,987990,1377.9727518558502,0.05002541392968851
330330,660662,330331,990993,1382.1831080913544,0.04984921791947272
331331,662664,331332,993996,1386.4450287818909,0.04967083075644041
332332,664666,332333,996999,1390.7986319065094,0.049497911293656216
333333,666668,333334,1000002,1395.1584980487823,0.049327015674862196
334334,668670,334335,1003005,1399.4754140377045,0.04915543411880208
335335,670672,335336,1006008,1404.033303976059,0.04898564734503452
336336,672674,336337,1009011,1408.647933959961,0.04881498788927274
337337,674676,337338,1012014,1413.6827139854431,0.0486425261151453
338338,676678,338339,1015017,1419.5801320075989,0.04847606619659928
339339,678680,339340,1018020,1424.4225630760193,0.048311585873307195
340340,680682,340341,1021023,1429.6636228561401,0.04814044620979985
341341,682684,341342,1024026,1434.6547808647156,0.047974894967410364
342342,684686,342343,1027029,1439.2440190315247,0.04781206494226353
343343,686688,343344,1030032,1443.739443063736,0.04765117110400752
344344,688690,344345,1033035,1448.2138860225677,0.04748884103537421
345345,690692,345346,1036038,1452.9589009284973,0.04733080626647279
346346,692694,346347,1039041,1457.5750479698181,0.04716929404094117
347347,694696,347348,1042044,1462.175528049469,0.047010728774694144
348348,696698,348349,1045047,1467.595967054367,0.04685283571052423
349349,698700,349350,1048050,1472.6678819656372,0.04669271315469814
350350,700702,350351,1051053,1477.1064541339874,0.04653653740933805
351351,702704,351352,1054056,1482.8788208961487,0.04637488254775235
352352,704706,352353,1057059,1488.2148990631104,0.04621758290704747
353353,706708,353354,1060062,1493.0646238327026,0.046063350071563036
354354,708710,354355,1063065,1497.5827479362488,0.04590932781502488
355355,710712,355356,1066068,1503.019248008728,0.045757941572446725
356356,712714,356357,1069071,1508.1637098789215,0.04560716612286342
357357,714716,357358,1072074,1513.3378601074219,0.04545624764068634
358358,716718,358359,1075077,1518.3599691390991,0.045307938460609876
359359,718720,359360,1078080,1523.388510942459,0.04515975670074113
360360,720722,360361,1081083,1528.4442739486694,0.04500741261472285
361361,722724,361362,1084086,1533.6441929340363,0.04485749819468765
362362,724726,362363,1087089,1538.6611142158508,0.04470969021167548
363363,726728,363364,1090092,1543.6120541095734,0.044566010330527206
364364,728730,364365,1093095,1548.6640660762787,0.044421509010135196
365365,730732,365366,1096098,1553.7200231552124,0.04427856866095681
366366,732734,366367,1099101,1558.8231790065765,0.04413917690362723
367367,734736,367368,1102104,1564.0453791618347,0.0439972136682627
368368,736738,368369,1105107,1569.2186679840088,0.04386076282753493
369369,738740,369370,1108110,1574.2954471111298,0.04372426187546807
370370,740742,370371,1111113,1579.3713128566742,0.043581809653915116
371371,742744,371372,1114116,1584.421725988388,0.043440588047815254
372372,744746,372373,1117119,1589.4576110839844,0.043301920415615314
373373,746748,373374,1120122,1594.4903259277344,0.04316419739370758
374374,748750,374375,1123125,1599.5889239311218,0.04302864734927425
375375,750752,375376,1126128,1604.7002379894257,0.04289396665808454
376376,752754,376377,1129131,1609.775190114975,0.04275948312533728
377377,754756,377378,1132134,1614.912794828415,0.042624812078429386
378378,756758,378379,1135137,1619.955677986145,0.042494374234593124
379379,758760,379380,1138140,1624.9883551597595,0.04236323380609974
380380,760762,380381,1141143,1629.9996769428253,0.04223205002381292
381381,762764,381382,1144146,1635.0428202152252,0.04210188959041261
382382,764766,382383,1147149,1640.0478339195251,0.04197493167157518
383383,766768,383384,1150152,1645.1299998760223,0.04184750352578703
384384,768770,384385,1153155,1650.4425179958344,0.041718936337929335
385385,770772,385386,1156158,1655.550038099289,0.041590581809941796
386386,772774,386387,1159161,1660.6501140594482,0.0414609066065168
387387,774776,387388,1162164,1665.6917481422424,0.04133366572023078
388388,776778,388389,1165167,1670.7405169010162,0.0412082675320562
389389,778780,389390,1168170,1675.7800810337067,0.04108608501155686
390390,780782,390391,1171173,1680.8514912128448,0.040962984356156085
391391,782784,391392,1174176,1685.9319622516632,0.0408419935429265
392392,784786,392393,1177179,1691.0303711891174,0.04072047852241667
393393,786788,393394,1180182,1696.1497480869293,0.04060268424655078
394394,788790,394395,1183185,1701.199126958847,0.040482558721123496
395395,790792,395396,1186188,1706.2635111808777,0.04036137088951364
396396,792794,396397,1189191,1711.332388162613,0.04024480269072228
397397,794796,397398,1192194,1716.4188060760498,0.040124972350895405
398398,796798,398399,1195197,1721.5751948356628,0.04000431529857451
399399,798800,399400,1198200,1726.7196140289307,0.03988512080468354
400400,800802,400401,1201203,1731.8441879749298,0.03977020697311673
401401,802804,401402,1204206,1736.960275888443,0.039653535810430185
402402,804806,402403,1207209,1742.0737080574036,0.039533675750135444
403403,806808,403404,1210212,1747.3468008041382,0.03941970781306736
404404,808810,404405,1213215,1753.1247239112854,0.03930946279797354
405405,810812,405406,1216218,1758.4514350891113,0.039194468101413804
406406,812814,406407,1219221,1763.8978259563446,0.03907710058228986
407407,814816,407408,1222224,1769.455883026123,0.03895875290436379
408408,816818,408409,1225227,1774.5593359470367,0.038845803232106846
409409,818820,409410,1228230,1779.6928341388702,0.03873352640584926
410410,820822,410411,1231233,1784.812143087387,0.03861791294548311
411411,822824,411412,1234236,1789.866250038147,0.03850806591253786
412412,824826,412413,1237239,1794.9593431949615,0.03839558967774792
413413,826828,413414,1240242,1800.0855360031128,0.038285840882963385
414414,828830,414415,1243245,1805.1076610088348,0.0381766406026145
415415,830832,415416,1246248,1810.1808540821075,0.03806774684562697
416416,832834,416417,1249251,1815.2640759944916,0.037960061728881556
417417,834836,417418,1252254,1820.3160152435303,0.03784918571182061
418418,836838,418419,1255257,1825.3528640270233,0.037742511714895954
419419,838840,419420,1258260,1830.3271119594574,0.03764060911271372
420420,840842,420421,1261263,1835.3754858970642,0.03753883842546202
421421,842844,421422,1264266,1840.3289148807526,0.037430369080539094
422422,844846,422423,1267269,1845.4228811264038,0.037325085804695846
423423,846848,423424,1270272,1850.51233792305,0.037221603575744666
424424,848850,424425,1273275,1855.59960603714,0.0371157511635829
425425,850852,425426,1276278,1860.67298579216,0.03701080606151663
426426,852854,426427,1279281,1865.7338471412659,0.03690726146669476
427427,854856,427428,1282284,1870.832051038742,0.03680133240050054
428428,856858,428429,1285287,1875.8745758533478,0.03669564176198037
429429,858860,429430,1288290,1880.892982006073,0.03659407235318213
430430,860862,430431,1291293,1885.9538187980652,0.03649444243819744
431431,862864,431432,1294296,1890.960589170456,0.036395170383912046
432432,864866,432433,1297299,1895.9707589149475,0.036292699243858806
433433,866868,433434,1300302,1901.2210619449615,0.036195224476614385
434434,868870,434435,1303305,1906.2994420528412,0.036095320912863826
435435,870872,435436,1306308,1911.3527340888977,0.03599710618073004
436436,872874,436437,1309311,1916.4280078411102,0.03590107568925305
437437,874876,437438,1312314,1921.4643788337708,0.035805823525151936
438438,876878,438439,1315317,1926.554846048355,0.035710251389900804
439439,878880,439440,1318320,1931.6845791339874,0.03561364046254312
440440,880882,440441,1321323,1936.8185939788818,0.035516636535248836
441441,882884,441442,1324326,1941.8904840946198,0.035420189658907475
442442,884886,442443,1327329,1946.9556930065155,0.03532763242947112
443443,886888,443444,1330332,1951.9991879463196,0.035229221984991455
444444,888890,444445,1333335,1957.057079076767,0.03513332899274246
445445,890892,445446,1336338,1962.063714981079,0.03503836212075839
446446,892894,446447,1339341,1967.073143005371,0.034945950899782474
447447,894896,447448,1342344,1972.1218750476837,0.034850748228564044
448448,896898,448449,1345347,1977.1782190799713,0.03475903026628657
449449,898900,449450,1348350,1982.2367029190063,0.03466451563872397
450450,900902,450451,1351353,1987.317284822464,0.03457361690016114
451451,902904,451452,1354356,1992.398607969284,0.034480550268199295
452452,904906,452453,1357359,1997.500526189804,0.03439088423692738
453453,906908,453454,1360362,2002.5449750423431,0.03429976174265903
454454,908910,454455,1363365,2007.6049630641937,0.03421080378211627
455455,910912,455456,1366368,2012.6559071540833,0.03412189520531683
456456,912914,456457,1369371,2017.726636171341,0.03403361251184833
457457,914916,457458,1372374,2022.8495681285858,0.03394727558224986
458458,916918,458459,1375377,2027.9665248394012,0.03386092021173681
459459,918920,459460,1378380,2033.0360901355743,0.033769838339139824
460460,920922,460461,1381383,2038.0941388607025,0.0336824520072696
461461,922924,461462,1384386,2043.1228449344635,0.03359842493409815
462462,924926,462463,1387389,2048.197168827057,0.03351182504775352
463463,926928,463464,1390392,2053.213039159775,0.033427153755837935
464464,928930,464465,1393395,2058.280753850937,0.03334321582769917
465465,930932,465466,1396398,2063.3822588920593,0.03326007237046724
466466,932934,466467,1399401,2068.4607050418854,0.03317654531565495
467467,934936,467468,1402404,2073.6470079421997,0.0330939364630467
468468,936938,468469,1405407,2078.6938619613647,0.033008914102538256
469469,938940,469470,1408410,2083.7873060703278,0.03292496244648646
470470,940942,470471,1411413,2088.861361026764,0.03284465470824216
471471,942944,471472,1414416,2093.86109995842,0.03276387186269858
472472,944946,472473,1417419,2098.8908009529114,0.03268489466063329
473473,946948,473474,1420422,2103.967283964157,0.03260604661227262
474474,948950,474475,1423425,2109.0084660053253,0.03252705502927711
475475,950952,475476,1426428,2114.0708129405975,0.0324487421894446
476476,952954,476477,1429431,2119.0964539051056,0.03237007860298036
477477,954956,477478,1432434,2124.1280069351196,0.03229219048262166
478478,956958,478479,1435437,2129.2044439315796,0.03221421306989214
479479,958960,479480,1438440,2134.2465369701385,0.03213578978102305
480480,960962,480481,1441443,2139.197616815567,0.032057712794994586
481481,962964,481482,1444446,2144.2372028827667,0.031977578402802465
482482,964966,482483,1447449,2149.329483985901,0.03189944287078106
483483,966968,483484,1450452,2154.3982331752777,0.03182352978910785
484484,968970,484485,1453455,2159.439774990082,0.03174579840924707
485485,970972,485486,1456458,2164.4984951019287,0.03166827814675344
486486,972974,486487,1459461,2169.5500481128693,0.03159003734253929
487487,974976,487488,1462464,2174.566032886505,0.03151240916486131
488488,976978,488489,1465467,2179.597470998764,0.031433211455805576
489489,978980,489490,1468470,2184.6584680080414,0.0313572668346751
490490,980982,490491,1471473,2189.682249069214,0.031281660729291616
491491,982984,491492,1474476,2194.667774915695,0.031205871053316514
492492,984986,492493,1477479,2199.6951019763947,0.03113351223510108
493493,986988,493494,1480482,2204.6832609176636,0.03106100780860288
494494,988990,494495,1483485,2209.700492143631,0.030986623220087495
495495,990992,495496,1486488,2214.737590074539,0.030912169513612753
496496,992994,496497,1489491,2219.7545421123505,0.03084027588556637
497497,994996,497498,1492494,2224.8419280052185,0.030768238348173327
498498,996998,498499,1495497,2229.946949005127,0.030697683891048655
499499,999000,499500,1498500,2234.9482839107513,0.030624584960605716
500501,1001004,500502,1501506,2239.9798018932343,0.03055277090606978
501502,1003006,501503,1504509,2245.163866996765,0.03048247186234221
502503,1005008,502504,1507512,2250.233274936676,0.030411687535888632
503504,1007010,503505,1510515,2255.3130609989166,0.03033823973419203
504505,1009012,504506,1513518,2260.363610982895,0.030267203534094733
505506,1011014,505507,1516521,2265.4386179447174,0.030196914483894943
506507,1013016,506508,1519524,2270.495674133301,0.030128009064355865
507508,1015018,507509,1522527,2275.55410695076,0.03005784659399069
508509,1017020,508510,1525530,2280.5331478118896,0.02998779078370717
509510,1019022,509511,1528533,2285.5011830329895,0.029918425954747363
510511,1021024,510512,1531536,2290.5240609645844,0.029849488400941482
511512,1023026,511513,1534539,2295.576826095581,0.02978057131622336
512513,1025028,512514,1537542,2300.602767944336,0.029711302599025657
513514,1027030,513515,1540545,2305.6484150886536,0.02964230059842521
514515,1029032,514516,1543548,2310.714085817337,0.02957351433178701
515516,1031034,515517,1546551,2315.762857913971,0.02950624296499882
516517,1033036,516518,1549554,2320.8116569519043,0.02943904551830201
517518,1035038,517519,1552557,2325.8354501724243,0.02937337247749383
518519,1037040,518520,1555560,2330.9279968738556,0.029306242666280014
519520,1039042,519521,1558563,2335.984943151474,0.02923958359315293
520521,1041044,520522,1561566,2340.8349299430847,0.029172906364692608
521522,1043046,521523,1564569,2345.8395688533783,0.029104296892910497
522523,1045048,522524,1567572,2350.854734182358,0.029038154541922268
523524,1047050,523525,1570575,2355.8821001052856,0.02897107864919235
524525,1049052,524526,1573578,2360.903522014618,0.02890371649482404
525526,1051054,525527,1576581,2365.946841955185,0.028837573052442167
526527,1053056,526528,1579584,2370.9811499118805,0.0287711929759098
527528,1055058,527529,1582587,2376.0850670337677,0.028706750792480307
528529,1057060,528530,1585590,2381.0882980823517,0.028642730379942805
529530,1059062,529531,1588593,2386.1125819683075,0.02857901329298329
530531,1061064,530532,1591596,2391.1785390377045,0.028514807316241786
531532,1063066,531533,1594599,2396.204950094223,0.028451865193346748
532533,1065068,532534,1597602,2401.247498989105,0.028387068887241185
533534,1067070,533535,1600605,2406.231716156006,0.028325738056082628
534535,1069072,534536,1603608,2411.23481798172,0.028264613980354625
535536,1071074,535537,1606611,2416.2891829013824,0.028202130588397267
536537,1073076,536538,1609614,2421.388920068741,0.02813884437091474
537538,1075078,537539,1612617,2426.4556879997253,0.02807657562152599
538539,1077080,538540,1615620,2431.556135892868,0.02801499728411727
539540,1079082,539541,1618623,2436.5519070625305,0.027954871995461872
540541,1081084,540542,1621626,2441.569060087204,0.02789443900473998
541542,1083086,541543,1624629,2446.587517976761,0.02783186986016517
542543,1085088,542544,1627632,2451.6421377658844,0.0277695474360371
543544,1087090,543545,1630635,2456.650676012039,0.027709299580237712
544545,1089092,544546,1633638,2461.6013209819794,0.027648888462863397
545546,1091094,545547,1636641,2466.649796962738,0.02758881116460543
546547,1093096,546548,1639644,2471.627110004425,0.02752798253277433
547548,1095098,547549,1642647,2476.6414120197296,0.027469175487567554
548549,1097100,548550,1645650,2481.637104988098,0.027410530761699192
549550,1099102,549551,1648653,2486.64240694046,0.027352244413123117
550551,1101104,550552,1651656,2491.68963098526,0.027293446133626276
551552,1103106,551553,1654659,2496.764561891556,0.027232852082306636
552553,1105108,552554,1657662,2501.7842450141907,0.027171640444066725
553554,1107110,553555,1660665,2506.818787097931,0.027109872333312524
554555,1109112,554556,1663668,2511.812516927719,0.027051153267166228
555556,1111114,555557,1666671,2516.8079030513763,0.02699237147317035
556557,1113116,556558,1669674,2521.8355457782745,0.026935664305710816
557558,1115118,557559,1672677,2526.8377289772034,0.026878572098212317
558559,1117120,558560,1675680,2531.9522619247437,0.026820778200999484
559560,1119122,559561,1678683,2537.0170118808746,0.02676137042544724
560561,1121124,560562,1681686,2542.074553012848,0.02670246244088048
561562,1123126,561563,1684689,2547.1770281791687,0.02664556944000651
562563,1125128,562564,1687692,2552.230341911316,0.026588856600938016
563564,1127130,563565,1690695,2557.339318037033,0.02653266406196053
564565,1129132,564566,1693698,2562.418394804001,0.026476221422853996
565566,1131134,565567,1696701,2567.475772857666,0.026419150137371616
566567,1133136,566568,1699704,2572.5508019924164,0.026362920694737113
567568,1135138,567569,1702707,2577.6086831092834,0.02630786900044768
568569,1137140,568570,1705710,2582.661028146744,0.026251921484799823
569570,1139142,569571,1708713,2587.792274951935,0.026195985517915688
570571,1141144,570572,1711716,2592.8876581192017,0.026140345240492024
571572,1143146,571573,1714719,2597.9339468479156,0.026085906491061905
572573,1145148,572574,1717722,2602.9822750091553,0.02603073666068667
573574,1147150,573575,1720725,2607.9923429489136,0.025975415454013273
574575,1149152,574576,1723728,2613.0521750450134,0.025920983131072717
575576,1151154,575577,1726731,2618.09507894516,0.02586824206082383
576577,1153156,576578,1729734,2623.1826298236847,0.02581461422232678
577578,1155158,577579,1732737,2628.279876947403,0.025759624508282286
578579,1157160,578580,1735740,2633.4228279590607,0.025706399266709923
579580,1159162,579581,1738743,2638.390406847,0.0256536794713611
580581,1161164,580582,1741746,2643.3621780872345,0.02560013013862772
581582,1163166,581583,1744749,2648.4252989292145,0.025546816304995446
582583,1165168,582584,1747752,2653.4313740730286,0.02549512975201651
583584,1167170,583585,1750755,2658.4795949459076,0.02544167430824018
584585,1169172,584586,1753758,2663.5191061496735,0.025389089101736317
585586,1171174,585587,1756761,2668.70921087265,0.02533710865827743
586587,1173176,586588,1759764,2675.5508880615234,0.025284614821430296
587588,1175178,587589,1762767,2681.4723358154297,0.025233764932636404
588589,1177180,588590,1765770,2687.0584042072296,0.025182962212056736
589590,1179182,589591,1768773,2692.1324710845947,0.025132862510872656
590591,1181184,590592,1771776,2697.2480289936066,0.025082192338231835
591592,1183186,591593,1774779,2702.2971761226654,0.025030706687175552
592593,1185188,592594,1777782,2707.4709718227386,0.02497998540820845
593594,1187190,593595,1780785,2712.6002650260925,0.02492929537402233
594595,1189192,594596,1783788,2717.7122070789337,0.02487930429924745
595596,1191194,595597,1786791,2722.8287942409515,0.024828896755934693
596597,1193196,596598,1789794,2727.9777789115906,0.02477845186331251
597598,1195198,597599,1792797,2733.086852788925,0.02472811682309839
598599,1197200,598600,1795800,2738.217730998993,0.024678895049873972
599600,1199202,599601,1798803,2743.3140890598297,0.024628056862638914
600601,1201204,600602,1801806,2748.397339820862,0.024577403821240296
601602,1203206,601603,1804809,2753.4855811595917,0.024526854256691877
602603,1205208,602604,1807812,2758.589607000351,0.024476873430103296
603604,1207210,603605,1810815,2763.680558204651,0.02442747150780633
604605,1209212,604606,1813818,2768.7533388137817,0.024378649513892015
605606,1211214,605607,1816821,2773.8556730747223,0.024329544270585757
606607,1213216,606608,1819824,2778.9536340236664,0.024280602068756707
607608,1215218,607609,1822827,2784.007075071335,0.02423231538887194
608609,1217220,608610,1825830,2789.1208119392395,0.024183603027267964
609610,1219222,609611,1828833,2794.222640991211,0.024136176105457707
610611,1221224,610612,1831836,2799.280015230179,0.024088882139039924
611612,1223226,611613,1834839,2804.3602209091187,0.0240423479135643
612613,1225228,612614,1837842,2809.4332160949707,0.023995380655833287
613614,1227230,613615,1840845,2814.499589920044,0.023947172387124738
614615,1229232,614616,1843848,2819.5928819179535,0.02389893206236593
615616,1231234,615617,1846851,2824.6283588409424,0.023852137028370635
616617,1233236,616618,1849854,2829.708373069763,0.023804748278053012
617618,1235238,617619,1852857,2834.75927901268,0.023758095618177322
618619,1237240,618620,1855860,2839.7856290340424,0.023711841395197553
619620,1239242,619621,1858863,2844.801190853119,0.023666363253141753
620621,1241244,620622,1861866,2849.936150074005,0.023620231742825126
621622,1243246,621623,1864869,2855.0306289196014,0.023573961601869087
622623,1245248,622624,1867872,2860.1009290218353,0.023526917439085082
623624,1247250,623625,1870875,2865.1959869861603,0.023479902285544085
624625,1249252,624626,1873878,2870.32169508934,0.023434427934262203
625626,1251254,625627,1876881,2875.420555114746,0.02338964815317013
626627,1253256,626628,1879884,2880.481360912323,0.02334406360932917
627628,1255258,627629,1882887,2885.5173370838165,0.023298564163269475
628629,1257260,628630,1885890,2890.6042170524597,0.023253674065927044
629630,1259262,629631,1888893,2895.6669471263885,0.023208806214825017
630631,1261264,630632,1891896,2900.7354822158813,0.02316362495366775
631632,1263266,631633,1894899,2905.767075061798,0.02311850535807025
632633,1265268,632634,1897902,2910.810198068619,0.02307336948979355
633634,1267270,633635,1900905,2915.9093911647797,0.023028804749628762
634635,1269272,634636,1903908,2920.997645139694,0.022985105206316803
635636,1271274,635637,1906911,2926.0861167907715,0.02293994057981763
636637,1273276,636638,1909914,2931.141484975815,0.022895582536875736
637638,1275278,637639,1912917,2936.189961910248,0.022851990534036304
638639,1277280,638640,1915920,2941.241902112961,0.022808519051977783
639640,1279282,639641,1918923,2946.2738728523254,0.022763765651689027
640641,1281284,640642,1921926,2951.3692610263824,0.022720093986208667
641642,1283286,641643,1924929,2956.427929162979,0.022676230079014204
642643,1285288,642644,1927932,2961.4770748615265,0.02263369298998441
643644,1287290,643645,1930935,2966.5330288410187,0.022590768201553146
644645,1289292,644646,1933938,2971.802234172821,0.022547086562553886
645646,1291294,645647,1936941,2976.863373041153,0.022504133492475376
646647,1293296,646648,1939944,2981.819939136505,0.02246051405563776
647648,1295298,647649,1942947,2986.946756839752,0.022417340695028543
648649,1297300,648650,1945950,2992.017895936966,0.022375768239726312
649650,1299302,649651,1948953,2997.104129076004,0.022332702112180414
650651,1301304,650652,1951956,3002.156389951706,0.022291132758255117
651652,1303306,651653,1954959,3007.3000252246857,0.022248990935622714
652653,1305308,652654,1957962,3012.362287044525,0.022207021342182998
653654,1307310,653655,1960965,3017.4444348812103,0.022165781339936075
654655,1309312,654656,1963968,3022.505744934082,0.02212286667781882
655656,1311314,655657,1966971,3027.5205240249634,0.022080154456489254
656657,1313316,656658,1969974,3032.631113052368,0.022038802797396784
657658,1315318,657659,1972977,3037.725741147995,0.02199714380731166
658659,1317320,658660,1975980,3042.754639863968,0.021956053935355158
659660,1319322,659661,1978983,3048.391279220581,0.021914605940764886
660661,1321324,660662,1981986,3053.491203069687,0.02187375237008382
661662,1323326,661663,1984989,3058.938863992691,0.021832442242157413
662663,1325328,662664,1987992,3064.021273136139,0.021791986742755398
663664,1327330,663665,1990995,3069.0647439956665,0.021752671427748282
664665,1329332,664666,1993998,3074.084265947342,0.021711908808356384
665666,1331334,665667,1997001,3079.0882618427277,0.02167105288026505
666667,1333336,666668,2000004,3084.102189064026,0.02163062789441028
667668,1335338,667669,2003007,3089.149281024933,0.02159244432732521
668669,1337340,668670,2006010,3094.2049539089203,0.021553048745772685
669670,1339342,669671,2009013,3099.2505819797516,0.02151257345940394
670671,1341344,670672,2012016,3104.3393399715424,0.021472844668096513
671672,1343346,671673,2015019,3109.4389219284058,0.021434119233163074
672673,1345348,672674,2018022,3114.4794340133667,0.02139573952263163
673674,1347350,673675,2021025,3119.5785150527954,0.021357074843763257
674675,1349352,674676,2024028,3124.5783910751343,0.021317314120096853
675676,1351354,675677,2027031,3129.597018957138,0.021277616257066256
676677,1353356,676678,2030034,3134.599982023239,0.021239871959551238
677678,1355358,677679,2033037,3139.506089925766,0.021201863508395036
678679,1357360,678680,2036040,3144.551132917404,0.021164025307371048
679680,1359362,679681,2039043,3149.6110990047455,0.021127415328010102
680681,1361364,680682,2042046,3154.6832780838013,0.02108831848454429
681682,1363366,681683,2045049,3159.827050924301,0.021049933471658733
682683,1365368,682684,2048052,3164.8989861011505,0.021011512671975652
683684,1367370,683685,2051055,3169.987279176712,0.02097443275852129
684685,1369372,684686,2054058,3175.0385389328003,0.020936598170010257
685686,1371374,685687,2057061,3180.113821029663,0.020898914484860143
686687,1373376,686688,2060064,3185.1560440063477,0.02086181468439463
687688,1375378,687689,2063067,3190.166235923767,0.020824324656132376
688689,1377380,688690,2066070,3195.224860906601,0.020785998451174237
689690,1379382,689691,2069073,3200.2928099632263,0.02074845155220828
690691,1381384,690692,2072076,3205.3089740276337,0.02071170715316839
691692,1383386,691693,2075079,3210.3009548187256,0.020675080457294825
692693,1385388,692694,2078082,3215.355717897415,0.020637165900552645
693694,1387390,693695,2081085,3220.399067878723,0.02060045347570849
694695,1389392,694696,2084088,3225.510549068451,0.02056390410689346
695696,1391394,695697,2087091,3230.5540289878845,0.02052722582811839
696697,1393396,696698,2090094,3235.6033878326416,0.02049065571372921
697698,1395398,697699,2093097,3240.6557791233063,0.02045390738203423
698699,1397400,698700,2096100,3245.700420856476,0.02041757850565773
699700,1399402,699701,2099103,3250.8384029865265,0.02038132037341711
700701,1401404,700702,2102106,3255.923697948456,0.020346176646853564
701702,1403406,701703,2105109,3260.979302883148,0.020310221229010494
702703,1405408,702704,2108112,3266.093628883362,0.02027410071059421
703704,1407410,703705,2111115,3271.2174830436707,0.02023745402584609
704705,1409412,704706,2114118,3276.320612192154,0.020202626157697523
705706,1411414,705707,2117121,3281.4372680187225,0.020166510896160617
706707,1413416,706708,2120124,3286.5603201389313,0.02013018356410612
707708,1415418,707709,2123127,3291.6646699905396,0.020094705318115302
708709,1417420,708710,2126130,3296.7947731018066,0.020058495736520854
709710,1419422,709711,2129133,3301.86936712265,0.020023780978590366
710711,1421424,710712,2132136,3306.9589791297913,0.01998935609299224
711712,1423426,711713,2135139,3312.028855085373,0.019954092143962043
712713,1425428,712714,2138142,3317.139322042465,0.019919357924663927
713714,1427430,713715,2141145,3322.1897950172424,0.01988521732891968
714715,1429432,714716,2144148,3327.284959077835,0.019850751321428106
715716,1431434,715717,2147151,3332.393529176712,0.01981542357316357
716717,1433436,716718,2150154,3337.4942779541016,0.019780362094024895
717718,1435438,717719,2153157,3342.591475009918,0.019745738261917722
718719,1437440,718720,2156160,3347.6817829608917,0.01971149326345767
719720,1439442,719721,2159163,3352.7471430301666,0.019677375947139808
720721,1441444,720722,2162166,3357.8745028972626,0.019642150362415123
721722,1443446,721723,2165169,3362.9416630268097,0.0196084205454099
722723,1445448,722724,2168172,3368.0154390335083,0.01957379544910509
723724,1447450,723725,2171175,3373.0658071041107,0.019538946380635025
724725,1449452,724726,2174178,3378.190851211548,0.019505525522617972
725726,1451454,725727,2177181,3383.3185460567474,0.019472166168270633
726727,1453456,726728,2180184,3388.347388982773,0.019438200783042703
727728,1455458,727729,2183187,3393.39053106308,0.01940469520377519
728729,1457460,728730,2186190,3398.4673862457275,0.019371583288375405
729730,1459462,729731,2189193,3403.5831089019775,0.01933799470134545
730731,1461464,730732,2192196,3408.683351993561,0.019305455340145272
731732,1463466,731733,2195199,3413.73095703125,0.019272699566499796
732733,1465468,732734,2198202,3418.8322370052338,0.019238240927734296
733734,1467470,733735,2201205,3423.9878220558167,0.019205243179385434
734735,1469472,734736,2204208,3429.0612239837646,0.019172515587342787
735736,1471474,735737,2207211,3434.7410459518433,0.01913939547011978
736737,1473476,736738,2210214,3440.001937866211,0.019106712210486876
737738,1475478,737739,2213217,3445.147306919098,0.019073901195952203
738739,1477480,738740,2216220,3450.345160007477,0.019040668405068573
739740,1479482,739741,2219223,3455.4186811447144,0.01900848418517853
740741,1481484,740742,2222226,3460.535646915436,0.018975230002979515
741742,1483486,741743,2225229,3465.6222410202026,0.018943326509543112
742743,1485488,742744,2228232,3470.7019789218903,0.018911324443251942
743744,1487490,743745,2231235,3475.797894001007,0.018878664248404675
744745,1489492,744746,2234238,3480.6814579963684,0.018846175004000543
745746,1491494,745747,2237241,3485.774365901947,0.018813040987879504
746747,1493496,746748,2240244,3490.9132208824158,0.018780595461066696
747748,1495498,747749,2243247,3495.9678630828857,0.018748884978776914
748749,1497500,748750,2246250,3501.079297065735,0.018717261518759187
749750,1499502,749751,2249253,3506.16854596138,0.018686197789065773
750751,1501504,750752,2252256,3511.22429895401,0.018655106501682894
751752,1503506,751753,2255259,3516.30717587471,0.018622587511345046
752753,1505508,752754,2258262,3521.36355304718,0.018591095251395018
753754,1507510,753755,2261265,3526.491029024124,0.01855975334547111
754755,1509512,754756,2264268,3531.5351190567017,0.01852727485129435
755756,1511514,755757,2267271,3536.6377930641174,0.018496565926398034
756757,1513516,756758,2270274,3541.7792451381683,0.018465420153006562
757758,1515518,757759,2273277,3546.8566529750824,0.018433846857078606
758759,1517520,758760,2276280,3551.9935359954834,0.018401963210635586
759760,1519522,759761,2279283,3557.18279504776,0.01837119712763524
760761,1521524,760762,2282286,3562.246603012085,0.018339682808800717
761762,1523526,761763,2285289,3567.3695390224457,0.01830861701637332
762763,1525528,762764,2288292,3572.4393570423126,0.018277748855325626
763764,1527530,763765,2291295,3577.5254011154175,0.01824668247718364
764765,1529532,764766,2294298,3582.583316087723,0.018216928099718643
765766,1531534,765767,2297301,3587.7051849365234,0.018186513740147348
766767,1533536,766768,2300304,3592.7822189331055,0.01815564065145736
767768,1535538,767769,2303307,3597.9041001796722,0.01812537418481952
768769,1537540,768770,2306310,3603.0079958438873,0.018095942035870394
769770,1539542,769771,2309313,3608.104528903961,0.018065209638734814
770771,1541544,770772,2312316,3613.191265106201,0.018034809503660654
771772,1543546,771773,2315319,3618.2624049186707,0.01800459305741242
772773,1545548,772774,2318322,3623.363918066025,0.017974527947444585
773774,1547550,773775,2321325,3628.4337599277496,0.01794458064796345
774775,1549552,774776,2324328,3633.520315885544,0.017914650359671214
775776,1551554,775777,2327331,3638.5606348514557,0.017884473281810642
776777,1553556,776778,2330334,3643.596621990204,0.0178548501462501
777778,1555558,777779,2333337,3648.6340239048004,0.017825533062932664
778779,1557560,778780,2336340,3653.765609025955,0.017796169040593668
779780,1559562,779781,2339343,3658.8834948539734,0.017767054956493666
780781,1561564,780782,2342346,3663.952523946762,0.017738355145411333
781782,1563566,781783,2345349,3669.0253808498383,0.01770831338581047
782783,1565568,782784,2348352,3674.1155869960785,0.017679680888250005
783784,1567570,783785,2351355,3679.2047171592712,0.01764980896587076
784785,1569572,784786,2354358,3684.2631299495697,0.017620852144318633
785786,1571574,785787,2357361,3689.3140370845795,0.017592166224858374
786787,1573576,786788,2360364,3694.360384941101,0.017563413515745196
787788,1575578,787789,2363367,3699.406674861908,0.017534088094180333
788789,1577580,788790,2366370,3704.4990870952606,0.01750681214798533
789790,1579582,789791,2369373,3709.587635040283,0.017479266027294216
790791,1581584,790792,2372376,3714.636505126953,0.0174508406289533
791792,1583586,791793,2375379,3719.7214138507843,0.01742308816028526
792793,1585588,792794,2378382,3724.7597692012787,0.0173952777768136
793794,1587590,793795,2381385,3729.827425956726,0.017367892411130015
794795,1589592,794796,2384388,3734.9145851135254,0.017340188556772773
795796,1591594,795797,2387391,3739.9804100990295,0.017312131290964317
796797,1593596,796798,2390394,3745.042585849762,0.017284340407059062
797798,1595598,797799,2393397,3750.117518186569,0.017256205890589627
798799,1597600,798800,2396400,3755.198007106781,0.01722920649444859
799800,1599602,799801,2399403,3760.3092589378357,0.017201798775204225
800801,1601604,800802,2402406,3765.4493792057037,0.017175068922369974
801802,1603606,801803,2405409,3770.49005484581,0.01714843032641511
802803,1605608,802804,2408412,3775.5708980560303,0.01712084924110968
803804,1607610,803805,2411415,3780.6436910629272,0.0170937045422761
804805,1609612,804806,2414418,3785.693081140518,0.017067357743144385
805806,1611614,805807,2417421,3790.7975721359253,0.017040923188687884
806807,1613616,806808,2420424,3795.849420070648,0.017014018949339516
807808,1615618,807809,2423427,3800.9105780124664,0.016986821832688292
808809,1617620,808810,2426430,3805.964513063431,0.016959119817329338
809810,1619622,809811,2429433,3810.9970569610596,0.016932852977333823
810811,1621624,810812,2432436,3816.068302154541,0.016906371565710288
811812,1623626,811813,2435439,3821.10653591156,0.016879748725841637
812813,1625628,812814,2438442,3826.3623371124268,0.01685351315245498
813814,1627630,813815,2441445,3831.425033092499,0.016827408548124367
814815,1629632,814816,2444448,3836.477447986603,0.016801436628156807
815816,1631634,815817,2447451,3841.6295969486237,0.016775100824816036
816817,1633636,816818,2450454,3846.739065170288,0.01674938899486733
817818,1635638,817819,2453457,3851.830878973007,0.01672272205723857
818819,1637640,818820,2456460,3856.9327590465546,0.01669733927883499
819820,1639642,819821,2459463,3862.0156140327454,0.016672141007802566
820821,1641644,820822,2462466,3867.1237041950226,0.016645970363242668
821822,1643646,821823,2465469,3872.419163942337,0.016620562360913027
822823,1645648,822824,2468472,3877.530163049698,0.01659451690102287
823824,1647650,823825,2471475,3882.648535013199,0.016568963161262218
824825,1649652,824826,2474478,3887.733654975891,0.01654359622443735
825826,1651654,825827,2477481,3892.784110069275,0.016518663434908376
826827,1653656,826828,2480484,3897.9392352104187,0.01649397358414717
827828,1655658,827829,2483487,3903.06041097641,0.016468055291625205
828829,1657660,828830,2486490,3908.104063987732,0.016442739652120508
829830,1659662,829831,2489493,3913.1634271144867,0.016417400824138895
830831,1661664,830832,2492496,3918.2480981349945,0.016391861032388988
831832,1663666,831833,2495499,3923.341726064682,0.01636632837653451
832833,1665668,832834,2498502,3928.46239900589,0.016341779717549798
833834,1667670,833835,2501505,3933.5214989185333,0.016316090632244595
834835,1669672,834836,2504508,3938.6032581329346,0.01629134506219998
835836,1671674,835837,2507511,3943.7309861183167,0.016266791275484138
836837,1673676,836838,2510514,3948.8425850868225,0.0162426154493005
837838,1675678,837839,2513517,3954.0122740268707,0.016217877935559954
838839,1677680,838840,2516520,3959.1584310531616,0.016192726132430835
839840,1679682,839841,2519523,3964.2685110569,0.016168718435437768
840841,1681684,840842,2522526,3969.3612768650055,0.01614502326810907
841842,1683686,841843,2525529,3974.467148065567,0.016120098100145697
842843,1685688,842844,2528532,3979.602703809738,0.016095582373964135
843844,1687690,843845,2531535,3984.6663269996643,0.016071317619207548
844845,1689692,844846,2534538,3989.7571761608124,0.016046715065385797
845846,1691694,845847,2537541,3994.86066699028,0.01602274656033842
846847,1693696,846848,2540544,3999.9304950237274,0.015998575816411176
847848,1695698,847849,2543547,4005.0533640384674,0.015974887257470982
848849,1697700,848850,2546550,4010.1683089733124,0.015950065080687637
849850,1699702,849851,2549553,4015.245239019394,0.01592538413387956
850851,1701704,850852,2552556,4020.376783847809,0.015900744871032657
851852,1703706,851853,2555559,4025.5274341106415,0.015876584457146237
852853,1705708,852854,2558562,4030.646073102951,0.01585215645172866
853854,1707710,853855,2561565,4035.7305238246918,0.015827993765924475
854855,1709712,854856,2564568,4040.81675696373,0.015804769147507614
855856,1711714,855857,2567571,4045.9190599918365,0.0157816136143083
856857,1713716,856858,2570574,4051.8485050201416,0.015758167099193088
857858,1715718,857859,2573577,4057.1110379695892,0.015734627462734352
858859,1717720,858860,2576580,4062.3244631290436,0.015710691821368528
859860,1719722,859861,2579583,4067.3830420970917,0.015686904214817332
860861,1721724,860862,2582586,4072.4930980205536,0.015663748206861783
861862,1723726,861863,2585589,4077.5593349933624,0.015640081761375768
862863,1725728,862864,2588592,4082.6404659748077,0.015616759101249045
863864,1727730,863865,2591595,4087.712558031082,0.015593018693834892
864865,1729732,864866,2594598,4092.809909105301,0.015569747456538607
865866,1731734,865867,2597601,4097.87025308609,0.0155470107729343
866867,1733736,866868,2600604,4102.967668056488,0.015524093701969832
867868,1735738,867869,2603607,4108.047170162201,0.015500818724831333
868869,1737740,868870,2606610,4113.198755025864,0.015477497699976084
869870,1739742,869871,2609613,4118.336612224579,0.015455133194336668
870871,1741744,870872,2612616,4123.39834189415,0.01543115102685988
871872,1743746,871873,2615619,4128.554255962372,0.015408698438477586
872873,1745748,872874,2618622,4133.630530118942,0.015384998519948567
873874,1747750,873875,2621625,4138.766978025436,0.01536263652087655
874875,1749752,874876,2624628,4143.885117053986,0.015340115813160082
875876,1751754,875877,2627631,4149.019075155258,0.015317424542445224
876877,1753756,876878,2630634,4154.102138996124,0.01529539241528255
877878,1755758,877879,2633637,4159.14902305603,0.015272579477823456
878879,1757760,878880,2636640,4164.243474006653,0.015250306414600345
879880,1759762,879881,2639643,4169.373923063278,0.015227724621581729
880881,1761764,880882,2642646,4174.4378299713135,0.0152056121150963
881882,1763766,881883,2645649,4179.542949914932,0.015183518418780295
882883,1765768,882884,2648652,4184.604154825211,0.015160993341851281
883884,1767770,883885,2651655,4189.648718118668,0.015138812648729072
884885,1769772,884886,2654658,4194.745015144348,0.0151165903389483
885886,1771774,885887,2657661,4199.979943037033,0.015093827760210843
886887,1773776,886888,2660664,4205.039128065109,0.015071400597662432
887888,1775778,887889,2663667,4210.142323970795,0.01504968779590854
888889,1777780,888890,2666670,4215.247072935104,0.015027497320261318
889890,1779782,889891,2669673,4220.356239080429,0.0150053524885152
890891,1781784,890892,2672676,4225.431928157806,0.014983353137722588
891892,1783786,891893,2675679,4230.581293106079,0.0149615927166451
892893,1785788,892894,2678682,4235.657039880753,0.014939856439013965
893894,1787790,893895,2681685,4240.723741054535,0.014917786007572431
894895,1789792,894896,2684688,4245.828486919403,0.014895786367560504
895896,1791794,895897,2687691,4250.903079986572,0.014873959384203772
896897,1793796,896898,2690694,4255.965214014053,0.014852244648864144
897898,1795798,897899,2693697,4261.032084941864,0.014830353493380244
898899,1797800,898900,2696700,4266.08957695961,0.0148088260248187
899900,1799802,899901,2699703,4271.171262025833,0.014787133470235858
900901,1801804,900902,2702706,4276.225015163422,0.014766357569897082
901902,1803806,901903,2705709,4281.274971961975,0.014744889065696043
902903,1805808,902904,2708712,4286.358780860901,0.01472325760187232
903904,1807810,903905,2711715,4291.455300807953,0.014702588703585207
904905,1809812,904906,2714718,4296.587146997452,0.014680973634312977
905906,1811814,905907,2717721,4301.702888011932,0.01466020716179628
906907,1813816,906908,2720724,4306.84165096283,0.014638854523582268
907908,1815818,907909,2723727,4311.969553947449,0.014618471917856368
908909,1817820,908910,2726730,4317.004378795624,0.014596956822060747
909910,1819822,909911,2729733,4322.08340716362,0.014576108049368486
910911,1821824,910912,2732736,4327.1218910217285,0.014555144482073956
911912,1823826,911913,2735739,4332.20153093338,0.014534422494762111
912913,1825828,912914,2738742,4337.231876134872,0.01451347226065991
913914,1827830,913915,2741745,4342.263226985931,0.014493131051494856
914915,1829832,914916,2744748,4347.34670996666,0.014472658282102202
915916,1831834,915917,2747751,4352.427247047424,0.014451878218096681
916917,1833836,916918,2750754,4357.52149605751,0.014431131934543373
917918,1835838,917919,2753757,4362.566132068634,0.014410289248189656
918919,1837840,918920,2756760,4367.644317865372,0.014389462487088167
919920,1839842,919921,2759763,4372.737969875336,0.014369398088092566
920921,1841844,920922,2762766,4377.693478822708,0.014349069979289197
921922,1843846,921923,2765769,4382.669604063034,0.014328979401398101
922923,1845848,922924,2768772,4387.799116134644,0.014309152860732866
923924,1847850,923925,2771775,4392.912702083588,0.0142889055859996
924925,1849852,924926,2774778,4397.85480594635,0.01426850606003427
925926,1851854,925927,2777781,4402.904017925262,0.014247683300709468
926927,1853856,926928,2780784,4407.955713033676,0.014226935265469365
927928,1855858,927929,2783787,4413.071985006332,0.014206585601641564
928929,1857860,928930,2786790,4418.1576471328735,0.014186792506734491
929930,1859862,929931,2789793,4423.2482759952545,0.014166029110128875
930931,1861864,930932,2792796,4428.26637005806,0.014145797760647838
931932,1863866,931933,2795799,4433.270223140717,0.014125997411611024
932933,1865868,932934,2798802,4438.30912899971,0.014105643009315827
933934,1867870,933935,2801805,4443.451858997345,0.014085241107750335
934935,1869872,934936,2804808,4448.546061038971,0.014065102272070362
935936,1871874,935937,2807811,4453.634725809097,0.014045045150851365
936937,1873876,936938,2810814,4458.65873003006,0.01402482492630952
937938,1875878,937939,2813817,4463.728119134903,0.014004706328705652
938939,1877880,938940,2816820,4468.779617071152,0.013984996505314484
939940,1879882,939941,2819823,4473.868222951889,0.013964926631160779
940941,1881884,940942,2822826,4478.926600933075,0.013945865739515284
941942,1883886,941943,2825829,4483.981558084488,0.013925866007411969
942943,1885888,942944,2828832,4489.05570101738,0.01390708944745711
943944,1887890,943945,2831835,4494.111169099808,0.013886947286664508
944945,1889892,944946,2834838,4499.232390880585,0.013867587411368731
945946,1891894,945947,2837841,4504.339838027954,0.013848298052835162
946947,1893896,946948,2840844,4509.452238082886,0.013829078243361437
947948,1895898,947949,2843847,4514.528733968735,0.013809987551212544
948949,1897900,948950,2846850,4520.523329973221,0.013790714954666328
949950,1899902,949951,2849853,4525.791663169861,0.013771430833003251
950951,1901904,950952,2852856,4530.928453922272,0.013752439288509777
951952,1903906,951953,2855859,4536.030052185059,0.013732727642491227
952953,1905908,952954,2858862,4541.160413980484,0.013712737549212761
953954,1907910,953955,2861865,4546.317992925644,0.013693695500478498
954955,1909912,954956,2864868,4551.398238897324,0.013674060754055972
955956,1911914,955957,2867871,4556.570384979248,0.013654651314936928
956957,1913916,956958,2870874,4561.642952919006,0.013635697403515223
957958,1915918,957959,2873877,4566.692248106003,0.013616412947158096
958959,1917920,958960,2876880,4571.783644914627,0.013597691042377846
959960,1919922,959961,2879883,4576.915172100067,0.01357834760165133
960961,1921924,960962,2882886,4582.020961046219,0.013559566465119133
961962,1923926,961963,2885889,4587.100341081619,0.013540189203922637
962963,1925928,962964,2888892,4592.1946840286255,0.013521358330763178
963964,1927930,963965,2891895,4597.277769088745,0.013503047406629776
964965,1929932,964966,2894898,4602.369556903839,0.013484580373187782
965966,1931934,965967,2897901,4607.4918830394745,0.01346570071655151
966967,1933936,966968,2900904,4612.5626718997955,0.013447053257550579
967968,1935938,967969,2903907,4617.533753156662,0.013427770480120671
968969,1937940,968970,2906910,4622.566130876541,0.013409364015387837
969970,1939942,969971,2909913,4627.662883043289,0.013391120599408168
970971,1941944,970972,2912916,4632.751710891724,0.01337333478841174
971972,1943946,971973,2915919,4637.705342054367,0.013354957865885808
972973,1945948,972974,2918922,4642.73305606842,0.01333652027642529
973974,1947950,973975,2921925,4647.766247034073,0.013318349809196661
974975,1949952,974976,2924928,4652.946713924408,0.013300056149091688
975976,1951954,975977,2927931,4658.085014104843,0.013281990361065255
976977,1953956,976978,2930934,4663.202142953873,0.0132636335438292
977978,1955958,977979,2933937,4668.257688999176,0.013245369496871717
978979,1957960,978980,2936940,4673.34935593605,0.013227413361164508
979980,1959962,979981,2939943,4678.409354925156,0.01320918763121881
980981,1961964,980982,2942946,4683.492333173752,0.013191154957894469
981982,1963966,981983,2945949,4688.6017780303955,0.013172833843782428
982983,1965968,982984,2948952,4693.656134843826,0.013154374362784438
983984,1967970,983985,2951955,4698.720791101456,0.013136908972228412
984985,1969972,984986,2954958,4703.769487142563,0.013118996857883758
985986,1971974,985987,2957961,4709.264213085175,0.013101335749524878
986987,1973976,986988,2960964,4714.362923145294,0.013083759789878968
987988,1975978,987989,2963967,4719.4905071258545,0.013066122961390647
988989,1977980,988990,2966970,4724.595649957657,0.013048490749497432
989990,1979982,989991,2969973,4729.699789047241,0.013030834859819151
990991,1981984,990992,2972976,4734.866631031036,0.013012743198487442
991992,1983986,991993,2975979,4739.99410200119,0.012995333854632918
992993,1985988,992994,2978982,4745.122359991074,0.01297767075629963
993994,1987990,993995,2981985,4750.418992996216,0.012960078045580303
994995,1989992,994996,2984988,4755.540995121002,0.01294264793250477
995996,1991994,995997,2987991,4760.665301084518,0.01292502881551627
996997,1993996,996998,2990994,4765.802766084671,0.012907340180390747
997998,1995998,997999,2993997,4771.116171121597,0.012890412088381709
998999,1998000,999000,2997000,4776.185784101486,0.012873223600763595
1000000,2000002,1000001,3000003,4781.300567150116,0.012855969429438119


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0041158199310302734,12064.44795143716
1001,2003,2002,4005,3.324941635131836,17.92880950331164
2002,4005,4004,8009,6.630133867263794,16.401999899311704
3003,6007,6006,12013,10.223201990127563,15.070671778463293
4004,8009,8008,16017,13.486610889434814,13.902342173496436
5005,10011,10010,20021,16.71485686302185,12.871259313851624
6006,12013,12012,24025,20.087517976760864,11.956797952941997
7007,14015,14014,28029,23.67992377281189,11.142266176926569
8008,16017,16016,32033,27.441759824752808,10.413826686319226
9009,18019,18018,36037,30.956442832946777,9.760046656858322
10010,20021,20020,40041,34.775346755981445,9.171386866471948
11011,22023,22022,44045,38.70197296142578,8.639782031601499
12012,24025,24024,48049,42.04182505607605,8.158381768433173
13013,26027,26026,52053,46.04702591896057,7.721333615045296
14014,28029,28028,56057,50.85399079322815,7.323603309418104
15015,30031,30030,60061,54.865328788757324,6.960836875367022
16016,32033,32032,64065,59.13472366333008,6.629250251957274
17017,34035,34034,68069,63.31971788406372,6.3255402110498835
18018,36037,36036,72073,67.14822196960449,6.046811860220259
19019,38039,38038,76077,70.96784996986389,5.790519169438994
20020,40041,40040,80081,76.05370378494263,5.55441580515253
21021,42043,42042,84085,80.11780667304993,5.336514185966735
22022,44045,44044,88089,84.58468580245972,5.135051147446575
23023,46047,46046,92093,88.50550174713135,4.948458960898279
24024,48049,48048,96097,92.02466893196106,4.77534072236449
25025,50051,50050,100101,95.72560000419617,4.614449335365862
26026,52053,52052,104105,99.34877276420593,4.464669470045919
27027,54055,54054,108109,102.66942572593689,4.325002004370617
28028,56057,56056,112113,106.3328697681427,4.194550548676489
29029,58059,58058,116117,109.63951373100281,4.072509729601734
30030,60061,60060,120121,113.11764788627625,3.9581549682989134
31031,62063,62062,124125,116.5249457359314,3.850833534499543
32032,64065,64064,128129,119.72111582756042,3.7499566952210444
33033,66067,66066,132133,123.18446278572083,3.6549960559823376
34034,68069,68068,136137,127.53291082382202,3.5654789983273076
35035,70071,70070,140141,131.82025861740112,3.48095852951883
36036,72073,72072,144145,136.16951179504395,3.401040469940199
37037,74075,74074,148149,140.3315508365631,3.3253672696118883
38038,76077,76076,152153,144.3822226524353,3.2536142538538115
39039,78079,78078,156157,148.35342693328857,3.1854862845193566
40040,80081,80080,160161,152.07024002075195,3.12071478695907
41041,82083,82082,164165,156.2957158088684,3.0590550995293597
42042,84085,84084,168169,160.0401737689972,3.0002841079913196
43043,86087,86086,172173,163.79556584358215,2.944198131977828
44044,88089,88088,176177,167.36362481117249,2.8906110348489165
45045,90091,90090,180181,171.55208587646484,2.839352531671466
46046,92093,92092,184185,175.83548998832703,2.790266673255246
47047,94095,94094,188189,180.2948169708252,2.7432104867111775
48048,96097,96096,192193,184.3102147579193,2.6980527553678257
49049,98099,98098,196197,188.35195064544678,2.6546729228812183
50050,100101,100100,200201,191.87412190437317,2.6129601080592693
51051,102103,102102,204205,195.75852489471436,2.5728122185937536
52052,104105,104104,208209,199.43206882476807,2.5341351530551037
53053,106107,106106,212213,203.36970806121826,2.4968420819113817
54054,108109,108108,216217,206.70710277557373,2.4608527991731535
55055,110111,110110,220221,210.3947787284851,2.426094178099447
56056,112113,112112,224225,214.15370178222656,2.3924973407592915
57057,114115,114114,228229,218.60742092132568,2.3599977922349353
58058,116117,116116,232233,222.77012491226196,2.3285365085448575
59059,118119,118118,236237,226.79618096351624,2.2980586779831356
60060,120121,120120,240241,230.12700176239014,2.2685133439390484
61061,122123,122122,244245,233.8624119758606,2.2398530838327133
62062,124125,124124,248249,237.82881379127502,2.2120337177875626
63063,126127,126126,252253,241.49989295005798,2.18501404412018
64064,128129,128128,256257,245.23371386528015,2.1587555990008696
65065,130131,130130,260261,248.8006546497345,2.1332224378129467
66066,132133,132132,264265,252.577565908432,2.108380936218964
67067,134135,134134,268269,256.91417384147644,2.084199608894778
68068,136137,136136,272273,260.4874439239502,2.060648944305285
69069,138139,138138,276277,264.47605085372925,2.0377012539447605
70070,140141,140140,280281,268.16710591316223,2.0153305346648267
71071,142143,142142,284285,271.82746291160583,1.993512342860413
72072,144145,144144,288289,275.6107017993927,1.9722236793841148
73073,146147,146146,292293,279.2464928627014,1.951442884208518
74074,148149,148148,296297,282.7101628780365,1.9311495398887928
75075,150151,150150,300301,286.18091797828674,1.911324383065221
76076,152153,152152,304305,289.49778985977173,1.8919492232271296
77077,154155,154154,308309,292.97616481781006,1.8730068681143166
78078,156157,156156,312313,296.9077696800232,1.8544810551120463
79079,158159,158158,316317,300.66420578956604,1.8363563881612208
80080,160161,160160,320321,303.91416788101196,1.8186182796343928
81081,162163,162162,324325,307.1186807155609,1.8012528967847174
82082,164165,164164,328329,310.3492269515991,1.7842471123440191
83083,166167,166166,332333,313.6125648021698,1.7675884589152702
84084,168169,168168,336337,317.30382895469666,1.7512650868393393
85085,170171,170170,340341,320.7290508747101,1.7352680557069107
86086,172173,172172,344345,324.80642676353455,1.7195843450936081
87087,174175,174174,348349,328.9288697242737,1.7042035396716528
88088,176177,176176,352353,332.7513380050659,1.689115905761355
89089,178179,178178,356357,336.619993686676,1.6743121591498493
90090,180181,180180,360361,341.02839970588684,1.6597834384137968
91091,182183,182182,364365,344.8284306526184,1.645521280112007
92092,184185,184184,368369,348.0961380004883,1.631517595727928
93093,186187,186186,372373,351.4033269882202,1.6177646502110292
94094,188189,188188,376377,354.8166558742523,1.6042550419915642
95095,190191,190190,380381,358.0861837863922,1.5909816843413864
96096,192193,192192,384385,361.6288409233093,1.5779377880044194
97097,194195,194194,388389,365.25761580467224,1.5651168449712713
98098,196197,196196,392393,368.90152978897095,1.5525126133215963
99099,198199,198198,396397,372.5045759677887,1.5401191030505288
100100,200201,200200,400401,375.78626465797424,1.527930562824622
101101,202203,202202,404405,379.2514708042145,1.5159414675545122
102102,204205,204204,408409,382.9693019390106,1.5041465067697573
103103,206207,206206,412413,386.5322186946869,1.4925405737230903
104104,208209,208208,416417,390.09463381767273,1.4811187551531475
105105,210211,210210,420421,393.40246391296387,1.4698763216802035
106106,212213,212212,424425,396.6301517486572,1.4588087187821657
107107,214215,214214,428429,400.2193078994751,1.4479115583144448
108108,216217,216216,432433,403.4312677383423,1.4371806105209544
109109,218219,218218,436437,406.6360728740692,1.4266117965325975
110110,220221,220220,440441,409.825532913208,1.4162011812804849
111111,222223,222222,444445,413.05437898635864,1.4059449668202433
112112,224225,224224,448449,416.2739977836609,1.3958394860655972
113113,226227,226226,452453,419.4558298587799,1.3858811968220834
114114,228229,228228,456457,422.6840350627899,1.376066676202754
115115,230231,230230,460461,425.90293192863464,1.3663926153112698
116116,232233,232232,464465,429.1213538646698,1.3568558142560505
117117,234235,234234,468469,432.3138370513916,1.3474531773990748
118118,236237,236236,472473,435.5760450363159,1.3381817088811658
119119,238239,238238,476477,438.81749081611633,1.3290385083746514
120120,240241,240240,480481,442.1486117839813,1.3200207670543023
121121,242243,242242,484485,445.3962998390198,1.3111257637920062
122122,244245,244244,488489,448.5914077758789,1.3023508615460742
123123,246247,246246,492493,451.800345659256,1.2936935039178934
124124,248249,248248,496497,454.9857647418976,1.2058881962057058
125125,250251,250250,500501,458.18637681007385,1.1984658891433355
126126,252253,252252,504505,461.6445598602295,1.191133968279246
127127,254255,254254,508509,464.91990971565247,1.1838907270266645
128128,256257,256256,512513,468.2354938983917,1.1767345040207147
129129,258259,258258,516517,472.9939639568329,1.1696636815649981
130130,260261,260260,520521,477.83856678009033,1.1626766841054632
131131,262263,262262,524525,482.7037079334259,1.1557719767952221
132132,264265,264264,528529,486.6636378765106,1.1489480640902912
133133,266267,266266,532533,490.45665669441223,1.142203488458108
134134,268269,268268,536537,494.02960205078125,1.1355368290678598
135135,270271,270270,540541,497.6901879310608,1.1289467006063205
136136,272273,272272,544545,500.9822647571564,1.1224317520864133
137137,274275,274274,548549,504.4122910499573,1.1159906657485408
138138,276277,276276,552553,507.9495987892151,1.1096221559782862
139139,278279,278278,556557,511.2153947353363,1.1033249682732276
140140,280281,280280,560561,514.5224659442902,1.0970978782679595
141141,282283,282282,564565,517.7735288143158,1.0909396907627524
142142,284285,284284,568569,520.9895269870758,1.0848492388395243
143143,286287,286286,572573,524.1599490642548,1.0788253829614405
144144,288289,288288,576577,527.635321855545,1.0728670101452735
145145,290291,290290,580581,531.0791099071503,1.0669730331446772
146146,292293,292292,584585,534.7461287975311,1.0611423896771157
147147,294295,294294,588589,539.8920576572418,1.0553740416671644
148148,296297,296296,592593,543.435183763504,1.0496669745298277
149149,298299,298298,596597,546.7762968540192,1.0440201964811422
150150,300301,300300,600601,550.2225368022919,1.0384327378560556
151151,302303,302302,604605,553.8503308296204,1.0329036504735996
152152,304305,304304,608609,557.2358620166779,1.02743200702389
153153,306307,306306,612613,560.4129078388214,1.022016900449671
154154,308309,308308,616617,563.6492767333984,1.016657443382428
155155,310311,310310,620621,567.7310807704926,1.0113527675894147
156156,312313,312312,624625,572.3401217460632,1.0061020234279567
157157,314315,314314,628629,577.3512289524078,1.0009043793288583
158158,316317,316316,632633,581.032461643219,0.9957590213089134
159159,318319,318318,636637,584.3221907615662,0.9906651524652261
160160,320321,320320,640641,587.8244769573212,0.985621992533197
161161,322323,322322,644645,591.7850968837738,0.9806287774190423
162162,324325,324324,648649,595.5266859531403,0.9756847587741504
163163,326327,326326,652653,599.6498627662659,0.9707892035712575
164164,328329,328328,656657,604.208646774292,0.965941393706089
165165,330331,330330,660661,608.923811674118,0.9611406255789916
166166,332333,332332,664665,612.881454706192,0.9563862097511446
167167,334335,334334,668669,616.5729279518127,0.9516774705534772
168168,336337,336336,672673,620.6299998760223,0.9470137457337842
169169,338339,338338,676677,625.1332867145538,0.9423943861129374
170170,340341,340340,680681,628.8158609867096,0.9378187552629242
171171,342343,342342,684685,632.2945778369904,0.933286229166697
172172,344345,344344,688689,635.7035520076752,0.9287961959198583
173173,346347,346346,692693,639.0017538070679,0.924348055414157
174174,348349,348348,696697,642.5461559295654,0.9199412190591829
175175,350351,350350,700701,646.2068059444427,0.9155751094895095
176176,352353,352352,704705,650.5352230072021,0.9112491602882073
177177,354355,354354,708709,653.9783086776733,0.9069628157230909
178178,356357,356356,712713,658.8707618713379,0.9027155304866028
179179,358359,358358,716717,663.6995067596436,0.8985067694466125
180180,360361,360360,720721,668.5300738811493,0.8943360073972144
181181,362363,362362,724725,672.9234209060669,0.8902027288295358
182182,364365,364364,728729,676.8934090137482,0.8861064276970865
183183,366367,366366,732733,681.7767198085785,0.8820466071865667
184184,368369,368368,736737,686.706536769867,0.8780227795232349
185185,370371,370370,740741,690.308671951294,0.8740344657362584
186186,372373,372372,744745,693.8199667930603,0.8700811954713572
187187,374375,374374,748749,698.2579047679901,0.8661625067816203
188188,376377,376376,752753,702.2339887619019,0.8622779459437879
189189,378379,378378,756757,705.7588078975677,0.8584270672672574
190190,380381,380380,760761,709.497368812561,0.8546094329121843
191191,382383,382382,764765,713.5711879730225,0.8508246127112216
192192,384385,384384,768769,718.0500726699829,0.8470721840039914
193193,386387,386386,772773,721.9442648887634,0.8433517314606434
194194,388389,388388,776777,726.0648078918457,0.83966284692724
195195,390391,390390,780781,731.680253982544,0.8360051292675053
196196,392393,392392,784785,735.4549238681793,0.8323781842045719
197197,394395,394394,788789,738.8122527599335,0.8287816241700057
198198,396397,396396,792793,742.8294429779053,0.8006585201146663
199199,398399,398398,796797,747.5361127853394,0.7973228817372728
200200,400401,400400,800801,751.9038078784943,0.7940140466398589
201201,402403,402402,804805,755.4648959636688,0.790731693017733
202202,404405,404404,808809,758.8297426700592,0.7874755042375909
203203,406407,406406,812813,762.526930809021,0.7842451687556604
204204,408409,408408,816817,766.5029847621918,0.7810403799903725
205205,410411,410410,820821,770.5114579200745,0.7778608362368686
206206,412413,412412,824825,774.3705847263336,0.7747062405578617
207207,414415,414414,828829,778.3196406364441,0.7715763007017813
208208,416417,416416,832833,782.0509879589081,0.7684707289954531
209209,418419,418418,836837,785.807089805603,0.7653892422640638
210210,420421,420420,840841,789.129576921463,0.7623315617347544
211211,422423,422422,844845,792.8498718738556,0.7592974129565846
212212,424425,424424,848849,796.6503069400787,0.7562865257023077
213213,426427,426426,852853,800.4470720291138,0.7532986339065246
214214,428429,428428,856857,804.5177438259125,0.7503334755710966
215215,430431,430430,860861,808.843475818634,0.7473907926887478
216216,432433,432432,864865,813.6537280082703,0.7444703311630292
217217,434435,434434,868869,817.6274697780609,0.7415718407410168
218218,436437,436436,872873,821.996090888977,0.7386950749405514
219219,438439,438438,876877,826.4506378173828,0.7358397909683845
220220,440441,440440,880881,830.9624879360199,0.7330057496583322
221221,442443,442442,884885,835.2373778820038,0.7301927153985162
222222,444445,444444,888889,839.5415060520172,0.7274004560713365
223223,446447,446446,892893,843.3176918029785,0.7246287429843505
224224,448449,448448,896897,847.1073698997498,0.7218773507993319
225225,450451,450450,900901,852.0985679626465,0.7191460574849771
226226,452453,452452,904905,857.6403877735138,0.7164346442441456
227227,454455,454454,908909,862.0304179191589,0.7137428954592906
228228,456457,456456,912913,866.2176048755646,0.7110706113708147
229229,458459,458458,916917,870.1368708610535,0.7084176078114979
230230,460461,460460,920921,874.3818647861481,0.7057836423027766
231231,462463,462462,924925,878.2574646472931,0.7031685113088315
232232,464465,464464,928929,883.5893890857697,0.7005720141951315
233233,466467,466466,932933,887.5309250354767,0.6979939531720447
234234,468469,468468,936937,891.0923347473145,0.69543413325664
235235,470471,470470,940941,894.8885507583618,0.6928923622126604
236236,472473,472472,944945,898.7092039585114,0.6903684505032288
237237,474475,474474,948949,902.453795671463,0.687862211249012
238238,476477,476476,952953,906.0678288936615,0.6853734601718315
239239,478479,478478,956957,910.1148347854614,0.6829020155528269
240240,480481,480480,960961,913.9672248363495,0.6804476981978951
241241,482483,482482,964965,917.9687879085541,0.6780103313740256
242242,484485,484484,968969,921.9592278003693,0.6755897407892917
243243,486487,486486,972973,925.6251268386841,0.673185754523729
244244,488489,488488,976977,929.1665637493134,0.6707982030166022
245245,490491,490490,980981,933.034717798233,0.6684269190118357
246246,492493,492492,984985,936.5925559997559,0.6660717375089007
247247,494495,494494,988989,940.1783969402313,0.6637324957537203
248248,496497,496496,992993,944.2013058662415,0.661409033162272
249249,498499,498498,996997,948.4024839401245,0.6591011913187685
250250,500501,500500,1001001,952.173889875412,0.6568088139156316
251251,502503,502502,1005005,956.2669937610626,0.6545317467353016
252252,504505,504504,1009009,959.8834018707275,0.6522698375993059
253253,506507,506506,1013013,963.2590379714966,0.6500229363446124
254254,508509,508508,1017017,967.0817520618439,0.6477908947890683
255255,510511,510510,1021021,970.8757948875427,0.6455735666968394
256256,512513,512512,1025025,974.6752030849457,0.6433708077438496
257257,514515,514514,1029029,978.2858469486237,0.6411824754923146
258258,516517,516516,1033033,981.8917548656464,0.6390084293543623
259259,518519,518518,1037037,985.7488157749176,0.6368485305683862
260260,520521,520520,1041041,989.1861748695374,0.6347026421608462
261261,522523,522522,1045045,992.4754590988159,0.6325706289244408
262262,524525,524524,1049049,995.7813267707825,0.6304523573817278
263263,526527,526526,1053053,999.3207778930664,0.6283476957742096
264264,528529,528528,1057057,1002.9319317340851,0.62625651401504
265265,530531,530530,1061061,1006.2803666591644,0.6241786836671963
266266,532533,532532,1065065,1009.9811868667603,0.6221140779271082
267267,534535,534534,1069069,1013.9625227451324,0.6200664479729312
268268,536537,536536,1073073,1018.9425799846649,0.6180325114873995
269269,538539,538538,1077077,1023.6329107284546,0.6160115079728712
270270,540541,540540,1081081,1027.6393427848816,0.6140032741277537
271271,542543,542542,1085085,1032.5578680038452,0.612007665235069
272272,544545,544544,1089089,1036.5431008338928,0.6100245481538877
273273,546547,546546,1093093,1040.628928899765,0.6080537972666207
274274,548549,548548,1097097,1044.3775389194489,0.6060952920797718
275275,550551,550550,1101101,1047.738163948059,0.6041489158014883
276276,552553,552552,1105105,1052.357260942459,0.6022145544284285
277277,554555,554554,1109109,1056.2178449630737,0.6002920962146163
278278,556557,556556,1113113,1059.5908846855164,0.5983814313203766
279279,558559,558558,1117117,1064.7304317951202,0.5964824515740474
280280,560561,560560,1121121,1068.1757838726044,0.5945989224783261
281281,562563,562562,1125125,1071.9927887916565,0.592727324412408
282282,564565,564564,1129129,1075.5849568843842,0.5908671640045213
283283,566567,566566,1133133,1079.1380050182343,0.589018285030761
284284,568569,568568,1137137,1084.83500790596,0.587180562901267
285285,570571,570570,1141141,1089.4366698265076,0.5853538873197976
286286,572573,572572,1145145,1094.51238489151,0.5835381549222802
287287,574575,574574,1149149,1098.6729667186737,0.5817332660644752
288288,576577,576576,1153153,1102.105204820633,0.5799391234213545
289289,578579,578578,1157157,1106.4149029254913,0.5781556313340843
290290,580581,580580,1161161,1110.857988834381,0.57638269553172
291291,582583,582582,1165165,1114.5154139995575,0.5746202229674964
292292,584585,584584,1169169,1118.6037440299988,0.5728681217588019
293293,586587,586586,1173173,1122.8781349658966,0.5711263011271512
294294,588589,588588,1177177,1127.0753998756409,0.569394671379996
295295,590591,590590,1181181,1130.9752397537231,0.5676731438688876
296296,592593,592592,1185185,1135.4399280548096,0.5659616309876583
297297,594595,594594,1189189,1139.8837478160858,0.5642600461487746
298298,596597,596596,1193193,1143.6044127941132,0.562568303756052
299299,598599,598598,1197197,1148.0008687973022,0.5608863192082936
300300,600601,600600,1201201,1152.5375957489014,0.5592140088720043
301301,602603,602602,1205205,1156.7624158859253,0.557551290061383
302302,604605,604604,1209209,1160.770537853241,0.5558980810383218
303303,606607,606606,1213213,1165.1745216846466,0.5542543009887595
304304,608609,608608,1217217,1169.6184928417206,0.5526198700154055
305305,610611,610610,1221221,1174.0004658699036,0.550994709114093
306306,612613,612612,1225225,1178.324185848236,0.5493787401737791
307307,614615,614614,1229229,1182.2744088172913,0.5477718859565357
308308,616617,616616,1233233,1185.8036358356476,0.5461740700829978
309309,618619,618618,1237237,1189.2868168354034,0.5445852170305443
310310,620621,620620,1241241,1193.5482187271118,0.5430052521096513
311311,622623,622622,1245245,1198.021714925766,0.5414341014566162
312312,624625,624624,1249249,1202.3812339305878,0.5398716920262814
313313,626627,626626,1253253,1206.624452829361,0.5383179515720258
314314,628629,628628,1257257,1210.6311378479004,0.5367728086475836
315315,630631,630630,1261261,1214.682848930359,0.5352361925797595
316316,632633,632632,1265265,1219.0255496501923,0.5337080334684288
317317,634635,634634,1269269,1223.4383099079132,0.5321882621774421
318318,636637,636636,1273273,1227.872309923172,0.5306768103182549
319319,638639,638638,1277277,1231.9106287956238,0.5291736102390132
320320,640641,640640,1281281,1235.9528419971466,0.5276785950245539
321321,642643,642642,1285285,1239.651175737381,0.5261916984727577
322322,644645,644644,1289289,1243.2435009479523,0.524712855098187
323323,646647,646646,1293293,1246.887461900711,0.5232420001102582
324324,648649,648648,1297297,1250.5796809196472,0.5217790694132418
325325,650651,650650,1301301,1254.0643157958984,0.5203239995935292
326326,652653,652652,1305305,1257.6226449012756,0.5188767279105377
327327,654655,654654,1309309,1261.3220298290253,0.5174371922857972
328328,656657,656656,1313313,1264.8095967769623,0.5160053312956734
329329,658659,658658,1317317,1268.262764930725,0.5145810841713683
330330,660661,660660,1321321,1271.8544147014618,0.5131643907734542
331331,662663,662662,1325325,1276.769453048706,0.5117551915955119
332332,664665,664664,1329329,1281.7848727703094,0.5103534277532162
333333,666667,666666,1333333,1287.2740919589996,0.5089590409752418
334334,668669,668668,1337337,1292.098040819168,0.5075719735978055
335335,670671,670670,1341341,1296.275075674057,0.5061921685537527
336336,672673,672672,1345345,1300.1250019073486,0.5048195693598245
337337,674675,674674,1349349,1303.580547094345,0.5034541201312095
338338,676677,676676,1353353,1307.7742857933044,0.5020957655415259
339339,678679,678678,1357357,1315.721935749054,0.5007444508391927
340340,680681,680680,1361361,1320.444816827774,0.49940012183287763
341341,682683,682682,1365365,1325.2421298027039,0.4980627248842211
342342,684685,684684,1369369,1329.656350851059,0.4967322068987414
343343,686687,686686,1373373,1335.575157880783,0.4954085153294727
344344,688689,688688,1377377,1339.6985578536987,0.4940915981460421
345345,690691,690690,1381381,1343.9325637817383,0.49278140386195446
346346,692693,692692,1385385,1347.9146358966827,0.4914778814982128
347347,694695,694694,1389389,1352.0370228290558,0.4901809805905941
348348,696697,696696,1393393,1357.4650647640228,0.4888906511805544
349349,698699,698698,1397397,1362.3820507526398,0.4876068438115908
350350,700701,700700,1401401,1367.7355320453644,0.48632950951832754
351351,702703,702702,1405405,1372.339558839798,0.485058599830154
352352,704705,704704,1409409,1376.4531137943268,0.48379406674393977
353353,706707,706706,1413413,1382.4526557922363,0.4825358627440437
354354,708709,708708,1417417,1387.7686078548431,0.4812839407786669
355355,710711,710710,1421421,1392.1185657978058,0.4800382542616717
356356,712713,712712,1425425,1396.5254809856415,0.4787987570671248
357357,714715,714714,1429429,1400.9866807460785,0.4775654035147454
358358,716717,716716,1433433,1406.0982458591461,0.4763381483753619
359359,718719,718718,1437437,1411.6822409629822,0.47511694686545525
360360,720721,720720,1441441,1416.2734189033508,0.47390175463078776
361361,722723,722722,1445445,1420.8931000232697,0.4726925277518603
362362,724725,724724,1449449,1425.4123587608337,0.4714892227311793
363363,726727,726726,1453453,1431.0877847671509,0.47029179649871367
364364,728729,728728,1457457,1436.5228867530823,0.4691002063882479
365365,730731,730730,1461461,1442.044564962387,0.4679144101555721
366366,732733,732732,1465465,1447.8734579086304,0.46673436595847306
367367,734735,734734,1469469,1452.9658377170563,0.4655600323494582
368368,736737,736736,1473473,1458.1136498451233,0.4643913682866696
369369,738739,738738,1477477,1463.0914158821106,0.46322833311023714
370370,740741,740740,1481481,1468.2335050106049,0.4620708865550114
371371,742743,742742,1485485,1475.2202229499817,0.46091898872509773
372372,744745,744744,1489489,1481.5091440677643,0.4597726001211413
373373,746747,746746,1493493,1487.6842679977417,0.4586316815984901
374374,748749,748748,1497497,1494.4154307842255,0.457496194392661
375375,750751,750750,1501501,1500.6838960647583,0.45636610009751166
376376,752753,752752,1505505,1507.2555058002472,0.45524136066887877
377377,754755,754754,1509509,1514.7166168689728,0.45412193841912085
378378,756757,756756,1513513,1521.6667687892914,0.4530077960098424
379379,758759,758758,1517517,1527.1572227478027,0.45189889645371295
380380,760761,760760,1521521,1533.4854528903961,0.45079520310173393
381381,762763,762762,1525525,1540.0162868499756,0.4496966796468769
382382,764765,764764,1529529,1544.4858798980713,0.4486032901240833
383383,766767,766766,1533533,1549.5390558242798,0.44751499888661783
384384,768769,768768,1537537,1554.6188459396362,0.44643177063153416
385385,770771,770770,1541541,1559.3165807724,0.44535357036329515
386386,772773,772772,1545545,1563.2846639156342,0.4442803634210577
387387,774775,774774,1549549,1566.9910509586334,0.4432121154568449
388388,776777,776776,1553553,1570.8058428764343,0.4421487924282701
389389,778779,778778,1557557,1574.4296338558197,0.4410903606094507
390390,780781,780780,1561561,1578.0822179317474,0.4400367865800945
391391,782783,782782,1565565,1582.1022758483887,0.4389880372254993
392392,784785,784784,1569569,1586.2350850105286,0.43794407972200133
393393,786787,786786,1573573,1590.2301638126373,0.4369048815497081
394394,788789,788788,1577577,1594.7154307365417,0.4358704104779463
395395,790791,790790,1581581,1598.8912320137024,0.43484063455980504
396396,792793,792792,1585585,1603.030954837799,0.4338155221485067
397397,794795,794794,1589589,1606.7308809757233,0.4327950418664841
398398,796797,796796,1593593,1610.7494938373566,0.4317791626217513
399399,798799,798798,1597597,1614.650382757187,0.43076785359880887
400400,800801,800800,1601601,1619.0070457458496,0.4297610842531867
401401,802803,802802,1605605,1623.0202569961548,0.42875882431690115
402402,804805,804804,1609609,1627.102255821228,0.427761043780265
403403,806807,806806,1613613,1632.5093927383423,0.42676771289370663
404404,808809,808808,1617617,1636.949308872223,0.4257788021641318
405405,810811,810810,1621621,1640.6492178440094,0.42479428235674277
406406,812813,812812,1625625,1644.2109627723694,0.4238141244950384
407407,814815,814814,1629629,1647.768905878067,0.422838299857176
408408,816817,816816,1633633,1651.7398090362549,0.4218667799686955
409409,818819,818818,1637637,1656.2286348342896,0.42089953661161417
410410,820821,820820,1641641,1660.5043478012085,0.4199365418062371
411411,822823,822822,1645645,1664.8841667175293,0.41897776781843277
412412,824825,824824,1649649,1668.6724858283997,0.4180231871559954
413413,826827,826826,1653653,1672.7822136878967,0.41707277256500674
414414,828829,828828,1657657,1677.6370527744293,0.4161264970243792
415415,830831,830830,1661661,1682.5661268234253,0.41518433374585584
416416,832833,832832,1665665,1687.511513710022,0.41424625617401034
417417,834835,834834,1669669,1691.517413854599,0.4133122379771521
418418,836837,836836,1673673,1695.366348028183,0.4123822530509642
419419,838839,838838,1677677,1699.3428909778595,0.4114562755148654
420420,840841,840840,1681681,1703.0434937477112,0.4105342797065532
421421,842843,842842,1685685,1706.8292388916016,0.4096162401856418
422422,844845,844844,1689689,1710.4723420143127,0.40870213172456715
423423,846847,846846,1693693,1714.2975406646729,0.40779192930313
424424,848849,848848,1697697,1717.88631772995,0.40688560812486685
425425,850851,850850,1701701,1721.6449069976807,0.4059831435952219
426426,852853,852852,1705705,1725.2954549789429,0.4050845113233663
427427,854855,854854,1709709,1729.452096939087,0.4041896871276549
428428,856857,856856,1713713,1733.0219948291779,0.40329864703198837
429429,858859,858858,1717717,1736.5907068252563,0.4024113672476233
430430,860861,860860,1721721,1740.1389858722687,0.40152782420227595
431431,862863,862862,1725725,1743.5231947898865,0.4006479945019237
432432,864865,864864,1729729,1747.0380239486694,0.3997718549599085
433433,866867,866866,1733733,1750.5632908344269,0.3988993825732905
434434,868869,868868,1737737,1754.2332339286804,0.39803055453194247
435435,870871,870870,1741741,1757.8466589450836,0.3971653482167312
436436,872873,872872,1745745,1761.7935569286346,0.39630374118860345
437437,874875,874874,1749749,1765.9667358398438,0.3954457111976808
438438,876877,876876,1753753,1770.7700617313385,0.3945912361759838
439439,878879,878878,1757757,1775.1647357940674,0.393740294231975
440440,880881,880880,1761761,1778.788004875183,0.3928928636596538
441441,882883,882882,1765765,1782.7751557826996,0.39204892292036675
442442,884885,884884,1769769,1786.7211277484894,0.3912084506573592
443443,886887,886886,1773773,1790.5766878128052,0.3903714256848616
444444,888889,888888,1777777,1794.8417909145355,0.3895378269953653
445445,890891,890890,1781781,1799.8997039794922,0.38870763373415684
446446,892893,892892,1785785,1804.2881426811218,0.3878808252320596
447447,894895,894894,1789789,1807.9331016540527,0.387057380978149
448448,896897,896896,1793793,1812.4253330230713,0.38623728062702867
449449,898899,898898,1797797,1816.705058813095,0.3854205039970111
450450,900901,900900,1801801,1821.607677936554,0.384607031064661
451451,902903,902902,1805805,1826.7935559749603,0.38379684197388997
452452,904905,904904,1809809,1832.050853729248,0.38298991701594787
453453,906907,906906,1813813,1836.97913980484,0.38218623664761253
454454,908909,908908,1817817,1841.4663848876953,0.3742215231377486
455455,910911,910910,1821821,1846.0782489776611,0.36149026241037063
456456,912913,912912,1825825,1850.652662038803,0.3607718103121442
457457,914915,914914,1829829,1855.9738428592682,0.36005609045787423
458458,916917,916916,1833833,1861.9441299438477,0.3593430873934267
459459,918919,918918,1837837,1867.5956008434296,0.35863278577926394
460460,920921,920920,1841841,1873.147864818573,0.3579251703922637
461461,922923,922922,1845845,1878.210881948471,0.3572202261275379
462462,924925,924924,1849849,1883.3109438419342,0.356517937978424
463463,926927,926926,1853853,1887.5685648918152,0.3558182910637697
464464,928929,928928,1857857,1891.9712717533112,0.3551212706024671
465465,930931,930930,1861861,1896.3279390335083,0.3544268619389186
466466,932933,932932,1865865,1901.5897808074951,0.353735050508476
467467,934935,934934,1869869,1906.2153708934784,0.35304582185926847
468468,936937,936936,1873873,1910.3317527770996,0.3523591616540216
469469,938939,938938,1877877,1914.1164968013763,0.3516750556482293
470470,940941,940940,1881881,1918.8843219280243,0.35099348971198197
471471,942943,942942,1885885,1923.4185328483582,0.3503144498135953
472472,944945,944944,1889889,1927.5844378471375,0.3496379220250674
473473,946947,946946,1893893,1931.6891477108002,0.3489638925238978
474474,948949,948948,1897897,1935.4539608955383,0.34829234758035454
475475,950951,950950,1901901,1939.6212847232819,0.34762327357202594
476476,952953,952952,1905905,1943.6794559955597,0.3469566569710878
477477,954955,954954,1909909,1947.241882801056,0.3462924843533983
478478,956957,956956,1913913,1950.7584340572357,0.3456307423821272
479479,958959,958958,1917917,1954.743379831314,0.34497141782594554
480480,960961,960960,1921921,1958.3609399795532,0.34431449754447385
481481,962963,962962,1925925,1962.4050376415253,0.34365996849373914
482482,964965,964964,1929929,1966.1609318256378,0.34300781772253686
483483,966967,966966,1933933,1970.242925643921,0.3423580323706119
484484,968969,968968,1937937,1974.7275698184967,0.34171059967593465
485485,970971,970970,1941941,1978.7310078144073,0.34106550695651094
486486,972973,972972,1945945,1982.926727771759,0.34042274163584807
487487,974975,974974,1949949,1987.2708768844604,0.33978229121203185
488488,976977,976976,1953953,1991.5768308639526,0.33914414328319253
489489,978979,978978,1957957,1995.6968667507172,0.3385082855311339
490490,980981,980980,1961961,2000.8932490348816,0.33787470572315215
491491,982983,982982,1965965,2005.84791970253,0.3372433917138551
492492,984985,984984,1969969,2010.0364758968353,0.33661433144516195
493493,986987,986986,1973973,2013.882917881012,0.3359875129444845
494494,988989,988988,1977977,2018.040312051773,0.33536292432290793
495495,990991,990990,1981981,2022.0556569099426,0.3347405537751911
496496,992993,992992,1985985,2026.8820238113403,0.33412038957249024
497497,994995,994994,1989989,2031.6968128681183,0.3335024200787302
498498,996997,996996,1993993,2036.2201647758484,0.33288663372877636
499499,998999,998998,1997997,2040.556412935257,0.33227301904662454
500501,1001003,1001002,2002005,2044.8325397968292,0.3316609548674023
501502,1003005,1003004,2006009,2049.225912809372,0.33105165154302085
502503,1005007,1005006,2010013,2052.8892107009888,0.3304444859131763
503504,1007009,1007008,2014017,2056.5206730365753,0.3298394468129118
504505,1009011,1009010,2018021,2060.2105028629303,0.3292365231554868
505506,1011013,1011012,2022025,2063.9766159057617,0.3286357039323775
506507,1013015,1013014,2026029,2067.5822677612305,0.32803697820600064
507508,1015017,1015016,2030033,2071.2226388454437,0.3274403351206274
508509,1017019,1017018,2034037,2075.085922718048,0.3268457638896507
509510,1019021,1019020,2038041,2078.6903989315033,0.32625325380104186
510511,1021023,1021022,2042045,2082.3156168460846,0.32566279422098887
511512,1023025,1023024,2046049,2085.9722168445587,0.3250743745811633
512513,1025027,1025026,2050053,2089.667641878128,0.32448798438781523
513514,1027029,1027028,2054057,2093.295697927475,0.3239036132235924
514515,1029031,1029030,2058061,2096.918212890625,0.3233212507348071
515516,1031033,1031032,2062065,2100.5289237499237,0.3227408866441692
516517,1033035,1033034,2066069,2104.1426360607147,0.32216251073623425
517518,1035037,1035036,2070073,2108.056923866272,0.32158611287377425
518519,1037039,1037038,2074077,2111.725907802582,0.32101168297958793
519520,1039041,1039040,2078081,2115.315244913101,0.32043921105105255
520521,1041043,1041042,2082085,2118.936168909073,0.319868687151029
521522,1043045,1043044,2086089,2122.875895023346,0.3193001014042238
522523,1045047,1045046,2090093,2127.429765701294,0.3187334440062841
523524,1047049,1047048,2094097,2131.5107576847076,0.3181687052219786
524525,1049051,1049050,2098101,2135.4526147842407,0.31760587537246465
525526,1051053,1051052,2102105,2139.231696844101,0.31704494484984025
526527,1053055,1053054,2106109,2143.6121039390564,0.316485904108049
527528,1055057,1055056,2110113,2147.1682460308075,0.31592874366651813
528529,1057059,1057058,2114117,2151.1298859119415,0.31537345410106354
529530,1059061,1059060,2118121,2154.9449458122253,0.3148200260584417
530531,1061063,1061062,2122125,2158.5591280460358,0.3142684502454358
531532,1063065,1063064,2126129,2162.2488429546356,0.31371871742157964
532533,1065067,1065066,2130133,2165.830778837204,0.3131708184209856
533534,1067069,1067068,2134137,2169.2973098754883,0.3126247441286978
534535,1069071,1069070,2138141,2172.7287118434906,0.31208048548796796
535536,1071073,1071072,2142145,2176.1484248638153,0.3115380335129885
536537,1073075,1073074,2146149,2179.58766579628,0.3109973792688834
537538,1075077,1075076,2150153,2183.6703717708588,0.3104585138771654
538539,1077079,1077078,2154157,2187.6244139671326,0.3099214285193739
539540,1079081,1079080,2158161,2191.064523935318,0.30938611443707487
540541,1081083,1081082,2162165,2195.3819057941437,0.30885256293004204
541542,1083085,1083084,2166169,2200.0529747009277,0.3083207653453428
542543,1085087,1085086,2170173,2205.1945729255676,0.30779071309916617
543544,1087089,1087088,2174177,2211.9050998687744,0.30726239765317587
544545,1089091,1089090,2178181,2218.477370738983,0.3067358105272433
545546,1091093,1091092,2182185,2225.1350107192993,0.30621094329944754
546547,1093095,1093094,2186189,2231.7545840740204,0.30568778759879933
547548,1095097,1095096,2190193,2236.9117319583893,0.30516633510524116
548549,1097099,1097098,2194197,2242.1501858234406,0.3046465775605611
549550,1099101,1099100,2198201,2248.6768786907196,0.30412850675566006
550551,1101103,1101102,2202205,2254.927337884903,0.3036121145287325
551552,1103105,1103104,2206209,2260.9818527698517,0.30309739277436165
552553,1105107,1105106,2210213,2266.31010389328,0.30258433344170044
553554,1107109,1107108,2214217,2270.8581218719482,0.30207292852901446
554555,1109111,1109110,2218221,2275.908758878708,0.30156317008368205
555556,1111113,1111112,2222225,2281.361030817032,0.3010550502076512
556557,1113115,1113114,2226229,2287.394870996475,0.3005485610483447
557558,1115117,1115116,2230233,2293.6209008693695,0.30004369480593596
558559,1117119,1117118,2234237,2299.455641746521,0.2995404437278921
559560,1119121,1119120,2238241,2305.75741481781,0.29903880011625006
560561,1121123,1121122,2242245,2311.863963842392,0.29853875631306437
561562,1123125,1123124,2246249,2318.4077808856964,0.29804030471495935
562563,1125127,1125126,2250253,2324.054884672165,0.29754343776221504
563564,1127129,1127128,2254257,2328.984248638153,0.29704814794968115
564565,1129131,1129130,2258261,2334.9620718955994,0.2965544278067682
565566,1131133,1131132,2262265,2339.81800699234,0.2960622699265514
566567,1133135,1133134,2266269,2344.827488899231,0.2955716669330286
567568,1135137,1135136,2270273,2349.520320892334,0.2950826115011296
568569,1137139,1137138,2274277,2354.11368393898,0.29459509635671566
569570,1139141,1139140,2278281,2358.6788268089294,0.294109114265666
570571,1141143,1141142,2282285,2363.3485958576202,0.2936246580375155
571572,1143145,1143144,2286289,2368.2870347499847,0.2931417205345497
572573,1145147,1145146,2290293,2373.081207036972,0.292660294649977
573574,1147149,1147148,2294297,2377.8714706897736,0.2921803733333945
574575,1149151,1149150,2298301,2381.834977865219,0.2917019495725981
575576,1151153,1151152,2302305,2385.60213971138,0.2912250163990393
576577,1153155,1153154,2306309,2389.3901488780975,0.2907495668860065
577578,1155157,1155156,2310313,2393.4639286994934,0.2902755941522628
578579,1157159,1157158,2314317,2397.699189901352,0.289803091356589
579580,1159161,1159160,2318321,2401.606738805771,0.28933205169960274
580581,1161163,1161162,2322325,2406.1934456825256,0.2888624684237584
581582,1163165,1163164,2326329,2410.4613387584686,0.28839433481698507
582583,1165167,1165166,2330333,2414.4073729515076,0.28792764419631567
583584,1167169,1167168,2334337,2418.23957490921,0.2874623899351718
584585,1169171,1169170,2338341,2423.2556779384613,0.28699856543607893
585586,1171173,1171172,2342345,2428.3553149700165,0.2865361641452182
586587,1173175,1173174,2346349,2434.433511734009,0.28607517955242656
587588,1175177,1175176,2350353,2438.482707977295,0.28561560518028273
588589,1177179,1177178,2354357,2444.335681915283,0.2851574345913832
589590,1179181,1179180,2358361,2448.8951008319855,0.28470066139016126
590591,1181183,1181182,2362365,2453.2339067459106,0.2842452792210679
591592,1183185,1183184,2366369,2459.01474404335,0.283791281761296
592593,1185187,1185186,2370373,2464.3572018146515,0.28333866273351305
593594,1187189,1187188,2374377,2469.67120885849,0.2828874158876715
594595,1189191,1189190,2378381,2474.6067218780518,0.2824375350246555
595596,1191193,1191192,2382385,2479.2544288635254,0.281989013967177
596597,1193195,1193194,2386389,2484.949017763138,0.2815418465870607
597598,1195197,1195196,2390393,2490.0826058387756,0.2810960267906921
598599,1197199,1197198,2394397,2494.5398037433624,0.28065154851174157
599600,1199201,1199200,2398401,2498.9406328201294,0.2802084057311731
600601,1201203,1201202,2402405,2503.236294746399,0.27976659245905466
601602,1203205,1203204,2406409,2507.4265546798706,0.27932610274729086
602603,1205207,1205206,2410413,2511.6113216876984,0.2788869306787092
603604,1207209,1207208,2414417,2515.46680188179,0.2784490703652409
604605,1209211,1209210,2418421,2519.8469178676605,0.2780125159606541
605606,1211213,1211212,2422425,2524.2970638275146,0.27757726165873464
606607,1213215,1213214,2426429,2528.5062787532806,0.27714330167691514
607608,1215217,1215216,2430433,2532.394630908966,0.2767106302708271
608609,1217219,1217218,2434437,2536.925117969513,0.27627924173066276
609610,1219221,1219220,2438441,2540.9458050727844,0.2758491303775372
610611,1221223,1221222,2442445,2545.6947009563446,0.27542029057076434
611612,1223225,1223224,2446449,2551.0204207897186,0.27499271669330483
612613,1225227,1225226,2450453,2555.305030822754,0.27456640317359415
613614,1227229,1227228,2454457,2558.986738920212,0.27414134446371463
614615,1229231,1229230,2458461,2563.4682297706604,0.2737175350484904
615616,1231233,1231232,2462465,2567.841829776764,0.27329496944912535
616617,1233235,1233234,2466469,2571.87472987175,0.27287364221592725
617618,1235237,1235236,2470473,2576.47994184494,0.27245354793012666
618619,1237239,1237238,2474477,2579.9365317821503,0.27203468120387697
619620,1239241,1239240,2478481,2583.5812406539917,0.27161703668571135
620621,1241243,1241242,2482485,2588.212193965912,0.27120060904599086
621622,1243245,1243244,2486489,2592.3405208587646,0.27078539300055127
622623,1245247,1245246,2490493,2596.4530107975006,0.2703713832761423
623624,1247249,1247248,2494497,2600.660953760147,0.2699585746431694
624625,1249251,1249250,2498501,2605.4251997470856,0.2695469618993229
625626,1251253,1251252,2502505,2609.360321044922,0.26913653987321595
626627,1253255,1253254,2506509,2613.347054719925,0.2687273034171085
627628,1255257,1255256,2510513,2617.631491661072,0.2683192474250973
628629,1257259,1257258,2514517,2621.991857767105,0.267912366802193
629630,1259261,1259260,2518521,2626.6542768478394,0.26750665650070005
630631,1261263,1261262,2522525,2631.5695848464966,0.26710211148929375
631632,1263265,1263264,2526529,2635.8527569770813,0.2666987267730292
632633,1265267,1265266,2530533,2640.195891857147,0.26629649737697036
633634,1267269,1267268,2534537,2644.6621749401093,0.26589541836256103
634635,1269271,1269270,2538541,2649.32909488678,0.2654954848185298
635636,1271273,1271272,2542545,2653.3045399188995,0.2650966918536142
636637,1273275,1273274,2546549,2657.8391489982605,0.2646990346147504
637638,1275277,1275276,2550553,2662.339572906494,0.2643025082670647
638639,1277279,1277278,2554557,2666.318499803543,0.263907108006606
639640,1279281,1279280,2558561,2670.3150520324707,0.26351282905852713
640641,1281283,1281282,2562565,2674.519570827484,0.2631196666716278
641642,1283285,1283284,2566569,2679.373345851898,0.26272761612563045
642643,1285287,1285286,2570573,2683.7674050331116,0.2623366727184475
643644,1287289,1287288,2574577,2687.3731520175934,0.2619468317825522
644645,1289291,1289290,2578581,2690.8295068740845,0.2615580886758835
645646,1291293,1291292,2582585,2694.315222978592,0.26117043877820834
646647,1293295,1293294,2586589,2697.8112308979034,0.2607838774947595
647648,1295297,1295296,2590593,2701.2965466976166,0.2603984002580546
648649,1297299,1297298,2594597,2704.8080339431763,0.2600140025278961
649650,1299301,1299300,2598601,2708.3597197532654,0.25963067978955223
650651,1301303,1301302,2602605,2711.812643766403,0.25924842755011923
651652,1303305,1303304,2606609,2715.229898929596,0.2588672413385211
652653,1305307,1305306,2610613,2718.7503039836884,0.25848711672006175
653654,1307309,1307308,2614617,2722.230530977249,0.2581080492709589
654655,1309311,1309310,2618621,2725.7167208194733,0.25773003460199106
655656,1311313,1311312,2622625,2729.1529989242554,0.2573530683421268
656657,1313315,1313314,2626629,2733.7946009635925,0.25697714614761935
657658,1315317,1315316,2630633,2738.132884979248,0.2566022636983689
658659,1317319,1317318,2634637,2742.6304240226746,0.25622841669246554
659660,1319321,1319320,2638641,2747.132806777954,0.2558556008589221
660661,1321323,1321322,2642645,2751.7760198116302,0.2554838119485794
661662,1323325,1323324,2646649,2755.928713798523,0.255113045732287
662663,1325327,1325326,2650653,2759.662071943283,0.2547432980063604
663664,1327329,1327328,2654657,2763.5456037521362,0.25437456458894303
664665,1329331,1329330,2658661,2767.691009044647,0.25400684132182505
665666,1331333,1331332,2662665,2772.0890057086945,0.2536401240686246
666667,1333335,1333334,2666669,2776.101720094681,0.25327440871660656
667668,1335337,1335336,2670673,2781.4926319122314,0.25290969117304485
668669,1337339,1337338,2674677,2785.8912518024445,0.2525459673724981
669670,1339341,1339340,2678681,2790.4071097373962,0.252183233264077
670671,1341343,1341342,2682685,2795.192625761032,0.2518214848205389
671672,1343345,1343344,2686689,2800.0170817375183,0.25146071804374515
672673,1345347,1345346,2690693,2804.3834507465363,0.25110092894828995
673674,1347349,1347348,2694697,2808.90957903862,0.25074211357423337
674675,1349351,1349350,2698701,2813.4600989818573,0.25038426798346336
675676,1351353,1351352,2702705,2817.871077775955,0.25002738825423876
676677,1353355,1353354,2706709,2822.299571990967,0.24967147049574123
677678,1355357,1355356,2710713,2826.633657693863,0.24931651082260942
678679,1357359,1357358,2714717,2831.127420902252,0.24896250538586173
679680,1359361,1359360,2718721,2835.7032418251038,0.24860945035106852
680681,1361363,1361362,2722725,2840.303611755371,0.24825734189653303
681682,1363365,1363364,2726729,2844.742038011551,0.24790617623330036
682683,1365367,1365366,2730733,2849.268275976181,0.24755594958696747
683684,1367369,1367368,2734737,2853.9601278305054,0.24720665820314025
684685,1369371,1369370,2738741,2858.230297803879,0.24685829834197648
685686,1371373,1371372,2742745,2864.331550836563,0.24651086629637575
686687,1373375,1373374,2746749,2870.6694378852844,0.24616435836833261
687688,1375377,1375376,2750753,2875.652879714966,0.24581877088166948
688689,1377379,1377378,2754757,2879.955429792404,0.24547410018385563
689690,1379381,1379380,2758761,2884.789486646652,0.24513034263145528
690691,1381383,1381382,2762765,2889.410856962204,0.24478749461377447
691692,1383385,1383384,2766769,2894.4624519348145,0.2444455525273952
692693,1385387,1385386,2770773,2899.281720638275,0.2441045127943653
693694,1387389,1387388,2774777,2903.9548358917236,0.2437643718549225
694695,1389391,1389390,2778781,2908.999627828598,0.24342512616567547
695696,1391393,1391392,2782785,2914.267712831497,0.24308677219960373
696697,1393395,1393394,2786789,2919.1123287677765,0.2427493064551527
697698,1395397,1395396,2790793,2923.7481977939606,0.24241272544531967
698699,1397399,1397398,2794797,2927.710518836975,0.24207702569947287
699700,1399401,1399400,2798801,2932.2261476516724,0.24174220376517042
700701,1401403,1401402,2802805,2937.036244869232,0.2414082562117983
701702,1403405,1403404,2806809,2941.3627650737762,0.24107517962511338
702703,1405407,1405406,2810813,2945.1754927635193,0.2407429706017865
703704,1407409,1407408,2814817,2949.163949728012,0.24041162576759234
704705,1409411,1409410,2818821,2952.8469808101654,0.24008114175921946
705706,1411413,1411412,2822825,2956.5351328849792,0.23975151522972737
706707,1413415,1413414,2826829,2960.2062578201294,0.23942274285218446
707708,1415417,1415416,2830833,2963.922313928604,0.239094821314211
708709,1417419,1417418,2834837,2967.589695930481,0.2387677473252552
709710,1419421,1419420,2838841,2971.2685129642487,0.23844151760386012
710711,1421423,1421422,2842845,2974.8970329761505,0.23811612889221578
711712,1423425,1423424,2846849,2978.5189859867096,0.23779157795070205
712713,1425427,1425426,2850853,2982.1703679561615,0.23746786154515576
713714,1427429,1427428,2854857,2985.8433096408844,0.23714497647051758
714715,1429431,1429430,2858861,2989.5031938552856,0.23682291953264212
715716,1431433,1431432,2862865,2993.138036966324,0.2365016875519359
716717,1433435,1433434,2866869,2996.7645778656006,0.23618127736881434
717718,1435437,1435436,2870873,3000.349557876587,0.23586168583642575
718719,1437439,1437438,2874877,3004.1474339962006,0.23554290982610837
719720,1439441,1439440,2878881,3007.903217792511,0.23522494622193335
720721,1441443,1441442,2882885,3011.5561068058014,0.2349077919316187
721722,1443445,1443444,2886889,3015.1535007953644,0.23410214331306634
722723,1445447,1445446,2890893,3018.884165763855,0.23378788202171563
723724,1447449,1447448,2894897,3022.6068489551544,0.23347441631813126
724725,1449451,1449450,2898901,3026.205041885376,0.23316174314823002
725726,1451453,1451452,2902905,3029.828929901123,0.23284985949794645
726727,1453455,1453454,2906909,3033.418187856674,0.23253876236958604
727728,1455457,1455456,2910913,3037.0964727401733,0.23222844879273907
728729,1457459,1457458,2914917,3040.728461742401,0.2319189158079098
729730,1459461,1459460,2918921,3044.3316328525543,0.2316101604810683
730731,1461463,1461462,2922925,3047.99046087265,0.23130217988182267
731732,1463465,1463464,2926929,3051.671684741974,0.23099497109797085
732733,1465467,1465466,2930933,3055.2713158130646,0.23068853124277666
733734,1467469,1467468,2934937,3058.8492007255554,0.2303828574331419
734735,1469471,1469470,2938941,3062.447569847107,0.23007794680415827
735736,1471473,1471472,2942945,3066.049865961075,0.2297737964981934
736737,1473475,1473474,2946949,3069.6924958229065,0.22947040368853777
737738,1475477,1475476,2950953,3073.2678887844086,0.22916776554666285
738739,1477479,1477478,2954957,3076.8580737113953,0.228865879265868
739740,1479481,1479480,2958961,3080.578707933426,0.2285647420485475
740741,1481483,1481482,2962965,3084.25533080101,0.22826435111528554
741742,1483485,1483484,2966969,3087.8153426647186,0.22796470369576127
742743,1485487,1485486,2970973,3091.466614961624,0.2276657970414817
743744,1487489,1487488,2974977,3095.0807087421417,0.22736762840941083
744745,1489491,1489490,2978981,3098.6595997810364,0.2270701950728835
745746,1491493,1491492,2982985,3102.2575738430023,0.22677349431978655
746747,1493495,1493494,2986989,3105.873510837555,0.2264775234489207
747748,1495497,1495496,2990993,3109.4987750053406,0.22618227977363858
748749,1497499,1497498,2994997,3113.1273028850555,0.2258877606218448
749750,1499501,1499500,2999001,3116.7391879558563,0.22559396333053883
750751,1501503,1501502,3003005,3120.3792717456818,0.22530088525127212
751752,1503505,1503504,3007009,3123.995851993561,0.225008523753786
752753,1505507,1505506,3011013,3127.5515038967133,0.22471687621327874
753754,1507509,1507508,3015017,3131.152140855789,0.22442594002131955
754755,1509511,1509510,3019021,3134.73290681839,0.22413571257857257
755756,1511513,1511512,3023025,3138.3300478458405,0.22384619130571082
756757,1513515,1513514,3027029,3141.973912000656,0.2235573736288643
757758,1515517,1515516,3031033,3145.579670906067,0.22326925698871491
758759,1517519,1517518,3035037,3149.199034690857,0.2229818388386775
759760,1519521,1519520,3039041,3152.776062965393,0.22269511664671882
760761,1521523,1521522,3043045,3156.386976957321,0.22240908788990055
761762,1523525,1523524,3047049,3159.97908782959,0.22212375005619833
762763,1525527,1525526,3051053,3163.581766843796,0.2218391006499587
763764,1527529,1527528,3055057,3167.2012169361115,0.22155513718644215
764765,1529531,1529530,3059061,3170.822250843048,0.2212718571881851
765766,1531533,1531532,3063065,3174.4879398345947,0.22098925819409487
766767,1533535,1533534,3067069,3178.0719270706177,0.22070733775581175
767768,1535537,1535536,3071073,3181.726245880127,0.22042609343407094
768769,1537539,1537538,3075077,3185.3984158039093,0.22014552280234057
769770,1539541,1539540,3079081,3189.052486896515,0.21986562344318372
770771,1541543,1541542,3083085,3192.6217699050903,0.2195863929537154
771772,1543545,1543544,3087089,3196.225849866867,0.21930782894378353
772773,1545547,1545546,3091093,3199.8191406726837,0.219029929030512
773774,1547549,1547548,3095097,3203.4723057746887,0.2187526908437576
774775,1549551,1549550,3099101,3207.047405719757,0.21847611202429107
775776,1551553,1551552,3103105,3210.7616577148438,0.21820019022925408
776777,1553555,1553554,3107109,3214.406893014908,0.21792492311760725
777778,1555557,1555556,3111113,3218.001667022705,0.21765030836468213
778779,1557559,1557558,3115117,3221.5872247219086,0.2173763436585432
779780,1559561,1559560,3119121,3225.207083940506,0.21710302669634984
780781,1561563,1561562,3123125,3228.8774857521057,0.21683035518253746
781782,1563565,1563564,3127129,3232.5179419517517,0.21655832683791232
782783,1565567,1565566,3131133,3236.0817399024963,0.21628693939237564
783784,1567569,1567568,3135137,3239.668076992035,0.21601619058128563
784785,1569571,1569570,3139141,3243.260766983032,0.21574607816000935
785786,1571573,1571572,3143145,3247.0055170059204,0.21547659988755186
786787,1573575,1573574,3147149,3250.642616033554,0.21520775353383215
787788,1575577,1575576,3151153,3254.2246708869934,0.21493953688514011
788789,1577579,1577578,3155157,3257.8281667232513,0.21467194772776566
789790,1579581,1579580,3159161,3261.613182783127,0.21440498386800755
790791,1581583,1581582,3163165,3265.3281819820404,0.21413864311762154
791792,1583585,1583584,3167169,3268.952100753784,0.21387292329927732
792793,1585587,1585586,3171173,3272.57976603508,0.2136078222447395
793794,1587589,1587588,3175177,3276.1618428230286,0.21334333780032466
794795,1589591,1589590,3179181,3279.750385761261,0.2130794678159873
795796,1591593,1591592,3183185,3283.4695217609406,0.20885690041541238
796797,1593595,1593594,3187189,3287.251095056534,0.2020343063340988
797798,1595597,1595596,3191193,3290.933069705963,0.19568280861676612
798799,1597599,1597598,3195197,3294.724268913269,0.19029158085504605
799800,1599601,1599600,3199201,3298.4257867336273,0.1847958872658637
800801,1601603,1601602,3203205,3302.193165063858,0.17965895112138242
801802,1603605,1603604,3207209,3305.9695858955383,0.17487518094094412
802803,1605607,1605606,3211213,3309.7116837501526,0.1704392269894015
803804,1607609,1607608,3215217,3313.4262409210205,0.16640104659200006
804805,1609611,1609610,3219221,3317.1055936813354,0.16238411661652208
805806,1611613,1611612,3223225,3320.8052599430084,0.1586518068688747
806807,1613615,1613614,3227229,3324.5275609493256,0.15526963089723722
807808,1615617,1615616,3231233,3328.131694793701,0.1519450352752756
808809,1617619,1617618,3235237,3331.7380516529083,0.14897826765445643
809810,1619621,1619620,3239241,3335.3310327529907,0.1459649997195811
810811,1621623,1621622,3243245,3338.9058890342712,0.144699126462001
811812,1623625,1623624,3247249,3342.50847196579,0.1445712373006245
812813,1625627,1625626,3251253,3346.1098868846893,0.1444435557386896
813814,1627629,1627628,3255257,3349.748548746109,0.1443160812723363
814815,1629631,1629630,3259261,3353.4126749038696,0.1441888133995235
815816,1631633,1631632,3263265,3357.0011699199677,0.1440617516200291
816817,1633635,1633634,3267269,3360.6238758563995,0.14393489544090698
817818,1635637,1635636,3271273,3364.216481924057,0.14380824436193507
818819,1637639,1637638,3275277,3367.8062887191772,0.14368179789016722
819820,1639641,1639640,3279281,3371.401440858841,0.1435555555344763
820821,1641643,1641642,3283285,3374.997018814087,0.14342951680555416
821822,1643645,1643644,3287289,3378.5854988098145,0.1433036812068167
822823,1645647,1645646,3291293,3382.252492904663,0.14317804825986968
823824,1647649,1647648,3295297,3385.8855378627777,0.143052617471767
824825,1649651,1649650,3299301,3389.4992558956146,0.14292738836047647
825826,1651653,1651652,3303305,3393.127963781357,0.14280236044578487
826827,1653655,1653654,3307309,3396.772750854492,0.14267753323838406
827828,1655657,1655656,3311313,3400.497256755829,0.1425529062653368
828829,1657659,1657658,3315317,3404.141907930374,0.14242847904642986
829830,1659661,1659660,3319321,3407.7591989040375,0.14230425110508804
830831,1661663,1661662,3323325,3411.406584739685,0.14218022196291713
831832,1663665,1663664,3327329,3415.076231956482,0.14205639115061786
832833,1665667,1665666,3331333,3418.693960905075,0.141932758189796
833834,1667669,1667668,3335337,3422.3535227775574,0.14180932261660928
834835,1669671,1669670,3339341,3425.9507958889008,0.14168608395630145
835836,1671673,1671672,3343345,3429.5650696754456,0.14156304174321122
836837,1673675,1673674,3347349,3433.1536309719086,0.1414401955134963
837838,1675677,1675676,3351353,3436.7503967285156,0.14131754479421943
838839,1677679,1677678,3355357,3440.4416887760162,0.1411950891288143
839840,1679681,1679680,3359361,3444.0830488204956,0.14107282805707655
840841,1681683,1681682,3363365,3447.6803319454193,0.14095076111152594
841842,1683685,1683684,3367369,3451.2785589694977,0.14082888783923408
842843,1685687,1685686,3371373,3454.878748893738,0.14070720777999668
843844,1687689,1687688,3375377,3458.448063850403,0.1405857204754284
844845,1689691,1689690,3379381,3462.018306016922,0.14046442547441984
845846,1691693,1691692,3383385,3465.642936706543,0.14034332232222368
846847,1693695,1693694,3387389,3469.327234983444,0.14022241056591156
847848,1695697,1695696,3391393,3472.9340119361877,0.14010168975619308
848849,1697699,1697698,3395397,3476.563300848007,0.13998115944559686
849850,1699701,1699700,3399401,3480.159147977829,0.1398608191848325
850851,1701703,1701702,3403405,3483.7811279296875,0.13974066852824762
851852,1703705,1703704,3407409,3487.4079928398132,0.13962070702837082
852853,1705707,1705706,3411413,3491.007845878601,0.13950093424500665
853854,1707709,1707708,3415417,3494.635505914688,0.13938134973795968
854855,1709711,1709710,3419421,3498.270605802536,0.13926195306157751
855856,1711713,1711712,3423425,3501.919126033783,0.1391427437793027
856857,1713715,1713714,3427429,3505.5143270492554,0.13902372145275876
857858,1715717,1715716,3431433,3509.1144268512726,0.1389048856435693
858859,1717719,1717718,3435437,3512.7101340293884,0.13878623592063377
859860,1719721,1719720,3439441,3516.2975590229034,0.13866777184739476
860861,1721723,1721722,3443445,3519.8821120262146,0.13854949299275177
861862,1723725,1723724,3447449,3523.4605448246,0.1384313989256043
862863,1725727,1725726,3451453,3527.1027069091797,0.13831348921303288
863864,1727729,1727728,3455457,3530.698008775711,0.13819576343121298
864865,1729731,1729730,3459461,3534.3392267227173,0.13807822114722512
865866,1731733,1731732,3463465,3538.0009326934814,0.13796086194452073
866867,1733735,1733734,3467469,3541.6069350242615,0.13784368539018033
867868,1735737,1735736,3471473,3545.211637020111,0.13772669106219837
868869,1737739,1737738,3475477,3548.7985389232635,0.1376098785403883
869870,1739741,1739740,3479481,3552.408362865448,0.13749324741002056
870871,1741743,1741742,3483485,3556.003350019455,0.13737679724181362
871872,1743745,1743744,3487489,3559.580186843872,0.13726052761921892
872873,1745747,1745746,3491493,3563.208492040634,0.13714443813296384
873874,1747749,1747748,3495497,3566.7719280719757,0.13702852836104285
874875,1749751,1749750,3499501,3570.384217739105,0.1369127978941833
875876,1751753,1751752,3503505,3574.006630897522,0.13679724631401768
876877,1753755,1753754,3507509,3577.573017835617,0.13668187321491132
877878,1755757,1755756,3511513,3581.298736810684,0.13656667818031565
878879,1757759,1757758,3515517,3584.897894859314,0.13645166080641502
879880,1759761,1759760,3519521,3588.582797050476,0.13633682068393682
880881,1761763,1761762,3523525,3592.1988627910614,0.1362221574072464
881882,1763765,1763764,3527529,3595.8108468055725,0.13610767056889017
882883,1765767,1765766,3531533,3599.4466817379,0.13599335976687144
883884,1767769,1767768,3535537,3603.0808687210083,0.1358792245919176
884885,1769771,1769770,3539541,3606.6961369514465,0.1357652646547649
885886,1771773,1771772,3543545,3610.3384687900543,0.13565147954250278
886887,1773775,1773774,3547549,3613.9637529850006,0.1355378688658675
887888,1775777,1775776,3551553,3617.5885560512543,0.1354244322210434
888889,1777779,1777778,3555557,3621.234988927841,0.13531116921330977
889890,1779781,1779780,3559561,3624.927244901657,0.13519807944794593
890891,1781783,1781782,3563565,3628.7190656661987,0.13508516252841218
891892,1783785,1783784,3567569,3632.345482826233,0.1349724180636258
892893,1785787,1785786,3571573,3636.0097818374634,0.13485984566250409
893894,1787789,1787788,3575577,3639.6281888484955,0.1347474449321453
894895,1789791,1789790,3579581,3643.224168777466,0.13463521548146673
895896,1791793,1791792,3583585,3646.8232119083405,0.1345231569284806
896897,1793795,1793794,3587589,3650.4349949359894,0.13441126887846622
897898,1795797,1795796,3591593,3654.105963945389,0.1342995509494358
898899,1797799,1797798,3595597,3657.710335969925,0.13418800275758258
899900,1799801,1799800,3599601,3661.3174679279327,0.1340766239172808
900901,1801803,1801802,3603605,3664.967038869858,0.13396541404654272
901902,1803805,1803804,3607609,3668.565277814865,0.13385437276519951
902903,1805807,1805806,3611613,3672.175880908966,0.13374349968944443
903904,1807809,1807808,3615617,3675.73659491539,0.13363279444456566
904905,1809811,1809810,3619621,3679.3892827033997,0.1335222566522134
905906,1811813,1811812,3623625,3683.034810781479,0.13341188593403785
906907,1813815,1813814,3627629,3686.7658207416534,0.13330168190987024
907908,1815817,1815816,3631633,3690.3774857521057,0.13319164421409369
908909,1817819,1817818,3635637,3694.0404238700867,0.1330817724665394
909910,1819821,1819820,3639641,3697.6284358501434,0.13297206629977154
910911,1821823,1821822,3643645,3701.44717168808,0.13286252534089726
911912,1823825,1823824,3647649,3705.149317741394,0.13275314921884274
912913,1825827,1825826,3651653,3708.8040878772736,0.1326439375643531
913914,1827829,1827828,3655657,3712.4334387779236,0.13253489000999252
914915,1829831,1829830,3659661,3716.019847869873,0.1324260061901441
915916,1831833,1831832,3663665,3719.630683898926,0.132317285739191
916917,1833835,1833834,3667669,3723.283770799637,0.13220872828969732
917918,1835837,1835836,3671673,3726.901026725769,0.13210033348332217
918919,1837839,1837838,3675677,3730.4797019958496,0.1319921009544487
919920,1839841,1839840,3679681,3734.1462666988373,0.13188403034109797
920921,1841843,1841842,3683685,3737.7254610061646,0.13177612128311011
921922,1843845,1843844,3687689,3741.343384027481,0.1316683734221442
922923,1845847,1845846,3691693,3744.9897940158844,0.13156078640167834
923924,1847849,1847848,3695697,3748.5683748722076,0.13145335986519058
924925,1849851,1849850,3699701,3752.191475868225,0.13134609345252102
925926,1851853,1851852,3703705,3755.7461297512054,0.13123898680896673
926927,1853855,1853854,3707709,3759.38619184494,0.13113203958528175
927928,1855857,1855856,3711713,3763.0257267951965,0.13102525142312516
928929,1857859,1857858,3715717,3766.6464257240295,0.13091862197688897
929930,1859861,1859860,3719721,3770.3396258354187,0.13081215089187026
930931,1861863,1861862,3723725,3773.947581768036,0.13070583781700407
931932,1863865,1863864,3727729,3777.551880836487,0.1305996824066824
932933,1865867,1865866,3731733,3781.166429758072,0.1304936843134783
933934,1867869,1867868,3735737,3784.731048822403,0.13038784318814578
934935,1869871,1869870,3739741,3788.3327407836914,0.13028215868689585
935936,1871873,1871872,3743745,3791.922129869461,0.13017663046230155
936937,1873875,1873874,3747749,3795.5117678642273,0.13007125817603082
937938,1875877,1875876,3751753,3799.0858857631683,0.1299660414824757
938939,1877879,1877878,3755757,3802.754678964615,0.1298609800360282
939940,1879881,1879880,3759761,3806.354826927185,0.12975607350563223
940941,1881883,1881882,3763765,3809.974511861801,0.12965132154386083
941942,1883885,1883884,3767769,3813.5975069999695,0.12954672381420096
942943,1885887,1885886,3771773,3817.250095844269,0.12944227998013957
943944,1887889,1887888,3775777,3820.853320837021,0.12933798970516364
944945,1889891,1889890,3779781,3824.485050678253,0.12923385265094112
945946,1891893,1891892,3783785,3828.122454881668,0.12912986848641594
946947,1893895,1893894,3787789,3831.7527170181274,0.1290260368732561
947948,1895897,1895896,3791793,3835.3385016918182,0.12892235748404346
948949,1897899,1897898,3795797,3838.92968082428,0.128818829985903
949950,1899901,1899900,3799801,3842.566512823105,0.12871545404595963
950951,1901903,1901902,3803805,3846.2441399097443,0.1286122293349763
951952,1903905,1903904,3807809,3850.0734508037567,0.1285091555237159
952953,1905907,1905906,3811813,3853.6472907066345,0.12840623228476034
953954,1907909,1907908,3815817,3857.2542808055878,0.12830345929251052
954955,1909911,1909910,3819821,3860.8393547534943,0.12820083621954836
955956,1911913,1911912,3823825,3864.4552929401398,0.12809836274209374
956957,1913915,1913914,3827829,3868.062983751297,0.12799603853272856
957958,1915917,1915916,3831833,3871.6920108795166,0.12789386327494867
958959,1917919,1917918,3835837,3875.3489048480988,0.127791836637698
959960,1919921,1919920,3839841,3878.9932746887207,0.12768995830629137
960961,1921923,1921922,3843845,3882.631864786148,0.12758822795694869
961962,1923925,1923924,3847849,3886.2068848609924,0.12748664527316578
962963,1925927,1925926,3851853,3889.8488509655,0.1273852099366195
963964,1927929,1927928,3855857,3893.468845844269,0.12728392162352975
964965,1929931,1929930,3859861,3897.0943479537964,0.12718278002284933
965966,1931933,1931932,3863865,3900.7011518478394,0.12708178481807408
966967,1933935,1933934,3867869,3904.286017894745,0.12698093569451885
967968,1935937,1935936,3871873,3907.9062128067017,0.12688023233567947
968969,1937939,1937938,3875877,3911.494158744812,0.12677967443232774
969970,1939941,1939940,3879881,3915.0775077342987,0.12667926166614052
970971,1941943,1941942,3883885,3918.6577668190002,0.1265789937315276
971972,1943945,1943944,3887889,3922.2792177200317,0.12647887031562277
972973,1945947,1945946,3891893,3925.901725769043,0.12637889111101686
973974,1947949,1947948,3895897,3929.532614707947,0.12627905580666265
974975,1949951,1949950,3899901,3933.119994878769,0.12617936409696995
975976,1951953,1951952,3903905,3936.765904903412,0.12607981567089155
976977,1953955,1953954,3907909,3940.3606638908386,0.1259804102282942
977978,1955957,1955956,3911913,3943.9799506664276,0.12588114745813073
978979,1957959,1957958,3915917,3947.637640953064,0.12578202706026786
979980,1959961,1959960,3919921,3951.283096075058,0.1256830487309344
980981,1961963,1961962,3923925,3954.9614968299866,0.12558421216635907
981982,1963965,1963964,3927929,3958.566120862961,0.12548551706822764
982983,1965967,1965966,3931933,3962.2098937034607,0.1253869631254929
983984,1967969,1967968,3935937,3965.880481004715,0.12528855005075457
984985,1969971,1969970,3939941,3969.5183777809143,0.12519027754024137
985986,1971973,1971972,3943945,3973.076618909836,0.12509214529200108
986987,1973975,1973974,3947949,3976.6769938468933,0.1249941530131764
987988,1975977,1975976,3951953,3980.3022577762604,0.12489630040545308
988989,1977979,1977978,3955957,3983.9372918605804,0.12479858717233583
989990,1979981,1979980,3959961,3987.570255756378,0.12470101302096737
990991,1981983,1981982,3963965,3991.2121448516846,0.12460357765485242
991992,1983985,1983984,3967969,3994.841962814331,0.12450628078477166
992993,1985987,1985986,3971973,3998.4472119808197,0.12440912211241084
993994,1987989,1987988,3975977,4002.0632367134094,0.12431210134855064
994995,1989991,1989990,3979981,4005.71049785614,0.12421521820397174
995996,1991993,1991992,3983985,4009.3665368556976,0.12411847239127383
996997,1993995,1993994,3987989,4013.0476636886597,0.1240218636157806
997998,1995997,1995996,3991993,4017.1067719459534,0.12392539159009175
998999,1997999,1997998,3995997,4020.8275089263916,0.12382905602862593
1000000,2000001,2000000,4000001,4024.4522228240967,0.12373285664216382


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0035982131958007812,12064.44795143716
1001,2003,2002,4005,3.8882622718811035,65.38449138327269
2002,4005,4004,8009,7.948341369628906,42.2154127642043
3003,6007,6006,12013,12.002243041992188,33.90174222643145
4004,8009,8008,16017,16.12182116508484,28.84319011385014
5005,10011,10010,20021,19.728594303131104,25.22268890097439
6006,12013,12012,24025,23.365817070007324,22.42065265709971
7007,14015,14014,28029,26.99235725402832,20.15004075854631
8008,16017,16016,32033,30.618634939193726,18.255867237425264
9009,18019,18018,36037,34.21288323402405,16.644924627120417
10010,20021,20020,40041,37.8082001209259,15.256259435958782
11011,22023,22022,44045,41.40822124481201,14.04716756882226
12012,24025,24024,48049,45.06582021713257,12.986141411429344
13013,26027,26026,52053,48.61799430847168,12.049111192072814
14014,28029,28028,56057,52.23655128479004,11.217231971750152
15015,30031,30030,60061,55.7975013256073,10.475259290258691
16016,32033,32032,64065,59.39685821533203,9.810784742190663
17017,34035,34034,68069,62.946776151657104,9.213588128843185
18018,36037,36036,72073,66.51810503005981,8.67509578481804
19019,38039,38038,76077,70.11822938919067,8.188094868561166
20020,40041,40040,80081,73.85724115371704,7.746456546892659
21021,42043,42042,84085,77.44075417518616,7.344936499697724
22022,44045,44044,88089,80.98412322998047,6.979019482529111
23023,46047,46046,92093,84.5825400352478,6.644796545697318
24024,48049,48048,96097,88.25771307945251,6.338866989019152
25025,50051,50050,100101,91.83079814910889,6.058259293347874
26026,52053,52052,104105,95.38628125190735,5.8003667720786325
27027,54055,54054,108109,99.05189323425293,5.562894754204535
28028,56057,56056,112113,102.7015471458435,5.34381688436406
29029,58059,58058,116117,106.29325723648071,5.14133869384932
30030,60061,60060,120121,109.9285101890564,4.953867018881283
31031,62063,62062,124125,113.50830936431885,4.779984159364176
32032,64065,64064,128129,117.11837005615234,4.618425910906808
33033,66067,66066,132133,120.65442419052124,4.46806278542681
34034,68069,68068,136137,124.24468922615051,4.327883875652333
35035,70071,70070,140141,128.4076452255249,4.196982926987403
36036,72073,72072,144145,131.98642301559448,4.0745462642044
37037,74075,74074,148149,135.53232407569885,3.9598422862709413
38038,76077,76076,152153,139.14230918884277,3.8522122943613795
39039,78079,78078,156157,142.6928472518921,3.7510624592814565
40040,80081,80080,160161,146.2425491809845,3.6558613114921172
41041,82083,82082,164165,149.8064842224121,3.566129789558545
42042,84085,84084,168169,153.39581322669983,3.4814190444340056
43043,86087,86086,172173,156.94034814834595,3.401332075274695
44044,88089,88088,176177,160.565269947052,3.32550887767502
45045,90091,90090,180181,164.15765023231506,3.2536226351949153
46046,92093,92092,184185,167.77509117126465,3.185376335550245
47047,94095,94094,188189,171.3869071006775,3.120499759867016
48048,96097,96096,192193,174.9719033241272,3.058746800541485
49049,98099,98098,196197,178.60749101638794,2.9998930688743712
50050,100101,100100,200201,182.15090036392212,2.9437337589097297
51051,102103,102102,204205,185.72179913520813,2.8900817379417276
52052,104105,104104,208209,189.3591160774231,2.8387658380506764
53053,106107,106106,212213,192.92078304290771,2.7896293259727827
54054,108109,108108,216217,196.56375908851624,2.742528531491189
55055,110111,110110,220221,200.1053171157837,2.697331616869633
56056,112113,112112,224225,203.74623608589172,2.653917471836394
57057,114115,114114,228229,207.32011723518372,2.6121747205324937
58058,116117,116116,232233,211.02904415130615,2.572000828349701
59059,118119,118118,236237,214.59930419921875,2.533301297957223
60060,120121,120120,240241,218.25865817070007,2.4959889450437913
61061,122123,122122,244245,221.86557531356812,2.4599832453677664
62062,124125,124124,248249,225.45019721984863,2.425211069314173
63063,126127,126126,252253,229.03374409675598,2.391602714491455
64064,128129,128128,256257,232.73784804344177,2.3590937382832635
65065,130131,130130,260261,236.27825117111206,2.3276249103255395
66066,132133,132132,264265,239.8943111896515,2.2971412315273483
67067,134135,134134,268269,243.4142882823944,2.267591576312043
68068,136137,136136,272273,247.03720426559448,2.238928369633868
69069,138139,138138,276277,250.5957863330841,2.2111072939496808
70070,140141,140140,280281,254.28893518447876,2.1840870231935696
71071,142143,142142,284285,258.7126340866089,2.1578289810713613
72072,144145,144144,288289,262.7164611816406,2.1322971212430275
73073,146147,146146,292293,266.8357570171356,2.107457727290239
74074,148149,148148,296297,270.51077818870544,2.0832792305045587
75075,150151,150150,300301,274.27176213264465,2.0597320438027964
76076,152153,152152,304305,278.496089220047,2.0367884101960954
77077,154155,154154,308309,282.7754900455475,2.0144222644375986
78078,156157,156156,312313,287.1283640861511,1.9926091065881337
79079,158159,158158,316317,291.7021441459656,1.971325886379418
80080,160161,160160,320321,295.12670516967773,1.9505508973688848
81081,162163,162162,324325,298.4981760978699,1.9302636799784523
82082,164165,164164,328329,301.89953112602234,1.9104449325750466
83083,166167,166166,332333,305.31486415863037,1.8910764298871072
84084,168169,168168,336337,308.7006850242615,1.8721409480604052
85085,170171,170170,340341,313.13223910331726,1.853622195785647
86086,172173,172172,344345,318.19966101646423,1.8355047509230644
87087,174175,174174,348349,322.58982014656067,1.8177740021492355
88088,176177,176176,352353,326.4793472290039,1.8004160951877566
89089,178179,178178,356357,330.31257700920105,1.7834178832090402
90090,180181,180180,360361,334.1131420135498,1.766766881044532
91091,182183,182182,364365,338.2126262187958,1.7504515684831858
92092,184185,184184,368369,342.0464291572571,1.7344624748329807
93093,186187,186186,372373,346.4044840335846,1.7187865341365978
94094,188189,188188,376377,350.41197896003723,1.7034135223966587
95095,190191,190190,380381,354.18487334251404,1.6883336949704244
96096,192193,192192,384385,357.82920598983765,1.6735377577206236
97097,194195,194194,388389,361.4940941333771,1.6590168402235577
98098,196197,196196,392393,365.4502053260803,1.6447624709071533
99099,198199,198198,396397,369.2518062591553,1.6307665539043228
100100,200201,200200,400401,372.6926131248474,1.617021347536138
101101,202203,202202,404405,376.72474122047424,1.603519444252015
102102,204205,204204,408409,380.42090916633606,1.5902537519468751
103103,206207,206206,412413,384.3952491283417,1.5772174765352247
104104,208209,208208,416417,387.94224095344543,1.5644041056784772
105105,210211,210210,420421,392.1014862060547,1.5518073935854773
106106,212213,212212,424425,395.59817695617676,1.5394213468080125
107107,214215,214214,428429,399.2603623867035,1.527240210938544
108108,216217,216216,432433,403.6152853965759,1.5152584581774136
109109,218219,218218,436437,408.7325973510742,1.5034707756622083
110110,220221,220220,440441,413.17922925949097,1.4918720545556425
111111,222223,222222,444445,418.6150851249695,1.480457379759173
112112,224225,224224,448449,424.1068410873413,1.4692220203178294
113113,226227,226226,452453,428.9699430465698,1.4581614203507343
114114,228229,228228,456457,433.19059205055237,1.447271190569154
115115,230231,230230,460461,436.7775421142578,1.4365471002583945
116116,232233,232232,464465,440.15698623657227,1.4259850697617367
117117,234235,234234,468469,443.54811120033264,1.4155811633736448
118118,236237,236236,472473,446.9386281967163,1.4053315826786275
119119,238239,238238,476477,450.45614528656006,1.3952326602247922
120120,240241,240240,480481,454.1458752155304,1.3852808535921213
121121,242243,242242,484485,457.8456561565399,1.3754727397590614
122122,244245,244244,488489,461.29187512397766,1.3658050098201784
123123,246247,246246,492493,464.685583114624,1.3562744639420998
124124,248249,248248,496497,468.1335690021515,1.3468780066377803
125125,250251,250250,500501,471.57833218574524,1.337612642271779
126126,252253,252252,504505,475.0053360462189,1.3284754708038236
127127,254255,254254,508509,478.57123708724976,1.319463683765207
128128,256257,256256,512513,481.98952317237854,1.3105745604425465
129129,258259,258258,516517,485.33553409576416,1.3018054642470815
130130,260261,260260,520521,488.7066111564636,1.2931538392822404
131131,262263,262262,524525,492.2223711013794,1.2846189332267386
132132,264265,264264,528529,495.75946021080017,1.2761968457252806
133133,266267,266266,532533,499.3893401622772,1.2678849911717407
134134,268269,268268,536537,502.7874963283539,1.2596811055791477
135135,270271,270270,540541,506.1599111557007,1.2515829910626053
136136,272273,272272,544545,509.56912207603455,1.2435885131653777
137137,274275,274274,548549,512.9699552059174,1.2356955984068918
138138,276277,276276,552553,516.3512990474701,1.227902231970802
139139,278279,278278,556557,519.8855800628662,1.2202064555076504
140140,280281,280280,560561,523.4368870258331,1.2126063650557626
141141,282283,282282,564565,527.0931262969971,1.205100109022169
142142,284285,284284,568569,530.7019560337067,1.1976858863072266
143143,286287,286286,572573,536.0508699417114,1.1903619444656215
144144,288289,288288,576577,539.7955021858215,1.183126577978328
145145,290291,290290,580581,543.1456291675568,1.1759781266009668
146146,292293,292292,584585,546.480535030365,1.1689149737703701
147147,294295,294294,588589,549.8182771205902,1.1619355450930016
148148,296297,296296,592593,553.198361158371,1.1550383068934025
149149,298299,298298,596597,556.5192470550537,1.148221764828122
150150,300301,300300,600601,559.9051420688629,1.1414844625542173
151151,302303,302302,604605,563.2308993339539,1.134824980465055
152152,304305,304304,608609,566.7772052288055,1.1282419344570371
153153,306307,306306,612613,570.2426452636719,1.1217339747709048
154154,308309,308308,616617,573.6279730796814,1.1152997848730593
155155,310311,310310,620621,577.0635502338409,1.1089380803732638
156156,312313,312312,624625,580.3887951374054,1.1026476080023713
157157,314315,314314,628629,583.8351261615753,1.096427144604604
158158,316317,316316,632633,587.1637032032013,1.0902754962116887
159159,318319,318318,636637,590.9735562801361,1.08419149711699
160160,320321,320320,640641,595.032909154892,1.078174008986025
161161,322323,322322,644645,598.5550403594971,1.0722219200451946
162162,324325,324324,648649,602.4061682224274,1.0663341442304954
163163,326327,326326,652653,606.7079672813416,1.060509620456287
164164,328329,328328,656657,611.4131321907043,1.0547473118112975
165165,330331,330330,660661,615.1866359710693,1.0490462048801419
166166,332333,332332,664665,619.1476762294769,1.0434053090284579
167167,334335,334334,668669,623.6023690700531,1.0378236557371565
168168,336337,336336,672673,627.4817492961884,1.0323002979566809
169169,338339,338338,676677,631.1769051551819,1.0268343094867305
170170,340341,340340,680681,635.0655381679535,1.021424784377814
171171,342343,342342,684685,640.0242962837219,1.0160708363564481
172172,344345,344344,688689,644.9028842449188,1.0107715982721857
173173,346347,346346,692693,649.1954381465912,1.005526221542823
174174,348349,348348,696697,652.9757113456726,1.000333875655997
175175,350351,350350,700701,656.5776813030243,0.9951937476635067
176176,352353,352352,704705,660.2646253108978,0.9901050416865473
177177,354355,354354,708709,663.8679192066193,0.9850669784755155
178178,356357,356356,712713,668.0356051921844,0.9800787949352525
179179,358359,358358,716717,671.919319152832,0.9751397436939442
180180,360361,360360,720721,675.9488081932068,0.970249092699305
181181,362363,362362,724725,679.559582233429,0.9654061247983918
182182,364365,364364,728729,682.8860001564026,0.9606101373392448
183183,366367,366366,732733,686.8987760543823,0.955860441805271
184184,368369,368368,736737,690.3873200416565,0.951156363440532
185185,370371,370370,740741,693.8249850273132,0.9464972408986796
186186,372373,372372,744745,697.9178631305695,0.9418824258827954
187187,374375,374374,748749,701.2998189926147,0.9373112828379817
188188,376377,376376,752753,704.6782472133636,0.9327831886112108
189189,378379,378378,756757,708.2353031635284,0.9282975321366393
190190,380381,380380,760761,712.0029621124268,0.9238537141445704
191191,382383,382382,764765,715.782338142395,0.91945114686132
192192,384385,384384,768769,719.7723503112793,0.9150892537309119
193193,386387,386386,772773,723.2217342853546,0.910767469129496
194194,388389,388388,776777,726.5924451351166,0.9064852381070523
195195,390391,390390,780781,729.9082312583923,0.9022420161218179
196196,392393,392392,784785,734.1089992523193,0.8980372688001808
197197,394395,394394,788789,737.932046175003,0.8938704716838402
198198,396397,396396,792793,741.7402150630951,0.8897411099860619
199199,398399,398398,796797,746.1522212028503,0.8856486783879518
200200,400401,400400,800801,749.815181016922,0.8815926807874348
201201,402403,402402,804805,753.6073632240295,0.8775726300973474
202202,404405,404404,808809,758.0359883308411,0.8735880480435299
203203,406407,406406,812813,762.6959691047668,0.8696384649338142
204204,408409,408408,816817,766.1974220275879,0.8657234194943157
205205,410411,410410,820821,770.0588102340698,0.8618424586456968
206206,412413,412412,824825,773.8684332370758,0.8579951373467338
207207,414415,414414,828829,778.128396987915,0.854181018377858
208208,416417,416416,832833,782.325679063797,0.8503996722065494
209209,418419,418418,836837,786.1213111877441,0.8466506767672399
210210,420421,420420,840841,789.8103301525116,0.8429336173394404
211211,422423,422422,844845,793.9313831329346,0.8392480863567471
212212,424425,424424,848849,797.7769801616669,0.8355936832595035
213213,426427,426426,852853,801.7052111625671,0.831970014345643
214214,428429,428428,856857,805.401641368866,0.8283766926051612
215215,430431,430430,860861,809.1752700805664,0.8248135627745796
216216,432433,432432,864865,813.0948390960693,0.8212803906553745
217217,434435,434434,868869,817.9788892269135,0.8177764469292015
218218,436437,436436,872873,822.8108930587769,0.8143013615190284
219219,438439,438438,876877,827.7778301239014,0.8108547787942371
220220,440441,440440,880881,832.3343253135681,0.8074363490995893
221221,442443,442442,884885,836.6380832195282,0.8040457285442244
222222,444445,444444,888889,840.0414340496063,0.8006825788870628
223223,446447,446446,892893,843.734904050827,0.7973465674112958
224224,448449,448448,896897,847.261194229126,0.7940373668116081
225225,450451,450450,900901,851.175971031189,0.7907546550759434
226226,452453,452452,904905,855.2420210838318,0.7874981153800036
227227,454455,454454,908909,858.750764131546,0.7842674359853845
228228,456457,456456,912913,862.1784932613373,0.7810623101322562
229229,458459,458458,916917,866.0286903381348,0.7778824359320424
230230,460461,460460,920921,870.2608001232147,0.7747275162801088
231231,462463,462462,924925,875.1588530540466,0.7715972587575379
232232,464465,464464,928929,879.619104385376,0.7684913755329035
233233,466467,466466,932933,883.7147121429443,0.765409583269502
234234,468469,468468,936937,888.9980461597443,0.7623516030453175
235235,470471,470470,940941,893.8469052314758,0.7593171602602524
236236,472473,472472,944945,898.5353002548218,0.7563059845524549
237237,474475,474474,948949,903.1606271266937,0.7533178097128257
238238,476477,476476,952953,907.6903049945831,0.7503523736104398
239239,478479,478478,956957,912.0796432495117,0.7474094181088731
240240,480481,480480,960961,916.4654712677002,0.7444886889898044
241241,482483,482482,964965,921.3947072029114,0.7415899358729803
242242,484485,484484,968969,926.1949019432068,0.7387129121598264
243243,486487,486486,972973,930.7813920974731,0.7358573749443167
244244,488489,488488,976977,935.5699870586395,0.7330230849456711
245245,490491,490490,980981,941.1516101360321,0.7302098064465099
246246,492493,492492,984985,946.1918830871582,0.7274173072255508
247247,494495,494494,988989,950.4976282119751,0.7246453584848496
248248,496497,496496,992993,955.6843943595886,0.7218937347915926
249249,498499,498498,996997,959.8007261753082,0.7191622140180698
250250,500501,500500,1001001,964.1884820461273,0.7164505772707344
251251,502503,502502,1005005,968.6207082271576,0.7137586088410899
252252,504505,504504,1009009,973.6453042030334,0.7110861044602643
253253,506507,506506,1013013,978.6540422439575,0.7084328886212461
254254,508509,508508,1017017,982.9233803749084,0.7057987144507933
255255,510511,510510,1021021,986.8508930206299,0.7031833783294132
256256,512513,512512,1025025,991.4910881519318,0.7005866795407201
257257,514515,514514,1029029,995.2930431365967,0.6980084202241414
258258,516517,516516,1033033,999.7409472465515,0.6954484053239867
259259,518519,518518,1037037,1004.2620091438293,0.6929064425221441
260260,520521,520520,1041041,1008.8224623203278,0.6903823422162532
261261,522523,522522,1045045,1012.7507922649384,0.687875917461497
262262,524525,524524,1049049,1016.9264371395111,0.6853869839069375
263263,526527,526526,1053053,1020.7484021186829,0.6829153597773256
264264,528529,528528,1057057,1024.876347064972,0.6804608658057987
265265,530531,530530,1061061,1029.2141313552856,0.6780233252047765
266266,532533,532532,1065065,1033.5218570232391,0.6756025636168488
267267,534535,534534,1069069,1037.2364153862,0.6731984090711194
268268,536537,536536,1073073,1040.7161831855774,0.6708106919468264
269269,538539,538538,1077077,1044.14586019516,0.6684392449278675
270270,540541,540540,1081081,1047.6245560646057,0.6660839029682393
271271,542543,542542,1085085,1052.2278912067413,0.663744503253838
272272,544545,544544,1089089,1056.7511463165283,0.6614208851533476
273273,546547,546546,1093093,1061.4749891757965,0.6591128902036871
274274,548549,548548,1097097,1065.5449793338776,0.6568203620463464
275275,550551,550550,1101101,1069.6838593482971,0.6545431464146532
276276,552553,552552,1105105,1074.3656511306763,0.6522810910882981
277277,554555,554554,1109109,1078.5629041194916,0.6500340458551364
278278,556557,556556,1113113,1082.4044601917267,0.6478018624911783
279279,558559,558558,1117117,1086.1876270771027,0.6455843947205722
280280,560561,560560,1121121,1089.8606872558594,0.6433814981719479
281281,562563,562562,1125125,1093.5893912315369,0.6411930303711415
282282,564565,564564,1129129,1097.8954610824585,0.6390188506920822
283283,566567,566566,1133133,1102.2103481292725,0.6368588203295076
284284,568569,568568,1137137,1106.5552382469177,0.6347128022753168
285285,570571,570570,1141141,1110.6858241558075,0.6325806612840097
286286,572573,572572,1145145,1115.17293715477,0.630462263847221
287287,574575,574574,1149149,1119.0555832386017,0.6283574781664356
288288,576577,576576,1153153,1123.0218741893768,0.6262661741184274
289289,578579,578578,1157157,1126.8736600875854,0.6241882232425269
290290,580581,580580,1161161,1131.5062642097473,0.6221234986933268
291291,582583,582582,1165165,1136.3736109733582,0.620075567620006
292292,584585,584584,1169169,1141.506997346878,0.6180415113940398
293293,586587,586586,1173173,1145.6248261928558,0.6160203920262575
294294,588589,588588,1177177,1149.7534823417664,0.6140120452710107
295295,590591,590590,1181181,1154.401908159256,0.6120163258565299
296296,592593,592592,1185185,1159.0058062076569,0.6100331002871826
297297,594595,594594,1189189,1163.2603282928467,0.608062242723463
298298,596597,596596,1193193,1167.385400056839,0.6061036325336318
299299,598599,598598,1197197,1171.1011183261871,0.6041571528203349
300300,600601,600600,1201201,1174.6044752597809,0.6022226895129279
301301,602603,602602,1205205,1178.0783081054688,0.6003001308090461
302302,604605,604604,1209209,1181.543424129486,0.5983893668289966
303303,606607,606606,1213213,1185.1531882286072,0.5964902893610997
304304,608609,608608,1217217,1188.6234080791473,0.5946064948675485
305305,610611,610610,1221221,1192.1017031669617,0.5927347973192809
306306,612613,612612,1225225,1195.5969820022583,0.5908745419401384
307307,614615,614614,1229229,1199.034418106079,0.589025570643571
308308,616617,616616,1233233,1202.4582509994507,0.587187758032087
309309,618619,618618,1237237,1205.9368391036987,0.5853609934511042
310310,620621,620620,1241241,1209.4567711353302,0.5835451733692025
311311,622623,622622,1245245,1212.9010820388794,0.5817401980475552
312312,624625,624624,1249249,1216.3419570922852,0.5799459701065643
313313,626627,626626,1253253,1219.7905042171478,0.5781623938655684
314314,628629,628628,1257257,1223.1667261123657,0.5763893750154239
315315,630631,630630,1261261,1226.7409892082214,0.5746268204984517
316316,632633,632632,1265265,1230.3473782539368,0.5728746384047554
317317,634635,634634,1269269,1233.9139420986176,0.5711327379449358
318318,636637,636636,1273273,1239.0840742588043,0.5694010293955216
319319,638639,638638,1277277,1243.9810991287231,0.5676794241007883
320320,640641,640640,1281281,1247.4920091629028,0.5659678344381973
321321,642643,642642,1285285,1251.2219722270966,0.5642661737947492
322322,644645,644644,1289289,1255.0074911117554,0.5625743565706216
323323,646647,646646,1293293,1259.3197371959686,0.5608922981409705
324324,648649,648648,1297297,1263.515601158142,0.5592199148577492
325325,650651,650650,1301301,1267.8572373390198,0.5575571240224235
326326,652653,652652,1305305,1272.4200892448425,0.5559038438805146
327327,654655,654654,1309309,1277.1754531860352,0.5542599936070474
328328,656657,656656,1313313,1281.3545053005219,0.5526254932847223
329329,658659,658658,1317317,1286.2246491909027,0.5510002639020968
330330,660661,660660,1321321,1290.7185173034668,0.5493842273299379
331331,662663,662662,1325325,1295.1890811920166,0.5477773063194036
332332,664665,664664,1329329,1299.783907175064,0.546179424480215
333333,666667,666666,1333333,1304.6851303577423,0.544590506271561
334334,668669,668668,1337337,1309.4837012290955,0.543010476998461
335335,670671,670670,1341341,1313.4726431369781,0.5414392627772031
336336,672673,672672,1345345,1317.733546257019,0.5398767905589921
337337,674675,674674,1349349,1322.330244064331,0.5383229880826548
338338,676677,676676,1353353,1325.865757226944,0.5367777838837355
339339,678679,678678,1357357,1329.3155381679535,0.5352411072890391
340340,680681,680680,1361361,1332.8576292991638,0.5337128883784317
341341,682683,682682,1365365,1336.4902420043945,0.5321930580103071
342342,684685,684684,1369369,1339.993324995041,0.53068154777975
343343,686687,686686,1373373,1344.6457033157349,0.5291782900349062
344344,688689,688688,1377377,1350.2570459842682,0.5276832178387849
345345,690691,690690,1381381,1356.005315065384,0.5261962649892666
346346,692693,692692,1385385,1360.6808743476868,0.524717365982724
347347,694695,694694,1389389,1364.989179134369,0.5232464560231165
348348,696697,696696,1393393,1368.9566712379456,0.5217834710038005
349349,698699,698698,1397397,1372.7180552482605,0.5203283475020726
350350,700701,700700,1401401,1376.601849079132,0.5188810227682552
351351,702703,702702,1405405,1381.4420561790466,0.5174414347147831
352352,704705,704704,1409409,1386.0807271003723,0.5160095219143841
353353,706707,706706,1413413,1390.0318830013275,0.5145852235818893
354354,708709,708708,1417417,1394.1821072101593,0.5131684795705951
355355,710711,710710,1421421,1398.2742471694946,0.5117592303686251
356356,712713,712712,1425425,1402.4046802520752,0.5103574170825596
357357,714715,714714,1429429,1406.4652881622314,0.5089629814319778
358358,716717,716716,1433433,1412.4596982002258,0.5075758657476399
359359,718719,718718,1437437,1417.2204620838165,0.5061960129478393
360360,720721,720720,1441441,1421.8511400222778,0.5048233665547741
361361,722723,722722,1445445,1426.4552931785583,0.5034578706618049
362362,724725,724724,1449449,1431.2153673171997,0.5020994699407311
363363,726727,726726,1453453,1436.4769971370697,0.5007481096363335
364364,728729,728728,1457457,1441.5361881256104,0.4994037355463661
365365,730731,730730,1461461,1446.2551171779633,0.4980662940251932
366366,732733,732732,1465465,1450.9590542316437,0.49673573197287624
367367,734735,734734,1469469,1456.796420097351,0.49541199683335435
368368,736737,736736,1473473,1462.2334172725677,0.49409503657807363
369369,738739,738738,1477477,1468.5720052719116,0.49278479969871114
370370,740741,740740,1481481,1473.936504125595,0.49148123521990783
371371,742743,742742,1485485,1478.8655881881714,0.49018429266834573
372372,744745,744744,1489489,1483.782291173935,0.4888939220854809
373373,746747,746746,1493493,1488.8481931686401,0.48761007400025846
374374,748749,748748,1497497,1494.4667613506317,0.48633269944548374
375375,750751,750750,1501501,1500.1719789505005,0.48506174993963214
376376,752753,752752,1505505,1505.535562992096,0.48379717748321127
377377,754755,754754,1509509,1510.2867341041565,0.48253893454420904
378378,756757,756756,1513513,1515.2033281326294,0.48128697407264553
379379,758759,758758,1517517,1519.9594333171844,0.4800412494751072
380380,760761,760760,1521521,1524.7632203102112,0.47880171461656573
381381,762763,762762,1525525,1529.5435631275177,0.4775683238131023
382382,764765,764764,1529529,1534.5856742858887,0.47634103183554544
383383,766767,766766,1533533,1539.4419281482697,0.475119793887643
384384,768769,768768,1537537,1544.2431001663208,0.4739045656151575
385385,770771,770770,1541541,1549.1065862178802,0.4726953030876757
386386,772773,772772,1545545,1553.9089422225952,0.4714919628095231
387387,774775,774774,1549549,1558.737622976303,0.4702945016997546
388388,776777,776776,1553553,1563.4843802452087,0.4691028770957928
389389,778779,778778,1557557,1568.6419591903687,0.4679170467388758
390390,780781,780780,1561561,1573.4107670783997,0.4667369687849714
391391,782783,782782,1565565,1578.3499341011047,0.46556260178658704
392392,784785,784784,1569569,1583.1400320529938,0.46439390469458885
393393,786787,786786,1573573,1588.0486941337585,0.46323083683819277
394394,788789,788788,1577577,1592.781967163086,0.46207335795588733
395395,790791,790790,1581581,1597.619972229004,0.46092142815177795
396396,792793,792792,1585585,1602.3776743412018,0.4597750079083198
397397,794795,794794,1589589,1607.1510062217712,0.45863405808631796
398398,796797,796796,1593593,1612.0480470657349,0.45749853991401324
399399,798799,798798,1597597,1616.7545430660248,0.4563684149816254
400400,800801,800800,1601601,1622.0734519958496,0.4552436452413531
401401,802803,802802,1605605,1627.0845229625702,0.4541241930000979
402402,804805,804804,1609609,1631.9854190349579,0.4530100209176453
403403,806807,806806,1613613,1637.0663783550262,0.45190109200302686
404404,808809,808808,1617617,1641.2258653640747,0.4507973695999681
405405,810811,810810,1621621,1645.8773260116577,0.44969881740325945
406406,812813,812812,1625625,1650.1589500904083,0.44860539943692856
407407,814815,814814,1629629,1653.856714963913,0.447517080061516
408408,816817,816816,1633633,1658.0349543094635,0.4464338239540666
409409,818819,818818,1637637,1661.9289720058441,0.4453555961335951
410410,820821,820820,1641641,1666.130210161209,0.4442823619247065
411411,822823,822822,1645645,1669.6481840610504,0.4432140869739669
412412,824825,824824,1649649,1673.4715340137482,0.44215073724080867
413413,826827,826826,1653653,1677.1264083385468,0.4410922789993492
414414,828829,828828,1657657,1680.6413581371307,0.4400386788202013
415415,830831,830830,1661661,1684.4364511966705,0.43898990358684387
416416,832833,832832,1665665,1688.616670370102,0.4379459204737941
417417,834835,834834,1669669,1692.2700412273407,0.4369066969575215
418418,836837,836836,1673673,1696.1736302375793,0.4358722008000768
419419,838839,838838,1677677,1700.5045311450958,0.4348424000581872
420420,840841,840840,1681681,1704.9272429943085,0.43381726307598
421421,842843,842842,1685685,1708.7812809944153,0.43279675847770704
422422,844845,844844,1689689,1712.5898931026459,0.43178085516592546
423423,846847,846846,1693693,1716.4002873897552,0.4307695223233168
424424,848849,848848,1697697,1721.0046591758728,0.42976272940177296
425425,850851,850850,1701701,1725.0590620040894,0.42876044612967235
426426,852853,852852,1705705,1729.6357321739197,0.4277626424936898
427427,854855,854854,1709709,1733.244648218155,0.42676928874789155
428428,856857,856856,1713713,1737.080070257187,0.42578035538645054
429429,858859,858858,1717717,1740.6764752864838,0.424795813180026
430430,860861,860860,1721721,1744.0223271846771,0.4238156331466598
431431,862863,862862,1725725,1747.410441160202,0.4228397865608713
432432,864865,864864,1729729,1750.8246581554413,0.4218682449482003
433433,866867,866866,1733733,1754.2602121829987,0.4209009800833883
434434,868869,868868,1737737,1757.6699981689453,0.4199379639903782
435435,870871,870870,1741741,1761.033910036087,0.41897916892958165
436436,872873,872872,1745745,1764.4561681747437,0.4180245674069738
437437,874875,874874,1749749,1767.9414582252502,0.41707413216317946
438438,876877,876876,1753753,1771.2986731529236,0.41612783617893
439439,878879,878878,1757757,1774.6986773014069,0.41518565266051155
440440,880881,880880,1761761,1778.0653681755066,0.4142475550506788
441441,882883,882882,1765765,1781.472073316574,0.4133135170177411
442442,884885,884884,1769769,1784.9698233604431,0.4123835124555626
443443,886887,886886,1773773,1788.2921640872955,0.41145751547810505
444444,888889,888888,1777777,1791.7067413330078,0.41053550042306597
445445,890891,890890,1781781,1796.610784292221,0.4096174418446026
446446,892893,892892,1785785,1801.6142671108246,0.40870331451515085
447447,894895,894894,1789789,1805.6892442703247,0.4077930934181495
448448,896897,896896,1793793,1809.9175691604614,0.4068867537462211
449449,898899,898898,1797797,1813.8758211135864,0.4059842709048098
450450,900901,900900,1801801,1818.9941339492798,0.4050856205049058
451451,902903,902902,1805805,1823.1029653549194,0.40419077836122597
452452,904905,904904,1809809,1827.0884501934052,0.403299720490395
453453,906907,906906,1813813,1831.6608412265778,0.40241242311458336
454454,908909,908908,1817817,1835.7834141254425,0.40152886264331755
455455,910911,910910,1821821,1839.8921611309052,0.40064901569348876
456456,912913,912912,1825825,1844.373458147049,0.39977285906752513
457457,914915,914914,1829829,1847.9315283298492,0.39890036976612464
458458,916917,916916,1833833,1851.3296251296997,0.39803152498097916
459459,918919,918918,1837837,1854.7605612277985,0.3971663020820415
460460,920921,920920,1841841,1858.1779391765594,0.3963046786320774
461461,922923,922922,1845845,1861.7013471126556,0.39544663238302746
462462,924925,924924,1849849,1865.1827402114868,0.3945921412578173
463463,926927,926926,1853853,1868.885555267334,0.39374118337036634
464464,928929,928928,1857857,1872.2696101665497,0.39289373700739816
465465,930931,930930,1861861,1875.8367280960083,0.39204978063389717
466466,932933,932932,1865865,1879.2131371498108,0.3912092928912898
467467,934935,934934,1869869,1882.6602239608765,0.3903722525883495
468468,936937,936936,1873873,1886.0829710960388,0.3895386387139297
469469,938939,938938,1877877,1889.628573179245,0.3887084304169548
470470,940941,940940,1881881,1892.9925680160522,0.38788160702642926
471471,942943,942942,1885885,1896.4744791984558,0.3870581480296096
472472,944945,944944,1889889,1899.8893361091614,0.3862380330756423
473473,946947,946946,1893893,1903.4184532165527,0.385421241984659
474474,948949,948948,1897897,1906.8314232826233,0.3846077547332243
475475,950951,950950,1901901,1910.2604310512543,0.3837975514561549
476476,952953,952952,1905905,1913.6364710330963,0.3829906124537956
477477,954955,954954,1909909,1917.1315541267395,0.3821869181738293
478478,956957,956956,1913913,1920.5220773220062,0.3813866466007312
479479,958959,958958,1917917,1923.9538233280182,0.38059045380578027
480480,960961,960960,1921921,1927.5849850177765,0.37979747100507666
481481,962963,962962,1925925,1931.3182101249695,0.3790076554978441
482482,964965,964964,1929929,1935.6588401794434,0.3782209870478255
483483,966967,966966,1933933,1940.141041278839,0.3774374464137509
484484,968969,968968,1937937,1944.5798723697662,0.37665701482728764
485485,970971,970970,1941941,1948.4910531044006,0.3758796738293313
486486,972973,972972,1945945,1952.9113702774048,0.37510540515722823
487487,974975,974974,1949949,1956.485532283783,0.3743341907284048
488488,976977,976976,1953953,1959.788553237915,0.37356601630199293
489489,978979,978978,1957957,1963.1790392398834,0.3728008618181775
490490,980981,980980,1961961,1966.78635430336,0.37203870870143874
491491,982983,982982,1965965,1970.1354880332947,0.37127953921299195
492492,984985,984984,1969969,1973.5113971233368,0.370523335866892
493493,986987,986986,1973973,1976.9553091526031,0.3697700813681877
494494,988989,988988,1977977,1980.3737442493439,0.3690197585765418
495495,990991,990990,1981981,1983.9994843006134,0.3682723505080503
496496,992993,992992,1985985,1988.610433101654,0.36752784030977637
497497,994995,994994,1989989,1993.0840141773224,0.3667862112615694
498498,996997,996996,1993993,1997.769424200058,0.366047446781522
499499,998999,998998,1997997,2002.0296003818512,0.36531153041141806
500501,1001003,1001002,2002005,2006.0177471637726,0.3645777148758498
501502,1003005,1003004,2006009,2010.097617149353,0.3638474486560881
502503,1005007,1005006,2010013,2014.3587582111359,0.3631199819064932
503504,1007009,1007008,2014017,2018.309172153473,0.3623952986636141
504505,1009011,1009010,2018021,2022.11687707901,0.36167338308951
505506,1011013,1011012,2022025,2026.289174079895,0.3609542194590176
506507,1013015,1013014,2026029,2030.2054562568665,0.36023779217430274
507508,1015017,1015016,2030033,2034.0663380622864,0.3595240857448516
508509,1017019,1017018,2034037,2037.88183426857,0.3588130848020228
509510,1019021,1019020,2038041,2041.7393951416016,0.3581047740917711
510511,1021023,1021022,2042045,2045.560776233673,0.35739913847646676
511512,1023025,1023024,2046049,2049.4223160743713,0.35669616292216233
512513,1025027,1025026,2050053,2053.353338241577,0.3559958325186017
513514,1027029,1027028,2054057,2058.6507182121277,0.35529813245739206
514515,1029031,1029030,2058061,2064.006545305252,0.3546030480410991
515516,1031033,1031032,2062065,2068.5824749469757,0.35391056469052273
516517,1033035,1033034,2066069,2073.737066268921,0.35322066792105034
517518,1035037,1035036,2070073,2080.0226442813873,0.35253334336084663
518519,1037039,1037038,2074077,2085.249703168869,0.35184857674175873
519520,1039041,1039040,2078081,2090.1787481307983,0.3511663539065921
520521,1041043,1041042,2082085,2095.0051572322845,0.3504866607945587
521522,1043045,1043044,2086089,2099.3284101486206,0.34980948345582874
522523,1045047,1045046,2090093,2103.5663232803345,0.349134808029703
523524,1047049,1047048,2094097,2107.8050141334534,0.3484626207700785
524525,1049051,1049050,2098101,2112.1243031024933,0.34779290801998286
525526,1051053,1051052,2102105,2116.386913061142,0.34712565623522096
526527,1053055,1053054,2106109,2120.741932153702,0.34646085194981424
527528,1055057,1055056,2110113,2125.278600215912,0.34579848181783746
528529,1057059,1057058,2114117,2129.532879114151,0.3451385325697629
529530,1059061,1059060,2118121,2133.945965051651,0.3444809910488402
530531,1061063,1061062,2122125,2138.333424091339,0.3438258441783546
531532,1063065,1063064,2126129,2142.5362071990967,0.3431730789852736
532533,1065067,1065066,2130133,2147.9036540985107,0.3425226825875143
533534,1067069,1067068,2134137,2152.117287158966,0.34187464219030517
534535,1069071,1069070,2138141,2156.0139582157135,0.3412289451007382
535536,1071073,1071072,2142145,2159.9061481952667,0.34058557870412187
536537,1073075,1073074,2146149,2163.906302213669,0.3399445304839901
537538,1075077,1075076,2150153,2167.7261941432953,0.33930578801300726
538539,1077079,1077078,2154157,2171.6819932460785,0.3386693389438733
539540,1079081,1079080,2158161,2175.5847132205963,0.33803517102751357
540541,1081083,1081082,2162165,2179.4896721839905,0.33740327209488896
541542,1083085,1083084,2166169,2183.43017911911,0.33677363006245287
542543,1085087,1085086,2170173,2187.4664533138275,0.33614623293760815
543544,1087089,1087088,2174177,2191.489891052246,0.3355210688041552
544545,1089091,1089090,2178181,2195.374687194824,0.334898125836844
545546,1091093,1091092,2182185,2199.280172109604,0.33427739228864084
546547,1093095,1093094,2186189,2203.2208292484283,0.33365885649618576
547548,1095097,1095096,2190193,2207.152501344681,0.3330425068779732
548549,1097099,1097098,2194197,2211.382154941559,0.33242833193617116
549550,1099101,1099100,2198201,2215.4820053577423,0.3318163202438882
550551,1101103,1101102,2202205,2219.4628479480743,0.3312064604670013
551552,1103105,1103104,2206209,2223.4993681907654,0.3305987413350522
552553,1105107,1105106,2210213,2227.656678199768,0.32999315166671295
553554,1107109,1107108,2214217,2231.4911301136017,0.3293896803570533
554555,1109111,1109110,2218221,2235.7479553222656,0.3287883163757215
555556,1111113,1111112,2222225,2239.6273012161255,0.32818904875966837
556557,1113115,1113114,2226229,2243.7461450099945,0.32759186664043227
557558,1115117,1115116,2230233,2247.6856219768524,0.3269967592059402
558559,1117119,1117118,2234237,2251.7518503665924,0.3264037157277926
559560,1119121,1119120,2238241,2255.7585892677307,0.32581272555034957
560561,1121123,1121122,2242245,2259.882063150406,0.3252237780889118
561562,1123125,1123124,2246249,2263.9423060417175,0.3246368628297205
562563,1125127,1125126,2250253,2268.0437881946564,0.3240519693317765
563564,1127129,1127128,2254257,2271.9162571430206,0.3234690872304782
564565,1129131,1129130,2258261,2275.9665870666504,0.3228882062212506
565566,1131133,1131132,2262265,2279.932613134384,0.3223093160777353
566567,1133135,1133134,2266269,2284.8305191993713,0.32173240663905744
567568,1135137,1135136,2270273,2289.645221233368,0.32115746781528287
568569,1137139,1137138,2274277,2294.2820081710815,0.320584489578323
569570,1139141,1139140,2278281,2298.329277276993,0.3200134619783057
570571,1141143,1141142,2282285,2302.459857225418,0.3194443751217477
571572,1143145,1143144,2286289,2306.1786201000214,0.3188772191879252
572573,1145147,1145146,2290293,2309.7698612213135,0.31831198441977904
573574,1147149,1147148,2294297,2313.1011922359467,0.31774866112391464
574575,1149151,1149150,2298301,2316.5494000911713,0.3171872396742401
575576,1151153,1151152,2302305,2320.0270183086395,0.31662771050832816
576577,1153155,1153154,2306309,2323.513035058975,0.3160700641292351
577578,1155157,1155156,2310313,2327.233255147934,0.31551429109458695
578579,1157159,1157158,2314317,2330.7878980636597,0.31496038203658827
579580,1159161,1159160,2318321,2334.642966032028,0.3144083276420133
580581,1161163,1161162,2322325,2339.2455921173096,0.313858118657663
581582,1163165,1163164,2326329,2343.2196111679077,0.3133097459012788
582583,1165167,1165166,2330333,2347.2988801002502,0.31276320023971493
583584,1167169,1167168,2334337,2351.2134730815887,0.3122184726053092
584585,1169171,1169170,2338341,2355.0969161987305,0.3116755539922451
585586,1171173,1171172,2342345,2358.8451471328735,0.3111344354456378
586587,1173175,1173174,2346349,2363.0910251140594,0.310595108077905
587588,1175177,1175176,2350353,2367.8284211158752,0.31005756305785326
588589,1177179,1177178,2354357,2372.640011072159,0.30952179160158266
589590,1179181,1179180,2358361,2377.980401277542,0.30898778500340995
590591,1181183,1181182,2362365,2382.0924232006073,0.30845553459039365
591592,1183185,1183184,2366369,2386.3172092437744,0.30792503176598984
592593,1185187,1185186,2370373,2390.540163040161,0.30739626797549136
593594,1187189,1187188,2374377,2395.822480201721,0.3068692347242177
594595,1189191,1189190,2378381,2400.6161913871765,0.30634392357751494
595596,1191193,1191192,2382385,2406.2859382629395,0.30582032614438504
596597,1193195,1193194,2386389,2411.311756134033,0.30529843410113244
597598,1195197,1195196,2390393,2415.6853642463684,0.3047782391658984
598599,1197199,1197198,2394397,2420.255615234375,0.30425973311685084
599600,1199201,1199200,2398401,2425.0329761505127,0.30374290778127033
600601,1201203,1201202,2402405,2430.7922642230988,0.3032277550428262
601602,1203205,1203204,2406409,2435.797045946121,0.3027142668288434
602603,1205207,1205206,2410413,2440.4683990478516,0.30220243512849265
603604,1207209,1207208,2414417,2444.99489402771,0.30169225197823835
604605,1209211,1209210,2418421,2449.1912171840668,0.3011837094600196
605606,1211213,1211212,2422425,2453.6202170848846,0.3006767997103452
606607,1213215,1213214,2426429,2457.7583191394806,0.3001715149202937
607608,1215217,1215216,2430433,2462.241960287094,0.2996678473227803
608609,1217219,1217218,2434437,2466.2153992652893,0.29916578920165193
609610,1219221,1219220,2438441,2470.095078229904,0.2986653328916873
610611,1221223,1221222,2442445,2474.1374802589417,0.2981664707749587
611612,1223225,1223224,2446449,2478.094075202942,0.2976691952771944
612613,1225227,1225226,2450453,2482.6767992973328,0.297173498884149
613614,1227229,1227228,2454457,2487.823217153549,0.2966793741143192
614615,1229231,1229230,2458461,2492.723930120468,0.29618681353895226
615616,1231233,1231232,2462465,2497.2767663002014,0.29569580977658916
616617,1233235,1233234,2466469,2501.11354804039,0.2952063554948836
617618,1235237,1235236,2470473,2505.6589481830597,0.2947184433978691
618619,1237239,1237238,2474477,2510.700328350067,0.2942320662441489
619620,1239241,1239240,2478481,2515.5438010692596,0.29374721683052485
620621,1241243,1241242,2482485,2520.4555842876434,0.29326388800836867
621622,1243245,1243244,2486489,2524.7237679958344,0.2927820726599748
622623,1245247,1245246,2490493,2528.6877710819244,0.2923017637240264
623624,1247249,1247248,2494497,2533.1125180721283,0.29182295417194837
624625,1249251,1249250,2498501,2536.9188022613525,0.2913456370260974
625626,1251253,1251252,2502505,2540.84997010231,0.29086980535248586
626627,1253255,1253254,2506509,2544.691376209259,0.29039545224986796
627628,1255257,1255256,2510513,2548.484896183014,0.2899225708733866
628629,1257259,1257258,2514517,2552.3949921131134,0.2894511544109264
629630,1259261,1259260,2518521,2556.3258333206177,0.28898119609402784
630631,1261263,1261262,2522525,2560.107931137085,0.2885126891960681
631632,1263265,1263264,2526529,2563.9389741420746,0.2880456270304421
632633,1265267,1265266,2530533,2567.7882602214813,0.2875800029542006
633634,1267269,1267268,2534537,2571.6607241630554,0.28711581036077405
634635,1269271,1269270,2538541,2575.7631862163544,0.2866530426854297
635636,1271273,1271272,2542545,2580.1092541217804,0.2861916934052715
636637,1273275,1273274,2546549,2584.019475221634,0.2857317560374213
637638,1275277,1275276,2550553,2587.9754853248596,0.2852732241299236
638639,1277279,1277278,2554557,2591.904461145401,0.2848160912817548
639640,1279281,1279280,2558561,2595.849263191223,0.2843603511191759
640641,1281283,1281282,2562565,2599.668538093567,0.2839059973193798
641642,1283285,1283284,2566569,2603.565357208252,0.2834530235868442
642643,1285287,1285286,2570573,2607.4621522426605,0.2830014236642455
643644,1287289,1287288,2574577,2611.6844589710236,0.28255119134155393
644645,1289291,1289290,2578581,2615.736438035965,0.28210232043420547
645646,1291293,1291292,2582585,2620.3500893115997,0.28165480480674887
646647,1293295,1293294,2586589,2624.816430091858,0.28120863834556076
647648,1295297,1295296,2590593,2629.486376285553,0.28076381498431147
648649,1297299,1297298,2594597,2634.4627912044525,0.2803203286930511
649650,1299301,1299300,2598601,2638.6784512996674,0.2798781734727527
650651,1301303,1301302,2602605,2642.7129940986633,0.2794373433589499
651652,1303305,1303304,2606609,2647.37988615036,0.2789978324290132
652653,1305307,1305306,2610613,2652.0488970279694,0.278559634791236
653654,1307309,1307308,2614617,2656.4028720855713,0.2781227445884724
654655,1309311,1309310,2618621,2660.9182393550873,0.2776871559963183
655656,1311313,1311312,2622625,2665.8875682353973,0.27725286323220644
656657,1313315,1313314,2626629,2670.738715171814,0.2768198605408543
657658,1315317,1315316,2630633,2675.213366985321,0.2763881422015402
658659,1317319,1317318,2634637,2679.9327280521393,0.27595770253174123
659660,1319321,1319320,2638641,2684.6244921684265,0.2755285358725814
660661,1321323,1321322,2642645,2688.6398482322693,0.27510063660884043
661662,1323325,1323324,2646649,2692.4339802265167,0.27467399915258284
662663,1325327,1325326,2650653,2696.3190472126007,0.27424861795225297
663664,1327329,1327328,2654657,2700.2591800689697,0.273824487481761
664665,1329331,1329330,2658661,2704.3001792430878,0.27340160225321597
665666,1331333,1331332,2662665,2708.256058216095,0.2729799568114686
666667,1333335,1333334,2666669,2712.452346086502,0.2725595457250165
667668,1335337,1335336,2670673,2716.377921104431,0.27214036360237515
668669,1337339,1337338,2674677,2720.2181470394135,0.27172240507934475
669670,1339341,1339340,2678681,2724.2023112773895,0.2713056648262864
670671,1341343,1341342,2682685,2728.238890171051,0.2708901375372079
671672,1343345,1343344,2686689,2732.1759662628174,0.2704758179424971
672673,1345347,1345346,2690693,2736.212969303131,0.2700627007998264
673674,1347349,1347348,2694697,2740.6351573467255,0.26965078090324823
674675,1349351,1349350,2698701,2745.145215988159,0.26924005306864274
675676,1351353,1351352,2702705,2749.8501551151276,0.26883051214463194
676677,1353355,1353354,2706709,2754.412851333618,0.2684221530089417
677678,1355357,1355356,2710713,2759.1700100898743,0.2680149705702206
678679,1357359,1357358,2714717,2763.8282899856567,0.26760895976622123
679680,1359361,1359360,2718721,2768.4428951740265,0.26720411556198087
680681,1361363,1361362,2722725,2773.308799266815,0.2668004329480027
681682,1363365,1363364,2726729,2778.3421223163605,0.2663979069511697
682683,1365367,1365366,2730733,2783.4723110198975,0.2659965326220117
683684,1367369,1367368,2734737,2788.474067211151,0.2655963050365244
684685,1369371,1369370,2738741,2793.131668329239,0.2651972193052643
685686,1371373,1371372,2742745,2798.152595281601,0.2647992705587967
686687,1373375,1373374,2746749,2803.0262660980225,0.26440245395860984
687688,1375377,1375376,2750753,2807.7096843719482,0.2640067646989337
688689,1377379,1377378,2754757,2812.440008163452,0.26361219799036917
689690,1379381,1379380,2758761,2817.4404122829437,0.26321874908171594
690691,1381383,1381382,2762765,2822.302119255066,0.2628264132363256
691692,1383385,1383384,2766769,2827.1937172412872,0.26243518575574853
692693,1385387,1385386,2770773,2832.816375017166,0.262045061959725
693694,1387389,1387388,2774777,2838.0903301239014,0.2616560371952801
694695,1389391,1389390,2778781,2842.8503732681274,0.2612681068403617
695696,1391393,1391392,2782785,2848.632763147354,0.26088126629474573
696697,1393395,1393394,2786789,2853.7768721580505,0.26049551098549273
697698,1395397,1395396,2790793,2858.6637670993805,0.2601108363633102
698699,1397399,1397398,2794797,2863.4022283554077,0.2597272379007336
699700,1399401,1399400,2798801,2868.3988831043243,0.259344711106678
700701,1401403,1401402,2802805,2873.8751032352448,0.25896325150279154
701702,1403405,1403404,2806809,2880.345852136612,0.2585828546416451
702703,1405407,1405406,2810813,2886.342609167099,0.25820351610127545
703704,1407409,1407408,2814817,2891.6619622707367,0.25782523147972825
704705,1409411,1409410,2818821,2896.974911212921,0.25744799640051497
705706,1411413,1411412,2822825,2901.8947381973267,0.25707180651625094
706707,1413415,1413414,2826829,2906.718607187271,0.2566966574995604
707708,1415417,1415416,2830833,2911.559735059738,0.2563225450430764
708709,1417419,1417418,2834837,2916.515273332596,0.25594946486853587
709710,1419421,1419420,2838841,2921.601709127426,0.2555774127213226
710711,1421423,1421422,2842845,2926.680436372757,0.25520638436137233
711712,1423425,1423424,2846849,2931.905862092972,0.2548363755850005
712713,1425427,1425426,2850853,2938.114709377289,0.2544673822048935
713714,1427429,1427428,2854857,2944.3923723697662,0.25409940005374665
714715,1429431,1429430,2858861,2949.3946681022644,0.25373242498790205
715716,1431433,1431432,2862865,2954.424651145935,0.25336645289462467
716717,1433435,1433434,2866869,2959.3020589351654,0.25300147966845543
717718,1435437,1435436,2870873,2963.3436920642853,0.25263750124031503
718719,1437439,1437438,2874877,2967.8830151557922,0.2522745135556761
719720,1439441,1439440,2878881,2971.655750274658,0.2519125125836581
720721,1441443,1441442,2882885,2975.401031255722,0.2515514943133894
721722,1443445,1443444,2886889,2978.7874920368195,0.25119145475946425
722723,1445447,1445446,2890893,2982.1913599967957,0.2508323899546667
723724,1447449,1447448,2894897,2985.6497342586517,0.2504742959536088
724725,1449451,1449450,2898901,2989.4414851665497,0.2501171688309114
725726,1451453,1451452,2902905,2992.9159893989563,0.24976100468848017
726727,1453455,1453454,2906909,2996.559947013855,0.24940579963913478
727728,1455457,1455456,2910913,3001.002346277237,0.2490515498247987
728729,1457459,1457458,2914917,3005.6408910751343,0.24869825140376633
729730,1459461,1459460,2918921,3010.6413333415985,0.2483459005579789
730731,1461463,1461462,2922925,3015.144773244858,0.24799449348574854
731732,1463465,1463464,2926929,3018.5315062999725,0.24764402640721528
732733,1465467,1465466,2930933,3022.0127601623535,0.24729449556434702
733734,1467469,1467468,2934937,3025.8483831882477,0.24694589721730154
734735,1469471,1469470,2938941,3029.3338911533356,0.24659822764442652
735736,1471473,1471472,2942945,3032.80007314682,0.2462514831495355
736737,1473475,1473474,2946949,3036.2491402626038,0.24590566004735592
737738,1475477,1475476,2950953,3039.5801362991333,0.24556075467808114
738739,1477479,1477478,2954957,3043.0785291194916,0.24521676340191334
739740,1479481,1479480,2958961,3046.484062194824,0.24487368259360665
740741,1481483,1481482,2962965,3049.875679254532,0.24453150865156204
741742,1483485,1483484,2966969,3053.265248298645,0.24419023799237038
742743,1485487,1485486,2970973,3057.1912240982056,0.24384986705081246
743744,1487489,1487488,2974977,3061.1397643089294,0.24351039227258298
744745,1489491,1489490,2978981,3064.5405061244965,0.24317181013429945
745746,1491493,1491492,2982985,3067.9453961849213,0.24283411712531233
746747,1493495,1493494,2986989,3071.5221722126007,0.24249730975316197
747748,1495497,1495496,2990993,3075.844973087311,0.24216138454175962
748749,1497499,1497498,2994997,3079.9878561496735,0.24182633804048237
749750,1499501,1499500,2999001,3084.420312166214,0.2414921668059833
750751,1501503,1501502,3003005,3088.7487790584564,0.24115886742220027
751752,1503505,1503504,3007009,3093.312391281128,0.24082643648398516
752753,1505507,1505506,3011013,3097.003988265991,0.24049487061165564
753754,1507509,1507508,3015017,3100.8956921100616,0.24016416643280536
754755,1509511,1509510,3019021,3105.2026612758636,0.2398343206004938
755756,1511513,1511512,3023025,3109.9316132068634,0.23950532978051342
756757,1513515,1513514,3027029,3114.186671257019,0.2391771906586655
757758,1515517,1515516,3031033,3118.471620082855,0.23884989993894123
758759,1517519,1517518,3035037,3121.98721408844,0.2385234543344268
759760,1519521,1519520,3039041,3126.3245401382446,0.23819785058549314
760761,1521523,1521522,3043045,3131.1259241104126,0.23787308544524421
761762,1523525,1523524,3047049,3135.306313276291,0.23754915567769785
762763,1525527,1525526,3051053,3140.3014571666718,0.23722605806869979
763764,1527529,1527528,3055057,3145.992125272751,0.2369037894259236
764765,1529531,1529530,3059061,3151.3027822971344,0.2365823465606809
765766,1531533,1531532,3063065,3156.391442298889,0.23626172631156805
766767,1533535,1533534,3067069,3160.949261188507,0.23594192552809545
767768,1535537,1535536,3071073,3165.844600200653,0.23562294107614434
768769,1537539,1537538,3075077,3173.175401210785,0.23530476983978588
769770,1539541,1539540,3079081,3181.5291740894318,0.23498740871582413
770771,1541543,1541542,3083085,3187.409699201584,0.2346708546156151
771772,1543545,1543544,3087089,3193.2137322425842,0.23435510447052366
772773,1545547,1545546,3091093,3198.5261261463165,0.23404015522828558
773774,1547549,1547548,3095097,3203.9737191200256,0.23372602167728473
774775,1549551,1549550,3099101,3210.027833223343,0.23341270703349437
775776,1551553,1551552,3103105,3215.4425930976868,0.233100185289004
776777,1553555,1553554,3107109,3220.2418780326843,0.2327884526566777
777778,1555557,1555556,3111113,3225.1430792808533,0.2324775060515094
778779,1557559,1557558,3115117,3229.9782462120056,0.23216734247580462
779780,1559561,1559560,3119121,3234.6858479976654,0.23185795895915362
780781,1561563,1561562,3123125,3239.458393096924,0.23154935255843156
781782,1563565,1563564,3127129,3245.164924144745,0.23124152034324652
782783,1565567,1565566,3131133,3253.1613070964813,0.23093445940503443
783784,1567569,1567568,3135137,3260.6484310626984,0.23062816684978316
784785,1569571,1569570,3139141,3268.2834134101868,0.23032263980530843
785786,1571573,1571572,3143145,3275.715228319168,0.23001787539760699
786787,1573575,1573574,3147149,3283.326473236084,0.22971387078723637
787788,1575577,1575576,3151153,3290.8169481754303,0.22941062313111615
788789,1577579,1577578,3155157,3298.6061103343964,0.2291081296170887
789790,1579581,1579580,3159161,3306.7663872241974,0.22880638743299642
790791,1581583,1581582,3163165,3315.0606923103333,0.22850539378850954
791792,1583585,1583584,3167169,3323.192142009735,0.22820514590603125
792793,1585587,1585586,3171173,3330.971155166626,0.22790564101887867
793794,1587589,1587588,3175177,3338.572552204132,0.22760687637492083
794795,1589591,1589590,3179181,3346.577210187912,0.22730884923839767
795796,1591593,1591592,3183185,3354.6717162132263,0.22701155688446306
796797,1593595,1593594,3187189,3362.530310153961,0.2267149966010038
797798,1595597,1595596,3191193,3370.58385515213,0.2264191656922776
798799,1597599,1597598,3195197,3378.985915184021,0.22612406147527508
799800,1599601,1599600,3199201,3387.114328145981,0.22582968127426284
800801,1601603,1601602,3203205,3395.2907671928406,0.22553602243533533
801802,1603605,1603604,3207209,3403.3951210975647,0.22524308231186296
802803,1605607,1605606,3211213,3412.8424570560455,0.2249508582699491
803804,1607609,1607608,3215217,3421.914238214493,0.22465934769206797
804805,1609611,1609610,3219221,3431.744725227356,0.22436854797160777
805806,1611613,1611612,3223225,3441.067983150482,0.22407845650923264
806807,1613615,1613614,3227229,3449.6597340106964,0.22378907073289156
807808,1615617,1615616,3231233,3458.3735830783844,0.22350038806507655
808809,1617619,1617618,3235237,3467.110871076584,0.22321240595374547
809810,1619621,1619620,3239241,3475.7241451740265,0.22292512185413216
810811,1621623,1621622,3243245,3484.437296152115,0.22263853323056537
811812,1623625,1623624,3247249,3493.1625320911407,0.22235263757102075
812813,1625627,1625626,3251253,3501.786389350891,0.22206743235983595
813814,1627629,1627628,3255257,3511.1194140911102,0.2217829151031765
814815,1629631,1629630,3259261,3519.8272802829742,0.22149908332175983
815816,1631633,1631632,3263265,3529.253045320511,0.22121593453994137
816817,1633635,1633634,3267269,3538.170619249344,0.22093346629844746
817818,1635637,1635636,3271273,3546.709141969681,0.22065167614891834
818819,1637639,1637638,3275277,3555.255844116211,0.2203705616575462
819820,1639641,1639640,3279281,3564.0813863277435,0.2200901203941612
820821,1641643,1641642,3283285,3573.626139163971,0.21981034995405935
821822,1643645,1643644,3287289,3582.618198156357,0.21953124792707968
822823,1645647,1645646,3291293,3591.990026950836,0.2192528119267081
823824,1647649,1647648,3295297,3600.7386631965637,0.21897503957552544
824825,1649651,1649650,3299301,3611.086451292038,0.21869792850156955
825826,1651653,1651652,3303305,3621.493383169174,0.2184214763565251
826827,1653655,1653654,3307309,3632.2160172462463,0.2181456807829818
827828,1655657,1655656,3311313,3643.796555995941,0.2178705394580902
828829,1657659,1657658,3315317,3652.3333423137665,0.21759605005354388
829830,1659661,1659660,3319321,3661.0143580436707,0.21732221025740728
830831,1661663,1661662,3323325,3669.7670860290527,0.2170490177704778
831832,1663665,1663664,3327329,3679.4889709949493,0.21677647029900982
832833,1665667,1665666,3331333,3688.910982131958,0.21650456556562858
833834,1667669,1667668,3335337,3697.777684211731,0.21623330130205431
834835,1669671,1669670,3339341,3706.673821210861,0.21596267524910218
835836,1671673,1671672,3343345,3715.5988132953644,0.21569268516032025
836837,1673675,1673674,3347349,3724.51518201828,0.2154233287947136
837838,1675677,1675676,3351353,3734.454131126404,0.21515460393129615
838839,1677679,1677678,3355357,3744.1093401908875,0.21488650834908185
839840,1679681,1679680,3359361,3753.1913273334503,0.21461903984345554
840841,1681683,1681682,3363365,3761.715914964676,0.21435219622253499
841842,1683685,1683684,3367369,3771.4179232120514,0.21408597529443796
842843,1685687,1685686,3371373,3781.7828600406647,0.2138203748872911
843844,1687689,1687688,3375377,3791.0950503349304,0.21355539283649705
844845,1689691,1689690,3379381,3800.0930433273315,0.21329102698655333
845846,1691693,1691692,3383385,3808.9316811561584,0.2130272769718431
846847,1693695,1693694,3387389,3817.876328229904,0.21276418453999213
847848,1695697,1695696,3391393,3826.821038007736,0.21250172047621163
848849,1697699,1697698,3395397,3835.865839242935,0.21223986901895842
849850,1699701,1699700,3399401,3847.2713062763214,0.21197862445842475
850851,1701703,1701702,3403405,3856.249873161316,0.21171798366958683
851852,1703705,1703704,3407409,3868.3184020519257,0.2114579442604736
852853,1705707,1705706,3411413,3879.034994125366,0.2111985040592117
853854,1707709,1707708,3415417,3888.714592218399,0.21093966098123929
854855,1709711,1709710,3419421,3897.3154151439667,0.21068141295472742
855856,1711713,1711712,3423425,3907.1747171878815,0.21042375792967505
856857,1713715,1713714,3427429,3916.089472055435,0.21016669386517606
857858,1715717,1715716,3431433,3925.0854601860046,0.20991021873305726
858859,1717719,1717718,3435437,3934.195997238159,0.2096543305178784
859860,1719721,1719720,3439441,3943.012731075287,0.20939902720056125
860861,1721723,1721722,3443445,3951.8431169986725,0.20914430678567442
861862,1723725,1723724,3447449,3960.7453951835632,0.20889016727960552
862863,1725727,1725726,3451453,3970.5131661891937,0.2086366066996561
863864,1727729,1727728,3455457,3982.2728292942047,0.2083836230685847
864865,1729731,1729730,3459461,3993.298065185547,0.20813121442552074
865866,1731733,1731732,3463465,4007.0637571811676,0.2078793788114126
866867,1733735,1733734,3467469,4018.218947172165,0.20762811427994166
867868,1735737,1735736,3471473,4030.386236190796,0.2073774188902462
868869,1737739,1737738,3475477,4040.7734031677246,0.20712729071783542
869870,1739741,1739740,3479481,4050.4507870674133,0.20687772783458058
870871,1741743,1741742,3483485,4060.231951236725,0.20662872833418078
871872,1743745,1743744,3487489,4069.759891271591,0.20638029030669713
872873,1745747,1745746,3491493,4078.793795108795,0.20613241186219966
873874,1747749,1747748,3495497,4087.775068283081,0.20588509111257736
874875,1749751,1749750,3499501,4096.989281177521,0.20563832617881417
875876,1751753,1751752,3503505,4107.576776266098,0.205392115190989
876877,1753755,1753754,3507509,4117.1283440589905,0.20514645628463768
877878,1755757,1755756,3511513,4126.010889291763,0.204901347613486
878879,1757759,1757758,3515517,4134.800635099411,0.20465678732580272
879880,1759761,1759760,3519521,4143.671045064926,0.20441277358986554
880881,1761763,1761762,3523525,4154.312458276749,0.2041693045739521
881882,1763765,1763764,3527529,4165.739144325256,0.203926378460892
882883,1765767,1765766,3531533,4174.545470237732,0.20368399343533383
883884,1767769,1767768,3535537,4184.747846126556,0.20344214769465907
884885,1769771,1769770,3539541,4193.78284907341,0.20320083944352518
885886,1771773,1771772,3543545,4202.544151067734,0.2029600668902276
886887,1773775,1773774,3547549,4211.24317407608,0.2027198282594327
887888,1775777,1775776,3551553,4221.23131108284,0.20248012177398778
888889,1777779,1777778,3555557,4230.983318090439,0.20224094567129214
889890,1779781,1779780,3559561,4240.972854137421,0.20200229819784
890891,1781783,1781782,3563565,4251.770377159119,0.20176417760012555
891892,1783785,1783784,3567569,4262.78558921814,0.20152658213737595
892893,1785787,1785786,3571573,4273.086463928223,0.2012895100779133
893894,1787789,1787788,3575577,4283.075603246689,0.20105295969369763
894895,1789791,1789790,3579581,4293.474320173264,0.20081692926942196
895896,1791793,1791792,3583585,4304.189484119415,0.20058141709159827
896897,1793795,1793794,3587589,4315.0615911483765,0.20034642145583348
897898,1795797,1795796,3591593,4325.998502254486,0.20011194066682947
898899,1797799,1797798,3595597,4336.343725204468,0.19987797303838306
899900,1799801,1799800,3599601,4347.153606176376,0.19964451688611007
900901,1801803,1801802,3603605,4356.663206100464,0.19941157053835923
901902,1803805,1803804,3607609,4367.09770321846,0.19917913233075524
902903,1805807,1805806,3611613,4376.971967935562,0.19894720060074178
903904,1807809,1807808,3615617,4387.987623214722,0.1987157736930385
904905,1809811,1809810,3619621,4398.496542215347,0.19848484997237392
905906,1811813,1811812,3623625,4408.608777284622,0.19825442779256264
906907,1813815,1813814,3627629,4419.4725041389465,0.19802450552379014
907908,1815817,1815816,3631633,4429.519345283508,0.19779508154715586
908909,1817819,1817818,3635637,4440.020916223526,0.19756615424194024
909910,1819821,1819820,3639641,4449.6171362400055,0.19733772200015665
910911,1821823,1821822,3643645,4459.046957015991,0.19710978321927541
911912,1823825,1823824,3647649,4467.704124212265,0.19688233630768082
912913,1825827,1825826,3651653,4476.222738265991,0.19665537966648117
913914,1827829,1827828,3655657,4484.727791070938,0.19642891172406962
914915,1829831,1829830,3659661,4493.278173208237,0.1962029308961064
915916,1831833,1831832,3663665,4501.421577215195,0.19597743562189862
916917,1833835,1833834,3667669,4510.451247215271,0.19575242433529638
917918,1835837,1835836,3671673,4520.291295289993,0.19552789548470173
918919,1837839,1837838,3675677,4528.923567056656,0.1953038475185167
919920,1839841,1839840,3679681,4537.500285148621,0.19508027889787627
920921,1841843,1841842,3683685,4546.021283149719,0.1948571880839154
921922,1843845,1843844,3687689,4554.5576202869415,0.19463457355050195
922923,1845847,1845846,3691693,4563.071155309677,0.19441243377696082
923924,1847849,1847848,3695697,4571.571081161499,0.19419076724625484
924925,1849851,1849850,3699701,4580.107153177261,0.1939695724468038
925926,1851853,1851852,3703705,4588.690680027008,0.19374884788157942
926927,1853855,1853854,3707709,4597.1876101493835,0.19352859204627748
927928,1855857,1855856,3711713,4605.695560216904,0.1933088034620596
928929,1857859,1857858,3715717,4614.6655061244965,0.19308948063735443
929930,1859861,1859860,3719721,4624.978462219238,0.19287062209150463
930931,1861863,1861862,3723725,4635.393958091736,0.1926522263620427
931932,1863865,1863864,3727729,4646.32662820816,0.19243429198104423
932933,1865867,1865866,3731733,4656.876565217972,0.19221681748786068
933934,1867869,1867868,3735737,4666.822055101395,0.19199980142911954
934935,1869871,1869870,3739741,4676.5471522808075,0.19178324236236222
935936,1871873,1871872,3743745,4685.7976541519165,0.1915671388433111
936937,1873875,1873874,3747749,4694.472738027573,0.19135148944042157
937938,1875877,1875876,3751753,4703.2395231723785,0.19113629272578692
938939,1877879,1877878,3755757,4712.114273071289,0.19092154727331945
939940,1879881,1879880,3759761,4721.51641535759,0.1907072516678454
940941,1881883,1881882,3763765,4731.005597114563,0.190493404503286
941942,1883885,1883884,3767769,4739.924067020416,0.19028001099650282
942943,1885887,1885886,3771773,4749.016988277435,0.19006707363769237
943944,1887889,1887888,3775777,4758.048006296158,0.18985458207498596
944945,1889891,1889890,3779781,4767.1040761470795,0.18964253366539197
945946,1891893,1891892,3783785,4775.739253282547,0.18943092683912255
946947,1893895,1893894,3787789,4784.359100103378,0.18921976019191789
947948,1895897,1895896,3791793,4792.984539270401,0.18900903235225996
948949,1897899,1897898,3795797,4801.630628108978,0.18879874195044977
949950,1899901,1899900,3799801,4810.209264278412,0.18858888763134019
950951,1901903,1901902,3803805,4818.197125196457,0.18837946803432715
951952,1903905,1903904,3807809,4827.01046705246,0.18817048182063445
952953,1905907,1905906,3811813,4836.147899150848,0.18796192764239095
953954,1907909,1907908,3815817,4847.292273283005,0.18775380416445842
954955,1909911,1909910,3819821,4860.074617147446,0.1875461100553366
955956,1911913,1911912,3823825,4870.719047307968,0.18733884399443923
956957,1913915,1913914,3827829,4880.5382261276245,0.18713200465754198
957958,1915917,1915916,3831833,4890.9580950737,0.18692559072951553
958959,1917919,1917918,3835837,4902.074375152588,0.1867196009043255
959960,1919921,1919920,3839841,4912.292825222015,0.18651403387593746
960961,1921923,1921922,3843845,4921.8882212638855,0.186308888347412
961962,1923925,1923924,3847849,4932.224029302597,0.18610416302362864
962963,1925927,1925926,3851853,4942.5497941970825,0.1858998566185619
963964,1927929,1927928,3855857,4952.748279094696,0.18569596785164322
964965,1929931,1929930,3859861,4961.617380142212,0.18549249544230406
965966,1931933,1931932,3863865,4971.307018995285,0.18528943811907084
966967,1933935,1933934,3867869,4980.264045000076,0.1850867946195649
967968,1935937,1935936,3871873,4990.033259153366,0.18488456367413164
968969,1937939,1937938,3875877,4999.563332080841,0.18468274403312535
969970,1939941,1939940,3879881,5008.93634724617,0.18448133444144332
970971,1941943,1941942,3883885,5017.949813365936,0.18428033365489682
971972,1943945,1943944,3887889,5027.139635324478,0.18407974043111608
972973,1945947,1945946,3891893,5036.580265283585,0.1838795535350073
973974,1947949,1947948,3895897,5047.704317331314,0.18367977173147665
974975,1949951,1949950,3899901,5058.097496032715,0.18348039379816328
975976,1951953,1951952,3903905,5067.44180226326,0.18328141851452528
976977,1953955,1953954,3907909,5076.29954123497,0.18308284466365876
977978,1955957,1955956,3911913,5085.118828058243,0.18288467103047878
978979,1957959,1957958,3915917,5094.376396179199,0.18268689640899538
979980,1959961,1959960,3919921,5104.26030421257,0.1824895196041325
980981,1961963,1961962,3923925,5114.71527504921,0.1822925394099002
981982,1963965,1963964,3927929,5124.97597527504,0.18209595464031736
982983,1965967,1965966,3931933,5135.3084881305695,0.18189976410576492
983984,1967969,1967968,3935937,5144.642578125,0.18170396662389976
984985,1969971,1969970,3939941,5153.781028032303,0.18150856101601676
985986,1971973,1971972,3943945,5162.335116147995,0.18131354611068673
986987,1973975,1973974,3947949,5170.809029102325,0.18111892074011848
987988,1975977,1975976,3951953,5180.338858366013,0.1809246837401588
988989,1977979,1977978,3955957,5189.785209178925,0.18073083394665446
989990,1979981,1979980,3959961,5199.039835214615,0.18053737021182314
990991,1981983,1981982,3963965,5208.225892066956,0.18034429138424457
991992,1983985,1983984,3967969,5217.232542276382,0.18015159631431743
992993,1985987,1985986,3971973,5227.1373081207275,0.17995928386699234
993994,1987989,1987988,3975977,5235.683979988098,0.17976735290358192
994995,1989991,1989990,3979981,5244.524653196335,0.17957580229267478
995996,1991993,1991992,3983985,5253.694795131683,0.1793846309028595
996997,1993995,1993994,3987989,5262.784217119217,0.17919383761727659
997998,1995997,1995996,3991993,5271.923894166946,0.17900342131360958
998999,1997999,1997998,3995997,5281.427743196487,0.17881338088227494
1000000,2000001,2000000,4000001,5290.428626298904,0.17862371521187015


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.003580331802368164,12064.44795143716
1001,2003,1001,3004,3.297255277633667,1.0208544809865998
2002,4005,2002,6007,6.5950400829315186,0.1963330649305135
3003,6007,3003,9010,10.403073072433472,0.07454063132900046
4004,8009,4004,12013,14.045221328735352,0.036095311308599776
5005,10011,5005,15016,17.96530818939209,0.0203003074911976
6006,12013,6006,18019,21.80432415008545,0.01303998796720407
7007,14015,7007,21022,25.312960147857666,0.008390385557504487
8008,16017,8008,24025,28.575016975402832,0.005935084329394158
9009,18019,9009,27028,32.209025144577026,0.004151742561589344
10010,20021,10010,30031,35.89528703689575,0.002722964271015371
11011,22023,11011,33034,39.16694140434265,0.001570305317727616
12012,24025,12012,36037,44.19223618507385,0.0011662387132673757
13013,26027,13013,39040,48.38088822364807,0.0009639094387239311
14014,28029,14014,42043,52.51697635650635,0.0008122627114062198
15015,30031,15015,45046,56.256795167922974,0.0008630201446067076
16016,32033,16016,48049,60.85531711578369,0.0008201777545764344
17017,34035,17017,51052,64.16259717941284,0.0007163337904785294
18018,36037,18018,54055,68.25585412979126,0.0006060321884433506
19019,38039,19019,57058,71.88515424728394,0.0005556192627409473
20020,40041,20020,60061,75.46630024909973,0.0003564142516552238
21021,42043,21021,63064,78.91943407058716,0.00029010928483330645
22022,44045,22022,66067,82.78361916542053,0.0003425906706979731
23023,46047,23023,69070,86.4918761253357,0.00017186377226607874
24024,48049,24024,72073,89.95764923095703,0.000212398945222958
25025,50051,25025,75076,93.41383123397827,0.00018215225281892344
26026,52053,26026,78079,97.03635931015015,0.00017645176194491796
27027,54055,27027,81082,100.83073735237122,0.00017036563622241374
28028,56057,28028,84085,105.0214033126831,0.00010074830788653344
29029,58059,29029,87088,108.204763174057,0.0001371430462313583
30030,60061,30030,90091,111.40122604370117,0.00014272142107074615
31031,62063,31031,93094,114.60598921775818,0.00011921375335077755
32032,64065,32032,96097,117.8048882484436,0.00012144873471697792
33033,66067,33033,99100,120.94433617591858,0.00015765292846481316
34034,68069,34034,102103,124.10033321380615,9.251608207705431e-05
35035,70071,35035,105106,127.30742025375366,9.336265065940097e-05
36036,72073,36036,108109,130.45642113685608,6.60748773952946e-05
37037,74075,37037,111112,133.7576870918274,7.306640145543497e-05
38038,76077,38038,114115,136.9587631225586,7.999372792255599e-05
39039,78079,39039,117118,140.1417043209076,3.6568211726262234e-05
40040,80081,40040,120121,143.3206582069397,6.276683052419685e-05
41041,82083,41041,123124,146.49146914482117,5.126327778270934e-05
42042,84085,42042,126127,149.62916111946106,4.9657883209874853e-05
43043,86087,43043,129130,152.79939723014832,5.61745237064315e-05
44044,88089,44044,132133,155.93991231918335,4.753062785312068e-05
45045,90091,45045,135136,159.14311623573303,5.61164542887127e-05
46046,92093,46046,138139,162.32872414588928,4.3460244341986254e-05
47047,94095,47047,141142,165.60465717315674,4.160032403888181e-05
48048,96097,48048,144145,168.97816014289856,4.0584447560831904e-05
49049,98099,49049,147148,172.19834923744202,3.739330713870004e-05
50050,100101,50050,150151,175.40866613388062,2.1718948119087145e-05
51051,102103,51051,153154,178.58151721954346,2.4137611035257578e-05
52052,104105,52052,156157,181.86277723312378,2.3374417651211843e-05
53053,106107,53053,159160,185.03511714935303,2.8929569452884607e-05
54054,108109,54054,162163,188.17504739761353,2.57865776802646e-05
55055,110111,55055,165166,191.3879861831665,2.516750646464061e-05
56056,112113,56056,168169,194.57408022880554,1.990168857446406e-05
57057,114115,57057,171172,197.73601007461548,1.9727178369066678e-05
58058,116117,58058,174175,200.9184992313385,1.7300282706855796e-05
59059,118119,59059,177178,204.0706250667572,1.5901217921054922e-05
60060,120121,60060,180181,207.30166220664978,1.4990311683504842e-05
61061,122123,61061,183184,210.49787020683289,1.7393573216395453e-05
62062,124125,62062,186187,213.66258215904236,1.2470214642235078e-05
63063,126127,63063,189190,216.85601615905762,1.3740555004915223e-05
64064,128129,64064,192193,220.01064229011536,1.1518548490130343e-05
65065,130131,65065,195196,223.1496262550354,1.0775558621389791e-05
66066,132133,66066,198199,226.34386920928955,1.0985613698721863e-05
67067,134135,67067,201202,229.5062391757965,6.312797268037684e-06
68068,136137,68068,204205,232.69480228424072,8.129776688292623e-06
69069,138139,69069,207208,235.8570532798767,8.23834488983266e-06
70070,140141,70070,210211,239.08361506462097,7.72059865994379e-06
71071,142143,71071,213214,242.2823622226715,6.724583727191202e-06
72072,144145,72072,216217,245.42807817459106,6.124108040239662e-06
73073,146147,73073,219220,248.5796720981598,4.367906512925401e-06
74074,148149,74074,222223,251.74220418930054,3.304276106064208e-06
75075,150151,75075,225226,254.87605142593384,3.2687148632248864e-06
76076,152153,76076,228229,258.0489022731781,2.1690939320251346e-06
77077,154155,77077,231232,261.1933083534241,1.6267495084321126e-06
78078,156157,78078,234235,264.29287815093994,2.0032184693263844e-06
79079,158159,79079,237238,267.44551706314087,2.462809788994491e-06
80080,160161,80080,240241,270.559451341629,2.8357189876260236e-06
81081,162163,81081,243244,273.76848125457764,3.2661500881658867e-06
82082,164165,82082,246247,276.85422801971436,3.326456862851046e-06
83083,166167,83083,249250,279.99240016937256,3.2561856642132625e-06
84084,168169,84084,252253,283.1654920578003,3.1800173019291833e-06
85085,170171,85085,255256,286.2973051071167,2.623892214614898e-06
86086,172173,86086,258259,289.4583013057709,2.0789993868675083e-06
87087,174175,87087,261262,292.642804145813,1.5854766388656572e-06
88088,176177,88088,264265,295.8160722255707,9.143132047029212e-07
89089,178179,89089,267268,299.010498046875,8.343868103111163e-07
90090,180181,90090,270271,302.1786892414093,8.144979801727459e-07
91091,182183,91091,273274,306.8746192455292,8.688512025400996e-07
92092,184185,92092,276277,310.2984571456909,1.3256794773042202e-06
93093,186187,93093,279280,313.5646622180939,1.5226760297082365e-06
94094,188189,94094,282283,316.79523730278015,1.8473419913789257e-06
95095,190191,95095,285286,320.26638627052307,2.193231921410188e-06
96096,192193,96096,288289,323.7895612716675,2.11359110835474e-06
97097,194195,97097,291292,327.32075214385986,1.9830913515761495e-06
98098,196197,98098,294295,330.8375811576843,1.7146630852948874e-06
99099,198199,99099,297298,335.1216871738434,1.246815372724086e-06
100100,200201,100100,300301,338.8825333118439,9.155774023383856e-07
101101,202203,101101,303304,342.3950500488281,6.462068995460868e-07
102102,204205,102102,306307,345.76324915885925,3.758286766242236e-07
103103,206207,103103,309310,349.089768409729,3.674704203149304e-07
104104,208209,104104,312313,352.5329473018646,4.931334842694923e-07
105105,210211,105105,315316,355.8682162761688,6.672198651358485e-07
106106,212213,106106,318319,359.23396730422974,9.961604519048706e-07
107107,214215,107107,321322,363.0134162902832,1.22525125334505e-06
108108,216217,108108,324325,366.3960962295532,1.3425215001916513e-06
109109,218219,109109,327328,370.4585871696472,1.433800207450986e-06
110110,220221,110110,330331,374.30129623413086,1.32111381390132e-06
111111,222223,111111,333334,377.81336522102356,1.1299871403025463e-06
112112,224225,112112,336337,380.9395761489868,9.039413271239027e-07
113113,226227,113113,339340,384.14056396484375,5.773890734417364e-07
114114,228229,114114,342343,387.321622133255,3.665591066237539e-07
115115,230231,115115,345346,390.44110012054443,2.54722181125544e-07
116116,232233,116116,348349,393.5697112083435,1.8745959096122533e-07
117117,234235,117117,351352,396.7194871902466,3.028253559023142e-07
118118,236237,118118,354355,399.91465520858765,4.525572876445949e-07
119119,238239,119119,357358,403.0905044078827,6.094778655096889e-07
120120,240241,120120,360361,406.212354183197,8.387705747736618e-07
121121,242243,121121,363364,409.3611693382263,9.45403371588327e-07
122122,244245,122122,366367,412.5560541152954,9.721879905555397e-07
123123,246247,123123,369370,415.87339425086975,9.503000910626724e-07
124124,248249,124124,372373,419.0607831478119,7.860271580284461e-07
125125,250251,125125,375376,422.20889234542847,6.07578840572387e-07
126126,252253,126126,378379,425.35492730140686,4.390694812173024e-07
127127,254255,127127,381382,428.4773733615875,2.5410918169654906e-07
128128,256257,128128,384385,431.6292722225189,1.5341538528446108e-07
129129,258259,129129,387388,434.7275803089142,1.406751835020259e-07
130130,260261,130130,390391,438.0094599723816,1.7588536138646305e-07
131131,262263,131131,393394,441.2619512081146,2.9684633773285896e-07
132132,264265,132132,396397,444.4083571434021,4.5144042815081775e-07
133133,266267,133133,399400,447.53328824043274,5.589354259427637e-07
134134,268269,134134,402403,450.66063022613525,6.648970156675205e-07
135135,270271,135135,405406,453.8954863548279,7.018825272098184e-07
136136,272273,136136,408409,457.01966619491577,6.507216312456876e-07
137137,274275,137137,411412,460.14765906333923,5.851870810147375e-07
138138,276277,138138,414415,463.3576192855835,4.4223452277947217e-07
139139,278279,139139,417418,466.5001952648163,2.9618058761116117e-07
140140,280281,140140,420421,469.66695618629456,1.982516550924629e-07
141141,282283,141141,423424,472.90657210350037,1.0734220268204808e-07
142142,284285,142142,426427,477.9913651943207,1.0315125109627843e-07
143143,286287,143143,429430,482.01249837875366,1.4760189515072852e-07
144144,288289,144144,432433,485.731121301651,2.109773049596697e-07
145145,290291,145145,435436,489.2296311855316,3.2230855140369385e-07
146146,292293,146146,438439,492.86696910858154,4.164212441537529e-07
147147,294295,147147,441442,496.3175003528595,4.791345418198034e-07
148148,296297,148148,444445,499.48525738716125,5.109413905302063e-07
149149,298299,149149,447448,503.25299525260925,4.840130714001134e-07
150150,300301,150150,450451,507.1379282474518,4.1035673348233104e-07
151151,302303,151151,453454,511.13674330711365,3.258573997300118e-07
152152,304305,152152,456457,515.7137973308563,2.2945096134208143e-07
153153,306307,153153,459460,519.9109551906586,1.3869248505216092e-07
154154,308309,154154,462463,524.0524742603302,9.924042387865484e-08
155155,310311,155155,465466,527.869707107544,8.159440767485648e-08
156156,312313,156156,468469,532.6489143371582,1.0572694009169936e-07
157157,314315,157157,471472,536.6530072689056,1.7883576219901443e-07
158158,316317,158158,474475,540.5184662342072,2.393790055066347e-07
159159,318319,159159,477478,544.3114802837372,3.11465555569157e-07
160160,320321,160160,480481,548.1780722141266,3.6365418054629117e-07
161161,322323,161161,483484,552.2479212284088,3.666864358820021e-07
162162,324325,162162,486487,556.0151982307434,3.572367859305814e-07
163163,326327,163163,489490,559.9871129989624,3.061777533730492e-07
164164,328329,164164,492493,563.5196161270142,2.345077518839389e-07
165165,330331,165165,495496,567.2732653617859,1.7125967133324593e-07
166166,332333,166166,498499,571.1982622146606,1.0875010048039258e-07
167167,334335,167167,501502,575.0881590843201,7.592461770400405e-08
168168,336337,168168,504505,578.6301991939545,7.547896530013531e-08
169169,338339,169169,507508,582.1504702568054,9.775067155715078e-08
170170,340341,170170,510511,585.7338240146637,1.4158104022499174e-07
171171,342343,171171,513514,589.3606162071228,1.9676554074976593e-07
172172,344345,172172,516517,593.0365533828735,2.427295839879662e-07
173173,346347,173173,519520,596.691504240036,2.725155354710296e-07
174174,348349,174174,522523,600.5350782871246,2.849719749065116e-07
175175,350351,175175,525526,604.7113630771637,2.6173620426561683e-07
176176,352353,176176,528529,609.6812691688538,2.244760253233835e-07
177177,354355,177177,531532,613.5665583610535,1.78561094799079e-07
178178,356357,178178,534535,617.5913071632385,1.2122109183110297e-07
179179,358359,179179,537538,621.1076142787933,8.796450856607407e-08
180180,360361,180180,540541,624.6756701469421,6.60929799778387e-08
181181,362363,181181,543544,628.3491752147675,6.247501005418599e-08
182182,364365,182182,546547,631.9639141559601,9.06111381482333e-08
183183,366367,183183,549550,635.5171382427216,1.2089003575965762e-07
184184,368369,184184,552553,639.7546441555023,1.6050580597948283e-07
185185,370371,185185,555556,643.2861351966858,1.9730214262381196e-07
186186,372373,186186,558559,646.813449382782,2.1265259420033544e-07
187187,374375,187187,561562,650.8220753669739,2.1603773348033428e-07
188188,376377,188188,564565,655.1491982936859,1.9921390048693866e-07
189189,378379,189189,567568,659.2043421268463,1.6637204680591822e-07
190190,380381,190190,570571,662.9885582923889,1.2870077625848353e-07
191191,382383,191191,573574,666.5117242336273,9.279392543248832e-08
192192,384385,192192,576577,670.1399192810059,6.525806384161115e-08
193193,386387,193193,579580,673.8844721317291,5.4047632147558033e-08
194194,388389,194194,582583,677.4621760845184,6.157824827823788e-08
195195,390391,195195,585586,681.0028622150421,7.847484084777534e-08
196196,392393,196196,588589,684.7254571914673,1.0863732313737273e-07
197197,394395,197197,591592,688.2639622688293,1.3879616744816303e-07
198198,396397,198198,594595,692.0071370601654,1.588941813679412e-07
199199,398399,199199,597598,695.6107652187347,1.743010216159746e-07
200200,400401,200200,600601,699.1460702419281,1.6844023775774986e-07
201201,402403,201201,603604,702.8883442878723,1.5061050362419337e-07
202202,404405,202202,606607,707.4539241790771,1.2697091733571142e-07
203203,406407,203203,609610,712.1870472431183,9.291761671192944e-08
204204,408409,204204,612613,717.1675882339478,6.851223588455468e-08
205205,410411,205205,615616,722.4786350727081,5.135007086209953e-08
206206,412413,206206,618619,726.368860244751,4.424691724125296e-08
207207,414415,207207,621622,729.8849720954895,5.4898919188417494e-08
208208,416417,208208,624625,733.5643000602722,7.226663001347333e-08
209209,418419,209209,627628,737.3000960350037,9.596988093107939e-08
210210,420421,210210,630631,741.2170603275299,1.1974225344602019e-07
211211,422423,211211,633634,744.9905710220337,1.3559838407672942e-07
212212,424425,212212,636637,748.9725542068481,1.407825038768351e-07
213213,426427,213213,639640,753.2986931800842,1.3443059287965298e-07
214214,428429,214214,642643,757.046795129776,1.1800511856563389e-07
215215,430431,215215,645646,760.5621271133423,9.310133464168757e-08
216216,432433,216216,648649,764.4663150310516,7.01074895914644e-08
217217,434435,217217,651652,768.9625542163849,4.9569280236028135e-08
218218,436437,218218,654655,773.3335492610931,3.713466867338866e-08
219219,438439,219219,657658,776.8104393482208,3.936474968213588e-08
220220,440441,220220,660661,780.4282743930817,4.7475623432546854e-08
221221,442443,221221,663664,784.8535051345825,6.603477231692523e-08
222222,444445,222222,666667,789.1819462776184,8.768984116613865e-08
223223,446447,223223,669670,792.7778642177582,1.0352050594519824e-07
224224,448449,224224,672673,796.3341481685638,1.1696829460561275e-07
225225,450451,225225,675676,800.0525844097137,1.1766314855776727e-07
226226,452453,226226,678679,803.5481052398682,1.0859912435989827e-07
227227,454455,227227,681682,807.0784330368042,9.343602869194001e-08
228228,456457,228228,684685,811.7108631134033,7.106973498594016e-08
229229,458459,229229,687688,815.8964853286743,5.135007086209953e-08
230230,460461,230230,690691,819.5051522254944,3.608874976634979e-08
231231,462463,231231,693694,822.8244171142578,2.8774593374691904e-08
232232,464465,232232,696697,826.1715121269226,3.16504156216979e-08
233233,466467,233233,699700,829.5032742023468,4.2755345930345356e-08
234234,468469,234234,702703,832.8586812019348,5.973015504423529e-08
235235,470471,235235,705706,836.1645362377167,7.714697858318686e-08
236236,472473,236236,708709,839.4943952560425,9.287577995564789e-08
237237,474475,237237,711712,842.814935207367,1.0018811735790223e-07
238238,476477,238238,714715,846.1391360759735,9.908217180054635e-08
239239,478479,239239,717718,849.4112660884857,9.066206985153258e-08
240240,480481,240240,720721,852.6966421604156,7.308335625566542e-08
241241,482483,241241,723724,856.0682492256165,5.544461600948125e-08
242242,484485,242242,726727,859.3855392932892,3.8155121728777885e-08
243243,486487,243243,729730,862.6605021953583,2.515480446163565e-08
244244,488489,244244,732733,866.2431411743164,2.2688254830427468e-08
245245,490491,245245,735736,870.4019992351532,2.5956978788599372e-08
246246,492493,246246,738739,874.4645733833313,3.786772140301764e-08
247247,494495,247247,741742,878.178572177887,5.419860826805234e-08
248248,496497,248248,744745,881.7521800994873,6.90961314830929e-08
249249,498499,249249,747748,885.7161211967468,8.217102731578052e-08
250250,500501,250250,750751,889.654158115387,8.733513823244721e-08
251251,502503,251251,753754,892.9297332763672,8.488495950587094e-08
252252,504505,252252,756757,896.2202570438385,7.519702194258571e-08
253253,506507,253253,759760,899.5308690071106,5.988840712234378e-08
254254,508509,254254,762763,902.8108253479004,4.331013769842684e-08
255255,510511,255255,765766,906.0389711856842,2.8172507882118225e-08
256256,512513,256256,768769,909.3159942626953,1.9248545868322253e-08
257257,514515,257257,771772,912.8224601745605,1.663283910602331e-08
258258,516517,258258,774775,916.1385793685913,2.209890226367861e-08
259259,518519,259259,777778,919.7754471302032,3.3927790354937315e-08
260260,520521,260260,780781,923.6313152313232,4.7522917157039046e-08
261261,522523,261261,783784,928.0428280830383,6.253139872569591e-08
262262,524525,262262,786787,931.6499762535095,7.229209586512297e-08
263263,526527,263263,789790,935.1990432739258,7.593916961923242e-08
264264,528529,264264,792793,938.7020783424377,7.35071807866916e-08
265265,530531,265265,795796,942.2780282497406,6.269874575082213e-08
266266,532533,266266,798799,945.6212034225464,4.934736352879554e-08
267267,534535,267267,801802,949.2798571586609,3.432978701312095e-08
268268,536537,268268,804805,952.8654112815857,2.1165760699659586e-08
269269,538539,269269,807808,956.434953212738,1.4380930224433541e-08
270270,540541,270270,810811,959.6467282772064,1.3009412214159966e-08
271271,542543,271271,813814,962.870658159256,1.907937985379249e-08
272272,544545,272272,816817,966.2136001586914,3.000604920089245e-08
273273,546547,273273,819820,969.7196662425995,4.305184120312333e-08
274274,548549,274274,822823,973.2172532081604,5.5631971918046474e-08
275275,550551,275275,825826,976.7209930419922,6.385926099028438e-08
276276,552553,276276,828829,980.035961151123,6.689879228360951e-08
277277,554555,277277,831832,983.6406753063202,6.278605724219233e-08
278278,556557,278278,834835,987.0575802326202,5.361471266951412e-08
279279,558559,279279,837838,990.6119680404663,4.099638317711651e-08
280280,560561,280280,840841,994.2274522781372,2.7224814402870834e-08
281281,562563,281281,843844,997.7959711551666,1.707303454168141e-08
282282,564565,282282,846847,1001.2741451263428,1.057560439221561e-08
283283,566567,283283,849850,1004.8791811466217,1.0722942533902824e-08
284284,568569,284284,852853,1008.3681161403656,1.696207618806511e-08
285285,570571,285285,855856,1011.8631024360657,2.6408088160678744e-08
286286,572573,286286,858859,1015.3900873661041,3.892091626767069e-08
287287,574575,287287,861862,1018.6910762786865,4.937282938044518e-08
288288,576577,288288,864865,1022.239128112793,5.634501576423645e-08
289289,578579,289289,867868,1026.1240870952606,5.853144102729857e-08
290290,580581,290290,870871,1030.0159192085266,5.404945113696158e-08
291291,582583,291291,873874,1034.0195672512054,4.5656634029001e-08
292292,584585,292292,876877,1037.8162910938263,3.399509296286851e-08
293293,586587,293293,879880,1041.4148013591766,2.229717210866511e-08
294294,588589,294294,882883,1044.6740591526031,1.3335011317394674e-08
295295,590591,295295,885886,1048.1651301383972,8.414644980803132e-09
296296,592593,296296,888889,1052.0424420833588,9.40781319513917e-09
297297,594595,297297,891892,1055.4161961078644,1.4902980183251202e-08
298298,596597,298298,894895,1058.777096271515,2.4383552954532206e-08
299299,598599,299299,897898,1062.1974611282349,3.4933691495098174e-08
300300,600601,300300,900901,1065.562902212143,4.394860297907144e-08
301301,602603,301301,903904,1069.1020963191986,5.016045179218054e-08
302302,604605,302302,906907,1072.54741024971,5.0702510634437203e-08
303303,606607,303303,909910,1076.1711213588715,4.691173671744764e-08
304304,608609,304304,912913,1080.3752629756927,3.890818334184587e-08
305305,610611,305305,915916,1084.2200713157654,2.8272552299313247e-08
306306,612613,306306,918919,1087.8659942150116,1.866646925918758e-08
307307,614615,307307,921922,1091.3681662082672,1.0611984180286527e-08
308308,616617,308308,924925,1095.198043346405,7.137714419513941e-09
309309,618619,309309,927928,1099.008723974228,8.481947588734329e-09
310310,620621,310310,930931,1103.2485401630402,1.3640601537190378e-08
311311,622623,311311,933934,1107.651560306549,2.2417225409299135e-08
312312,624625,312312,936937,1111.584478378296,3.143577487207949e-08
313313,626627,313313,939940,1115.6237502098083,3.9384758565574884e-08
314314,628629,314314,942943,1120.2629492282867,4.411595000419766e-08
315315,630631,315315,945946,1124.4143471717834,4.426510713528842e-08
316316,632633,316316,948949,1127.7497782707214,4.0477971197105944e-08
317317,634635,317317,951952,1131.761773109436,3.282912075519562e-08
318318,636637,318318,954955,1135.3627922534943,2.391607267782092e-08
319319,638639,319319,957958,1138.7875893115997,1.51885615196079e-08
320320,640641,320320,960961,1142.6090512275696,8.769347914494574e-09
321321,642643,321321,963964,1146.1748201847076,6.422851583920419e-09
322322,644645,322322,966967,1150.0042932033539,7.674316293559968e-09
323323,646647,323323,969970,1153.4393231868744,1.3191311154514551e-08
324324,648649,324324,972973,1157.019893169403,2.0700099412351847e-08
325325,650651,325325,975976,1160.8284742832184,2.8598151402547956e-08
326326,652653,326326,978979,1165.0779721736908,3.5521225072443485e-08
327327,654655,327327,981982,1168.9638051986694,3.8773578125983477e-08
328328,656657,328328,984985,1173.3059933185577,3.876448317896575e-08
329329,658659,329329,987988,1177.7016232013702,3.4784534364007413e-08
330330,660661,330330,990991,1182.1085031032562,2.7837813831865788e-08
331331,662663,331331,993994,1186.5642082691193,2.013257471844554e-08
332332,664665,332332,996997,1190.6040351390839,1.2496457202360034e-08
333333,666667,333333,1000000,1194.776700258255,7.517883204855025e-09
334334,668669,334334,1003003,1199.148383140564,5.73345459997654e-09
335335,670671,335335,1006006,1203.5001153945923,7.499693310819566e-09
336336,672673,336336,1009009,1207.8804681301117,1.2643795344047248e-08
337337,674675,337337,1012012,1212.2740232944489,1.923217496369034e-08
338338,676677,338338,1015015,1216.6082119941711,2.6364432414993644e-08
339339,678679,339339,1018018,1221.0556952953339,3.173408913426101e-08
340340,680681,340340,1021021,1225.3189933300018,3.4387994674034417e-08
341341,682683,341341,1024024,1228.9710652828217,3.38241079589352e-08
342342,684685,342342,1027027,1233.194803237915,2.9682269087061286e-08
343343,686687,343343,1030030,1236.9912242889404,2.373599272686988e-08
344344,688689,344344,1033033,1240.3909041881561,1.659827830735594e-08
345345,690691,345345,1036036,1244.2511103153229,1.0355506674386561e-08
346346,692693,346346,1039039,1248.5125651359558,6.484697223640978e-09
347347,694695,347347,1042042,1252.6473290920258,5.211404641158879e-09
348348,696697,348348,1045045,1257.0008990764618,7.583366823382676e-09
349349,698699,349349,1048048,1261.2100772857666,1.2187229003757238e-08
350350,700701,350350,1051051,1265.289705991745,1.8217178876511753e-08
351351,702703,351351,1054054,1269.5393691062927,2.43635440710932e-08
352352,704705,352352,1057057,1273.9944331645966,2.858359948731959e-08
353353,706707,353353,1060060,1278.3605921268463,3.0622686608694494e-08
354354,708709,354354,1063063,1282.6865541934967,2.9409420676529408e-08
355355,710711,355355,1066066,1287.2398731708527,2.5542249204590917e-08
356356,712713,356356,1069069,1291.4561762809753,2.0019797375425696e-08
357357,714715,357357,1072072,1295.7476541996002,1.3737007975578308e-08
358358,716717,358358,1075075,1300.2396001815796,8.692950359545648e-09
359359,718719,359359,1078078,1304.2871811389923,5.4551492212340236e-09
360360,720721,360360,1081081,1308.1786141395569,5.0895323511213064e-09
361361,722723,361361,1084084,1311.5802462100983,7.503331289626658e-09
362362,724725,362362,1087087,1315.6508994102478,1.1799784260801971e-08
363363,726727,363363,1090090,1319.2439692020416,1.742409949656576e-08
364364,728729,364364,1093093,1323.2681481838226,2.238448360003531e-08
365365,730731,365365,1096096,1326.9301261901855,2.5986082619056106e-08
366366,732733,366366,1099099,1330.9406452178955,2.722663339227438e-08
367367,734735,367367,1102102,1335.7637422084808,2.5573172024451196e-08
368368,736737,368368,1105105,1339.6438663005829,2.2000676835887134e-08
369369,738739,369369,1108108,1343.886057138443,1.6696503735147417e-08
370370,740741,370370,1111111,1348.0380942821503,1.1381416697986424e-08
371371,742743,371371,1114114,1352.6129071712494,7.148628355935216e-09
372372,744745,372372,1117117,1356.1618392467499,4.676621756516397e-09
373373,746747,373373,1120120,1360.148954153061,4.998582880944014e-09
374374,748749,374374,1123123,1364.8761851787567,7.397829904220998e-09
375375,750751,375375,1126126,1368.9015443325043,1.165062712971121e-08
376376,752753,376376,1129129,1372.3676953315735,1.657645043451339e-08
377377,754755,377377,1132132,1375.9112582206726,2.0809238776564598e-08
378378,756757,378378,1135135,1379.4242544174194,2.3728716769255698e-08
379379,758759,379379,1138138,1383.0964653491974,2.417982614133507e-08
380380,760761,380380,1141141,1386.583280324936,2.247179509140551e-08
381381,762763,381381,1144144,1390.3724942207336,1.8810169422067702e-08
382382,764765,382382,1147147,1394.4236001968384,1.3991666492074728e-08
383383,766767,383383,1150150,1397.83779835701,9.455106919631362e-09
384384,768769,384384,1153153,1401.2077140808105,5.764377419836819e-09
385385,770771,385385,1156156,1404.7439172267914,4.200046532787383e-09
386386,772773,386386,1159159,1408.0531301498413,4.793037078343332e-09
387387,774775,387387,1162162,1411.4393632411957,7.325070328079164e-09
388388,776777,388388,1165165,1414.8145911693573,1.145781425293535e-08
389389,778779,389389,1168168,1418.1441671848297,1.5688783605583012e-08
390390,780781,390390,1171171,1421.5825374126434,1.9457729649730027e-08
391391,782783,391391,1174174,1424.8746492862701,2.1604137145914137e-08
392392,784785,392392,1177177,1428.191665172577,2.1593223209492862e-08
393393,786787,393393,1180180,1431.6645550727844,1.973239704966545e-08
394394,788789,394394,1183183,1435.1935131549835,1.602711563464254e-08
395395,790791,395395,1186186,1438.544798374176,1.1761585483327508e-08
396396,792793,396396,1189189,1442.9886972904205,7.683411240577698e-09
397397,794795,397397,1192192,1447.761105298996,4.718458512797952e-09
398398,796797,398398,1195195,1452.7962112426758,3.752575139515102e-09
399399,798799,399399,1198198,1456.9255402088165,4.5947672333568335e-09
400400,800801,400400,1201201,1461.188047170639,7.374183041974902e-09
401401,802803,401401,1204204,1465.408194065094,1.1123120202682912e-08
402402,804805,402402,1207207,1469.449018239975,1.499574864283204e-08
403403,806807,403403,1210210,1473.1918063163757,1.8208083929494023e-08
404404,808809,404404,1213213,1476.8824772834778,1.9677827367559075e-08
405405,810811,405405,1216216,1480.560042142868,1.944681571330875e-08
406406,812813,406406,1219219,1484.227233171463,1.7264028429053724e-08
407407,814815,407407,1222222,1488.1228852272034,1.376247382722795e-08
408408,816817,408408,1225225,1491.344093322754,9.884388418868184e-09
409409,818819,409409,1228228,1494.5997960567474,6.2045728554949164e-09
410410,820821,410410,1231231,1497.8381161689758,3.954482963308692e-09
411411,822823,411411,1234234,1501.1086132526398,3.308741725049913e-09
412412,824825,412412,1237237,1504.4736561775208,4.49108483735472e-09
413413,826827,413413,1240240,1507.8459112644196,7.303242455236614e-09
414414,828829,414414,1243243,1511.126587152481,1.0741132427938282e-08
415415,830831,415415,1246246,1514.414588212967,1.4335455489344895e-08
416416,832833,416416,1249249,1517.6720242500305,1.6929334378801286e-08
417417,834835,417417,1252252,1520.8678493499756,1.802982296794653e-08
418418,836837,418418,1255255,1524.171203136444,1.7462298274040222e-08
419419,838839,419419,1258258,1528.089774131775,1.5115801943466067e-08
420420,840841,420420,1261261,1531.9908633232117,1.1867086868733168e-08
421421,842843,421421,1264264,1535.3770833015442,8.185452315956354e-09
422422,844845,422422,1267267,1538.7243301868439,5.078618414700031e-09
423423,846847,423423,1270270,1541.970857143402,3.27054294757545e-09
424424,848849,424424,1273273,1545.6634449958801,2.9576767701655626e-09
425425,850851,425425,1276276,1548.969876050949,4.474713932722807e-09
426426,852853,426426,1279279,1552.2052292823792,7.132257451303303e-09
427427,854855,427427,1282282,1555.4774241447449,1.0459189070388675e-08
428428,856857,428428,1285285,1559.1084952354431,1.3642420526593924e-08
429429,858859,429429,1288288,1562.54035115242,1.5752448234707117e-08
430430,860861,430430,1291291,1565.8432312011719,1.6581907402724028e-08
431431,862863,431431,1294294,1569.476490020752,1.5637851902283728e-08
432432,864865,432432,1297297,1572.7444741725922,1.3338649296201766e-08
433433,866867,433433,1300300,1575.9444181919098,1.0208168532699347e-08
434434,868869,434434,1303303,1579.3908281326294,6.8121153162792325e-09
435435,870871,435435,1306306,1583.0966620445251,4.2018655221909285e-09
436436,872873,436436,1309309,1586.871336221695,2.68664734903723e-09
437437,874875,437437,1312312,1590.387410402298,2.775777829810977e-09
438438,876877,438438,1315315,1594.0656032562256,4.380126483738422e-09
439439,878879,439439,1318318,1597.6384000778198,6.96672941558063e-09
440440,880881,440440,1321321,1601.0260531902313,1.014086592476815e-08
441441,882883,441441,1324324,1604.6435792446136,1.2872988008894026e-08
442442,884885,442442,1327327,1608.138776063919,1.4713805285282433e-08
443443,886887,443443,1330330,1611.6681292057037,1.5159457689151168e-08
444444,888889,444444,1333333,1615.3485991954803,1.40262272907421e-08
445445,890891,445445,1336336,1620.0544531345367,1.1785232345573604e-08
446446,892893,446446,1339339,1624.2304420471191,8.712959242984653e-09
447447,894895,447447,1342342,1627.8702092170715,5.727997631765902e-09
448448,896897,448448,1345345,1631.470540046692,3.4251570468768477e-09
449449,898899,449449,1348348,1635.3794882297516,2.2610038286074996e-09
450450,900901,450450,1351351,1639.57488322258,2.6684574550017715e-09
451451,902903,451451,1354354,1643.5655171871185,4.270987119525671e-09
452452,904905,452452,1357357,1647.3497982025146,6.883055903017521e-09
453453,906907,453453,1360360,1650.9587502479553,9.760697139427066e-09
454454,908909,454454,1363363,1655.4612562656403,1.2174496077932417e-08
455455,910911,455455,1366366,1659.6716012954712,1.3727913028560579e-08
456456,912913,456456,1369369,1664.0435950756073,1.3818862498737872e-08
457457,914915,457457,1372372,1668.694999217987,1.263833837583661e-08
458458,916917,458458,1375375,1673.0838272571564,1.0362782632000744e-08
459459,918919,459459,1378378,1676.959604024887,7.490598363801837e-09
460460,920921,460460,1381381,1680.7406902313232,4.833054845221341e-09
461461,922923,461461,1384384,1685.8441591262817,2.7921487344428897e-09
462462,924925,462462,1387387,1690.822219133377,2.013621269725263e-09
463463,926927,463463,1390390,1695.8724312782288,2.5429471861571074e-09
464464,928929,464464,1393393,1700.5608041286469,4.220055416226387e-09
465465,930931,465465,1396396,1705.2654333114624,6.750269676558673e-09
466466,932933,466466,1399399,1709.8331441879272,9.325958671979606e-09
467467,934935,467467,1402402,1713.1751990318298,1.153239281848073e-08
468468,936937,468468,1405405,1717.0151071548462,1.2714735930785537e-08
469469,938939,469469,1408408,1721.026349067688,1.261651050299406e-08
470470,940941,470470,1411411,1725.3068282604218,1.1359588825143874e-08
471471,942943,471471,1414414,1729.1611211299896,9.067662176676095e-09
472472,944945,472472,1417417,1733.548433303833,6.468326319009066e-09
473473,946947,473473,1420420,1737.9936780929565,4.02542355004698e-09
474474,948949,474474,1423423,1742.3084502220154,2.3228494683280587e-09
475475,950951,475475,1426426,1746.3931493759155,1.82626536116004e-09
476476,952953,476476,1429429,1750.2061502933502,2.4629116524010897e-09
477477,954955,477477,1432432,1753.748300075531,4.238245310261846e-09
478478,956957,478478,1435435,1757.2830522060394,6.579284672625363e-09
479479,958959,479479,1438438,1761.1673271656036,8.96397978067398e-09
480480,960961,480480,1441441,1764.7549221515656,1.0888470569625497e-08
481481,962963,481481,1444444,1768.8421580791473,1.175612851511687e-08
482482,964965,482482,1447447,1772.261283159256,1.1537849786691368e-08
483483,966967,483483,1450450,1775.7402131557465,1.0149960871785879e-08
484484,968969,484484,1453453,1779.0564811229706,7.978087523952127e-09
485485,970971,485485,1456456,1782.360374212265,5.571564543060958e-09
486486,972973,486486,1459459,1785.9987852573395,3.356035449542105e-09
487487,974975,487487,1462462,1789.6570081710815,2.002707333303988e-09
488488,976977,488488,1465465,1793.5226323604584,1.6625563148409128e-09
489489,978979,489489,1468468,1797.7382462024689,2.4629116524010897e-09
490490,980981,490490,1471471,1801.29843211174,4.225512384437025e-09
491491,982983,491491,1474474,1805.0262310504913,6.397385732270777e-09
492492,984985,492492,1477477,1808.897881269455,8.614733815193176e-09
493493,986987,493493,1480480,1812.3549933433533,1.0209987522102892e-08
494494,988989,494494,1483483,1815.814614057541,1.0886651580221951e-08
495495,990991,495495,1486486,1819.3383402824402,1.0499206837266684e-08
496496,992993,496496,1489489,1822.7878391742706,9.045834303833544e-09
497497,994995,497497,1492492,1826.2569663524628,7.0158421294763684e-09
498498,996997,498498,1495495,1830.240157365799,4.742105375044048e-09
499499,998999,499499,1498498,1833.91251206398,2.8339854907244444e-09
500501,1001003,500501,1501504,1837.9024012088776,1.7207639757543802e-09
501502,1003005,501502,1504507,1841.8051960468292,1.5679688658565283e-09
502503,1005007,502503,1507510,1845.569467306137,2.5174813345074654e-09
503504,1007009,503504,1510513,1849.1389961242676,4.192770575173199e-09
504505,1009011,504505,1513516,1852.639876127243,6.275513442233205e-09
505506,1011013,505506,1516519,1856.169622182846,8.249116945080459e-09
506507,1013015,506507,1519522,1859.671166419983,9.582436177879572e-09
507508,1015017,507508,1522525,1863.7899851799011,1.0082658263854682e-08
508509,1017019,508509,1525528,1867.0675110816956,9.507857612334192e-09
509510,1019021,509510,1528531,1870.3279030323029,8.087226888164878e-09
510511,1021023,510511,1531534,1874.0298812389374,6.129994289949536e-09
511512,1023025,511512,1534537,1877.7560122013092,4.043613444082439e-09
512513,1025027,512513,1537540,1881.2735192775726,2.4137989385053515e-09
513514,1027029,513514,1540543,1884.794504404068,1.482476363889873e-09
514515,1029031,514515,1543546,1888.7608833312988,1.5497789718210697e-09
515516,1031033,515516,1546549,1892.068627357483,2.546585164964199e-09
516517,1033035,516517,1549552,1895.9819951057434,4.174580681137741e-09
517518,1035037,517518,1552555,1899.5497300624847,6.146365194581449e-09
518519,1037039,518519,1555558,1903.2177772521973,7.8580342233181e-09
519520,1039041,519520,1558561,1906.6960361003876,9.009454515762627e-09
520521,1041043,520521,1561564,1910.2201390266418,9.289578883908689e-09
521522,1043045,521522,1564567,1913.8591930866241,8.602000889368355e-09
522523,1045047,522523,1567570,1917.815264225006,7.206836016848683e-09
523524,1047049,523524,1570573,1921.0469992160797,5.313268047757447e-09
524525,1049051,524525,1573576,1924.7149341106415,3.459717845544219e-09
525526,1051053,525526,1576579,1928.5968520641327,2.02817318495363e-09
526527,1053055,526527,1579582,1931.8853392601013,1.318767317570746e-09
527528,1055057,527528,1582585,1935.3473641872406,1.5643308870494366e-09
528529,1057059,528529,1585588,1938.9294731616974,2.5756889954209328e-09
529530,1059061,529530,1588591,1942.8052201271057,4.200046532787383e-09
530531,1061063,530531,1591594,1946.5932371616364,5.9881131164729595e-09
531532,1063065,531532,1594597,1950.4266769886017,7.508788257837296e-09
532533,1065067,532533,1597600,1954.6548643112183,8.465576684102416e-09
533534,1067069,533534,1600603,1958.6647872924805,8.534698281437159e-09
534535,1069071,534535,1603606,1962.755511045456,7.803464541211724e-09
535536,1071073,535536,1606609,1967.303278207779,6.384652806445956e-09
536537,1073075,536537,1609612,1970.9511172771454,4.611138137988746e-09
537538,1075077,537538,1612615,1975.0986533164978,2.9576767701655626e-09
538539,1077079,538539,1615618,1979.152723312378,1.7025740817189217e-09
539540,1079081,539540,1618621,1983.1255731582642,1.2278178473934531e-09
540541,1081083,540541,1621624,1986.8060421943665,1.5661498764529824e-09
541542,1083085,541542,1624627,1990.4876492023468,2.6266206987202168e-09
542543,1085087,542543,1627630,1994.7731420993805,4.200046532787383e-09
543544,1087089,543544,1630633,1998.1107211112976,5.817128112539649e-09
544545,1089091,544545,1633636,2001.3938512802124,7.185008144006133e-09
545546,1091093,545546,1636639,2004.5964679718018,7.914422894828022e-09
546547,1093095,546547,1639642,2008.3726241588593,7.84893927630037e-09
547548,1095097,547548,1642645,2012.22403216362,7.05040292814374e-09
548549,1097099,548549,1645648,2016.2050611972809,5.626134225167334e-09
549550,1099101,549550,1648651,2019.7617211341858,4.00359567720443e-09
550551,1101103,550551,1651654,2023.2295081615448,2.4883775040507317e-09
551552,1103105,551552,1654657,2026.6996462345123,1.4497345546260476e-09
552553,1105107,552553,1657660,2030.1920402050018,1.1550582712516189e-09
553554,1107109,553554,1660663,2033.649587392807,1.5788828022778034e-09
554555,1109111,554555,1663666,2037.1850962638855,2.7030182536691427e-09
555556,1111113,555556,1666669,2041.1870641708374,4.174580681137741e-09
556557,1113115,556557,1669672,2044.8916773796082,5.6716089602559805e-09
557558,1115117,557558,1672675,2049.009145259857,6.859409040771425e-09
558559,1117119,558559,1675678,2052.5379803180695,7.390553946606815e-09
559560,1119121,559560,1678681,2056.1092932224274,7.228663889691234e-09
560561,1121123,560561,1681684,2059.6444861888885,6.3428160501644015e-09
561562,1123125,561562,1684687,2063.1020271778107,4.973117029294372e-09
562563,1125127,562563,1687690,2066.5742332935333,3.457898856140673e-09
563564,1127129,563564,1690693,2070.0343692302704,2.0863808458670974e-09
564565,1129131,564565,1693696,2074.033324241638,1.2605596566572785e-09
565566,1131133,565566,1696699,2077.3018333911896,1.0841176845133305e-09
566567,1133135,566567,1699702,2080.592852115631,1.622538547962904e-09
567568,1135137,567568,1702705,2084.3288362026215,2.7539499569684267e-09
568569,1137139,568569,1705708,2088.0034470558167,4.140019882470369e-09
569570,1139141,569570,1708711,2091.5371532440186,5.529727786779404e-09
570571,1141143,570571,1711714,2095.4029953479767,6.517439032904804e-09
571572,1143145,571572,1714717,2099.8325192928314,6.912159733474255e-09
572573,1145147,572573,1717720,2103.913843393326,6.630216375924647e-09
573574,1147149,573574,1720723,2107.841821193695,5.689798854291439e-09
574575,1149151,574575,1723726,2112.1729390621185,4.38558345194906e-09
575576,1151153,575576,1726729,2115.47185921669,2.950400812551379e-09
576577,1153155,576577,1729732,2119.0502462387085,1.762600732035935e-09
577578,1155157,577578,1732735,2122.780804157257,1.0913936421275139e-09
578579,1157159,578579,1735738,2126.2674412727356,1.0422809282317758e-09
579580,1159161,579580,1738741,2130.1511821746826,1.684384187683463e-09
580581,1161163,580581,1741744,2133.4775512218475,2.7812347980216146e-09
581582,1163165,581582,1744747,2136.810883283615,4.118192009627819e-09
582583,1165167,582583,1747750,2140.090053319931,5.366018740460277e-09
583584,1167169,583584,1750753,2143.390540122986,6.193658919073641e-09
584585,1169171,584585,1753756,2146.678922176361,6.4701453084126115e-09
585586,1171173,585586,1756759,2150.396532058716,6.06269168201834e-09
586587,1173175,586587,1759762,2154.40625,5.120455170981586e-09
587588,1175177,587588,1762765,2158.3732900619507,3.848981577903032e-09
588589,1177179,588589,1765768,2161.887267112732,2.5193003239110112e-09
589590,1179181,589590,1768771,2165.4509811401367,1.4970282791182399e-09
590591,1181183,590591,1771774,2168.9442150592804,9.440555004402995e-10
591592,1183185,591592,1774777,2172.416310071945,1.038642949424684e-09
592593,1185187,592593,1777780,2176.462948322296,1.722582965157926e-09
593594,1187189,593594,1780783,2179.8404512405396,2.8103386284783483e-09
594595,1189191,594595,1783786,2183.238263130188,4.083631210960448e-09
595596,1191193,595596,1786789,2186.5199213027954,5.180481821298599e-09
596597,1193195,596597,1789792,2189.782261133194,5.891706678085029e-09
597598,1195197,597598,1792795,2193.047008037567,6.0263118939474225e-09
598599,1197199,598599,1795798,2196.344351053238,5.542460712604225e-09
599600,1199201,599600,1798801,2199.6192440986633,4.596586222760379e-09
600601,1201203,600601,1801804,2202.9141511917114,3.3542164601385593e-09
601602,1203205,601602,1804807,2206.176778078079,2.1591404220089316e-09
602603,1205207,602603,1807810,2209.5101273059845,1.255102688446641e-09
603604,1207209,603604,1810813,2212.783844232559,8.440110832452774e-10
604605,1209211,604605,1813816,2216.1447591781616,1.0495568858459592e-09
605606,1211213,605606,1816819,2219.5993463993073,1.7571437638252974e-09
606607,1213215,606607,1819822,2224.034769296646,2.8485374059528112e-09
607608,1215217,607608,1822825,2228.3071942329407,4.0236045606434345e-09
608609,1217219,608609,1825828,2232.6150941848755,5.007677827961743e-09
609610,1219221,609610,1828831,2236.6122632026672,5.593392415903509e-09
610611,1221223,610611,1831834,2240.274564266205,5.5970303947106e-09
611612,1223225,611612,1834837,2243.7558352947235,5.071342457085848e-09
612613,1225227,612613,1837840,2247.7989661693573,4.105459083802998e-09
613614,1227229,613614,1840843,2251.4872193336487,2.928572939708829e-09
614615,1229231,614615,1843846,2255.315894126892,1.8408172763884068e-09
615616,1231233,615616,1846849,2259.0968194007874,1.0495568858459592e-09
616617,1233235,616617,1849852,2263.432407140732,7.821654435247183e-10
617618,1235237,617618,1852855,2267.262869119644,1.053194864653051e-09
618619,1237239,618619,1855858,2270.874014377594,1.8026184989139438e-09
619620,1239241,619620,1858861,2275.1698141098022,2.86672729998827e-09
620621,1241243,620621,1861864,2279.178287267685,3.9472070056945086e-09
621622,1243245,621622,1864867,2283.3358912467957,4.836692824028432e-09
622623,1245247,622623,1867870,2286.8618171215057,5.284164217300713e-09
623624,1247249,623624,1870873,2290.30233502388,5.2023096941411495e-09
624625,1249251,624625,1873876,2293.6476941108704,4.625690053217113e-09
625626,1251253,625626,1876879,2297.2872200012207,3.648892743512988e-09
626627,1253255,626627,1879882,2300.937591075897,2.5556801119819283e-09
627628,1255257,627628,1882885,2304.224819421768,1.5552359400317073e-09
628629,1257259,628629,1885888,2307.531107187271,8.949427865445614e-10
629630,1259261,629630,1888891,2310.791617155075,7.34871719032526e-10
630631,1261263,630631,1891894,2314.1805140972137,1.0677467798814178e-09
631632,1263265,631632,1894897,2317.4895050525665,1.8553691916167736e-09
632633,1265267,632633,1897900,2320.736481189728,2.86672729998827e-09
633634,1267269,633634,1900903,2324.0958280563354,3.87626641895622e-09
634635,1269271,634635,1903906,2327.4058492183685,4.654793883673847e-09
635636,1271273,635636,1906909,2330.5996313095093,4.984030965715647e-09
636637,1273275,636637,1909912,2333.8403000831604,4.833054845221341e-09
637638,1275277,637638,1912915,2337.061793088913,4.198227543383837e-09
638639,1277279,638639,1915918,2340.330974340439,3.2541720429435372e-09
639640,1279281,639640,1918921,2343.5193321704865,2.2209860617294908e-09
640641,1281283,640641,1921924,2346.711131334305,1.3114913599565625e-09
641642,1283285,641642,1924927,2349.868310213089,7.767084753140807e-10
642643,1285287,642643,1927930,2353.1361973285675,6.930349627509713e-10
643644,1287289,643644,1930933,2356.266009092331,1.102307578548789e-09
644645,1289291,644645,1933936,2359.5486583709717,1.8953869584947824e-09
645646,1291293,645646,1936939,2362.850431203842,2.8594513423740864e-09
646647,1293295,646647,1939942,2366.066677093506,3.799868864007294e-09
647648,1295297,647648,1942945,2369.2692873477936,4.456524038687348e-09
648649,1297299,648649,1945948,2372.5291261672974,4.698449629358947e-09
649650,1299301,649650,1948951,2375.802319288254,4.472894943319261e-09
650651,1301303,650651,1951954,2378.918338060379,3.803506842814386e-09
651652,1303305,651652,1954957,2382.072918176651,2.892193151637912e-09
652653,1305307,652653,1957960,2385.2435472011566,1.911757863126695e-09
653654,1307309,653654,1960963,2388.5028071403503,1.1132215149700642e-09
654655,1309311,654655,1963966,2391.659942150116,6.766640581190586e-10
655656,1311313,655656,1966969,2394.791353225708,6.784830475226045e-10
656657,1313315,656657,1969972,2397.978793144226,1.1477823136374354e-09
657658,1315317,657658,1972975,2401.1379630565643,1.924490788951516e-09
658659,1317319,658659,1975978,2404.2990663051605,2.8558133635669947e-09
659660,1319321,659660,1978981,2407.5262594223022,3.7052814150229096e-09
660661,1321323,660661,1981984,2412.460277080536,4.261892172507942e-09
661662,1323325,661662,1984987,2416.9079802036285,4.425601218827069e-09
662663,1325327,662663,1987990,2420.7513811588287,4.120010999031365e-09
663664,1327329,663664,1990993,2424.426408290863,3.448803909122944e-09
664665,1329331,664665,1993996,2427.997693300247,2.557499101385474e-09
665666,1331333,665666,1996999,2432.06596827507,1.648004399612546e-09
666667,1333335,666667,2000002,2435.9330933094025,9.51331458054483e-10
667668,1335337,667668,2003005,2440.02756524086,5.948095349594951e-10
668669,1337339,668669,2006008,2444.512073278427,6.857590051367879e-10
669670,1339341,669670,2009011,2448.5094830989838,1.1823431123048067e-09
670671,1341343,670671,2012014,2452.0840542316437,1.9554136088117957e-09
671672,1343345,671672,2015017,2455.267348051071,2.8430804377421737e-09
672673,1345347,672673,2018020,2458.559526205063,3.59978002961725e-09
673674,1347349,673674,2021023,2461.7706441879272,4.076355253346264e-09
674675,1349351,674675,2024026,2464.972827196121,4.145476850681007e-09
675676,1351353,675676,2027029,2468.173994064331,3.790773916989565e-09
676677,1353355,676677,2030032,2471.3498752117157,3.115928848274052e-09
677678,1355357,677678,2033035,2474.5874240398407,2.2464519133791327e-09
678679,1357359,678679,2036038,2477.8902671337128,1.418811734765768e-09
679680,1359361,679680,2039041,2481.1050040721893,8.039933163672686e-10
680681,1361363,680681,2042044,2484.3446152210236,5.402398528531194e-10
681682,1363365,681682,2045047,2487.520992040634,7.021299097687006e-10
682683,1365367,682683,2048050,2490.694133043289,1.2205418897792697e-09
683684,1367369,683684,2051053,2493.866065263748,1.991793396882713e-09
684685,1369371,684685,2054056,2497.221679210663,2.812157617881894e-09
685686,1371373,685686,2057059,2502.7470202445984,3.496097633615136e-09
686687,1373375,686687,2060062,2508.615662097931,3.887180355377495e-09
687688,1375377,687688,2063065,2513.567031145096,3.874447429552674e-09
688689,1377379,688689,2066068,2518.446862220764,3.4888216760009527e-09
689690,1379381,689690,2069071,2523.111448287964,2.799424692057073e-09
690691,1381383,690691,2072074,2527.5141501426697,1.9754224922508e-09
691692,1383385,691692,2075077,2532.5236213207245,1.2187229003757238e-09
692693,1385387,692693,2078080,2537.231582403183,6.821210263296962e-10
693694,1387389,693694,2081083,2541.927297115326,5.111360223963857e-10
694695,1389391,694695,2084086,2546.4231700897217,7.22138793207705e-10
695696,1391393,695696,2087089,2550.692679166794,1.2623786460608244e-09
696697,1393395,696697,2090092,2555.359990119934,2.015440259128809e-09
697698,1395397,697698,2093095,2559.4040372371674,2.773958840407431e-09
698699,1397399,698699,2096098,2563.2002432346344,3.3869582694023848e-09
699700,1399401,699700,2099101,2567.1812691688538,3.6907294997945428e-09
700701,1401403,700701,2102104,2571.1982831954956,3.6179699236527085e-09
701702,1403405,701702,2105107,2575.078835248947,3.19596438203007e-09
702703,1405407,702703,2108110,2579.232953310013,2.5047484086826444e-09
703704,1407409,703704,2111113,2582.875641107559,1.7316779121756554e-09
704705,1409411,704705,2114116,2586.6285331249237,1.0368239600211382e-09
705706,1411413,705706,2117119,2590.3936882019043,5.875335773453116e-10
706707,1413415,706707,2120122,2593.729389190674,4.893081495538354e-10
707708,1415417,707708,2123125,2597.382571220398,7.457856554538012e-10
708709,1417419,708709,2126128,2601.268566131592,1.3114913599565625e-09
709710,1419421,709710,2129131,2604.604564189911,2.02817318495363e-09
710711,1421423,710711,2132134,2608.1259472370148,2.7412170311436057e-09
711712,1423425,711712,2135137,2611.4229102134705,3.2778189051896334e-09
712713,1425427,712713,2138140,2615.128274202347,3.496097633615136e-09
713714,1427429,713714,2141143,2619.268974304199,3.3742253435775638e-09
714715,1429431,714715,2144146,2623.339537382126,2.915840013884008e-09
715716,1431433,715716,2147149,2626.762392282486,2.2391759557649493e-09
716717,1433435,716717,2150152,2630.4689421653748,1.5115801943466067e-09
717718,1435437,717718,2153155,2634.4279811382294,8.785718819126487e-10
718719,1437439,718719,2156158,2638.256607055664,5.147740012034774e-10
719720,1439441,719720,2159161,2642.331586122513,4.747562343254685e-10
720721,1441443,720721,2162164,2646.23282623291,7.803464541211724e-10
721722,1443445,721722,2165167,2650.396065235138,1.3515091268345714e-09
722723,1445447,722723,2168170,2654.251409292221,2.039087121374905e-09
723724,1447449,723724,2171173,2657.8031141757965,2.697561285458505e-09
724725,1449451,724725,2174176,2661.7179741859436,3.1523086363449693e-09
725726,1451453,725726,2177179,2665.337967157364,3.3105607144534588e-09
726727,1453455,726727,2180182,2668.849778175354,3.1341187423095107e-09
727728,1455457,727728,2183185,2672.3663680553436,2.6520865503698587e-09
728729,1457459,728729,2186188,2675.88538813591,1.9972503650933504e-09
729730,1459461,729730,2189191,2679.417528152466,1.304215402342379e-09
730731,1461463,730731,2192194,2683.6929881572723,7.494236342608929e-10
731732,1463465,731732,2195197,2687.3584911823273,4.5292836148291826e-10
732733,1465467,732733,2198200,2691.463066339493,4.747562343254685e-10
733734,1467469,733734,2201203,2695.4947032928467,8.221832104027271e-10
734735,1469471,734735,2204206,2699.3586270809174,1.3842509360983968e-09
735736,1471473,735736,2207209,2703.3454842567444,2.0500010577961802e-09
736737,1473475,736737,2210212,2706.7353100776672,2.646629582159221e-09
737738,1475477,737738,2213215,2710.0335800647736,3.0322553357109427e-09
738739,1477479,738739,2216218,2713.3239171504974,3.130480763502419e-09
739740,1479481,739740,2219221,2716.5936381816864,2.8994691092520952e-09
740741,1481483,740741,2222224,2719.9031682014465,2.4119799491018057e-09
741742,1483485,741742,2225227,2723.204814195633,1.7716956790536642e-09
742743,1485487,742743,2228230,2726.4522371292114,1.1259544407948852e-09
743744,1487489,743744,2231233,2729.69784116745,6.402842700481415e-10
744745,1489491,744745,2234236,2732.922909259796,4.0381564758718014e-10
745746,1491493,745746,2237239,2736.476382255554,4.874891601502895e-10
746747,1493495,746747,2240242,2740.046219110489,8.549250196665525e-10
747748,1495497,747748,2243245,2745.448000192642,1.418811734765768e-09
748749,1497499,748749,2246248,2751.395127058029,2.051820047199726e-09
749750,1499501,749750,2249251,2755.9028232097626,2.586602931842208e-09
750751,1501503,750751,2252254,2759.8565921783447,2.9122020350769162e-09
751752,1503505,751752,2255257,2763.9447071552277,2.9467628337442875e-09
752753,1505507,752753,2258260,2768.188818216324,2.6793713914230466e-09
753754,1507509,753754,2261263,2771.972650051117,2.1827872842550278e-09
754755,1509511,754755,2264266,2775.160377264023,1.558873918838799e-09
755756,1511513,755756,2267269,2778.3834130764008,9.713403414934874e-10
756757,1513515,756757,2270272,2781.599817276001,5.420588422566652e-10
757758,1515517,757758,2273275,2784.920111179352,3.710738383233547e-10
758759,1517519,758759,2276278,2788.1362001895905,5.056790541857481e-10
759760,1519521,759760,2279281,2791.5473721027374,8.931237971410155e-10
760761,1521523,760761,2282284,2794.73854637146,1.4533725334331393e-09
761762,1523525,761762,2285287,2798.033088207245,2.042725100181997e-09
762763,1525527,762763,2288290,2801.425119161606,2.5247572921216488e-09
763764,1527529,763764,2291293,2804.6460983753204,2.790329745039344e-09
764765,1529531,764765,2294296,2807.94069814682,2.7666828827932477e-09
765766,1531533,765766,2297299,2811.5006172657013,2.472006599418819e-09
766767,1533535,766767,2300302,2815.070963382721,1.9681465346366167e-09
767768,1535537,767768,2303305,2818.294783115387,1.3733369996771216e-09
768769,1537539,768769,2306308,2821.4617381095886,8.330971468240023e-10
769770,1539541,769770,2309311,2824.713522195816,4.5838532969355583e-10
770771,1541543,770771,2312314,2827.9184432029724,3.5288394428789616e-10
771772,1543545,771772,2315317,2831.0510931015015,5.220499588176608e-10
772773,1545547,772773,2318320,2834.734838247299,9.276845958083868e-10
773774,1547549,773774,2321323,2837.9560811519623,1.4806573744863272e-09
774775,1549551,774775,2324326,2841.1554062366486,2.026354195550084e-09
775776,1551553,775776,2327329,2844.3567481040955,2.461092662997544e-09
776777,1553555,776777,2330332,2847.888763189316,2.663000486791134e-09
777778,1555557,777778,2333335,2852.8667330741882,2.5938788894563913e-09
778779,1557559,778779,2336338,2857.3033742904663,2.2737367544323206e-09
779780,1559561,779780,2339341,2861.037922143936,1.7644197214394808e-09
780781,1561563,780781,2342344,2864.464655160904,1.204170985147357e-09
781782,1563565,781782,2345347,2867.912141084671,7.057678885757923e-10
782783,1565567,782783,2348350,2871.336527109146,3.9472070056945086e-10
783784,1567569,783784,2351353,2874.7458782196045,3.41970007866621e-10
784785,1569571,784785,2354356,2878.203850030899,5.438778316602111e-10
785786,1571573,785786,2357359,2882.1107251644135,9.695213520899415e-10
786787,1573575,786787,2360362,2885.5899741649628,1.4970282791182399e-09
787788,1575577,787788,2363365,2889.013243198395,2.0118022803217173e-09
788789,1577579,788789,2366368,2892.306687116623,2.3919710656628013e-09
789790,1579581,789790,2369371,2896.7727570533752,2.535671228542924e-09
790791,1581583,790791,2372374,2901.8932774066925,2.4301698431372643e-09
791792,1583585,791792,2375377,2907.0032012462616,2.0827428670600057e-09
792793,1585587,792793,2378380,2912.1032230854034,1.584339770488441e-09
793794,1587589,793794,2381383,3043.178678035736,1.0495568858459592e-09
794795,1589591,794795,2384386,3048.5091631412506,5.984475137665868e-10
795796,1591593,795796,2387389,3060.5326499938965,3.4560798667371273e-10
796797,1593595,796797,2390392,3077.6459782123566,3.346940502524376e-10
797798,1595597,797798,2393395,3094.0000302791595,5.766196409240365e-10
798799,1597599,798799,2396398,3316.1863560676575,1.002263161353767e-09
799800,1599601,799800,2399401,3321.483691215515,1.5097612049430609e-09
800801,1601603,800801,2402404,3337.2648293972015,1.988155418075621e-09
801802,1603605,801802,2405407,3581.2890853881836,2.3119355319067836e-09
802803,1605607,802803,2408410,3586.9609100818634,2.4119799491018057e-09
803804,1607609,803804,2411413,3601.7909801006317,2.2646418074145913e-09
804805,1609611,804805,2414416,3972.7191112041473,1.90084392670542e-09
805806,1611613,805806,2417419,3978.3842282295227,1.4151737559586763e-09
806807,1613615,806807,2420422,3993.465014219284,9.094947017729282e-10
807808,1615617,807808,2423425,4004.3358783721924,5.093170329928398e-10
808809,1617619,808809,2426428,4009.426323413849,3.0740920919924974e-10
809810,1619621,809810,2429431,4520.010407209396,3.383320290595293e-10
810811,1621623,810811,2432434,4551.249640226364,6.075424607843161e-10
811812,1623625,811812,2435437,4556.752989292145,1.0331859812140465e-09
812813,1625627,812813,2438440,4564.881210327148,1.5243131201714277e-09
813814,1627629,813814,2441443,4906.97042632103,1.9572325982153416e-09
814815,1629631,814815,2444446,4919.416699171066,2.2337189875543118e-09
815816,1631633,815816,2447449,4924.866777181625,2.2901076590642333e-09
816817,1633635,816817,2450452,4931.835343122482,2.104570739902556e-09
817818,1635637,817818,2453455,4950.770079135895,1.7316779121756554e-09
818819,1637639,818819,2456458,4983.057963132858,1.2569216778501868e-09
819820,1639641,819820,2459461,4988.196266174316,7.839844329282641e-10
820821,1641643,820821,2462464,4999.778615236282,4.347384674474597e-10
821822,1643645,821822,2465467,5016.007645368576,2.7466739993542433e-10
822823,1645647,822823,2468470,6735.698296070099,3.510649548843503e-10
823824,1647649,823824,2471473,6742.3715903759,6.348273018375039e-10
824825,1649651,824825,2474476,6747.2542362213135,1.0604708222672343e-09
825826,1651653,825826,2477479,6751.537607192993,1.5297700883820653e-09
826827,1653655,826827,2480482,6755.901738166809,1.9208528101444244e-09
827828,1655657,827828,2483485,6759.965269088745,2.153683453798294e-09
828829,1657659,828829,2486488,6764.275462150574,2.164597390219569e-09
829830,1659661,829830,2489491,6768.620796203613,1.951775630004704e-09
830831,1661663,830831,2492494,6772.492253303528,1.5752448234707117e-09
831832,1663665,831832,2495497,6776.140933275223,1.1077645467594266e-09
832833,1665667,832833,2498500,6779.407901287079,6.766640581190586e-10
833834,1667669,833834,2501503,6782.907155990601,3.6561687011271715e-10
834835,1669671,834835,2504506,6786.668029308319,2.5283952709287405e-10
835836,1671673,835836,2507509,6790.101169347763,3.6561687011271715e-10
836837,1673675,836837,2510512,6793.7152371406555,6.675691111013293e-10
837838,1675677,837838,2513515,6797.51366519928,1.089574652723968e-09
838839,1677679,838839,2516518,6801.667042255402,1.5279510989785194e-09
839840,1679681,839840,2519521,6805.492425441742,1.8826540326699615e-09
840841,1681683,840841,2522524,6809.691873073578,2.0700099412351847e-09
841842,1683685,841842,2525527,6813.410325050354,2.039087121374905e-09
842843,1685687,842843,2528530,6816.913640975952,1.8062564777210355e-09
843844,1687689,843844,2531533,6820.383045196533,1.4224497135728598e-09
844845,1689691,844845,2534536,6823.862487077713,9.786162991076708e-10
845846,1691693,845846,2537539,6828.046031236649,5.802576197311282e-10
846847,1693695,846847,2540542,6832.7320392131805,3.128661774098873e-10
847848,1695697,847848,2543545,6837.4867742061615,2.4374458007514477e-10
848849,1697699,848849,2546548,6841.78751206398,3.838067641481757e-10
849850,1699701,849850,2549551,6846.938661336899,6.984919309616089e-10
850851,1701703,850851,2552554,6851.415395259857,1.1114025255665183e-09
851852,1703705,851852,2555557,6855.737832307816,1.520675141364336e-09
852853,1705707,852853,2558560,6859.781392335892,1.838998286984861e-09
853854,1707709,853854,2561563,6863.166802406311,1.9826984498649836e-09
854855,1709711,854855,2564566,6866.815851211548,1.9172148313373327e-09
855856,1711713,855856,2567569,6870.090624094009,1.6661942936480045e-09
856857,1713715,856857,2570572,6873.423003196716,1.278749550692737e-09
857858,1715717,857858,2573575,6876.76368522644,8.585629984736443e-10
858859,1717719,858859,2576578,6880.035274028778,4.911271389573812e-10
859860,1719721,859860,2579581,6883.949195146561,2.6921043172478676e-10
860861,1721723,860861,2582584,6888.359049320221,2.382876118645072e-10
861862,1723725,861862,2585587,6892.1287753582,4.0381564758718014e-10
862863,1725727,862863,2588590,6897.872997283936,7.294147508218884e-10
863864,1727729,863864,2591593,6902.682107210159,1.1314114090055227e-09
864865,1729731,864865,2594596,6907.34006023407,1.5152181731536984e-09
865866,1731733,865866,2597599,6910.851347208023,1.7917045624926686e-09
866867,1733735,866867,2600602,6914.40172123909,1.8917489796876907e-09
867868,1735737,867868,2603605,6917.918593168259,1.800799509510398e-09
868869,1737739,868869,2606608,6921.51734828949,1.5297700883820653e-09
869870,1739741,869870,2609611,6924.992821216583,1.1496013030409813e-09
870871,1741743,870871,2612614,6929.397313117981,7.494236342608929e-10
871872,1743745,871872,2615617,6933.215014219284,4.1654857341200113e-10
872873,1745747,872873,2618620,6937.069431066513,2.346496330574155e-10
873874,1747749,873874,2621623,6940.337334156036,2.382876118645072e-10
874875,1749751,874875,2624626,6943.652614355087,4.2928149923682213e-10
875876,1751753,875876,2627629,6947.167523145676,7.585185812786222e-10
876877,1753755,876877,2630632,6950.668491125107,1.1441443348303437e-09
877878,1755757,877878,2633635,6954.827015399933,1.5024852473288774e-09
878879,1757759,878879,2636638,6959.060093402863,1.737134880386293e-09
879880,1759761,879880,2639641,6962.633086204529,1.8044374883174896e-09
880881,1761763,880881,2642644,6966.303299188614,1.6807462088763714e-09
881882,1763765,881882,2645647,6970.0769102573395,1.3988028513267636e-09
882883,1765767,882883,2648650,6974.428118228912,1.027729013003409e-09
883884,1767769,883884,2651653,6979.0549330711365,6.475602276623249e-10
884885,1769771,884885,2654656,6984.340147256851,3.5288394428789616e-10
885886,1771773,885886,2657659,6989.2647223472595,2.091837814077735e-10
886887,1773775,886887,2660662,6992.76113319397,2.4374458007514477e-10
887888,1775777,887888,2663665,6996.285879135132,4.5656634029001e-10
888889,1777779,888889,2666668,6999.562583208084,7.839844329282641e-10
889890,1779781,889890,2669671,7002.86917924881,1.1568772606551647e-09
890891,1781783,890891,2672674,7006.640300035477,1.4842953532934189e-09
891892,1783785,891892,2675677,7010.080147981644,1.6825651982799172e-09
892893,1785787,892893,2678680,7015.166558265686,1.7153070075437427e-09
893894,1787789,893894,2681683,7020.91349196434,1.5661498764529824e-09
894895,1789791,894895,2684686,7025.922127246857,1.278749550692737e-09
895896,1791793,895896,2687689,7029.24610209465,9.149516699835658e-10
896897,1793795,896897,2690692,7032.483439207077,5.584297468885779e-10
897898,1795797,897898,2693695,7035.705412149429,3.001332515850663e-10
898899,1797799,898899,2696698,7038.958849191666,1.8917489796876907e-10
899900,1799801,899900,2699701,7042.189169168472,2.5647750589996576e-10
900901,1801803,900901,2702704,7045.476186275482,4.82032191939652e-10
901902,1803805,901902,2705707,7048.815662145615,8.094502845779061e-10
902903,1805807,902903,2708710,7052.049074172974,1.165972207672894e-09
903904,1807809,903904,2711713,7055.320916175842,1.4588295016437769e-09
904905,1809811,904905,2714716,7058.541572093964,1.6261765267699957e-09
905906,1811813,905906,2717719,7061.842265129089,1.6243575373664498e-09
906907,1813815,906907,2720722,7065.036437034607,1.4551915228366852e-09
907908,1815817,907908,2723725,7068.209545373917,1.1623342288658023e-09
908909,1817819,908909,2726728,7071.375659227371,8.076312951743603e-10
909910,1819821,909910,2729731,7074.59802031517,4.802132025361061e-10
910911,1821823,910911,2732734,7077.761850118637,2.5283952709287405e-10
911912,1823825,911912,2735737,7080.9590582847595,1.7826096154749393e-10
912913,1825827,912913,2738740,7084.162415266037,2.710294211283326e-10
913914,1827829,913914,2741743,7087.311136007309,5.07498043589294e-10
914915,1829831,914915,2744746,7090.52698135376,8.349161362275481e-10
915916,1831833,915916,2747749,7093.699334144592,1.1696101864799857e-09
916917,1833835,916917,2750752,7096.888296365738,1.433363649994135e-09
917918,1835837,917918,2753755,7100.0612070560455,1.5661498764529824e-09
918919,1837839,918919,2756758,7103.253433227539,1.5352270565927029e-09
919920,1839841,919920,2759761,7106.496868133545,1.3515091268345714e-09
920921,1841843,920921,2762764,7109.658318281174,1.051375875249505e-09
921922,1843845,921922,2765767,7112.785790205002,7.112248567864299e-10
922923,1845847,922923,2768770,7116.008377313614,4.1109160520136356e-10
923924,1847849,923924,2771773,7119.135715246201,2.1464074961841106e-10
924925,1849851,924925,2774776,7122.292296409607,1.7280399333685637e-10
925926,1851853,925926,2777779,7125.463452339172,2.874003257602453e-10
926927,1853855,926927,2780782,7128.630537986755,5.347828846424818e-10
927928,1855857,927928,2783785,7131.777525186539,8.549250196665525e-10
928929,1857859,928929,2786788,7134.991672277451,1.1677911970764399e-09
929930,1859861,929930,2789791,7138.1582572460175,1.4042598195374012e-09
930931,1861863,930931,2792794,7141.381271123886,1.5043042367324233e-09
931932,1863865,931932,2795797,7144.550966024399,1.446096575818956e-09
932933,1865867,932933,2798800,7147.694025278091,1.2478267308324575e-09
933934,1867869,933934,2801803,7150.881658315659,9.476934792473912e-10
934935,1869871,934935,2804806,7154.056929111481,6.257323548197746e-10
935936,1871873,935936,2807809,7157.265622138977,3.474269760772586e-10
936937,1873875,936937,2810812,7160.406618118286,1.8553691916167736e-10
937938,1875877,937938,2813815,7163.592141151428,1.709850039333105e-10
938939,1877879,938939,2816818,7166.8051471710205,3.055902197957039e-10
939940,1879881,939940,2819821,7169.995300292969,5.620677256956697e-10
940941,1881883,940941,2822824,7173.135371208191,8.731149137020111e-10
941942,1883885,941942,2825827,7176.327881336212,1.165972207672894e-09
942943,1885887,942943,2828830,7179.4462831020355,1.36969902087003e-09
943944,1887889,943944,2831833,7182.6290991306305,1.4406396076083183e-09
944945,1889891,944945,2834836,7185.810330152512,1.3587850844487548e-09
945946,1891893,945946,2837839,7189.015078306198,1.1477823136374354e-09
946947,1893895,946947,2840842,7192.165714263916,8.49468051455915e-10
947948,1895897,947948,2843845,7195.343794345856,5.438778316602111e-10
948949,1897899,948949,2846848,7198.517322063446,2.9103830456733704e-10
949950,1899901,949950,2849851,7201.708632230759,1.6189005691558123e-10
950951,1901903,950951,2852854,7204.921075344086,1.7280399333685637e-10
951952,1903905,951952,2855857,7208.099728345871,3.2741809263825417e-10
952953,1905907,952953,2858860,7211.461229085922,5.857145879417658e-10
953954,1907909,953954,2861863,7214.749589204788,8.858478395268321e-10
954955,1909911,954955,2864866,7217.9327030181885,1.1568772606551647e-09
955956,1911913,955956,2867869,7221.068781137466,1.331500243395567e-09
956957,1913915,956957,2870872,7224.269334077835,1.3751559890806675e-09
957958,1915917,957958,2873875,7227.524897098541,1.2732925824820995e-09
958959,1917919,958959,2876878,7230.71652507782,1.0495568858459592e-09
959960,1919921,959960,2879881,7233.924180030823,7.60337570682168e-10
960961,1921923,960961,2882884,7237.128484249115,4.69299266114831e-10
961962,1923925,961962,2885887,7240.3002161979675,2.473825588822365e-10
962963,1925927,962963,2888890,7243.448436021805,1.418811734765768e-10
963964,1927929,963964,2891893,7246.632872343063,1.800799509510398e-10
964965,1929931,964965,2894896,7249.772546052933,3.510649548843503e-10
965966,1931933,965966,2897899,7252.9374232292175,6.093614501878619e-10
966967,1933935,966967,2900902,7256.135243177414,8.967617759481072e-10
967968,1935937,967968,2903905,7259.3071372509,1.1459633242338896e-09
968969,1937939,968969,2906908,7262.475455999374,1.293301465921104e-09
969970,1939941,969970,2909911,7265.636107206345,1.3096723705530167e-09
970971,1941943,970971,2912914,7268.760858297348,1.1896190699189901e-09
971972,1943945,971972,2915917,7272.094693183899,9.604264050722122e-10
972973,1945947,972973,2918920,7275.408621072769,6.748450687155128e-10
973974,1947949,973974,2921923,7278.606066226959,4.0381564758718014e-10
974975,1949951,974975,2924926,7281.759749174118,2.0736479200422764e-10
975976,1951953,975976,2927929,7285.0685613155365,1.291482476517558e-10
976977,1953955,976977,2930932,7288.266876220703,1.9099388737231493e-10
977978,1955957,977978,2933935,7291.418568372726,3.728928277269006e-10
978979,1957959,978979,2936938,7294.595208406448,6.293703336268663e-10
979980,1959961,979980,2939941,7297.788108110428,9.040377335622907e-10
980981,1961963,980981,2942944,7301.004690408707,1.1295924196019769e-09
981982,1963965,981982,2945947,7304.180283308029,1.2532836990430951e-09
982983,1965967,982983,2948950,7307.383549213409,1.2441887520253658e-09
983984,1967969,983984,2951953,7310.529706001282,1.1059455573558807e-09
984985,1969971,984985,2954956,7313.7852873802185,8.712959242984653e-10
985986,1971973,985986,2957959,7316.961370229721,5.966285243630409e-10
986987,1973975,986987,2960962,7320.201455116272,3.4560798667371273e-10
987988,1975977,987988,2963965,7323.36323428154,1.7462298274040222e-10
988989,1977979,988989,2966968,7326.555935144424,1.2369127944111824e-10
989990,1979981,989990,2969971,7329.906496047974,2.0372681319713593e-10
990991,1981983,990991,2972974,7333.1927921772,3.92901711165905e-10
991992,1983985,991992,2975977,7336.542483329773,6.511982064694166e-10
992993,1985987,992993,2978980,7339.712801218033,9.113136911764741e-10
993994,1987989,993994,2981983,7342.91934633255,1.1132215149700642e-09
994995,1989991,994995,2984986,7346.115130186081,1.2096279533579946e-09
995996,1991993,995996,2987989,7349.297986268997,1.1768861440941691e-09
996997,1993995,996997,2990992,7352.441415309906,1.027729013003409e-09
997998,1995997,997998,2993995,7355.626323223114,7.894414011389017e-10
998999,1997999,998999,2996998,7359.094793319702,5.238689482212067e-10
1000000,2000001,1000000,3000001,7362.588329076767,2.9103830456733704e-10


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0057239532470703125,12064.44795143716
2002,2003,2002,4005,12.436393976211548,60.51993723720079
4004,4005,4004,8009,25.71987295150757,39.88241343054506
6006,6007,6006,12013,38.19901394844055,32.00320195854874
8008,8009,8008,16017,50.22892189025879,27.11878342527234
10010,10011,10010,20021,62.043492794036865,23.600809461513563
12012,12013,12012,24025,74.60394597053528,20.87201122395527
14014,14015,14014,28029,86.38209104537964,18.662265440172632
16016,16017,16016,32033,98.00693202018738,16.824269278082284
18018,18019,18018,36037,110.01513075828552,15.26812653666093
20020,20021,20020,40041,122.02707886695862,13.933915243173033
22022,22023,22022,44045,134.24667978286743,12.7789585000246
24024,24025,24024,48049,146.3578817844391,11.771532716749789
26026,26027,26026,52053,158.34342575073242,10.887304434972975
28028,28029,28028,56057,170.08169078826904,10.106940923971706
30030,30031,30030,60061,181.90570878982544,9.415009303915213
32032,32033,32032,64065,193.57988691329956,8.798924690163403
34034,34035,34034,68069,205.30493688583374,8.248303509202742
36036,36037,36036,72073,218.9467749595642,7.754504986927714
38038,38039,38038,76077,231.09176397323608,7.310268688397628
40040,40041,40040,80081,243.01428389549255,6.909446919986294
42042,42043,42042,84085,254.84966778755188,6.546798895624306
44044,44045,44044,88089,266.65815782546997,6.217830272196807
46046,46047,46046,92093,278.47862792015076,5.9186665376364544
48048,48049,48048,96097,290.37919998168945,5.64595199842006
50050,50051,50050,100101,302.99673771858215,5.396768357961264
52052,52053,52052,104105,315.020770072937,5.168568454482738
54054,54055,54054,108109,327.00134086608887,4.959121853180477
56056,56057,56056,112113,338.9367609024048,4.7664698020507785
58058,58059,58058,116117,350.7897849082947,4.58888765613483
60060,60061,60060,120121,364.6209900379181,4.424853314429129
62062,62063,62062,124125,376.65045189857483,4.2730205407206086
64064,64065,64064,128129,388.3451919555664,4.132196285041573
66066,66067,66066,132133,400.19295167922974,4.001321308174738
68068,68069,68068,136137,412.1706256866455,3.879453553347048
70070,70071,70070,140141,424.5643730163574,3.7657538182211283
72072,72073,72072,144145,436.7355830669403,3.6594773410542984
74074,74075,74074,148149,448.8546619415283,3.5599631590121135
76076,76077,76076,152153,461.0212297439575,3.466599750589012
78078,78079,78078,156157,473.01087188720703,3.378850675193462
80080,80081,80080,160161,484.99418091773987,3.296234586088758
82082,82083,82082,164165,496.9757888317108,3.2183189854094962
84084,84085,84084,168169,508.9748728275299,3.144714744823432
86086,86087,86086,172173,521.1559927463531,3.075071289913467
88088,88089,88088,176177,534.1229887008667,3.009072361419385
90090,90091,90090,180181,547.4847009181976,2.946432278959037
92092,92093,92092,184185,560.69677901268,2.886892643324245
94094,94095,94094,188189,574.0359108448029,2.830219422305163
96096,96097,96096,192193,587.1588208675385,2.776200372385574
98098,98099,98098,196197,599.5922870635986,2.7246427550617227
100100,100101,100100,200201,612.2796759605408,2.6753713119760505
102102,102103,102102,204205,624.2887878417969,2.6282264676283376
104104,104105,104104,208209,636.6425428390503,2.5830627325176465
106106,106107,106106,212213,649.4141659736633,2.539747282902681
108108,108109,108108,216217,661.291729927063,2.4981586964659073
110110,110111,110110,220221,674.5944588184357,2.458185825658802
112112,112113,112112,224225,687.0721189975739,2.419728418746672
114114,114115,114114,228229,700.1456429958344,2.3826917704482184
116116,116117,116116,232233,712.5705690383911,2.3469894577210653
118118,118119,118118,236237,726.6118957996368,2.3125424037352786
120120,120121,120120,240241,739.7932078838348,2.2792777431986906
122122,122123,122122,244245,753.282194852829,2.2471282462211093
124124,124125,124124,248249,766.1182217597961,2.2160318020432896
126126,126127,126126,252253,779.7206218242645,2.185930955405638
128128,128129,128128,256257,792.6831839084625,2.156772489848663
130130,130131,130130,260261,805.3283257484436,2.1285070527756034
132132,132133,132132,264265,818.0841867923737,2.101088817762502
134134,134135,134134,268269,832.237548828125,2.074475180121226
136136,136137,136136,272273,845.7020077705383,2.0486264821665827
138138,138139,138138,276277,858.3537449836731,2.0235057650261297
140140,140141,140140,280281,871.7645168304443,1.999078544205986
142142,142143,142142,284285,884.2345380783081,1.9753126064442768
144144,144145,144144,288289,896.6575119495392,1.9521778256057587
146146,146147,146146,292293,911.8370177745819,1.9296459957095067
148148,148149,148148,296297,928.2627310752869,1.907690679301595
150150,150151,150150,300301,942.5262930393219,1.8862870696302707
152152,152153,152152,304305,956.9589538574219,1.8654118652539182
154154,154155,154154,308309,969.4725189208984,1.8450431557976117
156156,156157,156156,312313,981.6946058273315,1.8251603178177902
158158,158159,158158,316317,994.0580518245697,1.8057439197345957
160160,160161,160160,320321,1005.7127039432526,1.786775634966034
162162,162163,162162,324325,1019.3803677558899,1.7682381624836125
164164,164165,164164,328329,1032.294604063034,1.750115555969387
166166,166167,166166,332333,1047.8579938411713,1.7323943171086285
168168,168169,168168,336337,1061.5030510425568,1.7150572421560355
170170,170171,170170,340341,1074.345566034317,1.6980904722713603
172172,172173,172172,344345,1088.7563667297363,1.6814808655835805
174174,174175,174174,348349,1101.6455948352814,1.6652159496188688
176176,176177,176176,352353,1113.6186158657074,1.6492838775011478
178178,178179,178178,356357,1128.7404947280884,1.633673387554154
180180,180181,180180,360361,1141.9701509475708,1.618373766043078
182182,182183,182182,364365,1155.8671288490295,1.6033748127374565
184184,184185,184184,368369,1168.6076848506927,1.588666809066126
186186,186187,186186,372373,1180.1918830871582,1.5742404886641452
188188,188189,188188,376377,1193.8216331005096,1.5600870100624888
190190,190191,190190,380381,1207.136992931366,1.5461979313786287
192192,192193,192192,384385,1219.127534866333,1.5325651868151908
194194,194195,194194,388389,1231.8551909923553,1.5191810648429964
196196,196197,196196,392393,1243.8286719322205,1.5060381879084161
198198,198199,198198,396397,1256.722396850586,1.4931294935413462
200200,200201,200200,400401,1268.4278347492218,1.4804482167728565
202202,202203,202202,404405,1280.7494778633118,1.4679878737460967
204204,204205,204204,408409,1293.9298660755157,1.4557422464022238
206206,206207,206206,412413,1307.349361896515,1.4437053682177066
208208,208209,208208,416417,1319.3975067138672,1.4318715108456672
210210,210211,210210,420421,1331.3609087467194,1.4202351716412522
212212,212213,212212,424425,1343.1036500930786,1.4087910619764443
214214,214215,214214,428429,1354.8843069076538,1.3975340963006602
216216,216217,216216,432433,1367.5499289035797,1.3864593818798312
218218,218219,218218,436437,1384.2030079364777,1.3755622091830446
220220,220221,220220,440441,1397.7674989700317,1.364838042845804
222222,222223,222222,444445,1411.605272769928,1.3542825131826248
224224,224225,224224,448449,1424.8626708984375,1.3438914082180418
226226,226227,226226,452453,1438.3287608623505,1.3336606661760015
228228,228229,228228,456457,1451.3452298641205,1.323586368424003
230230,230231,230230,460461,1464.2619998455048,1.313664732810139
232232,232233,232232,464465,1476.928631067276,1.3038921074039536
234234,234235,234234,468469,1489.2473368644714,1.294264964564718
236236,236237,236236,472473,1502.4832429885864,1.284781583435688
238238,238239,238238,476477,1515.8099808692932,1.2754374627220386
240240,240241,240240,480481,1528.5791397094727,1.2662289049112587
242242,242243,242242,484485,1541.096617937088,1.257152827014579
244244,244245,244244,488489,1553.6392469406128,1.2482062455619598
246246,246247,246246,492493,1566.2238228321075,1.239386272194679
248248,248249,248248,496497,1578.7233929634094,1.2306901096308138
250250,250251,250250,500501,1591.0744078159332,1.2221150478617346
252252,252253,252252,504505,1603.4611568450928,1.213658460557781
254254,254255,254254,508509,1616.454274892807,1.2053178016558377
256256,256257,256256,512513,1629.264592885971,1.1970906021233532
258258,258259,258258,516517,1643.3768830299377,1.1889744668806088
260260,260261,260260,520521,1657.1598699092865,1.1809670718939742
262262,262263,262262,524525,1670.782167673111,1.1730661613728444
264264,264265,264264,528529,1683.5909428596497,1.165269545157571
266266,266267,266266,532533,1697.804841041565,1.1575750961819722
268268,268269,268268,536537,1711.2884407043457,1.1499807480904565
270270,270271,270270,540541,1724.6725058555603,1.142484492962467
272272,272273,272272,544545,1737.6296887397766,1.1350843791242369
274274,274275,274274,548549,1750.2737798690796,1.1277785090842372
276276,276277,276276,552553,1762.9676077365875,1.1205650375632104
278278,278279,278278,556557,1775.440813779831,1.113442169589689
280280,280281,280280,560561,1788.0645167827606,1.106408158715567
282282,282283,282282,564565,1800.469456911087,1.0994613052844215
284284,284285,284284,568569,1815.9201438426971,1.092599954790785
286286,286287,286286,572573,1830.4021179676056,1.0858224963048997
288288,288289,288288,576577,1843.8353190422058,1.079127360972052
290290,290291,290290,580581,1857.1701409816742,1.0725130205682945
292292,292293,292292,584585,1872.0150468349457,1.065977986128928
294294,294295,294294,588589,1884.6017858982086,1.0595208066242776
296296,296297,296296,592593,1897.4450199604034,1.0531400676991325
298298,298299,298298,596597,1910.5697510242462,1.0468343904612993
300300,300301,300300,600601,1922.6424479484558,1.04060243031563
302302,302303,302302,604605,1936.4769790172577,1.0344428758617141
304304,304305,304304,608609,1949.7964890003204,1.028354447806123
306306,306307,306306,612613,1962.519910812378,1.022335897965604
308308,308309,308308,616617,1975.4930489063263,1.0163860082484462
310310,310311,310310,620621,1988.8836948871613,1.0105035897377093
312312,312313,312312,624625,2002.3053770065308,1.0046874817689968
314314,314315,314314,628629,2016.0459520816803,0.9989365510573407
316316,316317,316316,632633,2030.028657913208,0.9932496908622852
318318,318319,318318,636637,2043.6190469264984,0.9876258201802557
320320,320321,320320,640641,2056.511157989502,0.9820638829642121
322322,322323,322322,644645,2069.0415139198303,0.9765628473796824
324324,324325,324324,648649,2082.677750110626,0.9711217050808045
326326,326327,326326,652653,2095.9720509052277,0.9657394705227489
328328,328329,328328,656657,2107.9979219436646,0.9604151802941487
330330,330331,330330,660661,2121.4130918979645,0.9551478924713592
332332,332333,332332,664665,2135.2459127902985,0.9499366860000009
334334,334335,334334,668669,2148.730887889862,0.9447806600946933
336336,336337,336336,672673,2162.387978076935,0.9396789336697111
338338,338339,338338,676677,2175.961683034897,0.9346306447750976
340340,340341,340340,680681,2190.5152208805084,0.9296349500655197
342342,342343,342342,684685,2202.984610080719,0.9246910242891317
344344,344345,344344,688689,2215.7431168556213,0.919798059765526
346346,346347,346346,692693,2228.665988922119,0.9149552659291658
348348,348349,348348,696697,2241.1729769706726,0.9101618688546296
350350,350351,350350,700701,2253.857395887375,0.9054171107909497
352352,352353,352352,704705,2266.3755128383636,0.9007202497523394
354354,354355,354354,708709,2278.7559299468994,0.896070559079817
356356,356357,356356,712713,2291.195673942566,0.8914673270392086
358358,358359,358358,716717,2304.1715857982635,0.8869098564282467
360360,360361,360360,720721,2317.039179086685,0.8823974641964014
362362,362363,362362,724725,2329.9535529613495,0.8779294810738065
364364,364365,364364,728729,2342.473002910614,0.8735052512238326
366366,366367,366366,732733,2355.018185853958,0.869124131886565
368368,368369,368368,736737,2366.9916837215424,0.8647854930513859
370370,370371,370370,740741,2378.997701883316,0.8604887171313749
372372,372373,372372,744745,2392.327955007553,0.8562331986540812
374374,374375,374374,748749,2405.3300170898438,0.8520183439468383
376376,376377,376376,752753,2418.4522778987885,0.8478435708675534
378378,378379,378378,756757,2431.81685090065,0.8437083084827464
380380,380381,380380,760761,2444.863914012909,0.8396119968274434
382382,382383,382382,764765,2456.9826679229736,0.8355540866105002
384384,384385,384384,768769,2468.972272872925,0.8315340389726771
386386,386387,386386,772773,2480.946861743927,0.8275513252247038
388388,388389,388388,776777,2494.5223019123077,0.823605849289379
390390,390391,390390,780781,2508.3469598293304,0.8196969175605773
392392,392393,392392,784785,2521.7119858264923,0.8158237875995837
394394,394395,394394,788789,2535.266530752182,0.811985967480723
396396,396397,396396,792793,2548.3147678375244,0.808182975899399
398398,398399,398398,796797,2561.3257191181183,0.804414340396761
400400,400401,400400,800801,2574.0794739723206,0.800679597121416
402402,402403,402402,804805,2586.815207004547,0.7969782906257024
404404,404405,404404,808809,2598.9453258514404,0.7933099736819713
406406,406407,406406,812813,2611.8092958927155,0.7896742070752225
408408,408409,408408,816817,2625.302619934082,0.7860705594393949
410410,410411,410410,820821,2637.18074798584,0.7824986070663726
412412,412413,412412,824825,2650.405716896057,0.7789579337368195
414414,414415,414414,828829,2662.7680048942566,0.7754481305619265
416416,416417,416416,832833,2675.2952420711517,0.7719687957978749
418418,418419,418418,836837,2686.934940814972,0.7685195347148692
420420,420421,420420,840841,2699.8706629276276,0.7650999594152381
422422,422423,422422,844845,2713.025932788849,0.7617096887133812
424424,424425,424424,848849,2727.2112929821014,0.7583483479575079
426426,426427,426426,852853,2740.7151119709015,0.7550155689077656
428428,428429,428428,856857,2754.4733397960663,0.7517109895998146
430430,430431,430430,860861,2767.3416709899902,0.7484342541920341
432432,432433,432432,864865,2778.824870824814,0.745185012856382
434434,434435,434434,868869,2790.198425769806,0.7419629216274188
436436,436437,436436,872873,2802.393215894699,0.738767642298626
438438,438439,438438,876877,2816.1583228111267,0.7355988422896189
440440,440441,440440,880881,2829.272639989853,0.7324561945260939
442442,442443,442442,884885,2843.0711948871613,0.7293393773379648
444444,444445,444444,888889,2855.3805010318756,0.7262480743265769
446446,446447,446446,892893,2868.363438844681,0.723181974281033
448448,448449,448448,896897,2881.4017260074615,0.7201407710435888
450450,450451,450450,900901,2893.8148880004883,0.7171241634277976
452452,452453,452452,904905,2906.279236793518,0.7141318551039149
454454,454455,454454,908909,2919.3031549453735,0.7111635613619001
456456,456457,456456,912913,2932.065527677536,0.7082190378696396
458458,458459,458458,916917,2944.88738489151,0.705297955288188
460460,460461,460460,920921,2959.066305875778,0.7024000356959732
462462,462463,462462,924925,2972.166332960129,0.6995250055406359
464464,464465,464464,928929,2987.2646107673645,0.6966725955990114
466466,466467,466466,932933,3004.01775097847,0.6938425408516196
468468,468469,468468,936937,3016.986512899399,0.6910345804280951
470470,470471,470470,940941,3030.527004957199,0.688248457514419
472472,472473,472472,944945,3042.49551486969,0.6854839192710642
474474,474475,474474,948949,3054.28698182106,0.682740716758417
476476,476477,476476,952953,3065.7613368034363,0.6800186048676551
478478,478479,478478,956957,3077.402570962906,0.6773173422279797
480480,480481,480480,960961,3089.2032039165497,0.6746366911593213
482482,482483,482482,964965,3100.793107032776,0.6719764175868477
484484,484485,484484,968969,3112.444744825363,0.6693362909718417
486486,486487,486486,972973,3123.9330229759216,0.6667160842498561
488488,488489,488488,976977,3135.5045788288116,0.6641155737615918
490490,490491,490490,980981,3147.569133758545,0.6615345391965093
492492,492493,492492,984985,3160.3730659484863,0.6589727635109739
494494,494495,494494,988989,3172.4351818561554,0.6564300328955142
496496,496497,496496,992993,3184.71506690979,0.6539061366820533
498498,498499,498498,996997,3197.372960090637,0.6514008673239005
500501,500502,500501,1001003,3209.6635839939117,0.6489127826826007
502503,502504,502503,1005007,3221.5128247737885,0.6464441655152768
504505,504506,504505,1009011,3233.2372949123383,0.6439935704584059
506507,506508,506507,1013015,3244.9402298927307,0.641560801794185
508509,508510,508509,1017019,3256.222494840622,0.6391456666369777
510511,510512,510511,1021023,3267.246356010437,0.6367479748732876
512513,512514,512513,1025027,3278.258519887924,0.6343675391108263
514515,514516,514515,1029031,3289.5222997665405,0.6320041746421339
516517,516518,516517,1033035,3300.7477419376373,0.629657699380914
518519,518520,518519,1037039,3311.7653279304504,0.6273279338274733
520521,520522,520521,1041043,3322.668732881546,0.6250147010177898
522523,522524,522523,1045047,3333.583937883377,0.6227178264725808
524525,524526,524525,1049051,3344.539895772934,0.6204400265232834
526527,526528,526527,1053055,3355.457500934601,0.6181804328025464
528529,528530,528529,1057059,3366.358989715576,0.6159367944001133
530531,530532,530531,1061063,3377.19726896286,0.6137088857522031
532533,532534,532533,1065067,3388.1366369724274,0.6114965098204266
534535,534536,534535,1069071,3398.940510034561,0.6092994864266075
536537,536538,536537,1073075,3410.1583087444305,0.6071176459354319
538539,538540,538539,1077079,3421.1507778167725,0.6049508256819536
540541,540542,540541,1081083,3431.9294810295105,0.602798867968886
542543,542544,542543,1085087,3442.9948921203613,0.6006616188460612
544545,544546,544545,1089091,3454.2583696842194,0.598538927415575
546547,546548,546547,1093095,3465.4883248806,0.5964306453988684
548549,548550,548549,1097099,3476.714877843857,0.594340935585933
550551,550552,550551,1101103,3488.4569249153137,0.5922658603249147
552553,552554,552553,1105107,3499.696594953537,0.5902048294192355
554555,554556,554555,1109111,3510.7623360157013,0.5881576432420843
556557,556558,556557,1113115,3521.9187738895416,0.586124140132597
558559,558560,558559,1117119,3532.941642999649,0.5841041745170514
560561,560562,560561,1121123,3544.064374923706,0.5820976083541609
562563,562564,562563,1125127,3554.8622949123383,0.5801043077408394
564565,564566,564565,1129131,3564.4470448493958,0.5781241414933902
566567,566568,566567,1133135,3572.042683839798,0.5761569805854379
568569,568570,568569,1137139,3582.5840079784393,0.5742026978496142
570571,570572,570571,1141143,3593.5576848983765,0.5722611678866087
572573,572574,572573,1145147,3604.4027438163757,0.5703322669596673
574575,574576,574575,1149151,3615.5273637771606,0.5684158729618503
576577,576578,576577,1153155,3626.2027378082275,0.5665118653705576
578579,578580,578579,1157159,3634.974147796631,0.5646201252202445
580581,580582,580581,1161163,3641.5354340076447,0.562740535076955
582583,582584,582583,1165167,3648.0535349845886,0.5608729790055804
584585,584586,584585,1169171,3657.0430369377136,0.5590173425407556
586587,586588,586587,1173175,3666.3478269577026,0.557173512670488
588589,588590,588589,1177179,3674.1167368888855,0.5553413778106915
590591,590592,590591,1181183,3681.3372209072113,0.553520827774264
592593,592594,592593,1185187,3688.7228679656982,0.5517117537656304
594595,594596,594595,1189191,3695.3708579540253,0.5499140483298106
596597,596598,596597,1193195,3701.553076982498,0.5481276053633337
598599,598600,598599,1197199,3707.55463886261,0.5463523200705822
600601,600602,600601,1201203,3713.6492817401886,0.544588088952878
602603,602604,602603,1205207,3720.201534986496,0.5428348097848357
604605,604606,604605,1209211,3726.053242921829,0.5410923815961723
606607,606608,606607,1213215,3731.1867849826813,0.539360704655337
608609,608610,608609,1217219,3736.9457080364227,0.5376396804404067
610611,610612,610611,1221223,3743.1484208106995,0.5359292116336292
612613,612614,612613,1225227,3748.3595221042633,0.5342292020923196
614615,614616,614615,1229231,3754.0804460048676,0.5325395568379463
616617,616618,616617,1233235,3760.2432539463043,0.5308601820361218
618619,618620,618619,1237239,3767.4221358299255,0.5291909849784133
620621,620622,620621,1241243,3774.479855775833,0.5275318740659714
622623,622624,622623,1245247,3779.7799627780914,0.5258827587967971
624625,624626,624625,1249251,3785.6613528728485,0.5242435497402766
626627,626628,626627,1253255,3792.0845420360565,0.5226141585335426
628629,628630,628629,1257259,3798.340866804123,0.5209944978523708
630631,630632,630631,1261263,3804.2628648281097,0.5193844814075419
632633,632634,632633,1265267,3810.685384988785,0.5177840239211946
634635,634636,634635,1269271,3816.843044757843,0.5161930411195499
636637,636638,636637,1273275,3822.501832008362,0.514611449705626
638639,638640,638639,1277279,3827.8420050144196,0.5130391673665144
640641,640642,640641,1281283,3832.6859877109528,0.5114761127351812
642643,642644,642643,1285287,3837.6897218227386,0.5099222053922858
644645,644646,644645,1289291,3843.2958719730377,0.5083773658443533
646647,646648,646647,1293295,3848.598186969757,0.5068415155219554
648649,648650,648649,1297299,3853.8505368232727,0.5053145767469687
650651,650652,650651,1301303,3858.698084831238,0.5037964727362123
652653,652654,652653,1305307,3863.7135388851166,0.5022871275923535
654655,654656,654655,1309311,3869.2474088668823,0.5007864662638895
656657,656658,656657,1313315,3875.1999328136444,0.4992944145706133
658659,658660,658659,1317319,3881.073315858841,0.49781089916177734
660661,660662,660661,1321323,3887.456116914749,0.49633584751973103
662663,662664,662663,1325327,3893.6296210289,0.4948691879380931
664665,664666,664665,1329331,3899.438309907913,0.4934108495217515
666667,666668,666667,1333335,3906.207049846649,0.4919607621650357
668669,668670,668669,1337339,3913.0087287425995,0.49051885655353544
670671,670672,670671,1341343,3919.13432097435,0.4890850641295401
672673,672674,672673,1345347,3925.240109682083,0.48765931711386656
674675,674676,674675,1349351,3931.8753249645233,0.4862415484676603
676677,676678,676677,1353355,3937.8133749961853,0.4848316918942146
678679,678680,678679,1357359,3943.2455937862396,0.48342968182805635
680681,680682,680681,1361363,3948.995223760605,0.4820354534258513
682683,682684,682683,1365367,3954.1421320438385,0.4806489425518521
684685,684686,684685,1369371,3959.1747648715973,0.47927008577062225
686687,686688,686687,1373375,3963.844841003418,0.4778988203379413
688689,688690,688689,1377379,3968.5268239974976,0.4765350841989857
690691,690692,690691,1381383,3973.3278846740723,0.4751788159574062
692693,692694,692693,1385387,3978.614935874939,0.4738299548935174
694695,694696,694695,1389391,3983.558469772339,0.4724884409315564
696697,696698,696697,1393395,3988.5291221141815,0.47115421464877727
698699,698700,698699,1397399,3993.8383429050446,0.4698272172608995
700701,700702,700701,1401403,3998.907707929611,0.4685073906020989
702703,702704,702703,1405407,4003.955164909363,0.46719467713592167
704705,704706,704705,1409411,4009.4379110336304,0.46588901993527543
706707,706708,706707,1413415,4015.5749378204346,0.4645903626769723
708709,708710,708709,1417419,4021.614762067795,0.4632986496308149
710711,710712,710711,1421423,4028.330680847168,0.4620138256595965
712713,712714,712713,1425427,4034.325530767441,0.46073583620272984
714715,714716,714715,1429431,4040.505446910858,0.4594646272762475
716717,716718,716717,1433435,4046.3376269340515,0.45820014545461163
718719,718720,718719,1437439,4052.4025559425354,0.4569423378779902
720721,720722,720721,1441443,4058.796544075012,0.45569115222861
722723,722724,722723,1445447,4066.0419347286224,0.45444653674167057
724725,724726,724725,1449451,4072.074672937393,0.4532084401780594
726727,726728,726727,1453455,4078.134169816971,0.4519768118407228
728729,728730,728729,1457459,4084.5070950984955,0.4507516015419242
730731,730732,730731,1461463,4090.039997816086,0.4495327596214338
732733,732734,732733,1465467,4097.180171966553,0.44832023692106304
734735,734736,734735,1469471,4104.195430994034,0.44711398478648334
736737,736738,736737,1473475,4110.199882030487,0.44591395506176923
738739,738740,738739,1477479,4116.189069747925,0.4447201000784844
740741,740742,740741,1481483,4121.483787059784,0.4435323726538627
742743,742744,742743,1485487,4127.149904966354,0.4423507260835322
744745,744746,744745,1489491,4134.121069908142,0.44117511413787724
746747,746748,746747,1493495,4140.203313827515,0.44000549104202946
748749,748750,748749,1497499,4146.345674037933,0.4388418114904198
750751,750752,750751,1501503,4152.68705201149,0.4376840306358645
752753,752754,752753,1505507,4158.5335948467255,0.43653210406409926
754755,754756,754755,1509511,4164.172788858414,0.43538598781378823
756757,756758,756757,1513515,4169.73092675209,0.4342456383692479
758759,758760,758759,1517519,4175.036051988602,0.43311101262588636
760761,760762,760761,1521523,4180.482174873352,0.4319820679247641
762763,762764,762763,1525527,4185.853889703751,0.4308587620180333
764765,764766,764765,1529531,4191.072395086288,0.42974105308167054
766767,766768,766767,1533535,4196.578696012497,0.42862889969183016
768769,768770,768769,1537539,4202.032540798187,0.42752226083757705
770771,770772,770771,1541543,4207.483628034592,0.4264210958936019
772773,772774,772773,1545547,4213.024808883667,0.4253253646184021
774775,774776,774775,1549551,4219.182490825653,0.4242350271797477
776777,776778,776777,1553555,4226.657056093216,0.4231500441183016
778779,778780,778779,1557559,4232.362294912338,0.42207037636399036
780781,780782,780781,1561563,4237.35993885994,0.4209959852287284
782783,782784,782783,1565567,4242.128581762314,0.4199268323936849
784785,784786,784785,1569571,4247.405993938446,0.4188628799129219
786787,786788,786787,1573575,4253.0028438568115,0.41780409020248044
788789,788790,788789,1577579,4258.875963926315,0.41675042604219925
790791,790792,790791,1581583,4264.308646917343,0.4157018505666201
792793,792794,792793,1585587,4270.012740850449,0.4146583272595308
794795,794796,794795,1589591,4275.094332933426,0.41361981996124086
796797,796798,796797,1593595,4280.355321884155,0.4125862928431161
798799,798800,798799,1597599,4284.934052944183,0.41155771042758715
800801,800802,800801,1601603,4289.486024856567,0.4105340375663218
802803,802804,802803,1605607,4294.145545959473,0.40951523944022483
804805,804806,804805,1609611,4298.64532995224,0.4085012815630762
806807,806808,806807,1613615,4303.5122628211975,0.4074921297724359
808809,808810,808809,1617619,4308.115703821182,0.40648775021873007
810811,810812,810811,1621623,4312.738679885864,0.4054881093743461
812813,812814,812813,1625627,4318.657091856003,0.4044931740281754
814815,814816,814815,1629631,4323.645150899887,0.4035029112656048
816817,816818,816817,1633635,4328.781987905502,0.4025172884885251
818819,818820,818819,1637639,4333.698354005814,0.4015362733935035
820821,820822,820821,1641643,4338.880596876144,0.4005598339736025
822823,822824,822823,1645647,4344.440878868103,0.39958793852929375
824825,824826,824825,1649651,4349.821624755859,0.3986205556357163
826827,826828,826827,1653655,4354.698379993439,0.39765765416814247
828829,828830,828829,1657659,4359.818124771118,0.39669920328014996
830831,830832,830831,1661663,4364.365699768066,0.3957451724072598
832833,832834,832833,1665667,4369.40478181839,0.39479553126329847
834835,834836,834835,1669671,4374.282012939453,0.3938502498422167
836837,836838,836837,1673675,4379.809066057205,0.39290929839989985
838839,838840,838839,1677679,4384.809836864471,0.3919726474705385
840841,840842,840841,1681683,4390.680941820145,0.3910402678484388
842843,842844,842843,1685687,4395.737122774124,0.3901121305916604
844845,844846,844845,1689691,4400.957841873169,0.3891882070201973
846847,846848,846847,1693695,4406.166111946106,0.38826846870506415
848849,848850,848849,1697699,4410.715786933899,0.38735288748102903
850851,850852,850851,1701703,4415.242920875549,0.3864414354266046
852853,852854,852853,1705707,4419.828320980072,0.38553408486768603
854855,854856,854855,1709711,4424.637412786484,0.38463080837937014
856857,856858,856857,1713715,4429.2001140117645,0.38373157878231723
858859,858860,858859,1717719,4433.846656084061,0.3828363691300183
860861,860862,860861,1721723,4439.972784757614,0.3819451527160709
862863,862864,862863,1725727,4445.461322069168,0.38105852941771445
864865,864866,864865,1729731,4450.412357807159,0.3801764308936981
866867,866868,866867,1733735,4455.410667896271,0.3792982493778254
868869,868870,868869,1737739,4461.505923748016,0.37842395435836806
870871,870872,870871,1741743,4466.759452819824,0.3775535191907693
872873,872874,872873,1745747,4472.1079750061035,0.37668691810176824
874875,874876,874875,1749751,4477.80911898613,0.37582412579831725
876877,876878,876877,1753755,4482.8341319561005,0.37496511731842475
878879,878880,878879,1757759,4487.430838108063,0.37410986874419905
880881,880882,880881,1761763,4492.139890909195,0.3732583589753631
882883,882884,882883,1765767,4496.743131875992,0.37241056059792754
884885,884886,884885,1769771,4501.257176876068,0.3715664489845949
886887,886888,886887,1773775,4505.858793020248,0.3707260000792303
888889,888890,888889,1777779,4510.331367969513,0.36988919015493593
890891,890892,890891,1781783,4514.860918998718,0.36905599572855863
892893,892894,892893,1785787,4519.398862838745,0.36822639354431885
894895,894896,894895,1789791,4523.979068994522,0.3674003605628968
896897,896898,896897,1793795,4528.520212888718,0.36657787393414765
898899,898900,898899,1797799,4533.085356712341,0.3657589110225672
900901,900902,900901,1801803,4537.613943099976,0.36494344937455026
902903,902904,902903,1805807,4542.344341993332,0.36413146672566654
904905,904906,904905,1809811,4546.985957860947,0.3633229410115746
906907,906908,906907,1813815,4551.672353982925,0.3625178503425559
908909,908910,908909,1817819,4556.694780826569,0.3617161730180669
910911,910912,910911,1821823,4563.372940778732,0.36091788752310094
912913,912914,912913,1825827,4569.038534879684,0.3601229725063604
914915,914916,914915,1829831,4574.6852197647095,0.3593314068202744
916917,916918,916917,1833835,4580.95414185524,0.3585431694646104
918919,918920,918919,1837839,4586.19809794426,0.3577582396410435
920921,920922,920921,1841843,4591.294232845306,0.35697659669676796
922923,922924,922923,1845847,4596.954165935516,0.35619822017179104
924925,924926,924925,1849851,4602.492560863495,0.355423089764372
926927,926928,926927,1853855,4607.61025595665,0.3546511853401171
928929,928930,928929,1857859,4612.381989955902,0.35388248693197966
930931,930932,930931,1861863,4617.600532054901,0.3531169747348031
932933,932934,932933,1865867,4622.490839719772,0.35235462911077775
934935,934936,934935,1869871,4627.107048988342,0.3515954305712512
936937,936938,936937,1873875,4631.616614818573,0.35083935980037495
938939,938940,938939,1877879,4636.0397799015045,0.3500863976260007
940941,940942,940941,1881883,4640.693208694458,0.34933652504332713
942943,942944,942943,1885887,4645.204140663147,0.34858972319307213
944945,944946,944945,1889891,4649.620880842209,0.3478459733687487
946947,946948,946947,1893895,4654.76638007164,0.3471052570221218
948949,948950,948949,1897899,4659.889716863632,0.34636755574501876
950951,950952,950951,1901903,4664.326145648956,0.3456328512838809
952953,952954,952953,1905907,4669.112834692001,0.34490112552884966
954955,954956,954955,1909911,4675.287544727325,0.34417236051558575
956957,956958,956957,1913915,4681.316027879715,0.343446538419812
958959,958960,958959,1917919,4686.2646498680115,0.34272364156277035
960961,960962,960961,1921923,4691.537542819977,0.342003652405765
962963,962964,962963,1925927,4696.296371936798,0.34128655355016235
964965,964966,964965,1929931,4700.895061969757,0.3405723277337529
966967,966968,966967,1933935,4705.689305782318,0.33986095783075143
968969,968970,968969,1937939,4710.825269937515,0.33915242684997793
970971,970972,970971,1941943,4715.3773357868195,0.33844671793849557
972973,972974,972973,1945947,4719.931447029114,0.3377438143652398
974975,974976,974975,1949951,4724.482553720474,0.3370436995428463
976977,976978,976977,1953955,4729.054510831833,0.3363463570094609
978979,978980,978979,1957959,4733.677906990051,0.33565177042328287
980981,980982,980981,1961963,4738.34775185585,0.3349599235862115
982983,982984,982983,1965967,4742.955549001694,0.3342708004111046
984985,984986,984985,1969971,4747.568529844284,0.33358438494542497
986987,986988,986987,1973975,4752.112090826035,0.33290066135305096
988989,988990,988989,1977979,4756.658801794052,0.33221961393064703
990991,990992,990991,1981983,4761.270407915115,0.331541227084017
992993,992994,992993,1985987,4765.886277914047,0.330865485346294
994995,994996,994995,1989991,4770.433772087097,0.3301923733706644
996997,996998,996997,1993995,4774.9511387348175,0.329521875921273
998999,999000,998999,1997999,4779.627534866333,0.3288539778877748
1001001,1001002,1001001,2002003,4784.221988916397,0.3281886642653262
1003003,1003004,1003003,2006007,4788.768249750137,0.3275259201764129
1005005,1005006,1005005,2010011,4793.354526042938,0.32686573084720294
1007007,1007008,1007007,2014015,4797.92226099968,0.3262080816184607
1009009,1009010,1009009,2018019,4802.52365899086,0.32555295794009
1011011,1011012,1011011,2022023,4807.055500745773,0.3249003453802288
1013013,1013014,1013013,2026027,4811.63431596756,0.32425022960524075
1015015,1015016,1015015,2030031,4816.191326856613,0.32360259640336153
1017017,1017018,1017017,2034035,4820.73074388504,0.32295743165195745
1019019,1019020,1019019,2038039,4825.303936004639,0.32231472135026706
1021021,1021022,1021021,2042043,4829.807498931885,0.32167445159757335
1023023,1023024,1023023,2046047,4834.363724708557,0.3210366085950227
1025025,1025026,1025025,2050051,4838.909561872482,0.3204011786474439
1027027,1027028,1027027,2054055,4843.4537088871,0.3197681481633481
1029029,1029030,1029029,2058059,4847.97435092926,0.3191375036549289
1031031,1031032,1031031,2062063,4852.530962944031,0.3185092317289673
1033033,1033034,1033033,2066067,4857.181500911713,0.3178833190959267
1035035,1035036,1035035,2070071,4862.260901927948,0.317259752564496
1037037,1037038,1037037,2074075,4867.09419798851,0.31663851903977047
1039039,1039040,1039039,2078079,4871.778208971024,0.3160196055214328
1041041,1041042,1041041,2082083,4876.48356795311,0.3154029991110292
1043043,1043044,1043043,2086087,4881.64897108078,0.31478868699741724
1045045,1045046,1045045,2090091,4886.412800073624,0.314176656471318
1047047,1047048,1047047,2094095,4891.264453887939,0.31356689491076395
1049049,1049050,1049049,2098099,4896.417747974396,0.31295938978655613
1051051,1051052,1051051,2102103,4901.729318857193,0.31235412866772094
1053053,1053054,1053053,2106107,4906.6482989788055,0.31175109920150135
1055055,1055056,1055055,2110111,4912.025633096695,0.3111502891388227
1057057,1057058,1057057,2114115,4917.264209985733,0.3105516863124649
1059059,1059060,1059059,2118119,4922.56670498848,0.3099552786370623
1061061,1061062,1061061,2122123,4927.632023096085,0.3093610541327507
1063063,1063064,1063063,2126127,4932.736760854721,0.30876900088878756
1065065,1065066,1065065,2130131,4937.935338020325,0.30817910708537966
1067067,1067068,1067067,2134135,4943.164881944656,0.30759136099186435
1069069,1069070,1069069,2138139,4947.923549890518,0.3070057509594335
1071071,1071072,1071071,2142143,4952.480514764786,0.3064222654229525
1073073,1073074,1073073,2146147,4957.173677682877,0.30584089290096017
1075075,1075076,1075075,2150151,4961.701231956482,0.305261621988393
1077077,1077078,1077077,2154155,4966.293132066727,0.30468444136931794
1079079,1079080,1079079,2158159,4971.234192848206,0.3041093398078374
1081081,1081082,1081081,2162163,4975.964017868042,0.3035363061426324
1083083,1083084,1083083,2166167,4980.6173787117,0.3029653292942385
1085085,1085086,1085085,2170171,4985.141084909439,0.30239639826322673
1087087,1087088,1087087,2174175,4989.659781932831,0.3018295021265658
1089089,1089090,1089089,2178179,4994.3680419921875,0.3012646300394408
1091091,1091092,1091091,2182183,4998.955102920532,0.3007017712297966
1093093,1093094,1093093,2186187,5003.597646713257,0.30014091500743234
1095095,1095096,1095095,2190191,5008.241469860077,0.299582050751269
1097097,1097098,1097097,2194195,5013.090375900269,0.2990251679184439
1099099,1099100,1099099,2198199,5017.966705799103,0.2984702560406731
1101101,1101102,1101101,2202203,5022.799950838089,0.2979173047206132
1103103,1103104,1103103,2206207,5027.627104997635,0.29736630363186123
1105105,1105106,1105105,2210211,5033.2843408584595,0.296817242524412
1107107,1107108,1107107,2214215,5039.418381690979,0.2962701112155628
1109109,1109110,1109109,2218219,5045.356537818909,0.2957248995971895
1111111,1111112,1111111,2222223,5051.8577709198,0.2951815976284706
1113113,1113114,1113113,2226227,5058.337679862976,0.29464019533952523
1115115,1115116,1115115,2230231,5064.143140792847,0.29410068282231805
1117117,1117118,1117117,2234235,5068.66331076622,0.2935630502488493
1119119,1119120,1119119,2238239,5073.323064804077,0.29302728785296495
1121121,1121122,1121121,2242243,5078.792990922928,0.2924933859358134
1123123,1123124,1123123,2246247,5083.628935813904,0.29196133486402687
1125125,1125126,1125125,2250251,5088.68439078331,0.291431125073359
1127127,1127128,1127127,2254255,5093.7575969696045,0.2909027470595902
1129129,1129130,1129129,2258259,5098.669502019882,0.2903761913894414
1131131,1131132,1131131,2262263,5103.360232830048,0.2898514486896602
1133133,1133134,1133133,2266267,5108.4453728199005,0.2893285096524778
1135135,1135136,1135135,2270271,5113.471379995346,0.2888073650337901
1137137,1137138,1137137,2274275,5118.075543880463,0.2882880056531576
1139139,1139140,1139139,2278279,5122.614551782608,0.2877704223883484
1141141,1141142,1141141,2282283,5127.2440440654755,0.28725460618079524
1143143,1143144,1143143,2286287,5131.789764881134,0.28674054803559557
1145145,1145146,1145145,2290291,5136.343441963196,0.28622823901605443
1147147,1147148,1147147,2294295,5140.921498775482,0.28571767024550354
1149149,1149150,1149149,2298299,5146.244611740112,0.28520883290548227
1151151,1151152,1151151,2302303,5152.02401471138,0.2847017182393756
1153153,1153154,1153153,2306307,5156.928164720535,0.2841963175469573
1155155,1155156,1155155,2310311,5162.495882034302,0.28369262219348457
1157157,1157158,1157157,2314315,5166.982992887497,0.2831906235842325
1159159,1159160,1159159,2318319,5171.416391849518,0.28269031320633076
1161161,1161162,1161161,2322323,5175.825987815857,0.28219168257965066
1163163,1163164,1163163,2326327,5180.395891904831,0.2816947232968232
1165165,1165166,1165165,2330331,5184.838183879852,0.2811994269959541
1167167,1167168,1167167,2334335,5189.243308067322,0.28070578537881374
1169169,1169170,1169169,2338339,5193.788635969162,0.2802137901999231
1171171,1171172,1171171,2342343,5198.275225877762,0.27972343326291593
1173173,1173174,1173173,2346347,5202.702685832977,0.2792347064259957
1175175,1175176,1175175,2350351,5207.331475973129,0.2787476016092114
1177177,1177178,1177177,2354355,5211.832864046097,0.27826211077808694
1179179,1179180,1179179,2358359,5216.293675899506,0.27777822595089674
1181181,1181182,1181181,2362363,5220.781254768372,0.277295939204123
1183183,1183184,1183183,2366367,5225.370840787888,0.27681524265972257
1185185,1185186,1185185,2370371,5229.8007118701935,0.2763361284924031
1187187,1187188,1187187,2374375,5234.2492599487305,0.27585858893326076
1189189,1189190,1189189,2378379,5238.7202298641205,0.27538261625522864
1191191,1191192,1191191,2382383,5243.0998730659485,0.27490820278217143
1193193,1193194,1193193,2386387,5247.610431909561,0.2744353408997995
1195195,1195196,1195195,2390391,5252.03733587265,0.27396402303020295
1197197,1197198,1197197,2394395,5256.432172775269,0.2734942416464037
1199199,1199200,1199199,2398399,5260.873626947403,0.2730259892759932
1201201,1201202,1201201,2402403,5265.2876517772675,0.2725592584883998
1203203,1203204,1203203,2406407,5269.67730307579,0.27209404190580244
1205205,1205206,1205205,2410411,5274.176853895187,0.2716303321922169
1207207,1207208,1207207,2414415,5278.613901853561,0.27116812206440954
1209209,1209210,1209209,2418419,5283.018865823746,0.2707074042809836
1211211,1211212,1211211,2422423,5287.394817113876,0.270248171649655
1213213,1213214,1213213,2426427,5292.341337919235,0.2697904170236143
1215215,1215216,1215215,2430431,5297.856072902679,0.2693341333015269
1217217,1217218,1217217,2434435,5303.989568948746,0.2688793134275329
1219219,1219220,1219219,2438439,5308.90336894989,0.2684259503876092
1221221,1221222,1221221,2442443,5314.444131851196,0.2679740372168453
1223223,1223224,1223223,2446447,5320.235439777374,0.2675235669921676
1225225,1225226,1225225,2450451,5325.988439083099,0.2670745328323392
1227227,1227228,1227227,2454455,5331.5082218647,0.2666269279034168
1229229,1229230,1229229,2458459,5336.723392963409,0.2661807454114751
1231231,1231232,1231231,2462463,5342.065901756287,0.2657359786098823
1233233,1233234,1233233,2466467,5348.554561853409,0.2652926207847486
1235235,1235236,1235235,2470471,5354.512899875641,0.2648506652767537
1237237,1237238,1237237,2474475,5359.764008998871,0.2644101054593193
1239239,1239240,1239239,2478479,5364.842181921005,0.26397093474588473
1241241,1241242,1241241,2482483,5370.059077978134,0.26353314660264004
1243243,1243244,1243243,2486487,5375.3752319812775,0.26309673452669813
1245245,1245246,1245245,2490491,5380.8680629730225,0.2626616920588276
1247247,1247248,1247247,2494495,5385.982218027115,0.26222801277253893
1249249,1249250,1249249,2498499,5390.602140903473,0.2617956902977312
1251251,1251252,1251251,2502503,5395.1891458034515,0.2613647182861314
1253253,1253254,1253253,2506507,5399.901926994324,0.2609350904440362
1255255,1255256,1255255,2510511,5405.548369884491,0.2605068004995701
1257257,1257258,1257257,2514515,5411.069795846939,0.26007984223906533
1259259,1259260,1259259,2518519,5416.668910741806,0.25965420947250095
1261261,1261262,1261261,2522523,5421.210109949112,0.2592298960498738
1263263,1263264,1263263,2526527,5426.370733737946,0.2588068958666554
1265265,1265266,1265265,2530531,5432.042713880539,0.2583852028456022
1267267,1267268,1267267,2534535,5437.793962955475,0.25796481095858326
1269269,1269270,1269269,2538539,5443.2271847724915,0.2575457142029336
1271271,1271272,1271271,2542543,5448.116353034973,0.2571279066178249
1273273,1273274,1273273,2546547,5452.830889940262,0.25671138228062773
1275275,1275276,1275275,2550551,5458.39186000824,0.25629613530145434
1277277,1277278,1277277,2554555,5464.297344923019,0.25588215982497786
1279279,1279280,1279279,2558559,5469.749102830887,0.25546945003588917
1281281,1281282,1281281,2562563,5475.112411975861,0.25505800015343993
1283283,1283284,1283283,2566567,5480.1780071258545,0.2546478044241667
1285285,1285286,1285285,2570571,5485.53879404068,0.25423885714371863
1287287,1287288,1287287,2574575,5490.779470920563,0.2538311526295729
1289289,1289290,1289289,2578579,5496.53626704216,0.25342468523922435
1291291,1291292,1291291,2582583,5501.119783878326,0.2530194493592717
1293293,1293294,1293293,2586587,5505.680660009384,0.25261543941451237
1295295,1295296,1295295,2590591,5510.27424788475,0.2522126498679427
1297297,1297298,1297297,2594595,5514.92941904068,0.2518110752043867
1299299,1299300,1299299,2598599,5519.602097988129,0.2514107099486864
1301301,1301302,1301301,2602603,5525.052471876144,0.25101154865660646
1303303,1303304,1303303,2606607,5530.554458856583,0.25061358592029137
1305305,1305306,1305305,2610611,5535.964621782303,0.2502168163518945
1307307,1307308,1307307,2614615,5542.371006011963,0.24982123461268202
1309309,1309310,1309309,2618619,5548.2586669921875,0.24942683538574784
1311311,1311312,1311311,2622623,5554.1238489151,0.24903361338692775
1313313,1313314,1313313,2626627,5559.052188873291,0.2486415633593424
1315315,1315316,1315315,2630631,5564.188989877701,0.24825068008431117
1317317,1317318,1317317,2634635,5569.606400966644,0.2478609583740763
1319319,1319320,1319319,2638639,5575.4299829006195,0.24747239306452684
1321321,1321322,1321321,2642643,5580.566390037537,0.2470849790279317
1323323,1323324,1323323,2646647,5586.241718053818,0.24669871116384456
1325325,1325326,1325325,2650651,5590.833034038544,0.24631358440274198
1327327,1327328,1327327,2654655,5595.787615060806,0.2459295937060233
1329329,1329330,1329329,2658659,5600.623514890671,0.2455467340623727
1331331,1331332,1331331,2662663,5605.950741052628,0.24516500048775924
1333333,1333334,1333333,2666667,5610.827143907547,0.2447843880381697
1335335,1335336,1335335,2670671,5615.685125827789,0.24440489178232383
1337337,1337338,1337337,2674675,5620.3902468681335,0.2440265068271401
1339339,1339340,1339339,2678679,5624.967035770416,0.24364922831045988
1341341,1341342,1341341,2682683,5629.560567855835,0.2432730513937713
1343343,1343344,1343343,2686687,5634.488076686859,0.24289797126402846
1345345,1345346,1345345,2690691,5639.639261960983,0.24252398314274615
1347347,1347348,1347347,2694695,5644.757818937302,0.2421510822732671
1349349,1349350,1349349,2698699,5649.486265897751,0.24177926392803784
1351351,1351352,1351351,2702703,5654.058301925659,0.24140852341224672
1353353,1353354,1353353,2706707,5659.435300827026,0.241038856049272
1355355,1355356,1355355,2710711,5664.890222787857,0.24067025719523372
1357357,1357358,1357357,2714715,5670.067280769348,0.2403027222280798
1359359,1359360,1359359,2718719,5674.716387748718,0.23993624656031898
1361361,1361362,1361361,2722723,5679.299602985382,0.23957082562264986
1363363,1363364,1363363,2726727,5683.9174427986145,0.2392064548748749
1365365,1365366,1365365,2730731,5688.498087882996,0.2388431298059004
1367367,1367368,1367367,2734735,5693.517944812775,0.23848084592464147
1369369,1369370,1369369,2738739,5698.4071209430695,0.23811959876729816
1371371,1371372,1371371,2742743,5703.138248920441,0.23775938389917428
1373373,1373374,1373373,2746747,5707.770149946213,0.23740019690376357
1375375,1375376,1375375,2750751,5712.396089792252,0.23704203339912056
1377377,1377378,1377377,2754755,5716.949668884277,0.23668488902148965
1379379,1379380,1379379,2758759,5721.529042959213,0.23632875942894316
1381381,1381382,1381381,2762763,5726.103996992111,0.23597364031411416
1383383,1383384,1383383,2766767,5730.792006969452,0.23561952738418768
1385385,1385386,1385385,2770771,5735.483191013336,0.23526641637363355
1387387,1387388,1387387,2774775,5740.106241703033,0.23491430304602545
1389389,1389390,1389389,2778779,5745.107842683792,0.23456318318130798
1391391,1391392,1391391,2782783,5750.598644018173,0.23421305258489156
1393393,1393394,1393393,2786787,5756.120817899704,0.23386390940868296
1395395,1395396,1395395,2790791,5762.277685880661,0.23351578891742975
1397397,1397398,1397397,2794795,5768.080096960068,0.2331686487668776
1399399,1399400,1399399,2798799,5774.113744974136,0.23282248175928544
1401401,1401402,1401401,2802803,5779.2142589092255,0.23247728362730413
1403403,1403404,1403403,2806807,5785.013068675995,0.2321330502636556
1405405,1405406,1405405,2810811,5790.609031915665,0.2317897776101745
1407407,1407408,1407407,2814815,5796.261479854584,0.23144746163779928
1409409,1409410,1409409,2818819,5802.047855854034,0.2311060983556672
1411411,1411412,1411411,2822823,5808.544107913971,0.2307656837929244
1413413,1413414,1413413,2826827,5814.755990028381,0.23042621400054486
1415415,1415416,1415415,2830831,5820.644172668457,0.23008768505860644
1417417,1417418,1417417,2834835,5826.975443840027,0.22975009306173888
1419419,1419420,1419419,2838839,5833.2618889808655,0.2294134341282188
1421421,1421422,1421421,2842843,5839.591372013092,0.22907770440360764
1423423,1423424,1423423,2846847,5846.025762796402,0.2287429000461998
1425425,1425426,1425425,2850851,5852.751660823822,0.22840901724521245
1427427,1427428,1427427,2854855,5858.934088945389,0.22807605220077676
1429429,1429430,1429429,2858859,5864.3177399635315,0.22774400114030868
1431431,1431432,1431431,2862863,5868.975678920746,0.2274128603094141
1433433,1433434,1433433,2866867,5874.006974935532,0.22708262597734574
1435435,1435436,1435435,2870871,5879.046786785126,0.22675329442790826
1437437,1437438,1437437,2874875,5885.342272043228,0.22642486197037215
1439439,1439440,1439439,2878879,5891.342223882675,0.2260973249340168
1441441,1441442,1441441,2882883,5897.284862041473,0.2257706796608545
1443443,1443444,1443443,2886887,5903.725106954575,0.22544492252200143
1445445,1445446,1445445,2890891,5908.689918041229,0.2251200499049446
1447447,1447448,1447447,2894895,5913.858527898788,0.22479605821354198
1449449,1449450,1449449,2898899,5918.988556861877,0.22447294387529837
1451451,1451452,1451451,2902903,5923.750787734985,0.22415070333408948
1453453,1453454,1453453,2906907,5928.554456710815,0.22382933305561892
1455455,1455456,1455455,2910911,5933.597282886505,0.22350882952014217
1457457,1457458,1457457,2914915,5938.735731840134,0.2231891892333806
1459459,1459460,1459459,2918919,5943.839911937714,0.2228704087137885
1461461,1461462,1461461,2922923,5949.7272210121155,0.222552484501648
1463463,1463464,1463463,2926927,5955.243183851242,0.22223541315361217
1465465,1465466,1465465,2930931,5961.148135900497,0.22191919124634296
1467467,1467468,1467467,2934935,5965.766874790192,0.22160381537833018
1469469,1469470,1469469,2938939,5970.735469818115,0.2212892821571586
1471471,1471472,1471471,2942943,5975.203907728195,0.22097558821405983
1473473,1473474,1473473,2946947,5979.687976837158,0.22066273020391236
1475475,1475476,1475475,2950951,5984.198615074158,0.22035070478523267
1477477,1477478,1477477,2954955,5989.016486883163,0.22003950864200306
1479479,1479480,1479479,2958959,5993.7781410217285,0.2197291384836717
1481481,1481482,1481481,2962963,5998.8136649131775,0.21941959102150577
1483483,1483484,1483483,2966967,6003.347090005875,0.21911086299769522
1485485,1485486,1485485,2970971,6007.939852714539,0.218802951161706
1487487,1487488,1487487,2974975,6013.395589828491,0.21849585228483193
1489489,1489490,1489489,2978979,6018.788200855255,0.21818956316019467
1491491,1491492,1491491,2982983,6023.925347805023,0.21788408058455389
1493493,1493494,1493493,2986987,6028.496406078339,0.21757940138195409
1495495,1495496,1495495,2990991,6033.377789974213,0.21727552239099168
1497497,1497498,1497497,2994995,6038.375821828842,0.216972440466634
1499499,1499500,1499499,2998999,6043.004897117615,0.21667015247840027
1501502,1501503,1501502,3003005,6047.592898845673,0.21636850491449877
1503504,1503505,1503504,3007009,6052.111756801605,0.21606779587091296
1505506,1505507,1505506,3011013,6057.069021940231,0.21576787147387222
1507508,1507509,1507508,3015017,6061.772212028503,0.2154687286601984
1509510,1509511,1509510,3019021,6066.331017971039,0.21517036437580828
1511512,1511513,1511512,3023025,6070.972116947174,0.2148727755939035
1513514,1513515,1513514,3027029,6076.17863202095,0.21457595929678064
1515516,1515517,1515516,3031033,6081.014851808548,0.21427991247765021
1517518,1517519,1517518,3035037,6085.804709911346,0.21398463215700758
1519520,1519521,1519520,3039041,6091.129111766815,0.21369011536444305
1521522,1521523,1521522,3043045,6096.239576816559,0.21339635913864186
1523524,1523525,1523524,3047049,6100.849698066711,0.21310336054375512
1525526,1525527,1525526,3051053,6105.727855920792,0.21281115536476136
1527528,1527529,1527528,3055057,6110.339494943619,0.21251973512516997
1529530,1529531,1529530,3059061,6114.8319680690765,0.21222907061383012
1531532,1531533,1531532,3063065,6119.85812997818,0.21193915371441108
1533534,1533535,1533534,3067069,6124.245937824249,0.21164998025415116
1535536,1535537,1535536,3071073,6128.7326118946075,0.21136154704072396
1537538,1537539,1537538,3075077,6133.24310874939,0.21107385115828947
1539540,1539541,1539540,3079081,6137.69180393219,0.2107868897546723
1541542,1541543,1541542,3083085,6142.107456922531,0.21050066002135281
1543544,1543545,1543544,3087089,6146.592581748962,0.21021515916436329
1545546,1545547,1545546,3091093,6151.070791959763,0.20993038440064993
1547548,1547549,1547548,3095097,6155.4467878341675,0.20964633297080582
1549550,1549551,1549550,3099101,6159.822592020035,0.209363002119062
1551552,1551553,1551552,3103105,6164.205864906311,0.20908038911693438
1553554,1553555,1553554,3107109,6168.862958908081,0.20879849123593885
1555556,1555557,1555556,3111113,6173.361418008804,0.20851730576941918
1557558,1557559,1557558,3115117,6177.808700799942,0.20823683002163307
1559560,1559561,1559560,3119121,6182.455990076065,0.20795706131139013
1561562,1561563,1561562,3123125,6186.936721801758,0.2076779969738709
1563564,1563565,1563564,3127129,6191.332417726517,0.20739963435335085
1565566,1565567,1565566,3131133,6195.7386469841,0.20712197080501937
1567568,1567569,1567568,3135137,6200.1335299015045,0.20684500370771275
1569570,1569571,1569570,3139141,6204.512003898621,0.20656873044026725
1571572,1571573,1571572,3143145,6208.9010617733,0.206293148405166
1573574,1573575,1573574,3147149,6213.3188490867615,0.20601825501216808
1575576,1575577,1575576,3151153,6217.705935955048,0.20574404768558452
1577578,1577579,1577578,3155157,6222.331023931503,0.20547052386245923
1579580,1579581,1579580,3159161,6226.708256959915,0.20519768099620705
1581582,1581583,1581582,3163165,6231.146019697189,0.2049255165438808
1583584,1583585,1583584,3167169,6235.574204921722,0.20465402798254217
1585586,1585587,1585586,3171173,6239.933876991272,0.2043832128001668
1587588,1587589,1587588,3175177,6244.352187871933,0.20411306849928224
1589590,1589591,1589590,3179181,6248.733810901642,0.203843592587873
1591592,1591593,1591592,3183185,6253.133549690247,0.20357478259211348
1593594,1593595,1593594,3187189,6257.593024015427,0.20330663605273003
1595596,1595597,1595596,3191193,6262.067286968231,0.20303915051226795
1597598,1597599,1597598,3195197,6266.4606828689575,0.20277232353691943
1599600,1599601,1599600,3199201,6270.8758227825165,0.2025061526983336
1601602,1601603,1601602,3203205,6275.241010904312,0.20224063557907357
1603604,1603605,1603604,3207209,6279.663468837738,0.20197576978171128
1605606,1605607,1605606,3211213,6284.081244945526,0.2017115529069997
1607608,1607609,1607608,3215217,6288.57399892807,0.2014479825811577
1609610,1609611,1609610,3219221,6292.966054916382,0.20118505643404205
1611612,1611613,1611612,3223225,6297.413215875626,0.2009227721100615
1613614,1613615,1613614,3227229,6301.828366756439,0.20066112726271967
1615616,1615617,1615616,3231233,6306.264003753662,0.2004001195582532
1617618,1617619,1617618,3235237,6310.661834001541,0.2001397466756316
1619620,1619621,1619620,3239241,6315.059362888336,0.19988000630473834
1621622,1621623,1621622,3243245,6319.500789880753,0.1996208961445518
1623624,1623625,1623624,3247249,6324.011469841003,0.19936241390314535
1625626,1625627,1625626,3251253,6328.446273088455,0.19910455730678223
1627628,1627629,1627628,3255257,6332.841107845306,0.19884732408718264
1629630,1629631,1629630,3259261,6337.235272884369,0.19859071199061873
1631632,1631633,1631632,3263265,6341.6473977565765,0.19833471877245756
1633634,1633635,1633634,3267269,6346.0207459926605,0.19807934219534218
1635636,1635637,1635636,3271273,6350.467463970184,0.19782458003646752
1637638,1637639,1637638,3275277,6354.8812890052795,0.19757043008758046
1639640,1639641,1639640,3279281,6359.302092075348,0.19731689014042786
1641642,1641643,1641642,3283285,6363.774348020554,0.19706395801222243
1643644,1643645,1643644,3287289,6368.186816930771,0.19681163151290093
1645646,1645647,1645646,3291293,6372.549284934998,0.19655990847786597
1647648,1647649,1647648,3295297,6376.951040029526,0.19630878674070118
1649650,1649651,1649650,3299301,6381.328193664551,0.19605826415863703
1651652,1651653,1651652,3303305,6385.712616920471,0.195808338590723
1653654,1653655,1653654,3307309,6390.135596036911,0.1955590079032845
1655656,1655657,1655656,3311313,6394.503906011581,0.19531026998265588
1657658,1657659,1657658,3315317,6398.900309085846,0.19506212271517143
1659660,1659661,1659660,3319321,6403.319543838501,0.19481456400171737
1661662,1661663,1661662,3323325,6407.85279583931,0.19456759175591287
1663664,1663665,1663664,3327329,6412.520545005798,0.19432120389683405
1665666,1665667,1665666,3331333,6417.124979019165,0.19407539835447096
1667668,1667669,1667668,3335337,6421.532407045364,0.1938301730715466
1669670,1669671,1669670,3339341,6425.928443908691,0.19358552599260292
1671672,1671673,1671672,3343345,6431.476413011551,0.1933414550821908
1673674,1673675,1673674,3347349,6436.547544717789,0.19309795830849907
1675676,1675677,1675676,3351353,6442.4235298633575,0.1928550336506305
1677678,1677679,1677678,3355357,6447.5134489536285,0.19261267909314483
1679680,1679681,1679680,3359361,6452.6167278289795,0.1923708926369727
1681682,1681683,1681682,3363365,6457.50807094574,0.19212967228850175
1683684,1683685,1683684,3367369,6462.4428169727325,0.1918890160632145
1685686,1685687,1685686,3371373,6467.304271936417,0.1916489219856885
1687688,1687689,1687688,3375377,6472.15213394165,0.19140938809505315
1689690,1689691,1689690,3379381,6478.3225219249725,0.19117041243043786
1691692,1691693,1691692,3383385,6484.694344997406,0.19093199304916197
1693694,1693695,1693694,3387389,6490.671014785767,0.1906941280085448
1695696,1695697,1695696,3391393,6496.091022729874,0.19045681538591452
1697698,1697699,1697698,3395397,6502.0760707855225,0.19022006432714988
1699700,1699701,1699700,3399401,6507.209232807159,0.18998387071223988
1701702,1701703,1701702,3403405,6512.601669788361,0.1897482247932203
1703704,1703705,1703704,3407409,6517.470152854919,0.18951312386889185
1705706,1705707,1705706,3411413,6522.207150936127,0.1892785659583751
1707708,1707709,1707708,3415417,6528.179767131805,0.18904454916992108
1709710,1709711,1709710,3419421,6533.5065269470215,0.18881107163724664
1711712,1711713,1711712,3423425,6538.619865894318,0.18857813149406866
1713714,1713715,1713714,3427429,6543.604341030121,0.18834572689411289
1715716,1715717,1715716,3431433,6548.598554849625,0.18811385599292407
1717718,1717719,1717718,3435437,6553.379396915436,0.18788251696059888
1719720,1719721,1719720,3439441,6558.547029018402,0.18765170796541497
1721722,1721723,1721722,3443445,6563.175659894943,0.1874214271974779
1723724,1723725,1723724,3447449,6567.8244659900665,0.18719167284325522
1725726,1725727,1725726,3451453,6572.363568782806,0.18696244310376642
1727728,1727729,1727728,3455457,6577.03283572197,0.18673373618912592
1729730,1729731,1729730,3459461,6581.619139909744,0.18650555031490512
1731732,1731733,1731732,3463465,6586.059822797775,0.18627788370395137
1733734,1733735,1733734,3467469,6591.695126056671,0.186050734586388
1735736,1735737,1735736,3471473,6597.147672891617,0.18582410120870918
1737738,1737739,1737738,3475477,6601.540307998657,0.1855979818119522
1739740,1739741,1739740,3479481,6605.95348572731,0.18537237466080114
1741742,1741743,1741742,3483485,6610.377541780472,0.18514727801266417
1743744,1743745,1743744,3487489,6615.01743888855,0.18492269014132034
1745746,1745747,1745746,3491493,6619.6053059101105,0.18469860932964366
1747748,1747749,1747748,3495497,6624.072289943695,0.18447503385868913
1749750,1749751,1749750,3499501,6628.444972038269,0.18425196203133964
1751752,1751753,1751752,3503505,6632.907791852951,0.1840293921468401
1753754,1753755,1753754,3507509,6637.503868818283,0.18380732251534937
1755756,1755757,1755756,3511513,6642.10107088089,0.18358575145612122
1757758,1757759,1757758,3515517,6646.578812837601,0.1833646772938664
1759760,1759761,1759760,3519521,6651.060322761536,0.18314409836239065
1761762,1761763,1761762,3523525,6655.505933761597,0.1829240130027756
1763764,1763765,1763764,3527529,6659.980808019638,0.1827044195633789
1765766,1765767,1765766,3531533,6664.448819875717,0.18248531639983412
1767768,1767769,1767768,3535537,6668.859917879105,0.1822667018732318
1769770,1769771,1769770,3539541,6673.23977971077,0.18204857435557642
1771772,1771773,1771772,3543545,6677.635067939758,0.18183093222432944
1773774,1773775,1773774,3547549,6682.004834890366,0.1816137738624093
1775776,1775777,1775776,3551553,6686.4007749557495,0.18139709766182932
1777778,1777779,1777778,3555557,6690.792168855667,0.18118090202369785
1779780,1779781,1779780,3559561,6695.18464589119,0.1809651853509422
1781782,1781783,1781782,3563565,6699.752811908722,0.18074994605922257
1783784,1783785,1783784,3567569,6704.285532951355,0.18053518256783718
1785786,1785787,1785786,3571573,6708.711842060089,0.1803208933051792
1787788,1787789,1787788,3575577,6713.136353969574,0.18010707669964177
1789790,1789791,1789790,3579581,6717.7407858371735,0.17989373120144592
1791792,1791793,1791792,3583585,6722.137866020203,0.17968085524989874
1793794,1793795,1793794,3587589,6726.572706699371,0.17946844730431621
1795796,1795797,1795796,3591593,6730.949846982956,0.17925650582219532
1797798,1797799,1797798,3595597,6735.328789949417,0.17904502927376598
1799800,1799801,1799800,3599601,6739.759479045868,0.17883401613835304
1801802,1801803,1801802,3603605,6744.1750910282135,0.1786234648898244
1803804,1803805,1803804,3607609,6748.515212059021,0.17841337402205681
1805806,1805807,1805806,3611613,6752.941475868225,0.1782037420252891
1807808,1807809,1807808,3615617,6757.328505754471,0.17799456740794994
1809810,1809811,1809810,3619621,6761.726157903671,0.1777858486675541
1811812,1811813,1811812,3623625,6766.087419986725,0.17757758432890114
1813814,1813815,1813814,3627629,6770.455399990082,0.17736977290405775
1815816,1815817,1815816,3631633,6774.878770828247,0.17716241292691848
1817818,1817819,1817818,3635637,6779.295504808426,0.17695550292773987
1819820,1819821,1819820,3639641,6783.671586751938,0.17674904144587344
1821822,1821823,1821822,3643645,6788.083201885223,0.17654302703158464
1823824,1823825,1823824,3647649,6792.514917850494,0.1763374582351389
1825826,1825827,1825826,3651653,6796.891375780106,0.17613233361225866
1827828,1827829,1827828,3655657,6801.241739988327,0.17592765173503722
1829830,1829831,1829830,3659661,6805.62225985527,0.17572341117011092
1831832,1831833,1831832,3663665,6809.991852045059,0.17551961049321108
1833834,1833835,1833834,3667669,6814.360536813736,0.1753162482909829
1835836,1835837,1835836,3671673,6818.762189865112,0.17511332315552863
1837838,1837839,1837838,3675677,6823.232143878937,0.17491083367713145
1839840,1839841,1839840,3679681,6827.644805908203,0.17470877846244548
1841842,1841843,1841842,3683685,6832.124967813492,0.17450715611448686
1843844,1843845,1843844,3687689,6837.024589776993,0.17430596525082365
1845846,1845847,1845846,3691693,6841.598299980164,0.1741052044890239
1847848,1847849,1847848,3695697,6846.078585863113,0.1739048724539316
1849850,1849851,1849850,3699701,6851.3495218753815,0.17370496777948574
1851852,1851853,1851852,3703705,6855.984461784363,0.17350548910144425
1853854,1853855,1853854,3707709,6860.851053714752,0.17330643506466004
1855856,1855857,1855856,3711713,6866.131582021713,0.17310780431580497
1857858,1857859,1857858,3715717,6871.142914772034,0.1729095955070079
1859860,1859861,1859860,3719721,6875.792916059494,0.17271180730494962
1861862,1861863,1861862,3723725,6880.874497652054,0.1725144383708539
1863864,1863865,1863864,3727729,6886.673879861832,0.17231748737685848
1865866,1865867,1865866,3731733,6891.133558034897,0.17212095300055807
1867868,1867869,1867868,3735737,6895.530143022537,0.17192483392682334
1869870,1869871,1869870,3739741,6900.00271987915,0.17172912884052494
1871872,1871873,1871872,3743745,6904.40402674675,0.17153383643926645
1873874,1873875,1873874,3747749,6908.8742089271545,0.17133895541883248
1875876,1875877,1875876,3751753,6913.285845041275,0.17114448448592157
1877878,1877879,1877878,3755757,6919.633762121201,0.1709504223526892
1879880,1879881,1879880,3759761,6928.348181009293,0.1707567677312909
1881882,1881883,1881882,3763765,6934.842335939407,0.17056351934479608
1883884,1883885,1883884,3767769,6939.889405012131,0.17037067591991217
1885886,1885887,1885886,3771773,6944.701292037964,0.1701782361851656
1887888,1887889,1887888,3775777,6950.125039815903,0.16998619888363464
1889890,1889891,1889890,3779781,6955.367079973221,0.1697945627529407
1891892,1891893,1891892,3783785,6960.580970048904,0.169603326545257
1893894,1893895,1893894,3787789,6965.927808046341,0.1694124890054809
1895896,1895897,1895896,3791793,6972.040957927704,0.16922204890215653
1897898,1897899,1897898,3795797,6977.9625589847565,0.16903200499109516
1899900,1899901,1899900,3799801,6982.59140586853,0.16884235604084097
1901902,1901903,1901902,3803805,6987.440189838409,0.16865310082903306
1903904,1903905,1903904,3807809,6992.618392705917,0.16846423813149158
1905906,1905907,1905906,3811813,6997.519407749176,0.16827576673131261
1907908,1907909,1907908,3815817,7002.885993003845,0.1680879560408357
1909910,1909911,1909910,3819821,7008.125239133835,0.16790073889569612
1911912,1911913,1911912,3823825,7014.502367973328,0.16771393165618065
1913914,1913915,1913914,3827829,7019.827627897263,0.16752751768217422
1915916,1915917,1915916,3831833,7024.659764051437,0.16734149122385134
1917918,1917919,1917918,3835837,7029.373505115509,0.16715584919620596
1919920,1919921,1919920,3839841,7034.784754991531,0.16697058960198774
1921922,1921923,1921922,3843845,7040.972080945969,0.16678571091324557
1923924,1923925,1923924,3847849,7047.324033737183,0.1666012118148501
1925926,1925927,1925926,3851853,7052.560672044754,0.16641709106625058
1927928,1927929,1927928,3855857,7058.868510961533,0.1662333474814659
1929930,1929931,1929930,3859861,7064.408024787903,0.16604997989634285
1931932,1931933,1931932,3863865,7069.954263687134,0.16586698714127124
1933934,1933935,1933934,3867869,7075.766191959381,0.16568436807574471
1935936,1935937,1935936,3871873,7081.740336894989,0.16550212155379995
1937938,1937939,1937938,3875877,7089.591381072998,0.16532024643674958
1939940,1939941,1939940,3879881,7096.938350915909,0.1651387415931822
1941942,1941943,1941942,3883885,7102.7548089027405,0.1649576058916864
1943944,1943945,1943944,3887889,7109.46373295784,0.1647768382099457
1945946,1945947,1945946,3891893,7115.765955924988,0.16459643743110064
1947948,1947949,1947948,3895897,7122.296474933624,0.1644164024401107
1949950,1949951,1949950,3899901,7129.6875948905945,0.16423673212739232
1951952,1951953,1951952,3903905,7136.325741767883,0.164057425383362
1953954,1953955,1953954,3907909,7141.586328744888,0.16387848111298808
1955956,1955957,1955956,3911913,7146.68771481514,0.16369989821942
1957958,1957959,1957958,3915917,7151.741986751556,0.16352167560944508
1959960,1959961,1959960,3919921,7156.924081802368,0.1633438121953077
1961962,1961963,1961962,3923925,7162.092285871506,0.16316630689470912
1963964,1963965,1963964,3927929,7167.352110862732,0.16298915863262664
1965966,1965967,1965966,3931933,7172.583300828934,0.16281236633221852
1967968,1967969,1967968,3935937,7178.253123760223,0.16263592892391898
1969970,1969971,1969970,3939941,7184.047181844711,0.16245984534361924
1971972,1971973,1971972,3943945,7190.673936843872,0.16228411452721048
1973974,1973975,1973974,3947949,7197.509047031403,0.16210873542331683
1975976,1975977,1975976,3951953,7203.211173772812,0.16193370697692444
1977978,1977979,1977978,3955957,7208.897807836533,0.1617590281402954
1979980,1979981,1979980,3959961,7214.114971876144,0.16158469786932983
1981982,1981983,1981982,3963965,7218.608076810837,0.16141071512356575
1983984,1983985,1983984,3967969,7223.11546087265,0.1612370788698172
1985986,1985987,1985986,3971973,7227.622876882553,0.1610637880730792
1987988,1987989,1987988,3975977,7232.08314704895,0.1608908417110797
1989990,1989991,1989990,3979981,7236.588862895966,0.1607182387560897
1991992,1991993,1991992,3983985,7241.0296268463135,0.16054597819129413
1993994,1993995,1993994,3987989,7245.438562870026,0.16037405900351587
1995996,1995997,1995996,3991993,7249.903501749039,0.16020248017775884
1997998,1997999,1997998,3995997,7254.350649833679,0.1600312407081219
2000000,2000001,2000000,4000001,7258.835234880447,0.15986033959961787


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002052783966064453,12064.44795143716
360,2490,2490,4980,3.3353936672210693,0.4583388177998131
721,5280,5280,10560,6.8332908153533936,0.31035213555878727
1081,8008,8008,16016,10.319485902786255,0.084708208543816
1441,10812,10812,21624,14.013197660446167,0.075534563688052
1802,13592,13592,27184,17.588513612747192,0.07000530239565705
2162,16390,16390,32780,21.251136541366577,0.06674257136910455
2522,19216,19216,38432,25.123957872390747,0.06501342345109151
2883,21988,21988,43976,28.911458730697632,0.042276417383618536
3243,24824,24824,49648,33.084638833999634,0.04189340341872594
3603,27640,27640,55280,36.932971715927124,0.03895886525060632
3964,30498,30498,60996,40.92040395736694,0.03852479658598895
4324,33332,33332,66664,44.85427665710449,0.036593014219761244
4684,36176,36176,72352,48.99788284301758,0.03639800104974711
5045,39004,39004,78008,53.31104588508606,0.03505098634377646
5405,41846,41846,83692,57.235915660858154,0.03422757205044036
5765,44694,44694,89388,61.188965797424316,0.033605409085794236
6125,47462,47462,94924,65.0127899646759,0.02106791718506429
6486,50328,50328,100656,68.98988962173462,0.02096373889435199
6846,53182,53182,106364,73.06409859657288,0.02072342238170677
7206,56010,56010,112020,76.96991276741028,0.016745869048463646
7567,58852,58852,117704,80.86206483840942,0.015371178300483734
7927,61708,61708,123416,84.80714964866638,0.015061802192576579
8287,64588,64588,129176,88.77300882339478,0.01506090143993788
8648,67460,67460,134920,92.78398895263672,0.015026678371214075
9008,70320,70320,140640,96.66565775871277,0.01495941970642889
9368,73184,73184,146368,100.69606971740723,0.014889309371937998
9729,76068,76068,152136,104.76848483085632,0.014882211386066047
10089,78932,78932,157864,108.74544477462769,0.01487767334401724
10449,81740,81740,163480,112.62320375442505,0.012236906235557399
10810,84608,84608,169216,116.68013882637024,0.01209875820131856
11170,87480,87480,174960,120.74181461334229,0.012095590962417191
11530,90346,90346,180692,124.70021986961365,0.012090483271094854
11891,93220,93220,186440,128.6783139705658,0.01206702594026865
12251,96082,96082,192164,132.74566173553467,0.011993510708634858
12611,98940,98940,197880,136.80996179580688,0.011832022402813891
12972,101782,101782,203564,140.87783670425415,0.009120136966885184
13332,104628,104628,209256,144.9932506084442,0.009104670496526523
13692,107496,107496,214992,149.18883085250854,0.009087816193641629
14053,110374,110374,220748,153.33507990837097,0.009061853392267949
14413,113240,113240,226480,157.36819195747375,0.009013164191856049
14773,116116,116116,232232,161.61079573631287,0.009005905843878281
15134,118998,118998,237996,165.74559879302979,0.008988955909444485
15494,121868,121868,243736,169.76634287834167,0.00897036396418116
15854,124740,124740,249480,173.85708856582642,0.00896236650805804
16215,127622,127622,255244,178.03062558174133,0.008816968862447538
16575,130498,130498,260996,182.09035682678223,0.008809027935058111
16935,133366,133366,266732,186.15984463691711,0.008682629058966995
17296,136238,136238,272476,190.36952757835388,0.008609743659690139
17656,139116,139116,278232,194.37928676605225,0.008608470227045473
18016,141988,141988,283976,198.51495671272278,0.008584949066062109
18376,144854,144854,289708,202.67348670959473,0.008553359422876383
18737,147734,147734,295468,206.71412682533264,0.008527686753950547
19097,150608,150608,301216,210.76261973381042,0.008524251115886727
19457,153486,153486,306972,214.86557960510254,0.008507006514264503
19818,156374,156374,312748,219.004953622818,0.008506609439791646
20178,159230,159230,318460,223.16551876068115,0.008488776265949127
20538,162092,162092,324184,227.187668800354,0.008461368299322203
20899,164934,164934,329868,231.21090078353882,0.006427179288948537
21259,167792,167792,335584,235.4808168411255,0.006412034876120742
21619,170656,170656,341312,239.5808026790619,0.006399188607247197
21980,173542,173542,347084,243.9259488582611,0.006394464737240924
22340,176418,176418,352836,248.09308886528015,0.006387159050063929
22700,179290,179290,358580,252.12749791145325,0.006381962242812733
23061,182174,182174,364348,256.106187582016,0.0063699157362862024
23421,185046,185046,370092,260.2386736869812,0.006355530191285652
23781,187916,187916,375832,264.2830798625946,0.006208932549270685
24142,190792,190792,381584,268.222553730011,0.006097746154409833
24502,193652,193652,387304,272.289963722229,0.006023392013958073
24862,196528,196528,393056,276.2908058166504,0.006016313802319928
25223,199410,199410,398820,280.23147678375244,0.006008175267197657
25583,202288,202288,404576,284.27365279197693,0.0060071994939789874
25943,205160,205160,410320,288.2586245536804,0.0059793454074679175
26304,208044,208044,416088,292.3207778930664,0.005972126915366971
26664,210922,210922,421844,296.28816175460815,0.005969061607174808
27024,213800,213800,427600,300.35339856147766,0.005967906687146751
27385,216684,216684,433368,304.5117027759552,0.005956985676675686
27745,219548,219548,439096,308.47636580467224,0.005869015360076446
28105,222420,222420,444840,312.477041721344,0.0058457958220969886
28466,225306,225306,450612,316.56445956230164,0.005844947505465825
28826,228176,228176,456352,320.5863926410675,0.005832664604895399
29186,231052,231052,462104,324.69407892227173,0.005813408077301574
29547,233938,233938,467876,328.8415606021881,0.0058091604896617355
29907,236816,236816,473632,332.8843057155609,0.005807076180644799
30267,239690,239690,479380,336.9142436981201,0.005798968237286317
30627,242570,242570,485140,341.02860283851624,0.005798699405204388
30988,245454,245454,490908,345.1152517795563,0.005793268486740999
31348,248328,248328,496656,349.2731728553772,0.005775922127213562
31708,251204,251204,502408,353.36934185028076,0.005772443004389061
32069,254090,254090,508180,357.38579177856445,0.005766655089246342
32429,256964,256964,513928,361.40272879600525,0.005758415076343226
32789,259830,259830,519660,365.55172300338745,0.0053337458721216535
33150,262716,262716,525432,369.6553888320923,0.005330852565748501
33510,265592,265592,531184,373.763623714447,0.005324668083630968
33870,268470,268470,536940,377.9181807041168,0.005322854412952438
34231,271348,271348,542696,381.8716707229614,0.005285292701955768
34591,274224,274224,548448,385.91061186790466,0.005281117644699407
34951,277084,277084,554168,389.9327266216278,0.004602130144121475
35312,279968,279968,559936,393.9751806259155,0.0045990878588781925
35672,282846,282846,565692,398.1381776332855,0.004597971070325002
36032,285722,285722,571444,402.15420269966125,0.0045806038160662865
36393,288608,288608,577216,406.1867399215698,0.004578413176204776
36753,291486,291486,582972,410.2378816604614,0.004575917868351098
37113,294360,294360,588720,414.34069561958313,0.004531525901256828
37474,297248,297248,594496,418.4928078651428,0.004531292368483264
37834,300124,300124,600248,422.62343764305115,0.00452272832262679
38194,302998,302998,605996,426.5814719200134,0.004499914288317086
38555,305886,305886,611772,430.6800436973572,0.004499681523157051
38915,308758,308758,617516,434.850882768631,0.004487060690735234
39275,311636,311636,623272,438.8841679096222,0.004480711017095018
39636,314522,314522,629044,443.10919189453125,0.00447958900622325
39996,317400,317400,634800,447.3195598125458,0.004474376251891954
40356,320280,320280,640560,451.3234717845917,0.004474144705454819
40717,323146,323146,646292,455.36489272117615,0.004464152705622837
41077,326022,326022,652044,459.4878237247467,0.0044607604595512385
41437,328898,328898,657796,463.54856181144714,0.004457288476260146
41798,331776,331776,663552,467.6924488544464,0.004441116701855208
42158,334644,334644,669288,471.8770658969879,0.004402272257721052
42518,337520,337520,675040,475.91535472869873,0.004397147202325868
42878,340398,340398,680796,480.0683755874634,0.004395147932882537
43239,343284,343284,686568,484.1691966056824,0.004384983665659092
43599,346160,346160,692320,488.1107656955719,0.004381034268590156
43959,349040,349040,698080,492.12537384033203,0.004380821161248605
44320,351924,351924,703848,496.2549297809601,0.004376170481918962
44680,354794,354794,709588,500.3214998245239,0.004132255719014211
45040,357672,357672,715344,504.2895197868347,0.004131050740397768
45401,360554,360554,721108,508.3818476200104,0.004113830007554498
45761,363426,363426,726852,512.4446818828583,0.004075867875144468
46121,366300,366300,732600,516.4898936748505,0.004010892816950218
46482,369186,369186,738372,520.7574617862701,0.004006257884611841
46842,372062,372062,744124,524.750706911087,0.004003319874755107
47202,374936,374936,749872,528.7624537944794,0.003982096906838706
47563,377824,377824,755648,532.8949267864227,0.003981893609307008
47923,380700,380700,761400,536.9890098571777,0.003976790578235523
48283,383576,383576,767152,540.9299228191376,0.003965028043239727
48644,386464,386464,772928,545.0166988372803,0.00396482520045538
49004,389338,389338,778676,549.0717198848724,0.00395472758282267
49364,392214,392214,784428,553.2202968597412,0.0039448465322493576
49725,395102,395102,790204,557.4690697193146,0.003944644195144065
50085,397980,397980,795960,561.5275738239288,0.0039409578166669235
50445,400856,400856,801712,565.5206699371338,0.003926970222892123
50806,403742,403742,807484,569.5925557613373,0.003926134380890289
51166,406620,406620,813240,573.685144662857,0.003922709342077724
51526,409498,409498,818996,577.6863358020782,0.003916148658390739
51887,412386,412386,824772,581.6201527118683,0.003915947027053335
52247,415262,415262,830524,585.6673467159271,0.0039041849104251014
52607,418140,418140,836280,589.7348258495331,0.0038991129586065654
52968,421026,421026,842052,593.8865888118744,0.003897436732586357
53328,423904,423904,847808,598.0542478561401,0.003894548686730559
53688,426782,426782,853564,602.1762449741364,0.0038927511468500597
54048,429662,429662,859324,606.1676378250122,0.0038925506505620433
54409,432534,432534,865068,610.2281057834625,0.003414816874283133
54769,435412,435412,870824,614.2493648529053,0.0034128114821214695
55129,438288,438288,876576,618.302916765213,0.003410123666981235
55490,441174,441174,882348,622.3793489933014,0.0034085990064340876
55850,444052,444052,888104,626.4387776851654,0.003405427987672738
56210,446932,446932,893864,630.4185826778412,0.0034052387709380127
56571,449820,449820,899640,634.4527056217194,0.003405049032153329
56931,452700,452700,905400,638.5189027786255,0.0034048598263325403
57291,455580,455580,911160,642.4950368404388,0.0034046706205117516
57652,458468,458468,916936,646.5817227363586,0.0034044809617626015
58012,461324,461324,922648,650.6146628856659,0.0034009343908110168
58372,464202,464202,928404,654.6489567756653,0.00339376753072429
58733,467088,467088,934176,658.7596297264099,0.003392539905689773
59093,469966,469966,939932,662.7940275669098,0.003389185709238518
59453,472838,472838,945676,666.8695726394653,0.003357433315613889
59814,475724,475724,951448,671.028874874115,0.0033570766827324405
60174,478602,478602,957204,674.9857678413391,0.00335170047947031
60534,481482,481482,962964,679.0052528381348,0.0033515407722006785
60895,484368,484368,968736,683.0636117458344,0.003349256474393769
61255,487248,487248,974496,687.0662908554077,0.003349096839883714
61615,490126,490126,980252,691.0877659320831,0.0033449243874201784
61976,493010,493010,986020,695.1397969722748,0.003342034598972532
62336,495890,495890,991780,699.2062315940857,0.0033418751427234383
62696,498768,498768,997536,703.2705538272858,0.0033385187034582486
63057,501656,501656,1003312,707.2679796218872,0.003338358887049253
63417,504532,504532,1009064,711.4207878112793,0.0033369388547725976
63777,507388,507388,1014776,715.4386458396912,0.0026911954664683435
64138,510274,510274,1020548,719.455308675766,0.0026893833546637325
64498,513150,513150,1026300,723.5859487056732,0.002686730842469842
64858,516028,516028,1032056,727.6045339107513,0.0026819470385817112
65219,518916,518916,1037832,731.6121258735657,0.0026818020924110897
65579,521796,521796,1043592,735.7511277198792,0.002681657555513084
65939,524672,524672,1049344,739.904632806778,0.002675767007531249
66299,527550,527550,1055100,743.9543647766113,0.0026742113986983895
66660,530438,530438,1060876,748.0455837249756,0.002674066650797613
67020,533316,533316,1066632,752.2100417613983,0.002670618996489793
67380,536196,536196,1072392,756.3145868778229,0.002670474723345251
67741,539080,539080,1078160,760.3623096942902,0.0026660581643227488
68101,541958,541958,1083916,764.4918527603149,0.0026606294286466436
68461,544836,544836,1089672,768.5904886722565,0.002658502135091112
68822,547724,547724,1095448,772.6416757106781,0.0026583577073324705
69182,550602,550602,1101204,776.746396780014,0.0026565437110548373
69542,553480,553480,1106960,780.9229388237,0.002655607224369305
69903,556362,556362,1112724,784.9986958503723,0.0026019391589215957
70263,559240,559240,1118480,789.030131816864,0.002598473241960164
70623,562120,562120,1124240,793.1079947948456,0.002598330380351399
70984,565004,565004,1130008,797.2102167606354,0.0025949201026378432
71344,567882,567882,1135764,801.3298716545105,0.0025836730455921497
71704,570758,570758,1141516,805.2889997959137,0.002582971357696806
72065,573642,573642,1147284,809.3860218524933,0.002570169826867641
72425,576518,576518,1153036,813.4822568893433,0.002566636232586461
72785,579398,579398,1158796,817.6243007183075,0.0025664939894340932
73146,582280,582280,1164560,821.800274848938,0.002526628524719854
73506,585158,585158,1170316,825.9656608104706,0.0025258072037104284
73866,588038,588038,1176076,830.1046888828278,0.002525665719076642
74227,590922,590922,1181844,834.3835499286652,0.0025197915856551845
74587,593800,593800,1187600,838.4888668060303,0.00251829375338275
74947,596678,596678,1193356,842.6165859699249,0.0025139975787169533
75308,599562,599562,1199124,846.6492428779602,0.0025063898665393936
75668,602440,602440,1204880,850.5570785999298,0.002504969959773007
76028,605318,605318,1210636,854.5579497814178,0.0025043783007276943
76389,608204,608204,1216408,858.5424077510834,0.0025017317802848993
76749,611084,611084,1222168,862.6046998500824,0.002501590739484527
77109,613960,613960,1227920,866.8267426490784,0.0024980243269965285
77470,616846,616846,1233692,870.8194527626038,0.002494614185707178
77830,619724,619724,1239448,874.7776277065277,0.0024934723078331444
78190,622602,622602,1245204,878.8084359169006,0.0024921989133872557
78550,625480,625480,1250960,882.8658995628357,0.0024883495534595568
78911,628366,628366,1256732,886.8664667606354,0.0024859102613845607
79271,631242,631242,1262484,890.8581387996674,0.002482669673554483
79631,634116,634116,1268232,895.1170587539673,0.0024612405177322216
79992,637002,637002,1274004,899.178201675415,0.0024592006138846045
80352,639882,639882,1279764,903.239284992218,0.0024590603443357395
80712,642758,642758,1285516,907.262987613678,0.002453694058203837
81073,645646,645646,1291292,911.2256577014923,0.0024535534848837415
81433,648522,648522,1297044,915.2235708236694,0.002447731034408207
81793,651402,651402,1302804,919.2176089286804,0.0024475909704051446
82154,654284,654284,1308568,923.1146328449249,0.002442342289214139
82514,657162,657162,1314324,927.0625128746033,0.002441210353936185
82874,660038,660038,1320076,931.054381608963,0.0024355015866603935
83235,662924,662924,1325848,935.0053586959839,0.002433891964756185
83595,665804,665804,1331608,938.9870536327362,0.0024337521572306287
83955,668682,668682,1337364,943.004264831543,0.0024305080260091927
84316,671568,671568,1343136,946.9801347255707,0.002429659596600686
84676,674446,674446,1348892,950.9459898471832,0.0024274485167552484
85036,677324,677324,1354648,955.0038678646088,0.0024231885272456566
85397,680210,680210,1360420,959.0314376354218,0.002422560781269567
85757,683088,683088,1366176,962.9594886302948,0.0024108089892251883
86117,685968,685968,1371936,966.9540228843689,0.002410669580058311
86478,688854,688854,1377708,971.0747518539429,0.0024088814188871766
86838,691732,691732,1383464,975.0277309417725,0.002407491807389306
87198,694612,694612,1389224,979.019428730011,0.0024073524728009943
87559,697496,697496,1394992,983.049195766449,0.002387289598118514
87919,700374,700374,1400748,986.9622666835785,0.0023860242108639795
88279,703252,703252,1406504,990.9804468154907,0.002384664705459727
88640,706138,706138,1412276,995.0871276855469,0.0023801713086868403
89000,709018,709018,1418036,999.1443247795105,0.002380032452492742
89360,711896,711896,1423792,1003.2563388347626,0.0023753740952088265
89721,714782,714782,1429564,1007.2537887096405,0.002372833580011502
90081,717660,717660,1435320,1011.2365758419037,0.0023712936435913434
90441,720538,720538,1441076,1015.354095697403,0.0023707389354967745
90801,723416,723416,1446832,1019.2862956523895,0.0023694472529314226
91162,726296,726296,1452592,1023.3313097953796,0.0022110275822342373
91522,729176,729176,1458352,1027.348112821579,0.002210891643699142
91882,732054,732054,1464108,1031.3568568229675,0.0022045213991077617
92243,734942,734942,1469884,1035.2881295681,0.0022043851640773937
92603,737820,737820,1475640,1039.3002407550812,0.002203261477916385
92963,740700,740700,1481400,1043.315388917923,0.0022031256739865057
93324,743586,743586,1487172,1047.2348380088806,0.0022021557688276516
93684,746462,746462,1492924,1051.2478725910187,0.002188822154494119
94044,749342,749342,1498684,1055.2732226848602,0.002188686577937915
94405,752228,752228,1504456,1059.5195965766907,0.0021874364701943705
94765,755106,755106,1510212,1063.4574909210205,0.0021812454651808366
95125,757986,757986,1515972,1067.4221827983856,0.0021811099904880393
95486,760872,760872,1521744,1071.4980607032776,0.0021783564043289516
95846,763750,763750,1527500,1075.530134677887,0.002177891321480274
96206,766628,766628,1533256,1079.5382537841797,0.002173863904317841
96567,769516,769516,1539032,1083.6357429027557,0.002173728205889347
96927,772394,772394,1544788,1087.7629268169403,0.002168460794564453
97287,775272,775272,1550544,1091.8990626335144,0.002167176751754596
97648,778148,778148,1556296,1095.8861849308014,0.0018803617094818037
98008,781018,781018,1562036,1099.878318786621,0.0018798621549649397
98368,783896,783896,1567792,1103.908813714981,0.0018790987323882291
98729,786782,786782,1573564,1107.9643766880035,0.0018767761248454917
99089,789662,789662,1579324,1112.0939917564392,0.0018766454904834973
99449,792538,792538,1585076,1116.2387146949768,0.0018751689785858616
99810,795422,795422,1590844,1120.3134138584137,0.0018699975898925913
100170,798298,798298,1596596,1124.3440928459167,0.001860456741269445
100530,801178,801178,1602356,1128.4043507575989,0.0018603263542900095
100891,804062,804062,1608124,1132.5588088035583,0.001855630967838806
101251,806940,806940,1613880,1136.5131478309631,0.0018538937238190556
101611,809818,809818,1619636,1140.56995677948,0.0018524292863730807
101972,812704,812704,1625408,1144.7227597236633,0.001848921894634259
102332,815582,815582,1631164,1148.7310168743134,0.0018487552370061167
102692,818462,818462,1636924,1152.735800743103,0.0018486250264686532
103052,821340,821340,1642680,1156.7565257549286,0.001845391536335228
103413,824228,824228,1648456,1160.7257068157196,0.0018452610111125978
103773,827108,827108,1654216,1164.6551659107208,0.001845130853325827
104133,829988,829988,1659976,1168.6856718063354,0.0018450006973580457
104494,832876,832876,1665752,1172.662666797638,0.0018448701812303625
104854,835756,835756,1671512,1176.591736793518,0.0018447400270815706
105214,838636,838636,1677272,1180.6508688926697,0.0018446098783897469
105575,841524,841524,1683048,1184.7020127773285,0.0018444793677190319
105935,844404,844404,1688808,1188.6280629634857,0.0018443492208461976
106295,847284,847284,1694568,1192.5813319683075,0.001844219077611342
106656,850172,850172,1700344,1196.8208618164062,0.0018440885705786059
107016,852990,852990,1705980,1200.8661468029022,0.0018336224602535367
107376,855860,855860,1711720,1204.798770904541,0.001831862862673006
107737,858740,858740,1717480,1208.8066718578339,0.0018247201078338549
108097,861610,861610,1723220,1212.9002668857574,0.0018188319209002657
108457,864488,864488,1728976,1216.8332617282867,0.0018173775533796288
108818,867346,867346,1734692,1220.8389329910278,0.0016767214438004885
109178,870222,870222,1740444,1224.8504047393799,0.0016751186158217024
109538,873098,873098,1746196,1228.8806986808777,0.0016749873975641094
109899,875972,875972,1751944,1232.9422497749329,0.0016737355563236633
110259,878844,878844,1757688,1237.1623549461365,0.0016698318031558301
110619,881718,881718,1763436,1241.2732815742493,0.0016671604207658675
110980,884606,884606,1769212,1245.3118867874146,0.0016670816658006515
111340,887484,887484,1774968,1249.3188407421112,0.0016663639580656309
111700,890360,890360,1780720,1253.4353857040405,0.0016641367055854062
112061,893244,893244,1786488,1257.4265348911285,0.0016634208241157467
112421,896108,896108,1792216,1261.3941869735718,0.0016137878574227216
112781,898984,898984,1797968,1265.4555327892303,0.001609892720807693
113142,901870,901870,1803740,1269.5256378650665,0.0016089994041976752
113502,904744,904744,1809488,1273.6419398784637,0.0016052439586928813
113862,907620,907620,1815240,1277.6200377941132,0.001603634995262837
114222,910494,910494,1820988,1281.6604647636414,0.0016025372060539667
114583,913376,913376,1826752,1285.7491688728333,0.0016002713200578
114943,916250,916250,1832500,1289.8556337356567,0.00159216038264276
115303,919124,919124,1838248,1293.7953147888184,0.0015859757368161809
115664,922010,922010,1844020,1297.8203446865082,0.0015854956272960408
116024,924886,924886,1849772,1301.8403508663177,0.0015813266836630646
116384,927764,927764,1855528,1305.8795099258423,0.0015811016037332593
116745,930650,930650,1861300,1309.809782743454,0.001577561124577187
117105,933524,933524,1867048,1313.7968208789825,0.001575492715346627
117465,936400,936400,1872800,1317.8110988140106,0.0015726842375443084
117826,939282,939282,1878564,1321.756740808487,0.00156996477926441
118186,942158,942158,1884316,1325.8068268299103,0.0015689387400925625
118546,945032,945032,1890064,1329.7917618751526,0.0015649931356165325
118907,947916,947916,1895832,1333.7985427379608,0.0015636085572623415
119267,950796,950796,1901592,1337.8338649272919,0.0015635329018550692
119627,953672,953672,1907344,1341.8773567676544,0.0015616484452039003
119988,956558,956558,1913116,1345.8775129318237,0.001560672197228996
120348,959438,959438,1918876,1349.9666516780853,0.0015605966254952364
120708,962318,962318,1924636,1354.2104687690735,0.001560521055580466
121069,965206,965206,1930412,1358.2521197795868,0.0015604452764819143
121429,968086,968086,1936172,1362.2928187847137,0.0015603697102051228
121789,970966,970966,1941932,1366.3357276916504,0.0015602941475663101
122150,973854,973854,1947708,1370.3754317760468,0.0015602183739247266
122510,976734,976734,1953468,1374.5100858211517,0.0015601428149238927
122870,979614,979614,1959228,1378.613811969757,0.0015600672559230588
123231,982502,982502,1965004,1382.8619756698608,0.0015599914913764223
123591,985382,985382,1970764,1386.9857556819916,0.0015599159378325567
123951,988262,988262,1976524,1391.014791727066,0.001559840384288691
124312,991150,991150,1982300,1395.0258848667145,0.0015597646251990227
124672,994030,994030,1988060,1399.0665159225464,0.0015596890771121252
125032,996910,996910,1993820,1403.0466239452362,0.0015596135308442172
125393,999798,999798,1999596,1407.0829648971558,0.0015595377753925277
125753,1002678,1002678,2005356,1411.1723308563232,0.0015594622345815878
126113,1005554,1005554,2011108,1415.1755237579346,0.0015571375479339622
126473,1008416,1008416,2016832,1419.0643298625946,0.001550882088849903
126834,1011300,1011300,2022600,1423.0176796913147,0.0015496883097512182
127194,1014170,1014170,2028340,1426.9891138076782,0.0015384055695903953
127554,1017048,1017048,2034096,1430.897118806839,0.0015377621093648486
127915,1019934,1019934,2039868,1434.8423907756805,0.0015362127578555373
128275,1022804,1022804,2045608,1438.8513488769531,0.0015321468345064204
128635,1025682,1025682,2051364,1442.9894227981567,0.0015318603873311076
128996,1028562,1028562,2057124,1447.009332895279,0.0015283634147635894
129356,1031430,1031430,2062860,1450.9699356555939,0.0015203038419713266
129716,1034306,1034306,2068612,1454.974514722824,0.001519528897915734
130077,1037190,1037190,2074380,1459.0992939472198,0.001518280460004462
130437,1040066,1040066,2080132,1463.0643198490143,0.0015156247427512426
130797,1042944,1042944,2085888,1467.0698266029358,0.0015150246981647797
131158,1045828,1045828,2091656,1471.1828668117523,0.0015130550109461183
131518,1048706,1048706,2097412,1475.2054116725922,0.0015120673524506856
131878,1051584,1051584,2103168,1479.1512308120728,0.001511092166765593
132239,1054446,1054446,2108892,1483.3795137405396,0.0002813263163261581
132599,1057322,1057322,2114644,1487.4343066215515,0.0002810723690345185
132959,1060202,1060202,2120404,1491.49653673172,0.0002810307614709018
133320,1063090,1063090,2126180,1495.6846487522125,0.00028098903749196324
133680,1065970,1065970,2131940,1499.8129577636719,0.00028094743174733594
134040,1068850,1068850,2137700,1503.9717757701874,0.00028090582964068744
134401,1071738,1071738,2143476,1508.0281698703766,0.0002808641111187171
134761,1074618,1074618,2149236,1512.1066718101501,0.000280822510831058
135121,1077386,1077386,2154772,1516.2314977645874,0.0002785170800052583
135482,1080268,1080268,2160536,1520.2348017692566,0.00027830168801301625
135842,1083140,1083140,2166280,1524.2069098949432,0.00027807996957562864
136202,1086018,1086018,2172036,1528.2301478385925,0.00027784229860117193
136563,1088896,1088896,2177792,1532.212671995163,0.0002770501778286416
136923,1091746,1091746,2183492,1536.2887697219849,0.0002668294710019836
137283,1094620,1094620,2189240,1540.337884902954,0.0002666221062099794
137644,1097500,1097500,2195000,1544.255474805832,0.0002663766990735894
138004,1100374,1100374,2200748,1548.3228137493134,0.0002660690042830538
138364,1103246,1103246,2206492,1552.554027557373,0.00026419975256430916
138724,1106116,1106116,2212232,1556.7284607887268,0.00026327379055146594
139085,1108964,1108964,2217928,1560.7137558460236,0.00010899851804424543
139445,1111782,1111782,2223564,1564.7729978561401,0.00010844979260582477
139805,1114640,1114640,2229280,1568.7258577346802,0.00010793309593282174
140166,1117514,1117514,2235028,1572.6891419887543,0.00010715404278016649
140526,1120390,1120390,2240780,1576.901516675949,0.00010702284998842515
140886,1123268,1123268,2246536,1580.9353559017181,0.00010694200864236336
141247,1126152,1126152,2252304,1584.9160528182983,0.00010688125075830612
141607,1129026,1129026,2258052,1588.8693985939026,0.0001065200394805288
141967,1131904,1131904,2263808,1592.8669328689575,0.00010629459393385332
142328,1134786,1134786,2269572,1596.76508975029,0.00010619000386213884
142688,1137656,1137656,2275312,1600.6639957427979,0.00010497380208107643
143048,1140534,1140534,2281068,1604.5668306350708,0.00010493063746253029
143409,1143418,1143418,2286836,1608.4658596515656,0.00010475033923285082
143769,1146292,1146292,2292584,1612.3682239055634,0.00010461359124747105
144129,1149172,1149172,2298344,1616.3403327465057,0.0001046069974108832
144490,1152060,1152060,2304120,1620.4391658306122,0.0001046003817464225
144850,1154940,1154940,2309880,1624.589323759079,0.00010459378427185584
145210,1157820,1157820,2315640,1628.5630836486816,0.00010458718861627858
145571,1160616,1160616,2321232,1632.4521605968475,0.00010397378537163604
145931,1163428,1163428,2326856,1636.4229328632355,0.00010239637776976451
146291,1166276,1166276,2332552,1640.3980107307434,0.00010175865645578597
146652,1169114,1169114,2338228,1644.2932579517365,0.00010034730985353235
147012,1171978,1171978,2343956,1648.3045797348022,0.00010020252739195712
147372,1174700,1174700,2349400,1652.166919708252,3.189343260601163e-07
147733,1177496,1177496,2354992,1656.0235269069672,3.164386725984514e-07
148093,1180358,1180358,2360716,1660.0092039108276,3.158020263072103e-07
148453,1183222,1183222,2366444,1664.0204167366028,3.1491435947827995e-07
148814,1186090,1186090,2372180,1667.9807176589966,3.1226772989612073e-07
149174,1188962,1188962,2377924,1671.8995189666748,3.1204217521008104e-07
149534,1191838,1191838,2383676,1675.918999671936,3.113109414698556e-07
149895,1194720,1194720,2389440,1679.953192949295,3.1120907806325704e-07
150255,1197592,1197592,2395184,1683.9032068252563,3.1020681490190327e-07
150615,1200470,1200470,2400940,1687.906789779663,3.0999945010989904e-07
150975,1203346,1203346,2406692,1692.1361169815063,3.0992850952316076e-07
151336,1206226,1206226,2412452,1696.2200796604156,3.0919909477233887e-07
151696,1209100,1209100,2418200,1700.137199640274,3.081659087911248e-07
152056,1211968,1211968,2423936,1704.2561717033386,3.080094757024199e-07
152417,1214848,1214848,2429696,1708.2578887939453,3.0774572223890573e-07
152777,1217726,1217726,2435452,1712.2245078086853,3.077129804296419e-07
153137,1220592,1220592,2441184,1716.2640867233276,3.051736712222919e-07
153498,1223478,1223478,2446956,1720.3045806884766,3.0513183446601033e-07
153858,1226346,1226346,2452692,1724.2160766124725,2.9805232770740986e-07
154218,1229214,1229214,2458428,1728.1309587955475,2.977558324346319e-07
154579,1232100,1232100,2464200,1732.2622096538544,2.9771399567835033e-07
154939,1234972,1234972,2469944,1736.249434709549,2.956694515887648e-07
155299,1237838,1237838,2475676,1740.1697657108307,2.9542934498749673e-07
155660,1240722,1240722,2481444,1744.251339673996,2.9533111955970526e-07
156020,1243596,1243596,2487192,1748.2612385749817,2.9524017008952796e-07
156380,1246466,1246466,2492932,1752.2772998809814,2.929773472715169e-07
156741,1249354,1249354,2498708,1756.2538278102875,2.929646143456921e-07
157101,1252232,1252232,2504464,1760.2129187583923,2.929136826423928e-07
157461,1255104,1255104,2510208,1764.2505469322205,2.9182047001086175e-07
157822,1257984,1257984,2515968,1768.2101256847382,2.917022356996313e-07
158182,1260860,1260860,2521720,1772.2117757797241,2.916403900599107e-07
158542,1263724,1263724,2527448,1776.1649918556213,2.914021024480462e-07
158903,1266604,1266604,2533208,1780.0744347572327,2.911601768573746e-07
159263,1269472,1269472,2538944,1784.0681076049805,2.2676613298244774e-07
159623,1272292,1272292,2544584,1788.0840456485748,2.6697307475842535e-08
159984,1275148,1275148,2550296,1792.1952848434448,2.6358975446783006e-08
160344,1277962,1277962,2555924,1796.324461698532,2.4507244233973324e-08
160704,1280836,1280836,2561672,1800.5232865810394,2.448723535053432e-08
161065,1283722,1283722,2567444,1804.7920336723328,2.4489054339937866e-08
161425,1286600,1286600,2573200,1808.8175837993622,2.4476321414113045e-08
161785,1289478,1289478,2578956,1812.8380358219147,2.4472683435305953e-08
162145,1292356,1292356,2584712,1816.9946947097778,2.4470864445902407e-08
162506,1295242,1295242,2590484,1821.0498926639557,2.4461769498884678e-08
162866,1298120,1298120,2596240,1825.256918668747,2.4445398594252765e-08
163226,1301000,1301000,2602000,1829.4251098632812,2.4445398594252765e-08
163587,1303884,1303884,2607768,1833.4539709091187,2.4407199816778302e-08
163947,1306762,1306762,2613524,1837.486498594284,2.436900103930384e-08
164307,1309642,1309642,2619284,1841.5835168361664,2.4367182049900293e-08
164668,1312528,1312528,2625056,1845.6258778572083,2.43635440710932e-08
165028,1315408,1315408,2630816,1849.6446409225464,2.4361725081689656e-08
165388,1318286,1318286,2636572,1853.6510179042816,2.4348992155864835e-08
165749,1321174,1321174,2642348,1857.7902138233185,2.435081114526838e-08
166109,1324052,1324052,2648104,1861.833863735199,2.4327164283022285e-08
166469,1326930,1326930,2653860,1865.8398067951202,2.4318069336004555e-08
166830,1329818,1329818,2659636,1869.7734367847443,2.43198883254081e-08
167190,1332692,1332692,2665384,1873.7514407634735,2.4261680664494634e-08
167550,1335570,1335570,2671140,1877.752713918686,2.4228938855230808e-08
167911,1338458,1338458,2676916,1881.6627316474915,2.4227119865827262e-08
168271,1341336,1341336,2682672,1885.5600218772888,2.4225300876423717e-08
168631,1344216,1344216,2688432,1889.502837896347,2.4227119865827262e-08
168992,1347102,1347102,2694204,1893.502460718155,2.421984390821308e-08
169352,1349980,1349980,2699960,1897.5147547721863,2.4172550183720887e-08
169712,1352858,1352858,2705716,1901.4538958072662,2.417073119431734e-08
170073,1355744,1355744,2711488,1905.5030808448792,2.412707544863224e-08
170433,1358624,1358624,2717248,1909.482509613037,2.4125256459228694e-08
170793,1361502,1361502,2723004,1913.510729789734,2.4125256459228694e-08
171154,1364388,1364388,2728776,1917.6320927143097,2.4112523533403873e-08
171514,1367268,1367268,2734536,1921.7291786670685,2.4110704544000328e-08
171874,1370146,1370146,2740292,1925.7774348258972,2.4108885554596782e-08
172235,1373034,1373034,2746068,1929.9569137096405,2.4107066565193236e-08
172595,1375910,1375910,2751820,1934.0855119228363,2.4057953851297498e-08
172955,1378790,1378790,2757580,1938.042457818985,2.4057953851297498e-08
173316,1381678,1381678,2763356,1942.0446107387543,2.4056134861893952e-08
173676,1384556,1384556,2769112,1946.1991558074951,2.4045220925472677e-08
174036,1387434,1387434,2774868,1950.5252096652985,2.4003384169191122e-08
174396,1390314,1390314,2780628,1954.558861732483,2.399974619038403e-08
174757,1393200,1393200,2786400,1958.6791307926178,2.4001565179787576e-08
175117,1396078,1396078,2792156,1963.1097688674927,2.399610821157694e-08
175477,1398956,1398956,2797912,1967.302963733673,2.395609044469893e-08
175838,1401844,1401844,2803688,1971.274250984192,2.3954271455295384e-08
176198,1404722,1404722,2809444,1975.332308769226,2.3952452465891838e-08
176558,1407602,1407602,2815204,1979.3879368305206,2.3952452465891838e-08
176919,1410488,1410488,2820976,1983.3255228996277,2.3948814487084746e-08
177279,1413366,1413366,2826732,1987.4013347625732,2.3910615709610283e-08
177639,1416244,1416244,2832488,1991.452553987503,2.3910615709610283e-08
178000,1419130,1419130,2838260,1995.5059819221497,2.3901520762592554e-08
178360,1422010,1422010,2844020,1999.5430719852448,2.3901520762592554e-08
178720,1424888,1424888,2849776,2003.465684890747,2.3897882783785462e-08
179081,1427772,1427772,2855544,2007.5809297561646,2.383239916525781e-08
179441,1430652,1430652,2861304,2011.8018028736115,2.3830580175854266e-08
179801,1433530,1433530,2867060,2016.1680927276611,2.381057129241526e-08
180162,1436416,1436416,2872832,2021.313954591751,2.3808752303011715e-08
180522,1439292,1439292,2878584,2025.9573638439178,2.3786924430169165e-08
180882,1442172,1442172,2884344,2030.106009721756,2.3786924430169165e-08
181243,1445052,1445052,2890104,2034.3417489528656,2.3717802832834423e-08
181603,1447930,1447930,2895860,2038.679040670395,2.371416485402733e-08
181963,1450806,1450806,2901612,2043.462554693222,2.3641405277885497e-08
182324,1453694,1453694,2907388,2048.266612768173,2.3643224267289042e-08
182684,1456570,1456570,2913140,2053.024683713913,2.362685336265713e-08
183044,1459450,1459450,2918900,2057.7197246551514,2.3625034373253584e-08
183405,1462336,1462336,2924672,2062.297724723816,2.3621396394446492e-08
183765,1465214,1465214,2930428,2066.4484128952026,2.3615939426235855e-08
184125,1468094,1468094,2936188,2070.6229887008667,2.36177584156394e-08
184486,1470976,1470976,2941952,2074.737708568573,2.3506800062023103e-08
184846,1473856,1473856,2947712,2078.9663639068604,2.3504981072619557e-08
185206,1476734,1476734,2953468,2083.2641699314117,2.349952410440892e-08
185567,1479622,1479622,2959244,2088.068870782852,2.3497705115005374e-08
185927,1482500,1482500,2965000,2093.247412919998,2.3443135432898998e-08
186287,1485380,1485380,2970760,2098.8033599853516,2.3441316443495452e-08
186647,1488256,1488256,2976512,2103.371319770813,2.3395841708406806e-08
187008,1491140,1491140,2982280,2107.4937467575073,2.3395841708406806e-08
187368,1494018,1494018,2988036,2111.6036248207092,2.339038474019617e-08
187728,1496894,1496894,2993788,2115.8155739307404,2.3330358089879155e-08
188089,1499780,1499780,2999560,2119.920970916748,2.3330358089879155e-08
188449,1502660,1502660,3005320,2123.924115896225,2.332853910047561e-08
188809,1505538,1505538,3011076,2128.0475997924805,2.3324901121668518e-08
189170,1508424,1508424,3016848,2132.147962808609,2.3317625164054334e-08
189530,1511304,1511304,3022608,2136.1799318790436,2.3315806174650788e-08
189890,1514182,1514182,3028364,2140.303640604019,2.331034920644015e-08
190251,1517070,1517070,3034140,2144.4814257621765,2.331034920644015e-08
190611,1519948,1519948,3039896,2148.611836910248,2.3308530217036605e-08
190971,1522820,1522820,3045640,2152.704917907715,2.3215761757455766e-08
191332,1525708,1525708,3051416,2156.897519826889,2.321394276805222e-08
191692,1528586,1528586,3057172,2160.958869934082,2.320484782103449e-08
192052,1531466,1531466,3062932,2165.4247579574585,2.320484782103449e-08
192413,1534352,1534352,3068704,2170.8978576660156,2.318301994819194e-08
192773,1537230,1537230,3074460,2175.639812707901,2.3181200958788395e-08
193133,1540110,1540110,3080220,2180.260452747345,2.3181200958788395e-08
193494,1542996,1542996,3085992,2185.048796892166,2.317028702236712e-08
193854,1545876,1545876,3091752,2190.216796875,2.317028702236712e-08
194214,1548752,1548752,3097504,2194.5490548610687,2.3141183191910386e-08
194575,1551636,1551636,3103272,2198.864629983902,2.313936420250684e-08
194935,1554512,1554512,3109024,2203.749034881592,2.3122993297874928e-08
195295,1557392,1557392,3114784,2208.857181787491,2.3122993297874928e-08
195656,1560274,1560274,3120548,2213.2994287014008,2.3068423615768552e-08
196016,1563154,1563154,3126308,2217.5695888996124,2.3068423615768552e-08
196376,1566034,1566034,3132068,2221.8852999210358,2.3068423615768552e-08
196737,1568918,1568918,3137836,2226.2040917873383,2.3044776753522456e-08
197097,1571796,1571796,3143592,2231.0893869400024,2.3017491912469268e-08
197457,1574676,1574676,3149352,2236.217805624008,2.3015672923065722e-08
197818,1577562,1577562,3155124,2240.6794838905334,2.3006577976047993e-08
198178,1580440,1580440,3160880,2244.7335228919983,2.299930201843381e-08
198538,1583320,1583320,3166640,2248.8476238250732,2.299930201843381e-08
198898,1586198,1586198,3172396,2252.9809918403625,2.2993845050223172e-08
199259,1589086,1589086,3178172,2257.0403838157654,2.2993845050223172e-08
199619,1591964,1591964,3183928,2261.310980796814,2.2993845050223172e-08
199979,1594838,1594838,3189676,2265.4424448013306,2.2848325897939503e-08
200340,1597722,1597722,3195444,2269.5377867221832,2.284104994032532e-08
200700,1600602,1600602,3201204,2273.610765695572,2.284104994032532e-08
201060,1603480,1603480,3206960,2277.7958776950836,2.2833773982711136e-08
201421,1606368,1606368,3212736,2283.300372838974,2.2833773982711136e-08
201781,1609244,1609244,3218488,2288.353967666626,2.2830136003904045e-08
202141,1612122,1612122,3224244,2292.5549437999725,2.2764652385376394e-08
202502,1615010,1615010,3230020,2297.263193845749,2.2761014406569302e-08
202862,1617888,1617888,3235776,2302.2028658390045,2.274828148074448e-08
203222,1620768,1620768,3241536,2306.56685590744,2.2746462491340935e-08
203583,1623654,1623654,3247308,2310.9537427425385,2.2742824512533844e-08
203943,1626532,1626532,3253064,2315.478418827057,2.2741005523130298e-08
204303,1629412,1629412,3258824,2320.265790939331,2.2739186533726752e-08
204664,1632294,1632294,3264588,2326.9239938259125,2.2680978872813284e-08
205024,1635172,1635172,3270344,2332.1129677295685,2.264278009533882e-08
205384,1638052,1638052,3276104,2336.559072971344,2.2640961105935276e-08
205745,1640938,1640938,3281876,2342.122130870819,2.263914211653173e-08
206105,1643818,1643818,3287636,2348.4120547771454,2.2637323127128184e-08
206465,1646686,1646686,3293372,2354.3551087379456,2.229171514045447e-08
206826,1649572,1649572,3299144,2359.9639108181,2.2289896151050925e-08
207186,1652452,1652452,3304904,2364.4694147109985,2.228807716164738e-08
207546,1655328,1655328,3310656,2368.890483856201,2.2249878384172916e-08
207907,1658214,1658214,3316428,2373.1154465675354,2.224805939476937e-08
208267,1661092,1661092,3322184,2377.2142946720123,2.224442141596228e-08
208627,1663970,1663970,3327940,2381.852790594101,2.219167072325945e-08
208988,1666858,1666858,3333716,2386.0732197761536,2.219167072325945e-08
209348,1669736,1669736,3339472,2390.1900238990784,2.218621375504881e-08
209708,1672616,1672616,3345232,2394.360668897629,2.218621375504881e-08
210068,1675494,1675494,3350988,2398.453575849533,2.2171661839820445e-08
210429,1678382,1678382,3356764,2402.891300678253,2.2171661839820445e-08
210789,1681260,1681260,3362520,2407.611290693283,2.2166204871609807e-08
211149,1684138,1684138,3368276,2412.3206646442413,2.216438588220626e-08
211510,1687020,1687020,3374040,2416.4606835842133,2.207707439083606e-08
211870,1689900,1689900,3379800,2420.4870688915253,2.207707439083606e-08
212230,1692776,1692776,3385552,2424.6774389743805,2.2053427528589964e-08
212591,1695662,1695662,3391324,2428.9927899837494,2.2047970560379326e-08
212951,1698542,1698542,3397084,2433.6568179130554,2.2047970560379326e-08
213311,1701416,1701416,3402832,2438.083863735199,2.1966116037219763e-08
213672,1704304,1704304,3408608,2442.48193359375,2.1966116037219763e-08
214032,1707182,1707182,3414364,2446.9904177188873,2.1953383111394942e-08
214392,1710060,1710060,3420120,2451.235229730606,2.1944288164377213e-08
214753,1712948,1712948,3425896,2455.729246854782,2.1944288164377213e-08
215113,1715826,1715826,3431652,2461.0990509986877,2.1871528588235378e-08
215473,1718706,1718706,3437412,2466.68740773201,2.1871528588235378e-08
215834,1721592,1721592,3443184,2471.648412704468,2.1869709598831832e-08
216194,1724472,1724472,3448944,2476.6809096336365,2.1869709598831832e-08
216554,1727350,1727350,3454700,2481.969719648361,2.1864252630621195e-08
216915,1730234,1730234,3460468,2486.676855802536,2.1833329810760915e-08
217275,1733114,1733114,3466228,2491.545940876007,2.1833329810760915e-08
217635,1735992,1735992,3471984,2496.0289556980133,2.1827872842550278e-08
217996,1738880,1738880,3477760,2500.408362865448,2.1827872842550278e-08
218356,1741756,1741756,3483512,2505.97709774971,2.1753294277004898e-08
218716,1744634,1744634,3489268,2510.862913608551,2.1751475287601352e-08
219077,1747522,1747522,3495044,2515.293940782547,2.1749656298197806e-08
219437,1750400,1750400,3500800,2520.069007873535,2.1744199329987168e-08
219797,1753278,1753278,3506556,2524.4785068035126,2.1740561351180077e-08
220158,1756166,1756166,3512332,2528.7703437805176,2.1740561351180077e-08
220518,1759042,1759042,3518084,2533.1912717819214,2.1706000552512705e-08
220878,1761920,1761920,3523840,2537.8513889312744,2.170418156310916e-08
221239,1764808,1764808,3529616,2543.0637958049774,2.1702362573705614e-08
221599,1767684,1767684,3535368,2548.340161561966,2.166416379623115e-08
221959,1770564,1770564,3541128,2552.7882030010223,2.1662344806827605e-08
222319,1773444,1773444,3546888,2557.75470161438,2.1662344806827605e-08
222680,1776328,1776328,3552656,2563.614450931549,2.163869794458151e-08
223040,1779208,1779208,3558416,2567.9142467975616,2.1635059965774417e-08
223400,1782086,1782086,3564172,2572.3021278381348,2.1596861188299954e-08
223761,1784972,1784972,3569944,2576.879426717758,2.1595042198896408e-08
224121,1787852,1787852,3575704,2581.4799869060516,2.1595042198896408e-08
224481,1790730,1790730,3581460,2586.47833275795,2.1591404220089316e-08
224842,1793616,1793616,3587232,2590.6730806827545,2.158594725187868e-08
225202,1796496,1796496,3592992,2595.455641746521,2.1582309273071587e-08
225562,1799374,1799374,3598748,2601.133986711502,2.1542291506193578e-08
225923,1802262,1802262,3604524,2606.3435287475586,2.1542291506193578e-08
226283,1805140,1805140,3610280,2611.8690598011017,2.1538653527386487e-08
226643,1808016,1808016,3616032,2616.7952115535736,2.148044586647302e-08
227004,1810902,1810902,3621804,2622.289661884308,2.1478626877069473e-08
227364,1813778,1813778,3627556,2627.068473815918,2.1456799004226923e-08
227724,1816658,1816658,3633316,2631.6286277770996,2.1456799004226923e-08
228085,1819544,1819544,3639088,2637.064178943634,2.145316102541983e-08
228445,1822424,1822424,3644848,2641.7602138519287,2.145316102541983e-08
228805,1825302,1825302,3650604,2646.2236108779907,2.144952304661274e-08
229166,1828188,1828188,3656376,2650.68145775795,2.140950527973473e-08
229526,1831066,1831066,3662132,2655.093069791794,2.1360392565838993e-08
229886,1833942,1833942,3667884,2660.033100605011,2.1360392565838993e-08
230247,1836830,1836830,3673660,2665.303678750992,2.1358573576435447e-08
230607,1839708,1839708,3679416,2669.86367893219,2.13567545870319e-08
230967,1842586,1842586,3685172,2674.581178665161,2.135311660822481e-08
231328,1845472,1845472,3690944,2679.049566745758,2.1345840650610626e-08
231688,1848352,1848352,3696704,2684.0000348091125,2.1345840650610626e-08
232048,1851228,1851228,3702456,2689.0279817581177,2.1338564692996442e-08
232409,1854112,1854112,3708224,2693.809685945511,2.1305822883732617e-08
232769,1856984,1856984,3713968,2698.499107837677,2.1302184904925525e-08
233129,1859862,1859862,3719724,2702.8261897563934,2.130036591552198e-08
233490,1862748,1862748,3725496,2707.0256838798523,2.1227606339380145e-08
233850,1865628,1865628,3731256,2711.1973328590393,2.12257873499766e-08
234210,1868506,1868506,3737012,2715.3244726657867,2.1227606339380145e-08
234570,1871380,1871380,3742760,2719.903144836426,2.1187588572502136e-08
234931,1874268,1874268,3748536,2724.3246598243713,2.1187588572502136e-08
235291,1877146,1877146,3754292,2728.476920604706,2.117667463608086e-08
235651,1880026,1880026,3760052,2732.7066287994385,2.117667463608086e-08
236012,1882912,1882912,3765824,2737.7043278217316,2.1169398678466678e-08
236372,1885788,1885788,3771576,2742.819718837738,2.116394171025604e-08
236732,1888668,1888668,3777336,2747.4873967170715,2.116394171025604e-08
237093,1891550,1891550,3783100,2752.0676698684692,2.112392394337803e-08
237453,1894430,1894430,3788860,2756.7633757591248,2.112392394337803e-08
237813,1897308,1897308,3794616,2762.3142836093903,2.1113010006956756e-08
238174,1900196,1900196,3800392,2766.736150741577,2.111119101755321e-08
238534,1903070,1903070,3806140,2771.011683702469,2.0629158825613558e-08
238894,1905944,1905944,3811888,2775.1312777996063,2.0627339836210012e-08
239255,1908832,1908832,3817664,2779.268969774246,2.0627339836210012e-08
239615,1911710,1911710,3823420,2783.4041736125946,2.0625520846806467e-08
239975,1914588,1914588,3829176,2787.4783487319946,2.0621882867999375e-08
240336,1917472,1917472,3834944,2791.619095802307,2.0618244889192283e-08
240696,1920348,1920348,3840696,2795.6825788021088,2.0605511963367462e-08
241056,1923228,1923228,3846456,2799.8525156974792,2.0605511963367462e-08
241417,1926114,1926114,3852228,2804.0252459049225,2.059277903754264e-08
241777,1928988,1928988,3857976,2808.0756447315216,2.0498191588558257e-08
242137,1931868,1931868,3863736,2812.1814708709717,2.0498191588558257e-08
242498,1934754,1934754,3869508,2816.354877948761,2.049637259915471e-08
242858,1937630,1937630,3875260,2820.40700173378,2.048363967332989e-08
243218,1940510,1940510,3881020,2824.4451987743378,2.0481820683926344e-08
243579,1943392,1943392,3886784,2828.5860679149628,2.0379957277327776e-08
243939,1946272,1946272,3892544,2832.7738676071167,2.037813828792423e-08
244299,1949150,1949150,3898300,2837.2280967235565,2.0372681319713593e-08
244660,1952036,1952036,3904072,2841.326315641403,2.03690433409065e-08
245020,1954912,1954912,3909824,2845.4456708431244,2.034721546806395e-08
245380,1957792,1957792,3915584,2849.719714641571,2.0345396478660405e-08
245741,1960676,1960676,3921352,2853.942790746689,2.0305378711782396e-08
246101,1963554,1963554,3927108,2858.3656067848206,2.0305378711782396e-08
246461,1966432,1966432,3932864,2862.464081764221,2.0301740732975304e-08
246821,1969312,1969312,3938624,2866.536012649536,2.0299921743571758e-08
247182,1972198,1972198,3944396,2870.7614719867706,2.0298102754168212e-08
247542,1975074,1975074,3950148,2875.0381219387054,2.0267179934307933e-08
247902,1977954,1977954,3955908,2879.107084751129,2.0265360944904387e-08
248263,1980840,1980840,3961680,2883.195101737976,2.026354195550084e-08
248623,1983716,1983716,3967432,2887.2978036403656,2.021624823100865e-08
248983,1986596,1986596,3973192,2891.4525775909424,2.0214429241605103e-08
249344,1989482,1989482,3978964,2895.5132637023926,2.016713551711291e-08
249704,1992362,1992362,3984724,2899.5552546977997,2.0168954506516457e-08
250064,1995240,1995240,3990480,2903.6367769241333,2.016713551711291e-08
250425,1998128,1998128,3996256,2907.696657896042,2.016349753830582e-08
250785,2001006,2001006,4002012,2911.759621858597,2.0159859559498727e-08
251145,2003884,2003884,4007768,2915.75483584404,2.015804057009518e-08
251506,2006768,2006768,4013536,2920.012847661972,2.0152583601884544e-08
251866,2009646,2009646,4019292,2924.4197697639465,2.0112565835006535e-08
252226,2012526,2012526,4025052,2928.4708528518677,2.0112565835006535e-08
252587,2015410,2015410,4030820,2932.6193528175354,2.009255695156753e-08
252947,2018290,2018290,4036580,2938.058931827545,2.009255695156753e-08
253307,2021168,2021168,4042336,2942.862607717514,2.008891897276044e-08
253668,2024054,2024054,4048108,2947.2652275562286,2.0085280993953347e-08
254028,2026932,2026932,4053864,2951.7573566436768,2.0056177163496614e-08
254388,2029812,2029812,4059624,2956.3736917972565,2.0052539184689522e-08
254749,2032698,2032698,4065396,2961.164933681488,2.003616828005761e-08
255109,2035578,2035578,4071156,2965.8532989025116,2.003616828005761e-08
255469,2038456,2038456,4076912,2970.2804396152496,2.0034349290654063e-08
255830,2041344,2041344,4082688,2975.041823863983,2.0032530301250517e-08
256190,2044222,2044222,4088444,2979.917187690735,2.0028892322443426e-08
256550,2047102,2047102,4094204,2984.7749347686768,2.002707333303988e-08
256911,2049986,2049986,4099972,2989.776422739029,1.9985236576758325e-08
257271,2052862,2052862,4105724,2994.891504764557,1.9981598597951233e-08
257631,2055740,2055740,4111480,2999.0613617897034,1.9914295990020037e-08
257991,2058618,2058618,4117236,3003.1104588508606,1.991247700061649e-08
258352,2061506,2061506,4123012,3007.1929848194122,1.9914295990020037e-08
258712,2064384,2064384,4128768,3011.238262653351,1.9905201043002307e-08
259072,2067264,2067264,4134528,3015.4531667232513,1.9905201043002307e-08
259433,2070150,2070150,4140300,3019.391910791397,1.989974407479167e-08
259793,2073028,2073028,4146056,3023.4262647628784,1.9897925085388124e-08
260153,2075906,2075906,4151812,3027.578373670578,1.9892468117177486e-08
260514,2078792,2078792,4157584,3031.6407396793365,1.984699338208884e-08
260874,2081670,2081670,4163340,3035.784863948822,1.984699338208884e-08
261234,2084550,2084550,4169100,3039.9111337661743,1.984699338208884e-08
261595,2087436,2087436,4174872,3044.02410697937,1.9841536413878202e-08
261955,2090316,2090316,4180632,3049.0097477436066,1.9841536413878202e-08
262315,2093194,2093194,4186388,3054.0870547294617,1.983789843507111e-08
262676,2096078,2096078,4192156,3058.3909339904785,1.9832441466860473e-08
263036,2098956,2098956,4197912,3062.3622148036957,1.9826984498649836e-08
263396,2101836,2101836,4203672,3066.5867426395416,1.9826984498649836e-08
263757,2104722,2104722,4209444,3072.0732595920563,1.9821527530439198e-08
264117,2107600,2107600,4215200,3076.414261817932,1.9821527530439198e-08
264477,2110478,2110478,4220956,3080.638945579529,1.9801518647000194e-08
264838,2113366,2113366,4226732,3084.9513866901398,1.9799699657596648e-08
265198,2116240,2116240,4232480,3089.3342068195343,1.9765138858929276e-08
265558,2119118,2119118,4238236,3093.4947838783264,1.9739673007279634e-08
265919,2122004,2122004,4244008,3097.753609895706,1.9736035028472543e-08
266279,2124884,2124884,4249768,3102.2094116210938,1.973785401787609e-08
266639,2127762,2127762,4255524,3106.627217769623,1.972875907085836e-08
267000,2130648,2130648,4261296,3110.943238735199,1.9725121092051268e-08
267360,2133526,2133526,4267052,3115.2750086784363,1.9723302102647722e-08
267720,2136404,2136404,4272808,3120.1649737358093,1.971966412384063e-08
268081,2139290,2139290,4278580,3124.761791944504,1.9621438696049154e-08
268441,2142168,2142168,4284336,3129.2165718078613,1.9615981727838516e-08
268801,2145046,2145046,4290092,3133.2980756759644,1.9615981727838516e-08
269162,2147930,2147930,4295860,3137.2056319713593,1.9528670236468315e-08
269522,2150810,2150810,4301620,3141.234712600708,1.952685124706477e-08
269882,2153684,2153684,4307368,3145.8658187389374,1.9521394278854132e-08
270242,2156562,2156562,4313124,3151.571588754654,1.9510480342432857e-08
270603,2159450,2159450,4318900,3155.976133823395,1.950866135302931e-08
270963,2162328,2162328,4324656,3160.2594878673553,1.950866135302931e-08
271323,2165206,2165206,4330412,3166.0816926956177,1.950502337422222e-08
271684,2168092,2168092,4336184,3170.1874418258667,1.9501385395415127e-08
272044,2170970,2170970,4341940,3174.17928981781,1.9497747416608036e-08
272404,2173848,2173848,4347696,3178.235188961029,1.9497747416608036e-08
272765,2176730,2176730,4353460,3182.3765897750854,1.9432263798080385e-08
273125,2179608,2179608,4359216,3186.5558807849884,1.943044480867684e-08
273485,2182484,2182484,4364968,3190.6468527317047,1.9379513105377555e-08
273846,2185372,2185372,4370744,3194.720607995987,1.9379513105377555e-08
274206,2188250,2188250,4376500,3198.8069398403168,1.9332219380885363e-08
274566,2191128,2191128,4382256,3202.9597675800323,1.933403837028891e-08
274927,2194016,2194016,4388032,3206.9994246959686,1.9330400391481817e-08
275287,2196894,2196894,4393788,3211.056858778,1.9330400391481817e-08
275647,2199774,2199774,4399548,3215.213100671768,1.9330400391481817e-08
276008,2202658,2202658,4405316,3219.1433238983154,1.9299477571621537e-08
276368,2205536,2205536,4411072,3223.8735597133636,1.92940206034109e-08
276728,2208416,2208416,4416832,3228.6669178009033,1.9295839592814445e-08
277089,2211302,2211302,4422604,3233.787077665329,1.9292201614007354e-08
277449,2214178,2214178,4428356,3238.328024625778,1.9252183847129345e-08
277809,2217058,2217058,4434116,3243.068797826767,1.9255821825936437e-08
278170,2219944,2219944,4439888,3248.0422966480255,1.924126991070807e-08
278530,2222824,2222824,4445648,3252.8463218212128,1.9239450921304524e-08
278890,2225700,2225700,4451400,3257.3401288986206,1.9199433154426515e-08
279251,2228584,2228584,4457168,3262.2555928230286,1.919761416502297e-08
279611,2231462,2231462,4462924,3266.982183933258,1.9192157196812332e-08
279971,2234342,2234342,4468684,3271.769203901291,1.9192157196812332e-08
280332,2237228,2237228,4474456,3276.23978972435,1.9173967302776873e-08
280692,2240106,2240106,4480212,3280.680942773819,1.9173967302776873e-08
281052,2242984,2242984,4485968,3285.4399275779724,1.9121216610074043e-08
281413,2245870,2245870,4491740,3290.324005842209,1.911757863126695e-08
281773,2248748,2248748,4497496,3294.725512742996,1.9115759641863406e-08
282133,2251624,2251624,4503248,3298.85630774498,1.9110302673652768e-08
282493,2254502,2254502,4509004,3302.9831957817078,1.9084836822003126e-08
282854,2257390,2257390,4514780,3307.3509197235107,1.9084836822003126e-08
283214,2260268,2260268,4520536,3312.30885887146,1.907937985379249e-08
283574,2263148,2263148,4526296,3317.2351248264313,1.907937985379249e-08
283935,2266034,2266034,4532068,3321.899136543274,1.9066646927967668e-08
284295,2268914,2268914,4537828,3326.600266933441,1.9063008949160576e-08
284655,2271792,2271792,4543584,3331.0730097293854,1.9064827938564122e-08
285016,2274680,2274680,4549360,3335.4580779075623,1.9063008949160576e-08
285376,2277556,2277556,4555112,3340.0905599594116,1.9022991182282567e-08
285736,2280436,2280436,4560872,3345.0428416728973,1.902117219287902e-08
286097,2283320,2283320,4566640,3349.2581696510315,1.9019353203475475e-08
286457,2286198,2286198,4572396,3354.256385564804,1.9015715224668384e-08
286817,2289074,2289074,4578148,3358.634217977524,1.8975697457790375e-08
287178,2291960,2291960,4583920,3363.296413898468,1.896842150017619e-08
287538,2294840,2294840,4589680,3367.900018930435,1.896842150017619e-08
287898,2297716,2297716,4595432,3372.886338710785,1.8932041712105274e-08
288259,2300604,2300604,4601208,3377.4380297660828,1.8932041712105274e-08
288619,2303482,2303482,4606964,3382.0024058818817,1.8919308786280453e-08
288979,2306362,2306362,4612724,3386.969740629196,1.891567080747336e-08
289340,2309248,2309248,4618496,3391.377111673355,1.8897480913437903e-08
289700,2312128,2312128,4624256,3395.6923298835754,1.8897480913437903e-08
290060,2315006,2315006,4630012,3400.575266599655,1.8895661924034357e-08
290421,2317892,2317892,4635784,3405.168040752411,1.8842911231331527e-08
290781,2320770,2320770,4641540,3409.357596874237,1.884109224192798e-08
291141,2323646,2323646,4647292,3414.6436347961426,1.8839273252524436e-08
291502,2326534,2326534,4653068,3419.372496843338,1.883745426312089e-08
291862,2329412,2329412,4658824,3423.5342106819153,1.8835635273717344e-08
292222,2332290,2332290,4664580,3427.5460076332092,1.878834154922515e-08
292583,2335176,2335176,4670352,3431.931500673294,1.8773789633996785e-08
292943,2338056,2338056,4676112,3436.052515745163,1.8773789633996785e-08
293303,2340932,2340932,4681864,3440.247738838196,1.8770151655189693e-08
293664,2343820,2343820,4687640,3444.477398633957,1.8768332665786147e-08
294024,2346696,2346696,4693392,3448.5233767032623,1.8724676920101047e-08
294384,2349574,2349574,4699148,3452.6412127017975,1.87228579306975e-08
294744,2352450,2352450,4704900,3456.751980781555,1.871921995189041e-08
295105,2355336,2355336,4710672,3460.9375648498535,1.870103005785495e-08
295465,2358216,2358216,4716432,3465.181047677994,1.8699211068451405e-08
295825,2361096,2361096,4722192,3469.2751359939575,1.8699211068451405e-08
296186,2363974,2363974,4727948,3473.5925776958466,1.8579157767817378e-08
296546,2366850,2366850,4733700,3477.7482466697693,1.8575519789010286e-08
296906,2369728,2369728,4739456,3481.9955537319183,1.8562786863185465e-08
297267,2372616,2372616,4745232,3486.272297859192,1.856460585258901e-08
297627,2375494,2375494,4750988,3490.3093235492706,1.8522769096307456e-08
297987,2378372,2378372,4756744,3494.3860898017883,1.852095010690391e-08
298348,2381260,2381260,4762520,3498.73673081398,1.852095010690391e-08
298708,2384136,2384136,4768272,3502.7638766765594,1.851731212809682e-08
299068,2387016,2387016,4774032,3506.740118741989,1.8515493138693273e-08
299429,2389902,2389902,4779804,3510.8946266174316,1.8513674149289727e-08
299789,2392778,2392778,4785556,3515.0073778629303,1.8470018403604627e-08
300149,2395658,2395658,4791316,3519.270738840103,1.8470018403604627e-08
300510,2398542,2398542,4797084,3523.4805738925934,1.8448190530762076e-08
300870,2401420,2401420,4802840,3527.722856760025,1.84372765943408e-08
301230,2404298,2404298,4808596,3532.0905187129974,1.8435457604937255e-08
301591,2407184,2407184,4814368,3536.7333278656006,1.843363861553371e-08
301951,2410064,2410064,4820128,3541.49293589592,1.843363861553371e-08
302311,2412940,2412940,4825880,3546.1592009067535,1.83499651029706e-08
302672,2415828,2415828,4831656,3551.1289489269257,1.8348146113567054e-08
303032,2418706,2418706,4837412,3556.475759744644,1.8348146113567054e-08
303392,2421584,2421584,4843168,3561.447790622711,1.834632712416351e-08
303753,2424470,2424470,4848940,3565.850157737732,1.8342689145356417e-08
304113,2427348,2427348,4854696,3570.3535108566284,1.8320861272513866e-08
304473,2430228,2430228,4860456,3575.126728773117,1.8320861272513866e-08
304834,2433112,2433112,4866224,3579.6575837135315,1.829357643146068e-08
305194,2435988,2435988,4871976,3584.217933654785,1.8291757442057133e-08
305554,2438868,2438868,4877736,3588.794379711151,1.8291757442057133e-08
305915,2441754,2441754,4883508,3594.2619268894196,1.8286300473846495e-08
306275,2444632,2444632,4889264,3598.596974849701,1.8282662495039403e-08
306635,2447510,2447510,4895020,3602.7017498016357,1.8246282706968486e-08
306995,2450388,2450388,4900776,3607.1153178215027,1.824446371756494e-08
307356,2453274,2453274,4906548,3611.5247616767883,1.823536877054721e-08
307716,2456152,2456152,4912304,3615.703008890152,1.822263584472239e-08
308076,2459032,2459032,4918064,3619.9882748126984,1.822263584472239e-08
308437,2461918,2461918,4923836,3624.359893798828,1.8198988982476294e-08
308797,2464798,2464798,4929596,3628.3992528915405,1.8198988982476294e-08
309157,2467676,2467676,4935352,3632.577778816223,1.8197169993072748e-08
309518,2470564,2470564,4941128,3636.8206589221954,1.8195351003669202e-08
309878,2473442,2473442,4946884,3641.6193726062775,1.819171302486211e-08
310238,2476320,2476320,4952640,3645.9803977012634,1.8186256056651473e-08
310599,2479206,2479206,4958412,3650.444263935089,1.8186256056651473e-08
310959,2482080,2482080,4964160,3655.418373823166,1.8153514247387648e-08
311319,2484958,2484958,4969916,3660.3740496635437,1.8146238289773464e-08
311680,2487846,2487846,4975692,3665.5468537807465,1.8146238289773464e-08
312040,2490724,2490724,4981448,3670.17453789711,1.8137143342755735e-08
312400,2493602,2493602,4987204,3674.6657857894897,1.812986738514155e-08
312761,2496490,2496490,4992980,3679.5925629138947,1.8128048395738006e-08
313121,2499368,2499368,4998736,3684.108011007309,1.811349648050964e-08
313481,2502248,2502248,5004496,3689.0499198436737,1.8111677491106093e-08
313842,2505136,2505136,5010272,3693.5738768577576,1.8111677491106093e-08
314202,2508012,2508012,5016024,3698.1604957580566,1.8106220522895455e-08
314562,2510888,2510888,5021776,3703.04611992836,1.8058926798403263e-08
314923,2513774,2513774,5027548,3707.606219768524,1.8058926798403263e-08
315283,2516650,2516650,5033300,3712.2971057891846,1.803346094675362e-08
315643,2519528,2519528,5039056,3716.574967622757,1.8031641957350075e-08
316004,2522414,2522414,5044828,3721.1160538196564,1.802982296794653e-08
316364,2525292,2525292,5050584,3725.5213136672974,1.8028003978542984e-08
316724,2528172,2528172,5056344,3730.9291257858276,1.8028003978542984e-08
317085,2531056,2531056,5062112,3736.2468717098236,1.7982529243454337e-08
317445,2533936,2533936,5067872,3743.5951647758484,1.798071025405079e-08
317805,2536814,2536814,5073628,3750.859871864319,1.7973434296436608e-08
318165,2539690,2539690,5079380,3758.54842877388,1.7953425412997603e-08
318526,2542576,2542576,5085152,3766.261151790619,1.7947968444786966e-08
318886,2545456,2545456,5090912,3773.9783828258514,1.794614945538342e-08
319246,2548336,2548336,5096672,3780.5006217956543,1.794614945538342e-08
319607,2551216,2551216,5102432,3785.658171892166,1.7898855730891228e-08
319967,2554096,2554096,5108192,3789.950305700302,1.7897036741487682e-08
320327,2556974,2556974,5113948,3793.9891607761383,1.789339876268059e-08
320688,2559862,2559862,5119724,3798.379609823227,1.789339876268059e-08
321048,2562736,2562736,5125472,3802.9503498077393,1.7771526472643018e-08
321408,2565616,2565616,5131232,3807.1512398719788,1.7771526472643018e-08
321769,2568500,2568500,5137000,3811.8356528282166,1.7760612536221743e-08
322129,2571380,2571380,5142760,3815.9933297634125,1.7760612536221743e-08
322489,2574256,2574256,5148512,3820.079509973526,1.775333657860756e-08
322850,2577144,2577144,5154288,3824.151716709137,1.7755155568011105e-08
323210,2580022,2580022,5160044,3828.2790546417236,1.7729689716361463e-08
323570,2582902,2582902,5165804,3832.4848897457123,1.7727870726957917e-08
323931,2585788,2585788,5171576,3836.705338716507,1.7727870726957917e-08
324291,2588664,2588664,5177328,3841.277996778488,1.7662387108430266e-08
324651,2591542,2591542,5183084,3845.7111258506775,1.7662387108430266e-08
325012,2594430,2594430,5188860,3850.457128763199,1.7662387108430266e-08
325372,2597310,2597310,5194620,3854.645491838455,1.766056811902672e-08
325732,2600188,2600188,5200376,3858.9981648921967,1.766056811902672e-08
326093,2603074,2603074,5206148,3863.1955115795135,1.761691237334162e-08
326453,2605954,2605954,5211908,3867.59570980072,1.7615093383938074e-08
326813,2608832,2608832,5217664,3872.273717880249,1.7613274394534528e-08
327174,2611718,2611718,5223436,3876.4550788402557,1.7609636415727437e-08
327534,2614596,2614596,5229192,3880.4774730205536,1.759872247930616e-08
327894,2617476,2617476,5234952,3884.6082158088684,1.759872247930616e-08
328255,2620358,2620358,5240716,3888.782961845398,1.7562342691235244e-08
328615,2623236,2623236,5246472,3893.546134710312,1.7535057850182056e-08
328975,2626114,2626114,5252228,3898.7606909275055,1.753323886077851e-08
329336,2629002,2629002,5258004,3903.0195248126984,1.7535057850182056e-08
329696,2631880,2631880,5263760,3907.443579673767,1.7516867956146598e-08
330056,2634760,2634760,5269520,3911.935358762741,1.7515048966743052e-08
330416,2637638,2637638,5275276,3916.1014268398285,1.7515048966743052e-08
330777,2640524,2640524,5281048,3920.447411775589,1.751141098793596e-08
331137,2643402,2643402,5286804,3925.2015948295593,1.7495040083304048e-08
331497,2646282,2646282,5292564,3930.2849338054657,1.7493221093900502e-08
331858,2649170,2649170,5298340,3934.706168651581,1.7495040083304048e-08
332218,2652040,2652040,5304080,3939.57084274292,1.734042598400265e-08
332578,2654920,2654920,5309840,3946.768500804901,1.7338606994599104e-08
332939,2657806,2657806,5315612,3954.1734778881073,1.7334969015792012e-08
333299,2660682,2660682,5321364,3961.8591496944427,1.7293132259510458e-08
333659,2663560,2663560,5327120,3969.6397025585175,1.7293132259510458e-08
334020,2666448,2666448,5332896,3977.0535638332367,1.7293132259510458e-08
334380,2669326,2669326,5338652,3983.643107652664,1.7291313270106912e-08
334740,2672204,2672204,5344408,3988.5992488861084,1.728767529129982e-08
335101,2675088,2675088,5350176,3992.927635908127,1.7245838535018265e-08
335461,2677968,2677968,5355936,3997.2320036888123,1.7245838535018265e-08
335821,2680846,2680846,5361692,4001.7359249591827,1.7242200556211174e-08
336182,2683732,2683732,5367464,4009.723568677902,1.7224010662175715e-08
336542,2686606,2686606,5373212,4017.6623265743256,1.7218553693965077e-08
336902,2689484,2689484,5378968,4025.155924797058,1.7209458746947348e-08
337263,2692370,2692370,5384740,4032.3579766750336,1.7207639757543802e-08
337623,2695250,2695250,5390500,4039.329527616501,1.720400177873671e-08
337983,2698128,2698128,5396256,4046.0127696990967,1.7176716937683523e-08
338344,2701012,2701012,5402024,4051.2434797286987,1.7176716937683523e-08
338704,2703892,2703892,5407784,4055.542356967926,1.7174897948279977e-08
339064,2706770,2706770,5413540,4059.720435857773,1.717307895887643e-08
339425,2709658,2709658,5419316,4064.258918762207,1.7171259969472885e-08
339785,2712536,2712536,5425072,4068.5967679023743,1.7165803001262248e-08
340145,2715414,2715414,5430828,4073.2399458885193,1.7162165022455156e-08
340506,2718302,2718302,5436604,4077.847771883011,1.7162165022455156e-08
340866,2721176,2721176,5442352,4082.2464456558228,1.7149432096630335e-08
341226,2724052,2724052,5448104,4086.407493829727,1.7143975128419697e-08
341587,2726940,2726940,5453880,4090.774323940277,1.714215613901615e-08
341947,2729816,2729816,5459632,4095.4947578907013,1.7140337149612606e-08
342307,2732694,2732694,5465388,4099.888446807861,1.7109414329752326e-08
342667,2735574,2735574,5471148,4104.626206874847,1.7109414329752326e-08
343028,2738460,2738460,5476920,4109.466094732285,1.710395736154169e-08
343388,2741338,2741338,5482676,4114.525926828384,1.709850039333105e-08
343748,2744218,2744218,5488436,4118.863149642944,1.7100319382734597e-08
344109,2747104,2747104,5494208,4123.375774860382,1.7096681403927505e-08
344469,2749982,2749982,5499964,4127.74947476387,1.7091224435716867e-08
344829,2752860,2752860,5505720,4131.945068597794,1.7080310499295592e-08
345190,2755748,2755748,5511496,4136.15613079071,1.7080310499295592e-08
345550,2758628,2758628,5517256,4140.388199806213,1.7078491509892046e-08
345910,2761500,2761500,5523000,4144.846319675446,1.7025740817189217e-08
346271,2764386,2764386,5528772,4149.2713396549225,1.7022102838382125e-08
346631,2767266,2767266,5534532,4153.528617858887,1.7022102838382125e-08
346991,2770144,2770144,5540288,4157.756012678146,1.701482688076794e-08
347352,2773028,2773028,5546056,4162.098173856735,1.6991180018521845e-08
347712,2775908,2775908,5551816,4166.232213973999,1.69893610291183e-08
348072,2778788,2778788,5557576,4170.484130620956,1.6987542039714754e-08
348433,2781674,2781674,5563348,4175.102346897125,1.696207618806511e-08
348793,2784554,2784554,5569108,4179.621218681335,1.6960257198661566e-08
349153,2787430,2787430,5574860,4183.953980922699,1.69457052834332e-08
349514,2790318,2790318,5580636,4188.4249086380005,1.69457052834332e-08
349874,2793196,2793196,5586392,4192.8143038749695,1.6942067304626107e-08
350234,2796076,2796076,5592152,4197.282493829727,1.6942067304626107e-08
350595,2798962,2798962,5597924,4202.664827823639,1.6938429325819016e-08
350955,2801840,2801840,5603680,4208.2084147930145,1.6907506505958736e-08
351315,2804718,2804718,5609436,4213.191251754761,1.6907506505958736e-08
351676,2807604,2807604,5615208,4218.341681718826,1.69020495377481e-08
352036,2810484,2810484,5620968,4222.809587955475,1.69020495377481e-08
352396,2813360,2813360,5626720,4226.903668880463,1.6898411558941007e-08
352757,2816248,2816248,5632496,4231.006661653519,1.689659256953746e-08
353117,2819124,2819124,5638248,4235.130917787552,1.687476469669491e-08
353477,2822002,2822002,5644004,4239.256595849991,1.6872945707291365e-08
353838,2824890,2824890,5649780,4243.414589881897,1.6872945707291365e-08
354198,2827768,2827768,5655536,4247.613415718079,1.6869307728484273e-08
354558,2830646,2830646,5661292,4252.0276618003845,1.6863850760273635e-08
354918,2833526,2833526,5667052,4256.143405675888,1.686203177087009e-08
355279,2836412,2836412,5672824,4260.329142570496,1.6858393792062998e-08
355639,2839292,2839292,5678584,4264.788489818573,1.6858393792062998e-08
355999,2842170,2842170,5684340,4268.898906707764,1.6856574802659452e-08
356360,2845056,2845056,5690112,4272.9347977638245,1.6854755813255906e-08
356720,2847934,2847934,5695868,4277.192501783371,1.6842022887431085e-08
357080,2850814,2850814,5701628,4281.491809606552,1.684384187683463e-08
357441,2853702,2853702,5707404,4285.751234769821,1.6842022887431085e-08
357801,2856580,2856580,5713160,4289.86142373085,1.684020389802754e-08
358161,2859456,2859456,5718912,4294.033836603165,1.6811100067570806e-08
358522,2862344,2862344,5724688,4299.153206586838,1.6811100067570806e-08
358882,2865220,2865220,5730440,4304.221641778946,1.680928107816726e-08
359242,2868098,2868098,5736196,4309.173952579498,1.680018613114953e-08
359603,2870986,2870986,5741972,4313.764647722244,1.6798367141745985e-08
359963,2873828,2873828,5747656,4318.172541856766,5.820766091346741e-11


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namea9a/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.008523941040039062,12064.44795143716
18,78,78,156,0.545835018157959,186.6780789084769
35,130,130,260,0.9698019027709961,52.03996526174706
53,182,182,364,1.3502981662750244,31.390393178175145
70,234,234,468,1.7225189208984375,23.792855511128437
88,288,288,576,2.128303050994873,13.383975569950053
105,344,344,688,2.6043498516082764,11.226262697015045
123,400,400,800,2.9871420860290527,6.399659026390509
141,456,456,912,3.351170063018799,4.988719561508333
158,510,510,1020,3.7232398986816406,3.448211087104937
176,566,566,1132,4.081860065460205,2.9030140740560455
193,628,628,1256,4.498257875442505,2.798770119148685
211,692,692,1384,5.043619155883789,2.447700696713582
229,756,756,1512,5.475239038467407,2.1403247818852833
246,814,814,1628,5.874090909957886,1.8867371270152944
264,876,876,1752,6.229607105255127,1.6031077646130143
281,934,934,1868,6.609287977218628,1.5252701746157982
299,1000,1000,2000,7.113217115402222,1.3431818714198016
316,1058,1058,2116,7.482725143432617,1.2664874232741568
334,1128,1128,2256,7.883991003036499,1.1101710653056216
352,1188,1188,2376,8.327441215515137,0.9636950304975471
369,1258,1258,2516,8.774407148361206,0.87101092652847
387,1318,1318,2636,9.237066984176636,0.7009521903055429
404,1374,1374,2748,9.576102018356323,0.5714227668559033
422,1446,1446,2892,10.009589910507202,0.5391367563479434
439,1518,1518,3036,10.587734937667847,0.47245098192433943
457,1584,1584,3168,11.00003719329834,0.45551057767988823
475,1650,1650,3300,11.449191093444824,0.4078379964339547
492,1716,1716,3432,11.848550081253052,0.3929713399429602
510,1780,1780,3560,12.199944972991943,0.35762860208524216
527,1838,1838,3676,12.570460796356201,0.33090880640156684
545,1902,1902,3804,12.98271894454956,0.3070690127369744
563,1968,1968,3936,13.494712114334106,0.29074154691443255
580,2040,2040,4080,13.982043027877808,0.2719217648555059
598,2110,2110,4220,14.452256917953491,0.26564294296076696
615,2170,2170,4340,14.848871946334839,0.24919297657106654
633,2244,2244,4488,15.262983083724976,0.2373433865050174
650,2310,2310,4620,15.633616209030151,0.227475689847779
668,2378,2378,4756,16.02666401863098,0.21458056677511195
686,2450,2450,4900,16.459550857543945,0.20297222315821273
703,2516,2516,5032,16.847686052322388,0.1979835620004451
721,2588,2588,5176,17.24881100654602,0.19269977658768767
738,2656,2656,5312,17.57779097557068,0.18583770886652928
756,2728,2728,5456,17.951308012008667,0.1760501370044949
773,2794,2794,5588,18.31699800491333,0.1698913127547712
791,2872,2872,5744,18.728942155838013,0.16329731778023415
809,2942,2942,5884,19.14528512954712,0.15506569339049747
826,3010,3010,6020,19.531729221343994,0.14898546385848022
844,3082,3082,6164,19.889671087265015,0.13840658656954474
861,3146,3146,6292,20.261607885360718,0.12795234242730658
879,3218,3218,6436,20.660335063934326,0.11906224482117977
897,3286,3286,6572,21.036291122436523,0.11721991901322326
914,3364,3364,6728,21.48008394241333,0.11069107493494812
932,3436,3436,6872,21.910665035247803,0.10888695742505661
949,3510,3510,7020,22.311100244522095,0.10763013629366469
967,3586,3586,7172,22.743237018585205,0.1057322159231262
984,3654,3654,7308,23.146135091781616,0.10523171477325377
1002,3726,3726,7452,23.550729990005493,0.10403917851181177
1020,3800,3800,7600,24.059110164642334,0.1015293894433853
1037,3868,3868,7736,24.550487995147705,0.09966841277127969
1055,3940,3940,7880,24.96114706993103,0.09832279377405939
1072,4010,4010,8020,25.338443994522095,0.09670935535541503
1090,4088,4088,8176,25.846252918243408,0.09348689385478792
1107,4156,4156,8312,26.267674207687378,0.09110278210755496
1125,4234,4234,8468,26.725542068481445,0.08788807355813333
1143,4314,4314,8628,27.310423135757446,0.08554775925040303
1160,4394,4394,8788,27.83256506919861,0.07909236179693835
1178,4508,4508,9016,28.53194308280945,0.07895669340723543
1195,4576,4576,9152,29.0047709941864,0.0787548444022832
1213,4648,4648,9296,29.46639895439148,0.07832095040976128
1231,4720,4720,9440,29.844398975372314,0.07805732872657245
1248,4788,4788,9576,30.268410205841064,0.07770945152697095
1266,4860,4860,9720,30.695609092712402,0.07725835209930665
1283,4928,4928,9856,31.110475063323975,0.07671861768358212
1301,5000,5000,10000,31.521543979644775,0.07576696926844306
1318,5068,5068,10136,31.97202706336975,0.07539443228415621
1336,5146,5146,10292,32.454379081726074,0.07475594474817626
1354,5258,5258,10516,33.07144021987915,0.07454996628621302
1371,5376,5376,10752,33.621039152145386,0.07446180805527547
1389,5504,5504,11008,34.22784996032715,0.07428604468441335
1406,5628,5628,11256,34.798628091812134,0.0742105614826869
1424,5766,5766,11532,35.58963394165039,0.07421123716630973
1441,5902,5902,11804,36.31736493110657,0.07421057616556936
1459,6046,6046,12092,37.02195191383362,0.07420987640580279
1477,6190,6190,12380,37.76164102554321,0.07420917678427941
1494,6326,6326,12652,38.40672516822815,0.07420851629285607
1512,6422,6422,12844,38.925060987472534,0.07399582759535406
1529,6498,6498,12996,39.3047080039978,0.07334019194058783
1547,6636,6636,13272,39.949265241622925,0.07333339225624513
1564,6768,6768,13536,40.563623905181885,0.07333035421106615
1582,6910,6910,13820,41.2497341632843,0.07332960193343752
1600,7050,7050,14100,41.901556968688965,0.07332841976676718
1617,7186,7186,14372,42.53762602806091,0.07332778036652599
1635,7330,7330,14660,43.214483976364136,0.07332710345144733
1652,7440,7440,14880,43.74110794067383,0.07316289164373302
1670,7512,7512,15024,44.116791009902954,0.07259251369214326
1688,7584,7584,15168,44.500104904174805,0.0703509640898119
1705,7652,7652,15304,44.852880001068115,0.06760904184739047
1723,7744,7744,15488,45.318695068359375,0.0645243733724783
1740,7840,7840,15680,45.791651010513306,0.06266497388423886
1758,7934,7934,15868,46.261778831481934,0.05991226545484096
1775,8006,8006,16012,46.62340712547302,0.05797107000944379
1793,8086,8086,16172,47.0198130607605,0.055519242716400186
1811,8200,8200,16400,47.58934020996094,0.051366101750318194
1828,8270,8270,16540,47.947964906692505,0.04931000967917498
1846,8368,8368,16736,48.43897008895874,0.04513350788147363
1863,8432,8432,16864,48.77931308746338,0.04441637552372413
1881,8508,8508,17016,49.16467308998108,0.04235202087147627
1898,8628,8628,17256,49.76086497306824,0.042337817652878584
1916,8766,8766,17532,50.47520995140076,0.04233678526543372
1934,8864,8864,17728,51.10572695732117,0.04225873280847736
1951,8932,8932,17864,51.487711906433105,0.04216218196961563
1969,9040,9040,18080,52.19878816604614,0.042090108938282356
1986,9174,9174,18348,52.87075400352478,0.042090412385732634
2004,9270,9270,18540,53.353610038757324,0.04203328695803066
2022,9366,9366,18732,53.85330820083618,0.04194276494126825
2039,9500,9500,19000,54.525131940841675,0.04194024002754304
2057,9644,9644,19288,55.25265192985535,0.041939938557334244
2074,9758,9758,19516,55.88354802131653,0.04188858088673442
2092,9888,9888,19776,56.60247015953064,0.04184613780853397
2109,10022,10022,20044,57.33397698402405,0.04184594533398922
2127,10160,10160,20320,57.99653601646423,0.041837825052425615
2145,10238,10238,20476,58.417054891586304,0.04160594208224211
2162,10306,10306,20612,58.79260492324829,0.040858187598132645
2180,10378,10378,20756,59.40687417984009,0.04052009352017194
2197,10466,10466,20932,59.95050382614136,0.04033674614765914
2215,10602,10602,21204,60.70676398277283,0.040333216051294585
2232,10720,10720,21440,61.33024501800537,0.04029477586846042
2250,10792,10792,21584,61.74459218978882,0.0401673544129153
2268,10864,10864,21728,62.22864007949829,0.040055680021396256
2285,10968,10968,21936,62.91841983795166,0.04000629514666798
2303,11108,11108,22216,63.75286293029785,0.04000604071006819
2320,11234,11234,22468,64.48812890052795,0.039968471335669165
2338,11320,11320,22640,65.02715396881104,0.03981168126301782
2356,11392,11392,22784,65.47428512573242,0.039610215866559884
2373,11460,11460,22920,65.95159387588501,0.03940086136572063
2391,11532,11532,23064,66.50221991539001,0.03892961228666536
2408,11610,11610,23220,67.03638005256653,0.03810218225589779
2426,11684,11684,23368,67.58377003669739,0.03738585050996335
2443,11752,11752,23504,68.0487310886383,0.036817678479565075
2461,11832,11832,23664,68.6975769996643,0.03523130999565183
2479,11942,11942,23884,69.4107928276062,0.034954862254380714
2496,12068,12068,24136,70.20440602302551,0.03480777388722345
2514,12206,12206,24412,71.0616660118103,0.03480180729275162
2531,12330,12330,24660,71.81856799125671,0.03478460891165014
2549,12402,12402,24804,72.25790619850159,0.03472452671849169
2566,12470,12470,24940,72.65760612487793,0.03463161746367405
2584,12542,12542,25084,73.09338688850403,0.03448598078284704
2602,12618,12618,25236,73.52142596244812,0.03432832358703308
2619,12686,12686,25372,73.94265222549438,0.03415210035745986
2637,12758,12758,25516,74.41770696640015,0.034042763960314915
2654,12888,12888,25776,75.17619919776917,0.03403196551153087
2672,13030,13030,26060,75.9875099658966,0.0340317599093396
2690,13148,13148,26296,76.73203301429749,0.034006799942289945
2707,13222,13222,26444,77.1757161617279,0.03390038332872791
2725,13294,13294,26588,77.63348293304443,0.03381265519601584
2742,13362,13362,26724,78.12707614898682,0.03364946367764787
2760,13438,13438,26876,78.58268117904663,0.0333410408529744
2777,13506,13506,27012,79.04088497161865,0.03299004089058144
2795,13578,13578,27156,79.52771925926208,0.03264416602360143
2813,13680,13680,27360,80.22253108024597,0.03251358694797091
2830,13806,13806,27612,80.91199612617493,0.03250740065050195
2848,13946,13946,27892,81.71867108345032,0.03250666927669954
2865,14022,14022,28044,82.18233609199524,0.032483992692505126
2883,14094,14094,28188,82.63901114463806,0.03241519443872676
2900,14162,14162,28324,83.02828311920166,0.03229077217838494
2918,14238,14238,28476,83.60348105430603,0.032159971098735696
2936,14310,14310,28620,84.07139301300049,0.03195683087869838
2953,14378,14378,28756,84.54113101959229,0.03186416369317158
2971,14450,14450,28900,85.01906609535217,0.03168441400157462
2988,14518,14518,29036,85.42106604576111,0.03141069114280981
3006,14590,14590,29180,85.8934919834137,0.030948915589760873
3024,14662,14662,29324,86.36121606826782,0.03046025154799281
3041,14730,14730,29460,86.78989005088806,0.030022271690540947
3059,14810,14810,29620,87.26087021827698,0.028814357763621956
3076,14886,14886,29772,87.71902203559875,0.027176566612979514
3094,14976,14976,29952,88.26751112937927,0.02638744842624874
3111,15110,15110,30220,89.14347100257874,0.026387212310510222
3129,15240,15240,30480,89.9553849697113,0.026380495490229805
3147,15338,15338,30676,90.5274109840393,0.02634680687697255
3164,15406,15406,30812,90.92484712600708,0.02630407502692833
3182,15478,15478,30956,91.35534310340881,0.026262699379003607
3199,15606,15606,31212,92.03050398826599,0.026258748741383897
3217,15750,15750,31500,92.75168800354004,0.026258635811245767
3234,15886,15886,31772,93.4345440864563,0.026258529176629963
3252,16030,16030,32060,94.15711903572083,0.02625841628287162
3270,16168,16168,32336,94.86783504486084,0.026258599133143434
3287,16300,16300,32600,95.55170392990112,0.02625850265212648
3305,16444,16444,32888,96.25719809532166,0.026258389831127715
3322,16580,16580,33160,96.93067598342896,0.02625828329655633
3340,16714,16714,33428,97.61455011367798,0.026242778096275288
3358,16824,16824,33648,98.19057822227478,0.026215071919068578
3375,16892,16892,33784,98.57954406738281,0.02616503918397939
3393,16990,16990,33980,99.10375714302063,0.026121965667698532
3410,17058,17058,34116,99.49130487442017,0.026065244577694102
3428,17130,17130,34260,99.89805316925049,0.02594316118666029
3445,17198,17198,34396,100.27371215820312,0.02587820162261778
3463,17270,17270,34540,100.66981506347656,0.02579127331773634
3481,17342,17342,34684,101.07755303382874,0.02570823692076374
3498,17410,17410,34820,101.45288181304932,0.025491299802524736
3516,17482,17482,34964,101.84963512420654,0.02531920409637678
3533,17550,17550,35100,102.240895986557,0.024990319669086603
3551,17626,17626,35252,102.68439197540283,0.024568217379055568
3568,17740,17740,35480,103.37634897232056,0.024526684332158766
3586,17878,17878,35756,104.1561689376831,0.024526814317141543
3604,18016,18016,36032,105.08208298683167,0.02452649185215705
3621,18148,18148,36296,105.93827700614929,0.024526383853299194
3639,18292,18292,36584,106.75659418106079,0.02452628310129512
3656,18378,18378,36756,107.41911125183105,0.02449397659074748
3674,18450,18450,36900,107.90521812438965,0.024429582117591053
3692,18522,18522,37044,108.33397817611694,0.02435453991893155
3709,18590,18590,37180,108.81491613388062,0.02429720657892176
3727,18662,18662,37324,109.35216999053955,0.024216623274696758
3744,18730,18730,37460,109.84938311576843,0.02417620209416782
3762,18802,18802,37604,110.3812038898468,0.024098694570056978
3779,18870,18870,37740,111.0084159374237,0.02402477322721097
3797,18942,18942,37884,111.5519630908966,0.023863075675762957
3815,19018,19018,38036,112.09682297706604,0.023612840530404355
3832,19086,19086,38172,112.53091716766357,0.023234433096149587
3850,19158,19158,38316,112.95603394508362,0.022780598141252995
3867,19236,19236,38472,113.51561903953552,0.021723235497120186
3885,19312,19312,38624,114.00390815734863,0.01972160160948988
3902,19380,19380,38760,114.45456790924072,0.018998856054167845
3920,19490,19490,38980,115.1525309085846,0.018647401846465073
3938,19596,19596,39192,115.7950451374054,0.018659541890883702
3955,19716,19716,39432,116.48945307731628,0.01859928679004952
3973,19836,19836,39672,117.18318009376526,0.018593362761748722
3990,19960,19960,39920,117.89746403694153,0.018589678236821783
4008,20098,20098,40196,118.68223094940186,0.018587480031783343
4025,20198,20198,40396,119.27022194862366,0.018525234150729375
4043,20270,20270,40540,119.72670412063599,0.018490253656636924
4061,20342,20342,40684,120.17842197418213,0.018468559319444466
4078,20410,20410,40820,120.6351969242096,0.018446740295985364
4096,20482,20482,40964,121.15259099006653,0.01844126507967303
4113,20550,20550,41100,121.66359186172485,0.01839108361127728
4131,20622,20622,41244,122.15210008621216,0.01833499560234486
4149,20694,20694,41388,122.61934518814087,0.018205746358944452
4166,20762,20762,41524,123.03242206573486,0.0180268891799642
4184,20834,20834,41668,123.46773600578308,0.01784447077443474
4201,20902,20902,41804,123.89955186843872,0.017636931217566598
4219,20974,20974,41948,124.34090495109558,0.01752824459981639
4236,21050,21050,42100,124.83719897270203,0.01718426701700082
4254,21122,21122,42244,125.30485510826111,0.01692548412938777
4272,21196,21196,42392,125.7641179561615,0.016321574667017558
4289,21264,21264,42528,126.260409116745,0.016121167534947745
4307,21342,21342,42684,126.7505431175232,0.015584370376018342
4324,21412,21412,42824,127.17525911331177,0.014690482741571032
4342,21502,21502,43004,127.79208302497864,0.01386903189268196
4359,21624,21624,43248,128.52743697166443,0.013870380071239197
4377,21744,21744,43488,129.2276029586792,0.013859320633855532
4395,21844,21844,43688,129.80545711517334,0.01385223228862742
4412,21974,21974,43948,130.55839204788208,0.013851939969754312
4430,22118,22118,44236,131.36100697517395,0.013851896257619956
4447,22216,22216,44432,131.9265170097351,0.013844327213519136
4465,22288,22288,44576,132.361093044281,0.013810319203912513
4483,22360,22360,44720,132.81728100776672,0.013786508974590106
4500,22428,22428,44856,133.23837304115295,0.013774424291113974
4518,22564,22564,45128,134.00305891036987,0.01377365419648413
4535,22642,22642,45284,134.4741690158844,0.013753324554272695
4553,22748,22748,45496,135.09693217277527,0.013737421086261747
4570,22880,22880,45760,135.8334288597107,0.013736609200350358
4588,22956,22956,45912,136.29758095741272,0.01372609926147561
4606,23028,23028,46056,136.7424190044403,0.013701612100703642
4623,23096,23096,46192,137.1652889251709,0.013652567549797823
4641,23172,23172,46344,137.6272828578949,0.013571686131399474
4658,23240,23240,46480,138.04583501815796,0.01343190068291733
4676,23312,23312,46624,138.49663090705872,0.013336078271095175
4693,23380,23380,46760,138.91206407546997,0.01331087830112665
4711,23452,23452,46904,139.3679769039154,0.013279866296215914
4729,23524,23524,47048,139.80642890930176,0.013149649170372868
4746,23592,23592,47184,140.22260189056396,0.013055095485469792
4764,23664,23664,47328,140.66240620613098,0.012818376282666577
4781,23732,23732,47464,141.08987307548523,0.012620019901078194
4799,23842,23842,47684,141.73637914657593,0.01260578407709545
4817,23974,23974,47948,142.48466086387634,0.012606457041329122
4834,24102,24102,48204,143.21557903289795,0.012606558089828468
4852,24234,24234,48468,143.97088098526,0.012602390517713502
4869,24308,24308,48616,144.41491508483887,0.012581143313582288
4887,24384,24384,48768,144.89505004882812,0.012567660298373085
4904,24458,24458,48916,145.3417489528656,0.012537724756839452
4922,24598,24598,49196,146.13024997711182,0.012537695958599215
4940,24710,24710,49420,146.76891016960144,0.012532046537671704
4957,24778,24778,49556,147.19289207458496,0.012515169129983406
4975,24850,24850,49700,147.64376711845398,0.012493170939706033
4992,24918,24918,49836,148.07389116287231,0.012472348344090278
5010,24990,24990,49980,148.52246713638306,0.012416091147315456
5027,25058,25058,50116,148.9388620853424,0.012361425451672403
5045,25178,25178,50356,149.63174080848694,0.012342407635514974
5063,25288,25288,50576,150.27484107017517,0.012338688147792709
5080,25396,25396,50792,150.896959066391,0.012335609548244975
5098,25476,25476,50952,151.38562512397766,0.012322412028879626
5115,25544,25544,51088,151.79587507247925,0.01229985743702855
5133,25632,25632,51264,152.33212304115295,0.012282744242838817
5151,25772,25772,51544,153.1202630996704,0.012281194403840345
5168,25906,25906,51812,153.86199188232422,0.012280903931241482
5186,26018,26018,52036,154.51976490020752,0.012268638836758328
5203,26088,26088,52176,154.94658708572388,0.012250086954736616
5221,26160,26160,52320,155.39313101768494,0.012222971927258186
5238,26228,26228,52456,155.80633997917175,0.012180584702946362
5256,26326,26326,52652,156.3978888988495,0.012121727590056253
5274,26422,26422,52844,156.97381711006165,0.01196530547895236
5291,26496,26496,52992,157.4249279499054,0.011478279273433145
5309,26568,26568,53136,157.88466620445251,0.01089015879733779
5326,26636,26636,53272,158.30004000663757,0.009480361213718425
5344,26712,26712,53424,158.78026914596558,0.008859945262884139
5361,26780,26780,53560,159.20347118377686,0.008370275021661655
5379,26896,26896,53792,159.86822390556335,0.008171864137693774
5397,27010,27010,54020,160.51787495613098,0.008180136581358965
5414,27120,27120,54240,161.16302800178528,0.00817768545493891
5432,27248,27248,54496,161.88889908790588,0.008173308722689399
5449,27366,27366,54732,162.57725310325623,0.008171301298716571
5467,27498,27498,54996,163.3320550918579,0.008170939971023472
5485,27638,27638,55276,164.11354994773865,0.008170922150384285
5502,27762,27762,55524,164.81671810150146,0.008170397404683172
5520,27840,27840,55680,165.29429292678833,0.008162858459400013
5537,27908,27908,55816,165.72025203704834,0.008146494461470866
5555,27994,27994,55988,166.23602890968323,0.008135874093568418
5572,28126,28126,56252,166.98286700248718,0.008135730580761447
5590,28270,28270,56540,167.78539109230042,0.008135711001159507
5608,28414,28414,56828,168.59288215637207,0.008135691427014535
5625,28504,28504,57008,169.12176704406738,0.008129452146022231
5643,28576,28576,57152,169.57958602905273,0.008119266480207443
5660,28644,28644,57288,170.0054430961609,0.008113528370813583
5678,28716,28716,57432,170.4404001235962,0.00809843152637768
5695,28830,28830,57660,171.0909869670868,0.00809202471646131
5713,28972,28972,57944,171.886461019516,0.008091957608485245
5731,29116,29116,58232,172.68498396873474,0.008091938982033753
5748,29230,29230,58460,173.3424859046936,0.008089511711659725
5766,29302,29302,58604,173.78017783164978,0.008079374634689884
5783,29370,29370,58740,174.20945620536804,0.008074845376540907
5801,29442,29442,58884,174.65987610816956,0.008056907281570602
5819,29514,29514,59028,175.0967080593109,0.008007414977328153
5836,29582,29582,59164,175.51601004600525,0.00795119142094336
5854,29654,29654,59308,175.96108412742615,0.007932945951324655
5871,29722,29722,59444,176.38174414634705,0.007923986624518875
5889,29794,29794,59588,176.82802891731262,0.007913189259852516
5906,29862,29862,59724,177.25171494483948,0.00788600959640462
5924,29934,29934,59868,177.7088439464569,0.007842152186640305
5942,30012,30012,60024,178.19022011756897,0.007811032402969431
5959,30080,30080,60160,178.6309711933136,0.0077713203099847306
5977,30152,30152,60304,179.07430815696716,0.007735495979432017
5994,30220,30220,60440,179.48997902870178,0.007652421752936789
6012,30296,30296,60592,179.950679063797,0.007554743910077377
6029,30364,30364,60728,180.37750005722046,0.007499740384446341
6047,30436,30436,60872,180.8351800441742,0.007438555378030287
6065,30508,30508,61016,181.28532910346985,0.007355783289312967
6082,30576,30576,61152,181.71383023262024,0.007242336734634591
6100,30648,30648,61296,182.18061518669128,0.007210789815871976
6117,30716,30716,61432,182.61383390426636,0.007160437411585008
6135,30792,30792,61584,183.08780002593994,0.006943693364519277
6153,30868,30868,61736,183.5629198551178,0.006717043439493864
6170,30940,30940,61880,184.01540207862854,0.006535545577207813
6188,31012,31012,62024,184.46927785873413,0.006334904303002986
6205,31084,31084,62168,184.9262478351593,0.006195413048772025
6223,31158,31158,62316,185.38512301445007,0.006154844615593902
6240,31226,31226,62452,185.8141520023346,0.00604445305725676
6258,31298,31298,62596,186.2640061378479,0.005842124599439558
6276,31370,31370,62740,186.7110080718994,0.005649297345371451
6293,31442,31442,62884,187.17379093170166,0.005510435368705657
6311,31514,31514,63028,187.64945006370544,0.005373657748350524
6328,31586,31586,63172,188.1236321926117,0.005275599572996725
6346,31658,31658,63316,188.60972118377686,0.0051757395413005725
6363,31726,31726,63452,189.05004501342773,0.00503670180842164
6381,31798,31798,63596,189.52609705924988,0.004909123383185943
6399,31870,31870,63740,190.02074098587036,0.004620091784090619
6416,31938,31938,63876,190.47470784187317,0.004186211936030304
6434,32034,32034,64068,191.09317708015442,0.004099266712728422
6451,32154,32154,64308,191.82345008850098,0.004042110869704629
6469,32258,32258,64516,192.44185209274292,0.004039587853185367
6486,32374,32374,64748,193.14999103546143,0.0040383432951784926
6504,32518,32518,65036,194.07416915893555,0.004038331302581355
6522,32600,32600,65200,194.64214611053467,0.004035298074086313
6539,32670,32670,65340,195.0757281780243,0.004029777706819004
6557,32766,32766,65532,195.6422519683838,0.004026773860459798
6574,32834,32834,65668,196.07771801948547,0.004021072660179925
6592,32906,32906,65812,196.52176094055176,0.003990070053987438
6610,32978,32978,65956,196.96317887306213,0.003964629300753586
6627,33046,33046,66092,197.38338994979858,0.00394159770985425
6645,33118,33118,66236,197.8403241634369,0.0039279970314964885
6662,33186,33186,66372,198.26970314979553,0.003907657994204783
6680,33258,33258,66516,198.71776795387268,0.0038851795143273193
6697,33326,33326,66652,199.1416370868683,0.0038764416312915273
6715,33398,33398,66796,199.59131503105164,0.0038664105431962525
6733,33470,33470,66940,200.04475378990173,0.003853693833661964
6750,33538,33538,67076,200.47167420387268,0.00384491323166003
6768,33610,33610,67220,200.9136519432068,0.0038315946239890764
6785,33678,33678,67356,201.34684205055237,0.0038242170703597367
6803,33750,33750,67500,201.79806995391846,0.0038155211150296964
6820,33818,33818,67636,202.21934509277344,0.0038113771752250614
6838,33890,33890,67780,202.67801809310913,0.0037995540551492013
6856,33962,33962,67924,203.11886310577393,0.003781776094911038
6873,34030,34030,68060,203.5418210029602,0.0037552217254415154
6891,34102,34102,68204,203.98447799682617,0.003737160002856399
6908,34170,34170,68340,204.40234899520874,0.0037210530226730043
6926,34242,34242,68484,204.85165214538574,0.0037025295769126387
6944,34314,34314,68628,205.29064297676086,0.003687470116346958
6961,34382,34382,68764,205.79144406318665,0.0036603408116206992
6979,34454,34454,68908,206.23673486709595,0.00364053996054281
6996,34522,34522,69044,206.67499899864197,0.0036237539916328387
7014,34594,34594,69188,207.1325650215149,0.0035862187814927893
7031,34662,34662,69324,207.56559109687805,0.0035538304637157125
7049,34734,34734,69468,208.0306429862976,0.003481805484625511
7067,34806,34806,69612,208.48696899414062,0.0034582694843265926
7084,34874,34874,69748,208.91766905784607,0.00342713249483495
7102,34946,34946,69892,209.39818596839905,0.003360558217536891
7119,35014,35014,70028,209.8230540752411,0.003275851282523945
7137,35086,35086,70172,210.28209400177002,0.003178304777975427
7154,35154,35154,70308,210.702810049057,0.0030798253064858727
7172,35226,35226,70452,211.15587496757507,0.0030357458508660784
7190,35352,35352,70704,211.87515592575073,0.0030222718778532
7207,35474,35474,70948,212.56598901748657,0.003022025795871741
7225,35614,35614,71228,213.37332391738892,0.003021984330189298
7242,35708,35708,71416,213.92241883277893,0.0030213120953703765
7260,35782,35782,71564,214.38041591644287,0.0030204085778677836
7278,35854,35854,71708,214.83151197433472,0.0030191782425390556
7295,35922,35922,71844,215.24862003326416,0.0030154550968291005
7313,35994,35994,71988,215.70488214492798,0.003008557207067497
7330,36062,36062,72124,216.1262969970703,0.0030046626889088657
7348,36134,36134,72268,216.55832695960999,0.0030010210484761046
7365,36202,36202,72404,216.97973203659058,0.002996529256051872
7383,36274,36274,72548,217.4153871536255,0.0029892684196966
7401,36346,36346,72692,217.8757610321045,0.0029776458777632797
7418,36414,36414,72828,218.30001401901245,0.002965821484394837
7436,36486,36486,72972,218.74509596824646,0.0029605413328681607
7453,36554,36554,73108,219.16454195976257,0.0029565419936261605
7471,36626,36626,73252,219.6051061153412,0.0029518049814214464
7488,36694,36694,73388,220.04410696029663,0.0029450468719005585
7506,36766,36766,73532,220.47873306274414,0.002926752718849457
7524,36838,36838,73676,220.91318082809448,0.0029176470397942467
7541,36906,36906,73812,221.33536314964294,0.0029020361689617857
7559,36978,36978,73956,221.7783968448639,0.0028838900434493553
7576,37046,37046,74092,222.20946192741394,0.002861809267415083
7594,37118,37118,74236,222.65412187576294,0.002817647155097802
7612,37190,37190,74380,223.10288000106812,0.002784195490676211
7629,37258,37258,74516,223.52048802375793,0.0027581742506299634
7647,37330,37330,74660,223.95103788375854,0.002725969583480037
7664,37400,37400,74800,224.39624691009521,0.002677054344530916
7682,37472,37472,74944,224.83997702598572,0.0026507882812438766
7699,37540,37540,75080,225.26056504249573,0.002614579763758229
7717,37612,37612,75224,225.70110297203064,0.0025389223392267013
7735,37684,37684,75368,226.15409088134766,0.0023649565173400333
7752,37754,37754,75508,226.5911250114441,0.0022144558733998565
7770,37826,37826,75652,227.03689002990723,0.002087119990392239
7787,37900,37900,75800,227.49165511131287,0.0018970614910358563
7805,37988,37988,75976,228.01623916625977,0.0016976477418211289
7822,38110,38110,76220,228.70877695083618,0.001695095614195452
7840,38248,38248,76496,229.4879879951477,0.0016950179706327617
7858,38392,38392,76784,230.28879618644714,0.0016950116969383089
7875,38454,38454,76908,230.69243597984314,0.0016905606662476202
7893,38526,38526,77052,231.15338706970215,0.0016900438731681788
7910,38594,38594,77188,231.57673001289368,0.0016893879437702708
7928,38666,38666,77332,232.02274203300476,0.0016883714888535906
7946,38738,38738,77476,232.458172082901,0.0016870250274223508
7963,38806,38806,77612,232.88303518295288,0.0016861135372892022
7981,38878,38878,77756,233.3412630558014,0.0016848885679792147
7998,38946,38946,77892,233.75241208076477,0.0016829090636747424
8016,39018,39018,78036,234.2042829990387,0.001680854549704236
8033,39086,39086,78172,234.617928981781,0.0016776471238699742
8051,39158,39158,78316,235.07199692726135,0.0016722034615668235
8069,39230,39230,78460,235.5247721672058,0.0016686677627149038
8086,39298,39298,78596,235.94563508033752,0.0016669047381583368
8104,39370,39370,78740,236.38514494895935,0.0016573666034673806
8121,39438,39438,78876,236.79933404922485,0.001647879771553562
8139,39510,39510,79020,237.2606270313263,0.0016294463694066508
8156,39578,39578,79156,237.6875069141388,0.0016166757668543141
8174,39650,39650,79300,238.13563108444214,0.001601913025297108
8192,39722,39722,79444,238.59161901474,0.0015865312016103417
8209,39790,39790,79580,239.01021313667297,0.001580852089318796
8227,39862,39862,79724,239.4533019065857,0.0015664552011003252
8244,39930,39930,79860,239.88110208511353,0.0015535499405814335
8262,40002,40002,80004,240.3205590248108,0.0015541652755928226
8280,40074,40074,80148,240.76506304740906,0.0015343930244853254
8297,40142,40142,80284,241.18977308273315,0.0015190195063041756
8315,40214,40214,80428,241.64485907554626,0.00150893130012264
8332,40286,40286,80572,242.08255004882812,0.001490674976594164
8350,40382,40382,80764,242.6490020751953,0.0014778006661799736
8367,40500,40500,81000,243.3128640651703,0.0014789859360462287
8385,40628,40628,81256,244.06019616127014,0.0014785840085096424
8403,40768,40768,81536,244.85751509666443,0.001478671700169798
8420,40900,40900,81800,245.60486388206482,0.0014777528631384484
8438,41040,41040,82080,246.40218806266785,0.0014776787284063175
8455,41174,41174,82348,247.17049288749695,0.0014776770094613312
8473,41318,41318,82636,248.00115084648132,0.0014776734242332168
8490,41444,41444,82888,248.7249038219452,0.0014775723921047756
8508,41528,41528,83056,249.24086022377014,0.0014766865915589733
8526,41600,41600,83200,249.6926920413971,0.0014746030210517347
8543,41668,41668,83336,250.1240701675415,0.0014705532321386272
8561,41740,41740,83480,250.59250807762146,0.0014613480689149583
8578,41808,41808,83616,251.0169689655304,0.001456582695027464
8596,41880,41880,83760,251.46322894096375,0.0014520109707518714
8614,41976,41976,83952,252.03485298156738,0.001447796526917955
8631,42094,42094,84188,252.70384001731873,0.001447954740797286
8649,42212,42212,84424,253.4076120853424,0.0014478724042419344
8666,42346,42346,84692,254.17509293556213,0.0014477140794042498
8684,42488,42488,84976,255.26796007156372,0.0014476913656835677
8701,42624,42624,85248,256.03619289398193,0.0014476880824076943
8719,42766,42766,85532,256.82829904556274,0.0014476831256615696
8737,42910,42910,85820,257.6367690563202,0.0014476796495728195
8754,43038,43038,86076,258.3566892147064,0.0014467047221842222
8772,43122,43122,86244,258.8681719303131,0.0014433751130127348
8789,43190,43190,86380,259.30317401885986,0.0014412937525776215
8807,43262,43262,86524,259.74973320961,0.0014408285151148448
8824,43330,43330,86660,260.16955494880676,0.0014396651276911143
8842,43402,43402,86804,260.6181402206421,0.00143824301812856
8860,43474,43474,86948,261.06806802749634,0.001437261898900033
8877,43542,43542,87084,261.5037889480591,0.0014355462535604602
8895,43614,43614,87228,261.9468448162079,0.0014314974832814187
8912,43682,43682,87364,262.3651828765869,0.0014208963420969667
8930,43754,43754,87508,262.8012809753418,0.0014110976408119313
8947,43822,43822,87644,263.2201430797577,0.0013869471677026013
8965,43894,43894,87788,263.68461298942566,0.0013237965376902139
8983,43966,43966,87932,264.1311049461365,0.0012812032418878516
9000,44034,44034,88068,264.5462441444397,0.0012626292791537708
9018,44106,44106,88212,265.0093159675598,0.0012593337032740237
9035,44174,44174,88348,265.41939997673035,0.0012465621184674092
9053,44246,44246,88492,265.8746769428253,0.0012320387013460277
9071,44318,44318,88636,266.3075420856476,0.001217236917000264
9088,44386,44386,88772,266.7331099510193,0.0012121684976591496
9106,44458,44458,88916,267.1724269390106,0.0012015514657832682
9123,44530,44530,89060,267.61313104629517,0.0011883013721671887
9141,44602,44602,89204,268.065447807312,0.001157748100013123
9158,44670,44670,89340,268.4849531650543,0.0011250974330323515
9176,44742,44742,89484,268.9287760257721,0.0010532398719078628
9194,44814,44814,89628,269.3716778755188,0.0009688213795016054
9211,44882,44882,89764,269.78682017326355,0.000904743783394224
9229,44954,44954,89908,270.2385039329529,0.0008737725311220856
9246,45026,45026,90052,270.6846570968628,0.0008357916831300827
9264,45102,45102,90204,271.1519470214844,0.0007303331767616328
9281,45170,45170,90340,271.58580708503723,0.0007268191584444139
9299,45242,45242,90484,272.03606510162354,0.0006561591617355589
9317,45318,45318,90636,272.5163850784302,0.0005036812381149502
9334,45392,45392,90784,272.9617249965668,0.0004523912193690194
9352,45468,45468,90936,273.419771194458,0.00036558655119733885
9369,45536,45536,91072,273.84405493736267,0.0002830583780450979
9387,45638,45638,91276,274.4509561061859,0.00024119429326674435
9405,45744,45744,91488,275.0829141139984,0.00024864643819455523
9422,45840,45840,91680,275.6311228275299,0.0002454401364957448
9440,45972,45972,91944,276.37260603904724,0.0002520927409932483
9457,46090,46090,92180,277.0539610385895,0.00024066955847956706
9475,46200,46200,92400,277.6826000213623,0.00024274415227409918
9492,46314,46314,92628,278.33503794670105,0.0002410593442618847
9510,46438,46438,92876,279.0493860244751,0.0002403953294560779
9528,46574,46574,93148,279.8015179634094,0.00024039613708737306
9545,46702,46702,93404,280.5305540561676,0.00024039545496634673
9563,46844,46844,93688,281.3238480091095,0.0002403938415227458
9580,46972,46972,93944,282.0533890724182,0.000240077437410946
9598,47032,47032,94064,282.44266390800476,0.00023962733030202799
9615,47098,47098,94196,282.8607852458954,0.00023943864653119817
9633,47170,47170,94340,283.3153541088104,0.0002391540056123631
9651,47240,47240,94480,283.77162504196167,0.00023865421098889783
9668,47310,47310,94620,284.21414399147034,0.00023833375234971754
9686,47382,47382,94764,284.66203904151917,0.0002380777496000519
9703,47450,47450,94900,285.09081387519836,0.000237802119954722
9721,47522,47522,95044,285.55673694610596,0.0002370625861658482
9739,47594,47594,95188,286.00532603263855,0.00023574416627525352
9756,47702,47702,95404,286.6274869441986,0.0002349266505916603
9774,47794,47794,95588,287.17506885528564,0.000234790355534642
9791,47928,47928,95856,287.9313440322876,0.00023478883122152183
9809,48052,48052,96104,288.648638010025,0.0002347317185922293
9826,48154,48154,96308,289.23221707344055,0.0002344589156564325
9844,48298,48298,96596,290.05710792541504,0.00023445827719115186
9862,48428,48428,96856,290.78179597854614,0.00023442374003934674
9879,48496,48496,96992,291.20616006851196,0.00023430288820236456
9897,48568,48568,97136,291.65761613845825,0.00023271836653293576
9914,48636,48636,97272,292.0907380580902,0.00023137012613005936
9932,48708,48708,97416,292.53445291519165,0.00023072879230312537
9949,48776,48776,97552,292.9446110725403,0.0002285295158799272
9967,48848,48848,97696,293.39341592788696,0.00022634949345956556
9985,48920,48920,97840,293.83472895622253,0.0002238841298094485
10002,48988,48988,97976,294.2660129070282,0.00022367535348166712
10020,49060,49060,98120,294.7095820903778,0.000223223551074625
10037,49128,49128,98256,295.1369888782501,0.0002226449578301981
10055,49200,49200,98400,295.5899691581726,0.00022224232270673383
10073,49272,49272,98544,296.0454828739166,0.0002218363206338836
10090,49340,49340,98680,296.47853684425354,0.00022142099624034017
10108,49416,49416,98832,296.94588899612427,0.00022127771080704406
10125,49484,49484,98968,297.3762800693512,0.00022109189194452483
10143,49560,49560,99120,297.8484752178192,0.00022061208437662572
10160,49628,49628,99256,298.26730394363403,0.00022029256797395647
10178,49700,49700,99400,298.71511006355286,0.00021981890859024134
10196,49772,49772,99544,299.15923404693604,0.00021889450727030635
10213,49840,49840,99680,299.5847120285034,0.0002175496756535722
10231,49912,49912,99824,300.0163309574127,0.00021617931997752748
10248,49980,49980,99960,300.43440890312195,0.00021273571292113047
10266,50052,50052,100104,300.882737159729,0.000205797994567547
10283,50120,50120,100240,301.29133200645447,0.00020037022295582574
10301,50192,50192,100384,301.73591899871826,0.00019491208331601229
10319,50264,50264,100528,302.1772999763489,0.00018904679745901376
10336,50332,50332,100664,302.60194087028503,0.00018238758275401779
10354,50404,50404,100808,303.0472528934479,0.0001709638090687804
10371,50472,50472,100944,303.4609489440918,0.0001599399056431139
10389,50544,50544,101088,303.8988130092621,0.00014700911196996458
10407,50618,50618,101236,304.3497290611267,0.00014114294026512653
10424,50686,50686,101372,304.77114391326904,0.00014007023128215224
10442,50762,50762,101524,305.2404520511627,0.00012189529479655903
10459,50830,50830,101660,305.6557459831238,0.0001148887076851679
10477,50902,50902,101804,306.10032510757446,0.00010475193084857892
10494,51008,51008,102016,306.71082401275635,0.000103642374597257
10512,51138,51138,102276,307.45897221565247,0.00010342069435864687
10530,51242,51242,102484,308.0726499557495,0.00010336796185583808
10547,51378,51378,102756,308.81920623779297,0.00010336759078199975
10565,51454,51454,102908,309.2947430610657,0.00010324814684281591
10582,51522,51522,103044,309.7150650024414,0.00010321127047063783
10600,51594,51594,103188,310.1639349460602,0.00010316825137124397
10617,51662,51662,103324,310.5826590061188,0.00010312612539564725
10635,51734,51734,103468,311.0243079662323,0.00010299366840627044
10653,51806,51806,103612,311.4759521484375,0.00010250188097415958
10670,51874,51874,103748,311.90017199516296,0.00010184966413362417
10688,51946,51946,103892,312.3523051738739,0.00010166763422603253
10705,52014,52014,104028,312.76515102386475,0.00010141648999706376
10723,52086,52086,104172,313.2082450389862,0.00010090160867548548
10741,52158,52158,104316,313.66693091392517,0.00010045789349533152
10758,52226,52226,104452,314.0883700847626,0.00010023588220064994
10776,52298,52298,104596,314.54194712638855,0.00010003837996919174
10793,52366,52366,104732,314.9696629047394,9.971853251045104e-05
10811,52438,52438,104876,315.40252900123596,9.915515511238482e-05
10828,52506,52506,105012,315.83110904693604,9.884091377898585e-05
10846,52578,52578,105156,316.288724899292,9.877719276119024e-05
10864,52650,52650,105300,316.7293059825897,9.859442798187956e-05
10881,52720,52720,105440,317.1635630130768,9.824397966440301e-05
10899,52792,52792,105584,317.6043050289154,9.76749124674825e-05
10916,52860,52860,105720,318.0371539592743,9.754752863955218e-05
10934,52932,52932,105864,318.4813129901886,9.730656347528566e-05
10951,53000,53000,106000,318.9026801586151,9.71981389739085e-05
10969,53072,53072,106144,319.3499331474304,9.691367449704558e-05
10987,53144,53144,106288,319.7840430736542,9.659554234531242e-05
11004,53212,53212,106424,320.2171981334686,9.638520896260161e-05
11022,53284,53284,106568,320.66186594963074,9.581505582900718e-05
11039,53356,53356,106712,321.10296297073364,9.559195132169407e-05
11057,53428,53428,106856,321.5461881160736,9.505678463028744e-05
11075,53500,53500,107000,321.99758100509644,9.463752030569594e-05
11092,53568,53568,107136,322.4241452217102,9.378116010339e-05
11110,53640,53640,107280,322.85344099998474,9.355902511742897e-05
11127,53708,53708,107416,323.26676082611084,9.26680750126252e-05
11145,53780,53780,107560,323.7129981517792,9.13631356525002e-05
11162,53848,53848,107696,324.14174699783325,9.088255501410458e-05
11180,53920,53920,107840,324.59850811958313,9.00181275937939e-05
11198,53992,53992,107984,325.04811120033264,8.936119593272451e-05
11215,54060,54060,108120,325.4686179161072,8.837439054332208e-05
11233,54132,54132,108264,325.905305147171,8.801575313555077e-05
11250,54200,54200,108400,326.31748604774475,8.69482355483342e-05
11268,54272,54272,108544,326.7752799987793,8.477127266814932e-05
11285,54340,54340,108680,327.2001910209656,8.12177240732126e-05
11303,54416,54416,108832,327.6695590019226,7.731395817245357e-05
11321,54488,54488,108976,328.11119318008423,7.294298666238319e-05
11338,54556,54556,109112,328.52862524986267,7.007899512245785e-05
11356,54628,54628,109256,328.98190903663635,6.30374106549425e-05
11373,54696,54696,109392,329.4003219604492,5.7625964473118074e-05
11391,54766,54766,109532,329.83529806137085,4.69499354949221e-05
11408,54834,54834,109668,330.25649189949036,4.091543814865872e-05
11426,54906,54906,109812,330.6993169784546,3.989858851127792e-05
11444,54974,54974,109948,331.14095091819763,3.645724427769892e-05
11461,55040,55040,110080,331.5488979816437,2.8676089641521685e-05
11479,55106,55106,110212,331.96558594703674,2.3979244360816665e-05
11496,55168,55168,110336,332.36027002334595,1.8356442524236627e-05
11514,55240,55240,110480,332.80074310302734,1.677115142229013e-05
11532,55310,55310,110620,333.24342918395996,1.6061732821981423e-05
11549,55378,55378,110756,333.6677510738373,1.6867881640791893e-05
11567,55442,55442,110884,334.0772850513458,1.363454430247657e-05
11584,55506,55506,111012,334.47969102859497,1.1780237400671467e-05
11602,55576,55576,111152,334.90942001342773,1.1317115422571078e-05
11619,55640,55640,111280,335.30877113342285,9.78926800598856e-06
11637,55708,55708,111416,335.7449531555176,7.999313311302103e-06
11655,55778,55778,111556,336.1932919025421,6.615675374632701e-06
11672,55846,55846,111692,336.61773014068604,5.493222488439642e-06
11690,55916,55916,111832,337.0620369911194,5.012418114347383e-06
11707,55984,55984,111968,337.47475004196167,4.788058504345827e-06
11725,56056,56056,112112,337.96133303642273,3.994640792370774e-06
11742,56122,56122,112244,338.376051902771,3.524299245327711e-06
11760,56190,56190,112380,338.80019998550415,2.6945363060804084e-06
11778,56254,56254,112508,339.21297311782837,2.080601916532032e-06
11795,56312,56312,112624,339.5832939147949,1.6603898984612897e-06
11813,56374,56374,112748,339.99017000198364,1.2346663424978033e-06
11830,56428,56428,112856,340.32919812202454,5.49189280718565e-07
11848,56488,56488,112976,340.7160098552704,2.2394669940695167e-07
11866,56550,56550,113100,341.11321210861206,1.7676211427897215e-07
11883,56602,56602,113204,341.4483959674835,7.389462552964687e-08
11901,56662,56662,113324,341.8332860469818,7.536800694651902e-08
11918,56718,56718,113436,342.20435094833374,5.477704689837992e-08
11936,56782,56782,113564,342.61551785469055,3.713830665219575e-08
11953,56840,56840,113680,342.98881793022156,2.74376361630857e-08
11971,56898,56898,113796,343.3552739620209,1.5519617591053247e-08
11989,56960,56960,113920,343.7490129470825,1.3489625416696072e-08
12006,57024,57024,114048,344.1659698486328,1.1497832019813359e-08
12024,57088,57088,114176,344.57024097442627,1.0459189070388675e-08
12041,57146,57146,114292,344.93530011177063,9.897121344693005e-09
12059,57214,57214,114428,345.3643569946289,1.0144503903575242e-08
12076,57276,57276,114552,345.7522349357605,1.0601070243865252e-08
12094,57336,57336,114672,346.1397738456726,1.1033989721909165e-08
12112,57400,57400,114800,346.56052803993225,1.2096279533579946e-08
12129,57468,57468,114936,346.9719910621643,1.2239979696460068e-08
12147,57534,57534,115068,347.38385701179504,1.1772499419748783e-08
12164,57604,57604,115208,347.81546998023987,1.1394149623811245e-08
12182,57674,57674,115348,348.24487709999084,1.1063093552365899e-08
12200,57750,57750,115500,348.7126362323761,1.0990333976224065e-08
12217,57816,57816,115632,349.12638306617737,1.0952135198749602e-08
12235,57882,57882,115764,349.5457270145416,1.0804797057062387e-08
12252,57942,57942,115884,349.91609501838684,1.0479197953827679e-08
12270,58002,58002,116004,350.2870240211487,1.0275471140630543e-08
12287,58070,58070,116140,350.78876304626465,1.0111762094311416e-08
12305,58140,58140,116280,351.2380449771881,1.0029907571151853e-08
12323,58206,58206,116412,351.67058086395264,9.78070602286607e-09
12340,58270,58270,116540,352.08577609062195,9.516952559351921e-09
12358,58342,58342,116684,352.5355272293091,9.43873601499945e-09
12375,58410,58410,116820,352.9610469341278,9.391442290507257e-09
12393,58480,58480,116960,353.3968198299408,9.265932021662593e-09
12410,58548,58548,117096,353.8126268386841,9.07857611309737e-09
12428,58620,58620,117240,354.25100207328796,8.947608876042068e-09
12446,58692,58692,117384,354.69634199142456,8.87666828930378e-09
12463,58764,58764,117528,355.15522503852844,8.813003660179675e-09
12481,58840,58840,117680,355.62704706192017,8.8020897237584e-09
12498,58910,58910,117820,356.06824493408203,8.77116690389812e-09
12516,58986,58986,117972,356.53270387649536,8.747520041652024e-09
12534,59066,59066,118132,357.02104806900024,8.70932126417756e-09
12551,59138,59138,118276,357.47382712364197,8.700226317159832e-09
12569,59214,59214,118428,357.9383909702301,8.702045306563377e-09
12586,59296,59296,118592,358.42308616638184,8.698407327756286e-09
12604,59374,59374,118748,358.89332818984985,8.694769348949194e-09
12621,59446,59446,118892,359.3347849845886,8.689312380738556e-09
12639,59538,59538,119076,359.889906167984,8.682036423124373e-09
12657,59614,59614,119228,360.34460496902466,8.656570571474731e-09
12674,59702,59702,119404,360.8629810810089,8.647475624457002e-09
12692,59810,59810,119620,361.5025670528412,8.642018656246364e-09
12709,59894,59894,119788,362.00697803497314,8.623828762210906e-09
12727,59984,59984,119968,362.54458379745483,8.620190783403814e-09
12744,60066,60066,120132,363.0304071903229,8.611095836386085e-09
12762,60158,60158,120316,363.5738790035248,8.605638868175447e-09
12780,60266,60266,120532,364.2073760032654,8.60018189996481e-09
12797,60352,60352,120704,364.71674704551697,8.594724931754172e-09
12815,60442,60442,120884,365.2546350955963,8.585629984736443e-09
12832,60526,60526,121052,365.7570490837097,8.580173016525805e-09
12850,60602,60602,121204,366.2291069030762,8.571078069508076e-09
12868,60686,60686,121372,366.72724199295044,8.5601641330868e-09
12885,60764,60764,121528,367.1903910636902,8.541974239051342e-09
12903,60862,60862,121724,367.77194380760193,8.521965355612338e-09
12920,60948,60948,121896,368.29545283317566,8.50741344038397e-09
12938,61032,61032,122064,368.79594588279724,8.500137482769787e-09
12955,61118,61118,122236,369.2950110435486,8.480128599330783e-09
12973,61212,61212,122424,369.8552601337433,8.456481737084687e-09
12991,61300,61300,122600,370.3909249305725,8.434653864242136e-09
13008,61400,61400,122800,370.98450994491577,8.425558917224407e-09
13026,61490,61490,122980,371.53358793258667,8.363713277503848e-09
13043,61572,61572,123144,372.03139996528625,8.303686627186835e-09
13061,61658,61658,123316,372.55646204948425,8.247297955676913e-09
13078,61742,61742,123484,373.0532238483429,8.176357368938625e-09
13096,61826,61826,123652,373.5559780597687,8.096321835182607e-09
13114,61910,61910,123820,374.0685098171234,8.078131941147149e-09
13131,61986,61986,123972,374.5836081504822,7.979906513355672e-09
13149,62074,62074,124148,375.1235771179199,7.856215233914554e-09
13166,62158,62158,124316,375.6333291530609,7.719791028648615e-09
13184,62250,62250,124500,376.183562040329,7.654307410120964e-09
13202,62348,62348,124696,376.78191685676575,7.585185812786222e-09
13219,62442,62442,124884,377.34219694137573,7.45421857573092e-09
13237,62524,62524,125048,377.8477449417114,7.374183041974902e-09
13254,62596,62596,125192,378.28739619255066,7.201379048638046e-09
13272,62672,62672,125344,378.771653175354,7.17773218639195e-09
13289,62754,62754,125508,379.2717502117157,7.117705536074936e-09
13307,62830,62830,125660,379.7417299747467,7.037670002318919e-09
13325,62912,62912,125824,380.2275900840759,7.0140231400728226e-09
13342,62988,62988,125976,380.6891050338745,7.008566171862185e-09
13360,63070,63070,126140,381.1955900192261,6.884874892421067e-09
13377,63146,63146,126292,381.6649498939514,6.76482159178704e-09
13395,63222,63222,126444,382.1294798851013,6.515620043501258e-09
13412,63290,63290,126580,382.5504870414734,6.280970410443842e-09
13430,63372,63372,126744,383.0476861000061,6.088157533667982e-09
13448,63450,63450,126900,383.52926683425903,5.888068699277937e-09
13465,63526,63526,127052,383.97959899902344,5.7098077377304435e-09
13483,63604,63604,127208,384.44085907936096,5.2787072490900755e-09
13500,63672,63672,127344,384.8569190502167,5.034962669014931e-09
13518,63752,63752,127504,385.34279108047485,4.86397766508162e-09
13536,63828,63828,127656,385.80226707458496,4.585672286339104e-09
13553,63896,63896,127792,386.2326190471649,4.380126483738422e-09
13571,63972,63972,127944,386.6943008899689,3.965396899729967e-09
13588,64040,64040,128080,387.1222689151764,3.941750037483871e-09
13606,64112,64112,128224,387.55932807922363,3.6598066799342632e-09
13623,64184,64184,128368,388.01223492622375,3.445165930315852e-09
13641,64256,64256,128512,388.4551019668579,3.246896085329354e-09
13659,64328,64328,128656,388.8964750766754,2.6393536245450377e-09
13676,64400,64400,128800,389.32992005348206,2.3410393623635173e-09
13694,64470,64470,128940,389.76746106147766,2.042725100181997e-09
13711,64540,64540,129080,390.21354389190674,1.6061676433309913e-09
13729,64612,64612,129224,390.652636051178,1.5661498764529824e-09
13746,64680,64680,129360,391.0710279941559,1.4424585970118642e-09
13764,64758,64758,129516,391.54775190353394,1.2205418897792697e-09
13782,64828,64828,129656,391.97892808914185,9.49512468650937e-10
13799,64900,64900,129800,392.4260129928589,8.549250196665525e-10
13817,64968,64968,129936,392.8543019294739,7.548806024715304e-10
13834,65032,65032,130064,393.2503969669342,6.912159733474255e-10
13852,65104,65104,130208,393.698566198349,6.784830475226045e-10
13869,65174,65174,130348,394.13183403015137,6.657501216977835e-10
13887,65256,65256,130512,394.6343080997467,6.639311322942376e-10
13905,65326,65326,130652,395.0708920955658,6.657501216977835e-10
13922,65386,65386,130772,395.4371500015259,6.821210263296962e-10
13940,65458,65458,130916,395.881227016449,6.96672941558063e-10
13957,65534,65534,131068,396.34519386291504,7.112248567864299e-10
13975,65608,65608,131216,396.8054687976837,7.22138793207705e-10
13993,65680,65680,131360,397.24649691581726,7.275957614183426e-10
14010,65762,65762,131524,397.7366211414337,7.257767720147967e-10
14028,65838,65838,131676,398.2167510986328,7.275957614183426e-10
14045,65910,65910,131820,398.66164207458496,7.166818249970675e-10
14063,65988,65988,131976,399.1421160697937,7.166818249970675e-10
14080,66064,66064,132128,399.59959506988525,7.185008144006133e-10
14098,66144,66144,132288,400.08025217056274,7.112248567864299e-10
14116,66226,66226,132452,400.5742530822754,7.148628355935216e-10
14133,66312,66312,132624,401.09697103500366,7.130438461899757e-10
14151,66398,66398,132796,401.60869097709656,7.057678885757923e-10
14168,66474,66474,132948,402.0704929828644,7.057678885757923e-10
14186,66560,66560,133120,402.58385825157166,7.075868779793382e-10
14203,66636,66636,133272,403.05891704559326,7.075868779793382e-10
14221,66710,66710,133420,403.5173370838165,6.96672941558063e-10
14239,66786,66786,133572,403.9763288497925,6.893969839438796e-10
14256,66862,66862,133724,404.4338631629944,6.857590051367879e-10
14274,66956,66956,133912,404.9949131011963,6.803020369261503e-10
14291,67032,67032,134064,405.46851921081543,6.784830475226045e-10
14309,67140,67140,134280,406.09042406082153,6.766640581190586e-10
14327,67226,67226,134452,406.60156416893005,6.730260793119669e-10
14344,67308,67308,134616,407.0906710624695,6.675691111013293e-10
14362,67394,67394,134788,407.61927700042725,6.621121428906918e-10
14379,67482,67482,134964,408.131224155426,6.621121428906918e-10
14397,67566,67566,135132,408.63950419425964,6.566551746800542e-10
14414,67650,67650,135300,409.1297469139099,6.566551746800542e-10
14432,67748,67748,135496,409.7136290073395,6.548361852765083e-10
14450,67836,67836,135672,410.24290704727173,6.530171958729625e-10
14467,67932,67932,135864,410.80012583732605,6.511982064694166e-10
14485,68008,68008,136016,411.27218103408813,6.493792170658708e-10
14502,68088,68088,136176,411.76123809814453,6.45741238258779e-10
14520,68190,68190,136380,412.358717918396,6.421032594516873e-10
14537,68266,68266,136532,412.81666898727417,6.348273018375039e-10
14555,68370,68370,136740,413.43403601646423,6.330083124339581e-10
14573,68472,68472,136944,414.03968715667725,6.330083124339581e-10
14590,68558,68558,137116,414.5464520454407,6.293703336268663e-10
14608,68656,68656,137312,415.12228083610535,6.257323548197746e-10
14625,68732,68732,137464,415.5786349773407,6.220943760126829e-10
14643,68824,68824,137648,416.13301396369934,6.184563972055912e-10
14661,68916,68916,137832,416.6749920845032,6.166374078020453e-10
14678,68998,68998,137996,417.1590600013733,6.129994289949536e-10
14696,69088,69088,138176,417.6977798938751,6.057234713807702e-10
14713,69188,69188,138376,418.2852919101715,6.057234713807702e-10
14731,69292,69292,138584,418.9085569381714,6.020854925736785e-10
14748,69376,69376,138752,419.32754611968994,6.002665031701326e-10
14766,69468,69468,138936,419.70752000808716,6.002665031701326e-10
14784,69568,69568,139136,420.2383668422699,5.948095349594951e-10
14801,69678,69678,139356,420.93699979782104,5.966285243630409e-10
14819,69778,69778,139556,421.61164116859436,5.966285243630409e-10
14836,69864,69864,139728,422.1672029495239,5.929905455559492e-10
14854,69958,69958,139916,422.74544882774353,5.911715561524034e-10
14871,70030,70030,140060,423.2034192085266,5.893525667488575e-10
14889,70116,70116,140232,423.73933696746826,5.838955985382199e-10
14907,70202,70202,140404,424.27164697647095,5.802576197311282e-10
14924,70296,70296,140592,424.8629779815674,5.784386303275824e-10
14942,70394,70394,140788,425.4918301105499,5.711626727133989e-10
14959,70468,70468,140936,425.96573209762573,5.566107574850321e-10
14977,70554,70554,141108,426.5047228336334,5.420588422566652e-10
14995,70636,70636,141272,427.0237410068512,5.275069270282984e-10
15012,70748,70748,141496,427.68577098846436,5.238689482212067e-10
15030,70832,70832,141664,428.2180678844452,5.165929906070232e-10
15047,70918,70918,141836,428.76767897605896,5.07498043589294e-10
15065,71000,71000,142000,429.3991050720215,5.056790541857481e-10
15082,71084,71084,142168,429.84851598739624,4.94765117764473e-10
15100,71170,71170,142340,430.32856917381287,4.929461283609271e-10
15118,71260,71260,142520,430.96519589424133,4.984030965715647e-10
15135,71332,71332,142664,431.5500102043152,4.965841071680188e-10
15153,71416,71416,142832,432.19306325912476,4.856701707467437e-10
15170,71504,71504,143008,432.7588551044464,4.765752237290144e-10
15188,71588,71588,143176,433.30138397216797,4.5838532969355583e-10
15205,71664,71664,143328,433.8081030845642,4.5292836148291826e-10
15223,71746,71746,143492,434.37489891052246,4.43833414465189e-10
15241,71830,71830,143660,434.91682505607605,4.3655745685100555e-10
15258,71922,71922,143844,435.5434250831604,4.2382453102618456e-10
15276,72002,72002,144004,436.0765309333801,4.147295840084553e-10
15293,72104,72104,144208,436.70938205718994,4.092726157978177e-10
15311,72196,72196,144392,437.2989430427551,4.0745362639427185e-10
15329,72276,72276,144552,437.8275079727173,3.9472070056945086e-10
15346,72356,72356,144712,438.35712003707886,3.892637323588133e-10
15364,72456,72456,144912,438.99555921554565,3.8562575355172157e-10
15381,72536,72536,145072,439.50918102264404,3.8198777474462986e-10
15399,72628,72628,145256,440.0900819301605,3.7834979593753815e-10
15416,72712,72712,145424,440.6483860015869,3.728928277269006e-10
15434,72804,72804,145608,441.23346495628357,3.6925484891980886e-10
15452,72898,72898,145796,441.82425594329834,3.728928277269006e-10
15469,72986,72986,145972,442.3923919200897,3.710738383233547e-10
15487,73092,73092,146184,443.0391962528229,3.6561687011271715e-10
15504,73176,73176,146352,443.59133410453796,3.67435859516263e-10
15522,73260,73260,146520,444.12137484550476,3.67435859516263e-10
15539,73346,73346,146692,444.68535017967224,3.6561687011271715e-10
15557,73430,73430,146860,445.22390818595886,3.6561687011271715e-10
15575,73516,73516,147032,445.77087688446045,3.6561687011271715e-10
15592,73600,73600,147200,446.3084089756012,3.6197889130562544e-10
15610,73688,73688,147376,446.8800208568573,3.6197889130562544e-10
15627,73778,73778,147556,447.44548201560974,3.6197889130562544e-10
15645,73860,73860,147720,447.97000002861023,3.601599019020796e-10
15663,73940,73940,147880,448.49221086502075,3.583409124985337e-10
15680,74024,74024,148048,449.03001403808594,3.5652192309498787e-10
15698,74112,74112,148224,449.5948979854584,3.583409124985337e-10
15715,74190,74190,148380,450.0838530063629,3.583409124985337e-10
15733,74292,74292,148584,450.7187809944153,3.5652192309498787e-10
15750,74396,74396,148792,451.3751950263977,3.5652192309498787e-10
15768,74496,74496,148992,452.01466393470764,3.5652192309498787e-10
15786,74604,74604,149208,452.70705103874207,3.5652192309498787e-10
15803,74708,74708,149416,453.35921001434326,3.5652192309498787e-10
15821,74810,74810,149620,454.00413703918457,3.54702933691442e-10
15838,74894,74894,149788,454.52926802635193,3.54702933691442e-10
15856,74984,74984,149968,455.0930528640747,3.54702933691442e-10
15873,75102,75102,150204,455.7884290218353,3.54702933691442e-10
15891,75208,75208,150416,456.43153619766235,3.54702933691442e-10
15909,75326,75326,150652,457.1358001232147,3.54702933691442e-10
15926,75446,75446,150892,457.8502209186554,3.54702933691442e-10
15944,75566,75566,151132,458.592787027359,3.5652192309498787e-10
15961,75650,75650,151300,459.1157760620117,3.54702933691442e-10
15979,75746,75746,151492,459.6998920440674,3.54702933691442e-10
15997,75856,75856,151712,460.3777780532837,3.54702933691442e-10
16014,75962,75962,151924,461.02243304252625,3.54702933691442e-10
16032,76070,76070,152140,461.6770570278168,3.5288394428789616e-10
16049,76160,76160,152320,462.2340478897095,3.54702933691442e-10
16067,76282,76282,152564,462.9714369773865,3.510649548843503e-10
16084,76366,76366,152732,463.52081990242004,3.510649548843503e-10
16102,76474,76474,152948,464.1717429161072,3.510649548843503e-10
16120,76586,76586,153172,464.83589005470276,3.510649548843503e-10
16137,76690,76690,153380,465.4724621772766,3.510649548843503e-10
16155,76782,76782,153564,466.05231404304504,3.510649548843503e-10
16172,76892,76892,153784,466.7129011154175,3.4924596548080444e-10
16190,76998,76998,153996,467.33819794654846,3.4924596548080444e-10
16207,77082,77082,154164,467.8602201938629,3.474269760772586e-10
16225,77184,77184,154368,468.49118208885193,3.41970007866621e-10
16243,77276,77276,154552,469.0895240306854,3.3651303965598345e-10
16260,77364,77364,154728,469.6559250354767,3.310560714453459e-10
16278,77450,77450,154900,470.20124316215515,3.2741809263825417e-10
16295,77548,77548,155096,470.8158960342407,3.255991032347083e-10
16313,77636,77636,155272,471.3794209957123,3.255991032347083e-10
16330,77728,77728,155456,471.9452919960022,3.219611244276166e-10
16348,77814,77814,155628,472.49620294570923,3.1468516681343317e-10
16366,77928,77928,155856,473.1958260536194,3.0377123039215803e-10
16383,78008,78008,156016,473.69225692749023,3.019522409886122e-10
16401,78100,78100,156200,474.2686960697174,2.9831426218152046e-10
16418,78178,78178,156356,474.7724220752716,2.9831426218152046e-10
16436,78268,78268,156536,475.3477749824524,2.9467628337442875e-10
16454,78350,78350,156700,475.8767569065094,2.9103830456733704e-10
16471,78426,78426,156852,476.36575198173523,2.892193151637912e-10
16489,78516,78516,157032,476.938236951828,2.874003257602453e-10
16506,78602,78602,157204,477.49523305892944,2.837623469531536e-10
16524,78684,78684,157368,478.0161249637604,2.8194335754960775e-10
16541,78778,78778,157556,478.6189639568329,2.7830537874251604e-10
16559,78884,78884,157768,479.2693519592285,2.801243681460619e-10
16577,78970,78970,157940,479.83618998527527,2.7466739993542433e-10
16594,79072,79072,158144,480.4481899738312,2.7466739993542433e-10
16612,79172,79172,158344,481.06986808776855,2.7284841053187847e-10
16629,79270,79270,158540,481.6625180244446,2.7284841053187847e-10
16647,79358,79358,158716,482.2307481765747,2.7284841053187847e-10
16664,79450,79450,158900,482.8076651096344,2.710294211283326e-10
16682,79546,79546,159092,483.4167709350586,2.6921043172478676e-10
16700,79632,79632,159264,483.9752640724182,2.710294211283326e-10
16717,79726,79726,159452,484.56347703933716,2.710294211283326e-10
16735,79820,79820,159640,485.14606404304504,2.6921043172478676e-10
16752,79910,79910,159820,485.71405506134033,2.673914423212409e-10
16770,80008,80008,160016,486.3300609588623,2.673914423212409e-10
16788,80094,80094,160188,486.88350009918213,2.6921043172478676e-10
16805,80182,80182,160364,487.4285922050476,2.6557245291769505e-10
16823,80292,80292,160584,488.1125519275665,2.673914423212409e-10
16840,80382,80382,160764,488.6902229785919,2.673914423212409e-10
16858,80500,80500,161000,489.4087920188904,2.673914423212409e-10
16875,80602,80602,161204,490.0428788661957,2.673914423212409e-10
16893,80710,80710,161420,490.7089898586273,2.6557245291769505e-10
16911,80822,80822,161644,491.3992519378662,2.6557245291769505e-10
16928,80916,80916,161832,491.9764018058777,2.673914423212409e-10
16946,81024,81024,162048,492.63805890083313,2.673914423212409e-10
16963,81136,81136,162272,493.3031370639801,2.6557245291769505e-10
16981,81246,81246,162492,493.98095512390137,2.6557245291769505e-10
16998,81352,81352,162704,494.66614389419556,2.673914423212409e-10
17016,81484,81484,162968,495.44978880882263,2.6557245291769505e-10
17034,81602,81602,163204,496.1712911128998,2.6557245291769505e-10
17051,81704,81704,163408,496.7886610031128,2.6557245291769505e-10
17069,81812,81812,163624,497.46503806114197,2.637534635141492e-10
17086,81896,81896,163792,497.9870309829712,2.6557245291769505e-10
17104,82004,82004,164008,498.6457772254944,2.637534635141492e-10
17122,82106,82106,164212,499.27056193351746,2.637534635141492e-10
17139,82214,82214,164428,499.94007301330566,2.637534635141492e-10
17157,82328,82328,164656,500.6296570301056,2.637534635141492e-10
17174,82446,82446,164892,501.3366279602051,2.637534635141492e-10
17192,82554,82554,165108,502.005038022995,2.6193447411060333e-10
17209,82652,82652,165304,502.60765409469604,2.6193447411060333e-10
17227,82744,82744,165488,503.17577505111694,2.601154847070575e-10
17245,82820,82820,165640,503.6708002090454,2.582964953035116e-10
17262,82910,82910,165820,504.22543501853943,2.510205376893282e-10
17280,83002,83002,166004,504.7994108200073,2.4920154828578234e-10
17297,83098,83098,166196,505.38690209388733,2.455635694786906e-10
17315,83186,83186,166372,505.9483959674835,2.419255906715989e-10
17332,83278,83278,166556,506.5407910346985,2.3283064365386963e-10
17350,83362,83362,166724,507.0845649242401,2.3101165425032377e-10
17368,83450,83450,166900,507.6479160785675,2.1100277081131935e-10
17385,83518,83518,167036,508.1091070175171,1.8917489796876907e-10
17403,83602,83602,167204,508.6669280529022,1.7644197214394808e-10
17420,83676,83676,167352,509.1769971847534,1.7462298274040222e-10
17438,83766,83766,167532,509.8193678855896,1.709850039333105e-10
17456,83866,83866,167732,510.51147413253784,1.6552803572267294e-10
17473,83934,83934,167868,511.0028851032257,1.5279510989785194e-10
17491,84016,84016,168032,511.5217831134796,1.4370016288012266e-10
17508,84084,84084,168168,511.95978903770447,1.291482476517558e-10
17526,84170,84170,168340,512.518630027771,1.2732925824820995e-10
17543,84256,84256,168512,513.0579509735107,1.1459633242338896e-10
17561,84344,84344,168688,513.6188111305237,9.822542779147625e-11


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.0016930103302001953,846.9037197860796
29,60,30,90,0.039572954177856445,60.951221914780945
58,118,59,177,0.07233691215515137,53.228602328563966
87,176,88,264,0.10537409782409668,49.275385401012954
116,234,117,351,0.13831686973571777,46.25781249962188
146,294,147,441,0.17371201515197754,43.918484493305186
175,352,176,528,0.20476508140563965,41.83134364314242
204,410,205,615,0.23752188682556152,39.92161091974481
233,468,234,702,0.27086591720581055,38.198276928415225
262,526,263,789,0.30205202102661133,36.58449389617044
291,584,292,876,0.3333439826965332,35.14654932934695
320,642,321,963,0.3637509346008301,33.67963510577556
349,700,350,1050,0.39542508125305176,32.53935789042907
379,760,380,1140,0.4283139705657959,31.191326678237147
408,818,409,1227,0.4605698585510254,30.152408010080308
437,876,438,1314,0.49192190170288086,29.06048061384331
466,934,467,1401,0.5230629444122314,28.10302663556422
495,992,496,1488,0.5544657707214355,27.255525696333734
524,1050,525,1575,0.5861020088195801,26.455033537691634
553,1108,554,1662,0.6179070472717285,25.414717880271155
582,1166,583,1749,0.649616003036499,24.60193441237061
611,1224,612,1836,0.682790994644165,23.930370450290184
641,1284,642,1926,0.7174570560455322,23.163079723194187
670,1342,671,2013,0.7518038749694824,22.459298269544433
699,1400,700,2100,0.7862107753753662,21.82455376283201
728,1458,729,2187,0.8212869167327881,21.243206171056045
757,1516,758,2274,0.8529648780822754,20.603258079325542
786,1574,787,2361,0.8880488872528076,19.91399805876722
815,1632,816,2448,0.9206008911132812,19.354075068272323
844,1690,845,2535,0.9523780345916748,18.917193060691034
874,1750,875,2625,0.9891128540039062,18.34961304335411
903,1808,904,2712,1.0222117900848389,17.899635458278453
932,1866,933,2799,1.054142951965332,17.43428428506695
961,1924,962,2886,1.088385820388794,16.975013422579423
990,1982,991,2973,1.1202208995819092,16.498502633626686
1019,2040,1020,3060,1.1516618728637695,16.03499723517507
1048,2098,1049,3147,1.1833600997924805,15.618203430524318
1077,2156,1078,3234,1.2144410610198975,15.252971766646397
1106,2214,1107,3321,1.2463188171386719,14.771383511103522
1136,2274,1137,3411,1.2791588306427002,14.232319153182289
1165,2332,1166,3498,1.3104310035705566,13.894681214127786
1194,2390,1195,3585,1.342052936553955,13.529045718075395
1223,2448,1224,3672,1.374709129333496,13.202526950457013
1252,2506,1253,3759,1.406402826309204,12.85889646039368
1281,2564,1282,3846,1.4387521743774414,12.45263506059132
1310,2622,1311,3933,1.470823049545288,12.23029731707038
1339,2680,1340,4020,1.502579927444458,11.847923136651048
1369,2740,1370,4110,1.535027027130127,11.542563283272102
1398,2798,1399,4197,1.5672509670257568,11.189579971601802
1427,2856,1428,4284,1.5988719463348389,10.917991457380367
1456,2914,1457,4371,1.6308271884918213,10.622263968651964
1485,2972,1486,4458,1.6625409126281738,10.387834290546834
1514,3030,1515,4545,1.6953349113464355,10.13172567487618
1543,3088,1544,4632,1.7265748977661133,9.881284007480417
1572,3146,1573,4719,1.758241891860962,9.645403989764077
1601,3204,1602,4806,1.7896971702575684,9.39275562897285
1631,3264,1632,4896,1.822234869003296,9.150557959200569
1660,3322,1661,4983,1.8532838821411133,8.919474765848122
1689,3380,1690,5070,1.8840699195861816,8.660853633872534
1718,3438,1719,5157,1.9159698486328125,8.447753447746209
1747,3496,1748,5244,1.9476749897003174,8.250129587882498
1776,3554,1777,5331,1.9797170162200928,8.050550228831753
1805,3612,1806,5418,2.011215925216675,7.854436751350704
1834,3670,1835,5505,2.0433759689331055,7.677896798261031
1863,3728,1864,5592,2.0776150226593018,7.498090308653332
1893,3788,1894,5682,2.1102778911590576,7.325775498949611
1922,3846,1923,5769,2.1423168182373047,7.130687095118674
1951,3904,1952,5856,2.174175977706909,6.954575164519838
1980,3962,1981,5943,2.205399990081787,6.789757109955076
2009,4020,2010,6030,2.23836612701416,6.632740179676148
2038,4078,2039,6117,2.2700459957122803,6.474404224974251
2067,4136,2068,6204,2.3011317253112793,6.307933758705417
2096,4194,2097,6291,2.3328909873962402,6.15268277504731
2126,4254,2127,6381,2.3642029762268066,5.994241092332231
2155,4312,2156,6468,2.395737886428833,5.830024772650177
2184,4370,2185,6555,2.427137851715088,5.676245522320073
2213,4428,2214,6642,2.4573569297790527,5.5598247995751535
2242,4486,2243,6729,2.489691972732544,5.4315186543615255
2271,4544,2272,6816,2.526550769805908,5.310211170384264
2300,4602,2301,6903,2.557508945465088,5.176127152685581
2329,4660,2330,6990,2.5884108543395996,5.051405803971079
2358,4718,2359,7077,2.617927074432373,4.935355849076586
2388,4778,2389,7167,2.649061918258667,4.819528935714402
2417,4836,2418,7254,2.680598735809326,4.71596452314418
2446,4894,2447,7341,2.7099108695983887,4.617080319237743
2475,4952,2476,7428,2.741237163543701,4.512429562220063
2504,5010,2505,7515,2.773329019546509,4.397105606100467
2533,5068,2534,7602,2.803753137588501,4.315307898798437
2562,5126,2563,7689,2.835939884185791,4.18466676952653
2591,5184,2592,7776,2.8681480884552,4.089463573012836
2621,5244,2622,7866,2.901458978652954,3.998652784037631
2650,5302,2651,7953,2.9350128173828125,3.905425323696022
2679,5360,2680,8040,2.970883846282959,3.8089198927424377
2708,5418,2709,8127,3.0028328895568848,3.7212423425719408
2737,5476,2738,8214,3.0356388092041016,3.6310773960460665
2766,5534,2767,8301,3.0675108432769775,3.543207383011577
2795,5592,2796,8388,3.098602056503296,3.466161284867553
2824,5650,2825,8475,3.1299338340759277,3.3836124373485745
2853,5708,2854,8562,3.160325050354004,3.313289292518334
2883,5768,2884,8652,3.1923270225524902,3.22664018309365
2912,5826,2913,8739,3.223345994949341,3.158045593478505
2941,5884,2942,8826,3.254225969314575,3.0686442192785535
2970,5942,2971,8913,3.2859909534454346,3.003744298642232
2999,6000,3000,9000,3.317633867263794,2.9323665394699674
3028,6058,3029,9087,3.3510711193084717,2.863301116070147
3057,6116,3058,9174,3.386721134185791,2.801095254321126
3086,6174,3087,9261,3.417452812194824,2.73484812053357
3116,6234,3117,9351,3.450334072113037,2.660501050153357
3145,6292,3146,9438,3.482532024383545,2.6082797022216937
3174,6350,3175,9525,3.513150930404663,2.547743920578
3203,6408,3204,9612,3.5455498695373535,2.4927409477489846
3232,6466,3233,9699,3.5763227939605713,2.4348603042082004
3261,6524,3262,9786,3.606624126434326,2.3819470878109996
3290,6582,3291,9873,3.637624979019165,2.3264743533139836
3319,6640,3320,9960,3.6685938835144043,2.276706777553727
3348,6698,3349,10047,3.6991817951202393,2.2344986860829295
3378,6758,3379,10137,3.731281042098999,2.178202127424811
3407,6816,3408,10224,3.761666774749756,2.1258783925002263
3436,6874,3437,10311,3.792301893234253,2.0862036443031684
3465,6932,3466,10398,3.824105978012085,2.0320216268862623
3494,6990,3495,10485,3.8546979427337646,1.9875914201483056
3523,7048,3524,10572,3.885382890701294,1.9434519061711626
3552,7106,3553,10659,3.916184902191162,1.8948053698981084
3581,7164,3582,10746,3.9466159343719482,1.8460580897603904
3611,7224,3612,10836,3.9793617725372314,1.80611971459075
3640,7282,3641,10923,4.0102219581604,1.768951809888108
3669,7340,3670,11010,4.041441202163696,1.7300598009387613
3698,7398,3699,11097,4.074518918991089,1.6903075722818812
3727,7456,3728,11184,4.10517692565918,1.6514278754756333
3756,7514,3757,11271,4.136922836303711,1.61171944017417
3785,7572,3786,11358,4.168210029602051,1.5777931214203136
3814,7630,3815,11445,4.199465990066528,1.5442127271118125
3843,7688,3844,11532,4.230730056762695,1.5112407042005316
3873,7748,3874,11622,4.262557029724121,1.4664823571225725
3902,7806,3903,11709,4.293398141860962,1.434422203608051
3931,7864,3932,11796,4.325336933135986,1.4050488647088741
3960,7922,3961,11883,4.3560631275177,1.3793675958723952
3989,7980,3990,11970,4.388200044631958,1.3451372946462925
4018,8038,4019,12057,4.419524908065796,1.3186524726515927
4047,8096,4048,12144,4.450844049453735,1.2917370951885232
4076,8154,4077,12231,4.48339319229126,1.2651580976557852
4106,8214,4107,12321,4.516021013259888,1.2375177784992957
4135,8272,4136,12408,4.548692941665649,1.2104617874526866
4164,8330,4165,12495,4.5808117389678955,1.1800067770142277
4193,8388,4194,12582,4.611126184463501,1.156634294208402
4222,8446,4223,12669,4.642241954803467,1.1308184059843143
4251,8504,4252,12756,4.673821926116943,1.1068154901275875
4280,8562,4281,12843,4.704502105712891,1.085513387746687
4309,8620,4310,12930,4.735284090042114,1.0586986739530175
4338,8678,4339,13017,4.76633095741272,1.0356971710839389
4368,8738,4369,13107,4.797612190246582,1.0143041563455881
4397,8796,4398,13194,4.828818082809448,0.9935661950909207
4426,8854,4427,13281,4.8595311641693115,0.9713619451797513
4455,8912,4456,13368,4.890197038650513,0.9501976300565502
4484,8970,4485,13455,4.921787977218628,0.9315564651490149
4513,9028,4514,13542,4.9526097774505615,0.9129445177630942
4542,9086,4543,13629,4.985087156295776,0.894284711491423
4571,9144,4572,13716,5.017228841781616,0.8720143617262011
4601,9204,4602,13806,5.052308082580566,0.8540746060050424
4630,9262,4631,13893,5.084568977355957,0.8343483698336058
4659,9320,4660,13980,5.117369890213013,0.8182596662786636
4688,9378,4689,14067,5.149121046066284,0.8003067976788998
4717,9436,4718,14154,5.180513143539429,0.7823803154426514
4746,9494,4747,14241,5.210700750350952,0.7642233674662293
4775,9552,4776,14328,5.241745948791504,0.7482667492616883
4804,9610,4805,14415,5.272559881210327,0.7329584684711108
4833,9668,4834,14502,5.302897930145264,0.7171808864000013
4863,9728,4864,14592,5.334881782531738,0.702129367978273
4892,9786,4893,14679,5.364887952804565,0.6876833976565422
4921,9844,4922,14766,5.396244049072266,0.6738568646106842
4950,9902,4951,14853,5.427511930465698,0.6573097095285902
4979,9960,4980,14940,5.458127021789551,0.6444668237600126
5008,10018,5009,15027,5.48919415473938,0.6288499107412235
5037,10076,5038,15114,5.519880056381226,0.6169541525623572
5066,10134,5067,15201,5.550632953643799,0.6024051319574255
5095,10192,5096,15288,5.58176589012146,0.589703682042682
5125,10252,5126,15378,5.614714860916138,0.5757010456799208
5154,10310,5155,15465,5.645753860473633,0.5653805056331294
5183,10368,5184,15552,5.676687955856323,0.5524794183560289
5212,10426,5213,15639,5.7071051597595215,0.5420401781201463
5241,10484,5242,15726,5.738207101821899,0.5313745140515493
5270,10542,5271,15813,5.769248008728027,0.5185334140790019
5299,10600,5300,15900,5.799830913543701,0.5080535371452015
5328,10658,5329,15987,5.831647157669067,0.4974109724653317
5358,10718,5359,16077,5.86326003074646,0.4874389058529687
5387,10776,5388,16164,5.89489483833313,0.47727617315149473
5416,10834,5417,16251,5.926530838012695,0.46832990156622145
5445,10892,5446,16338,5.956541061401367,0.45909970667878497
5474,10950,5475,16425,5.987181901931763,0.44887137429395807
5503,11008,5504,16512,6.0181121826171875,0.43902943262321514
5532,11066,5533,16599,6.049593925476074,0.4301195441217942
5561,11124,5562,16686,6.0821919441223145,0.42171527337518455
5590,11182,5591,16773,6.112838983535767,0.41253010082368746
5620,11242,5621,16863,6.145243883132935,0.4025907782651075
5649,11300,5650,16950,6.177121877670288,0.39473960348891524
5678,11358,5679,17037,6.20865797996521,0.3865221029651593
5707,11416,5708,17124,6.240890979766846,0.3790474057252595
5736,11474,5737,17211,6.273207902908325,0.37055440953804464
5765,11532,5766,17298,6.304973840713501,0.36340829730204405
5794,11590,5795,17385,6.3378119468688965,0.3559195359523528
5823,11648,5824,17472,6.370161056518555,0.34888247867343125
5853,11708,5854,17562,6.4029541015625,0.3417026331701436
5882,11766,5883,17649,6.435777902603149,0.3333816996959058
5911,11824,5912,17736,6.468667984008789,0.32835750796652974
5940,11882,5941,17823,6.500825881958008,0.31991201460971297
5969,11940,5970,17910,6.532867908477783,0.3140749010528907
5998,11998,5999,17997,6.565505027770996,0.30774299773349867
6027,12056,6028,18084,6.598207950592041,0.3015486240580003
6056,12114,6057,18171,6.630064964294434,0.29474056910135005
6085,12172,6086,18258,6.661743879318237,0.289585509084759
6115,12232,6116,18348,6.694607973098755,0.2838041139150391
6144,12290,6145,18435,6.727094888687134,0.2774220372655236
6173,12348,6174,18522,6.758849859237671,0.2725147962173651
6202,12406,6203,18609,6.790631055831909,0.26729226273869244
6231,12464,6232,18696,6.823275089263916,0.2620876888630619
6260,12522,6261,18783,6.855681896209717,0.2564890560789763
6289,12580,6290,18870,6.8871588706970215,0.2514814360223454
6318,12638,6319,18957,6.918459892272949,0.24671333433707332
6348,12698,6349,19047,6.951575994491577,0.24163939113839206
6377,12756,6378,19134,6.983794927597046,0.2367817596310715
6406,12814,6407,19221,7.0154571533203125,0.22940041304957504
6435,12872,6436,19308,7.047777891159058,0.22522457782645233
6464,12930,6465,19395,7.080045938491821,0.2208107165840829
6493,12988,6494,19482,7.112185001373291,0.21648997169540962
6522,13046,6523,19569,7.145473957061768,0.21211885850379986
6551,13104,6552,19656,7.179941892623901,0.2076170916401452
6580,13162,6581,19743,7.213392972946167,0.20296928092784583
6610,13222,6611,19833,7.249237060546875,0.19880007804772504
6639,13280,6640,19920,7.284289836883545,0.19527162752297045
6668,13338,6669,20007,7.316338062286377,0.19097310158770142
6697,13396,6698,20094,7.348922967910767,0.18747884222193534
6726,13454,6727,20181,7.381350040435791,0.18294216952733677
6755,13512,6756,20268,7.412744045257568,0.17939313180738736
6784,13570,6785,20355,7.445637941360474,0.17583308599409975
6813,13628,6814,20442,7.477927923202515,0.17216165367835856
6843,13688,6844,20532,7.511029005050659,0.1685689380030908
6872,13746,6873,20619,7.544081926345825,0.16532197315927988
6901,13804,6902,20706,7.576236963272095,0.16231887987851223
6930,13862,6931,20793,7.608198881149292,0.15802129524456632
6959,13920,6960,20880,7.643280029296875,0.15502768236274278
6988,13978,6989,20967,7.675903081893921,0.1520496433763583
7017,14036,7018,21054,7.706954002380371,0.1485699421315303
7046,14094,7047,21141,7.738860845565796,0.14569961617939953
7075,14152,7076,21228,7.771007061004639,0.1426705738072087
7105,14212,7106,21318,7.803532838821411,0.13987352919832574
7134,14270,7135,21405,7.835726976394653,0.13720931978150475
7163,14328,7164,21492,7.867788791656494,0.1345769493638045
7192,14386,7193,21579,7.899536848068237,0.13194543659767533
7221,14444,7222,21666,7.931519985198975,0.12889272057316248
7250,14502,7251,21753,7.963287830352783,0.12649929196504672
7279,14560,7280,21840,7.995000839233398,0.12416689282292737
7308,14618,7309,21927,8.026902914047241,0.12166306891697332
7338,14678,7339,22017,8.059254884719849,0.11925453036099043
7367,14736,7368,22104,8.091273069381714,0.11678076250814229
7396,14794,7397,22191,8.123235940933228,0.11428962398281328
7425,14852,7426,22278,8.15447211265564,0.11195618863155232
7454,14910,7455,22365,8.185526847839355,0.10984442175094955
7483,14968,7484,22452,8.216684103012085,0.10765981280871983
7512,15026,7513,22539,8.247800827026367,0.10542855784569838
7541,15084,7542,22626,8.27950382232666,0.10321481563482848
7570,15142,7571,22713,8.311347007751465,0.10117566687404178
7600,15202,7601,22803,8.34654712677002,0.09888128879890701
7629,15260,7630,22890,8.37751293182373,0.09699103132788878
7658,15318,7659,22977,8.408145904541016,0.09512163807130491
7687,15376,7688,23064,8.440208911895752,0.09340798263747274
7716,15434,7717,23151,8.472330093383789,0.09122767871679116
7745,15492,7746,23238,8.503190755844116,0.08926532634859541
7774,15550,7775,23325,8.535510063171387,0.08767078931839478
7803,15608,7804,23412,8.5696861743927,0.08572644913965632
7833,15668,7834,23502,8.603244066238403,0.0839397593637159
7862,15726,7863,23589,8.635893106460571,0.08210917598989909
7891,15784,7892,23676,8.670467853546143,0.0807106057859528
7920,15842,7921,23763,8.70349907875061,0.07894205043112379
7949,15900,7950,23850,8.736982107162476,0.07743172451318969
7978,15958,7979,23937,8.773235082626343,0.07592929110001023
8007,16016,8008,24024,8.807416915893555,0.07435606534079398
8036,16074,8037,24111,8.84226393699646,0.0729381069234023
8065,16132,8066,24198,8.876715183258057,0.07138375287479448
8095,16192,8096,24288,8.909446001052856,0.0699216771713509
8124,16250,8125,24375,8.94206690788269,0.06868792836507964
8153,16308,8154,24462,8.98051905632019,0.06717125438319727
8182,16366,8183,24549,9.011476993560791,0.0657506236991594
8211,16424,8212,24636,9.043601989746094,0.0644714782677056
8240,16482,8241,24723,9.078067064285278,0.06303540590681678
8269,16540,8270,24810,9.111089944839478,0.06191786381907605
8298,16598,8299,24897,9.143879890441895,0.06050318309519298
8327,16656,8328,24984,9.17539381980896,0.05927667362709599
8357,16716,8358,25074,9.207780838012695,0.0580998416176044
8386,16774,8387,25161,9.239696025848389,0.05700011927649484
8415,16832,8416,25248,9.273388147354126,0.05578596596183161
8444,16890,8445,25335,9.305535078048706,0.054742738961522264
8473,16948,8474,25422,9.339708089828491,0.053382350122546995
8502,17006,8503,25509,9.372128009796143,0.05242216916258258
8531,17064,8532,25596,9.403770923614502,0.05142260473235183
8560,17122,8561,25683,9.437663078308105,0.050569342566745945
8590,17182,8591,25773,9.471410036087036,0.049534206706312034
8619,17240,8620,25860,9.504122972488403,0.04847687162418879
8648,17298,8649,25947,9.53747010231018,0.047516398397419835
8677,17356,8678,26034,9.57016897201538,0.04660236926633843
8706,17414,8707,26121,9.601435899734497,0.04573560227731832
8735,17472,8736,26208,9.633634805679321,0.044677959096475206
8764,17530,8765,26295,9.66714096069336,0.04387944902896379
8793,17588,8794,26382,9.699862003326416,0.042896895824924286
8822,17646,8823,26469,9.734046936035156,0.042179280616892356
8852,17706,8853,26559,9.772485971450806,0.0413134367265684
8881,17764,8882,26646,9.809260845184326,0.04047712294493522
8910,17822,8911,26733,9.852044820785522,0.039696430603044064
8939,17880,8940,26820,9.88949203491211,0.03891861693421106
8968,17938,8969,26907,9.921656847000122,0.03823840841926085
8997,17996,8998,26994,9.95350694656372,0.03747799083703285
9026,18054,9027,27081,9.98790192604065,0.036805622854785724
9055,18112,9056,27168,10.020561933517456,0.03612392496177108
9085,18172,9086,27258,10.056823968887329,0.03540308177593943
9114,18230,9115,27345,10.094748973846436,0.03468051087884305
9143,18288,9144,27432,10.128682136535645,0.03393495673799407
9172,18346,9173,27519,10.162568092346191,0.033348775377248785
9201,18404,9202,27606,10.198042869567871,0.03266560644169658
9230,18462,9231,27693,10.231553077697754,0.03208484094648156
9259,18520,9260,27780,10.263713121414185,0.031507217790135655
9288,18578,9289,27867,10.296050071716309,0.03075835704396468
9317,18636,9318,27954,10.328837871551514,0.03016285945625441
9347,18696,9348,28044,10.360673904418945,0.029608473912389854
9376,18754,9377,28131,10.392300844192505,0.0289135948397643
9405,18812,9406,28218,10.42335295677185,0.028323685928853592
9434,18870,9435,28305,10.454155921936035,0.027759340438365143
9463,18928,9464,28392,10.487997055053711,0.0271198705183906
9492,18986,9493,28479,10.525300979614258,0.026689979954539922
9521,19044,9522,28566,10.55988097190857,0.02614016588108825
9550,19102,9551,28653,10.596662759780884,0.025630748120534008
9580,19162,9581,28743,10.637542963027954,0.025106049065357183
9609,19220,9610,28830,10.677089929580688,0.02463892584455607
9638,19278,9639,28917,10.720012903213501,0.024133006984243366
9667,19336,9668,29004,10.757045984268188,0.02349037152555411
9696,19394,9697,29091,10.792165040969849,0.023095694954236023
9725,19452,9726,29178,10.830573797225952,0.02259599267915746
9754,19510,9755,29265,10.866929054260254,0.022193790001438174
9783,19568,9784,29352,10.906100034713745,0.021740111008625718
9812,19626,9813,29439,10.950599908828735,0.021283344994571962
9842,19686,9843,29529,10.992140769958496,0.020860828510421925
9871,19744,9872,29616,11.031058073043823,0.020458655789298064
9900,19802,9901,29703,11.067085981369019,0.020085897173999
9929,19860,9930,29790,11.103982925415039,0.019640079298369528
9958,19918,9959,29877,11.138510942459106,0.019261896764191988
9987,19976,9988,29964,11.17615294456482,0.01889321330554594
10016,20034,10017,30051,11.212494850158691,0.018464012303525124
10045,20092,10046,30138,11.25209093093872,0.018155800764816377
10075,20152,10076,30228,11.28978705406189,0.01777600457785411
10104,20210,10105,30315,11.32607913017273,0.017425127384854022
10133,20268,10134,30402,11.360295057296753,0.017092864647111128
10162,20326,10163,30489,11.398244857788086,0.01677353288823724
10191,20384,10192,30576,11.440684795379639,0.016414455802873817
10220,20442,10221,30663,11.490529775619507,0.01620419723201394
10249,20500,10250,30750,11.531763076782227,0.015754060776657752
10278,20558,10279,30837,11.58162808418274,0.015477299433769076
10307,20616,10308,30924,11.618864059448242,0.015161483628503447
10337,20676,10338,31014,11.66131591796875,0.014861609904301076
10366,20734,10367,31101,11.715622901916504,0.014586538744538302
10395,20792,10396,31188,11.749862909317017,0.014257890731869338
10424,20850,10425,31275,11.788789987564087,0.014004832416048885
10453,20908,10454,31362,11.824993133544922,0.013683826489796047
10482,20966,10483,31449,11.864131927490234,0.013415066681545795
10511,21024,10512,31536,11.902066946029663,0.013269456266584712
10540,21082,10541,31623,11.941003799438477,0.012894481273974634
10570,21142,10571,31713,11.97578501701355,0.012632382177912405
10599,21200,10600,31800,12.012027025222778,0.012405170182660186
10628,21258,10629,31887,12.05566692352295,0.012176589839441476
10657,21316,10658,31974,12.098566055297852,0.011926653904993145
10686,21374,10687,32061,12.134987831115723,0.011646920430166574
10715,21432,10716,32148,12.173557043075562,0.011446218893752302
10744,21490,10745,32235,12.211055994033813,0.011226079500715969
10773,21548,10774,32322,12.25102710723877,0.011009751445158145
10802,21606,10803,32409,12.292464017868042,0.010761774400407376
10832,21666,10833,32499,12.33395791053772,0.010554556684610361
10861,21724,10862,32586,12.369045972824097,0.010350667094940036
10890,21782,10891,32673,12.403892040252686,0.010200458664257894
10919,21840,10920,32760,12.44006896018982,0.009953710973036323
10948,21898,10949,32847,12.478790044784546,0.00976606834501581
10977,21956,10978,32934,12.51141095161438,0.009544857339619739
11006,22014,11007,33021,12.550462007522583,0.009368611558670636
11035,22072,11036,33108,12.586288928985596,0.009169786250708967
11065,22132,11066,33198,12.626658916473389,0.008982299190506637
11094,22190,11095,33285,12.662121057510376,0.00881314335447314
11123,22248,11124,33372,12.697684049606323,0.008640835678875192
11152,22306,11153,33459,12.733206748962402,0.008474465615108784
11181,22364,11182,33546,12.7672860622406,0.008315187064454221
11210,22422,11211,33633,12.80234980583191,0.008121814970195373
11239,22480,11240,33720,12.850359916687012,0.007977447662256054
11268,22538,11269,33807,12.885967016220093,0.007835050074277206
11297,22596,11298,33894,12.921030044555664,0.0076498794693407035
11327,22656,11328,33984,12.953319072723389,0.007488845576745007
11356,22714,11357,34071,12.984071016311646,0.00736406434100445
11385,22772,11386,34158,13.01477599143982,0.00718293154022831
11414,22830,11415,34245,13.045942783355713,0.0070522350209785145
11443,22888,11444,34332,13.077129125595093,0.006910796121132989
11472,22946,11473,34419,13.107703924179077,0.006752544284154283
11501,23004,11502,34506,13.138571739196777,0.00662803027978498
11530,23062,11531,34593,13.169251918792725,0.0065018655900530575
11559,23120,11560,34680,13.199732065200806,0.00637221995600612
11589,23180,11590,34770,13.232017993927002,0.006244417251878076
11618,23238,11619,34857,13.26266098022461,0.006135546149607762
11647,23296,11648,34944,13.29380202293396,0.005993968793404747
11676,23354,11677,35031,13.324934959411621,0.005881609537595978
11705,23412,11706,35118,13.355571985244751,0.005749322527208278
11734,23470,11735,35205,13.388023853302002,0.005632539635939793
11763,23528,11764,35292,13.41978406906128,0.005525608093876144
11792,23586,11793,35379,13.452595949172974,0.005431863625858568
11822,23646,11823,35469,13.49531102180481,0.005305183096879773
11851,23704,11852,35556,13.533642053604126,0.005200911509973594
11880,23762,11881,35643,13.56827712059021,0.005095285126003546
11909,23820,11910,35730,13.599952936172485,0.00497671615892159
11938,23878,11939,35817,13.633462905883789,0.004888063726411929
11967,23936,11968,35904,13.670928001403809,0.00479798091032535
11996,23994,11997,35991,13.703648090362549,0.004711990677606082
12025,24052,12026,36078,13.737281084060669,0.004618253003059181
12054,24110,12055,36165,13.769069910049438,0.004521186076885897
12084,24170,12085,36255,13.801131010055542,0.0044210089383796
12113,24228,12114,36342,13.832444906234741,0.004342341737697097
12142,24286,12143,36429,13.86284613609314,0.0042529098695922585
12171,24344,12172,36516,13.895238876342773,0.004174577923208744
12200,24402,12201,36603,13.926599979400635,0.00416642033530934
12229,24460,12230,36690,13.956979036331177,0.0039813839948692475
12258,24518,12259,36777,13.988667964935303,0.003904232460399726
12287,24576,12288,36864,14.019259929656982,0.003837919507532206
12317,24636,12318,36954,14.051721096038818,0.003764454693168773
12346,24694,12347,37041,14.083359956741333,0.003691869232056888
12375,24752,12376,37128,14.113852977752686,0.00361647018792155
12404,24810,12405,37215,14.145378828048706,0.0035449284954438554
12433,24868,12434,37302,14.177927017211914,0.003484058416916014
12462,24926,12463,37389,14.208120822906494,0.0034081847185234437
12491,24984,12492,37476,14.239758968353271,0.0033407391573518908
12520,25042,12521,37563,14.271785020828247,0.0032763040730969806
12549,25100,12550,37650,14.303668022155762,0.003215975399712079
12579,25160,12580,37740,14.336013793945312,0.0031542400172384077
12608,25218,12609,37827,14.366461038589478,0.003097820114021488
12637,25276,12638,37914,14.39707612991333,0.0030328074180943076
12666,25334,12667,38001,14.42812705039978,0.0029755122704955284
12695,25392,12696,38088,14.458499908447266,0.002914194639629386
12724,25450,12725,38175,14.489812135696411,0.0028593097442808357
12753,25508,12754,38262,14.520061016082764,0.0028008659651277412
12782,25566,12783,38349,14.551020860671997,0.002747838300138028
12812,25626,12813,38439,14.583074808120728,0.0026942699798837566
12841,25684,12842,38526,14.61365294456482,0.002642318771108876
12870,25742,12871,38613,14.644659042358398,0.0025917020064980534
12899,25800,12900,38700,14.676844120025635,0.0025418230208060777
12928,25858,12929,38787,14.708530902862549,0.002475328436162272
12957,25916,12958,38874,14.739276885986328,0.00242247597759615
12986,25974,12987,38961,14.769859790802002,0.0023769582188606364
13015,26032,13016,39048,14.800136089324951,0.002335318877726422
13044,26090,13045,39135,14.83086085319519,0.0022828991818641953
13074,26150,13075,39225,14.863914012908936,0.002230963634701766
13103,26208,13104,39312,14.895987033843994,0.0021872128844506733
13132,26266,13133,39399,14.925755977630615,0.002140972423489984
13161,26324,13162,39486,14.955007076263428,0.0021033281989275565
13190,26382,13191,39573,14.98500680923462,0.002068062843250118
13219,26440,13220,39660,15.014111995697021,0.002029677284326681
13248,26498,13249,39747,15.044431924819946,0.001988614474953465
13277,26556,13278,39834,15.07497787475586,0.0019511744902729333
13307,26616,13308,39924,15.10522985458374,0.001924333455121996
13336,26674,13337,40011,15.135035037994385,0.0018779796986336805
13365,26732,13366,40098,15.164186954498291,0.001842091946173241
13394,26790,13395,40185,15.194923162460327,0.0018057395037658353
13423,26848,13424,40272,15.224922895431519,0.0017681957344848342
13452,26906,13453,40359,15.254562854766846,0.0017442445716824295
13481,26964,13482,40446,15.285380840301514,0.0017034216416504933
13510,27022,13511,40533,15.314950942993164,0.0016708416648043567
13539,27080,13540,40620,15.345386981964111,0.0016410550417731429
13569,27140,13570,40710,15.375917911529541,0.0016048302018134564
13598,27198,13599,40797,15.404989004135132,0.001570428315631034
13627,27256,13628,40884,15.434823036193848,0.0015400237562062102
13656,27314,13657,40971,15.464834928512573,0.0015119285919809045
13685,27372,13686,41058,15.494795799255371,0.0014817587085644846
13714,27430,13715,41145,15.527734756469727,0.0014395110089253649
13743,27488,13744,41232,15.55699896812439,0.0014173436350120028
13772,27546,13773,41319,15.588976860046387,0.001387604144042598
13802,27606,13803,41409,15.619745969772339,0.0013601856969671644
13831,27664,13832,41496,15.649409770965576,0.001334190085458431
13860,27722,13861,41583,15.680194854736328,0.0013071752988480512
13889,27780,13890,41670,15.709681034088135,0.0012830383990376504
13918,27838,13919,41757,15.739753007888794,0.0012552079435863561
13947,27896,13948,41844,15.770594835281372,0.0012326663062367516
13976,27954,13977,41931,15.802250146865845,0.0012110360078168014
14005,28012,14006,42018,15.835054874420166,0.0011883411154940404
14034,28070,14035,42105,15.866114854812622,0.0011665135353950973
14064,28130,14065,42195,15.902318954467773,0.001144460508157863
14093,28188,14094,42282,15.9322509765625,0.0011228299977119605
14122,28246,14123,42369,15.96189284324646,0.0011013851491270543
14151,28304,14152,42456,15.992034912109375,0.001079671517004499
14180,28362,14181,42543,16.022155046463013,0.0010604266252585148
14209,28420,14210,42630,16.05188298225403,0.0010392201046443006
14238,28478,14239,42717,16.08375883102417,0.0010187432297925625
14267,28536,14268,42804,16.11275815963745,0.0009975916530038376
14297,28596,14298,42894,16.143792867660522,0.000977173022874922
14326,28654,14327,42981,16.17385697364807,0.0009589664833811185
14355,28712,14356,43068,16.203269004821777,0.0009401520708252065
14384,28770,14385,43155,16.233014822006226,0.0009238423201622936
14413,28828,14414,43242,16.262216091156006,0.0009053976683617293
14442,28886,14443,43329,16.291831970214844,0.0008872526871073205
14471,28944,14472,43416,16.321359872817993,0.0008697774503616529
14500,29002,14501,43503,16.35172986984253,0.0008551508155960619
14529,29060,14530,43590,16.38328504562378,0.0008381891345834447
14559,29120,14560,43680,16.413676023483276,0.0008220329558525918
14588,29178,14589,43767,16.449821949005127,0.0008005191996289795
14617,29236,14618,43854,16.480228900909424,0.0007847961695688355
14646,29294,14647,43941,16.509418964385986,0.000769388628782508
14675,29352,14676,44028,16.539873838424683,0.0007543602135910987
14704,29410,14705,44115,16.569676876068115,0.0007374676322342566
14733,29468,14734,44202,16.599446773529053,0.0007231674724152981
14762,29526,14763,44289,16.62946891784668,0.0007097382213032688
14791,29584,14792,44376,16.65936017036438,0.0006973699217951435
14821,29644,14822,44466,16.69030213356018,0.0006849001948694422
14850,29702,14851,44553,16.72021484375,0.0006714505294667106
14879,29760,14880,44640,16.749879837036133,0.0006587284575516605
14908,29818,14909,44727,16.779457092285156,0.0006455275147345674
14937,29876,14938,44814,16.808660984039307,0.0006358413507996374
14966,29934,14967,44901,16.83819818496704,0.0006215565838374459
14995,29992,14996,44988,16.86756420135498,0.0006099295161448026
15024,30050,15025,45075,16.896867990493774,0.0005967783453115771
15054,30110,15055,45165,16.928165912628174,0.0005846520248269371
15083,30168,15084,45252,16.95869493484497,0.0005740098446267439
15112,30226,15113,45339,16.989969968795776,0.0005639550570322172
15141,30284,15142,45426,17.020540952682495,0.0005541514105971146
15170,30342,15171,45513,17.05134606361389,0.000543837296959282
15199,30400,15200,45600,17.086882829666138,0.0005327806139803215
15228,30458,15229,45687,17.117491960525513,0.0005219209679125925
15257,30516,15258,45774,17.14653491973877,0.0005121356659856247
15286,30574,15287,45861,17.176331758499146,0.0005022362267936842
15316,30634,15317,45951,17.2064688205719,0.0004931996280674866
15345,30692,15346,46038,17.236403942108154,0.00048398472426924855
15374,30750,15375,46125,17.268635034561157,0.0004744023254943386
15403,30808,15404,46212,17.298789024353027,0.000465862296891828
15432,30866,15433,46299,17.32812809944153,0.0004558879362548396
15461,30924,15462,46386,17.35725712776184,0.00044658327146862575
15490,30982,15491,46473,17.387269020080566,0.00043879084694253834
15519,31040,15520,46560,17.416883945465088,0.000429251957143606
15549,31100,15550,46650,17.447686910629272,0.0004210210491919497
15578,31158,15579,46737,17.477521896362305,0.0004129353997086582
15607,31216,15608,46824,17.506664991378784,0.0004046590064490374
15636,31274,15637,46911,17.53656506538391,0.00039726674106077553
15665,31332,15666,46998,17.566111087799072,0.0003897854386423205
15694,31390,15695,47085,17.596536874771118,0.00038165413013757643
15723,31448,15724,47172,17.626276969909668,0.0003730794753664668
15752,31506,15753,47259,17.655583143234253,0.0003655054712226047
15781,31564,15782,47346,17.685658931732178,0.0003589112537838446
15811,31624,15812,47436,17.715837001800537,0.00035108908809888817
15840,31682,15841,47523,17.745502948760986,0.0003441465249807152
15869,31740,15870,47610,17.774930000305176,0.0003361099965104586
15898,31798,15899,47697,17.804126024246216,0.0003308043187644216
15927,31856,15928,47784,17.833834171295166,0.0003244334952796635
15956,31914,15957,47871,17.8639178276062,0.0003172714555148559
15985,31972,15986,47958,17.89406180381775,0.00031061284357747354
16014,32030,16015,48045,17.925405979156494,0.00030471887453131785
16044,32090,16045,48135,17.98616099357605,0.0002993699865783128
16073,32148,16074,48222,18.0226149559021,0.0002933372763891384
16102,32206,16103,48309,18.056176900863647,0.0002877423031577564
16131,32264,16132,48396,18.089503049850464,0.0002819435898118172
16160,32322,16161,48483,18.119753122329712,0.000276166888284024
16189,32380,16190,48570,18.150357007980347,0.00027137316544667556
16218,32438,16219,48657,18.180511951446533,0.0002664800003913115
16247,32496,16248,48744,18.21019697189331,0.00026013523768142477
16276,32554,16277,48831,18.240808963775635,0.0002547403439621121
16306,32614,16307,48921,18.272382974624634,0.0002498473968444159
16335,32672,16336,49008,18.30630087852478,0.00024529286667984707
16364,32730,16365,49095,18.336984872817993,0.00024092873525205505
16393,32788,16394,49182,18.366662979125977,0.00023640855340545386
16422,32846,16423,49269,18.396320104599,0.00023203543844374508
16451,32904,16452,49356,18.42597198486328,0.0002272502781579533
16480,32962,16481,49443,18.458826065063477,0.0002227107336238987
16509,33020,16510,49530,18.49289298057556,0.00021864167342755536
16539,33080,16540,49620,18.523783922195435,0.00021419861161575682
16568,33138,16569,49707,18.55443000793457,0.0002099276647413717
16597,33196,16598,49794,18.584264039993286,0.00020564065471262438
16626,33254,16627,49881,18.613837957382202,0.00020080608669559297
16655,33312,16656,49968,18.643388986587524,0.0001970703150391273
16684,33370,16685,50055,18.672863006591797,0.00019327262430124392
16713,33428,16714,50142,18.70227599143982,0.00018880276991239953
16742,33486,16743,50229,18.732560873031616,0.0001848512512196976
16771,33544,16772,50316,18.762197971343994,0.00018121737775800284
16801,33604,16802,50406,18.793179035186768,0.00017775865899238852
16830,33662,16831,50493,18.822661876678467,0.00017447702566641965
16859,33720,16860,50580,18.85321879386902,0.0001711652338372005
16888,33778,16889,50667,18.883493900299072,0.0001680188059935972
16917,33836,16918,50754,18.91436195373535,0.0001641816601249957
16946,33894,16947,50841,18.945794820785522,0.00016072818448265025
16975,33952,16976,50928,18.97816514968872,0.00015788131042882014
17004,34010,17005,51015,19.009400844573975,0.00015506000966070133
17034,34070,17035,51105,19.046530961990356,0.00015210933599973941
17063,34128,17064,51192,19.0843448638916,0.00014900745395607373
17092,34186,17093,51279,19.115803956985474,0.00014594654021493625
17121,34244,17122,51366,19.147568941116333,0.00014309945345303277
17150,34302,17151,51453,19.17928695678711,0.00014019818388533167
17179,34360,17180,51540,19.210449934005737,0.00013784831207885873
17208,34418,17209,51627,19.243553161621094,0.00013476104948040302
17237,34476,17238,51714,19.278038024902344,0.0001322303016877413
17266,34534,17267,51801,19.310703992843628,0.00012973693674211972
17296,34594,17297,51891,19.345052003860474,0.00012728744786727475
17325,34652,17326,51978,19.37859797477722,0.00012494669749685272
17354,34710,17355,52065,19.408023834228516,0.00012245095683738327
17383,34768,17384,52152,19.440746068954468,0.00011994345049970434
17412,34826,17413,52239,19.47328281402588,0.00011783855563862744
17441,34884,17442,52326,19.505764961242676,0.00011531568043210427
17470,34942,17471,52413,19.536356925964355,0.00011334290059039631
17499,35000,17500,52500,19.56590700149536,0.00011107137231647357
17529,35060,17530,52590,19.59785795211792,0.00010898318441832089
17558,35118,17559,52677,19.629857778549194,0.00010681985190785781
17587,35176,17588,52764,19.662891149520874,0.00010478573733507801
17616,35234,17617,52851,19.695466995239258,0.0001027540552058781
17645,35292,17646,52938,19.7260320186615,0.00010085456688102568
17674,35350,17675,53025,19.755393028259277,9.883089046525129e-05
17703,35408,17704,53112,19.786623001098633,9.684311373803212e-05
17732,35466,17733,53199,19.824150800704956,9.48483574347847e-05
17761,35524,17762,53286,19.85405397415161,9.318763761712034e-05
17791,35584,17792,53376,19.88606595993042,9.137589438523719e-05
17820,35642,17821,53463,19.915777921676636,8.973868057182699e-05
17849,35700,17850,53550,19.95297598838806,8.78112983855317e-05
17878,35758,17879,53637,19.984994888305664,8.612624105808209e-05
17907,35816,17908,53724,20.01465606689453,8.510960219609842e-05
17936,35874,17937,53811,20.04548215866089,8.264940902336093e-05
17965,35932,17966,53898,20.076705932617188,8.121155701701355e-05
17994,35990,17995,53985,20.107932090759277,7.962187635257578e-05
18023,36048,18024,54072,20.14154601097107,7.819569145794958e-05
18053,36108,18054,54162,20.181108951568604,7.666314229481941e-05
18082,36166,18083,54249,20.212162971496582,7.509532895255688e-05
18111,36224,18112,54336,20.252924919128418,7.376329222097411e-05
18140,36282,18141,54423,20.286422967910767,7.233853330035345e-05
18169,36340,18170,54510,20.31767988204956,7.092831833688251e-05
18198,36398,18199,54597,20.348809003829956,6.96206079737749e-05
18227,36456,18228,54684,20.37957787513733,6.828535526892665e-05
18256,36514,18257,54771,20.408516883850098,6.702839107219916e-05
18286,36574,18287,54861,20.440542936325073,6.577928400020028e-05
18315,36632,18316,54948,20.477442979812622,6.447649127494515e-05
18344,36690,18345,55035,20.50822901725769,6.313326662166219e-05
18373,36748,18374,55122,20.542707920074463,6.19561149051151e-05
18402,36806,18403,55209,20.57528781890869,6.0775292581638496e-05
18431,36864,18432,55296,20.605217933654785,5.947610907242051e-05
18460,36922,18461,55383,20.638251066207886,5.848444698131061e-05
18489,36980,18490,55470,20.669686794281006,5.735671652473684e-05
18518,37038,18519,55557,20.703542947769165,5.630666714750987e-05
18548,37098,18549,55647,20.735332012176514,5.5115913596637256e-05
18577,37156,18578,55734,20.764750003814697,5.37931381359158e-05
18606,37214,18607,55821,20.79511308670044,5.2820386827079346e-05
18635,37272,18636,55908,20.83195400238037,5.177615639695432e-05
18664,37330,18665,55995,20.87677812576294,5.076279023796815e-05
18693,37388,18694,56082,20.906325101852417,4.981339452569955e-05
18722,37446,18723,56169,20.941472053527832,4.8946258630166994e-05
18751,37504,18752,56256,20.971987009048462,4.805469257007644e-05
18781,37564,18782,56346,21.00275206565857,4.716682383332227e-05
18810,37622,18811,56433,21.03352689743042,4.6261314196271996e-05
18839,37680,18840,56520,21.062886953353882,4.536748349437403e-05
18868,37738,18869,56607,21.093580961227417,4.4502433752313664e-05
18897,37796,18898,56694,21.123565912246704,4.35711235695635e-05
18926,37854,18927,56781,21.152922868728638,4.2704047359620745e-05
18955,37912,18956,56868,21.183068990707397,4.192728272300883e-05
18984,37970,18985,56955,21.212941884994507,4.112957310553611e-05
19013,38028,19014,57042,21.243948936462402,4.018701224595134e-05
19043,38088,19044,57132,21.283692836761475,3.942875991924666e-05
19072,38146,19073,57219,21.31360101699829,3.874568733408523e-05
19101,38204,19102,57306,21.35516905784607,3.801819673299178e-05
19130,38262,19131,57393,21.394623041152954,3.7250388459142414e-05
19159,38320,19160,57480,21.43054699897766,3.648555946256238e-05
19188,38378,19189,57567,21.460375785827637,3.573774222331849e-05
19217,38436,19218,57654,21.492353200912476,3.506534051211929e-05
19246,38494,19247,57741,21.5225670337677,3.4335045029365574e-05
19276,38554,19277,57831,21.553004026412964,3.3672337508505734e-05
19305,38612,19306,57918,21.583671808242798,3.306147129933379e-05
19334,38670,19335,58005,21.612925052642822,3.244634456223139e-05
19363,38728,19364,58092,21.644093990325928,3.182237594501203e-05
19392,38786,19393,58179,21.675534963607788,3.122276041267469e-05
19421,38844,19422,58266,21.706350803375244,3.0692748282490356e-05
19450,38902,19451,58353,21.745950937271118,3.008125338510581e-05
19479,38960,19480,58440,21.78766393661499,2.951434453279944e-05
19508,39018,19509,58527,21.829267024993896,2.895277543757402e-05
19538,39078,19539,58617,21.860449075698853,2.8370082418405218e-05
19567,39136,19568,58704,21.90279984474182,2.78121007113441e-05
19596,39194,19597,58791,21.942392826080322,2.7265746666671475e-05
19625,39252,19626,58878,21.974507093429565,2.6640817509360204e-05
19654,39310,19655,58965,22.005282878875732,2.613908418425126e-05
19683,39368,19684,59052,22.037766933441162,2.5601386255402758e-05
19712,39426,19713,59139,22.07314705848694,2.5076416022784542e-05
19741,39484,19742,59226,22.10479497909546,2.465571753873519e-05
19771,39544,19772,59316,22.140310764312744,2.410591764601122e-05
19800,39602,19801,59403,22.177778005599976,2.3630749183212174e-05
19829,39660,19830,59490,22.20933485031128,2.3191809418676712e-05
19858,39718,19859,59577,22.245776891708374,2.2735788661520928e-05
19887,39776,19888,59664,22.280375957489014,2.2305633365249378e-05
19916,39834,19917,59751,22.313249826431274,2.1910631176069728e-05
19945,39892,19946,59838,22.34829092025757,2.152937236132857e-05
19974,39950,19975,59925,22.382774829864502,2.1088711719130515e-05
20003,40008,20004,60012,22.414297819137573,2.0700633854175976e-05
20033,40068,20034,60102,22.452419996261597,2.030835798905173e-05
20062,40126,20063,60189,22.49514603614807,1.9833402461699734e-05
20091,40184,20092,60276,22.536343812942505,1.9558119106477534e-05
20120,40242,20121,60363,22.573680877685547,1.907601858874841e-05
20149,40300,20150,60450,22.606915950775146,1.868735603238747e-05
20178,40358,20179,60537,22.642218112945557,1.82904716439225e-05
20207,40416,20208,60624,22.67529797554016,1.7934603874891764e-05
20236,40474,20237,60711,22.70619797706604,1.759421184033272e-05
20266,40534,20267,60801,22.73852801322937,1.7191384472425852e-05
20295,40592,20296,60888,22.76930594444275,1.690625242645183e-05
20324,40650,20325,60975,22.802342891693115,1.6598249771959672e-05
20353,40708,20354,61062,22.834693908691406,1.625990296361124e-05
20382,40766,20383,61149,22.866328954696655,1.5954458376654657e-05
20411,40824,20412,61236,22.899653911590576,1.5644599898223532e-05
20440,40882,20441,61323,22.938273191452026,1.535365970539715e-05
20469,40940,20470,61410,22.977433919906616,1.5069399296407937e-05
20498,40998,20499,61497,23.014028787612915,1.4789507076784503e-05
20528,41058,20529,61587,23.050002098083496,1.4488472288576304e-05
20557,41116,20558,61674,23.088406085968018,1.4204780995896726e-05
20586,41174,20587,61761,23.121590852737427,1.3911230553276255e-05
20615,41232,20616,61848,23.1598699092865,1.3614998579214443e-05
20644,41290,20645,61935,23.200129747390747,1.3364599453780102e-05
20673,41348,20674,62022,23.245875120162964,1.3062807738606352e-05
20702,41406,20703,62109,23.28574800491333,1.2763154359163309e-05
20731,41464,20732,62196,23.319477081298828,1.2479265819820284e-05
20761,41524,20762,62286,23.353603839874268,1.2236447560098895e-05
20790,41582,20791,62373,23.388503789901733,1.1974751032539643e-05
20819,41640,20820,62460,23.43289303779602,1.173110968011315e-05
20848,41698,20849,62547,23.476903915405273,1.1493490546854446e-05
20877,41756,20878,62634,23.507819175720215,1.1278663464509009e-05
20906,41814,20907,62721,23.55040693283081,1.104304544696788e-05
20935,41872,20936,62808,23.592947006225586,1.0831389658960688e-05
20964,41930,20965,62895,23.63287091255188,1.062838850884873e-05
20993,41988,20994,62982,23.663340091705322,1.0379462651144422e-05
21023,42048,21024,63072,23.705272912979126,1.021042328375188e-05
21052,42106,21053,63159,23.73805809020996,9.980577942769742e-06
21081,42164,21082,63246,23.76912498474121,9.817405612011498e-06
21110,42222,21111,63333,23.800182104110718,9.618820058676647e-06
21139,42280,21140,63420,23.832481145858765,9.42721806040936e-06
21168,42338,21169,63507,23.866971969604492,9.229399779542291e-06
21197,42396,21198,63594,23.89829993247986,9.07222056412138e-06
21226,42454,21227,63681,23.931344032287598,8.892205642041517e-06
21255,42512,21256,63768,23.962602138519287,8.693876452525728e-06
21285,42572,21286,63858,23.99613904953003,8.527647310074826e-06
21314,42630,21315,63945,24.028895139694214,8.366676979676413e-06
21343,42688,21344,64032,24.059355974197388,8.195719146897318e-06
21372,42746,21373,64119,24.091284036636353,8.026730142773886e-06
21401,42804,21402,64206,24.123180866241455,7.888511845521862e-06
21430,42862,21431,64293,24.15436601638794,7.714118282819982e-06
21459,42920,21460,64380,24.194358110427856,7.557411549896642e-06
21488,42978,21489,64467,24.23822593688965,7.410775651806034e-06
21518,43038,21519,64557,24.28326416015625,7.262208669089887e-06
21547,43096,21548,64644,24.330167770385742,7.1489664605906e-06
21576,43154,21577,64731,24.361403942108154,6.987305823713541e-06
21605,43212,21606,64818,24.407012939453125,6.855091783108946e-06
21634,43270,21635,64905,24.452502965927124,6.713075663355994e-06
21663,43328,21664,64992,24.499172925949097,6.5791700762929395e-06
21692,43386,21693,65079,24.536648988723755,6.4507091792620486e-06
21721,43444,21722,65166,24.570065021514893,6.326773018372478e-06
21750,43502,21751,65253,24.6025390625,6.207595220075746e-06
21780,43562,21781,65343,24.638493061065674,6.0906531871296465e-06
21809,43620,21810,65430,24.670977115631104,5.979501338515547e-06
21838,43678,21839,65517,24.70610785484314,5.872201882084482e-06
21867,43736,21868,65604,24.739288806915283,5.759349505751743e-06
21896,43794,21897,65691,24.783151865005493,5.652035383718612e-06
21925,43852,21926,65778,24.827385902404785,5.543867132473679e-06
21954,43910,21955,65865,24.8591890335083,5.449808895718888e-06
21983,43968,21984,65952,24.901614904403687,5.352998869057046e-06
22013,44028,22014,66042,24.94395089149475,5.235814796833438e-06
22042,44086,22043,66129,24.9862539768219,5.130145950715814e-06
22071,44144,22072,66216,25.027027130126953,5.032015337746998e-06
22100,44202,22101,66303,25.05866813659668,4.935396418659366e-06
22129,44260,22130,66390,25.095183849334717,4.840527367377945e-06
22158,44318,22159,66477,25.12839412689209,4.736679215966433e-06
22187,44376,22188,66564,25.160424947738647,4.644697241928952e-06
22216,44434,22217,66651,25.192800998687744,4.552254949885537e-06
22245,44492,22246,66738,25.224284887313843,4.473418812267482e-06
22275,44552,22276,66828,25.25570797920227,4.384485237096669e-06
22304,44610,22305,66915,25.287340879440308,4.301510443838197e-06
22333,44668,22334,67002,25.328798055648804,4.203207140562881e-06
22362,44726,22363,67089,25.360389947891235,4.123722419535625e-06
22391,44784,22392,67176,25.402112007141113,4.047439006171771e-06
22420,44842,22421,67263,25.442019939422607,3.9781831446816796e-06
22449,44900,22450,67350,25.481218814849854,3.878343477481394e-06
22478,44958,22479,67437,25.51162099838257,3.797294539253926e-06
22508,45018,22509,67527,25.553609132766724,3.712137186084874e-06
22537,45076,22538,67614,25.59365200996399,3.6423734854906797e-06
22566,45134,22567,67701,25.633466958999634,3.5709867916011717e-06
22595,45192,22596,67788,25.66436791419983,3.5016727224501665e-06
22624,45250,22625,67875,25.70063805580139,3.4319828046136536e-06
22653,45308,22654,67962,25.733274936676025,3.365607540217752e-06
22682,45366,22683,68049,25.762502908706665,3.3036176319001243e-06
22711,45424,22712,68136,25.793381929397583,3.2400794225395657e-06
22740,45482,22741,68223,25.824362993240356,3.167693762406998e-06
22770,45542,22771,68313,25.854636907577515,3.102795403719938e-06
22799,45600,22800,68400,25.885719776153564,3.0379388817891595e-06
22828,45658,22829,68487,25.915699005126953,2.985852916026488e-06
22857,45716,22858,68574,25.946638822555542,2.92795914447197e-06
22886,45774,22887,68661,25.977808952331543,2.872112531804305e-06
22915,45832,22916,68748,26.006969928741455,2.818334110088472e-06
22944,45890,22945,68835,26.037222862243652,2.770089395198738e-06
22973,45948,22974,68922,26.06690788269043,2.7141353484694264e-06
23003,46008,23004,69012,26.09786605834961,2.65864957782469e-06
23032,46066,23033,69099,26.128354787826538,2.6060733944177628e-06
23061,46124,23062,69186,26.157864093780518,2.5424329805900925e-06
23090,46182,23091,69273,26.188756942749023,2.4866410512913717e-06
23119,46240,23120,69360,26.218204021453857,2.4410338710367796e-06
23148,46298,23149,69447,26.248334884643555,2.3918761371533037e-06
23177,46356,23178,69534,26.278897047042847,2.3436455194314476e-06
23206,46414,23207,69621,26.308865070343018,2.3095640244719107e-06
23235,46472,23236,69708,26.338721752166748,2.2525094891534536e-06
23265,46532,23266,69798,26.369295835494995,2.2092170866017113e-06
23294,46590,23295,69885,26.399361848831177,2.1491412098839646e-06
23323,46648,23324,69972,26.42909288406372,2.106631427523098e-06
23352,46706,23353,70059,26.458359956741333,2.0712044488391257e-06
23381,46764,23382,70146,26.488550901412964,2.0264966451577493e-06
23410,46822,23411,70233,26.517996788024902,1.9900335246347822e-06
23439,46880,23440,70320,26.548972845077515,1.9521360172802815e-06
23468,46938,23469,70407,26.58166003227234,1.915450980050082e-06
23498,46998,23499,70497,26.61321997642517,1.8799953522830037e-06
23527,47056,23528,70584,26.645572900772095,1.8369211147728493e-06
23556,47114,23557,70671,26.67868709564209,1.8058202613246976e-06
23585,47172,23586,70758,26.709557056427002,1.7655343071965035e-06
23614,47230,23615,70845,26.739692211151123,1.7345262222079327e-06
23643,47288,23644,70932,26.769665956497192,1.6988084325930686e-06
23672,47346,23673,71019,26.79877781867981,1.6617154869891237e-06
23701,47404,23702,71106,26.828396797180176,1.631522536627017e-06
23730,47462,23731,71193,26.85826277732849,1.598087123966252e-06
23760,47522,23761,71283,26.891674041748047,1.5661784118492506e-06
23789,47580,23790,71370,26.921120166778564,1.5364274759122054e-06
23818,47638,23819,71457,26.950618982315063,1.5050018191686831e-06
23847,47696,23848,71544,26.980735063552856,1.4750248737982474e-06
23876,47754,23877,71631,27.010493993759155,1.4450043863689643e-06
23905,47812,23906,71718,27.04121494293213,1.416068698745221e-06
23934,47870,23935,71805,27.070791959762573,1.3906009144193376e-06
23963,47928,23964,71892,27.100564002990723,1.3539429346565157e-06
23993,47988,23994,71982,27.131290912628174,1.3247148444861523e-06
24022,48046,24023,72069,27.160823822021484,1.3012098634135327e-06
24051,48104,24052,72156,27.19133496284485,1.2753389455610886e-06
24080,48162,24081,72243,27.220911979675293,1.2509660791693022e-06
24109,48220,24110,72330,27.250513076782227,1.2251645102878683e-06
24138,48278,24139,72417,27.28067374229431,1.1976114819844952e-06
24167,48336,24168,72504,27.309969902038574,1.1710160379152512e-06
24196,48394,24197,72591,27.339958906173706,1.1492973044369137e-06
24225,48452,24226,72678,27.37005090713501,1.1274885309831006e-06
24255,48512,24256,72768,27.40063500404358,1.101699467653816e-06
24284,48570,24285,72855,27.430917978286743,1.07924915937474e-06
24313,48628,24314,72942,27.463001012802124,1.0585373502181028e-06
24342,48686,24343,73029,27.50547218322754,1.0368388529968797e-06
24371,48744,24372,73116,27.540467023849487,1.0159571957046865e-06
24400,48802,24401,73203,27.57779312133789,9.926717439157073e-07
24429,48860,24430,73290,27.608389854431152,9.71353983914014e-07
24458,48918,24459,73377,27.65056300163269,9.509897154202918e-07
24487,48976,24488,73464,27.691514015197754,9.328671239927644e-07
24517,49036,24518,73554,27.73319411277771,9.134959100265405e-07
24546,49094,24547,73641,27.762924909591675,8.950451046985108e-07
24575,49152,24576,73728,27.80402112007141,8.774027264735196e-07
24604,49210,24605,73815,27.844559907913208,8.624934935141937e-07
24633,49268,24634,73902,27.88814091682434,8.43995735522185e-07
24662,49326,24663,73989,27.931001901626587,8.264474899988272e-07
24691,49384,24692,74076,27.962317943572998,8.0810184499569e-07
24720,49442,24721,74163,27.994548082351685,7.917614084362867e-07
24750,49502,24751,74253,28.02641201019287,7.746600658720126e-07
24779,49560,24780,74340,28.055835008621216,7.594119324494386e-07
24808,49618,24809,74427,28.086731910705566,7.440995659635519e-07
24837,49676,24838,74514,28.11637306213379,7.299755679923692e-07
24866,49734,24867,74601,28.14729595184326,7.15702299203258e-07
24895,49792,24896,74688,28.178112983703613,6.999329116297304e-07
24924,49850,24925,74775,28.2079119682312,6.85950908518862e-07
24953,49908,24954,74862,28.238287925720215,6.715306426485768e-07
24982,49966,24983,74949,28.268322944641113,6.589875738427509e-07
25012,50026,25013,75039,28.302134037017822,6.450601404139888e-07
25041,50084,25042,75126,28.34648895263672,6.314425036180182e-07
25070,50142,25071,75213,28.38944387435913,6.183501000123215e-07
25099,50200,25100,75300,28.421813011169434,6.055383892089594e-07
25128,50258,25129,75387,28.453507900238037,5.930979796175961e-07
25157,50316,25158,75474,28.486783027648926,5.818534418722265e-07
25186,50374,25187,75561,28.529435873031616,5.705486501028645e-07
25215,50432,25216,75648,28.574640035629272,5.57159637537552e-07
25245,50492,25246,75738,28.60849118232727,5.455402742882143e-07
25274,50550,25275,75825,28.65116596221924,5.331240799932857e-07
25303,50608,25304,75912,28.690838098526,5.22460709362349e-07
25332,50666,25333,75999,28.732687950134277,5.129901410327875e-07
25361,50724,25362,76086,28.763415813446045,5.0165817810921e-07
25390,50782,25391,76173,28.80258798599243,4.9041216243495e-07
25419,50840,25420,76260,28.842772006988525,4.790347247762838e-07
25448,50898,25449,76347,28.88181781768799,4.685695103034959e-07
25477,50956,25478,76434,28.910754919052124,4.5874685383751057e-07
25507,51016,25508,76524,28.948171138763428,4.4887542571814265e-07
25536,51074,25537,76611,28.991771936416626,4.3978820940537844e-07
25565,51132,25566,76698,29.084707975387573,4.3027409901696956e-07
25594,51190,25595,76785,29.130148887634277,4.2053568449773593e-07
25623,51248,25624,76872,29.159934997558594,4.1368764414073667e-07
25652,51306,25653,76959,29.195854902267456,4.03403646487277e-07
25681,51364,25682,77046,29.231196880340576,3.947152436012402e-07
25710,51422,25711,77133,29.260915994644165,3.848294909403194e-07
25740,51482,25741,77223,29.29952907562256,3.7568918287433917e-07
25769,51540,25770,77310,29.341737031936646,3.678238726934069e-07
25798,51598,25799,77397,29.384535789489746,3.600932814151747e-07
25827,51656,25828,77484,29.41614603996277,3.5215077787142945e-07
25856,51714,25857,77571,29.45371699333191,3.4540232718427433e-07
25885,51772,25886,77658,29.492758750915527,3.3748699479474453e-07
25914,51830,25915,77745,29.54266595840454,3.3040112157323165e-07
25943,51888,25944,77832,29.589242935180664,3.226959961466491e-07
25972,51946,25973,77919,29.63338804244995,3.1490583296545083e-07
26002,52006,26003,78009,29.67902183532715,3.0786998195253545e-07
26031,52064,26032,78096,29.712574005126953,3.011430180777097e-07
26060,52122,26061,78183,29.750337839126587,2.9392674605333013e-07
26089,52180,26090,78270,29.78938889503479,2.876489588743425e-07
26118,52238,26119,78357,29.83120894432068,2.8149258923804155e-07
26147,52296,26148,78444,29.861371994018555,2.7501471322466386e-07
26176,52354,26177,78531,29.904866933822632,2.6949078346660826e-07
26205,52412,26206,78618,29.945921897888184,2.631722963997163e-07
26235,52472,26236,78708,29.986008882522583,2.553231297497405e-07
26264,52530,26265,78795,30.033087968826294,2.505794327589683e-07
26293,52588,26294,78882,30.077862977981567,2.4451674107695e-07
26322,52646,26323,78969,30.107218980789185,2.385205561949988e-07
26351,52704,26352,79056,30.151428937911987,2.3283553218789166e-07
26380,52762,26381,79143,30.192997932434082,2.2639210328634363e-07
26409,52820,26410,79230,30.227200031280518,2.221166823801468e-07
26438,52878,26439,79317,30.256489038467407,2.171739197365241e-07
26467,52936,26468,79404,30.289308071136475,2.1215760170889553e-07
26497,52996,26498,79494,30.323330879211426,2.074198164336849e-07
26526,53054,26527,79581,30.353869915008545,2.0237280295987148e-07
26555,53112,26556,79668,30.39570689201355,1.978377213163185e-07
26584,53170,26585,79755,30.435851097106934,1.936687112902291e-07
26613,53228,26614,79842,30.466317892074585,1.8860100681195036e-07
26642,53286,26643,79929,30.500854969024658,1.8442119653627742e-07
26671,53344,26672,80016,30.53305983543396,1.8000355339609087e-07
26700,53402,26701,80103,30.562665939331055,1.7528088847029721e-07
26730,53462,26731,80193,30.596932888031006,1.7067759472411126e-07
26759,53520,26760,80280,30.638383865356445,1.657513166719582e-07
26788,53578,26789,80367,30.679797172546387,1.6173589756363072e-07
26817,53636,26818,80454,30.714584827423096,1.575089072503033e-07
26846,53694,26847,80541,30.807987928390503,1.5382795481855283e-07
26875,53752,26876,80628,30.850913047790527,1.500999360359856e-07
26904,53810,26905,80715,30.892449855804443,1.4665204162156442e-07
26933,53868,26934,80802,30.94045400619507,1.432011913493625e-07
26962,53926,26963,80889,30.982383012771606,1.396248308083159e-07
26992,53986,26993,80979,31.01396894454956,1.3608860172098503e-07
27021,54044,27022,81066,31.05334210395813,1.3274484444991685e-07
27050,54102,27051,81153,31.097004890441895,1.2907639757031575e-07
27079,54160,27080,81240,31.134080171585083,1.2594875897775637e-07
27108,54218,27109,81327,31.1663761138916,1.2272664662305033e-07
27137,54276,27138,81414,31.197402000427246,1.1903989616257604e-07
27166,54334,27167,81501,31.233131170272827,1.1658607945719268e-07
27195,54392,27196,81588,31.262609004974365,1.1298072877252707e-07
27225,54452,27226,81678,31.307544946670532,1.0986570941895479e-07
27254,54510,27255,81765,31.34969997406006,1.0714222753449576e-07
27283,54568,27284,81852,31.389124870300293,1.0426424523757305e-07
27312,54626,27313,81939,31.42640709877014,1.0131418548553484e-07
27341,54684,27342,82026,31.455985069274902,9.802499789657304e-08
27370,54742,27371,82113,31.486698150634766,9.559562386129983e-08
27399,54800,27400,82200,31.51749587059021,9.313851023762254e-08
27428,54858,27429,82287,31.54803991317749,9.029974989971379e-08
27457,54916,27458,82374,31.578490018844604,8.766744485910749e-08
27487,54976,27488,82464,31.608755111694336,8.501262982463231e-08
27516,55034,27517,82551,31.639319896697998,8.260144568339456e-08
27545,55092,27546,82638,31.669832944869995,8.033657650230452e-08
27574,55150,27575,82725,31.70025897026062,7.790799827489536e-08
27603,55208,27604,82812,31.730498790740967,7.546509550593328e-08
27632,55266,27633,82899,31.759648084640503,7.303901838895399e-08
27661,55324,27662,82986,31.791148900985718,7.08148490957683e-08
27690,55382,27691,83073,31.822057962417603,6.857715106889373e-08
27719,55440,27720,83160,31.852150917053223,6.657137419097126e-08
27749,55500,27750,83250,31.885108947753906,6.422123988159001e-08
27778,55558,27779,83337,31.915423154830933,6.226457571756328e-08
27807,55616,27808,83424,31.951364994049072,6.024913545843447e-08
27836,55674,27837,83511,31.988078832626343,5.815570602862863e-08
27865,55732,27866,83598,32.02492594718933,5.614731435343856e-08
27894,55790,27895,83685,32.05873107910156,5.433173555502435e-08
27923,55848,27924,83772,32.10167098045349,5.246238288236782e-08
27952,55906,27953,83859,32.14052104949951,5.013168902223697e-08
27982,55966,27983,83949,32.17709493637085,4.815706233785022e-08
28011,56024,28012,84036,32.208839893341064,4.667356279242085e-08
28040,56082,28041,84123,32.241211891174316,4.4549096855917014e-08
28069,56140,28070,84210,32.27468705177307,4.299738520785468e-08
28098,56198,28099,84297,32.30714988708496,4.108699158678064e-08
28127,56256,28128,84384,32.33984017372131,3.9242081584234256e-08
28156,56314,28157,84471,32.37233209609985,3.784009550145129e-08
28185,56372,28186,84558,32.40425205230713,3.634340828284621e-08
28214,56430,28215,84645,32.43646001815796,3.479772203718312e-08
28244,56490,28245,84735,32.46820402145386,3.324203134980053e-08
28273,56548,28274,84822,32.499255895614624,3.182969976478489e-08
28302,56606,28303,84909,32.529435873031616,3.0435558073804714e-08
28331,56664,28332,84996,32.55926299095154,2.9063130568829365e-08
28360,56722,28361,85083,32.58969187736511,2.7617602427199017e-08
28389,56780,28390,85170,32.61989092826843,2.6356133275839966e-08
28418,56838,28419,85257,32.650554895401,2.5006215764733497e-08
28447,56896,28448,85344,32.680809020996094,2.3195411813503597e-08
28477,56956,28478,85434,32.7118079662323,2.1954292606096715e-08
28506,57014,28507,85521,32.74192500114441,2.071521976176882e-08
28535,57072,28536,85608,32.77291798591614,1.966486706805881e-08
28564,57130,28565,85695,32.80322790145874,1.8336208995606285e-08
28593,57188,28594,85782,32.8334379196167,1.7252659745281562e-08
28622,57246,28623,85869,32.862919092178345,1.616001554793911e-08
28651,57304,28652,85956,32.89459490776062,1.5117848306545056e-08
28680,57362,28681,86043,32.925647020339966,1.3975181900605094e-08
28709,57420,28710,86130,32.9557089805603,1.2800001059076749e-08
28739,57480,28740,86220,32.98841094970703,1.1771817298722453e-08
28768,57538,28769,86307,33.02295899391174,1.06649622466648e-08
28797,57596,28798,86394,33.05431604385376,9.702944225864485e-09
28826,57654,28827,86481,33.086246967315674,8.636334314360283e-09
28855,57712,28856,86568,33.11931896209717,7.549488145741634e-09
28884,57770,28885,86655,33.15017509460449,6.58121734886663e-09
28913,57828,28914,86742,33.1803719997406,5.662514013238251e-09
28942,57886,28943,86829,33.211215019226074,4.320781954447739e-09
28972,57946,28973,86919,33.24301195144653,3.3888909456436522e-09
29001,58004,29002,87006,33.273301124572754,2.482920535840094e-09
29030,58062,29031,87093,33.303414821624756,1.6307240002788603e-09
29059,58120,29060,87180,33.33357906341553,9.115410648519173e-10
29088,58178,29089,87267,33.36736297607422,6.673417374258861e-11


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007259845733642578,2180.042156630883
1001,2003,2002,4005,1.1795940399169922,26.14702239094254
2002,4005,4004,8009,2.3262481689453125,25.525668687436337
3003,6007,6006,12013,3.71964693069458,24.927473239068604
4004,8009,8008,16017,4.8932459354400635,24.350708440477774
5005,10011,10010,20021,5.921699047088623,23.793850993024307
6006,12013,12012,24025,7.118941307067871,23.255550456593937
7007,14015,14014,28029,8.222760200500488,22.73460611589303
8008,16017,16016,32033,9.309657096862793,22.229947315816844
9009,18019,18018,36037,10.399500131607056,21.74061641815024
10010,20021,20020,40041,11.526769161224365,21.265754038815658
11011,22023,22022,44045,12.682967185974121,20.804586294355204
12012,24025,24024,48049,13.776388168334961,20.35641380682364
13013,26027,26026,52053,14.854856967926025,19.920602236250488
14014,28029,28028,56057,15.909304141998291,19.49657413254613
15015,30031,30030,60061,17.004013061523438,19.0838019223811
16016,32033,32032,64065,18.055104970932007,18.68180186959694
17017,34035,34034,68069,19.10994815826416,18.29012886914711
18018,36037,36036,72073,20.18428897857666,11.918281582526106
19019,38039,38038,76077,21.4948410987854,11.684517022200112
20020,40041,40040,80081,22.78827428817749,11.455797829887729
21021,42043,42042,84085,24.064653158187866,11.231997822684548
22022,44045,44044,88089,25.176217079162598,11.012995041667182
23023,46047,46046,92093,26.286429166793823,10.798671525875193
24024,48049,48048,96097,27.385496139526367,10.588913105067604
25025,50051,50050,100101,28.64294409751892,10.38360920928801
26026,52053,52052,104105,30.02674412727356,10.182652693471141
27027,54055,54054,108109,31.32183814048767,9.985939675502777
28028,56057,56056,112113,32.619301080703735,9.793369386336622
29029,58059,58058,116117,33.885931968688965,9.60484403092164
30030,60061,60060,120121,35.14361810684204,9.420268658853502
31031,62063,62062,124125,36.387397050857544,9.239551043784331
32032,64065,64064,128129,37.625450134277344,9.062601570740298
33033,66067,66066,132133,38.86813807487488,8.889333130602267
34034,68069,68068,136137,40.11537504196167,8.719661021083539
35035,70071,70070,140141,41.366605043411255,8.553502853622945
36036,72073,72072,144145,42.61755013465881,8.390778465685457
37037,74075,74074,148149,43.875221967697144,8.231409838005902
38038,76077,76076,152153,45.13353109359741,8.075321016384578
39039,78079,78078,156157,46.41010308265686,7.922438037678944
40040,80081,80080,160161,47.71730709075928,7.772688859676464
41041,82083,82082,164165,48.958730936050415,7.626003294577117
42042,84085,84084,168169,50.21700310707092,7.482312945832632
43043,86087,86086,172173,51.50854825973511,7.341551148130634
44044,88089,88088,176177,53.02587604522705,7.20365291031851
45045,90091,90090,180181,54.42783308029175,7.068554861092025
46046,92093,92092,184185,55.861876010894775,6.936195197286793
47047,94095,94094,188189,57.218971252441406,6.806513634615385
48048,96097,96096,192193,58.51663112640381,6.679451360717508
49049,98099,98098,196197,59.82755208015442,6.554950990383759
50050,100101,100100,200201,61.13320016860962,6.432956522836093
51051,102103,102102,204205,62.415101289749146,6.313413300938578
52052,104105,104104,208209,63.69599199295044,6.196267972230999
53053,106107,106106,212213,65.00720405578613,6.081468451671753
54054,108109,108108,216217,66.28872799873352,5.96896388599032
55055,110111,110110,220221,67.61755704879761,5.858704619544483
56056,112113,112112,224225,68.98797702789307,5.750642161593305
57057,114115,114114,228229,70.32323408126831,5.644729154886704
58058,116117,116116,232233,71.65373015403748,5.540919345498196
59059,118119,118118,236237,72.95379400253296,5.439167553805987
60060,120121,120120,240241,74.2729001045227,5.339429646559211
61061,122123,122122,244245,75.62810802459717,5.241662509952107
62062,124125,124124,248249,76.95198893547058,5.145824023643854
63063,126127,126126,252253,78.27419114112854,5.051873035662538
64064,128129,128128,256257,79.57120513916016,4.959769338139267
65065,130131,130130,260261,80.86096000671387,4.869473643823085
66066,132133,132132,264265,82.17218518257141,4.780947563328482
67067,134135,134134,268269,83.42770624160767,4.694153583074467
68068,136137,136136,272273,84.8796181678772,4.609055043879607
69069,138139,138138,276277,86.36798119544983,4.525616120176437
70070,140141,140140,280281,88.19514918327332,4.443801799813059
71071,142143,142142,284285,89.67325520515442,4.363577864417721
72072,144145,144144,288289,91.43114018440247,4.284910870297722
73073,146147,146146,292293,93.28204607963562,4.207768129848205
74074,148149,148148,296297,94.98753619194031,4.132117693455598
75075,150151,150150,300301,96.4235692024231,4.057928331867629
76076,152153,152152,304305,97.81100606918335,3.9851695190202463
77077,154155,154154,308309,99.26710915565491,3.9138114153007564
78078,156157,156156,312313,101.05611228942871,3.8438248512326254
79079,158159,158158,316317,103.13152527809143,3.7751813115697814
80080,160161,160160,320321,104.61657333374023,3.707852919785182
81081,162163,162162,324325,106.32327008247375,3.6418124229431896
82082,164165,164164,328329,107.70073819160461,3.5770331769455197
83083,166167,166166,332333,109.41236090660095,3.5134891321358737
84084,168169,168168,336337,111.78809118270874,3.451154819258136
85085,170171,170170,340341,114.22790908813477,3.390005335756655
86086,172173,172172,344345,116.28816723823547,3.3300163324073537
87087,174175,174174,348349,118.05696201324463,3.2711640002773947
88088,176177,176176,352353,119.66448402404785,3.2134250579944137
89089,178179,178178,356357,121.26038026809692,3.1567767393310078
90090,180181,180180,360361,122.7654070854187,3.1011967810850365
91091,182183,182182,364365,124.23370313644409,3.0466634112548263
92092,184185,184184,368369,125.74173307418823,2.993155337499502
93093,186187,186186,372373,127.24480628967285,2.9406517358798965
94094,188189,188188,376377,128.7165629863739,2.8891322398704915
95095,190191,190190,380381,130.22077703475952,2.8385769296378385
96096,192193,192192,384385,131.7515721321106,2.7889663215786413
97097,194195,194194,388389,133.32785606384277,2.7402813581106784
98098,196197,196196,392393,134.9156632423401,2.69250339771213
99099,198199,198198,396397,136.42434811592102,2.6456142052011273
100100,200201,200200,400401,137.92635917663574,2.5995959422509713
101101,202203,202202,404405,139.39918303489685,2.554431158137618
102102,204205,204204,408409,140.9534990787506,2.510102780708962
103103,206207,206206,412413,142.4923939704895,2.466594107574224
104104,208209,208208,416417,143.99782824516296,2.4238887975091075
105105,210211,210210,420421,145.55578422546387,2.3819708620668507
106106,212213,212212,424425,147.12378025054932,2.340824657395501
107107,214215,214214,428429,148.6491482257843,2.3004348762527798
108108,216217,216216,432433,150.1728072166443,2.2607865402159177
109109,218219,218218,436437,151.65597224235535,2.221864992079304
110110,220221,220220,440441,153.1646511554718,2.183655888439489
111111,222223,222222,444445,154.65175414085388,2.1461451924579933
112112,224225,224224,448449,156.13468527793884,2.1093191668012423
113113,226227,226226,452453,157.67368602752686,2.0731643667526214
114114,228229,228228,456457,159.19512391090393,2.0376676334899457
115115,230231,230230,460461,160.73475098609924,2.0028160875287995
116116,232233,232232,464465,162.28593730926514,1.9685971223231036
117117,234235,234234,468469,163.80637407302856,1.934998398021321
118118,236237,236236,472473,165.30495715141296,1.9020078353759118
119119,238239,238238,476477,166.82346320152283,1.8696136097973977
120120,240241,240240,480481,168.34947419166565,1.8378041455559924
121121,242243,242242,484485,169.85480308532715,1.8065681101206792
122122,244245,244244,488489,171.41497325897217,1.775894408637214
123123,246247,246246,492493,172.95771431922913,1.7457721785399372
124124,248249,248248,496497,174.47086691856384,1.7161907842914843
125125,250251,250250,500501,175.98939108848572,1.6871398122522123
126126,252253,252252,504505,177.51455211639404,1.6586090656724082
127127,254255,254254,508509,179.02296018600464,1.6305885598046643
128128,256257,256256,512513,180.5037522315979,1.6030685171351706
129129,258259,258258,516517,182.00149416923523,1.576039362728693
130130,260261,260260,520521,183.54354214668274,1.5494917196859888
131131,262263,262262,524525,185.07923197746277,1.5234164047108152
132132,264265,264264,528529,186.8024880886078,1.4978044237818722
133133,266267,266266,532533,188.54477429389954,1.4726469679309275
134134,268269,268268,536537,190.18777513504028,1.4479354091182586
135135,270271,270270,540541,191.8640420436859,1.4236612962107529
136136,272273,272272,544545,193.5749990940094,1.3998163510535733
137137,274275,274274,548549,195.17804217338562,1.3763924646360692
138138,276277,276276,552553,196.70530200004578,1.3533816933494336
139139,278279,278278,556557,198.17506313323975,1.3307762553329212
140140,280281,280280,560561,199.67023730278015,1.3085685269072656
141141,282283,282282,564565,201.17241024971008,1.2867510390917687
142142,284285,284284,568569,202.6632161140442,1.2653164742059744
143143,286287,286286,572573,204.3516390323639,1.2442576625493302
144144,288289,288288,576577,206.0634422302246,1.2235675791613403
145145,290291,290290,580581,207.77424716949463,1.203239340656296
146146,292293,292292,584585,209.47972512245178,1.183266202135087
147147,294295,294294,588589,211.74727296829224,1.1636415541661336
148148,296297,296296,592593,213.6308789253235,1.1443589198412383
149149,298299,298298,596597,215.14835619926453,1.1254119518971493
150150,300301,300300,600601,216.61712098121643,1.106794429906813
151151,302303,302302,604605,218.10503125190735,1.0885002575352019
152152,304305,304304,608609,219.5931911468506,1.0705234598590323
153153,306307,306306,612613,221.05269193649292,1.0528581807502633
154154,308309,308308,616617,222.5551791191101,1.0354986803187103
155155,310311,310310,620621,224.02160716056824,1.018439332416051
156156,312313,312312,624625,225.48346710205078,1.001674622195992
157157,314315,314314,628629,226.99916219711304,0.9851991437313927
158158,316317,316316,632633,228.47133612632751,0.96900759768846
159159,318319,318318,636637,230.00146508216858,0.9530947890505104
160160,320321,320320,640641,231.47496509552002,0.9374556248991439
161161,322323,322322,644645,232.9546821117401,0.9220851122425984
162162,324325,324324,648649,234.43201518058777,0.9069783558959443
163163,326327,326326,652653,235.96005010604858,0.8921305564089153
164164,328329,328328,656657,237.44164109230042,0.8775370080428502
165165,330331,330330,660661,238.93870520591736,0.8631930967909511
166166,332333,332332,664665,240.43890404701233,0.8490942984474259
167167,334335,334334,668669,241.96577095985413,0.8352361767173306
168168,336337,336336,672673,243.5674171447754,0.8216143813713188
169169,338339,338338,676677,245.31973314285278,0.8082246464417722
170170,340341,340340,680681,247.0700011253357,0.7950627884599726
171171,342343,342342,684685,248.71241331100464,0.7821247047317001
172172,344345,344344,688689,250.42980027198792,0.7694063716559185
173173,346347,346346,692693,252.18307828903198,0.7569038430748378
174174,348349,348348,696697,253.75297832489014,0.7446132486683155
175175,350351,350350,700701,255.6963551044464,0.7325307923786113
176176,352353,352352,704705,257.34341621398926,0.7206527508733416
177177,354355,354354,708709,258.93831515312195,0.7089754720423116
178178,356357,356356,712713,260.61542201042175,0.6974953735289091
179179,358359,358358,716717,262.21469616889954,0.6862089412910564
180180,360361,360360,720721,263.72581028938293,0.6751127281978597
181181,362363,362362,724725,265.35804533958435,0.6642033526565001
182182,364365,364364,728729,267.2003011703491,0.6534774972679998
183183,366367,366366,732733,268.9291250705719,0.6429319075140256
184184,368369,368368,736737,270.50851106643677,0.6325633904739334
185185,370371,370370,740741,272.124587059021,0.62236881356705
186186,372373,372372,744745,273.784019947052,0.6123451033257652
187187,374375,374374,748749,275.3061990737915,0.6024892441938619
188188,376377,376376,752753,276.9939179420471,0.5927982773522444
189189,378379,378378,756757,278.5402190685272,0.5832692995684283
190190,380381,380380,760761,280.0576729774475,0.5738994620750191
191191,382383,382382,764765,281.5452160835266,0.5646859694684281
192192,384385,384384,768769,283.0817000865936,0.555626078634532
193193,386387,386386,772773,284.7252290248871,0.5467170976962734
194194,388389,388388,776777,286.61313819885254,0.5379563849847955
195195,390391,390390,780781,288.6849820613861,0.5293413480334266
196196,392393,392392,784785,290.27971625328064,0.5208694425912199
197197,394395,394394,788789,292.6612300872803,0.5125381716610491
198198,396397,396396,792793,295.1947331428528,0.50434508455578
199199,398399,398398,796797,297.2018790245056,0.49628777597592943
200200,400401,400400,800801,298.97299909591675,0.48836388510744655
201201,402403,402402,804805,300.86432218551636,0.48057109473791115
202202,404405,404404,808809,302.99670028686523,0.47290713039274124
203203,406407,406406,812813,304.6389181613922,0.46536975948879444
204204,408409,408408,816817,306.21801018714905,0.45795679050741
205205,410411,410410,820821,307.866464138031,0.4506660721835942
206206,412413,412412,824825,309.80682706832886,0.4434954927135095
207207,414415,414414,828829,312.64795112609863,0.4364429789782207
208208,416417,416416,832833,315.58292603492737,0.4295064957842669
209209,418419,418418,836837,318.0308301448822,0.4226840451209455
210210,420421,420420,840841,320.91439723968506,0.41597366543123826
211211,422423,422422,844845,323.2616980075836,0.40937343090058675
212212,424425,424424,848849,324.79346990585327,0.4028814507586276
213213,426427,426426,852853,326.28093218803406,0.3964958685972988
214214,428429,428428,856857,327.7789659500122,0.390214861702475
215215,430431,430430,860861,329.25873708724976,0.3840366403982216
216216,432433,432432,864865,330.79500102996826,0.37795944740821596
217217,434435,434434,868869,332.28206515312195,0.37198155722717274
218218,436437,436436,872873,333.7859010696411,0.3661012755071624
219219,438439,438438,876877,335.4068121910095,0.3603169384555258
220220,440441,440440,880881,336.9550371170044,0.3546269122469994
221221,442443,442442,884885,338.49807119369507,0.34902959244629983
222222,444445,444444,888889,339.995548248291,0.3435234034437826
223223,446447,446446,892893,341.51244711875916,0.33810679790212816
224224,448449,448448,896897,343.00766611099243,0.33277825621496504
225225,450451,450450,900901,344.53441619873047,0.3275362859760662
226226,452453,452452,904905,345.9988579750061,0.3223794214602549
227227,454455,454454,908909,347.47288393974304,0.3173062231142012
228228,456457,456456,912913,349.00755500793457,0.31231527705836015
229229,458459,458458,916917,350.7804663181305,0.3074051945980045
230230,460461,460460,920921,352.28906321525574,0.30257461174608125
231231,462463,462462,924925,353.981290102005,0.297822188753571
232232,464465,464464,928929,355.5675640106201,0.29314660965121675
233233,466467,466466,932933,357.0582709312439,0.2885465818001194
234234,468469,468468,936937,359.20693826675415,0.284020835450292
235235,470471,470470,940941,361.2550621032715,0.2795681233103551
236236,472473,472472,944945,363.4934060573578,0.2751872201243941
237237,474475,474474,948949,365.15199732780457,0.2708769222565479
238238,476477,476476,952953,366.75338912010193,0.26663604728685186
239239,478479,478478,956957,368.3124601840973,0.2624634336125382
240240,480481,480480,960961,369.87755012512207,0.2583579400582039
241241,482483,482482,964965,371.43376302719116,0.2543184454945049
242242,484485,484484,968969,373.0047879219055,0.2503438484634444
243243,486487,486486,972973,374.592493057251,0.2464330668119601
244244,488489,488488,976977,376.17693519592285,0.24258503733233283
245245,490491,490490,980981,377.6888921260834,0.23879871541021203
246246,492493,492492,984985,379.30817317962646,0.23507307467878036
247247,494495,494494,988989,380.9773449897766,0.23140710668064912
248248,496497,496496,992993,382.53432607650757,0.2277998205372569
249249,498499,498498,996997,384.05974292755127,0.22425024262213356
250250,500501,500500,1001001,385.63947224617004,0.22075741624360035
251251,502503,502502,1005005,387.20777130126953,0.21732040133122155
252252,504505,504504,1009009,388.7677011489868,0.21393827413135114
253253,506507,506506,1013013,390.25963592529297,0.21061012690518055
254254,508509,508508,1017017,391.84009313583374,0.20733506763610876
255255,510511,510510,1021021,393.3335340023041,0.20411221973995453
256256,512513,512512,1025025,394.8935899734497,0.20094072178369515
257257,514515,514514,1029029,396.52060532569885,0.19781972720636531
258258,516517,516516,1033033,398.2976040840149,0.19474840404859606
259259,518519,518518,1037037,399.87741708755493,0.19172593468647392
260260,520521,520520,1041041,401.3858461380005,0.1887515155683559
261261,522523,522522,1045045,402.9370491504669,0.18582435696089306
262262,524525,524524,1049049,404.66888213157654,0.1829436826960773
263263,526527,526526,1053053,406.20707726478577,0.18010872992624627
264264,528529,528528,1057057,407.94826912879944,0.17731874888102084
265265,530531,530530,1061061,409.95349192619324,0.1745730026318597
266266,532533,532532,1065065,411.50649213790894,0.1718707668588877
267267,534535,534534,1069069,413.2206621170044,0.16921132962306729
268268,536537,536536,1073073,414.7425501346588,0.1665939911431451
269269,538539,538538,1077077,416.93540930747986,0.16401806357669102
270270,540541,540540,1081081,418.53764605522156,0.16148287080409318
271271,542543,542542,1085085,420.11750507354736,0.15898774821891948
272272,544545,544544,1089089,421.64338421821594,0.15653204252055275
273273,546547,546546,1093093,423.6504690647125,0.15411511151160084
274274,548549,548548,1097097,425.66623306274414,0.15173632389883096
275275,550551,550550,1101101,427.2003390789032,0.14939505909808304
276276,552553,552552,1105105,428.721204996109,0.14709070704270744
277277,554555,554554,1109109,430.7197461128235,0.1448226679964364
278278,556557,556556,1113113,432.34219908714294,0.14259035236784712
279279,558559,558558,1117117,433.8383810520172,0.14039318053107763
280280,560561,560560,1121121,435.33324122428894,0.13823058264813426
281281,562563,562562,1125125,436.8505551815033,0.13610199849381388
282282,564565,564564,1129129,438.31437706947327,0.1340068772867653
283283,566567,566566,1133133,439.83183097839355,0.13194467752134642
284284,568569,568568,1137137,441.3703889846802,0.12991486680266462
285285,570571,570570,1141141,442.86720609664917,0.1279169216866194
286286,572573,572572,1145145,444.34007716178894,0.12595032752051338
287287,574575,574574,1149149,445.8329322338104,0.12401457828934781
288288,576577,576576,1153153,447.3150372505188,0.12210917646223152
289289,578579,578578,1157157,449.32796597480774,0.12023363284311017
290290,580581,580580,1161161,451.41433119773865,0.11838746642513343
291291,582583,582582,1165165,453.0999901294708,0.11657020424570419
292292,584585,584584,1169169,455.19635009765625,0.11478138124550696
293293,586587,586586,1173173,457.5887451171875,0.11302054013026464
294294,588589,588588,1177177,459.6534252166748,0.11128723123465534
295295,590591,590590,1181181,461.363379240036,0.10958101238850304
296296,592593,592592,1185185,463.14642810821533,0.10790144878603769
297297,594595,594594,1189189,464.7587630748749,0.10624811285708802
298298,596597,596596,1193193,466.25017499923706,0.10462058414123021
299299,598599,598598,1197197,467.73979806900024,0.10301844916364189
300300,600601,600600,1201201,469.26269793510437,0.10144130131379825
301301,602603,602602,1205205,471.1866521835327,0.09988874072575982
302302,604605,604604,1209209,473.1780331134796,0.09836037416130239
303303,606607,606606,1213213,474.9058561325073,0.09685581489463857
304304,608609,608608,1217217,476.59424209594727,0.09537468259952675
305305,610611,610610,1221221,478.1454691886902,0.09391660323979067
306306,612613,612612,1225225,479.7596561908722,0.09248120895779266
307307,614615,614614,1229229,481.3715012073517,0.09106813797041013
308308,616617,616616,1233233,482.89807510375977,0.0896770344622837
309309,618619,618618,1237237,484.39459705352783,0.08830754848452216
310310,620621,620620,1241241,485.875675201416,0.08695933585170224
311311,622623,622622,1245245,487.516371011734,0.08563205804443896
312312,624625,624624,1249249,489.1335492134094,0.08432538211093288
313313,626627,626626,1253253,490.69351720809937,0.08303898057181414
314314,628629,628628,1257257,492.29329204559326,0.08177253132555506
315315,630631,630630,1261261,493.8545620441437,0.080525717557407
316316,632633,632632,1265265,495.39056730270386,0.07929822764765504
317317,634635,634634,1269269,497.0248181819916,0.07808975508351068
318318,636637,636636,1273273,498.61791610717773,0.07689999837145933
319319,638639,638638,1277277,500.20578622817993,0.07572866095199515
320320,640641,640640,1281281,501.78021907806396,0.07457545111446962
321321,642643,642642,1285285,503.315443277359,0.07344008191546436
322322,644645,644644,1289289,504.8793489933014,0.07232227109648193
323323,646647,646646,1293293,506.4813241958618,0.07122174100584289
324324,648649,648648,1297297,508.06101512908936,0.07013821851865032
325325,650651,650650,1301301,509.5917110443115,0.06907143496118806
326326,652653,652652,1305305,511.08121705055237,0.06802112603475052
327327,654655,654654,1309309,512.6914203166962,0.06698703174106413
328328,656657,656656,1313313,514.3622419834137,0.0659688963106646
329329,658659,658658,1317317,516.1433589458466,0.06496646813047846
330330,660661,660660,1321321,517.7964069843292,0.06397949967333716
331331,662663,662662,1325325,520.2968990802765,0.06300774742953763
332332,664665,664664,1329329,523.2275912761688,0.06205097183919861
333333,666667,666666,1333333,525.8577771186829,0.06110893722450328
334334,668669,668668,1337337,528.0438961982727,0.060181411725466205
335335,670671,670670,1341341,529.8068730831146,0.05926816723558659
336336,672673,672672,1345345,531.390064239502,0.05836897933738783
337337,674675,674674,1349349,532.9355289936066,0.05748362724239087
338338,676677,676676,1353353,534.5206830501556,0.056611893728700124
339339,678679,678678,1357357,536.0964012145996,0.055753565081545275
340340,680681,680680,1361361,537.663003206253,0.05490843103518728
341341,682683,682682,1365365,539.7003610134125,0.0540762847139149
342342,684685,684684,1369369,542.3308391571045,0.05325692257611081
343343,686687,686686,1373373,545.1068360805511,0.052450144358545
344344,688689,688688,1377377,548.5826501846313,0.05165575302146408
345345,690691,690690,1381381,551.3040211200714,0.05087355469413524
346346,692693,692692,1385385,552.901643037796,0.05010335862334614
347347,694695,694694,1389389,554.8709750175476,0.04934497712008579
348348,696697,696696,1393393,557.1469252109528,0.04859822550952231
349349,698699,698698,1397397,559.3552892208099,0.0478629220797302
350350,700701,700700,1401401,561.3339900970459,0.04713888803394184
351351,702703,702702,1405405,562.9791371822357,0.04642594744063899
352352,704705,704704,1409409,564.5845000743866,0.04572392718739593
353353,706707,706706,1413413,567.077445268631,0.04503265693222147
354354,708709,708708,1417417,568.6232941150665,0.04435196905956218
355355,710711,710710,1421421,570.1065752506256,0.043681698634486565
356356,712713,712712,1425425,571.6650969982147,0.04302168335755141
357357,714715,714714,1429429,573.1418361663818,0.042371763522510264
358358,716717,716716,1433433,574.6664183139801,0.04173178197220295
359359,718719,718718,1437437,576.1841042041779,0.041101584057628315
360360,720721,720720,1441441,577.6829092502594,0.04048101759542533
361361,722723,722722,1445445,579.2352561950684,0.0398699328281964
362362,724725,724724,1449449,581.0741429328918,0.039268182384375905
363363,726727,726726,1453453,582.7797319889069,0.038675621238098756
364364,728729,728728,1457457,585.1400640010834,0.038092106671570036
365365,730731,730730,1461461,586.7927751541138,0.037517498236752544
366366,732733,732732,1465465,588.3198721408844,0.03695165771830489
367367,734735,734734,1469469,590.1658930778503,0.03639444909640588
368368,736737,736736,1473473,591.7107923030853,0.035845738510829506
369369,738739,738738,1477477,593.2155442237854,0.035305394226725184
370370,740741,740740,1481481,594.7619199752808,0.0347732865980106
371371,742743,742742,1485485,596.4641170501709,0.0342492880346299
372372,744745,744744,1489489,598.000785112381,0.033733272967765515
373373,746747,746746,1493493,599.5298130512238,0.03322511781789217
374374,748749,748748,1497497,601.0883829593658,0.03272470096123925
375375,750751,750750,1501501,602.7636561393738,0.03223190269909537
376376,752753,752752,1505505,604.3578491210938,0.0317466052247255
377377,754755,754754,1509509,605.8951869010925,0.031268692594494496
378378,756757,756756,1513513,607.6248090267181,0.030798050695807433
379379,758759,758758,1517517,609.2632071971893,0.03033456721868788
380380,760761,760760,1521521,610.8217370510101,0.029878131624627713
381381,762763,762762,1525525,612.3644690513611,0.02942863512043914
382382,764765,764764,1529529,614.0532360076904,0.02898597062733188
383383,766767,766766,1533533,615.7891619205475,0.028550032754424137
384384,768769,768768,1537537,617.6531262397766,0.028120717771230375
385385,770771,770770,1541541,619.1610281467438,0.027697923580603856
386386,772773,772772,1545545,620.6630730628967,0.027281549691679174
387387,774775,774774,1549549,622.171067237854,0.026871497195429583
388388,776777,776776,1553553,623.644562959671,0.026467668737041095
389389,778779,778778,1557557,625.1332352161407,0.02606996849283405
390390,780781,780780,1561561,626.8594212532043,0.025678302143319343
391391,782783,782782,1565565,628.3972952365875,0.025292576851256854
392392,784785,784784,1569569,629.907014131546,0.024912701235507484
393393,786787,786786,1573573,631.4175832271576,0.02453858534909159
394394,788789,788788,1577577,633.0173420906067,0.024170140655883188
395395,790791,790790,1581581,634.5330770015717,0.02380728000639465
396396,792793,792792,1585585,636.0590801239014,0.023449917617767824
397397,794795,794794,1589589,637.8171992301941,0.023097969050127176
398398,796797,796796,1593593,639.4200539588928,0.02275135118520666
399399,798799,798798,1597597,640.9992492198944,0.022409982205658707
400400,800801,800800,1601601,642.5034720897675,0.022073781574022178
401401,802803,802802,1605605,644.0190951824188,0.02174267001134922
402402,804805,804804,1609609,645.7599742412567,0.021416569478105885
403403,806807,806806,1613613,647.3812081813812,0.02109540315382219
404404,808809,808808,1617617,649.3574032783508,0.020779095417424287
405405,810811,810810,1621621,651.4843780994415,0.020467571828589826
406406,812813,812812,1625625,653.5293941497803,0.020160759107398007
407407,814815,814814,1629629,655.5177159309387,0.01985858511807237
408408,816817,816816,1633633,657.5923199653625,0.019560978848062405
409409,818819,818818,1637637,660.1882429122925,0.019267870392809527
410410,820821,820820,1641641,662.0819020271301,0.018979190935851875
411411,822823,822822,1645645,665.397066116333,0.018694872732112344
412412,824825,824824,1649649,667.6630783081055,0.01841484909130031
413413,826827,826826,1653653,669.7466340065002,0.018139054360631235
414414,828829,828828,1657657,672.384458065033,0.01786742390845575
415415,830831,830830,1661661,674.3378810882568,0.01759989410788876
416416,832833,832832,1665665,677.810711145401,0.01733640232112066
417417,834835,834834,1669669,681.4378671646118,0.01707688688259168
418418,836837,836836,1673673,684.5225789546967,0.016821287085349468
419419,838839,838838,1677677,686.9299609661102,0.016569543164109746
420420,840841,840840,1681681,688.788064956665,0.016321596281272832
421421,842843,842842,1685685,692.3182451725006,0.016077388512030666
422422,844845,844844,1689689,695.3223762512207,0.015836862829360143
423423,846847,846846,1693693,697.3879821300507,0.015599963090835445
424424,848849,848848,1697697,698.9617540836334,0.015366634023052939
425425,850851,850850,1701701,700.4826261997223,0.015136821209580376
426426,852853,852852,1705705,702.8047559261322,0.01491047107583654
427427,854855,854854,1709709,705.8013679981232,0.014687530877381505
428428,856857,856856,1713713,708.7302520275116,0.01446794868456891
429429,858859,858858,1717717,711.6042001247406,0.014251673372427831
430430,860861,860860,1721721,714.3998332023621,0.014038654605542433
431431,862863,862862,1725725,717.0025761127472,0.013828842826569598
432432,864865,864864,1729729,718.6707310676575,0.013622189244188121
433433,866867,866866,1733733,720.3875179290771,0.013418645820479469
434434,868869,868868,1737737,722.1322441101074,0.013218165259786474
435435,870871,870870,1741741,723.5288870334625,0.013020700995639345
436436,872873,872872,1745745,725.3416330814362,0.012826207180864913
437437,874875,874874,1749749,727.169379234314,0.012634638674967391
438438,876877,876876,1753753,728.9817941188812,0.012445951033782876
439439,878879,878878,1757757,730.949716091156,0.01226010049845172
440440,880881,880880,1761761,732.792720079422,0.012077043983822477
441441,882883,882882,1765765,734.568883895874,0.011896739069470641
442442,884885,884884,1769769,736.3967680931091,0.011719143987193092
443443,886887,886886,1773773,738.2464921474457,0.011544217612595276
444444,888889,888888,1777777,740.0928580760956,0.011371919453836199
445445,890891,890890,1781781,741.8705153465271,0.011202209642306116
446446,892893,892892,1785785,743.6093370914459,0.011035048922394708
447447,894895,894894,1789789,745.5456829071045,0.01087039864239614
448448,896897,896896,1793793,747.0367112159729,0.010708220744277241
449449,898899,898898,1797797,748.555260181427,0.010548477755264685
450450,900901,900900,1801801,750.401407957077,0.01039113277784054
451451,902903,902902,1805805,752.6495380401611,0.010236149481784196
452452,904905,904904,1809809,754.1847331523895,0.010083492093713176
453453,906907,906906,1813813,755.7092111110687,0.009933125390489295
454454,908909,908908,1817817,757.2073981761932,0.009785014688418414
455455,910911,910910,1821821,758.7280261516571,0.009639125836315543
456456,912913,912912,1825825,760.2682130336761,0.009495425206523578
457457,914915,914914,1829829,761.7895221710205,0.009353879687068911
458458,916917,916916,1833833,763.3428790569305,0.009214456673134919
459459,918919,918918,1837837,764.8480451107025,0.009077124060354436
460460,920921,920920,1841841,766.5401821136475,0.008941850234805315
461461,922923,922922,1845845,768.1959221363068,0.00880860406755346
462462,924925,924924,1849849,769.8621640205383,0.008677354906353685
463463,926927,926926,1853853,771.8039722442627,0.0085480725671232
464464,928929,928928,1857857,773.4362001419067,0.008420727328484645
465465,930931,930930,1861861,775.0396552085876,0.00829528992358064
466466,932933,932932,1865865,776.6521451473236,0.008171731532911508
467467,934935,934934,1869869,778.1301419734955,0.008050023777400384
468468,936937,936936,1873873,779.7703700065613,0.00793013871191306
469469,938939,938938,1877877,781.3749771118164,0.007812048818664152
470470,940941,940940,1881881,783.583419084549,0.007695726999486396
471471,942943,942942,1885885,785.4646000862122,0.007581146570259989
472472,944945,944944,1889889,787.9025871753693,0.007468281254887188
473473,946947,946946,1893893,790.5282521247864,0.007357105178016354
474474,948949,948948,1897897,792.4607989788055,0.007247592858561802
475475,950951,950950,1901901,794.0889840126038,0.007139719205156325
476476,952953,952952,1905905,795.7511191368103,0.007033459507965745
477477,954955,954954,1909909,797.3106770515442,0.006928789434937244
478478,956957,956956,1913913,798.8483581542969,0.0068256850249781564
479479,958959,958958,1917917,800.5611410140991,0.006724122681362132
480480,960961,960960,1921921,802.0570139884949,0.00662407916763641
481481,962963,962962,1925925,803.5787560939789,0.006525531600573231
482482,964965,964964,1929929,805.2137882709503,0.006428457446645552
483483,966967,966966,1933933,806.7932181358337,0.0063328345140689635
484484,968969,968968,1937937,808.3869462013245,0.006238640949845831
485485,970971,970970,1941941,809.9829759597778,0.0061458552328303995
486486,972973,972972,1945945,811.5577092170715,0.006054456170204503
487487,974975,974974,1949949,813.1222379207611,0.005964422890542664
488488,976977,976976,1953953,814.5959300994873,0.0058757348407425525
489489,978979,978978,1957957,816.1297950744629,0.0057883717792037714
490490,980981,980980,1961961,817.8149790763855,0.005702313772872003
491491,982983,982982,1965965,819.3522491455078,0.005617541191440978
492492,984985,984984,1969969,820.8476331233978,0.005534034702691315
493493,986987,986986,1973973,822.3351612091064,0.005451775267829362
494494,988989,988988,1977977,823.8725380897522,0.005370744137849215
495495,990991,990990,1981981,825.6499111652374,0.005290922847962065
496496,992993,992992,1985985,827.3890151977539,0.005212293213844532
497497,994995,994994,1989989,829.4466390609741,0.005134837326977504
498498,996997,996996,1993993,831.0240662097931,0.005058537551008158
499499,998999,998998,1997997,833.0552780628204,0.0049833765167477395
500501,1001003,1001002,2002005,836.1048760414124,0.004909263707872924
501502,1003005,1003004,2006009,838.6466691493988,0.004836330194734728
502503,1005007,1005006,2010013,841.2880780696869,0.004764484864153928
503504,1007009,1007008,2014017,843.5925559997559,0.004693711376830834
504505,1009011,1009010,2018021,845.8557350635529,0.004623993641530433
505506,1011013,1011012,2022025,847.6878709793091,0.004555315810421234
506507,1013015,1013014,2026029,849.3420243263245,0.004487662275892035
507508,1015017,1015016,2030033,850.9028761386871,0.004421017666686566
508509,1017019,1017018,2034037,852.5422389507294,0.004355366844492892
509510,1019021,1019020,2038041,854.0552771091461,0.004290694900191738
510511,1021023,1021022,2042045,855.5235331058502,0.0042269871496500855
511512,1023025,1023024,2046049,857.0147771835327,0.004164229132015862
512513,1025027,1025026,2050053,858.5559821128845,0.0041024066042609775
513514,1027029,1027028,2054057,860.50776720047,0.0040415055392486465
514515,1029031,1029030,2058061,862.3261382579803,0.00398151212209541
515516,1031033,1031032,2062065,864.1315839290619,0.003922412746874215
516517,1033035,1033034,2066069,866.2438342571259,0.0038641940129764407
517518,1035037,1035036,2070073,868.0963389873505,0.0038068427224970947
518519,1037039,1037038,2074077,869.6889662742615,0.00375034587727896
519520,1039041,1039040,2078081,871.1749949455261,0.0036946906751609276
520521,1041043,1041042,2082085,872.776819229126,0.00363986450770426
521522,1043045,1043044,2086089,874.3531792163849,0.003585854956440926
522523,1045047,1045046,2090093,875.880743265152,0.003532649791281983
523524,1047049,1047048,2094097,877.4042181968689,0.003480236966083794
524525,1049051,1049050,2098101,878.8895652294159,0.0034286046166016604
525526,1051053,1051052,2102105,880.3550572395325,0.0033777410579887146
526527,1053055,1053054,2106109,881.9977781772614,0.0033276347814990004
527528,1055057,1055056,2110113,883.6058731079102,0.003278274452327423
528529,1057059,1057058,2114117,885.1387960910797,0.0032296489058580846
529530,1059061,1059060,2118121,886.6425981521606,0.003181747147209535
530531,1061063,1061062,2122125,888.1362800598145,0.0031345583460051785
531532,1063065,1063064,2126129,889.636155128479,0.00308807183580484
532533,1065067,1065066,2130133,891.1420862674713,0.003042277110694158
533534,1067069,1067068,2134137,892.7921981811523,0.002997163823692972
534535,1069071,1069070,2138141,894.3886179924011,0.002952721783231027
535536,1071073,1071072,2142145,896.070867061615,0.002908940950874239
536537,1073075,1073074,2146149,897.6103191375732,0.002865811440642574
537538,1075077,1075076,2150153,899.7677550315857,0.0028233235142351987
538539,1077079,1077078,2154157,901.8834321498871,0.0027814675809167966
539540,1079081,1079080,2158161,903.6667912006378,0.0027402341936522134
540541,1081083,1081082,2162165,905.810506105423,0.0026996140481969633
541542,1083085,1083084,2166169,907.4173691272736,0.00265959797980031
542543,1085087,1085086,2170173,909.201238155365,0.0026201769624094595
543544,1087089,1087088,2174177,910.911865234375,0.002581342105031581
544545,1089091,1089090,2178181,912.5965192317963,0.002543084651051686
545546,1091093,1091092,2182185,914.1418323516846,0.002505395974935709
546547,1093095,1093094,2186189,915.7088830471039,0.002468267581662076
547548,1095097,1095096,2190193,917.4667460918427,0.002431691102970035
548549,1097099,1097098,2194197,919.2477612495422,0.0023956582973596596
549550,1099101,1099100,2198201,921.2025473117828,0.002360161047135989
550551,1101103,1101102,2202205,923.8152089118958,0.002325191355680545
551552,1103105,1103104,2206209,925.7929100990295,0.002290741347792391
552553,1105107,1105106,2210213,927.7145531177521,0.002256803265936469
553554,1107109,1107108,2214217,929.5067710876465,0.0022233694692204153
554555,1109111,1109110,2218221,931.4372930526733,0.002190432431575573
555556,1111113,1111112,2222225,933.7844779491425,0.0021579847399380014
556557,1113115,1113114,2226229,936.6204779148102,0.002126019092884235
557558,1115117,1115116,2230233,938.9176681041718,0.0020945282980164848
558559,1117119,1117118,2234237,940.7468600273132,0.0020635052715078928
559560,1119121,1119120,2238241,942.8552482128143,0.002032943035487733
560561,1121123,1121122,2242245,944.837485074997,0.002002834717245605
561562,1123125,1123124,2246249,947.1041362285614,0.0019731735466166356
562563,1125127,1125126,2250253,949.239520072937,0.001943952855867792
563564,1127129,1127128,2254257,951.1296372413635,0.0019151660764009648
564565,1129131,1129130,2258261,953.1783459186554,0.0018868067386392795
565566,1131133,1131132,2262265,955.0523393154144,0.0018588684698670477
566567,1133135,1133134,2266269,956.9866979122162,0.001831344993206585
567568,1135137,1135136,2270273,959.0573220252991,0.001804230125912909
568569,1137139,1137138,2274277,961.0046830177307,0.001777517777554749
569570,1139141,1139140,2278281,962.9685859680176,0.0017512019492187392
570571,1141143,1141142,2282285,964.7051980495453,0.0017252767320314888
571572,1143145,1143144,2286289,967.0113160610199,0.001699736305681654
572573,1145147,1145146,2290293,968.9869351387024,0.0016745749368283214
573574,1147149,1147148,2294297,971.2727501392365,0.001649786978305201
574575,1149151,1149150,2298301,972.9682869911194,0.0016253668671879495
575576,1151153,1151152,2302305,974.5549621582031,0.0016013091244531097
576577,1153155,1153154,2306309,976.6750421524048,0.0015776083524770002
577578,1155157,1155156,2310313,978.4744801521301,0.001554259235263089
578579,1157159,1157158,2314317,980.1851179599762,0.00153125653571351
579580,1159161,1159160,2318321,982.3390951156616,0.0015085950956290617
580581,1161163,1161162,2322325,984.3168849945068,0.0014862698335491586
581582,1163165,1163164,2326329,986.2876541614532,0.0014642757444107701
582583,1165167,1165166,2330333,988.1852931976318,0.0014426078982978652
583584,1167169,1167168,2334337,990.7245411872864,0.0014212614386224232
584585,1169171,1169170,2338341,992.9262919425964,0.001400231581214939
585586,1171173,1171172,2342345,995.0768890380859,0.001379513614665484
586587,1173175,1173174,2346349,997.1208891868591,0.0013591028966857266
587588,1175177,1175176,2350353,999.3885953426361,0.0013389948552458009
588589,1177179,1177178,2354357,1001.8025572299957,0.0013191849866416305
589590,1179181,1179180,2358361,1004.1730370521545,0.0012996688541306867
590591,1181183,1181182,2362365,1006.6939721107483,0.001280442087818301
591592,1183185,1183184,2366369,1008.4283781051636,0.0012615003824976156
592593,1185187,1185186,2370373,1010.0879952907562,0.0012428394981043311
593594,1187189,1187188,2374377,1012.2809252738953,0.0012244552572155953
594595,1189191,1189190,2378381,1014.340765953064,0.001206343545618438
595596,1191193,1191192,2382385,1016.4234330654144,0.0011885003099223468
596597,1193195,1193194,2386389,1018.1745882034302,0.0011709215574455811
597598,1195197,1195196,2390393,1020.2896840572357,0.0011536033555330505
598599,1197199,1197198,2394397,1022.3095669746399,0.0011365418298510122
599600,1199201,1199200,2398401,1024.4930229187012,0.0011197331642733843
600601,1201203,1201202,2402405,1026.4428851604462,0.0011031735991764435
601602,1203205,1203204,2406409,1028.563856124878,0.0010868594321209457
602603,1205207,1205206,2410413,1030.449823141098,0.0010707870146688947
603604,1207209,1207208,2414417,1032.1830151081085,0.0010549527538614711
604605,1209211,1209210,2418421,1033.8438053131104,0.0010393531098316089
605606,1211213,1211212,2422425,1035.5546402931213,0.001023984595803995
606607,1213215,1213214,2426429,1037.469918012619,0.0010088437769582015
607608,1215217,1215216,2430433,1039.2710070610046,0.0009939272695191903
608609,1217219,1217218,2434437,1041.124252319336,0.0009792317409846873
609610,1219221,1219220,2438441,1042.7576892375946,0.0009647539076240719
610611,1221223,1221222,2442445,1045.0053009986877,0.0009504905353878712
611612,1223225,1223224,2446449,1047.0057060718536,0.0009364384382024582
612613,1225227,1225226,2450453,1049.0252270698547,0.0009225944777426776
613614,1227229,1227228,2454457,1050.8084700107574,0.0009089555619539169
614615,1229231,1229230,2458461,1052.5128309726715,0.0008955186457342279
615616,1231233,1231232,2462465,1054.4367260932922,0.0008822807286605894
616617,1233235,1233234,2466469,1056.3818521499634,0.0008692388554436548
617618,1235237,1235236,2470473,1058.1422581672668,0.0008563901147908837
618619,1237239,1237238,2474477,1060.458722114563,0.0008437316386107341
619620,1239241,1239240,2478481,1062.5679411888123,0.0008312606021263491
620621,1241243,1241242,2482485,1064.3781960010529,0.0008189742220565677
621622,1243245,1243244,2486489,1066.6340773105621,0.0008068697568432981
622623,1245247,1245246,2490493,1068.7439920902252,0.0007949445059693971
623624,1247249,1247248,2494497,1070.7350809574127,0.0007831958089354885
624625,1249251,1249250,2498501,1072.57355594635,0.0007716210452599626
625626,1251253,1251252,2502505,1074.807636976242,0.0007602176326599874
626627,1253255,1253254,2506509,1076.6504321098328,0.0007489830281883769
627628,1255257,1255256,2510513,1078.6804699897766,0.0007379147267556618
628629,1257259,1257258,2514517,1080.8538491725922,0.0007270102598795347
629630,1259261,1259260,2518521,1083.2362382411957,0.0007162671965943446
630631,1261263,1261262,2522525,1084.943349123001,0.0007056831418594811
631632,1263265,1263264,2526529,1086.8966190814972,0.0006952557362183143
632633,1265267,1265266,2530533,1088.6470441818237,0.0006849826553434468
633634,1267269,1267268,2534537,1090.7213671207428,0.0006748616095819671
634635,1269271,1269270,2538541,1092.9485449790955,0.0006648903436143883
635636,1271273,1271272,2542545,1095.1926550865173,0.0006550666354314671
636637,1273275,1273274,2546549,1097.6387820243835,0.0006453882961068302
637638,1275277,1275276,2550553,1099.8760421276093,0.0006358531694559133
638639,1277279,1277278,2554557,1101.7378532886505,0.0006264591310127798
639640,1279281,1279280,2558561,1103.745126247406,0.0006172040885985552
640641,1281283,1281282,2562565,1105.421198129654,0.000608085980843498
641642,1283285,1283284,2566569,1107.0709722042084,0.0005991027763911916
642643,1285287,1285286,2570573,1109.1360230445862,0.0005902524752627869
643644,1287289,1287288,2574577,1110.9205050468445,0.0005815331065832652
644645,1289291,1289290,2578581,1112.705765247345,0.0005729427291498723
645646,1291293,1291292,2582585,1114.3673241138458,0.0005644794296131295
646647,1293295,1293294,2586589,1115.9042291641235,0.0005561413249779434
647648,1295297,1295296,2590593,1117.8419771194458,0.0005479265581698201
648649,1297299,1297298,2594597,1120.411992073059,0.0005398333013317824
649650,1299301,1299300,2598601,1122.5229182243347,0.0005318597532095737
650651,1301303,1301302,2602605,1124.1293733119965,0.0005240041390379702
651652,1303305,1303304,2606609,1125.9328451156616,0.0005162647107681551
652653,1305307,1305306,2610613,1127.6989431381226,0.0005086397466129711
653654,1307309,1307308,2614617,1129.26234126091,0.0005011275496826784
654655,1309311,1309310,2618621,1131.1913652420044,0.0004937264488944493
655656,1311313,1311312,2622625,1134.038523197174,0.0004864347980628736
656657,1313315,1313314,2626629,1135.550742149353,0.0004792509747630902
657658,1315317,1315316,2630633,1137.053551197052,0.0004721733814676554
658659,1317319,1317318,2634637,1138.558718919754,0.0004652004439549273
659660,1319321,1319320,2638641,1140.029333114624,0.00045833061165012623
660661,1321323,1321322,2642645,1141.633619070053,0.00045156235694321367
661662,1323325,1323324,2646649,1143.218913078308,0.00044489417473414505
662663,1325327,1325326,2650653,1144.7095112800598,0.000438324582887617
663664,1327329,1327328,2654657,1146.2268772125244,0.00043185212007301743
664665,1329331,1329330,2658661,1147.706570148468,0.0004254753481518492
665666,1331333,1331332,2662665,1149.2136871814728,0.00041919284944924584
666667,1333335,1333334,2666669,1150.6863832473755,0.00041300322709503234
667668,1335337,1335336,2670673,1152.1645390987396,0.00040690510604690644
668669,1337339,1337338,2674677,1153.6583542823792,0.0004008971309303888
669670,1339341,1339340,2678681,1155.1403529644012,0.0003949779663798836
670671,1341343,1341342,2682685,1156.6232681274414,0.0003891462973797388
671672,1343345,1343344,2686689,1158.100084066391,0.00038340082801369135
672673,1345347,1345346,2690693,1159.5596780776978,0.00037774028191961406
673674,1347349,1347348,2694697,1161.0412640571594,0.0003721634014937081
674675,1349351,1349350,2698701,1162.5260531902313,0.00036666894789050275
675676,1351353,1351352,2702705,1163.9969742298126,0.00036125570045442146
676677,1353355,1353354,2706709,1165.489140033722,0.00035592245706084213
677678,1355357,1355356,2710713,1166.9646751880646,0.0003506680330929157
678679,1357359,1357358,2714717,1168.4246530532837,0.00034549126166893984
679680,1359361,1359360,2718721,1169.9142792224884,0.0003403909929602378
680681,1361363,1361362,2722725,1171.4346911907196,0.0003353660948732795
681682,1363365,1363364,2726729,1172.9302740097046,0.00033041545123069227
682683,1365367,1365366,2730733,1174.4462399482727,0.0003255379632491895
683684,1367369,1367368,2734737,1175.917473077774,0.000320732547947955
684685,1369371,1369370,2738741,1177.3984150886536,0.0003159981381486432
685686,1371373,1371372,2742745,1178.8831129074097,0.00031133368338487344
686687,1373375,1373374,2746749,1180.1753251552582,0.0003067381481969278
687688,1375377,1375376,2750753,1181.4831261634827,0.00030221051235912455
688689,1377379,1377378,2754757,1182.7399821281433,0.0002977497713345656
689690,1379381,1379380,2758761,1184.3211450576782,0.00029335493456983386
690691,1381383,1381382,2762765,1186.0672602653503,0.0002890250275413564
691692,1383385,1383384,2766769,1187.6541812419891,0.00028475908902692026
692693,1385387,1385386,2770773,1189.273950099945,0.00028055617235622776
693694,1387389,1387388,2774777,1190.9278650283813,0.00027641534529720957
694695,1389391,1389390,2778781,1192.5045340061188,0.00027233568914653006
695696,1391393,1391392,2782785,1194.6502752304077,0.0002683162987295873
696697,1393395,1393394,2786789,1196.8003051280975,0.00026435628228682617
697698,1395397,1395396,2790793,1198.4386641979218,0.00026045476136005163
698699,1397399,1397398,2794797,1200.1201589107513,0.0002566108710198023
699700,1399401,1399400,2798801,1201.8520221710205,0.00025282375838742155
700701,1401403,1401402,2802805,1203.379240989685,0.0002490925835445523
701702,1403405,1403404,2806809,1204.8545279502869,0.000245416518851016
702703,1405407,1405406,2810813,1206.3943011760712,0.00024179474951324664
703704,1407409,1407408,2814817,1207.859764099121,0.0002382264722200489
704705,1409411,1409410,2818821,1209.394294977188,0.0002347108957110322
705706,1411413,1411412,2822825,1210.9610311985016,0.0002312472403218635
706707,1413415,1413414,2826829,1212.5359771251678,0.00022783473843901447
707708,1415417,1415416,2830833,1214.005359172821,0.00022447263347658009
708709,1417419,1417418,2834837,1215.5132751464844,0.00022116018010365224
709710,1419421,1419420,2838841,1216.9898490905762,0.0002178966437895724
710711,1421423,1421422,2842845,1218.4537200927734,0.00021468130159973953
711712,1423425,1423424,2846849,1219.9899730682373,0.00021151344037662057
712713,1425427,1425426,2850853,1221.4534380435944,0.00020839235821767943
713714,1427429,1427428,2854857,1222.9378671646118,0.00020531736345219542
714715,1429431,1429430,2858861,1224.4180312156677,0.00020228777430020273
715716,1431433,1431432,2862865,1225.9127271175385,0.00019930292000935879
716717,1433435,1433434,2866869,1227.3811662197113,0.00019636213835383387
717718,1435437,1435436,2870873,1228.8646421432495,0.0001934647783627952
718719,1437439,1437438,2874877,1230.3324520587921,0.00019061019793298328
719720,1439441,1439440,2878881,1231.8465023040771,0.00018779776416977256
720721,1441443,1441442,2882885,1233.3193731307983,0.00018502685452403966
721722,1443445,1443444,2886889,1234.8403189182281,0.0001822968548594872
722723,1445447,1445446,2890893,1236.311795949936,0.00017960716036213853
723724,1447449,1447448,2894897,1237.805507183075,0.00017695717531296395
724725,1449451,1449450,2898901,1239.2577311992645,0.00017434631274682033
725726,1451453,1451452,2902905,1240.726408958435,0.00017177399433876417
726727,1453455,1453454,2906909,1242.241277217865,0.0001692396502903648
727728,1455457,1455456,2910913,1243.695701122284,0.00016674271967076493
728729,1457459,1457458,2914917,1245.1624381542206,0.00016428264882506483
729730,1459461,1459460,2918921,1246.6203610897064,0.00016185889307962498
730731,1461463,1461462,2922925,1248.0880651474,0.00015947091651469236
731732,1463465,1463464,2926929,1249.5760011672974,0.00015711818946329004
732733,1465467,1465466,2930933,1251.0676860809326,0.00015480019135338807
733734,1467469,1467468,2934937,1252.5247139930725,0.00015251640877522732
734735,1469471,1469470,2938941,1253.9946522712708,0.00015026633627712727
735736,1471473,1471472,2942945,1255.5083701610565,0.00014804947556967818
736737,1473475,1473474,2946949,1256.9979321956635,0.00014586533586680162
737738,1475477,1475476,2950953,1258.4680042266846,0.00014371343377206358
738739,1477479,1477478,2954957,1259.9480981826782,0.00014159329271024035
739740,1479481,1479480,2958961,1261.399138212204,0.00013950444372312631
740741,1481483,1481482,2962965,1262.962158203125,0.00013744642410529195
741742,1483485,1483484,2966969,1264.4427120685577,0.00013541877819989168
742743,1485487,1485486,2970973,1265.9812381267548,0.0001334210576260375
743744,1487489,1487488,2974977,1267.4172711372375,0.00013145282025561755
744745,1489491,1489490,2978981,1268.8862390518188,0.00012951363032698282
745746,1491493,1491492,2982985,1270.3767092227936,0.0001276030586723209
746747,1493495,1493494,2986989,1271.8566052913666,0.00012572068249028234
747748,1495497,1495496,2990993,1273.326651096344,0.00012386608511860686
748749,1497499,1497498,2994997,1274.804897069931,0.00012203885660255764
749750,1499501,1499500,2999001,1276.250473022461,0.00012023859233067924
750751,1501503,1501502,3003005,1277.7197711467743,0.00011846489394429227
751752,1503505,1503504,3007009,1279.1945521831512,0.00011671736911011976
752753,1505507,1505506,3011013,1280.6656460762024,0.00011499563117922662
753754,1507509,1507508,3015017,1282.1467792987823,0.00011329929930070648
754755,1509511,1509510,3019021,1283.6323840618134,0.00011162799808062118
755756,1511513,1511512,3023025,1285.119388103485,0.00010998135780937446
756757,1513515,1513514,3027029,1286.5922842025757,0.00010835901423433825
757758,1515517,1515516,3031033,1288.0661182403564,0.00010676060878722637
758759,1517519,1517518,3035037,1289.523192167282,0.00010518578767459985
759760,1519521,1519520,3039041,1290.998630285263,0.0001036342025599879
760761,1521523,1521522,3043045,1292.4833362102509,0.0001021055101091406
761762,1523525,1523524,3047049,1294.126531124115,0.00010059937255846307
762763,1525527,1525526,3051053,1295.924741268158,9.911545669183397e-05
763764,1527529,1527528,3055057,1298.0007631778717,9.76534340679791e-05
764765,1529531,1529530,3059061,1299.8159942626953,9.621298181627935e-05
765766,1531533,1531532,3063065,1301.5041000843048,9.479378127252858e-05
766767,1533535,1533534,3067069,1303.3658742904663,9.339551854736783e-05
767768,1535537,1535536,3071073,1305.2397429943085,9.20178844125985e-05
768769,1537539,1537538,3075077,1307.1685922145844,9.066057407380868e-05
769770,1539541,1539540,3079081,1308.780030965805,8.93232878524941e-05
770771,1541543,1541542,3083085,1310.8228311538696,8.80057298218162e-05
771772,1543545,1543544,3087089,1312.683410167694,8.670760882978357e-05
772773,1545547,1545546,3091093,1314.6852040290833,8.542863770344411e-05
773774,1547549,1547548,3095097,1316.7753820419312,8.416853358994558e-05
774775,1549551,1549550,3099101,1319.0006589889526,8.292701841128292e-05
775776,1551553,1551552,3103105,1321.785082101822,8.17038172726825e-05
776777,1553555,1553554,3107109,1324.0883209705353,8.049865994053107e-05
777778,1555557,1555556,3111113,1326.1459131240845,7.931127993288101e-05
778779,1557559,1557558,3115117,1327.9328520298004,7.814141474682401e-05
779780,1559561,1559560,3119121,1330.1700451374054,7.698880608586478e-05
780781,1561563,1561562,3123125,1332.0521640777588,7.585319906411314e-05
781782,1563565,1563564,3127129,1334.400348186493,7.47343426610314e-05
782783,1565567,1565566,3131133,1336.1840062141418,7.363198949406069e-05
783784,1567569,1567568,3135137,1338.1559779644012,7.25458960459946e-05
784785,1569571,1569570,3139141,1339.7689571380615,7.147582221023185e-05
785786,1571573,1571572,3143145,1341.5361862182617,7.042153163183684e-05
786787,1573575,1573574,3147149,1343.5233480930328,6.93827914801659e-05
787788,1575577,1575576,3151153,1345.4359459877014,6.83593716530595e-05
788789,1577579,1577578,3155157,1347.1237812042236,6.735104648214474e-05
789790,1579581,1579580,3159161,1348.9574053287506,6.635759302753286e-05
790791,1581583,1581582,3163165,1350.6482701301575,6.537879175994021e-05
791792,1583585,1583584,3167169,1352.4088501930237,6.441442667437514e-05
792793,1585587,1585586,3171173,1354.1909341812134,6.346428426695638e-05
793794,1587589,1587588,3175177,1355.863750219345,6.25281548991552e-05
794795,1589591,1589590,3179181,1357.6513741016388,6.160583143355325e-05
795796,1591593,1591592,3183185,1359.4865732192993,6.069711059808469e-05
796797,1593595,1593594,3187189,1361.142441034317,5.9801791280733596e-05
797798,1595597,1595596,3191193,1363.3625841140747,5.891967566640233e-05
798799,1597599,1597598,3195197,1364.9259362220764,5.805056900953787e-05
799800,1599601,1599600,3199201,1366.4412951469421,5.719427940675814e-05
800801,1601603,1601602,3203205,1367.9900102615356,5.635061768316518e-05
801802,1603605,1603604,3207209,1369.4622631072998,5.551939727865829e-05
802803,1605607,1605606,3211213,1371.0080161094666,5.470043493005505e-05
803804,1607609,1607608,3215217,1372.5911331176758,5.389354930684931e-05
804805,1609611,1609610,3219221,1374.127594947815,5.30985627165137e-05
805806,1611613,1611612,3223225,1375.6303012371063,5.231529894444975e-05
806807,1613615,1613614,3227229,1377.1238770484924,5.154358541403781e-05
807808,1615617,1615616,3231233,1378.6791121959686,5.078325182239496e-05
808809,1617619,1617618,3235237,1380.3344750404358,5.003412979931454e-05
809810,1619621,1619620,3239241,1381.8631191253662,4.9296054157821345e-05
810811,1621623,1621622,3243245,1383.3513872623444,4.8568861984676914e-05
811812,1623625,1623624,3247249,1384.8357191085815,4.785239264037955e-05
812813,1625627,1625626,3251253,1386.3304121494293,4.7146487645477464e-05
813814,1627629,1627628,3255257,1388.056279182434,4.6450991590063495e-05
814815,1629631,1629630,3259261,1389.6160991191864,4.576575054215937e-05
815816,1631633,1631632,3263265,1391.1879510879517,4.509061318458407e-05
816817,1633635,1633634,3267269,1392.6760601997375,4.442543070126703e-05
817818,1635637,1635636,3271273,1394.1461582183838,4.37700558677534e-05
818819,1637639,1637638,3275277,1395.7135632038116,4.31243444154461e-05
819820,1639641,1639640,3279281,1397.4430561065674,4.248815343999013e-05
820821,1641643,1641642,3283285,1399.4645512104034,4.1861342651827727e-05
821822,1643645,1643644,3287289,1401.0643162727356,4.124377358039055e-05
822823,1645647,1645646,3291293,1402.6035220623016,4.063530991516018e-05
823824,1647649,1647648,3295297,1404.2919840812683,4.0035817278294417e-05
824825,1649651,1649650,3299301,1405.8808162212372,3.944516322462732e-05
825826,1651653,1651652,3303305,1407.643802165985,3.88632175827297e-05
826827,1653655,1653654,3307309,1409.4559891223907,3.82898517727881e-05
827828,1655657,1655656,3311313,1411.0166709423065,3.772493937503896e-05
828829,1657659,1657658,3315317,1412.7797529697418,3.7168355561334465e-05
829830,1659661,1659660,3319321,1414.477902173996,3.661997709514253e-05
830831,1661663,1661662,3323325,1416.138798236847,3.6079683695788844e-05
831832,1663665,1663664,3327329,1417.6176362037659,3.554735553734645e-05
832833,1665667,1665666,3331333,1419.1013071537018,3.502287529499881e-05
833834,1667669,1667668,3335337,1420.676244020462,3.45061271218583e-05
834835,1669671,1669670,3339341,1422.128454208374,3.399699721740035e-05
835836,1671673,1671672,3343345,1423.6029570102692,3.3495373145342455e-05
836837,1673675,1673674,3347349,1425.1045832633972,3.3001143833644164e-05
837838,1675677,1675676,3351353,1427.175921201706,3.2514200597688614e-05
838839,1677679,1677678,3355357,1428.7404990196228,3.2034435662353644e-05
839840,1679681,1679680,3359361,1430.24556016922,3.156174341256701e-05
840841,1681683,1681682,3363365,1431.7221250534058,3.109601948381169e-05
841842,1683685,1683684,3367369,1433.2802681922913,3.06371608758127e-05
842843,1685687,1685686,3371373,1434.84446310997,3.0185066862031817e-05
843844,1687689,1687688,3375377,1436.4043781757355,2.9739636829617666e-05
844845,1689691,1689690,3379381,1438.104483127594,2.9300773235263478e-05
845846,1691693,1691692,3383385,1439.827542066574,2.8868378876723e-05
846847,1693695,1693694,3387389,1441.7396709918976,2.844235859811306e-05
847848,1695697,1695696,3391393,1443.407114982605,2.8022618153045187e-05
848849,1697699,1697698,3395397,1444.9305431842804,2.76090647730598e-05
849850,1699701,1699700,3399401,1446.4595119953156,2.720160750868672e-05
850851,1701703,1701702,3403405,1447.9628551006317,2.6800156661010988e-05
851852,1703705,1703704,3407409,1449.5107691287994,2.6404623099551827e-05
852853,1705707,1705706,3411413,1451.065895318985,2.6014919853878382e-05
853854,1707709,1707708,3415417,1452.5575292110443,2.5630960976741335e-05
854855,1709711,1709710,3419421,1454.0501880645752,2.5252661544072907e-05
855856,1711713,1711712,3423425,1455.515715122223,2.4879938337107887e-05
856857,1713715,1713714,3427429,1457.0000083446503,2.4512709160262602e-05
857858,1715717,1715716,3431433,1458.4716160297394,2.415089272744808e-05
858859,1717719,1717718,3435437,1459.9624071121216,2.379440934419108e-05
859860,1719721,1719720,3439441,1461.4653732776642,2.3443180339199898e-05
860861,1721723,1721722,3443445,1462.945475101471,2.3097128291738045e-05
861862,1723725,1723724,3447449,1464.415817975998,2.275617691793741e-05
862863,1725727,1725726,3451453,1465.941281080246,2.2420250843424583e-05
863864,1727729,1727728,3455457,1467.4283571243286,2.2089276171755046e-05
864865,1729731,1729730,3459461,1468.9277131557465,2.176317946123163e-05
865866,1731733,1731732,3463465,1470.4211602210999,2.144188954389392e-05
866867,1733735,1733734,3467469,1471.8837912082672,2.112533456966048e-05
867868,1735737,1735736,3471473,1473.3883829116821,2.0813445416933973e-05
868869,1737739,1737738,3475477,1474.8875000476837,2.050615319149074e-05
869870,1739741,1739740,3479481,1476.41956615448,2.020338990860182e-05
870871,1741743,1741742,3483485,1477.901884317398,1.9905088947780314e-05
871872,1743745,1743744,3487489,1479.3943552970886,1.9611184598034015e-05
872873,1745747,1745746,3491493,1480.9001562595367,1.9321611603118072e-05
873874,1747749,1747748,3495497,1482.3828420639038,1.903630675315071e-05
874875,1749751,1749750,3499501,1483.8908700942993,1.8755206724563322e-05
875876,1751753,1751752,3503505,1485.3725371360779,1.8478249103281996e-05
876877,1753755,1753754,3507509,1486.8388900756836,1.8205373521595902e-05
877878,1755757,1755756,3511513,1488.3212931156158,1.7936519952854724e-05
878879,1757759,1757758,3515517,1489.8125250339508,1.767162802934763e-05
879880,1759761,1759760,3519521,1491.2867913246155,1.7410640339221573e-05
880881,1761763,1761762,3523525,1492.675504207611,1.7153498902189313e-05
881882,1763765,1763764,3527529,1493.9964752197266,1.6900147215892503e-05
882883,1765767,1765766,3531533,1495.3226659297943,1.6650529119033308e-05
883884,1767769,1767768,3535537,1496.615854024887,1.6404589814555948e-05
884885,1769771,1769770,3539541,1497.8712639808655,1.616227496015199e-05
885886,1771773,1771772,3543545,1499.1373591423035,1.5923531009320868e-05
886887,1773775,1773774,3547549,1500.4207501411438,1.5688305779804068e-05
887888,1775777,1775776,3551553,1502.086906194687,1.5456546748282562e-05
888889,1777779,1777778,3555557,1503.6469650268555,1.5228203210426727e-05
889890,1779781,1779780,3559561,1505.1670620441437,1.5003224802967452e-05
890891,1781783,1781782,3563565,1506.6773209571838,1.4781561617382977e-05
891892,1783785,1783784,3567569,1508.1809830665588,1.4563165223080432e-05
892893,1785787,1785786,3571573,1509.8570611476898,1.4347987416840624e-05
893894,1787789,1787788,3575577,1511.4946439266205,1.4135980222818034e-05
894895,1789791,1789790,3579581,1513.0153031349182,1.392709737046971e-05
895896,1791793,1791792,3583585,1514.6558442115784,1.3721292816626374e-05
896897,1793795,1793794,3587589,1516.376960992813,1.3518520745492424e-05
897898,1795797,1795796,3591593,1518.0871522426605,1.3318737160261662e-05
898899,1797799,1797798,3595597,1519.7219140529633,1.3121897382006864e-05
899900,1799801,1799800,3599601,1521.879565000534,1.2927958323416533e-05
900901,1801803,1801802,3603605,1525.0349071025848,1.273687701086601e-05
901902,1803805,1803804,3607609,1527.555426120758,1.2548611607599014e-05
902903,1805807,1805806,3611613,1530.9658181667328,1.23631203905461e-05
903904,1807809,1807808,3615617,1534.5319900512695,1.218036243244569e-05
904905,1809811,1809810,3619621,1537.246267080307,1.2000297715530905e-05
905906,1811813,1811812,3623625,1539.442698955536,1.1822886222034867e-05
906907,1813815,1813814,3627629,1541.5444490909576,1.1648088957372238e-05
907908,1815817,1815816,3631633,1543.1435840129852,1.1475867495391867e-05
908909,1817819,1817818,3635637,1545.0557811260223,1.1306183751003118e-05
909910,1819821,1819820,3639641,1547.2851729393005,1.113900032123638e-05
910911,1821823,1821822,3643645,1549.5982332229614,1.0974280485243071e-05
911912,1823825,1823824,3647649,1551.8800649642944,1.081198774954828e-05
912913,1825827,1825826,3651653,1553.8020231723785,1.0652086302798125e-05
913914,1827829,1827828,3655657,1555.7871642112732,1.0494541243133426e-05
914915,1829831,1829830,3659661,1557.5675330162048,1.0339317441321327e-05
915916,1831833,1831832,3663665,1559.4563109874725,1.018638090499735e-05
916917,1833835,1833834,3667669,1561.0996589660645,1.0035697755483852e-05
917918,1835837,1835836,3671673,1562.6293921470642,9.887234909911058e-06
918919,1837839,1837838,3675677,1564.1890811920166,9.740959853843378e-06
919920,1839841,1839840,3679681,1566.07808303833,9.596839959158388e-06
920921,1841843,1841842,3683685,1568.123250246048,9.454843507228361e-06
921922,1843845,1843844,3687689,1569.9234881401062,9.314939234172925e-06
922923,1845847,1845846,3691693,1572.045599937439,9.177096558232734e-06
923924,1847849,1847848,3695697,1573.5674800872803,9.041285011335276e-06
924925,1849851,1849850,3699701,1575.9708452224731,8.907474352781719e-06
925926,1851853,1851852,3703705,1578.1308600902557,8.77563525136793e-06
926927,1853855,1853854,3707709,1580.2869811058044,8.64573871695029e-06
927928,1855857,1855856,3711713,1582.503086090088,8.51775632781937e-06
928929,1857859,1857858,3715717,1584.4652032852173,8.391659434892063e-06
929930,1859861,1859860,3719721,1586.3545231819153,8.26742052595364e-06
930931,1861863,1861862,3723725,1588.3904871940613,8.145011975102534e-06
931932,1863865,1863864,3727729,1590.2164311408997,8.02440717961872e-06
932933,1865867,1865866,3731733,1592.08789396286,7.905579195721657e-06
933934,1867869,1867868,3735737,1593.873463153839,7.788502102812345e-06
934935,1869871,1869870,3739741,1595.5922832489014,7.67315009397862e-06
935936,1871873,1871872,3743745,1597.3785772323608,7.559497589681996e-06
936937,1873875,1873874,3747749,1599.0709221363068,7.447519465131336e-06
937938,1875877,1875876,3751753,1600.862879037857,7.337191163969692e-06
938939,1877879,1877878,3755757,1602.6017379760742,7.228488470900629e-06
939940,1879881,1879880,3759761,1604.2669780254364,7.121387284314551e-06
940941,1881883,1881882,3763765,1605.966586112976,7.015864071036049e-06
941942,1883885,1883884,3767769,1607.9571330547333,6.9118955252633896e-06
942943,1885887,1885886,3771773,1610.1803262233734,6.809458909629029e-06
943944,1887889,1887888,3775777,1612.228375196457,6.708531486765423e-06
944945,1889891,1889890,3779781,1614.2180371284485,6.609090860365541e-06
945946,1891893,1891892,3783785,1616.1885521411896,6.511115429930214e-06
946947,1893895,1893894,3787789,1618.4973471164703,6.414583594960277e-06
947948,1895897,1895896,3791793,1620.4924139976501,6.319473754956562e-06
948949,1897899,1897898,3795797,1622.5704741477966,6.225765218914603e-06
949950,1899901,1899900,3799801,1624.5796620845795,6.133437182143098e-06
950951,1901903,1901902,3803805,1626.5768933296204,6.042469749445445e-06
951952,1903905,1903904,3807809,1628.5990390777588,5.952842229817179e-06
952953,1905907,1905906,3811813,1630.9603073596954,5.8645352964958875e-06
953954,1907909,1907908,3815817,1633.098001241684,5.777529167971807e-06
954955,1909911,1909910,3819821,1634.7033472061157,5.691804972229875e-06
955956,1911913,1911912,3823825,1636.2653131484985,5.607343723568192e-06
956957,1913915,1913914,3827829,1637.8252251148224,5.524126777345373e-06
957958,1915917,1915916,3831833,1639.4252090454102,5.442135829980543e-06
958959,1917919,1917918,3835837,1640.962368965149,5.361352918953344e-06
959960,1919921,1919920,3839841,1642.4751360416412,5.281759854369739e-06
960961,1921923,1921922,3843845,1643.9751522541046,5.203339696890907e-06
961962,1923925,1923924,3847849,1645.4951710700989,5.126074825057003e-06
962963,1925927,1925926,3851853,1647.0081470012665,5.04994807215553e-06
963964,1927929,1927928,3855857,1648.6602230072021,4.9749429535950185e-06
964965,1929931,1929930,3859861,1651.172401189804,4.901042530036648e-06
965966,1931933,1931932,3863865,1652.6815810203552,4.82823122638365e-06
966967,1933935,1933934,3867869,1654.4367191791534,4.756492330670881e-06
967968,1935937,1935936,3871873,1655.993567943573,4.685810267801571e-06
968969,1937939,1937938,3875877,1657.6239531040192,4.616169576365792e-06
969970,1939941,1939940,3879881,1659.2502851486206,4.547554794953612e-06
970971,1941943,1941942,3883885,1660.780151128769,4.479950916902453e-06
971972,1943945,1943944,3887889,1662.2691791057587,4.413342821862898e-06
972973,1945947,1945946,3891893,1663.751177072525,4.347716185293393e-06
973974,1947949,1947948,3895897,1665.5003461837769,4.2830562279050355e-06
974975,1949951,1949950,3899901,1667.4020512104034,4.2193487388431095e-06
975976,1951953,1951952,3903905,1669.2245502471924,4.156579962000251e-06
976977,1953955,1953954,3907909,1670.7720410823822,4.094735572834907e-06
977978,1955957,1955956,3911913,1672.8186581134796,4.033802611047577e-06
978979,1957959,1957958,3915917,1674.5404651165009,3.973767093157221e-06
979980,1959961,1959960,3919921,1676.154095172882,3.914615831490664e-06
980981,1961963,1961962,3923925,1677.67529129982,3.856336093122081e-06
981982,1963965,1963964,3927929,1679.5216071605682,3.798914917751972e-06
982983,1965967,1965966,3931933,1681.209328174591,3.7423396861413494e-06
983984,1967969,1967968,3935937,1683.5186879634857,3.686597892738064e-06
984985,1969971,1969970,3939941,1685.0886399745941,3.631677031989966e-06
985986,1971973,1971972,3943945,1686.544186115265,3.5775653941527708e-06
986987,1973975,1973974,3947949,1688.0586659908295,3.5242508147348417e-06
987988,1975977,1975976,3951953,1689.5228962898254,3.471721811365569e-06
988989,1977979,1977978,3955957,1691.1935470104218,3.419966446926992e-06
989990,1979981,1979980,3959961,1692.9723241329193,3.368973466422176e-06
990991,1981983,1981982,3963965,1694.5143291950226,3.3187317285410245e-06
991992,1983985,1983984,3967969,1696.0308611392975,3.2692300919734407e-06
992993,1985987,1985986,3971973,1697.4996333122253,3.2204576427830034e-06
993994,1987989,1987988,3975977,1699.1104292869568,3.1724036944069667e-06
994995,1989991,1989990,3979981,1700.560563325882,3.125057446595747e-06
995996,1991993,1991992,3983985,1702.0206820964813,3.078408894907625e-06
996997,1993995,1993994,3987989,1703.5521399974823,3.0324473527798546e-06
997998,1995997,1995996,3991993,1705.0981981754303,2.987162929457554e-06
998999,1997999,1997998,3995997,1707.171144247055,2.942545620499004e-06
1000000,2000001,2000000,4000001,1708.7047271728516,2.898585535149323e-06


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.013862848281860352,2180.042156630883
1001,2003,2002,4005,2.1144208908081055,59.50785960800022
2002,4005,4004,8009,3.806501865386963,53.069953055727865
3003,6007,6006,12013,6.497259855270386,50.23287214458628
4004,8009,8008,16017,8.870810747146606,48.011470954668084
5005,10011,10010,20021,10.446680068969727,46.034239271139995
6006,12013,12012,24025,12.066550970077515,44.22397270747979
7007,14015,14014,28029,13.955816984176636,42.551356224505525
8008,16017,16016,32033,15.77367091178894,40.99882237549582
9009,18019,18018,36037,17.638158798217773,39.55358199049692
10010,20021,20020,40041,20.43228006362915,38.205379619941596
11011,22023,22022,44045,22.122371673583984,36.94544630893597
12012,24025,24024,48049,24.016366720199585,35.76595715561052
13013,26027,26026,52053,25.488724946975708,34.65975853578084
14014,28029,28028,56057,27.060860872268677,33.620244488709886
15015,30031,30030,60061,28.558502912521362,32.64131021783305
16016,32033,32032,64065,30.07087469100952,31.717339273637435
17017,34035,34034,68069,31.671834707260132,30.843199816600873
18018,36037,36036,72073,33.103928089141846,30.01423768535301
19019,38039,38038,76077,34.613853931427,29.226261611111795
20020,40041,40040,80081,36.03676700592041,28.475520193335797
21021,42043,42042,84085,37.560017824172974,27.758672299758928
22022,44045,44044,88089,38.97228288650513,27.072753240235443
23023,46047,46046,92093,40.39877200126648,26.41513900422433
24024,48049,48048,96097,41.83213782310486,25.78351044992087
25025,50051,50050,100101,43.2357497215271,25.17581882966465
26026,52053,52052,104105,44.79340887069702,24.59025355898507
27027,54055,54054,108109,46.3217978477478,24.02521274135711
28028,56057,56056,112113,47.88962388038635,23.47927666178134
29029,58059,58058,116117,49.3883159160614,22.951184252855683
30030,60061,60060,120121,51.22951889038086,22.439812401351446
31031,62063,62062,124125,52.718047857284546,21.94415788401261
32032,64065,64064,128129,54.11799693107605,21.46332168241679
33033,66067,66066,132133,55.730883836746216,20.99649541523695
34034,68069,68068,136137,57.19547700881958,20.54294963220218
35035,70071,70070,140141,58.66676092147827,20.102023730283918
36036,72073,72072,144145,60.72150492668152,19.673117274136075
37037,74075,74074,148149,62.98289084434509,19.255682526329565
38038,76077,76076,152153,64.49984574317932,18.84921801638393
39039,78079,78078,156157,65.93615484237671,18.453262999794106
40040,80081,80080,160161,67.36772608757019,18.06772520472282
41041,82083,82082,164165,68.78239679336548,17.692301676856687
42042,84085,84084,168169,70.73880887031555,17.326216665661605
43043,86087,86086,172173,72.55309677124023,16.969117112451613
44044,88089,88088,176177,74.83304691314697,16.620678670884445
45045,90091,90090,180181,76.55391097068787,16.280599832997723
46046,92093,92092,184185,78.25416088104248,15.948598824924602
47047,94095,94094,188189,80.33215093612671,15.624411281018638
48048,96097,96096,192193,82.36047887802124,15.307788331851498
49049,98099,98098,196197,83.88169479370117,14.99849499324273
50050,100101,100100,200201,85.4631290435791,14.696308793875687
51051,102103,102102,204205,86.95214796066284,14.401018596686981
52052,104105,104104,208209,88.83047485351562,14.112423579519941
53053,106107,106106,212213,90.40578293800354,13.830332347910826
54054,108109,108108,216217,92.17846179008484,13.5545621584223
55055,110111,110110,220221,94.6769118309021,13.284938235176355
56056,112113,112112,224225,96.60566091537476,13.021293165528618
57057,114115,114114,228229,98.09316182136536,12.763466363368366
58058,116117,116116,232233,99.94396996498108,12.511303590553098
59059,118119,118118,236237,101.54084992408752,12.264656528564501
60060,120121,120120,240241,103.19280195236206,12.023382393771726
61061,122123,122122,244245,104.75357389450073,11.787343590700743
62062,124125,124124,248249,106.28275489807129,11.556407398568922
63063,126127,126126,252253,107.82523488998413,11.330445687023143
64064,128129,128128,256257,109.50667476654053,11.109334657604222
65065,130131,130130,260261,111.03550577163696,10.892954607934712
66066,132133,132132,264265,112.57132387161255,10.681189716030985
67067,134135,134134,268269,114.22957682609558,10.473927842483363
68068,136137,136136,272273,115.78842806816101,10.27106034853523
69069,138139,138138,276277,117.35763883590698,10.072481928344473
70070,140141,140140,280281,118.9733099937439,9.878090453921118
71071,142143,142142,284285,120.48506903648376,9.687786831418066
72072,144145,144144,288289,121.90334892272949,9.501474867617162
73073,146147,146146,292293,123.27881193161011,9.319061145587284
74074,148149,148148,296297,124.56561470031738,9.140454908614515
75075,150151,150150,300301,125.854012966156,8.965567951612229
76076,152153,152152,304305,127.1259138584137,8.79431451931191
77077,154155,154154,308309,128.44260501861572,8.626611210618535
78078,156157,156156,312313,129.7790448665619,8.462376888585254
79079,158159,158158,316317,131.07860589027405,8.301532595530489
80080,160161,160160,320321,132.6848497390747,8.144001472874265
81081,162163,162162,324325,134.39307069778442,7.989708685318078
82082,164165,164164,328329,136.06289982795715,7.838581349042329
83083,166167,166166,332333,137.8710117340088,7.69054846362792
84084,168169,168168,336337,139.69441390037537,7.545540847441998
85085,170171,170170,340341,141.51062488555908,7.403491076259002
86086,172173,172172,344345,143.27926182746887,7.264333424909296
87087,174175,174174,348349,145.0389039516449,7.128003811768053
88088,176177,176176,352353,146.74304580688477,6.994439745915088
89089,178179,178178,356357,148.44142985343933,6.863580276808648
90090,180181,180180,360361,150.46890497207642,6.73536594633174
91091,182183,182182,364365,152.07852697372437,6.609738743068647
92092,184185,184184,368369,153.7125220298767,6.486642058692496
93093,186187,186186,372373,155.28264808654785,6.366020646336096
94094,188189,188188,376377,156.89172077178955,6.247820580833263
95095,190191,190190,380381,158.63695573806763,6.131989220719106
96096,192193,192192,384385,160.30103278160095,6.018475171882187
97097,194195,194194,388389,161.92124104499817,5.907228252769983
98098,196197,196196,392393,163.50998401641846,5.798199461044533
99099,198199,198198,396397,165.05253291130066,5.691340941603016
100100,200201,200200,400401,166.59953999519348,5.58660595586889
101101,202203,202202,404405,168.1648907661438,5.483948852274807
102102,204205,204204,408409,169.76540803909302,5.383325037858299
103103,206207,206206,412413,171.46410584449768,5.284690950897925
104104,208209,208208,416417,173.1182918548584,5.188004034522692
105105,210211,210210,420421,174.75783395767212,5.093222711230851
106106,212213,212212,424425,176.43683981895447,5.0003063582644245
107107,214215,214214,428429,177.95281982421875,4.909215283783851
108108,216217,216216,432433,179.51908087730408,4.819910703796268
109109,218219,218218,436437,181.06799793243408,4.732354719794671
110110,220221,220220,440441,182.84424686431885,4.646510297065902
111111,222223,222222,444445,184.9273316860199,4.562341243635501
112112,224225,224224,448449,186.68183279037476,4.479812189812833
113113,226227,226226,452453,188.54801297187805,4.398888568310213
114114,228229,228228,456457,190.3177080154419,4.319536594907959
115115,230231,230230,460461,191.78791880607605,4.241723249640472
116116,232233,232232,464465,193.25264382362366,4.16541625848356
117117,234235,234234,468469,194.681786775589,4.090584075518791
118118,236237,236236,472473,196.159117937088,4.017195865562712
119119,238239,238238,476477,197.60028290748596,3.945221487236495
120120,240241,240240,480481,199.03476667404175,3.874631476467698
121121,242243,242242,484485,200.4725697040558,3.805397030403583
122122,244245,244244,488489,201.96619391441345,3.7374899917276707
123123,246247,246246,492493,203.45116090774536,3.67088283336318
124124,248249,248248,496497,204.9722580909729,3.6055486435553803
125125,250251,250250,500501,206.58128476142883,3.541461111318199
126126,252253,252252,504505,208.25682997703552,3.4785945122380326
127127,254255,254254,508509,209.84695887565613,3.4169236946225965
128128,256257,256256,512513,211.3993489742279,3.3564240659883353
129129,258259,258258,516517,213.18768310546875,3.297071579873432
130130,260261,260260,520521,214.90505480766296,3.2388427229732315
131131,262263,262262,524525,216.42531204223633,3.181714502584896
132132,264265,264264,528529,218.01518201828003,3.125664434358441
133133,266267,266266,532533,219.61183190345764,3.0706705303413173
134134,268269,268268,536537,221.2239270210266,3.0167112873145925
135135,270271,270270,540541,222.74138188362122,2.963765675409718
136136,272273,272272,544545,224.32001996040344,2.911813127001892
137137,274275,274274,548549,226.0165376663208,2.8608335258705893
138138,276277,276276,552553,227.74670696258545,2.8108071966245234
139139,278279,278278,556557,229.22333598136902,2.761714894380134
140140,280281,280280,560561,230.7668800354004,2.713537794693366
141141,282283,282282,564565,232.52838492393494,2.6662574837314423
142142,284285,284284,568569,234.1241888999939,2.619855948687132
143143,286287,286286,572573,235.74911093711853,2.5743155684215253
144144,288289,288288,576577,237.50642466545105,2.5296191043375984
145145,290291,290290,580581,239.28449392318726,2.485749691472506
146146,292293,292292,584585,240.93807005882263,2.442690829806793
147147,294295,294294,588589,242.71904468536377,2.4004263757867648
148148,296297,296296,592593,244.5451009273529,2.3589405340496796
149149,298299,298298,596597,246.29083895683289,2.3182178493519814
150150,300301,300300,600601,247.73667979240417,2.278243198693872
151151,302303,302302,604605,249.25366282463074,2.2390017836347624
152152,304305,304304,608609,251.035484790802,2.2004791227944906
153153,306307,306306,612613,252.57309007644653,2.162661044539391
154154,308309,308308,616617,254.1163878440857,2.1255336798438975
155155,310311,310310,620621,255.50708985328674,2.0890834553263176
156156,312313,312312,624625,256.94729685783386,2.053297086455359
157157,314315,314314,628629,258.28710889816284,2.0181615709182097
158158,316317,316316,632633,259.6331169605255,1.9836641821536887
159159,318319,318318,636637,260.9882388114929,1.9497924630398984
160160,320321,320320,640641,262.32428073883057,1.9165342197352402
161161,322323,322322,644645,263.88084077835083,1.8838775156701786
162162,324325,324324,648649,265.4737777709961,1.8518106656836153
163163,326327,326326,652653,266.9676887989044,1.820322230300917
164164,328329,328328,656657,268.9258608818054,1.7894010101522326
165165,330331,330330,660661,270.59731793403625,1.7590360405238243
166166,332333,332332,664665,272.17492389678955,1.7292165860430941
167167,334335,334334,668669,273.7603099346161,1.6999321354899166
168168,336337,336336,672673,275.39829182624817,1.6711723967355283
169169,338339,338338,676677,277.32773876190186,1.6429272918018114
170170,340341,340340,680681,279.258798122406,1.615186952040517
171171,342343,342342,684685,280.96760177612305,1.5879417134279947
172172,344345,344344,688689,283.4140169620514,1.5611821119737215
173173,346347,346346,692693,285.1190218925476,1.5348988792381988
174174,348349,348348,696697,286.89527702331543,1.509082937959647
175175,350351,350350,700701,288.55931782722473,1.4837253977859746
176176,352353,352352,704705,290.2405219078064,1.4588175511053123
177177,354355,354354,708709,291.92757773399353,1.4343508689813689
178178,356357,356356,712713,293.4851429462433,1.4103169971824627
179179,358359,358358,716717,295.1461989879608,1.3867077523075295
180180,360361,360360,720721,296.72603487968445,1.3635151180009188
181181,362363,362362,724725,298.3772737979889,1.340731241262688
182182,364365,364364,728729,299.9497368335724,1.318348428841091
183183,366367,366366,732733,301.76080679893494,1.2963591437148807
184184,368369,368368,736737,303.61338806152344,1.2747560016571242
185185,370371,370370,740741,305.10129404067993,1.2535317678797355
186186,372373,372372,744745,306.5703959465027,1.2326793537594085
187187,374375,374374,748749,308.00961089134216,1.2121918136394925
188188,376377,376376,752753,309.4510688781738,1.1920623417067873
189189,378379,378378,756757,310.9323778152466,1.1722842689435993
190190,380381,380380,760761,312.38937187194824,1.152851060149942
191191,382383,382382,764765,313.8443830013275,1.1337563110359952
192192,384385,384384,768769,315.3201138973236,1.1149937453830034
193193,386387,386386,772773,316.8454267978668,1.096557212270909
194194,388389,388388,776777,318.26972484588623,1.078440683369763
195195,390391,390390,780781,319.7279508113861,1.0606382502953693
196196,392393,392392,784785,321.17313289642334,1.04314412202541
197197,394395,394394,788789,322.74239206314087,1.02595262237719
198198,396397,396396,792793,324.24584794044495,1.0090581875423368
199199,398399,398398,796797,325.89395689964294,0.9924553636801647
200200,400401,400400,800801,327.6289620399475,0.9761388045651529
201201,402403,402402,804805,329.2377369403839,0.9601032692900162
202202,404405,404404,808809,330.9758358001709,0.9443436200218684
203203,406407,406406,812813,332.6294677257538,0.9288548198084072
204204,408409,408408,816817,334.14356780052185,0.9136319304367362
205205,410411,410410,820821,335.64502787590027,0.8986701103399355
206206,412413,412412,824825,337.1516718864441,0.883964612552063
207207,414415,414414,828829,338.7228238582611,0.8695107827094262
208208,416417,416416,832833,340.16077995300293,0.8553040570986923
209209,418419,418418,836837,341.6165277957916,0.8413399607485417
210210,420421,420420,840841,343.06130290031433,0.8276141055644075
211211,422423,422422,844845,344.46720790863037,0.8141221885068717
212212,424425,424424,848849,345.89508080482483,0.800859989810192
213213,426427,426426,852853,347.3481788635254,0.7878233712420979
214214,428429,428428,856857,348.84115505218506,0.775008274402694
215215,430431,430430,860861,350.2943048477173,0.76241071906054
216216,432433,432432,864865,351.74511981010437,0.7500268015282927
217217,434435,434434,868869,353.1664879322052,0.7378526930735916
218218,436437,436436,872873,354.64158272743225,0.7258846383653008
219219,438439,438438,876877,356.10124492645264,0.714118953956131
220220,440441,440440,880881,357.5421268939972,0.702552026797207
221221,442443,442442,884885,358.9781439304352,0.6911803127879921
222222,444445,444444,888889,360.4863998889923,0.680000335355885
223223,446447,446446,892893,361.9301817417145,0.6690086840701497
224224,448449,448448,896897,363.46474599838257,0.6582020132855178
225225,450451,450450,900901,365.0041389465332,0.6475770408145536
226226,452453,452452,904905,366.50223207473755,0.6371305466320791
227227,454455,454454,908909,368.01187777519226,0.6268593716055193
228228,456457,456456,912913,369.58196783065796,0.616760416255488
229229,458459,458458,916917,371.03687286376953,0.6068306395427499
230230,460461,460460,920921,372.4777977466583,0.5970670576806469
231231,462463,462462,924925,373.93252301216125,0.5874667429762894
232232,464465,464464,928929,375.4169428348541,0.5780268226947101
233233,466467,466466,932933,376.94908905029297,0.568744477948826
234234,468469,468468,936937,378.4169490337372,0.5596169426141842
235235,470471,470470,940941,380.089567899704,0.5506415022658757
236236,472473,472472,944945,381.69663095474243,0.5418154931398931
237237,474475,474474,948949,383.14546298980713,0.533136301116997
238238,476477,476476,952953,384.5869507789612,0.524601360727388
239239,478479,478478,956957,386.0482397079468,0.5162081541783436
240240,480481,480480,960961,387.4985408782959,0.5079542104023176
241241,482483,482482,964965,388.9465899467468,0.4998371041252767
242242,484485,484484,968969,390.41764879226685,0.4918544549549324
243243,486487,486486,972973,391.93841791152954,0.48400392649000423
244244,488489,488488,976977,393.4370517730713,0.4762832254469913
245245,490491,490490,980981,395.2219429016113,0.4686901008062705
246246,492493,492492,984985,396.97860407829285,0.46122234297547493
247247,494495,494494,988989,398.59185576438904,0.453877782973791
248248,496497,496496,992993,400.190043926239,0.446654291629784
249249,498499,498498,996997,401.8790919780731,0.43954977879798207
250250,500501,500500,1001001,403.3226737976074,0.43256219259376394
251251,502503,502502,1005005,404.7409658432007,0.4256895186404108
252252,504505,504504,1009009,406.19427394866943,0.4189297793367359
253253,506507,506506,1013013,407.6685209274292,0.41228103313619613
254254,508509,508508,1017017,409.13446283340454,0.40574137384419373
255255,510511,510510,1021021,410.5524799823761,0.39930892992822464
256256,512513,512512,1025025,412.00243306159973,0.3929818638436018
257257,514515,514514,1029029,413.5419189929962,0.3867583713725935
258258,516517,516516,1033033,415.0876479148865,0.3806366809780002
259259,518519,518518,1037037,416.68630290031433,0.37461505317037336
260260,520521,520520,1041041,418.3098340034485,0.3686917798868308
261261,522523,522522,1045045,419.83580899238586,0.362865183885674
262262,524525,524524,1049049,421.3105237483978,0.35713361815089684
263263,526527,526526,1053053,422.73610281944275,0.3514954653098812
264264,528529,528528,1057057,424.18474793434143,0.34594913706519037
265265,530531,530530,1061061,425.6454520225525,0.3404930736339793
266266,532533,532532,1065065,427.13373279571533,0.3351257432033208
267267,534535,534534,1069069,428.59644174575806,0.3298456413938311
268268,536537,536536,1073073,430.09413981437683,0.3246512907352326
269269,538539,538538,1077077,431.5842549800873,0.31954124015373964
270270,540541,540540,1081081,433.02210688591003,0.31451406446808505
271271,542543,542542,1085085,434.5503017902374,0.3095683638969149
272272,544545,544544,1089089,436.0314438343048,0.3047027635767563
273273,546547,546546,1093093,437.57390999794006,0.29991591308839816
274274,548549,548548,1097097,439.0514888763428,0.29520648599498145
275275,550551,550550,1101101,440.50590109825134,0.29057317938679716
276276,552553,552552,1105105,441.9276957511902,0.28601471343768026
277277,554555,554554,1109109,443.3998279571533,0.28152983096958906
278278,556557,556556,1113113,444.8656487464905,0.2771172970257112
279279,558559,558558,1117117,446.322705745697,0.2727758984525508
280280,560561,560560,1121121,447.8077178001404,0.26850444349031477
281281,562563,562562,1125125,449.25231099128723,0.2643017613710299
282282,564565,564564,1129129,450.69699573516846,0.2601667019270053
283283,566567,566566,1133133,452.145201921463,0.25609813520327407
284284,568569,568568,1137137,453.61426997184753,0.2520949510819719
285285,570571,570570,1141141,455.05595088005066,0.2481560589108085
286286,572573,572572,1145145,456.4677209854126,0.24428038714142986
287287,574575,574574,1149149,457.94344186782837,0.24046688297335095
288288,576577,576576,1153153,459.41764783859253,0.23671451200618776
289289,578579,578578,1157157,460.93534207344055,0.23302225789780096
290290,580581,580580,1161161,462.37557077407837,0.22938912203017026
291291,582583,582582,1165165,463.8108289241791,0.22581412318106686
292292,584585,584584,1169169,465.23941588401794,0.2222962972030018
293293,586587,586586,1173173,466.6848089694977,0.21883469670763134
294294,588589,588588,1177177,468.16278195381165,0.21542839075743814
295295,590591,590590,1181181,470.2547698020935,0.2120764645625286
296296,592593,592592,1185185,472.47871685028076,0.20877801918402383
297297,594595,594594,1189189,474.1548008918762,0.20553217124302137
298298,596597,596596,1193193,475.88162779808044,0.20233805263546856
299299,598599,598598,1197197,477.69382977485657,0.1991948102521519
300300,600601,600600,1201201,479.26684284210205,0.19610160570516655
301301,602603,602602,1205205,480.7535889148712,0.19305761505813734
302302,604605,604604,1209209,482.2598829269409,0.19006202856394339
303303,606607,606606,1213213,483.7219789028168,0.1871140504044888
304304,608609,608608,1217217,485.19603991508484,0.1842128984392275
305305,610611,610610,1221221,486.6816029548645,0.18135780395505208
306306,612613,612612,1225225,488.1754937171936,0.17854801142345877
307307,614615,614614,1229229,489.7905237674713,0.17578277826157773
308308,616617,616616,1233233,491.3449308872223,0.17306137459763704
309309,618619,618618,1237237,493.0115840435028,0.1703830830407469
310310,620621,620620,1241241,494.6836779117584,0.16774719845705022
311311,622623,622622,1245245,496.2642538547516,0.165153027746328
312312,624625,624624,1249249,497.741436958313,0.16259988962713123
313313,626627,626626,1253253,499.2059369087219,0.16008711442384538
314314,628629,628628,1257257,500.6600968837738,0.1576140438570519
315315,630631,630630,1261261,502.11505579948425,0.1551800308403699
316316,632633,632632,1265265,503.60949993133545,0.15278443927900298
317317,634635,634634,1269269,505.07317090034485,0.15042664387306104
318318,636637,636636,1273273,506.5312440395355,0.14810602992429267
319319,638639,638638,1277277,508.03394389152527,0.14582199314793343
320320,640641,640640,1281281,509.52919602394104,0.14357393948489516
321321,642643,642642,1285285,511.00053882598877,0.14136128492134503
322322,644645,644644,1289289,512.5424177646637,0.13918345530839815
323323,646647,646646,1293293,513.9914228916168,0.13703988618829044
324324,648649,648648,1297297,515.4520750045776,0.1349300226208925
325325,650651,650650,1301301,516.9132189750671,0.1328533190157941
326326,652653,652652,1305305,518.3990199565887,0.1308092389659805
327327,654655,654654,1309309,519.8533089160919,0.12879725508560114
328328,656657,656656,1313313,521.3227188587189,0.12681684885069444
329329,658659,658658,1317317,522.8085277080536,0.12486751044252742
330330,660661,660660,1321321,524.2952938079834,0.12294873859354993
331331,662663,662662,1325325,525.7818238735199,0.12106004043744178
332332,664665,664664,1329329,527.2843339443207,0.11920093136109244
333333,666667,666666,1333333,528.7735307216644,0.11737093485919559
334334,668669,668668,1337337,530.2075479030609,0.11556958239191317
335335,670671,670670,1341341,531.6931538581848,0.11379641324549539
336336,672673,672672,1345345,533.1990888118744,0.11205097439460587
337337,674675,674674,1349349,534.6645770072937,0.11033282036839864
338338,676677,676676,1353353,536.1470749378204,0.10864151311773185
339339,678679,678678,1357357,537.6130278110504,0.10697662188601953
340340,680681,680680,1361361,539.0774779319763,0.10533772308178868
341341,682683,682682,1365365,540.6029939651489,0.10372440015339635
342342,684685,684684,1369369,542.100823879242,0.10213624346783945
343343,686687,686686,1373373,543.5675110816956,0.10057285018797302
344344,688689,688688,1377377,545.0319449901581,0.09903382415723172
345345,690691,690690,1381381,546.5108940601349,0.09751877578150925
346346,692693,692692,1385385,548.0106148719788,0.09602732191603991
347347,694695,694694,1389389,549.5390157699585,0.09455908575455396
348348,696697,696696,1393393,550.9920530319214,0.09311369671809189
349349,698699,698698,1397397,552.4517188072205,0.09169079034825245
350350,700701,700700,1401401,554.1354448795319,0.09029000820146393
351351,702703,702702,1405405,555.7805287837982,0.0889109977449607
352352,704705,704704,1409409,557.4148168563843,0.08755341225491975
353353,706707,706706,1413413,559.1161720752716,0.08621691071653004
354354,708709,708708,1417417,560.7918589115143,0.084901157725767
355355,710711,710710,1421421,562.3000960350037,0.08360582339287248
356356,712713,712712,1425425,563.7890758514404,0.0823305832478809
357357,714715,714714,1429429,565.3675248622894,0.08107511814773716
358358,716717,716716,1433433,566.8146297931671,0.07983911418443768
359359,718719,718718,1437437,568.3247747421265,0.0786222625957862
360360,720721,720720,1441441,569.819121837616,0.07742425967774125
361361,722723,722722,1445445,571.2688598632812,0.0762448066975594
362362,724725,724724,1449449,572.891371011734,0.07508360980887119
363363,726727,726726,1453453,574.425656080246,0.0739403799681213
364364,728729,728728,1457457,575.980771780014,0.0728148328540783
365365,730731,730730,1461461,577.4601888656616,0.07170668878552533
366366,732733,732732,1465465,578.9620578289032,0.07061567264418045
367367,734735,734734,1469469,580.417074918747,0.06954151379511586
368368,736737,736736,1473473,581.9401950836182,0.06848394601297514
369369,738739,738738,1477477,583.5206298828125,0.06744270740512093
370370,740741,740740,1481481,585.0879848003387,0.06641754033978486
371371,742743,742742,1485485,586.5905058383942,0.06540819137273957
372372,744745,744744,1489489,588.0915768146515,0.06441441117715385
373373,746747,746746,1493493,589.5670309066772,0.06343595447424377
374374,748749,748748,1497497,591.0401318073273,0.06247257996380995
375375,750751,750750,1501501,592.4848399162292,0.061524050258185525
376376,752753,752752,1505505,593.9677350521088,0.06059013181584305
377377,754755,754754,1509509,595.4768860340118,0.05967059487670667
378378,756757,756756,1513513,596.9986937046051,0.05876521339860119
379379,758759,758758,1517517,598.4643619060516,0.05787376499495167
380380,760761,760760,1521521,599.9389278888702,0.05699603087191463
381381,762763,762762,1525525,601.4980900287628,0.05613179577051142
382382,764765,764764,1529529,602.9750277996063,0.05528084790591947
383383,766767,766766,1533533,604.4621288776398,0.054442978908355144
384384,768769,768768,1537537,605.921984910965,0.05361798376816296
385385,770771,770770,1541541,607.3771789073944,0.05280566077817639
386386,772773,772772,1545545,608.8913488388062,0.052005811478238684
387387,774775,774774,1549549,610.3508427143097,0.051218240601883736
388388,776777,776776,1553553,611.8300940990448,0.050442756022675894
389389,778779,778778,1557557,613.338131904602,0.049679168701800336
390390,780781,780780,1561561,614.8007071018219,0.048927292636562925
391391,782783,782782,1565565,617.0965230464935,0.048186944810026944
392392,784785,784784,1569569,619.1884858608246,0.047457945141445634
393393,786787,786786,1573573,621.2590398788452,0.04674011643680842
394394,788789,788788,1577577,623.1846327781677,0.04603328434188825
395395,790791,790790,1581581,624.8901040554047,0.045337277294493106
396396,792793,792792,1585585,626.4074969291687,0.04465192647796812
397397,794795,794794,1589589,627.8726327419281,0.04397706577651661
398398,796797,796796,1593593,629.3652107715607,0.04331253172972538
399399,798799,798798,1597597,630.8402438163757,0.04265816348902263
400400,800801,800800,1601601,632.3015208244324,0.04201380277447697
401401,802803,802802,1605605,633.8002827167511,0.04137929383171013
402402,804805,804804,1609609,635.2883048057556,0.04075448339176546
403403,806807,806806,1613613,636.8738067150116,0.040139220628475414
404404,808809,808808,1617617,638.4286887645721,0.03953335711889849
405405,810811,810810,1621621,640.0165717601776,0.038936746803983624
406406,812813,812812,1625625,641.4329447746277,0.03834924594957556
407407,814815,814814,1629629,642.8371729850769,0.037770713107079246
408408,816817,816816,1633633,644.3126137256622,0.03720100907798951
409409,818819,818818,1637637,645.7816927433014,0.03663999687512387
410410,820821,820820,1641641,647.2602250576019,0.036087541687152225
411411,822823,822822,1645645,648.7618386745453,0.03554351084278551
412412,824825,824824,1649649,650.2440869808197,0.03500777377576014
413413,826827,826826,1653653,651.7075629234314,0.034480201990049864
414414,828829,828828,1657657,653.1610207557678,0.03396066902689654
415415,830831,830830,1661661,654.6450927257538,0.03344905042990831
416416,832833,832832,1665665,656.1270608901978,0.03294522371413677
417417,834835,834834,1669669,657.5983588695526,0.03244906833231198
418418,836837,836836,1673673,659.0698528289795,0.031960465644601754
419419,838839,838838,1677677,660.5707807540894,0.03147929888655199
420420,840841,840840,1681681,662.0455558300018,0.03100545313884595
421421,842843,842842,1685685,663.5074319839478,0.03053881529717728
422422,844845,844844,1689689,664.9679307937622,0.030079274043032456
423423,846847,846846,1693693,666.4468958377838,0.029626719814245916
424424,848849,848848,1697697,667.9403839111328,0.029181044776237286
425425,850851,850850,1701701,669.4628400802612,0.028742142795067593
426426,852853,852852,1705705,671.0493988990784,0.028309909408562817
427427,854855,854854,1709709,672.5961577892303,0.027884241799938536
428428,856857,856856,1713713,674.1630227565765,0.027465038770742467
429429,858859,858858,1717717,675.7380349636078,0.02705220071527492
430430,860861,860860,1721721,677.3197839260101,0.026645629593645026
431431,862863,862862,1725725,678.8544597625732,0.02624522890789649
432432,864865,864864,1729729,680.3575568199158,0.025850903675518566
433433,866867,866866,1733733,681.8274238109589,0.02546256040636763
434434,868869,868868,1737737,683.4795618057251,0.02508010707788344
435435,870871,870870,1741741,685.1207499504089,0.024703453111442286
436436,872873,872872,1745745,686.7814719676971,0.02433250934905118
437437,874875,874874,1749749,688.4105439186096,0.023967188030269426
438438,876877,876876,1753753,690.1855227947235,0.023607402770267072
439439,878879,878878,1757757,691.7262740135193,0.02325306853776965
440440,880881,880880,1761761,693.3034517765045,0.022904101631752383
441441,882883,882882,1765765,694.8006629943848,0.022560419662113418
442442,884885,884884,1769769,696.2891447544098,0.022221941527163835
443443,886887,886886,1773773,697.7535979747772,0.021888587393505077
444444,888889,888888,1777777,699.2088639736176,0.021560278675906375
445445,890891,890890,1781781,700.6941130161285,0.021236938016841123
446446,892893,892892,1785785,702.2820868492126,0.020918489266250617
447447,894895,894894,1789789,703.8661508560181,0.020604857463808912
448448,896897,896896,1793793,705.4181339740753,0.020295968818459187
449449,898899,898898,1797797,706.9168167114258,0.019991750690564913
450450,900901,900900,1801801,708.4181728363037,0.019692131572583094
451451,902903,902902,1805805,709.8972778320312,0.019397041071556487
452452,904905,904904,1809809,711.4498560428619,0.01910640989149215
453453,906907,906906,1813813,713.0435299873352,0.018820169815626286
454454,908909,908908,1817817,714.591050863266,0.018538253688916484
455455,910911,910910,1821821,716.163792848587,0.018260595401329738
456456,912913,912912,1825825,717.6968996524811,0.017987129871471552
457457,914915,914914,1829829,719.1900658607483,0.017717793029760287
458458,916917,916916,1833833,720.6543328762054,0.017452521802283627
459459,918919,918918,1837837,722.1359570026398,0.017191254095223485
460460,920921,920920,1841841,723.6618340015411,0.01693392877984934
461461,922923,922922,1845845,725.1717579364777,0.016680485675124146
462462,924925,924924,1849849,726.6834506988525,0.01643086553519879
463463,926927,926926,1853853,728.1932709217072,0.016185010033154867
464464,928929,928928,1857857,729.6734027862549,0.015942861746452763
465465,930931,930930,1861861,731.1744089126587,0.015704364142379745
466466,932933,932932,1865865,732.6980168819427,0.015469461564975973
467467,934935,934934,1869869,734.2121467590332,0.015238099220482582
468468,936937,936936,1873873,735.6489708423615,0.015010223162903458
469469,938939,938938,1877877,737.1606419086456,0.014785780282409178
470470,940941,940940,1881881,738.6222116947174,0.014564718290330347
471471,942943,942942,1885885,740.0508117675781,0.014346985706879423
472472,944945,944944,1889889,741.564740896225,0.014132531848986218
473473,946947,946946,1893893,743.1438939571381,0.013921306816428114
474474,948949,948948,1897897,744.665549993515,0.01371326148046137
475475,950951,950950,1901901,746.1525597572327,0.013508347471201887
476476,952953,952952,1905905,747.6910438537598,0.013306517165688092
477477,954955,954954,1909909,749.2769448757172,0.013107723676398564
478478,956957,956956,1913913,750.826751947403,0.012911920839087543
479479,958959,958958,1917917,752.3405539989471,0.012719063201984682
480480,960961,960960,1921921,753.8371829986572,0.0125291060140853
481481,962963,962962,1925925,755.3108158111572,0.012342005214691198
482482,964965,964964,1929929,756.7515330314636,0.012157717421700909
483483,966967,966966,1933933,758.2367808818817,0.011976199921832631
484484,968969,968968,1937937,759.7676129341125,0.011797410659255547
485485,970971,970970,1941941,761.3050050735474,0.011621308226381188
486486,972973,972972,1945945,762.8467798233032,0.01144785185249475
487487,974975,974974,1949949,764.3547329902649,0.011277001393750652
488488,976977,976976,1953953,765.870414018631,0.01110871732544183
489489,978979,978978,1957957,767.3464179039001,0.010942960729153128
490490,980981,980980,1961961,768.8093156814575,0.010779693285257963
491491,982983,982982,1965965,770.3039517402649,0.010618877263368631
492492,984985,984984,1969969,771.7829697132111,0.010460475512445555
493493,986987,986986,1973973,773.2459666728973,0.010304451452157082
494494,988989,988988,1977977,774.7573759555817,0.010150769063784537
495495,990991,990990,1981981,776.2972726821899,0.009999392882036773
496496,992993,992992,1985985,777.8357338905334,0.009850287985159412
497497,994995,994994,1989989,779.3317837715149,0.00970341998731783
498498,996997,996996,1993993,780.9711217880249,0.009558755030411703
499499,998999,998998,1997997,782.6284689903259,0.009416259775207436
500501,1001003,1001002,2002005,784.3374209403992,0.009275762232732632
501502,1003005,1003004,2006009,786.2453119754791,0.009137510485743405
502503,1005007,1005006,2010013,787.9230668544769,0.009001331425565695
503504,1007009,1007008,2014017,789.5997266769409,0.008867193710329957
504505,1009011,1009010,2018021,791.2721848487854,0.008735066477811415
505506,1011013,1011012,2022025,792.9900639057159,0.008604919338381478
506507,1013015,1013014,2026029,794.561399936676,0.008476722367277034
507508,1015017,1015016,2030033,796.0658197402954,0.008350446097665554
508509,1017019,1017018,2034037,798.1062128543854,0.008226061513255445
509510,1019021,1019020,2038041,799.9522259235382,0.00810354004158853
510511,1021023,1021022,2042045,801.9086079597473,0.007982853546650404
511512,1023025,1023024,2046049,803.6116049289703,0.007863974322731337
512513,1025027,1025026,2050053,805.3055658340454,0.007746875087264016
513514,1027029,1027028,2054057,807.0136587619781,0.0076315289742296955
514515,1029031,1029030,2058061,808.7631969451904,0.0075179095281328046
515516,1031033,1031032,2062065,810.3768517971039,0.007405990696952358
516517,1033035,1033034,2066069,811.9506690502167,0.007295746826798677
517518,1035037,1035036,2070073,813.6604070663452,0.00718715265463743
518519,1037039,1037038,2074077,815.2666518688202,0.007080183302946352
519520,1039041,1039040,2078081,817.1360387802124,0.006974814274258279
520521,1041043,1041042,2082085,818.8677768707275,0.006871021443316749
521522,1043045,1043044,2086089,820.6930229663849,0.006768781053665407
522523,1045047,1045046,2090093,822.5621449947357,0.006668069710599411
523524,1047049,1047048,2094097,824.418338060379,0.006568864375481098
524525,1049051,1049050,2098101,826.108720779419,0.006471142361078819
525526,1051053,1051052,2102105,827.9768397808075,0.006374881325200477
526527,1053055,1053054,2106109,829.8522288799286,0.006280059266032367
527528,1055057,1055056,2110113,831.6175827980042,0.0061866545167958975
528529,1057059,1057058,2114117,833.4183087348938,0.006094645739608495
529530,1059061,1059060,2118121,835.081426858902,0.006004011922527752
530531,1061063,1061062,2122125,836.8658077716827,0.005914732371934406
531532,1063065,1063064,2126129,838.646194934845,0.0058267867094627945
532533,1065067,1065066,2130133,840.5334599018097,0.005740154866657576
533534,1067069,1067068,2134137,842.299544095993,0.005654817079744134
534535,1069071,1069070,2138141,843.9808497428894,0.005570753885535851
535536,1071073,1071072,2142145,845.7714958190918,0.005487946116318199
536537,1073075,1073074,2146149,847.5491418838501,0.0054063748957560165
537538,1075077,1075076,2150153,849.1058449745178,0.005326021633663913
538539,1077079,1077078,2154157,850.6846950054169,0.005246868022936724
539540,1079081,1079080,2158161,852.240975856781,0.005168896033637793
540541,1081083,1081082,2162165,853.9465839862823,0.005092087909815746
541542,1083085,1083084,2166169,855.5093150138855,0.005016426164502263
542543,1085087,1085086,2170173,857.1428830623627,0.004941893576187795
543544,1087089,1087088,2174177,858.8009119033813,0.004868473184956201
544545,1089091,1089090,2178181,860.3578178882599,0.004796148287368851
545546,1091093,1091092,2182185,861.8506097793579,0.004724902433736133
546547,1093095,1093094,2186189,863.5056269168854,0.004654719423228926
547548,1095097,1095096,2190193,865.1371088027954,0.0045855833008090485
548549,1097099,1097098,2194197,866.8665618896484,0.004517478353363913
549550,1099101,1099100,2198201,868.7048008441925,0.00445038910504536
550551,1101103,1101102,2202205,870.3324747085571,0.004384300315109613
551552,1103105,1103104,2206209,871.9666728973389,0.004319196973142425
552553,1105107,1105106,2210213,873.474488735199,0.004255064296216915
553554,1107109,1107108,2214217,874.9701118469238,0.004191887724687149
554555,1109111,1109110,2218221,876.4769809246063,0.004129652919914406
555556,1111113,1111112,2222225,878.0148589611053,0.004068345759492331
556557,1113115,1113114,2226229,879.5124769210815,0.0040079523354279445
557558,1115117,1115116,2230233,881.0310180187225,0.003948458948912048
558559,1117119,1117118,2234237,882.5198037624359,0.003889852109182357
559560,1119121,1119120,2238241,884.0113620758057,0.0038321185293170856
560561,1121123,1121122,2242245,885.5191769599915,0.0037752451228243444
561562,1123125,1123124,2246249,887.0841557979584,0.0037192190012547144
562563,1125127,1125126,2250253,889.0279810428619,0.003664027470790643
563564,1127129,1127128,2254257,890.4949197769165,0.0036096580294042724
564565,1129131,1129130,2258261,891.9591391086578,0.0035560983637878962
565566,1131133,1131132,2262265,893.4582278728485,0.003503336346625474
566567,1133135,1133134,2266269,894.9415059089661,0.0034513600337504613
567568,1135137,1135136,2270273,896.4265668392181,0.0034001576613036377
568569,1137139,1137138,2274277,897.9348719120026,0.003349717642890937
569570,1139141,1139140,2278281,899.6875467300415,0.0033000285668549623
570571,1141143,1141142,2282285,901.3366787433624,0.003251079193660189
571572,1143145,1143144,2286289,903.2111239433289,0.003202858453846602
572573,1145147,1145146,2290293,904.8023657798767,0.0031553554441643428
573574,1147149,1147148,2294297,906.2858397960663,0.003108559426323154
574575,1149151,1149150,2298301,908.3917880058289,0.0030624598235817757
575576,1151153,1151152,2302305,909.9233129024506,0.00301704621870158
576577,1153155,1153154,2306309,911.4107618331909,0.0029723083517865234
577578,1155157,1155156,2310313,912.9318978786469,0.00292823611687254
578579,1157159,1157158,2314317,914.3902928829193,0.0028848195609043614
579580,1159161,1159160,2318321,915.8708107471466,0.00284204888032491
580581,1161163,1161162,2322325,917.3713629245758,0.0027999144194836845
581582,1163165,1163164,2326329,918.8861298561096,0.002758406668021962
582583,1165167,1165166,2330333,920.3260757923126,0.002717516258599062
583584,1167169,1167168,2334337,921.8298759460449,0.002677233965414416
584585,1169171,1169170,2338341,923.3148028850555,0.0026375507007969645
585586,1171173,1171172,2342345,924.887218952179,0.0025984575146367206
586587,1173175,1173174,2346349,926.3870520591736,0.0025599455908604796
587588,1175177,1175176,2350353,927.867547750473,0.002522006246181263
588589,1177179,1177178,2354357,929.4365267753601,0.0024846309279382695
589590,1179181,1179180,2358361,931.1442427635193,0.0024478112125052576
590591,1181183,1181182,2362365,932.865504026413,0.002411538801993629
591592,1183185,1183184,2366369,935.3355538845062,0.0023758055245934884
592593,1185187,1185186,2370373,937.2412989139557,0.002340603329912483
593594,1187189,1187188,2374377,938.79984998703,0.002305924289316863
594595,1189191,1189190,2378381,940.4784798622131,0.0022717605937714325
595596,1191193,1191192,2382385,942.1493167877197,0.002238104550428943
596597,1193195,1193194,2386389,943.7630929946899,0.002204948583312216
597598,1195197,1195196,2390393,945.299103975296,0.002172285229107729
598599,1197199,1197198,2394397,946.9106900691986,0.0021401071369382407
599600,1199201,1199200,2398401,948.3856558799744,0.0021084070667711785
600601,1201203,1201202,2402405,949.8504378795624,0.0020771778871448987
601602,1203205,1203204,2406409,951.3147037029266,0.002046412572894951
602603,1205207,1205206,2410413,952.9986097812653,0.002016104205267766
603604,1207209,1207208,2414417,954.559898853302,0.0019862459690784817
604605,1209211,1209210,2418421,956.4462478160858,0.0019568311510056446
605606,1211213,1211212,2422425,958.0999810695648,0.0019278531391364595
606607,1213215,1213214,2426429,960.055330991745,0.0018993054202383064
607608,1215217,1215216,2430433,962.0162208080292,0.0018711815788492459
608609,1217219,1217218,2434437,963.3304979801178,0.00184347529580009
609610,1219221,1219220,2438441,964.7453429698944,0.001816180347077534
610611,1221223,1221222,2442445,966.1545579433441,0.0017892906010956722
611612,1223225,1223224,2446449,968.0262126922607,0.0017628000190370585
612613,1225227,1225226,2450453,969.7936828136444,0.0017367026521242224
613614,1227229,1227228,2454457,971.3377730846405,0.0017109926411649212
614615,1229231,1229230,2458461,973.0177547931671,0.0016856642143920908
615616,1231233,1231232,2462465,974.6280038356781,0.001660711686781724
616617,1233235,1233234,2466469,976.3413798809052,0.0016361294580065078
617618,1235237,1235236,2470473,978.1947147846222,0.001611912012663197
618619,1237239,1237238,2474477,980.0930869579315,0.0015880539166346352
619620,1239241,1239240,2478481,981.9073848724365,0.0015645498182266238
620621,1241243,1241242,2482485,983.7527589797974,0.0015413944454394368
621622,1243245,1243244,2486489,985.5337338447571,0.0015185826051720142
622623,1245247,1245246,2490493,987.5273268222809,0.0014961091827672135
623624,1247249,1247248,2494497,990.1847269535065,0.0014739691390559528
624625,1249251,1249250,2498501,991.922632932663,0.001452157510698271
625626,1251253,1251252,2502505,993.7002489566803,0.0014306694093875194
626627,1253255,1253254,2506509,995.6486699581146,0.001409500018894505
627628,1255257,1255256,2510513,997.1132049560547,0.0013886445952948634
628629,1257259,1257258,2514517,998.716470003128,0.0013680984664006246
629630,1259261,1259260,2518521,1000.5155987739563,0.0013478570290317293
630631,1261263,1261262,2522525,1002.0257089138031,0.0013279157491297156
631632,1263265,1263264,2526529,1003.6967198848724,0.001308270160848224
632633,1265267,1265266,2530533,1005.5444939136505,0.0012889158643929477
633634,1267269,1267268,2534537,1008.0369987487793,0.0012698485264763804
634635,1269271,1269270,2538541,1009.8587439060211,0.0012510638781577654
635636,1271273,1271272,2542545,1011.5214788913727,0.0012325577143883493
636637,1273275,1273274,2546549,1013.1815187931061,0.0012143258931018863
637638,1275277,1275276,2550553,1014.7015590667725,0.001196364333850397
638639,1277279,1277278,2554557,1016.314778804779,0.0011786690175767944
639640,1279281,1279280,2558561,1017.8613178730011,0.0011612359851369547
640641,1281283,1281282,2562565,1019.6178276538849,0.001144061336390223
641642,1283285,1283284,2566569,1021.3212299346924,0.001127141229744666
642643,1285287,1285286,2570573,1023.0592617988586,0.0011104718802243951
643644,1287289,1287288,2574577,1024.7128639221191,0.0010940495604927492
644645,1289291,1289290,2578581,1026.4174058437347,0.0010778705983511827
645646,1291293,1291292,2582585,1028.0658690929413,0.0010619313763982063
646647,1293295,1293294,2586589,1029.574266910553,0.0010462283312335785
647648,1295297,1295296,2590593,1031.2828669548035,0.0010307579526624977
648649,1297299,1297298,2594597,1032.917011976242,0.0010155167830134815
649650,1299301,1299300,2598601,1034.5513410568237,0.0010005014161151848
650651,1301303,1301302,2602605,1036.2795209884644,0.0009857084969553398
651652,1303305,1303304,2606609,1038.1882178783417,0.0009711347198617659
652653,1305307,1305306,2610613,1039.88906788826,0.0009567768295255519
653654,1307309,1307308,2614617,1042.0243587493896,0.0009426316183862582
654655,1309311,1309310,2618621,1043.6962230205536,0.0009286959267456041
655656,1311313,1311312,2622625,1045.2048139572144,0.0009149666428811543
656657,1313315,1313314,2626629,1046.7168130874634,0.0009014407004315217
657658,1315317,1315316,2630633,1048.4215638637543,0.0008881150793058623
658659,1317319,1317318,2634637,1050.1648769378662,0.0008749868046606935
659660,1319321,1319320,2638641,1052.0008897781372,0.0008620529456493387
660661,1321323,1321322,2642645,1053.6579377651215,0.0008493106150808671
661662,1323325,1323324,2646649,1055.2346138954163,0.0008367569690790333
662663,1325327,1325326,2650653,1056.7534918785095,0.000824389206172782
663664,1327329,1327328,2654657,1058.3178670406342,0.0008122045665004407
664665,1329331,1329330,2658661,1059.852826833725,0.0008002003312412853
665666,1331333,1331332,2662665,1061.4032278060913,0.0007883738225018533
666667,1333335,1333334,2666669,1063.0067319869995,0.0007767224017243279
667668,1335337,1335336,2670673,1064.566969871521,0.0007652434702549726
668669,1337339,1337338,2674677,1066.3552329540253,0.0007539344676388282
669670,1339341,1339340,2678681,1068.1277260780334,0.0007427928719607735
670671,1341343,1341342,2682685,1069.9071049690247,0.0007318161990497174
671672,1343345,1343344,2686689,1071.4136147499084,0.0007210020007732965
672673,1345347,1345346,2690693,1073.02002286911,0.0007103478667431773
673674,1347349,1347348,2694697,1074.611249923706,0.0006998514215865725
674675,1349351,1349350,2698701,1076.5512907505035,0.0006895103256283619
675676,1351353,1351352,2702705,1078.0598809719086,0.0006793222739815974
676677,1353355,1353354,2706709,1079.5843057632446,0.0006692849959790692
677678,1355357,1355356,2710713,1081.2196538448334,0.0006593962550596189
678679,1357359,1357358,2714717,1083.0285558700562,0.0006496538478586444
679680,1359361,1359360,2718721,1084.986722946167,0.000640055603298606
680681,1361363,1361362,2722725,1087.1133108139038,0.0006305993833848333
681682,1363365,1363364,2726729,1089.0682470798492,0.000621283081841284
682683,1365367,1365366,2730733,1090.6421728134155,0.0006121046229736749
683684,1367369,1367368,2734737,1092.236268043518,0.0006030619629200373
684685,1369371,1369370,2738741,1094.529109954834,0.0005941530876043544
685686,1371373,1371372,2742745,1096.462809085846,0.0005853760134186814
686687,1373375,1373374,2746749,1098.9542348384857,0.0005767287858589043
687688,1375377,1375376,2750753,1100.7411577701569,0.0005682094795247394
688689,1377379,1377378,2754757,1102.302486896515,0.0005598161980060468
689690,1379381,1379380,2758761,1104.039636850357,0.0005515470725185878
690691,1381383,1381382,2762765,1105.6042909622192,0.0005434002629272072
691692,1383385,1383384,2766769,1107.053288936615,0.0005353739556994697
692693,1385387,1385386,2770773,1108.5011599063873,0.0005274663647014677
693694,1387389,1387388,2774777,1109.9653198719025,0.0005196757300609534
694695,1389391,1389390,2778781,1111.3911418914795,0.0005120003180536514
695696,1391393,1391392,2782785,1112.8586807250977,0.000504438421330633
696697,1393395,1393394,2786789,1114.57342004776,0.0004969883574403866
697698,1395397,1395396,2790793,1116.529593706131,0.0004896484687151315
698699,1397399,1397398,2794797,1118.0498039722443,0.00048241712261187786
699700,1399401,1399400,2798801,1119.7612237930298,0.00047529271080293256
700701,1401403,1401402,2802805,1121.3404097557068,0.00046827364849377773
701702,1403405,1403404,2806809,1122.8122699260712,0.00046135837476413144
702703,1405407,1405406,2810813,1124.273675918579,0.00045454535177213984
703704,1407409,1407408,2814817,1125.8390378952026,0.0004478330647543771
704705,1409411,1409410,2818821,1127.7681069374084,0.000441220021002664
705706,1411413,1411412,2822825,1129.3797817230225,0.00043470475054618873
706707,1413415,1413414,2826829,1131.0800459384918,0.00042828580501463875
707708,1415417,1415416,2830833,1133.1014127731323,0.00042196175706976646
708709,1417419,1417418,2834837,1134.9192688465118,0.0004157312014285708
709710,1419421,1419420,2838841,1136.3909187316895,0.0004095927529306209
710711,1421423,1421422,2842845,1137.8250188827515,0.00040354504778861156
711712,1423425,1423424,2846849,1139.2743117809296,0.0003975867417693735
712713,1425427,1425426,2850853,1140.87677693367,0.0003917165109896814
713714,1427429,1427428,2854857,1142.755136013031,0.00038593305066569883
714715,1429431,1429430,2858861,1144.392017841339,0.00038023507636353315
715716,1431433,1431432,2862865,1145.8596317768097,0.00037462132183918584
716717,1433435,1433434,2866869,1147.2946078777313,0.00036909054017542076
717718,1435437,1435436,2870873,1148.7329490184784,0.00036364150275858265
718719,1437439,1437438,2874877,1150.177176952362,0.00035827299905122345
719720,1439441,1439440,2878881,1151.6239559650421,0.0003529838369331628
720721,1441443,1441442,2882885,1153.0523970127106,0.00034777284156461974
721722,1443445,1443444,2886889,1154.5005249977112,0.0003426388558409599
722723,1445447,1445446,2890893,1156.0989367961884,0.00033758073971057456
723724,1447449,1447448,2894897,1157.9578158855438,0.00033259736983382027
724725,1449451,1449450,2898901,1160.0334861278534,0.0003276876398103923
725726,1451453,1451452,2902905,1162.0306448936462,0.0003228504598382642
726727,1453455,1453454,2906909,1164.193202972412,0.0003180847555768196
727728,1455457,1455456,2910913,1166.2699048519135,0.00031338946962478076
728729,1457459,1457458,2914917,1168.1133818626404,0.00030876355924647214
729730,1459461,1459460,2918921,1169.754893064499,0.00030420599830449646
730731,1461463,1461462,2922925,1171.8540868759155,0.0002997157744175638
731732,1463465,1463464,2926929,1173.910395860672,0.0002952918915752889
732733,1465467,1465466,2930933,1176.0536530017853,0.00029093336820551485
733734,1467469,1467468,2934937,1178.9122788906097,0.0002866392363785053
734735,1469471,1469470,2938941,1181.045578956604,0.000282408544194368
735736,1471473,1471472,2942945,1183.4132108688354,0.0002782403523724497
736737,1473475,1473474,2946949,1185.4758548736572,0.00027413373607032554
737738,1475477,1475476,2950953,1187.5784549713135,0.0002700877844290517
738739,1477479,1477478,2954957,1189.5931210517883,0.00026610160000473115
739740,1479481,1479480,2958961,1191.4309628009796,0.0002621742983137665
740741,1481483,1481482,2962965,1193.0886788368225,0.0002583050084012939
741742,1483485,1483484,2966969,1194.5604877471924,0.00025449287193168857
742743,1485487,1485486,2970973,1196.3736109733582,0.0002507370434159384
743744,1487489,1487488,2974977,1197.9523267745972,0.0002470366899842702
744745,1489491,1489490,2978981,1199.6173958778381,0.00024339099093140248
745746,1491493,1491492,2982985,1202.0499110221863,0.00023979913794391905
746747,1493495,1493494,2986989,1204.1816980838776,0.00023626033430446114
747748,1495497,1495496,2990993,1206.120440006256,0.0002327737956875353
748749,1497499,1497498,2994997,1208.5531919002533,0.00022933874879527139
749750,1499501,1499500,2999001,1210.1815967559814,0.00022595443238060398
750751,1501503,1501502,3003005,1212.6180090904236,0.00022262009588303044
751752,1503505,1503504,3007009,1214.6489398479462,0.00021933500022441876
752753,1505507,1505506,3011013,1216.5740087032318,0.00021609841724057333
753754,1507509,1507508,3015017,1218.0564279556274,0.00021290962968123495
754755,1509511,1509510,3019021,1219.505816936493,0.000209767930414273
755756,1511513,1511512,3023025,1220.9283289909363,0.00020667262322149327
756757,1513515,1513514,3027029,1222.405014038086,0.00020362302245757746
757758,1515517,1515516,3031033,1223.8707818984985,0.0002006184521405885
758759,1517519,1517518,3035037,1225.6113839149475,0.00019765824617934413
759760,1519521,1519520,3039041,1227.586539030075,0.00019474174871447758
760761,1521523,1521522,3043045,1229.1482989788055,0.00019186831400475057
761762,1523525,1523524,3047049,1230.6639318466187,0.00018903730472175084
762763,1525527,1525526,3051053,1232.2137548923492,0.00018624809388256836
763764,1527529,1527528,3055057,1233.7239327430725,0.00018350006382661377
764765,1529531,1529530,3059061,1235.2535219192505,0.00018079260541981057
765766,1531533,1531532,3063065,1237.1498680114746,0.0001781251193051503
766767,1533535,1533534,3067069,1238.6546988487244,0.0001754970140837031
767768,1535537,1535536,3071073,1240.1641159057617,0.00017290770790623355
768769,1537539,1537538,3075077,1241.5507400035858,0.000170356627450019
769770,1539541,1539540,3079081,1243.0010077953339,0.00016784320723672863
770771,1541543,1541542,3083085,1244.5229077339172,0.00016536689099666546
771772,1543545,1543544,3087089,1246.0037078857422,0.0001629271301908375
772773,1545547,1545546,3091093,1247.4939618110657,0.00016052338446570502
773774,1547549,1547548,3095097,1248.9029669761658,0.00015815512165318069
774775,1549551,1549550,3099101,1250.4508028030396,0.00015582181731588207
775776,1551553,1551552,3103105,1252.111828804016,0.00015352295486081857
776777,1553555,1553554,3107109,1253.9536929130554,0.00015125802508464403
777778,1555557,1555556,3111113,1255.6091659069061,0.00014902652685577777
778779,1557559,1557558,3115117,1257.0617978572845,0.00014682796575016255
779780,1559561,1559560,3119121,1258.5001509189606,0.00014466185552919342
780781,1561563,1561562,3123125,1259.919843673706,0.00014252771632072836
781782,1563565,1563564,3127129,1261.387990951538,0.00014042507575595664
782783,1565567,1565566,3131133,1262.8153839111328,0.00013835346851465147
783784,1567569,1567568,3135137,1264.2728538513184,0.00013631243587042263
784785,1569571,1569570,3139141,1265.701635837555,0.00013430152637283754
785786,1571573,1571572,3143145,1267.1188097000122,0.00013232029482423968
786787,1573575,1573574,3147149,1268.527718782425,0.00013036830250712228
787788,1575577,1575576,3151153,1269.9681730270386,0.00012844511786624935
788789,1577579,1577578,3155157,1271.403558731079,0.00012655031503072678
789790,1579581,1579580,3159161,1272.857558965683,0.00012468347460981022
790791,1581583,1581582,3163165,1274.3189239501953,0.00012284418357921822
791792,1583585,1583584,3167169,1275.778638124466,0.00012103203505375859
792793,1585587,1585586,3171173,1278.3077340126038,0.00011924662828732835
793794,1587589,1587588,3175177,1280.5714848041534,0.0001174875678771059
794795,1589591,1589590,3179181,1282.6968340873718,0.0001157544645593589
795796,1591593,1591592,3183185,1284.4341859817505,0.00011404693555050471
796797,1593595,1593594,3187189,1286.092236995697,0.00011236460227337375
797798,1595597,1595596,3191193,1288.4804940223694,0.00011070709319938032
798799,1597599,1597598,3195197,1290.088917016983,0.00010907404123372544
799800,1599601,1599600,3199201,1291.5291998386383,0.00010746508542069932
800801,1601603,1601602,3203205,1292.9642658233643,0.00010587986992049991
801802,1603605,1603604,3207209,1294.4031238555908,0.00010431804366817232
802803,1605607,1605606,3211213,1295.8450129032135,0.00010277926162416406
803804,1607609,1607608,3215217,1297.3644659519196,0.000101263183410083
804805,1609611,1609610,3219221,1299.258094072342,9.97694737634447e-05
805806,1611613,1611612,3223225,1301.1244139671326,9.829780196923821e-05
806807,1613615,1613614,3227229,1302.9172847270966,9.68478429967945e-05
807808,1615617,1615616,3231233,1305.1363897323608,9.541927590817068e-05
808809,1617619,1617618,3235237,1307.8950567245483,9.401178510870523e-05
809810,1619621,1619620,3239241,1311.0492379665375,9.262505909646279e-05
810811,1621623,1621622,3243245,1313.132670879364,9.125879159910255e-05
811812,1623625,1623624,3247249,1314.9935097694397,8.991267998226249e-05
812813,1625627,1625626,3251253,1316.698980808258,8.858642695486196e-05
813814,1627629,1627628,3255257,1318.4191617965698,8.727973931854649e-05
814815,1629631,1629630,3259261,1319.8999009132385,8.599232819506142e-05
815816,1631633,1631632,3263265,1321.5038557052612,8.472390879887826e-05
816817,1633635,1633634,3267269,1323.3447318077087,8.347420066456834e-05
817818,1635637,1635636,3271273,1325.0557188987732,8.224292787417653e-05
818819,1637639,1637638,3275277,1326.6761629581451,8.102981803403964e-05
819820,1639641,1639640,3279281,1328.35196185112,7.983460284322064e-05
820821,1641643,1641642,3283285,1329.9181249141693,7.865701843456918e-05
821822,1643645,1643644,3287289,1331.3665280342102,7.749680423785321e-05
822823,1645647,1645646,3291293,1332.816508769989,7.63537040029405e-05
823824,1647649,1647648,3295297,1334.2447159290314,7.522746489030396e-05
824825,1649651,1649650,3299301,1335.9561228752136,7.411783803945582e-05
825826,1651653,1651652,3303305,1338.8577799797058,7.302457845526078e-05
826827,1653655,1653654,3307309,1341.1140730381012,7.194744409844134e-05
827828,1655657,1655656,3311313,1342.9546637535095,7.088619736350665e-05
828829,1657659,1657658,3315317,1344.4688758850098,6.984060348713683e-05
829830,1659661,1659660,3319321,1345.9433958530426,6.881043145767762e-05
830831,1661663,1661662,3323325,1347.4171090126038,6.779545356039307e-05
831832,1663665,1663664,3327329,1350.0611789226532,6.679544560483919e-05
832833,1665667,1665666,3331333,1351.7679789066315,6.581018669749028e-05
833834,1667669,1667668,3335337,1353.732712984085,6.483945890067844e-05
834835,1669671,1669670,3339341,1355.2237360477448,6.388304791471455e-05
835836,1671673,1671672,3343345,1356.7223489284515,6.294074262314098e-05
836837,1673675,1673674,3347349,1358.209017753601,6.201233441061049e-05
837838,1675677,1675676,3351353,1359.7032570838928,6.109761829975469e-05
838839,1677679,1677678,3355357,1361.3262519836426,6.01963924964366e-05
839840,1679681,1679680,3359361,1363.4774677753448,5.930845748025604e-05
840841,1681683,1681682,3363365,1364.9409310817719,5.84336173687916e-05
841842,1683685,1683684,3367369,1366.4258427619934,5.757167878073233e-05
842843,1685687,1685686,3371373,1367.9436929225922,5.6722451517998707e-05
843844,1687689,1687688,3375377,1369.3912630081177,5.5885747769934824e-05
844845,1689691,1689690,3379381,1370.8511517047882,5.506138290911622e-05
845846,1691693,1691692,3383385,1372.3312108516693,5.4249174695542024e-05
846847,1693695,1693694,3387389,1373.779364824295,5.344894361769548e-05
847848,1695697,1695696,3391393,1375.2336146831512,5.2660513119917596e-05
848849,1697699,1697698,3395397,1376.7238988876343,5.188370903397299e-05
849850,1699701,1699700,3399401,1378.2641298770905,5.111835992011038e-05
850851,1701703,1701702,3403405,1380.177484035492,5.0364296384941554e-05
851852,1703705,1703704,3407409,1382.102077960968,4.9621352331996604e-05
852853,1705707,1705706,3411413,1385.086744070053,4.888936348379502e-05
853854,1707709,1707708,3415417,1387.2790310382843,4.816816817765357e-05
854855,1709711,1709710,3419421,1389.317463874817,4.745760702462576e-05
855856,1711713,1711712,3423425,1391.4199569225311,4.675752347793605e-05
856857,1713715,1713714,3427429,1393.670891046524,4.606776246873778e-05
857858,1715717,1715716,3431433,1395.2207489013672,4.538817222510261e-05
858859,1717719,1717718,3435437,1396.906798839569,4.471860211197054e-05
859860,1719721,1719720,3439441,1398.423178911209,4.4058904677513056e-05
860861,1721723,1721722,3443445,1399.9123487472534,4.340893440257787e-05
861862,1723725,1723724,3447449,1401.4438619613647,4.276854735962843e-05
862863,1725727,1725726,3451453,1403.263070821762,4.213760223592544e-05
863864,1727729,1727728,3455457,1404.9326887130737,4.1515960106153216e-05
864865,1729731,1729730,3459461,1406.9414117336273,4.090348318186443e-05
865866,1731733,1731732,3463465,1408.466784954071,4.030003674415639e-05
866867,1733735,1733734,3467469,1410.4937028884888,3.970548721099476e-05
867868,1735737,1735736,3471473,1412.3728818893433,3.911970350145566e-05
868869,1737739,1737738,3475477,1414.488226890564,3.854255623991776e-05
869870,1739741,1739740,3479481,1416.2526128292084,3.7973918097122805e-05
870871,1741743,1741742,3483485,1418.0151557922363,3.741366356280196e-05
871872,1743745,1743744,3487489,1419.6593868732452,3.686166860461526e-05
872873,1745747,1745746,3491493,1421.1739447116852,3.631781180502003e-05
873874,1747749,1747748,3495497,1422.7853429317474,3.5781973224402464e-05
874875,1749751,1749750,3499501,1424.381609916687,3.525403394633031e-05
875876,1751753,1751752,3503505,1425.857302904129,3.473387812391593e-05
876877,1753755,1753754,3507509,1427.660033941269,3.422139047870587e-05
877878,1755757,1755756,3511513,1429.4007768630981,3.3716458347043954e-05
878879,1757759,1757758,3515517,1431.0491378307343,3.321896986108186e-05
879880,1759761,1759760,3519521,1432.3759417533875,3.272881519933435e-05
880881,1761763,1761762,3523525,1433.6993207931519,3.22458867003661e-05
881882,1763765,1763764,3527529,1434.9607639312744,3.177007715748914e-05
882883,1765767,1765766,3531533,1436.228453874588,3.1301282092499605e-05
883884,1767769,1767768,3535537,1437.5865757465363,3.083939770931465e-05
884885,1769771,1769770,3539541,1438.847068786621,3.0384322258214524e-05
885886,1771773,1771772,3543545,1440.2869129180908,2.9935955012660997e-05
886887,1773775,1773774,3547549,1441.8507568836212,2.9494197406165767e-05
887888,1775777,1775776,3551553,1443.4000618457794,2.905895189542207e-05
888889,1777779,1777778,3555557,1445.0059688091278,2.8630122187678353e-05
889890,1779781,1779780,3559561,1446.5039298534393,2.8207614036546147e-05
890891,1781783,1781782,3563565,1448.3179769515991,2.779133376407117e-05
891892,1783785,1783784,3567569,1450.258292913437,2.738118996603589e-05
892893,1785787,1785786,3571573,1451.9864220619202,2.6977091692970134e-05
893894,1787789,1787788,3575577,1453.6352219581604,2.657895015545364e-05
894895,1789791,1789790,3579581,1455.890956878662,2.6186677246187173e-05
895896,1791793,1791792,3583585,1458.2495198249817,2.5800186563174066e-05
896897,1793795,1793794,3587589,1460.1230220794678,2.5419392841286026e-05
897898,1795797,1795796,3591593,1461.7365407943726,2.5044212065949978e-05
898899,1797799,1797798,3595597,1463.39612698555,2.4674561359461222e-05
899900,1799801,1799800,3599601,1465.4730479717255,2.431035932204395e-05
900901,1801803,1801802,3603605,1467.0349488258362,2.3951525463417056e-05
901902,1803805,1803804,3607609,1468.566555738449,2.3597980657541484e-05
902903,1805807,1805806,3611613,1470.0191888809204,2.3249647028933396e-05
903904,1807809,1807808,3615617,1471.4652190208435,2.2906447611603653e-05
904905,1809811,1809810,3619621,1472.9162647724152,2.2568306576431496e-05
905906,1811813,1811812,3623625,1474.4281969070435,2.2235149572225055e-05
906907,1813815,1813814,3627629,1475.8588087558746,2.190690315728716e-05
907908,1815817,1815816,3631633,1477.3321678638458,2.1583494458354835e-05
908909,1817819,1817818,3635637,1478.8353006839752,2.1264852762215014e-05
909910,1819821,1819820,3639641,1480.2928688526154,2.095090712828096e-05
910911,1821823,1821822,3643645,1481.7269339561462,2.064158888970269e-05
911912,1823825,1823824,3647649,1483.1803557872772,2.0336829493317055e-05
912913,1825827,1825826,3651653,1484.6174457073212,2.003656197757664e-05
913914,1827829,1827828,3655657,1486.0719459056854,1.9740719721994537e-05
914915,1829831,1829830,3659661,1487.5402429103851,1.944923781138641e-05
915916,1831833,1831832,3663665,1489.1120519638062,1.9162051671628433e-05
916917,1833835,1833834,3667669,1490.647341966629,1.8879098320212506e-05
917918,1835837,1835836,3671673,1493.045637845993,1.8600315115691046e-05
918919,1837839,1837838,3675677,1494.4724879264832,1.8325640667171683e-05
919920,1839841,1839840,3679681,1495.8947451114655,1.8055014265883074e-05
920921,1841843,1841842,3683685,1497.3440277576447,1.778837633992225e-05
921922,1843845,1843844,3687689,1498.8062818050385,1.752566788582044e-05
922923,1845847,1845846,3691693,1500.2637376785278,1.7266831150664075e-05
923924,1847849,1847848,3695697,1501.6871438026428,1.701180917734746e-05
924925,1849851,1849850,3699701,1503.1335060596466,1.676054569088592e-05
925926,1851853,1851852,3703705,1504.5898077487946,1.6512984984728973e-05
926927,1853855,1853854,3707709,1506.0187330245972,1.626907260288135e-05
927928,1855857,1855856,3711713,1507.4618458747864,1.602875488515565e-05
928929,1857859,1857858,3715717,1508.8911318778992,1.579197873979865e-05
929930,1859861,1859860,3719721,1510.4490458965302,1.555869209823868e-05
930931,1861863,1861862,3723725,1512.5386259555817,1.5328843119277735e-05
931932,1863865,1863864,3727729,1514.1214110851288,1.5102381780707219e-05
932933,1865867,1865866,3731733,1515.8948678970337,1.4879257378197508e-05
933934,1867869,1867868,3735737,1517.4125518798828,1.4659421140095219e-05
934935,1869871,1869870,3739741,1518.8952770233154,1.444282474949432e-05
935936,1871873,1871872,3743745,1520.3681910037994,1.4229420003175619e-05
936937,1873875,1873874,3747749,1521.781301021576,1.4019160289535648e-05
937938,1875877,1875876,3751753,1523.17201089859,1.3811998883284105e-05
938939,1877879,1877878,3755757,1524.61110496521,1.36078903096859e-05
939940,1879881,1879880,3759761,1526.021934747696,1.340678977612697e-05
940941,1881883,1881882,3763765,1527.3919439315796,1.3208652376306418e-05
941942,1883885,1883884,3767769,1528.8269398212433,1.3013434909225907e-05
942943,1885887,1885886,3771773,1530.2505469322205,1.2821094173887104e-05
943944,1887889,1887888,3775777,1531.6416997909546,1.2631587765099539e-05
944945,1889891,1889890,3779781,1533.027864933014,1.2444873505046417e-05
945946,1891893,1891892,3783785,1534.4300708770752,1.2260911034900346e-05
946947,1893895,1893894,3787789,1535.843554019928,1.2079659200026072e-05
947948,1895897,1895896,3791793,1537.2858917713165,1.1901078551090905e-05
948949,1897899,1897898,3795797,1538.6855590343475,1.1725129070327966e-05
949950,1899901,1899900,3799801,1540.5908510684967,1.1551772331586108e-05
950951,1901903,1901902,3803805,1542.376450061798,1.1380970022401016e-05
951952,1903905,1903904,3807809,1544.0899667739868,1.121268473980308e-05
952953,1905907,1905906,3811813,1546.2242999076843,1.1046878967135854e-05
953954,1907909,1907908,3815817,1547.7297358512878,1.088351655198494e-05
954955,1909911,1909910,3819821,1549.282557964325,1.0722561114562268e-05
955956,1911913,1911912,3823825,1550.88272190094,1.0563977411948144e-05
956957,1913915,1913914,3827829,1552.4594287872314,1.0407730542283389e-05
957958,1915917,1915916,3831833,1553.9791049957275,1.0253786058456171e-05
958959,1917919,1917918,3835837,1555.5028448104858,1.0102109854415176e-05
959960,1919921,1919920,3839841,1557.049036026001,9.952668392543274e-06
960961,1921923,1921922,3843845,1558.5137889385223,9.80542904471804e-06
961962,1923925,1923924,3847849,1560.110701084137,9.660359296503884e-06
962963,1925927,1925926,3851853,1561.59525680542,9.517426974525733e-06
963964,1927929,1927928,3855857,1563.4327018260956,9.376600587529538e-06
964965,1929931,1929930,3859861,1565.744600057602,9.237849326382275e-06
965966,1931933,1931932,3863865,1567.6659047603607,9.101142381950922e-06
966967,1933935,1933934,3867869,1569.1091630458832,8.966449968283996e-06
967968,1935937,1935936,3871873,1570.6018407344818,8.833741958369501e-06
968969,1937939,1937938,3875877,1572.0389947891235,8.702989362063818e-06
969970,1939941,1939940,3879881,1573.613891839981,8.574163189223327e-06
970971,1941943,1941942,3883885,1575.1189138889313,8.447235245512275e-06
971972,1943945,1943944,3887889,1576.643573999405,8.322177677655418e-06
972973,1945947,1945946,3891893,1578.1158657073975,8.198962291317002e-06
973974,1947949,1947948,3895897,1579.5258748531342,8.077562597463839e-06
974975,1949951,1949950,3899901,1581.0197818279266,7.95795153862855e-06
975976,1951953,1951952,3903905,1582.53679895401,7.840102625777945e-06
976977,1953955,1953954,3907909,1584.088654756546,7.723990279373538e-06
977978,1955957,1955956,3911913,1585.6160428524017,7.609588692503166e-06
978979,1957959,1957958,3915917,1587.015862941742,7.4968725130020175e-06
979980,1959961,1959960,3919921,1588.4822657108307,7.3858172981999815e-06
980981,1961963,1961962,3923925,1589.9382038116455,7.276398150679597e-06
981982,1963965,1963964,3927929,1591.368080854416,7.168591082518105e-06
982983,1965967,1965966,3931933,1592.812540769577,7.06237244685326e-06
983984,1967969,1967968,3935937,1594.2706108093262,6.957718596822815e-06
984985,1969971,1969970,3939941,1595.7517681121826,6.854606795059226e-06
985986,1971973,1971972,3943945,1597.1654210090637,6.753014190508111e-06
986987,1973975,1973974,3947949,1598.6018559932709,6.652918386862439e-06
987988,1975977,1975976,3951953,1600.0442008972168,6.5542972151888534e-06
988989,1977979,1977978,3955957,1601.429100036621,6.4571289613013505e-06
989990,1979981,1979980,3959961,1602.8317487239838,6.361392365761276e-06
990991,1981983,1981982,3963965,1604.2393300533295,6.267066396503651e-06
991992,1983985,1983984,3967969,1605.6557450294495,6.17412990777666e-06
992993,1985987,1985986,3971973,1607.0788757801056,6.082562663323188e-06
993994,1987989,1987988,3975977,1608.4785888195038,5.992344654259796e-06
994995,1989991,1989990,3979981,1609.889886856079,5.9034556443293695e-06
995996,1991993,1991992,3983985,1611.3209290504456,5.8158761930826586e-06
996997,1993995,1993994,3987989,1612.7654919624329,5.729587087444088e-06
997998,1995997,1995996,3991993,1614.1833610534668,5.6445692280249204e-06
998999,1997999,1997998,3995997,1615.6372537612915,5.560803856496932e-06
1000000,2000001,2000000,4000001,1617.1285779476166,5.478272555592412e-06


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007669925689697266,2180.042156630883
7,15,7,22,0.008723974227905273,414.4111683940796
13,27,13,40,0.014967918395996094,225.76746587107368
20,41,20,61,0.02197098731994629,145.8255695275161
27,55,27,82,0.029317855834960938,109.4558204131788
34,69,34,103,0.03636884689331055,89.98215269380376
40,81,40,121,0.0422520637512207,80.0340112122251
47,95,47,142,0.048967838287353516,72.7699283998536
54,109,54,163,0.0559999942779541,67.80266873069786
61,123,61,184,0.06306791305541992,64.10175602888171
67,135,67,202,0.07184195518493652,61.530190712698186
74,149,74,223,0.07957601547241211,58.976714359307834
81,163,81,244,0.08729290962219238,56.940181479457124
87,175,87,262,0.0940859317779541,55.611295282713854
94,189,94,283,0.10444188117980957,54.452590750704076
101,203,101,304,0.1129310131072998,53.61782095360809
108,217,108,325,0.12169909477233887,52.99222110110145
114,229,114,343,0.13109779357910156,52.53022394126674
121,243,121,364,0.13997387886047363,51.98460723043809
128,257,128,385,0.14846372604370117,51.38980050307123
135,271,135,406,0.15711474418640137,50.74694300645342
141,283,141,424,0.1645660400390625,50.16612764397519
148,297,148,445,0.17325115203857422,49.45580092378714
155,311,155,466,0.1821918487548828,48.7095318171946
161,323,161,484,0.18962574005126953,48.04562499645499
168,337,168,505,0.19829201698303223,47.253653677788634
175,351,175,526,0.20679879188537598,46.45569110584097
182,365,182,547,0.21551799774169922,45.66533931462459
188,377,188,565,0.22286391258239746,45.001134976618005
195,391,195,586,0.2322707176208496,44.2425491882625
202,405,202,607,0.2408139705657959,43.49633609495163
208,417,208,625,0.2482891082763672,42.86208948378135
215,431,215,646,0.25704097747802734,42.12520450817465
222,445,222,667,0.2655768394470215,41.38954354363432
229,459,229,688,0.27443885803222656,40.65323818727302
235,471,235,706,0.28116297721862793,40.02031819670037
242,485,242,727,0.2887568473815918,39.2786870518255
249,499,249,748,0.2966759204864502,38.53332037409382
256,513,256,769,0.30486488342285156,37.78563492192961
262,525,262,787,0.3119380474090576,37.14539769593989
269,539,269,808,0.3208029270172119,36.40299364617749
276,553,276,829,0.33077502250671387,35.66911733455731
282,565,282,847,0.33883070945739746,35.04861649648842
289,579,289,868,0.3465709686279297,34.33517557985215
296,593,296,889,0.3541378974914551,33.63250644917821
303,607,303,910,0.36156702041625977,32.939811044314865
309,619,309,928,0.36805200576782227,32.35371008696575
316,633,316,949,0.3757157325744629,31.678948806985318
323,647,323,970,0.3832120895385742,31.014084959764887
330,661,330,991,0.39032602310180664,30.358875431820024
336,673,336,1009,0.39616990089416504,29.8044238340442
343,687,343,1030,0.4029860496520996,29.165267235209512
350,701,350,1051,0.4098937511444092,28.534103425470676
356,713,356,1069,0.41562986373901367,27.99963246411062
363,727,363,1090,0.4224729537963867,27.384228608230615
370,741,370,1111,0.4296739101409912,26.77819890737328
377,755,377,1132,0.4367978572845459,26.181895294742844
383,767,383,1150,0.44255685806274414,25.678499301055353
390,781,390,1171,0.4494028091430664,25.099967548544782
397,795,397,1192,0.45648884773254395,24.530564136124667
404,809,404,1213,0.46324777603149414,23.970014281525437
410,821,410,1231,0.4689500331878662,23.49639410504551
417,835,417,1252,0.4759397506713867,22.951552706779694
424,849,424,1273,0.48305487632751465,22.414652347854826
430,861,430,1291,0.4890298843383789,21.96046758489115
437,875,437,1312,0.49574708938598633,21.437310512274507
444,889,444,1333,0.5026679039001465,20.92120623908386
451,903,451,1354,0.5095758438110352,20.412083209952243
457,915,457,1372,0.5153779983520508,19.981251411032872
464,929,464,1393,0.5222017765045166,19.48512240123273
471,943,471,1414,0.5291588306427002,18.996327111850178
478,957,478,1435,0.536125898361206,18.51486899101519
484,969,484,1453,0.5419950485229492,18.107860215944584
491,983,491,1474,0.5486741065979004,17.639705741797115
498,997,498,1495,0.5554580688476562,17.178797089765794
504,1009,504,1513,0.5613298416137695,16.789474965864656
511,1023,511,1534,0.5680367946624756,16.341862533067797
518,1037,518,1555,0.5749790668487549,15.901201822247913
525,1051,525,1576,0.5836780071258545,15.467348692518499
531,1063,531,1594,0.5897858142852783,15.100825477237777
538,1077,538,1615,0.5967748165130615,14.679427221110814
545,1091,545,1636,0.6040699481964111,14.264706183517205
552,1105,552,1657,0.6110978126525879,13.856636789370441
558,1117,558,1675,0.6171388626098633,13.512124176411703
565,1131,565,1696,0.624600887298584,13.116298502528252
572,1145,572,1717,0.6318938732147217,12.727053828106023
578,1157,578,1735,0.6381168365478516,12.398700963227498
585,1171,585,1756,0.6451678276062012,12.021882830427671
592,1185,592,1777,0.6524348258972168,11.65191153299395
599,1199,599,1798,0.6598179340362549,11.28886233424032
605,1211,605,1816,0.6659750938415527,10.983202551963359
612,1225,612,1837,0.6730499267578125,10.63301846025854
619,1239,619,1858,0.6803650856018066,10.289684190610615
625,1251,625,1876,0.6866309642791748,10.00078570080916
632,1265,632,1897,0.6937949657440186,9.669942977327764
639,1279,639,1918,0.7007298469543457,9.34569966113429
646,1293,646,1939,0.7078249454498291,9.027983471360585
652,1305,652,1957,0.7138957977294922,8.760816718877663
659,1319,659,1978,0.720923900604248,8.455136229150867
666,1333,666,1999,0.7283380031585693,8.155955260663859
673,1347,673,2020,0.7355568408966064,7.863316018115825
679,1359,679,2038,0.7417027950286865,7.617721170625032
686,1373,686,2059,0.748701810836792,7.337330548253249
693,1387,693,2080,0.7558679580688477,7.063556065419107
699,1399,699,2098,0.7620139122009277,6.83414962201789
706,1413,706,2119,0.7690958976745605,6.572616662409814
713,1427,713,2140,0.776425838470459,6.317616476460671
720,1441,720,2161,0.7838699817657471,6.069082552529039
726,1453,726,2179,0.7900009155273438,5.861136310380061
733,1467,733,2200,0.7969248294830322,5.624378830025307
740,1481,740,2221,0.8039870262145996,5.393828971483572
747,1495,747,2242,0.8110380172729492,5.169406383814021
753,1507,753,2260,0.8171539306640625,4.981874160683674
760,1521,760,2281,0.8243019580841064,4.76868269622787
767,1535,767,2302,0.831881046295166,4.561486880269854
773,1547,773,2320,0.8381249904632568,4.3886399735954456
780,1561,780,2341,0.8452448844909668,4.192495035150841
787,1575,787,2362,0.8524050712585449,4.002237597218823
794,1589,794,2383,0.8595988750457764,3.817801270280256
800,1601,800,2401,0.8657159805297852,3.664281085762127
807,1615,807,2422,0.8731729984283447,3.4904132930605556
814,1629,814,2443,0.8807859420776367,3.3220818650618185
821,1643,821,2464,0.8883929252624512,3.1591768633614947
827,1655,827,2482,0.8944289684295654,3.023786992698547
834,1669,834,2503,0.901663064956665,2.8707062638105754
841,1683,841,2524,0.9089059829711914,2.7228053824909466
847,1695,847,2542,0.9149179458618164,2.6001068027339898
854,1709,854,2563,0.9220719337463379,2.461654882073958
861,1723,861,2584,0.9297358989715576,2.328195759421533
868,1737,868,2605,0.9370548725128174,2.199653147041886
874,1749,874,2623,0.9430508613586426,2.0933224203929512
881,1763,881,2644,0.9500858783721924,1.9736785233990304
888,1777,888,2665,0.9572470188140869,1.8586910133519723
895,1791,895,2686,0.964378833770752,1.7482638740259517
901,1803,901,2704,0.9704709053039551,1.6571709646921136
908,1817,908,2725,0.9779930114746094,1.5549686120125443
915,1831,915,2746,0.9855659008026123,1.4570688506368015
921,1843,921,2764,0.991786003112793,1.3765122807221815
928,1857,928,2785,0.9990668296813965,1.286364800185197
935,1871,935,2806,1.0062029361724854,1.2002529046000063
942,1885,942,2827,1.013481855392456,1.1180699083614627
948,1897,948,2845,1.0195777416229248,1.0506689451440252
955,1911,955,2866,1.0271077156066895,0.9754804432019455
962,1925,962,2887,1.0346460342407227,0.9038931211264298
969,1939,969,2908,1.0418260097503662,0.8357965957684428
975,1951,975,2926,1.047834873199463,0.780129479672155
982,1965,982,2947,1.0552020072937012,0.7182560416480328
989,1979,989,2968,1.062134027481079,0.6596148376531801
995,1991,995,2986,1.0681829452514648,0.611869597013424
1002,2005,1002,3007,1.0756618976593018,0.5590457038110799
1009,2019,1009,3028,1.0851011276245117,0.5092565690873698
1016,2033,1016,3049,1.0934100151062012,0.4624274808484188
1022,2045,1022,3067,1.0996589660644531,0.42458159468003487
1029,2059,1029,3088,1.1068379878997803,0.3830238808086506
1036,2073,1036,3109,1.1138911247253418,0.3441708306613691
1042,2085,1042,3127,1.1200687885284424,0.3129471096389125
1049,2099,1049,3148,1.1274988651275635,0.27885953081920434
1056,2113,1056,3169,1.1346559524536133,0.2472029825167965
1063,2127,1063,3190,1.1420018672943115,0.21788721670998257
1069,2139,1069,3208,1.148155927658081,0.19455576980601563
1076,2153,1076,3229,1.1553409099578857,0.16935405576009543
1083,2167,1083,3250,1.1625280380249023,0.1462417102040945
1090,2181,1090,3271,1.1696269512176514,0.12512977737208075
1096,2193,1096,3289,1.1761200428009033,0.10855976274660861
1103,2207,1103,3310,1.1835057735443115,0.09093549237059051
1110,2221,1110,3331,1.1906428337097168,0.07507941753738123
1116,2233,1116,3349,1.1967859268188477,0.06284676637653774
1123,2247,1123,3370,1.203887939453125,0.050110279903378796
1130,2261,1130,3391,1.2109549045562744,0.0389778551514155
1137,2275,1137,3412,1.217998743057251,0.029397919748475942
1143,2287,1143,3430,1.224323034286499,0.022379646674380638
1150,2301,1150,3451,1.2319560050964355,0.015527599217648458
1157,2315,1157,3472,1.2393360137939453,0.01004705638536052
1164,2329,1164,3493,1.2464048862457275,0.0058625435859767094
1170,2341,1170,3511,1.2526118755340576,0.0032490617454641324
1177,2355,1177,3532,1.2600409984588623,0.0012693949472577515
1184,2369,1184,3553,1.2673008441925049,0.00037476265515579144
1190,2381,1190,3571,1.2751009464263916,0.0004225870362688511
1197,2395,1197,3592,1.283538818359375,0.0013760386623289378
1204,2409,1204,3613,1.2908217906951904,0.003242479096570605
1211,2423,1211,3634,1.2978079319000244,0.005967132288333232
1217,2435,1217,3652,1.3041260242462158,0.008944692467480309
1224,2449,1224,3673,1.311302900314331,0.013120831767423624
1231,2463,1231,3694,1.3182578086853027,0.018004869596097706
1238,2477,1238,3715,1.3256456851959229,0.023549315761329126
1244,2489,1244,3733,1.332258939743042,0.02879440748210982
1251,2503,1251,3754,1.3395969867706299,0.03545338799506226
1258,2517,1258,3775,1.3466298580169678,0.04265797144421413
1264,2529,1264,3793,1.35274076461792,0.04923951710952679
1271,2543,1271,3814,1.3598778247833252,0.05735789105767708
1278,2557,1278,3835,1.366905927658081,0.0659110867252366
1285,2571,1285,3856,1.3743958473205566,0.07485591620024934
1291,2583,1291,3874,1.3813297748565674,0.08280096652356406
1298,2597,1298,3895,1.3888518810272217,0.09235573423552523
1305,2611,1305,3916,1.3960049152374268,0.1021780827186376
1312,2625,1312,3937,1.4032268524169922,0.11222896030074025
1318,2637,1318,3955,1.4092659950256348,0.12099845669240494
1325,2651,1325,3976,1.4163079261779785,0.13137967665977612
1332,2665,1332,3997,1.4235658645629883,0.14189151912341913
1338,2677,1338,4015,1.4302940368652344,0.15098158465900724
1345,2691,1345,4036,1.438391923904419,0.16165282907525125
1352,2705,1352,4057,1.445694923400879,0.1723679604518793
1359,2719,1359,4078,1.4530251026153564,0.18310094540447608
1365,2731,1365,4096,1.4592549800872803,0.19229746327323483
1372,2745,1372,4117,1.4664487838745117,0.20300511693710632
1379,2759,1379,4138,1.4737648963928223,0.2136717202275804
1385,2771,1385,4156,1.4804737567901611,0.22276786578720476
1392,2785,1392,4177,1.4879648685455322,0.23330849933267928
1399,2799,1399,4198,1.495116949081421,0.24375239028108808
1406,2813,1406,4219,1.5022118091583252,0.25407784051287763
1412,2825,1412,4237,1.5083320140838623,0.26281740329102377
1419,2839,1419,4258,1.5154109001159668,0.2728657483397683
1426,2853,1426,4279,1.5225458145141602,0.2827365650825868
1433,2867,1433,4300,1.5304248332977295,0.2924125358672427
1439,2879,1439,4318,1.536942720413208,0.3005393299010848
1446,2893,1446,4339,1.5439369678497314,0.30981317412613407
1453,2907,1453,4360,1.5510878562927246,0.31885062993364954
1459,2919,1459,4378,1.5572559833526611,0.32639881892964695
1466,2933,1466,4399,1.5643420219421387,0.3349624899410628
1473,2947,1473,4420,1.5713598728179932,0.34325354068857905
1480,2961,1480,4441,1.579150915145874,0.35126123528164044
1486,2973,1486,4459,1.5855648517608643,0.3578924883051968
1493,2987,1493,4480,1.592736005783081,0.36535102450454815
1500,3001,1500,4501,1.5998280048370361,0.3725043453996477
1507,3015,1507,4522,1.607011079788208,0.37934716618701714
1513,3027,1513,4540,1.6132228374481201,0.3849616623855354
1520,3041,1520,4561,1.620668888092041,0.3912152098550905
1527,3055,1527,4582,1.6284308433532715,0.39714482691874764
1533,3067,1533,4600,1.6350829601287842,0.40196609382269344
1540,3081,1540,4621,1.6425888538360596,0.4072822996145078
1547,3095,1547,4642,1.6501109600067139,0.412262419442186
1554,3109,1554,4663,1.6576550006866455,0.4169029333116896
1560,3121,1560,4681,1.664160966873169,0.42060783455644923
1567,3135,1567,4702,1.6714911460876465,0.42460960867617814
1574,3149,1574,4723,1.6798100471496582,0.428263801011326
1581,3163,1581,4744,1.6879990100860596,0.4315685353677736
1587,3175,1587,4762,1.694502830505371,0.4341222023812179
1594,3189,1594,4783,1.7019739151000977,0.4367759741805912
1601,3203,1601,4804,1.7094647884368896,0.4390802291294449
1607,3215,1607,4822,1.715775966644287,0.4407787074156886
1614,3229,1614,4843,1.723397970199585,0.4424401353116991
1621,3243,1621,4864,1.7312419414520264,0.4437600139621054
1628,3257,1628,4885,1.739001750946045,0.44474187051741865
1634,3269,1634,4903,1.745412826538086,0.4453170919034619
1641,3283,1641,4924,1.7531960010528564,0.44568051210546855
1648,3297,1648,4945,1.761136770248413,0.4457160086137719
1655,3311,1655,4966,1.768779993057251,0.44542740836720895
1661,3323,1661,4984,1.775115966796875,0.4449252588337913
1668,3337,1668,5005,1.7829010486602783,0.4440462578526194
1675,3351,1675,5026,1.7900879383087158,0.44285634085724723
1681,3363,1681,5044,1.796072006225586,0.44159304425420487
1688,3377,1688,5065,1.8031589984893799,0.43984035478172245
1695,3391,1695,5086,1.810241937637329,0.43779315797655727
1702,3405,1702,5107,1.8174619674682617,0.4354578358652361
1708,3417,1708,5125,1.8238310813903809,0.4332318523822778
1715,3431,1715,5146,1.8315799236297607,0.43037928139210635
1722,3445,1722,5167,1.8392009735107422,0.4272580977343523
1729,3459,1729,5188,1.8464488983154297,0.4238752859426995
1735,3471,1735,5206,1.852691888809204,0.4207727688359455
1742,3485,1742,5227,1.8602428436279297,0.4169225243639403
1749,3499,1749,5248,1.8674230575561523,0.41283063439004763
1755,3511,1755,5266,1.8739609718322754,0.4091365380534171
1762,3525,1762,5287,1.8817028999328613,0.404615750131029
1769,3539,1769,5308,1.8893508911132812,0.3998756286380285
1776,3553,1776,5329,1.8965251445770264,0.39492497775734137
1782,3565,1782,5347,1.902590036392212,0.39052096256102686
1789,3579,1789,5368,1.909881830215454,0.3852038765646739
1796,3593,1796,5389,1.9169847965240479,0.37970288928704576
1802,3605,1802,5407,1.9232048988342285,0.37484840587592316
1809,3619,1809,5428,1.930804967880249,0.36903028051847286
1816,3633,1816,5449,1.9381167888641357,0.36305416007098756
1823,3647,1823,5470,1.945328950881958,0.35692879485156936
1829,3659,1829,5488,1.9514269828796387,0.35156627667140583
1836,3673,1836,5509,1.958622932434082,0.3451867516080256
1843,3687,1843,5530,1.9659268856048584,0.33868271089568225
1850,3701,1850,5551,1.9731528759002686,0.3320627558882734
1856,3713,1856,5569,1.9796478748321533,0.3263027535213041
1863,3727,1863,5590,1.9870216846466064,0.319490303770408
1870,3741,1870,5611,1.994196891784668,0.3125865594188326
1876,3753,1876,5629,2.0001578330993652,0.30660308823075866
1883,3767,1883,5650,2.007290840148926,0.2995533689623926
1890,3781,1890,5671,2.0143489837646484,0.2924380872899519
1897,3795,1897,5692,2.0215160846710205,0.2852665288735352
1903,3807,1903,5710,2.027956962585449,0.27908171971773754
1910,3821,1910,5731,2.0355329513549805,0.2718301566911805
1917,3835,1917,5752,2.0427017211914062,0.26454841558506814
1924,3849,1924,5773,2.049889087677002,0.25724525137172805
1930,3861,1930,5791,2.0559589862823486,0.25097483965430456
1937,3875,1937,5812,2.0629889965057373,0.2436544911375904
1944,3889,1944,5833,2.0699949264526367,0.23633680552723035
1950,3901,1950,5851,2.0764400959014893,0.23007281691843673
1957,3915,1957,5872,2.084192991256714,0.22278159158622657
1964,3929,1964,5893,2.0914299488067627,0.21551578259573034
1971,3943,1971,5914,2.0984699726104736,0.20828282446734647
1977,3955,1977,5932,2.1045339107513428,0.20211470202082182
1984,3969,1984,5953,2.111680030822754,0.194961473750368
1991,3983,1991,5974,2.1187970638275146,0.1878609000328879
1998,3997,1998,5995,2.1279358863830566,0.1808197176063686
2004,4009,2004,6013,2.1347768306732178,0.17483683835155261
2011,4023,2011,6034,2.141869068145752,0.16792405095804952
2018,4037,2018,6055,2.1489977836608887,0.16109027085849448
2024,4049,2024,6073,2.1551380157470703,0.15530085905356827
2031,4063,2031,6094,2.1622750759124756,0.14863200816284916
2038,4077,2038,6115,2.1694228649139404,0.14206145680884674
2045,4091,2045,6136,2.1771469116210938,0.1355955152818069
2051,4103,2051,6154,2.1837990283966064,0.13014109519849626
2058,4117,2058,6175,2.1910629272460938,0.12388508023809663
2065,4131,2065,6196,2.1982977390289307,0.11774987899161715
2072,4145,2072,6217,2.2055540084838867,0.11174042690231545
2078,4157,2078,6235,2.211664915084839,0.106692977630928
2085,4171,2085,6256,2.218660831451416,0.10092866290199254
2092,4185,2092,6277,2.2261340618133545,0.09530180231945451
2098,4197,2098,6295,2.2325758934020996,0.0905907324013242
2105,4211,2105,6316,2.239896059036255,0.08522786689252371
2112,4225,2112,6337,2.2470388412475586,0.08001151256667072
2119,4239,2119,6358,2.25426983833313,0.07494465146191942
2125,4251,2125,6376,2.2604379653930664,0.07072288591155029
2132,4265,2132,6397,2.2675719261169434,0.06594162752674038
2139,4279,2139,6418,2.2750298976898193,0.06131843517709967
2146,4293,2146,6439,2.283108949661255,0.05685619789630891
2152,4305,2152,6457,2.291167974472046,0.05316159600135961
2159,4319,2159,6478,2.2986271381378174,0.04900531180453527
2166,4333,2166,6499,2.305753707885742,0.045017105085776166
2172,4345,2172,6517,2.312203884124756,0.04173390990547432
2179,4359,2179,6538,2.3196370601654053,0.038062782508973214
2186,4373,2186,6559,2.3276407718658447,0.03456439239619158
2193,4387,2193,6580,2.3355777263641357,0.03123961006645004
2199,4399,2199,6598,2.342072010040283,0.02852829921346256
2206,4413,2206,6619,2.3495659828186035,0.02552667333361569
2213,4427,2213,6640,2.3571767807006836,0.02269863667845584
2219,4439,2219,6658,2.3635828495025635,0.020412195246422016
2226,4453,2226,6679,2.371532917022705,0.01790432149755361
2233,4467,2233,6700,2.379661798477173,0.015567293354820322
2240,4481,2240,6721,2.3881449699401855,0.013399933601021985
2246,4493,2246,6739,2.394460916519165,0.011676348048695218
2253,4507,2253,6760,2.4018988609313965,0.009820980896165565
2260,4521,2260,6781,2.409398078918457,0.008131941531132725
2267,4535,2267,6802,2.416727066040039,0.006608005714269893
2273,4547,2273,6820,2.423342704772949,0.005432176660178811
2280,4561,2280,6841,2.4316248893737793,0.004211196576534348
2287,4575,2287,6862,2.439290761947632,0.0031510242092736007
2293,4587,2293,6880,2.445773124694824,0.0023688243903734474
2300,4601,2300,6901,2.4535129070281982,0.0016018869647496103
2307,4615,2307,6922,2.4613020420074463,0.0009893391028299447
2314,4629,2314,6943,2.4687459468841553,0.0005282736865410698
2320,4641,2320,6961,2.4763619899749756,0.00025118601774920535
2327,4655,2327,6982,2.4844439029693604,6.258705775508133e-05
2334,4669,2334,7003,2.4917848110198975,1.5430387520609656e-05
2341,4683,2341,7024,2.4988298416137695,0.00010579604941085563
2347,4695,2347,7042,2.5050408840179443,0.00028967623131848086
2354,4709,2354,7063,2.5123329162597656,0.0006248066156331333
2361,4723,2361,7084,2.519489049911499,0.0010859965024110352
2367,4735,2367,7102,2.5257949829101562,0.0015786064852818527
2374,4749,2374,7123,2.5334529876708984,0.0022633103794760245
2381,4763,2381,7144,2.5407228469848633,0.003062648032141624
2388,4777,2388,7165,2.5478599071502686,0.003972563986849309
2394,4789,2394,7183,2.554028034210205,0.004837378629304112
2401,4803,2401,7204,2.561173915863037,0.00594164365963934
2408,4817,2408,7225,2.5688140392303467,0.007144455546722384
2415,4831,2415,7246,2.5766139030456543,0.008441399083494616
2421,4843,2421,7264,2.5835649967193604,0.009624548161241364
2428,4857,2428,7285,2.590902090072632,0.0110841641441084
2435,4871,2435,7306,2.5980679988861084,0.012624598939964926
2441,4883,2441,7324,2.6041719913482666,0.014005592632202024
2448,4897,2448,7345,2.6112377643585205,0.01568307966078919
2455,4911,2455,7366,2.6183128356933594,0.017427209280981515
2462,4925,2462,7387,2.625688076019287,0.019232931609053594
2468,4937,2468,7405,2.632481098175049,0.02082589169685889
2475,4951,2475,7426,2.6399760246276855,0.02273263781114565
2482,4965,2482,7447,2.6470448970794678,0.02468665277638138
2489,4979,2489,7468,2.6542088985443115,0.026683016179390506
2495,4991,2495,7486,2.6603620052337646,0.028424209341437745
2502,5005,2502,7507,2.667393922805786,0.030486397029903856
2509,5019,2509,7528,2.674860954284668,0.03257725970001957
2515,5031,2515,7546,2.6814358234405518,0.03438872798687953
2522,5045,2522,7567,2.6888508796691895,0.03652056828093464
2529,5059,2529,7588,2.6960740089416504,0.03866796467355016
2536,5073,2536,7609,2.7032909393310547,0.0408264062912167
2542,5085,2542,7627,2.7092747688293457,0.042681883914383434
2549,5099,2549,7648,2.7163939476013184,0.044848926134704925
2556,5113,2556,7669,2.7238378524780273,0.04701421101606229
2563,5127,2563,7690,2.7313599586486816,0.049173301639143574
2569,5139,2569,7708,2.737764835357666,0.051015695598607635
2576,5153,2576,7729,2.7448489665985107,0.05315171131860552
2583,5167,2583,7750,2.7519538402557373,0.05526923685215479
2589,5179,2589,7768,2.7580769062042236,0.05706643503719988
2596,5193,2596,7789,2.76515793800354,0.05913886423286385
2603,5207,2603,7810,2.772359848022461,0.061181478860362404
2610,5221,2610,7831,2.7797298431396484,0.0631905971309834
2616,5233,2616,7849,2.78597092628479,0.06488335381516208
2623,5247,2623,7870,2.7931110858917236,0.06682098699911876
2630,5261,2630,7891,2.800520896911621,0.06871537588597221
2636,5273,2636,7909,2.806705951690674,0.07030231004091547
2643,5287,2643,7930,2.8136887550354004,0.07210804971862217
2650,5301,2650,7951,2.820828914642334,0.07386176246552623
2657,5315,2657,7972,2.8280839920043945,0.07556058515763198
2663,5327,2663,7990,2.8343539237976074,0.07697095110256669
2670,5341,2670,8011,2.84161376953125,0.07856067610396167
2677,5355,2677,8032,2.8487799167633057,0.08008807664043616
2684,5369,2684,8053,2.85591197013855,0.08155086445447068
2690,5381,2690,8071,2.8620479106903076,0.08275165233669668
2697,5395,2697,8092,2.869036912918091,0.08408898245579621
2704,5409,2704,8113,2.876585006713867,0.08535613190258573
2710,5421,2710,8131,2.8829569816589355,0.08638515499808364
2717,5435,2717,8152,2.890084743499756,0.08751771892946181
2724,5449,2724,8173,2.8973379135131836,0.08857575698198161
2731,5463,2731,8194,2.904461145401001,0.08955797140549748
2737,5475,2737,8212,2.910651922225952,0.09033861247905861
2744,5489,2744,8233,2.9176671504974365,0.09117692704251112
2751,5503,2751,8254,2.9248907566070557,0.091936304234423
2758,5517,2758,8275,2.9323649406433105,0.09261589532206926
2764,5529,2764,8293,2.938720941543579,0.09313436751017434
2771,5543,2771,8314,2.9458019733428955,0.0936640719675097
2778,5557,2778,8335,2.953075885772705,0.09411247666855616
2784,5569,2784,8353,2.959152936935425,0.09443198583892354
2791,5583,2791,8374,2.9662578105926514,0.09472911989689692
2798,5597,2798,8395,2.9735779762268066,0.09494500346261248
2805,5611,2805,8416,2.9813120365142822,0.0950800084834782
2811,5623,2811,8434,2.9878180027008057,0.09513174905532651
2818,5637,2818,8455,2.994929790496826,0.09511804348926489
2825,5651,2825,8476,3.0021581649780273,0.09502528385110054
2832,5665,2832,8497,3.0091938972473145,0.09485430222071045
2838,5677,2838,8515,3.0154669284820557,0.09464617198614178
2845,5691,2845,8536,3.0226707458496094,0.09433237001996986
2852,5705,2852,8557,3.0305731296539307,0.09394310438642606
2858,5717,2858,8575,3.037202835083008,0.09355021644898898
2865,5731,2865,8596,3.044234037399292,0.09302378513905296
2872,5745,2872,8617,3.051265001296997,0.09242526815535257
2879,5759,2879,8638,3.0591509342193604,0.09175604620781996
2885,5771,2885,8656,3.0655128955841064,0.09112728893148869
2892,5785,2892,8677,3.0728588104248047,0.09033084900636368
2899,5799,2899,8698,3.0805158615112305,0.08946835402491615
2906,5813,2906,8719,3.0882108211517334,0.08854168714742627
2912,5825,2912,8737,3.0944318771362305,0.08769784426351634
2919,5839,2919,8758,3.101464033126831,0.08665741224160683
2926,5853,2926,8779,3.1086997985839844,0.0855588282406643
2932,5865,2932,8797,3.115341901779175,0.08457262765034557
2939,5879,2939,8818,3.123198986053467,0.08337214200605558
2946,5893,2946,8839,3.130788803100586,0.08212015759579572
2953,5907,2953,8860,3.1383578777313232,0.08081906672634886
2959,5919,2959,8878,3.144526720046997,0.07966658001123506
2966,5933,2966,8899,3.151798963546753,0.07828065651483485
2973,5947,2973,8920,3.158947706222534,0.07685247877748225
2979,5959,2979,8938,3.1650469303131104,0.07559651422718616
2986,5973,2986,8959,3.1720540523529053,0.07409624037916274
2993,5987,2993,8980,3.1799910068511963,0.07256061317082185
3000,6001,3000,9001,3.1874399185180664,0.07099210486705942
3006,6013,3006,9019,3.1934568881988525,0.06962340836412295
3013,6027,3013,9040,3.200511932373047,0.0680005674506674
3020,6041,3020,9061,3.2077560424804688,0.06635219974145912
3027,6055,3027,9082,3.214991807937622,0.06468098447817283
3033,6067,3033,9100,3.221176862716675,0.06323239043376816
3040,6081,3040,9121,3.229592800140381,0.06152597810375937
3047,6095,3047,9142,3.237541913986206,0.05980453441077316
3053,6107,3053,9160,3.2440378665924072,0.05831911625762132
3060,6121,3060,9181,3.251640796661377,0.05657696514992949
3067,6135,3067,9202,3.2591748237609863,0.054827458948693675
3074,6149,3074,9223,3.267021894454956,0.05307317187157423
3080,6161,3080,9241,3.2741029262542725,0.051567591317052575
3087,6175,3087,9262,3.283331871032715,0.04981101417615719
3094,6189,3094,9283,3.2921218872070312,0.048056632524662746
3101,6203,3101,9304,3.2998249530792236,0.046306779284577715
3107,6215,3107,9322,3.3072240352630615,0.044812250704694634
3114,6229,3114,9343,3.3150908946990967,0.04307688053677339
3121,6243,3121,9364,3.3230090141296387,0.041352540251409664
3127,6255,3127,9382,3.330656051635742,0.039885014653577855
3134,6269,3134,9403,3.3384499549865723,0.03818710229768385
3141,6283,3141,9424,3.3459620475769043,0.036506591668171495
3148,6297,3148,9445,3.353379726409912,0.0348456693712933
3154,6309,3154,9463,3.3600358963012695,0.0334392398503951
3161,6323,3161,9484,3.367777109146118,0.03182034397013922
3168,6337,3168,9505,3.3828659057617188,0.030227001312027824
3175,6351,3175,9526,3.391004800796509,0.028661152375548227
3181,6363,3181,9544,3.3974478244781494,0.027342279078538922
3188,6377,3188,9565,3.40516996383667,0.025832302126900686
3195,6391,3195,9586,3.413655996322632,0.024354809167448366
3201,6403,3201,9604,3.4207699298858643,0.023115416213158824
3208,6417,3208,9625,3.429743766784668,0.021702281215652874
3215,6431,3215,9646,3.4387898445129395,0.020325803289551914
3222,6445,3222,9667,3.446729898452759,0.01898728365745228
3228,6457,3228,9685,3.4535417556762695,0.017871131111064642
3235,6471,3235,9706,3.4616289138793945,0.016606340395810548
3242,6485,3242,9727,3.4691238403320312,0.01538289056497888
3249,6499,3249,9748,3.4774861335754395,0.014201863291418704
3255,6511,3255,9766,3.4842917919158936,0.013224098903833692
3262,6525,3262,9787,3.4916679859161377,0.012124533007181526
3269,6539,3269,9808,3.498973846435547,0.01107014975571019
3275,6551,3275,9826,3.505326747894287,0.010202978959569009
3282,6565,3282,9847,3.5127298831939697,0.009234613747366893
3289,6579,3289,9868,3.5202088356018066,0.008313523825904667
3296,6593,3296,9889,3.527817964553833,0.007440246127089267
3302,6605,3302,9907,3.5345840454101562,0.006730106861141394
3309,6619,3309,9928,3.542232036590576,0.005946690821815537
3316,6633,3316,9949,3.5496199131011963,0.0052120558503929715
3323,6647,3323,9970,3.5572218894958496,0.0045263645648674355
3329,6659,3329,9988,3.5635321140289307,0.003977651900527235
3336,6673,3336,10009,3.570823907852173,0.0033830351204642284
3343,6687,3343,10030,3.578681707382202,0.0028374379148772277
3349,6699,3349,10048,3.585000991821289,0.002408733825973286
3356,6713,3356,10069,3.5924458503723145,0.0019538992030447844
3363,6727,3363,10090,3.6001389026641846,0.001547687697893707
3370,6741,3370,10111,3.6075119972229004,0.001189849109437091
3376,6753,3376,10129,3.613830804824829,0.000921393845487728
3383,6767,3383,10150,3.6212427616119385,0.000652499165653353
3390,6781,3390,10171,3.6292059421539307,0.00043088166398774774
3396,6793,3396,10189,3.635877847671509,0.00027815089606519905
3403,6807,3403,10210,3.643286943435669,0.00014285866609498044
3410,6821,3410,10231,3.650819778442383,5.310701794769557e-05
3417,6835,3417,10252,3.658521890640259,8.137844247357862e-06
3423,6847,3423,10270,3.664918899536133,4.6106458739814116e-06
3430,6861,3430,10291,3.672466993331909,4.0567501173427445e-05
3437,6875,3437,10312,3.6808598041534424,0.00011878734528636414
3444,6889,3444,10333,3.688978910446167,0.000238290352626791
3450,6901,3450,10351,3.695481777191162,0.00037280842116160784
3457,6915,3457,10372,3.7030510902404785,0.0005662527520371441
3464,6929,3464,10393,3.7104477882385254,0.0007979848948025392
3470,6941,3470,10411,3.7168357372283936,0.001026249237384036
3477,6955,3477,10432,3.724514961242676,0.0013261332446745655
3484,6969,3484,10453,3.732408046722412,0.0016610708609050562
3491,6983,3491,10474,3.740032911300659,0.002029871126183025
3497,6995,3497,10492,3.74635910987854,0.0023720090077858913
3504,7009,3504,10513,3.753955125808716,0.002800414410671692
3511,7023,3511,10534,3.7614259719848633,0.0032590745288416656
3518,7037,3518,10555,3.768795967102051,0.0037466476608187804
3524,7049,3524,10573,3.7756128311157227,0.004186532912058283
3531,7063,3531,10594,3.7833521366119385,0.004724104842921406
3538,7077,3538,10615,3.791207790374756,0.005286543522743159
3544,7089,3544,10633,3.797576904296875,0.00578730839902164
3551,7103,3551,10654,3.8054420948028564,0.0063920016413021585
3558,7117,3558,10675,3.8134069442749023,0.00701730641173981
3565,7131,3565,10696,3.821230888366699,0.007661718424174069
3571,7143,3571,10714,3.828760862350464,0.008228142202142408
3578,7157,3578,10735,3.837127923965454,0.008904066913601127
3585,7171,3585,10756,3.8449690341949463,0.009594840894010304
3592,7185,3592,10777,3.8526289463043213,0.010298996905817148
3598,7197,3598,10795,3.8604719638824463,0.010912106092177964
3605,7211,3605,10816,3.869119882583618,0.011637256649123628
3612,7225,3612,10837,3.8782129287719727,0.012371645048460778
3618,7237,3618,10855,3.8856430053710938,0.013007377214989901
3625,7251,3625,10876,3.8934919834136963,0.013755082108332317
3632,7265,3632,10897,3.901279926300049,0.014507882665725447
3639,7279,3639,10918,3.909233808517456,0.015264321820723126
3645,7291,3645,10936,3.9164528846740723,0.015914489902570494
3652,7305,3652,10957,3.924445867538452,0.01667382625339542
3659,7319,3659,10978,3.931968927383423,0.017432661697739604
3666,7333,3666,10999,3.939687967300415,0.018189578247870486
3672,7345,3672,11017,3.945917844772339,0.018835782546261726
3679,7359,3679,11038,3.9530739784240723,0.01958547601736882
3686,7373,3686,11059,3.960441827774048,0.020329377690700312
3692,7385,3692,11077,3.966791868209839,0.020961427080578687
3699,7399,3699,11098,3.97428297996521,0.021691209830237312
3706,7413,3706,11119,3.9818010330200195,0.022411653107042184
3713,7427,3713,11140,3.989137887954712,0.023121587823766276
3719,7439,3719,11158,3.9952640533447266,0.023720876096945176
3726,7453,3726,11179,4.0025410652160645,0.02440829687668611
3733,7467,3733,11200,4.009848117828369,0.02508202781075397
3740,7481,3740,11221,4.017202854156494,0.025741001788560425
3746,7493,3746,11239,4.023971796035767,0.02629329935837177
3753,7507,3753,11260,4.0319437980651855,0.02692211757471341
3760,7521,3760,11281,4.039638042449951,0.027533267969829467
3766,7533,3766,11299,4.045874834060669,0.028042321811426518
3773,7547,3773,11320,4.053358793258667,0.028618149618750977
3780,7561,3780,11341,4.060913801193237,0.02917368458099645
3787,7575,3787,11362,4.068557024002075,0.02970809914563688
3793,7587,3793,11380,4.075085878372192,0.030148770868663632
3800,7601,3800,11401,4.08306097984314,0.030641952329119704
3807,7615,3807,11422,4.090616703033447,0.031111952379887953
3813,7627,3813,11440,4.096826791763306,0.0314958919215087
3820,7641,3820,11461,4.104413986206055,0.03192125029408999
3827,7655,3827,11482,4.112018823623657,0.032321806783215834
3834,7669,3834,11503,4.119624853134155,0.032697084705091584
3840,7681,3840,11521,4.126416921615601,0.032998299837800005
3847,7695,3847,11542,4.134432077407837,0.033325501176364014
3854,7709,3854,11563,4.1420509815216064,0.033626271455545975
3861,7723,3861,11584,4.149708986282349,0.03390027329226086
3867,7735,3867,11602,4.156481027603149,0.0341135955760592
3874,7749,3874,11623,4.164358854293823,0.03433710697584047
3881,7763,3881,11644,4.172309875488281,0.0345330815143825
3887,7775,3887,11662,4.183315992355347,0.03467899686575038
3894,7789,3894,11683,4.191461801528931,0.034823361593566915
3901,7803,3901,11704,4.198925733566284,0.03493977334301235
3908,7817,3908,11725,4.20662784576416,0.03502818623837811
3914,7829,3914,11743,4.213223934173584,0.03508168969722192
3921,7843,3921,11764,4.220920085906982,0.03511817237483683
3928,7857,3928,11785,4.230967998504639,0.035126829785667724
3935,7871,3935,11806,4.238724946975708,0.035107824455621994
3941,7883,3941,11824,4.245000839233398,0.035069674262786066
3948,7897,3948,11845,4.2524309158325195,0.034999881623775764
3955,7911,3955,11866,4.260438919067383,0.034903129443819125
3961,7923,3961,11884,4.266932964324951,0.034798978247295054
3968,7937,3968,11905,4.274990081787109,0.03465301119376818
3975,7951,3975,11926,4.283168077468872,0.034481052295177506
3982,7965,3982,11947,4.29079794883728,0.034283489552876745
3988,7977,3988,11965,4.297098875045776,0.03409408418690418
3995,7991,3995,11986,4.304595947265625,0.033850089311954434
4002,8005,4002,12007,4.312211990356445,0.03358174764048272
4009,8019,4009,12028,4.3197550773620605,0.03328956016503071
4015,8031,4015,12046,4.326766729354858,0.03302054118353226
4022,8045,4022,12067,4.334517002105713,0.03268552577526407
4029,8059,4029,12088,4.341956853866577,0.032328307134889656
4035,8071,4035,12106,4.348197937011719,0.0320049412298431
4042,8085,4042,12127,4.355751991271973,0.031608247906660836
4049,8099,4049,12148,4.3633599281311035,0.03119131412177012
4056,8113,4056,12169,4.371043920516968,0.030754891122455774
4062,8125,4062,12187,4.3780837059021,0.03036589037469639
4069,8139,4069,12208,4.386244773864746,0.029895347676870188
4076,8153,4076,12229,4.39353084564209,0.02940758125339471
4083,8167,4083,12250,4.400959014892578,0.0289034093303826
4089,8179,4089,12268,4.407927989959717,0.028458829838427846
4096,8193,4096,12289,4.415513753890991,0.02792638355163035
4103,8207,4103,12310,4.423215866088867,0.027379902683946966
4109,8219,4109,12328,4.429859161376953,0.026900956909912566
4116,8233,4116,12349,4.437583923339844,0.026330647188729017
4123,8247,4123,12370,4.445044994354248,0.025748726858864757
4130,8261,4130,12391,4.453892946243286,0.025156065980468156
4136,8273,4136,12409,4.460469961166382,0.024640192928359284
4143,8287,4143,12430,4.467988967895508,0.02402994645012768
4150,8301,4150,12451,4.47583270072937,0.02341153266411311
4156,8313,4156,12469,4.482648134231567,0.022875668966094054
4163,8327,4163,12490,4.490492820739746,0.022244568639507634
4170,8341,4170,12511,4.497675895690918,0.0216079936768665
4177,8355,4177,12532,4.505144119262695,0.020966901098177004
4183,8367,4183,12550,4.5118248462677,0.02041452268304056
4190,8381,4190,12571,4.519531011581421,0.019767573644003278
4197,8395,4197,12592,4.527200937271118,0.01911882097556372
4204,8409,4204,12613,4.535107135772705,0.018469193065243417
4210,8421,4210,12631,4.541385889053345,0.017912364418407378
4217,8435,4217,12652,4.548768043518066,0.0172635178469136
4224,8449,4224,12673,4.556510925292969,0.01661635601544731
4230,8461,4230,12691,4.562947750091553,0.01606364178314834
4237,8475,4237,12712,4.570734024047852,0.015421888822174878
4244,8489,4244,12733,4.5786659717559814,0.014784251275955285
4251,8503,4251,12754,4.586443901062012,0.014151557155400951
4257,8515,4257,12772,4.592957973480225,0.013613803561725035
4264,8529,4264,12793,4.600560903549194,0.01299245683674144
4271,8543,4271,12814,4.608257055282593,0.012378371439467628
4278,8557,4278,12835,4.615714073181152,0.011772340792958857
4284,8569,4284,12853,4.622365951538086,0.011259889359962472
4291,8583,4291,12874,4.630843877792358,0.010670878231962888
4298,8597,4298,12895,4.6385416984558105,0.010092109960851303
4304,8609,4304,12913,4.644848823547363,0.009604727613805153
4311,8623,4311,12934,4.652305841445923,0.009046893368577003
4318,8637,4318,12955,4.659800052642822,0.008501312215912549
4325,8651,4325,12976,4.667369842529297,0.007968633429186411
4331,8663,4331,12994,4.674030065536499,0.00752279062692196
4338,8677,4338,13015,4.682055950164795,0.0070156912238417135
4345,8691,4345,13036,4.69166374206543,0.006523179909777355
4352,8705,4352,13057,4.699400901794434,0.006045788243568495
4358,8717,4358,13075,4.705910921096802,0.00564901123573236
4365,8731,4365,13096,4.7134788036346436,0.00520101168160636
4372,8745,4372,13117,4.721077919006348,0.00476949534868254
4378,8757,4378,13135,4.727713108062744,0.004413066923007136
4385,8771,4385,13156,4.735652923583984,0.004013272019278702
4392,8785,4392,13177,4.743063926696777,0.003631107345086093
4399,8799,4399,13198,4.750426769256592,0.003266923097385188
4405,8811,4405,13216,4.756980895996094,0.002969321205569031
4412,8825,4412,13237,4.764631032943726,0.0026393622002842676
4419,8839,4419,13258,4.7723541259765625,0.002328226223880847
4426,8853,4426,13279,4.780243873596191,0.0020361490190907716
4432,8865,4432,13297,4.78670597076416,0.001801121335802236
4439,8879,4439,13318,4.793977737426758,0.0015449531490503432
4446,8893,4446,13339,4.801394939422607,0.0013083362191537162
4452,8905,4452,13357,4.808043003082275,0.0011211655912575225
4459,8919,4459,13378,4.8156468868255615,0.0009211192575548921
4466,8933,4466,13399,4.823314905166626,0.0007408451299397711
4473,8947,4473,13420,4.831121921539307,0.0005803585272587952
4479,8959,4479,13438,4.837614059448242,0.0004585370179484016
4486,8973,4486,13459,4.844963073730469,0.0003347354332845498
4493,8987,4493,13480,4.852466821670532,0.00023059934630964563
4500,9001,4500,13501,4.860450029373169,0.00014603052534312155
4506,9013,4506,13519,4.867125988006592,8.902198158011743e-05
4513,9027,4513,13540,4.877519845962524,4.043635954076308e-05
4520,9041,4520,13561,4.885625839233398,1.0983416018461867e-05
4526,9053,4526,13579,4.892096996307373,8.10708570497809e-07
4533,9067,4533,13600,4.899610757827759,6.322122317214962e-06
4540,9081,4540,13621,4.907290935516357,3.03032641113532e-05
4547,9095,4547,13642,4.9150710105896,7.246830205076549e-05
4553,9107,4553,13660,4.92178201675415,0.00012284609886137332
4560,9121,4560,13681,4.929797887802124,0.00019793076592122816
4567,9135,4567,13702,4.937502861022949,0.00029023598960975505
4573,9147,4573,13720,4.9439170360565186,0.0003827696497182842
4580,9161,4580,13741,4.9514079093933105,0.0005060171013155923
4587,9175,4587,13762,4.9590840339660645,0.0006453258322380862
4594,9189,4594,13783,4.966640949249268,0.0008002494747643141
4600,9201,4600,13801,4.9731810092926025,0.0009451168770056029
4607,9215,4607,13822,4.981168985366821,0.0011277900557615794
4614,9229,4614,13843,4.98882794380188,0.0013246986680996997
4621,9243,4621,13864,4.996222019195557,0.0015353250515772743
4627,9255,4627,13882,5.00262975692749,0.001726374939607922
4634,9269,4634,13903,5.010770797729492,0.0019610441569284376
4641,9283,4641,13924,5.019052982330322,0.002207856720019663
4647,9295,4647,13942,5.027544736862183,0.002428634198849977
4654,9309,4654,13963,5.037016868591309,0.002696441614034484
4661,9323,4661,13984,5.0449090003967285,0.0029746895310154287
4668,9337,4668,14005,5.053153991699219,0.003262757172478814
4674,9349,4674,14023,5.059660911560059,0.00351701010083616
4681,9363,4681,14044,5.067551851272583,0.0038216347529669292
4688,9377,4688,14065,5.07635498046875,0.004134256799602554
4695,9391,4695,14086,5.085377931594849,0.004454226761026803
4701,9403,4701,14104,5.092685699462891,0.004733839905497916
4708,9417,4708,14125,5.101020812988281,0.005065720315087674
4715,9431,4715,14146,5.109606981277466,0.00540307430037501
4721,9443,4721,14164,5.116788864135742,0.005696090519222707
4728,9457,4728,14185,5.125226974487305,0.0060418548938514505
4735,9471,4735,14206,5.133877992630005,0.006391199265863179
4742,9485,4742,14227,5.142008066177368,0.006743457302832212
4748,9497,4748,14245,5.149194002151489,0.007047205855883476
4755,9511,4755,14266,5.157716989517212,0.00740310389824117
4762,9525,4762,14287,5.165708065032959,0.007760008797276896
4769,9539,4769,14308,5.174242973327637,0.008117255958495662
4775,9551,4775,14326,5.181692838668823,0.008423239476201161
4782,9565,4782,14347,5.19023585319519,0.008779374824257502
4789,9579,4789,14368,5.198807954788208,0.009133983507013
4795,9591,4795,14386,5.206166982650757,0.009436235154453243
4802,9605,4802,14407,5.214404821395874,0.009786325873278656
4809,9619,4809,14428,5.22358775138855,0.010133099850463623
4816,9633,4816,14449,5.233016014099121,0.01047595549482594
4822,9645,4822,14467,5.2402801513671875,0.010766267420081022
4829,9659,4829,14488,5.2481958866119385,0.011100298584892698
4836,9673,4836,14509,5.256390810012817,0.0114287711758152
4843,9687,4843,14530,5.264430046081543,0.011751138589715993
4849,9699,4849,14548,5.271408796310425,0.012022190138623046
4856,9713,4856,14569,5.279232978820801,0.012331816585060551
4863,9727,4863,14590,5.286958932876587,0.012633852561521053
4869,9739,4869,14608,5.293407917022705,0.012886325195040627
4876,9753,4876,14629,5.3007659912109375,0.01317296840511517
4883,9767,4883,14650,5.3085808753967285,0.013450653398194845
4890,9781,4890,14671,5.31621789932251,0.013718932822371244
4896,9793,4896,14689,5.323117017745972,0.013941074905346795
4903,9807,4903,14710,5.331213712692261,0.014190764046020377
4910,9821,4910,14731,5.338842868804932,0.014429876269559827
4917,9835,4917,14752,5.3460328578948975,0.014658043406598154
4923,9847,4923,14770,5.352419137954712,0.014844641900140232
4930,9861,4930,14791,5.360214948654175,0.015051586151344054
4937,9875,4937,14812,5.367771863937378,0.015246664440837776
4943,9887,4943,14830,5.374696969985962,0.015404220431605609
4950,9901,4950,14851,5.38249397277832,0.01557654846112655
4957,9915,4957,14872,5.390044927597046,0.01573628523226489
4964,9929,4964,14893,5.397380828857422,0.015883221060107644
4970,9941,4970,14911,5.40380072593689,0.015998834569359133
4977,9955,4977,14932,5.411401987075806,0.016121514989094976
4984,9969,4984,14953,5.419137954711914,0.016230914105562988
4990,9981,4990,14971,5.425992012023926,0.01631401680901945
4997,9995,4997,14992,5.43407678604126,0.016398428866978065
5004,10009,5004,15013,5.441673040390015,0.01646925270574684
5011,10023,5011,15034,5.449096918106079,0.016526423417303704
5017,10035,5017,15052,5.455862998962402,0.016564527785931205
5024,10049,5024,15073,5.463854789733887,0.016596249770373106
5031,10063,5031,15094,5.471556901931763,0.01661426250268505
5038,10077,5038,15115,5.479726076126099,0.016618592950976563
5044,10089,5044,15133,5.486276865005493,0.016611452944744087
5051,10103,5051,15154,5.49360203742981,0.016590527332709826
5058,10117,5058,15175,5.501131057739258,0.016556128322918084
5064,10129,5064,15193,5.5078558921813965,0.0165160079202451
5071,10143,5071,15214,5.515448093414307,0.01645691368298685
5078,10157,5078,15235,5.523101806640625,0.01638473608068125
5085,10171,5085,15256,5.53068995475769,0.016299649980510367
5091,10183,5091,15274,5.537229061126709,0.016216590916428686
5098,10197,5098,15295,5.544685125350952,0.016108057973042378
5105,10211,5105,15316,5.552199840545654,0.015987215248628672
5112,10225,5112,15337,5.559973955154419,0.01585430558702683
5118,10237,5118,15355,5.566509008407593,0.015730975251926793
5125,10251,5125,15376,5.574086904525757,0.015576357974282473
5132,10265,5132,15397,5.582107782363892,0.01541046160116366
5138,10277,5138,15415,5.588810920715332,0.015259521019856948
5145,10291,5145,15436,5.596375942230225,0.015073509590820322
5152,10305,5152,15457,5.603844881057739,0.014877145565833416
5159,10319,5159,15478,5.611501932144165,0.014670784540498971
5165,10331,5165,15496,5.61802077293396,0.014486227363818216
5172,10345,5172,15517,5.625798940658569,0.014262294066270442
5179,10359,5179,15538,5.633635759353638,0.01402945814402301
5186,10373,5186,15559,5.641092777252197,0.013788126144959278
5192,10385,5192,15577,5.6474738121032715,0.013574823499084232
5199,10399,5199,15598,5.654998064041138,0.013318825024157377
5206,10413,5206,15619,5.662576913833618,0.01305554331975145
5212,10425,5212,15637,5.669209718704224,0.012824409134282178
5219,10439,5219,15658,5.677306890487671,0.012548771339311315
5226,10453,5226,15679,5.6851959228515625,0.012267121503441558
5233,10467,5233,15700,5.693231821060181,0.011979915744859682
5239,10479,5239,15718,5.699649095535278,0.011729666914675363
5246,10493,5246,15739,5.707259893417358,0.011433370829877276
5253,10507,5253,15760,5.7147767543792725,0.011132849852060644
5260,10521,5260,15781,5.722651958465576,0.010828578306472991
5266,10533,5266,15799,5.72970175743103,0.010565151024479746
5273,10547,5273,15820,5.737421751022339,0.010255183502181353
5280,10561,5280,15841,5.7447309494018555,0.009942836266645827
5286,10573,5286,15859,5.751016855239868,0.009673581507172457
5293,10587,5293,15880,5.7585649490356445,0.009358093594642014
5300,10601,5300,15901,5.76618504524231,0.009041601116791753
5307,10615,5307,15922,5.7739458084106445,0.008724581538672282
5313,10627,5313,15940,5.780781984329224,0.008452790234628083
5320,10641,5320,15961,5.788561820983887,0.0081360455186541
5327,10655,5327,15982,5.795869827270508,0.007820115208005518
5334,10669,5334,16003,5.803260803222656,0.007505458753257699
5340,10681,5340,16021,5.8096699714660645,0.007237110967253102
5347,10695,5347,16042,5.81715989112854,0.00692601827472572
5354,10709,5354,16063,5.824792146682739,0.00661747744902641
5360,10721,5360,16081,5.831480026245117,0.006355374033660155
5367,10735,5367,16102,5.839183807373047,0.0060527175523930055
5374,10749,5374,16123,5.846617937088013,0.005753831467359305
5381,10763,5381,16144,5.854182958602905,0.005459125792981467
5387,10775,5387,16162,5.860733985900879,0.005210151920550743
5394,10789,5394,16183,5.868438005447388,0.004924264004785073
5401,10803,5401,16204,5.876728057861328,0.00464367184895309
5407,10815,5407,16222,5.883858919143677,0.00440765880091476
5414,10829,5414,16243,5.893471002578735,0.004137869252872406
5421,10843,5421,16264,5.90116286277771,0.00387439396672562
5428,10857,5428,16285,5.908920049667358,0.0036175639068005694
5434,10869,5434,16303,5.91543984413147,0.0034029536673187977
5441,10883,5441,16324,5.923827886581421,0.0031592953916970146
5448,10897,5448,16345,5.932147026062012,0.0029231509491864927
5455,10911,5455,16366,5.939949035644531,0.0026947969646471392
5461,10923,5461,16384,5.946694850921631,0.0025054647716160616
5468,10937,5468,16405,5.954463005065918,0.002292263796903171
5475,10951,5475,16426,5.9625608921051025,0.0020875644433999696
5481,10963,5481,16444,5.969781875610352,0.0019190421926396084
5488,10977,5488,16465,5.978307723999023,0.0017307058868709646
5495,10991,5495,16486,5.986311912536621,0.00155146186955335
5502,11005,5502,16507,5.994428873062134,0.0013814870329724727
5508,11017,5508,16525,6.001097917556763,0.0012432941118731833
5515,11031,5515,16546,6.00892186164856,0.0010909473451192753
5522,11045,5522,16567,6.016709804534912,0.0009482847401613981
5529,11059,5529,16588,6.024786949157715,0.0008154188034268373
5535,11071,5535,16606,6.032014846801758,0.0007094037115393803
5542,11085,5542,16627,6.039911985397339,0.0005949711279527037
5549,11099,5549,16648,6.047769784927368,0.0004905615950292486
5555,11111,5555,16666,6.054543733596802,0.00040908088544711063
5562,11125,5562,16687,6.062877893447876,0.00032339627443889185
5569,11139,5569,16708,6.073307991027832,0.00024782397179023974
5576,11153,5576,16729,6.083317041397095,0.00018236443418118142
5582,11165,5582,16747,6.090009927749634,0.00013429432931388874
5589,11179,5589,16768,6.097346067428589,8.756477745919256e-05
5596,11193,5596,16789,6.104888916015625,5.086573628432234e-05
5603,11207,5603,16810,6.112441778182983,2.4139760853358894e-05
5609,11219,5609,16828,6.118973970413208,9.115170541917905e-06
5616,11233,5616,16849,6.126997947692871,7.076876045175595e-07
5623,11247,5623,16870,6.134954929351807,2.0274059124858468e-06
5629,11259,5629,16888,6.141397953033447,1.0814012284754426e-05
5636,11273,5636,16909,6.148861885070801,2.9882596322750032e-05
5643,11287,5643,16930,6.156548738479614,5.8310949384576816e-05
5650,11301,5650,16951,6.1646599769592285,9.594234370524646e-05
5656,11313,5656,16969,6.171478986740112,0.00013539370445414534
5663,11327,5663,16990,6.1796958446502686,0.00018965362107792316
5670,11341,5670,17011,6.187473773956299,0.0002525942749116439
5677,11355,5677,17032,6.194950819015503,0.00032400897566731146
5683,11367,5683,17050,6.201145887374878,0.0003918013869679271
5690,11381,5690,17071,6.2087507247924805,0.00047836773921972053
5697,11395,5697,17092,6.216355800628662,0.0005727585336217089
5703,11407,5703,17110,6.2229039669036865,0.0006597062368882689
5710,11421,5710,17131,6.230916738510132,0.0007679683538981408
5717,11435,5717,17152,6.238749980926514,0.000883328023633112
5724,11449,5724,17173,6.246145009994507,0.0010055139916858025
5730,11461,5730,17191,6.252639055252075,0.0011154661804084753
5737,11475,5737,17212,6.260453939437866,0.001249581074944217
5744,11489,5744,17233,6.2680089473724365,0.0013897010323944414
5750,11501,5750,17251,6.274677991867065,0.0015143539376367698
5757,11515,5757,17272,6.28286600112915,0.0016648166607637904
5764,11529,5764,17293,6.2904887199401855,0.0018203994003442858
5771,11543,5771,17314,6.29786491394043,0.0019807794568578174
5777,11555,5777,17332,6.304313898086548,0.0021218177236050906
5784,11569,5784,17353,6.312010049819946,0.002290232970494799
5791,11583,5791,17374,6.3197197914123535,0.0024624965855082337
5798,11597,5798,17395,6.327779054641724,0.002638269940689497
5804,11609,5804,17413,6.334810733795166,0.0027914681916172412
5811,11623,5811,17434,6.342423915863037,0.00297285532224123
5818,11637,5818,17455,6.349870920181274,0.0031567767522346912
5824,11649,5824,17473,6.356487989425659,0.0033161814048980887
5831,11663,5831,17494,6.3640828132629395,0.0035039017828921715
5838,11677,5838,17515,6.372114896774292,0.0036931797529859978
5845,11691,5845,17536,6.380082845687866,0.0038836745197841083
5851,11703,5851,17554,6.386989116668701,0.004047666455221588
5858,11717,5858,17575,6.39431095123291,0.004239519580778506
5865,11731,5865,17596,6.4016969203948975,0.004431620582067808
5872,11745,5872,17617,6.409430027008057,0.004623632643415476
5878,11757,5878,17635,6.415970087051392,0.004787889596286732
5885,11771,5885,17656,6.423872947692871,0.004978849349981829
5892,11785,5892,17677,6.431984901428223,0.005168769603642431
5898,11797,5898,17695,6.438628911972046,0.005330483435500355
5905,11811,5905,17716,6.446051836013794,0.0055176104084466715
5912,11825,5912,17737,6.453662872314453,0.0057027777243092714
5919,11839,5919,17758,6.461305856704712,0.005885674081014258
5925,11851,5925,17776,6.467844724655151,0.006040403902147773
5932,11865,5932,17797,6.475743055343628,0.006218280653683905
5939,11879,5939,17818,6.483844757080078,0.006393036735175883
5946,11893,5946,17839,6.491513729095459,0.006564390179846669
5952,11905,5952,17857,6.49786901473999,0.0067083487713262
5959,11919,5959,17878,6.50548791885376,0.006872663815101987
5966,11933,5966,17899,6.513147830963135,0.007032817350591358
5972,11945,5972,17917,6.5197179317474365,0.007166590485326196
5979,11959,5979,17938,6.527523756027222,0.007318360893577847
5986,11973,5986,17959,6.535402059555054,0.0074652804714787635
5993,11987,5993,17980,6.542909860610962,0.0076071245126740905
5999,11999,5999,17998,6.549147844314575,0.0077245015436346876
6006,12013,6006,18019,6.556736946105957,0.00785635387626371
6013,12027,6013,18040,6.564407110214233,0.007982538626606583
6020,12041,6020,18061,6.571923017501831,0.008102867322918428
6026,12053,6026,18079,6.578746795654297,0.008201210072343201
6033,12067,6033,18100,6.586606740951538,0.008310199437119081
6040,12081,6040,18121,6.594040870666504,0.008412853857976188
6046,12093,6046,18139,6.600387096405029,0.008495690759218633
6053,12107,6053,18160,6.608125925064087,0.008586203798358838
6060,12121,6060,18181,6.615808963775635,0.008669998729487816
6067,12135,6067,18202,6.623591899871826,0.008746964978740834
6073,12147,6073,18220,6.630378007888794,0.008807426065231994
6080,12161,6080,18241,6.638054847717285,0.008871458553926459
6087,12175,6087,18262,6.645417928695679,0.008928412984232637
6094,12189,6094,18283,6.653079986572266,0.008978224750308073
6100,12201,6100,18301,6.659860849380493,0.00901519493959313
6107,12215,6107,18322,6.66776704788208,0.009051609125435789
6114,12229,6114,18343,6.675740957260132,0.009080758346044604
6120,12241,6120,18361,6.682755708694458,0.009099944581407726
6127,12255,6127,18382,6.690496921539307,0.009115553467836435
6134,12269,6134,18403,6.697800874710083,0.009123865873220893
6141,12283,6141,18424,6.705626964569092,0.009124892396130235
6147,12295,6147,18442,6.712384939193726,0.009119989671148687
6154,12309,6154,18463,6.72041392326355,0.009107552356454107
6161,12323,6161,18484,6.729145765304565,0.009087922583375985
6167,12335,6167,18502,6.736119985580444,0.009065413806297329
6174,12349,6174,18523,6.743557929992676,0.009032581125211436
6181,12363,6181,18544,6.751003980636597,0.008992743301860173
6188,12377,6188,18565,6.758652925491333,0.008945987510287523
6194,12389,6194,18583,6.765125751495361,0.008900478914142695
6201,12403,6201,18604,6.77305793762207,0.008841143089512116
6208,12417,6208,18625,6.78161883354187,0.008775196200645041
6215,12431,6215,18646,6.7896177768707275,0.008702764642976035
6221,12443,6221,18664,6.795969009399414,0.008635621708208419
6228,12457,6228,18685,6.803489923477173,0.008551513545512535
6235,12471,6235,18706,6.8109519481658936,0.008461331128046368
6241,12483,6241,18724,6.817274808883667,0.008379318233551203
6248,12497,6248,18745,6.825101137161255,0.008278285090341342
6255,12511,6255,18766,6.833302021026611,0.008171655180376547
6262,12525,6262,18787,6.840908050537109,0.008059610366103698
6268,12537,6268,18805,6.847333908081055,0.007959405320775659
6275,12551,6275,18826,6.854783058166504,0.007837811454578514
6282,12565,6282,18847,6.862137794494629,0.00771136168771136
6289,12579,6289,18868,6.869761943817139,0.007580264693388017
6295,12591,6295,18886,6.876446962356567,0.007464359803861953
6302,12605,6302,18907,6.884436845779419,0.007325207043095361
6309,12619,6309,18928,6.89191198348999,0.0071820366758856835
6315,12631,6315,18946,6.898244857788086,0.007056296415385077
6322,12645,6322,18967,6.905930995941162,0.006906280965381484
6329,12659,6329,18988,6.913335084915161,0.006752919907398791
6336,12673,6336,19009,6.920710802078247,0.006596456560828301
6342,12685,6342,19027,6.927374839782715,0.0064600629319784275
6349,12699,6349,19048,6.935281991958618,0.006298495196119802
6356,12713,6356,19069,6.942878007888794,0.006134537848765831
6363,12727,6363,19090,6.950225830078125,0.005968445005464673
6369,12739,6369,19108,6.956517934799194,0.005824573905329089
6376,12753,6376,19129,6.963868856430054,0.005655194802216101
6383,12767,6383,19150,6.9712278842926025,0.005484414140596527
6389,12779,6389,19168,6.978632926940918,0.005337111001381345
6396,12793,6396,19189,6.986158132553101,0.005164412888689185
6403,12807,6403,19210,6.993457794189453,0.004991051269371383
6410,12821,6410,19231,7.00081992149353,0.004817283751208379
6416,12833,6416,19249,7.007277011871338,0.004668211677198997
6423,12847,6423,19270,7.0146801471710205,0.004494370261681979
6430,12861,6430,19291,7.02209997177124,0.004320852489968274
6437,12875,6437,19312,7.0298779010772705,0.004147910369056262
6443,12887,6443,19330,7.036532878875732,0.004000321811190588
6450,12901,6450,19351,7.043910980224609,0.0038291093683255895
6457,12915,6457,19372,7.051417827606201,0.003659178968746346
6463,12927,6463,19390,7.05794095993042,0.0035147278374552116
6470,12941,6470,19411,7.06532096862793,0.0033478161742550583
6477,12955,6477,19432,7.072927951812744,0.0031828665551074664
6484,12969,6484,19453,7.080909013748169,0.0030201091984736195
6490,12981,6490,19471,7.089643955230713,0.0028825188732071183
6497,12995,6497,19492,7.097584962844849,0.0027244274933764245
6504,13009,6504,19513,7.1052727699279785,0.0025691591755503396
6511,13023,6511,19534,7.113173007965088,0.002416924040289814
6517,13035,6517,19552,7.120345830917358,0.0022890057443873957
6524,13049,6524,19573,7.1289379596710205,0.0021429399416774686
6531,13063,6531,19594,7.137464761734009,0.0020004727051627924
6537,13075,6537,19612,7.144270896911621,0.0018813622809830122
6544,13089,6544,19633,7.152318000793457,0.0017460625664398322
6551,13103,6551,19654,7.160745859146118,0.0016148696804521023
6558,13117,6558,19675,7.168566942214966,0.001487947100713427
6564,13129,6564,19693,7.174996852874756,0.0013826734251551898
6571,13143,6571,19714,7.182801961898804,0.0012640887827046754
6578,13157,6578,19735,7.190244913101196,0.0011501987315796214
6584,13169,6584,19753,7.196609020233154,0.0010564163873141297
6591,13183,6591,19774,7.204093933105469,0.0009515921096863167
6598,13197,6598,19795,7.211451768875122,0.0008518213746810943
6605,13211,6605,19816,7.219003915786743,0.0007572138255227401
6611,13223,6611,19834,7.225514888763428,0.0006803079710380189
6618,13237,6618,19855,7.233237981796265,0.0005955507349426625
6625,13251,6625,19876,7.241055965423584,0.0005162221063983452
6632,13265,6632,19897,7.248887062072754,0.00044239764031317463
6638,13277,6638,19915,7.2554240226745605,0.00038355088634034473
6645,13291,6645,19936,7.263079881668091,0.0003201171628006705
6652,13305,6652,19957,7.271542072296143,0.0002623519825419862
6658,13317,6658,19975,7.279984951019287,0.0002173806867631356
6665,13331,6665,19996,7.2876060009002686,0.0001702397767076036
6672,13345,6672,20017,7.295017957687378,0.0001288544849558093
6679,13359,6679,20038,7.302637100219727,9.323719962139876e-05
6685,13371,6685,20056,7.308974027633667,6.730163181600801e-05
6692,13385,6692,20077,7.316393852233887,4.239799170591141e-05
6699,13399,6699,20098,7.32398796081543,2.32476229484746e-05
6706,13413,6706,20119,7.3321027755737305,9.828263046074426e-06
6712,13425,6712,20137,7.338464021682739,2.8641520657401998e-06
6719,13439,6719,20158,7.345659971237183,4.955609256285243e-10


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012731552124023438,2180.042156630883
2002,2003,2002,4005,2.599030017852783,58.25374124224231
4004,4005,4004,8009,5.550410032272339,52.3325146079394
6006,6007,6006,12013,8.399940252304077,49.460442359107674
8008,8009,8008,16017,12.707967042922974,47.11599220764424
10010,10011,10010,20021,16.910256147384644,45.01839520660428
12012,12013,12012,24025,20.07123613357544,43.1041342096305
14014,14015,14014,28029,22.234843254089355,41.34442017011406
16016,16017,16016,32033,24.46739625930786,39.72023725225745
18018,18019,18018,36037,27.24409008026123,38.217042626841476
20020,20021,20020,40041,29.938059091567993,36.82271904943559
22022,22023,22022,44045,32.28457713127136,35.52660307526935
24024,24025,24024,48049,34.81133532524109,34.319031355813195
26026,26027,26026,52053,37.3308470249176,33.1911537993999
28028,28029,28028,56057,40.411330223083496,32.13487290836338
30030,30031,30030,60061,42.95606303215027,31.14282994231644
32032,32033,32032,64065,45.43171811103821,30.208397006197856
34034,34035,34034,68069,47.86099028587341,29.32565773483998
36036,36037,36036,72073,49.98659038543701,28.48937249582923
38038,38039,38038,76077,52.266645193099976,27.69493045643776
40040,40041,40040,80081,54.5657160282135,26.938293162014816
42042,42043,42042,84085,56.80834937095642,26.215934371844924
44044,44045,44044,88089,59.21900796890259,25.52478002400767
46046,46047,46046,92093,61.93172025680542,24.86215105790029
48048,48049,48048,96097,64.49579119682312,24.225710762503468
50050,50051,50050,100101,66.95311307907104,23.613417476868108
52052,52053,52052,104105,69.22466826438904,23.023482868537712
54054,54055,54054,108109,71.5374813079834,22.454335625142676
56056,56057,56056,112113,73.92988634109497,21.9045901665354
58058,58059,58058,116117,76.20664024353027,21.37301987265505
60060,60061,60060,120121,78.53979539871216,20.858534286747044
62062,62063,62062,124125,80.68638110160828,20.36015976509907
64064,64065,64064,128129,83.02073121070862,19.877023082339747
66066,66067,66066,132133,85.22011518478394,19.40833755175686
68068,68069,68068,136137,87.52609205245972,18.953391274319983
70070,70071,70070,140141,89.66470503807068,18.51153718304704
72072,72073,72072,144145,91.83437633514404,18.08248844999025
74074,74075,74074,148149,93.9465901851654,17.665934156932735
76076,76077,76076,152153,96.128573179245,17.26085446709567
78078,78079,78078,156157,98.71073007583618,16.866771724344744
80080,80081,80080,160161,101.05764722824097,16.483250035031688
82082,82083,82082,164165,103.2496120929718,16.109886687983817
84084,84085,84084,168169,105.5673291683197,15.746307450084714
86086,86087,86086,172173,107.6981360912323,15.392162986714538
88088,88089,88088,176177,109.82220315933228,15.047125936799148
90090,90091,90090,180181,111.91037797927856,14.710888475447632
92092,92093,92092,184185,114.02033829689026,14.383160260547015
94094,94095,94094,188189,116.21445226669312,14.0636666872972
96096,96097,96096,192193,118.42794418334961,13.752147392701886
98098,98099,98098,196197,120.60367894172668,13.448354965090061
100100,100101,100100,200201,122.67649936676025,13.152053823399683
102102,102103,102102,204205,124.52444219589233,12.863019238252946
104104,104105,104104,208209,126.45313310623169,12.581036472378742
106106,106107,106106,212213,128.38393807411194,12.305900022172523
108108,108109,108108,216217,130.4476113319397,12.037412945500591
110110,110111,110110,220221,133.10494828224182,11.775386263436417
112112,112113,112112,224225,135.7337942123413,11.519638425694438
114114,114115,114114,228229,138.11872625350952,11.269994831166741
116116,116117,116116,232233,140.4447832107544,11.026287396320754
118118,118119,118118,236237,142.82550406455994,10.788354165312285
120120,120121,120120,240241,145.2939100265503,10.556038956571342
122122,122123,122122,244245,147.74786925315857,10.329191041376816
124124,124125,124124,248249,150.317889213562,10.107664850561719
126126,126127,126126,252253,153.08126616477966,9.89131970602864
128128,128129,128128,256257,155.2761800289154,9.68001957420347
130130,130131,130130,260261,157.9019901752472,9.473632838940262
132132,132133,132132,264265,160.09006214141846,9.272032091716596
134134,134135,134134,268269,162.20411229133606,9.075093937253314
136136,136137,136136,272273,164.451913356781,8.88269881292183
138138,138139,138138,276277,166.6570851802826,8.694730820531163
140140,140141,140140,280281,168.84525227546692,8.511077569257509
142142,142143,142142,284285,171.0157151222229,8.331630028648988
144144,144145,144144,288289,173.1730432510376,8.156282390773413
146146,146147,146146,292293,175.36536598205566,7.984931940698175
148148,148149,148148,296297,177.62288522720337,7.8174789345964655
150150,150151,150150,300301,179.8526041507721,7.65382648486343
152152,152153,152152,304305,182.09009408950806,7.4938804517049675
154154,154155,154154,308309,184.30994415283203,7.337549340718169
156156,156157,156156,312313,186.50056910514832,7.184744206047526
158158,158159,158158,316317,188.61428308486938,7.03537855873833
160160,160161,160160,320321,190.8081452846527,6.889368279945643
162162,162163,162162,324325,193.01863503456116,6.746631538689144
164164,164165,164164,328329,195.25345826148987,6.607088713862709
166166,166167,166166,332333,197.5209641456604,6.470662320235874
168168,168169,168168,336337,199.76155018806458,6.337276938185369
170170,170171,170170,340341,201.88551926612854,6.20685914692308
172172,172173,172172,344345,204.01611638069153,6.079337460986267
174174,174175,174174,348349,206.16153216362,5.954642269773672
176176,176177,176176,352353,208.32231497764587,5.832705779917887
178178,178179,178178,356357,210.52235221862793,5.7134619602970815
180180,180181,180180,360361,212.75186109542847,5.596846489497466
182182,182183,182182,364365,214.98792338371277,5.4827967055521185
184184,184185,184184,368369,217.12072014808655,5.371251557790401
186186,186187,186186,372373,219.28395819664001,5.262151560649954
188188,188189,188188,376377,221.43391823768616,5.155438749303357
190190,190191,190190,380381,223.58544325828552,5.051056636979297
192192,192193,192192,384385,225.82999396324158,4.948950173855906
194194,194195,194194,388389,228.03504729270935,4.849065707421914
196196,196197,196196,392393,230.2543122768402,4.751350944211708
198198,198199,198198,396397,232.40882110595703,4.655754912823113
200200,200201,200200,400401,234.5628433227539,4.562227928148445
202202,202203,202202,404405,236.74334716796875,4.470721556741864
204204,204205,204204,408409,238.9401831626892,4.3811885832645885
206206,206207,206206,412413,241.2309021949768,4.293582977952951
208208,208209,208208,416417,243.68491220474243,4.207859865057912
210210,210211,210210,420421,246.08915209770203,4.123975492207933
212212,212213,212212,424425,248.49859023094177,4.041887200662131
214214,214215,214214,428429,250.66003036499023,3.9615533964076803
216216,216217,216216,432433,252.85056018829346,3.882933522074609
218218,218219,218218,436437,255.0303349494934,3.8059880296335677
220220,220221,220220,440441,257.40616607666016,3.7306783538494983
222222,222223,222222,444445,259.73456716537476,3.656966886465284
224224,224225,224224,448449,262.22797322273254,3.5848169510911703
226226,226227,226226,452453,264.7601342201233,3.5141927787757368
228228,228229,228228,456457,266.960488319397,3.445059484240346
230230,230231,230230,460461,269.2586522102356,3.3773830427541043
232232,232233,232232,464465,272.3837833404541,3.3111302676321657
234234,234235,234234,468469,274.5964252948761,3.2462687883398758
236236,236237,236236,472473,277.85747027397156,3.1827670291839922
238238,238239,238238,476477,280.7028751373291,3.1205941885766606
240240,240241,240240,480481,283.1667683124542,3.059720218854409
242242,242243,242242,484485,285.8840560913086,3.000115806639883
244244,244245,244244,488489,288.357084274292,2.9417523537283614
246246,246247,246246,492493,291.1954972743988,2.8846019584888154
248248,248249,248248,496497,293.7174391746521,2.8286373977613266
250250,250251,250250,500501,296.25027418136597,2.773832109243699
252252,252253,252252,504505,298.5271670818329,2.720160174347029
254254,254255,254254,508509,300.8274083137512,2.6675963015154593
256256,256257,256256,512513,303.5860722064972,2.6161158099912427
258258,258259,258258,516517,306.53852701187134,2.5656946140189802
260260,260261,260260,520521,308.8104512691498,2.5163092074714086
262262,262263,262262,524525,311.05359625816345,2.4679366488925325
264264,264265,264264,528529,313.37713408470154,2.420554546941048
266266,266267,266266,532533,315.7950382232666,2.374141046226555
268268,268269,268268,536537,318.08701515197754,2.328674813526277
270270,270271,270270,540541,320.52282524108887,2.284135024375587
272272,272273,272272,544545,323.5352282524109,2.2405013500176665
274274,274275,274274,548549,325.83986616134644,2.1977539447048002
276276,276277,276276,552553,328.11139726638794,2.1558734333435723
278278,278279,278278,556557,330.36385011672974,2.1148408994716874
280280,280281,280280,560561,333.96388721466064,2.0746378735589133
282282,282283,282282,564565,336.5761661529541,2.0352463216235037
284284,284285,284284,568569,340.1240303516388,1.9966486341548944
286286,286287,286286,572573,342.2639582157135,1.9588276153351671
288288,288289,288288,576577,344.51355600357056,1.9217664725491659
290290,290291,290290,580581,346.8835949897766,1.8854488061788288
292292,292293,292292,584585,349.0089011192322,1.8498585996693464
294294,294295,294294,588589,351.20543217658997,1.8149802098645296
296296,296297,296296,592593,353.4293041229248,1.7807983576008155
298298,298299,298298,596597,356.65806102752686,1.747298118552294
300300,300301,300300,600601,359.5782582759857,1.7144649143231163
302302,302303,302302,604605,362.0418653488159,1.6822845037768275
304304,304305,304304,608609,364.5471670627594,1.650742974599325
306306,306307,306306,612613,366.89907026290894,1.6198267350854394
308308,308309,308308,616617,369.2629702091217,1.5895225061460678
310310,310311,310310,620621,371.55578231811523,1.559817313528697
312312,312313,312312,624625,373.7832372188568,1.530698480244041
314314,314315,314314,628629,376.01899313926697,1.5021536191948144
316316,316317,316316,632633,378.2740032672882,1.4741706260010687
318318,318319,318318,636637,380.48268699645996,1.4467376720150469
320320,320321,320320,640641,382.72800731658936,1.4198431975216863
322322,322323,322322,644645,385.1314561367035,1.3934759051186347
324324,324325,324324,648649,387.3582401275635,1.3676247532722527
326326,326327,326326,652653,389.8724431991577,1.3422789500427825
328328,328329,328328,656657,392.2821843624115,1.317427946975954
330330,330331,330330,660661,394.56707406044006,1.2930614331538663
332332,332333,332332,664665,396.8106451034546,1.2691693294044626
334334,334335,334334,668669,398.98766016960144,1.245741782660275
336336,336337,336336,672673,401.20540618896484,1.2227691604679194
338338,338339,338338,676677,403.3750972747803,1.2002420456394702
340340,340341,340340,680681,405.6083400249481,1.1781512310425342
342342,342343,342342,684685,407.8965313434601,1.1564877145299306
344344,344345,344344,688689,410.07972621917725,1.1352426939970428
346346,346347,346346,692693,412.33556509017944,1.1144075625707046
348348,348349,348348,696697,414.6582541465759,1.0939739039216647
350350,350351,350350,700701,416.8442301750183,1.0739334876989233
352352,352353,352352,704705,419.0006101131439,1.0542782650812796
354354,354355,354354,708709,421.34193110466003,1.0350003644455228
356356,356357,356356,712713,423.76086926460266,1.0160920871442158
358358,358359,358358,716717,425.94870829582214,0.9975459033931884
360360,360361,360360,720721,428.20590901374817,0.979354448264985
362362,362363,362362,724725,430.4506323337555,0.961510517784177
364364,364365,364364,728729,432.63280510902405,0.9440070651229462
366366,366367,366366,732733,434.8005881309509,0.9268371968939846
368368,368369,368368,736737,436.9976010322571,0.9099941695378675
370370,370371,370370,740741,439.1478431224823,0.8934713858016039
372372,372373,372372,744745,441.3499262332916,0.8772623913085908
374374,374375,374374,748749,445.72120237350464,0.8613608712126961
376376,376377,376376,752753,449.2512662410736,0.845760646939766
378378,378379,378378,756757,452.43699312210083,0.8304556730099648
380380,380381,380380,760761,455.36054706573486,0.8154400339399217
382382,382383,382382,764765,458.5096733570099,0.8007079412240046
384384,384385,384384,768769,461.30771040916443,0.7862537303907402
386386,386387,386386,772773,463.81040930747986,0.7720718581329038
388388,388389,388388,776777,466.55113220214844,0.7581568995099133
390390,390391,390390,780781,469.1878089904785,0.7445035452194588
392392,392393,392392,784785,471.7414960861206,0.7311065989376857
394394,394395,394394,788789,474.4277970790863,0.7179609747248605
396396,396397,396396,792793,476.75355315208435,0.7050616944972035
398398,398399,398398,796797,479.04983615875244,0.6924038855587469
400400,400401,400400,800801,481.4195091724396,0.6799827781953809
402402,402403,402402,804805,483.7926080226898,0.667793703330176
404404,404405,404404,808809,486.13891410827637,0.6558320902331616
406406,406407,406406,812813,488.68701219558716,0.6440934642897673
408408,408409,408408,816817,491.01044821739197,0.6325734448231515
410410,410411,410410,820821,494.49910712242126,0.6212677429699625
412412,412413,412412,824825,497.4975152015686,0.6101721596085099
414414,414415,414414,828829,500.7863039970398,0.5992825833362758
416416,416417,416416,832833,503.6718981266022,0.5885949884981301
418418,418419,418418,836837,506.2159721851349,0.5781054332612712
420420,420421,420420,840841,508.6760470867157,0.5678100577383702
422422,422423,422422,844845,511.0462472438812,0.5577050821538023
424424,424425,424424,848849,513.425252199173,0.5477868050571715
426426,426427,426426,852853,515.6754050254822,0.5380516015763988
428428,428429,428428,856857,517.8295040130615,0.5284959217166261
430430,430431,430430,860861,520.0653700828552,0.5191162886969778
432432,432433,432432,864865,522.1543872356415,0.509909297328818
434434,434435,434434,868869,524.2443311214447,0.5008716124320927
436436,436437,436436,872873,526.3054902553558,0.4919999672902122
438438,438439,438438,876877,528.5027191638947,0.48329116214063106
440440,440441,440440,880881,531.5053412914276,0.4747420627026031
442442,442443,442442,884885,533.7638993263245,0.46634959873904336
444444,444445,444444,888889,536.3153171539307,0.4581107626526091
446446,446447,446446,892893,538.8093671798706,0.45002260811577344
448448,448449,448448,896897,541.2881033420563,0.4420822487315945
450450,450451,450450,900901,543.6329700946808,0.4342868567281357
452452,452453,452452,904905,545.9292690753937,0.4266336616809667
454454,454455,454454,908909,548.0692563056946,0.41911994926931584
456456,456457,456456,912913,550.252509355545,0.4117430600571197
458458,458459,458458,916917,552.3679301738739,0.404500388306019
460460,460461,460460,920921,554.4270961284637,0.39738938081438846
462462,462463,462462,924925,556.507618188858,0.3904075357833108
464464,464465,464464,928929,558.6371812820435,0.38355240171006244
466466,466467,466466,932933,561.6757130622864,0.3768215763062699
468468,468469,468468,936937,564.0395519733429,0.37021270544096296
470470,470471,470470,940941,566.7845942974091,0.36372348210966265
472472,472473,472472,944945,569.3374311923981,0.3573516454249557
474474,474475,474474,948949,571.6887652873993,0.3510949796324212
476476,476477,476476,952953,573.8977053165436,0.34495131314770333
478478,478479,478478,956957,576.1339371204376,0.3389185176159799
480480,480481,480480,960961,578.2656321525574,0.3329945069937139
482482,482483,482482,964965,580.822005033493,0.32717723665132326
484484,484485,484484,968969,583.5637440681458,0.32146470249517733
486486,486487,486486,972973,586.2939803600311,0.315854940110853
488488,488489,488488,976977,588.4221892356873,0.3103460239249216
490490,490491,490490,980981,590.8156261444092,0.304936066386972
492492,492493,492492,984985,593.1153881549835,0.29962321716811857
494494,494495,494494,988989,595.5117952823639,0.29440566238008614
496496,496497,496496,992993,597.7695543766022,0.2892816238107798
498498,498499,498498,996997,599.9802792072296,0.28424935817611185
500501,500502,500501,1001003,602.2109751701355,0.2793047099822843
502503,502504,502503,1005007,604.3505582809448,0.2744509401803725
504505,504506,504505,1009011,606.430902004242,0.26968391499815425
506507,506508,506507,1013015,609.0252101421356,0.26500202373938464
508509,508510,508509,1017019,611.665854215622,0.26040368714450324
510511,510512,510511,1021023,613.967395067215,0.2558873567380715
512513,512514,512513,1025027,616.0622432231903,0.2514515141907623
514515,514516,514515,1029031,618.117269039154,0.2470946706959012
516517,516518,516517,1033035,621.1099503040314,0.24281536635987777
518519,518520,518519,1037039,623.9097692966461,0.238612169605517
520521,520522,520521,1041043,626.0393011569977,0.23448367658920688
522523,522524,522523,1045047,628.4394171237946,0.23042851063109993
524525,524526,524525,1049051,630.8983891010284,0.22644532165656983
526527,526528,526527,1053055,633.0539042949677,0.22253278565165147
528529,528530,528529,1057059,635.9442501068115,0.21868960412882643
530531,530532,530531,1061063,638.4704382419586,0.21491450360610997
532533,532534,532533,1065067,641.0513052940369,0.21120623509602865
534535,534536,534535,1069071,643.7782850265503,0.20756357360676247
536537,536538,536537,1073075,646.2452630996704,0.20398531765420103
538539,538540,538539,1077079,648.8715472221375,0.2004702887829808
540541,540542,540541,1081083,651.6030471324921,0.19701733110105124
542543,542544,542543,1085087,654.3699731826782,0.1936253108206074
544545,544546,544545,1089091,657.3312261104584,0.19029311581266484
546547,546548,546547,1093095,659.9528503417969,0.1870196551672052
548549,548550,548549,1097099,662.3882741928101,0.18380385876776018
550551,550552,550551,1101103,664.7957491874695,0.18064467687031538
552553,552554,552553,1105107,667.2796142101288,0.17754107969403776
554555,554556,554555,1109111,670.3776512145996,0.17449205702030213
556557,556558,556557,1113115,672.6773381233215,0.17149661780069891
558559,558560,558559,1117119,674.9081931114197,0.16855378977140845
560561,560562,560561,1121123,677.4043221473694,0.16566261907883018
562563,562564,562563,1125127,679.9212071895599,0.16282216991112364
564565,564566,564565,1129131,682.183806180954,0.16003152413782118
566567,566568,566567,1133135,684.7545731067657,0.15728978095762614
568569,568570,568569,1137139,686.9668023586273,0.15459605655416908
570571,570572,570571,1141143,689.442066192627,0.1519494837577895
572573,572574,572573,1145147,691.7772531509399,0.149349211714366
574575,574576,574575,1149151,694.0166771411896,0.1467944055635826
576577,576578,576577,1153155,696.264909029007,0.1442842461208329
578579,578580,578579,1157159,698.5034801959991,0.1418179295678783
580581,580582,580581,1161163,700.7320640087128,0.1393946671496451
582583,582584,582583,1165167,702.959614276886,0.13701368487613763
584585,584586,584585,1169171,705.2019572257996,0.13467422323265055
586587,586588,586587,1173175,707.8620893955231,0.1323755368947559
588589,588590,588589,1177179,710.1241700649261,0.13011689444908825
590591,590592,590591,1181183,712.5426201820374,0.12789757812095104
592593,592594,592593,1185187,715.4310550689697,0.12571688350647037
594595,594596,594595,1189191,717.9289281368256,0.12357411931077422
596597,596598,596597,1193195,720.3487732410431,0.12146860709287921
598599,598600,598599,1197199,722.8753771781921,0.1193996810131921
600601,600602,600601,1201203,725.7763941287994,0.1173666875889694
602603,602604,602603,1205207,728.1169202327728,0.11536898545250551
604605,604606,604605,1209211,730.3668072223663,0.1134059451169378
606607,606608,606607,1213215,732.5367321968079,0.11147694874330227
608609,608610,608609,1217219,734.622896194458,0.10958138991679789
610611,610612,610611,1221223,736.7861721515656,0.10771867342305086
612613,612614,612613,1225227,738.9510593414307,0.1058882150334739
614615,614616,614615,1229231,741.0494582653046,0.10408944129096653
616617,616618,616617,1233235,743.1341121196747,0.102321789302664
618619,618620,618619,1237239,745.304749250412,0.10058470653609675
620621,620622,620621,1241243,747.383415222168,0.09887765061932896
622623,622624,622623,1245247,749.8839392662048,0.09720008914575828
624625,624626,624625,1249251,752.4292573928833,0.09555149948130293
626627,626628,626627,1253255,755.3200581073761,0.09393136857863738
628629,628630,628629,1257259,757.8690192699432,0.09233919279165548
630631,630632,630631,1261263,760.5983150005341,0.09077447769550417
632633,632634,632633,1265267,763.318311214447,0.08923673791139208
634635,634636,634635,1269271,765.9258680343628,0.08772549693162546
636637,636638,636637,1273275,768.6855113506317,0.08624028695169272
638639,638640,638639,1277279,771.1283621788025,0.08478064870314483
640641,640642,640641,1281283,773.3942201137543,0.08334613129238733
642643,642644,642643,1285287,776.521222114563,0.08193629203924502
644645,644646,644645,1289291,778.8189971446991,0.08055069632268896
646647,646648,646647,1293295,781.5466501712799,0.07918891742610867
648649,648650,648649,1297299,783.8294951915741,0.07785053638826867
650651,650652,650651,1301303,786.2195162773132,0.07653514185653876
652653,652654,652653,1305307,788.6756691932678,0.07524232994126123
654655,654656,654655,1309311,791.3919901847839,0.07397170407648446
656657,656658,656657,1313315,793.981448173523,0.07272287488058282
658659,658660,658659,1317319,796.5742721557617,0.07149546002040097
660661,660662,660661,1321323,799.1474380493164,0.07028908407869494
662663,662664,662663,1325327,801.8214793205261,0.06910337842396075
664665,664666,664665,1329331,804.3427422046661,0.067937981082423
666667,666668,666667,1333335,806.8578443527222,0.06679253661275197
668669,668670,668669,1337339,809.4228341579437,0.06566669598430508
670671,670672,670671,1341343,812.0417683124542,0.0645601164552545
672673,672674,672673,1345347,814.5414440631866,0.06347246145548979
674675,674676,674675,1349351,817.1821472644806,0.062403400471907844
676677,676678,676677,1353355,820.3440570831299,0.06135260893336181
678679,678680,678679,1357359,823.3435320854187,0.06031976810118067
680681,680682,680681,1361363,826.2980041503906,0.05930456495877934
682683,682684,682683,1365367,828.6375453472137,0.05830669210627093
684685,684686,684685,1369371,830.7203822135925,0.05732584765507909
686687,686688,686687,1373375,833.3922669887543,0.056361735124937695
688689,688690,688689,1377379,835.4090461730957,0.0554140633444149
690691,690692,690691,1381383,837.4944021701813,0.05448254635109606
692693,692694,692693,1385387,839.5661292076111,0.05356690329529101
694695,694696,694695,1389391,841.6200520992279,0.05266685834578766
696697,696698,696697,1393395,843.7994561195374,0.05178214059549191
698699,698700,698699,1397399,846.2595620155334,0.05091248397150139
700701,700702,700701,1401403,848.6687111854553,0.05005762714506545
702703,702704,702703,1405407,851.0102090835571,0.04921731344404634
704705,704706,704705,1409411,853.9002282619476,0.048391290766630846
706707,706708,706707,1413415,856.34543633461,0.047579311497429444
708709,708710,708709,1417419,858.4698503017426,0.04678113242493964
710711,710712,710711,1421423,860.6417682170868,0.04599651465946408
712713,712714,712713,1425427,862.8127369880676,0.04522522355409819
714715,714716,714715,1429431,865.1115162372589,0.04446702862765051
716717,716718,716717,1433435,867.3141303062439,0.043721703485971375
718719,718720,718719,1437439,869.6073253154755,0.04298902574953445
720721,720722,720721,1441443,871.776397228241,0.042268776977380185
722723,722724,722723,1445447,873.9626302719116,0.04156074259697107
724725,724726,724725,1449451,876.3805413246155,0.04086471183154572
726727,726728,726727,1453455,878.7173912525177,0.04018047763224786
728729,728730,728729,1457459,880.9949362277985,0.039507836608777325
730731,730732,730731,1461463,883.4875221252441,0.03884658896311066
732733,732734,732733,1465467,885.65052318573,0.038196538424585924
734735,734736,734735,1469471,887.8222773075104,0.03755749218419169
736737,736738,736737,1473475,890.2340512275696,0.03692926083215298
738739,738740,738739,1477479,892.4953742027283,0.03631165829699512
740741,740742,740741,1481483,894.7116811275482,0.03570450178256124
742743,742744,742743,1485487,896.9493532180786,0.03510761171105514
744745,744746,744745,1489491,899.181948184967,0.034520811662559936
746747,746748,746747,1493495,901.3989591598511,0.03394392831876303
748749,748750,748749,1497499,903.6443240642548,0.033376791406908524
750751,750752,750751,1501503,905.8149690628052,0.032819233643635926
752753,752754,752753,1505507,908.0367460250854,0.032271090681433634
754755,754756,754755,1509511,910.2208092212677,0.03173220105577457
756757,756758,756757,1513515,912.3933770656586,0.031202406132479155
758759,758760,758759,1517519,914.6077451705933,0.03068155005666995
760761,760762,760761,1521523,916.810967206955,0.030169479702976787
762763,762764,762763,1525527,919.0261042118073,0.029666044626424082
764765,764766,764765,1529531,921.2735261917114,0.029171097012522296
766767,766768,766767,1533535,923.4243183135986,0.028684491632589015
768769,768770,768769,1537539,925.6588962078094,0.028206085794408864
770771,770772,770771,1541543,927.8599412441254,0.02773573929880513
772773,772774,772773,1545547,930.0389680862427,0.02727331439371028
774775,774776,774775,1549551,932.312016248703,0.026818675730282848
776777,776778,776777,1553555,934.5373811721802,0.02637169032004749
778779,778780,778779,1557559,936.9308431148529,0.025932227492262427
780781,780782,780781,1561563,939.4397151470184,0.02550015885310586
782783,782784,782783,1565567,941.9095861911774,0.025075358243611845
784785,784786,784785,1569571,944.181624174118,0.024657701700789403
786787,786788,786787,1573575,946.4922091960907,0.024247067418173174
788789,788790,788789,1577579,948.7797422409058,0.023843335706487778
790791,790792,790791,1581583,951.0021071434021,0.02344638895715434
792793,792794,792793,1585587,953.3278300762177,0.023056111603864338
794795,794796,794795,1589591,955.7221081256866,0.022672390086540872
796797,796798,796797,1593595,958.0103240013123,0.022295112816095752
798799,798800,798799,1597599,960.3419110774994,0.021924170138959198
800801,800802,800801,1601603,962.6621050834656,0.021559454302177983
802803,802804,802803,1605607,964.7439570426941,0.02120085942044625
804805,804806,804805,1609611,966.9230542182922,0.020848281442567895
806807,806808,806807,1613615,969.0820751190186,0.02050161811803264
808809,808810,808809,1617619,971.2629392147064,0.02016076896643426
810811,810812,810811,1621623,973.5199680328369,0.01982563524506986
812813,812814,812813,1625627,975.8457911014557,0.019496119918812838
814815,814816,814815,1629631,978.0582630634308,0.019172127628735325
816817,816818,816817,1633635,980.1374151706696,0.01885356466414123
818819,818820,818819,1637639,982.2050533294678,0.01854033893164342
820821,820822,820821,1641643,984.4058282375336,0.0182323599275378
822823,822824,822823,1645647,986.9726850986481,0.01792953870949532
824825,824826,824825,1649651,989.2169153690338,0.01763178786904973
826827,826828,826827,1653655,991.307920217514,0.01733902150385802
828829,828830,828829,1657659,993.3736340999603,0.017051155192234546
830831,830832,830831,1661663,995.4372711181641,0.016768105966320945
832833,832834,832833,1665667,997.5036661624908,0.0164897922865066
834835,834836,834835,1669671,999.7129981517792,0.016216134016190153
836837,836838,836837,1673675,1001.7721991539001,0.015947052397336847
838839,838840,838839,1677679,1003.8407971858978,0.01568247002649059
840841,840842,840841,1681683,1005.9057061672211,0.015422310829649177
842843,842844,842843,1685687,1007.9787933826447,0.015166500040663777
844845,844846,844845,1689691,1010.0902872085571,0.014914964177023649
846847,846848,846847,1693695,1012.1309843063354,0.014667631017573513
848849,848850,848849,1697699,1014.1973650455475,0.01442442958079937
850851,850852,850851,1701703,1016.2897479534149,0.014185290102773251
852853,852854,852853,1705707,1018.349362373352,0.013950144015211663
854855,854856,854855,1709711,1020.8120741844177,0.013718923925921445
856857,856858,856857,1713715,1023.3971762657166,0.013491563596744527
858859,858860,858859,1717719,1025.875479221344,0.013267997924685915
860861,860862,860861,1721723,1028.5172500610352,0.013048162920426876
862863,862864,862863,1725727,1030.7523062229156,0.012831995690930853
864865,864866,864865,1729731,1032.9841811656952,0.012619434418297715
866867,866868,866867,1733735,1035.5241332054138,0.01241041834225598
868869,868870,868869,1737739,1037.9363882541656,0.01220488774106343
870871,870872,870871,1741743,1040.1812751293182,0.012002783914113024
872873,872874,872873,1745747,1043.2113621234894,0.01180404916271982
874875,874876,874875,1749751,1045.4340121746063,0.011608626774545883
876877,876878,876877,1753755,1047.4888801574707,0.011416461004614575
878879,878880,878879,1757759,1049.5528151988983,0.011227497059962843
880881,880882,880881,1761763,1052.1607780456543,0.011041681081906063
882883,882884,882883,1765767,1054.5190091133118,0.01085896013034926
884885,884886,884885,1769771,1057.3569102287292,0.010679282167870952
886887,886888,886887,1773775,1060.3795990943909,0.010502596043693302
888889,888890,888889,1777779,1062.6061980724335,0.010328851478902834
890891,890892,890891,1781783,1064.8008980751038,0.010157999050420585
892893,892894,892893,1785787,1066.9623851776123,0.009989990176791252
894895,894896,894895,1789791,1069.194337129593,0.009824777103290216
896897,896898,896897,1793795,1071.320400238037,0.009662312887940061
898899,898900,898899,1797799,1074.5202431678772,0.009502551386958658
900901,900902,900901,1801803,1076.8162531852722,0.009345447241116744
902903,902904,902903,1805807,1078.9454782009125,0.009190955862891315
904905,904906,904905,1809811,1081.0598289966583,0.009039033421345266
906907,906908,906907,1813815,1083.205830335617,0.008889636830645031
908909,908910,908909,1817819,1085.3578102588654,0.008742723736872904
910911,910912,910911,1821823,1087.425302028656,0.008598252504498305
912913,912914,912913,1825827,1089.709635257721,0.00845618220535016
914915,914916,914915,1829831,1091.8833441734314,0.008316472604974479
916917,916918,916917,1833835,1093.985100030899,0.00817908415194779
918919,918920,918919,1837839,1096.156655073166,0.008043977965030535
920921,920922,920921,1841843,1098.3118541240692,0.007911115822253123
922923,922924,922923,1845847,1100.4050223827362,0.007780460149319879
924925,924926,924925,1849851,1102.5804522037506,0.007651974008467732
926927,926928,926927,1853855,1104.7086441516876,0.007525621087552281
928929,928930,928929,1857859,1106.8215301036835,0.007401365689361228
930931,930932,930931,1861863,1108.8905100822449,0.007279172720586757
932933,932934,932933,1865867,1111.0044343471527,0.007159007682048468
934935,934936,934935,1869871,1113.104165315628,0.007040836658120497
936937,936938,936937,1873875,1115.2054042816162,0.006924626306840764
938939,938940,938939,1877879,1117.3523173332214,0.006810343849451783
940941,940942,940941,1881883,1119.4862871170044,0.006697957062328896
942943,942944,942943,1885887,1122.300695180893,0.006587434265043157
944945,944946,944945,1889891,1124.9055652618408,0.006478744313653806
946947,946948,946947,1893895,1127.6622033119202,0.006371856588998526
948949,948950,948949,1897899,1130.0714161396027,0.006266740989872233
950951,950952,950951,1901903,1132.9171230793,0.006163367922908947
952953,952954,952953,1905907,1135.6849291324615,0.0060617082938279054
954955,954956,954955,1909911,1138.36883020401,0.005961733499361799
956957,956958,956957,1913915,1140.9703443050385,0.00586341541929869
958959,958960,958959,1917919,1143.2789902687073,0.0057667264065912605
960961,960962,960961,1921923,1145.3919820785522,0.005671639280990348
962963,962964,962963,1925927,1147.5318593978882,0.0055781273197226255
964965,964966,964965,1929931,1150.1412091255188,0.005486164251465198
966967,966968,966967,1933935,1152.7992181777954,0.005395724245886413
968969,968970,968969,1937939,1155.3255171775818,0.005306781908871017
970971,970972,970971,1941943,1158.0445861816406,0.0052193122736525766
972973,972974,972973,1945947,1160.6136093139648,0.0051332907931964655
974975,974976,974975,1949951,1163.0657563209534,0.005048693334288146
976977,976978,976977,1953955,1165.7702062129974,0.004965496169006656
978979,978980,978979,1957959,1168.531524181366,0.004883675969267642
980981,980982,980981,1961963,1170.8666710853577,0.004803209798978969
982983,982984,982983,1965967,1173.1699299812317,0.004724075107674253
984985,984986,984985,1969971,1175.5082013607025,0.004646249723919027
986987,986988,986987,1973975,1177.7851531505585,0.004569711849285341
988989,988990,988989,1977979,1180.2882571220398,0.004494440050734738
990991,990992,990991,1981983,1182.9855341911316,0.004420413256411848
992993,992994,992993,1985987,1185.261782169342,0.0043476107470041825
994995,994996,994995,1989991,1187.6047410964966,0.004276012152445219
996997,996998,996997,1993995,1189.9512152671814,0.004205597443615261
998999,999000,998999,1997999,1192.3411672115326,0.004136346928135026
1001001,1001002,1001001,2002003,1194.8167781829834,0.004068241243658122
1003003,1003004,1003003,2006007,1197.1719810962677,0.0040012613528688235
1005005,1005006,1005005,2010011,1199.3794782161713,0.003935388537684048
1007007,1007008,1007007,2014015,1201.614478111267,0.0038706043940237578
1009009,1009010,1009009,2018019,1204.2271931171417,0.0038068908263539925
1011011,1011012,1011011,2022023,1206.2877871990204,0.003744230041888841
1013013,1013014,1013013,2026027,1208.5749261379242,0.003682604546725088
1015015,1015016,1015015,2030031,1210.9348783493042,0.0036219971400441864
1017017,1017018,1017017,2034035,1213.1880640983582,0.0035623909087689754
1019019,1019020,1019019,2038039,1215.3308563232422,0.0035037692230162065
1021021,1021022,1021021,2042043,1218.1480913162231,0.0034461157320038183
1023023,1023024,1023023,2046047,1220.1748132705688,0.0033894143579118463
1025025,1025026,1025025,2050051,1222.2618401050568,0.0033336492924718186
1027027,1027028,1027027,2054055,1224.407692193985,0.003278804991623474
1029029,1029030,1029029,2058059,1226.4741320610046,0.003224866172331531
1031031,1031032,1031031,2062063,1228.535471200943,0.00317181780599185
1033033,1033034,1033033,2066067,1230.6524722576141,0.0031196451154755778
1035035,1035036,1035035,2070071,1232.9386551380157,0.0030683335721732874
1037037,1037038,1037037,2074075,1235.1354501247406,0.0030178688883779614
1039039,1039040,1039039,2078079,1237.4506721496582,0.0029682370167165573
1041041,1041042,1041041,2082083,1239.6317381858826,0.0029194241435561707
1043043,1043044,1043043,2086087,1241.9600751399994,0.0028714166871850466
1045045,1045046,1045045,2090091,1244.5244841575623,0.0028242012916734893
1047047,1047048,1047047,2094095,1246.732135295868,0.0027777648246001263
1049049,1049050,1049049,2098099,1249.560039281845,0.002732094373413929
1051051,1051052,1051051,2102103,1251.9772911071777,0.0026871772399772453
1053053,1053054,1053053,2106107,1254.0928401947021,0.00264300093942893
1055055,1055056,1055055,2110111,1257.0956852436066,0.002599553194386317
1057057,1057058,1057057,2114115,1259.423079252243,0.0025568219325577957
1059059,1059060,1059059,2118119,1261.4677441120148,0.002514795283445892
1061061,1061062,1061061,2122123,1263.5260400772095,0.0024734615739134824
1063063,1063064,1063063,2126127,1265.5768942832947,0.002432809326478491
1065065,1065066,1065065,2130131,1267.6188271045685,0.0023928272539706086
1067067,1067068,1067067,2134135,1269.6467893123627,0.0023535042582807364
1069069,1069070,1069069,2138139,1271.7201263904572,0.0023148294260408875
1071071,1071072,1071071,2142143,1273.7711281776428,0.0022767920256683283
1073073,1073074,1073073,2146147,1275.9714543819427,0.002239381504409721
1075075,1075076,1075075,2150151,1278.037364244461,0.002202587485726326
1077077,1077078,1077077,2154155,1280.0908341407776,0.0021663997652012768
1079079,1079080,1079079,2158159,1283.5019991397858,0.002130808309289023
1081081,1081082,1081081,2162163,1285.7625510692596,0.0020958032511089186
1083083,1083084,1083083,2166167,1287.9974081516266,0.002061374887716738
1085085,1085086,1085085,2170171,1290.2491693496704,0.0020275136788541204
1087087,1087088,1087087,2174175,1292.4980311393738,0.001994210241946348
1089089,1089090,1089089,2178179,1294.7663700580597,0.0019614553509654797
1091091,1091092,1091091,2182183,1296.9687941074371,0.0019292399335881782
1093093,1093094,1093093,2186187,1299.1187472343445,0.0018975550681261666
1095095,1095096,1095095,2190191,1301.319542169571,0.001866391981934612
1097097,1097098,1097097,2194195,1303.7209441661835,0.0018357420473193997
1099099,1099100,1099099,2198199,1305.9268951416016,0.001805596780968699
1101101,1101102,1101101,2202203,1308.1688861846924,0.0017759478403149842
1103103,1103104,1103103,2206207,1310.4853880405426,0.0017467870217160453
1105105,1105106,1105105,2210211,1312.546067237854,0.0017181062573854433
1107107,1107108,1107107,2214215,1314.457887172699,0.001689897613687208
1109109,1109110,1109109,2218219,1316.3134751319885,0.001662153289885282
1111111,1111112,1111111,2222223,1318.1481909751892,0.0016348656134823614
1113113,1113114,1113113,2226227,1320.0358493328094,0.0016080270404472685
1115115,1115116,1115115,2230231,1322.2218461036682,0.0015816301516906606
1117117,1117118,1117117,2234235,1324.1415350437164,0.00155566765124604
1119119,1119120,1119119,2238239,1326.231944322586,0.0015301323646781384
1121121,1121122,1121121,2242243,1328.4589731693268,0.0015050172361270597
1123123,1123124,1123123,2246247,1330.8714501857758,0.0014803153276261583
1125125,1125126,1125125,2250251,1333.3365733623505,0.0014560198160324944
1127127,1127128,1127127,2254255,1335.7756612300873,0.0014321239910941586
1129129,1129130,1129129,2258259,1338.1173272132874,0.0014086212547681498
1131131,1131132,1131131,2262263,1340.5541491508484,0.0013855051174687105
1133133,1133134,1133133,2266267,1343.1789700984955,0.0013627691982946999
1135135,1135136,1135135,2270271,1345.793743133545,0.0013404072216189888
1137137,1137138,1137137,2274275,1348.1536660194397,0.0013184130160652785
1139139,1139140,1139139,2278279,1350.5362989902496,0.0012967805128027976
1141141,1141142,1141141,2282283,1353.0203230381012,0.001275503743045192
1143143,1143144,1143143,2286287,1355.7530512809753,0.0012545768379368383
1145145,1145146,1145145,2290291,1358.4144022464752,0.0012339940251422377
1147147,1147148,1147147,2294295,1361.3713910579681,0.0012137496283912697
1149149,1149150,1149149,2298299,1364.0423061847687,0.0011938380654328284
1151151,1151152,1151151,2302303,1366.824567079544,0.0011742538463295205
1153153,1153154,1153153,2306307,1369.5287051200867,0.0011549915724344828
1155155,1155156,1155155,2310311,1372.0178802013397,0.0011360459343450202
1157157,1157158,1157157,2314315,1374.3111772537231,0.0011174117111067972
1159159,1159160,1159159,2318319,1376.4112980365753,0.001099083767371667
1161161,1161162,1161161,2322323,1378.56765127182,0.001081057053738732
1163163,1163164,1163163,2326327,1380.7185153961182,0.0010633266039121736
1165165,1165166,1165165,2330331,1383.2383670806885,0.0010458875341328167
1167167,1167168,1167167,2334335,1385.8589360713959,0.0010287350413591412
1169169,1169170,1169169,2338339,1389.0954780578613,0.001011864401789353
1171171,1171172,1171171,2342343,1391.472924232483,0.0009952709705203233
1173173,1173174,1173173,2346347,1393.9734163284302,0.0009789501791601651
1175175,1175176,1175175,2350351,1396.4904992580414,0.000962897534577678
1177177,1177178,1177177,2354355,1398.9983921051025,0.0009471086187886613
1179179,1179180,1179179,2358359,1401.0524551868439,0.0009315790860000561
1181181,1181182,1181181,2362363,1402.9503972530365,0.0009163046635194405
1183183,1183184,1183183,2366367,1404.8616650104523,0.0009012811478896765
1185185,1185186,1185185,2370371,1406.7294611930847,0.0008865044065942129
1187187,1187188,1187187,2374375,1408.5671360492706,0.0008719703744191065
1189189,1189190,1189189,2378379,1410.370450258255,0.0008576750537940825
1191191,1191192,1191191,2382383,1412.1848492622375,0.0008436145135419792
1193193,1193194,1193193,2386387,1414.0001673698425,0.0008297848870597591
1195195,1195196,1195195,2390391,1415.8314633369446,0.0008161823717500738
1197197,1197198,1197197,2394395,1417.7210323810577,0.0008028032279980835
1199199,1199200,1199199,2398399,1419.5677301883698,0.0007896437782619614
1201201,1201202,1201201,2402403,1421.4268610477448,0.000776700405253905
1203203,1203204,1203203,2406407,1423.182498216629,0.0007639695514853884
1205205,1205206,1205205,2410411,1424.988319158554,0.0007514477191534752
1207207,1207208,1207207,2414415,1426.8349282741547,0.0007391314670712745
1209209,1209210,1209209,2418419,1428.7253832817078,0.0007270174114637484
1211211,1211212,1211211,2422423,1431.5391612052917,0.0007151022247171568
1213213,1213214,1213213,2426427,1433.33420920372,0.0007033826340148153
1215215,1215216,1215215,2430431,1435.0761482715607,0.0006918554200865401
1217217,1217218,1217217,2434435,1437.0924081802368,0.0006805174175497086
1219219,1219220,1219219,2438439,1438.9062063694,0.0006693655128628961
1221221,1221222,1221221,2442443,1441.0520651340485,0.0006583966442121891
1223223,1223224,1223223,2446447,1443.9855360984802,0.00064760780026063
1225225,1225226,1225225,2450451,1446.757259130478,0.000636996018897662
1227227,1227228,1227227,2454455,1448.8933081626892,0.0006265583876938763
1229229,1229230,1229229,2458459,1450.9510452747345,0.000616292041968336
1231231,1231232,1231231,2462463,1453.0181312561035,0.0006061941639927682
1233233,1233234,1233233,2466467,1455.055857181549,0.0005962619831052507
1235235,1235236,1235235,2470471,1457.0987341403961,0.0005864927740049097
1237237,1237238,1237237,2474475,1459.1687133312225,0.000576883856524546
1239239,1239240,1239239,2478479,1461.2784292697906,0.00056743259472114
1241241,1241242,1241241,2482483,1463.709720134735,0.0005581363960800445
1243243,1243244,1243243,2486487,1466.3196983337402,0.0005489927107191761
1245245,1245246,1245245,2490491,1469.0143122673035,0.000539999031161642
1247247,1247248,1247247,2494495,1471.172743320465,0.0005311528911988717
1249249,1249250,1249249,2498499,1473.6917560100555,0.0005224518650948085
1251251,1251252,1251251,2502503,1476.0801901817322,0.0005138935671311629
1253253,1253254,1253253,2506507,1478.391636133194,0.0005054756514937253
1255255,1255256,1255255,2510511,1480.4885032176971,0.0004971958099986296
1257257,1257258,1257257,2514515,1482.5204751491547,0.0004890517735702815
1259259,1259260,1259259,2518519,1484.550014257431,0.00048104130974024883
1261261,1261262,1261261,2522523,1486.5887641906738,0.00047316222389781615
1263263,1263264,1263263,2526527,1488.6121771335602,0.0004654123562204404
1265265,1265266,1265265,2530531,1490.602679014206,0.0004577895833790535
1267267,1267268,1267267,2534535,1492.5633862018585,0.00045029181717382016
1269269,1269270,1269269,2538539,1494.4360961914062,0.00044291700305620907
1271271,1271272,1271271,2542543,1496.579166173935,0.0004356631211521744
1273273,1273274,1273273,2546547,1499.0668642520905,0.0004285281843294797
1275275,1275276,1275275,2550551,1501.3359291553497,0.0004215102384250713
1277277,1277278,1277277,2554555,1503.6643161773682,0.0004146073614492707
1279279,1279280,1279279,2558559,1505.98495221138,0.0004078176632447139
1281281,1281282,1281281,2562563,1508.0931651592255,0.00040113928412210953
1283283,1283284,1283283,2566567,1510.6822972297668,0.00039457039599710697
1285285,1285286,1285285,2570571,1512.6912531852722,0.0003881092003439335
1287287,1287288,1287287,2574575,1514.6833033561707,0.00038175392830908095
1289289,1289290,1289289,2578579,1516.77956032753,0.0003755028400291849
1291291,1291292,1291291,2582583,1518.998693227768,0.00036935422451733757
1293293,1293294,1293293,2586587,1521.344279050827,0.0003633063988672802
1295295,1295296,1295295,2590591,1523.7385931015015,0.0003573577083670898
1297297,1297298,1297297,2594595,1525.587776184082,0.0003515065246801896
1299299,1299300,1299299,2598599,1527.5868201255798,0.0003457512466411572
1301301,1301302,1301301,2602603,1529.7176892757416,0.0003400902999146638
1303303,1303304,1303303,2606607,1531.7785782814026,0.0003345221351764849
1305305,1305306,1305305,2610611,1533.7900080680847,0.0003290452298188029
1307307,1307308,1307307,2614615,1535.7973229885101,0.00032365808499434934
1309309,1309310,1309309,2618619,1537.941004037857,0.00031835922720802046
1311311,1311312,1311311,2622623,1540.691546201706,0.00031314720729369583
1313313,1313314,1313313,2626627,1543.1299781799316,0.0003080205996184304
1315315,1315316,1315315,2630631,1545.335966348648,0.00030297800242351514
1317317,1317318,1317317,2634635,1547.9879002571106,0.0002980180364602347
1319319,1319320,1319319,2638639,1550.8601961135864,0.000293139345558302
1321321,1321322,1321321,2642643,1553.1318871974945,0.00028834059583005
1323323,1323324,1323323,2646647,1555.2193472385406,0.0002836204753293714
1325325,1325326,1325325,2650651,1557.2101881504059,0.0002789776935969712
1327327,1327328,1327327,2654655,1559.1453292369843,0.00027441098143299314
1329329,1329330,1329329,2658659,1561.9806201457977,0.000269919090555959
1331331,1331332,1331331,2662663,1564.384889125824,0.00026550079292064765
1333333,1333334,1333333,2666667,1566.757558107376,0.0002611548812865294
1335335,1335336,1335335,2670671,1568.8532102108002,0.00025688016785352374
1337337,1337338,1337337,2674675,1570.9877932071686,0.00025267548414831253
1339339,1339340,1339339,2678679,1573.35000705719,0.00024853968147908745
1341341,1341342,1341341,2682683,1576.0137991905212,0.0002444716300260552
1343343,1343344,1343343,2686687,1578.1671812534332,0.00024047021770456922
1345345,1345346,1345345,2690691,1580.3447680473328,0.00023653435152937163
1347347,1347348,1347347,2694695,1582.5681700706482,0.00023266295647772495
1349349,1349350,1349349,2698699,1585.2064383029938,0.0002288549744662305
1351351,1351352,1351351,2702703,1587.750158071518,0.00022510936571507045
1353353,1353354,1353353,2706707,1591.2707200050354,0.0002214251069290185
1355355,1355356,1355355,2710711,1594.3498821258545,0.00021780119197956083
1357357,1357358,1357357,2714715,1596.867522239685,0.00021423663099540136
1359359,1359360,1359359,2718719,1599.4958522319794,0.0002107304504761487
1361361,1361362,1361361,2722723,1601.9854242801666,0.00020728169329231605
1363363,1363364,1363363,2726727,1604.5351402759552,0.0002038894172073924
1365365,1365366,1365365,2730731,1607.1892552375793,0.00020055269612839766
1367367,1367368,1367367,2734735,1609.920359134674,0.00019727061942376167
1369369,1369370,1369369,2738739,1612.6001372337341,0.0001940422903317085
1371371,1371372,1371371,2742743,1615.296625137329,0.0001908668281203063
1373373,1373374,1373373,2746747,1619.2620830535889,0.00018774336547267012
1375375,1375376,1375375,2750751,1622.8189301490784,0.00018467105007857754
1377377,1377378,1377377,2754755,1626.7747201919556,0.00018164904315653985
1379379,1379380,1379379,2758759,1630.5735251903534,0.0001786765196811757
1381381,1381382,1381381,2762763,1634.1573061943054,0.00017575266895164532
1383383,1383384,1383383,2766767,1637.7038731575012,0.0001728766923179137
1385385,1385386,1385385,2770771,1641.2598819732666,0.0001700478054544874
1387387,1387388,1387387,2774775,1644.0515441894531,0.00016726523608667776
1389389,1389390,1389389,2778779,1645.939462184906,0.00016452822512746934
1391391,1391392,1391391,2782783,1647.8761520385742,0.00016183602542696462
1393393,1393394,1393393,2786787,1650.0838191509247,0.00015918790256819193
1395395,1395396,1395395,2790791,1652.4033341407776,0.00015658313418498437
1397397,1397398,1397397,2794795,1654.5120272636414,0.00015402100996197987
1399399,1399400,1399399,2798799,1656.922348022461,0.00015150083015669225
1401401,1401402,1401401,2802803,1659.7955520153046,0.00014902190787324798
1403403,1403404,1403403,2806807,1662.2319161891937,0.00014658356667496264
1405405,1405406,1405405,2810811,1664.49463224411,0.00014418514149383554
1407407,1407408,1407407,2814815,1666.3423421382904,0.00014182597840317612
1409409,1409410,1409409,2818819,1668.240555047989,0.00013950543359442236
1411411,1411412,1411411,2822823,1670.2248282432556,0.0001372228742866355
1413413,1413414,1413413,2826827,1672.1851062774658,0.00013497767815806583
1415415,1415416,1415415,2830831,1674.3281302452087,0.00013276923266403173
1417417,1417418,1417417,2834835,1676.1695411205292,0.00013059693617378798
1419419,1419420,1419419,2838839,1678.172904253006,0.00012846019558310218
1421421,1421422,1421421,2842843,1680.1632702350616,0.00012635842892905202
1423423,1423424,1423423,2846847,1682.0626561641693,0.00012429106266154122
1425425,1425426,1425425,2850851,1684.0048162937164,0.000122257533348602
1427427,1427428,1427427,2854855,1686.0637822151184,0.00012025728665321367
1429429,1429430,1429429,2858859,1687.9987063407898,0.00011828977721961564
1431431,1431432,1431431,2862863,1689.8602900505066,0.0001163544687869944
1433433,1433434,1433433,2866867,1691.7059090137482,0.00011445083373473608
1435435,1435436,1435435,2870871,1693.5749843120575,0.00011257835296873964
1437437,1437438,1437437,2874875,1695.4759922027588,0.00011073651637616422
1439439,1439440,1439439,2878879,1697.3360812664032,0.0001089248218022476
1441441,1441442,1441441,2882883,1699.214765071869,0.00010714277573242725
1443443,1443444,1443443,2886887,1701.1033961772919,0.0001053898921554719
1445445,1445446,1445445,2890891,1702.9999392032623,0.00010366569358666311
1447447,1447448,1447447,2894895,1704.9969279766083,0.00010196970993092691
1449449,1449450,1449449,2898899,1706.9692060947418,0.00010030147939232847
1451451,1451452,1451451,2902903,1708.9324610233307,9.866054710983008e-05
1453453,1453454,1453453,2906907,1710.7838802337646,9.70464660667858e-05
1455455,1455456,1455455,2910911,1712.6189119815826,9.545879640882049e-05
1457457,1457458,1457457,2914915,1714.462384223938,9.389710567120346e-05
1459459,1459460,1459459,2918919,1716.3520221710205,9.236096832410112e-05
1461461,1461462,1461461,2922923,1718.307018995285,9.084996577257698e-05
1463463,1463464,1463463,2926927,1720.2584981918335,8.936368647027848e-05
1465465,1465466,1465465,2930931,1722.2293412685394,8.79017255783765e-05
1467467,1467468,1467467,2934935,1724.1674642562866,8.64636848518785e-05
1469469,1469470,1469469,2938939,1726.068528175354,8.504917229856801e-05
1471471,1471472,1471471,2942943,1727.9444222450256,8.365780286112567e-05
1473473,1473474,1473473,2946947,1729.7966830730438,8.22891977350082e-05
1475475,1475476,1475475,2950951,1731.6467621326447,8.094298380001419e-05
1477477,1477478,1477477,2954955,1733.5285003185272,7.961879441609199e-05
1479479,1479480,1479479,2958959,1735.416570186615,7.831626942333969e-05
1481481,1481482,1481481,2962963,1737.3814573287964,7.70350537777631e-05
1483483,1483484,1483483,2966967,1739.332602262497,7.577479823339672e-05
1485485,1485486,1485485,2970971,1741.2400772571564,7.453516013811168e-05
1487487,1487488,1487487,2974975,1743.1468060016632,7.331580172831309e-05
1489489,1489490,1489489,2978979,1745.074909210205,7.211639081106114e-05
1491491,1491492,1491491,2982983,1746.9580841064453,7.093660099144472e-05
1493493,1493494,1493493,2986987,1748.774500131607,6.977611099046044e-05
1495495,1495496,1495495,2990991,1750.6107711791992,6.863460487238626e-05
1497497,1497498,1497497,2994995,1752.4298181533813,6.751177181740786e-05
1499499,1499500,1499499,2998999,1754.36927318573,6.640730589424493e-05
1501502,1501503,1501502,3003005,1756.2052080631256,6.53203687761561e-05
1503504,1503505,1503504,3007009,1758.025547027588,6.42517492224215e-05
1505506,1505507,1505506,3011013,1759.8068630695343,6.320060958842078e-05
1507508,1507509,1507508,3015017,1761.6572012901306,6.216666383807024e-05
1509510,1509511,1509510,3019021,1763.49964427948,6.1149630255386e-05
1511512,1511513,1511512,3023025,1765.3991022109985,6.014923212660506e-05
1513514,1513515,1513514,3027029,1767.2704641819,5.916519705806422e-05
1515516,1515517,1515516,3031033,1769.1513800621033,5.8197257317260664e-05
1517518,1517519,1517518,3035037,1771.0321111679077,5.724514937810454e-05
1519520,1519521,1519520,3039041,1772.9127123355865,5.630861403460585e-05
1521522,1521523,1521522,3043045,1774.7639203071594,5.5387396741934936e-05
1523524,1523525,1523524,3047049,1776.6182851791382,5.44812464795541e-05
1525526,1525527,1525526,3051053,1778.4508574008942,5.3589916547025496e-05
1527528,1527529,1527528,3055057,1780.5595331192017,5.2713164564011095e-05
1529530,1529531,1529530,3059061,1783.0683462619781,5.1850752129212196e-05
1531532,1531533,1531532,3063065,1785.6638813018799,5.100244391087472e-05
1533534,1533535,1533534,3067069,1787.9977202415466,5.016800992052595e-05
1535536,1535537,1535536,3071073,1790.135362148285,4.934722244342993e-05
1537538,1537539,1537538,3075077,1792.306223154068,4.853985842601105e-05
1539540,1539541,1539540,3079081,1794.458999156952,4.7745698338985676e-05
1541542,1541543,1541542,3083085,1796.509369134903,4.696452583630162e-05
1543544,1543545,1543544,3087089,1798.5196900367737,4.619612832357234e-05
1545546,1545547,1545546,3091093,1800.432097196579,4.544029707176378e-05
1547548,1547549,1547548,3095097,1802.333036184311,4.469682619401283e-05
1549550,1549551,1549550,3099101,1804.1762759685516,4.396551344143518e-05
1551552,1551553,1551552,3103105,1806.250158071518,4.3246159862064815e-05
1553554,1553555,1553554,3107109,1808.2610869407654,4.2538570028227696e-05
1555556,1555557,1555556,3111113,1810.1434559822083,4.1842551127047045e-05
1557558,1557559,1557558,3115117,1812.0528650283813,4.1157913983624894e-05
1559560,1559561,1559560,3119121,1813.8898780345917,4.048447203786054e-05
1561562,1561563,1561562,3123125,1815.7001264095306,3.982204259500577e-05
1563564,1563565,1563564,3127129,1817.8334941864014,3.917044546142279e-05
1565566,1565567,1565566,3131133,1820.2495889663696,3.852950294458424e-05
1567568,1567569,1567568,3135137,1822.6455261707306,3.789904098994157e-05
1569570,1569571,1569570,3139141,1824.8130853176117,3.7278888157743495e-05
1571572,1571573,1571572,3143145,1826.9305651187897,3.666887573672284e-05
1573574,1573575,1573574,3147149,1829.1158912181854,3.60688379714702e-05
1575576,1575577,1575576,3151153,1831.3170051574707,3.54786112666261e-05
1577578,1577579,1577578,3155157,1833.4672372341156,3.489803555112303e-05
1579580,1579581,1579580,3159161,1835.5658881664276,3.432695268656971e-05
1581582,1581583,1581582,3163165,1837.8032031059265,3.376520726305898e-05
1583584,1583585,1583584,3167169,1839.5869660377502,3.321264682654146e-05
1585586,1585587,1585586,3171173,1841.5174372196198,3.2669120855643996e-05
1587588,1587589,1587588,3175177,1843.5516772270203,3.213448178485123e-05
1589590,1589591,1589590,3179181,1845.6037240028381,3.1608583981324045e-05
1591592,1591593,1591592,3183185,1847.5273311138153,3.109128465439426e-05
1593594,1593595,1593594,3187189,1849.4603261947632,3.058244317344361e-05
1595596,1595597,1595596,3191193,1851.3735632896423,3.0081920954216912e-05
1597598,1597599,1597598,3195197,1853.3133962154388,2.9589581913569418e-05
1599600,1599601,1599600,3199201,1855.1879251003265,2.910529258315364e-05
1601602,1601603,1601602,3203205,1857.0550022125244,2.8628921086237824e-05
1603604,1603605,1603604,3207209,1858.899146080017,2.816033747876645e-05
1605606,1605607,1605606,3211213,1860.7347021102905,2.769941499991546e-05
1607608,1607609,1607608,3215217,1862.614827156067,2.7246027912042337e-05
1609610,1609611,1609610,3219221,1864.4746260643005,2.6800053092301823e-05
1611612,1611613,1611612,3223225,1866.3795471191406,2.6361369464211748e-05
1613614,1613615,1613614,3227229,1868.2723541259766,2.5929857656592503e-05
1615616,1615617,1615616,3231233,1870.2301633358002,2.5505400117253885e-05
1617618,1617619,1617618,3235237,1872.1608309745789,2.5087881795116118e-05
1619620,1619621,1619620,3239241,1874.017753124237,2.467718911702832e-05
1621622,1621623,1621622,3243245,1875.8831181526184,2.427321032882901e-05
1623624,1623625,1623624,3247249,1877.8915841579437,2.3875835836406623e-05
1625626,1625627,1625626,3251253,1879.7247092723846,2.348495729620481e-05
1627628,1627629,1627628,3255257,1881.5668280124664,2.3100468865777657e-05
1629630,1629631,1629630,3259261,1883.3421161174774,2.2722265612173942e-05
1631632,1631633,1631632,3263265,1885.1131629943848,2.235024498986604e-05
1633634,1633635,1633634,3267269,1886.908818244934,2.198430593125522e-05
1635636,1635637,1635636,3271273,1888.739580154419,2.1624348846671637e-05
1637638,1637639,1637638,3275277,1890.5690932273865,2.127027596543485e-05
1639640,1639641,1639640,3279281,1892.350063085556,2.0921991108480142e-05
1641642,1641643,1641642,3283285,1894.0895681381226,2.057939946098486e-05
1643644,1643645,1643644,3287289,1895.8543133735657,2.0242408027115744e-05
1645646,1645647,1645646,3291293,1897.6069633960724,1.991092517528159e-05
1647648,1647649,1647648,3295297,1899.3004369735718,1.9584860865506926e-05
1649650,1649651,1649650,3299301,1901.0030462741852,1.9264126649432e-05
1651652,1651653,1651652,3303305,1902.6930561065674,1.8948634874504933e-05
1653654,1653655,1653654,3307309,1904.4507982730865,1.8638300389284268e-05
1655656,1655657,1655656,3311313,1906.217740058899,1.8333038497075904e-05
1657658,1657659,1657658,3315317,1907.9893600940704,1.8032766206488304e-05
1659660,1659661,1659660,3319321,1909.7177662849426,1.7737402231432498e-05
1661662,1661663,1661662,3323325,1911.4169600009918,1.7446866195314215e-05
1663664,1663665,1663664,3327329,1913.1136441230774,1.716107908578124e-05
1665666,1665667,1665666,3331333,1914.9025242328644,1.687996314103657e-05
1667668,1667669,1667668,3335337,1916.7459602355957,1.660344219089893e-05
1669670,1669671,1669670,3339341,1918.6857752799988,1.6331440974681755e-05
1671672,1671673,1671672,3343345,1920.6089379787445,1.606388559594052e-05
1673674,1673675,1673674,3347349,1922.4648711681366,1.580070340878592e-05
1675676,1675677,1675676,3351353,1924.1271350383759,1.5541822790510196e-05
1677678,1677679,1677678,3355357,1925.8556821346283,1.5287173710021307e-05
1679680,1679681,1679680,3359361,1927.6517992019653,1.503668647728773e-05
1681682,1681683,1681682,3363365,1929.4878482818604,1.4790293789701536e-05
1683684,1683685,1683684,3367369,1931.3209471702576,1.4547927889907442e-05
1685686,1685687,1685686,3371373,1933.0615952014923,1.4309523294286919e-05
1687688,1687689,1687688,3375377,1934.8375651836395,1.4075015315029304e-05
1689690,1689691,1689690,3379381,1936.5531771183014,1.3844340173818637e-05
1691692,1691693,1691692,3383385,1938.2405281066895,1.3617435115520493e-05
1693694,1693695,1693694,3387389,1939.9355680942535,1.3394238635555666e-05
1695696,1695697,1695696,3391393,1941.6477313041687,1.3174690025152813e-05
1697698,1697699,1697698,3395397,1943.3906590938568,1.2958729939782643e-05
1699700,1699701,1699700,3399401,1945.1509461402893,1.2746298921229027e-05
1701702,1701703,1701702,3403405,1946.9084331989288,1.2537340239759942e-05
1703704,1703705,1703704,3407409,1948.678705215454,1.2331796597209177e-05
1705706,1705707,1705706,3411413,1950.357327222824,1.2129611832278897e-05
1707708,1707709,1707708,3415417,1952.074386358261,1.1930731943721185e-05
1709710,1709711,1709710,3419421,1953.7672402858734,1.1735101907106582e-05
1711712,1711713,1711712,3423425,1955.4566230773926,1.1542669426489738e-05
1713714,1713715,1713714,3427429,1957.1816849708557,1.1353381751177949e-05
1715716,1715717,1715716,3431433,1958.9523792266846,1.1167187608407403e-05
1717718,1717719,1717718,3435437,1960.7257351875305,1.0984036293848476e-05
1719720,1719721,1719720,3439441,1962.4351150989532,1.0803878353726759e-05
1721722,1721723,1721722,3443445,1964.1247701644897,1.0626664561641519e-05
1723724,1723725,1723724,3447449,1965.8320870399475,1.0452346941747237e-05
1725726,1725727,1725726,3451453,1967.5248801708221,1.0280878200319421e-05
1727728,1727729,1727728,3455457,1969.2094180583954,1.0112211384694092e-05
1729730,1729731,1729730,3459461,1970.9297263622284,9.946301247509837e-06
1731732,1731733,1731732,3463465,1972.6417860984802,9.783102314031566e-06
1733734,1733735,1733734,3467469,1974.3674981594086,9.622570360079408e-06
1735736,1735737,1735736,3471473,1976.1149580478668,9.464662070968188e-06
1737738,1737739,1737738,3475477,1977.8747293949127,9.309334018325899e-06
1739740,1739741,1739740,3479481,1979.5564501285553,9.156544592769933e-06
1741742,1741743,1741742,3483485,1981.2537262439728,9.00625195754401e-06
1743744,1743745,1743744,3487489,1982.8966131210327,8.858415299073386e-06
1745746,1745747,1745746,3491493,1984.588875055313,8.712994713278022e-06
1747748,1747749,1747748,3495497,1986.3765749931335,8.569950296077877e-06
1749750,1749751,1749750,3499501,1988.1390793323517,8.429243621321802e-06
1751752,1751753,1751752,3503505,1989.8781971931458,8.29083614917181e-06
1753754,1753755,1753754,3507509,1991.5771782398224,8.154690704031964e-06
1755756,1755757,1755756,3511513,1993.2520191669464,8.020769655558979e-06
1757758,1757759,1757758,3515517,1994.9563591480255,7.889037306085811e-06
1759760,1759761,1759760,3519521,1996.6587970256805,7.75945773057174e-06
1761762,1761763,1761762,3523525,1998.3666303157806,7.631995345036557e-06
1763764,1763765,1763764,3527529,2000.0707120895386,7.506616043428949e-06
1765766,1765767,1765766,3531533,2001.8123903274536,7.383285378637083e-06
1767768,1767769,1767768,3535537,2003.5480182170868,7.261970154104347e-06
1769770,1769771,1769770,3539541,2005.2449700832367,7.142637286960962e-06
1771772,1771773,1771772,3543545,2006.9343872070312,7.0252544901450165e-06
1773774,1773775,1773774,3547549,2008.6554334163666,6.9097899313419475e-06
1775776,1775777,1775776,3551553,2010.3440272808075,6.796211891924031e-06
1777778,1777779,1777778,3555557,2012.0510301589966,6.684489903818758e-06
1779780,1779781,1779780,3559561,2013.733852148056,6.574593271579943e-06
1781782,1781783,1781782,3563565,2015.4374871253967,6.466492664003454e-06
1783784,1783785,1783784,3567569,2017.0964033603668,6.360158295137808e-06
1785786,1785787,1785786,3571573,2018.8401362895966,6.255561629586737e-06
1787788,1787789,1787788,3575577,2020.6043021678925,6.152673904580297e-06
1789790,1789791,1789790,3579581,2022.3167653083801,6.051467494216922e-06
1791792,1791793,1791792,3583585,2024.005564212799,5.9519149999687215e-06
1793794,1793795,1793794,3587589,2025.6777453422546,5.853988909620966e-06
1795796,1795797,1795796,3591593,2027.379316329956,5.757662847827305e-06
1797798,1797799,1797798,3595597,2029.0701141357422,5.662911121362413e-06
1799800,1799801,1799800,3599601,2030.7804281711578,5.569707354879938e-06
1801802,1801803,1801802,3603605,2032.467357158661,5.478026537275582e-06
1803804,1803805,1803804,3607609,2034.1883692741394,5.3878438848187216e-06
1805806,1805807,1805806,3611613,2035.8775432109833,5.2991345000918955e-06
1807808,1807809,1807808,3615617,2037.5836012363434,5.211874736232858e-06
1809810,1809811,1809810,3619621,2039.2626371383667,5.126040946379362e-06
1811812,1811813,1811812,3623625,2041.0208671092987,5.041609483669163e-06
1813814,1813815,1813814,3627629,2043.0460443496704,4.958557497047877e-06
1815816,1815817,1815816,3631633,2044.9190912246704,4.876862703895313e-06
1817818,1817819,1817818,3635637,2046.7628381252289,4.7965027079044376e-06
1819820,1819821,1819820,3639641,2048.6271212100983,4.717455567515572e-06
1821822,1821823,1821822,3643645,2050.3191170692444,4.639700250663736e-06
1823824,1823825,1823824,3647649,2052.0325062274933,4.563215156849765e-06
1825826,1825827,1825826,3651653,2053.757273197174,4.487979936129705e-06
1827828,1827829,1827828,3655657,2055.326004266739,4.4139738974990905e-06
1829830,1829831,1829830,3659661,2056.92356133461,4.341177145761321e-06
1831832,1831833,1831832,3663665,2058.4569931030273,4.2695694446592825e-06
1833834,1833835,1833834,3667669,2060.033944129944,4.199132263238425e-06
1835836,1835837,1835836,3671673,2061.603980064392,4.129845592615311e-06
1837838,1837839,1837838,3675677,2063.157674074173,4.061691129209066e-06
1839840,1839841,1839840,3679681,2064.7104861736298,3.994650228378305e-06
1841842,1841843,1841842,3683685,2066.2768971920013,3.9287044728553155e-06
1843844,1843845,1843844,3687689,2067.8148663043976,3.8638363548670895e-06
1845846,1845847,1845846,3691693,2069.433662176132,3.800028139266942e-06
1847848,1847849,1847848,3695697,2070.992333173752,3.737262431968702e-06
1849850,1849851,1849850,3699701,2072.8066811561584,3.675522066259873e-06
1851852,1851853,1851852,3703705,2074.4963121414185,3.614790557548986e-06
1853854,1853855,1853854,3707709,2076.174430370331,3.555051193870895e-06
1855856,1855857,1855856,3711713,2077.8967730998993,3.49628805906832e-06
1857858,1857859,1857858,3715717,2079.6941282749176,3.4384847822366282e-06
1859860,1859861,1859860,3719721,2081.5870542526245,3.3816261293395655e-06
1861862,1861863,1861862,3723725,2083.654437303543,3.325696411593526e-06
1863864,1863865,1863864,3727729,2085.3642790317535,3.2706803949622554e-06
1865866,1865867,1865866,3731733,2087.057013988495,3.2165631864700117e-06
1867868,1867869,1867868,3735737,2088.740165233612,3.1633302342015668e-06
1869870,1869871,1869870,3739741,2090.428026199341,3.110966986241692e-06
1871872,1871873,1871872,3743745,2092.1682782173157,3.0594593454225105e-06
1873874,1873875,1873874,3747749,2093.9147300720215,3.0087931008893065e-06
1875876,1875877,1875876,3751753,2095.755023241043,2.9589546102215536e-06
1877878,1877879,1877878,3755757,2097.5728492736816,2.9099305720592383e-06
1879880,1879881,1879880,3759761,2099.3340632915497,2.8617071166081587e-06
1881882,1881883,1881882,3763765,2101.0775270462036,2.8142717383161653e-06
1883884,1883885,1883884,3767769,2102.79260802269,2.76761136319692e-06
1885886,1885887,1885886,3771773,2104.545634031296,2.721713372011436e-06
1887888,1887889,1887888,3775777,2106.4365150928497,2.6765650318338885e-06
1889890,1889891,1889890,3779781,2108.3222472667694,2.632154519233154e-06
1891892,1891893,1891892,3783785,2110.0844752788544,2.5884694423439214e-06
1893894,1893895,1893894,3787789,2111.7030081748962,2.5454979777350673e-06
1895896,1895897,1895896,3791793,2113.345516204834,2.5032287567228195e-06
1897898,1897899,1897898,3795797,2114.952176094055,2.4616498421892175e-06
1899900,1899901,1899900,3799801,2116.7417652606964,2.420750547571515e-06
1901902,1901903,1901902,3803805,2118.4592230319977,2.380519276812265e-06
1903904,1903905,1903904,3807809,2120.311215162277,2.3409452296618838e-06
1905906,1905907,1905906,3811813,2122.2345151901245,2.302017833244463e-06
1907908,1907909,1907908,3815817,2124.23056101799,2.263726400997257e-06
1909910,1909911,1909910,3819821,2126.0451531410217,2.226060473731195e-06
1911912,1911913,1911912,3823825,2127.8901782035828,2.1890099333177204e-06
1913914,1913915,1913914,3827829,2129.553138256073,2.1525644342546e-06
1915916,1915917,1915916,3831833,2131.2351911067963,2.1167146542211412e-06
1917918,1917919,1917918,3835837,2132.8204061985016,2.081450588775624e-06
1919920,1919921,1919920,3839841,2134.3503890037537,2.046762347163167e-06
1921922,1921923,1921922,3843845,2135.8582372665405,2.0126410618104273e-06
1923924,1923925,1923924,3847849,2137.3647632598877,1.9790769556493615e-06
1925926,1925927,1925926,3851853,2138.9628789424896,1.94606150216714e-06
1927928,1927929,1927928,3855857,2140.562608242035,1.9135851516693947e-06
1929930,1929931,1929930,3859861,2142.1781351566315,1.8816392639564583e-06
1931932,1931933,1931932,3863865,2143.7648010253906,1.850215653576015e-06
1933934,1933935,1933934,3867869,2145.390197992325,1.8193049982073717e-06
1935936,1935937,1935936,3871873,2146.9631791114807,1.788899680832401e-06
1937938,1937939,1937938,3875877,2148.5607800483704,1.7589908338777605e-06
1939940,1939941,1939940,3879881,2150.1272552013397,1.7295707266384852e-06
1941942,1941943,1941942,3883885,2151.7117261886597,1.7006310599754215e-06
1943944,1943945,1943944,3887889,2153.282216310501,1.6721645579309552e-06
1945946,1945947,1945946,3891893,2154.8831470012665,1.6441626939922571e-06
1947948,1947949,1947948,3895897,2156.5548782348633,1.6166184195753885e-06
1949950,1949951,1949950,3899901,2158.3143060207367,1.5895241176622221e-06
1951952,1951953,1951952,3903905,2159.89119720459,1.5628725122951437e-06
1953954,1953955,1953954,3907909,2161.4306581020355,1.5366561001428636e-06
1955956,1955957,1955956,3911913,2162.9929621219635,1.5108681736819563e-06
1957958,1957959,1957958,3915917,2164.572580099106,1.4855015706416452e-06
1959960,1959961,1959960,3919921,2166.1308732032776,1.460549128751154e-06
1961962,1961963,1961962,3923925,2167.70582818985,1.4360043678607326e-06
1963964,1963965,1963964,3927929,2169.3290281295776,1.4118608078206307e-06
1965966,1965967,1965966,3931933,2171.0279171466827,1.388111286360072e-06
1967968,1967969,1967968,3935937,2172.6648111343384,1.3647501191371703e-06
1969970,1969971,1969970,3939941,2174.233220100403,1.3417703712548246e-06
1971972,1971973,1971972,3943945,2175.8138790130615,1.3191661309974734e-06
1973974,1973975,1973974,3947949,2177.364848136902,1.2969310319022043e-06
1975976,1975977,1975976,3951953,2178.9230461120605,1.275059048566618e-06
1977978,1977979,1977978,3955957,2180.4912571907043,1.2535446103356662e-06
1979980,1979981,1979980,3959961,2182.073307275772,1.232381578120112e-06
1981982,1981983,1981982,3963965,2183.5830001831055,1.2115642675780691e-06
1983984,1983985,1983984,3967969,2185.098221063614,1.191086880680814e-06
1985986,1985987,1985986,3971973,2186.674784183502,1.1709441878338112e-06
1987988,1987989,1987988,3975977,2188.214732170105,1.1511305046951747e-06
1989990,1989991,1989990,3979981,2189.763837337494,1.131640374296694e-06
1991992,1991993,1991992,3983985,2191.301254272461,1.1124686807306716e-06
1993994,1993995,1993994,3987989,2192.8354251384735,1.09361030808941e-06
1995996,1995997,1995996,3991993,2194.319990158081,1.0750600267783739e-06
1997998,1997999,1997998,3995997,2195.7925910949707,1.0568124935161904e-06
2000000,2000001,2000000,4000001,2197.329564332962,1.0388632745161885e-06


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007841587066650391,2180.042156630883
1,4,4,8,0.0024390220642089844,1649.7561110534912
2,6,6,12,0.004012107849121094,785.7772573014074
3,8,8,16,0.005352973937988281,442.5565902014723
4,12,12,24,0.008124351501464844,299.58060016479703
5,20,20,40,0.012027263641357422,288.42098736223693
6,24,24,48,0.014342308044433594,222.79071163786648
7,32,32,64,0.019233226776123047,219.8174211852122
8,36,36,72,0.02129220962524414,182.82409958985522
9,44,44,88,0.025138139724731445,181.1625523972575
10,50,50,100,0.027877330780029297,180.18797708248076
11,56,56,112,0.03189730644226074,169.06558190080818
12,60,60,120,0.034420013427734375,147.797171410916
13,64,64,128,0.036414146423339844,132.88970567018487
14,70,70,140,0.03920412063598633,108.42904570778978
15,72,72,144,0.04049110412597656,81.2908408201049
16,76,76,152,0.04236316680908203,80.04216520899013
17,80,80,160,0.04428601264953613,78.11845813338005
18,88,88,176,0.047805070877075195,77.93138891778767
19,92,92,184,0.050045013427734375,74.64651519897939
20,96,96,192,0.05231809616088867,72.99211134776715
21,102,102,204,0.055663108825683594,72.548014062849
22,106,106,212,0.05771231651306152,69.85426173878295
23,110,110,220,0.059754133224487305,68.37483358601662
24,116,116,232,0.06266307830810547,67.62893753122967
25,124,124,248,0.06622123718261719,67.57982315185723
26,128,128,256,0.06877708435058594,64.59191084797544
27,134,134,268,0.07203221321105957,64.16374442350593
28,142,142,284,0.07604312896728516,64.13078866404521
29,146,146,292,0.07806706428527832,61.046931533643374
30,154,154,308,0.08182096481323242,61.02128696393902
31,158,158,316,0.08409500122070312,58.3318786823213
32,164,164,328,0.08736324310302734,57.88102457756281
33,168,168,336,0.08945727348327637,56.45686616600369
34,176,176,352,0.09334611892700195,56.444005438999966
35,180,180,360,0.09557318687438965,55.35707983153543
36,186,186,372,0.09884405136108398,55.172040298464026
37,192,192,384,0.10162210464477539,54.9249142956553
38,196,196,392,0.10362029075622559,54.285632034928994
39,200,200,400,0.10554814338684082,53.732067931315896
40,208,208,416,0.10900712013244629,53.72591086589023
41,212,212,424,0.11101436614990234,53.3163392683191
42,220,220,440,0.11576414108276367,53.31155104441427
43,224,224,448,0.11848020553588867,52.78026172633736
44,232,232,464,0.12180924415588379,52.77557731512297
45,238,238,476,0.12455606460571289,52.50272793667182
46,246,246,492,0.12804937362670898,52.49865468513076
47,252,252,504,0.13146400451660156,52.041562629835425
48,260,260,520,0.13524103164672852,52.03782986296483
49,266,266,532,0.13827013969421387,51.42412881481482
50,274,274,548,0.14178729057312012,51.420766245845016
51,280,280,560,0.14463520050048828,50.53798739544527
52,288,288,576,0.14831805229187012,50.534690665627295
53,296,296,592,0.15175914764404297,50.5314216142915
54,304,304,608,0.15506219863891602,50.52817776216534
55,310,310,620,0.15800023078918457,48.768255750700746
56,318,318,636,0.16224908828735352,48.76513156940473
57,326,326,652,0.16925716400146484,48.76205195984153
58,334,334,668,0.17270612716674805,48.759012511759465
59,340,340,680,0.17565703392028809,46.493711236571926
60,348,348,696,0.17908835411071777,46.49079841566868
61,354,354,708,0.18199825286865234,44.28085656875692
62,362,362,724,0.1853621006011963,44.27808342213916
63,370,370,740,0.18880796432495117,44.275346539714064
64,378,378,756,0.1921381950378418,44.272643166865464
65,386,386,772,0.19530010223388672,44.26997081023569
66,392,392,784,0.19812512397766113,41.563666509011455
67,400,400,800,0.20127320289611816,41.56128295640565
68,406,406,812,0.20400619506835938,39.05573219380585
69,414,414,828,0.2075052261352539,39.053450650393415
70,422,422,844,0.21389317512512207,39.051195564681166
71,428,428,856,0.21702027320861816,36.51277561082293
72,436,436,872,0.22063803672790527,36.510567505275276
73,442,442,884,0.22327613830566406,34.13993009750584
74,450,450,900,0.22646617889404297,34.13790166912759
75,456,456,912,0.22916007041931152,31.931261949557666
76,464,464,928,0.23267912864685059,31.92938752364421
77,470,470,940,0.23538517951965332,30.306012844679117
78,478,478,956,0.2388460636138916,30.30426986992211
79,484,484,968,0.24169707298278809,28.182758258589956
80,492,492,984,0.2452101707458496,28.181097247017306
81,498,498,996,0.24870610237121582,25.522167302695834
82,506,506,1012,0.25225305557250977,25.520546468070734
83,514,514,1028,0.255587100982666,25.518947020199448
84,520,520,1040,0.25855517387390137,23.254165606992956
85,528,528,1056,0.26393604278564453,23.25263986511095
86,534,534,1068,0.26691627502441406,20.852545308053777
87,542,542,1084,0.27046918869018555,20.851125056655746
88,550,550,1100,0.2738959789276123,20.849722731964675
89,558,558,1116,0.27712321281433105,20.848336805146573
90,564,564,1128,0.28014707565307617,18.352308650206623
91,572,572,1144,0.2835042476654053,18.351000233229115
92,580,580,1160,0.28681516647338867,18.34971246567261
93,586,586,1172,0.2896382808685303,16.208337035662453
94,594,594,1188,0.29318928718566895,16.207123809763743
95,600,600,1200,0.29630327224731445,13.80701082686403
96,608,608,1216,0.3005530834197998,13.80584871953181
97,614,614,1228,0.3031632900238037,11.856431004155183
98,622,622,1244,0.30671024322509766,11.85538920123895
99,628,628,1256,0.31057000160217285,10.12969781700474
100,636,636,1272,0.31565332412719727,10.12878681886707
101,642,642,1284,0.3190481662750244,8.636728036849263
102,650,650,1300,0.32240915298461914,8.635899590610165
103,656,656,1312,0.3254561424255371,7.459277379821401
104,664,664,1328,0.32889604568481445,7.458483184772717
105,670,670,1340,0.3318212032318115,6.5104547030983895
106,678,678,1356,0.335252046585083,6.509683370376251
107,686,686,1372,0.33898401260375977,6.508920661625325
108,692,692,1384,0.34189414978027344,5.6405075057772365
109,700,700,1400,0.3464682102203369,5.639760691997367
110,706,706,1412,0.34963321685791016,4.888544973648095
111,714,714,1428,0.3533132076263428,4.887893159784539
112,720,720,1440,0.35596799850463867,4.228695557667152
113,728,728,1456,0.3596763610839844,4.2280992488199445
114,734,734,1468,0.36237025260925293,3.63903782606792
115,740,740,1480,0.36522722244262695,3.150173823882483
116,748,748,1496,0.3688161373138428,3.1496625634127895
117,754,754,1508,0.37139415740966797,2.723046011101701
118,762,762,1524,0.3747901916503906,2.7225985839427267
119,768,768,1536,0.3774101734161377,2.324210980625594
120,774,774,1548,0.3799631595611572,2.0883573010875125
121,780,780,1560,0.38266706466674805,1.8042181646878817
122,788,788,1576,0.38603806495666504,1.803854243113392
123,794,794,1588,0.38901424407958984,1.5313382841387693
124,802,802,1604,0.39280223846435547,1.5310244127934993
125,806,806,1612,0.39477109909057617,0.8648810872601871
126,814,814,1628,0.39884018898010254,0.8646318182625237
127,818,818,1636,0.4010181427001953,0.49279549503728504
128,826,826,1652,0.40471506118774414,0.492587056028583
129,830,830,1660,0.40718817710876465,0.28753988447908796
130,838,838,1676,0.41142916679382324,0.2873468273943445
131,842,842,1684,0.41407108306884766,0.16876278010215628
132,850,850,1700,0.4177131652832031,0.16861658004881974
133,854,854,1708,0.4197711944580078,0.10366949346314414
134,862,862,1724,0.42305898666381836,0.10355420270093418
135,866,866,1732,0.42500925064086914,0.06542716339311028
136,874,874,1748,0.4286370277404785,0.06534397942346004
137,878,878,1756,0.430861234664917,0.04173566734539236
138,884,884,1768,0.4336540699005127,0.037750232559233154
139,888,888,1776,0.4355630874633789,0.02531091120442852
140,896,896,1792,0.43894004821777344,0.025265331456921558
141,900,900,1800,0.44122910499572754,0.01835837639350757
142,908,908,1816,0.44520115852355957,0.018327249257936273
143,912,912,1824,0.4474959373474121,0.013442600109442537
144,920,920,1840,0.4508821964263916,0.013420242567804053
145,924,924,1848,0.45279812812805176,0.009901279769678695
146,932,932,1864,0.45609307289123535,0.00988539804473021
147,936,936,1872,0.45862627029418945,0.007169918314843926
148,942,942,1884,0.4617140293121338,0.006708295288603949
149,946,946,1892,0.4639103412628174,0.005018852230818993
150,954,954,1908,0.4673800468444824,0.005009791490124371
151,958,958,1916,0.4694821834564209,0.003725994024648571
152,966,966,1932,0.4730050563812256,0.003719653896609998
153,970,970,1940,0.4750852584838867,0.002750046719143029
154,978,978,1956,0.4782412052154541,0.002745281307170444
155,982,982,1964,0.4802722930908203,0.0019438868719134916
156,990,990,1980,0.48340725898742676,0.001940203338676838
157,994,994,1988,0.4853072166442871,0.0013434714095410527
158,1000,1000,2000,0.487990140914917,0.0012409508383370849
159,1004,1004,2008,0.48995423316955566,0.0009532533691753997
160,1010,1010,2020,0.4925382137298584,0.0009032211474959695
161,1014,1014,2028,0.4943962097167969,0.0007083621352421687
162,1022,1022,2044,0.49772119522094727,0.00070698905858535
163,1026,1026,2052,0.49965429306030273,0.0005443137937390929
164,1032,1032,2064,0.502249002456665,0.0005158767912689655
165,1036,1036,2072,0.5043511390686035,0.0004098085497616921
166,1040,1040,2080,0.5062181949615479,0.0003567171451095419
167,1044,1044,2088,0.508418083190918,0.00031385052409405034
168,1050,1050,2100,0.5113821029663086,0.00030651137751647184
169,1056,1056,2112,0.5143871307373047,0.0002965251048863138
170,1062,1062,2124,0.5171811580657959,0.0002864219236471399
171,1066,1066,2132,0.5194733142852783,0.00025147978590212006
172,1074,1074,2148,0.5226421356201172,0.00025110603439770784
173,1078,1078,2156,0.5245051383972168,0.0002185415484063924
174,1086,1086,2172,0.5277619361877441,0.00021826697832239006
175,1090,1090,2180,0.5296740531921387,0.00018676089803193463
176,1098,1098,2196,0.5330450534820557,0.00018653284132597037
177,1102,1102,2204,0.5350039005279541,0.00015424448849898909
178,1108,1108,2216,0.5374631881713867,0.00014648222997948324
179,1114,1114,2228,0.5399312973022461,0.0001398359077029454
180,1118,1118,2236,0.5417571067810059,0.00011138416050471278
181,1126,1126,2252,0.5449061393737793,0.00011124470995582669
182,1130,1130,2260,0.5468113422393799,8.552440908715653e-05
183,1134,1134,2268,0.5486752986907959,6.597270396468957e-05
184,1142,1142,2284,0.5518221855163574,6.586321387658245e-05
185,1146,1146,2292,0.5538132190704346,5.109316180096357e-05
186,1154,1154,2308,0.5570733547210693,5.09960029830836e-05
187,1158,1158,2316,0.559333324432373,3.8775264783907915e-05
188,1162,1162,2324,0.5615301132202148,2.9847154223716643e-05
189,1170,1170,2340,0.5651531219482422,2.979014641368849e-05
190,1174,1174,2348,0.5672702789306641,2.240809180875658e-05
191,1178,1178,2356,0.5693283081054688,1.736970762067358e-05
192,1186,1186,2372,0.5723490715026855,1.7337641793346847e-05
193,1190,1190,2380,0.5741770267486572,1.3667561461261357e-05
194,1198,1198,2396,0.577390193939209,1.3643996680912096e-05
195,1202,1202,2404,0.5792660713195801,1.0814019674398878e-05
196,1210,1210,2420,0.5823521614074707,1.0795597859214467e-05
197,1214,1214,2428,0.5842199325561523,8.412962642978528e-06
198,1222,1222,2444,0.5873312950134277,8.399445505347103e-06
199,1226,1226,2452,0.5891931056976318,6.5001939901776495e-06
200,1230,1230,2460,0.5910420417785645,5.561638431572646e-06
201,1234,1234,2468,0.5929989814758301,4.869880740443477e-06
202,1240,1240,2480,0.5960409641265869,4.749642016577127e-06
203,1244,1244,2488,0.5984351634979248,4.304332378524123e-06
204,1250,1250,2500,0.6018099784851074,4.226418923281017e-06
205,1254,1254,2508,0.6037702560424805,3.942716375604505e-06
206,1260,1260,2520,0.6065301895141602,3.893126404364011e-06
207,1264,1264,2528,0.6088352203369141,3.7092759157530963e-06
208,1272,1272,2544,0.6127970218658447,3.707522068907565e-06
209,1276,1276,2552,0.615103006362915,3.523658051562961e-06
210,1284,1284,2568,0.6189150810241699,3.5223910117565538e-06
211,1288,1288,2576,0.6209652423858643,3.3652529509708984e-06
212,1296,1296,2592,0.6244051456451416,3.3643282222328708e-06
213,1300,1300,2600,0.6265602111816406,3.2171925568036386e-06
214,1306,1306,2612,0.6296069622039795,3.180710109518259e-06
215,1312,1312,2624,0.6324820518493652,3.1488646072830306e-06
216,1316,1316,2632,0.6344962120056152,3.035656618521898e-06
217,1322,1322,2644,0.6373310089111328,3.0092055567365605e-06
218,1328,1328,2656,0.6400871276855469,2.9861159873689758e-06
219,1332,1332,2664,0.6422910690307617,2.898373054449621e-06
220,1340,1340,2680,0.6459043025970459,2.8978878390262253e-06
221,1344,1344,2688,0.6484081745147705,2.8328261123533593e-06
222,1352,1352,2704,0.6519513130187988,2.832468567248725e-06
223,1356,1356,2712,0.6537952423095703,2.782742399176641e-06
224,1364,1364,2728,0.6573293209075928,2.7824645485452493e-06
225,1368,1368,2736,0.659644365310669,2.7427803388491157e-06
226,1376,1376,2752,0.6665170192718506,2.742547849265975e-06
227,1380,1380,2760,0.6684660911560059,2.7094326924270717e-06
228,1388,1388,2776,0.6717431545257568,2.709268414946564e-06
229,1392,1392,2784,0.6737570762634277,2.685227855181438e-06
230,1400,1400,2800,0.6770751476287842,2.6851030270336196e-06
231,1404,1404,2808,0.6789712905883789,2.6660883349904907e-06
232,1412,1412,2824,0.683305025100708,2.6659960212782607e-06
233,1416,1416,2832,0.6852080821990967,2.6497465341890347e-06
234,1424,1424,2848,0.6884710788726807,2.6496575173950987e-06
235,1430,1430,2860,0.6911540031433105,2.6444879495102214e-06
236,1436,1436,2872,0.6937973499298096,2.6400516617286485e-06
237,1442,1442,2884,0.6975600719451904,2.635880719026318e-06
238,1450,1450,2900,0.7009432315826416,2.6358086415712023e-06
239,1456,1456,2912,0.7035410404205322,2.6303558797735604e-06
240,1462,1462,2924,0.7060642242431641,2.6256459477735916e-06
241,1470,1470,2940,0.7095413208007812,2.6255842158207088e-06
242,1476,1476,2952,0.712285041809082,2.6191878532699775e-06
243,1484,1484,2968,0.717156171798706,2.6191328288405202e-06
244,1490,1490,2980,0.7198452949523926,2.611418153719569e-06
245,1498,1498,2996,0.7230911254882812,2.61136722201627e-06
246,1504,1504,3008,0.7256600856781006,2.600344600978133e-06
247,1512,1512,3024,0.729013204574585,2.6002940103353467e-06
248,1520,1520,3040,0.7334961891174316,2.6002437607530737e-06
249,1528,1528,3056,0.7367260456085205,2.6001937385444762e-06
250,1536,1536,3072,0.7399890422821045,2.600144057396392e-06
251,1540,1540,3080,0.7420182228088379,2.6039683689305093e-06
252,1544,1544,3088,0.7439560890197754,2.6030143089883495e-06
253,1548,1548,3096,0.7458431720733643,2.5930518177119666e-06
254,1556,1556,3112,0.7497711181640625,2.593007934592606e-06
255,1564,1564,3128,0.7529022693634033,2.5929643925337587e-06
256,1572,1572,3144,0.7561023235321045,2.5929210778485867e-06
257,1580,1580,3160,0.7596821784973145,2.5928777631634148e-06
258,1588,1588,3176,0.7632641792297363,2.5928345621650806e-06
259,1590,1590,3180,0.764721155166626,2.5592227075321716e-06
260,1594,1594,3188,0.7666971683502197,2.5606835833968944e-06
261,1596,1596,3192,0.7679293155670166,2.5650533643784e-06
262,1604,1604,3208,0.7711241245269775,2.565013005551009e-06
263,1612,1612,3224,0.7742111682891846,2.5649727604104555e-06
264,1620,1620,3240,0.7773680686950684,2.5649328563304152e-06
265,1628,1628,3256,0.7807350158691406,2.5648927248766995e-06
266,1632,1632,3264,0.7826640605926514,2.5580579858797137e-06
267,1640,1640,3280,0.7858850955963135,2.558018195486511e-06
268,1644,1644,3288,0.7880163192749023,2.552072260186833e-06
269,1652,1652,3304,0.7915310859680176,2.5520326971673057e-06
270,1660,1660,3320,0.7950930595397949,2.551993361521454e-06
271,1668,1668,3336,0.7988259792327881,2.5519539121887647e-06
272,1676,1676,3352,0.8027482032775879,2.5519143491692375e-06
273,1680,1680,3360,0.8050000667572021,2.5317555127912783e-06
274,1688,1688,3376,0.8086233139038086,2.5317166318927775e-06
275,1694,1694,3388,0.8114612102508545,2.523895091144368e-06
276,1702,1702,3404,0.8150100708007812,2.523856664993218e-06
277,1710,1710,3420,0.8184692859649658,2.523818011468393e-06
278,1718,1718,3436,0.8216531276702881,2.523779471630405e-06
279,1726,1726,3452,0.8249039649963379,2.5237409317924175e-06
280,1730,1730,3460,0.8268401622772217,2.5077413283725036e-06
281,1738,1738,3476,0.830125093460083,2.507703129595029e-06
282,1742,1742,3484,0.8319523334503174,2.4914122604968725e-06
283,1750,1750,3500,0.8350663185119629,2.491374402779911e-06
284,1758,1758,3516,0.8385522365570068,2.4913366587497876e-06
285,1766,1766,3532,0.8419163227081299,2.4912990284065017e-06
286,1774,1774,3548,0.8451461791992188,2.4912610570027027e-06
287,1778,1778,3556,0.8470311164855957,2.47308435064042e-06
288,1782,1782,3564,0.8489401340484619,2.455523031130724e-06
289,1790,1790,3580,0.8522109985351562,2.455485969221627e-06
290,1798,1798,3596,0.8554461002349854,2.4554485662520165e-06
291,1806,1806,3612,0.8586733341217041,2.4554112769692438e-06
292,1814,1814,3628,0.8621652126312256,2.4553743287469842e-06
293,1822,1822,3644,0.8655083179473877,2.455336925777374e-06
294,1828,1828,3656,0.8680531978607178,2.4558941049690475e-06
295,1836,1836,3672,0.871211051940918,2.4558569293731125e-06
296,1838,1838,3676,0.8724522590637207,2.382662955824344e-06
297,1846,1846,3692,0.875535249710083,2.382626576036273e-06
298,1852,1852,3704,0.8780550956726074,1.9949585521317204e-06
299,1860,1860,3720,0.881195068359375,1.9949229681515135e-06
300,1868,1868,3736,0.8843791484832764,1.994887270484469e-06
301,1876,1876,3752,0.8874802589416504,1.994852141251613e-06
302,1884,1884,3768,0.8905651569366455,1.9948168983319192e-06
303,1888,1888,3776,0.892484188079834,2.082751734633348e-06
304,1896,1896,3792,0.8957099914550781,2.0827179696425446e-06
305,1900,1900,3800,0.8974931240081787,2.1329913124645827e-06
306,1906,1906,3812,0.8999922275543213,1.8283180907019414e-06
307,1914,1914,3828,0.9030232429504395,1.828286826821568e-06
308,1918,1918,3836,0.9049670696258545,8.897465022528195e-07
309,1926,1926,3852,0.9081361293792725,8.897181942302268e-07
310,1932,1932,3864,0.9106771945953369,7.334622296184534e-07
311,1938,1938,3876,0.9132659435272217,6.038090987203759e-07
312,1946,1946,3892,0.9166059494018555,6.037855655449675e-07
313,1950,1950,3900,0.9185910224914551,2.8368685889290646e-07
314,1958,1958,3916,0.9218611717224121,2.83666622635792e-07
315,1962,1962,3924,0.9239561557769775,1.2550196970551042e-07
316,1970,1970,3940,0.9272041320800781,1.254844619325013e-07
317,1974,1974,3948,0.9291541576385498,4.663206709665246e-08
318,1982,1982,3964,0.9324991703033447,4.6618083615612704e-08
319,1986,1986,3972,0.9344289302825928,7.239236765599344e-09
320,1994,1994,3988,0.9375860691070557,7.225935405585915e-09
321,2000,2000,4000,0.9403483867645264,1.6336798580596223e-10
322,2006,2006,4012,0.943134069442749,5.699234861822333e-09


==> plot_data/logistic_regression_problem_lambda_param100overN_data_namespambase/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0013186931610107422,2180.042156630883
1,4,4,8,0.003532886505126953,1649.7561110534912
2,6,6,12,0.007798910140991211,810.127181747561
3,8,8,16,0.009359121322631836,539.389226626289
4,10,10,20,0.01087188720703125,339.4804780114555
5,12,12,24,0.013466835021972656,245.09872895812805
6,14,14,28,0.015086889266967773,178.2528852958667
7,18,18,36,0.01758408546447754,175.18675618515363
8,22,22,44,0.01940178871154785,178.59077517268156
9,24,24,48,0.020538806915283203,131.40293201501822
10,26,26,52,0.02160191535949707,126.53791140683165
11,28,28,56,0.022656917572021484,130.47739703622142
12,32,32,64,0.024371862411499023,126.01903467464103
13,34,34,68,0.02581191062927246,105.51311594862955
14,36,36,72,0.027257919311523438,101.96868056198309
15,40,40,80,0.030156850814819336,101.54805401814247
16,44,44,88,0.03237485885620117,100.9655802753091
17,48,48,96,0.03420376777648926,99.58113103139681
18,52,52,104,0.03631401062011719,90.95868771932965
19,54,54,108,0.038034915924072266,80.31014610159127
20,56,56,112,0.0395197868347168,80.71895976171572
21,58,58,116,0.040708065032958984,80.87330253928258
22,60,60,120,0.0425410270690918,80.42850369535881
23,62,62,124,0.04463791847229004,73.90294020393867
24,64,64,128,0.046437740325927734,74.2253497634697
25,66,66,132,0.04755091667175293,74.3708571145471
26,68,68,136,0.04864692687988281,74.21600448695972
27,70,70,140,0.049652814865112305,73.40675221629385
28,72,72,144,0.05070304870605469,73.25289053626398
29,74,74,148,0.051744937896728516,72.85164622381672
30,76,76,152,0.052845001220703125,70.73692845466871
31,78,78,156,0.05391407012939453,69.67930347464267
32,82,82,164,0.05567002296447754,69.59616793905843
33,84,84,168,0.05680084228515625,64.92930595163102
34,88,88,176,0.05921673774719238,64.91260165008316
35,90,90,180,0.060482025146484375,62.48231174591956
36,94,94,188,0.06221199035644531,62.50260711551414
37,96,96,192,0.06337404251098633,58.61465481275104
38,98,98,196,0.06461095809936523,58.598060825168204
39,102,102,204,0.06638097763061523,58.60825778646404
40,104,104,208,0.06771087646484375,56.59043284198333
41,106,106,212,0.06897783279418945,56.421337882904936
42,108,108,216,0.06999492645263672,56.17435295854989
43,110,110,220,0.0711359977722168,56.304039257365275
44,112,112,224,0.07230401039123535,55.66437197096457
45,114,114,228,0.07390475273132324,55.13469968746267
46,116,116,232,0.07520580291748047,54.95147441701647
47,118,118,236,0.07644200325012207,54.455596329665696
48,120,120,240,0.07774782180786133,54.07602739028562
49,124,124,248,0.07950592041015625,54.06672606934217
50,126,126,252,0.08053398132324219,53.840704873565755
51,128,128,256,0.0815730094909668,53.80459284000426
52,132,132,264,0.08314895629882812,53.79590168958816
53,134,134,268,0.08420395851135254,53.55199583474746
54,138,138,276,0.08584070205688477,53.544652597298864
55,140,140,280,0.08685088157653809,53.21127701114278
56,144,144,288,0.08854913711547852,53.20525298914322
57,146,146,292,0.08960986137390137,53.00005255428255
58,150,150,300,0.0914449691772461,52.99420109543894
59,152,152,304,0.09251976013183594,52.74678968815624
60,156,156,312,0.09411191940307617,52.735961984027654
61,160,160,320,0.09569883346557617,52.68804455249915
62,162,162,324,0.09674906730651855,52.22270398069827
63,166,166,332,0.09841680526733398,52.21525744506698
64,168,168,336,0.09946990013122559,51.697137968833886
65,172,172,344,0.10111093521118164,51.685990548468226
66,174,174,348,0.10216069221496582,51.29791100351781
67,178,178,356,0.10390901565551758,51.30086282069419
68,180,180,360,0.10503911972045898,50.907050916286835
69,184,184,368,0.10671401023864746,50.90838733254736
70,188,188,376,0.10854291915893555,50.90532450908904
71,192,192,384,0.11018896102905273,50.90365345442228
72,196,196,392,0.11181378364562988,50.90293554349137
73,200,200,400,0.11333489418029785,50.77757613508629
74,204,204,408,0.11493396759033203,50.67539995580887
75,206,206,412,0.11598992347717285,49.206591602504204
76,210,210,420,0.11753010749816895,49.18755919207001
77,212,212,424,0.11851787567138672,47.21836362704471
78,216,216,432,0.12007284164428711,47.22496645595015
79,218,218,436,0.12107992172241211,46.62540974549938
80,222,222,444,0.12266373634338379,46.59387425591967
81,226,226,452,0.12416410446166992,46.53719063911558
82,230,230,460,0.1257638931274414,46.43658969645003
83,234,234,468,0.12737083435058594,46.40927873939745
84,238,238,476,0.12898683547973633,46.37727093386252
85,240,240,480,0.12994885444641113,45.5816881468279
86,244,244,488,0.13149309158325195,45.52935455187003
87,248,248,496,0.13310575485229492,45.370244210982264
88,252,252,504,0.13468194007873535,45.23139474612526
89,254,254,508,0.13562679290771484,44.130109950136784
90,258,258,516,0.13711309432983398,44.070427866784485
91,262,262,524,0.13868284225463867,43.93074148847586
92,264,264,528,0.13970184326171875,43.01087875912981
93,268,268,536,0.14123988151550293,42.996726740230315
94,270,270,540,0.1422419548034668,41.05119781951407
95,276,276,552,0.1443018913269043,41.06158289924656
96,278,278,556,0.14529776573181152,40.623973252071664
97,282,282,564,0.14698004722595215,40.44528875859169
98,286,286,572,0.14858698844909668,40.14329880877608
99,288,288,576,0.14965295791625977,38.907943403519766
100,290,290,580,0.15068387985229492,38.27097375350445
101,294,294,588,0.15226483345031738,38.27019847418774
102,296,296,592,0.15328574180603027,37.60792659895651
103,300,300,600,0.15486884117126465,37.608139277216424
104,302,302,604,0.15590810775756836,36.73954260003461
105,306,306,612,0.15752792358398438,36.71389417079399
106,308,308,616,0.1585099697113037,34.06674003733201
107,312,312,624,0.1600348949432373,34.08144727329932
108,314,314,628,0.16106796264648438,32.34218926609833
109,316,316,632,0.16204595565795898,31.12709178457567
110,320,320,640,0.1635739803314209,30.998493740731874
111,322,322,644,0.16457271575927734,28.258091421225117
112,326,326,652,0.16610980033874512,28.43056041812656
113,330,330,660,0.16771292686462402,28.487179572653986
114,332,332,664,0.16869497299194336,25.467477824180833
115,336,336,672,0.17020893096923828,25.704290915149386
116,338,338,676,0.17118000984191895,27.393485636474225
117,342,342,684,0.17272591590881348,27.420517288618612
118,344,344,688,0.17370390892028809,26.679502734768676
119,348,348,696,0.17525076866149902,26.58051642041346
120,350,350,700,0.1762857437133789,24.7357096189603
121,354,354,708,0.17787575721740723,24.791918718938177
122,356,356,712,0.17888879776000977,21.12267827242158
123,360,360,720,0.180405855178833,21.275291131650874
124,362,362,724,0.1813957691192627,21.876982218154808
125,366,366,732,0.18322396278381348,21.939664254494346
126,368,368,736,0.18430209159851074,20.22887744074592
127,372,372,744,0.18588995933532715,20.2338929083694
128,374,374,748,0.18691086769104004,17.264112494586243
129,380,380,760,0.18935275077819824,17.241561096853957
130,384,384,768,0.19109082221984863,17.089968096257508
131,390,390,780,0.1933608055114746,17.044268590477714
132,392,392,784,0.19449687004089355,18.241337685322378
133,396,396,792,0.19622182846069336,18.33339393361075
134,398,398,796,0.19725298881530762,18.73062557532512
135,402,402,804,0.19901585578918457,18.625547142386267
136,406,406,812,0.20083093643188477,18.46299037701783
137,408,408,816,0.20195388793945312,16.94615155030965
138,412,412,824,0.20357990264892578,16.810062584168236
139,414,414,828,0.20457172393798828,16.277167015027317
140,418,418,836,0.20614910125732422,16.32882435472311
141,422,422,844,0.2077498435974121,16.367978166200373
142,424,424,848,0.20880579948425293,14.746524154090253
143,428,428,856,0.210493803024292,14.79719310734231
144,430,430,860,0.21159076690673828,13.640758649972895
145,434,434,868,0.21373200416564941,13.616246857723013
146,436,436,872,0.21488404273986816,12.282277414570899
147,440,440,880,0.21657395362854004,12.33994389655561
148,442,442,884,0.21761775016784668,10.668878569404797
149,446,446,892,0.21922683715820312,10.711602572986976
150,448,448,896,0.22025275230407715,8.419640325777436
151,456,456,912,0.22295904159545898,8.4193319631662
152,458,458,916,0.22404813766479492,7.552935557968453
153,466,466,932,0.2269117832183838,7.552637765085478
154,468,468,936,0.2279958724975586,8.268244553474233
155,472,472,944,0.22961187362670898,8.043434360266929
156,476,476,952,0.23130106925964355,8.066232489426056
157,478,478,956,0.23239803314208984,8.11201988075402
158,482,482,964,0.23398494720458984,8.105209442577689
159,484,484,968,0.23498272895812988,8.192359670403903
160,488,488,976,0.2366929054260254,8.172458336300565
161,490,490,980,0.23780488967895508,7.400200974148902
162,498,498,996,0.24060678482055664,7.399980551538647
163,502,502,1004,0.24234986305236816,7.229833180424862
164,510,510,1020,0.24547696113586426,7.2296168685358
165,512,512,1024,0.24652385711669922,6.58420562666322
166,520,520,1040,0.24923110008239746,6.58399589415626
167,522,522,1044,0.25029492378234863,6.687033232133217
168,524,524,1048,0.2513010501861572,6.395290940338441
169,532,532,1064,0.2539660930633545,6.39510304721864
170,534,534,1068,0.2550678253173828,6.212330300789631
171,538,538,1076,0.25678300857543945,6.218693251021705
172,540,540,1080,0.25789880752563477,6.092412965329572
173,542,542,1084,0.25897789001464844,5.840301059969761
174,546,546,1092,0.26059389114379883,5.82288934895098
175,550,550,1100,0.2622859477996826,5.823721596453197
176,554,554,1108,0.26396679878234863,5.794661799384585
177,556,556,1112,0.26510095596313477,5.64405635121534
178,558,558,1116,0.2661728858947754,5.380430347898027
179,562,562,1124,0.26786088943481445,5.3683366334483935
180,566,566,1132,0.2697887420654297,5.331311180194916
181,568,568,1136,0.27123403549194336,5.103626390068939
182,572,572,1144,0.27329182624816895,5.085362519662226
183,574,574,1148,0.2746407985687256,4.726565232063081
184,578,578,1156,0.27635979652404785,4.7252917540514545
185,580,580,1160,0.2778959274291992,4.714985581540759
186,584,584,1168,0.2798130512237549,4.717567464452372
187,586,586,1172,0.2809758186340332,4.341502687084812
188,590,590,1180,0.28262805938720703,4.351770285227417
189,592,592,1184,0.28375911712646484,3.94998843370297
190,596,596,1192,0.28543591499328613,3.953567705747787
191,598,598,1196,0.2865128517150879,3.765440667114376
192,602,602,1204,0.28813695907592773,3.764254273565598
193,604,604,1208,0.289154052734375,3.5146064881253096
194,608,608,1216,0.2908968925476074,3.516611877357832
195,610,610,1220,0.2921440601348877,3.3482877471685697
196,614,614,1228,0.29401087760925293,3.350150465877846
197,616,616,1232,0.29514288902282715,3.2735319530848983
198,620,620,1240,0.29768896102905273,3.2781486370812445
199,624,624,1248,0.2998230457305908,3.2772080619769213
200,628,628,1256,0.3015599250793457,3.2822605928686244
201,632,632,1264,0.3034207820892334,3.284312206804202
202,634,634,1268,0.3047058582305908,2.979699227729384
203,638,638,1276,0.3064858913421631,2.951037925447281
204,642,642,1284,0.30823683738708496,2.896052663499404
205,648,648,1296,0.3104979991912842,2.8807422356466077
206,656,656,1312,0.3134148120880127,2.880673167148757
207,658,658,1316,0.31450700759887695,2.6048240677197327
208,664,664,1328,0.3167107105255127,2.594979590284993
209,668,668,1336,0.3183767795562744,2.6241139725131006
210,676,676,1352,0.321213960647583,2.6240471525828752
211,680,680,1360,0.3229207992553711,2.564523215790473
212,682,682,1364,0.32404398918151855,2.6859655608931234
213,686,686,1372,0.32568907737731934,2.6868812205934773
214,688,688,1376,0.3268008232116699,2.7426717965544185
215,694,694,1388,0.3292107582092285,2.727157823440507
216,700,700,1400,0.3316018581390381,2.713321907436921
217,706,706,1412,0.33391475677490234,2.7072006462332183
218,710,710,1420,0.335676908493042,2.7034230664633014
219,714,714,1428,0.3373439311981201,2.6890978420200327
220,716,716,1432,0.3384208679199219,2.5909021363929696
221,720,720,1440,0.3400449752807617,2.589979328390882
222,722,722,1444,0.34116387367248535,2.4339638904541516
223,726,726,1452,0.34270572662353516,2.430775248374175
224,728,728,1456,0.3437349796295166,2.193415695046724
225,732,732,1464,0.34526991844177246,2.1920391501555514
226,734,734,1468,0.3463437557220459,2.019873415245229
227,738,738,1476,0.34809374809265137,2.020489930255735
228,740,740,1480,0.3491189479827881,1.985143344129483
229,744,744,1488,0.35075879096984863,1.9862878240725195
230,746,746,1492,0.35182785987854004,2.0124519220231605
231,750,750,1500,0.353543758392334,2.015269102101115
232,752,752,1504,0.3546149730682373,1.9256560156587739
233,756,756,1512,0.35630297660827637,1.9232920227367458
234,758,758,1516,0.3573570251464844,1.870394913832115
235,762,762,1524,0.3590860366821289,1.8691503857098724
236,766,766,1532,0.3606698513031006,1.8619088539551285
237,768,768,1536,0.36170291900634766,1.7503096479271107
238,772,772,1544,0.36356496810913086,1.7514546555714787
239,774,774,1548,0.3646578788757324,1.7190404887351178
240,778,778,1556,0.3663308620452881,1.7172456230649686
241,780,780,1560,0.3674659729003906,1.671705234441788
242,782,782,1564,0.3685569763183594,1.5919965089075276
243,786,786,1572,0.37022995948791504,1.5773718743495238
244,790,790,1580,0.371931791305542,1.5637772834567158
245,792,792,1584,0.37305498123168945,1.539804422827956
246,796,796,1592,0.3748018741607666,1.5399324976606295
247,798,798,1596,0.3759748935699463,1.4595216815865797
248,802,802,1604,0.3776588439941406,1.457492779633526
249,806,806,1612,0.3793158531188965,1.451351983615723
250,810,810,1620,0.38126587867736816,1.4441461736146266
251,812,812,1624,0.3824307918548584,1.3962984076256362
252,816,816,1632,0.3843538761138916,1.3943894129631644
253,818,818,1636,0.38561081886291504,1.3277647048759036
254,822,822,1644,0.38762903213500977,1.3238124109149112
255,824,824,1648,0.3889288902282715,1.1894627307544852
256,828,828,1656,0.3907890319824219,1.1889302402944395
257,830,830,1660,0.3918938636779785,1.0921027037509248
258,834,834,1668,0.39353179931640625,1.0945440605648855
259,836,836,1672,0.394608736038208,0.9863003129419212
260,840,840,1680,0.3961479663848877,0.9973781345938733
261,842,842,1684,0.39714670181274414,0.9948753715854082
262,844,844,1688,0.39816999435424805,0.9772026523509112
263,846,846,1692,0.3993048667907715,0.8573236492251226
264,848,848,1696,0.40035390853881836,0.8743930175274954
265,850,850,1700,0.401439905166626,0.754503721637434
266,854,854,1708,0.40308403968811035,0.7558048810915352
267,858,858,1716,0.4047539234161377,0.7587031211469366
268,860,860,1720,0.4058527946472168,0.7716867454963676
269,864,864,1728,0.40758395195007324,0.771385399726114
270,866,866,1732,0.40866684913635254,0.7242090134044474
271,870,870,1740,0.4103820323944092,0.7203558221382309
272,872,872,1744,0.41150403022766113,0.6308759675746387
273,876,876,1752,0.41318583488464355,0.6319081397109585
274,878,878,1756,0.41420578956604004,0.5667572657995379
275,882,882,1764,0.4158189296722412,0.5671467623543549
276,884,884,1768,0.4168848991394043,0.5086225884303985
277,888,888,1776,0.4185788631439209,0.5084680447280334
278,890,890,1780,0.41959595680236816,0.4486280803811269
279,894,894,1788,0.42117810249328613,0.45133379304809296
280,896,896,1792,0.4222707748413086,0.41860255537051216
281,900,900,1800,0.4239368438720703,0.4174434871081303
282,902,902,1804,0.4250187873840332,0.38735124546474253
283,906,906,1812,0.4266810417175293,0.39004057791385094
284,908,908,1816,0.4278247356414795,0.40530233886363476
285,910,910,1820,0.42917704582214355,0.4057127836173322
286,914,914,1828,0.4308500289916992,0.4031189305451335
287,916,916,1832,0.43187594413757324,0.33426900414190186
288,920,920,1840,0.433499813079834,0.33448825810171456
289,922,922,1844,0.43454408645629883,0.2848654882205892
290,926,926,1852,0.4361138343811035,0.2846243862148867
291,928,928,1856,0.4371068477630615,0.2384620617310702
292,932,932,1864,0.4387798309326172,0.23849762407769504
293,934,934,1868,0.4398839473724365,0.2100547479050192
294,938,938,1876,0.4415128231048584,0.21062888181336348
295,940,940,1880,0.4425027370452881,0.18409018853446923
296,944,944,1888,0.44402599334716797,0.18434489713990843
297,946,946,1892,0.4450507164001465,0.15992406703901452
298,950,950,1900,0.44677090644836426,0.16079331080436532
299,952,952,1904,0.4478340148925781,0.16029505669303035
300,954,954,1908,0.44883084297180176,0.1604635138901358
301,956,956,1912,0.44983911514282227,0.13108065334381536
302,960,960,1920,0.45154285430908203,0.13235792240323008
303,962,962,1924,0.4525768756866455,0.14060514807022173
304,966,966,1932,0.4541597366333008,0.1408280324212683
305,968,968,1936,0.45519471168518066,0.12263215844359365
306,970,970,1940,0.45627903938293457,0.11920363278613877
307,972,972,1944,0.457348108291626,0.10345324050013005
308,974,974,1948,0.4584319591522217,0.1053063422376681
309,978,978,1956,0.46015000343322754,0.09532300421017226
310,980,980,1960,0.46129679679870605,0.08712464280245058
311,984,984,1968,0.46297788619995117,0.08743290136499127
312,986,986,1972,0.46411895751953125,0.059991802363811075
313,990,990,1980,0.46582984924316406,0.06048623336118908
314,992,992,1984,0.4669978618621826,0.037213052649008205
315,994,994,1988,0.4681127071380615,0.03880695651287169
316,996,996,1992,0.4691479206085205,0.030890633285366675
317,1000,1000,2000,0.47072887420654297,0.03051995976852595
318,1002,1002,2004,0.4719359874725342,0.01824624274445341
319,1006,1006,2012,0.47362494468688965,0.018497229099125434
320,1008,1008,2016,0.47467899322509766,0.015044478316553977
321,1012,1012,2024,0.4763786792755127,0.015281504212566688
322,1014,1014,2028,0.4774138927459717,0.013159970866354342
323,1018,1018,2036,0.4790778160095215,0.013125264242717094
324,1020,1020,2040,0.48012471199035645,0.007427691634347866
325,1024,1024,2048,0.48179197311401367,0.007492982382018454
326,1026,1026,2052,0.4829699993133545,0.004969460768620593
327,1030,1030,2060,0.4846348762512207,0.0049983834584281794
328,1032,1032,2064,0.4857158660888672,0.004117810798220489
329,1036,1036,2072,0.48745083808898926,0.004145348536894744
330,1038,1038,2076,0.48874688148498535,0.004543947947468041
331,1042,1042,2084,0.4904508590698242,0.004590832591588878
332,1044,1044,2088,0.4915499687194824,0.005094218050658128
333,1048,1048,2096,0.4932279586791992,0.00504700694341409
334,1050,1050,2100,0.4943568706512451,0.004062382156007516
335,1054,1054,2108,0.4960057735443115,0.004052525135762153
336,1056,1056,2112,0.49709486961364746,0.0022521288677808116
337,1060,1060,2120,0.4987189769744873,0.002231443461255367
338,1062,1062,2124,0.4997899532318115,0.001953661173047294
339,1066,1066,2132,0.501413106918335,0.0019599522879616416
340,1068,1068,2136,0.5024549961090088,0.0017890079175231222
341,1072,1072,2144,0.5040907859802246,0.0017885119320908416
342,1074,1074,2148,0.5051476955413818,0.0016220983193306893
343,1078,1078,2156,0.5067758560180664,0.0015988236041266646
344,1080,1080,2160,0.5078277587890625,0.001309760402136817
345,1084,1084,2168,0.509443998336792,0.0013175341464375379
346,1086,1086,2172,0.5105068683624268,0.0013842497971836565
347,1088,1088,2176,0.5115368366241455,0.0013302389994578334
348,1092,1092,2184,0.5131468772888184,0.0013302050630272788
349,1094,1094,2188,0.514178991317749,0.0012356490050251523
350,1096,1096,2192,0.5151958465576172,0.0010869600306477878
351,1100,1100,2200,0.5167839527130127,0.0010834728612962863
352,1102,1102,2204,0.5178968906402588,0.0010692574192034954
353,1106,1106,2212,0.5195648670196533,0.0010763324435174582
354,1108,1108,2216,0.5206079483032227,0.0010432292019686429
355,1112,1112,2224,0.5222969055175781,0.0010413427842195233
356,1114,1114,2228,0.5234568119049072,0.0009379308415873311
357,1116,1116,2232,0.5244317054748535,0.0009690133158528624
358,1120,1120,2240,0.5260210037231445,0.0009698730060563321
359,1122,1122,2244,0.5270998477935791,0.0007656827336859351
360,1126,1126,2252,0.528846025466919,0.0007627885324836825
361,1128,1128,2256,0.5299897193908691,0.0006824496250601442
362,1132,1132,2264,0.5316469669342041,0.0006827453945561501
363,1134,1134,2268,0.5328118801116943,0.000710093037923798
364,1136,1136,2272,0.5339057445526123,0.0007159102344758139
365,1140,1140,2280,0.5355219841003418,0.0007156880801630905
366,1142,1142,2284,0.5365757942199707,0.0007186215414094477
367,1146,1146,2292,0.5383169651031494,0.0007242524734465405
368,1148,1148,2296,0.539438009262085,0.0007132210423606011
369,1152,1152,2304,0.5411298274993896,0.0007129911109586828
370,1154,1154,2308,0.5421369075775146,0.0007145973704609787
371,1156,1156,2312,0.5431699752807617,0.0006916273342767454
372,1160,1160,2320,0.5448460578918457,0.000691410778131285
373,1162,1162,2324,0.5459837913513184,0.0006693202099086193
374,1166,1166,2332,0.5476510524749756,0.0006689297832735974
375,1168,1168,2336,0.5488450527191162,0.0006408379225604222
376,1172,1172,2344,0.5505459308624268,0.0006399883427548048
377,1174,1174,2348,0.5516228675842285,0.0006064188684149485
378,1178,1178,2356,0.5534529685974121,0.0006062104910142807
379,1180,1180,2360,0.5545799732208252,0.0005725041925188634
380,1184,1184,2368,0.5562517642974854,0.0005695498996374226
381,1188,1188,2376,0.5579738616943359,0.0005664805835294828
382,1190,1190,2380,0.5591049194335938,0.0005412692418076404
383,1194,1194,2388,0.5607731342315674,0.0005407048988672614
384,1196,1196,2392,0.5618698596954346,0.0005206251781828541
385,1200,1200,2400,0.5635890960693359,0.0005203316314918993
386,1202,1202,2404,0.5647079944610596,0.0004865196059427035
387,1206,1206,2412,0.5663449764251709,0.00048635211021519353
388,1208,1208,2416,0.5674459934234619,0.0004703863062331948
389,1212,1212,2424,0.5690689086914062,0.00047006845238684036
390,1214,1214,2428,0.5701498985290527,0.0004538879855999767
391,1218,1218,2436,0.5717818737030029,0.0004524458557852995
392,1220,1220,2440,0.5728259086608887,0.0004461830535547051
393,1224,1224,2448,0.5744328498840332,0.0004460470754565904
394,1226,1226,2452,0.5754878520965576,0.00043044906340128364
395,1228,1228,2456,0.5766057968139648,0.0004198590888790932
396,1232,1232,2464,0.5782630443572998,0.0004196349591438775
397,1234,1234,2468,0.5793099403381348,0.00040597236727535346
398,1238,1238,2476,0.5809609889984131,0.00040617061392822507
399,1242,1242,2484,0.58266282081604,0.00040591005426904303
400,1246,1246,2492,0.5843949317932129,0.0004050892520126581
401,1250,1250,2500,0.5862069129943848,0.00040262266747959075
402,1254,1254,2508,0.5879578590393066,0.0004012647622175791
403,1258,1258,2516,0.5895757675170898,0.000400154734620628
404,1260,1260,2520,0.5906150341033936,0.00036911935876560165
405,1264,1264,2528,0.5924818515777588,0.00036903863281168015
406,1266,1266,2532,0.5937788486480713,0.00035618920105662255
407,1270,1270,2540,0.595465898513794,0.00035601043703081814
408,1272,1272,2544,0.5966000556945801,0.00034578333816170925
409,1276,1276,2552,0.598505973815918,0.0003458306305219594
410,1278,1278,2556,0.5998189449310303,0.0003234764535591239
411,1282,1282,2564,0.601524829864502,0.00032364377557314583
412,1284,1284,2568,0.6026170253753662,0.0003238208300899714
413,1288,1288,2576,0.6042778491973877,0.0003189317455962737
414,1292,1292,2584,0.6058709621429443,0.00031283232158330065
415,1294,1294,2588,0.6068918704986572,0.00028843903737652
416,1298,1298,2596,0.6084928512573242,0.00028803691714074375
417,1300,1300,2600,0.6095919609069824,0.00025929847811312356
418,1304,1304,2608,0.6114108562469482,0.000258920481428504
419,1306,1306,2612,0.6124420166015625,0.00024275955649954994
420,1310,1310,2620,0.6141397953033447,0.0002424792031661127
421,1312,1312,2624,0.6152598857879639,0.00021720905795064027
422,1316,1316,2632,0.6170098781585693,0.00021634213044308126
423,1318,1318,2636,0.618034839630127,0.00019605517945819884
424,1322,1322,2644,0.6195659637451172,0.00019418428917106212
425,1326,1326,2652,0.6211638450622559,0.00019109083177681896
426,1328,1328,2656,0.6222450733184814,0.00016028905122311699
427,1332,1332,2664,0.6238148212432861,0.00016006585735794943
428,1334,1334,2668,0.6248791217803955,0.00013955919973795972
429,1338,1338,2676,0.6264939308166504,0.00014020771266132215
430,1340,1340,2680,0.6275577545166016,0.0001355508503593228
431,1344,1344,2688,0.6292388439178467,0.00013459265687743027
432,1346,1346,2692,0.6302587985992432,0.0001195597285459371
433,1350,1350,2700,0.6319301128387451,0.00011874423330482387
434,1352,1352,2704,0.6330139636993408,8.351353392299643e-05
435,1356,1356,2712,0.6347377300262451,8.322630367274542e-05
436,1358,1358,2716,0.6357967853546143,5.609129743788799e-05
437,1362,1362,2724,0.6374220848083496,5.577578212978551e-05
438,1364,1364,2728,0.6384670734405518,3.922211465123837e-05
439,1368,1368,2736,0.6400139331817627,3.8842967455821054e-05
440,1370,1370,2740,0.6409897804260254,2.082645346490608e-05
441,1374,1374,2748,0.6424939632415771,2.1080664055261877e-05
442,1376,1376,2752,0.6434929370880127,1.9879524643329205e-05
443,1378,1378,2756,0.6445460319519043,1.5597757396790257e-05
444,1380,1380,2760,0.6455578804016113,1.2831606795771222e-05
445,1384,1384,2768,0.6471409797668457,1.2819439575650904e-05
446,1386,1386,2772,0.6481337547302246,1.1442085224189213e-05
447,1390,1390,2780,0.6496989727020264,1.1388267580514366e-05
448,1392,1392,2784,0.6507377624511719,8.61494572745869e-06
449,1396,1396,2792,0.6523020267486572,8.692821324984834e-06
450,1398,1398,2796,0.6533219814300537,1.1486233347568486e-05
451,1402,1402,2804,0.6549417972564697,1.1611519198595488e-05
452,1404,1404,2808,0.6560509204864502,9.78488253622345e-06
453,1408,1408,2816,0.6576719284057617,9.746538466970378e-06
454,1410,1410,2820,0.6586987972259521,4.3941130343228e-06
455,1414,1414,2828,0.6604530811309814,4.340223995313863e-06
456,1416,1416,2832,0.6615748405456543,9.697744189907098e-07
457,1418,1418,2836,0.6626338958740234,9.95300638351182e-07
458,1420,1420,2840,0.6637187004089355,4.734527010441525e-07
459,1422,1422,2844,0.664741039276123,2.6878444714384386e-07
460,1426,1426,2852,0.6663968563079834,2.6967529720423045e-07
461,1428,1428,2856,0.667515754699707,1.0036023923021276e-07
462,1432,1432,2864,0.6692500114440918,9.555753877066309e-08
463,1434,1434,2868,0.6703050136566162,6.447271516663022e-08
464,1436,1436,2872,0.6713290214538574,1.7600518731342163e-07
465,1440,1440,2880,0.6728477478027344,1.7922491224453552e-07
466,1442,1442,2884,0.6738460063934326,3.1787078569323057e-07
467,1446,1446,2892,0.6753509044647217,3.1926504107104847e-07
468,1448,1448,2896,0.676318883895874,2.570556034697802e-07
469,1452,1452,2904,0.6778719425201416,2.586766640888527e-07
470,1454,1454,2908,0.6788840293884277,2.982908426929498e-07
471,1456,1456,2912,0.6798808574676514,2.6638349481800105e-07
472,1460,1460,2920,0.6814918518066406,2.6620455173542723e-07
473,1462,1462,2924,0.6825180053710938,2.716778908506967e-07
474,1466,1466,2932,0.6840648651123047,2.708458168854122e-07
475,1468,1468,2936,0.6850826740264893,2.448339273541933e-07
476,1472,1472,2944,0.6866180896759033,2.388965185673442e-07
477,1474,1474,2948,0.6876001358032227,2.0013283119624248e-07
478,1478,1478,2956,0.6892688274383545,1.9955996322096325e-07
479,1480,1480,2960,0.6903998851776123,1.6573096672800602e-07
480,1484,1484,2968,0.692180871963501,1.6619446796539705e-07
481,1486,1486,2972,0.6932089328765869,1.402786438120529e-07
482,1490,1490,2980,0.6948719024658203,1.4062914033274865e-07
483,1492,1492,2984,0.6959989070892334,1.4943191217753338e-07
484,1494,1494,2988,0.697145938873291,1.57984800353006e-07
485,1498,1498,2996,0.6989238262176514,1.5818750398466364e-07
486,1500,1500,3000,0.7000119686126709,1.3792487152386457e-07
487,1504,1504,3008,0.7017068862915039,1.3722990388487233e-07
488,1506,1506,3012,0.7028217315673828,1.1580789305298822e-07
489,1510,1510,3020,0.7045228481292725,1.1562065083126072e-07
490,1512,1512,3024,0.7055940628051758,1.0055430266220355e-07
491,1516,1516,3032,0.7073509693145752,1.0022256446973188e-07
492,1518,1518,3036,0.708488941192627,9.07494950297405e-08
493,1520,1520,3040,0.7095599174499512,7.892776920925826e-08
494,1524,1524,3048,0.7112476825714111,7.849166649975814e-08
495,1526,1526,3052,0.7123351097106934,5.926051471760729e-08
496,1530,1530,3060,0.7139897346496582,5.915183010074543e-08
497,1532,1532,3064,0.7150099277496338,5.117976797919255e-08
498,1536,1536,3072,0.7166488170623779,5.1282086133142e-08
499,1538,1538,3076,0.7177300453186035,4.882883786194725e-08
500,1542,1542,3084,0.7193589210510254,4.8791207518661395e-08
501,1544,1544,3088,0.7203638553619385,5.1002302825509105e-08
502,1548,1548,3096,0.7220079898834229,5.125855295773363e-08
503,1550,1550,3100,0.7231459617614746,5.200149644224439e-08
504,1554,1554,3108,0.7248361110687256,5.1883830565202516e-08
505,1556,1556,3112,0.7258780002593994,4.9352024689142127e-08
506,1560,1560,3120,0.7275419235229492,4.923424512526253e-08
507,1562,1562,3124,0.7285959720611572,4.8583615352981724e-08
508,1564,1564,3128,0.7296481132507324,5.1394067668297794e-08
509,1568,1568,3136,0.731285810470581,5.139384029462235e-08
510,1570,1570,3140,0.7323451042175293,5.048639195592841e-08
511,1574,1574,3148,0.7339560985565186,5.024367055739276e-08
512,1576,1576,3152,0.7351059913635254,4.620892468665261e-08
513,1580,1580,3160,0.7368428707122803,4.616254045686219e-08
514,1582,1582,3164,0.7382907867431641,4.4338889892969746e-08
515,1586,1586,3172,0.7402360439300537,4.428125066624489e-08
516,1588,1588,3176,0.7414429187774658,4.0221152630692814e-08
517,1592,1592,3184,0.7434649467468262,4.0172039916797075e-08
518,1594,1594,3188,0.7447090148925781,3.649518021120457e-08
519,1598,1598,3196,0.7466080188751221,3.641366674855817e-08
520,1600,1600,3200,0.7477827072143555,3.2361072044295724e-08
521,1604,1604,3208,0.7497110366821289,3.239711077185348e-08
522,1606,1606,3212,0.7510168552398682,3.105628820776474e-08
523,1610,1610,3220,0.7527139186859131,3.09861434288905e-08
524,1612,1612,3224,0.7539377212524414,2.7630335353023838e-08
525,1616,1616,3232,0.7558038234710693,2.7509713618201204e-08
526,1618,1618,3236,0.7569899559020996,2.6181510293099564e-08
527,1622,1622,3244,0.758793830871582,2.58745558312512e-08
528,1626,1626,3252,0.7607729434967041,2.548756583564682e-08
529,1628,1628,3256,0.7623388767242432,2.3176994545792695e-08
530,1632,1632,3264,0.7641468048095703,2.301283075212268e-08
531,1636,1636,3272,0.7658827304840088,2.2868903215567116e-08
532,1638,1638,3276,0.7672328948974609,2.14466808756697e-08
533,1642,1642,3284,0.7693109512329102,2.1369942260207608e-08
534,1646,1646,3292,0.7714920043945312,2.1190885490796063e-08
535,1648,1648,3296,0.7729299068450928,2.1677237782569136e-08
536,1652,1652,3304,0.7753961086273193,2.167257662222255e-08
537,1656,1656,3312,0.777379035949707,2.170077095797751e-08
538,1660,1660,3320,0.7794308662414551,2.1776145331386942e-08
539,1664,1664,3328,0.7815148830413818,2.182230218750192e-08
540,1668,1668,3336,0.7834417819976807,2.1855726117792074e-08
541,1670,1670,3340,0.7845509052276611,2.1796154214825947e-08
542,1674,1674,3348,0.7867147922515869,2.1760001800430473e-08
543,1678,1678,3356,0.788672924041748,2.166893864341546e-08
544,1682,1682,3364,0.7904648780822754,2.160084022762021e-08
545,1686,1686,3372,0.7922537326812744,2.1553432816290297e-08
546,1688,1688,3376,0.7935528755187988,2.1363575797295198e-08
547,1692,1692,3384,0.7954549789428711,2.1364940039347857e-08
548,1696,1696,3392,0.7975778579711914,2.1345158529584296e-08
549,1700,1700,3400,0.7996447086334229,2.1219193513388745e-08
550,1704,1704,3408,0.8018128871917725,2.1121195459272712e-08
551,1708,1708,3416,0.803865909576416,2.103377028106479e-08
552,1712,1712,3424,0.8057169914245605,2.0959760149708018e-08
553,1716,1716,3432,0.8077778816223145,2.0901325115119107e-08
554,1720,1720,3440,0.809751033782959,2.0824359125981573e-08
555,1724,1724,3448,0.8115129470825195,2.075375959975645e-08
556,1728,1728,3456,0.8134660720825195,2.0626771402021404e-08
557,1732,1732,3464,0.8154327869415283,2.0541506273730192e-08
558,1736,1736,3472,0.8173727989196777,2.0509446585492697e-08
559,1740,1740,3480,0.8192570209503174,2.045135261141695e-08
560,1744,1744,3488,0.8211019039154053,2.0329366634541657e-08
561,1748,1748,3496,0.8230819702148438,2.023455181188183e-08
562,1752,1752,3504,0.8248398303985596,2.009880972764222e-08
563,1756,1756,3512,0.8268420696258545,2.001240773097379e-08
564,1760,1760,3520,0.8288378715515137,1.9916342353099026e-08
565,1764,1764,3528,0.8306670188903809,1.979572061827639e-08
566,1768,1768,3536,0.832460880279541,1.9626440916908905e-08
567,1772,1772,3544,0.8345730304718018,1.9470121515041683e-08
568,1776,1776,3552,0.8366110324859619,1.9124740902043413e-08
569,1780,1780,3560,0.8384718894958496,1.887121925392421e-08
570,1784,1784,3568,0.840634822845459,1.8325522432860453e-08
571,1788,1788,3576,0.8426821231842041,1.7929437490238342e-08
572,1792,1792,3584,0.8444609642028809,1.733349108690163e-08
573,1796,1796,3592,0.8465089797973633,1.6911712918954436e-08
574,1798,1798,3596,0.8479509353637695,1.468401933379937e-08
575,1802,1802,3604,0.8498799800872803,1.4437546269618906e-08
576,1806,1806,3612,0.851815938949585,1.4285546967585105e-08
577,1810,1810,3620,0.8538920879364014,1.4034185369382612e-08
578,1814,1814,3628,0.8558859825134277,1.3768953976978082e-08
579,1818,1818,3636,0.8576908111572266,1.3317730918060988e-08
580,1822,1822,3644,0.8596620559692383,1.290425188926747e-08
581,1826,1826,3652,0.8615458011627197,1.2113673619751353e-08
582,1830,1830,3660,0.8633708953857422,1.1212819117645267e-08
583,1832,1832,3664,0.8645498752593994,6.931600182724651e-09
584,1836,1836,3672,0.8670179843902588,6.8890813054167666e-09
585,1838,1838,3676,0.8683187961578369,3.9202632251544856e-09
586,1842,1842,3684,0.8700878620147705,3.88752141589066e-09
587,1846,1846,3692,0.8721320629119873,3.5196308090235107e-09
588,1848,1848,3696,0.8740339279174805,6.559730536537245e-10


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.00524592399597168,7527.142345757873
1001,2004,1002,3006,6.168606996536255,16.46376997585321
2002,4006,2003,6009,12.14425015449524,8.48514545168473
3003,6008,3004,9012,18.24251127243042,5.4522030773732695
4004,8010,4005,12015,24.106975078582764,3.9980777974433295
5005,10012,5006,15018,29.91569423675537,3.2173101267435413
6006,12014,6007,18021,35.73200798034668,2.7275645622394222
7007,14016,7008,21024,41.512919187545776,2.38735138289303
8008,16018,8009,24027,47.32386517524719,2.137019590698401
9009,18020,9010,27030,53.11449313163757,1.9399264741477964
10010,20022,10011,30033,58.97867703437805,1.7806732271183137
11011,22024,11012,33036,64.76487708091736,1.64475708925238
12012,24026,12013,36039,70.53877305984497,1.5329695017062477
13013,26028,13014,39042,76.28334903717041,1.4313600407931517
14014,28030,14015,42045,82.13335514068604,1.3467990983663185
15015,30032,15016,45048,87.98540592193604,1.2695771070029878
16016,32034,16017,48051,93.76351428031921,1.2018053093252092
17017,34036,17018,51054,99.60527801513672,1.1412659763827833
18018,36038,18019,54057,105.37843012809753,1.0865616033352126
19019,38040,19020,57060,111.21037697792053,1.0363326272981794
20020,40042,20021,60063,116.97914600372314,0.9916556226835382
21021,42044,21022,63066,122.7497091293335,0.9495090873260779
22022,44046,22023,66069,128.66459393501282,0.9115858801906143
23023,46048,23024,69072,134.3967580795288,0.877056067380181
24024,48050,24025,72075,140.2061471939087,0.8451090230355476
25025,50052,25026,75078,145.9766411781311,0.8151736349973362
26026,52054,26027,78081,151.76988124847412,0.7869517771960091
27027,54056,27028,81084,157.5638689994812,0.7602290669910872
28028,56058,28029,84087,163.4388620853424,0.735708273246928
29029,58060,29030,87090,169.26375722885132,0.7121296809018531
30030,60062,30031,90093,175.04315185546875,0.6905402140364458
31031,62064,31032,93096,180.84079504013062,0.6703500710937078
32032,64066,32033,96099,186.63061213493347,0.6510288220470102
33033,66068,33034,99102,192.45882201194763,0.6329364259781869
34034,68070,34035,102105,198.23517107963562,0.6157365104427299
35035,70072,35036,105108,203.9878900051117,0.5997400469223066
36036,72074,36037,108111,209.87749814987183,0.5843394932417141
37037,74076,37038,111114,215.65209817886353,0.5701002409387002
38038,76078,38039,114117,221.43722200393677,0.5562435481333523
39039,78080,39040,117120,227.19230103492737,0.5430425883459975
40040,80082,40041,120123,233.01116108894348,0.5305780116959795
41041,82084,41042,123126,238.94111013412476,0.5185390485494281
42042,84086,42043,126129,244.76317715644836,0.5072552916171844
43043,86088,43044,129132,250.5651650428772,0.4962846578055178
44044,88090,44045,132135,256.3382570743561,0.48589304602319316
45045,90092,45046,135138,262.2057890892029,0.4758671649124153
46046,92094,46047,138141,267.9462721347809,0.4663324039956933
47047,94096,47048,141144,273.74216508865356,0.4569982888951927
48048,96098,48049,144147,279.5212941169739,0.4481513049413479
49049,98100,49050,147150,285.2787630558014,0.43959602992799773
50050,100102,50051,150153,291.09027004241943,0.431607653537867
51051,102104,51052,153156,297.9381971359253,0.4236732652934734
52052,104106,52053,156159,303.48277401924133,0.41604045004532964
53053,106108,53054,159162,309.9316899776459,0.40859352535517246
54054,108110,54055,162165,316.2691740989685,0.40153939770425495
55055,110112,55056,165168,322.24494218826294,0.39457191845758643
56056,112114,56057,168171,328.1630132198334,0.38793356851783756
57057,114116,57058,171174,334.04368710517883,0.381523024305352
58058,116118,58059,174177,339.9151072502136,0.37542893896170426
59059,118120,59060,177180,345.74056100845337,0.3694781871927262
60060,120122,60061,180183,351.6556251049042,0.3637528583785752
61061,122124,61062,183186,357.6218190193176,0.35815365635426133
62062,124126,62063,186189,363.54300713539124,0.3527254153850663
63063,126128,63064,189192,369.41697907447815,0.3475516497474018
64064,128130,64065,192195,375.2745580673218,0.34242750683188206
65065,130132,65066,195198,381.07727909088135,0.3374594798333419
66066,132134,66067,198201,386.9293520450592,0.33262222276789544
67067,134136,67068,201204,392.7728269100189,0.3279226611593913
68068,136138,68069,204207,398.6041691303253,0.3234091668509791
69069,138140,69070,207210,404.70667123794556,0.3189813873850653
70070,140142,70071,210213,410.66291403770447,0.31460257780418033
71071,142144,71072,213216,416.9275121688843,0.31034069715497026
72072,144146,72073,216219,423.00449109077454,0.3062337285737158
73073,146148,73074,219222,428.8713710308075,0.30216377187934995
74074,148150,74075,222225,434.77087211608887,0.2983859369469428
75075,150152,75076,225228,440.6241149902344,0.29462508189499204
76076,152154,76077,228231,446.56535816192627,0.29096924982150085
77077,154156,77078,231234,452.37340211868286,0.28738530382725
78078,156158,78079,234237,458.14507508277893,0.28395255386385543
79079,158160,79080,237240,463.93813824653625,0.28057875588820025
80080,160162,80081,240243,469.7409780025482,0.2773005547169305
81081,162164,81082,243246,475.649729013443,0.27411371492962644
82082,164166,82083,246249,481.6122341156006,0.2709244806155766
83083,166168,83084,249252,487.4238700866699,0.26782627534339554
84084,168170,84085,252255,493.2290802001953,0.26481245578725066
85085,170172,85086,255258,499.08647990226746,0.26189055474242195
86086,172174,86087,258261,504.90303897857666,0.2589671402984095
87087,174176,87088,261264,510.8341152667999,0.25615314841525105
88088,176178,88089,264267,516.8106181621552,0.25336892163068114
89089,178180,89090,267270,522.6526551246643,0.2506037342845957
90090,180182,90091,270273,528.4534130096436,0.2479660567078099
91091,182184,91092,273276,534.2943832874298,0.24535204203675676
92092,184186,92093,276279,540.1380190849304,0.24281136033641815
93093,186188,93094,279282,545.9092390537262,0.24031717427533295
94094,188190,94095,282285,551.7672262191772,0.23791486212758173
95095,190192,95096,285288,557.5621240139008,0.23557761193478655
96096,192194,96097,288291,563.5387961864471,0.23322848237330618
97097,194196,97098,291294,569.3846161365509,0.23097349975250836
98098,196198,98099,294297,575.1747100353241,0.22871175598447735
99099,198200,99100,297300,580.9693460464478,0.22651056759787025
100100,200202,100101,300303,586.7766761779785,0.2243398152604641
101101,202204,101102,303306,592.6336052417755,0.22225886511296267
102102,204206,102103,306309,598.587249994278,0.2201789136215666
103103,206208,103104,309312,604.403774023056,0.21813595217281545
104104,208210,104105,312315,610.1745111942291,0.21609461194384494
105105,210212,105106,315318,616.0392909049988,0.21412555549977697
106106,212214,106107,318321,621.863254070282,0.21220098950834654
107107,214216,107108,321324,627.7097799777985,0.21033715482553816
108108,216218,108109,324327,633.5544030666351,0.20848555167685845
109109,218220,109110,327330,639.4589982032776,0.206694627444449
110110,220222,110111,330333,645.4049742221832,0.20489045552494645
111111,222224,111112,333336,651.2468740940094,0.20314364079422376
112112,224226,112113,336339,657.0266292095184,0.2014319482823339
113113,226228,113114,339342,662.8539600372314,0.1997364304279472
114114,228230,114115,342345,668.6839220523834,0.19806727497052634
115115,230232,115116,345348,674.580982208252,0.1964416926384729
116116,232234,116117,348351,680.4787971973419,0.19482293022156227
117117,234236,117118,351354,686.2968010902405,0.19323625365541375
118118,236238,118119,354357,692.1360692977905,0.19167494523935602
119119,238240,119120,357360,698.0135760307312,0.19015523517919064
120120,240242,120121,360363,703.972188949585,0.18865374462438922
121121,242244,121122,363366,709.875324010849,0.1871780400415446
122122,244246,122123,366369,715.6924180984497,0.18570897196696023
123123,246248,123124,369372,721.5590920448303,0.1842725486476411
124124,248250,124125,372375,727.3816781044006,0.1828258320256282
125125,250252,125126,375378,733.2056610584259,0.18138803901274514
126126,252254,126127,378381,739.2799570560455,0.18003050685183553
127127,254256,127128,381384,745.5255081653595,0.1786724548037455
128128,256258,128129,384387,751.3979971408844,0.1773289959110116
129129,258260,129130,387390,757.2427341938019,0.17602107230050024
130130,260262,130131,390393,763.0745980739594,0.1747086486338958
131131,262264,131132,393396,768.9903528690338,0.1734299444106
132132,264266,132133,396399,774.8265380859375,0.1721219385508448
133133,266268,133134,399402,780.6700301170349,0.17089104805381794
134134,268270,134135,402405,786.5174779891968,0.16968282992820605
135135,270272,135136,405408,792.45055103302,0.1684859566648811
136136,272274,136137,408411,798.2634990215302,0.16730126798756828
137137,274276,137138,411414,804.1004440784454,0.16612494951368717
138138,276278,138139,414417,809.884485244751,0.1649727831572818
139139,278280,139140,417420,815.7493410110474,0.1638340034878638
140140,280282,140141,420423,821.5696032047272,0.16272632714390056
141141,282284,141142,423426,827.3581142425537,0.16161944784835214
142142,284286,142143,426429,833.1705439090729,0.16054115742372232
143143,286288,143144,429432,839.0296010971069,0.15947271819823072
144144,288290,144145,432435,844.7957079410553,0.1584072389141511
145145,290292,145146,435438,850.4965331554413,0.15736335196379514
146146,292294,146147,438441,856.3133089542389,0.15631539871174027
147147,294296,147148,441444,862.1683280467987,0.15528106102101447
148148,296298,148149,444447,868.0054430961609,0.15427053528219403
149149,298300,149150,447450,873.8361251354218,0.15326301211644022
150150,300302,150151,450453,879.6572659015656,0.15227312663591874
151151,302304,151152,453456,885.4280421733856,0.15129672681177908
152152,304306,152153,456459,891.2643671035767,0.15033360670167895
153153,306308,153154,459462,897.0654480457306,0.14939380004580016
154154,308310,154155,462465,902.858724117279,0.14847284101051628
155155,310312,155156,465468,908.7203199863434,0.1475671823573066
156156,312314,156157,468471,914.6176111698151,0.14666071593092056
157157,314316,157158,471474,920.4799330234528,0.14574198285481543
158158,316318,158159,474477,926.3533620834351,0.1448546393057768
159159,318320,159160,477480,932.2089102268219,0.1439816642068763
160160,320322,160161,480483,938.1609301567078,0.14311205737976707
161161,322324,161162,483486,944.1884090900421,0.14225166074902518
162162,324326,162163,486489,950.0822122097015,0.14140785408199008
163163,326328,163164,489492,955.968670129776,0.14058788203874428
164164,328330,164165,492495,961.7843980789185,0.1397537621378433
165165,330332,165166,495498,967.5312662124634,0.13892438611219404
166166,332334,166167,498501,973.4250330924988,0.13812109531863825
167167,334336,167168,501504,979.319258928299,0.1373220195146132
168168,336338,168169,504507,985.1604082584381,0.1365360792278807
169169,338340,169170,507510,991.0741770267487,0.13576560800174775
170170,340342,170171,510513,996.895809173584,0.13500098550503026
171171,342344,171172,513516,1002.8029279708862,0.13424315989141178
172172,344346,172173,516519,1008.7429718971252,0.1334929506538174
173173,346348,173174,519522,1014.589497089386,0.13274187100614654
174174,348350,174175,522525,1020.5476880073547,0.13201288876734907
175175,350352,175176,525528,1026.4447031021118,0.13128923337535525
176176,352354,176177,528531,1032.3322150707245,0.13057848890275636
177177,354356,177178,531534,1038.1987462043762,0.12986629625629575
178178,356358,178179,534537,1044.0202810764313,0.12915547236116254
179179,358360,179180,537540,1049.9380490779877,0.12844716732979578
180180,360362,180181,540543,1055.821984052658,0.1277780954605987
181181,362364,181182,543546,1061.6632919311523,0.12707861620219774
182182,364366,182183,546549,1067.5321350097656,0.12640898462632322
183183,366368,183184,549552,1073.388952255249,0.12572043267573463
184184,368370,184185,552555,1079.400316953659,0.1250525660761923
185185,370372,185186,555558,1085.283503293991,0.12438902801113727
186186,372374,186187,558561,1091.1273910999298,0.12373923060658854
187187,374376,187188,561564,1097.0987479686737,0.12308724256945425
188188,376378,188189,564567,1102.96107006073,0.12244923271828156
189189,378380,189190,567570,1108.9395761489868,0.12180293255005381
190190,380382,190191,570573,1114.8520991802216,0.12117851017137582
191191,382384,191192,573576,1120.8473238945007,0.12054525416897377
192192,384386,192193,576579,1126.7932271957397,0.11993042180074553
193193,386388,193194,579582,1132.6801800727844,0.11930579677937203
194194,388390,194195,582585,1138.6787781715393,0.11867665530371596
195195,390392,195196,585588,1144.6325929164886,0.11808030541033077
196196,392394,196197,588591,1150.6567749977112,0.1174868297039211
197197,394396,197198,591594,1156.7400221824646,0.11687776174039755
198198,396398,198199,594597,1162.7759351730347,0.11630022701683629
199199,398400,199200,597600,1168.7674300670624,0.11572282843917492
200200,400402,200201,600603,1174.7755601406097,0.11514303961484984
201201,402404,201202,603606,1180.8318181037903,0.11457309933575743
202202,404406,202203,606609,1186.9059360027313,0.114010908317141
203203,406408,203204,609612,1192.9139821529388,0.11344295977323782
204204,408410,204205,612615,1198.9909970760345,0.11291881792385539
205205,410412,205206,615618,1204.9287309646606,0.11236807519344438
206206,412414,206207,618621,1210.997976064682,0.11183847311440331
207207,414416,207208,621624,1217.000277042389,0.11130251501344901
208208,416418,208209,624627,1222.9151151180267,0.11081021855898143
209209,418420,209210,627630,1228.8720951080322,0.11032931312001892
210210,420422,210211,630633,1234.8411331176758,0.10985254619845364
211211,422424,211212,633636,1240.7472982406616,0.10937979298796563
212212,424426,212213,636639,1246.6459341049194,0.10891093902864668
213213,426428,213214,639642,1252.6315469741821,0.10844587018618768
214214,428430,214215,642645,1258.6628329753876,0.10798446310400323
215215,430432,215216,645648,1264.594978094101,0.10752847626281437
216216,432434,216217,648651,1270.5260150432587,0.10707407495101506
217217,434436,217218,651654,1276.4392330646515,0.10662463740845851
218218,436438,218219,654657,1282.4797179698944,0.10617938954965211
219219,438440,219220,657660,1288.4002392292023,0.1057380052661756
220220,440442,220221,660663,1294.2937080860138,0.10530145844677463
221221,442444,221222,663666,1300.2251431941986,0.10484576932503842
222222,444446,222223,666669,1306.1267850399017,0.10435579082513868
223223,446448,223224,669672,1311.997267961502,0.10388100361160468
224224,448450,224225,672675,1317.9537770748138,0.10341459934170416
225225,450452,225226,675678,1323.8784720897675,0.10295467936884961
226226,452454,226227,678681,1329.8209171295166,0.10249081004440086
227227,454456,227228,681684,1335.763337135315,0.10202284718252486
228228,456458,228229,684687,1341.7797739505768,0.10157631143374601
229229,458460,229230,687690,1347.705164194107,0.10113154560349358
230230,460462,230231,690693,1353.5927832126617,0.10072797022257873
231231,462464,231232,693696,1359.5377600193024,0.10032745263197285
232232,464466,232233,696699,1365.449522972107,0.09992631787645223
233233,466468,233234,699702,1371.4506969451904,0.09952902292752697
234234,468470,234235,702705,1377.5097212791443,0.09913757622780395
235235,470472,235236,705708,1383.4411380290985,0.09875438753078924
236236,472474,236237,708711,1389.5388760566711,0.09832427443325287
237237,474476,237238,711714,1395.5064570903778,0.09790229306236142
238238,476478,238239,714717,1401.4664211273193,0.09747594391046732
239239,478480,239240,717720,1407.5031850337982,0.09705977148951206
240240,480482,240241,720723,1413.4592640399933,0.09663849666321767
241241,482484,241242,723726,1419.4675650596619,0.09622808482163236
242242,484486,242243,726729,1425.402330160141,0.09582709879214235
243243,486488,243244,729732,1431.3182458877563,0.09543003208818845
244244,488490,244245,732735,1437.3187379837036,0.09504475825815462
245245,490492,245246,735738,1443.2808289527893,0.09466365915614006
246246,492494,246247,738741,1449.2068700790405,0.09428639578982256
247247,494496,247248,741744,1455.1236202716827,0.09391276008136629
248248,496498,248249,744747,1461.071527004242,0.0935426774667576
249249,498500,249250,747750,1467.0196371078491,0.09317689506679017
250250,500502,250251,750753,1472.9241499900818,0.09281490913963353
251251,502504,251252,753756,1478.8638000488281,0.0924558951119252
252252,504506,252253,756759,1484.8179032802582,0.09210093125511776
253253,506508,253254,759762,1490.8700449466705,0.09174903343046026
254254,508510,254255,762765,1496.7930450439453,0.09139891977974912
255255,510512,255256,765768,1502.811734199524,0.09103830885760544
256256,512514,256257,768771,1508.724797964096,0.09067902943206718
257257,514516,257258,771774,1514.6530921459198,0.09032073061644041
258258,516518,258259,774777,1520.6287100315094,0.08996952444613271
259259,518520,259260,777780,1526.5969212055206,0.08962440159120888
260260,520522,260261,780783,1532.680652141571,0.08930525962932734
261261,522524,261262,783786,1538.6755661964417,0.08898871089695604
262262,524526,262263,786789,1544.7528729438782,0.0886754129514884
263263,526528,263264,789792,1550.788110256195,0.08836552932916675
264264,528530,264265,792795,1556.843961238861,0.08805941365972103
265265,530532,265266,795798,1562.8320331573486,0.08774605611870356
266266,532534,266267,798801,1568.8394770622253,0.08742265405817307
267267,534536,267268,801804,1574.833547115326,0.08708969907820574
268268,536538,268269,804807,1580.8308591842651,0.08676268521776365
269269,538540,269270,807810,1586.6785650253296,0.086432469990541
270270,540542,270271,810813,1592.585371017456,0.08610809290257748
271271,542544,271272,813816,1598.5943429470062,0.08578260872855026
272272,544546,272273,816819,1604.490956068039,0.08546084996305581
273273,546548,273274,819822,1610.413066148758,0.08513591253176855
274274,548550,274275,822825,1616.326093196869,0.08481708764338691
275275,550552,275276,825828,1622.2342081069946,0.08450090117185027
276276,552554,276277,828831,1628.0799779891968,0.0841862701709033
277277,554556,277278,831834,1633.9400792121887,0.08387538214810775
278278,556558,278279,834837,1639.869933128357,0.08355503254642827
279279,558560,279280,837840,1645.7473359107971,0.08324913440264936
280280,560562,280281,840843,1651.6712760925293,0.08293985928503389
281281,562564,281282,843846,1657.6738390922546,0.08263716535293497
282282,564566,282283,846849,1663.5592761039734,0.08233613666379824
283283,566568,283284,849852,1669.4589629173279,0.0820272650289553
284284,568570,284285,852855,1675.3732821941376,0.08173515734779357
285285,570572,285286,855858,1681.3507242202759,0.08144499394620652
286286,572574,286287,858861,1687.2704389095306,0.08116325298760785
287287,574576,287288,861864,1693.2577753067017,0.08087118736875709
288288,576578,288289,864867,1699.1739621162415,0.08059296972896846
289289,578580,289290,867870,1704.505851984024,0.08030881610466167
290290,580582,290291,870873,1709.628072977066,0.08002719546675507
291291,582584,291292,873876,1715.301931142807,0.07974968731286936
292292,584586,292293,876879,1721.3011021614075,0.0794773135894502
293293,586588,293294,879882,1727.2347221374512,0.07920218691106129
294294,588590,294295,882885,1733.1739451885223,0.07892955125680601
295295,590592,295296,885888,1739.1086852550507,0.07866142302736989
296296,592594,296297,888891,1745.0239770412445,0.07839333750052901
297297,594596,297298,891894,1750.9227540493011,0.0781235255599313
298298,596598,298299,894897,1756.8907611370087,0.07786317162572232
299299,598600,299300,897900,1762.8684811592102,0.07760599644825561
300300,600602,300301,900903,1768.8545689582825,0.07734371792685124
301301,602604,301302,903906,1774.6548750400543,0.07708481636473152
302302,604606,302303,906909,1780.6342680454254,0.07683821329737839
303303,606608,303304,909912,1786.5210859775543,0.07657845477660885
304304,608610,304305,912915,1792.4065222740173,0.0763233019188192
305305,610612,305306,915918,1798.3217549324036,0.07607083349284949
306306,612614,306307,918921,1804.1827290058136,0.0758287567714433
307307,614616,307308,921924,1810.098687171936,0.0755809684706037
308308,616618,308309,924927,1816.0868968963623,0.07533095331018558
309309,618620,309310,927930,1821.9811289310455,0.07508620026055723
310310,620622,310311,930933,1827.8422951698303,0.07484861741068016
311311,622624,311312,933936,1833.9309849739075,0.07461206399784714
312312,624626,312313,936939,1839.9085240364075,0.07437094065608107
313313,626628,313314,939942,1845.8512151241302,0.0741304615385161
314314,628630,314315,942945,1851.7970950603485,0.07389385086753464
315315,630632,315316,945948,1857.9082400798798,0.07365278374163609
316316,632634,316317,948951,1864.3657631874084,0.07341957479002303
317317,634636,317318,951954,1870.3236110210419,0.07319258436837117
318318,636638,318319,954957,1876.2774951457977,0.0729652427653491
319319,638640,319320,957960,1882.1805529594421,0.07273982718288607
320320,640642,320321,960963,1888.0865211486816,0.0725208781332185
321321,642644,321322,963966,1894.0013890266418,0.07229974071560719
322322,644646,322323,966969,1899.8574981689453,0.07207615140396229
323323,646648,323324,969972,1905.7969710826874,0.07184895607315411
324324,648650,324325,972975,1911.763034105301,0.07163645474975056
325325,650652,325326,975978,1917.7012190818787,0.07141815992326883
326326,652654,326327,978981,1923.6718490123749,0.07119859490376257
327327,654656,327328,981984,1929.5698170661926,0.07098062742807087
328328,656658,328329,984987,1935.4837939739227,0.07076166092883795
329329,658660,329330,987990,1941.3302690982819,0.07054840333148604
330330,660662,330331,990993,1947.2470469474792,0.07033354612758558
331331,662664,331332,993996,1953.1199660301208,0.07012106515321648
332332,664666,332333,996999,1958.995414018631,0.06991313997423276
333333,666668,333334,1000002,1964.9297530651093,0.0697044514818117
334334,668670,334335,1003005,1970.873946905136,0.06949276062186982
335335,670672,335336,1006008,1976.7221100330353,0.06928862006679992
336336,672674,336337,1009011,1982.6042120456696,0.06908105703405454
337337,674676,337338,1012014,1988.5642802715302,0.06887636077408388
338338,676678,338339,1015017,1994.5668742656708,0.06867409212100029
339339,678680,339340,1018020,2000.4918069839478,0.0684678822526621
340340,680682,340341,1021023,2006.4442460536957,0.06826474136323668
341341,682684,341342,1024026,2012.3350450992584,0.0680618735968892
342342,684686,342343,1027029,2018.3486022949219,0.06786254041799111
343343,686688,343344,1030032,2024.4026391506195,0.0676639480261656
344344,688690,344345,1033035,2030.3523721694946,0.06746002767977188
345345,690692,345346,1036038,2036.3521921634674,0.06726198054639099
346346,692694,346347,1039041,2042.280667066574,0.06706750419471064
347347,694696,347348,1042044,2048.326975107193,0.066876542978207
348348,696698,348349,1045047,2054.294336080551,0.06668445972900372
349349,698700,349350,1048050,2060.2489941120148,0.06648998583114007
350350,700702,350351,1051053,2066.280365228653,0.06630165760361706
351351,702704,351352,1054056,2072.227772951126,0.0661092765367357
352352,704706,352353,1057059,2078.148968935013,0.06591861234846874
353353,706708,353354,1060062,2084.042031288147,0.06572941586273373
354354,708710,354355,1063065,2089.964005947113,0.06553960581368301
355355,710712,355356,1066068,2095.904265165329,0.06535486467146256
356356,712714,356357,1069071,2101.795996904373,0.06517242415975488
357357,714716,357358,1072074,2107.6846611499786,0.06499041770075564
358358,716718,358359,1075077,2113.598596096039,0.06480684388588998
359359,718720,359360,1078080,2119.5634639263153,0.06462413651570387
360360,720722,360361,1081083,2125.8356630802155,0.0644431909568084
361361,722724,361362,1084086,2131.844194173813,0.06426216645741079
362362,724726,362363,1087089,2137.916430234909,0.06408413041936001
363363,726728,363364,1090092,2144.131779193878,0.0639103135872574
364364,728730,364365,1093095,2150.118113040924,0.06373443791198952
365365,730732,365366,1096098,2156.081029891968,0.06355856878872146
366366,732734,366367,1099101,2162.126820087433,0.06338433353448636
367367,734736,367368,1102104,2168.161299943924,0.06321349834433931
368368,736738,368369,1105107,2174.1346802711487,0.06303813353588339
369369,738740,369370,1108110,2180.003762960434,0.06286396560244611
370370,740742,370371,1111113,2185.9210419654846,0.0626958566281246
371371,742744,371372,1114116,2191.818237066269,0.06253027038292203
372372,744746,372373,1117119,2197.7643570899963,0.062364386749322875
373373,746748,373374,1120122,2203.665239095688,0.06219609163053974
374374,748750,374375,1123125,2209.553209066391,0.06203069273033179
375375,750752,375376,1126128,2215.4358270168304,0.06186887847434264
376376,752754,376377,1129131,2221.3088772296906,0.06170462828413292
377377,754756,377378,1132134,2227.2660870552063,0.0615429263907572
378378,756758,378379,1135137,2233.176374197006,0.06138324157655006
379379,758760,379380,1138140,2239.078533887863,0.06122056769163464
380380,760762,380381,1141143,2244.98286318779,0.061060298274242086
381381,762764,381382,1144146,2250.9499220848083,0.06089997234994371
382382,764766,382383,1147149,2256.8421483039856,0.06074177138725645
383383,766768,383384,1150152,2262.726500272751,0.06058353701882879
384384,768770,384385,1153155,2268.732104063034,0.060425492674767156
385385,770772,385386,1156158,2274.6438250541687,0.06027115297183627
386386,772774,386387,1159161,2280.6497790813446,0.06011649212632619
387387,774776,387388,1162164,2286.562005996704,0.05996089937252691
388388,776778,388389,1165167,2292.5477471351624,0.05981137978233164
389389,778780,389390,1168170,2298.5685069561005,0.0596585690836946
390390,780782,390391,1171173,2304.5329480171204,0.059503706952455104
391391,782784,391392,1174176,2310.478861093521,0.05935099839916802
392392,784786,392393,1177179,2316.526116132736,0.05920296025396965
393393,786788,393394,1180182,2322.5645229816437,0.05905186197742296
394394,788790,394395,1183185,2328.503087282181,0.058905144844175084
395395,790792,395396,1186188,2334.487225294113,0.05876187886497064
396396,792794,396397,1189191,2340.4059200286865,0.05861598527008027
397397,794796,397398,1192194,2346.3096170425415,0.05846905468933983
398398,796798,398399,1195197,2352.311109304428,0.05831840244172781
399399,798800,399400,1198200,2358.2245061397552,0.05817658436171769
400400,800802,400401,1201203,2364.1550509929657,0.05802870439947583
401401,802804,401402,1204206,2370.3334851264954,0.05788594532714342
402402,804806,402403,1207209,2375.9354209899902,0.05774257010125439
403403,806808,403404,1210212,2381.9594881534576,0.05759940478128556
404404,808810,404405,1213215,2387.930227994919,0.05745639806809777
405405,810812,405406,1216218,2393.793522119522,0.05731584597560868
406406,812814,406407,1219221,2399.81667304039,0.0571784624717111
407407,814816,407408,1222224,2405.698226928711,0.057049580123930355
408408,816818,408409,1225227,2411.54251909256,0.05692172511771787
409409,818820,409410,1228230,2417.625330924988,0.05679364110255847
410410,820822,410411,1231233,2423.5695021152496,0.056659400535863824
411411,822824,411412,1234236,2429.4947090148926,0.05652243381518929
412412,824826,412413,1237239,2435.557604074478,0.056386978956652456
413413,826828,413414,1240242,2441.456197977066,0.05625231519297813
414414,828830,414415,1243245,2447.376570224762,0.05611906938429456
415415,830832,415416,1246248,2453.292067050934,0.05598508734328789
416416,832834,416417,1249251,2459.4163432121277,0.05585262438034988
417417,834836,417418,1252254,2465.6939358711243,0.055722046352457255
418418,836838,418419,1255257,2472.204980134964,0.05558753363038704
419419,838840,419420,1258260,2478.288994073868,0.055454057293900405
420420,840842,420421,1261263,2484.2081310749054,0.05532098433468491
421421,842844,421422,1264266,2490.228786945343,0.055191688170452835
422422,844846,422423,1267269,2496.140745162964,0.055061135533833294
423423,846848,423424,1270272,2502.0654039382935,0.05493047750314872
424424,848850,424425,1273275,2507.9692721366882,0.054796986101791845
425425,850852,425426,1276278,2513.899752140045,0.05466918545971566
426426,852854,426427,1279281,2519.7959990501404,0.05454144629584334
427427,854856,427428,1282284,2525.8249349594116,0.05441804957445129
428428,856858,428429,1285287,2531.7623341083527,0.05429119392465509
429429,858860,429430,1288290,2537.7739520072937,0.05416661803974421
430430,860862,430431,1291293,2543.712461233139,0.054043663358243066
431431,862864,431432,1294296,2549.6032910346985,0.05391968598814856
432432,864866,432433,1297299,2555.561559200287,0.05379620611347491
433433,866868,433434,1300302,2561.5595421791077,0.05367155381463817
434434,868870,434435,1303305,2567.541130065918,0.0535490793408826
435435,870872,435436,1306308,2573.645776987076,0.053427838580319076
436436,872874,436437,1309311,2579.61509513855,0.05330431428956217
437437,874876,437438,1312314,2586.204750061035,0.05318313080533699
438438,876878,438439,1315317,2592.486512899399,0.05306278195894265
439439,878880,439440,1318320,2598.5104882717133,0.052942825943318894
440440,880882,440441,1321323,2604.5373220443726,0.052823980167886475
441441,882884,441442,1324326,2610.451952934265,0.05270596471564204
442442,884886,442443,1327329,2616.5132019519806,0.05258934214543842
443443,886888,443444,1330332,2622.555340051651,0.05247370304095966
444444,888890,444445,1333335,2628.5203750133514,0.05235644180538657
445445,890892,445446,1336338,2634.568125963211,0.05224011053542199
446446,892894,446447,1339341,2640.506739139557,0.05212522271358466
447447,894896,447448,1342344,2646.43731713295,0.05201096651580883
448448,896898,448449,1345347,2652.365769147873,0.05189496102684643
449449,898900,449450,1348350,2658.3147761821747,0.051778363953417283
450450,900902,450451,1351353,2664.2338712215424,0.051660210634508985
451451,902904,451452,1354356,2670.1961691379547,0.0515450945658813
452452,904906,452453,1357359,2676.141201019287,0.05143007588958426
453453,906908,453454,1360362,2682.0624051094055,0.05131820099632023
454454,908910,454455,1363365,2688.0651609897614,0.0512041421388858
455455,910912,455456,1366368,2694.0498299598694,0.05109185014953255
456456,912914,456457,1369371,2699.9741411209106,0.05098231719057367
457457,914916,457458,1372374,2705.9529852867126,0.050869180200606934
458458,916918,458459,1375377,2711.9189240932465,0.05075763394597743
459459,918920,459460,1378380,2717.8745369911194,0.05064701748415246
460460,920922,460461,1381383,2723.7996139526367,0.05053605537250405
461461,922924,461462,1384386,2729.8111340999603,0.05042898747342406
462462,924926,462463,1387389,2735.7359750270844,0.05032007618319767
463463,926928,463464,1390392,2741.6631529331207,0.05021441101234814
464464,928930,464465,1393395,2747.601678133011,0.05010577284701867
465465,930932,465466,1396398,2753.585291147232,0.04999945967392705
466466,932934,466467,1399401,2759.522177219391,0.04989252874474914
467467,934936,467468,1402404,2765.521878004074,0.04978796054820123
468468,936938,468469,1405407,2771.6038661003113,0.0496800280543539
469469,938940,469470,1408410,2777.6479501724243,0.04957539384668053
470470,940942,470471,1411413,2783.581712961197,0.049470438911157544
471471,942944,471472,1414416,2789.5636942386627,0.04936513062239101
472472,944946,472473,1417419,2795.595946073532,0.04926036002325418
473473,946948,473474,1420422,2801.6048760414124,0.04915806332064676
474474,948950,474475,1423425,2807.6218461990356,0.049053221877329634
475475,950952,475476,1426428,2813.5619621276855,0.04894980538119853
476476,952954,476477,1429431,2819.5252690315247,0.04884890140601783
477477,954956,477478,1432434,2825.453663110733,0.048745033867817256
478478,956958,478479,1435437,2831.3599491119385,0.0486444588204904
479479,958960,479480,1438440,2837.3357231616974,0.04854375630202412
480480,960962,480481,1441443,2843.35387301445,0.04844336047426623
481481,962964,481482,1444446,2849.323438167572,0.04834425718217972
482482,964966,482483,1447449,2855.332137107849,0.048243377215840155
483483,966968,483484,1450452,2861.26104927063,0.04814451791025931
484484,968970,484485,1453455,2867.155457019806,0.04804587716898823
485485,970972,485486,1456458,2873.0426802635193,0.04794755062357581
486486,972974,486487,1459461,2879.060882091522,0.047846943754848326
487487,974976,487488,1462464,2884.981786251068,0.04774991593694722
488488,976978,488489,1465467,2890.8400959968567,0.04765333165778429
489489,978980,489490,1468470,2896.7757980823517,0.04755554369694437
490490,980982,490491,1471473,2902.729198217392,0.04746093716858013
491491,982984,491492,1474476,2908.681568145752,0.047363138421133044
492492,984986,492493,1477479,2914.6368551254272,0.04726773676520679
493493,986988,493494,1480482,2920.6555330753326,0.04717168743991351
494494,988990,494495,1483485,2926.680925130844,0.04707814436915214
495495,990992,495496,1486488,2932.625396966934,0.04698609881961602
496496,992994,496497,1489491,2938.680324077606,0.046890938649085
497497,994996,497498,1492494,2944.6044211387634,0.04679628144731396
498498,996998,498499,1495497,2950.5620970726013,0.04670223916036775
499499,999000,499500,1498500,2956.5766983032227,0.04660974746548163
500501,1001004,500502,1501506,2962.597633123398,0.04651927880695439
501502,1003006,501503,1504509,2968.6872720718384,0.04642597649944946
502503,1005008,502504,1507512,2974.710160970688,0.0463352082970232
503504,1007010,503505,1510515,2980.6756801605225,0.04624382005385996
504505,1009012,504506,1513518,2986.6660590171814,0.04615378849848639
505506,1011014,505507,1516521,2992.6281139850616,0.04606142116972478
506507,1013016,506508,1519524,2998.64391207695,0.045971269168148865
507508,1015018,507509,1522527,3004.696156978607,0.04588234182665474
508509,1017020,508510,1525530,3010.6606442928314,0.04579399585418287
509510,1019022,509511,1528533,3016.6237618923187,0.04570254935606499
510511,1021024,510512,1531536,3022.7137820720673,0.045613799842612934
511512,1023026,511513,1534539,3028.7531020641327,0.04552274275920354
512513,1025028,512514,1537542,3034.7768211364746,0.04543297012060066
513514,1027030,513515,1540545,3040.8221950531006,0.04534179734218924
514515,1029032,514516,1543548,3046.802710056305,0.04525303141599579
515516,1031034,515517,1546551,3052.940104007721,0.04516509465247509
516517,1033036,516518,1549554,3060.7394630908966,0.04507798487065884
517518,1035038,517519,1552557,3068.93558716774,0.04499163968102948
518519,1037040,518520,1555560,3075.189688205719,0.04490560801968968
519520,1039042,519521,1558563,3081.330871105194,0.04482093913611607
520521,1041044,520522,1561566,3087.3282220363617,0.044736689582350664
521522,1043046,521523,1564569,3093.2577650547028,0.044650701243881485
522523,1045048,522524,1567572,3099.2191441059113,0.044564141773662413
523524,1047050,523525,1570575,3105.1614983081818,0.044480151003881474
524525,1049052,524526,1573578,3111.228073120117,0.04439505249138165
525526,1051054,525527,1576581,3117.5531611442566,0.04430925250380824
526527,1053056,526528,1579584,3123.6795320510864,0.04422400847033714
527528,1055058,527529,1582587,3129.5421481132507,0.044140438754766365
528529,1057060,528530,1585590,3135.4115750789642,0.04405879720252415
529530,1059062,529531,1588593,3141.277333021164,0.043975636775940075
530531,1061064,530532,1591596,3147.123090028763,0.04389280712894106
531532,1063066,531533,1594599,3153.0453419685364,0.043810574961753446
532533,1065068,532534,1597602,3159.0395143032074,0.04372939316635893
533534,1067070,533535,1600605,3165.0097501277924,0.043646740710755694
534535,1069072,534536,1603608,3170.902859210968,0.04356577650651161
535536,1071074,535537,1606611,3176.80842089653,0.043482897390276776
536537,1073076,536538,1609614,3183.115599155426,0.04340059301102883
537538,1075078,537539,1612617,3188.967120885849,0.043319837386661675
538539,1077080,538540,1615620,3194.3522090911865,0.04323661750277097
539540,1079082,539541,1618623,3199.5302650928497,0.04315767664957093
540541,1081084,540542,1621626,3204.618373155594,0.04307813871673716
541542,1083086,541543,1624629,3210.0585169792175,0.04299865288521687
542543,1085088,542544,1627632,3215.3828942775726,0.042919059298583306
543544,1087090,543545,1630635,3220.449171066284,0.042839948859182186
544545,1089092,544546,1633638,3225.5497410297394,0.042761939017509576
545546,1091094,545547,1636641,3231.0326931476593,0.0426828709878464
546547,1093096,546548,1639644,3237.0173971652985,0.04260394779339549
547548,1095098,547549,1642647,3242.901556968689,0.04252577901570476
548549,1097100,548550,1645650,3248.781718015671,0.04244736576038122
549550,1099102,549551,1648653,3254.671226978302,0.04237075705532334
550551,1101104,550552,1651656,3260.807384252548,0.042294648359529674
551552,1103106,551553,1654659,3267.04052901268,0.04221873370624962
552553,1105108,552554,1657662,3273.6114370822906,0.042141632120547
553554,1107110,553555,1660665,3281.308922290802,0.04206663368677255
554555,1109112,554556,1663668,3290.4779970645905,0.041990930014435435
555556,1111114,555557,1666671,3297.7542741298676,0.041915997077012435
556557,1113116,556558,1669674,3304.0784919261932,0.041839885840090574
557558,1115118,557559,1672677,3310.0311748981476,0.04176452657338814
558559,1117120,558560,1675680,3316.412852048874,0.04168990253128868
559560,1119122,559561,1678683,3322.325664997101,0.04161502056012978
560561,1121124,560562,1681686,3328.1804769039154,0.041541722717738594
561562,1123126,561563,1684689,3334.039618253708,0.04146762393247627
562563,1125128,562564,1687692,3339.8243799209595,0.04139204547027475
563564,1127130,563565,1690695,3345.6376490592957,0.04131918354869413
564565,1129132,564566,1693698,3351.477730035782,0.04124503537605051
565566,1131134,565567,1696701,3357.3558530807495,0.04117223726643715
566567,1133136,566568,1699704,3363.208976984024,0.04109838510157715
567568,1135138,567569,1702707,3369.040143251419,0.04102657316434488
568569,1137140,568570,1705710,3374.8628540039062,0.04095401260929066
569570,1139142,569571,1708713,3380.712666988373,0.04088268140912987
570571,1141144,570572,1711716,3386.849002122879,0.0408090242453909
571572,1143146,571573,1714719,3393.157539129257,0.04073773085838184
572573,1145148,572574,1717722,3399.211822271347,0.04066773316844774
573574,1147150,573575,1720725,3405.23007106781,0.04059669014532119
574575,1149152,574576,1723728,3410.8854129314423,0.040526132070226595
575576,1151154,575577,1726731,3416.692671060562,0.04045477314684831
576577,1153156,576578,1729734,3423.2906510829926,0.04038436875816842
577578,1155158,577579,1732737,3429.6005430221558,0.04031454216237762
578579,1157160,578580,1735740,3435.2574441432953,0.040244934789370745
579580,1159162,579581,1738743,3441.461201906204,0.04017431148713513
580581,1161164,580582,1741746,3447.2433862686157,0.04010398217542388
581582,1163166,581583,1744749,3453.2972979545593,0.0400354791963764
582583,1165168,582584,1747752,3459.8349142074585,0.039967050917766755
583584,1167170,583585,1750755,3464.972188949585,0.03989679811456881
584585,1169172,584586,1753758,3470.0490181446075,0.0398273567607248
585586,1171174,585587,1756761,3474.984283924103,0.039758144364896
586587,1173176,586588,1759764,3479.970865011215,0.03969003244674241
587588,1175178,587589,1762767,3484.888617038727,0.03962125495127111
588589,1177180,588590,1765770,3489.79319190979,0.03955461458645004
589590,1179182,589591,1768773,3495.0798070430756,0.03948578804374847
590591,1181184,590592,1771776,3500.033272266388,0.039418102483978146
591592,1183186,591593,1774779,3504.804344177246,0.039350858805846656
592593,1185188,592594,1777782,3509.9119670391083,0.03928486871882342
593594,1187190,593595,1780785,3514.9147679805756,0.03922026494910824
594595,1189192,594596,1783788,3519.8796060085297,0.03915428199979942
595596,1191194,595597,1786791,3524.892657995224,0.03908748959656805
596597,1193196,596598,1789794,3529.8984611034393,0.03902138136618305
597598,1195198,597599,1792797,3534.8296031951904,0.03895522800667095
598599,1197200,598600,1795800,3539.941635131836,0.03889025263379153
599600,1199202,599601,1798803,3544.9198982715607,0.03882451456411218
600601,1201204,600602,1801806,3549.932694196701,0.03876126591785578
601602,1203206,601603,1804809,3554.944319009781,0.038697125726685044
602603,1205208,602604,1807812,3559.9051790237427,0.03863249888672726
603604,1207210,603605,1810815,3564.8627891540527,0.03856902177903976
604605,1209212,604606,1813818,3569.922315120697,0.038504064939843374
605606,1211214,605607,1816821,3574.86705994606,0.03843962889732211
606607,1213216,606608,1819824,3579.847232103348,0.038374294177629054
607608,1215218,607609,1822827,3584.8146851062775,0.038309556292006164
608609,1217220,608610,1825830,3589.86168718338,0.03824494420769042
609610,1219222,609611,1828833,3594.885017156601,0.03818227692863729
610611,1221224,610612,1831836,3599.9008209705353,0.0381183478548337
611612,1223226,611613,1834839,3604.853245973587,0.03805729300074745
612613,1225228,612614,1837842,3609.9081571102142,0.03799485308263684
613614,1227230,613615,1840845,3614.850135087967,0.03793247570138192
614615,1229232,614616,1843848,3619.8242061138153,0.03786974236209062
615616,1231234,615617,1846851,3624.828330039978,0.03780796174942225
616617,1233236,616618,1849854,3629.974016189575,0.03774673260159034
617618,1235238,617619,1852857,3634.977156162262,0.03768504082472646
618619,1237240,618620,1855860,3639.948770046234,0.0376238577591721
619620,1239242,619621,1858863,3644.9480600357056,0.03756248648642213
620621,1241244,620622,1861866,3649.9010860919952,0.03750292582481052
621622,1243246,621623,1864869,3654.8406021595,0.03744205867042183
622623,1245248,622624,1867872,3659.816605091095,0.03738188605711912
623624,1247250,623625,1870875,3664.7868621349335,0.037321148189221276
624625,1249252,624626,1873878,3669.86771607399,0.03726170134359563
625626,1251254,625627,1876881,3674.8679690361023,0.03720386716850044
626627,1253256,626628,1879884,3679.8450360298157,0.0371443303720298
627628,1255258,627629,1882887,3684.9833459854126,0.03708497950901801
628629,1257260,628630,1885890,3690.050763130188,0.03702515874283563
629630,1259262,629631,1888893,3695.003566265106,0.03696585418219911
630631,1261264,630632,1891896,3699.9915022850037,0.036906734450894874
631632,1263266,631633,1894899,3705.062937259674,0.036848843345069326
632633,1265268,632634,1897902,3710.144896030426,0.0367906207775377
633634,1267270,633635,1900905,3715.1525592803955,0.03673170460751862
634635,1269272,634636,1903908,3720.1598279476166,0.03667492161366681
635636,1271274,635637,1906911,3724.9630489349365,0.036615999135392485
636637,1273276,636638,1909914,3729.3396430015564,0.03655905003142834
637638,1275278,637639,1912917,3734.592716217041,0.036500347288892954
638639,1277280,638640,1915920,3739.8798789978027,0.03644093954244454
639640,1279282,639641,1918923,3744.9856810569763,0.03638373286048591
640641,1281284,640642,1921926,3750.261799097061,0.03632488367111364
641642,1283286,641643,1924929,3755.3219542503357,0.036267289413444814
642643,1285288,642644,1927932,3760.295408964157,0.03620929890348634
643644,1287290,643645,1930935,3765.313574075699,0.03615273427203647
644645,1289292,644646,1933938,3770.2671802043915,0.03609747410155251
645646,1291294,645647,1936941,3775.182234287262,0.036040248718563817
646647,1293296,646648,1939944,3779.179750919342,0.035985487107609515
647648,1295298,647649,1942947,3784.522015094757,0.035929204312196816
648649,1297300,648650,1945950,3790.2499561309814,0.03587385927312425
649650,1299302,649651,1948953,3794.720137119293,0.03581786298127554
650651,1301304,650652,1951956,3798.322278022766,0.0357628915735404
651652,1303306,651653,1954959,3801.897190093994,0.035706998212845065
652653,1305308,652654,1957962,3805.469624042511,0.035651909027365036
653654,1307310,653655,1960965,3809.180104970932,0.03559651347131876
654655,1309312,654656,1963968,3812.7691881656647,0.035541880042728735
655656,1311314,655657,1966971,3816.3537380695343,0.03548729385875049
656657,1313316,656658,1969974,3819.932151079178,0.035432135193332215
657658,1315318,657659,1972977,3823.5282020568848,0.03537762440646475
658659,1317320,658660,1975980,3827.176442861557,0.03532349710621929
659660,1319322,659661,1978983,3830.8345742225647,0.03527096624202386
660661,1321324,660662,1981986,3834.4140009880066,0.03521660938895366
661662,1323326,661663,1984989,3837.9917771816254,0.03516227993895882
662663,1325328,662664,1987992,3841.652914047241,0.03510879472560191
663664,1327330,663665,1990995,3845.2410340309143,0.03505533102361369
664665,1329332,664666,1993998,3848.8887600898743,0.03500235488900216
665666,1331334,665667,1997001,3852.5195031166077,0.03494961107389827
666667,1333336,666668,2000004,3856.1175990104675,0.03489756725866755
667668,1335338,667669,2003007,3859.6956810951233,0.03484419893902668
668669,1337340,668670,2006010,3863.2507519721985,0.03479176240398374
669670,1339342,669671,2009013,3866.921201944351,0.03473989867234195
670671,1341344,670672,2012016,3870.5876631736755,0.034687625024162116
671672,1343346,671673,2015019,3874.1893079280853,0.03463577711954713
672673,1345348,672674,2018022,3877.74209523201,0.0345833372866764
673674,1347350,673675,2021025,3881.3364160060883,0.03453101173545292
674675,1349352,674676,2024028,3884.921741247177,0.034479148793252534
675676,1351354,675677,2027031,3888.6097869873047,0.03442735407043074
676677,1353356,676678,2030034,3892.1978759765625,0.034376209005131386
677678,1355358,677679,2033037,3895.844412088394,0.03432541850088455
678679,1357360,678680,2036040,3899.436177968979,0.03427407752315048
679680,1359362,679681,2039043,3903.0028779506683,0.03422227082046447
680681,1361364,680682,2042046,3906.5942752361298,0.034171408085967414
681682,1363366,681683,2045049,3910.2904081344604,0.03412190058224951
682683,1365368,682684,2048052,3913.9116880893707,0.03407152524050616
683684,1367370,683685,2051055,3917.4707729816437,0.034022073581581935
684685,1369372,684686,2054058,3921.05179810524,0.033971513801589026
685686,1371374,685687,2057061,3924.62278008461,0.03392190391969052
686687,1373376,686688,2060064,3928.269376039505,0.0338713330693281
687688,1375378,687689,2063067,3931.8962099552155,0.03382123881056032
688689,1377380,688690,2066070,3935.4907031059265,0.033772317112379824
689690,1379382,689691,2069073,3939.0546209812164,0.03372232394031016
690691,1381384,690692,2072076,3942.662842988968,0.03367301553043944
691692,1383386,691693,2075079,3946.326719045639,0.03362414431285288
692693,1385388,692694,2078082,3949.736554145813,0.0335757369230123
693694,1387390,693695,2081085,3954.087690114975,0.03352559458289761
694695,1389392,694696,2084088,3957.8777759075165,0.03347580746594758
695696,1391394,695697,2087091,3961.3489060401917,0.03342715415783459
696697,1393396,696698,2090094,3965.9299001693726,0.03337950893910602
697698,1395398,697699,2093097,3969.8125581741333,0.0333302716826438
698699,1397400,698700,2096100,3973.391210079193,0.03328111193695804
699700,1399402,699701,2099103,3976.9803841114044,0.033233744754397776
700701,1401404,700702,2102106,3980.549947977066,0.03318540135296644
701702,1403406,701703,2105109,3984.1973209381104,0.033137995093056816
702703,1405408,702704,2108112,3987.790521144867,0.033090087432356086
703704,1407410,703705,2111115,3991.372794151306,0.033042679458958446
704705,1409412,704706,2114118,3995.047255039215,0.032995245541314944
705706,1411414,705707,2117121,3998.6774320602417,0.03294828297839558
706707,1413416,706708,2120124,4002.299446105957,0.03290090647533361
707708,1415418,707709,2123127,4005.9148881435394,0.0328532822913985
708709,1417420,708710,2126130,4009.488953113556,0.032806645220262
709710,1419422,709711,2129133,4013.16197514534,0.03275998151366366
710711,1421424,710712,2132136,4018.6254370212555,0.03271373637835495
711712,1423426,711713,2135139,4024.0498089790344,0.03266729754250264
712713,1425428,712714,2138142,4028.4197912216187,0.032620248219245696
713714,1427430,713715,2141145,4032.0693509578705,0.032574063987340196
714715,1429432,714716,2144148,4035.9808461666107,0.03252797515960992
715716,1431434,715717,2147151,4040.574961900711,0.03248125507343502
716717,1433436,716718,2150154,4044.203872203827,0.03243399290840898
717718,1435438,717719,2153157,4047.837806224823,0.03238773170232889
718719,1437440,718720,2156160,4051.434667110443,0.032342027850972954
719720,1439442,719721,2159163,4055.033942222595,0.03229668805579422
720721,1441444,720722,2162166,4058.6165311336517,0.03225027805092395
721722,1443446,721723,2165169,4062.269697189331,0.03220450383014395
722723,1445448,722724,2168172,4065.989180088043,0.032158765503481845
723724,1447450,723725,2171175,4069.604840993881,0.03211377090701717
724725,1449452,724726,2174178,4073.2188811302185,0.03206855945791176
725726,1451454,725727,2177181,4076.784049987793,0.03202356756264635
726727,1453456,726728,2180184,4080.370714902878,0.03197844439819164
727728,1455458,727729,2183187,4084.036473274231,0.03193410393214435
728729,1457460,728730,2186190,4087.628781080246,0.03188968467657105
729730,1459462,729731,2189193,4091.251706123352,0.03184536077969824
730731,1461464,730732,2192196,4094.845039129257,0.03180217220506165
731732,1463466,731733,2195199,4098.459404230118,0.03175699846178759
732733,1465468,732734,2198202,4102.079535245895,0.03171261962779681
733734,1467470,733735,2201205,4105.638279914856,0.031668460704167956
734735,1469472,734736,2204208,4109.322656154633,0.03162467572838068
735736,1471474,735737,2207211,4113.026906967163,0.03157988480597851
736737,1473476,736738,2210214,4119.672650098801,0.03153676075999101
737738,1475478,737739,2213217,4124.923684120178,0.031492611202338594
738739,1477480,738740,2216220,4128.705730199814,0.03144864854584739
739740,1479482,739741,2219223,4132.309056997299,0.031405190984514775
740741,1481484,740742,2222226,4135.930690050125,0.03136206588897039
741742,1483486,741743,2225229,4139.701677083969,0.03131866979674669
742743,1485488,742744,2228232,4144.594056129456,0.03127602793756523
743744,1487490,743745,2231235,4149.519585132599,0.031233284926202032
744745,1489492,744746,2234238,4152.899504899979,0.031189918463496724
745746,1491494,745747,2237241,4156.429121017456,0.031147912213782547
746747,1493496,746748,2240244,4159.844330072403,0.03110482552438043
747748,1495498,747749,2243247,4163.374892234802,0.03106261358516349
748749,1497500,748750,2246250,4166.796897172928,0.031020719645312056
749750,1499502,749751,2249253,4170.722193956375,0.030977630412962753
750751,1501504,750752,2252256,4173.965283155441,0.03093589600393898
751752,1503506,751753,2255259,4177.448105096817,0.030893564591679024
752753,1505508,752754,2258262,4180.82533621788,0.030851305280521046
753754,1507510,753755,2261265,4184.985679149628,0.030810338374067214
754755,1509512,754756,2264268,4188.756808042526,0.030769264871196356
755756,1511514,755757,2267271,4192.892903089523,0.030728456817087135
756757,1513516,756758,2270274,4197.732096195221,0.030687421623952105
757758,1515518,757759,2273277,4202.446989059448,0.030646543185866904
758759,1517520,758760,2276280,4206.427613019943,0.030606144880948705
759760,1519522,759761,2279283,4210.71933221817,0.030564764552764245
760761,1521524,760762,2282286,4214.413261175156,0.030523228671881952
761762,1523526,761763,2285289,4218.199321269989,0.03048246585058223
762763,1525528,762764,2288292,4221.847665071487,0.03044177800802572
763764,1527530,763765,2291295,4225.397885084152,0.030401466938201338
764765,1529532,764766,2294298,4229.007274150848,0.030361044611709076
765766,1531534,765767,2297301,4232.621928930283,0.030320635980388033
766767,1533536,766768,2300304,4236.309000968933,0.0302812890313362
767768,1535538,767769,2303307,4239.882209062576,0.03024033648216573
768769,1537540,768770,2306310,4243.5003299713135,0.030200168655937887
769770,1539542,769771,2309313,4247.076085090637,0.030160407741277595
770771,1541544,770772,2312316,4250.649662971497,0.030120785053441068
771772,1543546,771773,2315319,4254.263866186142,0.030080464073762414
772773,1545548,772774,2318322,4257.917149066925,0.03004099044846953
773774,1547550,773775,2321325,4261.510010957718,0.030002337489349884
774775,1549552,774776,2324328,4265.076647043228,0.02996239400090417
775776,1551554,775777,2327331,4268.666544914246,0.02992353288209415
776777,1553556,776778,2330334,4272.260832071304,0.029884098257753067
777778,1555558,777779,2333337,4275.903802871704,0.029845524031770765
778779,1557560,778780,2336340,4279.490857124329,0.02980578282949864
779780,1559562,779781,2339343,4283.089323043823,0.02976624719121901
780781,1561564,780782,2342346,4286.679002285004,0.02972726225380029
781782,1563566,781783,2345349,4290.265934228897,0.029687995174754178
782783,1565568,782784,2348352,4293.927709102631,0.029649402988070506
783784,1567570,783785,2351355,4297.503190040588,0.029611687128635822
784785,1569572,784786,2354358,4301.089002132416,0.029573247014923254
785786,1571574,785787,2357361,4304.642335176468,0.02953563631126599
786787,1573576,786788,2360364,4308.219429016113,0.029496589235350257
787788,1575578,787789,2363367,4311.799654006958,0.029458239556333865
788789,1577580,788790,2366370,4315.422714948654,0.029420633405607077
789790,1579582,789791,2369373,4319.043575048447,0.029382691307546338
790791,1581584,790792,2372376,4322.626110076904,0.029344969278099597
791792,1583586,791793,2375379,4326.210574150085,0.029307458138646325
792793,1585588,792794,2378382,4330.626047134399,0.029269639440826722
793794,1587590,793795,2381385,4334.95227599144,0.029232788941953913
794795,1589592,794796,2384388,4339.125622034073,0.029194866532634478
795796,1591594,795797,2387391,4343.207997083664,0.029157567279980867
796797,1593596,796798,2390394,4347.131598234177,0.029120417346348404
797798,1595598,797799,2393397,4352.285303115845,0.029082540379022248
798799,1597600,798800,2396400,4357.946164131165,0.02904538314396632
799800,1599602,799801,2399403,4362.781071186066,0.029008655959842145
800801,1601604,800802,2402406,4366.384109258652,0.028972201303986367
801802,1603606,801803,2405409,4369.966699123383,0.028935925334735657
802803,1605608,802804,2408412,4374.159439086914,0.02889885690274241
803804,1607610,803805,2411415,4377.98385310173,0.02886278370351647
804805,1609612,804806,2414418,4381.969658136368,0.02882671425504668
805806,1611614,805807,2417421,4385.888370037079,0.028790058628146653
806807,1613616,806808,2420424,4389.779484987259,0.028753928461810574
807808,1615618,807809,2423427,4393.976613044739,0.02871681458054809
808809,1617620,808810,2426430,4397.549754858017,0.028680867129878607
809810,1619622,809811,2429433,4401.202252149582,0.028645083899391466
810811,1621624,810812,2432436,4404.840502023697,0.028609389144548913
811812,1623626,811813,2435439,4408.207571983337,0.02857410686374351
812813,1625628,812814,2438442,4411.604612112045,0.02853784403487225
813814,1627630,813815,2441445,4415.160931110382,0.02850289754314872
814815,1629632,814816,2444448,4418.697242975235,0.028468024589528795
815816,1631634,815817,2447451,4422.301651954651,0.028432329334464157
816817,1633636,816818,2450454,4425.84777712822,0.028396529885867494
817818,1635638,817819,2453457,4429.402448892593,0.02836179203586653
818819,1637640,818820,2456460,4432.671159029007,0.02832652885808784
819820,1639642,819821,2459463,4435.962363958359,0.028291282345890068
820821,1641644,820822,2462466,4439.311402082443,0.028257048636078252
821822,1643646,821823,2465469,4442.725155115128,0.028221540480444673
822823,1645648,822824,2468472,4446.620952129364,0.02818674418995215
823824,1647650,823825,2471475,4450.2669241428375,0.02815279149945127
824825,1649652,824826,2474478,4454.040655136108,0.028117997868321254
825826,1651654,825827,2477481,4458.658642053604,0.02808372097388201
826827,1653656,826828,2480484,4463.514562129974,0.02804975960862066
827828,1655658,827829,2483487,4469.0709619522095,0.028015166044497164
828829,1657660,828830,2486490,4473.948231935501,0.027981202791124815
829830,1659662,829831,2489493,4477.930210113525,0.027947399321419653
830831,1661664,830832,2492496,4481.57168006897,0.027913223073483096
831832,1663666,831833,2495499,4485.203506946564,0.027878806587978033
832833,1665668,832834,2498502,4488.885416030884,0.027845638192957267
833834,1667670,833835,2501505,4492.478076934814,0.02781180359670543
834835,1669672,834836,2504508,4496.076204061508,0.027778600011515664
835836,1671674,835837,2507511,4499.664499044418,0.02774370598672249
836837,1673676,836838,2510514,4503.3763909339905,0.027709159128789906
837838,1675678,837839,2513517,4506.907581090927,0.02767625791602768
838839,1677680,838840,2516520,4510.722527980804,0.027642571127216797
839840,1679682,839841,2519523,4514.300089120865,0.02760839692382433
840841,1681684,840842,2522526,4517.856367111206,0.02757462366571417
841842,1683686,841843,2525529,4521.572192192078,0.027540894827325246
842843,1685688,842844,2528532,4525.129437923431,0.027507952589076012
843844,1687690,843845,2531535,4529.403312921524,0.027475255559693323
844845,1689692,844846,2534538,4534.493212938309,0.027441441818155
845846,1691694,845847,2537541,4539.7282700538635,0.02740847794302681
846847,1693696,846848,2540544,4543.79484128952,0.027375959391065408
847848,1695698,847849,2543547,4547.508487939835,0.02734312558277452
848849,1697700,848850,2546550,4551.436943292618,0.027310940829920582
849850,1699702,849851,2549553,4555.214987039566,0.027278374349407386
850851,1701704,850852,2552556,4559.015660047531,0.02724591011974553
851852,1703706,851853,2555559,4562.76570391655,0.027213732077143504
852853,1705708,852854,2558562,4567.345380067825,0.02718130352877779
853854,1707710,853855,2561565,4571.145060300827,0.027148380542712403
854855,1709712,854856,2564568,4574.941719055176,0.027115387303638272
855856,1711714,855857,2567571,4578.7973918914795,0.0270829662840697
856857,1713716,856858,2570574,4582.626019239426,0.027051095785282087
857858,1715718,857859,2573577,4586.307020187378,0.02701863534275617
858859,1717720,858860,2576580,4590.2198531627655,0.026986877945091692
859860,1719722,859861,2579583,4593.9253718853,0.02695485682306753
860861,1721724,860862,2582586,4597.581705093384,0.02692260160438309
861862,1723726,861863,2585589,4601.39927315712,0.026891748299021856
862863,1725728,862864,2588592,4605.12947511673,0.02685989568090008
863864,1727730,863865,2591595,4608.854748010635,0.026829102062038146
864865,1729732,864866,2594598,4612.569361925125,0.026797994039952755
865866,1731734,865867,2597601,4616.304666996002,0.02676655764662428
866867,1733736,866868,2600604,4620.047667980194,0.026734968179880525
867868,1735738,867869,2603607,4623.841938972473,0.026704339203206473
868869,1737740,868870,2606610,4627.49610209465,0.026672670583138824
869870,1739742,869871,2609613,4631.2522439956665,0.02664165132046037
870871,1741744,870872,2612616,4634.960279226303,0.02661014045588672
871872,1743746,871873,2615619,4638.777961969376,0.026578657027130248
872873,1745748,872874,2618622,4642.632286071777,0.026547404797383933
873874,1747750,873875,2621625,4646.310128927231,0.026515854773606407
874875,1749752,874876,2624628,4650.024657964706,0.02648472005603253
875876,1751754,875877,2627631,4653.806225061417,0.02645349900558358
876877,1753756,876878,2630634,4657.6344220638275,0.026422780167195015
877878,1755758,877879,2633637,4661.311137199402,0.02639261246076785
878879,1757760,878880,2636640,4665.000982046127,0.02636187588905159
879880,1759762,879881,2639643,4668.752292871475,0.026331345523431082
880881,1761764,880882,2642646,4672.644864082336,0.026301501060515875
881882,1763766,881883,2645649,4676.3353753089905,0.02627106645013555
882883,1765768,882884,2648652,4679.993856191635,0.026241193067107815
883884,1767770,883885,2651655,4683.861720085144,0.02621045593332383
884885,1769772,884886,2654658,4687.536553144455,0.026180433203990106
885886,1771774,885887,2657661,4691.203224182129,0.02615049416453985
886887,1773776,886888,2660664,4695.066570043564,0.026120216803974472
887888,1775778,887889,2663667,4698.69656920433,0.026090061794093344
888889,1777780,888890,2666670,4702.3798542022705,0.026060275251438725
889890,1779782,889891,2669673,4706.151015996933,0.0260303523773473
890891,1781784,890892,2672676,4709.876564025879,0.026000741621828638
891892,1783786,891893,2675679,4713.529413223267,0.025970742643039557
892893,1785788,892894,2678682,4717.283397197723,0.02594119860805222
893894,1787790,893895,2681685,4720.96982884407,0.025911559503583703
894895,1789792,894896,2684688,4724.741505146027,0.025881861643938464
895896,1791794,895897,2687691,4728.3938331604,0.025852184580799076
896897,1793796,896898,2690694,4732.061085939407,0.025822433477515006
897898,1795798,897899,2693697,4735.85856795311,0.02579313690876006
898899,1797800,898900,2696700,4739.525421142578,0.025764049745703232
899900,1799802,899901,2699703,4743.213356018066,0.025734495948199765
900901,1801804,900902,2702706,4746.886339187622,0.025705258842208423
901902,1803806,901903,2705709,4750.578782081604,0.025675716085970635
902903,1805808,902904,2708712,4754.389224052429,0.025647219026723178
903904,1807810,903905,2711715,4758.07917714119,0.025617633926231065
904905,1809812,904906,2714718,4761.772860050201,0.025589115308321198
905906,1811814,905907,2717721,4765.44914317131,0.02555991779991018
906907,1813816,906908,2720724,4769.23005604744,0.02553125327176531
907908,1815818,907909,2723727,4772.918917179108,0.025502671547656064
908909,1817820,908910,2726730,4777.303389072418,0.025474426804066752
909910,1819822,909911,2729733,4781.086198091507,0.025445867899179575
910911,1821824,910912,2732736,4784.8488211631775,0.02541725882474566
911912,1823826,911913,2735739,4788.637771129608,0.025389071266545216
912913,1825828,912914,2738742,4792.456444978714,0.025360730824104394
913914,1827830,913915,2741745,4796.184367179871,0.025332704908578307
914915,1829832,914916,2744748,4799.870671272278,0.025305264920461923
915916,1831834,915917,2747751,4803.640620231628,0.02527741539051931
916917,1833836,916918,2750754,4807.468856096268,0.025248604448279366
917918,1835838,917919,2753757,4811.116362094879,0.025220773424734944
918919,1837840,918920,2756760,4814.811038017273,0.025192452581904945
919920,1839842,919921,2759763,4818.6436722278595,0.02516463818574266
920921,1841844,920922,2762766,4822.302489280701,0.025136675027169986
921922,1843846,921923,2765769,4826.082097053528,0.025108809568337165
922923,1845848,922924,2768772,4829.846273183823,0.02508108781876217
923924,1847850,923925,2771775,4833.548337936401,0.02505373193343985
924925,1849852,924926,2774778,4837.355832099915,0.02502573387391749
925926,1851854,925927,2777781,4841.129842996597,0.024998258260893635
926927,1853856,926928,2780784,4844.875138044357,0.024970584106995375
927928,1855858,927929,2783787,4848.557536125183,0.024943225438619265
928929,1857860,928930,2786790,4852.2311198711395,0.024915269197663292
929930,1859862,929931,2789793,4856.051962137222,0.024887839459552197
930931,1861864,930932,2792796,4859.757344007492,0.02486039706855081
931932,1863866,931933,2795799,4863.448132276535,0.024832908477037563
932933,1865868,932934,2798802,4867.239864110947,0.0248059333407582
933934,1867870,933935,2801805,4870.956741094589,0.024778717333902023
934935,1869872,934936,2804808,4874.659809112549,0.02475142345429049
935936,1871874,935937,2807811,4878.448730230331,0.024724156224692706
936937,1873876,936938,2810814,4882.191586256027,0.024697388929780573
937938,1875878,937939,2813817,4886.031396150589,0.024670113394677173
938939,1877880,938940,2816820,4889.709015130997,0.02464344445616007
939940,1879882,939941,2819823,4893.382992982864,0.024617199731437722
940941,1881884,940942,2822826,4897.247956037521,0.02459010093480174
941942,1883886,941943,2825829,4900.903735160828,0.024563086837588344
942943,1885888,942944,2828832,4904.591940164566,0.024536793574952753
943944,1887890,943945,2831835,4908.480502128601,0.02450975140891387
944945,1889892,944946,2834838,4912.146596908569,0.024482913369865855
945946,1891894,945947,2837841,4915.956915140152,0.024456681183437468
946947,1893896,946948,2840844,4919.665652990341,0.024429952914942987
947948,1895898,947949,2843847,4923.4818110466,0.024402969553193543
948949,1897900,948950,2846850,4927.174900054932,0.02437625419588585
949950,1899902,949951,2849853,4930.82301402092,0.02434994446048222
950951,1901904,950952,2852856,4934.633033037186,0.024323165485839127
951952,1903906,951953,2855859,4938.32973408699,0.02429730932453822
952953,1905908,952954,2858862,4942.064171075821,0.024271154748930712
953954,1907910,953955,2861865,4945.8258900642395,0.02424570813855098
954955,1909912,954956,2864868,4949.552706241608,0.02421965439680207
955956,1911914,955957,2867871,4953.313402891159,0.024193515455408487
956957,1913916,956958,2870874,4957.031565189362,0.024167328074327088
957958,1915918,957959,2873877,4960.699559926987,0.02414125892391894
958959,1917920,958960,2876880,4964.466386079788,0.02411569212199538
959960,1919922,959961,2879883,4968.185683965683,0.02408966661823797
960961,1921924,960962,2882886,4971.94556593895,0.024063639642918133
961962,1923926,961963,2885889,4975.620868206024,0.024038041116000386
962963,1925928,962964,2888892,4979.35409116745,0.024012575542656123
963964,1927930,963965,2891895,4983.000254154205,0.023987057526028366
964965,1929932,964966,2894898,4986.827459096909,0.023960556374731823
965966,1931934,965967,2897901,4990.488069295883,0.023935065257319366
966967,1933936,966968,2900904,4994.21648311615,0.023909504558105255
967968,1935938,967969,2903907,4997.974556922913,0.023884036345407367
968969,1937940,968970,2906910,5001.718122005463,0.02385872192644456
969970,1939942,969971,2909913,5005.409561157227,0.023833660690797842
970971,1941944,970972,2912916,5009.1232850551605,0.023808650783394114
971972,1943946,971973,2915919,5012.80522608757,0.023783421644111513
972973,1945948,972974,2918922,5016.610530138016,0.023758656629070174
973974,1947950,973975,2921925,5020.285452127457,0.023733277888823068
974975,1949952,974976,2924928,5024.058039188385,0.023708601394901052
975976,1951954,975977,2927931,5027.916615009308,0.023683605004407582
976977,1953956,976978,2930934,5031.580004930496,0.023658651851292234
977978,1955958,977979,2933937,5035.264101982117,0.02363346529818955
978979,1957960,978980,2936940,5039.127950191498,0.02360826427138818
979980,1959962,979981,2939943,5042.804676294327,0.023583294152558665
980981,1961964,980982,2942946,5046.502676010132,0.02355855132373108
981982,1963966,981983,2945949,5050.205860137939,0.023534480093076127
982983,1965968,982984,2948952,5053.976587057114,0.023509312872192822
983984,1967970,983985,2951955,5057.706377029419,0.02348480928048957
984985,1969972,984986,2954958,5061.337983131409,0.023460669017367763
985986,1971974,985987,2957961,5065.2006669044495,0.023436362060238025
986987,1973976,986988,2960964,5068.982138156891,0.02341205194898066
987988,1975978,987989,2963967,5072.631860971451,0.02338804069950129
988989,1977980,988990,2966970,5076.368000030518,0.02336411053147458
989990,1979982,989991,2969973,5080.156015872955,0.023340401214227313
990991,1981984,990992,2972976,5083.8304080963135,0.023316197022722918
991992,1983986,991993,2975979,5087.664262056351,0.023292363533983007
992993,1985988,992994,2978982,5091.329741239548,0.023268210605237982
993994,1987990,993995,2981985,5095.034898996353,0.023244042795340647
994995,1989992,994996,2984988,5098.715714216232,0.023220461753226118
995996,1991994,995997,2987991,5102.453720092773,0.023196308142360067
996997,1993996,996998,2990994,5106.294678211212,0.023172641293058405
997998,1995998,997999,2993997,5109.997317314148,0.023148600263084518
998999,1998000,999000,2997000,5113.611717224121,0.023124757975892862
1000000,2000002,1000001,3000003,5117.328367233276,0.023100391506886808


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.004189968109130859,12064.682476916567
1001,2003,2002,4005,8.30136489868164,21.074205127015375
2002,4005,4004,8009,15.927466869354248,19.073870623178664
3003,6007,6006,12013,23.074182748794556,17.372289908553284
4004,8009,8008,16017,30.281173944473267,15.906416381691088
5005,10011,10010,20021,37.65772008895874,14.631373993082889
6006,12013,12012,24025,44.682780742645264,13.513770899064184
7007,14015,14014,28029,52.491440773010254,12.527948884469879
8008,16017,16016,32033,62.14308977127075,11.653690998691673
9009,18019,18018,36037,71.10923886299133,10.874759810885735
10010,20021,20020,40041,78.67453169822693,10.177905979244315
11011,22023,22022,44045,87.9383270740509,9.552195649228452
12012,24025,24024,48049,95.80628609657288,8.988508349106269
13013,26027,26026,52053,103.72835779190063,8.479162481939056
14014,28029,28028,56057,110.53839468955994,8.01764140909836
15015,30031,30030,60061,117.89408683776855,7.598376535466741
16016,32033,32032,64065,125.22865796089172,7.216579546493449
17017,34035,34034,68069,132.52957892417908,6.868110005661947
18018,36037,36036,72073,139.1241810321808,6.549369756421584
19019,38039,38038,76077,146.08205485343933,6.257217886137369
20020,40041,40040,80081,153.92426586151123,5.988901629101747
21021,42043,42042,84085,163.27503776550293,5.741999743026099
22022,44045,44044,88089,171.18074798583984,5.514375734454006
23023,46047,46046,92093,179.05488991737366,5.304138927249369
24024,48049,48048,96097,187.14773869514465,5.109611828725974
25025,50051,50050,100101,195.37233090400696,4.9293025931237935
26026,52053,52052,104105,203.86585903167725,4.761881643187735
27027,54055,54054,108109,212.100919008255,4.606161709418302
28028,56057,56056,112113,219.7493109703064,4.461080698725709
29029,58059,58058,116117,227.4102840423584,4.325686921823944
30030,60061,60060,120121,234.46836304664612,4.199126299894488
31031,62063,62062,124125,241.40039587020874,4.080631242317395
32032,64065,64064,128129,248.7141261100769,3.969510943410569
33033,66067,66066,132133,255.9957938194275,3.8651428904740897
34034,68069,68068,136137,263.55916476249695,3.7669654109831754
35035,70071,70070,140141,270.62190198898315,3.674471241138235
36036,72073,72072,144145,277.51358675956726,3.587202720804271
37037,74075,74074,148149,284.7069969177246,3.5047429227015527
38038,76077,76076,152153,290.4854168891907,3.426715212297495
39039,78079,78078,156157,296.1500039100647,3.352777808724568
40040,80081,80080,160161,302.11019372940063,3.2826202209816984
41041,82083,82082,164165,309.6185758113861,3.2159600781378685
42042,84085,84084,168169,316.68725085258484,3.1525403063260455
43043,86087,86086,172173,323.8046588897705,3.092126611547428
44044,88089,88088,176177,331.01623797416687,3.034505232655647
45045,90091,90090,180181,338.35906410217285,2.9794809333798185
46046,92093,92092,184185,346.2917449474335,2.9268752062034764
47047,94095,94094,188189,355.2039988040924,2.8765246641833073
48048,96097,96096,192193,363.5561237335205,2.828279599785674
49049,98099,98098,196197,371.91515588760376,2.782002692199967
50050,100101,100100,200201,380.1844427585602,2.7375678469179547
51051,102103,102102,204205,388.294481754303,2.694859153121797
52052,104105,104104,208209,396.07781505584717,2.6537699462169257
53053,106107,106106,212213,404.23581886291504,2.6142019641883962
54054,108109,108108,216217,412.4059898853302,2.5760645878381183
55055,110111,110110,220221,420.50004386901855,2.539274155977182
56056,112113,112112,224225,428.81853890419006,2.503753347766178
57057,114115,114114,228229,436.6989607810974,2.469430625116729
58058,116117,116116,232233,444.89650678634644,2.436239729006047
59059,118119,118118,236237,453.67577171325684,2.404119224038368
60060,120121,120120,240241,461.0327408313751,2.3730120864292985
61061,122123,122122,244245,468.5896198749542,2.3428653309092624
62062,124125,124124,248249,475.77110505104065,2.313629672593379
63063,126127,126126,252253,483.36392092704773,2.285259220368971
64064,128129,128128,256257,492.8873689174652,2.2577111985938245
65065,130131,130130,260261,501.6746039390564,2.230945694287584
66066,132133,132132,264265,508.87274384498596,2.2049254273388215
67067,134135,134134,268269,515.7422018051147,2.179615541406747
68068,136137,136136,272273,522.6874008178711,2.154983501384777
69069,138139,138138,276277,529.8552989959717,2.13099871806844
70070,140141,140140,280281,537.1611950397491,2.1076324649147864
71071,142143,142142,284285,543.9829177856445,2.084857838044627
72072,144145,144144,288289,550.903990983963,2.062649558934936
73073,146147,146146,292293,558.7449977397919,2.040983853754369
74074,148149,148148,296297,566.9037058353424,2.0198383430015383
75075,150151,150150,300301,575.182835817337,1.9991919404128566
76076,152153,152152,304305,582.8094449043274,1.9790247603032185
77077,154155,154154,308309,590.5639827251434,1.9593180325755384
78078,156157,156156,312313,598.47407579422,1.9400540246715536
79079,158159,158158,316317,607.0114529132843,1.9212159698709002
80080,160161,160160,320321,615.0390219688416,1.9027880013363756
81081,162163,162162,324325,623.2447097301483,1.8847550913924351
82082,164165,164164,328329,630.5478389263153,1.86710299562219
83083,166167,166166,332333,638.0472497940063,1.8498182012772304
84084,168169,168168,336337,645.0450789928436,1.83288787971469
85085,170171,170170,340341,652.0925979614258,1.8162998424377292
86086,172173,172172,344345,659.8896586894989,1.8000425004720455
87087,174175,174174,348349,666.8113317489624,1.7841048267910082
88088,176177,176176,352353,673.6370806694031,1.76847632152203
89089,178179,178178,356357,680.4130239486694,1.7531469796958845
90090,180181,180180,360361,687.2037508487701,1.7381072613607103
91091,182183,182182,364365,693.8783898353577,1.7233481458606548
92092,184185,184184,368369,700.5123288631439,1.7088610304945178
93093,186187,186186,372373,707.5383260250092,1.694637423783206
94094,188189,188188,376377,714.3466558456421,1.6806693880425883
95095,190191,190190,380381,721.142808675766,1.6669493300269096
96096,192193,192192,384385,727.905280828476,1.6534699815711065
97097,194195,194194,388389,734.6147871017456,1.6402243815464317
98098,196197,196196,392393,741.2673869132996,1.6272058590493543
99099,198199,198198,396397,748.0748229026794,1.6144080176491116
100100,200201,200200,400401,754.8537647724152,1.601824720717559
101101,202203,202202,404405,761.588773727417,1.5894500776666973
102102,204205,204204,408409,768.6166708469391,1.5772784310938732
103103,206207,206206,412413,775.5905108451843,1.5653043447346136
104104,208209,208208,416417,782.5295779705048,1.5535225921557867
105105,210211,210210,420421,789.5153048038483,1.5419281461745413
106106,212213,212212,424425,796.4884097576141,1.5305161689084343
107107,214215,214214,428429,803.5625598430634,1.5192820024331013
108108,216217,216216,432433,810.5919427871704,1.5082211600129085
109109,218219,218218,436437,817.5104179382324,1.4973293178409222
110110,220221,220220,440441,824.5563488006592,1.4866023072627286
111111,222223,222222,444445,831.6251127719879,1.4760361074731918
112112,224225,224224,448449,838.7160696983337,1.4656268386097508
113113,226227,226226,452453,845.83846783638,1.4553707552640844
114114,228229,228228,456457,853.0078799724579,1.4452642403321079
115115,230231,230230,460461,859.9611048698425,1.4353037992441386
116116,232233,232232,464465,867.2763137817383,1.4254860544806434
117117,234235,234234,468469,874.242947101593,1.4158077404135838
118118,236237,236236,472473,880.9569756984711,1.4062656984133355
119119,238239,238238,476477,887.7838599681854,1.3968568722229975
120120,240241,240240,480481,894.1781990528107,1.387578303583723
121121,242243,242242,484485,899.8523859977722,1.3784271280837856
122122,244245,244244,488489,905.6481840610504,1.3694005712332
123123,246247,246246,492493,911.3355550765991,1.3604959447238798
124124,248249,248248,496497,917.1957318782806,1.351710642908074
125125,250251,250250,500501,924.288569688797,1.343042139436875
126126,252253,252252,504505,931.2487668991089,1.3344879840642534
127127,254255,254254,508509,938.1364316940308,1.3260457996238983
128128,256257,256256,512513,945.6963038444519,1.317713279151576
129129,258259,258258,516517,952.6517288684845,1.3094881831402745
130130,260261,260260,520521,958.5363237857819,1.3013683369390492
131131,262263,262262,524525,964.4033210277557,1.293351628268283
132132,264265,264264,528529,970.4707009792328,1.2854360048550006
133133,266267,266266,532533,976.3616578578949,1.2776194721827778
134134,268269,268268,536537,982.4331629276276,1.2699000913435157
135135,270271,270270,540541,988.2086520195007,1.2622759769983531
136136,272273,272272,544545,993.9072439670563,1.2547452954040637
137137,274275,274274,548549,999.6759181022644,1.2473062625722378
138138,276277,276276,552553,1005.4893729686737,1.2399571424630267
139139,278279,278278,556557,1011.3122508525848,1.2326962453098531
140140,280281,280280,560561,1017.084657907486,1.2255219259714067
141141,282283,282282,564565,1022.8709268569946,1.2184325823855033
142142,284285,284284,568569,1028.6567690372467,1.2114266540902463
143143,286287,286286,572573,1034.556035041809,1.2045027606709482
144144,288289,288288,576577,1040.988868713379,1.197659305862544
145145,290291,290290,580581,1046.8827159404755,1.1908948186337511
146146,292293,292292,584585,1052.873368024826,1.1842078912741272
147147,294295,294294,588589,1058.766343832016,1.1775971511269745
148148,296297,296296,592593,1064.7733418941498,1.171061259447015
149149,298299,298298,596597,1070.629968881607,1.164598910288987
150150,300301,300300,600601,1076.4115579128265,1.158208829450814
151151,302303,302302,604605,1082.3193588256836,1.1518897734658822
152152,304305,304304,608609,1088.1043388843536,1.1456405286280642
153153,306307,306306,612613,1093.9288198947906,1.1394599100531195
154154,308309,308308,616617,1099.766821861267,1.13334676078739
155155,310311,310310,620621,1105.498780965805,1.1272999509346846
156156,312313,312312,624625,1111.4390199184418,1.1213183768340969
157157,314315,314314,628629,1117.680814743042,1.1154009602614678
158158,316317,316316,632633,1123.4046049118042,1.109546647659954
159159,318319,318318,636637,1129.907450914383,1.1037544094033365
160160,320321,320320,640641,1135.805564880371,1.098023239081158
161161,322323,322322,644645,1141.9288036823273,1.092352152818421
162162,324325,324324,648649,1148.2590010166168,1.0867401886116568
163163,326327,326326,652653,1154.3172600269318,1.0811864057050116
164164,328329,328328,656657,1162.240609884262,1.0756898839645146
165165,330331,330330,660661,1169.3623349666595,1.0702497232960013
166166,332333,332332,664665,1175.0795488357544,1.0648650430666748
167167,334335,334334,668669,1180.962542772293,1.059534981581237
168168,336337,336336,672673,1187.7405717372894,1.0542586955216393
169169,338339,338338,676677,1193.9802458286285,1.0490353594468615
170170,340341,340340,680681,1200.0482790470123,1.0438641653181548
171171,342343,342342,684685,1205.9776079654694,1.038744321997001
172172,344345,344344,688689,1211.8845608234406,1.0336750547940028
173173,346347,346346,692693,1217.5689647197723,1.028655605035965
174174,348349,348348,696697,1223.3929719924927,1.0236852296202414
175175,350351,350350,700701,1229.2020018100739,1.0187632006091007
176176,352353,352352,704705,1234.9946689605713,1.0138888048295485
177177,354355,354354,708709,1240.8251078128815,1.0090613434804254
178178,356357,356356,712713,1247.6121878623962,1.004280131757696
179179,358359,358358,716717,1253.3846499919891,0.9995444984961068
180180,360361,360360,720721,1259.876529932022,0.9948537858144846
181181,362363,362362,724725,1266.1140069961548,0.9902073487810412
182182,364365,364364,728729,1272.3825018405914,0.9856045550732233
183183,366367,366366,732733,1278.3329448699951,0.9810447846684838
184184,368369,368368,736737,1284.53120303154,0.9765274295295967
185185,370371,370370,740741,1290.9129710197449,0.972051893320895
186186,372373,372372,744745,1296.7471318244934,0.9676175910917664
187187,374375,374374,748749,1302.7276957035065,0.9632239490201755
188188,376377,376376,752753,1308.9362790584564,0.958870404134359
189189,378379,378378,756757,1316.0921647548676,0.9545564040290628
190190,380381,380380,760761,1322.2539467811584,0.9502814066436258
191191,382383,382382,764765,1327.977217912674,0.946044879996407
192192,384385,384384,768769,1333.3731639385223,0.9418463019264891
193193,386387,386386,772773,1337.4626388549805,0.937685159897228
194194,388389,388388,776777,1341.5590467453003,0.9335609507361369
195195,390391,390390,780781,1345.7934198379517,0.9294731804384355
196196,392393,392392,784785,1349.7289500236511,0.9254213639342197
197197,394395,394394,788789,1354.0186479091644,0.9214050248956482
198198,396397,396396,792793,1357.9686410427094,0.9174236955295783
199199,398399,398398,796797,1361.8793530464172,0.9134769163792953
200200,400401,400400,800801,1365.7839710712433,0.9095642361335194
201201,402403,402402,804805,1369.7208168506622,0.9056852114554204
202202,404405,404404,808809,1373.7575869560242,0.9018394067788904
203203,406407,406406,812813,1377.7433898448944,0.8980263941539306
204204,408409,408408,816817,1381.5905079841614,0.8942457530720276
205205,410411,410410,820821,1385.4559507369995,0.8904970702933497
206206,412413,412412,824825,1389.3261868953705,0.8867799396957707
207207,414415,414414,828829,1394.256987810135,0.8830939621093421
208208,416417,416416,832833,1399.1770658493042,0.8794387451762304
209209,418419,418418,836837,1404.447501897812,0.8758139031888277
210210,420421,420420,840841,1409.3415658473969,0.8722190569606028
211211,422423,422422,844845,1414.174068927765,0.8686538336696685
212212,424425,424424,848849,1418.528615951538,0.8651178667350905
213213,426427,426426,852853,1423.4587128162384,0.8616107956822816
214214,428429,428428,856857,1428.2553327083588,0.858132266004759
215215,430431,430430,860861,1432.7594769001007,0.8546819290495478
216216,432433,432432,864865,1437.0802569389343,0.8512594418916706
217217,434435,434434,868869,1441.4116468429565,0.8478644672049995
218218,436437,436436,872873,1445.7897720336914,0.8444966731585737
219219,438439,438438,876877,1450.4798109531403,0.8411557332947268
220220,440441,440440,880881,1454.3725807666779,0.837841326425405
221221,442443,442442,884885,1459.755581855774,0.8345531365193892
222222,444445,444444,888889,1465.4932720661163,0.8312908525931562
223223,446447,446446,892893,1471.2488429546356,0.8280541686217475
224224,448449,448448,896897,1562.9826560020447,0.8248427834205359
225225,450451,450450,900901,1571.6620559692383,0.8216564005688269
226226,452453,452452,904905,1579.9600608348846,0.8184947282934445
227227,454455,454454,908909,1586.2999148368835,0.8153574793959706
228228,456457,456456,912913,1592.466080904007,0.8122443711454252
229229,458459,458458,916917,1597.7359569072723,0.80915512520005
230230,460461,460460,920921,1806.2405087947845,0.8060894675163581
231231,462463,462462,924925,1811.9891970157623,0.8030471282709186
232232,464465,464464,928929,1846.9234437942505,0.8000278417712252
233233,466467,466466,932933,1852.623939037323,0.7970313463756611
234234,468469,468468,936937,1860.418004989624,0.7940573844261962
235235,470471,470470,940941,1880.5764558315277,0.7911057021610759
236236,472473,472472,944945,1885.7446358203888,0.7881760496347852
237237,474475,474474,948949,1925.3699538707733,0.7852681806671171
238238,476477,476476,952953,1930.5370926856995,0.7823818527522235
239239,478479,478478,956957,1959.0680696964264,0.77951682699495
240240,480481,480480,960961,1964.2145388126373,0.7766728680453525
241241,482483,482482,964965,2436.757938861847,0.773849744027757
242242,484485,484484,968969,2441.8848638534546,0.7710472264843702
243243,486487,486486,972973,2449.2419028282166,0.7682650902988826
244244,488489,488488,976977,2456.4609699249268,0.7655031136491743
245245,490491,490490,980981,2461.6792047023773,0.762761077932737
246246,492493,492492,984985,2493.508116006851,0.7600387677193794
247247,494495,494494,988989,2498.6519799232483,0.7573359706857445
248248,496497,496496,992993,2505.9153850078583,0.7546524775661965
249249,498499,498498,996997,2511.075485944748,0.7519880820873368
250250,500501,500500,1001001,2518.374282836914,0.7493425809170731
251251,502503,502502,1005005,2523.5202028751373,0.7467157736191439
252252,504505,504504,1009009,2530.976210832596,0.7441074625985493
253253,506507,506506,1013013,2536.2180738449097,0.7415174530397053
254254,508509,508508,1017017,2543.569240808487,0.7389455528737017
255255,510511,510510,1021021,2548.7147488594055,0.7363915727200947
256256,512513,512512,1025025,2556.0581669807434,0.7338553258377942
257257,514515,514514,1029029,2561.1971237659454,0.731336628081408
258258,516517,516516,1033033,2568.5709187984467,0.7288352978684998
259259,518519,518518,1037037,2575.868574857712,0.7263511561068299
260260,520521,520520,1041041,2581.0806200504303,0.7238840261779842
261261,522523,522522,1045045,2588.425889968872,0.7214337338809855
262262,524525,524524,1049049,2593.661980867386,0.7190001073940948
263263,526527,526526,1053053,2601.373480796814,0.7165829772275174
264264,528529,528528,1057057,2606.7065467834473,0.7141821762070322
265265,530531,530530,1061061,2614.228712797165,0.7117975393975939
266266,532533,532532,1065065,2619.5162386894226,0.7094289040942385
267267,534535,534534,1069069,2627.0641379356384,0.707076126955144
268268,536537,536536,1073073,2632.1853597164154,0.7047390621501108
269269,538539,538538,1077077,2641.5878739356995,0.7024175234546419
270270,540541,540540,1081081,2646.7282700538635,0.700111356578418
271271,542543,542542,1085085,2654.1836709976196,0.6978204093720706
272272,544545,544544,1089089,2659.476749897003,0.6955445316889382
273273,546547,546546,1093093,2666.878012895584,0.6932835753632389
274274,548549,548548,1097097,2674.0783627033234,0.6910373941718717
275275,550551,550550,1101101,2679.5808367729187,0.6888058437925793
276276,552553,552552,1105105,2687.007374048233,0.6865887817857583
277277,554555,554554,1109109,2693.1337428092957,0.6843860675617179
278278,556557,556556,1113113,2700.8993978500366,0.6821975623352046
279279,558559,558558,1117117,2706.0386068820953,0.6800231291272212
280280,560561,560560,1121121,2713.4031937122345,0.6778626326995436
281281,562563,562562,1125125,2718.541023015976,0.6757159395547205
282282,564565,564564,1129129,2725.920329809189,0.6735829178978747
283283,566567,566566,1133133,2733.301367044449,0.6714634376039612
284284,568569,568568,1137137,2738.631938934326,0.6693573701977584
285285,570571,570570,1141141,2745.9373569488525,0.6672645888302213
286286,572573,572572,1145145,2751.115911960602,0.6651849682475586
287287,574575,574574,1149149,2758.46856880188,0.6631183847675857
288288,576577,576576,1153153,2764.062446117401,0.6610647162578971
289289,578579,578578,1157157,2771.518534898758,0.6590243013652071
290290,580581,580580,1161161,2776.840364933014,0.6569965880917152
291291,582583,582582,1165165,2784.2907218933105,0.654981430285261
292292,584585,584584,1169169,2789.4427649974823,0.6529787113868224
293293,586587,586586,1173173,2809.218505859375,0.6509883164253552
294294,588589,588588,1177177,2814.3507487773895,0.6490101319341193
295295,590591,590590,1181181,2885.1757209300995,0.6470440458924713
296296,592593,592592,1185185,2972.5932829380035,0.6450899476822087
297297,594595,594594,1189189,2977.8180301189423,0.6431477280475519
298298,596597,596596,1193193,2985.2168729305267,0.6412172790733166
299299,598599,598598,1197197,2990.3255150318146,0.6392984941521718
300300,600601,600600,1201201,2997.6324968338013,0.6373912679755449
301301,602603,602602,1205205,3002.743400812149,0.6354956016457436
302302,604605,604604,1209209,3010.078024864197,0.6336116482852958
303303,606607,606606,1213213,3015.163904905319,0.6317389440155239
304304,608609,608608,1217217,3033.1421868801117,0.629877387529632
305305,610611,610610,1221221,3038.260062932968,0.628026879267054
306306,612613,612612,1225225,3045.5628559589386,0.6261873210733029
307307,614615,614614,1229229,3050.6629848480225,0.62435861605627
308308,616617,616616,1233233,3057.956748008728,0.6225406685043708
309309,618619,618618,1237237,3063.072910785675,0.6207333838501654
310310,620621,620620,1241241,3070.366963863373,0.6189366686394351
311311,622623,622622,1245245,3075.493805885315,0.6171504305093549
312312,624625,624624,1249249,3082.776666879654,0.6153745781757607
313313,626627,626626,1253253,3087.8614547252655,0.613609021405864
314314,628629,628628,1257257,3095.2053139209747,0.6118536710218905
315315,630631,630630,1261261,3102.3695878982544,0.6101084388610616
316316,632633,632632,1265265,3107.6202487945557,0.608373237781052
317317,634635,634634,1269269,3114.8246309757233,0.6066479816345236
318318,636637,636636,1273273,3119.981657743454,0.6049325852563925
319319,638639,638638,1277277,3127.2696208953857,0.6032269644529151
320320,640641,640640,1281281,3132.432270050049,0.6015310359853174
321321,642643,642642,1285285,3139.666771888733,0.5998447175643378
322322,644645,644644,1289289,3144.7857599258423,0.5981679278138472
323323,646647,646646,1293293,3152.1177427768707,0.5965005862890393
324324,648649,648648,1297297,3157.343514919281,0.5948426134382316
325325,650651,650650,1301301,3164.768364906311,0.5931939306046843
326326,652653,652652,1305305,3170.1240158081055,0.5915544600065914
327327,654655,654654,1309309,3180.499778985977,0.5899241279730632
328328,656657,656656,1313313,3186.07879281044,0.5883028676744289
329329,658659,658658,1317317,3195.14310503006,0.5866905915427196
330330,660661,660660,1321321,3200.7489309310913,0.585087225164898
331331,662663,662662,1325325,3209.787137031555,0.5834926949537476
332332,664665,664664,1329329,3215.3638319969177,0.5819069281278644
333333,666667,666666,1333333,3224.387204885483,0.5803298527025618
334334,668669,668668,1337337,3229.617287874222,0.5787613974880514
335335,670671,670670,1341341,3438.2792670726776,0.5772014920585207
336336,672673,672672,1345345,3443.404467821121,0.5756500667594082
337337,674675,674674,1349349,3564.963096857071,0.5741070526873955
338338,676677,676676,1353353,3570.320767879486,0.5725723816958634
339339,678679,678678,1357357,3623.9655590057373,0.5710459863512369
340340,680681,680680,1361361,3629.584832906723,0.5695277999639075
341341,682683,682682,1365365,3746.456429004669,0.5680177565554914
342342,684685,684684,1369369,3752.1463339328766,0.56651579084064
343343,686687,686686,1373373,3760.7083308696747,0.5650218382434105
344344,688689,688688,1377377,3766.3376319408417,0.5635358348663431
345345,690691,690690,1381381,3925.3817789554596,0.562057717495918
346346,692693,692692,1385385,3930.9548258781433,0.5605874235807278
347347,694695,694694,1389389,3990.750072002411,0.5591248912296578
348348,696697,696696,1393393,3996.326826810837,0.5576700592082489
349349,698699,698698,1397397,4004.957382917404,0.5562228669186879
350350,700701,700700,1401401,4010.5531549453735,0.5547832543979894
351351,702703,702702,1405405,4085.1901519298553,0.5533511623088998
352352,704705,704704,1409409,4090.845739841461,0.5519265319344413
353353,706707,706706,1413413,4162.6697199344635,0.5505093051597214
354354,708709,708708,1417417,4168.445954084396,0.5490994244828471
355355,710711,710710,1421421,4232.722606658936,0.547696832984002
356356,712713,712712,1425425,4238.371393918991,0.5463014743363601
357357,714715,714714,1429429,4415.196980953217,0.5449132927878964
358358,716717,716716,1433433,4420.838457107544,0.5435322331577481
359359,718719,718718,1437437,4475.404349803925,0.5421582408380345
360360,720721,720720,1441441,4481.056569099426,0.5407912617592956
361361,722723,722722,1445445,4597.889928817749,0.5394312424214149
362362,724725,724724,1449449,4603.510618686676,0.5380781298536021
363363,726727,726726,1453453,4612.07719874382,0.5367318716198497
364364,728729,728728,1457457,4617.684996843338,0.5353924158243899
365365,730731,730730,1461461,4770.349407911301,0.5340597110825911
366366,732733,732732,1465465,4775.942314863205,0.5327337065318716
367367,734735,734734,1469469,4841.549667835236,0.5314143518171477
368368,736737,736736,1473473,4847.228066921234,0.5301015970835579
369369,738739,738738,1477477,4897.919805765152,0.5287953929764626
370370,740741,740740,1481481,4902.733299970627,0.5274956906305306
371371,742743,742742,1485485,4907.967903852463,0.5262024416624627
372372,744745,744744,1489489,4911.957054853439,0.5249155981709919
373373,746747,746746,1493493,4915.42110991478,0.5236351127223315
374374,748749,748748,1497497,4920.075690984726,0.5223609383574512
375375,750751,750750,1501501,4924.144910812378,0.5210930285666109
376376,752753,752752,1505505,4928.299319028854,0.5198313373057317
377377,754755,754754,1509509,4932.170143842697,0.5185758189782064
378378,756757,756756,1513513,4935.971458911896,0.5173264284239849
379379,758759,758758,1517517,4940.6628448963165,0.5160831209304888
380380,760761,760760,1521521,4944.939577102661,0.514845852218059
381381,762763,762762,1525525,4948.995139837265,0.513614578429042
382382,764765,764764,1529529,4952.917819738388,0.5123892561332468
383383,766767,766766,1533533,4957.030835866928,0.51116984231885
384384,768769,768768,1537537,4960.594947814941,0.5099562943869387
385385,770771,770770,1541541,4964.280186891556,0.5087485701405967
386386,772773,772772,1545545,4967.886094093323,0.5075466277994565
387387,774775,774774,1549549,4971.399572849274,0.5063504259615002
388388,776777,776776,1553553,4975.6549417972565,0.5051599236394395
389389,778779,778778,1557557,4979.203172683716,0.5039750802206981
390390,780781,780780,1561561,4982.708149909973,0.5027958554837824
391391,782783,782782,1565565,4986.073929786682,0.5016222095819103
392392,784785,784784,1569569,4989.379288673401,0.5004541030466498
393393,786787,786786,1573573,4992.816177845001,0.49929149678246176
394394,788789,788788,1577577,4996.133076906204,0.4981343520539667
395395,790791,790790,1581581,4999.383946895599,0.4969826304968592
396396,792793,792792,1585585,5002.826259851456,0.49583629409607965
397397,794795,794794,1589589,5006.184198856354,0.49469530519309046
398398,796797,796796,1593593,5009.6004049777985,0.4935596264876949
399399,798799,798798,1597597,5012.913302898407,0.4924292210089334
400400,800801,800800,1601601,5016.596334695816,0.4913040521387302
401401,802803,802802,1605605,5020.064617872238,0.49018408359916066
402402,804805,804804,1609609,5023.383249759674,0.48906927943971823
403403,806807,806806,1613613,5026.750888824463,0.4879596040391334
404404,808809,808808,1617617,5030.316337823868,0.4868550221053738
405405,810811,810810,1621621,5033.618598937988,0.48575549867200607
406406,812813,812812,1625625,5036.904784917831,0.48466099908364413
407407,814815,814814,1629629,5040.172940015793,0.48357148900868197
408408,816817,816816,1633633,5043.405771970749,0.4824869344192848
409409,818819,818818,1637637,5046.658061027527,0.48140730160048406
410410,820821,820820,1641641,5049.889401674271,0.48033255714290135
411411,822823,822822,1645645,5074.112232923508,0.4792626679318346
412412,824825,824824,1649649,5078.391801118851,0.4781976011581719
413413,826827,826826,1653653,5081.872451066971,0.4771373243038397
414414,828829,828828,1657657,5085.267144918442,0.47608180513998377
415415,830831,830830,1661661,5088.592904806137,0.47503101173060713
416416,832833,832832,1665665,5091.924836874008,0.4739849124180182
417417,834835,834834,1669669,5095.19616484642,0.47294347583374474
418418,836837,836836,1673673,5098.572375059128,0.4719066708803439
419419,838839,838838,1677677,5101.875315904617,0.47087446674049716
420420,840841,840840,1681681,5105.336683034897,0.46984683286245854
421421,842843,842842,1685685,5109.460011005402,0.46882373897824436
422422,844845,844844,1689689,5113.872211933136,0.4678051550690725
423423,846847,846846,1693693,5117.904023885727,0.4667910513908282
424424,848849,848848,1697697,5121.830605983734,0.4657813984540553
425425,850851,850850,1701701,5126.251508951187,0.46477616702941305
426426,852853,852852,1705705,5130.431729793549,0.4637753281476762
427427,854855,854854,1709709,5134.57128071785,0.4627788530815451
428428,856857,856856,1713713,5138.749388933182,0.4617867133583786
429429,858859,858858,1717717,5142.526726722717,0.4607988807510992
430430,860861,860860,1721721,5146.179615974426,0.45981532728001184
431431,862863,862862,1725725,5150.161900997162,0.45883602520007116
432432,864865,864864,1729729,5153.819809913635,0.45786094701361435
433433,866867,866866,1733733,5157.6517329216,0.45689006545035227
434434,868869,868868,1737737,5161.47345995903,0.4559233534782834
435435,870871,870870,1741741,5165.2692239284515,0.4549607843018748
436436,872873,872872,1745745,5169.096889734268,0.45400233134205337
437437,874875,874874,1749749,5193.39716386795,0.45304796825439553
438438,876877,876876,1753753,5197.841199874878,0.4520976689145755
439439,878879,878878,1757757,5202.181715965271,0.4511514074256411
440440,880881,880880,1761761,5205.9233548641205,0.45020915810528095
441441,882883,882882,1765765,5209.423542022705,0.44927089548218646
442442,884885,884884,1769769,5212.909881830215,0.44833659431424167
443443,886887,886886,1773773,5216.359706878662,0.44740622956123843
444444,888889,888888,1777777,5219.890236854553,0.4464797763903334
445445,890891,890890,1781781,5223.316337823868,0.44555721018696204
446446,892893,892892,1785785,5226.870623826981,0.4446385065366485
447447,894895,894894,1789789,5230.476490020752,0.44372364122318686
448448,896897,896896,1793793,5234.003228902817,0.442812590241374
449449,898899,898898,1797797,5237.770333766937,0.4419053297788196
450450,900901,900900,1801801,5241.202861070633,0.4410018362250412
451451,902903,902902,1805805,5244.672209739685,0.44010208616236923
452452,904905,904904,1809809,5248.299788951874,0.439206056362309
453453,906907,906906,1813813,5251.78440284729,0.4383137237982737
454454,908909,908908,1817817,5255.193441867828,0.4374250656219374
455455,910911,910910,1821821,5258.5715799331665,0.43654005917778704
456456,912913,912912,1825825,5262.043044805527,0.4356586819940276
457457,914915,914914,1829829,5265.453236818314,0.4347809117862198
458458,916917,916916,1833833,5268.986791849136,0.43390672644272854
459459,918919,918918,1837837,5272.491621732712,0.4330361040429125
460460,920921,920920,1841841,5276.0849609375,0.4321690228389343
461461,922923,922922,1845845,5279.648858785629,0.43130546125212277
462462,924925,924924,1849849,5283.229228973389,0.4304453978929814
463463,926927,926926,1853853,5286.697560071945,0.42958881153208495
464464,928929,928928,1857857,5290.094116687775,0.42873568111645
465465,930931,930930,1861861,5293.513497829437,0.4278859857622592
466466,932933,932932,1865865,5297.077081680298,0.4270397047512233
467467,934935,934934,1869869,5300.520126819611,0.42619681753058103
468468,936937,936936,1873873,5304.006173849106,0.4253573037167371
469469,938939,938938,1877877,5307.382255792618,0.4245211430843483
470470,940941,940940,1881881,5310.694012880325,0.4236883155645046
471471,942943,942942,1885885,5313.992281675339,0.4228588012574619
472472,944945,944944,1889889,5317.403005838394,0.42203258041627123
473473,946947,946946,1893893,5839.910350799561,0.42120963344859774
474474,948949,948948,1897897,5845.910577774048,0.42038994091853965
475475,950951,950950,1901901,5849.9435958862305,0.4195734835448093
476476,952953,952952,1905905,5856.055681943893,0.41876024219709507
477477,954955,954954,1909909,5860.91623878479,0.4179501978887856
478478,956957,956956,1913913,5865.13990187645,0.4171433317933406
479479,958959,958958,1917917,5869.286950826645,0.4163396252242819
480480,960961,960960,1921921,5872.846890926361,0.4155390596406505
481481,962963,962962,1925925,5876.390865802765,0.4147416166433686
482482,964965,964964,1929929,5880.165536880493,0.4139472779879725
483483,966967,966966,1933933,5883.8159947395325,0.41315602556096565
484484,968969,968968,1937937,5887.478606700897,0.40913828767043015
485485,970971,970970,1941941,5891.22571182251,0.40836570218561974
486486,972973,972972,1945945,5894.679506778717,0.4075960772934195
487487,974975,974974,1949949,5898.206205844879,0.40682939598445955
488488,976977,976976,1953953,5901.693073749542,0.4060656413803372
489489,978979,978978,1957957,5905.499679803848,0.40530479673361697
490490,980981,980980,1961961,5910.173569917679,0.40454684542237374
491491,982983,982982,1965965,5913.698553800583,0.4037917709483736
492492,984985,984984,1969969,5917.234534740448,0.4030395569443499
493493,986987,986986,1973973,5920.637149810791,0.4022901871630893
494494,988989,988988,1977977,5923.967542886734,0.40154364547379373
495495,990991,990990,1981981,5927.3744258880615,0.4007999158820894
496496,992993,992992,1985985,5930.748508930206,0.4000589824936469
497497,994995,994994,1989989,5934.049243927002,0.39932082955238
498498,996997,996996,1993993,5937.424050807953,0.3985854414058849
499499,998999,998998,1997997,5940.8154718875885,0.39785280253090605
500501,1001003,1001002,2002005,5944.210108757019,0.39712216969564906
501502,1003005,1003004,2006009,5947.544004678726,0.39639498593351163
502503,1005007,1005006,2010013,5950.889709949493,0.3956705055279599
503504,1007009,1007008,2014017,5954.289076805115,0.3949487134013907
504505,1009011,1009010,2018021,5957.625372886658,0.3942295945907972
505506,1011013,1011012,2022025,5961.138489723206,0.3935131342514069
506507,1013015,1013014,2026029,5964.466423034668,0.39279931763849163
507508,1015017,1015016,2030033,5967.722323894501,0.3920881301146437
508509,1017019,1017018,2034037,5971.029246807098,0.3913795571625087
509510,1019021,1019020,2038041,5974.374305009842,0.3906735843520437
510511,1021023,1021022,2042045,5977.68994307518,0.389970197375078
511512,1023025,1023024,2046049,5981.0524559021,0.3892693820234854
512513,1025027,1025026,2050053,5984.433490753174,0.38857112419100304
513514,1027029,1027028,2054057,5987.793662786484,0.38787540987141256
514515,1029031,1029030,2058061,5991.174389839172,0.3871822251639969
515516,1031033,1031032,2062065,5994.443053007126,0.3864915562717215
516517,1033035,1033034,2066069,5997.66711807251,0.3858033894921391
517518,1035037,1035036,2070073,6000.880594968796,0.385117711221028
518519,1037039,1037038,2074077,6004.131744861603,0.38443450795602985
519520,1039041,1039040,2078081,6007.316657781601,0.3837537662930117
520521,1041043,1041042,2082085,6010.554130792618,0.3830754729169712
521522,1043045,1043044,2086089,6013.762428760529,0.3823996146184072
522523,1045047,1045046,2090093,6016.974718809128,0.38172617827331123
523524,1047049,1047048,2094097,6020.174700021744,0.38105515085590014
524525,1049051,1049050,2098101,6023.400803089142,0.38038651943315926
525526,1051053,1051052,2102105,6026.783857822418,0.3797202711648424
526527,1053055,1053054,2106109,6029.997453927994,0.3790563932980149
527528,1055057,1055056,2110113,6033.208475828171,0.3783948731779674
528529,1057059,1057058,2114117,6036.3901998996735,0.37773569823184516
529530,1059061,1059060,2118121,6039.599805831909,0.37707885597774293
530531,1061063,1061062,2122125,6042.81046295166,0.3764243340247049
531532,1063065,1063064,2126129,6046.01531291008,0.3757721200636297
532533,1065067,1065066,2130133,6049.207731962204,0.37512220188000356
533534,1067069,1067068,2134137,6052.424901723862,0.37447456733752915
534535,1069071,1069070,2138141,6055.64915394783,0.37382920439267764
535536,1071073,1071072,2142145,6058.8744859695435,0.37318610107467975
536537,1073075,1073074,2146149,6062.1035788059235,0.3725452455055347
537538,1075077,1075076,2150153,6065.26314496994,0.37190662589091517
538539,1077079,1077078,2154157,6068.461692810059,0.3712702305147104
539540,1079081,1079080,2158161,6071.652441740036,0.37063604774084524
540541,1081083,1081082,2162165,6074.856686830521,0.37000406601509894
541542,1083085,1083084,2166169,6078.112847805023,0.36937427386692434
542543,1085087,1085086,2170173,6081.352867841721,0.3687466599039908
543544,1087089,1087088,2174177,6084.521222829819,0.3681212128049083
544545,1089091,1089090,2178181,6087.775859832764,0.3674979213410552
545546,1091093,1091092,2182185,6090.985559940338,0.3668767743438366
546547,1093095,1093094,2186189,6094.185478925705,0.366257760735607
547548,1095097,1095096,2190193,6097.4688448905945,0.3656408695042046
548549,1097099,1097098,2194197,6100.7093460559845,0.365026089724779
549550,1099101,1099100,2198201,6103.997699737549,0.36441341053250653
550551,1101103,1101102,2202205,6107.273837089539,0.36380282114805595
551552,1103105,1103104,2206209,6110.560940027237,0.3631943108612177
552553,1105107,1105106,2210213,6113.7539138793945,0.36258786903636064
553554,1107109,1107108,2214217,6116.996536016464,0.36198348510333744
554555,1109111,1109110,2218221,6120.235594987869,0.3613811485720362
555556,1111113,1111112,2222225,6123.41188287735,0.36078084902146657
556557,1113115,1113114,2226229,6126.597050905228,0.3601825760961219
557558,1115117,1115116,2230233,6129.976842880249,0.3595863195187121
558559,1117119,1117118,2234237,6133.399132966995,0.3589920690719737
559560,1119121,1119120,2238241,6136.629125833511,0.3583998146114027
560561,1121123,1121122,2242245,6139.880853891373,0.35780954605979787
561562,1123125,1123124,2246249,6143.161561727524,0.3572212534145365
562563,1125127,1125126,2250253,6146.4429268836975,0.35663492672756547
563564,1127129,1127128,2254257,6149.665116786957,0.35605055612541037
564565,1129131,1129130,2258261,6152.861638784409,0.35546813179280434
565566,1131133,1131132,2262265,6156.115131855011,0.3548876439945161
566567,1133135,1133134,2266269,6159.32959985733,0.3543090830444271
567568,1135137,1135136,2270273,6162.573276758194,0.3537324393309973
568569,1137139,1137138,2274277,6165.82018995285,0.3531577032954374
569570,1139141,1139140,2278281,6169.0782787799835,0.3525848654535366
570571,1141143,1141142,2282285,6172.296472787857,0.35201391637565393
571572,1143145,1143144,2286289,6175.489850759506,0.35144484670308884
572573,1145147,1145146,2290293,6178.742830038071,0.35087764712989156
573574,1147149,1147148,2294297,6181.979769706726,0.35031230840831995
574575,1149151,1149150,2298301,6185.219214677811,0.34974882137066743
575576,1151153,1151152,2302305,6188.372344017029,0.3491871768819692
576577,1153155,1153154,2306309,6191.590375900269,0.348627365892753
577578,1155157,1155156,2310313,6194.959495782852,0.3480693793899263
578579,1157159,1157158,2314317,6198.444140911102,0.3475132084386132
579580,1159161,1159160,2318321,6201.6735780239105,0.3469588441457745
580581,1161163,1161162,2322325,6204.864759922028,0.34640627768931154
581582,1163165,1163164,2326329,6208.097781896591,0.34585550029805745
582583,1165167,1165166,2330333,6211.400600671768,0.345306503253596
583584,1167169,1167168,2334337,6214.622406721115,0.34475927790117566
584585,1169171,1169170,2338341,6217.820101737976,0.3442138156387955
585586,1171173,1171172,2342345,6221.043345928192,0.34367010792448127
586587,1173175,1173174,2346349,6224.281507730484,0.3431281462580955
587588,1175177,1175176,2350353,6227.512709856033,0.3425879222104413
588589,1177179,1177178,2354357,6230.962674856186,0.34204942739233957
589590,1179181,1179180,2358361,6234.1771068573,0.34151265347827575
590591,1181183,1181182,2362365,6237.41570186615,0.3409775921936671
591592,1183185,1183184,2366369,6240.615739822388,0.3404442353112245
592593,1185187,1185186,2370373,6243.839738845825,0.3399125746636855
593594,1187189,1187188,2374377,6247.120523929596,0.3393826021292625
594595,1189191,1189190,2378381,6250.342760801315,0.3388543096407375
595596,1191193,1191192,2382385,6253.549154043198,0.33832768918728107
596597,1193195,1193194,2386389,6256.81320977211,0.3378027327944437
597598,1195197,1195196,2390393,6260.209843873978,0.33727943255507853
598599,1197199,1197198,2394397,6263.479825735092,0.3367577806020563
599600,1199201,1199200,2398401,6266.744500875473,0.3362377691173606
600601,1201203,1201202,2402405,6269.956709861755,0.33571939033390663
601602,1203205,1203204,2406409,6273.188636779785,0.3352026365355414
602603,1205207,1205206,2410413,6276.400862932205,0.3346875000552245
603604,1207209,1207208,2414417,6279.711944818497,0.3341739732713904
604605,1209211,1209210,2418421,6282.955922842026,0.33366204860794824
605606,1211213,1211212,2422425,6286.146018028259,0.3331517185379198
606607,1213215,1213214,2426429,6289.427794933319,0.3326429755834397
607608,1215217,1215216,2430433,6292.6889128685,0.3321358123102982
608609,1217219,1217218,2434437,6295.912497758865,0.33163022133521736
609610,1219221,1219220,2438441,6299.107882976532,0.3311261953149369
610611,1221223,1221222,2442445,6302.366129875183,0.3306237269534904
611612,1223225,1223224,2446449,6305.575927972794,0.33012280900220503
612613,1225227,1225226,2450453,6308.835145950317,0.3296234342524258
613614,1227229,1227228,2454457,6312.046718835831,0.3291255955464294
614615,1229231,1229230,2458461,6315.237732887268,0.3286292857646913
615616,1231233,1231232,2462465,6318.461894750595,0.3281344978367997
616617,1233235,1233234,2466469,6321.708469867706,0.3276412247305416
617618,1235237,1235236,2470473,6324.9146900177,0.3271494594609976
618619,1237239,1237238,2474477,6328.185785770416,0.32665919507962826
619620,1239241,1239240,2478481,6331.4122149944305,0.3261704246924637
620621,1241243,1241242,2482485,6334.635227918625,0.32568314143281896
621622,1243245,1243244,2486489,6337.834729909897,0.3251973384849407
622623,1245247,1245246,2490493,6341.081655025482,0.3247130090803694
623624,1247249,1247248,2494497,6344.309793949127,0.3242301464706543
624625,1249251,1249250,2498501,6347.517513990402,0.3237487439691904
625626,1251253,1251252,2502505,6350.761841773987,0.32326879492393346
626627,1253255,1253254,2506509,6354.012522935867,0.3227902927174
627628,1255257,1255256,2510513,6357.262953996658,0.32231323077758134
628629,1257259,1257258,2514517,6360.4809148311615,0.3218376025724865
629630,1259261,1259260,2518521,6363.692576885223,0.32136340160468535
630631,1261263,1261262,2522525,6366.932471036911,0.3208906214185845
631632,1263265,1263264,2526529,6370.246226787567,0.32041925560224627
632633,1265267,1265266,2530533,6373.4180018901825,0.3199492977710179
633634,1267269,1267268,2534537,6376.623393058777,0.31948074158572126
634635,1269271,1269270,2538541,6379.939043045044,0.3190135807490151
635636,1271273,1271272,2542545,6383.160787820816,0.3185478089944809
636637,1273275,1273274,2546549,6386.538491725922,0.3180834200920799
637638,1275277,1275276,2550553,6389.907367944717,0.31762040785179124
638639,1277279,1277278,2554557,6393.127936840057,0.3171587661236117
639640,1279281,1279280,2558561,6396.317310810089,0.31669848878846096
640641,1281283,1281282,2562565,6399.509551763535,0.31623956976363843
641642,1283285,1283284,2566569,6402.811353683472,0.3157820030119183
642643,1285287,1285286,2570573,6406.053098917007,0.3153257825124456
643644,1287289,1287288,2574577,6409.274647951126,0.3148709023007541
644645,1289291,1289290,2578581,6412.528207778931,0.3144173564396624
645646,1291293,1291292,2582585,6415.737134695053,0.31396513901745493
646647,1293295,1293294,2586589,6418.979748725891,0.31351424417152884
647648,1295297,1295296,2590593,6422.231261968613,0.31306466606474714
648649,1297299,1297298,2594597,6425.441141843796,0.3126163988999906
649650,1299301,1299300,2598601,6428.682209968567,0.31216943690378685
650651,1301303,1301302,2602605,6431.892110824585,0.3117237743535952
651652,1303305,1303304,2606609,6435.106912851334,0.31127940554506495
652653,1305307,1305306,2610613,6438.329462051392,0.31083632481204404
653654,1307309,1307308,2614617,6441.532304763794,0.3103945265211223
654655,1309311,1309310,2618621,6444.724603891373,0.3099540050716314
655656,1311313,1311312,2622625,6447.949589967728,0.3095147548974637
656657,1313315,1313314,2626629,6451.129544973373,0.3090767704652535
657658,1315317,1315316,2630633,6454.343020915985,0.30864004626528185
658659,1317319,1317318,2634637,6457.554259777069,0.30820457682784763
659660,1319321,1319320,2638641,6460.776715993881,0.3077703567178105
660661,1321323,1321322,2642645,6463.993994951248,0.307337380520039
661662,1323325,1323324,2646649,6467.226259946823,0.30690564285760047
662663,1325327,1325326,2650653,6470.5184898376465,0.306475138386304
663664,1327329,1327328,2654657,6473.774406909943,0.30604586178742466
664665,1329331,1329330,2658661,6476.995199918747,0.30561780777316017
665666,1331333,1331332,2662665,6480.23034787178,0.30519097109208815
666667,1333335,1333334,2666669,6483.479514837265,0.30476534651825204
667668,1335337,1335336,2670673,6486.716841936111,0.30434092885116115
668669,1337339,1337338,2674677,6489.907314777374,0.30391771293034253
669670,1339341,1339340,2678681,6493.131296873093,0.30349569361351314
670671,1341343,1341342,2682685,6496.347007989883,0.3030748657984077
671672,1343345,1343344,2686689,6499.599467992783,0.30265522440095083
672673,1345347,1345346,2690693,6502.848871946335,0.30223676437162794
673674,1347349,1347348,2694697,6506.342273950577,0.30181948069366626
674675,1349351,1349350,2698701,6509.680008888245,0.3014033683684829
675676,1351353,1351352,2702705,6512.877530813217,0.3009884224356938
676677,1353355,1353354,2706709,6516.227329969406,0.3005746379549237
677678,1355357,1355356,2710713,6519.473402738571,0.30016201001853915
678679,1357359,1357358,2714717,6522.698508024216,0.29975053374255367
679680,1359361,1359360,2718721,6525.908246040344,0.2993402042757225
680681,1361363,1361362,2722725,6529.12406873703,0.29893101679044776
681682,1363365,1363364,2726729,6532.34984087944,0.29852296648095944
682683,1365367,1365366,2730733,6535.596340894699,0.2981160485833243
683684,1367369,1367368,2734737,6538.853027820587,0.297710258344523
684685,1369371,1369370,2738741,6542.072066068649,0.2943088959909801
685686,1371373,1371372,2742745,6545.343966960907,0.29391358124485123
686687,1373375,1373374,2746749,6548.542407751083,0.2935193459052243
687688,1375377,1375376,2750753,6551.766793966293,0.29312618551375635
688689,1377379,1377378,2754757,6554.9666249752045,0.2927340956466651
689690,1379381,1379380,2758761,6558.185345888138,0.2923430718965392
690691,1381383,1381382,2762765,6561.483507871628,0.2919531098814332
691692,1383385,1383384,2766769,6564.695964813232,0.2915642052430485
692693,1385387,1385386,2770773,6567.965763092041,0.2911763536540093
693694,1387389,1387388,2774777,6571.159235715866,0.29078955079785374
694695,1389391,1389390,2778781,6574.377707958221,0.29040379239268077
695696,1391393,1391392,2782785,6577.629420995712,0.29001907417477923
696697,1393395,1393394,2786789,6580.940805912018,0.2896353919040848
697698,1395397,1395396,2790793,6584.301732778549,0.2892527413623611
698699,1397399,1397398,2794797,6587.5180468559265,0.28887111835865653
699700,1399401,1399400,2798801,6590.718092918396,0.28849051872020937
700701,1401403,1401402,2802805,6593.955326795578,0.2881109382997238
701702,1403405,1403404,2806809,6597.3157868385315,0.28773237296809384
702703,1405407,1405406,2810813,6600.527693986893,0.28735481862349843
703704,1407409,1407408,2814817,6603.7732837200165,0.2869782711859443
704705,1409411,1409410,2818821,6606.971773862839,0.2866027265881712
705706,1411413,1411412,2822825,6610.196675777435,0.2862281807974796
706707,1413415,1413414,2826829,6613.3851749897,0.28585462979572185
707708,1415417,1415416,2830833,6616.615641832352,0.2854820695883973
708709,1417419,1417418,2834837,6619.8359088897705,0.28511049620101403
709710,1419421,1419420,2838841,6623.053678035736,0.28473990567908913
710711,1421423,1421422,2842845,6626.321953058243,0.2843702940936055
711712,1423425,1423424,2846849,6629.537410020828,0.28400165753191686
712713,1425427,1425426,2850853,6632.773181915283,0.28363399210502394
713714,1427429,1427428,2854857,6636.152781009674,0.2832672939457552
714715,1429431,1429430,2858861,6639.485549926758,0.2829015591996722
715716,1431433,1431432,2862865,6642.716091871262,0.2825367840450781
716717,1433435,1433434,2866869,6645.925002813339,0.28217296466755215
717718,1435437,1435436,2870873,6649.341100931168,0.2818100972835964
718719,1437439,1437438,2874877,6652.769978761673,0.28144817812062684
719720,1439441,1439440,2878881,6656.115115880966,0.28108720343516325
720721,1441443,1441442,2882885,6659.440594911575,0.2807271694964584
721722,1443445,1443444,2886889,6662.85814499855,0.2803680725955928
722723,1445447,1445446,2890893,6666.239275932312,0.2800099090418371
723724,1447449,1447448,2894897,6669.56826376915,0.27965267516628955
724725,1449451,1449450,2898901,6672.920606851578,0.2792963673182385
725726,1451453,1451452,2902905,6676.202261924744,0.27894098186516203
726727,1453455,1453454,2906909,6679.644003868103,0.27858651519454725
727728,1455457,1455456,2910913,6682.9373087883,0.2782329637102521
728729,1457459,1457458,2914917,6686.205605745316,0.27788032384160033
729730,1459461,1459460,2918921,6689.518411874771,0.27752859202701075
730731,1461463,1461462,2922925,6692.831146001816,0.2771777647303679
731732,1463465,1463464,2926929,6696.110265016556,0.2768278384319274
732733,1465467,1465466,2930933,6699.52019572258,0.2764788096264965
733734,1467469,1467468,2934937,6702.927377939224,0.2761306748343486
734735,1469471,1469470,2938941,6706.31231880188,0.27578343058848986
735736,1471473,1471472,2942945,6709.699546813965,0.27543707344193535
736737,1473475,1473474,2946949,6713.0672607421875,0.27509159996407107
737738,1475477,1475476,2950953,6716.548014879227,0.2747470067388349
738739,1477479,1477478,2954957,6720.012903928757,0.2744032903792686
739740,1479481,1479480,2958961,6723.420598983765,0.27406044750205183
740741,1481483,1481482,2962965,6726.849880695343,0.2737184747475112
741742,1483485,1483484,2966969,6730.505563735962,0.27337736877780117
742743,1485487,1485486,2970973,6733.952852964401,0.2730371262587141
743744,1487489,1487488,2974977,6737.376483678818,0.2726977438887843
744745,1489491,1489490,2978981,6740.862755060196,0.27235921837200294
745746,1491493,1491492,2982985,6744.236685991287,0.27202154643600807
746747,1493495,1493494,2986989,6747.6382830142975,0.2716847248211707
747748,1495497,1495496,2990993,6750.997195959091,0.27134875028605165
748749,1497499,1497498,2994997,6754.522047996521,0.2710136196037638
749750,1499501,1499500,2999001,6757.997802972794,0.2706793295674288
750751,1501503,1501502,3003005,6761.363619804382,0.27034587698108226
751752,1503505,1503504,3007009,6764.7736740112305,0.27001325867240666
752753,1505507,1505506,3011013,6768.152971982956,0.26968147147817945
753754,1507509,1507508,3015017,6771.540175676346,0.26935051225154893
754755,1509511,1509510,3019021,6774.97492980957,0.26902037786749133
755756,1511513,1511512,3023025,6778.631997823715,0.2686910652100778
756757,1513515,1513514,3027029,6782.131858825684,0.26836257118702633
757758,1515517,1515516,3031033,6785.53738284111,0.26803489271151193
758759,1517519,1517518,3035037,6788.921717882156,0.26770802671671845
759760,1519521,1519520,3039041,6792.331095933914,0.26738197015765763
760761,1521523,1521522,3043045,6795.730521678925,0.2670567199911602
761762,1523525,1523524,3047049,6799.064050912857,0.26673227319770376
762763,1525527,1525526,3051053,6802.419593811035,0.26640862677959376
763764,1527529,1527528,3055057,6805.847347974777,0.2660857777354977
764765,1529531,1529530,3059061,6809.422199010849,0.26576372309682483
765766,1531533,1531532,3063065,6812.928192853928,0.26544245990226045
766767,1533535,1533534,3067069,6816.334022760391,0.2651219852032227
767768,1535537,1535536,3071073,6819.649785757065,0.26480229606568173
768769,1537539,1537538,3075077,6823.013012886047,0.2644833895810734
769770,1539541,1539540,3079081,6826.380821943283,0.26416526283719577
770771,1541543,1541542,3083085,6829.84002995491,0.2638479129564075
771772,1543545,1543544,3087089,6833.374109983444,0.2635313370556105
772773,1545547,1545546,3091093,6836.833458900452,0.2632155322753533
773774,1547549,1547548,3095097,6840.274219989777,0.26290049577619357
774775,1549551,1549550,3099101,6843.728978872299,0.2625862247241457
775776,1551553,1551552,3103105,6847.100841999054,0.26227271629613824
776777,1553555,1553554,3107109,6850.50843000412,0.2619599676945654
777778,1555557,1555556,3111113,6853.967331647873,0.26164797612545954
778779,1557559,1557558,3115117,6857.373530864716,0.2613367388184997
779780,1559561,1559560,3119121,6860.836153745651,0.26102625299972715
780781,1561563,1561562,3123125,6864.2968780994415,0.26071651592974376
781782,1563565,1563564,3127129,6867.664527893066,0.26040752486915153
782783,1565567,1565566,3131133,6870.937626838684,0.26009927709128533
783784,1567569,1567568,3135137,6874.227132797241,0.2597917698913079
784785,1569571,1569570,3139141,6877.512289047241,0.259485000573477
785786,1571573,1571572,3143145,6880.795767068863,0.25917896645114524
786787,1573575,1573574,3147149,6884.065416812897,0.25887366485585517
787788,1575577,1575576,3151153,6887.391956806183,0.25856909313006327
788789,1577579,1577578,3155157,6890.71123790741,0.25826524862895894
789790,1579581,1579580,3159161,6894.022766113281,0.2579621287222835
790791,1581583,1581582,3163165,6897.340112924576,0.25765973079069227
791792,1583585,1583584,3167169,6900.66024184227,0.25735805222575436
792793,1585587,1585586,3171173,6903.975282907486,0.2570570904354099
793794,1587589,1587588,3175177,6907.269498825073,0.256756842836694
794795,1589591,1589590,3179181,6910.546430826187,0.25645730686665047
795796,1591593,1591592,3183185,6913.8371069431305,0.25615847996050434
796797,1593595,1593594,3187189,6917.123598098755,0.2558603595771274
797798,1595597,1595596,3191193,6920.378448724747,0.25556294318630535
798799,1597599,1597598,3195197,6923.673295736313,0.2552662282669189
799800,1599601,1599600,3199201,6926.985529661179,0.2549702123124007
800801,1601603,1601602,3203205,6930.261360883713,0.25467489282164024
801802,1603605,1603604,3207209,6933.62789773941,0.254380267315355
802803,1605607,1605606,3211213,6937.160803794861,0.2540863333197194
803804,1607609,1607608,3215217,6940.572773694992,0.2537930883736408
804805,1609611,1609610,3219221,6943.974435091019,0.2535005300269404
805806,1611613,1611612,3223225,6947.374233722687,0.2532086558476294
806807,1613615,1613614,3227229,6950.796676874161,0.252917463407357
807808,1615617,1615616,3231233,6954.181272029877,0.2526269502886862
808809,1617619,1617618,3235237,6957.625860691071,0.25233711409055104
809810,1619621,1619620,3239241,6961.150424718857,0.2520479524227994
810811,1621623,1621622,3243245,6964.561151981354,0.2517594629061932
811812,1623625,1623624,3247249,6967.938083648682,0.25147164316695125
812813,1625627,1625626,3251253,6971.343863964081,0.2511844908531202
813814,1627629,1627628,3255257,6974.71529173851,0.2508980036163848
814815,1629631,1629630,3259261,6978.114489078522,0.25061217911388667
815816,1631633,1631632,3263265,6981.457641839981,0.2503270150300523
816817,1633635,1633634,3267269,6984.750149726868,0.2500425090511271
817818,1635637,1635636,3271273,6988.030082941055,0.24975865886699467
818819,1637639,1637638,3275277,6991.314100980759,0.24947546218754724
819820,1639641,1639640,3279281,6994.778747797012,0.24919291673359112
820821,1641643,1641642,3283285,6998.22082567215,0.24891102023138956
821822,1643645,1643644,3287289,7001.5148549079895,0.2486297704253957
822823,1645647,1645646,3291293,7004.813850879669,0.24834916506188165
823824,1647649,1647648,3295297,7008.0989990234375,0.24806920190167148
824825,1649651,1649650,3299301,7011.406094074249,0.24778987871650315
825826,1651653,1651652,3303305,7014.843783855438,0.24751119328357163
826827,1653655,1653654,3307309,7018.318301916122,0.24723314340008073
827828,1655657,1655656,3311313,7021.867427825928,0.24695572686687228
828829,1657659,1657658,3315317,7025.278573036194,0.24667894149570202
829830,1659661,1659660,3319321,7028.67537689209,0.24640278510378266
830831,1661663,1661662,3323325,7032.120250701904,0.2461272555301548
831832,1663665,1663664,3327329,7035.519524812698,0.24585235061204003
832833,1665667,1665666,3331333,7038.943743944168,0.24557806820303085
833834,1667669,1667668,3335337,7042.335615873337,0.24530440616763372
834835,1669671,1669670,3339341,7045.780867099762,0.24503136237035505
835836,1671673,1671672,3343345,7049.195443868637,0.24475893469934817
836837,1673675,1673674,3347349,7052.57124876976,0.24448712104276638
837838,1675677,1675676,3351353,7055.927235841751,0.24421591930513387
838839,1677679,1677678,3355357,7059.262759923935,0.24394532738915586
839840,1679681,1679680,3359361,7062.552314758301,0.24367534322118445
840841,1681683,1681682,3363365,7065.834446668625,0.2434059647275717
841842,1683685,1683684,3367369,7069.360991001129,0.2431371898492216
842843,1685687,1685686,3371373,7072.8025987148285,0.24286901653249515
843844,1687689,1687688,3375377,7076.181993961334,0.2426014427364862
844845,1689691,1689690,3379381,7079.61301779747,0.24233446642574563
845846,1691693,1691692,3383385,7083.019444942474,0.2420680855793762
846847,1693695,1693694,3387389,7086.445501804352,0.24180229817829968
847848,1695697,1695696,3391393,7089.926592826843,0.24153710221798974
848849,1697699,1697698,3395397,7093.325985908508,0.241272495704834
849850,1699701,1699700,3399401,7096.899954795837,0.24100847664885805
850851,1701703,1701702,3403405,7100.40446472168,0.24074504307100142
851852,1703705,1703704,3407409,7103.898104906082,0.24048219300129858
852853,1705707,1705706,3411413,7107.4116678237915,0.24021992447887897
853854,1707709,1707708,3415417,7110.813421964645,0.23995823555560492
854855,1709711,1709710,3419421,7114.2797498703,0.2396971242815198
855856,1711713,1711712,3423425,7117.6988480091095,0.23943658872485685
856857,1713715,1713714,3427429,7121.128174781799,0.2391766269593063
857858,1715717,1715716,3431433,7124.550998926163,0.2389172370712913
858859,1717719,1717718,3435437,7127.963385105133,0.238658417147235
859860,1719721,1719720,3439441,7131.329593896866,0.2384001652862935
860861,1721723,1721722,3443445,7134.624567985535,0.23814247960035573
861862,1723725,1723724,3447449,7137.9521317481995,0.23788535820312973
862863,1725727,1725726,3451453,7141.255993843079,0.2376287992210564
863864,1727729,1727728,3455457,7144.549635648727,0.23737280078603362
864865,1729731,1729730,3459461,7147.964555978775,0.23711736104087322
865866,1731733,1731732,3463465,7151.406725883484,0.23686247813748196
866867,1733735,1733734,3467469,7154.836664915085,0.2366081502259476
867868,1735737,1735736,3471473,7158.244302034378,0.2363543754836428
868869,1737739,1737738,3475477,7161.871914863586,0.2361011520752072
869870,1739741,1739740,3479481,7165.368805885315,0.2358484781889274
870871,1741743,1741742,3483485,7168.755460739136,0.23559635201127094
871872,1743745,1743744,3487489,7172.217801809311,0.2353447717450763
872873,1745747,1745746,3491493,7175.641801834106,0.23509373559136293
873874,1747749,1747748,3495497,7179.0511820316315,0.23484324176752125
874875,1749751,1749750,3499501,7182.453596830368,0.2345932884963986
875876,1751753,1751752,3503505,7186.105235815048,0.23434387400084233
876877,1753755,1753754,3507509,7189.614628791809,0.23409499653098464
877878,1755757,1755756,3511513,7193.03270483017,0.23384665431876783
878879,1757759,1757758,3515517,7196.519917011261,0.23359884562523803
879880,1759761,1759760,3519521,7200.024370908737,0.23335156870780338
880881,1761763,1761762,3523525,7203.473123788834,0.23310482183842396
881882,1763765,1763764,3527529,7206.973905801773,0.23285860328724084
882883,1765767,1765766,3531533,7210.420163869858,0.232612911340766
883884,1767769,1767768,3535537,7213.92503285408,0.2323677442909684
884885,1769771,1769770,3539541,7217.360615968704,0.232123100429817
885886,1771773,1771772,3543545,7220.756438970566,0.2318789780692896
886887,1773775,1773774,3547549,7224.155162811279,0.23163537551954505
887888,1775777,1775776,3551553,7227.567172765732,0.23139229110165616
888889,1777779,1777778,3555557,7230.971856832504,0.23114972314033366
889890,1779781,1779780,3559561,7234.387432813644,0.23090766997302126
890891,1781783,1781782,3563565,7237.8413009643555,0.2306661299408006
891892,1783785,1783784,3567569,7241.263599872589,0.2304251013938483
892893,1785787,1785786,3571573,7244.7037088871,0.23018458268597897
893894,1787789,1787788,3575577,7248.1442539691925,0.2299445721801021
894895,1789791,1789790,3579581,7251.574720859528,0.22970506824640324
895896,1791793,1791792,3583585,7255.141051769257,0.2294660692641628
896897,1793795,1793794,3587589,7258.70156288147,0.2292275736162992
897898,1795797,1795796,3591593,7262.122880935669,0.2289895796966448
898899,1797799,1797798,3595597,7265.580028772354,0.22875208589721296
899900,1799801,1799800,3599601,7269.008943796158,0.22851509062820696
900901,1801803,1801802,3603605,7272.45382976532,0.22827859229619207
901902,1803805,1803804,3607609,7275.888356685638,0.22804258932410448
902903,1805807,1805806,3611613,7279.349608898163,0.22780708013488038
903904,1807809,1807808,3615617,7282.85325884819,0.2275720631605509
904905,1809811,1809810,3619621,7286.256347894669,0.22733753684042313
905906,1811813,1811812,3623625,7289.685081720352,0.22710349961744214
906907,1813815,1813814,3627629,7293.11092877388,0.22686994994728593
907908,1815817,1815816,3631633,7296.525981903076,0.2266368862838135
908909,1817819,1817818,3635637,7299.9357488155365,0.2264043070954358
909910,1819821,1819820,3639641,7303.340199947357,0.22617221085056372
910911,1821823,1821822,3643645,7306.92357301712,0.2259405960303411
911912,1823825,1823824,3647649,7310.452172994614,0.22570946111409285
912913,1825827,1825826,3651653,7313.867506980896,0.22547880459933367
913914,1827829,1827828,3655657,7317.3484308719635,0.22524862497630238
914915,1829831,1829830,3659661,7320.755743980408,0.22501892074978969
915916,1831833,1831832,3663665,7324.1989569664,0.22478969043004327
916917,1833835,1833834,3667669,7327.611304998398,0.22456093253640574
917918,1835837,1835836,3671673,7331.061192989349,0.22433264558640076
918919,1837839,1837838,3675677,7334.5588138103485,0.22410482810846588
919920,1839841,1839840,3679681,7337.9814016819,0.22387747864013363
920921,1841843,1841842,3683685,7341.733428955078,0.22365059571893653
921922,1843845,1843844,3687689,7345.153155088425,0.22342417789150204
922923,1845847,1845846,3691693,7348.615777015686,0.22319822371355258
923924,1847849,1847848,3695697,7352.017814874649,0.22297273174081056
924925,1849851,1849850,3699701,7355.4517476558685,0.22274770053991233
925926,1851853,1851852,3703705,7358.877898931503,0.22252312868113222
926927,1853855,1853854,3707709,7362.342315912247,0.22229901473838254
927928,1855857,1855856,3711713,7365.930358886719,0.22207535729830852
928929,1857859,1857858,3715717,7369.6276948452,0.2218521549475554
929930,1859861,1859860,3719721,7373.036388874054,0.22162940628004435
930931,1861863,1861862,3723725,7376.31768488884,0.22140710989879153
931932,1863865,1863864,3727729,7379.64874792099,0.2211852644031751
932933,1865867,1865866,3731733,7383.005628824234,0.2209638684107631
933934,1867869,1867868,3735737,7386.392657756805,0.22074292054094258
934935,1869871,1869870,3739741,7389.742038965225,0.2205224194094626
935936,1871873,1871872,3743745,7393.066790819168,0.22030236365026212
936937,1873875,1873874,3747749,7396.380449056625,0.22008275189182314
937938,1875877,1875876,3751753,7399.683681964874,0.2198635827826365
938939,1877879,1877878,3755757,7402.986771821976,0.21964485496209818
939940,1879881,1879880,3759761,7406.270724773407,0.21942656708415598
940941,1881883,1881882,3763765,7409.590646028519,0.21920871780639573
941942,1883885,1883884,3767769,7412.8522918224335,0.21899130578640325
942943,1885887,1885886,3771773,7416.166306018829,0.21877432969631627
943944,1887889,1887888,3775777,7419.445437908173,0.21855778820645355
944945,1889891,1889890,3779781,7422.74461889267,0.21834167999804777
945946,1891893,1891892,3783785,7426.233456850052,0.2181260037541506
946947,1893895,1893894,3787789,7429.687852859497,0.21791075816145167
947948,1895897,1895896,3791793,7433.128411769867,0.2176959419157356
948949,1897899,1897898,3795797,7436.812018871307,0.21748155372188194
949950,1899901,1899900,3799801,7440.471703052521,0.21726759227749426
950951,1901903,1901902,3803805,7444.065665960312,0.21705405629472807
951952,1903905,1903904,3807809,7447.68877696991,0.21684094449483382
952953,1905907,1905906,3811813,7451.211894035339,0.216628255593605
953954,1907909,1907908,3815817,7454.708169937134,0.216415988317749
954955,1909911,1909910,3819821,7458.259516954422,0.21620414139761124
955956,1911913,1911912,3823825,7461.886417865753,0.21599271357263206
956957,1913915,1913914,3827829,7465.564654827118,0.2157817035804328
957958,1915917,1915916,3831833,7469.161808729172,0.21557111016954877
958959,1917919,1917918,3835837,7472.877789974213,0.21536093209215323
959960,1919921,1919920,3839841,7476.55583691597,0.21515116810587642
960961,1921923,1921922,3843845,7480.20828795433,0.2149418169665296
961962,1923925,1923924,3847849,7483.843883037567,0.2147328774444759
962963,1925927,1925926,3851853,7487.241086959839,0.21452434831371647
963964,1927929,1927928,3855857,7490.697666883469,0.2143162283446145
964965,1929931,1929930,3859861,7494.080336809158,0.21410851632572303
965966,1931933,1931932,3863865,7497.6062977313995,0.21390121103650017
966967,1933935,1933934,3867869,7501.236473798752,0.21369431127095595
967968,1935937,1935936,3871873,7504.773106813431,0.21348781582491938
968969,1937939,1937938,3875877,7508.254099845886,0.21328172349785746
969970,1939941,1939940,3879881,7511.818331718445,0.21307603309469414
970971,1941943,1941942,3883885,7515.309058904648,0.21287074342944834
971972,1943945,1943944,3887889,7518.741774082184,0.21266585331250099
972973,1945947,1945946,3891893,7522.062552690506,0.21246136156332796
973974,1947949,1947948,3895897,7525.328372001648,0.21225726700868108
974975,1949951,1949950,3899901,7528.599142789841,0.2120535684753122
975976,1951953,1951952,3903905,7531.811594009399,0.2118502648008871
976977,1953955,1953954,3907909,7535.079395771027,0.21164735481943353
977978,1955957,1955956,3911913,7538.300035715103,0.21144483737407427
978979,1957959,1957958,3915917,7541.503690004349,0.21124271131157002
979980,1959961,1959960,3919921,7544.688993930817,0.21104097548777645
980981,1961963,1961962,3923925,7547.890095710754,0.21083962875491125
981982,1963965,1963964,3927929,7551.141891717911,0.21063866997428704
982983,1965967,1965966,3931933,7554.406288862228,0.21043809801267344
983984,1967969,1967968,3935937,7557.700528860092,0.21023791173684003
984985,1969971,1969970,3939941,7560.961875915527,0.21003811002447037
985986,1971973,1971972,3943945,7564.241085767746,0.20983869175324799
986987,1973975,1973974,3947949,7567.5286729335785,0.20963965580813237
987988,1975977,1975976,3951953,7570.840570688248,0.20944100107226404
988989,1977979,1977978,3955957,7574.133271932602,0.20924272643969744
989990,1979981,1979980,3959961,7577.419539928436,0.209044830804487
990991,1981983,1981982,3963965,7580.703362941742,0.2088473130697821
991992,1983985,1983984,3967969,7584.000538825989,0.20865017213873216
992993,1985987,1985986,3971973,7587.327582836151,0.20845340691994352
993994,1987989,1987988,3975977,7590.598361730576,0.2082570163274795
994995,1989991,1989990,3979981,7593.900473117828,0.20806099927540345
995996,1991993,1991992,3983985,7597.216379880905,0.20786535469233058
996997,1993995,1993994,3987989,7600.53817987442,0.20767008149596222
997998,1995997,1995996,3991993,7603.865211725235,0.20747517862218956
998999,1997999,1997998,3995997,7607.157012939453,0.20728064500144683
1000000,2000001,2000000,4000001,7610.409976005554,0.2070864795750822


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002474069595336914,12064.682476916567
1001,2003,2002,4005,3.6562042236328125,65.52576608160416
2002,4005,4004,8009,7.248206853866577,42.34509678336872
3003,6007,6006,12013,11.04786491394043,34.023520514219854
4004,8009,8008,16017,14.50561809539795,28.958911805193566
5005,10011,10010,20021,18.777812957763672,25.333523203886216
6006,12013,12012,24025,22.469918966293335,22.527300385168928
7007,14015,14014,28029,25.92417597770691,20.253121634779745
8008,16017,16016,32033,29.24285912513733,18.355877411981055
9009,18019,18018,36037,32.58391785621643,16.742261724328273
10010,20021,20020,40041,35.91790509223938,15.35118558117756
11011,22023,22022,44045,39.232887983322144,14.139884765472743
12012,24025,24024,48049,42.51778697967529,13.076857731883138
13013,26027,26026,52053,45.83771800994873,12.138017055509408
14014,28029,28028,56057,49.15849304199219,11.30442975218466
15015,30031,30030,60061,52.627357959747314,10.560884002585226
16016,32033,32032,64065,56.25014519691467,9.894970055029262
17017,34035,34034,68069,59.66333293914795,9.296433581814199
18018,36037,36036,72073,63.050535917282104,8.756706160584145
19019,38039,38038,76077,66.3240110874176,8.26856343260988
20020,40041,40040,80081,69.58702301979065,7.825866925420996
21021,42043,42042,84085,72.88530492782593,7.423363869536843
22022,44045,44044,88089,76.24873995780945,7.0565315885924065
23023,46047,46046,92093,79.6149959564209,6.721454575370444
24024,48049,48048,96097,82.89304304122925,6.414726327160679
25025,50051,50050,100101,86.15027785301208,6.133370176887183
26026,52053,52052,104105,89.4551408290863,5.874774859685203
27027,54055,54054,108109,92.77283215522766,5.636641623708783
28028,56057,56056,112113,96.0748679637909,5.4169404684380424
29029,58059,58058,116117,99.35476207733154,5.213873662669357
30030,60061,60060,120121,102.65840482711792,5.025845117053905
31031,62063,62062,124125,105.96915698051453,4.851434503312703
32032,64065,64064,128129,109.25755000114441,4.689375251909951
33033,66067,66066,132133,112.52728700637817,4.5385357427494455
34034,68069,68068,136137,115.8041181564331,4.397903143561052
35035,70071,70070,140141,119.08533096313477,4.266569458923186
36036,72073,72072,144145,122.33660697937012,4.143719436893662
37037,74075,74074,148149,125.63575887680054,4.028620046206925
38038,76077,76076,152153,128.90019488334656,3.920611288767759
39039,78079,78078,156157,132.17271399497986,3.8190981533571176
40040,80081,80080,160161,135.43414902687073,3.723543549363967
41041,82083,82082,164165,138.6763458251953,3.633462985213555
42042,84085,84084,168169,141.95461201667786,3.548416926021673
43043,86087,86086,172173,145.1573121547699,3.4680069331843697
44044,88089,88088,176177,148.52698612213135,3.3918722434391384
45045,90091,90090,180181,151.79118299484253,3.3196853393728816
46046,92093,92092,184185,155.0806930065155,3.251148560690126
47047,94095,94094,188189,158.55242800712585,3.185991089043455
48048,96097,96096,192193,161.91575694084167,3.123966261749956
49049,98099,98098,196197,165.22131204605103,3.0648491757310694
50050,100101,100100,200201,168.47206902503967,3.0084345479244803
51051,102103,102102,204205,171.7801821231842,2.9545348027186265
52052,104105,104104,208209,175.0591859817505,2.9029783606383717
53053,106107,106106,212213,178.31591987609863,2.8536081056681724
54054,108109,108108,216217,181.64597415924072,2.8062800112911646
55055,110111,110110,220221,184.99818086624146,2.760861907792787
56056,112113,112112,224225,188.2722098827362,2.7172323753002274
57057,114115,114114,228229,191.54824090003967,2.6752797489734803
58058,116117,116116,232233,194.83267307281494,2.634901224208079
59059,118119,118118,236237,198.1087019443512,2.5960020512011397
60060,120121,120120,240241,201.37652587890625,2.558494809345575
61061,122123,122122,244245,204.6800661087036,2.5222987530560204
62062,124125,124124,248249,207.94788098335266,2.4873392215158674
63063,126127,126126,252253,211.24517583847046,2.453547105709731
64064,128129,128128,256257,214.52350497245789,2.4208583667805215
65065,130131,130130,260261,217.7814919948578,2.3892136004760687
66066,132133,132132,264265,221.07138323783875,2.358557642886808
67067,134135,134134,268269,224.34233713150024,2.328839213394531
68068,136137,136136,272273,227.66224598884583,2.30001059096503
69069,138139,138138,276277,230.92909598350525,2.2720273204940895
70070,140141,140140,280281,234.21257305145264,2.244847946203663
71071,142143,142142,284285,237.47074484825134,2.2184337693543057
72072,144145,144144,288289,240.73543310165405,2.1927486279837467
73073,146147,146146,292293,243.99914717674255,2.16775870678066
74074,148149,148148,296297,247.25601482391357,2.1434324638539692
75075,150151,150150,300301,250.5529329776764,2.119740070320404
76076,152153,152152,304305,253.84342098236084,2.0966536762553005
77077,154155,154154,308309,257.14520502090454,2.074147128711047
78078,156157,156156,312313,260.4210031032562,2.052195844546077
79079,158159,158158,316317,263.70937395095825,2.0307766945152252
80080,160161,160160,320321,266.9841728210449,2.0098678971498884
81081,162163,162162,324325,270.24792313575745,1.9894489215548674
82082,164165,164164,328329,273.5666389465332,1.9695003982669732
83083,166167,166166,332333,276.8556070327759,1.9500040374550736
84084,168169,168168,336337,280.13468980789185,1.9309425537958305
85085,170171,170170,340341,283.3652811050415,1.9122995973975776
86086,172173,172172,344345,286.6167039871216,1.8940596902666584
87087,174175,174174,348349,289.8852550983429,1.876208167801451
88088,176177,176176,352353,293.12982511520386,1.8587311248629703
89089,178179,178178,356357,296.40201711654663,1.8416153660473356
90090,180181,180180,360361,299.9115159511566,1.82484835977084
91091,182183,182182,364365,303.32374000549316,1.808418195856575
92092,184185,184184,368369,306.59454798698425,1.7923135463061044
93093,186187,186186,372373,309.84522819519043,1.77652362900335
94094,188189,188188,376377,313.13743019104004,1.7610381741033052
95095,190191,190190,380381,316.41469407081604,1.7458473928472813
96096,192193,192192,384385,319.70901107788086,1.730941948671898
97097,194195,194194,388389,323.07644295692444,1.716313168311899
98098,196197,196196,392393,326.41600799560547,1.7019523075414327
99099,198199,198198,396397,329.7309579849243,1.6878512114781188
100100,200201,200200,400401,332.9953360557556,1.6740021029290801
101101,202203,202202,404405,336.29006814956665,1.6603975401721982
102102,204205,204204,408409,339.59982895851135,1.6470303982314363
103103,206207,206206,412413,342.89549493789673,1.6338938513763424
104104,208209,208208,416417,346.1728069782257,1.6209813568148093
105105,210211,210210,420421,349.4274709224701,1.6082866394281154
106106,212213,212212,424425,352.9198589324951,1.595803677533695
107107,214215,214214,428429,356.2989320755005,1.5835266895282984
108108,216217,216216,432433,359.5523750782013,1.5714501214133634
109109,218219,218218,436437,362.8417270183563,1.5595686350789038
110110,220221,220220,440441,366.06811714172363,1.5478770973513747
111111,222223,222222,444445,369.3235430717468,1.5363705696745455
112112,224225,224224,448449,372.5838689804077,1.525044298477951
113113,226227,226226,452453,375.9017939567566,1.5138937060619355
114114,228229,228228,456457,379.28878021240234,1.50291438208842
115115,230231,230230,460461,382.55477690696716,1.492102075528237
116116,232233,232232,464465,385.8574140071869,1.4814526871195994
117117,234235,234234,468469,389.130487203598,1.4709622622413008
118118,236237,236236,472473,392.3820071220398,1.4606269841842732
119119,238239,238238,476477,395.664932012558,1.450443167841513
120120,240241,240240,480481,398.93274307250977,1.440407253730882
121121,242243,242242,484485,402.25536489486694,1.430515802341688
122122,244245,244244,488489,405.5646619796753,1.4207654888195975
123123,246247,246246,492493,408.8249568939209,1.411153097913484
124124,248249,248248,496497,412.0990080833435,1.4016755192224082
125125,250251,250250,500501,415.3806710243225,1.3923297426754289
126126,252253,252252,504505,418.6388928890228,1.3831128542660736
127127,254255,254254,508509,421.9202241897583,1.3740220320014487
128128,256257,256256,512513,425.23567605018616,1.365054542065991
129129,258259,258258,516517,428.4683349132538,1.3562077351853077
130130,260261,260260,520521,431.7616879940033,1.3474790431719157
131131,262263,262262,524525,435.08780908584595,1.3388659756383277
132132,264265,264264,528529,438.50223302841187,1.330366116897494
133133,266267,266266,532533,441.7632899284363,1.3219771229923936
134134,268269,268268,536537,445.1087188720703,1.3136967188820563
135135,270271,270270,540541,448.43822598457336,1.3055226957658306
136136,272273,272272,544545,451.7961280345917,1.2974529085367976
137137,274275,274274,548549,455.1235649585724,1.2894852733516018
138138,276277,276276,552553,458.41097712516785,1.281617765320334
139139,278279,278278,556557,461.70008993148804,1.2738484163073736
140140,280281,280280,560561,465.00318598747253,1.2661753128159035
141141,282283,282282,564565,468.2995309829712,1.258596594005212
142142,284285,284284,568569,471.5778839588165,1.2511104497643828
143143,286287,286286,572573,474.8299810886383,1.2437151188787539
144144,288289,288288,576577,478.10858821868896,1.2364088873127912
145145,290291,290290,580581,481.3888268470764,1.229190086514791
146146,292293,292292,584585,484.6915080547333,1.2220570918361773
147147,294295,294294,588589,488.1047189235687,1.2150083210181037
148148,296297,296296,592593,491.56655383110046,1.208042283073155
149149,298299,298298,596597,494.9070348739624,1.2011575415090192
150150,300301,300300,600601,498.1964280605316,1.1943525150909409
151151,302303,302302,604605,501.44788002967834,1.187625777127323
152152,304305,304304,608609,504.74811911582947,1.180975936629693
153153,306307,306306,612613,508.0012879371643,1.1744016371158068
154154,308309,308308,616617,511.32931113243103,1.167901555494609
155155,310311,310310,620621,514.7023069858551,1.1614744009748392
156156,312313,312312,624625,518.0369141101837,1.1551189140373026
157157,314315,314314,628629,521.3588199615479,1.148833865438064
158158,316317,316316,632633,524.606173992157,1.142618055238927
159159,318319,318318,636637,527.8979170322418,1.1364703119179467
160160,320321,320320,640641,531.2918429374695,1.1303894914599368
161161,322323,322322,644645,534.659049987793,1.1243744765251904
162162,324325,324324,648649,537.9546790122986,1.1184241756291158
163163,326327,326326,652653,541.2264919281006,1.1125375223582523
164164,328329,328328,656657,544.5571799278259,1.1067134746172087
165165,330331,330330,660661,547.8248820304871,1.1009510139065242
166166,332333,332332,664665,551.2407691478729,1.0952491446150816
167167,334335,334334,668669,554.6758668422699,1.0896068933579954
168168,336337,336336,672673,557.9796187877655,1.0840233083272324
169169,338339,338338,676677,561.4323000907898,1.0784974586531462
170170,340341,340340,680681,564.7022368907928,1.073028433827858
171171,342343,342342,684685,568.0147080421448,1.0676153430977138
172172,344345,344344,688689,571.3126649856567,1.0622573149266827
173173,346347,346346,692693,574.827455997467,1.0569534964452032
174174,348349,348348,696697,578.1247460842133,1.0517030529299518
175175,350351,350350,700701,581.4054050445557,1.0465051673072594
176176,352353,352352,704705,584.7265040874481,1.0413590396601649
177177,354355,354354,708709,587.9840610027313,1.0362638867682108
178178,356357,356356,712713,591.2906489372253,1.0312189416436013
179179,358359,358358,716717,594.5910730361938,1.0262234531091963
180180,360361,360360,720721,597.9029960632324,1.0212766853655921
181181,362363,362362,724725,601.162572145462,1.016377917583668
182182,364365,364364,728729,604.4481348991394,1.0115264435098652
183183,366367,366366,732733,607.6983277797699,1.0067215710932942
184184,368369,368368,736737,610.9646019935608,1.001962622100109
185185,370371,370370,740741,614.2318758964539,0.9972489317715372
186186,372373,372372,744745,617.5393629074097,0.9925798484691768
187187,374375,374374,748749,620.7853138446808,0.9879547333403025
188188,376377,376376,752753,624.1564428806305,0.9833729599995422
189189,378379,378378,756757,627.5263910293579,0.9788339142123732
190190,380381,380380,760761,630.8961727619171,0.9743369935858937
191191,382383,382382,764765,634.2168669700623,0.9698816072850605
192192,384385,384384,768769,637.4863519668579,0.9654671757307369
193193,386387,386386,772773,640.8159608840942,0.9610931303413963
194194,388389,388388,776777,644.1124927997589,0.9567589132529974
195195,390391,390390,780781,647.4065208435059,0.9524639770606882
196196,392393,392392,784785,650.690623998642,0.9482077845750609
197197,394395,394394,788789,653.9536578655243,0.9439898085620371
198198,396397,396396,792793,657.2507309913635,0.9398095315154933
199199,398399,398398,796797,660.5189960002899,0.935666445429888
200200,400401,400400,800801,663.8212819099426,0.9315600515710685
201201,402403,402402,804805,667.1472988128662,0.9274898602525354
202202,404405,404404,808809,670.4779851436615,0.923455390638992
203203,406407,406406,812813,674.010124206543,0.9194561705353408
204204,408409,408408,816817,677.3476119041443,0.9154917361811385
205205,410411,410410,820821,680.636491060257,0.9115616320723348
206206,412413,412412,824825,683.9164659976959,0.907665410755726
207207,414415,414414,828829,687.1774809360504,0.9038026326543331
208208,416417,416416,832833,690.5222940444946,0.8999728659055108
209209,418419,418418,836837,693.956573009491,0.8961756861554022
210210,420421,420420,840841,697.3416700363159,0.8924106764297903
211211,422423,422422,844845,700.6394441127777,0.8886774269285524
212212,424425,424424,848849,703.910028219223,0.8849755349092447
213213,426427,426426,852853,707.2069058418274,0.8813046045052033
214214,428429,428428,856857,710.6217727661133,0.877664246585482
215215,430431,430430,860861,713.9312012195587,0.8740540786038764
216216,432433,432432,864865,717.3069670200348,0.8704737244624994
217217,434435,434434,868869,720.5840120315552,0.8669228143717191
218218,436437,436436,872873,723.8806071281433,0.8634009847173729
219219,438439,438438,876877,727.1975498199463,0.8599078779152478
220220,440441,440440,880881,730.4769208431244,0.8564431423092174
221221,442443,442442,884885,733.7769510746002,0.8530064320239035
222222,444445,444444,888889,737.0808839797974,0.849597406855537
223223,446447,446446,892893,740.3854911327362,0.8462157321482664
224224,448449,448448,896897,743.6926460266113,0.8428610786850186
225225,450451,450450,900901,746.9683649539948,0.8395331225656264
226226,452453,452452,904905,750.2578899860382,0.8362315451086033
227227,454455,454454,908909,753.6104731559753,0.8329560327347281
228228,456457,456456,912913,756.8961911201477,0.8297062768779142
229229,458459,458458,916917,760.1512269973755,0.8264819738633378
230230,460461,460460,920921,763.4508399963379,0.8232828248237638
231231,462463,462462,924925,766.7120530605316,0.8201085355995019
232232,464465,464464,928929,770.0832190513611,0.8169588166456379
233233,466467,466466,932933,773.5204660892487,0.813833382931989
234234,468469,468468,936937,776.954124212265,0.810731953864888
235235,470471,470470,940941,780.2987380027771,0.8076542531980522
236236,472473,472472,944945,783.59605884552,0.8046000089398149
237237,474475,474474,948949,786.8860719203949,0.8015689532767283
238238,476477,476476,952953,790.1826918125153,0.7985608224898897
239239,478479,478478,956957,793.4451529979706,0.795575356876725
240240,480481,480480,960961,796.8555150032043,0.7926123006782291
241241,482483,482482,964965,800.1606860160828,0.7896714019898354
242242,484485,484484,968969,803.4596259593964,0.7867524127013894
243243,486487,486486,972973,806.7077641487122,0.7838550884225697
244244,488489,488488,976977,810.0101981163025,0.7809791884028527
245245,490491,490490,980981,813.3696401119232,0.7781244754769432
246246,492493,492492,984985,816.6929080486298,0.7752907159938331
247247,494495,494494,988989,819.999959230423,0.7724776797349477
248248,496497,496496,992993,823.3164310455322,0.7696851398723084
249249,498499,498498,996997,826.6246738433838,0.766912872903049
250250,500501,500500,1001001,829.9313428401947,0.7641606585639238
251251,502503,502502,1005005,833.2326738834381,0.7614282798076601
252252,504505,504504,1009009,836.5013918876648,0.7587155227156472
253253,506507,506506,1013013,839.7979819774628,0.7560221764597372
254254,508509,508508,1017017,843.1445560455322,0.7533480332222098
255255,510511,510510,1021021,846.4197859764099,0.7506928881757631
256256,512513,512512,1025025,849.7902119159698,0.7480565393962024
257257,514515,514514,1029029,853.1425409317017,0.7454387878351554
258258,516517,516516,1033033,856.4272630214691,0.7428394372509501
259259,518519,518518,1037037,859.718887090683,0.7402582941722358
260260,520521,520520,1041041,862.9994320869446,0.7376951678379555
261261,522523,522522,1045045,866.2624289989471,0.7351498701555101
262262,524525,524524,1049049,869.5451219081879,0.7326222156552831
263263,526527,526526,1053053,872.8391489982605,0.7301120214397088
264264,528529,528528,1057057,876.137423992157,0.727619107139617
265265,530531,530530,1061061,879.3808100223541,0.7251432948760339
266266,532533,532532,1065065,882.6922309398651,0.7226844092056126
267267,534535,534534,1069069,885.9509038925171,0.7202422770878911
268268,536537,536536,1073073,889.239394903183,0.7178167278489127
269269,538539,538538,1077077,892.5410759449005,0.7154075931230182
270270,540541,540540,1081081,895.8130419254303,0.71301470682738
271271,542543,542542,1085085,899.1141121387482,0.7106379051183467
272272,544545,544544,1089089,902.3746058940887,0.7082770263587008
273273,546547,546546,1093093,905.6782448291779,0.7059319534273527
274274,548549,548548,1097097,908.8927597999573,0.7036024911103596
275275,550551,550550,1101101,912.1759219169617,0.7012884793366538
276276,552553,552552,1105105,915.4459409713745,0.698989764910948
277277,554555,554554,1109109,918.7596490383148,0.6967061966679466
278278,556557,556556,1113113,922.0627160072327,0.6944376254268718
279279,558559,558558,1117117,925.3326869010925,0.6921839039696351
280280,560561,560560,1121121,928.6086821556091,0.689944887004458
281281,562563,562562,1125125,931.9109210968018,0.6877204311258538
282282,564565,564564,1129129,935.2593381404877,0.685510394801895
283283,566567,566566,1133133,938.5244538784027,0.6833146383214626
284284,568569,568568,1137137,941.7877020835876,0.6811330237869697
285285,570571,570570,1141141,945.2825191020966,0.6789654150634306
286286,572573,572572,1145145,948.6165959835052,0.6768116777693649
287287,574575,574574,1149149,951.8775579929352,0.6746716792385996
288288,576577,576576,1153153,955.1650719642639,0.6725452884893457
289289,578579,578578,1157157,958.4299039840698,0.6704323762041895
290290,580581,580580,1161161,961.7261579036713,0.6683328147100838
291291,582583,582582,1165165,965.0805780887604,0.666246477927416
292292,584585,584584,1169169,968.4569721221924,0.6641732413772843
293293,586587,586586,1173173,971.8021199703217,0.6621129821323848
294294,588589,588588,1177177,975.073310136795,0.6600657826620591
295295,590591,590590,1181181,978.3883719444275,0.6580316018898884
296296,592593,592592,1185185,981.678230047226,0.6560100369242718
297297,594595,594594,1189189,985.0679979324341,0.6540009703348915
298298,596597,596596,1193193,988.3392310142517,0.6520042863485287
299299,598599,598598,1197197,991.5850510597229,0.650019870732649
300300,600601,600600,1201201,994.9405248165131,0.6480476107299182
301301,602603,602602,1205205,998.1988508701324,0.646087395010909
302302,604605,604604,1209209,1001.4539439678192,0.6441391136231687
303303,606607,606606,1213213,1004.7140440940857,0.642202657963935
304304,608609,608608,1217217,1008.1826639175415,0.640277920763765
305305,610611,610610,1221221,1011.5717670917511,0.6383647960501548
306306,612613,612612,1225225,1014.8374290466309,0.6364631791238935
307307,614615,614614,1229229,1018.1456201076508,0.6345732934460102
308308,616617,616616,1233233,1021.3960800170898,0.6326948488494963
309309,618619,618618,1237237,1024.7827038764954,0.6308276036452298
310310,620621,620620,1241241,1028.056895017624,0.6289714574322716
311311,622623,622622,1245245,1031.3908469676971,0.6271263113558234
312312,624625,624624,1249249,1034.8128311634064,0.6252920678944065
313313,626627,626626,1253253,1038.0985870361328,0.6234686307343509
314314,628629,628628,1257257,1041.3853709697723,0.6216559047243209
315315,630631,630630,1261261,1044.6636848449707,0.6198537958462111
316316,632633,632632,1265265,1047.97096991539,0.6180622111733101
317317,634635,634634,1269269,1051.261761188507,0.6162810588775756
318318,636637,636636,1273273,1054.6512248516083,0.6145102481896174
319319,638639,638638,1277277,1057.9627878665924,0.6127496893896023
320320,640641,640640,1281281,1061.2546899318695,0.6109992937981588
321321,642643,642642,1285285,1064.5492079257965,0.6092589737509115
322322,644645,644644,1289289,1068.1564371585846,0.6075286425930244
323323,646647,646646,1293293,1071.4963538646698,0.6058082146591914
324324,648649,648648,1297297,1074.7999169826508,0.604097605260904
325325,650651,650650,1301301,1078.077208995819,0.6023967306682607
326326,652653,652652,1305305,1081.3415229320526,0.6007055081099679
327327,654655,654654,1309309,1084.6526579856873,0.5990238557405974
328328,656657,656656,1313313,1087.9153008460999,0.5973516926442244
329329,658659,658658,1317317,1091.299950838089,0.5956889388107811
330330,660661,660660,1321321,1094.6236701011658,0.5940355151287804
331331,662663,662662,1325325,1097.9460439682007,0.592391343365307
332332,664665,664664,1329329,1101.2601389884949,0.5907563461696554
333333,666667,666666,1333333,1104.4982709884644,0.5891304577180563
334334,668669,668668,1337337,1107.7899050712585,0.5875135967944516
335335,670671,670670,1341341,1111.0678339004517,0.5859056835888623
336336,672673,672672,1345345,1114.3810420036316,0.5843066441011615
337337,674675,674674,1349349,1117.7056760787964,0.5827164051297586
338338,676677,676676,1353353,1121.0055360794067,0.5811348942879704
339339,678679,678678,1357357,1124.2931849956512,0.5795620399767358
340340,680681,680680,1361361,1127.589278936386,0.5779977713809785
341341,682683,682682,1365365,1130.899069070816,0.5764420184568735
342342,684685,684684,1369369,1134.1866598129272,0.5748947119136574
343343,686687,686686,1373373,1137.47021818161,0.5733557832172664
344344,688689,688688,1377377,1140.806035041809,0.5718251645776036
345345,690691,690690,1381381,1144.07732796669,0.5703027889194345
346346,692693,692692,1385385,1147.3843281269073,0.5687885899005778
347347,694695,694694,1389389,1150.6597950458527,0.5672825018846197
348348,696697,696696,1393393,1153.9313960075378,0.5657844599336386
349349,698699,698698,1397397,1157.1908929347992,0.5642943998045666
350350,700701,700700,1401401,1160.4759078025818,0.5628122579328192
351351,702703,702702,1405405,1163.7382860183716,0.5613379714286566
352352,704705,704704,1409409,1167.0201721191406,0.5598714780680893
353353,706707,706706,1413413,1170.2929830551147,0.5584127162765071
354354,708709,708708,1417417,1173.5695040225983,0.5569616251377738
355355,710711,710710,1421421,1176.8560650348663,0.5555181443560286
356356,712713,712712,1425425,1180.1523458957672,0.5540822142829711
357357,714715,714714,1429429,1183.4239571094513,0.5526537758833001
358358,716717,716716,1433433,1186.732558965683,0.551232770729257
359359,718719,718718,1437437,1190.1017169952393,0.5498191410133586
360360,720721,720720,1441441,1193.528963804245,0.5484128295156552
361361,722723,722722,1445445,1196.8889071941376,0.5470137796073686
362362,724725,724724,1449449,1200.2176887989044,0.5456219352417975
363363,726727,726726,1453453,1203.5243520736694,0.5442372409506788
364364,728729,728728,1457457,1206.7876241207123,0.5428596418296365
365365,730731,730730,1461461,1210.09667801857,0.5414890835345432
366366,732733,732732,1465465,1213.3304419517517,0.5401255122760631
367367,734735,734734,1469469,1216.6955709457397,0.5387688748141954
368368,736737,736736,1473473,1220.0235381126404,0.5374191184400843
369369,738739,738738,1477477,1223.2705161571503,0.5360761909814755
370370,740741,740740,1481481,1226.5366051197052,0.534740040793622
371371,742743,742742,1485485,1229.7918980121613,0.5334106167465507
372372,744745,744744,1489489,1233.0772738456726,0.5320878682268813
373373,746747,746746,1493493,1236.3449440002441,0.5307717451250937
374374,748749,748748,1497497,1239.6407718658447,0.5294621978318901
375375,750751,750750,1501501,1242.9194629192352,0.5281591772290994
376376,752753,752752,1505505,1246.2100429534912,0.5268626346878591
377377,754755,754754,1509509,1249.4997961521149,0.5255725220667955
378378,756757,756756,1513513,1252.7248888015747,0.5242887916883774
379379,758759,758758,1517517,1256.0234298706055,0.5230113963534677
380380,760761,760760,1521521,1259.2814719676971,0.5217402893213148
381381,762763,762762,1525525,1262.572590827942,0.5204754243131902
382382,764765,764764,1529529,1265.8325610160828,0.5192167555014748
383383,766767,766766,1533533,1269.1327900886536,0.5179642375023832
384384,768769,768768,1537537,1272.3999121189117,0.516717825379601
385385,770771,770770,1541541,1275.6531009674072,0.5154774746297335
386386,772773,772772,1545545,1278.9608981609344,0.5142431411786674
387387,774775,774774,1549549,1282.2128238677979,0.5130147813797521
388388,776777,776776,1553553,1285.4765529632568,0.5117923520083423
389389,778779,778778,1557557,1288.7756690979004,0.5105758102545224
390390,780781,780780,1561561,1292.063244819641,0.5093651137176494
391391,782783,782782,1565565,1295.376363992691,0.5081602203990769
392392,784785,784784,1569569,1298.6666851043701,0.5069610887112503
393393,786787,786786,1573573,1302.0223441123962,0.5057676774504216
394394,788789,788788,1577577,1305.2824411392212,0.5045799458166584
395395,790791,790790,1581581,1308.5956370830536,0.5033978533847403
396396,792793,792792,1585585,1312.1432027816772,0.5022213601205294
397397,794795,794794,1589589,1315.562399148941,0.5010504263591429
398398,796797,796796,1593593,1318.8288269042969,0.4998850128158665
399399,798799,798798,1597597,1322.1407370567322,0.498725080573422
400400,800801,800800,1601601,1325.4324760437012,0.49757059107651
401401,802803,802802,1605605,1328.7596571445465,0.49642150613181
402402,804805,804804,1609609,1332.0393459796906,0.4952777879025234
403403,806807,806806,1613613,1335.3689720630646,0.4941393988992786
404404,808809,808808,1617617,1338.7363669872284,0.4930063019874069
405405,810811,810810,1621621,1342.0315778255463,0.4918784603705717
406406,812813,812812,1625625,1345.3218939304352,0.4907558375962253
407407,814815,814814,1629629,1348.6033430099487,0.4896383975410572
408408,816817,816816,1633633,1351.925036907196,0.4885261044200888
409409,818819,818818,1637637,1355.258022069931,0.4874189227775787
410410,820821,820820,1641641,1358.5484399795532,0.48631681747428956
411411,822823,822822,1645645,1361.8691289424896,0.4852197536984022
412412,824825,824824,1649649,1365.2151560783386,0.48412769695278257
413413,826827,826826,1653653,1368.546136856079,0.4830406130586198
414414,828829,828828,1657657,1371.8271760940552,0.4819584681354172
415415,830831,830830,1661661,1375.181401014328,0.48088122862100136
416416,832833,832832,1665665,1378.472242116928,0.479808861249694
417417,834835,834834,1669669,1381.7680740356445,0.4787413330577692
418418,836837,836836,1673673,1385.1020901203156,0.4776786113779963
419419,838839,838838,1677677,1388.3906269073486,0.4766206638341828
420420,840841,840840,1681681,1391.713989019394,0.47556745833753666
421421,842843,842842,1685685,1395.0151591300964,0.47451896309576114
422422,844845,844844,1689689,1398.3271489143372,0.47347514658395085
423423,846847,846846,1693693,1401.6547889709473,0.4724359775718767
424424,848849,848848,1697697,1404.9349598884583,0.4714014250985201
425425,850851,850850,1701701,1408.2370898723602,0.4703714584775298
426426,852853,852852,1705705,1411.543184041977,0.46934604729540297
427427,854855,854854,1709709,1414.8309562206268,0.4683251614042092
428428,856857,856856,1713713,1418.1490278244019,0.4673087709215906
429429,858859,858858,1717717,1421.4646151065826,0.46629684623076173
430430,860861,860860,1721721,1424.7360458374023,0.4652893579641386
431431,862863,862862,1725725,1428.0370419025421,0.46428627702698577
432432,864865,864864,1729729,1431.3225870132446,0.4632875745592173
433433,866867,866866,1733733,1434.6039791107178,0.46229322196450084
434434,868869,868868,1737737,1437.8653810024261,0.4613031908884295
435435,870871,870870,1741741,1441.1679780483246,0.4603174532276171
436436,872873,872872,1745745,1444.4654200077057,0.45933598111514584
437437,874875,874874,1749749,1447.8399949073792,0.4583587469296617
438438,876877,876876,1753753,1451.26629114151,0.4573857232808223
439439,878879,878878,1757757,1454.6199398040771,0.4564168830165727
440440,880881,880880,1761761,1457.926020860672,0.4554521992231457
441441,882883,882882,1765765,1461.1980209350586,0.4544916452068719
442442,884885,884884,1769769,1464.4963040351868,0.4535351945069124
443443,886887,886886,1773773,1467.7922158241272,0.452582820886164
444444,888889,888888,1777777,1471.1071639060974,0.4516344983330782
445445,890891,890890,1781781,1474.50084400177,0.4506902010507474
446446,892893,892892,1785785,1477.8856449127197,0.4497499034659995
447447,894895,894894,1789789,1481.173982143402,0.4488135802166653
448448,896897,896896,1793793,1484.467406988144,0.44788120616249216
449449,898899,898898,1797797,1487.78151512146,0.44695275635785947
450450,900901,900900,1801801,1491.098820924759,0.4460282060827012
451451,902903,902902,1805805,1494.4893219470978,0.4451075308206782
452452,904905,904904,1809809,1497.9173610210419,0.44419070625190216
453453,906907,906906,1813813,1501.4753530025482,0.44327770826748747
454454,908909,908908,1817817,1504.7931969165802,0.4423685129513615
455455,910911,910910,1821821,1508.062628030777,0.4414630965929973
456456,912913,912912,1825825,1511.3499989509583,0.44056143567649997
457457,914915,914914,1829829,1514.6561870574951,0.4396635068751493
458458,916917,916916,1833833,1517.930615901947,0.4387692870623141
459459,918919,918918,1837837,1521.2129528522491,0.437878753293262
460460,920921,920920,1841841,1524.4604160785675,0.43699188282153045
461461,922923,922922,1845845,1527.8166921138763,0.43610865307528
462462,924925,924924,1849849,1531.0856959819794,0.435229041679122
463463,926927,926926,1853853,1534.3834850788116,0.4343530264304718
464464,928929,928928,1857857,1537.7184238433838,0.4334805853122816
465465,930931,930930,1861861,1540.975214958191,0.4326116964875837
466466,932933,932932,1865865,1544.286880016327,0.4317463382903952
467467,934935,934934,1869869,1547.577880859375,0.43088448924027034
468468,936937,936936,1873873,1550.8253769874573,0.43002612802047224
469469,938939,938938,1877877,1554.1496210098267,0.4291712334888871
470470,940941,940940,1881881,1557.4290339946747,0.428319784678024
471471,942943,942942,1885885,1560.7145297527313,0.4274717607822822
472472,944945,944944,1889889,1563.984990119934,0.42662714116522693
473473,946947,946946,1893893,1567.280506849289,0.4257859053577704
474474,948949,948948,1897897,1570.7772459983826,0.4249480330545339
475475,950951,950950,1901901,1574.1513969898224,0.4241135041029338
476476,952953,952952,1905905,1577.5807518959045,0.42328229852137156
477477,954955,954954,1909909,1581.0066499710083,0.42245439648468164
478478,956957,956956,1913913,1584.3785939216614,0.42162977831685566
479479,958959,958958,1917917,1587.6629450321198,0.4208084245055943
480480,960961,960960,1921921,1590.9512050151825,0.41999031569139333
481481,962963,962962,1925925,1594.253121137619,0.41917543266572466
482482,964965,964964,1929929,1597.581001996994,0.4183637563710363
483483,966967,966966,1933933,1600.8572480678558,0.4175552678952954
484484,968969,968968,1937937,1604.1759040355682,0.41674994848290225
485485,970971,970970,1941941,1607.5175938606262,0.4159477795165003
486486,972973,972972,1945945,1610.819407939911,0.4151487425297091
487487,974975,974974,1949949,1614.1022589206696,0.4143528191943915
488488,976977,976976,1953953,1617.4484858512878,0.4135599913333863
489489,978979,978978,1957957,1620.782742023468,0.41277024089686165
490490,980981,980980,1961961,1624.1220359802246,0.41198364838601265
491491,982983,982982,1965965,1627.4005279541016,0.4112001088888064
492492,984985,984984,1969969,1630.6570200920105,0.41041959323047195
493493,986987,986986,1973973,1633.9365730285645,0.40964208389414125
494494,988989,988988,1977977,1637.229609966278,0.4088675635175605
495495,990991,990990,1981981,1640.4990510940552,0.408096014871262
496496,992993,992992,1985985,1643.806482076645,0.4073274208640214
497497,994995,994994,1989989,1647.0738561153412,0.4065617645301245
498498,996997,996996,1993993,1650.3430018424988,0.4057990290421003
499499,998999,998998,1997997,1653.6238539218903,0.4050391976888932
500501,1001003,1001002,2002005,1656.970232963562,0.40428149914805545
501502,1003005,1003004,2006009,1660.2373991012573,0.40352742932554975
502503,1005007,1005006,2010013,1663.4718978404999,0.40277621426503174
503504,1007009,1007008,2014017,1666.8958489894867,0.4020278377665818
504505,1009011,1009010,2018021,1670.4100408554077,0.40128228374305763
505506,1011013,1011012,2022025,1673.728754043579,0.4005395362364652
506507,1013015,1013014,2026029,1677.0145909786224,0.3997995794034068
507508,1015017,1015016,2030033,1680.276673078537,0.39906239752235706
508509,1017019,1017018,2034037,1683.6103110313416,0.39832797498638683
509510,1019021,1019020,2038041,1686.8711009025574,0.3975962963049824
510511,1021023,1021022,2042045,1690.162439107895,0.39686734610586427
511512,1023025,1023024,2046049,1693.5087850093842,0.3961411091295304
512513,1025027,1025026,2050053,1696.8600101470947,0.39541757023107493
513514,1027029,1027028,2054057,1700.1370341777802,0.3946967143747315
514515,1029031,1029030,2058061,1703.4135100841522,0.3939785266375111
515516,1031033,1031032,2062065,1706.731833934784,0.3932629922073829
516517,1033035,1033034,2066069,1710.0031387805939,0.3925500963778177
517518,1035037,1035036,2070073,1713.2992079257965,0.3918398245550634
518519,1037039,1037038,2074077,1716.5879318714142,0.39113216225268843
519520,1039041,1039040,2078081,1719.8648209571838,0.3904270950843056
520521,1041043,1041042,2082085,1723.1468408107758,0.3897246087763051
521522,1043045,1043044,2086089,1726.4437971115112,0.38902468915148347
522523,1045047,1045046,2090093,1729.7412509918213,0.3883273221417767
523524,1047049,1047048,2094097,1732.9976468086243,0.3876324937791651
524525,1049051,1049050,2098101,1736.2815771102905,0.38694019020113046
525526,1051053,1051052,2102105,1739.5826539993286,0.386250397637923
526527,1053055,1053054,2106109,1742.8602890968323,0.38556310242529435
527528,1055057,1055056,2110113,1746.164234161377,0.3848782909954025
528529,1057059,1057058,2114117,1749.4030239582062,0.38419594987499295
529530,1059061,1059060,2118121,1752.7074120044708,0.3835160656963126
530531,1061063,1061062,2122125,1755.9678449630737,0.38283862518073875
531532,1063065,1063064,2126129,1759.2487378120422,0.38216361514605524
532533,1065067,1065066,2130133,1762.5306839942932,0.3814910225046333
533534,1067069,1067068,2134137,1765.778797864914,0.3808208342652506
534535,1069071,1069070,2138141,1769.0447881221771,0.38015303752217733
535536,1071073,1071072,2142145,1772.301841020584,0.3794876194697281
536537,1073075,1073074,2146149,1775.5975539684296,0.37882456738771
537538,1075077,1075076,2150153,1778.8684220314026,0.37816386864869855
538539,1077079,1077078,2154157,1782.165342092514,0.37750551071621885
539540,1079081,1079080,2158161,1785.4093539714813,0.3768494811356504
540541,1081083,1081082,2162165,1788.7299201488495,0.37619576754696027
541542,1083085,1083084,2166169,1792.0359539985657,0.3755443576756079
542543,1085087,1085086,2170173,1795.3011310100555,0.3748952393307263
543544,1087089,1087088,2174177,1798.6221981048584,0.37424840040876006
544545,1089091,1089090,2178181,1801.8823239803314,0.3736038288916461
545546,1091093,1091092,2182185,1805.315880060196,0.372961512844995
546547,1093095,1093094,2186189,1808.6755018234253,0.3723214404180908
547548,1095097,1095096,2190193,1811.939637184143,0.37168359984571
548549,1097099,1097098,2194197,1815.256551027298,0.3710479794317507
549550,1099101,1099100,2198201,1818.5206730365753,0.3704145675783366
550551,1101103,1101102,2202205,1821.832909822464,0.3697833527567127
551552,1103105,1103104,2206209,1825.2071161270142,0.3691543235217978
552553,1105107,1105106,2210213,1828.4535508155823,0.368527468510365
553554,1107109,1107108,2214217,1831.7700581550598,0.36790277643012814
554555,1109111,1109110,2218221,1835.102795124054,0.3672802360724745
555556,1111113,1111112,2222225,1838.3737711906433,0.36665983630700794
556557,1113115,1113114,2226229,1841.6521670818329,0.36604156607063487
557558,1115117,1115116,2230233,1844.9536101818085,0.36542541438939224
558559,1117119,1117118,2234237,1848.2653000354767,0.3648113703529816
559560,1119121,1119120,2238241,1851.7224099636078,0.36419942313295905
560561,1121123,1121122,2242245,1855.1653761863708,0.36358956197000225
561562,1123125,1123124,2246249,1858.4269080162048,0.36298177617936744
562563,1125127,1125126,2250253,1861.739557981491,0.3623760551454325
563564,1127129,1127128,2254257,1865.0956399440765,0.3617723883344297
564565,1129131,1129130,2258261,1868.4067521095276,0.36117076527625613
565566,1131133,1131132,2262265,1871.7554697990417,0.36057117557174934
566567,1133135,1133134,2266269,1875.0627768039703,0.35997360889450647
567568,1135137,1135136,2270273,1878.550908088684,0.3593780549854273
568569,1137139,1137138,2274277,1881.8516309261322,0.35878450365817116
569570,1139141,1139140,2278281,1885.1641600131989,0.35819294478642405
570571,1141143,1141142,2282285,1888.491447210312,0.3576033683257265
571572,1143145,1143144,2286289,1891.7264499664307,0.3570157642807317
572573,1145147,1145146,2290293,1895.077800989151,0.3564301227397664
573574,1147149,1147148,2294297,1898.3563060760498,0.355846433847546
574575,1149151,1149150,2298301,1901.6166081428528,0.35526468781790754
575576,1151153,1151152,2302305,1904.892233133316,0.35468487492653367
576577,1153155,1153154,2306309,1908.1709699630737,0.3541069855200476
577578,1155157,1155156,2310313,1911.5322089195251,0.35353101000146125
578579,1157159,1157158,2314317,1914.836716890335,0.35295693884108914
579580,1159161,1159160,2318321,1918.1146461963654,0.3523847625747294
580581,1161163,1161162,2322325,1921.4078710079193,0.35181447179093084
581582,1163165,1163164,2326329,1924.7044949531555,0.35124605715645885
582583,1165167,1165166,2330333,1928.006511926651,0.35067950938173453
583584,1167169,1167168,2334337,1931.2734589576721,0.35011481925357657
584585,1169171,1169170,2338341,1934.624027967453,0.3495519776024594
585586,1171173,1171172,2342345,1937.8694689273834,0.3489909753370739
586587,1173175,1173174,2346349,1941.1563091278076,0.34843180341158586
587588,1175177,1175176,2350353,1944.433249950409,0.34787445284564456
588589,1177179,1177178,2354357,1947.7365939617157,0.34731891471710696
589590,1179181,1179180,2358361,1950.9982089996338,0.34676518015658075
590591,1181183,1181182,2362365,1954.2984659671783,0.3462132403619762
591592,1183185,1183184,2366369,1957.6311709880829,0.3456630865784973
592593,1185187,1185186,2370373,1960.8885679244995,0.3451147101131937
593594,1187189,1187188,2374377,1964.1660299301147,0.34456810232950374
594595,1189191,1189190,2378381,1967.4036581516266,0.3440232546399784
595596,1191193,1191192,2382385,1970.795692205429,0.34348015852265235
596597,1193195,1193194,2386389,1974.2411751747131,0.34293880550285394
597598,1195197,1195196,2390393,1977.5241680145264,0.3423991871641192
598599,1197199,1197198,2394397,1980.7874729633331,0.3418612951390969
599600,1199201,1199200,2398401,1984.0923669338226,0.3413251211204624
600601,1201203,1201202,2402405,1987.3215928077698,0.34079065685182286
601602,1203205,1203204,2406409,1990.6322240829468,0.34025789412407903
602603,1205207,1205206,2410413,1993.9730219841003,0.33972682478452043
603604,1207209,1207208,2414417,1997.2353138923645,0.3391974407386442
604605,1209211,1209210,2418421,2000.5061919689178,0.33866973392832733
605606,1211213,1211212,2422425,2003.7420060634613,0.3381436963645683
606607,1213215,1213214,2426429,2007.0293459892273,0.3376193200892885
607608,1215217,1215216,2430433,2010.3082389831543,0.3370965972135309
608609,1217219,1217218,2434437,2013.6408910751343,0.33657551988471823
609610,1219221,1219220,2438441,2016.9168620109558,0.3360560803066619
610611,1221223,1221222,2442445,2020.181156873703,0.33553827072864806
611612,1223225,1223224,2446449,2023.4669630527496,0.33502208345089457
612613,1225227,1225226,2450453,2026.7258250713348,0.334507510819094
613614,1227229,1227228,2454457,2030.0121281147003,0.3339945452316897
614615,1229231,1229230,2458461,2033.2877221107483,0.33348317912714265
615616,1231233,1231232,2462465,2036.544970035553,0.3329734050003026
616617,1233235,1233234,2466469,2039.7966830730438,0.332465215386037
617618,1235237,1235236,2470473,2043.0928900241852,0.33195860286650714
618619,1237239,1237238,2474477,2046.3745670318604,0.3314535600729869
619620,1239241,1239240,2478481,2049.627187013626,0.3309500796785869
620621,1241243,1241242,2482485,2052.8880331516266,0.33044815440371167
621622,1243245,1243244,2486489,2056.1825659275055,0.32994777701787825
622623,1245247,1245246,2490493,2059.4481320381165,0.3294489403251646
623624,1247249,1247248,2494497,2062.7127480506897,0.32895163718421827
624625,1249251,1249250,2498501,2065.984852075577,0.3284558604900667
625626,1251253,1251252,2502505,2069.26845908165,0.32796160318684997
626627,1253255,1253254,2506509,2072.5665209293365,0.32746885825690697
627628,1255257,1255256,2510513,2075.8380270004272,0.3269776187335083
628629,1257259,1257258,2514517,2079.0971081256866,0.3264878776844853
629630,1259261,1259260,2518521,2082.3690991401672,0.3259996282249631
630631,1261263,1261262,2522525,2085.628154039383,0.3255128635064466
631632,1263265,1263264,2526529,2088.8884329795837,0.32502757672409643
632633,1265267,1265266,2530533,2092.1679549217224,0.32454376112582395
633634,1267269,1267268,2534537,2095.4226450920105,0.32406140997954935
634635,1269271,1269270,2538541,2098.7055299282074,0.3235805166168575
635636,1271273,1271272,2542545,2101.9123759269714,0.3231010743857041
636637,1273275,1273274,2546549,2105.2184870243073,0.32262307669589063
637638,1275277,1275276,2550553,2108.447530031204,0.32214651698450325
638639,1277279,1277278,2554557,2111.986167192459,0.32167138873046497
639640,1279281,1279280,2558561,2115.4592010974884,0.32119768545453553
640641,1281283,1281282,2562565,2118.6824321746826,0.32072540071749245
641642,1283285,1283284,2566569,2121.9435851573944,0.32025452810921706
642643,1285287,1285286,2570573,2125.2157049179077,0.31978506126870343
643644,1287289,1287288,2574577,2128.5158360004425,0.3193169938695064
644645,1289291,1289290,2578581,2131.7717509269714,0.31885031962156063
645646,1291293,1291292,2582585,2135.050948858261,0.3183850322729995
646647,1293295,1293294,2586589,2138.4400510787964,0.31792112561379327
647648,1295297,1295296,2590593,2141.724233150482,0.3174585934593779
648649,1297299,1297298,2594597,2145.0112500190735,0.3169974296761211
649650,1299301,1299300,2598601,2148.3021631240845,0.3165376281558565
650651,1301303,1301302,2602605,2151.5755620002747,0.31607918282861647
651652,1303305,1303304,2606609,2154.846652984619,0.3156220876680891
652653,1305307,1305306,2610613,2158.079924106598,0.3151663366734283
653654,1307309,1307308,2614617,2161.419888973236,0.3147119238819869
654655,1309311,1309310,2618621,2164.700478076935,0.3142588433711353
655656,1311313,1311312,2622625,2167.9830269813538,0.3138070892491669
656657,1313315,1313314,2626629,2171.2604508399963,0.3133566556571168
657658,1315317,1315316,2630633,2174.523545026779,0.3129075367742189
658659,1317319,1317318,2634637,2177.7969160079956,0.3124597268142679
659660,1319321,1319320,2638641,2181.0273830890656,0.31201322001652443
660661,1321323,1321322,2642645,2184.30274105072,0.3115680106657237
661662,1323325,1323324,2646649,2187.52970290184,0.3111240930720669
662663,1325327,1325326,2650653,2190.8254721164703,0.31068146158213494
663664,1327329,1327328,2654657,2194.10595703125,0.3102401105734316
664665,1329331,1329330,2658661,2197.3752360343933,0.3098000344562024
665666,1331333,1331332,2662665,2200.6729130744934,0.30936122767707275
666667,1333335,1333334,2666669,2203.949064016342,0.3089236847099528
667668,1335337,1335336,2670673,2207.2597880363464,0.3084874000578566
668669,1337339,1337338,2674677,2210.5166800022125,0.30805236826745386
669670,1339341,1339340,2678681,2213.8000688552856,0.3076185839054233
670671,1341343,1341342,2682685,2217.1622920036316,0.30718604157300433
671672,1343345,1343344,2686689,2220.5594120025635,0.30675473590417823
672673,1345347,1345346,2690693,2223.8801729679108,0.3063246615638491
673674,1347349,1347348,2694697,2227.1791911125183,0.3058958132423868
674675,1349351,1349350,2698701,2230.7408521175385,0.3054681856701791
675676,1351353,1351352,2702705,2234.091798067093,0.3050417735976225
676677,1353355,1353354,2706709,2237.340656042099,0.3046165718133125
677678,1355357,1355356,2710713,2240.6020390987396,0.30419257512767217
678679,1357359,1357358,2714717,2243.842849969864,0.30376977838568564
679680,1359361,1359360,2718721,2247.107396841049,0.30334817646325973
680681,1361363,1361362,2722725,2250.401249885559,0.30292776425994816
681682,1363365,1363364,2726729,2253.9253420829773,0.30250853670622746
682683,1365367,1365366,2730733,2257.397234916687,0.302090488763497
683684,1367369,1367368,2734737,2260.6762640476227,0.3016736154222599
684685,1369371,1369370,2738741,2263.9469311237335,0.3012579116948473
685686,1371373,1371372,2742745,2267.215760946274,0.30084337263178895
686687,1373375,1373374,2746749,2270.5279891490936,0.30042999330180464
687688,1375377,1375376,2750753,2273.9872760772705,0.3000177688045369
688689,1377379,1377378,2754757,2277.350861787796,0.2996066942669131
689690,1379381,1379380,2758761,2280.6216430664062,0.29919676485042146
690691,1381383,1381382,2762765,2283.932062149048,0.29878797573110205
691692,1383385,1383384,2766769,2287.253452062607,0.29838032212319376
692693,1385387,1385386,2770773,2290.5718290805817,0.2979737992554874
693694,1387389,1387388,2774777,2293.8365919589996,0.29756840299160103
694695,1389391,1389390,2778781,2297.219447851181,0.29716412939160364
695696,1391393,1391392,2782785,2300.464823961258,0.2967609726747469
696697,1393395,1393394,2786789,2303.7656950950623,0.29635892798432906
697698,1395397,1395396,2790793,2307.010807991028,0.29595799063645245
698699,1397399,1397398,2794797,2310.314491033554,0.295558156007246
699700,1399401,1399400,2798801,2313.660129070282,0.29515941950558044
700701,1401403,1401402,2802805,2316.944627046585,0.29476177657488734
701702,1403405,1403404,2806809,2320.2303869724274,0.2943652226767881
702703,1405407,1405406,2810813,2323.5191571712494,0.293969753305646
703704,1407409,1407408,2814817,2326.818810939789,0.2935753639831091
704705,1409411,1409410,2818821,2330.1714367866516,0.29318205024719646
705706,1411413,1411412,2822825,2333.5005888938904,0.2927898076650308
706707,1413415,1413414,2826829,2336.7860198020935,0.2923986318310199
707708,1415417,1415416,2830833,2340.057065010071,0.2920085183595802
708709,1417419,1417418,2834837,2343.338068008423,0.29161946288877516
709710,1419421,1419420,2838841,2346.610072851181,0.291231461085772
710711,1421423,1421422,2842845,2349.8764889240265,0.29084450863228994
711712,1423425,1423424,2846849,2353.154340028763,0.2904586012427899
712713,1425427,1425426,2850853,2356.4235711097717,0.2900737346517417
713714,1427429,1427428,2854857,2359.69206905365,0.2896899046118051
714715,1429431,1429430,2858861,2362.9416449069977,0.2893071069065627
715716,1431433,1431432,2862865,2366.233868122101,0.2889253373396059
716717,1433435,1433434,2866869,2369.505882024765,0.2885445917308971
717718,1435437,1435436,2870873,2373.061560869217,0.2881648659331404
718719,1437439,1437438,2874877,2376.457388162613,0.2877861558172299
719720,1439441,1439440,2878881,2379.7345130443573,0.2874084572758875
720721,1441443,1441442,2882885,2383.021094083786,0.287031766221844
721722,1443445,1443444,2886889,2386.4217879772186,0.2866560785932961
722723,1445447,1445446,2890893,2389.734097957611,0.28628139034663036
723724,1447449,1447448,2894897,2393.0426268577576,0.28590769746369915
724725,1449451,1449450,2898901,2396.4944038391113,0.2855349959445448
725726,1451453,1451452,2902905,2399.7927329540253,0.28516328181467543
726727,1453455,1453454,2906909,2403.088795900345,0.2847925511159701
727728,1455457,1455456,2910913,2406.2962651252747,0.2844227999157738
728729,1457459,1457458,2914917,2409.4754781723022,0.28405402429962123
729730,1459461,1459460,2918921,2412.6737570762634,0.2836862203748751
730731,1461463,1461462,2922925,2415.907392024994,0.283319384267088
731732,1463465,1463464,2926929,2419.1125090122223,0.2829535121272784
732733,1465467,1465466,2930933,2422.3320169448853,0.2825886001246545
733734,1467469,1467468,2934937,2425.5419311523438,0.28222464444479556
734735,1469471,1469470,2938941,2428.802092075348,0.2818616412969277
735736,1471473,1471472,2942945,2431.9710059165955,0.28149958691392385
736737,1473475,1473474,2946949,2435.219055891037,0.2811384775395709
737738,1475477,1475476,2950953,2438.8001589775085,0.2807783094467595
738739,1477479,1477478,2954957,2442.5116250514984,0.2804190789211134
739740,1479481,1479480,2958961,2445.8218429088593,0.280060782273722
740741,1481483,1481482,2962965,2449.1774921417236,0.27970341582658875
741742,1483485,1483484,2966969,2452.7440049648285,0.27934697592900193
742743,1485487,1485486,2970973,2456.315383911133,0.2789914589448017
743744,1487489,1487488,2974977,2459.6964869499207,0.2786368612632941
744745,1489491,1489490,2978981,2462.985577106476,0.2782831792792422
745746,1491493,1491492,2982985,2466.3845789432526,0.27793040942196967
746747,1493495,1493494,2986989,2469.7966301441193,0.2775785481262574
747748,1495497,1495496,2990993,2473.243639230728,0.2772275918559899
748749,1497499,1497498,2994997,2476.7831530570984,0.27687753708596574
749750,1499501,1499500,2999001,2480.2710201740265,0.27652838031099236
750751,1501503,1501502,3003005,2483.717260122299,0.27618011804770504
751752,1503505,1503504,3007009,2487.124382019043,0.275832746825472
752753,1505507,1505506,3011013,2490.4684171676636,0.2754862631936703
753754,1507509,1507508,3015017,2493.9391651153564,0.275140663721686
754755,1509511,1509510,3019021,2497.405412912369,0.27479594499163795
755756,1511513,1511512,3023025,2500.862226963043,0.27445210360929195
756757,1513515,1513514,3027029,2504.3584349155426,0.2741091361949657
757758,1515517,1515516,3031033,2507.7956659793854,0.27376703938534774
758759,1517519,1517518,3035037,2511.160124063492,0.2734258098334976
759760,1519521,1519520,3039041,2514.617882013321,0.2730854442124837
760761,1521523,1521522,3043045,2518.031502008438,0.2727459392099263
761762,1523525,1523524,3047049,2521.4637389183044,0.27240729153345455
762763,1525527,1525526,3051053,2524.894127845764,0.2720694979052496
763764,1527529,1527528,3055057,2528.3734369277954,0.2717325550656824
764765,1529531,1529530,3059061,2531.881576061249,0.2713964597642189
765766,1531533,1531532,3063065,2535.3336839675903,0.27106120878124784
766767,1533535,1533534,3067069,2538.7821300029755,0.270726798900796
767768,1535537,1535536,3071073,2542.224748849869,0.2703932269287179
768769,1537539,1537538,3075077,2545.6595549583435,0.2700604896836012
769770,1539541,1539540,3079081,2549.073093891144,0.2697285840076802
770771,1541543,1541542,3083085,2552.5134239196777,0.26939750675046525
771772,1543545,1543544,3087089,2556.126156806946,0.26906725478147564
772773,1545547,1545546,3091093,2559.6398758888245,0.2687378249847825
773774,1547549,1547548,3095097,2563.0575590133667,0.26840921426446585
774775,1549551,1549550,3099101,2566.514638900757,0.2680814195318817
775776,1551553,1551552,3103105,2569.9122610092163,0.2677544377202139
776777,1553555,1553554,3107109,2573.353273868561,0.26742826577537926
777778,1555557,1555556,3111113,2576.7634150981903,0.26710290065966547
778779,1557559,1557558,3115117,2580.1852581501007,0.2667783393535501
779780,1559561,1559560,3119121,2583.6028230190277,0.26645457884296775
780781,1561563,1561562,3123125,2586.9680919647217,0.2661316161429568
781782,1563565,1563564,3127129,2590.3084077835083,0.26580944826855557
782783,1565567,1565566,3131133,2593.697254896164,0.26548807226208737
783784,1567569,1567568,3135137,2597.12259888649,0.2651674851713324
784785,1569571,1569570,3139141,2600.5763380527496,0.26484768406589865
785786,1571573,1571572,3143145,2604.0331978797913,0.2645286660244892
786787,1573575,1573574,3147149,2607.459276199341,0.264210428142178
787788,1575577,1575576,3151153,2610.876424074173,0.2638929675304098
788789,1577579,1577578,3155157,2614.3600730895996,0.2635762813133624
789790,1579581,1579580,3159161,2617.8066890239716,0.2632603666279465
790791,1581583,1581582,3163165,2621.2701358795166,0.26294522062562464
791792,1583585,1583584,3167169,2624.726408958435,0.26263084047604934
792793,1585587,1585586,3171173,2628.1672310829163,0.26231722335614904
793794,1587589,1587588,3175177,2631.624083995819,0.2620043664592231
794795,1589591,1589590,3179181,2635.0928070545197,0.26169226699676074
795796,1591593,1591592,3183185,2638.5184211730957,0.26138092219116515
796797,1593595,1593594,3187189,2641.9872200489044,0.2610703292702965
797798,1595597,1595596,3191193,2645.440707921982,0.26076048548929975
798799,1597599,1597598,3195197,2648.956475019455,0.2604513881069579
799800,1599601,1599600,3199201,2652.525983095169,0.26014303440206277
800801,1601603,1601602,3203205,2656.038185119629,0.2598354216588632
801802,1603605,1603604,3207209,2659.4779291152954,0.2595285471834359
802803,1605607,1605606,3211213,2662.9558658599854,0.2592224082854955
803804,1607609,1607608,3215217,2666.4823150634766,0.25891700229658454
804805,1609611,1609610,3219221,2669.957128047943,0.25861232655734057
805806,1611613,1611612,3223225,2673.5765368938446,0.25830837842113397
806807,1613615,1613614,3227229,2677.0332429409027,0.2580051552540681
807808,1615617,1615616,3231233,2680.4905030727386,0.2577026544349792
808809,1617619,1617618,3235237,2683.947464942932,0.2574008733572555
809810,1619621,1619620,3239241,2687.3736641407013,0.25709980942519906
810811,1621623,1621622,3243245,2690.8136038780212,0.256799460055845
811812,1623625,1623624,3247249,2694.2427458763123,0.25649982267532323
812813,1625627,1625626,3251253,2697.6971690654755,0.2562008947297727
813814,1627629,1627628,3255257,2701.131061077118,0.25590267366897024
814815,1629631,1629630,3259261,2704.549940109253,0.2556051569627016
815816,1631633,1631632,3263265,2708.065313100815,0.25530834208620945
816817,1633635,1633634,3267269,2711.4464950561523,0.25501222653110744
817818,1635637,1635636,3271273,2714.924288034439,0.2547168077999231
818819,1637639,1637638,3275277,2718.377935886383,0.25442208340791694
819820,1639641,1639640,3279281,2721.7951471805573,0.25412805087762536
820821,1641643,1641642,3283285,2725.221936941147,0.2538347077497747
821822,1643645,1643644,3287289,2728.584846019745,0.2535420515760052
822823,1645647,1645646,3291293,2732.1771750450134,0.2532500799097761
823824,1647649,1647648,3295297,2736.7276759147644,0.25295879033001256
824825,1649651,1649650,3299301,2740.8574678897858,0.25266818041745864
825826,1651653,1651652,3303305,2744.41517496109,0.2523782477728673
826827,1653655,1653654,3307309,2747.7884590625763,0.2520889899988106
827828,1655657,1655656,3311313,2751.6885759830475,0.2518004047124123
828829,1657659,1657658,3315317,2755.1227390766144,0.2515124895471672
829830,1659661,1659660,3319321,2758.7074661254883,0.25122524213838915
830831,1661663,1661662,3323325,2762.0647189617157,0.25093866014321975
831832,1663665,1663664,3327329,2765.345705986023,0.25065274121880066
832833,1665667,1665666,3331333,2768.7592520713806,0.2503674830441014
833834,1667669,1667668,3335337,2772.048662185669,0.25008288330172945
834835,1669671,1669670,3339341,2775.2867469787598,0.24979893968520628
835836,1671673,1671672,3343345,2778.4956040382385,0.24951564990078623
836837,1673675,1673674,3347349,2781.6973400115967,0.24923301166927558
837838,1675677,1675676,3351353,2784.895306110382,0.2489510227151186
838839,1677679,1677678,3355357,2788.5442152023315,0.24866968077913043
839840,1679681,1679680,3359361,2791.7896630764008,0.24838898360212625
840841,1681683,1681682,3363365,2795.051162004471,0.24810892895038705
841842,1683685,1683684,3367369,2798.5029530525208,0.24782951459383185
842843,1685687,1685686,3371373,2801.9423592090607,0.2475507383060176
843844,1687689,1687688,3375377,2805.277256965637,0.24727259788414813
844845,1689691,1689690,3379381,2808.5828869342804,0.24699509112542728
845846,1691693,1691692,3383385,2811.9412710666656,0.24671821583797282
846847,1693695,1693694,3387389,2815.304136991501,0.2464419698480924
847848,1695697,1695696,3391393,2818.6467900276184,0.24616635097845574
848849,1697699,1697698,3395397,2821.9730298519135,0.24589135707901733
849850,1699701,1699700,3399401,2825.3482599258423,0.24561698599063675
850851,1701703,1701702,3403405,2828.7054789066315,0.24534323557963944
851852,1703705,1703704,3407409,2832.0701670646667,0.2450701037178078
852853,1705707,1705706,3411413,2835.4206280708313,0.2447975882787432
853854,1707709,1707708,3415417,2838.7724220752716,0.24452568715969392
854855,1709711,1709710,3419421,2842.1449270248413,0.2442543982542702
855856,1711713,1711712,3423425,2845.5071029663086,0.24398371947427222
856857,1713715,1713714,3427429,2848.867033958435,0.24371364873513812
857858,1715717,1715716,3431433,2852.255541086197,0.24344418397049594
858859,1717719,1717718,3435437,2855.636610031128,0.24317532311215473
859860,1719721,1719720,3439441,2859.119554042816,0.24290706410829443
860861,1721723,1721722,3443445,2862.518436908722,0.24263940491800895
861862,1723725,1723724,3447449,2865.9016761779785,0.24237234350221115
862863,1725727,1725726,3451453,2869.3265209198,0.24210587783818482
863864,1727729,1727728,3455457,2872.7009041309357,0.2418400059123087
864865,1729731,1729730,3459461,2876.109340906143,0.2415747257109615
865866,1731733,1731732,3463465,2879.472095012665,0.24131003524053085
866867,1733735,1733734,3467469,2882.8737511634827,0.24104593251286133
867868,1735737,1735736,3471473,2886.2600989341736,0.24078241554525448
868869,1737739,1737738,3475477,2889.6218869686127,0.24051948236774479
869870,1739741,1739740,3479481,2893.1398050785065,0.24025713101946167
870871,1741743,1741742,3483485,2896.6309971809387,0.23999535954317253
871872,1743745,1743744,3487489,2899.9751360416412,0.23973416599619668
872873,1745747,1745746,3491493,2903.351081132889,0.23947354844676738
873874,1747749,1747748,3495497,2906.7461519241333,0.2392135049612989
874875,1749751,1749750,3499501,2910.0903520584106,0.23895403362439538
875876,1751753,1751752,3503505,2913.514666080475,0.23869513252429897
876877,1753755,1753754,3507509,2916.870234966278,0.23843679976198473
877878,1755757,1755756,3511513,2920.2173278331757,0.2381790334420657
878879,1757759,1757758,3515517,2923.5965299606323,0.23792183168188785
879880,1759761,1759760,3519521,2926.970386981964,0.23766519260061614
880881,1761763,1761762,3523525,2930.492058992386,0.2374091143356054
881882,1763765,1763764,3527529,2934.0336468219757,0.2371535950260295
882883,1765767,1765766,3531533,2937.4193308353424,0.2368986328219762
883884,1767769,1767768,3535537,2940.776755094528,0.23664422587535228
884885,1769771,1769770,3539541,2944.1778151988983,0.23639037235443539
885886,1771773,1771772,3543545,2947.512226819992,0.23613707043114118
886887,1773775,1773774,3547549,2950.9002890586853,0.23588431828829926
887888,1775777,1775776,3551553,2954.248444080353,0.23563211411783413
888889,1777779,1777778,3555557,2957.7537689208984,0.23538045610803238
889890,1779781,1779780,3559561,2961.2255828380585,0.23512934247264639
890891,1781783,1781782,3563565,2964.601397037506,0.2348787714181526
891892,1783785,1783784,3567569,2967.9865159988403,0.2346287411692174
892893,1785787,1785786,3571573,2971.366229057312,0.23437924995596404
893894,1787789,1787788,3575577,2974.763421058655,0.23413029601215385
894895,1789791,1789790,3579581,2978.139976978302,0.23388187758246204
895896,1791793,1791792,3583585,2981.473958969116,0.2336339929188398
896897,1793795,1793794,3587589,2984.867394924164,0.23338664027869527
897898,1795797,1795796,3591593,2988.3475658893585,0.23313981793216954
898899,1797799,1797798,3595597,2991.8769450187683,0.23289352415304165
899900,1799801,1799800,3599601,2995.272336959839,0.23264775722236664
900901,1801803,1801802,3603605,2998.6482660770416,0.23240251543211343
901902,1803805,1803804,3607609,3002.029134988785,0.23215779707606998
902903,1805807,1805806,3611613,3005.4292809963226,0.23191360046075715
903904,1807809,1807808,3615617,3008.8109929561615,0.2316699238945148
904905,1809811,1809810,3619621,3012.179976940155,0.23142676570023468
905906,1811813,1811812,3623625,3015.545902967453,0.23118412420444656
906907,1813815,1813814,3627629,3018.9031801223755,0.23094199774095614
907908,1815817,1815816,3631633,3022.3222150802612,0.2307003846453881
908909,1817819,1817818,3635637,3025.6988549232483,0.23045928327155707
909910,1819821,1819820,3639641,3029.052722930908,0.2302186919732776
910911,1821823,1821822,3643645,3032.4138708114624,0.22997860910982126
911912,1823825,1823824,3647649,3035.808445930481,0.22973903305319254
912913,1825827,1825826,3651653,3039.1714210510254,0.2294999621790339
913914,1827829,1827828,3655657,3042.771243095398,0.22926139487026376
914915,1829831,1829830,3659661,3046.2581839561462,0.2290233295134385
915916,1831833,1831832,3663665,3049.595854997635,0.22878576451148547
916917,1833835,1833834,3667669,3053.0297989845276,0.22854869826369395
917918,1835837,1835836,3671673,3056.4009160995483,0.2283121291857242
918919,1837839,1837838,3675677,3059.768310070038,0.22807605568777944
919920,1839841,1839840,3679681,3063.2395548820496,0.22784047620007186
920921,1841843,1841842,3683685,3066.646488904953,0.2276053891509946
921922,1843845,1843844,3687689,3070.0205330848694,0.22737079297621676
922923,1845847,1845846,3691693,3073.3919591903687,0.22713668612595939
923924,1847849,1847848,3695697,3076.7440769672394,0.22690306704680552
924925,1849851,1849850,3699701,3080.0957651138306,0.22666993419261416
925926,1851853,1851852,3703705,3083.452296972275,0.22643728603179625
926927,1853855,1853854,3707709,3086.8584809303284,0.22620512103821966
927928,1855857,1855856,3711713,3090.2506980895996,0.22597343768029532
928929,1857859,1857858,3715717,3093.6555531024933,0.22574223444644304
929930,1859861,1859860,3719721,3097.0327620506287,0.2255115098250826
930931,1861863,1861862,3723725,3100.6893751621246,0.2252812623155478
931932,1863865,1863864,3727729,3104.227262020111,0.22505149041535333
932933,1865867,1865866,3731733,3107.5995841026306,0.2248221926329279
933934,1867869,1867868,3735737,3110.9644770622253,0.22459336748761416
934935,1869871,1869870,3739741,3114.346028804779,0.22436501349693572
935936,1871873,1871872,3743745,3117.7614319324493,0.22413712918933015
936937,1873875,1873874,3747749,3121.141902923584,0.223909713100511
937938,1875877,1875876,3751753,3124.5246200561523,0.22368276376801077
938939,1877879,1877878,3755757,3127.977847099304,0.22345627973663795
939940,1879881,1879880,3759761,3131.485990047455,0.22323025956029596
940941,1881883,1881882,3763765,3134.9101469516754,0.2230047017965262
941942,1883885,1883884,3767769,3138.3042390346527,0.22277960500650806
942943,1885887,1885886,3771773,3141.6707680225372,0.22255496776233485
943944,1887889,1887888,3775777,3145.044795036316,0.22233078864155686
944945,1889891,1889890,3779781,3148.501277923584,0.22210706622172438
945946,1891893,1891892,3783785,3151.832813978195,0.2218837990967586
946947,1893895,1893894,3787789,3155.31289601326,0.22166098585148575
947948,1895897,1895896,3791793,3158.715129852295,0.22143862509255996
948949,1897899,1897898,3795797,3162.088783979416,0.22121671542117838
949950,1899901,1899900,3799801,3165.473489046097,0.2209952554494521
950951,1901903,1901902,3803805,3168.9777669906616,0.22077424379494914
951952,1903905,1903904,3807809,3172.542151927948,0.22055367907705659
952953,1905907,1905906,3811813,3176.104173898697,0.22033355992789438
953954,1907909,1907908,3815817,3179.6442019939423,0.22011388497594453
954955,1909911,1909910,3819821,3183.250837087631,0.21989465286605991
955956,1911913,1911912,3823825,3186.7790229320526,0.21967586223763647
956957,1913915,1913914,3827829,3190.3302841186523,0.21945751174280304
957958,1915917,1915916,3831833,3193.863079071045,0.21923960004096443
958959,1917919,1917918,3835837,3197.4199628829956,0.21902212578970648
959960,1919921,1919920,3839841,3200.9888610839844,0.21880508765570994
960961,1921923,1921922,3843845,3204.533315896988,0.21858848431475053
961962,1923925,1923924,3847849,3208.165143966675,0.21837231444078498
962963,1925927,1925926,3851853,3211.708139181137,0.21815657672050293
963964,1927929,1927928,3855857,3215.2688710689545,0.21794126983513706
964965,1929931,1929930,3859861,3218.8349800109863,0.21772639248774794
965966,1931933,1931932,3863865,3222.3853969573975,0.21751194337412016
966967,1933935,1933934,3867869,3225.9300780296326,0.21729792119913327
967968,1935937,1935936,3871873,3229.4806611537933,0.2170843246676668
968969,1937939,1937938,3875877,3233.045751094818,0.21687115249915223
969970,1939941,1939940,3879881,3236.439852952957,0.216658403413021
970971,1941943,1941942,3883885,3239.8045399188995,0.21644607613598055
971972,1943945,1943944,3887889,3243.2018010616302,0.21623416939473827
972973,1945947,1945946,3891893,3246.59277009964,0.21602268193055352
973974,1947949,1947948,3895897,3249.9691169261932,0.21581161247740965
974975,1949951,1949950,3899901,3253.536642074585,0.21560095978202298
975976,1951953,1951952,3903905,3256.990730047226,0.21539072260384273
976977,1953955,1953954,3907909,3260.379774093628,0.21518089968776621
977978,1955957,1955956,3911913,3263.7804901599884,0.21497148979869962
978979,1957959,1957958,3915917,3267.1444220542908,0.21476249170518713
979980,1959961,1959960,3919921,3270.515394926071,0.2145539041757729
980981,1961963,1961962,3923925,3273.907637119293,0.21434572598263912
981982,1963965,1963964,3927929,3277.34232711792,0.21413795590888185
982983,1965967,1965966,3931933,3280.800950050354,0.21393059274487314
983984,1967969,1967968,3935937,3284.2156660556793,0.21372363527552807
984985,1969971,1969970,3939941,3287.600070953369,0.21351708229667565
985986,1971973,1971972,3943945,3290.9870748519897,0.2133109326077829
986987,1973975,1973974,3947949,3294.3648970127106,0.21310518501377373
987988,1975977,1975976,3951953,3297.7394251823425,0.21289983832502912
988989,1977979,1977978,3955957,3301.141799926758,0.21269489135556796
989990,1979981,1979980,3959961,3304.541310071945,0.21249034292304714
990991,1981983,1981982,3963965,3307.910754919052,0.2122861918505805
991992,1983985,1983984,3967969,3311.268275976181,0.21208243697219586
992993,1985987,1985986,3971973,3314.645651102066,0.21187907711282605
993994,1987989,1987988,3975977,3318.026892900467,0.21167611111377482
994995,1989991,1989990,3979981,3321.392380952835,0.21147353781634592
995996,1991993,1991992,3983985,3324.764140844345,0.21127135606730008
996997,1993995,1993994,3987989,3328.1265869140625,0.21106956471885496
997998,1995997,1995996,3991993,3331.6670711040497,0.21086816262504726
998999,1997999,1997998,3995997,3335.1974658966064,0.2106671486471896
1000000,2000001,2000000,4000001,3338.5692281723022,0.2104665216502326


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002852916717529297,12064.682476916567
775,1551,775,2326,2.745640993118286,1.7677786603617278
1550,3101,1550,4651,5.344280242919922,0.4014025325795956
2324,4649,2324,6973,7.957818031311035,0.1667746777930006
3099,6199,3099,9298,10.606822967529297,0.09114737647360016
3874,7749,3874,11623,13.439836025238037,0.056166856207710225
4649,9299,4649,13948,16.61601996421814,0.038495066579343984
5423,10847,5423,16270,19.813029050827026,0.02792227615827869
6198,12397,6198,18595,22.94659113883972,0.021325745914509753
6973,13947,6973,20920,25.835829973220825,0.016638080285702017
7748,15497,7748,23245,28.67917227745056,0.013368418583922903
8522,17045,8522,25567,31.304814100265503,0.010898089672991773
9297,18595,9297,27892,33.93050503730774,0.009102592601266224
10072,20145,10072,30217,36.53684210777283,0.007663005782887922
10847,21695,10847,32542,39.180908203125,0.006520347500554635
11621,23243,11621,34864,41.821572065353394,0.005626610769468243
12396,24793,12396,37189,44.44194006919861,0.004873611356742913
13171,26343,13171,39514,47.07123517990112,0.004269268079951871
13946,27893,13946,41839,49.74748921394348,0.003744532736163819
14721,29443,14721,44164,52.383578300476074,0.0033283825341641204
15495,30991,15495,46486,55.01123309135437,0.002958919632874313
16270,32541,16270,48811,57.63287925720215,0.002667349132025265
17045,34091,17045,51136,60.283698081970215,0.0023996528834686615
17820,35641,17820,53461,62.8657500743866,0.0021793110136059113
18594,37189,18594,55783,65.47942209243774,0.0019711316981556593
19369,38739,19369,58108,68.09490513801575,0.0017870550473162439
20144,40289,20144,60433,70.78429126739502,0.001615925328223966
20919,41839,20919,62758,73.67022013664246,0.0014607805514970096
21693,43387,21693,65080,76.42484784126282,0.001323564780250308
22468,44937,22468,67405,79.11635994911194,0.0011996704797638813
23243,46487,23243,69730,81.74084806442261,0.001092055576009443
24018,48037,24018,72055,84.34089303016663,0.000993107409158256
24792,49585,24792,74377,86.92521095275879,0.0008996737778943498
25567,51135,25567,76702,89.5535581111908,0.0008043631096370518
26342,52685,26342,79027,92.136953830719,0.0007156788597058039
27117,54235,27117,81352,94.80945897102356,0.0006237916804820998
27891,55783,27891,83674,97.48084092140198,0.000548225898455712
28666,57333,28666,85999,100.0959370136261,0.0004942133909935364
29441,58883,29441,88324,102.68812489509583,0.0004488420545385452
30216,60433,30216,90649,105.29028511047363,0.00040464819358021487
30991,61983,30991,92974,107.91358804702759,0.00036244392140361015
31765,63531,31765,95296,110.51516389846802,0.00032371085399063304
32540,65081,32540,97621,113.1130690574646,0.00028519438637886196
33315,66631,33315,99946,115.78718495368958,0.0002489538055669982
34090,68181,34090,102271,118.40932106971741,0.00021314061450539157
34864,69729,34864,104593,121.02134418487549,0.00018004104822466616
35639,71279,35639,106918,123.6182951927185,0.00014671289864054415
36414,72829,36414,109243,126.24045395851135,0.00012676610640482977
37189,74379,37189,111568,128.89652609825134,0.0001274834849027684
37963,75927,37963,113890,131.5113890171051,0.0001277419341931818
38738,77477,38738,116215,134.2838830947876,0.00012497166244429536
39513,79027,39513,118540,137.03791689872742,0.00012021554903185461
40288,80577,40288,120865,139.66226601600647,0.00011699726201186422
41062,82125,41062,123187,142.28595805168152,0.0001147355305874953
41837,83675,41837,125512,144.8837640285492,0.00011100803021690808
42612,85225,42612,127837,147.5332748889923,0.00010569814003247302
43387,86775,43387,130162,150.1225061416626,0.0001025164128805045
44162,88325,44162,132487,152.73624396324158,9.874528768705204e-05
44936,89873,44936,134809,155.32544898986816,9.786390546651091e-05
45711,91423,45711,137134,157.95757508277893,0.00010074950660055038
46486,92973,46486,139459,160.556654214859,0.0001031169140333077
47261,94523,47261,141784,163.14953303337097,0.00010510779611649923
48035,96071,48035,144106,165.88540387153625,0.0001062755545717664
48810,97621,48810,146431,168.64868903160095,0.00010579736044746824
49585,99171,49585,148756,171.47142004966736,0.00010525467405386735
50360,100721,50360,151081,174.22674417495728,0.00010384920642536599
51134,102269,51134,153403,176.99540615081787,0.00010185028804698959
51909,103819,51909,155728,179.73317408561707,9.897376185108442e-05
52684,105369,52684,158053,182.45862817764282,9.735794446896762e-05
53459,106919,53459,160378,185.2087481021881,9.82797791948542e-05
54233,108467,54233,162700,187.93822503089905,9.620645687391516e-05
55008,110017,55008,165025,190.6682391166687,9.431776379642542e-05
55783,111567,55783,167350,193.41566395759583,9.302177386416588e-05
56558,113117,56558,169675,196.16140818595886,9.342872363049537e-05
57333,114667,57333,172000,198.94582509994507,9.326197323389351e-05
58107,116215,58107,174322,201.67475199699402,9.177753236144781e-05
58882,117765,58882,176647,204.40849208831787,8.81782834767364e-05
59657,119315,59657,178972,207.1083242893219,8.425397209066432e-05
60432,120865,60432,181297,209.84565830230713,7.942208867461886e-05
61206,122413,61206,183619,212.55731105804443,7.564453881059308e-05
61981,123963,61981,185944,215.5026319026947,7.00463951943675e-05
62756,125513,62756,188269,218.32217502593994,6.581307934538927e-05
63531,127063,63531,190594,221.06718015670776,6.39132395008346e-05
64305,128611,64305,192916,223.8058681488037,6.276919884840026e-05
65080,130161,65080,195241,226.55526614189148,6.202607255545445e-05
65855,131711,65855,197566,229.26593899726868,6.137341733847279e-05
66630,133261,66630,199891,231.99581503868103,6.0511027186294086e-05
67404,134809,67404,202213,234.63794803619385,5.852079266333021e-05
68179,136359,68179,204538,237.37354397773743,5.621965647151228e-05
68954,137909,68954,206863,240.0160551071167,5.2604791562771425e-05
69729,139459,69729,209188,242.59821915626526,4.84391948702978e-05
70504,141009,70504,211513,245.19819712638855,4.3721418478526175e-05
71278,142557,71278,213835,247.82261610031128,4.0510372855351306e-05
72053,144107,72053,216160,250.4334590435028,4.003081267001107e-05
72828,145657,72828,218485,253.0189130306244,3.860147080558818e-05
73603,147207,73603,220810,255.62403106689453,3.656563785625622e-05
74377,148755,74377,223132,258.2696180343628,3.3460652048233896e-05
75152,150305,75152,225457,260.88443303108215,3.157551145704929e-05
75927,151855,75927,227782,263.4843740463257,2.8666167054325342e-05
76702,153405,76702,230107,266.09620904922485,2.693700480449479e-05
77476,154953,77476,232429,268.72795009613037,2.351377952436451e-05
78251,156503,78251,234754,271.3304650783539,2.454014975228347e-05
79026,158053,79026,237079,273.9328589439392,2.6714507839642465e-05
79801,159603,79801,239404,276.54637694358826,2.717930510698352e-05
80575,161151,80575,241726,279.182639837265,3.0102628443273716e-05
81350,162701,81350,244051,281.87464904785156,3.119765460724011e-05
82125,164251,82125,246376,284.4688210487366,3.097036460530944e-05
82900,165801,82900,248701,287.0893020629883,2.8824342734878883e-05
83674,167349,83674,251023,289.7398989200592,2.403824510111008e-05
84449,168899,84449,253348,292.35095620155334,2.073369614663534e-05
85224,170449,85224,255673,294.96246099472046,1.5199153494904749e-05
85999,171999,85999,257998,297.56201910972595,1.183923268399667e-05
86774,173549,86774,260323,300.25460505485535,1.1765241652028635e-05
87548,175097,87548,262645,302.8561010360718,1.2892120139440522e-05
88323,176647,88323,264970,305.4631612300873,1.5386647646664642e-05
89098,178197,89098,267295,308.09879994392395,1.8569018720882013e-05
89873,179747,89873,269620,310.7483949661255,2.1210846171015874e-05
90647,181295,90647,271942,313.35808205604553,2.2328007617034018e-05
91422,182845,91422,274267,315.9660301208496,2.2831973183201626e-05
92197,184395,92197,276592,318.6076989173889,2.1542937247431837e-05
92972,185945,92972,278917,321.2079482078552,1.9815743144135922e-05
93746,187493,93746,281239,323.83251690864563,2.1108891814947128e-05
94521,189043,94521,283564,326.4411871433258,2.292700082762167e-05
95296,190593,95296,285889,329.03459310531616,2.3089714886737056e-05
96071,192143,96071,288214,331.6668691635132,2.246791700599715e-05
96845,193691,96845,290536,334.27379989624023,2.3058833903633058e-05
97620,195241,97620,292861,336.86903190612793,2.2195834390004165e-05
98395,196791,98395,295186,339.4646589756012,1.9949737179558724e-05
99170,198341,99170,297511,342.0730769634247,2.0219467842252925e-05
99945,199891,99945,299836,344.68992805480957,2.0540855985018425e-05
100719,201439,100719,302158,347.3261489868164,1.991930002986919e-05
101494,202989,101494,304483,349.94937205314636,1.855997834354639e-05
102269,204539,102269,306808,352.5736620426178,1.7686255887383595e-05
103044,206089,103044,309133,355.18724727630615,1.7531572666484863e-05
103818,207637,103818,311455,357.8209240436554,1.6314696040353738e-05
104593,209187,104593,313780,360.48984003067017,1.2627886462723836e-05
105368,210737,105368,316105,363.09752106666565,9.35580101213418e-06
106143,212287,106143,318430,365.70304703712463,8.440449164481834e-06
106917,213835,106917,320752,368.35013723373413,1.210491063829977e-05
107692,215385,107692,323077,371.1088709831238,1.5667346815462224e-05
108467,216935,108467,325402,373.79383087158203,1.88503363460768e-05
109242,218485,109242,327727,376.6077380180359,1.9234568753745407e-05
110016,220033,110016,330049,379.3425438404083,1.8051121514872648e-05
110791,221583,110791,332374,381.95368099212646,1.5811820048838854e-05
111566,223133,111566,334699,384.5488269329071,1.324856566498056e-05
112341,224683,112341,337024,387.1522262096405,9.278041034121998e-06
113116,226233,113116,339349,389.7857758998871,6.417565600713715e-06
113890,227781,113890,341671,392.3829951286316,7.554262992925942e-06
114665,229331,114665,343996,394.9729549884796,1.026120298774913e-05
115440,230881,115440,346321,397.59638714790344,1.170631730929017e-05
116215,232431,116215,348646,400.25602197647095,1.198944664793089e-05
116989,233979,116989,350968,402.941232919693,1.2242708180565387e-05
117764,235529,117764,353293,405.5837490558624,1.219591467815917e-05
118539,237079,118539,355618,408.210333108902,1.2919916116516106e-05
119314,238629,119314,357943,410.8298602104187,1.3319102436071262e-05
120088,240177,120088,360265,413.4221131801605,1.3684311852557585e-05
120863,241727,120863,362590,416.04121708869934,1.2838274415116757e-05
121638,243277,121638,364915,418.6422860622406,1.2584298019646667e-05
122413,244827,122413,367240,421.28537106513977,1.0868310710065998e-05
123187,246375,123187,369562,423.870078086853,1.0482979632797651e-05
123962,247925,123962,371887,426.4902489185333,1.0073383236886002e-05
124737,249475,124737,374212,429.11045002937317,9.443641829420812e-06
125512,251025,125512,376537,431.7575891017914,9.667259291745722e-06
126286,252573,126286,378859,434.3851752281189,8.75638761499431e-06
127061,254123,127061,381184,437.14276790618896,6.131020199973136e-06
127836,255673,127836,383509,439.88828706741333,4.857853127759881e-06
128611,257223,128611,385834,442.4880909919739,4.247289325576276e-06
129386,258773,129386,388159,445.09362602233887,5.760231942986138e-06
130160,260321,130160,390481,447.70531606674194,8.511267878930084e-06
130935,261871,130935,392806,450.3397591114044,9.231502190232277e-06
131710,263421,131710,395131,452.93116307258606,9.867173503153026e-06
132485,264971,132485,397456,455.79060411453247,8.60466025187634e-06
133259,266519,133259,399778,458.48410820961,7.827222361811437e-06
134034,268069,134034,402103,461.10670018196106,5.042500561103225e-06
134809,269619,134809,404428,463.73003125190735,3.978726454079151e-06
135584,271169,135584,406753,466.3415639400482,5.256886652205139e-06
136358,272717,136358,409075,468.9438819885254,7.024626029306091e-06
137133,274267,137133,411400,471.5861608982086,7.304419341380708e-06
137908,275817,137908,413725,474.22146010398865,8.054643330979161e-06
138683,277367,138683,416050,476.82519721984863,8.78046193975024e-06
139457,278915,139457,418372,479.46450901031494,9.842533472692594e-06
140232,280465,140232,420697,482.2165541648865,1.0234269211650826e-05
141007,282015,141007,423022,484.8849501609802,9.010669600684196e-06
141782,283565,141782,425347,487.4891040325165,9.318553566117771e-06
142557,285115,142557,427672,490.1180500984192,9.162075002677739e-06
143331,286663,143331,429994,492.72211623191833,9.685210898169316e-06
144106,288213,144106,432319,495.3201632499695,9.174023944069631e-06
144881,289763,144881,434644,497.9609811306,9.238789061782882e-06
145656,291313,145656,436969,500.5933539867401,8.904356946004555e-06
146430,292861,146430,439291,503.20531606674194,7.72114253777545e-06
147205,294411,147205,441616,505.82760190963745,6.9441466621356085e-06
147980,295961,147980,443941,508.44168615341187,6.386082532117143e-06
148755,297511,148755,446266,511.0604159832001,5.5658565543126315e-06
149529,299059,149529,448588,513.6633100509644,4.209445251035504e-06
150304,300609,150304,450913,516.2868769168854,4.235032974975184e-06
151079,302159,151079,453238,518.9262721538544,6.225107426871546e-06
151854,303709,151854,455563,521.5352499485016,7.973192623467185e-06
152628,305257,152628,457885,524.1618921756744,8.497781891492195e-06
153403,306807,153403,460210,526.8418691158295,7.045169695629738e-06
154178,308357,154178,462535,529.4907321929932,4.977049684384838e-06
154953,309907,154953,464860,532.0958580970764,3.5085158742731437e-06
155728,311457,155728,467185,534.7237720489502,4.484696546569467e-06
156502,313005,156502,469507,537.3432719707489,5.256684744381346e-06
157277,314555,157277,471832,539.9644250869751,5.337660695658997e-06
158052,316105,158052,474157,542.5941309928894,5.4241845646174625e-06
158827,317655,158827,476482,545.205824136734,6.3309653342003e-06
159601,319203,159601,478804,547.8125472068787,6.3345851231133565e-06
160376,320753,160376,481129,550.4250130653381,6.526486686198041e-06
161151,322303,161151,483454,553.0365929603577,6.161477358546108e-06
161926,323853,161926,485779,555.6616299152374,6.674170435871929e-06
162700,325401,162700,488101,558.2926280498505,7.045575330266729e-06
163475,326951,163475,490426,560.9237780570984,6.345706424326636e-06
164250,328501,164250,492751,563.614825963974,5.786556357634254e-06
165025,330051,165025,495076,566.3376798629761,5.389196303440258e-06
165799,331599,165799,497398,569.0307359695435,4.6584918891312554e-06
166574,333149,166574,499723,571.7780170440674,3.6330420698504895e-06
167349,334699,167349,502048,574.4995651245117,2.848033545888029e-06
168124,336249,168124,504373,577.195739030838,1.456073732697405e-06
168899,337799,168899,506698,579.918331861496,2.708091415115632e-06
169673,339347,169673,509020,582.6349132061005,4.7812463890295476e-06
170448,340897,170448,511345,585.3622379302979,5.865429557161406e-06
171223,342447,171223,513670,588.1242849826813,5.558526027016342e-06
171998,343997,171998,515995,590.8497550487518,4.096244083484635e-06
172772,345545,172772,518317,593.6097390651703,2.726032107602805e-06
173547,347095,173547,520642,596.5480411052704,2.0210372895235196e-06
174322,348645,174322,522967,599.3574368953705,3.115877916570753e-06
175097,350195,175097,525292,602.0838751792908,3.316006768727675e-06
175871,351743,175871,527614,604.8349521160126,3.619450581027195e-06
176646,353293,176646,529939,607.558039188385,4.899149644188583e-06
177421,354843,177421,532264,610.2897641658783,5.4596675909124315e-06
178196,356393,178196,534589,613.0065290927887,5.28391137777362e-06
178970,357941,178970,536911,615.7746601104736,5.458885425468907e-06
179745,359491,179745,539236,618.5325441360474,5.85163252253551e-06
180520,361041,180520,541561,621.3339149951935,5.327563485479914e-06
181295,362591,181295,543886,624.0878391265869,4.272387741366401e-06
182069,364139,182069,546208,626.8048191070557,4.0225095290225e-06
182844,365689,182844,548533,629.5146200656891,3.2339048630092293e-06
183619,367239,183619,550858,632.1370460987091,2.0082443370483816e-06
184394,368789,184394,553183,634.7678029537201,2.217908331658691e-06
185169,370339,185169,555508,637.400139093399,3.4299555409234017e-06
185943,371887,185943,557830,640.0287871360779,4.501951480051503e-06
186718,373437,186718,560155,642.6331031322479,5.0911821745103225e-06
187493,374987,187493,562480,645.2510778903961,4.863744834437966e-06
188268,376537,188268,564805,647.8905642032623,3.0397422960959375e-06
189042,378085,189042,567127,650.4947230815887,2.188049620599486e-06
189817,379635,189817,569452,653.1078128814697,1.8584632925922051e-06
190592,381185,190592,571777,655.7045991420746,2.6758079911815003e-06
191367,382735,191367,574102,658.3114252090454,3.881936208927073e-06
192141,384283,192141,576424,660.9094860553741,4.059833372593857e-06
192916,385833,192916,578749,663.5393459796906,4.547073331195861e-06
193691,387383,193691,581074,666.1638770103455,4.733479727292433e-06
194466,388933,194466,583399,668.7777349948883,4.469198756851256e-06
195240,390481,195240,585721,671.3601140975952,4.205299774184823e-06
196015,392031,196015,588046,673.981153011322,3.7490990507649258e-06
196790,393581,196790,590371,676.6062998771667,3.012604793184437e-06
197565,395131,197565,592696,679.1994712352753,2.66384995484259e-06
198340,396681,198340,595021,681.7963840961456,1.8449372873874381e-06
199114,398229,199114,597343,684.3965640068054,1.8850805645342916e-06
199889,399779,199889,599668,687.0088400840759,2.7780679374700412e-06
200664,401329,200664,601993,689.6142420768738,3.475443008937873e-06
201439,402879,201439,604318,692.2077419757843,3.866776751237921e-06
202213,404427,202213,606640,694.8251020908356,3.1757299439050257e-06
202988,405977,202988,608965,697.4199891090393,1.928192432387732e-06
203763,407527,203763,611290,700.035236120224,1.1906759027624503e-06
204538,409077,204538,613615,702.6316821575165,1.6950525605352595e-06
205312,410625,205312,615937,705.2388410568237,2.5117169570876285e-06
206087,412175,206087,618262,707.8800342082977,2.5970457500079647e-06
206862,413725,206862,620587,710.4810869693756,3.4032764233415946e-06
207637,415275,207637,622912,713.0749220848083,3.4921995393233374e-06
208411,416823,208411,625234,715.8064610958099,3.0635728762717918e-06
209186,418373,209186,627559,718.5024859905243,3.0633582355221733e-06
209961,419923,209961,629884,721.1435351371765,3.140450644423254e-06
210736,421473,210736,632209,723.7795991897583,2.422924808342941e-06
211511,423023,211511,634534,726.4078950881958,2.4518139980500564e-06
212285,424571,212285,636856,729.0143141746521,1.6804660845082253e-06
213060,426121,213060,639181,731.7661321163177,1.2220298231113702e-06
213835,427671,213835,641506,734.4210121631622,2.1001033019274473e-06
214610,429221,214610,643831,737.0478370189667,2.259856046293862e-06
215384,430769,215384,646153,739.6393330097198,2.910957846324891e-06
216159,432319,216159,648478,742.387197971344,2.776447217911482e-06
216934,433869,216934,650803,745.1688561439514,2.1613195713143796e-06
217709,435419,217709,653128,747.8839602470398,1.625297954888083e-06
218483,436967,218483,655450,750.5355131626129,1.5734949556645006e-06
219258,438517,219258,657775,753.1657538414001,1.932410668814555e-06
220033,440067,220033,660100,755.7832200527191,2.36985033552628e-06
220808,441617,220808,662425,758.4568982124329,2.7162168407812715e-06
221582,443165,221582,664747,761.0529069900513,2.7323985705152154e-06
222357,444715,222357,667072,763.6542201042175,3.105347786913626e-06
223132,446265,223132,669397,766.2873330116272,3.2005154935177416e-06
223907,447815,223907,671722,768.8883430957794,2.730794221861288e-06
224681,449363,224681,674044,771.4799518585205,2.713639332796447e-06
225456,450913,225456,676369,774.0975959300995,2.086566382786259e-06
226231,452463,226231,678694,776.7039110660553,1.2512246030382812e-06
227006,454013,227006,681019,779.302953004837,1.3244534784462303e-06
227781,455563,227781,683344,781.912143945694,1.9272520148660988e-06
228555,457111,228555,685666,784.5509650707245,2.5354092940688133e-06
229330,458661,229330,687991,787.6050498485565,3.075872882618569e-06
230105,460211,230105,690316,790.4109740257263,2.5841418391792104e-06
230880,461761,230880,692641,793.2167320251465,2.3318953026318923e-06
231654,463309,231654,694963,795.9507138729095,1.6092180885607377e-06
232429,464859,232429,697288,798.7141242027283,7.67555320635438e-07
233204,466409,233204,699613,801.6599502563477,1.7249531083507463e-06
233979,467959,233979,701938,804.513069152832,1.9996004994027317e-06
234753,469507,234753,704260,807.3050911426544,2.544309609220363e-06
235528,471057,235528,706585,810.0514183044434,2.734899680945091e-06
236303,472607,236303,708910,812.7864971160889,2.3797183530405164e-06
237078,474157,237078,711235,815.5141232013702,2.5498247850919142e-06
237852,475705,237852,713557,818.2902801036835,2.1228406694717705e-06
238627,477255,238627,715882,821.0325410366058,1.8442297005094588e-06
239402,478805,239402,718207,823.7864201068878,1.6523754311492667e-06
240177,480355,240177,720532,826.5912530422211,8.154602255672216e-07
240952,481905,240952,722857,829.4441180229187,1.417502062395215e-06
241726,483453,241726,725179,832.1755731105804,1.7854072211775929e-06
242501,485003,242501,727504,834.9186398983002,1.969034201465547e-06
243276,486553,243276,729829,837.6561350822449,2.1786181605421007e-06
244051,488103,244051,732154,840.3922460079193,2.0307670638430864e-06
244825,489651,244825,734476,843.1557919979095,2.1912710508331656e-06
245600,491201,245600,736801,845.9046499729156,1.7875863704830408e-06
246375,492751,246375,739126,848.653158903122,1.4039505913387984e-06
247150,494301,247150,741451,851.3505439758301,7.132694008760154e-07
247924,495849,247924,743773,853.987722158432,9.008908818941563e-07
248699,497399,248699,746098,856.6152260303497,1.5033947420306504e-06
249474,498949,249474,748423,859.2446510791779,1.7441125237382948e-06
250249,500499,250249,750748,861.8809411525726,2.178852810175158e-06
251023,502047,251023,753070,864.4866991043091,2.0372553990455344e-06
251798,503597,251798,755395,867.0862550735474,2.0124789443798363e-06
252573,505147,252573,757720,869.7130219936371,1.554924892843701e-06
253348,506697,253348,760045,872.3150322437286,1.113297912525013e-06
254123,508247,254123,762370,874.9225862026215,7.488251867471263e-07
254897,509795,254897,764692,877.5160050392151,9.504674380877987e-07
255672,511345,255672,767017,880.1173911094666,1.5907789929769933e-06
256447,512895,256447,769342,882.7944431304932,1.635335138416849e-06
257222,514445,257222,771667,885.3958129882812,1.9297913240734488e-06
257996,515993,257996,773989,888.0245051383972,1.6469839465571567e-06
258771,517543,258771,776314,890.6313989162445,1.8146311049349606e-06
259546,519093,259546,778639,893.2430069446564,1.5965651982696727e-06
260321,520643,260321,780964,895.8388290405273,1.2821419659303501e-06
261095,522191,261095,783286,898.423173904419,7.454855222022161e-07
261870,523741,261870,785611,901.007269859314,1.107126081478782e-06
262645,525291,262645,787936,903.6254191398621,1.4240686141420156e-06
263420,526841,263420,790261,906.2506530284882,1.7107540770666674e-06
264194,528389,264194,792583,908.8697621822357,1.9630369934020564e-06
264969,529939,264969,794908,911.4970502853394,1.9011258700629696e-06
265744,531489,265744,797233,914.1162109375,1.7795537132769823e-06
266519,533039,266519,799558,916.7361118793488,1.2761447578668594e-06
267293,534587,267293,801880,919.343138217926,7.379330781986937e-07
268068,536137,268068,804205,921.9333808422089,8.929164323490113e-07
268843,537687,268843,806530,924.5354981422424,1.4916931831976399e-06
269618,539237,269618,808855,927.1493890285492,1.6785743355285376e-06
270393,540787,270393,811180,929.7446842193604,1.9136223272653297e-06
271167,542335,271167,813502,932.3443038463593,1.7436304915463552e-06
271942,543885,271942,815827,934.9860382080078,1.5834393707336858e-06
272717,545435,272717,818152,937.6153371334076,1.2692635209532455e-06
273492,546985,273492,820477,940.2072870731354,1.0622552508721128e-06
274266,548533,274266,822799,942.798770904541,7.447797543136403e-07
275041,550083,275041,825124,945.4128589630127,1.2474138202378526e-06
275816,551633,275816,827449,948.0390651226044,1.4484066923614591e-06
276591,553183,276591,829774,950.6528930664062,1.5054756659083068e-06
277365,554731,277365,832096,953.260645866394,1.6171525203390047e-06
278140,556281,278140,834421,955.8567440509796,1.5355926734628156e-06
278915,557831,278915,836746,958.4743571281433,1.2757154763676226e-06
279690,559381,279690,839071,961.0752410888672,7.530543371103704e-07
280464,560929,280464,841393,963.6622641086578,7.252965588122606e-07
281239,562479,281239,843718,966.2741351127625,9.727591532282531e-07
282014,564029,282014,846043,968.8832290172577,1.4184097381075844e-06
282789,565579,282789,848368,971.4852170944214,1.4555262168869376e-06
283564,567129,283564,850693,974.0844612121582,1.5753412299090996e-06
284338,568677,284338,853015,976.7026591300964,1.2215987226227298e-06
285113,570227,285113,855340,979.3257710933685,9.713348845252767e-07
285888,571777,285888,857665,981.962856054306,5.241272447165102e-07
286663,573327,286663,859990,984.6902952194214,7.220696716103703e-07
287437,574875,287437,862312,987.4323210716248,1.1276424629613757e-06
288212,576425,288212,864637,990.066890001297,1.3166572898626328e-06
288987,577975,288987,866962,992.6536159515381,1.3655080692842603e-06
289762,579525,289762,869287,995.2723960876465,1.1217925930395722e-06
290536,581073,290536,871609,997.8841800689697,1.1381798685761169e-06
291311,582623,291311,873934,1000.4899652004242,7.048220140859485e-07
292086,584173,292086,876259,1003.0706608295441,5.175334081286564e-07
292861,585723,292861,878584,1005.6525690555573,8.390252332901582e-07
293635,587271,293635,880906,1008.2909970283508,1.0274343367200345e-06
294410,588821,294410,883231,1010.9721779823303,1.279362550121732e-06
295185,590371,295185,885556,1013.6102101802826,1.2548171071102843e-06
295960,591921,295960,887881,1016.3691022396088,1.2532054824987426e-06
296735,593471,296735,890206,1018.9981510639191,8.916340448195115e-07
297509,595019,297509,892528,1021.6157791614532,3.979912435170263e-07
298284,596569,298284,894853,1024.2000210285187,6.737609510309994e-07
299059,598119,299059,897178,1026.8613090515137,9.866071195574477e-07
299834,599669,299834,899503,1029.5226299762726,1.32853165268898e-06
300608,601217,300608,901825,1032.128428220749,1.3305361790116876e-06
301383,602767,301383,904150,1034.7577538490295,1.1399151844670996e-06
302158,604317,302158,906475,1037.4094049930573,9.277209755964577e-07
302933,605867,302933,908800,1040.0223019123077,6.060035957489163e-07
303707,607415,303707,911122,1042.6992211341858,6.841819413239136e-07
304482,608965,304482,913447,1045.417032957077,1.0632138582877815e-06
305257,610515,305257,915772,1048.0898802280426,1.098418579204008e-06
306032,612065,306032,918097,1050.6801090240479,1.1998999980278313e-06
306806,613613,306806,920419,1053.2878699302673,1.211268681799993e-06
307581,615163,307581,922744,1055.8704981803894,9.348405001219362e-07
308356,616713,308356,925069,1058.5126330852509,6.299978849710897e-07
309131,618263,309131,927394,1061.2354640960693,6.724876584485173e-07
309906,619813,309906,929719,1063.8729538917542,8.267688826890662e-07
310680,621361,310680,932041,1066.5040199756622,1.1991214705631137e-06
311455,622911,311455,934366,1069.0954539775848,1.2862183211836964e-06
312230,624461,312230,936691,1071.6934931278229,1.1059837561333552e-06
313005,626011,313005,939016,1074.3039691448212,8.704973879503086e-07
313779,627559,313779,941338,1076.933392047882,4.924495442537591e-07
314554,629109,314554,943663,1079.541981935501,6.377558747772127e-07
315329,630659,315329,945988,1082.12970495224,9.773393685463816e-07
316104,632209,316104,948313,1084.7042078971863,1.1708852980518714e-06
316878,633757,316878,950635,1087.327430009842,1.0996827768394724e-06
317653,635307,317653,952960,1089.9455261230469,8.959941624198109e-07
318428,636857,318428,955285,1092.5408289432526,7.023481884971261e-07
319203,638407,319203,957610,1095.151554107666,4.3998807086609304e-07
319977,639955,319977,959932,1097.7849791049957,7.65929144108668e-07
320752,641505,320752,962257,1100.4096291065216,8.771530701778829e-07
321527,643055,321527,964582,1103.0200729370117,9.806590242078528e-07
322302,644605,322302,966907,1105.6157629489899,1.0331714292988181e-06
323076,646153,323076,969229,1108.2150909900665,8.83344910107553e-07
323851,647703,323851,971554,1110.8268649578094,5.297024472383782e-07
324626,649253,324626,973879,1113.4278030395508,3.235763870179653e-07
325401,650803,325401,976204,1116.347004890442,7.319085852941498e-07
326176,652353,326176,978529,1119.1206440925598,9.288251021644101e-07
326950,653901,326950,980851,1121.7215361595154,9.270861482946202e-07
327725,655451,327725,983176,1124.3302669525146,7.659727998543531e-07
328500,657001,328500,985501,1126.9660859107971,5.16602085554041e-07
329275,658551,329275,987826,1129.5697548389435,2.8878639568574727e-07
330049,660099,330049,990148,1132.192633152008,6.544541975017637e-07
330824,661649,330824,992473,1134.8950769901276,8.231254469137639e-07
331599,663199,331599,994798,1137.5126490592957,8.132701623253524e-07
332374,664749,332374,997123,1140.1283621788025,8.334573067259043e-07
333148,666297,333148,999445,1142.7497990131378,6.589161785086617e-07
333923,667847,333923,1001770,1145.3451120853424,2.90938260150142e-07
334698,669397,334698,1004095,1147.9580450057983,4.6051536628510803e-07
335473,670947,335473,1006420,1150.564973115921,7.281887519638985e-07
336247,672495,336247,1008742,1153.1676330566406,8.656825229991227e-07
337022,674045,337022,1011067,1155.7823832035065,8.025090210139751e-07
337797,675595,337797,1013392,1158.4099140167236,5.367110134102404e-07
338572,677145,338572,1015717,1161.008670091629,1.9807521312031895e-07
339347,678695,339347,1018042,1163.6160049438477,5.402198439696804e-07
340121,680243,340121,1020364,1166.2361290454865,7.846210792195052e-07
340896,681793,340896,1022689,1168.8604581356049,8.110764611046761e-07
341671,683343,341671,1025014,1171.4627652168274,7.066992111504078e-07
342446,684893,342446,1027339,1174.1985681056976,5.828787834616378e-07
343220,686441,343220,1029661,1176.9205901622772,2.7056194085162133e-07
343995,687991,343995,1031986,1179.6214580535889,5.207366484683007e-07
344770,689541,344770,1034311,1182.2078258991241,7.164417183957994e-07
345545,691091,345545,1036636,1184.7978792190552,8.230090315919369e-07
346319,692639,346319,1038958,1187.4134330749512,7.36457877792418e-07
347094,694189,347094,1041283,1190.0466902256012,4.5780689106322825e-07
347869,695739,347869,1043608,1192.667044878006,2.8940849006175995e-07
348644,697289,348644,1045933,1195.3384990692139,6.452428351622075e-07
349418,698837,349418,1048255,1197.9420280456543,7.663002179469913e-07
350193,700387,350193,1050580,1200.6052701473236,6.953196134418249e-07
350968,701937,350968,1052905,1203.2615630626678,6.182563083712012e-07
351743,703487,351743,1055230,1205.8444809913635,3.536424628691748e-07
352518,705037,352518,1057555,1208.4673421382904,4.352750693215057e-07
353292,706585,353292,1059877,1211.0588240623474,6.355476216413081e-07
354067,708135,354067,1062202,1213.675784111023,7.601520337630063e-07
354842,709685,354842,1064527,1216.27787399292,7.008602551650256e-07
355617,711235,355617,1066852,1218.9456520080566,4.323337634559721e-07
356391,712783,356391,1069174,1221.5581650733948,2.2262793208938092e-07
357166,714333,357166,1071499,1224.1616020202637,5.511683411896229e-07
357941,715883,357941,1073824,1226.7643189430237,6.774043868063018e-07
358716,717433,358716,1076149,1229.396686077118,6.258305802475661e-07
359490,718981,359490,1078471,1231.985778093338,5.409001460066065e-07
360265,720531,360265,1080796,1234.5906870365143,2.531032805563882e-07
361040,722081,361040,1083121,1237.2122812271118,3.852692316286266e-07
361815,723631,361815,1085446,1239.83726811409,5.665788194164634e-07
362589,725179,362589,1087768,1242.457594871521,6.441241566790268e-07
363364,726729,363364,1090093,1245.0747010707855,5.312667781254277e-07
364139,728279,364139,1092418,1247.7199010849,2.544566086726263e-07
364914,729829,364914,1094743,1250.3499519824982,3.0892442737240344e-07
365688,731377,365688,1097065,1253.094575881958,5.193596734898165e-07
366463,732927,366463,1099390,1255.8030421733856,5.280871846480295e-07
367238,734477,367238,1101715,1258.4480509757996,4.833073035115376e-07
368013,736027,368013,1104040,1261.0680301189423,2.602118911454454e-07
368788,737577,368788,1106365,1263.6735439300537,2.811393642332405e-07
369562,739125,369562,1108687,1266.2817080020905,4.800731403520331e-07
370337,740675,370337,1111012,1268.8710551261902,5.593246896751225e-07
371112,742225,371112,1113337,1271.5171661376953,4.5938577386550605e-07
371887,743775,371887,1115662,1274.1262691020966,1.964235707418993e-07
372661,745323,372661,1117984,1276.7715060710907,2.989345375681296e-07
373436,746873,373436,1120309,1279.4950699806213,4.7160210669972e-07
374211,748423,374211,1122634,1282.1276450157166,4.547855496639386e-07
374986,749973,374986,1124959,1284.7400760650635,4.164521669736132e-07
375760,751521,375760,1127281,1287.364166021347,1.7229467630386353e-07
376535,753071,376535,1129606,1289.9951729774475,2.847646101145074e-07
377310,754621,377310,1131931,1292.596313238144,4.711928340839222e-07
378085,756171,378085,1134256,1295.2334380149841,4.87883880850859e-07
378859,757719,378859,1136578,1297.8456320762634,2.963715814985335e-07
379634,759269,379634,1138903,1300.4785211086273,1.7541060515213758e-07
380409,760819,380409,1141228,1303.0967519283295,4.208359314361587e-07
381184,762369,381184,1143553,1305.7118651866913,4.657431418308988e-07
381959,763919,381959,1145878,1308.3325741291046,4.114626790396869e-07
382733,765467,382733,1148200,1310.9559319019318,2.2677704691886902e-07
383508,767017,383508,1150525,1313.5763399600983,2.99962266581133e-07
384283,768567,384283,1152850,1316.2066791057587,4.605135472957045e-07
385058,770117,385058,1155175,1318.8339021205902,4.765388439409435e-07
385832,771665,385832,1157497,1321.4510080814362,3.021959855686873e-07
386607,773215,386607,1159822,1324.0690660476685,2.2558560885954648e-07
387382,774765,387382,1162147,1326.6810810565948,4.332359822001308e-07
388157,776315,388157,1164472,1329.2954471111298,4.4064290705136955e-07
388931,777863,388931,1166794,1331.9481852054596,3.9312908484134823e-07
389706,779413,389706,1169119,1334.5581080913544,1.7840829968918115e-07
390481,780963,390481,1171444,1337.2016341686249,3.371187631273642e-07
391256,782513,391256,1173769,1339.9692602157593,4.651556082535535e-07
392030,784061,392030,1176091,1342.7373189926147,3.8699363358318806e-07
392805,785611,392805,1178416,1345.396388053894,2.0647166820708662e-07
393580,787161,393580,1180741,1348.0715589523315,3.1155468604993075e-07
394355,788711,394355,1183066,1350.7872650623322,4.118992364965379e-07
395130,790261,395130,1185391,1353.5803022384644,4.045159585075453e-07
395904,791809,395904,1187713,1356.294909954071,2.0527841115836054e-07
396679,793359,396679,1190038,1358.990739107132,2.825199771905318e-07
397454,794909,397454,1192363,1361.6311151981354,3.745790309039876e-07
398229,796459,398229,1194688,1364.2357079982758,3.5390803532209247e-07
399003,798007,399003,1197010,1366.8649621009827,1.7287857190240175e-07
399778,799557,399778,1199335,1369.4745001792908,2.5831832317635417e-07
400553,801107,400553,1201660,1372.0916390419006,3.4123695513699204e-07
401328,802657,401328,1203985,1374.799269914627,2.503147698007524e-07
402102,804205,402102,1206307,1377.417948961258,1.2431701179593801e-07
402877,805755,402877,1208632,1380.0546550750732,2.4598921299912035e-07
403652,807305,403652,1210957,1382.6813750267029,2.696524461498484e-07
404427,808855,404427,1213282,1385.3001201152802,1.0805524652823806e-07
405201,810403,405201,1215604,1387.9297349452972,2.255947038065642e-07
405976,811953,405976,1217929,1390.5644810199738,2.2660424292553216e-07
406751,813503,406751,1220254,1393.1682450771332,1.1245901987422258e-07
407526,815053,407526,1222579,1395.8167049884796,2.1851155906915665e-07
408301,816603,408301,1224904,1398.4715640544891,2.20945366891101e-07
409075,818151,409075,1227226,1401.0782091617584,7.456947059836239e-08
409850,819701,409850,1229551,1403.8200840950012,2.1099003788549453e-07
410625,821251,410625,1231876,1406.4773271083832,1.6345074982382357e-07
411400,822801,411400,1234201,1409.1005260944366,1.0473377187736332e-07
412174,824349,412174,1236523,1411.6908769607544,1.6247031453531235e-07
412949,825899,412949,1238848,1414.3312299251556,1.0256189852952957e-07
413724,827449,413724,1241173,1416.9285068511963,1.3928547559771687e-07
414499,828999,414499,1243498,1419.6768279075623,1.473545125918463e-07
415273,830547,415273,1245820,1422.4201030731201,9.31977410800755e-08
416048,832097,416048,1248145,1425.1307001113892,1.503340172348544e-07
416823,833647,416823,1250470,1427.818174123764,7.322341843973845e-08
417598,835197,417598,1252795,1430.470137834549,1.4516990631818771e-07
418372,836745,418372,1255117,1433.350641965866,1.2420605344232172e-07
419147,838295,419147,1257442,1436.0495512485504,1.320477167610079e-07
419922,839845,419922,1259767,1438.6693940162659,1.5126897778827697e-07
420697,841395,420697,1262092,1441.2789361476898,6.770642357878387e-08
421471,842943,421471,1264414,1443.9011640548706,1.539556251373142e-07
422246,844493,422246,1266739,1446.5470931529999,8.453207556158304e-08
423021,846043,423021,1269064,1449.181205034256,1.3989119906909764e-07
423796,847593,423796,1271389,1451.9040808677673,8.861934475135058e-08
424571,849143,424571,1273714,1454.6514530181885,1.352163963019848e-07
425345,850691,425345,1276036,1457.330715894699,7.382550393231213e-08
426120,852241,426120,1278361,1459.9468400478363,1.2643977242987603e-07
426895,853791,426895,1280686,1462.5553119182587,8.491588232573122e-08
427670,855341,427670,1283011,1465.275505065918,1.2619602784980088e-07
428444,856889,428444,1285333,1468.004019021988,9.929317457135767e-08
429219,858439,429219,1287658,1470.860671043396,8.980350685305893e-08
429994,859989,429994,1289983,1473.5991060733795,1.3150565791875124e-07
430769,861539,430769,1292308,1476.2160730361938,1.080607034964487e-07
431543,863087,431543,1294630,1478.85751414299,9.378527465742081e-08
432318,864637,432318,1296955,1481.465658903122,1.193893695017323e-07
433093,866187,433093,1299280,1484.0991780757904,1.0887197277043015e-07
433868,867737,433868,1301605,1486.786583185196,8.99963197298348e-08
434642,869285,434642,1303927,1489.4118139743805,1.0194526112172753e-07
435417,870835,435417,1306252,1492.102447271347,1.1013071343768388e-07
436192,872385,436192,1308577,1494.7534580230713,9.375798981636763e-08
436967,873935,436967,1310902,1497.369166135788,7.643211574759334e-08
437742,875485,437742,1313227,1499.9729690551758,8.664574124850333e-08
438516,877033,438516,1315549,1502.5764529705048,8.962160791270435e-08
439291,878583,439291,1317874,1505.1877870559692,7.788366929162294e-08
440066,880133,440066,1320199,1507.8096070289612,7.176822691690177e-08
440841,881683,440841,1322524,1510.4193470478058,7.814560376573354e-08
441615,883231,441615,1324846,1513.0346660614014,6.762638804502785e-08
442390,884781,442390,1327171,1515.662309885025,5.716719897463918e-08
443165,886331,443165,1329496,1518.316545009613,5.312722350936383e-08
443940,887881,443940,1331821,1520.918622970581,5.5402779253199697e-08
444714,889429,444714,1334143,1523.543033838272,4.33956302003935e-08
445489,890979,445489,1336468,1526.1882150173187,4.518551577348262e-08
446264,892529,446264,1338793,1528.8102469444275,5.127913027536124e-08
447039,894079,447039,1341118,1531.496992111206,4.174398782197386e-08
447813,895627,447813,1343440,1534.1954791545868,3.458990249782801e-08
448588,897177,448588,1345765,1536.8210492134094,3.97740222979337e-08
449363,898727,449363,1348090,1539.4318170547485,3.876812115777284e-08
450138,900277,450138,1350415,1542.036906003952,3.3940523280762136e-08
450913,901827,450913,1352740,1544.6555709838867,2.89292074739933e-08
451687,903375,451687,1355062,1547.2837481498718,3.5701305023394525e-08
452462,904925,452462,1357387,1549.9101169109344,3.460627340245992e-08
453237,906475,453237,1359712,1552.5049250125885,2.4334440240636468e-08
454012,908025,454012,1362037,1555.1604380607605,3.097557055298239e-08
454786,909573,454786,1364359,1557.7792909145355,3.331842890474945e-08
455561,911123,455561,1366684,1560.4086999893188,2.7746864361688495e-08
456336,912673,456336,1369009,1563.0096790790558,2.6488123694434762e-08
457111,914223,457111,1371334,1565.6316192150116,3.199784259777516e-08
457885,915771,457885,1373656,1568.223887205124,3.425884642638266e-08
458660,917321,458660,1375981,1570.825433254242,2.734486770350486e-08
459435,918871,459435,1378306,1573.4481010437012,3.2487150747328997e-08
460210,920421,460210,1380631,1576.0786690711975,3.9661244954913855e-08
460984,921969,460984,1382953,1578.7470421791077,3.499553713481873e-08
461759,923519,461759,1385278,1581.3519940376282,3.5837729228660464e-08
462534,925069,462534,1387603,1583.9570980072021,4.294270183891058e-08
463309,926619,463309,1389928,1586.5917670726776,4.579305823426694e-08
464083,928167,464083,1392250,1589.1940941810608,4.2145984480157495e-08
464858,929717,464858,1394575,1591.8073091506958,4.555840860120952e-08
465633,931267,465633,1396900,1594.4276940822601,5.3756593842990696e-08
466408,932817,466408,1399225,1597.0496981143951,5.019137461204082e-08
467183,934367,467183,1401550,1599.6606311798096,4.903085937257856e-08
467957,935915,467957,1403872,1602.2737019062042,5.589754437096417e-08
468732,937465,468732,1406197,1604.8767082691193,5.717447493225336e-08
469507,939015,469507,1408522,1607.5256369113922,5.314541340339929e-08
470282,940565,470282,1410847,1610.1331462860107,5.417132342699915e-08
471056,942113,471056,1413169,1612.733834028244,5.99011400481686e-08
471831,943663,471831,1415494,1615.343677997589,5.65414666198194e-08
472606,945213,472606,1417819,1617.9949488639832,5.232504918240011e-08
473381,946763,473381,1420144,1620.5853970050812,5.728361429646611e-08
474155,948311,474155,1422466,1623.1943349838257,5.766742106061429e-08
474930,949861,474930,1424791,1625.810917854309,5.1948518375866115e-08
475705,951411,475705,1427116,1628.4246101379395,5.174842954147607e-08
476480,952961,476480,1429441,1631.050784111023,5.519177648238838e-08
477254,954509,477254,1431763,1633.6788139343262,5.1935785450041294e-08
478029,956059,478029,1434088,1636.323410987854,4.6566128730773926e-08
478804,957609,478804,1436413,1638.9684329032898,4.924731911160052e-08
479579,959159,479579,1438738,1641.5738761425018,4.9876689445227385e-08
480354,960709,480354,1441063,1644.1803798675537,4.315734258852899e-08
481128,962257,481128,1443385,1646.8054521083832,4.1680323192849755e-08
481903,963807,481903,1445710,1649.4570829868317,4.4177795643918216e-08
482678,965357,482678,1448035,1652.1378660202026,4.0363374864682555e-08
483453,966907,483453,1450360,1654.8798170089722,3.47681634593755e-08
484227,968455,484227,1452682,1657.5867831707,3.5608536563813686e-08
485002,970005,485002,1455007,1660.2345201969147,3.613786248024553e-08
485777,971555,485777,1457332,1662.8474431037903,2.9756847652606666e-08
486552,973105,486552,1459657,1665.478904247284,2.68664734903723e-08
487326,974653,487326,1461979,1668.3256211280823,2.964588929899037e-08
488101,976203,488101,1464304,1671.0528309345245,2.6231646188534796e-08
488876,977753,488876,1466629,1673.7839081287384,2.0983861759305e-08
489651,979303,489651,1468954,1676.4993999004364,2.2149833966977894e-08
490425,980851,490425,1471276,1679.2572820186615,2.32448655879125e-08
491200,982401,491200,1473601,1682.0291690826416,1.8935679690912366e-08
491975,983951,491975,1475926,1684.763640165329,1.660737325437367e-08
492750,985501,492750,1478251,1687.4539561271667,2.0349034457467496e-08
493525,987051,493525,1480576,1690.1592478752136,1.9523213268257678e-08
494299,988599,494299,1482898,1692.888060092926,1.5455952961929142e-08
495074,990149,495074,1485223,1695.5832269191742,1.8075297703035176e-08
495849,991699,495849,1487548,1698.3278000354767,2.0925654098391533e-08
496624,993249,496624,1489873,1701.0517382621765,1.8575519789010286e-08
497398,994797,497398,1492195,1703.9554262161255,1.7851562006399035e-08
498173,996347,498173,1494520,1706.6526448726654,2.216438588220626e-08
498948,997897,498948,1496845,1709.395262002945,2.355227479711175e-08
499723,999447,499723,1499170,1712.1154351234436,2.072556526400149e-08
500497,1000995,500497,1501492,1714.8233759403229,2.3575921659357846e-08
501272,1002545,501272,1503817,1717.540889263153,2.7783244149759412e-08
502047,1004095,502047,1506142,1720.2667260169983,2.6231646188534796e-08
502822,1005645,502822,1508467,1722.9536740779877,2.6104316930286586e-08
503596,1007193,503596,1510789,1725.650407075882,3.038621798623353e-08
504371,1008743,504371,1513114,1728.4129750728607,3.235982148908079e-08
505146,1010293,505146,1515439,1731.1071560382843,3.0257069738581777e-08
505921,1011843,505921,1517764,1733.7339761257172,3.234526957385242e-08
506696,1013393,506696,1520089,1736.338900089264,3.6781784729100764e-08
507470,1014941,507470,1522411,1738.962720155716,3.552304406184703e-08
508245,1016491,508245,1524736,1741.5715131759644,3.487730282358825e-08
509020,1018041,509020,1527061,1744.1597290039062,3.866625775117427e-08
509795,1019591,509795,1529386,1746.7518842220306,4.024332156404853e-08
510569,1021139,510569,1531708,1749.3666551113129,3.810782800428569e-08
511344,1022689,511344,1534033,1751.969773054123,3.8915459299460053e-08
512119,1024239,512119,1536358,1754.5777008533478,4.2462488636374474e-08
512894,1025789,512894,1538683,1757.1767029762268,4.097637429367751e-08
513668,1027337,513668,1541005,1759.80095911026,3.882814780808985e-08
514443,1028887,514443,1543330,1762.4038531780243,4.140929377172142e-08
515218,1030437,515218,1545655,1765.013482093811,4.186586011201143e-08
515993,1031987,515993,1547980,1767.6220800876617,3.874083631671965e-08
516767,1033535,516767,1550302,1770.2497291564941,3.797686076723039e-08
517542,1035085,517542,1552627,1772.8457689285278,3.980494511779398e-08
518317,1036635,518317,1554952,1775.6856710910797,3.7698555388487875e-08
519092,1038185,519092,1557277,1778.401239156723,3.400054993107915e-08
519866,1039733,519866,1559599,1781.040297985077,3.496461431495845e-08
520641,1041283,520641,1561924,1783.6348259449005,3.468812792561948e-08
521416,1042833,521416,1564249,1786.2818729877472,3.0573573894798756e-08
522191,1044383,522191,1566574,1788.9341180324554,2.8823706088587642e-08
522966,1045933,522966,1568899,1791.5237481594086,2.9602233553305268e-08
523740,1047481,523740,1571221,1794.1104369163513,2.734486770350486e-08
524515,1049031,524515,1573546,1796.8091452121735,2.337219484616071e-08
525290,1050581,525290,1575871,1799.4454910755157,2.3426764528267086e-08
526065,1052131,526065,1578196,1802.058884859085,2.350861905142665e-08
526839,1053679,526839,1580518,1804.6870620250702,1.9615981727838516e-08
527614,1055229,527614,1582843,1807.310429096222,1.780608727131039e-08
528389,1056779,528389,1585168,1809.9230952262878,1.885928213596344e-08
529164,1058329,529164,1587493,1812.5094799995422,1.726948539726436e-08
529938,1059877,529938,1589815,1815.1198060512543,1.4084434951655567e-08
530713,1061427,530713,1592140,1817.7612528800964,1.4348188415169716e-08
531488,1062977,531488,1594465,1820.3975791931152,1.5319528756663203e-08
532263,1064527,532263,1596790,1823.0011761188507,1.2674718163907528e-08
533037,1066075,533037,1599112,1825.6003260612488,1.1401425581425428e-08
533812,1067625,533812,1601437,1828.2172422409058,1.3335011317394674e-08
534587,1069175,534587,1603762,1830.812684059143,1.2994860298931599e-08
535362,1070725,535362,1606087,1833.4502520561218,1.0928488336503506e-08
536137,1072275,536137,1608412,1836.050017118454,1.1990778148174286e-08
536911,1073823,536911,1610734,1838.6952772140503,1.3998942449688911e-08
537686,1075373,537686,1613059,1841.3164329528809,1.2860255083069205e-08
538461,1076923,538461,1615384,1843.8796999454498,1.2400050763972104e-08
539236,1078473,539236,1617709,1846.5039989948273,1.5183104551397264e-08
540010,1080021,540010,1620031,1849.0967218875885,1.617263478692621e-08
540785,1081571,540785,1622356,1851.707675933838,1.5104888007044792e-08
541560,1083121,541560,1624681,1854.3018090724945,1.6827470972202718e-08
542335,1084671,542335,1627006,1856.8756680488586,1.9625076674856246e-08
543109,1086219,543109,1629328,1859.474927186966,1.9501385395415127e-08
543884,1087769,543884,1631653,1862.1450719833374,1.9519575289450586e-08
544659,1089319,544659,1633978,1864.8682749271393,2.2519088815897703e-08
545434,1090869,545434,1636303,1867.3329269886017,2.4130713427439332e-08
546208,1092417,546208,1638625,1869.8474650382996,2.337219484616071e-08
546983,1093967,546983,1640950,1872.3513460159302,2.4880137061700225e-08
547758,1095517,547758,1643275,1874.9700429439545,2.7619535103440285e-08
548533,1097067,548533,1645600,1878.882327079773,2.752130967564881e-08
549308,1098617,549308,1647925,1882.7803809642792,2.7137502911500633e-08
550082,1100165,550082,1650247,1886.6666178703308,2.938577381428331e-08
550857,1101715,550857,1652572,1890.550763130188,3.060631570406258e-08
551632,1103265,551632,1654897,1893.8375749588013,2.9340299079194665e-08
552407,1104815,552407,1657222,1896.2952210903168,2.9762304620817304e-08
553181,1106363,553181,1659544,1898.7100820541382,3.1641320674680173e-08
553956,1107913,553956,1661869,1901.125836133957,3.086279320996255e-08
554731,1109463,554731,1664194,1903.5977311134338,2.9476723284460604e-08
555506,1111013,555506,1666519,1906.053871870041,3.0508090276271105e-08
556280,1112561,556280,1668841,1908.5065560340881,3.086279320996255e-08
557055,1114111,557055,1671166,1911.7695271968842,2.878914528992027e-08
557830,1115661,557830,1673491,1914.2046921253204,2.8008798835799098e-08
558605,1117211,558605,1675816,1916.823646068573,2.8827344067394733e-08
559379,1118759,559379,1678138,1919.3593952655792,2.741035132203251e-08
560154,1120309,560154,1680463,1921.7709078788757,2.5091139832511544e-08
560929,1121859,560929,1682788,1924.2025711536407,2.5120243662968278e-08
561704,1123409,561704,1685113,1926.713723897934,2.482920535840094e-08
562478,1124957,562478,1687435,1929.2732381820679,2.224805939476937e-08
563253,1126507,563253,1689760,1931.7388870716095,2.0749212126247585e-08
564028,1128057,564028,1692085,1934.1810839176178,2.0929292077198625e-08
564803,1129607,564803,1694410,1936.6182680130005,1.9379513105377555e-08
565578,1131157,565578,1696735,1939.058188199997,1.676016836427152e-08
566352,1132705,566352,1699057,1941.4793601036072,1.6378180589526892e-08
567127,1134255,567127,1701382,1943.9794130325317,1.611988409422338e-08
567902,1135805,567902,1703707,1946.48965716362,1.3733369996771216e-08
568677,1137355,568677,1706032,1948.9138140678406,1.2236341717652977e-08
569451,1138903,569451,1708354,1951.31134390831,1.257285475730896e-08
570226,1140453,570226,1710679,1953.741827249527,1.1557858670130372e-08
571001,1142003,571001,1713004,1956.191812992096,9.471477824263275e-09
571776,1143553,571776,1715329,1958.6353740692139,9.405994205735624e-09
572550,1145101,572550,1717651,1961.0487968921661,9.871655493043363e-09
573325,1146651,573325,1719976,1963.449203968048,8.394636097364128e-09
574100,1148201,574100,1722301,1965.8597340583801,7.536073098890483e-09
574875,1149751,574875,1724626,1968.283998966217,8.620190783403814e-09
575649,1151299,575649,1726948,1970.7182312011719,8.618371794000268e-09
576424,1152849,576424,1729273,1973.1269581317902,7.523340173065662e-09
577199,1154399,577199,1731598,1975.548122882843,8.172719390131533e-09
577974,1155949,577974,1733923,1977.9588391780853,9.56606527324766e-09
578749,1157499,578749,1736248,1980.3673431873322,9.185896487906575e-09
579523,1159047,579523,1738570,1982.8007941246033,9.07857611309737e-09
580298,1160597,580298,1740895,1985.2608740329742,1.0863004717975855e-08
581073,1162147,581073,1743220,1987.6891419887543,1.178705133497715e-08
581848,1163697,581848,1745545,1990.7133960723877,1.1465090210549533e-08
582622,1165245,582622,1747867,1995.4645781517029,1.2598320608958602e-08
583397,1166795,583397,1750192,1999.495033979416,1.4528268366120756e-08
584172,1168345,584172,1752517,2002.1752951145172,1.4799297787249088e-08
584947,1169895,584947,1754842,2004.8151681423187,1.5006662579253316e-08
585721,1171443,585721,1757164,2007.3204469680786,1.692387741059065e-08
586496,1172993,586496,1759489,2010.041160106659,1.8175342120230198e-08
587271,1174543,587271,1761814,2014.4834079742432,1.7993443179875612e-08
588046,1176093,588046,1764139,2017.2173252105713,1.8975697457790375e-08
588820,1177641,588820,1766461,2019.783716917038,2.0754669094458222e-08
589595,1179191,589595,1768786,2023.641662120819,2.097476681228727e-08
590370,1180741,590370,1771111,2027.4772679805756,2.0838342607021332e-08
591145,1182291,591145,1773436,2032.008952140808,2.2200765670277178e-08
591920,1183841,591920,1775761,2037.5540130138397,2.3097527446225286e-08
592694,1185389,592694,1778083,2040.9094150066376,2.244087227154523e-08
593469,1186939,593469,1780408,2044.3356540203094,2.267006493639201e-08
594244,1188489,594244,1782733,2047.8490362167358,2.373599272686988e-08
595019,1190039,595019,1785058,2051.6053869724274,2.3370375856757164e-08
595793,1191587,595793,1787380,2055.2977979183197,2.2453605197370052e-08
596568,1193137,596568,1789705,2059.280351161957,2.2886524675413966e-08
597343,1194687,597343,1792030,2062.642212867737,2.3039319785311818e-08
598118,1196237,598118,1794355,2066.618895292282,2.1698724594898522e-08
598892,1197785,598892,1796677,2070.5891880989075,2.0985680748708546e-08
599667,1199335,599667,1799002,2074.4344091415405,2.1233063307590783e-08
600442,1200885,600442,1801327,2078.4973871707916,2.0243533072061837e-08
601217,1202435,601217,1803652,2082.51348900795,1.861371856648475e-08
601991,1203983,601991,1805974,2086.575275182724,1.8268110579811037e-08
602766,1205533,602766,1808299,2090.7866151332855,1.7869751900434494e-08
603541,1207083,603541,1810624,2094.952605009079,1.6123522073030472e-08
604316,1208633,604316,1812949,2099.5947201251984,1.4850229490548372e-08
605090,1210181,605090,1815271,2104.438299894333,1.4673787518404424e-08
605865,1211731,605865,1817596,2109.0159361362457,1.3526005204766989e-08
606640,1213281,606640,1819921,2113.443778038025,1.1730662663467228e-08
607415,1214831,607415,1822246,2117.858983039856,1.1161318980157375e-08
608190,1216381,608190,1824571,2122.149496078491,1.0806616046465933e-08
608964,1217929,608964,1826893,2127.372107028961,9.260475053451955e-09
609739,1219479,609739,1829218,2131.9710490703583,8.107235771603882e-09
610514,1221029,610514,1831543,2135.741697072983,8.119968697428703e-09
611289,1222579,611289,1833868,2139.683396100998,7.452399586327374e-09
612063,1224127,612063,1836190,2145.014429092407,6.119080353528261e-09
612838,1225677,612838,1838515,2149.896196126938,5.9371814131736755e-09
613613,1227227,613613,1840840,2154.5180230140686,6.184563972055912e-09
614388,1228777,614388,1843165,2158.842262029648,5.360561772249639e-09
615162,1230325,615162,1845487,2163.491833925247,4.823959898203611e-09
615937,1231875,615937,1847812,2167.8377940654755,5.458787200041115e-09
616712,1233425,616712,1850137,2172.4419322013855,5.618858267553151e-09
617487,1234975,617487,1852462,2176.863035917282,5.0640664994716644e-09
618261,1236523,618261,1854784,2180.904286146164,5.527908797375858e-09
619036,1238073,619036,1857109,2184.732808113098,6.51016307529062e-09
619811,1239623,619811,1859434,2188.580407142639,6.517439032904804e-09
620586,1241173,620586,1861759,2193.7113020420074,6.6211214289069176e-09
621361,1242723,621361,1864084,2197.782562017441,7.82711140345782e-09
622135,1244271,622135,1866406,2201.970932006836,8.671122486703098e-09
622910,1245821,622910,1868731,2206.1604840755463,8.712959242984653e-09
623685,1247371,623685,1871056,2209.9077639579773,9.567884262651205e-09
624460,1248921,624460,1873381,2213.1929869651794,1.0953954188153148e-08
625234,1250469,625234,1875703,2216.910593032837,1.1408701539039612e-08
626009,1252019,626009,1878028,2220.1674501895905,1.173430064227432e-08
626784,1253569,626784,1880353,2223.584347009659,1.3047610991634429e-08
627559,1255119,627559,1882678,2227.5024840831757,1.4046236174181104e-08
628333,1256667,628333,1885000,2231.137754917145,1.4162651496008039e-08
629108,1258217,629108,1887325,2234.3670332431793,1.485568645875901e-08
629883,1259767,629883,1889650,2237.78378200531,1.6072590369731188e-08
630658,1261317,630658,1891975,2242.033210992813,1.638727553654462e-08
631432,1262865,631432,1894297,2245.5069031715393,1.638727553654462e-08
632207,1264415,632207,1896622,2249.0440080165863,1.7236743588000536e-08
632982,1265965,632982,1898947,2252.3779740333557,1.7842467059381306e-08
633757,1267515,633757,1901272,2255.863466978073,1.752414391376078e-08
634532,1269065,634532,1903597,2259.6011340618134,1.7584170564077795e-08
635306,1270613,635306,1905919,2264.205605983734,1.8184437067247927e-08
636081,1272163,636081,1908244,2269.162405014038,1.7949787434190512e-08
636856,1273713,636856,1910569,2274.1514041423798,1.7304046195931733e-08
637631,1275263,637631,1912894,2279.051768064499,1.7394995666109025e-08
638405,1276811,638405,1915216,2283.68141913414,1.7378624761477113e-08
639180,1278361,639180,1917541,2288.231355905533,1.6450940165668726e-08
639955,1279911,639955,1919866,2292.7585532665253,1.5801560948602855e-08
640730,1281461,640730,1922191,2297.2433140277863,1.5736077330075204e-08
641504,1283009,641504,1924513,2301.8853051662445,1.4984834706410766e-08
642279,1284559,642279,1926838,2306.421198129654,1.3791577657684684e-08
643054,1286109,643054,1929163,2310.951793909073,1.3302269508130848e-08
643829,1287659,643829,1931488,2315.4658901691437,1.2865712051279843e-08
644603,1289207,644603,1933810,2319.938945055008,1.161606633104384e-08
645378,1290757,645378,1936135,2324.521651983261,1.0601070243865252e-08
646153,1292307,646153,1938460,2329.0696489810944,1.0240910341963172e-08
646928,1293857,646928,1940785,2333.575016975403,9.391442290507257e-09
647703,1295407,647703,1943110,2338.061334133148,8.107235771603882e-09
648477,1296955,648477,1945432,2342.5641660690308,7.536073098890483e-09
649252,1298505,649252,1947757,2347.12312912941,7.163180271163583e-09
650027,1300055,650027,1950082,2351.6489431858063,6.1154423747211695e-09
650802,1301605,650802,1952407,2356.2831571102142,5.2532413974404335e-09
651576,1303153,651576,1954729,2360.7726900577545,5.133188096806407e-09
652351,1304703,652351,1957054,2365.3584661483765,4.672983777709305e-09
653126,1306253,653126,1959379,2369.856442928314,3.794411895796657e-09
653901,1307803,653901,1961704,2374.3774342536926,3.5943230614066124e-09
654675,1309351,654675,1964026,2378.969983100891,3.7180143408477306e-09
655450,1310901,655450,1966351,2383.44052195549,3.2669049687683582e-09
656225,1312451,656225,1968676,2387.968015909195,2.9303919291123748e-09
657000,1314001,657000,1971001,2392.4547250270844,3.332388587296009e-09
657774,1315549,657774,1973323,2397.0294840335846,3.523382474668324e-09
658549,1317099,658549,1975648,2401.564512014389,3.2905518310144544e-09
659324,1318649,659324,1977973,2406.0657081604004,3.6325218388810754e-09
660099,1320199,660099,1980298,2410.523325920105,4.349203663878143e-09
660873,1321747,660873,1982620,2414.977280139923,4.529283614829183e-09
661648,1323297,661648,1984945,2419.4757981300354,4.723915481008589e-09
662423,1324847,662423,1987270,2424.0137300491333,5.589754437096417e-09
663198,1326397,663198,1989595,2428.528783082962,6.295522325672209e-09
663973,1327947,663973,1991920,2433.0068459510803,6.51925802230835e-09
664747,1329495,664747,1994242,2437.478741168976,7.172275218181312e-09
665522,1331045,665522,1996567,2442.0443000793457,8.19636625237763e-09
666297,1332595,666297,1998892,2446.6600770950317,8.680217433720827e-09
667072,1334145,667072,2001217,2451.125673055649,9.044015314429998e-09
667846,1335693,667846,2003539,2455.6436760425568,9.968061931431293e-09
668621,1337243,668621,2005864,2460.238617181778,1.075568434316665e-08
669396,1338793,669396,2008189,2464.7532732486725,1.0988514986820519e-08
670171,1340343,670171,2010514,2469.2570979595184,1.150146999862045e-08
670945,1341891,670945,2012836,2473.716975212097,1.2343662092462182e-08
671720,1343441,671720,2015161,2478.2208211421967,1.2658347259275615e-08
672495,1344991,672495,2017486,2482.821130990982,1.2729287846013904e-08
673270,1346541,673270,2019811,2487.2805840969086,1.3258613762445748e-08
674044,1348089,674044,2022133,2491.7528860569,1.3682438293471932e-08
674819,1349639,674819,2024458,2496.242030143738,1.3511453289538622e-08
675594,1351189,675594,2026783,2500.749503135681,1.3511453289538622e-08
676369,1352739,676369,2029108,2505.3138670921326,1.3822500477544963e-08
677144,1354289,677144,2031433,2509.7925980091095,1.3662429410032928e-08
677918,1355837,677918,2033755,2514.2710399627686,1.3182216207496822e-08
678693,1357387,678693,2036080,2518.8136808872223,1.3116732588969171e-08
679468,1358937,679468,2038405,2523.395586013794,1.3002136256545782e-08
680243,1360487,680243,2040730,2527.869104862213,1.2332748156040907e-08
681017,1362035,681017,2043052,2532.3399629592896,1.1768861440941691e-08
681792,1363585,681792,2045377,2536.9233610630035,1.155422069132328e-08
682567,1365135,682567,2047702,2541.458778142929,1.0959411156363785e-08
683342,1366685,683342,2050027,2545.990532875061,1.0051735443994403e-08
684116,1368233,684116,2052349,2550.480310201645,9.5478753792122e-09
684891,1369783,684891,2054674,2554.9797582626343,9.098584996536374e-09
685666,1371333,685666,2056999,2559.524477005005,8.179995347745717e-09
686441,1372883,686441,2059324,2564.096251010895,7.346898200921714e-09
687215,1374431,687215,2061646,2568.6158430576324,6.933987606316805e-09
687990,1375981,687990,2063971,2573.028463125229,6.260961527004838e-09
688765,1377531,688765,2066296,2577.5476381778717,5.318725015968084e-09
689540,1379081,689540,2068621,2582.227005004883,4.782123141922057e-09
690315,1380631,690315,2070946,2586.7615439891815,4.420144250616431e-09
691089,1382179,691089,2073268,2591.2595660686493,3.677996573969722e-09
691864,1383729,691864,2075593,2595.798727989197,3.0249793780967593e-09
692639,1385279,692639,2077918,2600.358561038971,2.837623469531536e-09
693414,1386829,693414,2080243,2604.8640661239624,2.508386387489736e-09
694188,1388377,694188,2082565,2609.366068124771,1.940861693583429e-09
694963,1389927,694963,2084890,2613.87481713295,1.762600732035935e-09
695738,1391477,695738,2087215,2618.380690097809,1.8408172763884068e-09
696513,1393027,696513,2089540,2622.923243999481,1.6025296645238996e-09
697287,1394575,697287,2091862,2627.4600059986115,1.4279066817834973e-09
698062,1396125,698062,2094187,2631.9108521938324,1.7080310499295592e-09
698837,1397675,698837,2096512,2636.380527973175,1.926309778355062e-09
699612,1399225,699612,2098837,2640.8936409950256,1.889929990284145e-09
700386,1400773,700386,2101159,2645.3792049884796,2.1864252630621195e-09
701161,1402323,701161,2103484,2649.8582870960236,2.752130967564881e-09
701936,1403873,701936,2105809,2654.4187021255493,3.0213413992896676e-09
702711,1405423,702711,2108134,2658.9517719745636,3.2796378945931792e-09
703485,1406971,703485,2110456,2663.470216989517,3.938112058676779e-09
704260,1408521,704260,2112781,2667.958894252777,4.549292498268187e-09
705035,1410071,705035,2115106,2672.455075263977,4.858520696870983e-09
705810,1411621,705810,2117431,2677.103073120117,5.40421751793474e-09
706585,1413171,706585,2119756,2681.6738471984863,6.1791070038452744e-09
707359,1414719,707359,2122078,2686.2554030418396,6.655682227574289e-09
708134,1416269,708134,2124403,2690.8453080654144,7.0158421294763684e-09
708909,1417819,708909,2126728,2695.389216184616,7.703420124016702e-09
709684,1419369,709684,2129053,2699.956083059311,8.32369551062584e-09
710458,1420917,710458,2131375,2704.4268250465393,8.594724931754172e-09
711233,1422467,711233,2133700,2708.9351711273193,8.989445632323623e-09
712008,1424017,712008,2136025,2713.4558169841766,9.582436177879572e-09
712783,1425567,712783,2138350,2717.9750809669495,9.862560546025634e-09
713557,1427115,713557,2140672,2722.555022239685,9.948053047992289e-09
714332,1428665,714332,2142997,2727.023542165756,1.0288204066455364e-08
715107,1430215,715107,2145322,2731.5582370758057,1.0562871466390789e-08
715882,1431765,715882,2147647,2736.0620832443237,1.047010300680995e-08
716656,1433313,716656,2149969,2740.59742808342,1.0422809282317758e-08
717431,1434863,717431,2152294,2745.095188140869,1.0561052476987243e-08
718206,1436413,718206,2154619,2749.6640362739563,1.0410076356492937e-08
718981,1437963,718981,2156944,2754.1477591991425,1.003536453936249e-08
719756,1439513,719756,2159269,2758.6513962745667,9.877112461254e-09
720530,1441061,720530,2161591,2763.240662097931,9.704308467917144e-09
721305,1442611,721305,2163916,2767.7522649765015,9.182258509099483e-09
722080,1444161,722080,2166241,2772.2757132053375,8.682036423124373e-09
722855,1445711,722855,2168566,2776.8132400512695,8.39827407617122e-09
723629,1447259,723629,2170888,2781.342038154602,7.896233000792563e-09
724404,1448809,724404,2173213,2785.852485895157,7.183189154602587e-09
725179,1450359,725179,2175538,2790.368443965912,6.693881005048752e-09
725954,1451909,725954,2177863,2794.917077064514,6.26459950581193e-09
726728,1453457,726728,2180185,2799.367926120758,5.555193638429046e-09
727503,1455007,727503,2182510,2803.9016740322113,4.880348569713533e-09
728278,1456557,728278,2184835,2808.4169640541077,4.461981006897986e-09
729053,1458107,729053,2187160,2812.9658608436584,3.927198122255504e-09
729827,1459655,729827,2189482,2817.472995042801,3.219611244276166e-09
730602,1461205,730602,2191807,2821.968369960785,2.7539499569684267e-09
731377,1462755,731377,2194132,2826.4886910915375,2.4283508537337184e-09
732152,1464305,732152,2196457,2831.036728143692,1.8953869584947824e-09
732927,1465855,732927,2198782,2835.620947122574,1.407897798344493e-09
733701,1467403,733701,2201104,2840.1132550239563,1.216903910972178e-09
734476,1468953,734476,2203429,2844.692458152771,9.840732673183084e-10
735251,1470503,735251,2205754,2849.2079181671143,6.093614501878619e-10
736026,1472053,736026,2208079,2853.70321893692,4.747562343254685e-10
736800,1473601,736800,2210401,2858.1508009433746,5.238689482212067e-10
737575,1475151,737575,2212726,2862.7185311317444,4.147295840084553e-10
738350,1476701,738350,2215051,2867.2629430294037,3.3287506084889174e-10
739125,1478251,739125,2217376,2871.7518990039825,5.475158104673028e-10
739899,1479799,739899,2219698,2876.38503408432,7.548806024715304e-10
740674,1481349,740674,2222023,2880.9075951576233,8.203642209991813e-10
741449,1482899,741449,2224348,2885.4713549613953,1.0822986951097846e-09
742224,1484449,742224,2226673,2890.02325296402,1.5261321095749736e-09
742998,1485997,742998,2228995,2894.5820429325104,1.8189894035458565e-09
743773,1487547,743773,2231320,2899.1100239753723,2.0881998352706432e-09
744548,1489097,744548,2233645,2903.586959838867,2.610249794088304e-09
745323,1490647,745323,2235970,2908.084860086441,3.1213858164846897e-09
746098,1492197,746098,2238295,2912.569230079651,3.4524418879300356e-09
746872,1493745,746872,2240617,2917.0358250141144,3.901732270605862e-09
747647,1495295,747647,2242942,2921.5453090667725,4.507455741986632e-09
748422,1496845,748422,2245267,2926.075931072235,4.933099262416363e-09
749197,1498395,749197,2247592,2930.5744829177856,5.275069270282984e-09
749971,1499943,749971,2249914,2935.0724959373474,5.791662260890007e-09
750746,1501493,750746,2252239,2939.541831970215,6.282789399847388e-09
751521,1503043,751521,2254564,2944.0434839725494,6.548361852765083e-09
752296,1504593,752296,2256889,2948.535675048828,6.859409040771425e-09
753070,1506141,753070,2259211,2953.017170906067,7.285052561201155e-09
753845,1507691,753845,2261536,2957.4882559776306,7.516064215451479e-09
754620,1509241,754620,2263861,2961.9684591293335,7.605194696225226e-09
755395,1510791,755395,2266186,2966.5554740428925,7.818016456440091e-09
756169,1512339,756169,2268508,2971.1176199913025,7.999915396794677e-09
756944,1513889,756944,2270833,2975.60573387146,7.93261278886348e-09
757719,1515439,757719,2273158,2980.1211149692535,7.86712917033583e-09
758494,1516989,758494,2275483,2984.728908061981,7.899870979599655e-09
759268,1518537,759268,2277805,2989.237370967865,7.763446774333715e-09
760043,1520087,760043,2280130,2993.6680541038513,7.456037565134466e-09
760818,1521637,760818,2282455,2998.1523790359497,7.263224688358605e-09
761593,1523187,761593,2284780,3002.6383199691772,7.057678885757923e-09
762368,1524737,762368,2287105,3007.162068128586,6.6356733441352844e-09
763142,1526285,763142,2289427,3011.6413702964783,6.2045728554949164e-09
763917,1527835,763917,2291752,3016.1111590862274,5.895344656892121e-09
764692,1529385,764692,2294077,3020.6602811813354,5.4678821470588446e-09
765467,1530935,765467,2296402,3025.125888109207,4.893081495538354e-09
766241,1532483,766241,2298724,3029.6471519470215,4.443791112862527e-09
767016,1534033,767016,2301049,3034.351683139801,4.043613444082439e-09
767791,1535583,767791,2303374,3038.9575419425964,3.4797267289832234e-09
768566,1537133,768566,2305699,3043.5254039764404,2.9249349609017372e-09
769340,1538681,769340,2308021,3048.0572440624237,2.5374902179464698e-09
770115,1540231,770115,2310346,3052.5682549476624,2.091837814077735e-09
770890,1541781,770890,2312671,3057.067466020584,1.5497789718210697e-09
771665,1543331,771665,2314996,3061.5271339416504,1.1514202924445271e-09
772439,1544879,772439,2317318,3066.069405078888,8.62200977280736e-10
773214,1546429,773214,2319643,3070.6150500774384,4.656612873077393e-10
773989,1547979,773989,2321968,3075.100857257843,9.822542779147625e-11


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0024199485778808594,12064.682476916567
2002,2003,2002,4005,5.172716856002808,60.659557687866254
4004,4005,4004,8009,10.17728304862976,40.01013285976478
6006,6007,6006,12013,15.386091947555542,32.122823954647174
8008,8009,8008,16017,20.587572813034058,27.232249265985956
10010,10011,10010,20021,25.848038911819458,23.709264738188722
12012,12013,12012,24025,30.755960702896118,20.97624637750596
14014,14015,14014,28029,35.772347927093506,18.762942711508003
16016,16017,16016,32033,40.77490568161011,16.921908606920624
18018,18019,18018,36037,45.719876766204834,15.3630753883117
20020,20021,20020,40041,50.87304377555847,14.026422174050822
22022,22023,22022,44045,55.86635184288025,12.869279116112011
24024,24025,24024,48049,60.838228940963745,11.859884815996338
26026,26027,26026,52053,65.72886991500854,10.973807613236204
28028,28029,28028,56057,70.45732498168945,10.191772110585589
30030,30031,30030,60061,75.28628993034363,9.49831038087541
32032,32033,32032,64065,80.07366991043091,8.880821937249493
34034,34035,34034,68069,84.80838084220886,8.32891496922457
36036,36037,36036,72073,89.51976585388184,7.833935179643959
38038,38039,38038,76077,94.2336368560791,7.388610457366667
40040,40041,40040,80081,98.95079493522644,6.986782983762168
42042,42043,42042,84085,103.68086981773376,6.62320315895704
44044,44045,44044,88089,108.36869883537292,6.29336894071821
46046,46047,46046,92093,113.09729790687561,5.993399070212035
48048,48049,48048,96097,117.77982783317566,5.7199319244773505
50050,50051,50050,100101,122.51098275184631,5.470043981698836
52052,52053,52052,104105,127.17121362686157,5.241183463827838
54054,54055,54054,108109,131.89265203475952,5.031115848094487
56056,56057,56056,112113,136.58025193214417,4.837878754167832
58058,58059,58058,116117,141.3129117488861,4.659744309799862
60060,60061,60060,120121,146.00278973579407,4.495187537451784
62062,62063,62062,124125,150.69809579849243,4.342859631875399
64064,64065,64064,128129,155.48066091537476,4.201565244247831
66066,66067,66066,132133,160.13977909088135,4.0702430743695
68068,68069,68068,136137,164.84128093719482,3.947949214345499
70070,70071,70070,140141,169.5170590877533,3.83384279620077
72072,72073,72072,144145,174.28276681900024,3.7271735806662036
74074,74075,74074,148149,178.9806158542633,3.6272721958848706
76076,76077,76076,152153,183.6696548461914,3.53353834322661
78078,78079,78078,156157,188.4683277606964,3.445433793713164
80080,80081,80080,160161,193.34247875213623,3.3624761818246043
82082,82083,82082,164165,198.04426169395447,3.2842320765794284
84084,84085,84084,168169,202.82017874717712,3.210311494196503
86086,86087,86086,172173,207.5563247203827,3.140363075232017
88088,88089,88088,176177,212.2366750240326,3.074069839265576
90090,90091,90090,180181,217.0563566684723,3.011145442724228
92092,92093,92092,184185,221.77789902687073,2.9513308758487256
94094,94095,94094,188189,226.48492789268494,2.8943915437066607
96096,96097,96096,192193,231.19119477272034,2.840114683553111
98098,98099,98098,196197,235.92206001281738,2.7883070772695646
100100,100101,100100,200201,240.61104893684387,2.738793022943355
102102,102103,102102,204205,245.34230089187622,2.691412534448318
104104,104105,104104,208209,250.0317039489746,2.646019741678174
106106,106107,106106,212213,254.81864285469055,2.602481467751204
108108,108109,108108,216217,259.56136870384216,2.5606759623242397
110110,110111,110110,220221,264.31130599975586,2.5204917728224245
112112,112113,112112,224225,268.9788227081299,2.4818267375703726
114114,114115,114114,228229,273.68713784217834,2.444587086867614
116116,116117,116116,232233,278.36722683906555,2.408686639580992
118118,118119,118118,236237,283.12001299858093,2.3740460844965128
120120,120121,120120,240241,288.0113537311554,2.3405923368300137
122122,122123,122122,244245,292.8991389274597,2.3082579615002032
124124,124125,124124,248249,297.59548687934875,2.276980655711668
126126,126127,126126,252253,302.31019496917725,2.2467027843285905
128128,128129,128128,256257,307.0411629676819,2.2173709622347815
130130,130131,130130,260261,312.0076367855072,2.188935678534108
132132,132133,132132,264265,316.931129693985,2.161351008073325
134134,134135,134134,268269,321.87547278404236,2.1345742730918573
136136,136137,136136,272273,326.830689907074,2.1085655631977716
138138,138139,138138,276277,331.78523993492126,2.083287795738215
140140,140141,140140,280281,336.43759274482727,2.0587063696129917
142142,142143,142142,284285,340.9312376976013,2.034788961527738
144144,144145,144144,288289,345.38750100135803,2.0115053414428985
146146,146147,146146,292293,349.8347098827362,1.9888272051666718
148148,148149,148148,296297,354.3421368598938,1.9667280223657144
150150,150151,150150,300301,358.7761697769165,1.9451828983583255
152152,152153,152152,304305,363.3234508037567,1.9241684484150028
154154,154155,154154,308309,367.81097984313965,1.9036626832057664
156156,156157,156156,312313,372.3192718029022,1.8836449043810717
158158,158159,158158,316317,376.8059628009796,1.864095609249489
160160,160161,160160,320321,381.2854928970337,1.8449964036772144
162162,162163,162162,324325,385.79009985923767,1.8263299224126968
164164,164165,164164,328329,390.32827496528625,1.8080797561506188
166166,166167,166166,332333,394.7906799316406,1.79023038466039
168168,168169,168168,336337,399.2742488384247,1.772767115448005
170170,170171,170170,340341,404.05829882621765,1.7556760274110275
172172,172173,172172,344345,408.5186779499054,1.7389439190428675
174174,174175,174174,348349,412.9988007545471,1.7225583894924057
176176,176177,176176,352353,417.39266777038574,1.7065075560640253
178178,178179,178178,356357,421.96313977241516,1.6907799361633806
180180,180181,180180,360361,426.44036197662354,1.6753647669811471
182182,182183,182182,364365,430.8607428073883,1.6602518012787186
184184,184185,184184,368369,435.3015558719635,1.6454312754412967
186186,186187,186186,372373,439.8396170139313,1.6308938799375028
188188,188189,188188,376377,444.3333878517151,1.6166307319199404
190190,190191,190190,380381,448.76127195358276,1.6026333498321037
192192,192193,192192,384385,453.39943385124207,1.5888936298288172
194194,194195,194194,388389,457.9937627315521,1.5754038238846988
196196,196197,196196,392393,462.41339087486267,1.5621565194142022
198198,198199,198198,396397,466.8201730251312,1.5491446203395753
200200,200201,200200,400401,471.5895879268646,1.5363613294102834
202202,202203,202202,404405,476.2631359100342,1.5238001317684393
204204,204205,204204,408409,480.7883110046387,1.5114547795783437
206206,206207,206206,412413,485.38422989845276,1.499319277701943
208208,208209,208208,416417,490.39082980155945,1.4873878702819638
210210,210211,210210,420421,495.035826921463,1.4756550282218086
212212,212213,212212,424425,499.61464500427246,1.4641154374512553
214214,214215,214214,428429,504.4472498893738,1.4527639879343042
216216,216217,216216,432433,509.4147448539734,1.441595763377336
218218,218219,218218,436437,514.4516479969025,1.430606031555726
220220,220221,220220,440441,519.4096279144287,1.4197902352516394
222222,222223,222222,444445,524.3104927539825,1.40914398372297
224224,224225,224224,448449,529.0412929058075,1.3986630447034258
226226,226227,226226,452453,533.7500488758087,1.3883433368464466
228228,228229,228228,456457,538.409138917923,1.3781809226420592
230230,230231,230230,460461,543.0932638645172,1.3681720017357293
232232,232233,232232,464465,547.7499897480011,1.3583129046128306
234234,234235,234234,468469,552.4804139137268,1.3486000866632821
236236,236237,236236,472473,557.181765794754,1.3390301225754229
238238,238239,238238,476477,561.8875119686127,1.3295997010263818
240240,240241,240240,480481,566.5442008972168,1.320305619681676
242242,242243,242242,484485,571.1893849372864,1.3111447804585623
244244,244245,244244,488489,575.8557648658752,1.3021141850495042
246246,246247,246246,492493,580.5159428119659,1.2932109306748316
248248,248249,248248,496497,585.1758139133453,1.2844322060682316
250250,250251,250250,500501,589.8485717773438,1.2757752876696031
252252,252253,252252,504505,594.5028438568115,1.2672375360161823
254254,254255,254254,508509,599.1448707580566,1.2588163923082902
256256,256257,256256,512513,603.8060920238495,1.2505093751697132
258258,258259,258258,516517,608.6617708206177,1.2423140775463253
260260,260261,260260,520521,613.5248649120331,1.234228163773878
262262,262263,262262,524525,618.1910746097565,1.2262493667949457
264264,264265,264264,528529,622.8730418682098,1.2183754854941071
266266,266267,266266,532533,627.6471128463745,1.2106043821695494
268268,268269,268268,536537,632.3013107776642,1.202934153698152
270270,270271,270270,540541,637.0600759983063,1.1953626175982208
272272,272273,272272,544545,641.7243218421936,1.1878878010356857
274274,274275,274274,548549,646.3962647914886,1.1805077970748243
276276,276277,276276,552553,651.1146759986877,1.173220751243207
278278,278279,278278,556557,655.7257947921753,1.16602485963449
280280,280281,280280,560561,660.3696568012238,1.1589183670912462
282282,282283,282282,564565,665.0342099666595,1.151899565489657
284284,284285,284284,568569,669.6538558006287,1.1449667920660431
286286,286287,286286,572573,674.3150749206543,1.1381184278561705
288288,288289,288288,576577,678.9854609966278,1.131352896165481
290290,290291,290290,580581,683.7026789188385,1.124668661135729
292292,292293,292292,584585,688.3547866344452,1.1180642263516347
294294,294295,294294,588589,693.0857207775116,1.1115381335239363
296296,296297,296296,592593,697.753476858139,1.1050889612033643
298298,298299,298298,596597,702.6349680423737,1.0987153235892038
300300,300301,300300,600601,707.378616809845,1.092415869328761
302302,302303,302302,604605,712.0587389469147,1.0861892804277886
304304,304305,304304,608609,716.7120356559753,1.0800342711645499
306306,306307,306306,612613,721.4807198047638,1.0739495870548126
308308,308309,308308,616617,726.1133780479431,1.0679340038659575
310310,310311,310310,620621,730.7672169208527,1.0619863266729226
312312,312313,312312,624625,735.4493837356567,1.0561053889396135
314314,314315,314314,628629,740.1438248157501,1.0502900516348745
316316,316317,316316,632633,744.8246319293976,1.0445392024066678
318318,318319,318318,636637,749.7022426128387,1.0388517547507945
320320,320321,320320,640641,754.4954669475555,1.033226647243282
322322,322323,322322,644645,759.1546258926392,1.027662842783684
324324,324325,324324,648649,763.8460879325867,1.0221593278838554
326326,326327,326326,652653,768.516863822937,1.016715111945814
328328,328329,328328,656657,773.332879781723,1.0113292266214557
330330,330331,330330,660661,778.0000047683716,1.006000725141348
332332,332333,332332,664665,782.6441359519958,1.0007286817126442
334334,334335,334334,668669,787.2837629318237,0.9955121909024456
336336,336337,336336,672673,791.9317367076874,0.9903503670720966
338338,338339,338338,676677,796.5961027145386,0.9852423438060214
340340,340341,340340,680681,801.30402302742,0.9801872733787604
342342,342343,342342,684685,805.9291026592255,0.9751843262420152
344344,344345,344344,688689,810.8498198986053,0.9702326905080554
346346,346347,346346,692693,815.6836709976196,0.9653315714858763
348348,348349,348348,696697,820.3886368274689,0.9604801911827963
350350,350351,350350,700701,825.0294208526611,0.9556777878806315
352352,352353,352352,704705,829.7076318264008,0.9509236156845873
354354,354355,354354,708709,834.4448037147522,0.946216944103071
356356,356357,356356,712713,839.1285088062286,0.9415570576402388
358358,358359,358358,716717,843.7914397716522,0.9369432553939987
360360,360361,360360,720721,848.4395010471344,0.932374850688575
362362,362363,362362,724725,853.0795028209686,0.9278511706888821
364364,364365,364364,728729,857.7003738880157,0.9233715560549172
366366,366367,366366,732733,862.4178128242493,0.9189353605834185
368368,368369,368368,736737,867.1766629219055,0.914541950884086
370370,370371,370370,740741,871.984885931015,0.9101907060467056
372372,372373,372372,744745,876.6599538326263,0.9058810173319216
374374,374375,374374,748749,881.3133890628815,0.9016122878601891
376376,376377,376376,752753,886.0971558094025,0.8973839323189168
378378,378379,378378,756757,890.75221991539,0.8931953766841616
380380,380381,380380,760761,895.4906878471375,0.8890460579259525
382382,382383,382382,764765,900.1400289535522,0.8849354237590887
384384,384385,384384,768769,904.796868801117,0.8808629323648347
386386,386387,386386,772773,909.4653129577637,0.8768280521453562
388388,388389,388388,776777,914.0924398899078,0.8728302614854329
390390,390391,390390,780781,918.744414806366,0.8688690484923427
392392,392393,392392,784785,923.438071012497,0.8649439107939543
394394,394395,394394,788789,928.2786726951599,0.8610543552840682
396396,396397,396396,792793,933.0997738838196,0.857199897931423
398398,398399,398398,796797,937.7471768856049,0.8533800635486841
400400,400401,400400,800801,942.4403088092804,0.8495943855905352
402402,402403,402402,804805,947.1006078720093,0.845842405960866
404404,404405,404404,808809,951.9225389957428,0.842123674821778
406406,406407,406406,812813,956.570506811142,0.8384377503807627
408408,408409,408408,816817,961.2389848232269,0.834784198736088
410410,410411,410410,820821,965.8648838996887,0.8311625936839846
412412,412413,412412,824825,970.5104019641876,0.8275725165476615
414414,414415,414414,828829,975.2861549854279,0.8240135560081399
416416,416417,416416,832833,979.9538547992706,0.8204853079405439
418418,418419,418418,836837,984.6948857307434,0.8169873752631247
420420,420421,420420,840841,989.3410978317261,0.8135193677608186
422422,422423,422422,844845,994.0158467292786,0.8100809019579174
424424,424425,424424,848849,998.6874878406525,0.8066716009598167
426426,426427,426426,852853,1003.3254647254944,0.8032910943129536
428428,428429,428428,856857,1008.1348979473114,0.7999390178556496
430430,430431,430430,860861,1012.9378659725189,0.796615013599876
432432,432433,432432,864865,1017.6105048656464,0.7933187295839161
434434,434435,434434,868869,1022.4016849994659,0.790049819761407
436436,436437,436436,872873,1027.037977695465,0.7868079438521818
438438,438439,438438,876877,1031.8803668022156,0.7835927672422258
440440,440441,440440,880881,1036.5449159145355,0.7804039608508901
442442,442443,442442,884885,1041.2361946105957,0.7772412010272092
444444,444445,444444,888889,1045.9294548034668,0.7741041694280284
446446,446447,446446,892893,1050.5844888687134,0.7709925529015891
448448,448449,448448,896897,1055.2781088352203,0.7679060434020357
450450,450451,450450,900901,1059.91947889328,0.7648443378657248
452452,452453,452452,904905,1064.596291065216,0.7618071381148184
454454,454455,454454,908909,1069.2512118816376,0.7587941507681535
456456,456457,456456,912913,1073.9104309082031,0.755805087123008
458458,458459,458458,916917,1078.573865890503,0.7528396630841598
460460,460461,460460,920921,1083.2425520420074,0.7498975990456529
462462,462463,462462,924925,1087.9283850193024,0.7469786198362272
464464,464465,464464,928929,1092.591373682022,0.7440824545919895
466466,466467,466466,932933,1097.2412610054016,0.7412088367036631
468468,468469,468468,936937,1101.9237208366394,0.7383575037074479
470470,470471,470470,940941,1106.5770030021667,0.735528197230451
472472,472473,472472,944945,1111.2213706970215,0.7327206628760905
474474,474475,474474,948949,1115.8924448490143,0.7299346501913533
476476,476477,476476,952953,1120.5632548332214,0.7271699125376472
478478,478479,478478,956957,1125.2131807804108,0.7244262070726109
480480,480481,480480,960961,1129.8408498764038,0.7217032946264226
482482,482483,482482,964965,1134.517068862915,0.7190009396708774
484484,484485,484484,968969,1139.1597917079926,0.7163189102266188
486486,486487,486486,972973,1143.8224868774414,0.7136569778031117
488488,488489,488488,976977,1148.5849027633667,0.7110149173386162
490490,490491,490490,980981,1153.49329996109,0.708392507125609
492492,492493,492492,984985,1158.108981847763,0.7057895739853848
494494,494495,494494,988989,1162.795738697052,0.7032058642289485
496496,496497,496496,992993,1167.444524049759,0.7006411587281036
498498,498499,498498,996997,1172.0982949733734,0.698095248597383
500501,500502,500501,1001003,1176.8449668884277,0.6955666702251619
502503,502504,502503,1005007,1181.5380418300629,0.6930577454986633
504505,504506,504505,1009011,1186.223639011383,0.6905670075175294
506507,506508,506507,1013015,1190.8903639316559,0.6880942593106738
508509,508510,508509,1017019,1195.540267944336,0.6856393067355384
510511,510512,510511,1021023,1200.3979749679565,0.683201958438076
512513,512514,512513,1025027,1205.1801946163177,0.6807820258145512
514515,514516,514515,1029031,1210.0953719615936,0.6783793229406001
516517,516518,516517,1033035,1214.8797647953033,0.6759936665384885
518519,518520,518519,1037039,1219.5170948505402,0.6736248759243608
520521,520522,520521,1041043,1224.222039937973,0.6712727729627659
522523,522524,522523,1045047,1228.9095387458801,0.6689371820211818
524525,524526,524525,1049051,1233.6153600215912,0.6666179299318173
526527,526528,526527,1053055,1238.3745830059052,0.6643148459388613
528529,528530,528529,1057059,1243.0673768520355,0.6620277616566455
530531,530532,530531,1061063,1247.7044270038605,0.6597567888566118
532533,532534,532533,1065067,1252.3975937366486,0.6575017478335212
534535,534536,534535,1069071,1257.0911569595337,0.6552622127728682
536537,536538,536537,1073075,1261.9705348014832,0.6530380238073121
538539,538540,538539,1077079,1267.1222758293152,0.6508290235015011
540541,540542,540541,1081083,1272.0703349113464,0.6486350567247428
542543,542544,542543,1085087,1276.818282842636,0.6464559705345891
544545,544546,544545,1089091,1281.4993579387665,0.6442916140949819
546547,546548,546547,1093095,1286.2461559772491,0.6421418386398727
548549,548550,548549,1097099,1290.940016746521,0.6400064974113775
550551,550552,550551,1101103,1295.6373329162598,0.6378854456324916
552553,552554,552553,1105107,1300.290991783142,0.6357785697509826
554555,554556,554555,1109111,1304.9719789028168,0.6336861877607589
556557,556558,556557,1113115,1309.6656110286713,0.6316076709699701
558559,558560,558559,1117119,1314.3618278503418,0.6295428808189172
560561,560562,560561,1121123,1319.0469329357147,0.6274916813799791
562563,562564,562563,1125127,1323.728938817978,0.6254539388355624
564565,564566,564565,1129131,1328.3751428127289,0.6234295212234429
566567,566568,566567,1133135,1333.036367893219,0.6214182983621868
568569,568570,568569,1137139,1337.669065952301,0.6194201417802105
570571,570572,570571,1141143,1342.4198677539825,0.6174349246757629
572573,572574,572573,1145147,1347.0880329608917,0.6154625218860019
574575,574576,574575,1149151,1351.8378999233246,0.6135028098597104
576577,576578,576577,1153155,1356.5417199134827,0.6115556666281918
578579,578580,578579,1157159,1361.2214078903198,0.6096209717816237
580581,580582,580581,1161163,1365.8840289115906,0.6076986064508674
582583,582584,582583,1165167,1370.5450019836426,0.6057884532638127
584585,584586,584585,1169171,1375.193205833435,0.6038903963417397
586587,586588,586587,1173175,1379.8531308174133,0.6020043212629389
588589,588590,588589,1177179,1384.504109621048,0.6001301150427025
590591,590592,590591,1181183,1389.1815128326416,0.5982676661205915
592593,592594,592593,1185187,1393.8724510669708,0.5964168643240555
594595,594596,594595,1189191,1398.5260426998138,0.5945776008466055
596597,596598,596597,1193195,1403.2093107700348,0.5927497682459943
598599,598600,598599,1197199,1407.9872777462006,0.5909332603969233
600601,600602,600601,1201203,1412.6532537937164,0.5891279831848806
602603,602604,602603,1205207,1417.3133277893066,0.5873338292240078
604605,604606,604605,1209211,1421.956414937973,0.5855506895659346
606607,606608,606607,1213215,1426.6389486789703,0.5837784631821705
608609,608610,608609,1217219,1431.4347069263458,0.582017050275681
610611,610612,610611,1221223,1436.2134518623352,0.5802663522626972
612613,612614,612613,1225227,1440.8628509044647,0.5785262717581645
614615,614616,614615,1229231,1445.5614190101624,0.5767967125484574
616617,616618,616617,1233235,1450.2625379562378,0.5750775795841037
618619,618620,618619,1237239,1454.925316810608,0.5733687789579562
620621,620622,620621,1241243,1459.6795568466187,0.5716702178797277
622623,622624,622623,1245247,1464.3710038661957,0.5699818046796281
624625,624626,624625,1249251,1469.0291018486023,0.5683034487665282
626627,626628,626627,1253255,1473.7424638271332,0.5666350606315973
628629,628630,628629,1257259,1478.3872158527374,0.5649765518264758
630631,630632,630631,1261263,1483.096650838852,0.5633278349378088
632633,632634,632633,1265267,1487.7696540355682,0.5616888235854276
634635,634636,634635,1269271,1492.4245097637177,0.5600594324041595
636637,636638,636637,1273275,1497.090539932251,0.5584395770201809
638639,638640,638639,1277279,1501.7714607715607,0.5568291740546556
640641,640642,640641,1281283,1506.4445617198944,0.5552281410818978
642643,642644,642643,1285287,1511.1164238452911,0.553636396640286
644645,644646,644645,1289291,1515.782450914383,0.5520538602140732
646647,646648,646647,1293295,1520.4314849376678,0.5504804522024642
648649,648650,648649,1297299,1525.1435968875885,0.5489160939305293
650651,650652,650651,1301303,1529.9334697723389,0.5473607076146436
652653,652654,652653,1305307,1534.8150808811188,0.545814216369763
654655,654656,654655,1309311,1539.4454357624054,0.5442765441748634
656657,656658,656657,1313315,1544.132019996643,0.5427476158838545
658659,658660,658659,1317319,1548.824623823166,0.5412273571910191
660661,660662,660661,1321323,1553.6997587680817,0.5397156946346513
662663,662664,662663,1325327,1558.510776758194,0.5382125555788662
664665,664666,664665,1329331,1563.178645849228,0.5367178682045051
666667,666668,666667,1333335,1567.9506497383118,0.5352315614945837
668669,668670,668669,1337339,1572.9449808597565,0.5337535652251972
670671,670672,670671,1341343,1577.8541827201843,0.5322838099527871
672673,672674,672673,1345347,1582.601542711258,0.5308222270068654
674675,674676,674675,1349351,1587.4177577495575,0.5293687484791008
676677,676678,676677,1353355,1592.193060874939,0.5279233072033094
678679,678680,678679,1357359,1596.8944878578186,0.5264858367572742
680681,680682,680681,1361363,1601.5978360176086,0.525056271450012
682683,682684,682683,1365367,1606.2842197418213,0.5236345463054022
684685,684686,684685,1369371,1610.9681327342987,0.5222205970585492
686687,686688,686687,1373375,1615.6838908195496,0.5208143601466872
688689,688690,688689,1377379,1620.326239824295,0.5194157726909907
690691,690692,690691,1381383,1625.0662457942963,0.5180247724965739
692693,692694,692693,1385387,1629.7469367980957,0.5166412980433961
694695,694696,694695,1389391,1634.4088797569275,0.5152652884717099
696697,696698,696697,1393395,1639.1387848854065,0.5138966835693282
698699,698700,698699,1397399,1644.081367969513,0.5125354237807187
700701,700702,700701,1401403,1648.8433117866516,0.5111814501742629
702703,702704,702703,1405407,1653.5139698982239,0.5098347044568072
704705,704706,704705,1409411,1658.2185699939728,0.5084951289445598
706707,706708,706707,1413415,1662.9036538600922,0.5071626665776421
708709,708710,708709,1417419,1667.5488197803497,0.5058372608873469
710711,710712,710711,1421423,1672.2424788475037,0.5045188560034148
712713,712714,712713,1425427,1676.8884580135345,0.5032073966449389
714715,714716,714715,1429431,1681.5999248027802,0.5019028281112696
716717,716718,716717,1433435,1686.2412867546082,0.5006050962747395
718719,718720,718719,1437439,1690.8932039737701,0.4993141475661105
720721,720722,720721,1441443,1695.5503208637238,0.49802992897457443
722723,722724,722723,1445447,1700.1956977844238,0.4967523880513909
724725,724726,724725,1449451,1704.8564517498016,0.4954814728753263
726727,726728,726727,1453455,1709.5380578041077,0.49421713206720597
728729,728730,728729,1457459,1714.2414288520813,0.4929593147808191
730731,730732,730731,1461463,1718.9100768566132,0.49170797068290995
732733,732734,732733,1465467,1723.5568189620972,0.49046304996227263
734735,734736,734735,1469471,1728.357349872589,0.4892245033188374
736737,736738,736737,1473475,1733.1665179729462,0.4879922819472995
738739,738740,738739,1477479,1737.834378004074,0.48676633754439536
740741,740742,740741,1481483,1742.5537989139557,0.4855466222979885
742743,742744,742743,1485487,1747.2394287586212,0.4843330888706987
744745,744746,744745,1489491,1751.931447982788,0.48312569041445386
746747,746748,746747,1493495,1756.7122938632965,0.4819243805432052
748749,748750,748749,1497499,1761.4195828437805,0.4807291133402032
750751,750752,750751,1501503,1766.0675067901611,0.47953984334708366
752753,752754,752753,1505507,1770.7199838161469,0.4783565255620488
754755,754756,754755,1509511,1775.4081280231476,0.4771791154271341
756757,756758,756757,1513515,1780.1476888656616,0.47600756883548456
758759,758760,758759,1517519,1784.8835628032684,0.4748418421095266
760761,760762,760761,1521523,1789.5655386447906,0.4736818920046062
762763,762764,762763,1525527,1794.2431390285492,0.4725276757053507
764765,764766,764765,1529531,1798.909117937088,0.4713791508147551
766767,766768,766767,1533535,1803.5958907604218,0.470236275356001
768769,768770,768769,1537539,1808.2626519203186,0.46909900775972346
770771,770772,770771,1541543,1812.933974981308,0.4679673068658303
772773,772774,772773,1545547,1817.6174988746643,0.46684113191076904
774775,774776,774775,1549551,1822.2810130119324,0.4657204425329837
776777,776778,776777,1553555,1826.9726629257202,0.4646051987529063
778779,778780,778779,1557559,1831.687847852707,0.4634953609893273
780781,780782,780781,1561563,1836.3466138839722,0.4623908900339302
782783,782784,782783,1565567,1841.0295288562775,0.4612917470640241
784785,784786,784785,1569571,1845.746610879898,0.46019789362071606
786787,786788,786787,1573575,1850.4230227470398,0.45910929161800595
788789,788790,788789,1577579,1855.1288130283356,0.45802590333369153
790791,790792,790791,1581583,1859.7534000873566,0.45694769140573044
792793,792794,792793,1585587,1864.562032699585,0.45587461883042124
794795,794796,794795,1589591,1869.3386437892914,0.4548066489460325
796797,796798,796797,1593595,1873.9905018806458,0.45374374544917373
798799,798800,798799,1597599,1878.640707731247,0.45268587236751046
800801,800802,800801,1601603,1883.3278529644012,0.4516329940797732
802803,802804,802803,1605607,1888.0074009895325,0.45058507529211056
804805,804806,804805,1609611,1892.7875907421112,0.4495420810399082
806807,806808,806807,1613615,1897.4312357902527,0.44850397669142694
808809,808810,808809,1617619,1902.1387798786163,0.4474707279368886
810811,810812,810811,1621623,1906.79590177536,0.44644230078301916
812813,812814,812813,1625627,1911.4909608364105,0.44541866155486787
814815,814816,814815,1629631,1916.2655427455902,0.44439977688853105
816817,816818,816817,1633635,1920.918684720993,0.44338561372933327
818819,818820,818819,1637639,1925.606008052826,0.4423761393263703
820821,820822,820821,1641643,1930.5066738128662,0.4413713212325092
822823,822824,822823,1645647,1935.2333507537842,0.44037112729711225
824825,824826,824825,1649651,1939.8878200054169,0.439375525662399
826827,826828,826827,1653655,1944.5895838737488,0.43838448476526537
828829,828830,828829,1657659,1949.2600660324097,0.4373979733281885
830831,830832,830831,1661663,1954.0092358589172,0.43641596035922703
832833,832834,832833,1665667,1958.7530159950256,0.4354384151483828
834835,834836,834835,1669671,1963.5110697746277,0.43446530726032506
836837,836838,836837,1673675,1968.4026370048523,0.43349660654348554
838839,838840,838839,1677679,1973.1159448623657,0.43253228310459235
840841,840842,840841,1681683,1977.8078598976135,0.431572307332317
842843,842844,842843,1685687,1982.4603219032288,0.43061664987544646
844845,844846,844845,1689691,1987.1454319953918,0.4296652816428832
846847,846848,846847,1693695,1991.8266518115997,0.42871817381092114
848849,848850,848849,1697699,1996.4676480293274,0.42777529780505574
850851,850852,850851,1701703,2001.1461598873138,0.42683662531271693
852853,852854,852853,1705707,2005.826751947403,0.4259021282668982
854855,854856,854855,1709711,2010.4880578517914,0.42497177884979465
856857,856858,856857,1713715,2015.2318618297577,0.42404554948734585
858859,858860,858859,1717719,2019.9441268444061,0.423123412861969
860861,860862,860861,1721723,2024.633276939392,0.42220534187981684
862863,862864,862863,1725727,2029.2641746997833,0.4212913096907869
864865,864866,864865,1729731,2033.9725449085236,0.4203812896848831
866867,866868,866867,1733735,2038.6341319084167,0.4194752554776642
868869,868870,868869,1737739,2043.2893838882446,0.4185731809193385
870871,870872,870871,1741743,2047.9515960216522,0.417675040087488
872873,872874,872873,1745747,2052.6087398529053,0.4167808072816115
874875,874876,874875,1749751,2057.2653110027313,0.4158904570267623
876877,876878,876877,1753755,2061.93084692955,0.4150039640699106
878879,878880,878879,1757759,2066.5655286312103,0.4141213033708482
880881,880882,880881,1761763,2071.226672887802,0.4132424501058267
882883,882884,882883,1765767,2075.9032418727875,0.4123674244929134
884885,884886,884885,1769771,2080.612375020981,0.41149623426099424
886887,886888,886887,1773775,2085.3327968120575,0.410628777994134
888889,888890,888889,1777779,2089.9639418125153,0.40976503159618005
890891,890892,890891,1781783,2094.6928718090057,0.408904971278389
892893,892894,892893,1785787,2099.3567197322845,0.40804857346302015
894895,894896,894895,1789791,2104.023468017578,0.40719581476878375
896897,896898,896897,1793795,2108.67493391037,0.4063466720235738
898899,898900,898899,1797799,2113.331813812256,0.4055011222444591
900901,900902,900901,1801803,2117.982396841049,0.4046591426431405
902903,902904,902903,1805807,2122.6378479003906,0.4038207106223126
904905,904906,904905,1809811,2127.272843837738,0.4029858037811209
906907,906908,906907,1813815,2132.0563547611237,0.4021543998969719
908909,908910,908909,1817819,2136.866231918335,0.4013264769419038
910911,910912,910911,1821823,2141.5535707473755,0.40050201306257804
912913,912914,912913,1825827,2146.5325009822845,0.39968098659483076
914915,914916,914915,1829831,2150.9987177848816,0.3988633760563971
916917,916918,916917,1833835,2155.4913408756256,0.39804916012872127
918919,918920,918919,1837839,2160.084345817566,0.3972383176933363
920921,920922,920921,1841843,2164.5674607753754,0.3964308277827513
922923,922924,922923,1845847,2169.012887954712,0.39562666961501236
924925,924926,924925,1849851,2173.463747024536,0.3948258225755126
926927,926928,926927,1853855,2177.9280738830566,0.39402826622063003
928929,928930,928929,1857859,2182.448409795761,0.39323398027408984
930931,930932,930931,1861863,2186.90589594841,0.3924429446196882
932933,932934,932933,1865867,2191.3673300743103,0.3916551393158443
934935,934936,934935,1869871,2195.8082349300385,0.39087054457195336
936937,936938,936937,1873875,2200.252068758011,0.39008914076657675
938939,938940,938939,1877879,2204.7198157310486,0.3893109084365278
940941,940942,940941,1881883,2209.447165966034,0.3885358282677771
942943,942944,942943,1885887,2214.0623936653137,0.38776388111364213
944945,944946,944945,1889891,2218.49378991127,0.38699504797477857
946947,946948,946947,1893895,2222.903634786606,0.3862293100046372
948949,948950,948949,1897899,2227.4186198711395,0.385466648511283
950951,950952,950951,1901903,2231.883796930313,0.38470704495193786
952953,952954,952953,1905907,2236.4311497211456,0.383950480931162
954955,954956,954955,1909911,2240.9157297611237,0.3831969381953968
956957,956958,956957,1913915,2245.3766436576843,0.38244639864387864
958959,958960,958959,1917919,2249.7989118099213,0.38169884431954415
960961,960962,960961,1921923,2254.237858772278,0.38095425739993516
962963,962964,962963,1925927,2258.814796924591,0.3802126202153886
964965,964966,964965,1929931,2263.432856798172,0.37947391522175167
966967,966968,966967,1933935,2267.8893377780914,0.3787381250240287
968969,968970,968969,1937939,2272.369024991989,0.37800523236364825
970971,970972,970971,1941943,2276.806174993515,0.3772752201093681
972973,972974,972973,1945947,2281.3840239048004,0.3765480712736462
974975,974976,974975,1949951,2285.812519788742,0.3758237689962698
976977,976978,976977,1953955,2290.249300956726,0.3751022965479933
978979,978980,978979,1957959,2294.6878876686096,0.37438363733599545
980981,980982,980981,1961963,2299.1176567077637,0.3736677748893271
982983,982984,982983,1965967,2303.5781686306,0.3729546928698255
984985,984986,984985,1969971,2308.0430159568787,0.3722443750648381
986987,986988,986987,1973975,2312.4643597602844,0.37153680538540357
988989,988990,988989,1977979,2316.877180814743,0.37083196786625194
990991,990992,990991,1981983,2321.369585752487,0.3701298466658045
992993,992994,992993,1985987,2325.8580408096313,0.3694304260716308
994995,994996,994995,1989991,2330.329499721527,0.3687336904786207
996997,996998,996997,1993995,2334.794766664505,0.3680396244089934
998999,999000,998999,1997999,2339.236051797867,0.36734821250502137
1001001,1001002,1001001,2002003,2343.697945833206,0.3666594395235734
1003003,1003004,1003003,2006007,2348.3210277557373,0.3659732903342956
1005005,1005006,1005005,2010011,2352.992758989334,0.3652897499232495
1007007,1007008,1007007,2014015,2357.444658756256,0.36460880339836876
1009009,1009010,1009009,2018019,2361.998591899872,0.3639304359694506
1011011,1011012,1011011,2022023,2366.413864850998,0.36325463296452654
1013013,1013014,1013013,2026027,2370.9647669792175,0.36258137981894834
1015015,1015016,1015015,2030031,2375.465591907501,0.3619106620808452
1017017,1017018,1017017,2034035,2379.901015996933,0.36124246540202876
1019019,1019020,1019019,2038039,2384.361448764801,0.36057677555254486
1021021,1021022,1021021,2042043,2388.809471845627,0.3599135783952079
1023023,1023024,1023023,2046047,2393.3146460056305,0.3592528599056095
1025025,1025026,1025025,2050051,2397.7913637161255,0.35859460616484284
1027027,1027028,1027027,2054055,2402.198184967041,0.35793880335768335
1029029,1029030,1029029,2058059,2406.6403138637543,0.35728543776713195
1031031,1031032,1031031,2062063,2411.066788673401,0.3566344957853289
1033033,1033034,1033033,2066067,2415.484804868698,0.35598596389536397
1035035,1035036,1035035,2070071,2419.9010138511658,0.35533982868946623
1037037,1037038,1037037,2074075,2424.395686864853,0.35469607685445226
1039039,1039040,1039039,2078079,2428.8467288017273,0.354054695177183
1041041,1041042,1041041,2082083,2433.341367006302,0.35341567053728795
1043043,1043044,1043043,2086087,2437.7458589076996,0.3527789899144409
1045045,1045046,1045045,2090091,2442.169888973236,0.35214464038472215
1047047,1047048,1047047,2094095,2446.5976808071136,0.35151260911516147
1049049,1049050,1049049,2098099,2451.066989660263,0.35088288336919504
1051051,1051052,1051051,2102103,2455.52005982399,0.3502554505048465
1053053,1053054,1053053,2106107,2460.01008272171,0.34963029796381306
1055055,1055056,1055055,2110111,2464.4518809318542,0.34900741328783624
1057057,1057058,1057057,2114115,2468.9018857479095,0.34838678410415014
1059059,1059060,1059059,2118119,2473.3463039398193,0.3477683981327573
1061061,1061062,1061061,2122123,2477.7820518016815,0.3471522431791527
1063063,1063064,1063063,2126127,2482.232603788376,0.34653830713978095
1065065,1065066,1065065,2130131,2486.6657316684723,0.345926577992941
1067067,1067068,1067067,2134135,2491.1359798908234,0.3453170438115194
1069069,1069070,1069069,2138139,2495.5834918022156,0.3447096927466191
1071071,1071072,1071071,2142143,2500.00102686882,0.3441045130348357
1073073,1073074,1073073,2146147,2504.4899609088898,0.34350149300371413
1075075,1075076,1075075,2150151,2508.908465862274,0.342900621055378
1077077,1077078,1077077,2154155,2513.37645983696,0.34230188567926234
1079079,1079080,1079079,2158159,2517.8571088314056,0.34170527544483775
1081081,1081082,1081081,2162163,2522.3272478580475,0.34111077900524833
1083083,1083084,1083083,2166167,2526.7967908382416,0.34051838509003574
1085085,1085086,1085085,2170171,2531.5959117412567,0.33992808251241513
1087087,1087088,1087087,2174175,2536.1107230186462,0.33933986016018025
1089089,1089090,1089089,2178179,2540.587994813919,0.3387537070084363
1091091,1091092,1091091,2182183,2545.057801961899,0.3381696120941342
1093093,1093094,1093093,2186187,2549.5080230236053,0.33758756454699324
1095095,1095096,1095095,2190191,2554.0196237564087,0.33700755356039735
1097097,1097098,1097097,2194195,2558.5173478126526,0.336429568415042
1099099,1099100,1099099,2198199,2562.95832490921,0.33585359845892526
1101101,1101102,1101101,2202203,2567.392063856125,0.3352796331146237
1103103,1103104,1103103,2206207,2571.8755548000336,0.33470766188293055
1105105,1105106,1105105,2210211,2576.3674759864807,0.33413767433012254
1107107,1107108,1107107,2214215,2581.239311695099,0.333569660104331
1109109,1109110,1109109,2218219,2585.84863781929,0.33300360891189484
1111111,1111112,1111111,2222223,2590.458212852478,0.33243951055010257
1113113,1113114,1113113,2226227,2595.088709831238,0.3318773548671743
1115115,1115116,1115115,2230231,2599.582547903061,0.33131713179318467
1117117,1117118,1117117,2234235,2604.0553648471832,0.330758831320054
1119119,1119120,1119119,2238239,2608.5850858688354,0.3302024435124622
1121121,1121122,1121121,2242243,2613.056032896042,0.3296479585060297
1123123,1123124,1123123,2246247,2617.5193479061127,0.32909536650004156
1125125,1125126,1125125,2250251,2621.9640667438507,0.32854465775744757
1127127,1127128,1127127,2254255,2626.389930009842,0.32799582261759497
1129129,1129130,1129129,2258259,2630.9395220279694,0.32744885147258174
1131131,1131132,1131131,2262263,2635.4279108047485,0.3269037347909034
1133133,1133134,1133133,2266267,2640.1792356967926,0.3263604631029011
1135135,1135136,1135135,2270271,2644.7370369434357,0.32581902699712373
1137137,1137138,1137137,2274275,2649.2118027210236,0.32527941713306063
1139139,1139140,1139139,2278279,2653.676242828369,0.3247416242284089
1141141,1141142,1141141,2282283,2658.147668838501,0.3242056390718062
1143143,1143144,1143143,2286287,2662.6458168029785,0.32367145250100293
1145145,1145146,1145145,2290291,2667.170012950897,0.32313905542469
1147147,1147148,1147147,2294295,2671.665428876877,0.3226084388115851
1149149,1149150,1149149,2298299,2676.3211958408356,0.3220795936849754
1151151,1151152,1151151,2302303,2680.763462781906,0.3215525111372699
1153153,1153154,1153153,2306307,2685.221663951874,0.32102718230999017
1155155,1155156,1155155,2310311,2689.7104358673096,0.3205035984137794
1157157,1157158,1157157,2314315,2694.1950318813324,0.3199817507102125
1159159,1159160,1159159,2318319,2698.671891927719,0.31946163052271004
1161161,1161162,1161161,2322323,2703.1511178016663,0.3189432292347192
1163163,1163164,1163163,2326327,2707.584002017975,0.31842653828061884
1165165,1165166,1165165,2330331,2712.0589559078217,0.3179115491493576
1167167,1167168,1167167,2334335,2716.5739970207214,0.3173982533990056
1169169,1169170,1169169,2338339,2721.069772005081,0.31688664263310784
1171171,1171172,1171171,2342343,2725.609422683716,0.31637670850977884
1173173,1173174,1173173,2346347,2730.0865218639374,0.31586844274534087
1175175,1175176,1175175,2350351,2734.527319908142,0.3153618371106859
1177177,1177178,1177177,2354355,2738.9672219753265,0.3148568834294565
1179179,1179180,1179179,2358359,2743.4491798877716,0.3143535735744081
1181181,1181182,1181181,2362363,2747.9322040081024,0.31385189948741754
1183183,1183184,1183183,2366367,2752.406874895096,0.3133518531376467
1185185,1185186,1185185,2370371,2756.865383863449,0.31285342657247384
1187187,1187188,1187187,2374375,2761.3118607997894,0.31235661186838115
1189189,1189190,1189189,2378379,2765.7905609607697,0.3118614011709724
1191191,1191192,1191191,2382383,2770.235067844391,0.3113677866640501
1193193,1193194,1193193,2386387,2774.7361238002777,0.3108757605896244
1195195,1195196,1195195,2390391,2779.173821926117,0.3103853152351803
1197197,1197198,1197197,2394395,2783.6712770462036,0.3098964429427724
1199199,1199200,1199199,2398399,2788.2751338481903,0.30940913609811105
1201201,1201202,1201201,2402403,2792.847596883774,0.30892338714147627
1203203,1203204,1203203,2406407,2797.32484292984,0.30843918855498487
1205205,1205206,1205205,2410411,2801.8131499290466,0.3079565328771423
1207207,1207208,1207207,2414415,2806.2703337669373,0.3074754126882908
1209209,1209210,1209209,2418419,2810.752275943756,0.30699582061242836
1211211,1211212,1211211,2422423,2815.3075778484344,0.30651774933176057
1213213,1213214,1213213,2426427,2819.7509849071503,0.30604119156669185
1215215,1215216,1215215,2430431,2824.1857867240906,0.3055661400885583
1217217,1217218,1217217,2434435,2828.6890017986298,0.30509258770871384
1219219,1219220,1219219,2438439,2833.142375946045,0.304620527289444
1221221,1221222,1221221,2442443,2837.6155269145966,0.30414995173487114
1223223,1223224,1223223,2446447,2842.066946029663,0.3036808539964113
1225225,1225226,1225225,2450451,2846.5214116573334,0.30321322706731735
1227227,1227228,1227227,2454455,2851.2481818199158,0.3027470639881358
1229229,1229230,1229229,2458459,2855.789037704468,0.3022823578394309
1231231,1231232,1231231,2462463,2860.2342178821564,0.3018191017490608
1233233,1233234,1233233,2466467,2864.6641368865967,0.3013572888885392
1235235,1235236,1235235,2470471,2869.1509528160095,0.3008969124639407
1237237,1237238,1237237,2474475,2873.606034755707,0.30043796573227155
1239239,1239240,1239239,2478479,2878.151398897171,0.29998044199055585
1241241,1241242,1241241,2482483,2882.5994539260864,0.2995243345758354
1243243,1243244,1243243,2486487,2887.0407490730286,0.29906963686698873
1245245,1245246,1245245,2490491,2891.668032884598,0.2986163422847312
1247247,1247248,1247247,2494495,2896.0951437950134,0.2981644442916149
1249249,1249250,1249249,2498499,2900.582629919052,0.29771393648479716
1251251,1251252,1251251,2502503,2905.033144712448,0.29726481415309536
1253253,1253254,1253253,2506507,2909.47181892395,0.2968170695457957
1255255,1255256,1255255,2510511,2913.9085228443146,0.2963706958835246
1257257,1257258,1257257,2514515,2918.370110988617,0.2959256867507065
1259259,1259260,1259259,2518519,2922.8093860149384,0.29548203582089627
1261261,1261262,1261261,2522523,2927.323118686676,0.2950397368203994
1263263,1263264,1263263,2526527,2931.9846098423004,0.2945987835282722
1265265,1265266,1265265,2530531,2936.461989879608,0.29415916975085565
1267267,1267268,1267267,2534535,2940.9172258377075,0.29372088934178464
1269269,1269270,1269269,2538539,2945.3237318992615,0.29328393619107374
1271271,1271272,1271271,2542543,2949.8751690387726,0.2928483042287553
1273273,1273274,1273273,2546547,2954.407628059387,0.2924139874139655
1275275,1275276,1275275,2550551,2958.884541749954,0.2919809797494963
1277277,1277278,1277277,2554555,2963.3274188041687,0.2915492752690625
1279279,1279280,1279279,2558559,2967.8090858459473,0.2911188680536725
1281281,1281282,1281281,2562563,2972.2768199443817,0.2906897522043437
1283283,1283284,1283283,2566567,2976.7649488449097,0.29026192186938715
1285285,1285286,1285285,2570571,2981.2191627025604,0.2898353712298558
1287287,1287288,1287287,2574575,2985.6787338256836,0.28941009449772537
1289289,1289290,1289289,2578579,2990.144015789032,0.2889860859249893
1291291,1291292,1291291,2582583,2994.638478755951,0.28856333979456394
1293293,1293294,1293293,2586587,2999.1226308345795,0.28814185042392637
1295295,1295296,1295295,2590591,3003.580544948578,0.28772161216875247
1297297,1297298,1297297,2594595,3008.185703754425,0.28730261941382196
1299299,1299300,1299299,2598599,3012.8843507766724,0.28688486657847534
1301301,1301302,1301301,2602603,3017.308227777481,0.28646834811297595
1303303,1303304,1303303,2606607,3021.832177877426,0.28605305850942386
1305305,1305306,1305305,2610611,3026.2987728118896,0.28563899227992806
1307307,1307308,1307307,2614615,3030.746532678604,0.28522614398025325
1309309,1309310,1309309,2618619,3035.328012943268,0.284814508189811
1311311,1311312,1311311,2622623,3039.8187098503113,0.2844040795280307
1313313,1313314,1313313,2626627,3044.255057811737,0.2839948526434455
1315315,1315316,1315315,2630631,3048.716886997223,0.2835868222082354
1317317,1317318,1317317,2634635,3053.198595046997,0.2831799829400552
1319319,1319320,1319319,2638639,3057.6096477508545,0.28277432957474957
1321321,1321322,1321321,2642643,3062.3259558677673,0.28236985688636196
1323323,1323324,1323323,2646647,3066.791298866272,0.28196655967803963
1325325,1325326,1325325,2650651,3071.2643859386444,0.2815644327820337
1327327,1327328,1327327,2654655,3075.730829000473,0.28116347106697503
1329329,1329330,1329329,2658659,3080.173615694046,0.28076366941604647
1331331,1331332,1331331,2662663,3084.705451965332,0.2803650227615435
1333333,1333334,1333333,2666667,3089.180013656616,0.2799675260521326
1335335,1335336,1335335,2670671,3093.639797925949,0.27957117427285993
1337337,1337338,1337337,2674675,3098.1150999069214,0.2791759624324186
1339339,1339340,1339339,2678679,3102.591778755188,0.2787818855704245
1341341,1341342,1341341,2682683,3107.021948814392,0.2783889387592353
1343343,1343344,1343343,2686687,3111.518703699112,0.27799711709303665
1345345,1345346,1345345,2690691,3115.9676308631897,0.2776064156987559
1347347,1347348,1347347,2694695,3120.433316707611,0.27721682973060524
1349349,1349350,1349349,2698699,3124.8522827625275,0.2768283543682628
1351351,1351352,1351351,2702703,3129.3126430511475,0.2764409848223295
1353353,1353354,1353353,2706707,3133.79487490654,0.276054716330691
1355355,1355356,1355355,2710711,3138.2469868659973,0.275669544156699
1357357,1357358,1357357,2714715,3142.712154865265,0.2752854635928088
1359359,1359360,1359359,2718719,3147.1673159599304,0.2749024699569418
1361361,1361362,1361361,2722723,3151.609225988388,0.27452055859248503
1363363,1363364,1363363,2726727,3156.0798857212067,0.2741397248719295
1365365,1365366,1365365,2730731,3160.57941198349,0.273759964191413
1367367,1367368,1367367,2734735,3165.0814328193665,0.2733812719798152
1369369,1369370,1369369,2738739,3169.536469936371,0.2730036436805676
1371371,1371372,1371371,2742743,3174.033433675766,0.27262707477530057
1373373,1373374,1373373,2746747,3178.4821577072144,0.2722515607638343
1375375,1375376,1375375,2750751,3183.287090778351,0.2718770971696358
1377377,1377378,1377377,2754755,3187.8675198554993,0.2715036795470951
1379379,1379380,1379379,2758759,3192.3326630592346,0.27113130347424885
1381381,1381382,1381381,2762763,3196.7774698734283,0.2707599645545997
1383383,1383384,1383383,2766767,3201.2511427402496,0.2703896584116592
1385385,1385386,1385385,2770771,3205.712343931198,0.2700203806980426
1387387,1387388,1387387,2774775,3210.2566328048706,0.2696521270900121
1389389,1389390,1389389,2778779,3214.6987047195435,0.26928489328565774
1391391,1391392,1391391,2782783,3219.168876886368,0.2689186750103545
1393393,1393394,1393393,2786787,3223.6353657245636,0.26855346801676205
1395395,1395396,1395395,2790791,3228.094409942627,0.2681892680666351
1397397,1397398,1397397,2794795,3232.614804983139,0.26782607096174615
1399399,1399400,1399399,2798799,3237.0947058200836,0.26746387251660053
1401401,1401402,1401401,2802803,3241.558257818222,0.26710266857844545
1403403,1403404,1403403,2806807,3246.119950771332,0.26674245500908
1405405,1405406,1405405,2810811,3250.5675098896027,0.26638322769576916
1407407,1407408,1407407,2814815,3255.01078081131,0.26602498254942475
1409409,1409410,1409409,2818819,3259.428906917572,0.26566771550096746
1411411,1411412,1411411,2822823,3263.922521829605,0.26531142251042183
1413413,1413414,1413413,2826827,3268.3604307174683,0.2649560995560023
1415415,1415416,1415415,2830831,3272.8025467395782,0.2646017426304752
1417417,1417418,1417417,2834835,3277.234585762024,0.26424834776298667
1419419,1419420,1419419,2838839,3281.719790697098,0.26389591099359677
1421421,1421422,1421421,2842843,3286.2273919582367,0.26354442838783143
1423423,1423424,1423423,2846847,3290.700642824173,0.26319389603486343
1425425,1425426,1425425,2850851,3295.1578707695007,0.26284431004205544
1427427,1427428,1427427,2854855,3299.6257269382477,0.262495666538598
1429429,1429430,1429429,2858859,3304.20663189888,0.2621479616736906
1431431,1431432,1431431,2862863,3308.808266878128,0.26180119162199844
1433433,1433434,1433433,2866867,3313.2908647060394,0.26145535257455776
1435435,1435436,1435435,2870871,3317.7687468528748,0.26111044074241363
1437437,1437438,1437437,2874875,3322.236357688904,0.26076645236389595
1439439,1439440,1439439,2878879,3326.665105819702,0.2604233836864296
1441441,1441442,1441441,2882883,3331.330327987671,0.2600812309920002
1443443,1443444,1443443,2886887,3335.802985906601,0.2597399905680504
1445445,1445446,1445445,2890891,3340.2821497917175,0.25939965873840265
1447447,1447448,1447447,2894895,3344.7186057567596,0.2590602318250603
1449449,1449450,1449449,2898899,3349.1912047863007,0.2587217061936826
1451451,1451452,1451451,2902903,3353.806581020355,0.2583840782062907
1453453,1453454,1453453,2906907,3358.711338996887,0.2580473442667426
1455455,1455456,1455455,2910911,3363.1987776756287,0.25771150077889615
1457457,1457458,1457457,2914915,3367.6707026958466,0.25737654418298916
1459459,1459460,1459459,2918919,3372.248925924301,0.25704247092107835
1461461,1461462,1461461,2922923,3376.6718797683716,0.25670927746614325
1463463,1463464,1463463,2926927,3381.1500039100647,0.2563769603093533
1465465,1465466,1465465,2930931,3385.6510620117188,0.2560455159527919
1467467,1467468,1467467,2934935,3390.4568688869476,0.25571494092764624
1469469,1469470,1469469,2938939,3394.932543992996,0.2553852317723795
1471471,1471472,1471471,2942943,3399.321400642395,0.25505638505455863
1473473,1473474,1473473,2946947,3403.7524399757385,0.2547283973508456
1475475,1475476,1475475,2950951,3408.265925884247,0.25440126526336826
1477477,1477478,1477477,2954955,3412.948385953903,0.25407498540516826
1479479,1479480,1479479,2958959,3417.609045982361,0.2537495544147532
1481481,1481482,1481481,2962963,3422.2699949741364,0.25342496894154465
1483483,1483484,1483483,2966967,3426.923640012741,0.25310122565679194
1485485,1485486,1485485,2970971,3431.884080886841,0.2527783212481154
1487487,1487488,1487487,2974975,3436.709265947342,0.2524562524158682
1489489,1489490,1489489,2978979,3441.4602649211884,0.2521350158895075
1491491,1491492,1491491,2982983,3446.1580736637115,0.2518146084057662
1493493,1493494,1493493,2986987,3450.819674730301,0.25149502671774826
1495495,1495496,1495495,2990991,3455.5373587608337,0.25117626760038547
1497497,1497498,1497497,2994995,3460.264173746109,0.25085832784316153
1499499,1499500,1499499,2998999,3464.936582803726,0.250541204257388
1501502,1501503,1501502,3003005,3469.6490869522095,0.2502247358661407
1503504,1503505,1503504,3007009,3474.4458558559418,0.24990923550649313
1505506,1505507,1505506,3011013,3479.1443870067596,0.24959454183044727
1507508,1507509,1507508,3015017,3483.8048796653748,0.2492806517129793
1509510,1509511,1509510,3019021,3488.468822002411,0.24896756204361736
1511512,1511513,1511512,3023025,3493.174114704132,0.24865526972644147
1513514,1513515,1513514,3027029,3497.8956480026245,0.24834377168372157
1515516,1515517,1515516,3031033,3502.605334997177,0.24803306484682253
1517518,1517519,1517518,3035037,3507.305291891098,0.24772314617439406
1519520,1519521,1519520,3039041,3512.034862756729,0.24741401263418084
1521522,1521523,1521522,3043045,3516.7338438034058,0.24710566120666044
1523524,1523525,1523524,3047049,3521.428538799286,0.24679808889050037
1525526,1525527,1525526,3051053,3526.115233898163,0.24649129270619596
1527528,1527529,1527528,3055057,3530.817332983017,0.24618526967788057
1529530,1529531,1529530,3059061,3535.5280346870422,0.24588001685333438
1531532,1531533,1531532,3063065,3540.525541782379,0.24557553129125154
1533534,1533535,1533534,3067069,3545.4337668418884,0.24527181006669707
1535536,1535537,1535536,3071073,3550.359096765518,0.24496885027110693
1537538,1537539,1537538,3075077,3555.2632019519806,0.24466664900864998
1539540,1539541,1539540,3079081,3560.1814210414886,0.24436520339804702
1541542,1541543,1541542,3083085,3565.128075838089,0.24406451057438971
1543544,1543545,1543544,3087089,3570.2238597869873,0.2437645676873217
1545546,1545547,1545546,3091093,3575.2498359680176,0.24346537189740047
1547548,1547549,1547548,3095097,3580.18790602684,0.2431669203833735
1549550,1549551,1549550,3099101,3585.157889842987,0.24286921033672115
1551552,1551553,1551552,3103105,3590.075889825821,0.24257223896347568
1553554,1553555,1553554,3107109,3595.1521756649017,0.2422760034842213
1555556,1555557,1555556,3111113,3600.170257806778,0.2419805011322751
1557558,1557559,1557558,3115117,3605.0259828567505,0.2416857291573251
1559560,1559561,1559560,3119121,3609.764796733856,0.24139168481633533
1561562,1561563,1561562,3123125,3614.4399547576904,0.2410983653862786
1563564,1563565,1563564,3127129,3619.134809732437,0.2408057681604987
1565566,1565567,1565566,3131133,3623.82928276062,0.24051389043415838
1567568,1567569,1567568,3135137,3628.5455837249756,0.24022272953152424
1569570,1569571,1569570,3139141,3633.2114386558533,0.23993228277322487
1571572,1571573,1571572,3143145,3637.892250776291,0.23964254750899272
1573574,1573575,1573574,3147149,3642.567534685135,0.23935352109037922
1575576,1575577,1575576,3151153,3647.2247087955475,0.23906520088894467
1577578,1577579,1577578,3155157,3651.9149780273438,0.23877758428534435
1579580,1579581,1579580,3159161,3656.601791858673,0.2384906686784234
1581582,1581583,1581582,3163165,3661.261646747589,0.23820445146884595
1583584,1583585,1583584,3167169,3665.925223827362,0.23791893008092302
1585586,1585587,1585586,3171173,3670.9029376506805,0.23763410194806056
1587588,1587589,1587588,3175177,3675.6335048675537,0.23734996452003543
1589590,1589591,1589590,3179181,3680.318754673004,0.23706651525208144
1591592,1591593,1591592,3183185,3685.0491178035736,0.23678375161398435
1593594,1593595,1593594,3187189,3689.7823219299316,0.23650167109371978
1595596,1595597,1595596,3191193,3694.529932975769,0.23622027117926336
1597598,1597599,1597598,3195197,3699.1636888980865,0.23593954939133255
1599600,1599601,1599600,3199201,3703.8488409519196,0.23565950323973084
1601602,1601603,1601602,3203205,3708.483408689499,0.23538013026154658
1603604,1603605,1603604,3207209,3713.189651966095,0.2351014279993251
1605606,1605607,1605606,3211213,3717.8287539482117,0.2348233940119826
1607608,1607609,1607608,3215217,3722.490757703781,0.23454602586753026
1609610,1609611,1609610,3219221,3727.173594713211,0.23426932114671217
1611612,1611613,1611612,3223225,3731.9652638435364,0.23399327743754839
1613614,1613615,1613614,3227229,3736.6589188575745,0.2337178923517058
1615616,1615617,1615616,3231233,3741.4009437561035,0.23344316349903238
1617618,1617619,1617618,3235237,3746.0912578105927,0.23316908850392792
1619620,1619621,1619620,3239241,3750.7954139709473,0.23289566501080117
1621622,1621623,1621622,3243245,3755.4746758937836,0.2326228906695178
1623624,1623625,1623624,3247249,3760.1713337898254,0.23235076313903846
1625626,1625627,1625626,3251253,3764.8579268455505,0.23207928008741874
1627628,1627629,1627628,3255257,3769.502546787262,0.23180843920818006
1629630,1629631,1629630,3259261,3774.213552713394,0.2315382381912059
1631632,1631633,1631632,3263265,3778.889302968979,0.23126867473729362
1633634,1633635,1633634,3267269,3783.571063041687,0.2309997465708875
1635636,1635637,1635636,3271273,3788.2354488372803,0.2307314514182508
1637638,1637639,1637638,3275277,3792.906177997589,0.23046378701656067
1639640,1639641,1639640,3279281,3797.6448769569397,0.23019675111572724
1641642,1641643,1641642,3283285,3802.364015817642,0.22993034147839353
1643644,1643645,1643644,3287289,3807.0252809524536,0.22966455587265955
1645646,1645647,1645646,3291293,3811.7056138515472,0.22939939207935822
1647648,1647649,1647648,3295297,3816.3765058517456,0.2291348478938744
1649650,1649651,1649650,3299301,3821.053472995758,0.22887092111704987
1651652,1651653,1651652,3303305,3825.753942012787,0.2286076095606404
1653654,1653655,1653654,3307309,3830.5788626670837,0.22834491105459165
1655656,1655657,1655656,3311313,3835.3774189949036,0.22808282342339226
1657658,1657659,1657658,3315317,3840.2758548259735,0.22782134451881575
1659660,1659661,1659660,3319321,3845.0484018325806,0.22756047219081665
1661662,1661663,1661662,3323325,3849.8083448410034,0.2273002043039014
1663664,1663665,1663664,3327329,3854.6193828582764,0.22704053873530938
1665666,1665667,1665666,3331333,3859.5406336784363,0.22678147336591792
1667668,1667669,1667668,3335337,3864.270015001297,0.22652300609297527
1669670,1669671,1669670,3339341,3868.9443187713623,0.22626513481918664
1671672,1671673,1671672,3343345,3873.65487575531,0.2260078574581712
1673674,1673675,1673674,3347349,3878.3260538578033,0.22575117193446204
1675676,1675677,1675676,3351353,3883.075122833252,0.22549507618350617
1677678,1677679,1677678,3355357,3887.7547528743744,0.2252395681462076
1679680,1679681,1679680,3359361,3892.4480550289154,0.22498464577620325
1681682,1681683,1681682,3363365,3897.110958814621,0.22473030703804397
1683684,1683685,1683684,3367369,3901.8263030052185,0.22447654989809962
1685686,1685687,1685686,3371373,3906.5600419044495,0.2242233723445679
1687688,1687689,1687688,3375377,3911.2784378528595,0.22397077236382756
1689690,1689691,1689690,3379381,3916.007281780243,0.22371874795499025
1691692,1691693,1691692,3383385,3920.7038538455963,0.22346729712990054
1693694,1693695,1693694,3387389,3925.4380390644073,0.223216417907679
1695696,1695697,1695696,3391393,3930.097498893738,0.22296610831836006
1697698,1697699,1697698,3395397,3934.7512168884277,0.22271636639015924
1699700,1699701,1699700,3399401,3939.4036819934845,0.22246719017493888
1701702,1701703,1701702,3403405,3944.0867397785187,0.2222185777300183
1703704,1703705,1703704,3407409,3948.7450597286224,0.22197052711089782
1705706,1705707,1705706,3411413,3953.3997797966003,0.22172303640036262
1707708,1707709,1707708,3415417,3958.089661836624,0.2214761036757409
1709710,1709711,1709710,3419421,3962.801261663437,0.22122972702709376
1711712,1711713,1711712,3423425,3967.4663937091827,0.2209839045553963
1713714,1713715,1713714,3427429,3972.397640943527,0.22073863436344254
1715716,1715717,1715716,3431433,3977.106405735016,0.22049391457403544
1717718,1717719,1717718,3435437,3981.8229088783264,0.22024974330997793
1719720,1719721,1719720,3439441,3986.545358657837,0.2200061187013489
1721722,1721723,1721722,3443445,3991.2401757240295,0.21976303889823612
1723724,1723725,1723724,3447449,3996.1274988651276,0.2195205020452704
1725726,1725727,1725726,3451453,4000.7784440517426,0.21927850630527246
1727728,1727729,1727728,3455457,4005.439834833145,0.21903704984288197
1729730,1729731,1729730,3459461,4010.104943752289,0.21879613083365257
1731732,1731733,1731732,3463465,4014.8202917575836,0.2185557474658708
1733734,1733735,1733734,3467469,4019.510566711426,0.21831589792600425
1735736,1735737,1735736,3471473,4024.192091703415,0.21807658041871036
1737738,1737739,1737738,3475477,4028.9968798160553,0.21783779315592255
1739740,1739741,1739740,3479481,4033.947783946991,0.21759953434593626
1741742,1741743,1741742,3483485,4038.67791891098,0.2173618022170558
1743744,1743745,1743744,3487489,4043.4069187641144,0.21712459500486148
1745746,1745747,1745746,3491493,4048.118446826935,0.21688791094857152
1747748,1747749,1747748,3495497,4053.0235397815704,0.21665174829286116
1749750,1749751,1749750,3499501,4057.7224340438843,0.21641610530059552
1751752,1751753,1751752,3503505,4062.389865875244,0.21618098023100174
1753754,1753755,1753754,3507509,4067.1055529117584,0.21594637135785888
1755756,1755757,1755756,3511513,4071.825695991516,0.21571227696404094
1757758,1757759,1757758,3515517,4076.5072000026703,0.21547869533242192
1759760,1759761,1759760,3519521,4081.183007001877,0.21524562475860876
1761762,1761763,1761762,3523525,4085.8580327033997,0.2150130635509413
1763764,1763765,1763764,3527529,4090.535224676132,0.21478101001412142
1765766,1765767,1765766,3531533,4095.1890847682953,0.21454946246558393
1767768,1767769,1767768,3535537,4099.872920751572,0.21431841923367756
1769770,1769771,1769770,3539541,4104.588335752487,0.21408787865038903
1771772,1771773,1771772,3543545,4109.492630958557,0.213857839054981
1773774,1773775,1773774,3547549,4114.1963267326355,0.21362829879581113
1775776,1775777,1775776,3551553,4118.880134820938,0.21339925622669398
1777778,1777779,1777778,3555557,4123.579489946365,0.21317070971053909
1779780,1779781,1779780,3559561,4128.259147882462,0.21294265761571296
1781782,1781783,1781782,3563565,4133.076135873795,0.21271509831967705
1783784,1783785,1783784,3567569,4137.762216806412,0.21248803020898777
1785786,1785787,1785786,3571573,4142.4690680503845,0.21226145166656352
1787788,1787789,1787788,3575577,4147.186219930649,0.2120353610971506
1789790,1789791,1789790,3579581,4151.872799873352,0.21180975690185733
1791792,1791793,1791792,3583585,4156.800961017609,0.21158463749270595
1793794,1793795,1793794,3587589,4161.532459020615,0.21136000129263266
1795796,1795797,1795796,3591593,4166.203691959381,0.21113584672275465
1797798,1797799,1797798,3595597,4170.864436864853,0.21091217222056002
1799800,1799801,1799800,3599601,4175.5562748909,0.2106889762217179
1801802,1801803,1801802,3603605,4180.24162197113,0.2104662571728113
1803804,1803805,1803804,3607609,4184.920549869537,0.2102440135240613
1805806,1805807,1805806,3611613,4189.614594936371,0.2100222437402408
1807808,1807809,1807808,3615617,4194.315562963486,0.20980094628612278
1809810,1809811,1809810,3619621,4198.975764989853,0.2095801196373941
1811812,1811813,1811812,3623625,4203.6538598537445,0.20935976226792263
1813814,1813815,1813814,3627629,4208.481523990631,0.2091398726679472
1815816,1815817,1815816,3631633,4213.372496843338,0.20892044933134457
1817818,1817819,1817818,3635637,4218.0571320056915,0.2087014907538105
1819820,1819821,1819820,3639641,4222.802263021469,0.2084829954437737
1821822,1821823,1821822,3643645,4227.543690919876,0.2082649619133008
1823824,1823825,1823824,3647649,4232.327835798264,0.20804738867991546
1825826,1825827,1825826,3651653,4237.050398826599,0.20783027427387424
1827828,1827829,1827828,3655657,4241.862065792084,0.20761361721997673
1829830,1829831,1829830,3659661,4246.560670852661,0.20739741605939344
1831832,1831833,1831832,3663665,4251.236578702927,0.20718166933147586
1833834,1833835,1833834,3667669,4255.91992688179,0.2069663755937654
1835836,1835837,1835836,3671673,4260.62118601799,0.2067515334019845
1837838,1837839,1837838,3675677,4265.317982912064,0.20653714131003653
1839840,1839841,1839840,3679681,4270.0027866363525,0.2063231978972908
1841842,1841843,1841842,3683685,4274.844573974609,0.20610970173402166
1843844,1843845,1843844,3687689,4279.60024189949,0.20589665140141733
1845846,1845847,1845846,3691693,4284.448192834854,0.20568404548430408
1847848,1847849,1847848,3695697,4289.178664922714,0.20547188258024107
1849850,1849851,1849850,3699701,4294.065109968185,0.20526016128678748
1851852,1851853,1851852,3703705,4298.8365046978,0.20504888020695944
1853854,1853855,1853854,3707709,4303.498212814331,0.204838037956506
1855856,1855857,1855856,3711713,4308.197332859039,0.2046276331439003
1857858,1857859,1857858,3715717,4312.895216703415,0.2044176643994433
1859860,1859861,1859860,3719721,4317.603075027466,0.20420813034797902
1861862,1861863,1861862,3723725,4322.2865216732025,0.20399908705439884
1863864,1863865,1863864,3727729,4326.954115867615,0.20379047929782246
1865866,1865867,1865866,3731733,4331.652066707611,0.20358230218516837
1867868,1867869,1867868,3735737,4336.380632638931,0.20337455427034
1869870,1869871,1869870,3739741,4341.04328083992,0.2031672341763624
1871872,1871873,1871872,3743745,4345.726496934891,0.20296034054990741
1873874,1873875,1873874,3747749,4350.4202439785,0.20275387205765583
1875876,1875877,1875876,3751753,4355.103662729263,0.2025478273681074
1877878,1877879,1877878,3755757,4359.798361778259,0.2023422051606758
1879880,1879881,1879880,3759761,4364.502913951874,0.20213700412023172
1881882,1881883,1881882,3763765,4369.349982976913,0.20193222293710278
1883884,1883885,1883884,3767769,4374.150562763214,0.20172786030889256
1885886,1885887,1885886,3771773,4378.8143928050995,0.20152391493684263
1887888,1887889,1887888,3775777,4383.474269866943,0.20132038552583253
1889890,1889891,1889890,3779781,4388.25438284874,0.20111727079347475
1891892,1891893,1891892,3783785,4393.071036815643,0.20091456945374375
1893894,1893895,1893894,3787789,4397.719272851944,0.200712280229709
1895896,1895897,1895896,3791793,4402.414701700211,0.20051040185353486
1897898,1897899,1897898,3795797,4407.203769683838,0.20030893305556674
1899900,1899901,1899900,3799801,4411.8634197711945,0.20010787257706397
1901902,1901903,1901902,3803805,4416.58296585083,0.1999072191592859
1903904,1903905,1903904,3807809,4421.239204883575,0.19970697155804373
1905906,1905907,1905906,3811813,4425.924760818481,0.1995071285218728
1907908,1907909,1907908,3815817,4430.66232085228,0.1993076888120413
1909910,1909911,1909910,3819821,4435.3265788555145,0.19910865119527443
1911912,1911913,1911912,3823825,4439.981735944748,0.19891001444193535
1913914,1913915,1913914,3827829,4444.654137849808,0.1987117773223872
1915916,1915917,1915916,3831833,4449.332108974457,0.1985139386197261
1917918,1917919,1917918,3835837,4453.990757703781,0.1983164971225051
1919920,1919921,1919920,3839841,4458.6505398750305,0.19811945161745825
1921922,1921923,1921922,3843845,4463.394885778427,0.1979228008967766
1923924,1923925,1923924,3847849,4468.091209888458,0.1977265437672031
1925926,1925927,1925926,3851853,4472.811666965485,0.19753067902638577
1927928,1927929,1927928,3855857,4477.502029657364,0.1973352054883435
1929930,1929931,1929930,3859861,4482.197198867798,0.19714012196891417
1931932,1931933,1931932,3863865,4486.910160779953,0.19694542728393571
1933934,1933935,1933934,3867869,4491.604638814926,0.19675112025834096
1935936,1935937,1935936,3871873,4496.256569862366,0.19655719972251973
1937938,1937939,1937938,3875877,4501.150429964066,0.1963636645104998
1939940,1939941,1939940,3879881,4506.013249874115,0.19617051345812797
1941942,1941943,1941942,3883885,4510.668590784073,0.19597774541216495
1943944,1943945,1943944,3887889,4515.35954284668,0.19578535921755247
1945946,1945947,1945946,3891893,4520.051909685135,0.1955933537265082
1947948,1947949,1947948,3895897,4524.741318941116,0.19540172780034482
1949950,1949951,1949950,3899901,4529.542201757431,0.19521048029673693
1951952,1951953,1951952,3903905,4534.295393943787,0.19501961008427315
1953954,1953955,1953954,3907909,4538.979073047638,0.19482911602972308
1955956,1955957,1955956,3911913,4543.660290956497,0.19463899701440823
1957958,1957959,1957958,3915917,4548.305842876434,0.19444925191601214
1959960,1959961,1959960,3919921,4553.001691818237,0.1942598796194943
1961962,1961963,1961962,3923925,4557.732643842697,0.19407087901163322
1963964,1963965,1963964,3927929,4562.405180931091,0.19388224898466433
1965966,1965967,1965966,3931933,4567.069809913635,0.19369398844173702
1967968,1967969,1967968,3935937,4571.752575874329,0.19350609628054372
1969970,1969971,1969970,3939941,4576.472797870636,0.19331857141150977
1971972,1971973,1971972,3943945,4581.231864690781,0.19313141274324153
1973974,1973975,1973974,3947949,4585.995335817337,0.1929446191916213
1975976,1975977,1975976,3951953,4590.6841106414795,0.19275818967435043
1977978,1977979,1977978,3955957,4595.349401712418,0.19257212312004413
1979980,1979981,1979980,3959961,4600.051933765411,0.19238641845004167
1981982,1981983,1981982,3963965,4604.69038271904,0.19220107460205327
1983984,1983985,1983984,3967969,4609.349477767944,0.1920160905119701
1985986,1985987,1985986,3971973,4614.056988954544,0.19183146512295934
1987988,1987989,1987988,3975977,4618.719107866287,0.19164719737273117
1989990,1989991,1989990,3979981,4623.5196878910065,0.19146328621718567
1991992,1991993,1991992,3983985,4628.310809850693,0.19127973060858494
1993994,1993995,1993994,3987989,4633.000715970993,0.19109652950101008
1995996,1995997,1995996,3991993,4637.736422777176,0.1909136818612751
1997998,1997999,1997998,3995997,4642.414333820343,0.19073118665073707
2000000,2000001,2000000,4000001,4647.114407777786,0.19054904284166696


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0036039352416992188,12064.682476916567
1001,7376,7376,14752,18.16280508041382,0.2185577111922612
2002,15100,15100,30200,36.29642605781555,0.10515795791798155
3003,22762,22762,45524,55.961483001708984,0.006310511173069244
4004,30610,30610,61220,74.9745442867279,0.006166181057778886
5005,38584,38584,77168,93.57754707336426,0.0061183757625258295
6006,46568,46568,93136,113.38448905944824,0.006105341291913646
7007,54562,54562,109124,142.87890005111694,0.00609804192208685
8008,62554,62554,125108,177.2360281944275,0.006088372179874568
9009,70554,70554,141108,210.6262331008911,0.006084384294808842
10010,78552,78552,157104,243.88585495948792,0.006078809925384121
11011,86552,86552,173104,278.44044494628906,0.006076112389564514
12012,94546,94546,189092,312.65111804008484,0.006070468207326485
13013,102538,102538,205076,345.7434480190277,0.006055822785128839
14014,110542,110542,221084,382.3908441066742,0.006053901757695712
15015,118536,118536,237072,415.9855511188507,0.006029809774190653
16016,126516,126516,253032,449.01793217658997,0.004569394761347212
17017,134398,134398,268796,483.2819230556488,0.004537211319984635
18018,142386,142386,284772,518.3921480178833,0.004532146278506843
19019,150372,150372,300744,550.1638860702515,0.0045086469981470145
20020,158360,158360,316720,585.198468208313,0.004502913083342719
21021,166356,166356,332712,620.999340057373,0.004497499165154295
22022,174358,174358,348716,656.4476721286774,0.0044958962134842295
23023,182354,182354,364708,688.4954319000244,0.0044931493648618925
24024,190356,190356,380712,721.382621049881,0.004491351395699894
25025,198360,198360,396720,754.6736462116241,0.004490362911383272
26026,206346,206346,412692,787.703507900238,0.004464074212592095
27027,214348,214348,428696,821.9748229980469,0.004462264327230514
28028,222332,222332,444664,853.145613193512,0.004413959157318459
29029,230332,230332,460664,888.7861461639404,0.004411526042531477
30030,238336,238336,476672,925.3950181007385,0.004410199748235755
31031,246304,246304,492608,961.8196110725403,0.004038582866996876
32032,254300,254300,508600,998.8853759765625,0.004037275894006598
33033,262298,262298,524596,1035.3081619739532,0.0040345481647818815
34034,270300,270300,540600,1063.3009731769562,0.004032811650176882
35035,278302,278302,556604,1088.452163219452,0.004031622900583898
36036,286300,286300,572600,1111.8984880447388,0.004029210433145636
37037,294304,294304,588608,1134.603765964508,0.004028389123050147
38038,302298,302298,604596,1157.0772511959076,0.004018111469122232
39039,310298,310298,620596,1177.961655139923,0.004015640271973098
40040,318298,318298,636596,1203.168092250824,0.004013682415461517
41041,326304,326304,652608,1226.8443021774292,0.004012846737168729
42042,334300,334300,668600,1251.3533720970154,0.004012456953205401
43043,342298,342298,684596,1276.49449300766,0.004009942063930794
44044,350296,350296,700592,1301.2952420711517,0.004008084464658168
45045,358296,358296,716592,1325.3093860149384,0.004005187915026909
46046,366300,366300,732600,1350.2774209976196,0.0040041729207587196
47047,374302,374302,748604,1374.5554602146149,0.0040025338930718135
48048,382304,382304,764608,1393.232134103775,0.0040008795804169495
49049,390306,390306,780612,1410.6644310951233,0.00399958563320979
50050,398308,398308,796616,1428.066192150116,0.0039986009724088944
51051,406304,406304,812608,1445.5209431648254,0.003989975157310255
52052,414306,414306,828612,1462.8963301181793,0.003988224792919937
53053,422306,422306,844612,1480.2903361320496,0.003987019848864293
54054,430308,430308,860616,1497.4659650325775,0.003985179098890512
55055,438312,438312,876624,1514.6665861606598,0.003984542921898537
56056,446288,446288,892576,1531.6646001338959,0.003814730836893432
57057,454290,454290,908580,1548.7969889640808,0.003813430144873564
58058,462292,462292,924584,1566.6821298599243,0.0038122364749142434
59059,470294,470294,940588,1585.9281451702118,0.003806719418207649
60060,478294,478294,956588,1606.2770760059357,0.003803654752118746
61061,486292,486292,972584,1626.6950058937073,0.0038021814816602273
62062,494294,494294,988588,1647.4440021514893,0.0037996505343471654
63063,502296,502296,1004592,1667.8569700717926,0.0037984243499522563
64064,510298,510298,1020596,1688.225051164627,0.003797217659666785
65065,518264,518264,1036528,1708.464273929596,0.0035975307418993907
66066,526258,526258,1052516,1728.7690172195435,0.0035961042067356175
67067,534260,534260,1068520,1749.1775941848755,0.003594583062294987
68068,542260,542260,1084520,1769.2913711071014,0.0035922969909734093
69069,550268,550268,1100536,1789.5549800395966,0.003592217495679506
70070,558276,558276,1116552,1809.7798941135406,0.0035921380040235817
71071,566284,566284,1132568,1829.6877582073212,0.003592058514186647
72072,574288,574288,1148576,1849.6127271652222,0.0035918797038902994
73073,582290,582290,1164580,1869.8222362995148,0.0035910830865759635
74074,590280,590280,1180560,1890.259345293045,0.0035819142285618
75075,598278,598278,1196556,1910.4130811691284,0.0035802942929876735
76076,606280,606280,1212560,1930.5707750320435,0.0035784086903731804
77077,614280,614280,1228560,1950.6553170681,0.003576421018806286
78078,622282,622282,1244564,1970.8327660560608,0.0035756251272687223
79079,630286,630286,1260572,1990.9458129405975,0.003574803167794016
80080,638290,638290,1276580,2011.2244679927826,0.0035741694264288526
81081,646290,646290,1292580,2031.4125671386719,0.003571700503016473
82082,654292,654292,1308584,2051.3261392116547,0.003571106868548668
83083,662294,662294,1324588,2071.5119721889496,0.0035698300307558384
84084,670236,670236,1340472,2091.689558982849,0.00321327148230921
85085,678226,678226,1356452,2111.838219165802,0.0032118226099555613
86086,686218,686218,1372436,2132.3470990657806,0.0032042105194705073
87087,694216,694216,1388432,2152.5454251766205,0.0032011193652579095
88088,702216,702216,1404432,2172.865375995636,0.0031999948023440083
89089,710212,710212,1420424,2193.246793985367,0.0031940356275299564
90090,718208,718208,1436416,2213.7653822898865,0.0031919295124680502
91091,726210,726210,1452420,2233.684655189514,0.0031905471587378997
92092,734214,734214,1468428,2253.8622431755066,0.003189582421327941
93093,742218,742218,1484436,2274.2748651504517,0.0031887740315141855
94094,750220,750220,1500440,2294.7043042182922,0.003187344154866878
95095,758226,758226,1516452,2315.1024639606476,0.003187178283042158
96096,766222,766222,1532444,2335.378538131714,0.003175734944306896
97097,774226,774226,1548452,2355.9910740852356,0.0031753908915561624
98098,782230,782230,1564460,2376.6198251247406,0.0031747442990308627
99099,790236,790236,1580472,2397.168914079666,0.0031742060837132158
100100,798240,798240,1596480,2417.4661922454834,0.003173520406562602
101101,806244,806244,1612488,2437.890110015869,0.0031727931418572553
102102,814244,814244,1628488,2458.343760251999,0.0031697189806436654
103103,822246,822246,1644492,2478.8211481571198,0.003168674218613887
104104,830254,830254,1660508,2499.3358421325684,0.0031686091006122297
105105,838258,838258,1676516,2519.7117083072662,0.003167554779793136
106106,846258,846258,1692516,2540.084396123886,0.003165012063618633
107107,854264,854264,1708528,2560.4339730739594,0.003164593297697138
108108,862270,862270,1724540,2580.6224040985107,0.003163373959978344
109109,870274,870274,1740548,2601.0163803100586,0.003162213311952655
110110,878278,878278,1756556,2621.4079349040985,0.0031614803992852103
111111,886272,886272,1772544,2641.696823120117,0.003141903876894503
112112,894276,894276,1788552,2662.101217985153,0.0031413617871294264
113113,902282,902282,1804564,2683.194875240326,0.0031409441344294464
114114,910288,910288,1820576,2703.6829130649567,0.0031389806372317253
115115,918296,918296,1836592,2724.13276219368,0.003138916350508225
116116,926288,926288,1852576,2744.5488460063934,0.0031327863871410955
117117,934290,934290,1868580,2765.029587984085,0.0031321677033702144
118118,942288,942288,1884576,2785.4293920993805,0.0031239426625688793
119119,950294,950294,1900588,2805.724534034729,0.003123813610727666
120120,958296,958296,1916592,2826.111825942993,0.003122707012153114
121121,966300,966300,1932600,2846.4586210250854,0.0031217578343785135
122122,974308,974308,1948616,2866.8674092292786,0.003121695872323471
123123,982310,982310,1964620,2886.4738640785217,0.003117781319815549
124124,990314,990314,1980628,2903.5492658615112,0.003117078096693149
125125,998312,998312,1996624,2919.2882690429688,0.0030978669001342496
126126,1006314,1006314,2012628,2940.340908050537,0.0030973435186751885
127127,1014302,1014302,2028604,2956.7732491493225,0.003073490926908562
128128,1022306,1022306,2044612,2974.314189195633,0.0030728936126251938
129129,1030312,1030312,2060624,2991.304661989212,0.003072279901971342
130130,1038312,1038312,2076624,3008.705105304718,0.0030692137333971914
131131,1046312,1046312,2092624,3025.747143983841,0.0030628718395746546
132132,1054316,1054316,2108632,3042.5695600509644,0.0030626049683633028
133133,1062318,1062318,2124636,3059.319144010544,0.0030614239349233685
134134,1070324,1070324,2140648,3076.082262992859,0.0030607663411501562
135135,1078326,1078326,2156652,3092.8240311145782,0.003056192163057858
136136,1086330,1086330,2172660,3109.6917581558228,0.0030554855493392097
137137,1094332,1094332,2188664,3126.3019211292267,0.0030528913102898514
138138,1102336,1102336,2204672,3143.1099841594696,0.0030524231387971668
139139,1110320,1110320,2220640,3159.7179460525513,0.0029932763609394897
140140,1118322,1118322,2236644,3176.5145070552826,0.002992038129377761
141141,1126322,1126322,2252644,3193.6119890213013,0.0029907684875070117
142142,1134326,1134326,2268652,3210.2704231739044,0.0029904134062235244
143143,1142334,1142334,2284668,3227.2503321170807,0.002990355054862448
144144,1150274,1150274,2300548,3243.9866881370544,0.002012816312344512
145145,1158270,1158270,2316540,3261.2793600559235,0.0020119406653975602
146146,1166272,1166272,2332544,3278.0441200733185,0.002011584019783186
147147,1174272,1174272,2348544,3294.758646965027,0.002011063528698287
148148,1182274,1182274,2364548,3311.7303080558777,0.0020094083811272867
149149,1190278,1190278,2380556,3328.7029650211334,0.002008088009461062
150150,1198278,1198278,2396556,3345.64887714386,0.0020074933490832336
151151,1206278,1206278,2412556,3362.53417801857,0.0020013584198750323
152152,1214280,1214280,2428560,3379.6189329624176,0.0020009602176287444
153153,1222278,1222278,2444556,3396.2066271305084,0.0020004824400530197
154154,1230280,1230280,2460560,3413.147203207016,0.001999698710278608
155155,1238282,1238282,2476564,3429.8134059906006,0.0019974819515482523
156156,1246284,1246284,2492568,3446.621251106262,0.0019954700001107994
157157,1254288,1254288,2508576,3466.7952089309692,0.0019949774505221285
158158,1262294,1262294,2524588,3483.4357781410217,0.0019948639728681883
159159,1270296,1270296,2540592,3500.193377017975,0.001992493851503241
160160,1278296,1278296,2556592,3516.9355058670044,0.0019910818828066112
161161,1286296,1286296,2572592,3533.3914999961853,0.001990525974179036
162162,1294298,1294298,2588596,3549.932160139084,0.0019899763447028818
163163,1302304,1302304,2604608,3566.5633840560913,0.001989778033021139
164164,1310306,1310306,2620612,3582.951446056366,0.001987860594454105
165165,1318310,1318310,2636620,3599.49537730217,0.0019856102735502645
166166,1326314,1326314,2652628,3616.3786959648132,0.0019853122539643664
167167,1334294,1334294,2668588,3633.034252166748,0.0019845467122650007
168168,1342296,1342296,2684592,3649.7457191944122,0.001983988999199937
169169,1350296,1350296,2700592,3666.3260910511017,0.0019832599737128476
170170,1358296,1358296,2716592,3683.2027299404144,0.0019822367485176073
171171,1366302,1366302,2732604,3700.259552001953,0.0019820038542093243
172172,1374296,1374296,2748592,3717.1768839359283,0.001975770999706583
173173,1382298,1382298,2764596,3733.780612230301,0.0019751653635466937
174174,1390306,1390306,2780612,3750.534632921219,0.001975131224753568
175175,1398308,1398308,2796616,3767.1775040626526,0.0019732179353013635
176176,1406314,1406314,2812628,3783.911733150482,0.0019730018630070845
177177,1414314,1414314,2828628,3800.538777112961,0.00197175693938334
178178,1422318,1422318,2844636,3817.0367748737335,0.001971350076928502
179179,1430294,1430294,2860588,3833.829648256302,0.0019710092110472033
180180,1438296,1438296,2876592,3850.5510590076447,0.001970497571164742
181181,1446300,1446300,2892600,3867.3309450149536,0.001970207800695789
182182,1454302,1454302,2908604,3884.154228925705,0.0019698553005582653
183183,1462304,1462304,2924608,3900.8747022151947,0.0019684526305354666
184184,1470304,1470304,2940608,3917.8294270038605,0.0019675469575304305
185185,1478304,1478304,2956608,3934.805018186569,0.001961568781553069
186186,1486304,1486304,2972608,3951.380027294159,0.0019609681348811137
187187,1494304,1494304,2988608,3968.293745994568,0.0019605961279012263
188188,1502308,1502308,3004616,3985.004536151886,0.001960414721907
189189,1510304,1510304,3020608,4001.6913232803345,0.001955682830157457
190190,1518288,1518288,3036576,4018.4278621673584,0.0018290587649971712
191191,1526288,1526288,3052576,4035.2328720092773,0.0018285622536495794
192192,1534286,1534286,3068572,4052.7553882598877,0.0018279729501955444
193193,1542290,1542290,3084580,4069.5769662857056,0.0018277351427968824
194194,1550292,1550292,3100584,4086.3071212768555,0.0018274786398251308
195195,1558286,1558286,3116572,4103.909521102905,0.0018202762457804056
196196,1566288,1566288,3132576,4120.583676099777,0.0018199382229795447
197197,1574284,1574284,3148568,4137.250628232956,0.0018194191143265925
198198,1582282,1582282,3164564,4154.219115018845,0.0018179514390794793
199199,1590284,1590284,3180568,4170.845966100693,0.0018174982797063421
200200,1598286,1598286,3196572,4187.5428121089935,0.001817199250581325
201201,1606286,1606286,3212572,4203.965481996536,0.0018155416782974498
202202,1614286,1614286,3228572,4220.402921915054,0.0018150635587517172
203203,1622284,1622284,3244568,4237.092982053757,0.0018146104102925165
204204,1630282,1630282,3260564,4254.077873945236,0.0018138481937057804
205205,1638282,1638282,3276564,4270.717393159866,0.0018134473648387939
206206,1646282,1646282,3292564,4289.295325994492,0.0018130039461539127
207207,1654282,1654282,3308564,4308.083702087402,0.0018124156431440497
208208,1662282,1662282,3324564,4323.234523296356,0.0018118684238288552
209209,1670288,1670288,3340576,4344.794780254364,0.0018116208175342763
210210,1678278,1678278,3356556,4363.229255914688,0.0017842487068264745
211211,1686276,1686276,3372552,4381.167537927628,0.0017837964369391557
212212,1694274,1694274,3388548,4398.137850046158,0.0017833512392826378
213213,1702274,1702274,3404548,4415.227951049805,0.0017829008011176484
214214,1710278,1710278,3420556,4432.079571008682,0.0017825575887400191
215215,1718280,1718280,3436560,4449.0188620090485,0.0017822324680309976
216216,1726282,1726282,3452564,4465.793895959854,0.0017819373169913888
217217,1734282,1734282,3468564,4482.597526073456,0.0017811731831898214
218218,1742270,1742270,3484540,4499.925736904144,0.0017736832469381625
219219,1750268,1750268,3500536,4516.836786031723,0.0017728162365528988
220220,1758270,1758270,3516540,4533.880578041077,0.0017723042274155887
221221,1766274,1766274,3532548,4551.235173225403,0.001772128845914267
222222,1774268,1774268,3548536,4568.29233789444,0.0017555912017996889
223223,1782274,1782274,3564548,4585.513379096985,0.001755460407366627
224224,1790278,1790278,3580556,4602.482076883316,0.001755268820488709
225225,1798270,1798270,3596540,4619.510792970657,0.0017527921991131734
226226,1806270,1806270,3612540,4636.596781015396,0.0017524571885587648
227227,1814270,1814270,3628540,4653.705342054367,0.0017520185338071315
228228,1822270,1822270,3644540,4670.732409238815,0.0017516719944978831
229229,1830270,1830270,3660540,4687.642586231232,0.00175064630820998
230230,1838260,1838260,3676520,4704.435386180878,0.0017384937400493072
231231,1846260,1846260,3692520,4721.3544199466705,0.0017382769292453304
232232,1854262,1854262,3708524,4738.21338391304,0.0017375549614371266
233233,1862262,1862262,3724524,4754.949258089066,0.001737171793138259
234234,1870264,1870264,3740528,4771.908514022827,0.0017368439876008779
235235,1878258,1878258,3756516,4789.064076185226,0.001719924743156298
236236,1886256,1886256,3772512,4806.272969961166,0.0017192213144880952
237237,1894254,1894254,3788508,4823.683954954147,0.0017184096759592649
238238,1902254,1902254,3804508,4841.083744049072,0.0017177561403514119
239239,1910256,1910256,3820512,4858.519937038422,0.0017174608619825449
240240,1918256,1918256,3836512,4876.424715995789,0.0017168429912999272
241241,1926258,1926258,3852516,4893.527106046677,0.0017165755270980299
242242,1934258,1934258,3868516,4911.228709220886,0.0017115326518251095
243243,1942258,1942258,3884516,4928.559731006622,0.0017110288117692107
244244,1950258,1950258,3900516,4947.375263929367,0.0017106643608713057
245245,1958262,1958262,3916524,4964.439789056778,0.0017102404053730424
246246,1966262,1966262,3932524,4981.468001127243,0.00170963441269123
247247,1974262,1974262,3948524,4998.767392158508,0.0017078480959753506
248248,1982260,1982260,3964520,5015.841014146805,0.001707385063127731
249249,1990264,1990264,3980528,5032.906541109085,0.0017068949509848608
250250,1998272,1998272,3996544,5050.085644006729,0.0017068657853087643
251251,2006280,2006280,4012560,5067.311565160751,0.0017068366214516573
252252,2014280,2014280,4028560,5084.548743963242,0.0017067675798898563
253253,2022276,2022276,4044552,5101.971196174622,0.001706244436718407
254254,2030278,2030278,4060556,5119.445343971252,0.0017060651443898678
255255,2038274,2038274,4076548,5136.672102212906,0.0017034619177138666
256256,2046276,2046276,4092552,5153.91082906723,0.001703102683677571
257257,2054280,2054280,4108560,5171.499056100845,0.0017029346654453548
258258,2062280,2062280,4124560,5188.6377210617065,0.0017009885996230878
259259,2070278,2070278,4140556,5205.955778121948,0.001700369903119281
260260,2078282,2078282,4156564,5223.03466296196,0.0016999990621116012
261261,2086280,2086280,4172560,5240.277059078217,0.001696808276392403
262262,2094280,2094280,4188560,5257.764703989029,0.0016963875477813417
263263,2102280,2102280,4204560,5275.112316131592,0.0016959879958449164
264264,2110266,2110266,4220532,5292.422820091248,0.0016304316395689966
265265,2118268,2118268,4236536,5309.677940130234,0.0016300593688356457
266266,2126266,2126266,4252532,5327.434041023254,0.0016292834352498176
267267,2134268,2134268,4268536,5345.005412101746,0.0016291520678350935
268268,2142268,2142268,4284536,5362.532751083374,0.0016285408582916716
269269,2150270,2150270,4300540,5379.830721139908,0.0016279315768770175
270270,2158270,2158270,4316540,5397.139317035675,0.0016276572932838462
271271,2166270,2166270,4332540,5414.611145019531,0.0016271129170490894
272272,2174276,2174276,4348552,5435.4828979969025,0.0016270623927994166
273273,2182272,2182272,4364544,5453.294513940811,0.0016238256575888954
274274,2190272,2190272,4380544,5470.736958026886,0.0016232460602623178
275275,2198274,2198274,4396548,5487.744978904724,0.001619024551473558
276276,2206276,2206276,4412552,5504.918660163879,0.0016186785196623532
277277,2214278,2214278,4428556,5522.032348155975,0.0016184256310225464
278278,2222282,2222282,4444564,5539.12607216835,0.0016151934614754282
279279,2230286,2230286,4460572,5556.24990105629,0.0016149238745128969
280280,2238290,2238290,4476580,5573.244082927704,0.0016147779751918279
281281,2246290,2246290,4492580,5590.692441225052,0.0016115047747007338
282282,2254288,2254288,4508576,5607.719774007797,0.0016109825774037745
283283,2262290,2262290,4524580,5624.587826967239,0.0016105822505778633
284284,2270294,2270294,4540588,5641.221815109253,0.0016103760590340244
285285,2278294,2278294,4556588,5658.000732898712,0.001607112399142352
286286,2286296,2286296,4572592,5674.791819095612,0.0016067559117800556
287287,2294294,2294294,4588588,5691.802468061447,0.0016060873331298353
288288,2302298,2302298,4604596,5706.12522816658,0.0016058877008617856
289289,2310304,2310304,4620608,5720.3622789382935,0.0016057356206147233
290290,2318304,2318304,4636608,5734.615180015564,0.0016045548145484645
291291,2326304,2326304,4652608,5748.958498001099,0.001604182996743475
292292,2334304,2334304,4668608,5763.07520198822,0.0016038216544984607
293293,2342306,2342306,4684612,5777.285624027252,0.0016035226526582846
294294,2350310,2350310,4700620,5791.413829088211,0.0016032215899031144
295295,2358306,2358306,4716612,5805.5444622039795,0.0015998240323824575
296296,2366308,2366308,4732616,5819.955288171768,0.001599470564542571
297297,2374306,2374306,4748612,5834.293165206909,0.001598995724634733
298298,2382310,2382310,4764620,5848.977005004883,0.0015988195591489784
299299,2390316,2390316,4780632,5863.121335029602,0.0015985606041795108
300300,2398316,2398316,4796632,5877.2717361450195,0.001591165439094766
301301,2406318,2406318,4812636,5891.117640972137,0.001590890218722052
302302,2414322,2414322,4828644,5905.160263299942,0.0015896857512416318
303303,2422320,2422320,4844640,5919.1743841171265,0.0015891138937149663
304304,2430326,2430326,4860652,5933.477260112762,0.0015889955320744775
305305,2438334,2438334,4876668,5947.5183029174805,0.0015889690876065288
306306,2446340,2446340,4892680,5961.813734292984,0.0015889305341261206
307307,2454348,2454348,4908696,5976.074901103973,0.0015889040896581719
308308,2462356,2462356,4924712,5990.2950320243835,0.0015888776451902231
309309,2470364,2470364,4940728,6004.4217710494995,0.0015888512025412638
310310,2478372,2478372,4956744,6018.487023115158,0.0015888247617112938
311311,2486358,2486358,4972716,6032.93607711792,0.0015884447802818613
312312,2494360,2494360,4988720,6047.2323660850525,0.0015882031184446532
313313,2502360,2502360,5004720,6061.608931064606,0.0015876603010838153
314314,2510360,2510360,5020720,6082.786150217056,0.0015873239844950149
315315,2518362,2518362,5036724,6098.6028571128845,0.001587023130923626
316316,2526364,2526364,5052728,6113.883697271347,0.0015843082201172365
317317,2534360,2534360,5068720,6130.986830234528,0.0015821121123735793
318318,2542364,2542364,5084728,6147.470840215683,0.001581909700689721
319319,2550366,2550366,5100732,6162.920146942139,0.0015816230297787115
320320,2558366,2558366,5116732,6177.846074104309,0.001581221898959484
321321,2566368,2566368,5132736,6193.280166149139,0.0015809911437827395
322322,2574370,2574370,5148740,6208.609596252441,0.0015805898983671796
323323,2582372,2582372,5164744,6223.669548034668,0.001580210380780045
324324,2590372,2590372,5180744,6240.285578966141,0.0015794757582625607
325325,2598374,2598374,5196748,6261.034747123718,0.0015786115036462434
326326,2606376,2606376,5212752,6281.012468099594,0.0015783915932843229
327327,2614380,2614380,5228760,6297.827601909637,0.0015779262357682455
328328,2622382,2622382,5244764,6314.458093166351,0.0015761101349198725
329329,2630382,2630382,5260764,6331.048300981522,0.0015738257479824824
330330,2638384,2638384,5276768,6347.67218708992,0.001573407114847214
331331,2646382,2646382,5292764,6364.542471885681,0.0015729379829281243
332332,2654384,2654384,5308768,6381.197369098663,0.0015699497344030533
333333,2662384,2662384,5324768,6398.05962395668,0.0015693794903199887
334334,2670388,2670388,5340776,6415.056812047958,0.0015690304262534482
335335,2678390,2678390,5356780,6432.367347955704,0.0015656094219593797
336336,2686392,2686392,5372784,6448.893322944641,0.0015654728395020356
337337,2694380,2694380,5388760,6465.169562101364,0.0015273121334757889
338338,2702380,2702380,5404760,6481.716746091843,0.001526631205706508
339339,2710380,2710380,5420760,6498.221784114838,0.0015262289543898078
340340,2718382,2718382,5436764,6514.7818722724915,0.001525617808511015
341341,2726384,2726384,5452768,6531.204698085785,0.0015250881988322362
342342,2734384,2734384,5468768,6547.587015867233,0.0015214038467092905
343343,2742382,2742382,5484764,6564.125246047974,0.0015210888577712467
344344,2750382,2750382,5500764,6580.590044260025,0.0015207139440462925
345345,2758386,2758386,5516772,6597.162959098816,0.0015175961143540917
346346,2766388,2766388,5532776,6613.452949047089,0.0015174393429333577
347347,2774390,2774390,5548780,6630.442687034607,0.0015164504893618869
348348,2782388,2782388,5564776,6647.356224060059,0.0015159080267039826
349349,2790378,2790378,5580756,6664.287879943848,0.0014498840791929979
350350,2798378,2798378,5596756,6681.013375043869,0.001449638717531343
351351,2806382,2806382,5612764,6697.5081951618195,0.0014475410043814918
352352,2814384,2814384,5628768,6714.145865917206,0.0014472559469140833
353353,2822388,2822388,5644776,6730.593089103699,0.0014468089793808758
354354,2830392,2830392,5660784,6747.419090986252,0.0014466271350102033
355355,2838396,2838396,5676792,6763.923634052277,0.0014459622179856524
356356,2846400,2846400,5692800,6780.54120016098,0.001445618658181047
357357,2854404,2854404,5708808,6797.100882053375,0.0014453617131948704
358358,2862406,2862406,5724812,6813.816833972931,0.0014429976654355414
359359,2870410,2870410,5740820,6829.9813911914825,0.0014426911966438638
360360,2878414,2878414,5756828,6846.2686240673065,0.0014414297038456425
361361,2886418,2886418,5772836,6862.638086080551,0.0014413742846954847
362362,2894422,2894422,5788844,6879.103418111801,0.0014411463871510932
363363,2902422,2902422,5804844,6895.7084720134735,0.001440830734281917
364364,2910414,2910414,5820828,6912.146491289139,0.001423713274562033
365365,2918416,2918416,5836832,6928.87047123909,0.0014233820620574988
366366,2926418,2926418,5852836,6945.911933898926,0.0014229860480554635
367367,2934420,2934420,5868840,6962.763422966003,0.0014224668320821365
368368,2942420,2942420,5884840,6979.451199054718,0.0014221154469851172
369369,2950420,2950420,5900840,6996.133891105652,0.0014214807051757816
370370,2958420,2958420,5916840,7012.702589035034,0.0014212034038791899
371371,2966426,2966426,5932852,7029.49631524086,0.0014209827877493808
372372,2974426,2974426,5948852,7046.232782125473,0.0014177400043990929
373373,2982428,2982428,5964856,7062.976998090744,0.0014174136085784994
374374,2990430,2990430,5980860,7079.657286167145,0.001417136205418501
375375,2998432,2998432,5996864,7096.292495250702,0.0014169327459967462
376376,3006434,3006434,6012868,7112.931990146637,0.0014167562585498672
377377,3014438,3014438,6028876,7129.852472066879,0.0014161132839944912
378378,3022444,3022444,6044888,7146.961318254471,0.0014160477185214404
379379,3030450,3030450,6060900,7164.131192207336,0.001415953744071885
380380,3038458,3038458,6076916,7181.032028198242,0.0014159303373162402
381381,3046466,3046466,6092932,7197.704263210297,0.001415906928741606
382382,3054448,3054448,6108896,7214.210344076157,0.001091110903871595
383383,3062442,3062442,6124884,7230.553340911865,0.0010908970216405578
384384,3070440,3070440,6140880,7247.001633167267,0.0010904486116487533
385385,3078442,3078442,6156884,7263.255464076996,0.0010902238100243267
386386,3086444,3086444,6172888,7279.616072893143,0.0010897791744355345
387387,3094448,3094448,6188896,7296.124223947525,0.0010882545248023234
388388,3102456,3102456,6204912,7312.5552570819855,0.0010882354035857134
389389,3110458,3110458,6220916,7329.119206190109,0.001086270769519615
390390,3118462,3118462,6236924,7345.767804861069,0.0010859486683330033
391391,3126466,3126466,6252932,7362.300738096237,0.00108435772563098
392392,3134466,3134466,6268932,7379.657177209854,0.0010841186303878203
393393,3142472,3142472,6284944,7396.274076223373,0.0010839623300853418
394394,3150476,3150476,6300952,7412.931876182556,0.0010824661985679995
395395,3158482,3158482,6316964,7429.9169862270355,0.0010808389924932271
396396,3166484,3166484,6332968,7446.371974229813,0.0010806159607454902
397397,3174484,3174484,6348968,7462.836834192276,0.0010803574386955006
398398,3182488,3182488,6364976,7479.322140216827,0.001077916791473399
399399,3190494,3190494,6380988,7495.821266889572,0.0010778878422570415
400400,3198496,3198496,6396992,7512.261138916016,0.001076239044778049
401401,3206504,3206504,6413008,7528.891694068909,0.001076220027243835
402402,3214510,3214510,6429020,7545.3054258823395,0.001076162110621226
403403,3222512,3222512,6445024,7561.8538200855255,0.0010746818861662177
404404,3230516,3230516,6461032,7578.46585226059,0.001074563164365827
405405,3238516,3238516,6477032,7593.082453012466,0.0010714926611399278
406406,3246520,3246520,6493040,7607.215425014496,0.001071327524186927
407407,3254524,3254524,6509048,7621.2485382556915,0.001071103415597463
408408,3262532,3262532,6525064,7635.2091290950775,0.0010710844417189946
409409,3270526,3270526,6541052,7649.197813034058,0.0010488872685527895
410410,3278528,3278528,6557056,7663.3746790885925,0.001048572488798527
411411,3286532,3286532,6573064,7677.331822156906,0.0010484558133612154
412412,3294534,3294534,6589068,7691.325779914856,0.0010467718948348192
413413,3302542,3302542,6605084,7705.382393121719,0.0010467531174072064
414414,3310546,3310546,6621092,7719.521688222885,0.001046351333570783
415415,3318550,3318550,6637100,7733.6123032569885,0.0010462118807481602
416416,3326554,3326554,6653108,7747.658348083496,0.0010458358192408923
417417,3334558,3334558,6669116,7761.783930063248,0.0010456346044520615
418418,3342564,3342564,6685128,7776.630259037018,0.0010455685260239989
419419,3350566,3350566,6701132,7790.840553998947,0.0010443323062645504
420420,3358566,3358566,6717132,7804.037887096405,0.001040607676259242
421421,3366572,3366572,6733144,7816.821014165878,0.0010394996734248707
422422,3374576,3374576,6749152,7828.644674062729,0.0010394340370112332
423423,3382578,3382578,6765156,7840.061057090759,0.0010390969546278939
424424,3390582,3390582,6781164,8730.009188175201,0.0010383519584138412
425425,3398586,3398586,6797172,8770.025446176529,0.0010381912361481227
426426,3406592,3406592,6813184,9708.871412992477,0.0010381021638750099
427427,3414598,3414598,6829196,9760.416160106659,0.0010364648824179312
428428,3422604,3422604,6845208,9809.55641913414,0.0010364300615037791
429429,3430612,3430612,6861224,9856.093774080276,0.0010364113713876577
430430,3438582,3438582,6877164,10793.070572137833,0.001035652005157317
431431,3446574,3446574,6893148,11731.227354049683,0.0010354389087297022
432432,3454572,3454572,6909144,11779.0992770195,0.0010352147255616728
433433,3462572,3462572,6925144,11827.287668943405,0.0010349030962970573
434434,3470574,3470574,6941148,11875.54084610939,0.001034762117342325
435435,3478578,3478578,6957156,11923.957799911499,0.0010304359821020626
436436,3486578,3486578,6973156,11969.206002950668,0.001030145276672556
437437,3494578,3494578,6989156,12008.625719070435,0.001029986282446771
438438,3502578,3502578,7005156,12047.917563199997,0.0010296831369487336
439439,3510578,3510578,7021156,12087.398347139359,0.0010294921066815732
440440,3518580,3518580,7037160,12126.831684112549,0.0010292169099557213
441441,3526586,3526586,7053172,12166.268202066422,0.0010281007762387162
442442,3534584,3534584,7069168,12207.354279994965,0.0010278287845721934
443443,3542588,3542588,7085176,12255.768394947052,0.001027759466524003
444444,3550588,3550588,7101176,12303.986257076263,0.0010273242187395226
445445,3558588,3558588,7117176,12343.947348117828,0.0010269018202961888
446446,3566592,3566592,7133184,12383.657984972,0.0010258773691020906
447447,3574600,3574600,7149200,12423.346771001816,0.001025862839014735
448448,3582600,3582600,7165200,12462.77928185463,0.001025500294417725
449449,3590604,3590604,7181208,12502.207864046097,0.0010253737618768355
450450,3598606,3598606,7197212,12549.487977981567,0.0010248327107547084
451451,3606608,3606608,7213216,12598.053055047989,0.0010245113480777945
452452,3614612,3614612,7229224,12640.942888975143,0.0010243594733765349
453453,3622614,3622614,7245228,12680.503710985184,0.001023686965709203
454454,3630612,3630612,7261224,12719.856669902802,0.001020976276777219
455455,3638614,3638614,7277228,12759.254215240479,0.0010208529365627328
456456,3646618,3646618,7293236,12798.718556880951,0.0010193845118919853
457457,3654624,3654624,7309248,12844.793382167816,0.0010193434627581155
458458,3662624,3662624,7325248,12892.995398283005,0.0010178529701079242
459459,3670624,3670624,7341248,12939.046565055847,0.0010176196847169194
460460,3678626,3678626,7357252,12978.418396234512,0.0010159905068576336
461461,3686630,3686630,7373260,13018.143195152283,0.0010158222321479116
462462,3694632,3694632,7389264,13057.54843711853,0.0010153273069590796
463463,3702630,3702630,7405260,13096.957174062729,0.0010134018884855323
464464,3710632,3710632,7421264,13142.07751917839,0.0010132872776011936
465465,3718638,3718638,7437276,13190.421263217926,0.0010129373767995276
466466,3726638,3726638,7453276,13236.221063137054,0.0010112805157405091
467467,3734640,3734640,7469280,13275.669817209244,0.0010112105101143243
468468,3742642,3742642,7485284,13315.23275899887,0.0010110324474226218
469469,3750644,3750644,7501288,13354.53630900383,0.0010108584974659607
470470,3758648,3758648,7517296,13394.379642248154,0.0010088782419188647
471471,3766654,3766654,7533308,13440.969098091125,0.0010081726832140703
472472,3774654,3774654,7549308,13489.46995306015,0.0010064310172310797
473473,3782652,3782652,7565304,13534.901252031326,0.0010042013782367576
474474,3790654,3790654,7581308,13574.33845615387,0.0010039999378932407
475475,3798654,3798654,7597308,13613.698937177658,0.0010037285992439138
476476,3806658,3806658,7613316,13653.040405035019,0.0010029168206528993
477477,3814664,3814664,7629328,13692.688824176788,0.0010028201540990267
478478,3822668,3822668,7645336,13738.137032032013,0.0010025952869909815
479479,3830674,3830674,7661348,13786.835989952087,0.0010024546627391828
480480,3838678,3838678,7677356,13832.195088148117,0.0010017106360464823
481481,3846682,3846682,7693364,13871.704196214676,0.0010015435291279573
482482,3854682,3854682,7709364,13911.20905303955,0.0010009937996073859
483483,3862686,3862686,7725372,13950.973443031311,0.001000810059849755
484484,3870690,3870690,7741380,13990.26261305809,0.0009995849741244456
485485,3878698,3878698,7757396,14036.033931970596,0.0009995707259804476
486486,3886700,3886700,7773400,14085.651568174362,0.0009975938992283773
487487,3894704,3894704,7789408,14134.4519469738,0.0009975597204174846
488488,3902708,3902708,7805416,14175.69886302948,0.0009969372786144959
489489,3910712,3910712,7821424,14215.298135995865,0.000996853421384003
490490,3918716,3918716,7837432,14254.853105306625,0.0009966324960259954
491491,3926712,3926712,7853424,14294.288234949112,0.000990809581708163
492492,3934708,3934708,7869416,14336.167111873627,0.000990558761259308
493493,3942710,3942710,7885420,14384.636595964432,0.0009899303477141075
494494,3950714,3950714,7901428,14433.421742200851,0.0009898680509650148
495495,3958718,3958718,7917436,14477.014634132385,0.000988856379990466
496496,3966718,3966718,7933436,14516.625042915344,0.0009883805414574454
497497,3974726,3974726,7949452,14556.115123033524,0.0009883664170047268
498498,3982730,3982730,7965460,14595.625297307968,0.0009871443271549651
499499,3990732,3990732,7981464,14639.716610193253,0.000986959392321296
500501,3998746,3998746,7997492,14688.38225197792,0.0009855586376943393
501502,4006746,4006746,8013492,14736.436348199844,0.0009854153340711491
502503,4014748,4014748,8029496,14775.886017084122,0.0009852476432570256
503504,4022752,4022752,8045504,14815.269476175308,0.000985146298262407
504505,4030754,4030754,8061508,14854.807982206345,0.000984854386842926
505506,4038758,4038758,8077516,14894.257657051086,0.000983491805527592
506507,4046758,4046758,8093516,14939.122663974762,0.000983297810307704
507508,4054760,4054760,8109520,14987.845247983932,0.0009831162606133148
508509,4062766,4062766,8125532,15035.81881403923,0.0009829304417507956
509510,4070766,4070766,8141532,15075.281742095947,0.0009806921661947854
510511,4078772,4078772,8157544,15114.572703123093,0.0009805874269659398
511512,4086772,4086772,8173544,15153.960842132568,0.000979198752247612
512513,4094774,4094774,8189548,15193.79343008995,0.000978812102403026
513514,4102774,4102774,8205548,15238.883230924606,0.0009764142669155262
514515,4110776,4110776,8221552,15287.32487821579,0.0009762646113813389
515516,4118778,4118778,8237556,15334.306031227112,0.0009761278070072876
516517,4126774,4126774,8253548,15373.730783939362,0.0009493963825661922
517518,4134776,4134776,8269552,15413.074673891068,0.0009493280758761102
518519,4142776,4142776,8285552,15452.600355148315,0.0009491663367953151
519520,4150776,4150776,8301552,15492.551743984222,0.0009487139668635791
520521,4158782,4158782,8317564,15539.289608001709,0.0009486762191954767
521522,4166782,4166782,8333564,15587.677145242691,0.0009469208653172245
522523,4174788,4174788,8349576,15633.250422000885,0.0009461805584578542
523524,4182794,4182794,8365588,15672.554786205292,0.000946139318330097
524525,4190794,4190794,8381588,15711.975147008896,0.0009450095403735759
525526,4198796,4198796,8397592,15751.490264177322,0.0009439536206627963
526527,4206804,4206804,8413608,15790.880368232727,0.0009439399509574287
527528,4214806,4214806,8429612,15838.177994012833,0.0009437927019462222
528529,4222806,4222806,8445612,15886.932890176773,0.0009434334406250855
529530,4230812,4230812,8461624,15931.936845064163,0.0009433613413420971
530531,4238812,4238812,8477624,15971.316534996033,0.0009428736811969429
531532,4246816,4246816,8493632,16011.182700157166,0.0009416256616532337
532533,4254820,4254820,8509640,16050.566263198853,0.0009415099575562635
533534,4262826,4262826,8525652,16090.129743099213,0.0009414267424290301
534535,4270828,4270828,8541656,16138.262183904648,0.0009396855257364223
535536,4278832,4278832,8557664,16186.984627962112,0.000939561026825686
536537,4286834,4286834,8573668,16232.412539243698,0.0009386116234963993
537538,4294838,4294838,8589676,16271.939949035645,0.0009385178182128584
538539,4302836,4302836,8605672,16311.244721889496,0.0009383368796989089
539540,4310842,4310842,8621684,16350.637172937393,0.0009360353487863904
540541,4318848,4318848,8637696,16390.202007055283,0.0009360047461086651
541542,4326852,4326852,8653704,16438.25026512146,0.0009355818092444679
542543,4334860,4334860,8669720,16487.070801258087,0.0009355682213936234
543544,4342850,4342850,8685700,16531.854471206665,0.0009354416870337445
544545,4350834,4350834,8701668,16571.07764315605,0.000935287396714557
545546,4358832,4358832,8717664,16610.857329130173,0.0009350223735964391
546547,4366836,4366836,8733672,16650.336185216904,0.0009348607400170295
547548,4374838,4374838,8749676,16692.475993156433,0.0009347176037408644
548549,4382842,4382842,8765684,16740.713244199753,0.0009332767294836231
549550,4390844,4390844,8781688,16789.11185312271,0.00093230374113773
550551,4398842,4398842,8797684,16831.128580093384,0.0009321678335254546
551552,4406838,4406838,8813676,16870.413310050964,0.0009291510104958434
552553,4414840,4414840,8829680,16909.731667995453,0.0009290200960094808
553554,4422844,4422844,8845688,16949.12661910057,0.0009281726743211038
554555,4430844,4430844,8861688,16990.59442305565,0.000927965518712881
555556,4438842,4438842,8877684,17038.834884166718,0.0009273104151361622
556557,4446844,4446844,8893688,17087.18335199356,0.0009257304718630621
557558,4454840,4454840,8909680,17129.83329319954,0.0009256047742383089
558559,4462840,4462840,8925680,17169.407524108887,0.0009255074110114947
559560,4470842,4470842,8941684,17208.812999248505,0.000925225440369104
560561,4478840,4478840,8957680,17248.395651102066,0.0009249370123143308
561562,4486842,4486842,8973684,17291.429239034653,0.0009247395591955865
562563,4494840,4494840,8989680,17339.64773106575,0.0009246206700481707
563564,4502842,4502842,9005684,17388.235463142395,0.0009234883455064846
564565,4510842,4510842,9021684,17429.31130504608,0.0009232895154127618
565566,4518842,4518842,9037684,17468.646822929382,0.0009230931336787762
566567,4526844,4526844,9053688,17508.084364175797,0.0009226015536114573
567568,4534834,4534834,9069668,17547.47334098816,0.0009093751996260835
568569,4542830,4542830,9085660,17590.0454351902,0.0009090259063668782
569570,4550836,4550836,9101672,17638.339558124542,0.0009089821687666699
570571,4558832,4558832,9117664,17687.25378894806,0.0009077969625650439
571572,4566838,4566838,9133676,17728.868302106857,0.0009077349477593089
572573,4574840,4574840,9149680,17768.480419158936,0.000907627885680995
573574,4582842,4582842,9165684,17808.16235113144,0.0009074847821466392
574575,4590846,4590846,9181692,17847.45920729637,0.0009073822875507176
575576,4598846,4598846,9197692,17889.758854150772,0.0009070969517779304
576577,4606852,4606852,9213704,17938.07600212097,0.0009059835974767338
577578,4614850,4614850,9229700,17986.487910985947,0.0009057977022166597
578579,4622854,4622854,9245708,18028.23484802246,0.0009056051912921248
579580,4630850,4630850,9261700,18067.61696410179,0.0009054635393113131
580581,4638850,4638850,9277700,18107.045896053314,0.0009052756449818844
581582,4646850,4646850,9293700,18146.507389068604,0.0009051240485860035
582583,4654846,4654846,9309692,18190.627222061157,0.0009049640957528027
583584,4662844,4662844,9325688,18238.9017059803,0.0009046371869771974
584585,4670846,4670846,9341692,18287.39178299904,0.0009037327199621359
585586,4678850,4678850,9357700,18327.765547037125,0.0009030440633068793
586587,4686850,4686850,9373700,18367.29949903488,0.0009029394441313343
587588,4694852,4694852,9389704,18406.56869506836,0.0009012899208755698
588589,4702852,4702852,9405704,18446.252885103226,0.0009002403166959994
589590,4710852,4710852,9421704,18490.810840129852,0.0009000735590234399
590591,4718852,4718852,9437704,18538.938153982162,0.0008999248875625199
591592,4726856,4726856,9453712,18587.309746026993,0.0008989851230580825
592593,4734862,4734862,9469724,18626.829208135605,0.0008989316320366925
593594,4742864,4742864,9485728,18666.270438194275,0.0008979182421171572
594595,4750864,4750864,9501728,18706.19402909279,0.0008977720117400168
595596,4758866,4758866,9517732,18745.713248968124,0.0008974718984973151
596597,4766868,4766868,9533736,18792.327729940414,0.0008973958811111515
597598,4774870,4774870,9549740,18840.436472177505,0.0008972552841441939
598599,4782872,4782872,9565744,18887.298187971115,0.0008970335384219652
599600,4790878,4790878,9581756,18926.95513010025,0.0008969699683802901
600601,4798882,4798882,9597764,18966.635987997055,0.0008968444672063924
601602,4806884,4806884,9613768,19005.992882966995,0.000896765533980215
602603,4814888,4814888,9629776,19045.520119190216,0.0008965864526544465
603604,4822890,4822890,9645780,19093.829936265945,0.0008964149019448087
604605,4830890,4830890,9661780,19142.140773057938,0.0008963353120634565
605606,4838892,4838892,9677784,19186.25747203827,0.0008962576703197556
606607,4846890,4846890,9693780,19225.554188013077,0.0008960813520388911
607608,4854890,4854890,9709780,19265.489710092545,0.0008958977268775925
608609,4862890,4862890,9725780,19304.965707063675,0.0008933877070376184
609610,4870888,4870888,9741776,19346.698933124542,0.0008932143391575664
610611,4878886,4878886,9757772,19395.215715169907,0.0008930918029363966
611612,4886886,4886886,9773772,19443.59343099594,0.0008928334718802944
612613,4894888,4894888,9789776,19485.716962099075,0.0008927152248361381
613614,4902888,4902888,9805776,19525.29750919342,0.0008862561899150023
614615,4910890,4910890,9821780,19564.82728409767,0.0008860937487042975
615616,4918896,4918896,9837792,19604.282044887543,0.0008860358138917945
616617,4926892,4926892,9853784,19649.401239156723,0.0008853000799717847
617618,4934894,4934894,9869788,19697.715180158615,0.0008844625026540598
618619,4942898,4942898,9885796,19745.33118224144,0.0008837350615067407
619620,4950902,4950902,9901804,19785.261074066162,0.0008837142704578582
620621,4958902,4958902,9917804,19825.039817094803,0.0008833849715301767
621622,4966904,4966904,9933808,19864.631578207016,0.0008832604999042815
622623,4974900,4974900,9949800,19905.731548309326,0.0008830837014102144
623624,4982904,4982904,9965808,19954.145275115967,0.0008828892132441979
624625,4990908,4990908,9981816,20002.590667963028,0.0008827619203657378
625626,4998908,4998908,9997816,20045.16315817833,0.0008825513741612667
626627,5006912,5006912,10013824,20084.91286087036,0.0008809281607682351
627628,5014920,5014920,10029840,20124.54239010811,0.0008809176779323025
628629,5022922,5022922,10045844,20164.23545408249,0.0008799858769634739
629630,5030930,5030930,10061860,20209.403027057648,0.0008799754050414776
630631,5038900,5038900,10077800,20258.08243727684,0.0008798092694632942
631632,5046898,5046898,10093796,20306.86972308159,0.0008796283636911539
632633,5054900,5054900,10109800,20347.23977613449,0.000879393139257445
633634,5062898,5062898,10125796,20386.791515111923,0.0008792235166765749
634635,5070896,5070896,10141792,20426.25981593132,0.0008791056843620026
635636,5078898,5078898,10157796,20465.761579990387,0.0008790046504145721
636637,5086902,5086902,10173804,20511.32465004921,0.0008780426087469095
637638,5094902,5094902,10189804,20559.88543200493,0.0008770557324169204
638639,5102902,5102902,10205804,20607.79978609085,0.0008768895768298535
639640,5110902,5110902,10221804,20647.26097726822,0.0008767732306296239
640641,5118906,5118906,10237812,21663.786453962326,0.0008764566446188837
641642,5126904,5126904,10253808,21695.78417992592,0.0008746307976252865
642643,5134902,5134902,10269804,21743.99830198288,0.0008737235275475541
643644,5142906,5142906,10285812,21792.2275390625,0.000873631979629863
644645,5150906,5150906,10301812,21840.549160003662,0.0008734312286833301
645646,5158910,5158910,10317820,21889.302610874176,0.0008724294184503378
646647,5166908,5166908,10333816,21932.939080953598,0.000872187460117857
647648,5174906,5174906,10349812,21972.494771003723,0.000871749676662148
648649,5182906,5182906,10365812,22012.128821134567,0.0008715918702364434
649650,5190906,5190906,10381812,22051.619173049927,0.0008692684477864532
650651,5198906,5198906,10397812,22091.025842905045,0.000869158599016373
651652,5206906,5206906,10413812,22132.831834077835,0.0008690624326845864
652653,5214908,5214908,10429816,22181.221370220184,0.0008688734214956639
653654,5222910,5222910,10445820,22229.79891705513,0.0008685203174536582
654655,5230912,5230912,10461824,22269.61724805832,0.0008684024614922237
655656,5238912,5238912,10477824,22309.140522003174,0.0008682145980856149
656657,5246916,5246916,10493832,22348.568348169327,0.0008678165577293839
657658,5254916,5254916,10509832,22388.423590898514,0.0008657190392113989
658659,5262916,5262916,10525832,22436.50910305977,0.0008656089521537069
659660,5270916,5270916,10541832,22484.769936084747,0.0008652367814647732
660661,5278916,5278916,10557832,22527.49671125412,0.0008650515519548208
661662,5286918,5286918,10573836,22567.17841887474,0.0008649126048112521
662663,5294920,5294920,10589840,22606.575864076614,0.0008647572740301257
663664,5302920,5302920,10605840,22646.312976121902,0.0008646683036204195
664665,5310920,5310920,10621840,22685.683002233505,0.0008631138698547147
665666,5318924,5318924,10637848,22733.211273908615,0.000862997374497354
666667,5326930,5326930,10653860,22781.427723169327,0.000862903365487
667668,5334930,5334930,10669860,22825.06713604927,0.000862723010868649
668669,5342932,5342932,10685864,22864.707436084747,0.0008625970876892097
669670,5350936,5350936,10701872,22904.225986003876,0.0008623064386483748
670671,5358936,5358936,10717872,22944.10759305954,0.0008620862809038954
671672,5366940,5366940,10733880,22983.551233053207,0.0008611601115262602
672673,5374942,5374942,10749884,23032.01819396019,0.0008610875465819845
673674,5382942,5382942,10765884,23080.413093090057,0.0008597278501838446
674675,5390946,5390946,10781892,23125.59328007698,0.000859617584865191
675676,5398948,5398948,10797896,23165.163246154785,0.0008594294940849068
676677,5406956,5406956,10813912,23204.715538978577,0.0008594196442572866
677678,5414958,5414958,10829916,23244.0772690773,0.0008581901365687372
678679,5422954,5422954,10845908,23284.42505812645,0.0008567920831410447
679680,5430956,5430956,10861912,23332.729908943176,0.0008566836386307841
680681,5438964,5438964,10877928,23380.98162007332,0.000856673825182952
681682,5446968,5446968,10893936,23423.146461963654,0.0008565980115236016
682683,5454968,5454968,10909936,23463.579627990723,0.0008563179580960423
683684,5462972,5462972,10925944,23503.13823413849,0.0008562543807784095
684685,5470976,5470976,10941952,23542.74988102913,0.0008561832255509216
685686,5478954,5478954,10957908,23585.623568058014,0.0004885468133579707
686687,5486954,5486954,10973908,23633.885631084442,0.0004885312555416021
687688,5494952,5494952,10989904,23682.26042699814,0.0004884694008069346
688689,5502956,5502956,11005912,23722.32472205162,0.0004884330282948213
689690,5510962,5510962,11021924,23762.13770699501,0.0004883275323663838
690691,5518970,5518970,11037940,23801.409679174423,0.0004883214969595429
691692,5526970,5526970,11053940,23840.733636140823,0.0004873328980465885
692693,5534974,5534974,11069948,23885.93261694908,0.0004872557437920477
693694,5542982,5542982,11085964,23934.489269018173,0.00048724971384217497
694695,5550988,5550988,11101976,23981.76428604126,0.00048690404582885094
695696,5558994,5558994,11117988,24021.24706196785,0.0004868499036092544
696697,5567000,5567000,11134000,24061.17277121544,0.00048683418754080776
697698,5575000,5575000,11150000,24100.782286167145,0.00048621058522257954
698699,5583008,5583008,11166016,24140.307128190994,0.0004862045643676538
699700,5591012,5591012,11182024,24187.985157251358,0.000486090570120723
700701,5599020,5599020,11198040,24236.37485909462,0.00048608454562781844
701702,5607026,5607026,11214052,24280.99907398224,0.00048585191871097777
702703,5615034,5615034,11230068,24320.529563188553,0.00048584589785605203
703704,5623038,5623038,11246076,24360.013911008835,0.0004857917065237416
704705,5631044,5631044,11262088,24399.715486049652,0.0004854812359553762
705706,5639052,5639052,11278104,24439.067890882492,0.00048547521873842925
706707,5647060,5647060,11294120,24487.72128510475,0.0004854691997024929
707708,5655066,5655066,11310132,24536.313909053802,0.00048529997729929164
708709,5663074,5663074,11326148,24581.787434101105,0.0004852939564443659
709710,5671080,5671080,11342160,24621.20397901535,0.0004852351630688645
710711,5679088,5679088,11358176,24660.72308921814,0.00048522914403292816
711712,5687094,5687094,11374188,24700.160380125046,0.00048503872312721796
712713,5695102,5695102,11390204,24739.835705041885,0.00048503270591027103
713714,5703110,5703110,11406220,24787.944179058075,0.0004850266886933241
714715,5711114,5711114,11422228,24836.970885276794,0.0004847092968702782
715716,5719120,5719120,11438240,24882.158541202545,0.0004843901679123519
716717,5727124,5727124,11454248,24921.597280979156,0.0004843768219870981
717718,5735132,5735132,11470264,24961.07811999321,0.00048437080840812996
718719,5743136,5743136,11486272,25000.571092128754,0.00048433721349283587
719720,5751140,5751140,11502280,25041.83252310753,0.00048311265345546417
720721,5759144,5759144,11518288,25090.192164182663,0.00048307914585166145
721722,5767152,5767152,11534304,25138.52984714508,0.00048307314136764035
722723,5775156,5775156,11550312,25181.760250091553,0.00048262222117045894
723724,5783158,5783158,11566316,25221.393742084503,0.0004825814648938831
724725,5791164,5791164,11582328,25261.01671719551,0.00048252823398797773
725726,5799168,5799168,11598336,25301.10906815529,0.00048247813720081467
726727,5807172,5807172,11614344,25345.975255012512,0.00048178317774727475
727728,5815178,5815178,11630356,25394.2626349926,0.0004812698589375941
728729,5823182,5823182,11646364,25441.943697929382,0.0004812419902009424
729730,5831188,5831188,11662376,25481.329730033875,0.0004811980288650375
730731,5839192,5839192,11678384,25520.82314491272,0.00048099536797963083
731732,5847196,5847196,11694392,25560.677588939667,0.0004809245747310342
732733,5855204,5855204,11710408,25600.01916217804,0.00048091858297993895
733734,5863210,5863210,11726420,25646.80811023712,0.00048083722685987595
734735,5871218,5871218,11742436,25695.021356105804,0.00048083123328979127
735736,5879222,5879222,11758444,25740.965832948685,0.0004803054871445056
736737,5887226,5887226,11774452,29149.92858695984,0.00048027525372162927
737738,5895232,5895232,11790464,30200.600572109222,0.00048020040958363097
738739,5903240,5903240,11806480,30227.800886154175,0.0004801944214705145
739740,5911244,5911244,11822488,30275.708631038666,0.0004796868815901689
740741,5919248,5919248,11838496,30323.439146995544,0.0004796551111212466
741742,5927256,5927256,11854512,31385.643567085266,0.0004796491230081301
742743,5935262,5935262,11870524,31425.515169143677,0.0004795731802005321
743744,5943270,5943270,11886540,31473.194390058517,0.000479567193906405
744745,5951276,5951276,11902552,31520.384471178055,0.0004794590076926397
745746,5959284,5959284,11918568,31559.34072613716,0.00047945301957952324
746747,5967290,5967290,11934580,31597.95636987686,0.0004794220094481716
747748,5975298,5975298,11950596,31632.23523902893,0.0004794160231540445
748749,5983300,5983300,11966600,31663.130172252655,0.0004786897825397318
749750,5991306,5991306,11982612,31693.100288152695,0.0004784565062436741
750751,5999314,5999314,11998628,31723.066598892212,0.00047845052722550463
751752,6007320,6007320,12014640,32801.68294906616,0.00047842448293522466
752753,6015328,6015328,12030656,32838.65291810036,0.0004784185002790764
753754,6023330,6023330,12046660,32886.27066612244,0.0004782024880114477
754755,6031336,6031336,12062672,32934.14724826813,0.00047818013081268873
755756,6039342,6039342,12078684,32973.397439956665,0.000478114903671667
756757,6047348,6047348,12094696,33012.13684415817,0.0004775594024977181
757758,6055352,6055352,12110704,33047.01950216293,0.000477536990729277
758759,6063356,6063356,12126712,33078.31833910942,0.0004774937842739746
759760,6071362,6071362,12142724,33108.33161020279,0.00047733319661347196
760761,6079370,6079370,12158740,33138.37141919136,0.0004773272248712601
761762,6087378,6087378,12174756,33168.27379608154,0.00047732124767208006
762763,6095384,6095384,12190768,33197.89035105705,0.0004773046548507409
763764,6103388,6103388,12206776,33228.596640110016,0.0004772537104145158
764765,6111396,6111396,12222792,33260.991595983505,0.00047724773685331456
765766,6119400,6119400,12238800,33293.88696408272,0.00047597509728802834
766767,6127408,6127408,12254816,33326.22133517265,0.0004759691291837953
767768,6135410,6135410,12270820,33356.29237604141,0.00047550812632835004
768769,6143416,6143416,12286832,33386.195674180984,0.00047549355986120645
769770,6151422,6151422,12302844,33416.04671216011,0.00047541476124024484
770771,6159428,6159428,12318856,34472.45931601524,0.0004753730972879566
771772,6167432,6167432,12334864,34500.42791008949,0.00047413084575964604
772773,6175440,6175440,12350880,34548.32572412491,0.0004741248885693494
773774,6183448,6183448,12366896,34596.17824792862,0.0004741189313790528
774775,6191456,6191456,12382912,34637.55771112442,0.0004741129760077456
775776,6199462,6199462,12398924,34676.552289009094,0.0004740321764984401
776777,6207470,6207470,12414940,34712.897887945175,0.0004740262211271329
777778,6215478,6215478,12430956,34744.813343048096,0.0004740202657558257
778779,6223484,6223484,12446968,34774.848922252655,0.00047364079910039436
779780,6231492,6231492,12462984,34804.91082215309,0.00047363484554807656
780781,6239500,6239500,12479000,34834.89660692215,0.00047362889017676935
781782,6247508,6247508,12495016,34865.18705511093,0.00047362293480546214
782783,6255514,6255514,12511028,34896.32366323471,0.00047358666961372364
783784,6263518,6263518,12527036,34928.728654146194,0.0004733412861241959
784785,6271522,6271522,12543044,34961.08521223068,0.0004733148161903955
785786,6279526,6279526,12559052,34992.64360499382,0.00047244069719454274
786787,6287534,6287534,12575068,35022.43455004692,0.00047243474909919314
787788,6295540,6295540,12591080,35052.335506916046,0.0004724247737613041
788789,6303542,6303542,12607084,35082.378151893616,0.0004723448619188275
789790,6311550,6311550,12623100,35114.129553079605,0.00047233891564246733
790791,6319554,6319554,12639108,35146.760196208954,0.0004722750327346148
791792,6327558,6327558,12655116,35179.38994216919,0.00047174390238069464
792793,6335564,6335564,12671128,35211.77236914635,0.00047171995356620755
793794,6343572,6343572,12687144,35243.83094501495,0.00047171400910883676
794795,6351578,6351578,12703156,35273.66798520088,0.0004716630937764421
795796,6359584,6359584,12719168,35303.4870390892,0.0004716340627055615
796797,6367592,6367592,12735184,35333.19844913483,0.00047162812006718013
797798,6375596,6375596,12751192,35363.188175201416,0.00047129185804806184
798799,6383604,6383604,12767208,35395.39837408066,0.00047128591722866986
799800,6391608,6391608,12783216,36337.24374914169,0.0004709599725174485
800801,6399612,6399612,12799224,36385.55161809921,0.00047090317275433335
801802,6407618,6407618,12815236,36433.87005996704,0.00047078953139134683
802803,6415626,6415626,12831252,36482.2177400589,0.00047078359239094425
803804,6423632,6423632,12847264,36530.5534620285,0.0004707266180048464
804805,6431636,6431636,12863272,36573.57706284523,0.0004703165432147216
805806,6439642,6439642,12879284,36613.74948811531,0.00047030903078848496
806807,6447650,6447650,12895300,36653.38501000404,0.0004703030917880824
807808,6455654,6455654,12911308,36692.977993011475,0.0004698860793723725
808809,6463662,6463662,12927324,36732.50613617897,0.0004698801458289381
809810,6471668,6471668,12943336,36774.69319701195,0.00046983763058960903
810811,6479676,6479676,12959352,36823.01365303993,0.00046983169704617467
811812,6487682,6487682,12975364,36872.10605597496,0.0004697885269706603
812813,6495688,6495688,12991376,36911.74848198891,0.00046963768545538187
813814,6503692,6503692,13007384,36951.19838690758,0.00046960089275671635
814815,6511698,6511698,13023396,36990.966296195984,0.00046929976997489575
815816,6519702,6519702,13039404,37030.37082219124,0.00046929093514336273
816817,6527706,6527706,13055412,37074.81984901428,0.00046860758811817504
817818,6535708,6535708,13071416,37123.73140621185,0.0004685616495407885
818819,6543712,6543712,13087424,37170.25539302826,0.0004683084898715606
819820,6551720,6551720,13103440,37210.0817630291,0.00046830256542307325
820821,6559726,6559726,13119452,37249.71259903908,0.0004682098478951957
821822,6567732,6567732,13135464,37289.512909173965,0.00046817872316751163
822823,6575740,6575740,13151480,37328.96297597885,0.0004681727987190243
823824,6583744,6583744,13167488,37372.588475227356,0.0004677721080952324
824825,6591750,6591750,13183500,37420.902664899826,0.000467756217403803
825826,6599758,6599758,13199516,37467.78899717331,0.0004677502947743051
826827,6607762,6607762,13215524,37507.26983189583,0.00046771320194238797
827828,6615766,6615766,13231532,37546.963905096054,0.00046739810386497993
828829,6623774,6623774,13247548,37586.57736802101,0.000467392181235482
829830,6631782,6631782,13263564,37626.69105005264,0.00046738626224396285
830831,6639788,6639788,13279576,37670.54360294342,0.0004668547244364163
831832,6647790,6647790,13295580,37718.924666166306,0.000466841764136916
832833,6655798,6655798,13311596,37765.75266313553,0.0004668358451453969
833834,6663800,6663800,13327600,37805.28789305687,0.0004661294660763815
834835,6671808,6671808,13343616,37844.944184064865,0.0004661235525418306
835836,6679814,6679814,13359628,37884.61462020874,0.0004661142920667771
836837,6687818,6687818,13375636,37924.281635046005,0.0004660368213080801
837838,6695826,6695826,13391652,37969.28200125694,0.0004660309077735292
838839,6703832,6703832,13407664,38017.747608184814,0.00046569005280616693
839840,6711840,6711840,13423680,38063.87196588516,0.000465684139271616
840841,6719846,6719846,13439692,38103.38572502136,0.0004656423843698576
841842,6727854,6727854,13455708,38142.914021253586,0.0004656364744732855
842843,6735858,6735858,13471716,38182.99486017227,0.00046499368727381807
843844,6743864,6743864,13487728,38222.675729990005,0.00046494998241541907
844845,6751868,6751868,13503736,38270.165424108505,0.00046484943231916986
845846,6759876,6759876,13519752,38318.64678311348,0.00046484352606057655
846847,6767884,6767884,13535768,38362.882246255875,0.00046483761798299383
847848,6775888,6775888,13551776,38402.36021518707,0.0004646759643947007
848849,6783894,6783894,13567788,38442.0363881588,0.0004646504676202312
849850,6791900,6791900,13583800,38481.7661011219,0.0004646014676836785
850851,6799904,6799904,13599808,38521.38666296005,0.0004638901991711464
851852,6807912,6807912,13615824,38569.967900276184,0.00046388429655053187
852853,6815918,6815918,13631836,38618.37799119949,0.00046354498226719443
853854,6823926,6823926,13647852,38661.56035900116,0.0004635390814655693
854855,6831932,6831932,13663864,38701.16893410683,0.0004635135082935449
855856,6839940,6839940,13679880,38740.95467209816,0.00046350760567293037
856857,6847946,6847946,13695892,38780.49541401863,0.0004632935597328469
857858,6855952,6855952,13711904,38821.10061907768,0.0004632747641153401
858859,6863958,6863958,13727916,38869.41204094887,0.0004632297441276023
859860,6871960,6871960,13743920,38917.90443611145,0.0004619726132659707
860861,6879966,6879966,13759932,38960.276305913925,0.00046195883260224946
861862,6887972,6887972,13775944,38999.613234996796,0.00046192014451662544
862863,6895980,6895980,13791960,39039.210487127304,0.00046191425280994736
863864,6903986,6903986,13807972,39078.93575191498,0.0004617027152562514
864865,6911990,6911990,13823980,39120.89724493027,0.00046168705557647627
865866,6919996,6919996,13839992,39169.371166944504,0.00046164057130226865
866867,6928002,6928002,13856004,39217.75461292267,0.0004616121314029442
867868,6936010,6936010,13872020,39258.92408800125,0.00046160624151525553
868869,6944016,6944016,13888032,39298.40399622917,0.0004614663357642712
869870,6952024,6952024,13904048,39338.00872921944,0.0004614604458765825
870871,6960030,6960030,13920060,39377.59418606758,0.00046140736230881885
871872,6968036,6968036,13936072,39419.82843327522,0.0004609444586094469
872873,6976044,6976044,13952088,39468.28677916527,0.000460938572359737
873874,6984052,6984052,13968104,39516.48235321045,0.00046093268611002713
874875,6992058,6992058,13984116,39557.06812500954,0.0004608896797435591
875876,7000062,7000062,14000124,39596.56774020195,0.00046082148219284136
876877,7008068,7008068,14016136,39636.04406619072,0.0004608111503330292
877878,7016076,7016076,14032152,39675.644517183304,0.00046080526590230875
878879,7024078,7024078,14048156,39718.4975001812,0.0004603683210007148
879880,7032086,7032086,14064172,39766.85031700134,0.0004603624383889837
880881,7040092,7040092,14080184,39815.12604999542,0.000460332306829514
881882,7048100,7048100,14096200,39855.802861213684,0.0004603264242177829
882883,7056106,7056106,14112212,39895.26611304283,0.0004601882246788591
883884,7064110,7064110,14128220,39934.93170619011,0.0004598875566443894
884885,7072118,7072118,14144236,39974.374791145325,0.00045988167403265834
885886,7080126,7080126,14160252,40019.02478790283,0.0004598757950589061
886887,7088130,7088130,14176260,40067.45554304123,0.00045964288256072905
887888,7096138,7096138,14192276,40115.22585296631,0.000459636999948998
888889,7104144,7104144,14208288,40154.8656129837,0.00045962293916090857
889890,7112150,7112150,14224300,40194.27179002762,0.0004595528334903065
890891,7120158,7120158,14240316,40233.821918964386,0.00045954695451655425
891892,7128166,7128166,14256332,40273.97229528427,0.000459541075542802
892893,7136172,7136172,14272344,40322.37455415726,0.00045949985906190705
893894,7144180,7144180,14288360,40370.95243501663,0.0004594939819071442
894895,7152188,7152188,14304376,40415.059591293335,0.00045948810475238133
895896,7160190,7160190,14320380,40454.80555224419,0.0004591798842739081
896897,7168198,7168198,14336396,40494.34504389763,0.00045917400711914524
897898,7176202,7176202,14352404,40534.1350672245,0.00045883221355325077
898899,7184204,7184204,14368408,40579.71904420853,0.00045849767957406584
899900,7192212,7192212,14384424,40627.980384111404,0.000458491802419303
900901,7200216,7200216,14400432,40675.388337135315,0.00045845372005715035
901902,7208222,7208222,14416444,40715.0090470314,0.00045841156315873377
902903,7216230,7216230,14432460,40754.600716114044,0.0004584056878229603
903904,7224236,7224236,14448472,40794.468662023544,0.00045809027324139606
904905,7232240,7232240,14464480,40834.33956003189,0.0004580686036206316
905906,7240242,7240242,14480484,40882.62641787529,0.00045609796688950155
906907,7248244,7248244,14496488,40930.9399061203,0.0004560612051136559
907908,7256250,7256250,14512500,40975.41834115982,0.000455464027254493
908909,7264258,7264258,14528516,41014.77144026756,0.00045545816828962415
909910,7272266,7272266,14544532,41054.24870014191,0.00045545231114374474
910911,7280274,7280274,14560548,41093.64589905739,0.0004554464521788759
911912,7288280,7288280,14576560,41134.8017270565,0.00045531292926170863
912913,7296286,7296286,14592572,41183.27155303955,0.0004552902282739524
913914,7304292,7304292,14608584,41231.74224901199,0.00045524379311245866
914915,7312300,7312300,14624600,41274.37511920929,0.00045523793778556865
915916,7320302,7320302,14640604,41313.750338077545,0.00045452674021362327
916917,7328308,7328308,14656616,41353.36093211174,0.00045451333789969794
917918,7336314,7336314,14672628,41392.82120394707,0.0004544685798464343
918919,7344320,7344320,14688640,41436.0244140625,0.0004544409894151613
919920,7352328,7352328,14704656,41484.639545202255,0.0004544351377262501
920921,7360330,7360330,14720660,42934.942090034485,0.00045409766062221024
921922,7368336,7368336,14736672,42974.26832795143,0.00045369234248937573
922923,7376342,7376342,14752684,43022.640416145325,0.00045368374412646517
923924,7384350,7384350,14768700,43071.0513279438,0.00045367789425654337
924925,7392356,7392356,14784712,43119.4507830143,0.0004531659997155657
925926,7400362,7400362,14800724,43167.73885798454,0.00045314658200368285
926927,7408368,7408368,14816736,43208.39494013786,0.0004527355940808775
927928,7416374,7416374,14832748,43248.05476307869,0.0004527189685177291
928929,7424380,7424380,14848760,43287.58693408966,0.0004526313605310861
929930,7432386,7432386,14864772,43327.11792206764,0.0004526073917077156
930931,7440392,7440392,14880784,43366.68169403076,0.00045254325232235715
931932,7448400,7448400,14896800,43406.90069723129,0.00045253740790940356
932933,7456406,7456406,14912812,43455.30004811287,0.000452276415671804
933934,7464410,7464410,14928820,43503.989349126816,0.00045225372741697356
934935,7472416,7472416,14944832,43544.86364507675,0.0004520683032751549
935936,7480422,7480422,14960844,43584.384154081345,0.00045206196773506235
936937,7488428,7488428,14976856,43624.11368393898,0.0004520454658631934
937938,7496436,7496436,14992872,43663.62138915062,0.0004520396250882186
938939,7504442,7504442,15008884,43709.17789912224,0.0004516753633652115
939940,7512450,7512450,15024900,43757.484850883484,0.00045166952440922614
940941,7520456,7520456,15040912,43802.36233115196,0.00045165317533246707
941942,7528460,7528460,15056920,43842.05725693703,0.0004514023512456333
942943,7536466,7536466,15072932,43881.64790511131,0.000451385460110032
943944,7544474,7544474,15088948,43921.16597414017,0.0004513796247920254
944945,7552480,7552480,15104960,43960.502808094025,0.0004513426283665467
945946,7560484,7560484,15120968,44004.88704299927,0.0004506638324528467
946947,7568490,7568490,15136980,44053.31239295006,0.00045060885895509273
947948,7576496,7576496,15152992,44099.642952919006,0.0004505939650698565
948949,7584502,7584502,15169004,44139.38607907295,0.0004504659118538257
949950,7592510,7592510,15185020,44178.97829914093,0.0004504600783548085
950951,7600514,7600514,15201028,44218.53163123131,0.0004503800446400419
951952,7608522,7608522,15217044,44258.057749032974,0.0004503742129600141
952953,7616524,7616524,15233048,44305.11050701141,0.0004499941278481856
953954,7624528,7624528,15249056,44353.3977971077,0.00044946618072572164
954955,7632532,7632532,15265064,44397.61898112297,0.0004494289805734297
955956,7640536,7640536,15281072,44437.19870519638,0.00044814360444433987
956957,7648538,7648538,15297076,44476.842803001404,0.00044809312021243386
957958,7656546,7656546,15313092,44516.31602811813,0.0004480873012653319
958959,7664552,7664552,15329104,44555.99882221222,0.000447990290922462
959960,7672558,7672558,15345116,44602.55081009865,0.0004479553590499563
960961,7680566,7680566,15361132,44651.010788202286,0.00044794954010285437
961962,7688570,7688570,15377140,44696.34128808975,0.0004476327812881209
962963,7696576,7696576,15393152,44736.59025621414,0.0004476048379729036
963964,7704578,7704578,15409156,44775.99540805817,0.0004468033857847331
964965,7712584,7712584,15425168,44815.5469250679,0.0004467752769414801
965966,7720588,7720588,15441176,44857.48396420479,0.00044629945114138536
966967,7728592,7728592,15457184,44905.65909194946,0.0004462654651433695
967968,7736600,7736600,15473200,44954.1609249115,0.0004462596534722252
968969,7744606,7744606,15489212,44995.49449300766,0.0004462425695237471
969970,7752614,7752614,15505228,45035.01245903969,0.00044623675785260275
970971,7760620,7760620,15521240,45074.56973528862,0.0004462031174625736
971972,7768624,7768624,15537248,45114.179303884506,0.00044564121708390303
972973,7776632,7776632,15553264,45158.33217716217,0.0004456354108697269
973974,7784634,7784634,15569268,45206.72168803215,0.00044560562855622265
974975,7792640,7792640,15585280,45255.26041817665,0.0004454491390788462
975976,7800648,7800648,15601296,45295.24021100998,0.0004454433346836595
976977,7808654,7808654,15617308,45334.96514201164,0.00044540714588947594
977978,7816660,7816660,15633320,45374.48662495613,0.000445006946392823
978979,7824668,7824668,15649336,45414.03167104721,0.0004450011401786469
979980,7832676,7832676,15665352,45460.17820811272,0.0004449953376024496
980981,7840682,7840682,15681364,45508.8426630497,0.00044494704707176425
981982,7848690,7848690,15697380,45556.08993721008,0.00044494124267657753
982983,7856692,7856692,15713384,45595.68620419502,0.0004446292168722721
983984,7864700,7864700,15729400,45635.46771931648,0.00044462341429607477
984985,7872704,7872704,15745408,45674.88216614723,0.00044437059477786534
985986,7880712,7880712,15761424,45714.36330699921,0.00044436479583964683
986987,7888718,7888718,15777436,45762.33430600166,0.00044432829054130707
987988,7896726,7896726,15793452,45810.85006594658,0.00044432249160308857
988989,7904732,7904732,15809464,45855.591551065445,0.0004443028610694455
989990,7912736,7912736,15825472,45895.28424715996,0.0004442529534571804
990991,7920742,7920742,15841484,45934.95069217682,0.0004436001818248769
991992,7928750,7928750,15857500,45974.63481593132,0.0004435943847056478
992993,7936756,7936756,15873512,46016.14853310585,0.00044358460581861436
993994,7944760,7944760,15889520,46064.543909072876,0.00044323750444164034
994995,7952768,7952768,15905536,46112.77650523186,0.00044323170914140064
995996,7960774,7960774,15921548,46155.12911105156,0.00044319241715129465
996997,7968782,7968782,15937564,46194.678168058395,0.00044318662185105495
997998,7976788,7976788,15953576,46234.39041519165,0.00044311551937425975
998999,7984796,7984796,15969592,46273.96345615387,0.00044310972225503065
1000000,7992802,7992802,15985604,46319.63829302788,0.0004430947101354832


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namea9a/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.03208613395690918,12064.682476916567
36,146,146,292,1.104646921157837,52.30500082631261
71,248,248,496,1.7445580959320068,27.141848262002895
107,358,358,716,2.4315409660339355,11.933394474070155
142,466,466,932,3.2864770889282227,5.197580163256134
178,578,578,1156,4.076996088027954,3.1365870973932033
213,694,694,1388,4.858889102935791,2.479279129920542
249,822,822,1644,5.696300029754639,1.9649261214290163
284,950,950,1900,6.5995259284973145,1.594074333557728
320,1082,1082,2164,7.5958662033081055,1.3089532206158765
355,1214,1214,2428,8.631164073944092,1.0862390728598257
391,1358,1358,2716,9.67017912864685,0.9758987308323412
426,1482,1482,2964,10.545928001403809,0.7592629871105601
462,1610,1610,3220,11.465901136398315,0.5564759814660647
497,1740,1740,3480,12.333163976669312,0.45034559544728836
533,1860,1860,3720,13.108394145965576,0.3600335182836716
568,1998,1998,3996,13.907964944839478,0.33296849535690853
604,2128,2128,4256,14.744874000549316,0.29890755062479
640,2262,2262,4524,15.617071151733398,0.2696009202318237
675,2398,2398,4796,16.509824991226196,0.25181713265556027
711,2546,2546,5092,17.45164918899536,0.2370260315692576
746,2696,2696,5392,18.447766065597534,0.21919866958705825
782,2842,2842,5684,19.3876211643219,0.20245800934753788
817,3000,3000,6000,20.478121042251587,0.1781729139165691
853,3148,3148,6296,21.358756065368652,0.16321093675651355
888,3280,3280,6560,22.214028120040894,0.1559341810625483
924,3420,3420,6840,23.102277994155884,0.13586458643294463
959,3570,3570,7140,24.13960599899292,0.13091624469780072
995,3730,3730,7460,25.187839031219482,0.12349765578619554
1030,3884,3884,7768,26.132794857025146,0.11849342138339125
1066,4048,4048,8096,27.16092300415039,0.10630610299085674
1101,4208,4208,8416,28.1181161403656,0.09892259914158785
1137,4358,4358,8716,29.156046152114868,0.09272213218901015
1172,4500,4500,9000,30.16516900062561,0.08255026140250266
1208,4636,4636,9272,31.005311012268066,0.07082356795945088
1243,4768,4768,9536,31.811548948287964,0.06478122332555358
1279,4904,4904,9808,32.59728002548218,0.05939617703006661
1315,5048,5048,10096,33.41242504119873,0.05768445014109602
1350,5188,5188,10376,34.17873692512512,0.05684824076524819
1386,5332,5332,10664,34.998881101608276,0.05624914616055321
1421,5476,5476,10952,35.82648801803589,0.05355406722628686
1457,5622,5622,11244,36.617778062820435,0.052311414408904966
1492,5766,5766,11532,37.40172219276428,0.051610537126180134
1528,5914,5914,11828,38.248316049575806,0.04937863067971193
1563,6066,6066,12132,39.09885501861572,0.0477488277683733
1599,6214,6214,12428,39.93120789527893,0.04581970052822726
1634,6362,6362,12724,40.74213886260986,0.04461492495283892
1670,6526,6526,13052,41.63882398605347,0.04234772918061935
1705,6670,6670,13340,42.44318413734436,0.04154595709769637
1741,6818,6818,13636,43.30479598045349,0.039951398543053074
1776,6976,6976,13952,44.32193422317505,0.0359954647901759
1812,7138,7138,14276,45.511444091796875,0.03286750309962372
1847,7298,7298,14596,46.57936906814575,0.030447379613178782
1883,7448,7448,14896,47.660573959350586,0.029233557401312282
1919,7600,7600,15200,48.62986612319946,0.028034453900545486
1954,7740,7740,15480,49.65371918678284,0.02645723446221382
1990,7888,7888,15776,50.73527503013611,0.025766663024114678
2025,8028,8028,16056,51.90542793273926,0.024019976142881205
2061,8176,8176,16352,52.893226146698,0.023371382972982246
2096,8320,8320,16640,53.8654248714447,0.021384484238296864
2132,8472,8472,16944,54.86685013771057,0.018939170169687713
2167,8616,8616,17232,55.813512086868286,0.01702903140176204
2203,8754,8754,17508,56.6920599937439,0.015818984978977824
2238,8886,8886,17772,57.546345949172974,0.014432462732656859
2274,9018,9018,18036,58.40186405181885,0.012594293077199836
2309,9136,9136,18272,59.17098307609558,0.010613960239425069
2345,9278,9278,18556,60.07165813446045,0.010183783877437236
2380,9416,9416,18832,60.969993114471436,0.010048247655504383
2416,9568,9568,19136,62.066365003585815,0.009763846617715899
2451,9708,9708,19416,62.98412227630615,0.009689518954473897
2487,9852,9852,19704,63.876370906829834,0.009570026200890425
2523,9996,9996,19992,64.79013204574585,0.009380069606777397
2558,10142,10142,20284,65.73026609420776,0.009068069241038756
2594,10286,10286,20572,66.69977807998657,0.008748620521146222
2629,10434,10434,20868,67.61970686912537,0.008185995955500402
2665,10578,10578,21156,68.62773704528809,0.00782466590317199
2700,10718,10718,21436,69.53133916854858,0.007446860960044432
2736,10868,10868,21736,70.46383500099182,0.007046232585707912
2771,11008,11008,22016,71.34814429283142,0.00693053121540288
2807,11152,11152,22304,72.22943496704102,0.0067140253268007655
2842,11292,11292,22584,73.1023371219635,0.006437039834054303
2878,11440,11440,22880,74.01475501060486,0.0062620754943054635
2913,11586,11586,23172,74.91496515274048,0.0058995115159632405
2949,11730,11730,23460,75.81179189682007,0.005695157999070943
2984,11898,11898,23796,76.80902004241943,0.0053690798977186205
3020,12054,12054,24108,77.76813316345215,0.005062888469183235
3055,12194,12194,24388,78.62640309333801,0.004969327535945922
3091,12344,12344,24688,79.55316090583801,0.004836234316826449
3127,12488,12488,24976,80.43757915496826,0.004683102752096602
3162,12650,12650,25300,81.42260408401489,0.00473930924636079
3198,12804,12804,25608,82.38449692726135,0.004562167545373086
3233,12960,12960,25920,83.34723114967346,0.004274073586202576
3269,13116,13116,26232,84.31581807136536,0.004068812771947705
3304,13274,13274,26548,85.27389311790466,0.003883218527334975
3340,13438,13438,26876,86.26750898361206,0.0038821205071144504
3375,13578,13578,27156,87.12845492362976,0.0038947400698816637
3411,13724,13724,27448,88.03743410110474,0.003816092304987251
3446,13906,13906,27812,89.12543892860413,0.0037578973860945553
3482,14050,14050,28100,90.00696802139282,0.0037565188613370992
3517,14190,14190,28380,90.88628005981445,0.0037543962007475784
3553,14338,14338,28676,91.7997829914093,0.0037514242121687857
3588,14478,14478,28956,92.66328716278076,0.0037494813332159538
3624,14622,14622,29244,93.54816794395447,0.003745963149413001
3659,14762,14762,29524,94.42831492424011,0.003743111263247556
3695,14906,14906,29812,95.33014106750488,0.0037407408435683465
3730,15046,15046,30092,96.17762899398804,0.0037378223987616366
3766,15190,15190,30380,97.08587217330933,0.0037363583651313093
3802,15334,15334,30668,97.98681497573853,0.0037332647352741333
3837,15474,15474,30948,98.86529302597046,0.0037288173698470928
3873,15618,15618,31236,99.76038718223572,0.003713581434567459
3908,15758,15758,31516,100.62114691734314,0.003703098724145093
3944,15902,15902,31804,101.52966618537903,0.003681254169350723
3979,16054,16054,32108,102.46317601203918,0.003656962589957402
4015,16318,16318,32636,103.9655659198761,0.003656882081486401
4050,16544,16544,33088,105.26955699920654,0.0036566635717463214
4086,16688,16688,33376,106.15908622741699,0.0036551536122715333
4121,16832,16832,33664,107.0423948764801,0.0036533609636535402
4157,16976,16976,33952,107.94294500350952,0.0036508849552774336
4192,17116,17116,34232,108.81288814544678,0.0036476998757279944
4228,17262,17262,34524,109.71074509620667,0.003645095661340747
4263,17402,17402,34804,110.59325218200684,0.0036397482072061393
4299,17546,17546,35092,111.4796371459961,0.00362737919385836
4334,17686,17686,35372,112.36199498176575,0.0036172536802041577
4370,17872,17872,35744,113.44809913635254,0.0035850278072757646
4406,18132,18132,36264,114.92898607254028,0.003584899804991437
4441,18272,18272,36544,115.79930806159973,0.0035840696746163303
4477,18416,18416,36832,116.69552707672119,0.003582414514312404
4512,18556,18556,37112,117.58247923851013,0.003581278200726956
4548,18712,18712,37424,118.5514121055603,0.003579207803340978
4583,18852,18852,37704,119.44892406463623,0.003570682845747797
4619,18996,18996,37992,120.32674098014832,0.00356289674891741
4654,19136,19136,38272,121.22235703468323,0.0035573807053879136
4690,19280,19280,38560,122.12768602371216,0.003545022293110378
4725,19420,19420,38840,123.02446103096008,0.0035297159611218376
4761,19564,19564,39128,123.92833995819092,0.0035118006217089714
4796,19712,19712,39424,124.85492420196533,0.0034756314562400803
4832,19856,19856,39712,125.7763991355896,0.0034357377317064675
4867,19996,19996,39992,126.67367100715637,0.0033659067048574798
4903,20140,20140,40280,127.59209084510803,0.0033095090020651696
4938,20280,20280,40560,128.53000903129578,0.00319638389373722
4974,20470,20470,40940,129.71346616744995,0.0030951334920246154
5010,20710,20710,41420,131.22660398483276,0.0030948050916776992
5045,20854,20854,41708,132.18880891799927,0.0030931337514630286
5081,20998,20998,41996,133.12825202941895,0.003092151633609319
5116,21138,21138,42276,134.05877208709717,0.003090305155637907
5152,21282,21282,42564,135.07595920562744,0.0030883272593200672
5187,21422,21422,42844,135.9528350830078,0.0030852728596073575
5223,21566,21566,43132,136.852117061615,0.003082822047872469
5258,21706,21706,43412,137.71050906181335,0.003078379540966125
5294,21850,21850,43700,138.61057305335999,0.003072112704103347
5329,21990,21990,43980,139.47025513648987,0.003066566250709002
5365,22134,22134,44268,140.37233805656433,0.003063400699829799
5400,22274,22274,44548,141.23498010635376,0.0030616551339335274
5436,22418,22418,44836,142.14519095420837,0.003058913742279401
5471,22558,22558,45116,143.03204894065857,0.0030563251330022467
5507,22702,22702,45404,143.9253330230713,0.0030514060526911635
5542,22842,22842,45684,144.79886603355408,0.0030458132969215512
5578,22986,22986,45972,145.6841950416565,0.003039917199203046
5614,23130,23130,46260,146.65081906318665,0.003030993642823887
5649,23270,23270,46540,147.54149103164673,0.003018508243258111
5685,23414,23414,46828,148.47120904922485,0.002988317455674405
5720,23562,23562,47124,149.40033602714539,0.002954209969175281
5756,23706,23706,47412,150.34441089630127,0.0029217158335086424
5791,23860,23860,47720,151.28673911094666,0.0028629561802517856
5827,24104,24104,48208,152.70320010185242,0.0028557965761137893
5862,24340,24340,48680,154.0757350921631,0.0028554710315802367
5898,24560,24560,49120,155.34880995750427,0.002854980975826038
5933,24700,24700,49400,156.22162699699402,0.002852415153029142
5969,24844,24844,49688,157.11573004722595,0.0028493060563050676
6004,24984,24984,49968,157.9887261390686,0.0028459463483159197
6040,25128,25128,50256,158.8951771259308,0.0028437577620934462
6075,25268,25268,50536,159.7431812286377,0.0028428046134649776
6111,25412,25412,50824,160.65216898918152,0.0028398008635122096
6146,25552,25552,51104,161.50905084609985,0.0028370811087370384
6182,25696,25696,51392,162.41626906394958,0.002834510669345036
6217,25836,25836,51672,163.27114129066467,0.002830455829098355
6253,25980,25980,51960,164.15022897720337,0.0028284136787988245
6289,26126,26126,52252,165.04987716674805,0.002821279918862274
6324,26266,26266,52532,165.92557311058044,0.002817903916366049
6360,26410,26410,52820,166.8236858844757,0.0028127750738349278
6395,26550,26550,53100,167.6943109035492,0.002805656227792497
6431,26698,26698,53396,168.60294818878174,0.0027996928765787743
6466,26838,26838,53676,169.48104596138,0.002787332679872634
6502,26982,26982,53964,170.37532114982605,0.0027754692600865383
6537,27122,27122,54244,171.26277613639832,0.002772653764623101
6573,27266,27266,54532,172.1568021774292,0.002750843319518026
6608,27406,27406,54812,173.0144820213318,0.002691053387025022
6644,27552,27552,55104,173.93100214004517,0.0025960621551348595
6679,27730,27730,55460,174.9847710132599,0.0025365621950186323
6715,27954,27954,55908,176.29271912574768,0.002532480610170751
6750,28212,28212,56424,177.75188207626343,0.002532415219320683
6786,28492,28492,56984,179.32645416259766,0.0025324154557893053
6821,28640,28640,57280,180.24219918251038,0.002531931311750668
6857,28784,28784,57568,181.1188521385193,0.0025303665079263737
6893,28928,28928,57856,182.00891017913818,0.002529323848648346
6928,29068,29068,58136,182.89486384391785,0.0025286474792665103
6964,29212,29212,58424,183.78021717071533,0.0025278985303884838
6999,29352,29352,58704,184.67504596710205,0.0025265511030738708
7035,29496,29496,58992,185.58211612701416,0.002524901912693167
7070,29636,29636,59272,186.48955392837524,0.002522097245673649
7106,29780,29780,59560,187.40388417243958,0.002519368734283489
7141,29920,29920,59840,188.2943480014801,0.0025151253958028974
7177,30064,30064,60128,189.21166896820068,0.002513175311833038
7212,30206,30206,60412,190.097186088562,0.002510475269446033
7248,30356,30356,60712,191.04460906982422,0.0025065897880267585
7283,30496,30496,60992,191.92031598091125,0.0025011808465933427
7319,30642,30642,61284,192.8343071937561,0.002496802608220605
7354,30782,30782,61564,193.72205591201782,0.0024816540390020236
7390,30932,30932,61864,194.66074109077454,0.0024687676268513314
7425,31152,31152,62304,196.22542905807495,0.0024633146585983923
7461,31296,31296,62592,197.12376403808594,0.002464988090650877
7497,31444,31444,62888,198.05002117156982,0.002463416003593011
7532,31682,31682,63364,199.42306518554688,0.0024631916367070517
7568,31964,31964,63928,200.99514293670654,0.002463185905071441
7603,32244,32244,64488,202.5653510093689,0.002463184395310236
7639,32412,32412,64824,203.57759594917297,0.0024628251248941524
7674,32556,32556,65112,204.4762260913849,0.00246228561445605
7710,32704,32704,65408,205.4077160358429,0.002460658508425695
7745,32844,32844,65688,206.27986693382263,0.0024568783101130975
7781,32988,32988,65976,207.14893007278442,0.002452804577842471
7816,33128,33128,66256,208.01439905166626,0.0024519094531569863
7852,33272,33272,66544,208.9209921360016,0.002449375466312631
7887,33412,33412,66824,209.79807996749878,0.0024446945335512282
7923,33556,33556,67112,210.69050407409668,0.002439139609123231
7958,33696,33696,67392,211.56187295913696,0.002432211877021473
7994,33844,33844,67688,212.4968409538269,0.002430910331895575
8029,33984,33984,67968,213.38281917572021,0.002425083823254681
8065,34128,34128,68256,214.2828779220581,0.002419044778434909
8101,34272,34272,68544,215.18962407112122,0.002405657658528071
8136,34412,34412,68824,216.04854822158813,0.002395466170128202
8172,34558,34558,69116,216.97581911087036,0.00237367108638864
8207,34702,34702,69404,217.86104702949524,0.002331731629965361
8243,34854,34854,69708,218.79799604415894,0.002287804083607625
8278,34994,34994,69988,219.6745090484619,0.0022566417246707715
8314,35138,35138,70276,220.56731915473938,0.002237276148662204
8349,35280,35280,70560,221.46218609809875,0.0022076580517023103
8385,35428,35428,70856,222.37927198410034,0.0021749030602222774
8420,35574,35574,71148,223.29532384872437,0.002140520055036177
8456,35718,35718,71436,224.1865029335022,0.002043104204858537
8491,35890,35890,71780,225.2233669757843,0.0019191782903362764
8527,36102,36102,72204,226.48554110527039,0.001920222819535411
8562,36242,36242,72484,227.36492609977722,0.0019198070713173365
8598,36386,36386,72772,228.2613880634308,0.0019191296287317527
8633,36606,36606,73212,229.53957104682922,0.001918803944136016
8669,36894,36894,73788,231.16737699508667,0.0019188027326890733
8704,37120,37120,74240,232.47927713394165,0.0019185881774319569
8740,37264,37264,74528,233.36627793312073,0.0019181656007276615
8776,37408,37408,74816,234.26480412483215,0.001916736035127542
8811,37548,37548,75096,235.13935899734497,0.0019137909966957523
8847,37692,37692,75384,236.04197812080383,0.0019117132032988593
8882,37832,37832,75664,236.93503999710083,0.0019107345833617728
8918,37976,37976,75952,237.84375,0.0019097655276709702
8953,38120,38120,76240,238.72317504882812,0.0019084439245489193
8989,38264,38264,76528,239.6087350845337,0.0019066924342041602
9024,38404,38404,76808,240.48671221733093,0.0019055826796829933
9060,38552,38552,77104,241.40228414535522,0.0019046861034439644
9095,38692,38692,77384,242.27103996276855,0.0019039550807065098
9131,38846,38846,77692,243.22152495384216,0.001902968459035037
9166,38998,38998,77996,244.13879108428955,0.0019016964270122116
9202,39150,39150,78300,245.071946144104,0.001900381392260897
9237,39292,39292,78584,245.95686197280884,0.0018997961778950412
9273,39438,39438,78876,246.86858296394348,0.001898207250633277
9308,39578,39578,79156,247.73864912986755,0.0018965753006341401
9344,39722,39722,79444,248.63410687446594,0.001895553441499942
9380,39866,39866,79732,249.53940725326538,0.0018949460063595325
9415,40008,40008,80016,250.4219400882721,0.001887383068606141
9451,40152,40152,80304,251.30361008644104,0.001870563692136784
9486,40292,40292,80584,252.18470811843872,0.0018289638555870624
9522,40500,40500,81000,253.40388107299805,0.0017994799145526486
9557,40674,40674,81348,254.45532298088074,0.00179931971069891
9593,40920,40920,81840,255.85915398597717,0.0017992175708059222
9628,41064,41064,82128,256.74915409088135,0.0017986045331781497
9664,41212,41212,82424,257.65878200531006,0.0017982256922550732
9699,41352,41352,82704,258.5400199890137,0.0017974116799450712
9735,41500,41500,83000,259.46763920783997,0.0017965493152587442
9770,41640,41640,83280,260.3337609767914,0.0017958725638891337
9806,41784,41784,83568,261.21817922592163,0.001795283351384569
9841,41926,41926,83852,262.08546209335327,0.001794228286598809
9877,42078,42078,84156,263.02927589416504,0.0017924155999935465
9912,42220,42220,84440,263.9046070575714,0.001790995887859026
9948,42368,42368,84736,264.82581210136414,0.0017891616698761936
9984,42520,42520,85040,265.75614309310913,0.0017864327601273544
10019,42660,42660,85320,266.6122188568115,0.0017843362693383824
10055,42804,42804,85608,267.50891399383545,0.001782202021786361
10090,42944,42944,85888,268.37538504600525,0.0017774260122678243
10126,43090,43090,86180,269.272586107254,0.0017700350617815275
10161,43230,43230,86460,270.1305179595947,0.0017627927172725322
10197,43374,43374,86748,271.0188219547272,0.0017466400440753205
10232,43518,43518,87036,271.91815996170044,0.0017260132262890693
10268,43662,43662,87324,272.8075451850891,0.0017031029383360874
10303,43802,43802,87604,273.68194007873535,0.0016817914711282356
10339,43946,43946,87892,274.5761079788208,0.0016652028371026972
10374,44088,44088,88176,275.44962787628174,0.0016424377499788534
10410,44234,44234,88468,276.3604679107666,0.0016134666020661825
10445,44386,44386,88772,277.28621220588684,0.0015634638621122576
10481,44580,44580,89160,278.46285605430603,0.0015490341993427137
10516,44776,44776,89552,279.6079740524292,0.0015478305886063026
10552,45030,45030,90060,281.0548732280731,0.0015477482447749935
10588,45318,45318,90636,282.67920112609863,0.0015477473243663553
10623,45508,45508,91016,283.800390958786,0.0015476373100682395
10659,45652,45652,91304,284.70370626449585,0.0015474062747671269
10694,45792,45792,91584,285.5681240558624,0.001546133893498336
10730,45936,45936,91872,286.4630711078644,0.0015455205411853967
10765,46076,46076,92152,287.34320521354675,0.0015442248641193146
10801,46220,46220,92440,288.2382140159607,0.0015429763370775618
10836,46360,46360,92720,289.10703587532043,0.0015414570243592607
10872,46504,46504,93008,290.00767493247986,0.0015403674115077592
10907,46646,46646,93292,290.9412660598755,0.0015395402115245815
10943,46790,46790,93580,291.83337807655334,0.0015385825481644133
10978,46934,46934,93868,292.74101400375366,0.0015381053126475308
11014,47078,47078,94156,293.6513931751251,0.0015372282796306536
11049,47226,47226,94452,294.5580701828003,0.0015368165677500656
11085,47382,47382,94764,295.5298020839691,0.001535370198325836
11120,47534,47534,95068,296.4730360507965,0.0015340912814281182
11156,47680,47680,95360,297.3829710483551,0.0015336710948758991
11191,47832,47832,95664,298.3255889415741,0.0015325987715186784
11227,47984,47984,95968,299.24793100357056,0.00153078436414944
11263,48138,48138,96276,300.20142793655396,0.0015281449032045202
11298,48282,48282,96564,301.08076000213623,0.0015260843847499928
11334,48430,48430,96860,302.00446796417236,0.0015209398825390963
11369,48570,48570,97140,302.8711349964142,0.0015182974257186288
11405,48714,48714,97428,303.7584488391876,0.0015141894728003535
11440,48858,48858,97716,304.654736995697,0.0015065234601934208
11476,49002,49002,98004,305.54757499694824,0.0014889695867168484
11511,49142,49142,98284,306.41997385025024,0.001465678429667605
11547,49290,49290,98580,307.32529616355896,0.0014444761054619448
11582,49492,49492,98984,308.53262209892273,0.0014107015940680867
11618,49644,49644,99288,309.46654319763184,0.0014104544443398481
11653,49834,49834,99668,310.5739049911499,0.0014102592176641338
11689,49986,49986,99972,311.5192201137543,0.0014101684046181617
11724,50126,50126,100252,312.39610290527344,0.0014100097760092467
11760,50280,50280,100560,313.352890253067,0.001409369682733086
11795,50420,50420,100840,314.2090561389923,0.0014086865085118916
11831,50568,50568,101136,315.19610500335693,0.0014081794579396956
11867,50712,50712,101424,316.0924742221832,0.0014076961924729403
11902,50852,50852,101704,316.9818539619446,0.0014071403493289836
11938,51006,51006,102012,317.94697308540344,0.0014062243753869552
11973,51154,51154,102308,318.89321184158325,0.0014055463689146563
12009,51302,51302,102604,319.8230631351471,0.00140475152147701
12044,51444,51444,102888,320.6924500465393,0.0014042100319784367
12080,51592,51592,103184,321.61286997795105,0.0014027993438503472
12115,51732,51732,103464,322.4907500743866,0.0014008048729010625
12151,51894,51894,103788,323.479727268219,0.001398521209921455
12186,52038,52038,104076,324.376394033432,0.0013945639511803165
12222,52186,52186,104372,325.27784299850464,0.001386781132168835
12257,52326,52326,104652,326.1429650783539,0.001379980723868357
12293,52472,52472,104944,327.0384130477905,0.0013668875544681214
12328,52612,52612,105224,327.90120816230774,0.001350243514025351
12364,52756,52756,105512,328.80106806755066,0.0013310548056324478
12399,52900,52900,105800,329.67712807655334,0.0013153708241588902
12435,53044,53044,106088,330.56179094314575,0.001306321786614717
12471,53188,53188,106376,331.4483380317688,0.0012938240906805731
12506,53330,53330,106660,332.33460521698,0.00127051024355751
12542,53474,53474,106948,333.22320008277893,0.0012283703381399391
12577,53630,53630,107260,334.1674199104309,0.001159994326371816
12613,53894,53894,107788,335.67359805107117,0.001158573404609342
12648,54128,54128,108256,337.02373719215393,0.0011578231788007542
12684,54372,54372,108744,338.4356219768524,0.001157780816356535
12719,54552,54552,109104,339.5036630630493,0.0011576911219890462
12755,54712,54712,109424,340.47427797317505,0.0011573053980100667
12790,54852,54852,109704,341.35230588912964,0.00115664251097769
12826,55000,55000,110000,342.2634310722351,0.0011563281859707786
12861,55146,55146,110292,343.157653093338,0.0011558006626728456
12897,55290,55290,110580,344.04935002326965,0.0011555685614439426
12932,55440,55440,110880,344.96781492233276,0.0011551230163604487
12968,55584,55584,111168,345.8697118759155,0.0011536069741850952
13003,55732,55732,111464,346.7555079460144,0.001152626538896584
13039,55880,55880,111760,347.66857290267944,0.0011509413689054782
13074,56020,56020,112040,348.5170040130615,0.0011498107724037254
13110,56174,56174,112348,349.45013403892517,0.001149823878222378
13146,56330,56330,112660,350.4064042568207,0.0011494933387439232
13181,56476,56476,112952,351.31025314331055,0.001149268993685837
13217,56620,56620,113240,352.210813999176,0.0011488898653624346
13252,56790,56790,113580,353.2245042324066,0.0011485161321616033
13288,56944,56944,113888,354.16133999824524,0.0011476854688226013
13323,57094,57094,114188,355.0723571777344,0.0011468758530099876
13359,57246,57246,114492,355.99517798423767,0.0011456203737907344
13394,57396,57396,114792,356.93265199661255,0.0011437150442361599
13430,57544,57544,115088,357.84765005111694,0.0011373132310836809
13465,57684,57684,115368,358.72493386268616,0.0011313970771880122
13501,57830,57830,115660,359.58426308631897,0.0011216721541131847
13536,57970,57970,115940,360.212877035141,0.0011119094015157316
13572,58120,58120,116240,361.22081995010376,0.0011043647991755279
13607,58264,58264,116528,362.21690607070923,0.00109003792204021
13643,58408,58408,116816,363.1649420261383,0.001075515921911574
13678,58548,58548,117096,364.06456089019775,0.0010630689012032235
13714,58692,58692,117384,364.99498295783997,0.0010317157393728849
13750,58848,58848,117696,366.02529525756836,0.0009753078757057665
13785,59000,59000,118000,366.9986078739166,0.0009217417646141257
13821,59178,59178,118356,368.11111307144165,0.000876567160958075
13856,59422,59422,118844,369.7033140659332,0.0008718551125639351
13892,59614,59614,119228,370.7241380214691,0.0008717142136447364
13927,59808,59808,119616,372.1806721687317,0.000871590160386404
13963,60090,60090,120180,373.9531149864197,0.0008715886633581249
13998,60294,60294,120588,375.28170704841614,0.0008712292201380478
14034,60508,60508,121016,376.63396406173706,0.0008711725495231804
14069,60752,60752,121504,378.12901306152344,0.0008711500540812267
14105,60904,60904,121808,379.14373207092285,0.0008710767870070413
14140,61048,61048,122096,380.10202717781067,0.000870794488946558
14176,61198,61198,122396,381.1296100616455,0.0008705038271727972
14211,61340,61340,122680,382.07332825660706,0.0008700071593921166
14247,61484,61484,122968,383.041286945343,0.0008696159620740218
14282,61624,61624,123248,383.978728055954,0.0008690341455803718
14318,61774,61774,123548,384.9817259311676,0.0008680535502207931
14354,61924,61924,123848,385.97040605545044,0.0008676141878822818
14389,62082,62082,124164,386.987272977829,0.0008670919305586722
14425,62234,62234,124468,387.98608207702637,0.0008667775528010679
14460,62378,62378,124756,388.9240720272064,0.0008664475881232647
14496,62522,62522,125044,389.89109206199646,0.00086580146853521
14531,62676,62676,125352,390.88768315315247,0.0008654939338157419
14567,62832,62832,125664,391.9288160800934,0.0008653524237161037
14602,62982,62982,125964,392.9455180168152,0.000865078571223421
14638,63128,63128,126256,393.93148708343506,0.0008647949198348215
14673,63280,63280,126560,394.89767718315125,0.0008643649653095054
14709,63444,63444,126888,395.9426500797272,0.0008639083716843743
14744,63608,63608,127216,396.97042298316956,0.0008626619091955945
14780,63758,63758,127516,397.93960404396057,0.0008619263317086734
14815,63912,63912,127824,398.94891715049744,0.0008601469544373685
14851,64060,64060,128120,399.9003930091858,0.0008577746266382746
14886,64204,64204,128408,400.8407139778137,0.0008548058285668958
14922,64362,64362,128724,401.871857881546,0.0008512019885529298
14958,64508,64508,129016,402.8333692550659,0.0008464883740089135
14993,64648,64648,129296,403.7692120075226,0.000840872709886753
15029,64792,64792,129584,404.703919172287,0.0008330266064149328
15064,64932,64932,129864,405.59987711906433,0.0008200189240596956
15100,65116,65116,130232,406.77286410331726,0.0007934779860079288
15135,65272,65272,130544,407.75723695755005,0.0007933604556455975
15171,65458,65458,130916,408.9121558666229,0.000793252849689452
15206,65736,65736,131472,410.597088098526,0.000793252038420178
15242,66022,66022,132044,412.3048379421234,0.0007932515836728271
15277,66274,66274,132548,413.81386494636536,0.000793174698628718
15313,66442,66442,132884,414.8944170475006,0.0007931519121484598
15348,66582,66582,133164,415.8341271877289,0.000793090372098959
15384,66730,66730,133460,416.8054881095886,0.0007930336614663247
15419,66876,66876,133752,417.76847410202026,0.0007929456132842461
15455,67044,67044,134088,418.8572700023651,0.0007928152463136939
15490,67192,67192,134384,419.84128522872925,0.0007925200843601488
15526,67358,67358,134716,420.89489698410034,0.000792381488281535
15561,67510,67510,135020,421.88320112228394,0.000792295115388697
15597,67668,67668,135336,422.91631412506104,0.000792222877862514
15633,67830,67830,135660,423.95100116729736,0.0007918994160718285
15668,67984,67984,135968,424.97617626190186,0.0007911427292128792
15704,68168,68168,136336,426.1376881599426,0.0007907089748186991
15739,68336,68336,136672,427.2196249961853,0.0007904125031927833
15775,68588,68588,137176,428.75132489204407,0.0007902957386249909
15810,68866,68866,137732,430.39924788475037,0.0007902963734522928
15846,69146,69146,138292,432.08061695098877,0.000790242131188279
15881,69316,69316,138632,433.1773121356964,0.0007899823394836858
15917,69472,69472,138944,434.19479393959045,0.0007896952756709652
15952,69618,69618,139236,435.19223499298096,0.0007891203240433242
15988,69784,69784,139568,436.27079820632935,0.0007887449919508072
16023,69940,69940,139880,437.28167510032654,0.0007880558878241573
16059,70104,70104,140208,438.3361761569977,0.0007875109295127913
16094,70250,70250,140500,439.27746510505676,0.0007867722506489372
16130,70434,70434,140868,440.4412591457367,0.0007862883394409437
16165,70588,70588,141176,441.4419050216675,0.0007853523202356882
16201,70742,70742,141484,442.4378590583801,0.000784387057137792
16237,70886,70886,141772,443.3769931793213,0.000780425329139689
16272,71026,71026,142052,444.3026921749115,0.0007741904628346674
16308,71170,71170,142340,445.23135900497437,0.0007665427492611343
16343,71358,71358,142716,446.4185690879822,0.0007573926322947955
16379,71590,71590,143180,447.85360527038574,0.0007573648490506457
16414,71866,71866,143732,449.56836891174316,0.000757363552111201
16450,72012,72012,144024,450.68078207969666,0.0007573140355816577
16485,72152,72152,144304,451.64428210258484,0.0007572242902824655
16521,72298,72298,144596,452.59803009033203,0.00075714361264545
16556,72438,72438,144876,453.525887966156,0.0007569837453047512
16592,72596,72596,145192,454.55489706993103,0.0007568677719973493
16627,72746,72746,145492,455.47075724601746,0.0007565531614091014
16663,72898,72898,145796,456.37541818618774,0.0007560886224382557
16698,73050,73050,146100,457.318706035614,0.000756025883674738
16734,73208,73208,146416,458.2639329433441,0.0007559745208709501
16769,73364,73364,146728,459.1914849281311,0.0007557963417639257
16805,73518,73518,147036,460.1480882167816,0.0007556748241768219
16841,73704,73704,147408,461.2363929748535,0.0007555411266366718
16876,73896,73896,147792,462.31389021873474,0.0007553483301308006
16912,74054,74054,148108,463.2265040874481,0.0007551603739557322
16947,74328,74328,148656,464.6767590045929,0.0007551529870397644
16983,74608,74608,149216,466.2133800983429,0.0007551270664407639
17018,74888,74888,149776,467.723237991333,0.0007551267935923534
17054,75176,75176,150352,469.36522817611694,0.0007551265116489958
17089,75438,75438,150876,470.7835099697113,0.0007549210567958653
17125,75718,75718,151436,472.51305508613586,0.0007549148431280628
17160,75990,75990,151980,474.1272692680359,0.0007548773901362438
17196,76152,76152,152304,475.10847210884094,0.000753906188037945
17231,76300,76300,152600,476.02570128440857,0.0007521703519159928
17267,76450,76450,152900,476.94904708862305,0.0007465476737706922
17302,76592,76592,153184,477.8714950084686,0.0007400250869977754
17338,76740,76740,153480,478.834450006485,0.0007341337695834227
17373,76882,76882,153764,479.75919008255005,0.0007057567981973989
17409,77028,77028,154056,480.6993169784546,0.000658199169265572
17445,77184,77184,154368,481.63893723487854,0.0005368545735109365
17480,77324,77324,154648,482.5096700191498,0.00045682035124627873
17516,77480,77480,154960,483.50274419784546,0.00033321647424600087
17551,77648,77648,155296,484.50692987442017,0.0003331626739964122
17587,77792,77792,155584,485.4536461830139,0.0003330655235913582
17622,77932,77932,155864,486.37695503234863,0.0003329723695060238
17658,78080,78080,156160,487.3413550853729,0.0003329050068714423
17693,78224,78224,156448,488.26430106163025,0.0003328265102027217
17729,78368,78368,156736,489.1875419616699,0.00033269743107666727
17764,78516,78516,157032,490.13150119781494,0.0003326567730255192
17800,78712,78712,157424,491.3398220539093,0.00033260867166973185
17835,78864,78864,157728,492.3450679779053,0.00033259224983339664
17871,79012,79012,158024,493.34601497650146,0.000332562785843038
17906,79158,79158,158316,494.2562401294708,0.00033249258194700815
17942,79310,79310,158620,495.2454719543457,0.0003324521476315567
17977,79482,79482,158964,496.3263580799103,0.000332381610860466
18013,79648,79648,159296,497.4181959629059,0.00033223013269889634
18048,79796,79796,159592,498.4085490703583,0.00033207080196007155
18084,79958,79958,159916,499.4639871120453,0.0003317828868603101
18120,80114,80114,160228,500.4032452106476,0.0003316403726785211
18155,80268,80268,160536,501.34233808517456,0.0003314697605674155
18191,80484,80484,160968,502.55318212509155,0.0003312473854748532
18226,80652,80652,161304,503.555242061615,0.00033104846806963906
18262,80818,80818,161636,504.55547404289246,0.000330868491801084
18297,80970,80970,161940,505.4825279712677,0.0003307550068711862
18333,81152,81152,162304,506.5396611690521,0.00033067843469325453
18368,81322,81322,162644,507.5657489299774,0.00033056470965675544
18404,81520,81520,163040,508.7188789844513,0.0003304949259472778
18439,81706,81706,163412,509.8210859298706,0.00033036440254363697
18475,81908,81908,163816,510.96884512901306,0.0003301705619378481
18510,82180,82180,164360,512.4593999385834,0.00033015811095538083
18546,82466,82466,164932,514.0313658714294,0.0003301572342024883
18581,82742,82742,165484,515.5138781070709,0.00033014853215718176
18617,83028,83028,166056,517.0771460533142,0.0003301464348623995
18652,83308,83308,166616,518.5872042179108,0.0003301462948002154
18688,83586,83586,167172,520.1058571338654,0.0003301249653304694
18724,83872,83872,167744,521.6545281410217,0.00033012317726388574
18759,84148,84148,168296,523.1495649814606,0.000330069340634509
18795,84426,84426,168852,524.6499330997467,0.0003300520584161859
18830,84704,84704,169408,526.152890920639,0.00033005161276378203
18866,84992,84992,169984,527.7112550735474,0.00033005146724462975
18901,85270,85270,170540,529.2028002738953,0.0003300498392491136
18937,85554,85554,171108,530.7536189556122,0.0003300344724266324
18972,85832,85832,171664,532.2658140659332,0.00033003298995026853
19008,86120,86120,172240,533.8652439117432,0.00033003284443111625
19043,86396,86396,172792,535.3672981262207,0.0003300300995761063
19079,86624,86624,173248,536.6573650836945,0.00032961020951916
19114,86780,86780,173560,537.5652050971985,0.0003291168868599925
19150,86986,86986,173972,538.8229739665985,0.0003289350097475108
19185,87260,87260,174520,540.312059879303,0.0003289156247774372
19221,87546,87546,175092,541.8794219493866,0.0003289137948740972
19256,87810,87810,175620,543.4115340709686,0.00032888467649172526
19292,88080,88080,176160,545.1471841335297,0.00032875575016078074
19328,88320,88320,176640,546.6507329940796,0.0003286690443928819
19363,88594,88594,177188,548.1289041042328,0.0003286519931862131
19399,88878,88878,177756,549.6748449802399,0.00032864905369933695
19434,89152,89152,178304,551.1246700286865,0.0003286399951321073
19470,89438,89438,178876,552.6487090587616,0.0003286392839072505
19505,89716,89716,179432,554.1385600566864,0.00032863218257261906
19541,90002,90002,180004,555.7101340293884,0.00032863136038940866
19576,90280,90280,180560,557.2965710163116,0.00032862899024621584
19612,90488,90488,180976,558.5122141838074,0.00032846094109117985
19647,90768,90768,181536,560.0198311805725,0.0003284608028479852
19683,91054,91054,182108,561.592766046524,0.0003284582962805871
19718,91324,91324,182648,563.04030418396,0.00032841384199855383
19754,91610,91610,183220,564.5658838748932,0.00032841209576872643
19789,91888,91888,183776,566.0483441352844,0.00032841040592757054
19825,92172,92172,184344,567.5470089912415,0.00032840537642186973
19860,92452,92452,184904,569.0131788253784,0.00032840523635968566
19896,92712,92712,185424,570.4064419269562,0.0003279142856627004
19932,92870,92870,185740,571.319561958313,0.0003271659843449015
19967,93012,93012,186024,572.1395320892334,0.00032605271735519636
20003,93156,93156,186312,573.009889125824,0.0003184883953508688
20038,93296,93296,186592,573.8358931541443,0.00030322079328470863
20074,93474,93474,186948,574.8507578372955,0.00028257546364329755
20109,93736,93736,187472,576.2397949695587,0.00028262783416721504
20145,93976,93976,187952,577.5557971000671,0.00028135393949924037
20180,94176,94176,188352,578.7005891799927,0.00028133085470471997
20216,94454,94454,188908,580.1960020065308,0.00028132448278483935
20251,94620,94620,189240,581.129243850708,0.00028128353915235493
20287,94780,94780,189560,582.0546209812164,0.00028126810684625525
20322,94928,94928,189856,582.9146590232849,0.0002812103593896609
20358,95072,95072,190144,583.770072221756,0.00028107353500672616
20393,95216,95216,190432,584.5952372550964,0.0002810182049870491
20429,95360,95360,190720,585.4485561847687,0.00028098078109906055
20464,95502,95502,191004,586.3000020980835,0.0002809525285556447
20500,95658,95658,191316,587.200926065445,0.00028090259911550675
20535,95822,95822,191644,588.1471061706543,0.00028080467018298805
20571,95986,95986,191972,589.0902469158173,0.0002807378532452276
20607,96156,96156,192312,590.0999190807343,0.00028069298423361033
20642,96324,96324,192648,591.0452480316162,0.0002806162246997701
20678,96490,96490,192980,591.9914691448212,0.000280529166047927
20713,96710,96710,193420,593.1787750720978,0.00028044004102412146
20749,96896,96896,193792,594.2347021102905,0.00028033462695020717
20784,97172,97172,194344,595.6912560462952,0.00028032348927808926
20820,97458,97458,194916,597.2071740627289,0.0002803200677590212
20855,97732,97732,195464,598.6452639102936,0.00028030743305862416
20891,98016,98016,196032,600.1238679885864,0.0002803047318593599
20926,98296,98296,196592,601.595715045929,0.00028030461362504866
20962,98578,98578,197156,603.0703780651093,0.0002802610233629821
20997,98852,98852,197704,604.4955809116364,0.00028025581923429854
21033,99134,99134,198268,605.999922990799,0.0002802543058351148
21068,99400,99400,198800,607.428092956543,0.00028019267665513325
21104,99674,99674,199348,608.8791010379791,0.00028014189774694387
21139,99952,99952,199904,610.3556401729584,0.0002801376122079091
21175,100238,100238,200476,611.8609600067139,0.0002801362170430366
21211,100526,100526,201052,613.3831300735474,0.00028013609517074656
21246,100800,100800,201600,614.8441541194916,0.00028012171969749033
21282,101086,101086,202172,616.34330701828,0.00028011787435389124
21317,101366,101366,202732,617.819066286087,0.0002801177579385694
21353,101654,101654,203308,619.3303401470184,0.0002801176360662794
21388,101930,101930,203860,620.7932720184326,0.00028011531867377926
21424,102206,102206,204412,622.2343900203705,0.0002798901787173236
21459,102364,102364,204728,623.1472451686859,0.00027856525957759004
21495,102524,102524,205048,624.0592350959778,0.0002782040028250776
21530,102722,102722,205444,625.1783859729767,0.0002777410063572461
21566,102994,102994,205988,626.6209390163422,0.00027773078909376636
21601,103260,103260,206520,628.0485260486603,0.0002777292265818687
21637,103540,103540,207080,629.547581911087,0.00027771735221904237
21672,103816,103816,207632,631.0310881137848,0.00027771528039011173
21708,104054,104054,208108,632.3372161388397,0.0002774967924779048
21743,104210,104210,208420,633.2279198169708,0.0002773677570075961
21779,104412,104412,208824,634.3605530261993,0.0002772553234535735
21815,104644,104644,209288,635.6164391040802,0.00027725302606995683
21850,104922,104922,209844,637.0846180915833,0.000277250033832388
21886,105204,105204,210408,638.5937190055847,0.00027723153289116453
21921,105482,105482,210964,640.0589509010315,0.0002772312491288176
21957,105768,105768,211536,641.5587320327759,0.0002772294574242551
21992,106046,106046,212092,643.0234000682831,0.00027722849699785
22028,106334,106334,212668,644.5673279762268,0.00027722837512556
22063,106602,106602,213204,645.9801480770111,0.00027719106401491445
22099,106886,106886,213772,647.4942910671234,0.00027718968158296775
22134,107160,107160,214320,648.9683170318604,0.0002771861618384719
22170,107446,107446,214892,650.4771399497986,0.00027717938064597547
22205,107670,107670,215340,651.6959049701691,0.00027697801488102414
22241,107850,107850,215700,652.7108669281006,0.00027646533635561354
22276,108064,108064,216128,653.8942432403564,0.00027613635575107764
22312,108346,108346,216692,655.3815131187439,0.00027613103338808287
22347,108610,108610,217220,656.7640142440796,0.0002760947882052278
22383,108782,108782,217564,657.7504179477692,0.0002759216386039043
22419,109064,109064,218128,659.243330001831,0.00027591543039307
22454,109342,109342,218684,660.7198829650879,0.00027591089565248694
22490,109630,109630,219260,662.2372710704803,0.0002759107755991863
22525,109904,109904,219808,663.6684310436249,0.00027590786885411944
22561,110188,110188,220376,665.1753630638123,0.0002758825557975797
22596,110464,110464,220928,666.6519401073456,0.00027588124430621974
22632,110744,110744,221488,668.1253390312195,0.00027585005773289595
22667,111020,111020,222040,669.5596082210541,0.00027584840790950693
22703,111306,111306,222612,671.058266878128,0.00027584600502450485
22738,111584,111584,223168,672.5986320972443,0.00027584421695792116
22774,111866,111866,223732,674.4829361438751,0.0002758024656941416
22809,112142,112142,224284,676.0438048839569,0.00027579772722674534
22845,112430,112430,224860,677.5698320865631,0.0002757976053544553
22880,112708,112708,225416,679.04176902771,0.00027579310699366033
22916,112992,112992,225984,680.8619542121887,0.00027578917615755927
22951,113272,113272,226544,682.5563032627106,0.00027578905792324804
22987,113560,113560,227120,684.3253729343414,0.0002757889396889368
23022,113832,113832,227664,685.9020500183105,0.0002756656740530161
23058,114116,114116,228232,687.5277290344238,0.00027566256358113606
23094,114402,114402,228804,689.1952068805695,0.00027566096287046093
23129,114682,114682,229364,690.6864860057831,0.0002756608482741285
23165,114968,114968,229936,692.2176692485809,0.00027565799609874375
23200,115248,115248,230496,693.6836440563202,0.0002756578796834219
23236,115534,115534,231068,695.1952798366547,0.00027565754498937167
23271,115812,115812,231624,696.6747479438782,0.0002756511439656606
23307,116098,116098,232196,698.1899650096893,0.00027564820447878446
23342,116370,116370,232740,699.707967042923,0.0002755734367383411
23378,116652,116652,233304,701.4463429450989,0.0002755682980932761
23413,116932,116932,233864,703.0456631183624,0.00027556818167795427
23449,117218,117218,234436,704.8415911197662,0.00027555879205465317
23484,117496,117496,234992,706.379830121994,0.0002755576679192018
23520,117782,117782,235564,708.0224261283875,0.00027555606720852666
23555,118062,118062,236124,709.6002979278564,0.0002755559489742154
23591,118348,118348,236696,711.1994450092316,0.0002755543937382754
23626,118626,118626,237252,712.7316429615021,0.0002755525965767447
23662,118912,118912,237824,714.2360162734985,0.0002755492678261362
23698,119200,119200,238400,715.7135128974915,0.00027554914595384616
23733,119480,119480,238960,717.3891389369965,0.00027554902953852434
23769,119766,119766,239532,718.9026260375977,0.00027554431289900094
23804,120044,120044,240088,720.4995121955872,0.0002755418718152214
23840,120332,120332,240664,722.14102602005,0.00027554174994293135
23875,120572,120572,241144,723.5056481361389,0.00027208445499127265
23911,120720,120720,241440,724.3978409767151,0.0002451450982334791
23946,120918,120918,241836,725.4910349845886,0.0001651966285862727
23982,121062,121062,242124,726.3953878879547,0.00016517563381057698
24017,121206,121206,242412,727.3203730583191,0.00016515474271727726
24053,121360,121360,242720,728.3121762275696,0.00016512355250597466
24088,121514,121514,243028,729.2083189487457,0.0001651019829296274
24124,121664,121664,243328,730.0926668643951,0.0001650670383241959
24159,121818,121818,243636,730.9835450649261,0.00016501960453751963
24195,121980,121980,243960,731.910628080368,0.00016496559510414954
24230,122142,122142,244284,732.8192760944366,0.00016490327834617347
24266,122294,122294,244588,733.6966941356659,0.0001648143388592871
24302,122476,122476,244952,734.7158660888672,0.0001647347344260197
24337,122662,122662,245324,735.7418439388275,0.00016470454829686787
24373,122866,122866,245732,736.8580000400543,0.00016467767454741988
24408,123132,123132,246264,738.2662038803101,0.0001646727650950197
24444,123420,123420,246840,739.7972030639648,0.0001646726559556555
24479,123700,123700,247400,741.27499127388,0.0001646725468162913
24515,123988,123988,247976,742.818498134613,0.00016467243767692707
24550,124264,124264,248528,744.2700412273407,0.00016466919259983115
24586,124548,124548,249096,745.9274611473083,0.00016463872270833235
24621,124824,124824,249648,747.5298681259155,0.00016463620704598725
24657,125106,125106,250212,749.1548049449921,0.00016461609629914165
24692,125384,125384,250768,750.6868731975555,0.00016461485211038962
24728,125672,125672,251344,752.3599760532379,0.000164614741152036
24763,125952,125952,251904,753.9029331207275,0.0001646146338316612
24799,126238,126238,252476,755.4086890220642,0.0001646086329856189
24834,126516,126516,253032,756.8446180820465,0.0001646083328523673
24870,126804,126804,253608,758.4532680511475,0.0001646082237130031
24905,127072,127072,254144,759.8947122097015,0.00016449688337161206
24941,127340,127340,254680,761.2917370796204,0.0001644527874304913
24977,127626,127626,255252,762.8098530769348,0.0001644520252739312
25012,127904,127904,255808,764.2621750831604,0.00016445118308183737
25048,128186,128186,256372,765.6912460327148,0.00016444392531411722
25083,128464,128464,256928,767.1431679725647,0.0001644436124479398
25119,128742,128742,257484,768.5972480773926,0.0001643420873733703
25154,129018,129018,258036,770.0300920009613,0.00016433951168437488
25190,129304,129304,258608,771.5384211540222,0.00016433817290817387
25225,129580,129580,259160,772.9913420677185,0.00016433016389783006
25261,129864,129864,259728,774.4551260471344,0.00016432706615887582
25296,130144,130144,260288,775.891175031662,0.00016432695883850101
25332,130432,130432,260864,777.389543056488,0.0001643268496991368
25367,130708,130708,261416,778.8203821182251,0.00016431769472546875
25403,130996,130996,261992,780.3088059425354,0.00016431758194812573
25438,131274,131274,262548,781.7666659355164,0.0001643118666834198
25474,131562,131562,263124,783.2401731014252,0.00016431175572506618
25509,131842,131842,263684,784.7006001472473,0.00016431165022368077
25545,132130,132130,264260,786.1888520717621,0.00016431154108431656
25581,132366,132366,264732,787.4494771957397,0.00016336169392161537
25616,132596,132596,265192,788.6923069953918,0.00016345269432349596
25652,132864,132864,265728,790.093090057373,0.00016334732754330616
25687,133144,133144,266288,791.5372490882874,0.00016334722204192076
25723,133426,133426,266852,793.0284328460693,0.00016334552856278606
25758,133704,133704,267408,794.4773650169373,0.00016334351312252693
25794,133992,133992,267984,795.9578812122345,0.0001633434021641733
25829,134272,134272,268544,797.3979241847992,0.0001633432948437985
25865,134558,134558,269116,798.8924958705902,0.0001633425781619735
25900,134838,134838,269676,800.3399200439453,0.0001633424708415987
25936,135126,135126,270252,801.8529851436615,0.00016334236170223448
25971,135406,135406,270812,803.3136692047119,0.00016334225438185968
26007,135694,135694,271388,804.8131730556488,0.00016334214342350606
26042,135974,135974,271948,806.2793111801147,0.00016334203610313125
26078,136262,136262,272524,807.7841711044312,0.00016334192696376704
26113,136510,136510,273020,809.0712180137634,0.0001633375431993045
26149,136720,136720,273440,810.2109251022339,0.00016332817904185504
26185,137006,137006,274012,811.6808750629425,0.0001633265637792647
26220,137286,137286,274572,813.1362502574921,0.00016332645827787928
26256,137572,137572,275144,814.6388108730316,0.00016332425184373278
26291,137848,137848,275696,816.0716469287872,0.00016331624283338897
26327,138134,138134,276268,817.5529391765594,0.00016331580809492152
26362,138412,138412,276824,819.0296719074249,0.00016331530423485674
26398,138694,138694,277388,820.5426502227783,0.00016330737162206788
26433,138972,138972,277944,822.0846831798553,0.0001633030260563828
26469,139256,139256,278512,823.6734561920166,0.00016329521895386279
26504,139532,139532,279064,825.2330861091614,0.00016326451623172034
26540,139818,139818,279636,827.0403578281403,0.00016326205332006793
26575,140098,140098,280196,828.6689960956573,0.00016326194418070372
26611,140380,140380,280760,830.1599960327148,0.00016325559772667475
26646,140660,140660,281320,831.8042261600494,0.00016325549222528934
26682,140946,140946,281892,833.3947021961212,0.00016325343312928453
26717,141226,141226,282452,834.9151329994202,0.00016325332580890972
26753,141510,141510,283020,836.4997041225433,0.00016324908028764185
26789,141798,141798,283596,838.3131620883942,0.00016324897114827763
26824,142078,142078,284156,839.9009459018707,0.00016324886382790282
26860,142364,142364,284728,841.4655921459198,0.00016324262651323806
26895,142642,142642,285284,843.1139562129974,0.00016324219359376002
26931,142928,142928,285856,844.6386210918427,0.00016324185344274156
26966,143206,143206,286412,846.0946459770203,0.00016324013995472342
27002,143492,143492,286984,847.5937721729279,0.0001632381845411146
27037,143770,143770,287540,849.0518450737,0.00016323661111528054
27073,144058,144058,288116,850.5510149002075,0.00016323650197591633
27108,144338,144338,288676,852.0206878185272,0.00016323639465554152
27144,144626,144626,289252,853.5365839004517,0.0001632362836971879
27179,144862,144862,289724,854.8003950119019,0.00016108207273646258
27215,145038,145038,290076,855.7959549427032,0.00015968974912539124
27250,145186,145186,290372,856.6259920597076,0.00015755853928567376
27286,145338,145338,290676,857.5004422664642,0.00015133642773434985
27321,145482,145482,290964,858.3307280540466,0.00014751198978046887
27357,145630,145630,291260,859.1862530708313,0.00013984514589537866
27392,145770,145770,291540,860.0101251602173,0.00013453066640067846
27428,145930,145930,291860,860.9205939769745,0.00010811994798132218
27464,146172,146172,292344,862.2089960575104,0.00010798941184475552
27499,146380,146380,292760,863.3392939567566,0.00010797447794175241
27535,146614,146614,293228,864.5947070121765,0.00010794083209475502
27570,146758,146758,293516,865.4661099910736,0.00010793457295221742
27606,146902,146902,293804,866.475438117981,0.00010792350985866506
27641,147046,147046,294092,867.3869760036469,0.0001079116809705738
27677,147198,147198,294396,868.414489030838,0.00010790164196805563
27712,147354,147354,294708,869.3067572116852,0.00010789155930979177
27748,147508,147508,295016,870.1737291812897,0.00010785147424030583
27783,147652,147652,295304,871.0092730522156,0.0001077630204235902
27819,147806,147806,295612,871.8894729614258,0.00010773610847536474
27854,147964,147964,295928,872.9349410533905,0.00010772030691441614
27890,148194,148194,296388,874.3481631278992,0.00010769538675958756
27925,148382,148382,296764,875.3886280059814,0.0001076535445463378
27961,148574,148574,297148,876.4558100700378,0.00010761284283944406
27996,148844,148844,297688,877.8843882083893,0.00010758796815935057
28032,149126,149126,298252,879.3661539554596,0.000107585725345416
28068,149406,149406,298812,880.8232178688049,0.00010758327152871061
28103,149684,149684,299368,882.2708611488342,0.00010758159260149114
28139,149972,149972,299944,883.7730638980865,0.00010758153621281963
28174,150248,150248,300496,885.206433057785,0.00010757987001852598
28210,150506,150506,301012,886.5724930763245,0.00010752199523267336
28245,150742,150742,301484,887.8202090263367,0.00010747186024673283
28281,151022,151022,302044,889.2861561775208,0.00010747059604909737
28316,151290,151290,302580,890.6588742733002,0.00010746643238235265
28352,151480,151480,302960,891.69944190979,0.00010744267638074234
28387,151728,151728,303456,893.0057010650635,0.00010743314305727836
28423,152010,152010,304020,894.4833731651306,0.00010742913400463294
28458,152286,152286,304572,895.912623167038,0.000107427624243428
28494,152570,152570,305140,897.3867330551147,0.00010742721860879101
28529,152850,152850,305700,898.8333210945129,0.0001074271622201195
28565,153134,153134,306268,900.3005890846252,0.00010741703590610996
28600,153412,153412,306824,901.752424955368,0.000107416648461367
28636,153696,153696,307392,903.2179090976715,0.00010741595360741485
28672,153926,153926,307852,904.4477560520172,0.00010718928569986019
28707,154144,154144,308288,905.6178991794586,0.0001065936576196691
28743,154298,154298,308596,906.4943220615387,0.00010540259063418489
28778,154450,154450,308900,907.3687932491302,0.00010425148684589658
28814,154616,154616,309232,908.3261299133301,0.00010364617264713161
28849,154758,154758,309516,909.1438610553741,0.00010265979835821781
28885,154912,154912,309824,910.0290172100067,0.00010052404468297027
28920,155052,155052,310104,910.8488600254059,9.682539348432329e-05
28956,155208,155208,310416,911.7476532459259,9.327813677373342e-05
28991,155416,155416,310832,912.8853430747986,9.044095168064814e-05
29027,155658,155658,311316,914.1833591461182,9.045602746482473e-05
29062,155854,155854,311708,915.2320051193237,9.110439896176104e-05
29098,156018,156018,312036,916.1730461120605,9.133392268267926e-05
29133,156204,156204,312408,917.1910600662231,9.044445141626056e-05
29169,156424,156424,312848,918.3795690536499,9.043940190167632e-05
29204,156684,156684,313368,919.7517590522766,9.043870522873476e-05
29240,156960,156960,313920,921.197765827179,9.043286081578117e-05
29276,157104,157104,314208,922.0276050567627,9.038857751875184e-05
29311,157248,157248,314496,922.875333070755,9.037871132022701e-05
29347,157410,157410,314820,923.7963171005249,9.036941082740668e-05
29382,157564,157564,315128,924.6763589382172,9.03603940969333e-05
29418,157756,157756,315512,925.7259268760681,9.034822141984478e-05
29453,157922,157922,315844,926.6625680923462,9.031598528963514e-05
29489,158088,158088,316176,927.6001920700073,9.02789251995273e-05
29524,158288,158288,316576,928.6881589889526,9.024742212204728e-05
29560,158566,158566,317132,930.1572329998016,9.024472819874063e-05
29595,158758,158758,317516,931.220269203186,9.022899757837877e-05
29631,158936,158936,317872,932.22043800354,9.021211008075625e-05
29666,159106,159106,318212,933.1719648838043,9.017368392960634e-05
29702,159284,159284,318568,934.1984980106354,9.014409079100005e-05
29737,159494,159494,318988,935.4034402370453,9.004246203403454e-05
29773,159660,159660,319320,936.3915300369263,8.995393181976397e-05
29808,159818,159818,319636,937.3887870311737,8.991580943984445e-05
29844,159998,159998,319996,938.4992158412933,8.985047497844789e-05
29879,160252,160252,320504,939.9374599456787,8.984288251667749e-05
29915,160530,160530,321060,941.5449900627136,8.984059422800783e-05
29951,160778,160778,321556,943.0003509521484,8.982973849924747e-05
29986,161052,161052,322104,944.4302752017975,8.982756480691023e-05
30022,161314,161314,322628,945.7899429798126,8.978385631053243e-05
30057,161532,161532,323064,946.9469990730286,8.975057062343694e-05
30093,161818,161818,323636,948.4103670120239,8.974756747193169e-05
30128,162096,162096,324192,949.8670279979706,8.974716729426291e-05
30164,162376,162376,324752,951.3175821304321,8.974402408057358e-05
30199,162650,162650,325300,952.6964921951294,8.973258445621468e-05
30235,162936,162936,325872,954.1893770694733,8.973213698482141e-05
30270,163216,163216,326432,955.7333319187164,8.973208787210751e-05
30306,163498,163498,326996,957.4574029445648,8.97313620953355e-05
30341,163768,163768,327536,958.9743430614471,8.972138675744645e-05
30377,164054,164054,328108,960.5655879974365,8.972128125606105e-05
30412,164334,164334,328668,962.1552929878235,8.972123396233656e-05
30448,164614,164614,329228,963.6502740383148,8.971893657871988e-05
30483,164892,164892,329784,965.1243619918823,8.971857459982857e-05
30519,165176,165176,330352,966.6252150535583,8.97165919013787e-05
30555,165462,165462,330924,968.1411280632019,8.971537499746773e-05
30590,165738,165738,331476,969.5925529003143,8.97135632840218e-05
30626,166020,166020,332040,971.0920362472534,8.96962719707517e-05
30661,166216,166216,332432,972.1578931808472,8.926158807298634e-05
30697,166390,166390,332780,973.1381850242615,8.889622040442191e-05
30732,166538,166538,333076,973.9854872226715,8.742079626244958e-05
30768,166694,166694,333388,974.9518721103668,8.659271588840056e-05
30803,166862,166862,333724,975.8849761486053,8.557085129723419e-05
30839,167012,167012,334024,976.7612009048462,8.457644617010374e-05
30874,167166,167166,334332,977.8043200969696,8.28973115858389e-05
30910,167326,167326,334652,978.8115479946136,8.18791268102359e-05
30945,167474,167474,334948,979.7536981105804,7.989959158294369e-05
30981,167622,167622,335244,980.6190259456635,7.759575601085089e-05
31016,167764,167764,335528,981.4475772380829,7.133524195523933e-05
31052,167908,167908,335816,982.2933912277222,6.398268124030437e-05
31087,168052,168052,336104,983.1262350082397,5.544068153540138e-05
31123,168204,168204,336408,984.0084049701691,4.810762402485125e-05
31159,168348,168348,336696,984.894453048706,4.722105950349942e-05
31194,168488,168488,336976,985.7154240608215,4.670799171435647e-05
31230,168636,168636,337272,986.5814049243927,3.694379665830638e-05
31265,168780,168780,337560,987.4342601299286,2.5973920855903998e-05
31301,169026,169026,338052,988.7599229812622,2.4093949832604267e-05
31336,169268,169268,338536,990.0421171188354,2.4077779016806744e-05
31372,169544,169544,339088,991.4487071037292,2.4076680347207002e-05
31407,169734,169734,339468,992.5084159374237,2.4069247956504114e-05
31443,169874,169874,339748,993.3290500640869,2.4062655938905664e-05
31478,170012,170012,340024,994.1480441093445,2.4056591428234242e-05
31514,170158,170158,340316,994.9972422122955,2.405471241218038e-05
31549,170298,170298,340596,995.8022210597992,2.4047281840466894e-05
31585,170450,170450,340900,996.6628749370575,2.4036713512032293e-05
31620,170642,170642,341284,997.6937611103058,2.4033104637055658e-05
31656,170840,170840,341680,998.8111202716827,2.403055077593308e-05
31691,171000,171000,342000,999.7218198776245,2.4027265681070276e-05
31727,171154,171154,342308,1000.608724117279,2.401739766355604e-05
31763,171302,171302,342604,1001.4846980571747,2.3989288820303045e-05
31798,171454,171454,342908,1002.3470611572266,2.3974309442564845e-05
31834,171602,171602,343204,1003.2104299068451,2.395953742961865e-05
31869,171748,171748,343496,1004.0547158718109,2.3953465642989613e-05
31905,171894,171894,343788,1004.9022221565247,2.3945827706484124e-05
31940,172046,172046,344092,1005.7817878723145,2.3938049707794562e-05
31976,172206,172206,344412,1006.6928472518921,2.39265264099231e-05
32011,172370,172370,344740,1007.6309361457825,2.3921957108541392e-05
32047,172528,172528,345056,1008.5332000255585,2.391491216258146e-05
32082,172696,172696,345392,1009.4785301685333,2.390510962868575e-05
32118,172884,172884,345768,1010.5028109550476,2.3895872800494544e-05
32153,173092,173092,346184,1011.6321210861206,2.3890439479146153e-05
32189,173260,173260,346520,1012.5800859928131,2.3882495952420868e-05
32224,173436,173436,346872,1013.5407092571259,2.3869981305324472e-05
32260,173658,173658,347316,1014.7396841049194,2.3860529836383648e-05
32295,173892,173892,347784,1015.9962041378021,2.385781226621475e-05
32331,174078,174078,348156,1017.033774137497,2.3855927793192677e-05
32366,174244,174244,348488,1017.9705650806427,2.3847605916671455e-05
32402,174442,174442,348884,1019.0751402378082,2.3840004359954037e-05
32438,174690,174690,349380,1020.3930051326752,2.3838674678700045e-05
32473,174890,174890,349780,1021.4828870296478,2.3835536921978928e-05
32509,175082,175082,350164,1022.5528891086578,2.3832229999243282e-05
32544,175264,175264,350528,1023.5632441043854,2.3816837710910477e-05
32580,175488,175488,350976,1024.7917921543121,2.3793281798134558e-05
32615,175676,175676,351352,1025.8266010284424,2.3746413717162795e-05
32651,175828,175828,351656,1026.6829681396484,2.3613276425749063e-05
32686,175980,175980,351960,1027.5502121448517,2.3393035007757135e-05
32722,176128,176128,352256,1028.4084658622742,2.2880887627252378e-05
32757,176270,176270,352540,1029.229653120041,2.2628655642620288e-05
32793,176452,176452,352904,1030.2391710281372,2.2616892238147557e-05
32828,176604,176604,353208,1031.1086132526398,2.2673591956845485e-05
32864,176776,176776,353552,1032.0717260837555,2.2474443539977074e-05
32899,176924,176924,353848,1032.9249889850616,2.2062220523366705e-05
32935,177072,177072,354144,1033.7922520637512,2.1260408175294288e-05
32970,177218,177218,354436,1034.6462779045105,2.0862469682469964e-05
33006,177370,177370,354740,1035.5412049293518,2.0435671103768982e-05
33042,177522,177522,355044,1036.4125719070435,1.9987739506177604e-05
33077,177662,177662,355324,1037.2107660770416,1.8585862562758848e-05
33113,177810,177810,355620,1038.0864441394806,1.6498257537023164e-05
33148,177950,177950,355900,1038.901848077774,1.3833710909239016e-05
33184,178094,178094,356188,1039.7326200008392,1.1092590284533799e-05
33219,178304,178304,356608,1040.902459859848,9.296847565565258e-06
33255,178452,178452,356904,1041.8055412769318,9.294295523432083e-06
33290,178688,178688,357376,1043.1544120311737,9.293486073147506e-06
33326,178892,178892,357784,1044.3715488910675,9.292183676734567e-06
33361,179040,179040,358080,1045.2542231082916,9.291470632888377e-06
33397,179192,179192,358384,1046.1843130588531,9.28945155465044e-06
33432,179332,179332,358664,1047.0602071285248,9.281438906327821e-06
33468,179484,179484,358968,1048.113186120987,9.277795470552519e-06
33503,179640,179640,359280,1049.0178079605103,9.276740456698462e-06
33539,179792,179792,359584,1049.888128042221,9.272436727769673e-06
33574,179936,179936,359872,1050.7143139839172,9.266364941140637e-06
33610,180084,180084,360168,1051.5857601165771,9.261624654754996e-06
33646,180244,180244,360488,1052.5018730163574,9.256689736503176e-06
33681,180396,180396,360792,1053.3897001743317,9.250194125343114e-06
33717,180578,180578,361156,1054.4118490219116,9.2491609393619e-06
33752,180768,180768,361536,1055.4603550434113,9.245957699022256e-06
33788,180960,180960,361920,1056.5077571868896,9.244871762348339e-06
33823,181118,181118,362236,1057.4068710803986,9.242849046131596e-06
33859,181300,181300,362600,1058.4204621315002,9.240729923476465e-06
33894,181470,181470,362940,1059.4634492397308,9.238050552085042e-06
33930,181638,181638,363276,1060.3929979801178,9.234880053554662e-06
33965,181820,181820,363640,1061.7893152236938,9.233343007508665e-06
34001,182008,182008,364016,1062.9329640865326,9.231542207999155e-06
34036,182194,182194,364388,1064.2836139202118,9.229972420143895e-06
34072,182380,182380,364760,1065.7131509780884,9.228157068719156e-06
34107,182584,182584,365168,1066.9047801494598,9.226279871654697e-06
34143,182764,182764,365528,1068.0649752616882,9.222578228218481e-06
34178,182962,182962,365924,1069.5507760047913,9.2179707280593e-06
34214,183162,183162,366324,1070.9113790988922,9.214796591550112e-06
34250,183346,183346,366692,1072.0582389831543,9.205450623994693e-06
34285,183544,183544,367088,1073.3558950424194,9.192144716507755e-06
34321,183724,183724,367448,1074.6268830299377,9.179966582451016e-06
34356,183896,183896,367792,1075.6584131717682,9.159835826721974e-06
34392,184114,184114,368228,1076.8889548778534,9.136914741247892e-06
34427,184290,184290,368580,1077.8833589553833,9.105069693760015e-06
34463,184450,184450,368900,1078.9108889102936,9.080462405108847e-06
34498,184608,184608,369216,1080.1639811992645,9.054776455741376e-06
34534,184792,184792,369584,1082.107535123825,9.006025720736943e-06
34569,184950,184950,369900,1083.6726121902466,8.947052265284583e-06
34605,185104,185104,370208,1084.5707468986511,8.881632311386056e-06
34640,185276,185276,370552,1085.548525094986,8.774855814408511e-06
34676,185426,185426,370852,1086.4212369918823,8.636183338239789e-06
34711,185580,185580,371160,1087.304003238678,8.497418093611486e-06
34747,185732,185732,371464,1088.1913521289825,8.489394531352445e-06
34782,185888,185888,371776,1089.0712461471558,8.386341505683959e-06
34818,186040,186040,372080,1089.953663110733,8.057473678491078e-06
34853,186180,186180,372360,1090.7673921585083,7.74579712015111e-06
34889,186336,186336,372672,1091.6751170158386,7.492490112781525e-06
34925,186484,186484,372968,1092.5469450950623,7.093291060300544e-06
34960,186626,186626,373252,1093.3903832435608,6.706481144647114e-06
34996,186770,186770,373540,1094.2188129425049,6.0691127146128565e-06
35031,186914,186914,373828,1095.0699081420898,4.952315066475421e-06
35067,187064,187064,374128,1095.9133050441742,3.961758920922875e-06
35102,187206,187206,374412,1096.746433019638,3.022982127731666e-06
35138,187342,187342,374684,1097.5592651367188,1.8929567886516452e-06
35173,187460,187460,374920,1098.283075094223,7.780054147588089e-07
35209,187584,187584,375168,1099.050499200821,2.426950231892988e-07
35244,187700,187700,375400,1099.7601511478424,1.7196725821122527e-08
35280,187824,187824,375648,1100.4983401298523,1.0649091564118862e-07
35315,187942,187942,375884,1101.2272820472717,1.713851816020906e-08
35351,188064,188064,376128,1101.9810190200806,7.952621672302485e-09
35386,188188,188188,376376,1102.7342040538788,6.801201379857957e-09
35422,188332,188332,376664,1103.5915460586548,5.178662831895053e-09
35457,188472,188472,376944,1104.4045979976654,3.5324774216860533e-09
35493,188616,188616,377232,1105.2502081394196,6.45741238258779e-11


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.0013380050659179688,848.0296294260013
26,54,27,81,0.03875422477722168,64.55440294495315
52,106,53,159,0.07812714576721191,54.22509003574646
78,158,79,237,0.11524724960327148,51.2969092672995
104,210,105,315,0.16167616844177246,48.72297871866749
129,260,130,390,0.19779610633850098,46.74075616746313
155,312,156,468,0.2304689884185791,44.43631605511496
181,364,182,546,0.2641868591308594,42.71364398680453
207,416,208,624,0.29657506942749023,40.73060747976024
233,468,234,702,0.3298759460449219,39.087079665765486
259,520,260,780,0.36219024658203125,37.332305536422155
285,572,286,858,0.3932528495788574,36.03472597627729
311,624,312,936,0.4252650737762451,34.861416548359784
337,676,338,1014,0.4582381248474121,33.65773857761383
363,728,364,1092,0.48850321769714355,32.58253864491621
388,778,389,1167,0.5180909633636475,31.644703310142177
414,830,415,1245,0.5485019683837891,30.658344269839517
440,882,441,1323,0.5788891315460205,29.76121898938527
466,934,467,1401,0.6091899871826172,28.893073472229844
492,986,493,1479,0.6394820213317871,27.98442518028901
518,1038,519,1557,0.6700711250305176,27.27382269331838
544,1090,545,1635,0.7010071277618408,26.632419444260677
570,1142,571,1713,0.7323331832885742,25.776650215247628
596,1194,597,1791,0.7643001079559326,25.033858078960748
621,1244,622,1866,0.7956140041351318,24.38877585334626
647,1296,648,1944,0.8287889957427979,23.884737122102933
673,1348,674,2022,0.861004114151001,23.14966530322249
699,1400,700,2100,0.8920278549194336,22.523100178724917
725,1452,726,2178,0.9245262145996094,22.017996133548422
751,1504,752,2256,0.9587399959564209,21.464858332583844
777,1556,778,2334,0.9931089878082275,20.98192310671834
803,1608,804,2412,1.0267038345336914,20.460179121105284
829,1660,830,2490,1.060230016708374,19.99264850112104
855,1712,856,2568,1.0920259952545166,19.496596493037487
880,1762,881,2643,1.1272971630096436,19.096591161775223
906,1814,907,2721,1.1602060794830322,18.63602398024318
932,1866,933,2799,1.1920130252838135,18.217339574553534
958,1918,959,2877,1.223886251449585,17.743323062224817
984,1970,985,2955,1.2553470134735107,17.39954682883058
1010,2022,1011,3033,1.2863199710845947,16.899319557106082
1036,2074,1037,3111,1.317944049835205,16.544207100359245
1062,2126,1063,3189,1.3498179912567139,16.156176624285536
1088,2178,1089,3267,1.381343126296997,15.796283555119203
1113,2228,1114,3342,1.4142279624938965,15.413354952006898
1139,2280,1140,3420,1.4463071823120117,15.079879678087877
1165,2332,1166,3498,1.479072093963623,14.671344576619276
1191,2384,1192,3576,1.5109572410583496,14.321231743000794
1217,2436,1218,3654,1.5425889492034912,13.974641827623486
1243,2488,1244,3732,1.5741472244262695,13.691403627591512
1269,2540,1270,3810,1.6067490577697754,13.345334473184494
1295,2592,1296,3888,1.6377081871032715,13.056265189725991
1321,2644,1322,3966,1.669348955154419,12.756130723805086
1347,2696,1348,4044,1.7003378868103027,12.465504141307633
1372,2746,1373,4119,1.7315011024475098,12.179080601483747
1398,2798,1399,4197,1.7634949684143066,11.879805570098256
1424,2850,1425,4275,1.7955269813537598,11.573713554482993
1450,2902,1451,4353,1.8277971744537354,11.31738306363411
1476,2954,1477,4431,1.8599040508270264,11.010097380303932
1502,3006,1503,4509,1.8917372226715088,10.808895255114635
1528,3058,1529,4587,1.9249138832092285,10.510792807917142
1554,3110,1555,4665,1.9578461647033691,10.291354840989584
1580,3162,1581,4743,1.9896290302276611,10.072079031799376
1605,3212,1606,4818,2.020695209503174,9.826333154595545
1631,3264,1632,4896,2.053359270095825,9.5662735381718
1657,3316,1658,4974,2.087393045425415,9.377416467291368
1683,3368,1684,5052,2.1211960315704346,9.161177453901587
1709,3420,1710,5130,2.1535820960998535,8.954672917738094
1735,3472,1736,5208,2.1854941844940186,8.755777858355145
1761,3524,1762,5286,2.222170829772949,8.547245145683632
1787,3576,1788,5364,2.2604410648345947,8.365212184241841
1813,3628,1814,5442,2.296041965484619,8.176834833998214
1839,3680,1840,5520,2.3287570476531982,7.9789181397180755
1864,3730,1865,5595,2.3717310428619385,7.779077630457323
1890,3782,1891,5673,2.403496026992798,7.597797091993698
1916,3834,1917,5751,2.43458890914917,7.417125140957069
1942,3886,1943,5829,2.465837240219116,7.271273415001019
1968,3938,1969,5907,2.4967780113220215,7.100406416774035
1994,3990,1995,5985,2.5292410850524902,6.971343847407866
2020,4042,2021,6063,2.5706288814544678,6.794730799243325
2046,4094,2047,6141,2.6034839153289795,6.667588717332023
2072,4146,2073,6219,2.6346702575683594,6.518530663246111
2097,4196,2098,6294,2.66723895072937,6.395856717360402
2123,4248,2124,6372,2.702852249145508,6.249954589872232
2149,4300,2150,6450,2.7347099781036377,6.1285117852759186
2175,4352,2176,6528,2.7669310569763184,6.007991640511818
2201,4404,2202,6606,2.798927068710327,5.871239533860603
2227,4456,2228,6684,2.8321008682250977,5.741786242539092
2253,4508,2254,6762,2.865093946456909,5.595760754569483
2279,4560,2280,6840,2.897611141204834,5.4877420492554165
2305,4612,2306,6918,2.9300990104675293,5.381440312968493
2331,4664,2332,6996,2.962351083755493,5.2657242542974245
2356,4714,2357,7071,2.9924230575561523,5.164887049658773
2382,4766,2383,7149,3.0255730152130127,5.053946727879747
2408,4818,2409,7227,3.0620691776275635,4.934487992532581
2434,4870,2435,7305,3.09454607963562,4.830610095022735
2460,4922,2461,7383,3.126134157180786,4.723752453326824
2486,4974,2487,7461,3.1594879627227783,4.635206789783524
2512,5026,2513,7539,3.1907169818878174,4.534577580845621
2538,5078,2539,7617,3.2242910861968994,4.435307488862691
2564,5130,2565,7695,3.2558341026306152,4.343919424261458
2589,5180,2590,7770,3.28741717338562,4.248667728689838
2615,5232,2616,7848,3.320863962173462,4.1543978278222085
2641,5284,2642,7926,3.3543481826782227,4.06360321614261
2667,5336,2668,8004,3.3863251209259033,3.984443010754717
2693,5388,2694,8082,3.420681953430176,3.896648972354569
2719,5440,2720,8160,3.455435037612915,3.8055699341405216
2745,5492,2746,8238,3.4883241653442383,3.7277595080684023
2771,5544,2772,8316,3.522062063217163,3.643820797674721
2797,5596,2798,8394,3.5641160011291504,3.573484532991415
2823,5648,2824,8472,3.5975260734558105,3.5006644175980455
2848,5698,2849,8547,3.630237102508545,3.426478353845596
2874,5750,2875,8625,3.673424005508423,3.3493800544190435
2900,5802,2901,8703,3.714553117752075,3.2742872959531724
2926,5854,2927,8781,3.7573490142822266,3.1942545933353585
2952,5906,2953,8859,3.791774034500122,3.1325427138531268
2978,5958,2979,8937,3.8243770599365234,3.06671029882898
3004,6010,3005,9015,3.862215042114258,3.00314073330685
3030,6062,3031,9093,3.8950350284576416,2.9499246011569085
3056,6114,3057,9171,3.9272570610046387,2.876919439614767
3081,6164,3082,9246,3.9581000804901123,2.8235996358640705
3107,6216,3108,9324,3.99005389213562,2.761865547683101
3133,6268,3134,9402,4.026061058044434,2.711254818505722
3159,6320,3160,9480,4.067285060882568,2.65476738661323
3185,6372,3186,9558,4.101819038391113,2.6076291315226854
3211,6424,3212,9636,4.136611223220825,2.5537932540888733
3237,6476,3238,9714,4.1849470138549805,2.508017372308359
3263,6528,3264,9792,4.22446608543396,2.456689298007859
3289,6580,3290,9870,4.259695291519165,2.4017173389752315
3315,6632,3316,9948,4.302698135375977,2.358619146934643
3340,6682,3341,10023,4.3410749435424805,2.3102868630620605
3366,6734,3367,10101,4.380881071090698,2.2600065238076468
3392,6786,3393,10179,4.434319257736206,2.2192334923530552
3418,6838,3419,10257,4.478191137313843,2.171428242212528
3444,6890,3445,10335,4.522029161453247,2.130923903506414
3470,6942,3471,10413,4.569005012512207,2.089940858676073
3496,6994,3497,10491,4.609097957611084,2.0517985539448773
3522,7046,3523,10569,4.649423837661743,2.0101641931411223
3548,7098,3549,10647,4.691973924636841,1.9713055262566286
3573,7148,3574,10722,4.734377145767212,1.9326929940564241
3599,7200,3600,10800,4.7766640186309814,1.8920624705403952
3625,7252,3626,10878,4.820632219314575,1.8559192969501055
3651,7304,3652,10956,4.862404823303223,1.8169066127536553
3677,7356,3678,11034,4.904090166091919,1.7795488150221672
3703,7408,3704,11112,4.941892862319946,1.7432217596507371
3729,7460,3730,11190,4.980417013168335,1.7090260225927523
3755,7512,3756,11268,5.019272089004517,1.6775808948925715
3781,7564,3782,11346,5.062787055969238,1.6452358593304552
3807,7616,3808,11424,5.1071391105651855,1.6166003574123806
3832,7666,3833,11499,5.139852046966553,1.5823864060167807
3858,7718,3859,11577,5.175869941711426,1.5564857210861192
3884,7770,3885,11655,5.2115678787231445,1.523059778140805
3910,7822,3911,11733,5.248098134994507,1.4925730139952975
3936,7874,3937,11811,5.2874979972839355,1.456877339508651
3962,7926,3963,11889,5.32738995552063,1.4273020682762763
3988,7978,3989,11967,5.386125087738037,1.3935744952474352
4014,8030,4015,12045,5.448139190673828,1.364236196827278
4040,8082,4041,12123,5.506074905395508,1.3377185652051367
4065,8132,4066,12198,5.5661211013793945,1.3142417650691414
4091,8184,4092,12276,5.605145215988159,1.2865148508889206
4117,8236,4118,12354,5.643064022064209,1.2647977159991797
4143,8288,4144,12432,5.680459022521973,1.233356781428597
4169,8340,4170,12510,5.7168920040130615,1.2122239562174855
4195,8392,4196,12588,5.748471021652222,1.1857824146770781
4221,8444,4222,12666,5.7812340259552,1.1658052585477208
4247,8496,4248,12744,5.813474178314209,1.1409037775135857
4273,8548,4274,12822,5.844692945480347,1.1221698918147922
4299,8600,4300,12900,5.877887010574341,1.0983877708569025
4324,8650,4325,12975,5.909085988998413,1.0784264927693812
4350,8702,4351,13053,5.940519094467163,1.0575797244581508
4376,8754,4377,13131,5.9726879596710205,1.0411863819617793
4402,8806,4403,13209,6.004653215408325,1.0184627887803117
4428,8858,4429,13287,6.03909707069397,0.9996042567518089
4454,8910,4455,13365,6.071835994720459,0.9810410080719976
4480,8962,4481,13443,6.103454113006592,0.9619839900936995
4506,9014,4507,13521,6.136389970779419,0.9457512061624129
4532,9066,4533,13599,6.170150995254517,0.9263325188439921
4558,9118,4559,13677,6.2021472454071045,0.9078027159144995
4583,9168,4584,13752,6.232576131820679,0.8938890073335415
4609,9220,4610,13830,6.264657020568848,0.87397436363824
4635,9272,4636,13908,6.29597282409668,0.8554724705459194
4661,9324,4662,13986,6.328663110733032,0.8394402454010788
4687,9376,4688,14064,6.360320091247559,0.8211654535648449
4713,9428,4714,14142,6.391748905181885,0.8056871818102991
4739,9480,4740,14220,6.422648191452026,0.790487812439892
4765,9532,4766,14298,6.453912019729614,0.7766888413459583
4791,9584,4792,14376,6.484600067138672,0.7600927170526575
4816,9634,4817,14451,6.514842987060547,0.7482223485787927
4842,9686,4843,14529,6.545650959014893,0.7334171972430568
4868,9738,4869,14607,6.584417104721069,0.7206435594777076
4894,9790,4895,14685,6.617176055908203,0.7058119215914758
4920,9842,4921,14763,6.648874998092651,0.6934073755485315
4946,9894,4947,14841,6.682165145874023,0.6772689686090416
4972,9946,4973,14919,6.714212894439697,0.6654689520771626
4998,9998,4999,14997,6.749465227127075,0.6505907214433364
5024,10050,5025,15075,6.782247066497803,0.6392163299052527
5050,10102,5051,15153,6.813384056091309,0.6284885096171138
5075,10152,5076,15228,6.842666149139404,0.6198768841419451
5101,10204,5102,15306,6.874150991439819,0.6057195174215622
5127,10256,5128,15384,6.90506911277771,0.5933908032951649
5153,10308,5154,15462,6.935479164123535,0.5800412660561278
5179,10360,5180,15540,6.9665422439575195,0.5697731497725727
5205,10412,5206,15618,6.996830940246582,0.5604054627007145
5231,10464,5232,15696,7.028916120529175,0.5497396805941435
5257,10516,5258,15774,7.065083026885986,0.5400916386435028
5283,10568,5284,15852,7.098427057266235,0.529425072618892
5308,10618,5309,15927,7.129975080490112,0.5192307388290374
5334,10670,5335,16005,7.163006067276001,0.5084733481963895
5360,10722,5361,16083,7.1944899559021,0.4996620600282995
5386,10774,5387,16161,7.226233959197998,0.4891552348897221
5412,10826,5413,16239,7.2573230266571045,0.48046308450091146
5438,10878,5439,16317,7.2879040241241455,0.4730683393485151
5464,10930,5465,16395,7.319252967834473,0.4634995210934676
5490,10982,5491,16473,7.351169109344482,0.4550512076898485
5516,11034,5517,16551,7.3830389976501465,0.4461184943892249
5542,11086,5543,16629,7.413646221160889,0.43835492213122507
5567,11136,5568,16704,7.442866086959839,0.43029951304083625
5593,11188,5594,16782,7.474086046218872,0.4220698081852561
5619,11240,5620,16860,7.506273031234741,0.41429418135555807
5645,11292,5646,16938,7.53666615486145,0.406263227637055
5671,11344,5672,17016,7.568187952041626,0.39831266493195017
5697,11396,5698,17094,7.598288059234619,0.39144347363765064
5723,11448,5724,17172,7.628852128982544,0.38356540071458767
5749,11500,5750,17250,7.661334991455078,0.37719250395423387
5775,11552,5776,17328,7.691876173019409,0.3695133301864644
5800,11602,5801,17403,7.721864938735962,0.36341741761555113
5826,11654,5827,17481,7.754679203033447,0.35803129569615066
5852,11706,5853,17559,7.790459871292114,0.35017904103233377
5878,11758,5879,17637,7.82219123840332,0.3432850277616808
5904,11810,5905,17715,7.853384017944336,0.33790890550551467
5930,11862,5931,17793,7.883949041366577,0.3310126231664299
5956,11914,5957,17871,7.915164947509766,0.32562192316697747
5982,11966,5983,17949,7.951730012893677,0.3194317769539339
6008,12018,6009,18027,7.982860088348389,0.3134580888745404
6034,12070,6035,18105,8.014262199401855,0.31026669042546473
6059,12120,6060,18180,8.04348111152649,0.3013958757809405
6085,12172,6086,18258,8.074532270431519,0.29560097974763266
6111,12224,6112,18336,8.105309009552002,0.2904883282373021
6137,12276,6138,18414,8.135422945022583,0.28513431574469905
6163,12328,6164,18492,8.16641902923584,0.27949042546197234
6189,12380,6190,18570,8.19684886932373,0.27410297070389333
6215,12432,6216,18648,8.227320194244385,0.2689549259449677
6241,12484,6242,18726,8.258277893066406,0.2643893131931918
6267,12536,6268,18804,8.28885817527771,0.2601505303699696
6292,12586,6293,18879,8.318470001220703,0.2556296813726249
6318,12638,6319,18957,8.34899616241455,0.25120188370647156
6344,12690,6345,19035,8.379424095153809,0.24675192368317767
6370,12742,6371,19113,8.410167217254639,0.24266488816840592
6396,12794,6397,19191,8.440705060958862,0.23732272684583222
6422,12846,6423,19269,8.471289873123169,0.23353019644559936
6448,12898,6449,19347,8.501838207244873,0.22900756368039765
6474,12950,6475,19425,8.533529043197632,0.22534696479601735
6500,13002,6501,19503,8.564593076705933,0.22164246765498774
6526,13054,6527,19581,8.59515905380249,0.216779313194138
6551,13104,6552,19656,8.624577045440674,0.21277307556920277
6577,13156,6578,19734,8.65477204322815,0.2089080946749391
6603,13208,6604,19812,8.685086965560913,0.20526864150463098
6629,13260,6630,19890,8.71708607673645,0.2018618774618517
6655,13312,6656,19968,8.749024152755737,0.19852576664084154
6681,13364,6682,20046,8.781252145767212,0.1944866645727643
6707,13416,6708,20124,8.813515186309814,0.19108265468082664
6733,13468,6734,20202,8.846405029296875,0.18737646087186022
6759,13520,6760,20280,8.877554893493652,0.18362913660030245
6784,13570,6785,20355,8.908313274383545,0.18081628602567434
6810,13622,6811,20433,8.938575267791748,0.17728046171612277
6836,13674,6837,20511,8.978691101074219,0.17433096632760225
6862,13726,6863,20589,9.010382175445557,0.17085793207343158
6888,13778,6889,20667,9.040748119354248,0.1682536162836641
6914,13830,6915,20745,9.072538137435913,0.16524878835843992
6940,13882,6941,20823,9.104083061218262,0.1624781614237918
6966,13934,6967,20901,9.135408878326416,0.1596503243825964
6992,13986,6993,20979,9.170900106430054,0.15663714237769
7018,14038,7019,21057,9.201458930969238,0.15385398634043668
7043,14088,7044,21132,9.231657981872559,0.15123893502902774
7069,14140,7070,21210,9.263738870620728,0.14856723224352208
7095,14192,7096,21288,9.29410696029663,0.1459266517136939
7121,14244,7122,21366,9.325904846191406,0.14362365628551288
7147,14296,7148,21444,9.357009887695312,0.14089123533744896
7173,14348,7174,21522,9.387184858322144,0.13849925984618494
7199,14400,7200,21600,9.418501853942871,0.1364500228014549
7225,14452,7226,21678,9.449609994888306,0.1336749764037677
7251,14504,7252,21756,9.48045802116394,0.1312543777993369
7276,14554,7277,21831,9.511228084564209,0.12903376321617088
7302,14606,7303,21909,9.540970087051392,0.12691582243155608
7328,14658,7329,21987,9.571884155273438,0.12457272855192514
7354,14710,7355,22065,9.603344917297363,0.12234990420915892
7380,14762,7381,22143,9.633495092391968,0.11982795105268451
7406,14814,7407,22221,9.668429136276245,0.11836645006621893
7432,14866,7433,22299,9.700257062911987,0.11551027425093707
7458,14918,7459,22377,9.732004880905151,0.1135903207531328
7484,14970,7485,22455,9.765011072158813,0.11139088498134697
7510,15022,7511,22533,9.795522212982178,0.10923038313273992
7535,15072,7536,22608,9.825860261917114,0.10751843489549628
7561,15124,7562,22686,9.856727123260498,0.10563597551674775
7587,15176,7588,22764,9.887155055999756,0.10382577600159948
7613,15228,7614,22842,9.918303966522217,0.10190771639599916
7639,15280,7640,22920,9.949528217315674,0.10024671122994278
7665,15332,7666,22998,9.9810152053833,0.09821081722657254
7691,15384,7692,23076,10.012201070785522,0.09667445127365681
7717,15436,7718,23154,10.042577028274536,0.0949773691286282
7743,15488,7744,23232,10.073722839355469,0.09334166025507784
7768,15538,7769,23307,10.104496002197266,0.0914395299203079
7794,15590,7795,23385,10.135421991348267,0.09000832377398638
7820,15642,7821,23463,10.168284893035889,0.08821049298592243
7846,15694,7847,23541,10.198944091796875,0.08688784100627345
7872,15746,7873,23619,10.229673147201538,0.0852108892755723
7898,15798,7899,23697,10.260113954544067,0.08385603584338241
7924,15850,7925,23775,10.290777206420898,0.08236800755719287
7950,15902,7951,23853,10.321797847747803,0.08095640097985779
7976,15954,7977,23931,10.352734088897705,0.07955399309082622
8002,16006,8003,24009,10.384180068969727,0.07813762648243028
8027,16056,8028,24084,10.413737058639526,0.0768167213217339
8053,16108,8054,24162,10.444293975830078,0.07549074667952027
8079,16160,8080,24240,10.474820137023926,0.07427761329927307
8105,16212,8106,24318,10.505427122116089,0.07284356812783699
8131,16264,8132,24396,10.536548137664795,0.07170150689682941
8157,16316,8158,24474,10.572134971618652,0.07065221995492266
8183,16368,8184,24552,10.603354215621948,0.0693029813406838
8209,16420,8210,24630,10.633738040924072,0.06819869160460712
8235,16472,8236,24708,10.6651132106781,0.06688002723535647
8260,16522,8261,24783,10.69429612159729,0.0657233426794619
8286,16574,8287,24861,10.725342035293579,0.06466895018968444
8312,16626,8313,24939,10.7617769241333,0.06333753011460885
8338,16678,8339,25017,10.793783187866211,0.062332041616627976
8364,16730,8365,25095,10.823992013931274,0.06113743933747173
8390,16782,8391,25173,10.85550308227539,0.060142929059907146
8416,16834,8417,25251,10.888203144073486,0.059269714121342076
8442,16886,8443,25329,10.92152190208435,0.05791886051406436
8468,16938,8469,25407,10.960988998413086,0.0568997644712681
8494,16990,8495,25485,10.993587970733643,0.05590027288599231
8519,17040,8520,25560,11.02311396598816,0.05515550559607618
8545,17092,8546,25638,11.053644180297852,0.05393906585084096
8571,17144,8572,25716,11.083796977996826,0.05284338288629442
8597,17196,8598,25794,11.114490032196045,0.05193314175426167
8623,17248,8624,25872,11.144582033157349,0.05101799121325712
8649,17300,8650,25950,11.174890995025635,0.05020240031160483
8675,17352,8676,26028,11.205685138702393,0.04936630678423626
8701,17404,8702,26106,11.235870122909546,0.04854413220425613
8727,17456,8728,26184,11.26642107963562,0.04790934937500424
8752,17506,8753,26259,11.295475959777832,0.04688676432476768
8778,17558,8779,26337,11.326232194900513,0.04596797504132155
8804,17610,8805,26415,11.356861114501953,0.04516417242348325
8830,17662,8831,26493,11.386819124221802,0.044296912075537875
8856,17714,8857,26571,11.417515993118286,0.04362886433841595
8882,17766,8883,26649,11.447992086410522,0.042793640350055284
8908,17818,8909,26727,11.478531122207642,0.042059266734781886
8934,17870,8935,26805,11.509286880493164,0.041291289643709206
8960,17922,8961,26883,11.540311098098755,0.04053342329837051
8986,17974,8987,26961,11.571524143218994,0.03974861347410297
9011,18024,9012,27036,11.601087093353271,0.03917826547638015
9037,18076,9038,27114,11.631710052490234,0.03836834242167697
9063,18128,9064,27192,11.662652015686035,0.03766118792555062
9089,18180,9090,27270,11.692776918411255,0.03703914113600604
9115,18232,9116,27348,11.723703145980835,0.0363858990655217
9141,18284,9142,27426,11.754188060760498,0.0358210637641605
9167,18336,9168,27504,11.78414011001587,0.0352000306802438
9193,18388,9194,27582,11.815783977508545,0.0346211053188199
9219,18440,9220,27660,11.846233129501343,0.03400375144008194
9244,18490,9245,27735,11.875578880310059,0.033478040623435845
9270,18542,9271,27813,11.906332969665527,0.032895995827857405
9296,18594,9297,27891,11.936691999435425,0.03230258671419506
9322,18646,9323,27969,11.973550081253052,0.031799628180465334
9348,18698,9349,28047,12.004029035568237,0.031214365682330936
9374,18750,9375,28125,12.034533023834229,0.030741325615963433
9400,18802,9401,28203,12.064696073532104,0.03023488643179917
9426,18854,9427,28281,12.09466814994812,0.029666275324188973
9452,18906,9453,28359,12.1252760887146,0.02908188232743214
9478,18958,9479,28437,12.162349224090576,0.02854833405467616
9503,19008,9504,28512,12.1914381980896,0.02812304227700224
9529,19060,9530,28590,12.222298860549927,0.02746606777816396
9555,19112,9556,28668,12.252938985824585,0.027022938015306863
9581,19164,9582,28746,12.283424139022827,0.026583341293530793
9607,19216,9608,28824,12.313188076019287,0.02613677861177166
9633,19268,9634,28902,12.34334397315979,0.02569708863654796
9659,19320,9660,28980,12.374081134796143,0.025270543125884615
9685,19372,9686,29058,12.404804229736328,0.024759149780265943
9711,19424,9712,29136,12.435090065002441,0.024293315238196556
9736,19474,9737,29211,12.465342998504639,0.023931737920406704
9762,19526,9763,29289,12.494917869567871,0.023404925495242423
9788,19578,9789,29367,12.525799036026001,0.023025224281013834
9814,19630,9815,29445,12.556762218475342,0.022599532819299384
9840,19682,9841,29523,12.587041139602661,0.02226170270591865
9866,19734,9867,29601,12.617784023284912,0.021829928242937058
9892,19786,9893,29679,12.648612260818481,0.021476581578099285
9918,19838,9919,29757,12.679304122924805,0.021078265449887112
9944,19890,9945,29835,12.710097074508667,0.020740171298371024
9970,19942,9971,29913,12.74108600616455,0.020390993968476323
9995,19992,9996,29988,12.771228075027466,0.020013467702483467
10021,20044,10022,30066,12.802489042282104,0.019681002626839472
10047,20096,10048,30144,12.832722902297974,0.01932828532358144
10073,20148,10074,30222,12.86355209350586,0.019010603154697492
10099,20200,10100,30300,12.893818855285645,0.018657433395787848
10125,20252,10126,30378,12.92487096786499,0.018347040048865892
10151,20304,10152,30456,12.95596194267273,0.01801004488959279
10177,20356,10178,30534,12.986147165298462,0.017680436428236135
10203,20408,10204,30612,13.019095182418823,0.017375437133409832
10228,20458,10229,30687,13.050580978393555,0.01707532332034134
10254,20510,10255,30765,13.083285093307495,0.01677967606258335
10280,20562,10281,30843,13.115063190460205,0.01649467428603657
10306,20614,10307,30921,13.1478590965271,0.016255091361472296
10332,20666,10333,30999,13.18457293510437,0.01591705623161488
10358,20718,10359,31077,13.214852094650269,0.015661216963962943
10384,20770,10385,31155,13.244529008865356,0.015376889925391879
10410,20822,10411,31233,13.27544093132019,0.015142790237518966
10436,20874,10437,31311,13.305552959442139,0.01479123535295912
10462,20926,10463,31389,13.336405038833618,0.014563033815875315
10487,20976,10488,31464,13.375133991241455,0.014303746190421407
10513,21028,10514,31542,13.409913063049316,0.014092527382103981
10539,21080,10540,31620,13.446355104446411,0.013814872370403464
10565,21132,10566,31698,13.479172945022583,0.013590072667966524
10591,21184,10592,31776,13.513798952102661,0.013359083919795012
10617,21236,10618,31854,13.547969102859497,0.013139345458512253
10643,21288,10644,31932,13.585669994354248,0.012906688703083091
10669,21340,10670,32010,13.618137121200562,0.012691061606460607
10695,21392,10696,32088,13.651823282241821,0.012483065453807285
10720,21442,10721,32163,13.683304071426392,0.012264032322377716
10746,21494,10747,32241,13.71633505821228,0.012004634519371393
10772,21546,10773,32319,13.747781991958618,0.011827200856487252
10798,21598,10799,32397,13.779568910598755,0.011635777564379168
10824,21650,10825,32475,13.811958074569702,0.01142715072808187
10850,21702,10851,32553,13.842761993408203,0.011225133074503901
10876,21754,10877,32631,13.875174045562744,0.011041331547630762
10902,21806,10903,32709,13.906822919845581,0.01087053747050959
10928,21858,10929,32787,13.939275026321411,0.010692556481785687
10954,21910,10955,32865,13.97217583656311,0.010509707522487588
10979,21960,10980,32940,14.00613784790039,0.010356923756489778
11005,22012,11006,33018,14.037988901138306,0.010152342212450094
11031,22064,11032,33096,14.070021867752075,0.00996833453882573
11057,22116,11058,33174,14.10096001625061,0.009811577173877595
11083,22168,11084,33252,14.131911039352417,0.009657919374262747
11109,22220,11110,33330,14.1632399559021,0.009488174136322414
11135,22272,11136,33408,14.193786859512329,0.009313262999626204
11161,22324,11162,33486,14.225318908691406,0.009160491175180141
11187,22376,11188,33564,14.25690507888794,0.008970335886942848
11212,22426,11213,33639,14.285807847976685,0.008843064980851523
11238,22478,11239,33717,14.32391905784607,0.008682853099458043
11264,22530,11265,33795,14.358705043792725,0.00854350121483094
11290,22582,11291,33873,14.389219045639038,0.008414982245540159
11316,22634,11317,33951,14.420860052108765,0.0082333506205714
11342,22686,11343,34029,14.452591896057129,0.00810521157131916
11368,22738,11369,34107,14.483716249465942,0.007969246775132888
11394,22790,11395,34185,14.51593804359436,0.007830760895785716
11420,22842,11421,34263,14.547425031661987,0.007714161799299291
11446,22894,11447,34341,14.579077959060669,0.00756788392470753
11471,22944,11472,34416,14.609691858291626,0.007449795882848775
11497,22996,11498,34494,14.640176057815552,0.0072965499113024634
11523,23048,11524,34572,14.671756029129028,0.007177397455620849
11549,23100,11550,34650,14.703339099884033,0.007050978693087018
11575,23152,11576,34728,14.734235048294067,0.006932605383099144
11601,23204,11602,34806,14.766571998596191,0.006821257484261878
11627,23256,11628,34884,14.79712700843811,0.006686408589303028
11653,23308,11654,34962,14.828416109085083,0.00657920099013154
11679,23360,11680,35040,14.860100269317627,0.006461520536277021
11704,23410,11705,35115,14.889414072036743,0.006356209283126191
11730,23462,11731,35193,14.921099185943604,0.006235775411482791
11756,23514,11757,35271,14.953815221786499,0.006137127859119573
11782,23566,11783,35349,14.99067497253418,0.006024985869430566
11808,23618,11809,35427,15.022137880325317,0.005936524459002612
11834,23670,11835,35505,15.053898096084595,0.005846092722890717
11860,23722,11861,35583,15.08487606048584,0.00573886227971343
11886,23774,11887,35661,15.116288185119629,0.005639487441499114
11912,23826,11913,35739,15.154311895370483,0.005555319445988971
11938,23878,11939,35817,15.18673300743103,0.005454064652099078
11963,23928,11964,35892,15.21906304359436,0.005360395066190904
11989,23980,11990,35970,15.252618074417114,0.005257677990698539
12015,24032,12016,36048,15.284868955612183,0.005163561825611396
12041,24084,12042,36126,15.317935228347778,0.005087033223844628
12067,24136,12068,36204,15.349120140075684,0.004983408815178336
12093,24188,12094,36282,15.379763126373291,0.00488642962159247
12119,24240,12120,36360,15.411994218826294,0.004810679003981022
12145,24292,12146,36438,15.442528009414673,0.004721199541677379
12171,24344,12172,36516,15.473392963409424,0.0046527722281553
12196,24394,12197,36591,15.5031418800354,0.004565850845551722
12222,24446,12223,36669,15.534450054168701,0.0044964471441062415
12248,24498,12249,36747,15.566343069076538,0.00441222593542534
12274,24550,12275,36825,15.597445011138916,0.004342536301919608
12300,24602,12301,36903,15.62986707687378,0.004254985085935914
12326,24654,12327,36981,15.662904024124146,0.004190286872699289
12352,24706,12353,37059,15.694442987442017,0.004110031910045109
12378,24758,12379,37137,15.728109121322632,0.004048852140840609
12404,24810,12405,37215,15.7620849609375,0.003978238187073657
12430,24862,12431,37293,15.795981168746948,0.003911539194291436
12455,24912,12456,37368,15.827062129974365,0.003850522916764021
12481,24964,12482,37446,15.860130071640015,0.0037862932073267075
12507,25016,12508,37524,15.89181900024414,0.0037168048676221588
12533,25068,12534,37602,15.925425052642822,0.0036548769562614325
12559,25120,12560,37680,15.959191083908081,0.0035880679495221557
12585,25172,12586,37758,15.990777969360352,0.0035301488982213414
12611,25224,12612,37836,16.02352213859558,0.003470356710863598
12637,25276,12638,37914,16.056539058685303,0.003408599240174226
12663,25328,12664,37992,16.088608980178833,0.0033459062743759205
12688,25378,12689,38067,16.119502067565918,0.0032951458695151814
12714,25430,12715,38145,16.152495861053467,0.003236614031834506
12740,25482,12741,38223,16.189857006072998,0.003182480789860165
12766,25534,12767,38301,16.22245192527771,0.0031237987016083935
12792,25586,12793,38379,16.255038022994995,0.0030747391740533203
12818,25638,12819,38457,16.28677988052368,0.0029978725812043194
12844,25690,12845,38535,16.319273948669434,0.0029507449305583577
12870,25742,12871,38613,16.356736183166504,0.0028955946045243763
12896,25794,12897,38691,16.38817310333252,0.002848093405873442
12922,25846,12923,38769,16.420879125595093,0.002802428180075367
12947,25896,12948,38844,16.452434062957764,0.0027546552959165638
12973,25948,12974,38922,16.484699010849,0.002711363245339271
12999,26000,13000,39000,16.516448974609375,0.002656862336039012
13025,26052,13026,39078,16.54872703552246,0.0026131133471380963
13051,26104,13052,39156,16.58052706718445,0.002570924205542724
13077,26156,13078,39234,16.612727165222168,0.0025279558130932855
13103,26208,13104,39312,16.644158124923706,0.0024814658199829864
13129,26260,13130,39390,16.67659306526184,0.0024434735064460256
13155,26312,13156,39468,16.711310148239136,0.0023956342065503122
13181,26364,13182,39546,16.743946075439453,0.002358512733508178
13206,26414,13207,39621,16.77544903755188,0.002317422680562231
13232,26466,13233,39699,16.809290170669556,0.002278618679497413
13258,26518,13259,39777,16.840691089630127,0.0022392836966673713
13284,26570,13285,39855,16.873876094818115,0.002203797256811413
13310,26622,13311,39933,16.91006898880005,0.002162679286243474
13336,26674,13337,40011,16.94671320915222,0.0021293268722502035
13362,26726,13363,40089,16.98097586631775,0.002085144127931926
13388,26778,13389,40167,17.01611614227295,0.0020497139330473146
13414,26830,13415,40245,17.050270080566406,0.0020077260222706172
13439,26880,13440,40320,17.080480098724365,0.0019765827487390197
13465,26932,13466,40398,17.112277030944824,0.0019404413759502859
13491,26984,13492,40476,17.145787000656128,0.001910817721636704
13517,27036,13518,40554,17.180392026901245,0.0018808437780535314
13543,27088,13544,40632,17.213758945465088,0.0018481225050663852
13569,27140,13570,40710,17.245203018188477,0.0018186100908224034
13595,27192,13596,40788,17.27731704711914,0.0017839203208041
13621,27244,13622,40866,17.309764862060547,0.0017556195775796368
13647,27296,13648,40944,17.342955112457275,0.0017258100094750262
13673,27348,13674,41022,17.383996963500977,0.0016955061553289852
13698,27398,13699,41097,17.420538902282715,0.0016685563064129383
13724,27450,13725,41175,17.45999503135681,0.001641278772581245
13750,27502,13751,41253,17.494537115097046,0.0016147518276738992
13776,27554,13777,41331,17.52865695953369,0.0015822476742641811
13802,27606,13803,41409,17.566219091415405,0.0015565303061748637
13828,27658,13829,41487,17.598275184631348,0.0015297767223501069
13854,27710,13855,41565,17.63078808784485,0.0015027839568801937
13880,27762,13881,41643,17.665621042251587,0.001480048818962132
13906,27814,13907,41721,17.69742703437805,0.0014538053601427237
13931,27864,13932,41796,17.729629039764404,0.001432686805060257
13957,27916,13958,41874,17.76350998878479,0.0014072575995669467
13983,27968,13984,41952,17.797078132629395,0.0013762775458872056
14009,28020,14010,42030,17.831095218658447,0.0013568801160772637
14035,28072,14036,42108,17.86595606803894,0.001337236535619013
14061,28124,14062,42186,17.89841103553772,0.0013123803050802962
14087,28176,14088,42264,17.933094024658203,0.0012859949274570681
14113,28228,14114,42342,17.967563152313232,0.0012576245312629908
14139,28280,14140,42420,18.000375032424927,0.0012368451411930437
14165,28332,14166,42498,18.033594846725464,0.0012158557126440428
14190,28382,14191,42573,18.066556930541992,0.0011966560147129712
14216,28434,14217,42651,18.09949493408203,0.0011789361757337247
14242,28486,14243,42729,18.13431406021118,0.0011584958865569206
14268,28538,14269,42807,18.16724705696106,0.001141411858156971
14294,28590,14295,42885,18.201123237609863,0.0011202227985904756
14320,28642,14321,42963,18.23424792289734,0.0011022361328514307
14346,28694,14347,43041,18.2671480178833,0.0010838162270374596
14372,28746,14373,43119,18.30093216896057,0.001064037906530757
14398,28798,14399,43197,18.333919048309326,0.0010450978261360433
14423,28848,14424,43272,18.370234966278076,0.0010274209313365645
14449,28900,14450,43350,18.405349016189575,0.001009280687071623
14475,28952,14476,43428,18.43839693069458,0.0009924006051278411
14501,29004,14502,43506,18.472310066223145,0.0009788924076019612
14527,29056,14528,43584,18.506025075912476,0.0009580769183230586
14553,29108,14554,43662,18.538919925689697,0.0009406149125652519
14579,29160,14580,43740,18.572550058364868,0.000926533401298002
14605,29212,14606,43818,18.60586404800415,0.0009110320947911532
14631,29264,14632,43896,18.638272047042847,0.0008970984659981696
14657,29316,14658,43974,18.672482013702393,0.0008784171370734839
14682,29366,14683,44049,18.70553493499756,0.0008654957712224132
14708,29418,14709,44127,18.73911190032959,0.0008512253687058546
14734,29470,14735,44205,18.772320985794067,0.0008373083999231312
14760,29522,14761,44283,18.806869983673096,0.0008213506112042523
14786,29574,14787,44361,18.839653968811035,0.0008067576836765511
14812,29626,14813,44439,18.873560190200806,0.000792709897154964
14838,29678,14839,44517,18.905848026275635,0.0007803520857123658
14864,29730,14865,44595,18.938150882720947,0.0007652168468439413
14890,29782,14891,44673,18.971673250198364,0.0007539618085274924
14915,29832,14916,44748,19.003669023513794,0.0007404363559544436
14941,29884,14942,44826,19.036749124526978,0.0007270728746107125
14967,29936,14968,44904,19.069746017456055,0.0007140752090890601
14993,29988,14994,44982,19.102909088134766,0.0007031706185216535
15019,30040,15020,45060,19.13551902770996,0.0006900519621240164
15045,30092,15046,45138,19.168477058410645,0.0006797213910658684
15071,30144,15072,45216,19.20217514038086,0.00066697577267405
15097,30196,15098,45294,19.235471963882446,0.0006560787992384576
15123,30248,15124,45372,19.26852297782898,0.0006433095808233702
15149,30300,15150,45450,19.30143904685974,0.000633780734233369
15174,30350,15175,45525,19.334988117218018,0.0006222038973646704
15200,30402,15201,45603,19.373268127441406,0.0006128595854306695
15226,30454,15227,45681,19.410969257354736,0.000600846615611772
15252,30506,15253,45759,19.44485306739807,0.0005919546129007358
15278,30558,15279,45837,19.47978711128235,0.0005815335188117388
15304,30610,15305,45915,19.51742911338806,0.0005720944028553276
15330,30662,15331,45993,19.554498195648193,0.0005601757876547708
15356,30714,15357,46071,19.589177131652832,0.0005520507027085841
15382,30766,15383,46149,19.626582145690918,0.00054274747776617
15407,30816,15408,46224,19.658899068832397,0.0005336890841363129
15433,30868,15434,46302,19.69252109527588,0.0005241264302640047
15459,30920,15460,46380,19.726678133010864,0.0005157512883897653
15485,30972,15486,46458,19.76072096824646,0.0005075492072137422
15511,31024,15512,46536,19.7934250831604,0.0004981384769280339
15537,31076,15538,46614,19.826837062835693,0.0004890732818694232
15563,31128,15564,46692,19.860857248306274,0.00048097141382186237
15589,31180,15590,46770,19.894383192062378,0.0004727696658619607
15615,31232,15616,46848,19.929664134979248,0.00046507855540767196
15641,31284,15642,46926,19.963623046875,0.00045768465827222826
15666,31334,15667,47001,19.99545192718506,0.0004498248670188332
15692,31386,15693,47079,20.029343128204346,0.0004406004142083475
15718,31438,15719,47157,20.06278395652771,0.0004336775575666252
15744,31490,15745,47235,20.095980167388916,0.0004246105698939573
15770,31542,15771,47313,20.128690004348755,0.00041815239183051744
15796,31594,15797,47391,20.162756204605103,0.000409532020057668
15822,31646,15823,47469,20.196599006652832,0.0004010824964097992
15848,31698,15849,47547,20.230576038360596,0.0003939326740010074
15874,31750,15875,47625,20.263972282409668,0.0003877538731558161
15899,31800,15900,47700,20.296192169189453,0.00037978768443736044
15925,31852,15926,47778,20.330169200897217,0.000373302116031482
15951,31904,15952,47856,20.3631591796875,0.0003670270197062564
15977,31956,15978,47934,20.394917964935303,0.0003595786688492808
16003,32008,16004,48012,20.4274001121521,0.0003531611300786608
16029,32060,16030,48090,20.46025514602661,0.00034789733990692184
16055,32112,16056,48168,20.49196195602417,0.0003426742314331932
16081,32164,16082,48246,20.529855012893677,0.00033623242302383005
16107,32216,16108,48324,20.565150022506714,0.0003300533549008833
16133,32268,16134,48402,20.597334146499634,0.0003246704164894254
16158,32318,16159,48477,20.62870502471924,0.0003193652048594231
16184,32370,16185,48555,20.662626028060913,0.00031417050752224895
16210,32422,16211,48633,20.694857120513916,0.00030657097886432894
16236,32474,16237,48711,20.72712802886963,0.00030203626283764606
16262,32526,16263,48789,20.760184049606323,0.00029660940367648436
16288,32578,16289,48867,20.792006015777588,0.00029182425237195275
16314,32630,16315,48945,20.82429003715515,0.0002860978212311238
16340,32682,16341,49023,20.856747150421143,0.00028128496830959193
16366,32734,16367,49101,20.888381958007812,0.00027635744970666565
16391,32784,16392,49176,20.920006036758423,0.0002723520291283421
16417,32836,16418,49254,20.95384407043457,0.00026721196445578244
16443,32888,16444,49332,20.98541021347046,0.000262622246623323
16469,32940,16470,49410,21.01759099960327,0.00025775804124350543
16495,32992,16496,49488,21.049934148788452,0.00025361646521560033
16521,33044,16522,49566,21.081594944000244,0.00024917842074501095
16547,33096,16548,49644,21.11382508277893,0.00024506939109869563
16573,33148,16574,49722,21.145965099334717,0.00024062748082087637
16599,33200,16600,49800,21.177900075912476,0.00023653398545775417
16625,33252,16626,49878,21.210937976837158,0.00023226828648148512
16650,33302,16651,49953,21.241266012191772,0.00022855755548789602
16676,33354,16677,50031,21.27336812019348,0.0002248712985419843
16702,33406,16703,50109,21.305028200149536,0.00022111702924121346
16728,33458,16729,50187,21.337467908859253,0.00021796760950110183
16754,33510,16755,50265,21.368711948394775,0.00021296670968240505
16780,33562,16781,50343,21.400701999664307,0.00020875049949609092
16806,33614,16807,50421,21.432175159454346,0.00020542755726182804
16832,33666,16833,50499,21.46498417854309,0.00020198928984882514
16858,33718,16859,50577,21.497062921524048,0.0001991035236414973
16883,33768,16884,50652,21.528600215911865,0.00019613767244663904
16909,33820,16910,50730,21.561717987060547,0.00019253902360105712
16935,33872,16936,50808,21.593322038650513,0.0001889501857021969
16961,33924,16962,50886,21.628345251083374,0.00018625712277753337
16987,33976,16988,50964,21.663854122161865,0.00018310947882582695
17013,34028,17014,51042,21.698981046676636,0.00017975032835693128
17039,34080,17040,51120,21.733476161956787,0.00017614666148801916
17065,34132,17066,51198,21.770212173461914,0.00017356420437408815
17091,34184,17092,51276,21.80280089378357,0.00017055847820302006
17117,34236,17118,51354,21.83460307121277,0.0001676049846537353
17142,34286,17143,51429,21.866401195526123,0.00016514305718828837
17168,34338,17169,51507,21.898977041244507,0.00016229607365403353
17194,34390,17195,51585,21.931533098220825,0.00015957859784521133
17220,34442,17221,51663,21.96495008468628,0.0001569298648291806
17246,34494,17247,51741,21.997112035751343,0.00015410941239224485
17272,34546,17273,51819,22.029680967330933,0.0001512229010813826
17298,34598,17299,51897,22.06237006187439,0.0001488838669274628
17324,34650,17325,51975,22.09410786628723,0.00014636542243806616
17350,34702,17351,52053,22.12656307220459,0.00014364376545472624
17375,34752,17376,52128,22.156574964523315,0.00014064075628539285
17401,34804,17402,52206,22.188540935516357,0.00013861914851531765
17427,34856,17428,52284,22.22163200378418,0.00013576760875366745
17453,34908,17454,52362,22.253568172454834,0.00013368190866458463
17479,34960,17480,52440,22.288538217544556,0.0001314727325052445
17505,35012,17506,52518,22.321282148361206,0.00012880786641744635
17531,35064,17532,52596,22.353265047073364,0.00012624313887954486
17557,35116,17558,52674,22.38567090034485,0.00012417779794304806
17583,35168,17584,52752,22.418192863464355,0.00012181891145246482
17609,35220,17610,52830,22.450764179229736,0.00011986526521923224
17634,35270,17635,52905,22.481189012527466,0.00011771791332648718
17660,35322,17661,52983,22.51244020462036,0.00011578313569771126
17686,35374,17687,53061,22.544515132904053,0.0001137265238639884
17712,35426,17713,53139,22.577373027801514,0.00011200072185602039
17738,35478,17739,53217,22.60900092124939,0.00010997036986282183
17764,35530,17765,53295,22.64039707183838,0.0001080382829741211
17790,35582,17791,53373,22.673527002334595,0.00010620553302942426
17816,35634,17817,53451,22.70666193962097,0.00010443406745253014
17842,35686,17843,53529,22.737812042236328,0.0001026604508069795
17867,35736,17868,53604,22.769157886505127,0.00010095425341205555
17893,35788,17894,53682,22.80122709274292,9.937124002590281e-05
17919,35840,17920,53760,22.83355402946472,9.798083533496538e-05
17945,35892,17946,53838,22.86468195915222,9.566887274559122e-05
17971,35944,17972,53916,22.896272897720337,9.408141170297313e-05
17997,35996,17998,53994,22.928390979766846,9.245000194368913e-05
18023,36048,18024,54072,22.9624240398407,9.084858356800396e-05
18049,36100,18050,54150,22.99393582344055,8.940538407387066e-05
18075,36152,18076,54228,23.02626895904541,8.776112304076378e-05
18101,36204,18102,54306,23.059298038482666,8.627798865745717e-05
18126,36254,18127,54381,23.08929204940796,8.48965439672611e-05
18152,36306,18153,54459,23.12153196334839,8.339927489942056e-05
18178,36358,18179,54537,23.153871059417725,8.202980768601265e-05
18204,36410,18205,54615,23.18528699874878,8.042582089728967e-05
18230,36462,18231,54693,23.217693090438843,7.915411242720438e-05
18256,36514,18257,54771,23.249068021774292,7.798577803441731e-05
18282,36566,18283,54849,23.281136989593506,7.670317904739932e-05
18308,36618,18309,54927,23.31364417076111,7.494939063690254e-05
18334,36670,18335,55005,23.345088005065918,7.361170901276637e-05
18359,36720,18360,55080,23.37605094909668,7.24123977988711e-05
18385,36772,18386,55158,23.408290147781372,7.109099738045188e-05
18411,36824,18412,55236,23.439574003219604,6.97894703307611e-05
18437,36876,18438,55314,23.472261905670166,6.861415931780357e-05
18463,36928,18464,55392,23.504162073135376,6.751249793524039e-05
18489,36980,18490,55470,23.536739110946655,6.630114842209878e-05
18515,37032,18516,55548,23.5688898563385,6.533378291351255e-05
18541,37084,18542,55626,23.60118818283081,6.420158740638726e-05
18567,37136,18568,55704,23.63349986076355,6.293739750162786e-05
18593,37188,18594,55782,23.665749073028564,6.184569144807028e-05
18618,37238,18619,55857,23.696133852005005,6.0689494489452045e-05
18644,37290,18645,55935,23.72866415977478,5.961065380688524e-05
18670,37342,18671,56013,23.75974202156067,5.857711562384793e-05
18696,37394,18697,56091,23.79300308227539,5.7545357208255155e-05
18722,37446,18723,56169,23.828017950057983,5.6461845247213205e-05
18748,37498,18749,56247,23.862712144851685,5.556156861530326e-05
18774,37550,18775,56325,23.897247076034546,5.4731140608055284e-05
18800,37602,18801,56403,23.93175196647644,5.382215908866783e-05
18826,37654,18827,56481,23.96419095993042,5.2915868195668736e-05
18851,37704,18852,56556,23.995087146759033,5.1912887215621595e-05
18877,37756,18878,56634,24.027705907821655,5.111762300202827e-05
18903,37808,18904,56712,24.060132265090942,5.0376209969726915e-05
18929,37860,18930,56790,24.091233015060425,4.9419330252931104e-05
18955,37912,18956,56868,24.122716903686523,4.8371384536949336e-05
18981,37964,18982,56946,24.155609130859375,4.765074254464707e-05
19007,38016,19008,57024,24.18674898147583,4.674921547120903e-05
19033,38068,19034,57102,24.219347953796387,4.600112367825204e-05
19059,38120,19060,57180,24.251133918762207,4.5085550823387166e-05
19085,38172,19086,57258,24.282383918762207,4.42265148876686e-05
19110,38222,19111,57333,24.312673091888428,4.348735558323824e-05
19136,38274,19137,57411,24.343836069107056,4.277742311842303e-05
19162,38326,19163,57489,24.374540090560913,4.200563512313238e-05
19188,38378,19189,57567,24.40586495399475,4.13318133496432e-05
19214,38430,19215,57645,24.43804121017456,4.054839291711687e-05
19240,38482,19241,57723,24.469967126846313,3.971561989146721e-05
19266,38534,19267,57801,24.50182008743286,3.9115031768233166e-05
19292,38586,19293,57879,24.53355121612549,3.8473109384540294e-05
19318,38638,19319,57957,24.56610417366028,3.792988536588382e-05
19343,38688,19344,58032,24.59641408920288,3.7094285971761565e-05
19369,38740,19370,58110,24.628525018692017,3.6474966236710316e-05
19395,38792,19396,58188,24.661184072494507,3.5841492945110076e-05
19421,38844,19422,58266,24.692875146865845,3.5164323094249994e-05
19447,38896,19448,58344,24.725085973739624,3.4589957408570626e-05
19473,38948,19474,58422,24.757659912109375,3.403075129426725e-05
19499,39000,19500,58500,24.788881063461304,3.340468265378149e-05
19525,39052,19526,58578,24.820831060409546,3.278047245203197e-05
19551,39104,19552,58656,24.852609157562256,3.2265038271361846e-05
19577,39156,19578,58734,24.8844051361084,3.167471663800825e-05
19602,39206,19603,58809,24.91564917564392,3.1186903356683615e-05
19628,39258,19629,58887,24.947247982025146,3.061799986880942e-05
19654,39310,19655,58965,24.98053503036499,3.0093367058725562e-05
19680,39362,19681,59043,25.012463092803955,2.9552527394116623e-05
19706,39414,19707,59121,25.044109106063843,2.9058033533146954e-05
19732,39466,19733,59199,25.076029062271118,2.8526927394523227e-05
19758,39518,19759,59277,25.107373237609863,2.8070367989130318e-05
19784,39570,19785,59355,25.138806104660034,2.7519663717612275e-05
19810,39622,19811,59433,25.17009997367859,2.7089129616797436e-05
19835,39672,19836,59508,25.20008087158203,2.662818008047907e-05
19861,39724,19862,59586,25.23134708404541,2.6185044134763302e-05
19887,39776,19888,59664,25.262574195861816,2.563856673987175e-05
19913,39828,19914,59742,25.29349398612976,2.5232223038074153e-05
19939,39880,19940,59820,25.325413942337036,2.4751777004894393e-05
19965,39932,19966,59898,25.357008934020996,2.4348534452656168e-05
19991,39984,19992,59976,25.388087034225464,2.393093882346875e-05
20017,40036,20018,60054,25.419734001159668,2.350764498260105e-05
20043,40088,20044,60132,25.452057123184204,2.309686101398256e-05
20069,40140,20070,60210,25.484391927719116,2.2626115082857723e-05
20094,40190,20095,60285,25.514739990234375,2.225254331733595e-05
20120,40242,20121,60363,25.546425104141235,2.1857551701032207e-05
20146,40294,20147,60441,25.579647064208984,2.149140448182152e-05
20172,40346,20173,60519,25.613224029541016,2.1168064563426015e-05
20198,40398,20199,60597,25.645785093307495,2.0781482817255892e-05
20224,40450,20225,60675,25.67806601524353,2.0419873862920213e-05
20250,40502,20251,60753,25.710953950881958,2.0022770399918954e-05
20276,40554,20277,60831,25.742909908294678,1.9725864831343642e-05
20302,40606,20303,60909,25.776950120925903,1.9366018591426837e-05
20327,40656,20328,60984,25.809123039245605,1.905482952224702e-05
20353,40708,20354,61062,25.839969158172607,1.8716415297603817e-05
20379,40760,20380,61140,25.87345600128174,1.8382160192231822e-05
20405,40812,20406,61218,25.90627408027649,1.8097475503964233e-05
20431,40864,20432,61296,25.940934896469116,1.7804077742766822e-05
20457,40916,20458,61374,25.976934909820557,1.7546697108627995e-05
20483,40968,20484,61452,26.0127911567688,1.7214119793607097e-05
20509,41020,20510,61530,26.04624104499817,1.6949267205745855e-05
20535,41072,20536,61608,26.079782009124756,1.663240664129262e-05
20561,41124,20562,61686,26.11162805557251,1.6312739262502873e-05
20586,41174,20587,61761,26.141690969467163,1.6042366723922896e-05
20612,41226,20613,61839,26.17421293258667,1.5782168020450626e-05
20638,41278,20639,61917,26.206942081451416,1.5498265270252887e-05
20664,41330,20665,61995,26.23791003227234,1.5238915580084722e-05
20690,41382,20691,62073,26.270101070404053,1.4956110248931509e-05
20716,41434,20717,62151,26.301403045654297,1.4686063764202117e-05
20742,41486,20743,62229,26.332777976989746,1.4409842833629227e-05
20768,41538,20769,62307,26.36825919151306,1.4172841247273027e-05
20794,41590,20795,62385,26.40144419670105,1.3929108831689518e-05
20819,41640,20820,62460,26.430752992630005,1.3698751445190283e-05
20845,41692,20846,62538,26.46259093284607,1.3436642689157452e-05
20871,41744,20872,62616,26.49243712425232,1.3211187820161285e-05
20897,41796,20898,62694,26.524386167526245,1.2951835060448502e-05
20923,41848,20924,62772,26.556143283843994,1.2737311976707133e-05
20949,41900,20950,62850,26.58753204345703,1.2505927998063271e-05
20975,41952,20976,62928,26.61952018737793,1.2326378396210202e-05
21001,42004,21002,63006,26.65385913848877,1.2037769806738652e-05
21027,42056,21028,63084,26.68629002571106,1.179014952867874e-05
21053,42108,21054,63162,26.718799114227295,1.159461464794731e-05
21078,42158,21079,63237,26.75181293487549,1.1380250725778751e-05
21104,42210,21105,63315,26.78491497039795,1.1153421496601368e-05
21130,42262,21131,63393,26.81762409210205,1.0961390444208519e-05
21156,42314,21157,63471,26.850370168685913,1.074154670277494e-05
21182,42366,21183,63549,26.88209104537964,1.0563505497884762e-05
21208,42418,21209,63627,26.913472175598145,1.0393869956715207e-05
21234,42470,21235,63705,26.94416904449463,1.0213098448730307e-05
21260,42522,21261,63783,26.97500491142273,1.0016055966843851e-05
21286,42574,21287,63861,27.00599503517151,9.854829954747402e-06
21311,42624,21312,63936,27.03641700744629,9.670447298049112e-06
21337,42676,21338,64014,27.06831121444702,9.466421261095093e-06
21363,42728,21364,64092,27.098660945892334,9.29859788811882e-06
21389,42780,21390,64170,27.129671096801758,9.129918453254504e-06
21415,42832,21416,64248,27.160601139068604,8.946463253778347e-06
21441,42884,21442,64326,27.191213130950928,8.76481783507188e-06
21467,42936,21468,64404,27.222373962402344,8.568847306378302e-06
21493,42988,21494,64482,27.257911205291748,8.424915677096578e-06
21519,43040,21520,64560,27.288227081298828,8.269112186098937e-06
21545,43092,21546,64638,27.323076963424683,8.136678957271215e-06
21570,43142,21571,64713,27.35242199897766,7.967171882228286e-06
21596,43194,21597,64791,27.383033275604248,7.831996299501043e-06
21622,43246,21623,64869,27.41522216796875,7.688757932555745e-06
21648,43298,21649,64947,27.445794105529785,7.557011372227862e-06
21674,43350,21675,65025,27.477864980697632,7.4350333534312085e-06
21700,43402,21701,65103,27.51306390762329,7.295066211554513e-06
21726,43454,21727,65181,27.544484853744507,7.141498940654856e-06
21752,43506,21753,65259,27.57526206970215,7.001655148997088e-06
21778,43558,21779,65337,27.606364011764526,6.883322839712491e-06
21804,43610,21805,65415,27.637315034866333,6.751334126420261e-06
21829,43660,21830,65490,27.66739320755005,6.644710310865776e-06
21855,43712,21856,65568,27.697923183441162,6.515463724099391e-06
21881,43764,21882,65646,27.728703022003174,6.383901336448616e-06
21907,43816,21908,65724,27.76020908355713,6.265399406402139e-06
21933,43868,21934,65802,27.79248809814453,6.143393306956568e-06
21959,43920,21960,65880,27.826112031936646,6.031316047483415e-06
21985,43972,21986,65958,27.859282970428467,5.924355605202436e-06
22011,44024,22012,66036,27.892917156219482,5.821351123813656e-06
22037,44076,22038,66114,27.926521062850952,5.713848963750934e-06
22062,44126,22063,66189,27.958402156829834,5.611108917946694e-06
22088,44178,22089,66267,27.989854097366333,5.494281140272506e-06
22114,44230,22115,66345,28.021735906600952,5.407694743553293e-06
22140,44282,22141,66423,28.05405020713806,5.301464966578351e-06
22166,44334,22167,66501,28.088818073272705,5.206987225392368e-06
22192,44386,22193,66579,28.131327152252197,5.115011845191475e-06
22218,44438,22219,66657,28.16543483734131,5.0145768000220414e-06
22244,44490,22245,66735,28.198216915130615,4.915693239126995e-06
22270,44542,22271,66813,28.232664108276367,4.828286819247296e-06
22296,44594,22297,66891,28.26366114616394,4.7446378630411346e-06
22321,44644,22322,66966,28.29282522201538,4.671740612138819e-06
22347,44696,22348,67044,28.324196100234985,4.571311137624434e-06
22373,44748,22374,67122,28.355286121368408,4.4723226437781705e-06
22399,44800,22400,67200,28.385683059692383,4.391114998725243e-06
22425,44852,22426,67278,28.416927099227905,4.302809088585491e-06
22451,44904,22452,67356,28.44733214378357,4.22887774220726e-06
22477,44956,22478,67434,28.479076862335205,4.140867304158746e-06
22503,45008,22504,67512,28.514111042022705,4.068127623213513e-06
22529,45060,22530,67590,28.550308227539062,4.005916821370192e-06
22554,45110,22555,67665,28.596687078475952,3.916299306183646e-06
22580,45162,22581,67743,28.635507106781006,3.839096166302625e-06
22606,45214,22607,67821,28.673890113830566,3.7722295473940903e-06
22632,45266,22633,67899,28.71074628829956,3.703553488776379e-06
22658,45318,22659,67977,28.758610010147095,3.6280893027651473e-06
22684,45370,22685,68055,28.818695068359375,3.5515275840225513e-06
22710,45422,22711,68133,28.878320932388306,3.488090214887052e-06
22736,45474,22737,68211,28.91875195503235,3.4222997555843904e-06
22762,45526,22763,68289,28.971123933792114,3.3582855394342914e-06
22788,45578,22789,68367,29.006953954696655,3.2919856494117994e-06
22813,45628,22814,68442,29.039157152175903,3.2225281074715895e-06
22839,45680,22840,68520,29.07364797592163,3.156274146931537e-06
22865,45732,22866,68598,29.111225843429565,3.1005556593299843e-06
22891,45784,22892,68676,29.144922971725464,3.0335565952555044e-06
22917,45836,22918,68754,29.182029008865356,2.977498297696002e-06
22943,45888,22944,68832,29.21767497062683,2.9200780318205943e-06
22969,45940,22970,68910,29.252753973007202,2.858090851987072e-06
22995,45992,22996,68988,29.288986921310425,2.794861416077765e-06
23021,46044,23022,69066,29.326136112213135,2.7346633260094677e-06
23046,46094,23047,69141,29.36091899871826,2.6780809321280685e-06
23072,46146,23073,69219,29.39700412750244,2.629160235301242e-06
23098,46198,23099,69297,29.43955111503601,2.5768873683773563e-06
23124,46250,23125,69375,29.479537963867188,2.5270014702982735e-06
23150,46302,23151,69453,29.518079042434692,2.4734132466619485e-06
23176,46354,23177,69531,29.555366039276123,2.4154541051757406e-06
23202,46406,23203,69609,29.587049961090088,2.3677886247241986e-06
23228,46458,23229,69687,29.619357109069824,2.3305319700739346e-06
23254,46510,23255,69765,29.65213108062744,2.2697624899592483e-06
23280,46562,23281,69843,29.683940887451172,2.221603494945157e-06
23305,46612,23306,69918,29.71599006652832,2.1781587520308676e-06
23331,46664,23332,69996,29.74809193611145,2.1305742166077835e-06
23357,46716,23358,70074,29.782469034194946,2.0864955558863585e-06
23383,46768,23384,70152,29.81895613670349,2.0401610072440235e-06
23409,46820,23410,70230,29.851744174957275,1.9995359252789058e-06
23435,46872,23436,70308,29.88494896888733,1.957455765477789e-06
23461,46924,23462,70386,29.918181896209717,1.920405793498503e-06
23487,46976,23488,70464,29.950226068496704,1.879597448350978e-06
23513,47028,23514,70542,29.987940073013306,1.840377763073775e-06
23538,47078,23539,70617,30.021027088165283,1.8020361949311337e-06
23564,47130,23565,70695,30.065834045410156,1.7558055560584762e-06
23590,47182,23591,70773,30.104421854019165,1.7130890910266316e-06
23616,47234,23617,70851,30.15819025039673,1.6743888409109786e-06
23642,47286,23643,70929,30.209542989730835,1.639341007830808e-06
23668,47338,23669,71007,30.260426998138428,1.5967901845215238e-06
23694,47390,23695,71085,30.295520067214966,1.5659148857594118e-06
23720,47442,23721,71163,30.331125020980835,1.5309266245822073e-06
23746,47494,23747,71241,30.36556601524353,1.4914692201273283e-06
23772,47546,23773,71319,30.3988139629364,1.4584801419914584e-06
23797,47596,23798,71394,30.42951512336731,1.4292339756138972e-06
23823,47648,23824,71472,30.4632670879364,1.393855995956983e-06
23849,47700,23850,71550,30.49472427368164,1.3621984180645086e-06
23875,47752,23876,71628,30.526526927947998,1.3333291235539946e-06
23901,47804,23902,71706,30.55902600288391,1.30162914047105e-06
23927,47856,23928,71784,30.590593099594116,1.273122506972868e-06
23953,47908,23954,71862,30.622488021850586,1.2417161769917584e-06
23979,47960,23980,71940,30.654165029525757,1.212790266436059e-06
24005,48012,24006,72018,30.685538053512573,1.183671429316746e-06
24030,48062,24031,72093,30.716930150985718,1.157612246061035e-06
24056,48114,24057,72171,30.749495029449463,1.13179476102232e-06
24082,48166,24083,72249,30.78168511390686,1.1052758281948627e-06
24108,48218,24109,72327,30.81438708305359,1.0723682635216392e-06
24134,48270,24135,72405,30.845826148986816,1.0476088618815993e-06
24160,48322,24161,72483,30.877935886383057,1.0210823120360146e-06
24186,48374,24187,72561,30.909879207611084,9.944538987838314e-07
24212,48426,24213,72639,30.94123601913452,9.684745236882009e-07
24238,48478,24239,72717,30.97362518310547,9.465003358855029e-07
24264,48530,24265,72795,31.005450010299683,9.169284567178693e-07
24289,48580,24290,72870,31.036245107650757,8.933877779782051e-07
24315,48632,24316,72948,31.068325996398926,8.718997150936048e-07
24341,48684,24342,73026,31.100815057754517,8.500346666551195e-07
24367,48736,24368,73104,31.132527828216553,8.261747552751331e-07
24393,48788,24394,73182,31.170735120773315,8.044958121899981e-07
24419,48840,24420,73260,31.202575206756592,7.812500371073838e-07
24445,48892,24446,73338,31.234498023986816,7.618443760293303e-07
24471,48944,24472,73416,31.266802072525024,7.407340945064789e-07
24497,48996,24498,73494,31.29812788963318,7.182901526903152e-07
24522,49046,24523,73569,31.328931093215942,6.978056035222835e-07
24548,49098,24549,73647,31.36557102203369,6.803019232393126e-07
24574,49150,24575,73725,31.397248029708862,6.60963678456028e-07
24600,49202,24601,73803,31.429153203964233,6.428820142900804e-07
24626,49254,24627,73881,31.4614360332489,6.245109034352936e-07
24652,49306,24653,73959,31.49251627922058,6.063894488761434e-07
24678,49358,24679,74037,31.525731086730957,5.861014642505324e-07
24704,49410,24705,74115,31.557834148406982,5.678460865965462e-07
24730,49462,24731,74193,31.588830947875977,5.501856321643572e-07
24756,49514,24757,74271,31.62035608291626,5.317201612342615e-07
24781,49564,24782,74346,31.65095806121826,5.158362910151482e-07
24807,49616,24808,74424,31.68239688873291,4.989358330931282e-07
24833,49668,24834,74502,31.71449303627014,4.838346967517282e-07
24859,49720,24860,74580,31.74561905860901,4.692857373811421e-07
24885,49772,24886,74658,31.778218030929565,4.528282033788855e-07
24911,49824,24912,74736,31.810578107833862,4.2581200432323385e-07
24937,49876,24938,74814,31.842052221298218,4.123734242966748e-07
24963,49928,24964,74892,31.87377119064331,3.973790398958954e-07
24989,49980,24990,74970,31.905500888824463,3.8015650716261007e-07
25014,50030,25015,75045,31.93712592124939,3.6362507671583444e-07
25040,50082,25041,75123,31.969285011291504,3.503733978504897e-07
25066,50134,25067,75201,32.000710010528564,3.370250851730816e-07
25092,50186,25093,75279,32.03239822387695,3.189474000464543e-07
25118,50238,25119,75357,32.064424991607666,3.074263759117457e-07
25144,50290,25145,75435,32.09587788581848,2.9265936518640956e-07
25170,50342,25171,75513,32.1274151802063,2.806186785164755e-07
25196,50394,25197,75591,32.1604528427124,2.6791701657202793e-07
25222,50446,25223,75669,32.19258093833923,2.5538702175254e-07
25248,50498,25249,75747,32.22501516342163,2.415548578937887e-07
25273,50548,25274,75822,32.255680084228516,2.2963467927183956e-07
25299,50600,25300,75900,32.28741788864136,2.186054643971147e-07
25325,50652,25326,75978,32.31970691680908,2.0620791474357247e-07
25351,50704,25352,76056,32.351582050323486,1.965318006114103e-07
25377,50756,25378,76134,32.388777017593384,1.834591785154771e-07
25403,50808,25404,76212,32.423717975616455,1.7281399777857587e-07
25429,50860,25430,76290,32.45933389663696,1.6034198324632598e-07
25455,50912,25456,76368,32.4913969039917,1.510413767391583e-07
25481,50964,25482,76446,32.526543855667114,1.396880406900891e-07
25506,51014,25507,76521,32.563157081604004,1.2865132248407463e-07
25532,51066,25533,76599,32.59444999694824,1.191674527944997e-07
25558,51118,25559,76677,32.62686491012573,1.1406268640712369e-07
25584,51170,25585,76755,32.659334897994995,9.815710200200556e-08
25610,51222,25611,76833,32.69051003456116,8.64830553837237e-08
25636,51274,25637,76911,32.72359108924866,7.685571290494408e-08
25662,51326,25663,76989,32.755436182022095,6.954621767363278e-08
25688,51378,25689,77067,32.7870659828186,5.97801772528328e-08
25714,51430,25715,77145,32.819663286209106,5.122092261444777e-08
25740,51482,25741,77223,32.85837912559509,4.1632574721006677e-08
25765,51532,25766,77298,32.88984990119934,3.353909505676711e-08
25791,51584,25792,77376,32.924575090408325,2.540116383897839e-08
25817,51636,25818,77454,32.9577260017395,1.8109062693838496e-08
25843,51688,25844,77532,32.988577127456665,8.459892342216335e-09
25869,51740,25870,77610,33.02084803581238,8.503775461576879e-11


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0005269050598144531,2181.2938132599165
1001,2003,2002,4005,0.846794843673706,44.348860614599744
2002,4005,4004,8009,1.651149034500122,42.70063180611464
3003,6007,6006,12013,2.4800140857696533,41.168996973026196
4004,8009,8008,16017,3.480733871459961,39.74206310087607
5005,10011,10010,20021,4.483521938323975,38.41004779718355
6006,12013,12012,24025,5.221987009048462,37.164448983126476
7007,14015,14014,28029,5.988049745559692,35.99760366567284
8008,16017,16016,32033,6.831360816955566,34.902471575462414
9009,18019,18018,36037,7.552431106567383,33.872542806958336
10010,20021,20020,40041,8.32486081123352,32.90180687460929
11011,22023,22022,44045,9.032744884490967,31.984745863677517
12012,24025,24024,48049,9.78105092048645,31.11633127426262
13013,26027,26026,52053,10.633514881134033,30.29201507749076
14014,28029,28028,56057,11.476765871047974,29.507712053032492
15015,30031,30030,60061,12.202636957168579,28.75977398425357
16016,32033,32032,64065,12.939412832260132,28.04495782384788
17017,34035,34034,68069,13.64516806602478,27.360390316515804
18018,36037,36036,72073,14.372004985809326,26.70353133521121
19019,38039,38038,76077,15.072341918945312,26.07213770811404
20020,40041,40040,80081,15.74144983291626,25.464228788021728
21021,42043,42042,84085,16.445328950881958,24.878054546039948
22022,44045,44044,88089,17.13111686706543,24.312066596662817
23023,46047,46046,92093,17.816312074661255,23.764892286299073
24024,48049,48048,96097,18.494430780410767,23.235311790254627
25025,50051,50050,100101,19.183851957321167,22.722238046277653
26026,52053,52052,104105,19.88132905960083,22.224699288077773
27027,54055,54054,108109,20.619349002838135,21.741823914088855
28028,56057,56056,112113,21.315129041671753,21.272827422812497
29029,58059,58058,116117,22.028686046600342,20.81700115708236
30030,60061,60060,120121,22.742612838745117,20.373702619029018
31031,62063,62062,124125,23.42637300491333,19.942347140904758
32032,64065,64064,128129,24.11462378501892,19.522400721436952
33033,66067,66066,132133,24.86072587966919,19.113373861213176
34034,68069,68068,136137,25.565565824508667,18.71481625280444
35035,70071,70070,140141,26.25200891494751,18.326333749942933
36036,72073,72072,144145,26.933076858520508,17.947587045890714
37037,74075,74074,148149,27.60494899749756,17.57814805843327
38038,76077,76076,152153,28.280616760253906,17.217683326783117
39039,78079,78078,156157,28.97985601425171,16.8658811226353
40040,80081,80080,160161,29.64040994644165,16.52244917089979
41041,82083,82082,164165,30.31555986404419,16.187112688565094
42042,84085,84084,168169,30.978113889694214,15.859612674460664
43043,86087,86086,172173,31.681318044662476,15.539704411808543
44044,88089,88088,176177,32.34742283821106,15.227156153677015
45045,90091,90090,180181,33.03373885154724,14.921747966216799
46046,92093,92092,184185,33.72959876060486,14.623270708275413
47047,94095,94094,188189,34.408020973205566,14.331525129123861
48048,96097,96096,192193,35.095386028289795,14.04632106865813
49049,98099,98098,196197,35.79289484024048,13.767476746700595
50050,100101,100100,200201,36.49651098251343,13.494818129884152
51051,102103,102102,204205,37.199769020080566,13.228178366263819
52052,104105,104104,208209,37.946556091308594,12.967397279129386
53053,106107,106106,212213,38.751953125,12.71232091268189
54054,108109,108108,216217,39.52462887763977,12.462801123215854
55055,110111,110110,220221,40.29127097129822,12.218695210313967
56056,112113,112112,224225,41.063923835754395,11.979865583273522
57057,114115,114114,228229,42.30094790458679,11.746179458620531
58058,116117,116116,232233,43.449862003326416,11.517508585095584
59059,118119,118118,236237,44.58692383766174,11.293728992957654
60060,120121,120120,240241,45.70150279998779,11.074720764855897
61061,122123,122122,244245,47.03110599517822,10.860367825858475
62062,124125,124124,248249,48.17832803726196,10.650557750528947
63063,126127,126126,252253,49.3016459941864,10.445181585200203
64064,128129,128128,256257,50.3967490196228,10.244133683819769
65065,130131,130130,260261,51.480828046798706,10.04731155594402
66066,132133,132132,264265,52.56254506111145,9.85461572562349
67067,134135,134134,268269,53.67476296424866,9.665949600080012
68068,136137,136136,272273,54.71813893318176,9.481219347208025
69069,138139,138138,276277,55.75368690490723,9.30033378104747
70070,140141,140140,280281,56.86208772659302,9.12320425448354
71071,142143,142142,284285,57.93423295021057,8.949744558516727
72072,144145,144144,288289,59.04012489318848,8.779870827529066
73073,146147,146146,292293,60.17039608955383,8.613501450040417
74074,148149,148148,296297,61.29886984825134,8.450556984516084
75075,150151,150150,300301,62.37877082824707,8.290960079832871
76076,152153,152152,304305,63.465874910354614,8.134635400064326
77077,154155,154154,308309,64.54682111740112,7.981509553280148
78078,156157,156156,312313,65.6387288570404,7.831511024092947
79079,158159,158158,316317,66.72039794921875,7.684570109708716
80080,160161,160160,320321,67.7974328994751,7.540618859264441
81081,162163,162162,324325,68.85248494148254,7.399591016251065
82082,164165,164164,328329,69.89071607589722,7.261421963840689
83083,166167,166166,332333,70.92979502677917,7.126048672941238
84084,168169,168168,336337,72.02668309211731,6.993409652816922
85085,170171,170170,340341,73.10998487472534,6.863444904121366
86086,172173,172172,344345,74.22541689872742,6.736095874190255
87087,174175,174174,348349,75.3312418460846,6.611305414454705
88088,176177,176176,352353,76.44131088256836,6.489017739834253
89089,178179,178178,356357,77.52353286743164,6.369178389982608
90090,180181,180180,360361,78.603111743927,6.251734192253366
91091,182183,182182,364365,79.67991089820862,6.136633226273489
92092,184185,184184,368369,80.77050375938416,6.023824790005165
93093,186187,186186,372373,81.83539700508118,5.913259367192836
94094,188189,188188,376377,82.91001200675964,5.804888596094656
95095,190191,190190,380381,83.98654413223267,5.698665239408797
96096,192193,192192,384385,85.10086798667908,5.594543155305814
97097,194195,194194,388389,86.18544507026672,5.492477269492724
98098,196197,196196,392393,87.27712512016296,5.392423548238185
99099,198199,198198,396397,88.37706112861633,5.294338972292962
100100,200201,200200,400401,89.46467304229736,5.1981815116484995
101101,202203,202202,404405,90.55713391304016,5.10391010108367
102102,204205,204204,408409,91.65128898620605,5.011484616449707
103103,206207,206206,412413,92.73247599601746,4.920865851654412
104104,208209,208208,416417,93.96526980400085,4.8320154963057576
105105,210211,210210,420421,95.08342909812927,4.744896113984282
106106,212213,212212,424425,96.50510311126709,4.659471121108595
107107,214215,214214,428429,97.69749999046326,4.5757047663745425
108108,216217,216216,432433,98.82585000991821,4.493562110734729
109109,218219,218218,436437,100.01825499534607,4.413009007904293
110110,220221,220220,440441,101.18522310256958,4.334012085366339
111111,222223,222222,444445,102.59965586662292,4.256538725862697
112112,224225,224224,448449,103.77772688865662,4.180557049350909
113113,226227,226226,452453,104.99876093864441,4.106035895413925
114114,228229,228228,456457,106.41098213195801,4.032944806104979
115115,230231,230230,460461,107.63742995262146,3.9612540092181234
116116,232233,232232,464465,108.75116205215454,3.8909344019692753
117117,234235,234234,468469,109.87004494667053,3.8219575350775585
118118,236237,236236,472473,111.22925090789795,3.754295597233977
119119,238239,238238,476477,112.57147002220154,3.6879213999512785
120120,240241,240240,480481,113.75300812721252,3.6228083627790966
121121,242243,242242,484485,114.9441089630127,3.558930498880727
122122,244245,244244,488489,116.10821795463562,3.496262400958358
123123,246247,246246,492493,117.27981901168823,3.434779227520835
124124,248249,248248,496497,118.58339500427246,3.3744566894844183
125125,250251,250250,500501,119.87305903434753,3.315271037097318
126126,252253,252252,504505,120.9057970046997,3.2571990471838035
127127,254255,254254,508509,122.10547590255737,3.2002180106949254
128128,256257,256256,512513,123.18758296966553,3.144305720565626
129129,258259,258258,516517,124.31336688995361,3.089440459862317
130130,260261,260260,520521,125.39931797981262,3.035600990223429
131131,262263,262262,524525,126.52951502799988,2.982766540576449
132132,264265,264264,528529,127.6680498123169,2.930916796134966
133133,266267,266266,532533,128.79627585411072,2.880031887659129
134134,268269,268268,536537,129.87450098991394,2.8300923809808864
135135,270271,270270,540541,130.93505597114563,2.7810792667846727
136136,272273,272272,544545,132.0209457874298,2.7329739506359374
137137,274275,274274,548549,133.08933186531067,2.685758243255691
138138,276277,276276,552553,134.14940881729126,2.6394143510302683
139139,278279,278278,556557,135.22863793373108,2.593924866756197
140140,280281,280280,560561,136.45536184310913,2.5492727606089147
141141,282283,282282,564565,137.79334497451782,2.5054413713336317
142142,284285,284284,568569,139.11210894584656,2.4624143976521964
143143,286287,286286,572573,140.24226188659668,2.420175889879829
144144,288289,288288,576577,141.35783910751343,2.3787102417468304
145145,290291,290290,580581,142.45982003211975,2.3380021824222013
146146,292293,292292,584585,143.6945219039917,2.2980367687310945
147147,294295,294294,588589,145.07604503631592,2.2587993775630366
148148,296297,296296,592593,146.39265084266663,2.22027569846648
149149,298299,298298,596597,147.70488286018372,2.182451726424688
150150,300301,300300,600601,148.97782397270203,2.1453137548091945
151151,302303,302302,604605,150.24796795845032,2.108848368502663
152152,304305,304304,608609,151.49884295463562,2.07304243719409
153153,306307,306306,612613,152.74403882026672,2.037883108834535
154154,308309,308308,616617,153.99236607551575,2.003357803255426
155155,310311,310310,620621,155.2470200061798,1.9694542059398827
156156,312313,312312,624625,156.499351978302,1.9361602619483165
157157,314315,314314,628629,157.752427816391,1.9034641699915937
158158,316317,316316,632633,159.02469491958618,1.871354376648128
159159,318319,318318,636637,160.28739285469055,1.8398195707213745
160160,320321,320320,640641,161.5766577720642,1.8088486777367052
161161,322323,322322,644645,162.90400290489197,1.7784308545694785
162162,324325,324324,648649,164.15260410308838,1.7485554842052125
163163,326327,326326,652653,165.4223358631134,1.719212170626406
164164,328329,328328,656657,166.72118091583252,1.690390733823051
165165,330331,330330,660661,168.24943614006042,1.662081204923993
166166,332333,332332,664665,169.64585280418396,1.6342738214468682
167167,334335,334334,668669,171.10904788970947,1.6069590226618402
168168,336337,336336,672673,172.48027205467224,1.580127445066978
169169,338339,338338,676677,173.78836297988892,1.553769917974023
170170,340341,340340,680681,175.11111998558044,1.527877459199317
171171,342343,342342,684685,176.42052388191223,1.5024412708579575
172172,344345,344344,688689,177.7157130241394,1.4774527352608402
173173,346347,346346,692693,179.00280594825745,1.4529034109074246
174174,348349,348348,696697,180.32335782051086,1.428785028577181
175175,350351,350350,700701,181.62084794044495,1.4050894875124413
176176,352353,352352,704705,182.9992549419403,1.3818088516933358
177177,354355,354354,708709,184.34137988090515,1.3589353462011786
178178,356357,356356,712713,185.69275212287903,1.3364613536689376
179179,358359,358358,716717,187.0290470123291,1.3143794108159454
180180,360361,360360,720721,188.3356249332428,1.2926822050642386
181181,362363,362362,724725,189.6662518978119,1.2713625712364092
182182,364365,364364,728729,191.02089476585388,1.2504134883299685
183183,366367,366366,732733,192.34613704681396,1.229828076369813
184184,368369,368368,736737,193.65900683403015,1.2095995933327686
185185,370371,370370,740741,194.96078777313232,1.189721432147735
186186,372373,372372,744745,196.25232410430908,1.1701871177619978
187187,374375,374374,748749,197.56072115898132,1.150990304281322
188188,376377,376376,752753,198.8249499797821,1.1321247721730288
189189,378379,378378,756757,200.30167603492737,1.1135844255376242
190190,380381,380380,760761,201.80094981193542,1.0953632894415932
191191,382383,382382,764765,203.61433100700378,1.0774555073140846
192192,384385,384384,768769,205.0859980583191,1.0598553384048728
193193,386387,386386,772773,206.84682488441467,1.0425571552982547
194194,388389,388388,776777,208.68223595619202,1.0255554414889048
195195,390391,390390,780781,210.39403796195984,1.008844789010709
196196,392393,392392,784785,211.83275699615479,0.9924198961223283
197197,394395,394394,788789,213.22413897514343,0.9762755650442614
198198,396397,396396,792793,214.7055139541626,0.9604066997504788
199199,398399,398398,796797,216.55212998390198,0.9448083038091681
200200,400401,400400,800801,218.61302185058594,0.9294754782741848
201201,402403,402402,804805,220.05260396003723,0.9144034196234543
202202,404405,404404,808809,221.7380039691925,0.8995874177467158
203203,406407,406406,812813,223.12113499641418,0.8850228539769205
204204,408409,408408,816817,225.086040019989,0.8707051991681283
205205,410411,410410,820821,227.37898683547974,0.8566300118170602
206206,412413,412412,824825,229.68154311180115,0.842792936226715
207207,414415,414414,828829,231.85626792907715,0.8291897007117086
208208,416417,416416,832833,233.53342199325562,0.8158161158454504
209209,418419,418418,836837,235.13550686836243,0.8026680727455187
210210,420421,420420,840841,236.74081778526306,0.7897415413980298
211211,422423,422422,844845,238.23452997207642,0.7770325690207756
212212,424425,424424,848849,239.714262008667,0.764537278462285
213213,426427,426426,852853,241.21420407295227,0.7522518666371525
214214,428429,428428,856857,242.7296178340912,0.7401726029958127
215215,430431,430430,860861,244.1941258907318,0.7282958280300136
216216,432433,432432,864865,245.70529985427856,0.7166179518098943
217217,434435,434434,868869,247.26502299308777,0.705135452555055
218218,436437,436436,872873,248.84980082511902,0.6938448752368913
219219,438439,438438,876877,250.42459988594055,0.6827428302120779
220220,440441,440440,880881,251.93534088134766,0.671825991885953
221221,442443,442442,884885,253.42588591575623,0.66109109740637
222222,444445,444444,888889,254.90464401245117,0.6505349453856297
223223,446447,446446,892893,256.4673430919647,0.6401543946510628
224224,448449,448448,896897,257.9990828037262,0.6299463630225546
225225,450451,450450,900901,259.5130181312561,0.6199078261178101
226226,452453,452452,904905,261.1006729602814,0.6100358161830854
227227,454455,454454,908909,262.64175510406494,0.6003274209499523
228228,456457,456456,912913,264.1684970855713,0.5907797825167336
229229,458459,458458,916917,265.7041208744049,0.5813900962547223
230230,460461,460460,920921,267.185644865036,0.5721556097379334
231231,462463,462462,924925,268.69317388534546,0.5630736216965033
232232,464465,464464,928929,270.18683886528015,0.5541414809916887
233233,466467,466466,932933,271.679811000824,0.5453565856150817
234234,468469,468468,936937,273.2292070388794,0.5367163817076062
235235,470471,470470,940941,274.76948595046997,0.5282183626003416
236236,472473,472472,944945,276.2932929992676,0.519860067876607
237237,474475,474474,948949,277.8598120212555,0.5116390824531436
238238,476477,476476,952953,279.37238597869873,0.5035530356821027
239239,478479,478478,956957,280.8810019493103,0.4955996004711096
240240,480481,480480,960961,282.4030649662018,0.4877764924232224
241241,482483,482482,964965,283.9249289035797,0.4800814689957633
242242,484485,484484,968969,285.4462299346924,0.47251232867358794
243243,486487,486486,972973,287.01737904548645,0.46506691016577406
244244,488489,488488,976977,288.54580187797546,0.4577430916137928
245245,490491,490490,980981,290.0644679069519,0.45053878981980233
246246,492493,492492,984985,291.57761788368225,0.4434519594899484
247247,494495,494494,988989,293.0996677875519,0.436480592494604
248248,496497,496496,992993,294.60480308532715,0.4296227171433884
249249,498499,498498,996997,296.09216499328613,0.4228763974749654
250250,500501,500500,1001001,297.6021099090576,0.41623973256366753
251251,502503,502502,1005005,299.15310502052307,0.4097108558388527
252252,504505,504504,1009009,300.6987769603729,0.4032879344192679
253253,506507,506506,1013013,302.46104097366333,0.39696916846162367
254254,508509,508508,1017017,304.178270816803,0.3907527905217876
255255,510511,510510,1021021,305.8065640926361,0.38463706493075733
256256,512513,512512,1025025,307.57814502716064,0.37862028718188867
257257,514515,514514,1029029,309.28645181655884,0.37270078333222045
258258,516517,516516,1033033,310.8214781284332,0.3668769094165327
259259,518519,518518,1037037,312.33701395988464,0.3611470508702723
260260,520521,520520,1041041,313.8286838531494,0.3555096219703273
261261,522523,522522,1045045,315.3206388950348,0.34996306528069
262262,524525,524524,1049049,316.81392192840576,0.34450585111505916
263263,526527,526526,1053053,318.3845839500427,0.33913647700683214
264264,528529,528528,1057057,320.08091378211975,0.3338534671918296
265265,530531,530530,1061061,321.74983191490173,0.3286553721013661
266266,532533,532532,1065065,323.5185980796814,0.3235407678643014
267267,534535,534534,1069069,325.2097840309143,0.31850825582239395
268268,536537,536536,1073073,327.6420819759369,0.31355646205099674
269269,538539,538538,1077077,329.31807684898376,0.30868403689476054
270270,540541,540540,1081081,330.8071868419647,0.3038896545076568
271271,542543,542542,1085085,332.2753028869629,0.29917201240675695
272272,544545,544544,1089089,333.7654068470001,0.294529831031241
273273,546547,546546,1093093,335.26084184646606,0.28996185331322977
274274,548549,548548,1097097,336.73279786109924,0.2854668442564616
275275,550551,550550,1101101,338.23401379585266,0.2810435905222448
276276,552553,552552,1105105,339.6953980922699,0.2766909000247324
277277,554555,554554,1109109,341.1678738594055,0.2724076015351784
278278,556557,556556,1113113,342.67791509628296,0.26819254429233297
279279,558559,558558,1117117,344.16903591156006,0.26404459762204624
280280,560561,560560,1121121,345.6755139827728,0.259962650563466
281281,562563,562562,1125125,347.1594169139862,0.255945611504103
282282,564565,564564,1129129,348.646595954895,0.2519924078196709
283283,566567,566566,1133133,350.13740491867065,0.24810198552449947
284284,568569,568568,1137137,351.63466787338257,0.24427330892581267
285285,570571,570570,1141141,353.1371068954468,0.24050536028676106
286286,572573,572572,1145145,354.61867594718933,0.23679713949513825
287287,574575,574574,1149149,356.15162682533264,0.2331476637390324
288288,576577,576576,1153153,357.6463620662689,0.22955596718907145
289289,578579,578578,1157157,359.430716753006,0.2260211006865802
290290,580581,580580,1161161,361.09396290779114,0.22254213143799007
291291,582583,582582,1165165,362.8301627635956,0.21911814271493313
292292,584585,584584,1169169,364.48519587516785,0.215748233561726
293293,586587,586586,1173173,366.25773882865906,0.21243151850558206
294294,588589,588588,1177177,367.9345829486847,0.2091671272758049
295295,590591,590590,1181181,369.7898690700531,0.2059542045268472
296296,592593,592592,1185185,371.4723608493805,0.20279190956568982
297297,594595,594594,1189189,373.0910029411316,0.19967941608717865
298298,596597,596596,1193193,374.6895089149475,0.19661591191220396
299299,598599,598598,1197197,376.34150290489197,0.19360059873235969
300300,600601,600600,1201201,377.9531829357147,0.19063269185835452
301301,602603,602602,1205205,379.4543001651764,0.18771141997456198
302302,604605,604604,1209209,381.18099904060364,0.18483602489766326
303303,606607,606606,1213213,383.09646582603455,0.18200576133949653
304304,608609,608608,1217217,384.7024927139282,0.17921989667513571
305305,610611,610610,1221221,386.28163504600525,0.17647771071597163
306306,612613,612612,1225225,388.0269179344177,0.17377849548529412
307307,614615,614614,1229229,389.55559182167053,0.17112155500012705
308308,616617,616616,1233233,391.1168580055237,0.16850620505613279
309309,618619,618618,1237237,392.7620279788971,0.1659317730169505
310310,620621,620620,1241241,394.3363609313965,0.16339759760762718
311311,622623,622622,1245245,395.82070899009705,0.16090302871191398
312312,624625,624624,1249249,397.3330399990082,0.15844742717342797
313313,626627,626626,1253253,398.89075899124146,0.15603016459999708
314314,628629,628628,1257257,400.64159393310547,0.15365062317323464
315315,630631,630630,1261261,402.84445881843567,0.15130819546038765
316316,632633,632632,1265265,404.51822996139526,0.1490022842298231
317317,634635,634634,1269269,406.3373899459839,0.14673230227060685
318318,636637,636636,1273273,408.9023537635803,0.14449767221549337
319319,638639,638638,1277277,411.1798577308655,0.14229782636630262
320320,640641,640640,1281281,413.05169701576233,0.14013220652384462
321321,642643,642642,1285285,414.8720381259918,0.13800026381989028
322322,644645,644644,1289289,416.89326000213623,0.13590145855368974
323323,646647,646646,1293293,418.84522581100464,0.1338352600298549
324324,648649,648648,1297297,420.44632601737976,0.13180114640022111
325325,650651,650650,1301301,422.10391902923584,0.12979860450877823
326326,652653,652652,1305305,423.72987699508667,0.12782712974035348
327327,654655,654654,1309309,425.75492095947266,0.1258862258687259
328328,656657,656656,1313313,429.33060908317566,0.12397540491235759
329329,658659,658658,1317317,431.94296383857727,0.12209418698785157
330330,660661,660660,1321321,434.48207998275757,0.12024210017114001
331331,662663,662662,1325325,437.0490930080414,0.11841868035708103
332332,664665,664664,1329329,439.08752393722534,0.11662347112428506
333333,666667,666666,1333333,440.6355068683624,0.11485602360028224
334334,668669,668668,1337337,442.11727595329285,0.11311589633112362
335335,670671,670670,1341341,443.6087279319763,0.11140265515336978
336336,672673,672672,1345345,445.08628702163696,0.10971587306619313
337337,674675,674674,1349349,446.63984298706055,0.10805513010814138
338338,676677,676676,1353353,448.107106924057,0.10642001323537897
339339,678679,678678,1357357,449.64779901504517,0.1048101162017474
340340,680681,680680,1361361,451.29511284828186,0.10322503944223627
341341,682683,682682,1365365,452.84851813316345,0.10166438995679528
342342,684685,684684,1369369,454.35548305511475,0.10012778119744326
343343,686687,686686,1373373,455.8563051223755,0.09861483295810558
344344,688689,688688,1377377,457.35503792762756,0.09712517126433795
345345,690691,690690,1381381,458.8663969039917,0.09565842826748394
346346,692693,692692,1385385,460.3587329387665,0.09421424213826413
347347,694695,694694,1389389,461.84613704681396,0.09279225696502635
348348,696697,696696,1393393,463.3741660118103,0.0913921226514276
349349,698699,698698,1397397,464.95909905433655,0.09001349481741272
350350,700701,700700,1401401,466.64223885536194,0.08865603470178485
351351,702703,702702,1405405,468.1814298629761,0.08731940906511682
352352,704705,704704,1409409,469.92056012153625,0.08600329009766483
353353,706707,706706,1413413,471.4287278652191,0.0847073553240989
354354,708709,708708,1417417,472.9346179962158,0.08343128751607765
355355,710711,710710,1421421,475.11684799194336,0.08217477459970723
356356,712713,712712,1425425,477.6604039669037,0.08093750957027623
357357,714715,714714,1429429,479.47885513305664,0.0797191904051715
358358,716717,716716,1433433,481.09445691108704,0.07851951998020468
359359,718719,718718,1437437,482.629497051239,0.07733820598582497
360360,720721,720720,1441441,484.21379494667053,0.07617496084617414
361361,722723,722722,1445445,485.8023090362549,0.07502950163870992
362362,724725,724724,1449449,487.35829281806946,0.07390155001598941
363363,726727,726726,1453453,488.8801441192627,0.07279083212836213
364364,728729,728728,1457457,490.52039790153503,0.07169707854814078
365365,730731,730730,1461461,492.0639238357544,0.0706200241947954
366366,732733,732732,1465465,493.6206157207489,0.06955940826287588
367367,734735,734734,1469469,495.2520899772644,0.06851497414834284
368368,736737,736736,1473473,496.88177490234375,0.06748646937990088
369369,738739,738738,1477477,498.433002948761,0.06647364554862634
370370,740741,740740,1481481,499.9630661010742,0.06547625824032366
371371,742743,742742,1485485,501.5270240306854,0.06449406696742699
372372,744745,744744,1489489,503.129900932312,0.06352683510544921
373373,746747,746746,1493493,504.6562180519104,0.06257432982658884
374374,748749,748748,1497497,506.1606249809265,0.06163632203663383
375375,750751,750750,1501501,507.7278130054474,0.06071258631368437
376376,752753,752752,1505505,509.28214502334595,0.05980290084551143
377377,754755,754754,1509509,510.8286168575287,0.0589070473705533
378378,756757,756756,1513513,512.5875911712646,0.05802481111788893
379379,758759,758758,1517517,514.2447347640991,0.057155980749826085
380380,760761,760760,1521521,515.7849359512329,0.0563003483052853
381381,762763,762762,1525525,517.279501914978,0.05545770914181958
382382,764765,764764,1529529,518.941535949707,0.05462786188320479
383383,766767,766766,1533533,520.5773229598999,0.0538106083627099
384384,768769,768768,1537537,522.2372739315033,0.05300575357239268
385385,770771,770770,1541541,524.2917490005493,0.05221310560887105
386386,772773,772772,1545545,525.9052519798279,0.05143247562295983
387387,774775,774774,1549549,527.5095739364624,0.05066367776930747
388388,776777,776776,1553553,529.1405379772186,0.04990652915614646
389389,778779,778778,1557557,531.18425989151,0.049160849796976436
390390,780781,780780,1561561,532.8758981227875,0.04842646256292937
391391,782783,782782,1565565,534.4842119216919,0.0477031931353622
392392,784785,784784,1569569,536.0370547771454,0.04699086995969992
393393,786787,786786,1573573,538.0319328308105,0.046289324199847215
394394,788789,788788,1577577,540.0401329994202,0.0455983896943053
395395,790791,790790,1581581,541.6302790641785,0.04491790291081088
396396,792793,792792,1585585,543.1159439086914,0.04424770290518154
397397,794795,794794,1589589,544.872386932373,0.04358763127675047
398398,796797,796796,1593593,546.7623109817505,0.04293753212812135
399399,798799,798798,1597597,548.263298034668,0.04229725202424106
400400,800801,800800,1601601,549.7577500343323,0.0416666399511314
401401,802803,802802,1605605,551.2693648338318,0.04104554727757659
402402,804805,804804,1609609,552.7632608413696,0.040433827715219195
403403,806807,806806,1613613,554.2432260513306,0.03983133728070243
404404,808809,808808,1617617,555.7903280258179,0.03923793425860822
405405,810811,810810,1621621,557.3045279979706,0.03865347916325845
406406,812813,812812,1625625,558.7985508441925,0.03807783470404047
407407,814815,814814,1629629,560.2633588314056,0.037510865748117794
408408,816817,816816,1633633,561.7557349205017,0.03695243928666514
409409,818819,818818,1637637,563.4130959510803,0.0364024243995118
410410,820821,820820,1641641,565.4595999717712,0.035860692221831414
411411,822823,822822,1645645,567.3577988147736,0.035327115910263274
412412,824825,824824,1649649,569.1763119697571,0.0348015706103979
413413,826827,826826,1653653,571.9908010959625,0.03428393342517211
414414,828829,828828,1657657,573.7430799007416,0.03377408338144505
415415,830831,830830,1661661,575.6660869121552,0.033271901401121795
416416,832833,832832,1665665,577.4904499053955,0.03277727026932098
417417,834835,834834,1669669,579.2128307819366,0.032290074603679386
418418,836837,836836,1673673,580.7289960384369,0.031810200826612345
419419,838839,838838,1677677,582.196939945221,0.03133753713427723
420420,840841,840840,1681681,583.6870000362396,0.030871973469174918
421421,842843,842842,1685685,585.5821008682251,0.03041340149172811
422422,844845,844844,1689689,587.3647909164429,0.029961714552200647
423423,846847,846846,1693693,589.2385137081146,0.029516807664663247
424424,848849,848848,1697697,590.9570558071136,0.029078577478912848
425425,850851,850850,1701701,592.5800549983978,0.028646922254665697
426426,852853,852852,1705705,594.1970059871674,0.028221741836887304
427427,854855,854854,1709709,595.7936818599701,0.027802937627598112
428428,856857,856856,1713713,597.3500018119812,0.027390412564159305
429429,858859,858858,1717717,598.860239982605,0.02698407109244272
430430,860861,860860,1721721,600.3816409111023,0.026583819143411347
431431,862863,862862,1725725,601.9327578544617,0.02618956410969986
432432,864865,864864,1729729,603.5519490242004,0.025801214821512986
433433,866867,866866,1733733,605.178386926651,0.0254186815243429
434434,868869,868868,1737737,606.7482171058655,0.025041875855549733
435435,870871,870870,1741741,608.3374979496002,0.024670710823215813
436436,872873,872872,1745745,609.8530600070953,0.024305100783180933
437437,874875,874874,1749749,611.487795829773,0.0239449614186924
438438,876877,876876,1753753,613.0445721149445,0.023590209718349797
439439,878879,878878,1757757,614.6252219676971,0.023240763955413968
440440,880881,880880,1761761,616.2474977970123,0.022896543668025515
441441,882883,882882,1765765,617.816422700882,0.022557469638400107
442442,884885,884884,1769769,619.3814699649811,0.022223463873501714
443443,886887,886886,1773773,620.9302139282227,0.021894449585374787
444444,888889,888888,1777777,622.4981050491333,0.021570351171703805
445445,890891,890890,1781781,624.129723072052,0.02125109419796445
446446,892893,892892,1785785,625.6006979942322,0.020936605377869455
447447,894895,894894,1789789,627.1644718647003,0.02062681255551979
448448,896897,896896,1793793,628.7417368888855,0.020321644688351626
449449,898899,898898,1797797,630.6282768249512,0.020021031827582192
450450,900901,900900,1801801,632.2428667545319,0.01972490510308944
451451,902903,902902,1805805,634.1037368774414,0.019433196704881084
452452,904905,904904,1809809,637.0621438026428,0.01914583986706475
453453,906907,906906,1813813,640.0089898109436,0.01886276885090865
454454,908909,908908,1817817,642.2620298862457,0.018583918929266474
455455,910911,910910,1821821,644.3019948005676,0.018309226369183307
456456,912913,912912,1825825,645.9022209644318,0.018038628418480585
457457,914915,914914,1829829,647.4462268352509,0.017772063288475692
458458,916917,916916,1833833,649.0100920200348,0.017509470138975303
459459,918919,918918,1837837,650.6450469493866,0.017250789064974015
460460,920921,920920,1841841,652.202488899231,0.016995961079487643
461461,922923,922922,1845845,654.0951879024506,0.016744928100933976
462462,924925,924924,1849849,656.5506417751312,0.01649763293869455
463463,926927,926926,1853853,659.054918050766,0.016254019277880616
464464,928929,928928,1857857,662.0500888824463,0.016014031667168638
465465,930931,930930,1861861,665.3566670417786,0.01577761550447576
466466,932933,932932,1865865,667.4539377689362,0.015544717023544763
467467,934935,934934,1869869,669.1303369998932,0.01531528328132481
468468,936937,936936,1873873,671.3541460037231,0.015089262144215354
469469,938939,938938,1877877,673.4626758098602,0.014866602276811136
470470,940941,940940,1881881,675.5602600574493,0.014647253127577642
471471,942943,942942,1885885,677.4817168712616,0.014431164918846662
472472,944945,944944,1889889,679.1405549049377,0.014218288631809628
473473,946947,946946,1893893,681.5804440975189,0.014008575997650041
474474,948949,948948,1897897,683.2143950462341,0.01380197948424211
475475,950951,950950,1901901,684.6816439628601,0.013598452284213636
476476,952953,952952,1905905,686.2081871032715,0.013397948305168939
477477,954955,954954,1909909,687.7571461200714,0.01320042215684225
478478,956957,956956,1913913,689.2572009563446,0.013005829141775394
479479,958959,958958,1917917,690.7744328975677,0.012814125243380659
480480,960961,960960,1921921,692.2692210674286,0.012625267115936367
481481,962963,962962,1925925,693.8132750988007,0.0124392120731045
482482,964965,964964,1929929,695.6267371177673,0.012255918079745243
483483,966967,966966,1933933,697.2128179073334,0.012075343739525124
484484,968969,968968,1937937,699.041601896286,0.0118974482863905
485485,970971,970970,1941941,701.311164855957,0.011722191574222052
486486,972973,972972,1945945,702.9249861240387,0.011549534067739842
487487,974975,974974,1949949,704.5183401107788,0.011379436832271494
488488,976977,976976,1953953,706.3022549152374,0.011211861524657252
489489,978979,978978,1957957,707.8298778533936,0.011046770384609772
490490,980981,980980,1961961,709.3504319190979,0.010884126225278123
491491,982983,982982,1965965,711.0725758075714,0.01072389242403915
492492,984985,984984,1969969,712.593003988266,0.010566032914425705
493493,986987,986986,1973973,714.1360139846802,0.010410512176804332
494494,988989,988988,1977977,715.6908760070801,0.010257295230985619
495495,990991,990990,1981981,717.3047578334808,0.010106347626560819
496496,992993,992992,1985985,718.8944199085236,0.009957635435398515
497497,994995,994994,1989989,720.5185770988464,0.009811125244027608
498498,996997,996996,1993993,722.2114880084991,0.009666784144428675
499499,998999,998998,1997997,723.8643350601196,0.009524579727553828
500501,1001003,1001002,2002005,725.3938930034637,0.009384341157101517
501502,1003005,1003004,2006009,726.9445719718933,0.009246316888834372
502503,1005007,1005006,2010013,728.6314129829407,0.00911033495913216
503504,1007009,1007008,2014017,730.3314549922943,0.008976364876616572
504505,1009011,1009010,2018021,732.0776591300964,0.008844376611818916
505506,1011013,1011012,2022025,733.7866628170013,0.0087143405887673
506507,1013015,1013014,2026029,735.3026208877563,0.008586227678847536
507508,1015017,1015016,2030033,736.7969899177551,0.008460009193527185
508509,1017019,1017018,2034037,738.3090558052063,0.00833565687742066
509510,1019021,1019020,2038041,739.7793960571289,0.008213142902036452
510511,1021023,1021022,2042045,741.4289269447327,0.008092439858955913
511512,1023025,1023024,2046049,743.0194957256317,0.0079735207534668
512513,1025027,1025026,2050053,744.5682528018951,0.007856358998424184
513514,1027029,1027028,2054057,746.0737881660461,0.007740928407542924
514515,1029031,1029030,2058061,747.6613109111786,0.00762720318925858
515516,1031033,1031032,2062065,749.1550278663635,0.007515157941384132
516517,1033035,1033034,2066069,750.7064599990845,0.007404767644402455
517518,1035037,1035036,2070073,752.3603849411011,0.0072960076557819775
518519,1037039,1037038,2074077,754.0009109973907,0.007188853704064968
519520,1039041,1039040,2078081,755.610906124115,0.007083281883865311
520521,1041043,1041042,2082085,757.163213968277,0.0069792686492746725
521522,1043045,1043044,2086089,758.6527390480042,0.006876790809087652
522523,1045047,1045046,2090093,760.3182849884033,0.006775825521231127
523524,1047049,1047048,2094097,762.0338799953461,0.006676350287079913
524525,1049051,1049050,2098101,763.9876368045807,0.006578342946681914
525526,1051053,1051052,2102105,765.836226940155,0.006481781673073783
526527,1053055,1053054,2106109,767.9393708705902,0.006386644967733446
527528,1055057,1055056,2110113,769.9480118751526,0.0062929116551231346
528529,1057059,1057058,2114117,772.0404388904572,0.006200560878255601
529530,1059061,1059060,2118121,774.312924861908,0.006109572093009774
530531,1061063,1061062,2122125,776.5035948753357,0.006019925064265408
531532,1063065,1063064,2126129,779.3583889007568,0.0059315998605598
532533,1065067,1065066,2130133,782.0983099937439,0.005844576849654004
533534,1067069,1067068,2134137,783.9435520172119,0.005758836694099045
534535,1069071,1069070,2138141,786.6034009456635,0.005674360346802132
535536,1071073,1071072,2142145,789.0228018760681,0.0055911290460244345
536537,1073075,1073074,2146149,791.4830539226532,0.005509124311970481
537538,1075077,1075076,2150153,795.7295439243317,0.005428327941444877
538539,1077079,1077078,2154157,798.3904480934143,0.005348722004441697
539540,1079081,1079080,2158161,801.574285030365,0.005270288839710702
540541,1081083,1081082,2162165,803.248391866684,0.005193011050778296
541542,1083085,1083084,2166169,806.4006147384644,0.005116871501627429
542543,1085087,1085086,2170173,809.7725319862366,0.005041853312945932
543544,1087089,1087088,2174177,811.708582162857,0.004967939858261161
544545,1089091,1089090,2178181,813.672492980957,0.004895114760074648
545546,1091093,1091092,2182185,815.1961917877197,0.004823361886337807
546547,1093095,1093094,2186189,817.2457981109619,0.004752665345790774
547548,1095097,1095096,2190193,819.4475560188293,0.004683009485461298
548549,1097099,1097098,2194197,823.0283398628235,0.004614378886344639
549550,1099101,1099100,2198201,825.8486571311951,0.004546758360447711
550551,1101103,1101102,2202205,828.7495260238647,0.004480132946127924
551552,1103105,1103104,2206209,831.5472049713135,0.0044144879061605025
552553,1105107,1105106,2210213,833.410336971283,0.0043498087233047045
553554,1107109,1107108,2214217,835.0187849998474,0.004286081097234273
554555,1109111,1109110,2218221,836.8512959480286,0.004223290941467894
555556,1111113,1111112,2222225,838.334734916687,0.004161424379958589
556557,1113115,1113114,2226229,839.9075119495392,0.004100467743569425
557558,1115117,1115116,2230233,841.9142661094666,0.0040404075676860884
558559,1117119,1117118,2234237,843.6806309223175,0.00398123058857891
559560,1119121,1119120,2238241,845.5677280426025,0.003922923740560691
560561,1121123,1121122,2242245,847.3796279430389,0.003865474152689785
561562,1123125,1123124,2246249,849.2972929477692,0.0038088691462689894
562563,1125127,1125126,2250253,851.0920498371124,0.0037530962320033723
563564,1127129,1127128,2254257,852.8526599407196,0.003698143106362295
564565,1129131,1129130,2258261,854.8698830604553,0.0036439976494193616
565566,1131133,1131132,2262265,856.6073188781738,0.0035906479225786825
566567,1133135,1133134,2266269,858.3591327667236,0.0035380821641410876
567568,1135137,1135136,2270273,860.3096640110016,0.003486288788735692
568569,1137139,1137138,2274277,861.8617568016052,0.0034352563827724225
569570,1139141,1139140,2278281,863.3516368865967,0.0033849737034188365
570571,1141143,1141142,2282285,864.9593887329102,0.0033354296750758294
571572,1143145,1143144,2286289,866.9591310024261,0.0032866133864217772
572573,1145147,1145146,2290293,868.9856507778168,0.0032385140902988496
573574,1147149,1147148,2294297,870.5239789485931,0.0031911211975739207
574575,1149151,1149150,2298301,872.0383059978485,0.0031444242779343767
575576,1151153,1151152,2302305,873.5541348457336,0.003098413056136451
576577,1153155,1153154,2306309,875.0910770893097,0.0030530774096177993
577578,1155157,1155156,2310313,876.6360628604889,0.003008407366451138
578579,1157159,1157158,2314317,878.1541638374329,0.00296439310329788
579580,1159161,1159160,2318321,879.674339056015,0.0029210249423385903
580581,1161163,1161162,2322325,881.3871788978577,0.002878293350477179
581582,1163165,1163164,2326329,883.0122580528259,0.0028361889357029213
582583,1165167,1165166,2330333,884.6341459751129,0.0027947024461809633
583584,1167169,1167168,2334337,886.5595738887787,0.0027538247667280302
584585,1169171,1169170,2338341,888.2986800670624,0.0027135469185850525
585586,1171173,1171172,2342345,889.8467009067535,0.002673860055892874
586587,1173175,1173174,2346349,891.4872989654541,0.0026347554638732618
587588,1175177,1175176,2350353,892.993616104126,0.0025962245578057264
588589,1177179,1177178,2354357,894.6195409297943,0.002558258880299036
589590,1179181,1179180,2358361,896.20490193367,0.002520850099699601
590591,1181183,1181182,2362365,898.2905178070068,0.0024839900073629906
591592,1183185,1183184,2366369,900.3018698692322,0.0024476705170854984
592593,1185187,1185186,2370373,902.3751919269562,0.0024118836624893447
593594,1187189,1187188,2374377,904.9989428520203,0.0023766215957721215
594595,1189191,1189190,2378381,907.2902429103851,0.0023418765849783085
595596,1191193,1191192,2382385,908.9466700553894,0.0023076410130897784
596597,1193195,1193194,2386389,910.6148369312286,0.0022739073759794337
597598,1195197,1195196,2390393,912.1993980407715,0.0022406682812743384
598599,1197199,1197198,2394397,913.7500488758087,0.0022079164458546074
599600,1199201,1199200,2398401,915.385725736618,0.0021756446942617913
600601,1201203,1201202,2402405,916.9582769870758,0.0021438459579030678
601602,1203205,1203204,2406409,918.4857220649719,0.002112513273004879
602603,1205207,1205206,2410413,920.0872669219971,0.002081639778339195
603604,1207209,1207208,2414417,921.6497919559479,0.0020512187148824523
604605,1209211,1209210,2418421,923.2264668941498,0.0020212434237691923
605606,1211213,1211212,2422425,924.903443813324,0.001991707344700444
606607,1213215,1213214,2426429,926.4481687545776,0.0019626040144657964
607608,1215217,1215216,2430433,928.0093250274658,0.0019339270651244078
608609,1217219,1217218,2434437,929.5077338218689,0.0019056702238913203
609610,1219221,1219220,2438441,931.0429339408875,0.0018778273104089749
610611,1221223,1221222,2442445,932.6964039802551,0.001850392235610343
611612,1223225,1223224,2446449,934.282812833786,0.0018233590010368061
612613,1225227,1225226,2450453,935.7817659378052,0.0017967216963370447
613614,1227229,1227228,2454457,937.2670350074768,0.0017704744994944122
614615,1229231,1229230,2458461,938.765636920929,0.0017446116735300166
615616,1231233,1231232,2462465,940.5371329784393,0.0017191275674122153
616617,1233235,1233234,2466469,942.2548987865448,0.0016940166131007572
617618,1235237,1235236,2470473,944.33345079422,0.0016692733248646618
618619,1237239,1237238,2474477,945.972058057785,0.0016448922983727243
619620,1239241,1239240,2478481,947.911994934082,0.0016208682089882132
620621,1241243,1241242,2482485,950.6945838928223,0.0015971958108593753
621622,1243245,1243244,2486489,953.5133128166199,0.0015738699355551944
622623,1245247,1245246,2490493,956.0412049293518,0.001550885491496956
623624,1247249,1247248,2494497,958.304929971695,0.0015282374616845118
624625,1249251,1249250,2498501,960.7490148544312,0.0015059209034689047
625626,1251253,1251252,2502505,962.5501239299774,0.0014839309475291884
626627,1253255,1253254,2506509,964.274612903595,0.001462262796280811
627628,1255257,1255256,2510513,965.8648297786713,0.0014409117228524337
628629,1257259,1257258,2514517,967.4341180324554,0.0014198730701764362
629630,1259261,1259260,2518521,969.0035057067871,0.001399142250420482
630631,1261263,1261262,2522525,970.4820909500122,0.0013787147428274693
631632,1263265,1263264,2526529,971.9749097824097,0.0013585860938292171
632633,1265267,1265266,2530533,973.5043697357178,0.0013387519156822236
633634,1267269,1267268,2534537,975.4554390907288,0.0013192078846486766
634635,1269271,1269270,2538541,977.2738809585571,0.0012999497421333217
635636,1271273,1271272,2542545,979.0880239009857,0.0012809732908181104
636637,1273275,1273274,2546549,981.090213060379,0.0012622743965948757
637638,1275277,1275276,2550553,983.0610549449921,0.0012438489856094748
638639,1277279,1277278,2554557,984.635027885437,0.0012256930443754754
639640,1279281,1279280,2558561,986.1482379436493,0.001207802618750975
640641,1281283,1281282,2562565,987.7350850105286,0.001190173812346984
641642,1283285,1283284,2566569,989.2881908416748,0.0011728027869821744
642643,1285287,1285286,2570573,990.8536260128021,0.0011556857605228288
643644,1287289,1287288,2574577,992.3587999343872,0.001138819006769154
644645,1289291,1289290,2578581,993.866409778595,0.0011221988544320993
645646,1291293,1291292,2582585,995.3348867893219,0.001105821686451236
646647,1293295,1293294,2586589,996.986839056015,0.0010896839389715751
647648,1295297,1295296,2590593,998.5650427341461,0.0010737821003203862
648649,1297299,1297298,2594597,1000.1319448947906,0.0010581127112345712
649650,1299301,1299300,2598601,1001.6401419639587,0.0010426723632690482
650651,1301303,1301302,2602605,1003.1106128692627,0.0010274576978872574
651652,1303305,1303304,2606609,1004.6295168399811,0.0010124654058927263
652653,1305307,1305306,2610613,1006.1474030017853,0.00099769222742907
653654,1307309,1307308,2614617,1007.7550208568573,0.0009831349500473152
654655,1309311,1309310,2618621,1009.3748750686646,0.000968790409160647
655656,1311313,1311312,2622625,1011.0618150234222,0.0009546554864527934
656657,1313315,1313314,2626629,1012.6146337985992,0.0009407271093095915
657658,1315317,1315316,2630633,1014.5787398815155,0.0009270022509326736
658659,1317319,1317318,2634637,1016.9014329910278,0.0009134779285204786
659660,1319321,1319320,2638641,1018.6717929840088,0.0009001512034956249
660661,1321323,1321322,2642645,1020.846107006073,0.0008870191804817296
661662,1323325,1323324,2646649,1022.3842630386353,0.0008740790067349735
662663,1325327,1325326,2650653,1024.1450979709625,0.0008613278713482941
663664,1327329,1327328,2654657,1025.8875739574432,0.0008487630046829509
664665,1329331,1329330,2658661,1027.6364018917084,0.0008363816782548383
665666,1331333,1331332,2662665,1029.1591620445251,0.0008241812034839313
666667,1333335,1333334,2666669,1030.7429249286652,0.000812158931353224
667668,1335337,1335336,2670673,1032.504135131836,0.0008003122516129224
668669,1337339,1337338,2674677,1034.259377002716,0.0007886385925530703
669670,1339341,1339340,2678681,1035.938050031662,0.0007771354205488024
670671,1341343,1341342,2682685,1038.7895758152008,0.0007658002389234753
671672,1343345,1343344,2686689,1040.8018689155579,0.0007546305876076076
672673,1345347,1345346,2690693,1042.7336089611053,0.0007436240430251928
673674,1347349,1347348,2694697,1044.5449068546295,0.0007327782170705177
674675,1349351,1349350,2698701,1046.485694885254,0.0007220907565397283
675676,1351353,1351352,2702705,1048.7934310436249,0.0007115593431308298
676677,1353355,1353354,2706709,1051.5267729759216,0.0007011816927615655
677678,1355357,1355356,2710713,1053.9452548027039,0.0006909555543188617
678679,1357359,1357358,2714717,1055.801011800766,0.0006808787101135749
679680,1359361,1359360,2718721,1057.872503042221,0.0006709489750846842
680681,1361363,1361362,2722725,1059.877275943756,0.0006611641963445436
681682,1363365,1363364,2726729,1062.1330118179321,0.0006515222521557007
682683,1365367,1365366,2730733,1064.2749407291412,0.0006420210526130177
683684,1367369,1367368,2734737,1066.1940658092499,0.0006326585380520555
684685,1369371,1369370,2738741,1068.2363839149475,0.0006234326790490741
685686,1371373,1371372,2742745,1070.0838119983673,0.0006143414766484057
686687,1373375,1373374,2746749,1072.0394189357758,0.0006053829602024052
687688,1375377,1375376,2750753,1074.0964739322662,0.0005965551885083187
688689,1377379,1377378,2754757,1076.078132867813,0.0005878562491261619
689690,1379381,1379380,2758761,1078.0096580982208,0.0005792842574692258
690691,1381383,1381382,2762765,1079.808315038681,0.0005708373563493296
691692,1383385,1383384,2766769,1082.09028506279,0.0005625137160905069
692693,1385387,1385386,2770773,1084.0513038635254,0.0005543115341879457
693694,1387389,1387388,2774777,1086.3357429504395,0.000546229033830059
694695,1389391,1389390,2778781,1088.072126865387,0.0005382644650353541
695696,1391393,1391392,2782785,1089.6511409282684,0.0005304161030608157
696697,1393395,1393394,2786789,1091.6884257793427,0.0005226822486292804
697698,1395397,1395396,2790793,1093.5865178108215,0.0005150612272473154
698699,1397399,1397398,2794797,1095.286180973053,0.0005075513890915317
699700,1399401,1399400,2798801,1097.4419589042664,0.0005001511087812105
700701,1401403,1401402,2802805,1099.4427418708801,0.0004928587841277476
701702,1403405,1403404,2806809,1101.4005889892578,0.0004856728371578356
702703,1405407,1405406,2810813,1103.2842168807983,0.0004785917127492212
703704,1407409,1407408,2814817,1105.7644128799438,0.0004716138786307056
704705,1409411,1409410,2818821,1108.0766360759735,0.00046473782470002334
705706,1411413,1411412,2822825,1110.1058900356293,0.000457962063251216
706707,1413415,1413414,2826829,1112.263935804367,0.0004512851285198849
707708,1415417,1415416,2830833,1114.5132579803467,0.00044470557600106986
708709,1417419,1417418,2834837,1116.8761987686157,0.00043822198279031
709710,1419421,1419420,2838841,1119.3086698055267,0.00043183294610571465
710711,1421423,1421422,2842845,1121.7822880744934,0.00042553708442483185
711712,1423425,1423424,2846849,1123.565771818161,0.00041933303600671934
712713,1425427,1425426,2850853,1125.235633134842,0.00041321945911931834
713714,1427429,1427428,2854857,1127.4223818778992,0.0004071950322668272
714715,1429431,1429430,2858861,1129.499587059021,0.00040125845248439873
715716,1431433,1431432,2862865,1131.538594007492,0.00039540843636132195
716717,1433435,1433434,2866869,1133.3374569416046,0.00038964371958627453
717718,1435437,1435436,2870873,1135.4620079994202,0.0003839630553557072
718719,1437439,1437438,2874877,1137.4616298675537,0.00037836521653389354
719720,1439441,1439440,2878881,1139.5894589424133,0.0003728489924696987
720721,1441443,1441442,2882885,1141.6089899539948,0.0003674131914976897
721722,1443445,1443444,2886889,1143.6977598667145,0.00036205663877808547
722723,1445447,1445446,2890893,1145.6153509616852,0.00035677817675150436
723724,1447449,1447448,2894897,1147.370540857315,0.00035157666491159034
724725,1449451,1449450,2898901,1149.0188429355621,0.0003464509795776394
725726,1451453,1451452,2902905,1150.7432868480682,0.00034140001309879153
726727,1453455,1453454,2906909,1152.6495740413666,0.00033642267430877837
727728,1455457,1455456,2910913,1154.4542157649994,0.0003315178882985492
728729,1457459,1457458,2914917,1156.3145110607147,0.00032668459527940286
729730,1459461,1459460,2918921,1157.93581199646,0.0003219217513787953
730731,1461463,1461462,2922925,1160.1331088542938,0.00031722832818559255
731732,1463465,1463464,2926929,1162.171236038208,0.00031260331184057577
732733,1465467,1465466,2930933,1164.2199311256409,0.00030804570371856244
733734,1467469,1467468,2934937,1166.010407924652,0.00030355451951891155
734735,1469471,1469470,2938941,1167.6926429271698,0.0002991287899476447
735736,1471473,1471472,2942945,1169.6534860134125,0.00029476755901214347
736737,1473475,1473474,2946949,1171.574001789093,0.0002904698849306442
737738,1475477,1475476,2950953,1173.3555917739868,0.00028623484070067207
738739,1477479,1477478,2954957,1175.639055967331,0.00028206151171161764
739740,1479481,1479480,2958961,1177.772929906845,0.0002779489967679183
740741,1481483,1481482,2962965,1179.5903499126434,0.0002738964088848661
741742,1483485,1483484,2966969,1181.8399019241333,0.00026990287301487115
742743,1485487,1485486,2970973,1183.953290939331,0.0002659675275253903
743744,1487489,1487488,2974977,1185.9528968334198,0.0002620895227209985
744745,1489491,1489490,2978981,1187.7914559841156,0.0002582680223213174
745746,1491493,1491492,2982985,1190.0292310714722,0.0002545022014146525
746747,1493495,1493494,2986989,1191.882756948471,0.0002507912477085483
747748,1495497,1495496,2990993,1193.9159348011017,0.0002471343602792331
748749,1497499,1497498,2994997,1196.0919868946075,0.0002435307504811135
749750,1499501,1499500,2999001,1198.482300043106,0.00023997964080990641
750751,1501503,1501502,3003005,1200.1978950500488,0.00023648026490263874
751752,1503505,1503504,3007009,1202.153268814087,0.0002330318684471422
752753,1505507,1505506,3011013,1203.9267377853394,0.0002296337077041244
753754,1507509,1507508,3015017,1205.9810090065002,0.0002262850492797952
754755,1509511,1509510,3019021,1208.2191369533539,0.0002229851712627351
755756,1511513,1511512,3023025,1210.457477092743,0.00021973336197333992
756757,1513515,1513514,3027029,1212.916958808899,0.0002165289204185683
757758,1515517,1515516,3031033,1215.1418988704681,0.00021337115526876005
758759,1517519,1517518,3035037,1217.0084338188171,0.00021025938576713088
759760,1519521,1519520,3039041,1219.009686946869,0.0002071929410476514
760761,1521523,1521522,3043045,1220.6902680397034,0.00020417116002136027
761762,1523525,1523524,3047049,1222.352149963379,0.00020119339114899049
762763,1525527,1525526,3051053,1224.4275588989258,0.0001982589925546563
763764,1527529,1527528,3055057,1226.2191388607025,0.0001953673316847926
764765,1529531,1529530,3059061,1228.0005548000336,0.000192517785308155
765766,1531533,1531532,3063065,1229.670408964157,0.00018970973894738563
766767,1533535,1533534,3067069,1231.2094478607178,0.00018694258790219465
767768,1535537,1535536,3071073,1233.1523067951202,0.000184215735316684
768769,1537539,1537538,3075077,1235.809308052063,0.00018152859365727636
769770,1539541,1539540,3079081,1237.8355560302734,0.00017888058403059404
770771,1541543,1541542,3083085,1239.4434039592743,0.00017627113561502483
771772,1543545,1543544,3087089,1241.4177379608154,0.00017369968634284305
772773,1545547,1545546,3091093,1243.0251219272614,0.00017116568187702796
773774,1547549,1547548,3095097,1244.586613893509,0.00016866857640707167
774775,1549551,1549550,3099101,1246.6996488571167,0.00016620783219423174
775776,1551553,1551552,3103105,1249.365905046463,0.0001637829185483497
776777,1553555,1553554,3107109,1250.8773968219757,0.00016139331353315356
777778,1555557,1555556,3111113,1252.379448890686,0.00015903850214726845
778779,1557559,1557558,3115117,1253.8862807750702,0.00015671797723371128
779780,1559561,1559560,3119121,1255.3517470359802,0.00015443123902514344
780781,1561563,1561562,3123125,1256.9633519649506,0.00015217779503018392
781782,1563565,1563564,3127129,1258.548124074936,0.0001499571596923488
782783,1565567,1565566,3131133,1260.046600818634,0.00014776885495848546
783784,1567569,1567568,3135137,1261.559494972229,0.00014561240948296472
784785,1569571,1569570,3139141,1263.0458028316498,0.00014348735874136764
785786,1571573,1571572,3143145,1264.551974773407,0.0001413932454852329
786787,1573575,1573574,3147149,1266.0270149707794,0.00013932961860518844
787788,1575577,1575576,3151153,1267.505994796753,0.0001372960336993856
788789,1577579,1577578,3155157,1268.9965589046478,0.0001352920527324386
789790,1579581,1579580,3159161,1270.4853711128235,0.0001333172447175457
790791,1581583,1581582,3163165,1271.9631941318512,0.0001313711842385601
791792,1583585,1583584,3167169,1273.4438908100128,0.00012945345224579796
792793,1585587,1585586,3171173,1274.9034609794617,0.00012756363605603838
793794,1587589,1587588,3175177,1276.3936460018158,0.00012570132889777597
794795,1589591,1589590,3179181,1277.8780999183655,0.00012386612979753409
795796,1591593,1591592,3183185,1279.3542461395264,0.00012205764357986482
796797,1593595,1593594,3187189,1280.8320360183716,0.00012027548143578315
797798,1595597,1595596,3191193,1282.307846069336,0.00011851925921746442
798799,1597599,1597598,3195197,1283.7918298244476,0.00011678859937092056
799800,1599601,1599600,3199201,1285.270614862442,0.00011508312934438436
800801,1601603,1601602,3203205,1286.7935719490051,0.00011340248204305681
801802,1603605,1603604,3207209,1288.2892870903015,0.00011174629582910711
802803,1605607,1605606,3211213,1289.8050079345703,0.00011011421440798586
803804,1607609,1607608,3215217,1291.2809047698975,0.00010850588648736448
804805,1609611,1609610,3219221,1292.7582697868347,0.00010692096577713528
805806,1611613,1611612,3223225,1294.2292709350586,0.00010535911189890612
806807,1613615,1613614,3227229,1295.5240581035614,0.00010381998811226367
807808,1615617,1615616,3231233,1296.8411371707916,0.00010230326358851016
808809,1617619,1617618,3235237,1298.0839309692383,0.00010080861204642133
809810,1619621,1619620,3239241,1299.7081561088562,9.933571209330694e-05
810811,1621623,1621622,3243245,1301.4576649665833,9.78842464292029e-05
811812,1623625,1623624,3247249,1303.0418558120728,9.645390309742652e-05
812813,1625627,1625626,3251253,1304.65642786026,9.504437457508175e-05
813814,1627629,1627628,3255257,1306.327605009079,9.365535743199871e-05
814815,1629631,1629630,3259261,1307.8896570205688,9.228655289916787e-05
815816,1631633,1631632,3263265,1310.126643896103,9.093766664136638e-05
816817,1633635,1633634,3267269,1312.2132778167725,8.960840875715803e-05
817818,1635637,1635636,3271273,1313.8423500061035,8.829849286939861e-05
818819,1637639,1637638,3275277,1315.543293952942,8.700763760316477e-05
819820,1639641,1639640,3279281,1317.2821400165558,8.573556544888561e-05
820821,1641643,1641642,3283285,1318.780128955841,8.448200264865591e-05
821822,1643645,1643644,3287289,1320.2525088787079,8.324667942360975e-05
822823,1645647,1645646,3291293,1321.7966890335083,8.202933088341524e-05
823824,1647649,1647648,3295297,1323.2708089351654,8.082969452516409e-05
824825,1649651,1649650,3299301,1324.801232099533,7.964751250710833e-05
825826,1651653,1651652,3303305,1326.3721630573273,7.84825308528525e-05
826827,1653655,1653654,3307309,1327.9408581256866,7.733449911029311e-05
827828,1655657,1655656,3311313,1329.4162299633026,7.620317046530545e-05
828829,1657659,1657658,3315317,1330.9128019809723,7.508830140068312e-05
829830,1659661,1659660,3319321,1332.3906757831573,7.398965271931957e-05
830831,1661663,1661662,3323325,1333.8535799980164,7.290698772521864e-05
831832,1663665,1663664,3327329,1335.3884809017181,7.184007404248405e-05
832833,1665667,1665666,3331333,1336.8644618988037,7.078868213739042e-05
833834,1667669,1667668,3335337,1338.3443338871002,6.975258600050438e-05
834835,1669671,1669670,3339341,1339.8374450206757,6.873156303299766e-05
835836,1671673,1671672,3343345,1341.3246159553528,6.772539393296029e-05
836837,1673675,1673674,3347349,1342.7975449562073,6.673386189959274e-05
837838,1675677,1675676,3351353,1344.2859869003296,6.575675422482163e-05
838839,1677679,1677678,3355357,1345.7579708099365,6.479386070168403e-05
839840,1679681,1679680,3359361,1347.2893469333649,6.384497476119577e-05
840841,1681683,1681682,3363365,1348.7530658245087,6.290989222179633e-05
841842,1683685,1683684,3367369,1350.2690329551697,6.19884120851566e-05
842843,1685687,1685686,3371373,1351.7446870803833,6.108033630880527e-05
843844,1687689,1687688,3375377,1353.234512090683,6.018546980612882e-05
844845,1689691,1689690,3379381,1354.6878299713135,5.930362033268466e-05
845846,1691693,1691692,3383385,1356.1617777347565,5.843459848620114e-05
846847,1693695,1693694,3387389,1357.6684441566467,5.757821725183021e-05
847848,1695697,1695696,3391393,1359.1272299289703,5.673429279795528e-05
848849,1697699,1697698,3395397,1360.594969034195,5.5902643680383335e-05
849850,1699701,1699700,3399401,1362.0549519062042,5.5083091524466e-05
850851,1701703,1701702,3403405,1363.524003982544,5.427546000191796e-05
851852,1703705,1703704,3407409,1365.019569158554,5.347957551293803e-05
852853,1705707,1705706,3411413,1366.508148908615,5.2695267186209094e-05
853854,1707709,1707708,3415417,1367.9620220661163,5.192236653783766e-05
854855,1709711,1709710,3419421,1369.4443318843842,5.116070747135382e-05
855856,1711713,1711712,3423425,1370.952998161316,5.041012650508492e-05
856857,1713715,1713714,3427429,1372.4531779289246,4.967046209003456e-05
857858,1715717,1715716,3431433,1373.9150450229645,4.8941555633064127e-05
858859,1717719,1717718,3435437,1375.395026922226,4.822325070108491e-05
859860,1719721,1719720,3439441,1376.8651597499847,4.7515392679997603e-05
860861,1721723,1721722,3443445,1378.4070000648499,4.681782957050018e-05
861862,1723725,1723724,3447449,1379.9049689769745,4.613041153334052e-05
862863,1725727,1725726,3451453,1381.4221527576447,4.545299100300326e-05
863864,1727729,1727728,3455457,1382.8603377342224,4.478542246033612e-05
864865,1729731,1729730,3459461,1384.3347160816193,4.412756254623673e-05
865866,1731733,1731732,3463465,1385.8313629627228,4.347927006165264e-05
866867,1733735,1733734,3467469,1387.3279378414154,4.284040539914713e-05
867868,1735737,1735736,3471473,1388.785562992096,4.2210831907141255e-05
868869,1737739,1737738,3475477,1390.2688879966736,4.159041407092445e-05
869870,1739741,1739740,3479481,1391.715134859085,4.0979018649522914e-05
870871,1741743,1741742,3483485,1393.17950797081,4.0376514448325906e-05
871872,1743745,1743744,3487489,1394.6642599105835,3.9782772091712104e-05
872873,1745747,1745746,3491493,1396.1291718482971,3.919766379567591e-05
873874,1747749,1747748,3495497,1397.6149969100952,3.862106427732215e-05
874875,1749751,1749750,3499501,1399.113177061081,3.805284950431087e-05
875876,1751753,1751752,3503505,1400.6049449443817,3.7492897718038876e-05
876877,1753755,1753754,3507509,1402.0638608932495,3.6941088524145016e-05
877878,1755757,1755756,3511513,1403.5429890155792,3.639730334725755e-05
878879,1757759,1757758,3515517,1405.008817911148,3.5861425772054645e-05
879880,1759761,1759760,3519521,1406.479462146759,3.533334017902234e-05
880881,1761763,1761762,3523525,1407.979481935501,3.481293390450446e-05
881882,1763765,1763764,3527529,1409.6434428691864,3.430009462590533e-05
882883,1765767,1765766,3531533,1411.484699010849,3.3794712408052874e-05
883884,1767769,1767768,3535537,1413.5515389442444,3.329667913476442e-05
884885,1769771,1769770,3539541,1415.3629260063171,3.2805887371978315e-05
885886,1771773,1771772,3543545,1417.0535979270935,3.2322231845682836e-05
886887,1773775,1773774,3547549,1418.89950299263,3.1845608987168816e-05
887888,1775777,1775776,3551553,1420.8304669857025,3.137591625090863e-05
888889,1777779,1777778,3555557,1422.7317538261414,3.0913053137737734e-05
889890,1779781,1779780,3559561,1424.4330179691315,3.0456919830612605e-05
890891,1781783,1781782,3563565,1426.4975008964539,3.000741878622648e-05
891892,1783785,1783784,3567569,1428.2268159389496,2.9564453484454134e-05
892893,1785787,1785786,3571573,1430.4156420230865,2.912792842835188e-05
893894,1787789,1787788,3575577,1432.608125925064,2.8697750508399622e-05
894895,1789791,1789790,3579581,1434.7758378982544,2.8273827183511457e-05
895896,1791793,1791792,3583585,1437.3878519535065,2.7856067163156695e-05
896897,1793795,1793794,3587589,1439.9935519695282,2.7444381089480885e-05
897898,1795797,1795796,3591593,1441.7882459163666,2.7038680741497956e-05
898899,1797799,1797798,3595597,1443.655101776123,2.66388786940297e-05
899900,1799801,1799800,3599601,1445.8020498752594,2.6244889568260987e-05
900901,1801803,1801802,3603605,1447.7065749168396,2.5856628326437203e-05
901902,1803805,1803804,3607609,1450.1367328166962,2.5474011863479973e-05
902903,1805807,1805806,3611613,1451.8983829021454,2.50969582111793e-05
903904,1807809,1807808,3615617,1453.7612237930298,2.4725386424506723e-05
904905,1809811,1809810,3619621,1455.4466898441315,2.435921646792849e-05
905906,1811813,1811812,3623625,1457.2737147808075,2.3998370124900248e-05
906907,1813815,1813814,3627629,1459.1950969696045,2.364276986099867e-05
907908,1815817,1815816,3631633,1461.0484640598297,2.329233905129513e-05
908909,1817819,1817818,3635637,1462.7725780010223,2.2947003117224085e-05
909910,1819821,1819820,3639641,1464.5728459358215,2.2606687252846314e-05
910911,1821823,1821822,3643645,1466.3411450386047,2.2271319039646187e-05
911912,1823825,1823824,3647649,1468.1213910579681,2.194082628648175e-05
912913,1825827,1825826,3651653,1469.8348479270935,2.1615138166453107e-05
913914,1827829,1827828,3655657,1471.501788854599,2.1294184421094542e-05
914915,1829831,1829830,3659661,1473.4300210475922,2.0977896610929747e-05
915916,1831833,1831832,3663665,1475.1637349128723,2.0666206864916603e-05
916917,1833835,1833834,3667669,1477.0059559345245,2.0359048107820854e-05
917918,1835837,1835836,3671673,1478.9961309432983,2.0056354628650297e-05
918919,1837839,1837838,3675677,1480.5535039901733,1.975806117116008e-05
919920,1839841,1839840,3679681,1482.054827928543,1.9464104070721078e-05
920921,1841843,1841842,3683685,1483.614336013794,1.917442011745152e-05
921922,1843845,1843844,3687689,1485.1221470832825,1.8888947238338005e-05
922923,1845847,1845846,3691693,1486.632465839386,1.8607624269861844e-05
923924,1847849,1847848,3695697,1488.2514958381653,1.833039061693853e-05
924925,1849851,1849850,3699701,1489.789640903473,1.805718693503877e-05
925926,1851853,1851852,3703705,1491.274535894394,1.7787954675441142e-05
926927,1853855,1853854,3707709,1492.7660269737244,1.7522635971545242e-05
927928,1855857,1855856,3711713,1494.402529001236,1.726117397993221e-05
928929,1857859,1857858,3715717,1496.004823923111,1.7003512766677886e-05
929930,1859861,1859860,3719721,1497.5203218460083,1.674959662523179e-05
930931,1861863,1861862,3723725,1499.0119609832764,1.6499371554346e-05
931932,1863865,1863864,3727729,1500.5245537757874,1.62527835527726e-05
932933,1865867,1865866,3731733,1502.0019161701202,1.600978009719256e-05
933934,1867869,1867868,3735737,1503.7539639472961,1.577030855060002e-05
934935,1869871,1869870,3739741,1505.3386080265045,1.553431798129168e-05
935936,1871873,1871872,3743745,1506.864744901657,1.530175779862475e-05
936937,1873875,1873874,3747749,1508.3411228656769,1.5072577753016958e-05
937938,1875877,1875876,3751753,1509.8231809139252,1.4846728959128086e-05
938939,1877879,1877878,3755757,1511.507642030716,1.4624162758991588e-05
939940,1879881,1879880,3759761,1513.1447808742523,1.4404831745196134e-05
940941,1881883,1881882,3763765,1515.1914248466492,1.418868873770407e-05
941942,1883885,1883884,3767769,1516.7725749015808,1.3975687238598766e-05
942943,1885887,1885886,3771773,1518.4249818325043,1.3765781886831974e-05
943944,1887889,1887888,3775777,1519.9867010116577,1.3558927207668603e-05
944945,1889891,1889890,3779781,1521.6185750961304,1.3355079204302456e-05
945946,1891893,1891892,3783785,1523.4909060001373,1.315419410730101e-05
946947,1893895,1893894,3787789,1525.1843528747559,1.2956228601979092e-05
947948,1895897,1895896,3791793,1526.7677628993988,1.276114039683307e-05
948949,1897899,1897898,3795797,1528.5656139850616,1.2568888109854015e-05
949950,1899901,1899900,3799801,1530.2737839221954,1.237942956322513e-05
950951,1901903,1901902,3803805,1531.8696899414062,1.2192724966553214e-05
951952,1903905,1903904,3807809,1533.361788034439,1.2008733961010876e-05
952953,1905907,1905906,3811813,1534.8970580101013,1.182741686989175e-05
953954,1907909,1907908,3815817,1536.4033398628235,1.1648735153357848e-05
954955,1909911,1909910,3819821,1537.8795640468597,1.1472650498944859e-05
955956,1911913,1911912,3823825,1539.3513669967651,1.1299124821562145e-05
956957,1913915,1913914,3827829,1540.8749599456787,1.1128121172987449e-05
957958,1915917,1915916,3831833,1542.9959218502045,1.0959602946059022e-05
958959,1917919,1917918,3835837,1544.4957098960876,1.0793533760988794e-05
959960,1919921,1919920,3839841,1545.997329711914,1.0629878374857071e-05
960961,1921923,1921922,3843845,1547.4839498996735,1.0468601317370485e-05
961962,1923925,1923924,3847849,1549.0703799724579,1.0309668141417205e-05
962963,1925927,1925926,3851853,1550.6637721061707,1.0153044968319591e-05
963964,1927929,1927928,3855857,1552.1954097747803,9.998697805713164e-06
964965,1929931,1929930,3859861,1553.9368197917938,9.84659391178866e-06
965966,1931933,1931932,3863865,1555.8108568191528,9.696700658423651e-06
966967,1933935,1933934,3867869,1557.610366821289,9.54898564486939e-06
967968,1935937,1935936,3871873,1559.2241530418396,9.403417607245501e-06
968969,1937939,1937938,3875877,1560.7563989162445,9.259964713237423e-06
969970,1939941,1939940,3879881,1562.2928581237793,9.118596949519997e-06
970971,1941943,1941942,3883885,1563.8049409389496,8.979283620647038e-06
971972,1943945,1943944,3887889,1565.3481130599976,8.841994826980226e-06
972973,1945947,1945946,3891893,1566.8839600086212,8.706701237315428e-06
973974,1947949,1947948,3895897,1568.3782880306244,8.573373747822188e-06
974975,1949951,1949950,3899901,1569.8461270332336,8.441984050477913e-06
975976,1951953,1951952,3903905,1571.332997083664,8.312503496199497e-06
976977,1953955,1953954,3907909,1572.8247969150543,8.184904800145887e-06
977978,1955957,1955956,3911913,1574.3030829429626,8.059160336415516e-06
978979,1957959,1957958,3915917,1575.8027210235596,7.935243274914683e-06
979980,1959961,1959960,3919921,1577.2860589027405,7.81312701292336e-06
980981,1961963,1961962,3923925,1578.7963848114014,7.692785402468871e-06
981982,1963965,1963964,3927929,1580.2737619876862,7.574192409265379e-06
982983,1965967,1965966,3931933,1581.7904689311981,7.457322908521746e-06
983984,1967969,1967968,3935937,1583.3085758686066,7.3421518891336746e-06
984985,1969971,1969970,3939941,1584.7897918224335,7.228654339996865e-06
985986,1971973,1971972,3943945,1586.2635250091553,7.116806273188558e-06
986987,1973975,1973974,3947949,1587.7530798912048,7.00658347341232e-06
987988,1975977,1975976,3951953,1589.26691198349,6.897962521179579e-06
988989,1977979,1977978,3955957,1590.8007128238678,6.7909198833149276e-06
989990,1979981,1979980,3959961,1592.2923929691315,6.6854329361376585e-06
990991,1981983,1981982,3963965,1593.7760949134827,6.581478714906552e-06
991992,1983985,1983984,3967969,1595.2771549224854,6.479035164375091e-06
992993,1985987,1985986,3971973,1596.7735741138458,6.378080342983594e-06
993994,1987989,1987988,3975977,1598.2848460674286,6.278592422859219e-06
994995,1989991,1989990,3979981,1599.7650439739227,6.180550144563313e-06
995996,1991993,1991992,3983985,1601.247636795044,6.083932703404571e-06
996997,1993995,1993994,3987989,1602.7304220199585,5.988719067318016e-06
997998,1995997,1995996,3991993,1604.2101349830627,5.894889341107046e-06
998999,1997999,1997998,3995997,1605.7003049850464,5.8024224927066825e-06
1000000,2000001,2000000,4000001,1607.2158608436584,5.71129987747554e-06


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0009839534759521484,2181.2938132599165
1001,2003,2002,4005,1.6696579456329346,60.24885261358577
2002,4005,4004,8009,3.163712978363037,53.77859451869858
3003,6007,6006,12013,4.62731409072876,50.92243883003266
4004,8009,8008,16017,6.096297025680542,48.68494381511141
5005,10011,10010,20021,7.580941915512085,46.691969112691595
6006,12013,12012,24025,9.183863878250122,44.867160963980496
7007,14015,14014,28029,10.767898082733154,43.181007680888115
8008,16017,16016,32033,12.238910913467407,41.61577992971229
9009,18019,18018,36037,13.820996046066284,40.15858680114866
10010,20021,20020,40041,15.4914391040802,38.79909674755504
11011,22023,22022,44045,17.152826070785522,37.52847409324636
12012,24025,24024,48049,18.724649906158447,36.33883035729923
13013,26027,26026,52053,20.533782958984375,35.2229502662276
14014,28029,28028,56057,23.683632135391235,34.1741690618162
15015,30031,30030,60061,26.24609398841858,33.18632746839512
16016,32033,32032,64065,28.800775051116943,32.25376010823106
17017,34035,34034,68069,33.07889199256897,31.37129247508051
18018,36037,36036,72073,35.663373947143555,30.53423417371664
19019,38039,38038,76077,37.959240198135376,29.738363873788558
20020,40041,40040,80081,40.03615880012512,28.979905736756564
21021,42043,42042,84085,41.761090993881226,28.25549911295866
22022,44045,44044,88089,43.41641116142273,27.562163962825935
23023,46047,46046,92093,45.28204679489136,26.89726436380988
24024,48049,48048,96097,47.56490993499756,26.258472033869566
25025,50051,50050,100101,49.6177818775177,25.643731276923745
26026,52053,52052,104105,51.827003955841064,25.051226263215085
27027,54055,54054,108109,53.89559483528137,24.479351152850313
28028,56057,56056,112113,55.691056966781616,23.926683266755163
29029,58059,58058,116117,57.354275941848755,23.39195929771222
30030,60061,60060,120121,59.27090501785278,22.874054418249216
31031,62063,62062,124125,60.738879919052124,22.371964063629093
32032,64065,64064,128129,62.19211792945862,21.884788130571906
33033,66067,66066,132133,63.73110294342041,21.411717322285085
34034,68069,68068,136137,65.61202192306519,20.952021377713663
35035,70071,70070,140141,67.58785915374756,20.50503894039116
36036,72073,72072,144145,69.29348587989807,20.07016884483687
37037,74075,74074,148149,71.3541350364685,19.64686262284613
38038,76077,76076,152153,72.82718992233276,19.234618056184672
39039,78079,78078,156157,75.12943410873413,18.83297362496819
40040,80081,80080,160161,77.26256799697876,18.441503721751815
41041,82083,82082,164165,79.28955101966858,18.05989871991801
42042,84085,84084,168169,81.48197388648987,17.687711314216813
43043,86087,86086,172173,83.38214206695557,17.324595528035616
44044,88089,88088,176177,85.22617602348328,16.970233388048655
45045,90091,90090,180181,87.12790012359619,16.624327017803125
46046,92093,92092,184185,88.88261008262634,16.286596591251737
47047,94095,94094,188189,90.73016595840454,15.956778552026663
48048,96097,96096,192193,92.43196105957031,15.634624055713857
49049,98099,98098,196197,94.17009615898132,15.319897603406503
50050,100101,100100,200201,95.90395998954773,15.012375840133245
51051,102103,102102,204205,97.52496290206909,14.711846495718419
52052,104105,104104,208209,99.13337111473083,14.41810744892257
53053,106107,106106,212213,100.94622302055359,14.130965898484192
54054,108109,108108,216217,102.57635283470154,13.850237627052593
55055,110111,110110,220221,104.16241908073425,13.575746345965399
56056,112113,112112,224225,105.95493006706238,13.307323110548623
57057,114115,114114,228229,107.89903998374939,13.04480579704034
58058,116117,116116,232233,110.09079313278198,12.7880386334582
59059,118119,118118,236237,111.93464493751526,12.53687177778204
60060,120121,120120,240241,113.83798384666443,12.29116093771006
61061,122123,122122,244245,115.77823305130005,12.05076702700751
62062,124125,124124,248249,118.05190801620483,11.815555854122408
63063,126127,126126,252253,119.99100995063782,11.585397839303027
64064,128129,128128,256257,121.97187304496765,11.360167756933265
65065,130131,130130,260261,123.87839818000793,11.139744500219308
66066,132133,132132,264265,125.80260181427002,10.924010865721812
67067,134135,134134,268269,127.77046489715576,10.71285335553739
68068,136137,136136,272273,130.0548231601715,10.506161995206185
69069,138139,138138,276277,132.1311650276184,10.303830165656109
70070,140141,140140,280281,133.686420917511,10.105754447699951
71071,142143,142142,284285,135.21967196464539,9.911834477786101
72072,144145,144144,288289,136.73435997962952,9.721972813853085
73073,146147,146146,292293,138.29225420951843,9.536074810285413
74074,148149,148148,296297,139.75850582122803,9.354048501084549
75075,150151,150150,300301,141.22966694831848,9.175804490479663
76076,152153,152152,304305,142.67782282829285,9.001255850295024
77077,154155,154154,308309,144.1162040233612,8.83031802347898
78078,156157,156156,312313,145.59844708442688,8.662908733267386
79079,158159,158158,316317,147.1055290699005,8.498947897522385
80080,160161,160160,320321,149.5407431125641,8.338357547842861
81081,162163,162162,324325,151.11949396133423,8.181061753091512
82082,164165,164164,328329,152.829745054245,8.026986547022261
83083,166167,166166,332333,154.31337094306946,7.876059859733232
84084,168169,168168,336337,155.8827109336853,7.728211452692335
85085,170171,170170,340341,157.418527841568,7.583372857113432
86086,172173,172172,344345,158.95857906341553,7.441477315476504
87087,174175,174174,348349,160.39903807640076,7.302459726004599
88088,176177,176176,352353,161.83521509170532,7.166256589919158
89089,178179,178178,356357,163.3163230419159,7.032805961311624
90090,180181,180180,360361,165.3139591217041,6.902047399468074
91091,182183,182182,364365,166.83787989616394,6.773921923503281
92092,184185,184184,368369,168.6047878265381,6.64837196915289
93093,186187,186186,372373,170.0907051563263,6.525341347589574
94094,188189,188188,376377,172.08157515525818,6.404775206126601
95095,190191,190190,380381,173.73494601249695,6.286619990683107
96096,192193,192192,384385,175.29993414878845,6.170823409888385
97097,194195,194194,388389,176.77869510650635,6.057334400709124
98098,196197,196196,392393,178.56967210769653,5.9461030954939815
99099,198199,198198,396397,180.102303981781,5.837080790330106
100100,200201,200200,400401,182.4148828983307,5.730219914621898
101101,202203,202202,404405,184.00730800628662,5.625474001799489
102102,204205,204204,408409,185.44154524803162,5.522797661083928
103103,206207,206206,412413,186.90417098999023,5.422146550230082
104104,208209,208208,416417,188.3450710773468,5.3234773491861915
105105,210211,210210,420421,189.9736499786377,5.226747734608239
106106,212213,212212,424425,191.66082406044006,5.13191635517444
107107,214215,214214,428429,193.21473288536072,5.038942807655303
108108,216217,216216,432433,194.71286392211914,4.947787613692412
109109,218219,218218,436437,196.14271807670593,4.858412197248072
110110,220221,220220,440441,197.6390199661255,4.770778862692964
111111,222223,222222,444445,199.1283299922943,4.684850773497942
112112,224225,224224,448449,200.55268812179565,4.600591931503573
113113,226227,226226,452453,202.03079199790955,4.517967156740497
114114,228229,228228,456457,203.4871039390564,4.436942067780137
115115,230231,230230,460461,205.2219340801239,4.357483062592337
116116,232233,232232,464465,207.0720920562744,4.279557299893895
117117,234235,234234,468469,208.4624490737915,4.203132680966178
118118,236237,236236,472473,210.04730415344238,4.128177831932135
119119,238239,238238,476477,212.11453199386597,4.054662086471467
120120,240241,240240,480481,214.04526710510254,3.9825554689664386
121121,242243,242242,484485,215.4211459159851,3.9118286780598055
122122,244245,244244,488489,216.66057801246643,3.8424530706188307
123123,246247,246246,492493,219.16006803512573,3.7744006460890205
124124,248249,248248,496497,220.7719509601593,3.707644031230302
125125,250251,250250,500501,222.6248300075531,3.6421564652243887
126126,252253,252252,504505,225.8530468940735,3.5779117851444653
127127,254255,254254,508509,227.52686715126038,3.514884411777075
128128,256257,256256,512513,229.13877391815186,3.4530493357879095
129129,258259,258258,516517,230.9864330291748,3.392382104223998
130130,260261,260260,520521,232.8015341758728,3.3328588073426317
131131,262263,262262,524525,234.53265190124512,3.274456065760205
132132,264265,264264,528529,237.09429502487183,3.2171510179119878
133133,266267,266266,532533,239.28882503509521,3.1609213078180574
134134,268269,268268,536537,241.07564616203308,3.1057450731461813
135135,270271,270270,540541,242.73439502716064,3.051600933563236
136136,272273,272272,544545,244.28627490997314,2.998467979372208
137137,274275,274274,548549,245.80334305763245,2.94632576042477
138138,276277,276276,552553,247.29093503952026,2.895154275304776
139139,278279,278278,556557,248.88128995895386,2.844933960773915
140140,280281,280280,560561,250.40132904052734,2.795645681476799
141141,282283,282282,564565,251.88988995552063,2.7472707198971875
142142,284285,284284,568569,253.35518598556519,2.6997907665570438
143143,286287,286286,572573,254.90525007247925,2.6531879104605878
144144,288289,288288,576577,256.31336402893066,2.6074446297644727
145145,290291,290290,580581,257.7615761756897,2.5625437826835196
146146,292293,292292,584585,259.1866829395294,2.5184685986150726
147147,294295,294294,588589,260.608873128891,2.475202669481064
148148,296297,296296,592593,262.13785004615784,2.432729941282787
149149,298299,298298,596597,263.67859506607056,2.3910347058625803
150150,300301,300300,600601,265.21803092956543,2.350101592866622
151151,302303,302302,604605,266.75970005989075,2.309915561904859
152152,304305,304304,608609,268.63935804367065,2.2704618949030646
153153,306307,306306,612613,270.14275002479553,2.231726188642824
154154,308309,308308,616617,271.55128598213196,2.193694347482392
155155,310311,310310,620621,272.97471499443054,2.1563525762577456
156156,312313,312312,624625,274.6565852165222,2.119687373355873
157157,314315,314314,628629,276.13836097717285,2.0836855239583656
158158,316317,316316,632633,278.0097289085388,2.048334093449739
159159,318319,318318,636637,280.2850179672241,2.0136204209876496
160160,320321,320320,640641,282.0237910747528,1.9795321132280606
161161,322323,322322,644645,283.4800832271576,1.9460570382061633
162162,324325,324324,648649,284.91242694854736,1.9131833193656576
163163,326327,326326,652653,286.3386940956116,1.8808993297316192
164164,328329,328328,656657,288.0149040222168,1.8491936862288867
165165,330331,330330,660661,290.1029438972473,1.8180552441358486
166166,332333,332332,664665,292.3770809173584,1.7874730916739736
167167,334335,334334,668669,294.1020550727844,1.7574365447288756
168168,336337,336336,672673,295.7968502044678,1.7279351416999589
169169,338339,338338,676677,297.94375491142273,1.6989586384734139
170170,340341,340340,680681,299.9653389453888,1.6704970035186761
171171,342343,342342,684685,301.5440249443054,1.64254041310312
172172,344345,344344,688689,303.13552594184875,1.6150792466210078
173173,346347,346346,692693,304.6358880996704,1.5881040820366934
174174,348349,348348,696697,306.5122961997986,1.5616056914379897
175175,350351,350350,700701,308.1090998649597,1.5355750366945813
176176,352353,352352,704705,309.8981499671936,1.5100032652231903
177177,354355,354354,708709,312.41674304008484,1.484881705852672
178178,356357,356356,712713,314.35854601860046,1.460201864789724
179179,358359,358358,716717,315.8666977882385,1.4359554216796369
180180,360361,360360,720721,317.7357540130615,1.412134225763566
181181,362363,362362,724725,319.356586933136,1.3887302921250466
182182,364365,364364,728729,321.00889587402344,1.3657357980270035
183183,366367,366366,732733,322.57368302345276,1.343143079338006
184184,368369,368368,736737,324.13319993019104,1.3209446270398075
185185,370371,370370,740741,325.6753680706024,1.29913308382163
186186,372373,372372,744745,327.37358713150024,1.277701240752208
187187,374375,374374,748749,328.9097800254822,1.2566420340319837
188188,376377,376376,752753,330.46217584609985,1.235948541822836
189189,378379,378378,756757,332.12954902648926,1.2156139811509092
190190,380381,380380,760761,333.7189300060272,1.1956317048839082
191191,382383,382382,764765,335.3153929710388,1.1759951987791055
192192,384385,384384,768769,336.94352197647095,1.1566980785999021
193193,386387,386386,772773,338.43749499320984,1.137734087301169
194194,388389,388388,776777,339.8766419887543,1.1190970922805263
195195,390391,390390,780781,341.2344710826874,1.1007810826930609
196196,392393,392392,784785,342.53058409690857,1.0827801668285701
197197,394395,394394,788789,343.8428809642792,1.0650885695516763
198198,396397,396396,792793,345.1029019355774,1.0477006297995786
199199,398399,398398,796797,346.41079807281494,1.0306107981385821
200200,400401,400400,800801,347.74329113960266,1.0138136343782662
201201,402403,402402,804805,349.0555281639099,0.99730380523863
202202,404405,404404,808809,350.77065992355347,0.9810760820740825
203203,406407,406406,812813,352.4964859485626,0.9651253386472263
204204,408409,408408,816817,354.17509484291077,0.9494465489558479
205205,410411,410410,820821,356.0206320285797,0.9340347851087927
206206,412413,412412,824825,357.8198239803314,0.9188852152507252
207207,414415,414414,828829,359.66778206825256,0.9039931015354341
208208,416417,416416,832833,361.4510099887848,0.8893537981438158
209209,418419,418418,836837,363.2014911174774,0.8749627493481285
210210,420421,420420,840841,364.94093894958496,0.860815487621494
211211,422423,422422,844845,366.6757228374481,0.8469076317869622
212212,424425,424424,848849,368.6792092323303,0.8332348852131872
213213,426427,426426,852853,370.2458710670471,0.819793034046711
214214,428429,428428,856857,371.8934509754181,0.80657794548722
215215,430431,430430,860861,373.462033033371,0.7935855661008873
216216,432433,432432,864865,375.11010098457336,0.7808119201708905
217217,434435,434434,868869,376.93531107902527,0.7682531080861281
218218,436437,436436,872873,378.54048919677734,0.7559053047658608
219219,438439,438438,876877,380.1064670085907,0.7437647581198235
220220,440441,440440,880881,381.7310380935669,0.7318277875419881
221221,442443,442442,884885,383.29565620422363,0.7200907824393425
222222,444445,444444,888889,384.830952167511,0.7085502007923878
223223,446447,446446,892893,386.39608502388,0.6972025677483771
224224,448449,448448,896897,387.9812870025635,0.6860444742450227
225225,450451,450450,900901,389.8032958507538,0.6750725756654674
226226,452453,452452,904905,391.34513306617737,0.6642835905234961
227227,454455,454454,908909,393.08430004119873,0.6536742991762594
228228,456457,456456,912913,394.7148640155792,0.6432415425667841
229229,458459,458458,916917,396.19312596321106,0.6329822209938811
230230,460461,460460,920921,397.7707030773163,0.6228932929084294
231231,462463,462462,924925,399.29266905784607,0.6129717737373994
232232,464465,464464,928929,401.29933404922485,0.6032147347319778
233233,466467,466466,932933,403.229159116745,0.5936193018420681
234234,468469,468468,936937,405.00232911109924,0.5841826546159155
235235,470471,470470,940941,406.90173411369324,0.5749020251213324
236236,472473,472472,944945,408.5433487892151,0.5657746968934134
237237,474475,474474,948949,410.01588702201843,0.5567980039025997
238238,476477,476476,952953,411.4559841156006,0.5479693295466177
239239,478479,478478,956957,412.91487407684326,0.5392861056643596
240240,480481,480480,960961,414.3854429721832,0.5307458115685222
241241,482483,482482,964965,415.81877398490906,0.5223459731035973
242242,484485,484484,968969,417.26158809661865,0.5140841617194383
243243,486487,486486,972973,418.70071601867676,0.5059579935683587
244244,488489,488488,976977,420.20594906806946,0.49796512861928477
245245,490491,490490,980981,421.7397108078003,0.4901032697921437
246246,492493,492492,984985,423.23574209213257,0.48237016211021455
247247,494495,494494,988989,424.8937478065491,0.4747635918703281
248248,496497,496496,992993,426.5734930038452,0.46728138583216605
249249,498499,498498,996997,428.159282207489,0.45992141042222556
250250,500501,500500,1001001,429.7604720592499,0.4526815709575658
251251,502503,502502,1005005,431.52616691589355,0.44555981088353747
252252,504505,504504,1009009,433.17100405693054,0.4385541110293616
253253,506507,506506,1013013,434.68461513519287,0.43166248887848724
254254,508509,508508,1017017,436.2947781085968,0.4248829978549793
255255,510511,510510,1021021,437.92327213287354,0.41821372662400336
256256,512513,512512,1025025,439.5201289653778,0.411652798407772
257257,514515,514514,1029029,440.9994468688965,0.4051983703160431
258258,516517,516516,1033033,442.63205909729004,0.3988486326893508
259259,518519,518518,1037037,444.43250799179077,0.3926018084574707
260260,520521,520520,1041041,446.0130658149719,0.3864561525105046
261261,522523,522522,1045045,447.52954506874084,0.38040995108281095
262262,524525,524524,1049049,449.13062596321106,0.37446152115069253
263263,526527,526526,1053053,450.8875710964203,0.3686092098409972
264264,528529,528528,1057057,452.4840760231018,0.36285139385404364
265265,530531,530530,1061061,454.1752419471741,0.357186478896665
266266,532533,532532,1065065,455.85459184646606,0.35161289912787197
267267,534535,534534,1069069,457.6705560684204,0.3461291166159981
268268,536537,536536,1073073,459.33516693115234,0.34073362080619063
269269,538539,538538,1077077,461.1102559566498,0.33542492800006585
270270,540541,540540,1081081,463.0643298625946,0.33020158084468676
271271,542543,542542,1085085,464.5750410556793,0.3250621478332505
272272,544545,544544,1089089,466.03645610809326,0.32000522281487065
273273,546547,546546,1093093,467.6741669178009,0.31502942451572835
274274,548549,548548,1097097,469.3930480480194,0.3101333960685224
275275,550551,550550,1101101,470.95694398880005,0.305315804551924
276276,552553,552552,1105105,472.3938479423523,0.3005753405401492
277277,554555,554554,1109109,473.80244398117065,0.29591071766071764
278278,556557,556556,1113113,475.17788887023926,0.2913206721618735
279279,558559,558558,1117117,476.5411071777344,0.286803962487852
280280,560561,560560,1121121,477.88575410842896,0.2823593688640358
281281,562563,562562,1125125,479.22669506073,0.2779856928882509
282282,564565,564564,1129129,480.61730694770813,0.27368175713434084
283283,566567,566566,1133133,482.1757779121399,0.2694464047575593
284284,568569,568568,1137137,483.75297713279724,0.2652784991145154
285285,570571,570570,1141141,485.3954339027405,0.26117692338573306
286286,572573,572572,1145145,487.31657791137695,0.2571405802082154
287287,574575,574574,1149149,488.94406485557556,0.25316839131471625
288288,576577,576576,1153153,490.4817090034485,0.24925929718017414
289289,578579,578578,1157157,492.12048506736755,0.2454122566754222
290290,580581,580580,1161161,493.83285999298096,0.24162624672635502
291291,582583,582582,1165165,495.8299889564514,0.23790026198321357
292292,584585,584584,1169169,497.68215322494507,0.23423331449180296
293293,586587,586586,1173173,499.38504219055176,0.23062443337573768
294294,588589,588588,1177177,501.8713300228119,0.22707266452164276
295295,590591,590590,1181181,503.52168583869934,0.2235770702712898
296296,592593,592592,1185185,505.22984409332275,0.22013672912214588
297297,594595,594594,1189189,506.9760990142822,0.2167507354299687
298298,596597,596596,1193193,508.6503999233246,0.21341819912038318
299299,598599,598598,1197197,510.3311870098114,0.21013824540432324
300300,600601,600600,1201201,511.8785240650177,0.20691001449984014
301301,602603,602602,1205205,513.5470499992371,0.20373266135857193
302302,604605,604604,1209209,515.0871589183807,0.20060535539880675
303303,606607,606606,1213213,516.7402820587158,0.19752728024297994
304304,608609,608608,1217217,518.3992919921875,0.19449763345937754
305305,610611,610610,1221221,520.1949229240417,0.19151562631088836
306306,612613,612612,1225225,521.9581279754639,0.18858048350625722
307307,614615,614614,1229229,523.4217681884766,0.18569144295884144
308308,616617,616616,1233233,524.8570930957794,0.18284775554730004
309309,618619,618618,1237237,526.2965159416199,0.18004868488264947
310310,620621,620620,1241241,527.777557849884,0.17729350707929825
311311,622623,622622,1245245,529.2083430290222,0.1745815105307429
312312,624625,624624,1249249,530.6974198818207,0.17191199568833326
313313,626627,626626,1253253,532.1526761054993,0.16928427484674557
314314,628629,628628,1257257,533.6883990764618,0.1666976719309332
315315,630631,630630,1261261,535.125,0.16415152228807983
316316,632633,632632,1265265,536.5987901687622,0.16164517248546417
317317,634635,634634,1269269,538.0160109996796,0.15917798010809747
318318,636637,636636,1273273,539.5131828784943,0.1567493135642053
319319,638639,638638,1277277,541.0694680213928,0.1543585518920736
320320,640641,640640,1281281,542.6053149700165,0.15200508457144224
321321,642643,642642,1285285,544.2889561653137,0.14968831133785443
322322,644645,644644,1289289,545.986964225769,0.14740764200178091
323323,646647,646646,1293293,547.6532771587372,0.14516249626922217
324324,648649,648648,1297297,549.3766748905182,0.14295230356788124
325325,650651,650650,1301301,550.9445478916168,0.14077650287424603
326326,652653,652652,1305305,552.4848330020905,0.13863454254658336
327327,654655,654654,1309309,553.9793000221252,0.13652588015827405
328328,656657,656656,1313313,555.4910790920258,0.13444998233683236
329329,658659,658658,1317317,557.0482621192932,0.13240632460349389
330330,660661,660660,1321321,558.472804069519,0.1303943912188288
331331,662663,662662,1325325,559.9250028133392,0.12841367502767298
332332,664665,664664,1329329,561.3666439056396,0.12646367731008468
333333,666667,666666,1333333,562.7959489822388,0.12454390763298306
334334,668669,668668,1337337,564.2064440250397,0.1226538837059934
335335,670671,670670,1341341,565.6534790992737,0.12079313123842894
336336,672673,672672,1345345,567.1709840297699,0.118961183800252
337337,674675,674674,1349349,568.6026740074158,0.117157582685536
338338,676677,676676,1353353,570.0475978851318,0.11538187677740552
339339,678679,678678,1357357,571.4838471412659,0.11363362241672803
340340,680681,680680,1361361,572.9574601650238,0.11191238327194242
341341,682683,682682,1365365,574.4048690795898,0.11021773021286663
342342,684685,684684,1369369,575.8666501045227,0.10854924118461895
343343,686687,686686,1373373,577.3488941192627,0.10690650108722366
344344,688689,688688,1377377,578.797091960907,0.1052891016530566
345345,690691,690690,1381381,580.2893621921539,0.10369664133042988
346346,692693,692692,1385385,581.8208889961243,0.1021287251674039
347347,694695,694694,1389389,583.3374769687653,0.10058496469798683
348348,696697,696696,1393393,584.8461689949036,0.09906497782992574
349349,698699,698698,1397397,586.4084389209747,0.09756838873602192
350350,700701,700700,1401401,587.9082269668579,0.09609482774612843
351351,702703,702702,1405405,589.3546249866486,0.09464393124153503
352352,704705,704704,1409409,590.8081498146057,0.09321534155037625
353353,706707,706706,1413413,592.2702281475067,0.09180870684758702
354354,708709,708708,1417417,593.770182132721,0.09042368105338028
355355,710711,710710,1421421,595.2783370018005,0.08905992373559002
356356,712713,712712,1425425,596.7645599842072,0.08771710001315114
357357,714715,714714,1429429,598.492458820343,0.08639488046162569
358358,716717,716716,1433433,600.0350000858307,0.08509294101952491
359359,718719,718718,1437437,601.4958040714264,0.08381096289792822
360360,720721,720720,1441441,602.945139169693,0.08254863249078426
361361,722723,722722,1445445,604.3713519573212,0.08130564128532569
362362,724725,724724,1449449,605.8207380771637,0.08008168577828201
363363,726727,726726,1453453,607.2572090625763,0.07887646738856802
364364,728729,728728,1457457,608.762629032135,0.07768969237451984
365365,730731,730730,1461461,610.3029429912567,0.07652107175306355
366366,732733,732732,1465465,611.8888008594513,0.07537032121763332
367367,734735,734734,1469469,613.6215999126434,0.07423716106063694
368368,736737,736736,1473473,615.3494729995728,0.07312131609421613
369369,738739,738738,1477477,616.9775190353394,0.07202251557657746
370370,740741,740740,1481481,618.5902388095856,0.0709404931338895
371371,742743,742742,1485485,620.2123072147369,0.0698749866895696
372372,744745,744744,1489489,621.6367220878601,0.06882573839016004
373373,746747,746746,1493493,623.0945010185242,0.06779249453552438
374374,748749,748748,1497497,624.5372588634491,0.06677500550847526
375375,750751,750750,1501501,626.0132751464844,0.06577302570667598
376376,752753,752752,1505505,627.4589359760284,0.06478631347522423
377377,754755,754754,1509509,628.8710279464722,0.06381463104060003
378378,756757,756756,1513513,630.3584260940552,0.06285774444563685
379379,758759,758758,1517517,631.9238178730011,0.061915423486425425
380380,760761,760760,1521521,633.4860048294067,0.06098744164864911
381381,762763,762762,1525525,635.161367893219,0.0600735760463067
382382,764765,764764,1529529,636.6593909263611,0.059173607362026814
383383,766767,766766,1533533,638.1915829181671,0.058287319787154956
384384,768769,768768,1537537,639.6464040279388,0.05741450096252265
385385,770771,770770,1541541,641.0625400543213,0.05655494192308197
386386,772773,772772,1545545,642.5540599822998,0.055708437039356795
387387,774775,774774,1549549,643.9835119247437,0.05487478396366896
388388,776777,776776,1553553,645.4862229824066,0.05405378357488644
389389,778779,778778,1557557,646.9780042171478,0.05324523992567265
390390,780781,780780,1561561,648.4641110897064,0.05244896018916734
391391,782783,782782,1565565,649.9340319633484,0.051664754608054864
392392,784785,784784,1569569,651.3830277919769,0.05089243644351882
393393,786787,786786,1573573,652.8975739479065,0.05013182192499244
394394,788789,788788,1577577,654.3818590641022,0.04938273020229644
395395,790791,790790,1581581,655.9312360286713,0.048644983296867395
396396,792793,792792,1585585,657.401789188385,0.04791840605378184
397397,794795,794794,1589589,658.8330299854279,0.04720282609673632
398398,796797,796796,1593593,660.2873740196228,0.04649807378098103
399399,798799,798798,1597597,661.7559909820557,0.04580398214955039
400400,800801,800800,1601601,663.2076749801636,0.04512038688824305
401401,802803,802802,1605605,664.6898150444031,0.0444471262829893
402402,804805,804804,1609609,666.1517980098724,0.04378404117642276
403403,806807,806806,1613613,667.6000380516052,0.04313097492718043
404404,808809,808808,1617617,669.0415840148926,0.04248777336749754
405405,810811,810810,1621621,670.4828510284424,0.04185428476341713
406406,812813,812812,1625625,671.9608948230743,0.041230359774772296
407407,814815,814814,1629629,673.3998591899872,0.040615851416646365
408408,816817,816816,1633633,674.8461050987244,0.040010615019923534
409409,818819,818818,1637637,676.3115549087524,0.03941450819479542
410410,820821,820820,1641641,677.8078439235687,0.03882739079244857
411411,822823,822822,1645645,679.2971251010895,0.03824912486879839
412412,824825,824824,1649649,680.7185609340668,0.0376795746501557
413413,826827,826826,1653653,682.1737430095673,0.03711860649514165
414414,828829,828828,1657657,683.6113698482513,0.036566088862855395
415415,830831,830830,1661661,685.0468828678131,0.036021892276608014
416416,832833,832832,1665665,686.570060968399,0.03548588929231755
417417,834835,834834,1669669,689.2098321914673,0.03495795446349348
418418,836837,836836,1673673,690.9753849506378,0.034437964310995994
419419,838839,838838,1677677,692.6462140083313,0.03392579728972578
420420,840841,840840,1681681,694.4051649570465,0.03342133375770118
421421,842843,842842,1685685,696.1382439136505,0.032924455945590125
422422,844845,844844,1689689,697.6633570194244,0.03243504792646945
423423,846847,846846,1693693,699.1464660167694,0.03195299558547049
424424,848849,848848,1697697,700.6245868206024,0.03147818659147106
425425,850851,850850,1701701,702.0994689464569,0.03101051036719582
426426,852853,852852,1705705,703.6021540164948,0.030549858062272506
427427,854855,854854,1709709,705.0634100437164,0.030096122524582825
428428,856857,856856,1713713,706.6144869327545,0.029649198272750255
429429,858859,858858,1717717,708.2113530635834,0.02920898147021944
430430,860861,860860,1721721,709.878662109375,0.028775369898085046
431431,862863,862862,1725725,711.452586889267,0.028348262929171142
432432,864865,864864,1729729,713.1466720104218,0.02792756150279274
433433,866867,866866,1733733,714.6638031005859,0.027513168099631002
434434,868869,868868,1737737,716.1408429145813,0.027104986716722124
435435,870871,870870,1741741,717.582967042923,0.026702922843355736
436436,872873,872872,1745745,719.0356919765472,0.026306883437200668
437437,874875,874874,1749749,720.524374961853,0.025916776900885452
438438,876877,876876,1753753,722.0119321346283,0.025532513058919903
439439,878879,878878,1757757,723.4512269496918,0.025154003134503
440440,880881,880880,1761761,724.9574339389801,0.024781159728036073
441441,882883,882882,1765765,726.4278008937836,0.024413896794840184
442442,884885,884884,1769769,727.913323879242,0.024052129622873508
443443,886887,886886,1773773,729.430125951767,0.02369577481260876
444444,888889,888888,1777777,730.9219810962677,0.02334475025475058
445445,890891,890890,1781781,732.3799939155579,0.02299897511193194
446446,892893,892892,1785785,733.8626580238342,0.022658369795408362
447447,894895,894894,1789789,735.300201177597,0.022322855948686993
448448,896897,896896,1793793,736.772381067276,0.021992356424334503
449449,898899,898898,1797797,738.234601020813,0.021666795268288297
450450,900901,900900,1801801,739.7017419338226,0.02134609769814233
451451,902903,902902,1805805,741.2144930362701,0.02103019008609408
452452,904905,904904,1809809,742.6780059337616,0.020718999940072536
453453,906907,906906,1813813,744.1905798912048,0.020412455886003045
454454,908909,908908,1817817,745.6756520271301,0.020110487650072173
455455,910911,910910,1821821,747.149729013443,0.019813026041333615
456456,912913,912912,1825825,748.6158480644226,0.01952000293420042
457457,914915,914914,1829829,750.1117749214172,0.01923135125218778
458458,916917,916916,1833833,751.6019570827484,0.018947004950973678
459459,918919,918918,1837837,753.070004940033,0.018666899002369064
460460,920921,920920,1841841,754.5317118167877,0.018390969378174304
461461,922923,922922,1845845,755.9819691181183,0.01811915303414935
462462,924925,924924,1849849,757.4750790596008,0.017851387894552317
463463,926927,926926,1853853,758.9985311031342,0.017587612837587585
464464,928929,928928,1857857,760.4652781486511,0.017327767679944373
465465,930931,930930,1861861,761.9680449962616,0.01707179316122165
466466,932933,932932,1865865,763.4194002151489,0.016819630930967833
467467,934935,934934,1869869,764.8900499343872,0.016571223532992008
468468,936937,936936,1873873,766.4562449455261,0.016326514391948876
469469,938939,938938,1877877,767.9157190322876,0.016085447800264774
470470,940941,940940,1881881,769.3799841403961,0.01584796890256257
471471,942943,942942,1885885,770.9816439151764,0.015614023683951928
472472,944945,944944,1889889,772.5915930271149,0.015383558956727938
473473,946947,946946,1893893,774.2524840831757,0.015156522346501333
474474,948949,948948,1897897,775.9143130779266,0.014932862280147674
475475,950951,950950,1901901,777.595263004303,0.01471252797307443
476476,952953,952952,1905905,779.232006072998,0.014495469417397544
477477,954955,954954,1909909,780.703910112381,0.014281637368299016
478478,956957,956956,1913913,782.292023897171,0.014070983334477205
479479,958959,958958,1917917,783.7792038917542,0.013863459563935976
480480,960961,960960,1921921,785.2403402328491,0.013659019033980258
481481,962963,962962,1925925,786.7404689788818,0.013457615439506299
482482,964965,964964,1929929,788.2042038440704,0.01325920318140561
483483,966967,966966,1933933,789.8063237667084,0.013063737356105776
484484,968969,968968,1937937,791.3390340805054,0.012871173744088082
485485,970971,970970,1941941,792.912966966629,0.012681468800565199
486486,972973,972972,1945945,794.4055359363556,0.01249457964274825
487487,974975,974974,1949949,795.8648648262024,0.012310464041775049
488488,976977,976976,1953953,797.3643610477448,0.012129080411227733
489489,978979,978978,1957957,798.8611829280853,0.011950387797696749
490490,980981,980980,1961961,800.3559029102325,0.011774345870776415
491491,982983,982982,1965965,801.9685900211334,0.011600914912946791
492492,984985,984984,1969969,803.5017139911652,0.011430055810933482
493493,986987,986986,1973973,805.0025889873505,0.01126173004604425
494494,988989,988988,1977977,806.481164932251,0.011095899684391952
495495,990991,990990,1981981,807.9949688911438,0.010932527368254341
496496,992993,992992,1985985,809.4249520301819,0.010771576307206487
497497,994995,994994,1989989,810.893639087677,0.010613010269480583
498498,996997,996996,1993993,812.4361848831177,0.010456793572757306
499499,998999,998998,1997997,813.9162600040436,0.01030289107632143
500501,1001003,1001002,2002005,815.4065730571747,0.010151117828968381
501502,1003005,1003004,2006009,816.8923711776733,0.010001742659937918
502503,1005007,1005006,2010013,818.4386148452759,0.009854579399416252
503504,1007009,1007008,2014017,819.9042501449585,0.009709594990113146
504505,1009011,1009010,2018021,821.3893020153046,0.009566756874619387
505506,1011013,1011012,2022025,822.8900690078735,0.009426032988926636
506507,1013015,1013014,2026029,824.3536620140076,0.009287391754696728
507508,1015017,1015016,2030033,825.7930040359497,0.009150802070962527
508509,1017019,1017018,2034037,827.3069770336151,0.00901623330730672
509510,1019021,1019020,2038041,828.7627370357513,0.008883655296926918
510511,1021023,1021022,2042045,830.2559690475464,0.008753038329018636
511512,1023025,1023024,2046049,831.7478840351105,0.008624353141499341
512513,1025027,1025026,2050053,833.2845289707184,0.008497570914983044
513514,1027029,1027028,2054057,835.7876358032227,0.008372663265390656
514515,1029031,1029030,2058061,837.7868030071259,0.00824960223724247
515516,1031033,1031032,2062065,839.9445850849152,0.008128360297064319
516517,1033035,1033034,2066069,841.7072658538818,0.008008910326907426
517518,1035037,1035036,2070073,843.3236300945282,0.007891225618664066
518519,1037039,1037038,2074077,844.806036233902,0.007775279866336859
519520,1039041,1039040,2078081,846.3156588077545,0.0076610471616049836
520521,1041043,1041042,2082085,847.7583639621735,0.007548501985752409
521522,1043045,1043044,2086089,849.2749171257019,0.007437619205575174
522523,1045047,1045046,2090093,850.740510225296,0.007328374066446486
523524,1047049,1047048,2094097,852.2233719825745,0.007220742186859752
524525,1049051,1049050,2098101,853.7247619628906,0.00711469955172106
525526,1051053,1051052,2102105,855.3491880893707,0.007010222509052255
526527,1053055,1053054,2106109,856.9446449279785,0.006907287761464431
527528,1055057,1055056,2110113,858.4131319522858,0.00680587236320207
528529,1057059,1057058,2114117,859.8070387840271,0.006705953713321833
529530,1059061,1059060,2118121,861.2618319988251,0.006607509551372459
530531,1061063,1061062,2122125,862.7345309257507,0.006510517951255679
531532,1063065,1063064,2126129,864.211315870285,0.006414957316451364
532533,1065067,1065066,2130133,865.7080838680267,0.006320806375924803
533534,1067069,1067068,2134137,867.1753840446472,0.006228044177078118
534535,1069071,1069070,2138141,868.6521461009979,0.006136650083362838
535536,1071073,1071072,2142145,870.1315848827362,0.006046603767231318
536537,1073075,1073074,2146149,871.596687078476,0.0059578852072945665
537538,1075077,1075076,2150153,873.0787448883057,0.005870474682069471
538539,1077079,1077078,2154157,874.5608150959015,0.005784352766454504
539540,1079081,1079080,2158161,876.0117301940918,0.005699500326954876
540541,1081083,1081082,2162165,877.4779171943665,0.005615898517021378
541542,1083085,1083084,2166169,879.0255579948425,0.005533528772502905
542543,1085087,1085086,2170173,880.4559378623962,0.005452372808349537
543544,1087089,1087088,2174177,881.9250128269196,0.005372412613382949
544545,1089091,1089090,2178181,883.4006109237671,0.005293630445976305
545546,1091093,1091092,2182185,884.8798758983612,0.0052160088310984065
546547,1093095,1093094,2186189,886.3863840103149,0.005139530555311467
547548,1095097,1095096,2190193,887.9234819412231,0.005064178662678387
548549,1097099,1097098,2194197,889.5155827999115,0.004989936451806898
549550,1099101,1099100,2198201,891.0734620094299,0.004916787470733652
550551,1101103,1101102,2202205,892.6367011070251,0.004844715514764175
551552,1103105,1103104,2206209,894.2100839614868,0.004773704620561148
552553,1105107,1105106,2210213,895.8042430877686,0.004703739064666479
553554,1107109,1107108,2214217,897.2574388980865,0.004634803358499084
554555,1109111,1109110,2218221,898.7972378730774,0.004566882244603221
555556,1111113,1111112,2222225,900.3925218582153,0.004499960694829497
556557,1113115,1113114,2226229,901.9729990959167,0.004434023904764217
557558,1115117,1115116,2230233,903.6478490829468,0.004369057291910394
558559,1117119,1117118,2234237,905.3089320659637,0.004305046491253961
559560,1119121,1119120,2238241,906.9878799915314,0.004241977352535287
560561,1121123,1121122,2242245,908.6601960659027,0.004179835937293319
561562,1123125,1123124,2246249,910.2162971496582,0.004118608515000233
562563,1125127,1125126,2250253,911.7885820865631,0.004058281559991883
563564,1127129,1127128,2254257,913.2641661167145,0.00399884174851195
564565,1129131,1129130,2258261,914.733980178833,0.003940275956210826
565566,1131133,1131132,2262265,916.1966319084167,0.003882571254280265
566567,1133135,1133134,2266269,917.6605370044708,0.0038257149067248974
567568,1135137,1135136,2270273,919.1953361034393,0.0037696943677474337
568569,1137139,1137138,2274277,920.7724120616913,0.0037144972787928054
569570,1139141,1139140,2278281,922.3909401893616,0.003660111465251248
570571,1141143,1141142,2282285,923.8896570205688,0.0036065249342982497
571572,1143145,1143144,2286289,925.391438961029,0.0035537258718250087
572573,1145147,1145146,2290293,926.8707740306854,0.0035017026400510076
573574,1147149,1147148,2294297,928.4001331329346,0.0034504437742270966
574575,1149151,1149150,2298301,929.9638948440552,0.0033999379805891294
575576,1151153,1151152,2302305,931.5485119819641,0.0033501741337431667
576577,1153155,1153154,2306309,933.1118359565735,0.0033011412740506785
577578,1155157,1155156,2310313,934.6601948738098,0.0032528286045589994
578579,1157159,1157158,2314317,936.17067694664,0.003205225489637087
579580,1159161,1159160,2318321,937.6384098529816,0.0031583214519059766
580581,1161163,1161162,2322325,939.1339681148529,0.003112106169623985
581582,1163165,1163164,2326329,940.6095700263977,0.0030665694748677197
582583,1165167,1165166,2330333,942.1545219421387,0.00302170135103097
583584,1167169,1167168,2334337,943.6729960441589,0.0029774919304372816
584585,1169171,1169170,2338341,945.1663022041321,0.002933931492066222
585586,1171173,1171172,2342345,946.6570389270782,0.002891010459620702
586587,1173175,1173174,2346349,948.161553144455,0.002848719399366928
587588,1175177,1175176,2350353,949.6589920520782,0.002807049017292229
588589,1177179,1177178,2354357,951.1646339893341,0.00276599015796819
589590,1179181,1179180,2358361,952.6601808071136,0.0027255338018221664
590591,1181183,1181182,2362365,954.1357970237732,0.0026856710634319825
591592,1183185,1183184,2366369,955.6106588840485,0.002646393189252194
592593,1185187,1185186,2370373,957.0940709114075,0.0026076915557950997
593594,1187189,1187188,2374377,958.5478270053864,0.0025695576675843768
594595,1189191,1189190,2378381,960.0569751262665,0.00253198315579084
595596,1191193,1191192,2382385,961.6514971256256,0.0024949597748218366
596597,1193195,1193194,2386389,963.1564462184906,0.002458479402434932
597598,1195197,1195196,2390393,964.6486802101135,0.00242253403655468
598599,1197199,1197198,2394397,966.2585179805756,0.002387115793681005
599600,1199201,1199200,2398401,967.8026249408722,0.002352216907638649
600601,1201203,1201202,2402405,969.3474850654602,0.00231782972741712
601602,1203205,1203204,2406409,970.8424701690674,0.00228394671512433
602603,1205207,1205206,2410413,972.3074510097504,0.002250560445077099
603604,1207209,1207208,2414417,973.7870481014252,0.0022176636016411067
604605,1209211,1209210,2418421,975.2220280170441,0.002185248977411902
605606,1211213,1211212,2422425,976.7442281246185,0.002153309471850662
606607,1213215,1213214,2426429,978.2978310585022,0.002121838090147321
607608,1215217,1215216,2430433,979.8226430416107,0.0020908279406057773
608609,1217219,1217218,2434437,981.3593471050262,0.002060272233620708
609610,1219221,1219220,2438441,982.8812279701233,0.0020301642806543896
610611,1221223,1221222,2442445,984.36075091362,0.0020004974918492735
611612,1223225,1223224,2446449,985.8173680305481,0.001971265375459552
612613,1225227,1225226,2450453,987.2959480285645,0.0019424615347816143
613614,1227229,1227228,2454457,988.800507068634,0.0019140796691772266
614615,1229231,1229230,2458461,990.2631731033325,0.0018861135704355547
615616,1231233,1231232,2462465,991.7486598491669,0.0018585571222047292
616617,1233235,1233234,2466469,993.2999711036682,0.001831404299650785
617618,1235237,1235236,2470473,994.8137030601501,0.001804649165705996
618619,1237239,1237238,2474477,996.3613679409027,0.0017782858720920558
619620,1239241,1239240,2478481,997.8944029808044,0.0017523086569326551
620621,1241243,1241242,2482485,999.585776090622,0.0017267118431618655
621622,1243245,1243244,2486489,1001.2174649238586,0.0017014898380693921
622623,1245247,1245246,2490493,1003.1474840641022,0.001676637131708958
623624,1247249,1247248,2494497,1004.8228390216827,0.0016521482954203748
624625,1249251,1249250,2498501,1006.5412588119507,0.0016280179806926753
625626,1251253,1251252,2502505,1008.2175619602203,0.0016042409184819917
626627,1253255,1253254,2506509,1009.9228200912476,0.0015808119170515056
627628,1255257,1255256,2510513,1011.591854095459,0.0015577258619714485
628629,1257259,1257258,2514517,1013.1071579456329,0.0015349777144137988
629630,1259261,1259260,2518521,1014.5970752239227,0.0015125625093332928
630631,1261263,1261262,2522525,1016.8391320705414,0.0014904753555811112
631632,1263265,1263264,2526529,1018.8105208873749,0.0014687114340858898
632633,1265267,1265266,2530533,1020.5700809955597,0.0014472659971715984
633634,1267269,1267268,2534537,1022.2356698513031,0.0014261343671932991
634635,1269271,1269270,2538541,1023.9776301383972,0.0014053119351729038
635636,1271273,1271272,2542545,1025.6909868717194,0.0013847941606854874
636637,1273275,1273274,2546549,1027.3549621105194,0.0013645765702676727
637638,1275277,1275276,2550553,1028.9505569934845,0.0013446547563944478
638639,1277279,1277278,2554557,1030.5611670017242,0.0013250243764559855
639640,1279281,1279280,2558561,1032.241248846054,0.0013056811523028955
640641,1281283,1281282,2562565,1033.9475739002228,0.0012866208684272351
641642,1283285,1283284,2566569,1035.7794229984283,0.001267839372076196
642643,1285287,1285286,2570573,1037.633069038391,0.0012493325712057413
643644,1287289,1287288,2574577,1039.3415441513062,0.0012310964344806052
644645,1289291,1289290,2578581,1041.2948169708252,0.0012131269902511121
645646,1291293,1291292,2582585,1043.07150888443,0.0011954203246204997
646647,1293295,1293294,2586589,1044.7521052360535,0.001177972582354414
647648,1295297,1295296,2590593,1046.6623229980469,0.0011607799644934857
648649,1297299,1297298,2594597,1048.5111269950867,0.0011438387282396434
649650,1299301,1299300,2598601,1050.3828461170197,0.0011271451859329318
650651,1301303,1301302,2602605,1052.0471119880676,0.0011106957044830779
651652,1303305,1303304,2606609,1053.759477853775,0.0010944867040052486
652653,1305307,1305306,2610613,1055.4681930541992,0.001078514657820051
653654,1307309,1307308,2614617,1057.3323440551758,0.001062776090520856
654655,1309311,1309310,2618621,1059.206670999527,0.0010472675785422325
655656,1311313,1311312,2622625,1060.9619119167328,0.0010319857484546446
656657,1313315,1313314,2626629,1062.7591080665588,0.0010169272768507653
657658,1315317,1315316,2630633,1064.4725120067596,0.001002088888981234
658659,1317319,1317318,2634637,1066.0700809955597,0.0009874673579588489
659660,1319321,1319320,2638641,1067.6720650196075,0.0009730595053270008
660661,1321323,1321322,2642645,1069.298763036728,0.0009588621986722501
661662,1323325,1323324,2646649,1070.7653040885925,0.0009448723523064473
662663,1325327,1325326,2650653,1072.5233058929443,0.0009310869254477439
663664,1327329,1327328,2654657,1074.1142508983612,0.0009175029219932185
664665,1329331,1329330,2658661,1075.7679278850555,0.0009041173907462507
665666,1331333,1331332,2662665,1077.350042104721,0.0008909274230290976
666667,1333335,1333334,2666669,1078.9097349643707,0.0008779301535923878
667668,1335337,1335336,2670673,1080.411316871643,0.0008651227589098198
668669,1337339,1337338,2674677,1082.1776449680328,0.0008525024574055351
669670,1339341,1339340,2678681,1083.8216140270233,0.0008400665080898762
670671,1341343,1341342,2682685,1085.6235859394073,0.0008278122105593866
671672,1343345,1343344,2686689,1087.3318800926208,0.0008157369039736295
672673,1345347,1345346,2690693,1088.9311411380768,0.0008038379664867534
673674,1347349,1347348,2694697,1090.516657114029,0.0007921128150201184
674675,1349351,1349350,2698701,1092.0328760147095,0.000780558904807549
675676,1351353,1351352,2702705,1093.5442159175873,0.0007691737279174049
676677,1353355,1353354,2706709,1095.0189521312714,0.0007579548133662684
677678,1355357,1355356,2710713,1096.5820498466492,0.0007468997271189437
678679,1357359,1357358,2714717,1098.0759961605072,0.0007360060698147208
679680,1359361,1359360,2718721,1099.5886061191559,0.000725271478245304
680681,1361363,1361362,2722725,1101.0619370937347,0.0007146936242179436
681682,1363365,1363364,2726729,1102.5467290878296,0.0007042702125090727
682683,1365367,1365366,2730733,1104.1392030715942,0.0006939989826832971
683684,1367369,1367368,2734737,1105.6231789588928,0.0006838777071607183
684685,1369371,1369370,2738741,1107.565763950348,0.0006739041912169341
685686,1371373,1371372,2742745,1109.0655300617218,0.0006640762721872306
686687,1373375,1373374,2746749,1110.5355660915375,0.0006543918191255216
687688,1375377,1375376,2750753,1112.038321018219,0.0006448487328043484
688689,1377379,1377378,2754757,1113.529718875885,0.0006354449443506383
689690,1379381,1379380,2758761,1115.039491891861,0.0006261784153593908
690691,1381383,1381382,2762765,1116.667321920395,0.0006170471378936782
691692,1383385,1383384,2766769,1118.2892980575562,0.0006080491327793425
692693,1385387,1385386,2770773,1120.008414030075,0.00059918245017343
693694,1387389,1387388,2774777,1121.9042122364044,0.0005904451691094437
694695,1389391,1389390,2778781,1123.369271993637,0.0005818353967015355
695696,1391393,1391392,2782785,1125.0185780525208,0.0005733512673486985
696697,1393395,1393394,2786789,1127.022430896759,0.0005649909434168876
697698,1395397,1395396,2790793,1128.5270030498505,0.0005567526143295254
698699,1397399,1397398,2794797,1130.0200140476227,0.0005486344956580069
699700,1399401,1399400,2798801,1131.503798007965,0.0005406348292353869
700701,1401403,1401402,2802805,1132.9693942070007,0.0005327518828153188
701702,1403405,1403404,2806809,1134.4839599132538,0.0005249839498446818
702703,1405407,1405406,2810813,1135.9575440883636,0.0005173293483267116
703704,1407409,1407408,2814817,1137.4364259243011,0.0005097864207073144
704705,1409411,1409410,2818821,1138.9336380958557,0.0005023535347845609
705706,1411413,1411412,2822825,1140.4129419326782,0.0004950290814349501
706707,1413415,1413414,2826829,1141.9875328540802,0.00048781147540921665
707708,1415417,1415416,2830833,1143.501435995102,0.0004806991548775841
708709,1417419,1417418,2834837,1144.9736909866333,0.00047369058017920906
709710,1419421,1419420,2838841,1146.5002977848053,0.00046678423518642376
710711,1421423,1421422,2842845,1148.155044078827,0.00045997862571312
711712,1423425,1423424,2846849,1149.8434898853302,0.00045327227917368873
712713,1425427,1425426,2850853,1151.883367061615,0.00044666374481039384
713714,1427429,1427428,2854857,1154.275778055191,0.00044015159301125095
714715,1429431,1429430,2858861,1155.8585150241852,0.00043373441531002754
715716,1431433,1431432,2862865,1157.5141229629517,0.0004274108234767482
716717,1433435,1433434,2866869,1159.2696959972382,0.00042117945031350246
717718,1435437,1435436,2870873,1160.858808040619,0.0004150389482902028
718719,1437439,1437438,2874877,1162.4335479736328,0.00040898798931721103
719720,1439441,1439440,2878881,1163.9753680229187,0.0004030252652000854
720721,1441443,1441442,2882885,1165.513657093048,0.00039714948684377305
721722,1443445,1443444,2886889,1166.9901311397552,0.00039135938368417555
722723,1445447,1445446,2890893,1168.4439289569855,0.00038565370471133065
723724,1447449,1447448,2894897,1170.0548479557037,0.0003800312159683017
724725,1449451,1449450,2898901,1171.6928219795227,0.0003744907022564803
725726,1451453,1451452,2902905,1173.3579330444336,0.00036903096656715206
726727,1453455,1453454,2906909,1175.2281930446625,0.0003636508286035678
727728,1455457,1455456,2910913,1177.176595211029,0.0003583491258041249
728729,1457459,1457458,2914917,1178.9514548778534,0.0003531247126602466
729730,1459461,1459460,2918921,1180.571585893631,0.0003479764604890079
730731,1461463,1461462,2922925,1181.996768951416,0.00034290325675101485
731732,1463465,1463464,2926929,1183.3228919506073,0.0003379040056188387
732733,1465467,1465466,2930933,1184.8598408699036,0.0003329776267264606
733734,1467469,1467468,2934937,1186.8980882167816,0.0003281230565335136
734735,1469471,1469470,2938941,1188.3104848861694,0.00032333924627891975
735736,1471473,1471472,2942945,1190.0961380004883,0.00031862516254932416
736737,1473475,1473474,2946949,1191.7077071666718,0.00031397978739278187
737738,1475477,1475476,2950953,1193.345645904541,0.00030940211763663683
738739,1477479,1477478,2954957,1195.2483780384064,0.0003048911650012087
739740,1479481,1479480,2958961,1197.1071400642395,0.0003004459553039851
740741,1481483,1481482,2962965,1198.979387998581,0.0002960655286869951
741742,1483485,1483484,2966969,1200.8533370494843,0.00029174893927574885
742743,1485487,1485486,2970973,1202.7056438922882,0.00028749525574767176
743744,1487489,1487488,2974977,1204.5859160423279,0.00028330355928574136
744745,1489491,1489490,2978981,1206.9804329872131,0.0002791729453974767
745746,1491493,1491492,2982985,1209.1443297863007,0.00027510252255069645
746747,1493495,1493494,2986989,1210.8260688781738,0.00027109141194614494
747748,1495497,1495496,2990993,1212.7238850593567,0.0002671387481996135
748749,1497499,1497498,2994997,1214.3146409988403,0.0002632436782050718
749750,1499501,1499500,2999001,1215.8375022411346,0.0002594053612483549
750751,1501503,1501502,3003005,1217.6403529644012,0.0002556229693482237
751752,1503505,1503504,3007009,1219.2114589214325,0.0002518956863468702
752753,1505507,1505506,3011013,1220.794103860855,0.0002482227081372912
753754,1507509,1507508,3015017,1222.5017478466034,0.00024460324209485407
754755,1509511,1509510,3019021,1225.1106479167938,0.00024103650764573104
755756,1511513,1511512,3023025,1226.9152390956879,0.00023752173524371756
756757,1513515,1513514,3027029,1228.6737949848175,0.0002340581664839192
757758,1515517,1515516,3031033,1230.3884599208832,0.00023064505489855947
758759,1517519,1517518,3035037,1231.8597211837769,0.00022728166379692993
759760,1519521,1519520,3039041,1233.503175020218,0.00022396726819806645
760761,1521523,1521522,3043045,1235.006767988205,0.00022070115301175974
761762,1523525,1523524,3047049,1236.7943091392517,0.00021748261394805013
762763,1525527,1525526,3051053,1238.4712948799133,0.00021431095740354067
763764,1527529,1527528,3055057,1240.1956040859222,0.00021118549886978144
764765,1529531,1529530,3059061,1241.7940781116486,0.00020810556497963262
765766,1531533,1531532,3063065,1243.5371308326721,0.00020507049134721456
766767,1533535,1533534,3067069,1245.2883648872375,0.00020207962393214984
767768,1535537,1535536,3071073,1246.752291917801,0.00019913231767532125
768769,1537539,1537538,3075077,1248.4789669513702,0.00019622793752205325
769770,1539541,1539540,3079081,1250.1149821281433,0.00019336585717155685
770771,1541543,1541542,3083085,1251.7151770591736,0.0001905454598727374
771772,1543545,1543544,3087089,1253.424766778946,0.00018776613785576046
772773,1545547,1545546,3091093,1255.318983078003,0.0001850272916499307
773774,1547549,1547548,3095097,1256.9496638774872,0.00018232833156162087
774775,1549551,1549550,3099101,1259.1508529186249,0.00017966867585528234
775776,1551553,1551552,3103105,1260.9582860469818,0.00017704775086713198
776777,1553555,1553554,3107109,1262.462172985077,0.000174464992483081
777778,1555557,1555556,3111113,1263.9454700946808,0.00017191984386499826
778779,1557559,1557558,3115117,1265.6718680858612,0.00016941175692863908
779780,1559561,1559560,3119121,1267.2464711666107,0.00016694019086571643
780781,1561563,1561562,3123125,1269.1255300045013,0.00016450461350814294
781782,1563565,1563564,3127129,1270.8656768798828,0.00016210450007747568
782783,1565567,1565566,3131133,1272.5179450511932,0.00015973933363966353
783784,1567569,1567568,3135137,1274.0074779987335,0.00015740860465029982
784785,1569571,1569570,3139141,1275.5792210102081,0.00015511181095462234
785786,1571573,1571572,3143145,1277.0950560569763,0.00015284845812857384
786787,1573575,1573574,3147149,1278.6672611236572,0.00015061805834193365
787788,1575577,1575576,3151153,1280.291393995285,0.0001484201316088729
788789,1577579,1577578,3155157,1281.838761806488,0.00014625420431002567
789790,1579581,1579580,3159161,1283.5442049503326,0.00014411980998829677
790791,1581583,1581582,3163165,1285.3039419651031,0.00014201648946254863
791792,1583585,1583584,3167169,1287.2043330669403,0.0001399437892359856
792793,1585587,1585586,3171173,1288.7272958755493,0.0001379012633151433
793794,1587589,1587588,3175177,1290.2767369747162,0.00013588847184564656
794795,1589591,1589590,3179181,1291.8697781562805,0.0001339049816806437
795796,1591593,1591592,3183185,1293.7605381011963,0.00013195036535762483
796797,1593595,1593594,3187189,1295.372601032257,0.0001300242024626641
797798,1595597,1595596,3191193,1296.8628311157227,0.00012812607803880383
798799,1597599,1597598,3195197,1298.480129957199,0.0001262555837229229
799800,1599601,1599600,3199201,1300.2618479728699,0.00012441231660886842
800801,1601603,1601602,3203205,1302.296646118164,0.00012259588038432412
801802,1603605,1603604,3207209,1304.1042549610138,0.00012080588373919454
802803,1605607,1605606,3211213,1306.377802848816,0.00011904194150247349
803804,1607609,1607608,3215217,1307.9250900745392,0.00011730367384643614
804805,1609611,1609610,3219221,1309.4803829193115,0.00011559070696876006
805806,1611613,1611612,3223225,1311.2937581539154,0.00011390267206934368
806807,1613615,1613614,3227229,1313.5900111198425,0.00011223920580505364
807808,1615617,1615616,3231233,1316.098177909851,0.00011059995040341164
808809,1617619,1617618,3235237,1317.976224899292,0.00010898455286678654
809810,1619621,1619620,3239241,1319.6125988960266,0.00010739266610926279
810811,1621623,1621622,3243245,1321.3019318580627,0.00010582394702396414
811812,1623625,1623624,3247249,1322.9292168617249,0.00010427805830204306
812813,1625627,1625626,3251253,1324.393975019455,0.00010275466752318607
813814,1627629,1627628,3255257,1325.837590932846,0.00010125344681455317
814815,1629631,1629630,3259261,1327.2775039672852,9.977407307815156e-05
815816,1631633,1631632,3263265,1328.7261180877686,9.831622833189613e-05
816817,1633635,1633634,3267269,1330.1838262081146,9.687959880011476e-05
817818,1635637,1635636,3271273,1331.6372141838074,9.546387525460887e-05
818819,1637639,1637638,3275277,1333.7879300117493,9.406875346940069e-05
819820,1639641,1639640,3279281,1335.3626689910889,9.269393342492549e-05
820821,1641643,1641642,3283285,1336.9690890312195,9.133911919434468e-05
821822,1643645,1643644,3287289,1338.6724960803986,9.000401962566684e-05
822823,1645647,1645646,3291293,1340.1430869102478,8.868834731856623e-05
823824,1647649,1647648,3295297,1341.6152758598328,8.739181930650375e-05
824825,1649651,1649650,3299301,1343.1883518695831,8.611415694304014e-05
825826,1651653,1651652,3303305,1344.9554929733276,8.485508521971497e-05
826827,1653655,1653654,3307309,1346.7319989204407,8.361433378922811e-05
827828,1655657,1655656,3311313,1348.335212945938,8.239163548751094e-05
828829,1657659,1657658,3315317,1350.297730922699,8.118672769796831e-05
829830,1659661,1659660,3319321,1352.157086133957,7.999935110092338e-05
830831,1661663,1661662,3323325,1353.7375299930573,7.882925046942546e-05
831832,1663665,1663664,3327329,1355.1858348846436,7.7676173987129e-05
832833,1665667,1665666,3331333,1356.6340351104736,7.653987427147513e-05
833834,1667669,1667668,3335337,1358.2225329875946,7.542010655470222e-05
834835,1669671,1669670,3339341,1359.861876964569,7.431663038914849e-05
835836,1671673,1671672,3343345,1361.7233929634094,7.322920839669678e-05
836837,1673675,1673674,3347349,1363.2341449260712,7.215760683720873e-05
837838,1675677,1675676,3351353,1364.6535761356354,7.110159526746429e-05
838839,1677679,1677678,3355357,1366.1047458648682,7.006094699590903e-05
839840,1679681,1679680,3359361,1367.5489430427551,6.903543794578582e-05
840841,1681683,1681682,3363365,1368.9801199436188,6.80248480193768e-05
841842,1683685,1683684,3367369,1370.418783903122,6.702895984744828e-05
842843,1685687,1685686,3371373,1371.8683199882507,6.604755924399797e-05
843844,1687689,1687688,3375377,1373.3431839942932,6.508043543362874e-05
844845,1689691,1689690,3379381,1375.0546779632568,6.412738059680123e-05
845846,1691693,1691692,3383385,1377.0982871055603,6.318818986983388e-05
846847,1693695,1693694,3387389,1379.2729589939117,6.226266134490288e-05
847848,1695697,1695696,3391393,1381.176687002182,6.135059618372907e-05
848849,1697699,1697698,3395397,1383.4383490085602,6.045179850389104e-05
849850,1699701,1699700,3399401,1385.3560738563538,5.956607492407784e-05
850851,1701703,1701702,3403405,1387.0850999355316,5.869323547358363e-05
851852,1703705,1703704,3407409,1389.1415431499481,5.7833092114378815e-05
852853,1705707,1705706,3411413,1391.0924849510193,5.698546021903894e-05
853854,1707709,1707708,3415417,1392.9645080566406,5.6150157774936815e-05
854855,1709711,1709710,3419421,1395.9931600093842,5.5327005270555674e-05
855856,1711713,1711712,3423425,1398.1661868095398,5.45158260365497e-05
856857,1713715,1713714,3427429,1400.7975718975067,5.371644533624931e-05
857858,1715717,1715716,3431433,1402.8558249473572,5.292869184359006e-05
858859,1717719,1717718,3435437,1404.7230818271637,5.215239593781007e-05
859860,1719721,1719720,3439441,1406.7374789714813,5.1387391181378916e-05
860861,1721723,1721722,3443445,1408.7279419898987,5.063351329681609e-05
861862,1723725,1723724,3447449,1410.413722038269,4.9890600053004164e-05
862863,1725727,1725726,3451453,1411.965980052948,4.9158491833622975e-05
863864,1727729,1727728,3455457,1413.7008879184723,4.843703163714963e-05
864865,1729731,1729730,3459461,1415.3007969856262,4.772606439473748e-05
865866,1731733,1731732,3463465,1417.0062010288239,4.702543719758978e-05
866867,1733735,1733734,3467469,1419.0358970165253,4.633499986539391e-05
867868,1735737,1735736,3471473,1421.4312269687653,4.565460403682664e-05
868869,1737739,1737738,3475477,1423.3431611061096,4.498410339692782e-05
869870,1739741,1739740,3479481,1425.7673099040985,4.43233540181609e-05
870871,1741743,1741742,3483485,1427.5726308822632,4.3672214019352396e-05
871872,1743745,1743744,3487489,1429.7888958454132,4.3030543565691914e-05
872873,1745747,1745746,3491493,1432.0448858737946,4.23982047550453e-05
873874,1747749,1747748,3495497,1433.7473289966583,4.177506218638882e-05
874875,1749751,1749750,3499501,1435.4610199928284,4.11609814818803e-05
875876,1751753,1751752,3503505,1436.9235849380493,4.055583110584848e-05
876877,1753755,1753754,3507509,1438.3565249443054,3.9959480886864185e-05
877878,1755757,1755756,3511513,1439.829843044281,3.937180292723497e-05
878879,1757759,1757758,3515517,1441.2785708904266,3.879267103457096e-05
879880,1759761,1759760,3519521,1442.7362079620361,3.822196094915853e-05
880881,1761763,1761762,3523525,1444.9763679504395,3.765954988921294e-05
881882,1763765,1763764,3527529,1446.555813074112,3.710531723299937e-05
882883,1765767,1765766,3531533,1448.0586330890656,3.655914395039872e-05
883884,1767769,1767768,3535537,1449.622901916504,3.6020912830281304e-05
884885,1769771,1769770,3539541,1451.1217639446259,3.5490508366819995e-05
885886,1771773,1771772,3543545,1452.6513671875,3.4967816645803396e-05
886887,1773775,1773774,3547549,1454.5357291698456,3.4452725230949e-05
887888,1775777,1775776,3551553,1456.047613143921,3.394512373233738e-05
888889,1777779,1777778,3555557,1457.5973489284515,3.3444903237977996e-05
889890,1779781,1779780,3559561,1458.9955921173096,3.2951956313809205e-05
890891,1781783,1781782,3563565,1460.3394348621368,3.246617700369825e-05
891892,1783785,1783784,3567569,1461.8611371517181,3.19874609431281e-05
892893,1785787,1785786,3571573,1463.4121570587158,3.1515705813944805e-05
893894,1787789,1787788,3575577,1464.8973548412323,3.105080986642861e-05
894895,1789791,1789790,3579581,1466.337084054947,3.059267373828334e-05
895896,1791793,1791792,3583585,1467.8620829582214,3.014119897670753e-05
896897,1793795,1793794,3587589,1469.5185589790344,2.969628826576809e-05
897898,1795797,1795796,3591593,1471.3058359622955,2.9257846449581848e-05
898899,1797799,1797798,3595597,1472.954502105713,2.8825779736507684e-05
899900,1799801,1799800,3599601,1474.5004630088806,2.8399994789651828e-05
900901,1801803,1801802,3603605,1475.934121131897,2.7980400432170427e-05
901902,1803805,1803804,3607609,1477.362009048462,2.7566906737774843e-05
902903,1805807,1805806,3611613,1478.8305339813232,2.7159424917044817e-05
903904,1807809,1807808,3615617,1480.240014076233,2.675786754480214e-05
904905,1809811,1809810,3619621,1481.7307569980621,2.636214821905014e-05
905906,1811813,1811812,3623625,1483.146893978119,2.597218224309472e-05
906907,1813815,1813814,3627629,1484.555231809616,2.5587885943423316e-05
907908,1815817,1815816,3631633,1485.9812469482422,2.5209176669704902e-05
908909,1817819,1817818,3635637,1487.41832113266,2.4835973363224184e-05
909910,1819821,1819820,3639641,1488.8361320495605,2.4468195647386892e-05
910911,1821823,1821822,3643645,1490.3094320297241,2.410576496458816e-05
911912,1823825,1823824,3647649,1491.7587418556213,2.3748603211970476e-05
912913,1825827,1825826,3651653,1493.2060539722443,2.3396633991978888e-05
913914,1827829,1827828,3655657,1495.7261900901794,2.3049781702866312e-05
914915,1829831,1829830,3659661,1497.6433079242706,2.2707971766067203e-05
915916,1831833,1831832,3663665,1500.1190149784088,2.2371131194631744e-05
916917,1833835,1833834,3667669,1501.7877202033997,2.203918734267063e-05
917918,1835837,1835836,3671673,1503.5394768714905,2.1712069269597123e-05
918919,1837839,1837838,3675677,1505.7765438556671,2.1389706603258674e-05
919920,1839841,1839840,3679681,1507.538514137268,2.107202999468427e-05
920921,1841843,1841842,3683685,1509.0094120502472,2.0758971686518635e-05
921922,1843845,1843844,3687689,1510.442549943924,2.0450464603527507e-05
922923,1845847,1845846,3691693,1511.8903441429138,2.0146442011537147e-05
923924,1847849,1847848,3695697,1513.3440301418304,1.984683922273689e-05
924925,1849851,1849850,3699701,1514.7679798603058,1.9551591435629234e-05
925926,1851853,1851852,3703705,1516.7352831363678,1.926063578139292e-05
926927,1853855,1853854,3707709,1518.5433549880981,1.8973909618580365e-05
927928,1855857,1855856,3711713,1520.3625741004944,1.869135132892552e-05
928929,1857859,1857858,3715717,1522.3968801498413,1.8412900658404396e-05
929930,1859861,1859860,3719721,1525.2045831680298,1.8138497580366675e-05
930931,1861863,1861862,3723725,1528.2453429698944,1.786808354609093e-05
931932,1863865,1863864,3727729,1530.600214958191,1.7601600006855733e-05
932933,1865867,1865866,3731733,1532.4748170375824,1.7338990232929063e-05
933934,1867869,1867868,3735737,1534.1894659996033,1.7080197608265735e-05
934935,1869871,1869870,3739741,1535.9362120628357,1.6825166994749452e-05
935936,1871873,1871872,3743745,1537.404571056366,1.6573843367950758e-05
936937,1873875,1873874,3747749,1538.9803500175476,1.632617295399541e-05
937938,1875877,1875876,3751753,1540.8347299098969,1.6082102547443355e-05
938939,1877879,1877878,3755757,1542.5065791606903,1.584157985234924e-05
939940,1879881,1879880,3759761,1544.191143989563,1.560455336857558e-05
940941,1881883,1881882,3763765,1545.7862989902496,1.5370972164419072e-05
941942,1883885,1883884,3767769,1547.439936876297,1.5140786103984283e-05
942943,1885887,1885886,3771773,1548.892860174179,1.4913945960870478e-05
943944,1887889,1887888,3775777,1550.347697019577,1.46904027360506e-05
944945,1889891,1889890,3779781,1551.7736489772797,1.447010902211332e-05
945946,1891893,1891892,3783785,1553.4858889579773,1.425301718427363e-05
946947,1893895,1893894,3787789,1556.367651939392,1.4039080610928067e-05
947948,1895897,1895896,3791793,1558.4059100151062,1.3828253713654703e-05
948949,1897899,1897898,3795797,1560.4602599143982,1.3620491245092126e-05
949950,1899901,1899900,3799801,1561.9566910266876,1.3415748298939434e-05
950951,1901903,1901902,3803805,1563.4720940589905,1.3213981333137781e-05
951952,1903905,1903904,3807809,1564.9214429855347,1.3015147033001995e-05
952953,1905907,1905906,3811813,1567.4624650478363,1.2819202538594254e-05
953954,1907909,1907908,3815817,1569.2502369880676,1.2626106240531954e-05
954955,1909911,1909910,3819821,1571.2601640224457,1.2435816188371973e-05
955956,1911913,1911912,3823825,1572.7562358379364,1.2248292023286922e-05
956957,1913915,1913914,3827829,1574.2586369514465,1.2063493159075733e-05
957958,1915917,1915916,3831833,1575.7403030395508,1.1881380373779393e-05
958959,1917919,1917918,3835837,1577.2474138736725,1.1701914445438888e-05
959960,1919921,1919920,3839841,1578.8314390182495,1.1525056606842554e-05
960961,1921923,1921922,3843845,1581.0295221805573,1.1350769341333944e-05
961962,1923925,1923924,3847849,1582.5015668869019,1.1179015245943447e-05
962963,1925927,1925926,3851853,1583.9675960540771,1.1009757258761965e-05
963964,1927929,1927928,3855857,1585.5025119781494,1.0842959341061942e-05
964965,1929931,1929930,3859861,1586.9421200752258,1.0678585454115819e-05
965966,1931933,1931932,3863865,1588.411530971527,1.0516600582377578e-05
966967,1933935,1933934,3867869,1589.8875088691711,1.03569697103012e-05
967968,1935937,1935936,3871873,1591.3322970867157,1.0199659072895884e-05
968969,1937939,1937938,3875877,1592.7966549396515,1.0044634450423473e-05
969970,1939941,1939940,3879881,1594.2917149066925,9.891863101074705e-06
970971,1941943,1941942,3883885,1595.818659067154,9.741311941979802e-06
971972,1943945,1943944,3887889,1597.7190470695496,9.592948572390014e-06
972973,1945947,1945946,3891893,1599.494525194168,9.446741387364455e-06
973974,1947949,1947948,3895897,1602.4662098884583,9.302659236709587e-06
974975,1949951,1949950,3899901,1604.8130490779877,9.160670742858201e-06
975976,1951953,1951952,3903905,1606.8410160541534,9.020746119858813e-06
976977,1953955,1953954,3907909,1608.9003820419312,8.882854785952077e-06
977978,1955957,1955956,3911913,1611.233325958252,8.746967409933859e-06
978979,1957959,1957958,3915917,1612.8197829723358,8.613054660600028e-06
979980,1959961,1959960,3919921,1614.4832410812378,8.481088116241153e-06
980981,1961963,1961962,3923925,1616.0267088413239,8.351039468834642e-06
981982,1963965,1963964,3927929,1617.5113949775696,8.222880751418415e-06
982983,1965967,1965966,3931933,1618.986032962799,8.096584338090906e-06
983984,1967969,1967968,3935937,1620.8723409175873,7.97212351244525e-06
984985,1969971,1969970,3939941,1622.5403249263763,7.84947121701407e-06
985986,1971973,1971972,3943945,1624.5484068393707,7.72860130382469e-06
986987,1973975,1973974,3947949,1626.0817620754242,7.609488079651783e-06
987988,1975977,1975976,3951953,1628.0829770565033,7.492105737583188e-06
988989,1977979,1977978,3955957,1629.944734096527,7.376429266514606e-06
989990,1979981,1979980,3959961,1632.0998351573944,7.2624335416549e-06
990991,1981983,1981982,3963965,1633.8196840286255,7.150094575081312e-06
991992,1983985,1983984,3967969,1635.632374048233,7.039388037810568e-06
992993,1985987,1985986,3971973,1637.225596189499,6.930290169293585e-06
993994,1987989,1987988,3975977,1638.7887001037598,6.822777891102305e-06
994995,1989991,1989990,3979981,1640.396103143692,6.716827897434996e-06
995996,1991993,1991992,3983985,1642.0104250907898,6.612417564610951e-06
996997,1993995,1993994,3987989,1643.4547271728516,6.509524496323138e-06
997998,1995997,1995996,3991993,1645.269896030426,6.408126409951365e-06
998999,1997999,1997998,3995997,1646.998386144638,6.308201932370139e-06
1000000,2000001,2000000,4000001,1648.6927552223206,6.2097294630802935e-06


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0008897781372070312,2181.2938132599165
5,11,5,16,0.01314091682434082,551.6572936697758
9,19,9,28,0.018110990524291992,328.55966978448737
14,29,14,43,0.02493596076965332,210.09838993014114
18,37,18,55,0.030296802520751953,162.94770294226828
23,47,23,70,0.0363919734954834,128.02251159792422
27,55,27,82,0.04106593132019043,110.32071588270901
32,65,32,97,0.04689788818359375,95.32596105537482
36,73,36,109,0.05164909362792969,86.95884698182999
41,83,41,124,0.05733299255371094,79.58223819698173
46,93,46,139,0.06327390670776367,74.41726328357527
50,101,50,151,0.06794977188110352,71.2249660873008
55,111,55,166,0.07413101196289062,67.97957715833968
59,119,59,178,0.0791168212890625,65.82527310965133
64,129,64,193,0.08534407615661621,63.51994542126204
68,137,68,205,0.09254574775695801,61.885768455410926
73,147,73,220,0.09832191467285156,60.05414066981007
78,157,78,235,0.10694575309753418,58.48128388845657
82,165,82,247,0.11159896850585938,57.42541371166362
87,175,87,262,0.11749410629272461,56.337611548024825
91,183,91,274,0.12215614318847656,55.62582065774427
96,193,96,289,0.12974286079406738,54.903526621526225
100,201,100,301,0.13481497764587402,54.43580853555068
105,211,105,316,0.14109587669372559,53.95288888748814
109,219,109,328,0.14622282981872559,53.62066620994665
114,229,114,343,0.15337872505187988,53.23500935584639
119,239,119,358,0.1608419418334961,52.84674502919029
123,247,123,370,0.16715383529663086,52.51999195501844
128,257,128,385,0.1759939193725586,52.086835235855006
132,265,132,397,0.18344402313232422,51.722205659494875
137,275,137,412,0.1916518211364746,51.247821407905576
141,283,141,424,0.1981799602508545,50.8552389243423
146,293,146,439,0.20527386665344238,50.34828483045567
150,301,150,451,0.2113800048828125,49.92927072969201
155,311,155,466,0.21968793869018555,49.38915824350374
160,321,160,481,0.22803378105163574,48.83349698253892
164,329,164,493,0.23465204238891602,48.38066761506502
169,339,169,508,0.2427070140838623,47.808346037700176
173,347,173,520,0.25225305557250977,47.34865389378115
178,357,178,535,0.2617518901824951,46.77607651772769
182,365,182,547,0.26886677742004395,46.32248067424712
187,375,187,562,0.2780628204345703,45.76350953952533
192,385,192,577,0.28694677352905273,45.2139030816802
196,393,196,589,0.2934868335723877,44.779953190588685
201,403,201,604,0.30580997467041016,44.242660525023666
205,411,205,616,0.3157539367675781,43.815568779795285
210,421,210,631,0.32678890228271484,43.28382497862117
214,429,214,643,0.33498406410217285,42.8594880498008
219,439,219,658,0.34273791313171387,42.32973697368698
223,447,223,670,0.3491659164428711,41.906030828599114
228,457,228,685,0.35684990882873535,41.37594521439587
233,467,233,700,0.36447691917419434,40.84477224257489
237,475,237,712,0.3710191249847412,40.41869288449129
242,485,242,727,0.3817627429962158,39.88436746223124
246,493,246,739,0.38876795768737793,39.45548068444032
251,503,251,754,0.3971569538116455,38.91787524273991
255,511,255,766,0.40354490280151367,38.48710832692518
260,521,260,781,0.4116690158843994,37.94886614165375
265,531,265,796,0.4197659492492676,37.41232836878453
269,539,269,808,0.42676472663879395,36.9853949270489
274,549,274,823,0.43463683128356934,36.45572776871859
278,557,278,835,0.4408390522003174,36.035777873435336
283,567,283,850,0.4486348628997803,35.515977090220304
287,575,287,862,0.4546818733215332,35.104302450518844
292,585,292,877,0.4623398780822754,34.59476542014545
296,593,296,889,0.46848487854003906,34.1909875643305
301,603,301,904,0.47624778747558594,33.690831385122465
306,613,306,919,0.4840869903564453,33.195588629829444
310,621,310,931,0.490386962890625,32.802918095914265
315,631,315,946,0.49816083908081055,32.31655594594258
319,639,319,958,0.5040369033813477,31.931099714866377
324,649,324,973,0.5114378929138184,31.453811173767008
328,657,328,985,0.5182418823242188,31.075512708542874
333,667,333,1000,0.5291850566864014,30.60683691556187
337,675,337,1012,0.535559892654419,30.235068553143492
342,685,342,1027,0.5432078838348389,29.774116420396467
347,695,347,1042,0.5506210327148438,29.31722515055685
351,703,351,1054,0.556704044342041,28.95464893458916
356,713,356,1069,0.5645039081573486,28.50522798750285
360,721,360,1081,0.571448802947998,28.14887581576454
365,731,365,1096,0.583000898361206,27.70762615880153
369,739,369,1108,0.5890870094299316,27.358109050643407
374,749,374,1123,0.5965650081634521,26.92567026992174
379,759,379,1138,0.603538990020752,26.49820389088518
383,767,383,1150,0.6085379123687744,26.159769815116306
388,777,388,1165,0.6157279014587402,25.741057686879458
392,785,392,1177,0.6225359439849854,25.409475980466596
397,795,397,1192,0.6317269802093506,24.99914032670722
401,803,401,1204,0.6385118961334229,24.674124810152307
406,813,406,1219,0.647406816482544,24.271844947119916
410,821,410,1231,0.6541519165039062,23.953150333218446
415,831,415,1246,0.6619091033935547,23.558594156326535
420,841,420,1261,0.6690230369567871,23.16814416867078
424,849,424,1273,0.6747877597808838,22.858640213780063
429,859,429,1288,0.6824090480804443,22.475208243453153
433,867,433,1300,0.6870858669281006,22.171142587771783
438,877,438,1315,0.6928339004516602,21.79433103128008
442,885,442,1327,0.6974759101867676,21.495461233985452
447,895,447,1342,0.7033600807189941,21.12507498190871
451,903,451,1354,0.7079470157623291,20.83132344287833
456,913,456,1369,0.7139449119567871,20.46733606873454
461,923,461,1384,0.7197918891906738,20.106915813559453
465,931,465,1396,0.7246799468994141,19.821154891500782
470,941,470,1411,0.7345118522644043,19.467183120473464
474,949,474,1423,0.7411129474639893,19.186627262391312
479,959,479,1438,0.7471029758453369,18.839202110637416
483,967,483,1450,0.7517929077148438,18.563890703470634
488,977,488,1465,0.7575778961181641,18.22306292194753
493,987,493,1480,0.7633848190307617,17.885935216414964
497,995,497,1492,0.7681689262390137,17.618901135066608
502,1005,502,1507,0.7794640064239502,17.28842966477191
506,1013,506,1519,0.7851049900054932,17.026685481543154
511,1023,511,1534,0.7906818389892578,16.70275075904965
515,1031,515,1546,0.795191764831543,16.44616116392035
520,1041,520,1561,0.8008899688720703,16.128573898694867
524,1049,524,1573,0.8053348064422607,15.876996022481421
529,1059,529,1588,0.8110549449920654,15.565615100192645
534,1069,534,1603,0.8165929317474365,15.257658010921318
538,1077,538,1615,0.8210890293121338,15.013756043115563
543,1087,543,1630,0.8268020153045654,14.711958585836442
547,1095,547,1642,0.831981897354126,14.472982681018607
552,1105,552,1657,0.8375980854034424,14.177332639971041
556,1113,556,1669,0.8419489860534668,13.943259897983125
561,1123,561,1684,0.8476920127868652,13.653716932658654
566,1133,566,1699,0.853212833404541,13.36755499194328
570,1141,570,1711,0.8576920032501221,13.141063913062453
575,1151,575,1726,0.8631899356842041,12.861015855374035
579,1159,579,1738,0.8676979541778564,12.639450753999768
584,1169,584,1753,0.8737390041351318,12.365619523619443
588,1177,588,1765,0.8789031505584717,12.149079416987888
593,1187,593,1780,0.8846840858459473,11.881587944614353
597,1195,597,1792,0.889319896697998,11.670155076153492
602,1205,602,1807,0.8948848247528076,11.409071201653092
607,1215,607,1822,0.9005169868469238,11.151546047860506
611,1223,611,1834,0.9052670001983643,10.948077843647297
616,1233,616,1849,0.9110219478607178,10.69691315106013
620,1241,620,1861,0.9176018238067627,10.498500710600865
625,1251,625,1876,0.9262869358062744,10.253609254923049
629,1259,629,1888,0.9314048290252686,10.060176215003025
634,1269,634,1903,0.9371569156646729,9.821459751648604
638,1277,638,1915,0.9417328834533691,9.632928987784112
643,1287,643,1930,0.9474470615386963,9.400298575587271
648,1297,648,1945,0.9532818794250488,9.171022312944388
652,1305,652,1957,0.957838773727417,8.990010283336233
657,1315,657,1972,0.9633948802947998,8.766756701320787
661,1323,661,1984,0.968193769454956,8.590568141575318
666,1333,666,1999,0.974635124206543,8.373362138447987
670,1341,670,2011,0.9792039394378662,8.202031703210878
675,1351,675,2026,0.9849889278411865,7.990925689911251
680,1361,680,2041,0.9905989170074463,7.783229145637279
684,1369,684,2053,0.9951379299163818,7.619532821557755
689,1379,689,2068,1.0007050037384033,7.4179915223913895
693,1387,693,2080,1.0051679611206055,7.25922078543033
698,1397,698,2095,1.0108129978179932,7.06383002618486
702,1405,702,2107,1.0155839920043945,6.909968999084981
707,1415,707,2122,1.0216331481933594,6.720694806746678
711,1423,711,2134,1.026425838470459,6.571705137752133
716,1433,716,2149,1.0323069095611572,6.388485076060192
721,1443,721,2164,1.0380299091339111,6.208590475753454
725,1451,725,2176,1.042454719543457,6.067047308662836
730,1461,730,2191,1.0480749607086182,5.893054672673429
734,1469,734,2203,1.0525970458984375,5.756187601161514
739,1479,739,2218,1.058218002319336,5.587984272487688
743,1487,743,2230,1.0627260208129883,5.455707011671279
748,1497,748,2245,1.068444013595581,5.293195162420261
752,1505,752,2257,1.074145793914795,5.1654398938167105
757,1515,757,2272,1.0811328887939453,5.008548666132242
762,1525,762,2287,1.0869340896606445,4.854758117711185
766,1533,766,2299,1.0914459228515625,4.73394953278364
771,1543,771,2314,1.0970361232757568,4.585708191257709
775,1551,775,2326,1.1018540859222412,4.46932238278373
780,1561,780,2341,1.1073479652404785,4.326586556777897
784,1569,784,2353,1.1118619441986084,4.21458400679262
789,1579,789,2368,1.1176810264587402,4.0772958951991995
794,1589,794,2383,1.1236238479614258,3.9430015662455844
798,1597,798,2395,1.1283111572265625,3.8377027762541047
803,1607,803,2410,1.134186029434204,3.7087239211547285
807,1615,807,2422,1.1387898921966553,3.607635713046193
812,1625,812,2437,1.1444838047027588,3.4838650531818303
816,1633,816,2449,1.1490728855133057,3.3868986091982833
821,1643,821,2464,1.1546781063079834,3.268224791989155
825,1651,825,2476,1.1592469215393066,3.175292937862878
830,1661,830,2491,1.1649549007415771,3.061611277554448
835,1671,835,2506,1.1708159446716309,2.9506612982884235
839,1679,839,2518,1.1754648685455322,2.8638489584936906
844,1689,844,2533,1.181152105331421,2.7577442638909133
848,1697,848,2545,1.1855719089508057,2.674771098145243
853,1707,853,2560,1.1912047863006592,2.5734178712216362
857,1715,857,2572,1.1957488059997559,2.4942065686138903
862,1725,862,2587,1.2014808654785156,2.397504537380655
867,1735,867,2602,1.2072038650512695,2.3033404339682875
871,1743,871,2614,1.211824893951416,2.229813512816918
876,1753,876,2629,1.2175350189208984,2.140131120316596
880,1761,880,2641,1.222689151763916,2.070144362877045
885,1771,885,2656,1.2291457653045654,1.9848304953585512
889,1779,889,2668,1.2345249652862549,1.918293465458646
894,1789,894,2683,1.2402808666229248,1.8372361760960985
898,1797,898,2695,1.2448740005493164,1.7740607564173843
903,1807,903,2710,1.250601053237915,1.6971520945412522
908,1817,908,2725,1.2562110424041748,1.6225030310066586
912,1825,912,2737,1.260706901550293,1.564389189575877
917,1835,917,2752,1.2663748264312744,1.4937264601271636
921,1843,921,2764,1.2716097831726074,1.4387592172002996
926,1853,926,2779,1.2778599262237549,1.371974918841488
930,1861,930,2791,1.2825889587402344,1.3200648891820492
935,1871,935,2806,1.2882587909698486,1.2570426954473533
939,1879,939,2818,1.2927989959716797,1.2080930153356348
944,1889,944,2833,1.298487901687622,1.1487075278225802
949,1899,949,2848,1.3042020797729492,1.0912859938341626
953,1907,953,2860,1.3085949420928955,1.0467354776787943
958,1917,958,2875,1.3141670227050781,0.9927469211850166
962,1925,962,2887,1.318711757659912,0.9508912458189798
967,1935,967,2902,1.3250908851623535,0.9002088814869467
971,1943,971,2914,1.3301539421081543,0.8609503786333335
976,1953,976,2929,1.3359529972076416,0.8134581379129031
981,1963,981,2944,1.3418629169464111,0.767693079837386
985,1971,985,2956,1.346506118774414,0.7323047735238788
990,1981,990,2971,1.3526217937469482,0.6895755773830388
994,1989,994,2983,1.3573870658874512,0.656580220521505
999,1999,999,2998,1.3635740280151367,0.6167982410213426
1003,2007,1003,3010,1.3682167530059814,0.586125093566011
1008,2017,1008,3025,1.3742239475250244,0.5491998170975876
1012,2025,1012,3037,1.3799450397491455,0.5207734104808424
1017,2035,1017,3052,1.3858540058135986,0.4866055213284426
1022,2045,1022,3067,1.391706943511963,0.45392276140569265
1026,2053,1026,3079,1.39652681350708,0.4288222652414788
1031,2063,1031,3094,1.4023487567901611,0.3987237195681246
1035,2071,1035,3106,1.4068498611450195,0.3756441261219834
1040,2081,1040,3121,1.4125518798828125,0.3480138088195872
1044,2089,1044,3133,1.4175560474395752,0.32686314270824823
1049,2099,1049,3148,1.4237167835235596,0.30158829718675406
1053,2107,1053,3160,1.4288179874420166,0.28227865297367316
1058,2117,1058,3175,1.435241937637329,0.25925244438667505
1063,2127,1063,3190,1.441270112991333,0.23743119141022362
1067,2135,1067,3202,1.4462201595306396,0.22082086604859796
1072,2145,1072,3217,1.4522850513458252,0.20109022528572496
1076,2153,1076,3229,1.4569988250732422,0.18611205532022268
1081,2163,1081,3244,1.4633679389953613,0.1683709090151524
1085,2171,1085,3256,1.4684059619903564,0.15494364473022415
1090,2181,1090,3271,1.4744579792022705,0.13909050431061587
1095,2191,1095,3286,1.480578899383545,0.12424346140062426
1099,2199,1099,3298,1.4852187633514404,0.11307068200221693
1104,2209,1104,3313,1.4920458793640137,0.09996278264441116
1108,2217,1108,3325,1.4966418743133545,0.09014696674057632
1113,2227,1113,3340,1.5024700164794922,0.07869531592541534
1117,2235,1117,3352,1.5079219341278076,0.0701745379312797
1122,2245,1122,3367,1.5135319232940674,0.06030626747985934
1126,2253,1126,3379,1.5182170867919922,0.053024685727223186
1131,2263,1131,3394,1.5243017673492432,0.044671098483036076
1136,2273,1136,3409,1.530411958694458,0.03712834739292248
1140,2281,1140,3421,1.5350759029388428,0.03166222405980079
1145,2291,1145,3436,1.5408987998962402,0.025518793508467752
1149,2299,1149,3448,1.5454089641571045,0.021139105461088548
1154,2309,1154,3463,1.551048994064331,0.01631047345006209
1158,2317,1158,3475,1.5555920600891113,0.012946987328632531
1163,2327,1163,3490,1.5614349842071533,0.009343420959226023
1168,2337,1168,3505,1.567288875579834,0.0063816761188491
1172,2345,1172,3517,1.5720510482788086,0.00445641465614699
1177,2355,1177,3532,1.5778439044952393,0.0025835270397465138
1181,2363,1181,3544,1.582615852355957,0.0014970074001894318
1186,2373,1186,3559,1.5883710384368896,0.0006342480769490066
1190,2381,1190,3571,1.5929317474365234,0.0003266816243012727
1195,2391,1195,3586,1.5987091064453125,0.00040287007766437455
1199,2399,1199,3598,1.603261947631836,0.0008196230595558518
1204,2409,1204,3613,1.6088998317718506,0.0017685459372387413
1209,2419,1209,3628,1.6146299839019775,0.0031746293495871214
1213,2427,1213,3640,1.6192739009857178,0.004615571170688781
1218,2437,1218,3655,1.625791072845459,0.00679574581408815
1222,2445,1222,3667,1.6307017803192139,0.008831391092144258
1227,2455,1227,3682,1.6364197731018066,0.011725085590342132
1231,2463,1231,3694,1.640854835510254,0.014308477568761191
1236,2473,1236,3709,1.6464331150054932,0.01785928385106672
1240,2481,1240,3721,1.6509368419647217,0.020947263164089236
1245,2491,1245,3736,1.6565239429473877,0.02510355709966916
1250,2501,1250,3751,1.6621809005737305,0.029575179728453804
1254,2509,1254,3763,1.6667537689208984,0.03336955365045924
1259,2519,1259,3778,1.67252779006958,0.038371251428884534
1263,2527,1263,3790,1.6774730682373047,0.042569975265678295
1268,2537,1268,3805,1.6838629245758057,0.0480517101316309
1272,2545,1272,3817,1.688429832458496,0.052613508742410886
1277,2555,1277,3832,1.694303035736084,0.058522141630078295
1282,2565,1282,3847,1.7001910209655762,0.06464421919508823
1286,2573,1286,3859,1.7047100067138672,0.06968419402062409
1291,2583,1291,3874,1.7105748653411865,0.07614816373165922
1295,2591,1295,3886,1.7152600288391113,0.08144059136623127
1300,2601,1300,3901,1.7214338779449463,0.08819492369377713
1304,2609,1304,3913,1.7302470207214355,0.09370044486752249
1309,2619,1309,3928,1.7365119457244873,0.10069847189652137
1313,2627,1313,3940,1.7411751747131348,0.10638171384505313
1318,2637,1318,3955,1.746971845626831,0.11358136338003533
1323,2647,1323,3970,1.752701997756958,0.12087603521740675
1327,2655,1327,3982,1.7572789192199707,0.12677232587384424
1332,2665,1332,3997,1.7629518508911133,0.13420878094859745
1336,2673,1336,4009,1.767552137374878,0.1402038656235618
1341,2683,1341,4024,1.7769339084625244,0.14774607083938918
1345,2691,1345,4036,1.781944751739502,0.15381208087603682
1350,2701,1350,4051,1.7875988483428955,0.16142670521389846
1354,2709,1354,4063,1.792184829711914,0.1675383765857532
1359,2719,1359,4078,1.7978699207305908,0.17519571084449126
1364,2729,1364,4093,1.8036308288574219,0.18286519955302083
1368,2737,1368,4105,1.8080329895019531,0.18900430370717913
1373,2747,1373,4120,1.8137400150299072,0.19667613300839548
1377,2755,1377,4132,1.8182649612426758,0.20280713000909145
1382,2765,1382,4147,1.8244900703430176,0.21045612525608703
1386,2773,1386,4159,1.8295259475708008,0.21655839510458463
1391,2783,1391,4174,1.835669994354248,0.2241579444777244
1396,2793,1396,4189,1.8413138389587402,0.23171794608254004
1400,2801,1400,4201,1.845716953277588,0.23773158453570886
1405,2811,1405,4216,1.8525588512420654,0.24519840295840822
1409,2819,1409,4228,1.8571209907531738,0.25112642921499173
1414,2829,1414,4243,1.8627779483795166,0.25847294605819116
1418,2837,1418,4255,1.8672678470611572,0.26429464730347263
1423,2847,1423,4270,1.8741869926452637,0.27149649591933667
1427,2855,1427,4282,1.8789761066436768,0.27719369913472747
1432,2865,1432,4297,1.885037899017334,0.2842297925882349
1437,2875,1437,4312,1.8906638622283936,0.2911657427000591
1441,2883,1441,4324,1.895164966583252,0.2966388357388041
1446,2893,1446,4339,1.9007837772369385,0.30338138255899594
1450,2901,1450,4351,1.9052281379699707,0.308693344463677
1455,2911,1455,4366,1.9109320640563965,0.31522679332988446
1459,2919,1459,4378,1.9155139923095703,0.3203655661409357
1464,2929,1464,4393,1.9220287799835205,0.3266754834620542
1469,2939,1469,4408,1.9300718307495117,0.33285551201515773
1473,2947,1473,4420,1.9380578994750977,0.3377035089565652
1478,2957,1478,4435,1.9443888664245605,0.34364057182256147
1482,2965,1482,4447,1.9489538669586182,0.3482898710412883
1487,2975,1487,4462,1.9546990394592285,0.35397352773134116
1491,2983,1491,4474,1.9591879844665527,0.35841629670835573
1496,2993,1496,4489,1.9650850296020508,0.36383724781910587
1500,3001,1500,4501,1.9697070121765137,0.36806631788851973
1505,3011,1505,4516,1.9760048389434814,0.37321580295986223
1510,3021,1510,4531,1.9816999435424805,0.37821076651937346
1514,3029,1514,4543,1.9862017631530762,0.3820937344437425
1519,3039,1519,4558,1.991832971572876,0.3868040668027106
1523,3047,1523,4570,1.9963138103485107,0.3904561182243924
1528,3057,1528,4585,2.0021488666534424,0.39487399577137694
1532,3065,1532,4597,2.0067217350006104,0.39828922579761183
1537,3075,1537,4612,2.012410879135132,0.40240779158216355
1541,3083,1541,4624,2.017190933227539,0.40558116428962876
1546,3093,1546,4639,2.0230910778045654,0.40939468349733943
1551,3103,1551,4654,2.0290608406066895,0.41303663236908505
1555,3111,1555,4666,2.0339109897613525,0.41582577682163446
1560,3121,1560,4681,2.0397651195526123,0.41915569812363174
1564,3129,1564,4693,2.0442121028900146,0.4216937773585414
1569,3139,1569,4708,2.049907922744751,0.4247083125989093
1573,3147,1573,4720,2.0544850826263428,0.42699305678752353
1578,3157,1578,4735,2.0601518154144287,0.42968998489152455
1583,3167,1583,4750,2.065903902053833,0.43221004483336856
1587,3175,1587,4762,2.0707569122314453,0.4340987761671613
1592,3185,1592,4777,2.07686185836792,0.43630079786066744
1596,3193,1596,4789,2.081799030303955,0.43793562395899244
1601,3203,1601,4804,2.0874650478363037,0.4398212441248006
1605,3211,1605,4816,2.0920729637145996,0.44120391145406757
1610,3221,1610,4831,2.0978949069976807,0.44277568641837206
1614,3229,1614,4843,2.102555990219116,0.4439084102241395
1619,3239,1619,4858,2.108350992202759,0.44516917572673265
1624,3249,1624,4873,2.1155669689178467,0.446258350743733
1628,3257,1628,4885,2.122663974761963,0.4470066969166737
1633,3267,1633,4900,2.1289138793945312,0.447789072085925
1637,3275,1637,4912,2.1335837841033936,0.4482930471818918
1642,3285,1642,4927,2.1392440795898438,0.4487713497868526
1646,3293,1646,4939,2.143808126449585,0.44903325114171366
1651,3303,1651,4954,2.149472951889038,0.4492105709310863
1655,3311,1655,4966,2.1541409492492676,0.4492330864864016
1660,3321,1660,4981,2.1597959995269775,0.4491130902065379
1665,3331,1665,4996,2.1654469966888428,0.4488297460480908
1669,3339,1669,5008,2.1703057289123535,0.4484864354686806
1674,3349,1674,5023,2.176527976989746,0.447912824377795
1678,3357,1678,5035,2.1813488006591797,0.44733941641140973
1683,3367,1683,5050,2.1869897842407227,0.4464810472999261
1687,3375,1687,5062,2.191577911376953,0.44568229885919664
1692,3385,1692,5077,2.1971800327301025,0.4445455839611441
1697,3395,1697,5092,2.2029359340667725,0.44325735464622085
1701,3403,1701,5104,2.207468032836914,0.4421193022105854
1706,3413,1706,5119,2.213181972503662,0.44056452103268384
1710,3421,1710,5131,2.2176709175109863,0.4392165436019013
1715,3431,1715,5146,2.2237179279327393,0.43740358965953874
1719,3439,1719,5158,2.2284088134765625,0.4358524794832874
1724,3449,1724,5173,2.234375,0.4337898357315453
1728,3457,1728,5185,2.238968849182129,0.43204230142430333
1733,3467,1733,5200,2.2446439266204834,0.42973819667065527
1738,3477,1738,5215,2.2504630088806152,0.4273033811781488
1742,3485,1742,5227,2.2550108432769775,0.4252630400681028
1747,3495,1747,5242,2.2606987953186035,0.42259903989588565
1751,3503,1751,5254,2.265220880508423,0.42037852079306504
1756,3513,1756,5269,2.2709670066833496,0.4174933574967099
1760,3521,1760,5281,2.2756638526916504,0.41509925916716384
1765,3531,1765,5296,2.281571865081787,0.4120014772199738
1769,3539,1769,5308,2.286026954650879,0.40944089836148123
1774,3549,1774,5323,2.291680097579956,0.4061397001214573
1779,3559,1779,5338,2.2975308895111084,0.4027296806686991
1783,3567,1783,5350,2.302053928375244,0.39992538149545
1788,3577,1788,5365,2.3077011108398438,0.3963272736733643
1792,3585,1792,5377,2.313264846801758,0.39337656406496535
1797,3595,1797,5392,2.3189408779144287,0.3896005575121535
1801,3603,1801,5404,2.3236968517303467,0.38651164262705606
1806,3613,1806,5419,2.3297390937805176,0.38256804949946854
1811,3623,1811,5434,2.3355050086975098,0.37853584958168085
1815,3631,1815,5446,2.3400259017944336,0.37524846713608895
1820,3641,1820,5461,2.3456709384918213,0.3710649405835511
1824,3649,1824,5473,2.350245952606201,0.36766071136719347
1829,3659,1829,5488,2.3558928966522217,0.3633363931299982
1833,3667,1833,5500,2.3604679107666016,0.3598237281088359
1838,3677,1838,5515,2.3661229610443115,0.3553690708274644
1842,3685,1842,5527,2.370837926864624,0.35175625698957447
1847,3695,1847,5542,2.3765339851379395,0.34718150272419734
1852,3705,1852,5557,2.3823559284210205,0.3425443666509409
1856,3713,1856,5569,2.3868439197540283,0.33879180263829767
1861,3723,1861,5584,2.3923699855804443,0.334050097346676
1865,3731,1865,5596,2.3969268798828125,0.3302178471616344
1870,3741,1870,5611,2.4026451110839844,0.3253815244249836
1874,3749,1874,5623,2.4070990085601807,0.3214776090663918
1879,3759,1879,5638,2.4128270149230957,0.316556801614297
1884,3769,1884,5653,2.4185149669647217,0.3115935236100995
1888,3777,1888,5665,2.423103094100952,0.30759449273102746
1893,3787,1893,5680,2.4287660121917725,0.3025629206360918
1897,3795,1897,5692,2.433612823486328,0.2985134642676712
1902,3805,1902,5707,2.439350128173828,0.29342411963455106
1906,3813,1906,5719,2.443833827972412,0.28933263953592814
1911,3823,1911,5734,2.4495980739593506,0.28419598208324715
1915,3831,1915,5746,2.454103946685791,0.28007080456404765
1920,3841,1920,5761,2.459714889526367,0.2748971922496821
1925,3851,1925,5776,2.4653000831604004,0.269707497589593
1929,3859,1929,5788,2.46972393989563,0.26554629120164464
1934,3869,1934,5803,2.4754638671875,0.2603356234359353
1938,3877,1938,5815,2.480093002319336,0.2561617236268603
1943,3887,1943,5830,2.48579478263855,0.2509402620989931
1947,3895,1947,5842,2.490295171737671,0.24676174566263853
1952,3905,1952,5857,2.4959559440612793,0.24153945803357146
1956,3913,1956,5869,2.5005829334259033,0.23736416012184236
1961,3923,1961,5884,2.5062568187713623,0.23215062168685563
1966,3933,1966,5899,2.5120248794555664,0.22694589265461218
1970,3941,1970,5911,2.5171427726745605,0.22279027250556283
1975,3951,1975,5926,2.5228397846221924,0.21760816056382737
1979,3959,1979,5938,2.5274529457092285,0.21347400449394627
1984,3969,1984,5953,2.533313035964966,0.20832284584491845
1988,3977,1988,5965,2.5377800464630127,0.20421670430994254
1993,3987,1993,5980,2.543332815170288,0.1991045921922705
1998,3997,1998,5995,2.5490479469299316,0.19401764204917527
2002,4005,2002,6007,2.55351185798645,0.18996786670015808
2007,4015,2007,6022,2.5591378211975098,0.18493247041101313
2011,4023,2011,6034,2.5637331008911133,0.18092716959370136
2016,4033,2016,6049,2.569563865661621,0.17595141248796153
2020,4041,2020,6061,2.574144124984741,0.1719970583559416
2025,4051,2025,6076,2.5799827575683594,0.16708901617960237
2029,4059,2029,6088,2.584510087966919,0.16319204172452828
2034,4069,2034,6103,2.590287923812866,0.1583596996132428
2039,4079,2039,6118,2.5958800315856934,0.1535728035696593
2043,4087,2043,6130,2.6004600524902344,0.14977760383112582
2048,4097,2048,6145,2.6060569286346436,0.14507845615889892
2052,4105,2052,6157,2.6105339527130127,0.14135643885231275
2057,4115,2057,6172,2.616209030151367,0.13675239938538652
2061,4123,2061,6184,2.6208059787750244,0.13310928483133466
2066,4133,2066,6199,2.6268019676208496,0.12860725600876322
2070,4141,2070,6211,2.6315829753875732,0.12504833950413285
2075,4151,2075,6226,2.637249708175659,0.12065462391012716
2080,4161,2080,6241,2.643018960952759,0.11632355302288033
2084,4169,2084,6253,2.6475889682769775,0.11290488851648206
2089,4179,2089,6268,2.653204917907715,0.10869056901185559
2093,4187,2093,6280,2.657721996307373,0.10536721063851928
2098,4197,2098,6295,2.663367986679077,0.10127426710664622
2102,4205,2102,6307,2.6679229736328125,0.09804972014558189
2107,4215,2107,6322,2.6736998558044434,0.0940823419177832
2112,4225,2112,6337,2.679642915725708,0.09018643478816557
2116,4233,2116,6349,2.6844959259033203,0.08712196955161744
2121,4243,2121,6364,2.6901509761810303,0.0833577031941104
2125,4251,2125,6376,2.6947360038757324,0.08040007077829614
2130,4261,2130,6391,2.700612783432007,0.07677122758855148
2134,4269,2134,6403,2.70544171333313,0.07392342414675568
2139,4279,2139,6418,2.7115049362182617,0.07043370412202421
2143,4287,2143,6430,2.716114044189453,0.06769864410557602
2148,4297,2148,6445,2.7218990325927734,0.06435161865647387
2153,4307,2153,6460,2.7277328968048096,0.06108534486315875
2157,4315,2157,6472,2.7325329780578613,0.05853114448029828
2162,4325,2162,6487,2.738111972808838,0.05541272778657458
2166,4333,2166,6499,2.742609977722168,0.05297803409609969
2171,4343,2171,6514,2.7482528686523438,0.050010441499011904
2175,4351,2175,6526,2.7527198791503906,0.047697486161382585
2180,4361,2180,6541,2.7583377361297607,0.04488330102731197
2185,4371,2185,6556,2.764216899871826,0.04215527814176312
2189,4379,2189,6568,2.768803834915161,0.040035264190919406
2194,4389,2194,6583,2.774867057800293,0.03746362324545771
2198,4397,2198,6595,2.779520034790039,0.03546922236671435
2203,4407,2203,6610,2.7851641178131104,0.03305505675064069
2207,4415,2207,6622,2.789700984954834,0.03118687458959357
2212,4425,2212,6637,2.795320749282837,0.02893061570921418
2216,4433,2216,6649,2.7999298572540283,0.027188753694531442
2221,4443,2221,6664,2.8056068420410156,0.025090256255111854
2226,4453,2226,6679,2.81123685836792,0.02307917680798255
2230,4461,2230,6691,2.8157310485839844,0.021533099941962064
2235,4471,2235,6706,2.821603775024414,0.01967876361322851
2239,4479,2239,6718,2.8263649940490723,0.01825772059260089
2244,4489,2244,6733,2.8322629928588867,0.01655918961535008
2248,4497,2248,6745,2.8368120193481445,0.015262381673551317
2253,4507,2253,6760,2.8423879146575928,0.013718612215939174
2257,4515,2257,6772,2.846949815750122,0.012545173648163654
2262,4525,2262,6787,2.8526108264923096,0.011155045998975766
2267,4535,2267,6802,2.85829496383667,0.009849757899473843
2271,4543,2271,6814,2.8627641201019287,0.00886634595576652
2276,4553,2276,6829,2.869572877883911,0.00771274803344113
2280,4561,2280,6841,2.874551773071289,0.0068501175799156044
2285,4571,2285,6856,2.880380868911743,0.005846719507076159
2289,4579,2289,6868,2.884855031967163,0.005103569820334997
2294,4589,2294,6883,2.8904950618743896,0.004248582176387572
2299,4599,2299,6898,2.8961679935455322,0.0034751263308407943
2303,4607,2303,6910,2.900702953338623,0.0029145584115894962
2308,4617,2308,6925,2.9065070152282715,0.002285892548911761
2312,4625,2312,6937,2.910989761352539,0.0018400238277536118
2317,4635,2317,6952,2.916653871536255,0.001353182938714781
2321,4643,2321,6964,2.9213907718658447,0.0010194396409133333
2326,4653,2326,6979,2.927323818206787,0.0006709685461601111
2330,4661,2330,6991,2.9319069385528564,0.00044641321198923833
2335,4671,2335,7006,2.9376368522644043,0.0002324530382793455
2340,4681,2340,7021,2.9432787895202637,9.144633145297121e-05
2344,4689,2344,7033,2.9477410316467285,3.0288557468338695e-05
2349,4699,2349,7048,2.953263998031616,1.728579854898271e-05
2353,4707,2353,7060,2.9577369689941406,5.6803480561029573e-05
2358,4717,2358,7075,2.963418960571289,0.00016746933476952108
2362,4725,2362,7087,2.9679927825927734,0.0003041736218847291
2367,4735,2367,7102,2.9743409156799316,0.0005341293931451219
2371,4743,2371,7114,2.979033946990967,0.000764504842209135
2376,4753,2376,7129,2.984807014465332,0.0011093380454667567
2381,4763,2381,7144,2.990431070327759,0.001516066194085397
2385,4771,2385,7156,2.9949378967285156,0.0018850775865075775
2390,4781,2390,7171,3.0004889965057373,0.002399694086989257
2394,4789,2394,7183,3.0051138401031494,0.0028531773432405316
2399,4799,2399,7198,3.0107178688049316,0.0034710490223233137
2403,4807,2403,7210,3.0153439044952393,0.004005237663591288
2408,4817,2408,7225,3.0210719108581543,0.004721570465221703
2413,4827,2413,7240,3.0269358158111572,0.005490460180908485
2417,4835,2417,7252,3.0315659046173096,0.006142353299196657
2422,4845,2422,7267,3.037226915359497,0.007001840708085183
2426,4853,2426,7279,3.0417869091033936,0.007724098692506232
2431,4863,2431,7294,3.047287940979004,0.008668843684404237
2435,4871,2435,7306,3.0518698692321777,0.00945710961389068
2440,4881,2440,7321,3.057485818862915,0.01048156996034777
2444,4889,2444,7333,3.0620779991149902,0.011331343281199224
2449,4899,2449,7348,3.0677058696746826,0.012429826024913382
2454,4909,2454,7363,3.0737040042877197,0.01356693868444836
2458,4917,2458,7375,3.0783729553222656,0.014503239653208766
2463,4927,2463,7390,3.084047794342041,0.015705375538914268
2467,4935,2467,7402,3.088510036468506,0.016691376745143316
2472,4945,2472,7417,3.094241142272949,0.01795274754726961
2476,4953,2476,7429,3.098855972290039,0.018983832999765582
2481,4963,2481,7444,3.1044528484344482,0.020298694050438826
2486,4973,2486,7459,3.110037088394165,0.021640812573650692
2490,4981,2490,7471,3.1145098209381104,0.022732962256668543
2495,4991,2495,7486,3.120450735092163,0.0241197650121876
2499,4999,2499,7498,3.125549793243408,0.02524542763512727
2504,5009,2504,7513,3.1348938941955566,0.02667134762123169
2508,5017,2508,7525,3.1411657333374023,0.0278260983278642
2513,5027,2513,7540,3.1469359397888184,0.02928563756472613
2517,5035,2517,7552,3.1515719890594482,0.030465101103573033
2522,5045,2522,7567,3.1571080684661865,0.031952813396401325
2527,5055,2527,7582,3.1627390384674072,0.03345383436897009
2531,5063,2531,7594,3.167263984680176,0.03466310951819196
2536,5073,2536,7609,3.1731419563293457,0.03618387015387725
2540,5081,2540,7621,3.1776540279388428,0.03740676567849732
2545,5091,2545,7636,3.1832997798919678,0.03894183295210496
2549,5099,2549,7648,3.187757730484009,0.0401739958148255
2554,5109,2554,7663,3.1934139728546143,0.04171792349200132
2558,5117,2558,7675,3.1979708671569824,0.042954997922720395
2563,5127,2563,7690,3.203721046447754,0.04450235307808725
2568,5137,2568,7705,3.2093489170074463,0.04604928540629771
2572,5145,2572,7717,3.2137937545776367,0.047285423996072495
2577,5155,2577,7732,3.219489812850952,0.04882747878173177
2581,5163,2581,7744,3.224416971206665,0.0500576343706598
2586,5173,2586,7759,3.230199098587036,0.05158965652367442
2590,5181,2590,7771,3.234750986099243,0.05280978251471424
2595,5191,2595,7786,3.2403600215911865,0.05432682134721745
2600,5201,2600,7801,3.245987892150879,0.055833482869502404
2604,5209,2604,7813,3.2506461143493652,0.05703038912292868
2609,5219,2609,7828,3.2563648223876953,0.058514837277584775
2613,5227,2613,7840,3.260793924331665,0.059692211854212474
2618,5237,2618,7855,3.266469955444336,0.06115010288181111
2622,5245,2622,7867,3.2712059020996094,0.06230455823640568
2627,5255,2627,7882,3.2771849632263184,0.063731757773553
2631,5263,2631,7894,3.281888008117676,0.06486005855515486
2636,5273,2636,7909,3.2875258922576904,0.06625260145017364
2641,5283,2641,7924,3.2932469844818115,0.06762422617248376
2645,5291,2645,7936,3.297929048538208,0.06870568119200016
2650,5301,2650,7951,3.3037240505218506,0.07003672798282423
2654,5309,2654,7963,3.30834698677063,0.07108423983447665
2659,5319,2659,7978,3.315074920654297,0.07237103370516706
2663,5327,2663,7990,3.32318377494812,0.0733817064460709
2668,5337,2668,8005,3.3302109241485596,0.0746206903016855
2672,5345,2672,8017,3.3349249362945557,0.07559173636491323
2677,5355,2677,8032,3.3406829833984375,0.07677951081120682
2682,5365,2682,8047,3.346273899078369,0.07793744122977841
2686,5373,2686,8059,3.3509247303009033,0.07884166214500965
2691,5383,2691,8074,3.3565549850463867,0.07994352565106055
2695,5391,2695,8086,3.361158847808838,0.08080174991198419
2700,5401,2700,8101,3.3668220043182373,0.08184476227108917
2704,5409,2704,8113,3.371884822845459,0.08265487706250951
2709,5419,2709,8128,3.3775429725646973,0.08363654185143332
2714,5429,2714,8143,3.3832719326019287,0.0845831508363517
2718,5437,2718,8155,3.38798189163208,0.08531476845735142
2723,5447,2723,8170,3.3935139179229736,0.08619670153620973
2727,5455,2727,8182,3.398198127746582,0.08687582684024164
2732,5465,2732,8197,3.403860092163086,0.0876912645592256
2736,5473,2736,8209,3.408342123031616,0.08831653077436386
2741,5483,2741,8224,3.4138739109039307,0.08906386776084219
2745,5491,2745,8236,3.4184348583221436,0.08963406783288974
2750,5501,2750,8251,3.424499034881592,0.09031188610276786
2755,5511,2755,8266,3.4302449226379395,0.09095053367207129
2759,5519,2759,8278,3.4348130226135254,0.09143300888194972
2764,5529,2764,8293,3.4404890537261963,0.0920002730467786
2768,5537,2768,8305,3.44508695602417,0.09242523259104019
2773,5547,2773,8320,3.4508650302886963,0.09292013896163098
2777,5555,2777,8332,3.455387830734253,0.09328687935862945
2782,5565,2782,8347,3.4609038829803467,0.09370864934510337
2787,5575,2787,8362,3.4666199684143066,0.09408953108231799
2791,5583,2791,8374,3.471695899963379,0.09436470609591652
2796,5593,2796,8389,3.478257894515991,0.0946716814029287
2800,5601,2800,8401,3.4830169677734375,0.09488763077422391
2805,5611,2805,8416,3.488837957382202,0.09512051233139118
2809,5619,2809,8428,3.4935450553894043,0.0952771847855729
2814,5629,2814,8443,3.4994709491729736,0.09543603086626717
2818,5637,2818,8455,3.504450798034668,0.09553356928847734
2823,5647,2823,8470,3.510241746902466,0.09561867555635217
2828,5657,2828,8485,3.5167088508605957,0.09566302545067629
2832,5665,2832,8497,3.521451950073242,0.09566929112611433
2837,5675,2837,8512,3.5281169414520264,0.09564079544190918
2841,5683,2841,8524,3.5329558849334717,0.09558909599820709
2846,5693,2846,8539,3.539255142211914,0.0954885808932886
2850,5701,2850,8551,3.543980121612549,0.0953796494574135
2855,5711,2855,8566,3.5497379302978516,0.09520811765491999
2859,5719,2859,8578,3.554403781890869,0.09504282287582555
2864,5729,2864,8593,3.560241937637329,0.09480144029282656
2869,5739,2869,8608,3.566066026687622,0.0945218123374616
2873,5747,2873,8620,3.5707709789276123,0.0942708633182292
2878,5757,2878,8635,3.5767529010772705,0.09392350128166527
2882,5765,2882,8647,3.5815370082855225,0.09361896921484458
2887,5775,2887,8662,3.589263916015625,0.09320542123543873
2891,5783,2891,8674,3.593965768814087,0.09284860258776462
2896,5793,2896,8689,3.6000759601593018,0.09237056166853108
2901,5803,2901,8704,3.605865955352783,0.09185747631147478
2905,5811,2905,8716,3.610862970352173,0.09142217321459611
2910,5821,2910,8731,3.6170239448547363,0.09084751716977735
2914,5829,2914,8743,3.6218509674072266,0.09036376803328494
2919,5839,2919,8758,3.627586841583252,0.08972960465303004
2923,5847,2923,8770,3.632222890853882,0.08919911687223703
2928,5857,2928,8785,3.6379411220550537,0.08850764968872227
2932,5865,2932,8797,3.6423799991607666,0.08793223990949173
2937,5875,2937,8812,3.6481800079345703,0.08718580428899259
2942,5885,2942,8827,3.6538538932800293,0.08640988435058716
2946,5893,2946,8839,3.6584229469299316,0.08576844092294778
2951,5903,2951,8854,3.664155960083008,0.08494141754988505
2955,5911,2955,8866,3.6686758995056152,0.08426012666348015
2960,5921,2960,8881,3.6746819019317627,0.08338461104119688
2964,5929,2964,8893,3.6794159412384033,0.08266559570859044
2969,5939,2969,8908,3.6851608753204346,0.08174428068980433
2973,5947,2973,8920,3.6897048950195312,0.08098972415848493
2978,5957,2978,8935,3.6954410076141357,0.08002537235665841
2983,5967,2983,8950,3.7011258602142334,0.07903832777287789
2987,5975,2987,8962,3.705620050430298,0.07823294530658131
2992,5985,2992,8977,3.7112619876861572,0.07720728126059839
2996,5993,2996,8989,3.7158589363098145,0.07637216173327488
3001,6003,3001,9004,3.7216148376464844,0.0753107882576387
3005,6011,3005,9016,3.726285934448242,0.0744482806983342
3010,6021,3010,9031,3.732095956802368,0.07335415965599168
3015,6031,3015,9046,3.737783908843994,0.07224314334087012
3019,6039,3019,9058,3.7422099113464355,0.07134279492504447
3024,6049,3024,9073,3.747936964035034,0.07020373212333197
3028,6057,3028,9085,3.7523488998413086,0.06928217156200844
3033,6067,3033,9100,3.758063793182373,0.0681181326119713
3037,6075,3037,9112,3.7626569271087646,0.06717782662269656
3042,6085,3042,9127,3.768317937850952,0.06599190372935482
3046,6093,3046,9139,3.772979974746704,0.06503532962926784
3051,6103,3051,9154,3.7789688110351562,0.06383061892654496
3056,6113,3056,9169,3.7848339080810547,0.06261680359227739
3060,6121,3060,9181,3.7892749309539795,0.0616398321702718
3065,6131,3065,9196,3.7949440479278564,0.060412009349192886
3069,6139,3069,9208,3.7995219230651855,0.05942504753443245
3074,6149,3074,9223,3.8051180839538574,0.05818624539335815
3078,6157,3078,9235,3.809609889984131,0.05719169863425577
3083,6167,3083,9250,3.8152430057525635,0.05594490207386116
3087,6175,3087,9262,3.819689989089966,0.054945140994050234
3092,6185,3092,9277,3.82542085647583,0.05369329266352452
3097,6195,3097,9292,3.83123779296875,0.05243989545408567
3101,6203,3101,9304,3.835783004760742,0.05143666156618565
3106,6213,3106,9319,3.841491937637329,0.05018271886228831
3110,6221,3110,9331,3.8459479808807373,0.04918019501042181
3115,6231,3115,9346,3.8516199588775635,0.047928565633924336
3119,6239,3119,9358,3.856096029281616,0.04692902754675288
3124,6249,3124,9373,3.8616750240325928,0.04568254122887083
3129,6259,3129,9388,3.8674609661102295,0.044440122368996526
3133,6267,3133,9400,3.8720319271087646,0.0434496908710571
3138,6277,3138,9415,3.8778817653656006,0.0422167427605018
3142,6285,3142,9427,3.8826968669891357,0.04123498026820016
3147,6295,3147,9442,3.888439178466797,0.0400142171929474
3151,6303,3151,9454,3.8929879665374756,0.03904326751001008
3156,6313,3156,9469,3.898800849914551,0.037837329755802784
3160,6321,3160,9481,3.9034907817840576,0.03687926985787726
3165,6331,3165,9496,3.909661054611206,0.03569070481125891
3170,6341,3170,9511,3.9154069423675537,0.034512852191483034
3174,6349,3174,9523,3.9200119972229004,0.033578775682485684
3179,6359,3179,9538,3.9261510372161865,0.03242203581078229
3183,6367,3183,9550,3.930975914001465,0.03150576111909231
3188,6377,3188,9565,3.9366719722747803,0.030372380095968765
3192,6385,3192,9577,3.9411678314208984,0.029475653352847075
3197,6395,3197,9592,3.9467568397521973,0.028367751092901017
3202,6405,3202,9607,3.9524857997894287,0.027274875004764
3206,6413,3206,9619,3.956990957260132,0.026411795202307076
3211,6423,3211,9634,3.9627299308776855,0.025347460008333655
3215,6431,3215,9646,3.967345952987671,0.024507956559546074
3220,6441,3220,9661,3.9730279445648193,0.02347399625057278
3224,6449,3224,9673,3.977465867996216,0.02265949870241002
3229,6459,3229,9688,3.9831130504608154,0.021657655830949807
3233,6467,3233,9700,3.9876580238342285,0.020869524267936868
3238,6477,3238,9715,3.993346929550171,0.019901457792798283
3243,6487,3243,9730,3.9991397857666016,0.01895284272529807
3247,6495,3247,9742,4.003619909286499,0.01820827342260145
3252,6505,3252,9757,4.009365081787109,0.017295849927791096
3256,6513,3256,9769,4.013974905014038,0.016580817938461223
3261,6523,3261,9784,4.0198280811309814,0.015706019525850934
3265,6531,3265,9796,4.024526834487915,0.015021628858676195
3270,6541,3270,9811,4.0304200649261475,0.014185777264060562
3274,6549,3274,9823,4.034980773925781,0.01353303501434766
3279,6559,3279,9838,4.040509939193726,0.012737321444546978
3284,6569,3284,9853,4.046156883239746,0.01196436790394273
3288,6577,3288,9865,4.050766944885254,0.011362591919464649
3293,6587,3293,9880,4.056441783905029,0.010631333294213619
3297,6595,3297,9892,4.060895919799805,0.010063249392374018
3302,6605,3302,9907,4.066538095474243,0.0093744851867541
3306,6613,3306,9919,4.0713160037994385,0.008840670621339086
3311,6623,3311,9934,4.07725191116333,0.008195046960054242
3316,6633,3316,9949,4.083354949951172,0.007573617208208816
3320,6641,3320,9961,4.087865829467773,0.00709398393689753
3325,6651,3325,9976,4.093545913696289,0.006516428314853329
3329,6659,3329,9988,4.0982489585876465,0.006072035057854919
3334,6669,3334,10003,4.103919982910156,0.0055386790934335295
3338,6677,3338,10015,4.108475923538208,0.005129747361252157
3343,6687,3343,10030,4.114236831665039,0.004640823155568796
3347,6695,3347,10042,4.118780851364136,0.004267504988206383
3352,6705,3352,10057,4.124696969985962,0.0038231624175750767
3357,6715,3357,10072,4.130875825881958,0.0034036230855463145
3361,6723,3361,10084,4.135429859161377,0.003085855606741461
3366,6733,3366,10099,4.141134977340698,0.002710971304281884
3370,6741,3370,10111,4.145676136016846,0.002428911142146717
3375,6751,3375,10126,4.1514739990234375,0.002098614644182817
3379,6759,3379,10138,4.155967950820923,0.001852167274819294
3384,6769,3384,10153,4.161581754684448,0.0015662855385016883
3388,6777,3388,10165,4.166181802749634,0.0013552657732134321
3393,6787,3393,10180,4.172039031982422,0.0011135054741089334
3398,6797,3398,10195,4.177984952926636,0.0008960825165331698
3402,6805,3402,10207,4.182761907577515,0.0007395644672669732
3407,6815,3407,10222,4.188498020172119,0.0005655458226101473
3411,6823,3411,10234,4.19298791885376,0.00044351266149078583
3416,6833,3416,10249,4.19874382019043,0.0003122687481891262
3420,6841,3420,10261,4.203297853469849,0.00022416673220959638
3425,6851,3425,10276,4.208791732788086,0.00013494614722731058
3430,6861,3430,10291,4.214511871337891,6.870724894270097e-05
3434,6869,3434,10303,4.21896505355835,3.2074598607323423e-05
3439,6879,3439,10318,4.224740982055664,6.485020435320621e-06
3443,6887,3443,10330,4.229359865188599,1.9837827949231723e-06
3448,6897,3448,10345,4.235170841217041,1.6055097717071476e-05
3452,6905,3452,10357,4.239731073379517,4.286767057237739e-05
3457,6915,3457,10372,4.245463848114014,9.554777193443442e-05
3461,6923,3461,10384,4.250020980834961,0.00015281049559234816
3466,6933,3466,10399,4.255573034286499,0.00024299447920839157
3471,6943,3471,10414,4.261337995529175,0.0003535190323873394
3475,6951,3475,10426,4.266077995300293,0.00045633981744686025
3480,6961,3480,10441,4.2720348834991455,0.0006025556048143699
3484,6969,3484,10453,4.276839017868042,0.0007334437607369182
3489,6979,3489,10468,4.282676935195923,0.0009141233346099398
3493,6987,3493,10480,4.2871928215026855,0.0010720755832380746
3498,6997,3498,10495,4.292857885360718,0.001285936407043664
3503,7007,3503,10510,4.298450946807861,0.0015176544865198593
3507,7015,3507,10522,4.3028810024261475,0.0017156000367322122
3512,7025,3512,10537,4.3086419105529785,0.0019783786929110647
3516,7033,3516,10549,4.3133158683776855,0.0022005994887877023
3521,7043,3521,10564,4.319093942642212,0.002492987471782726
3525,7051,3525,10576,4.324351072311401,0.0027382945659155666
3530,7061,3530,10591,4.333079814910889,0.003058771502082891
3534,7069,3534,10603,4.33965277671814,0.0033259222951755874
3539,7079,3539,10618,4.345654010772705,0.00367290411486465
3544,7089,3544,10633,4.351223945617676,0.004033906138488419
3548,7097,3548,10645,4.355699062347412,0.004332457670898293
3553,7107,3553,10660,4.361399173736572,0.0047173987544510965
3557,7115,3557,10672,4.365966796875,0.0050344265492867635
3562,7125,3562,10687,4.371692895889282,0.005441612880190405
3566,7133,3566,10699,4.376415967941284,0.005775753498596714
3571,7143,3571,10714,4.382375955581665,0.006203473946584381
3575,7151,3575,10726,4.38692307472229,0.006553355494361313
3580,7161,3580,10741,4.392685890197754,0.006999894336217949
3585,7171,3585,10756,4.3984479904174805,0.00745614784227655
3589,7179,3589,10768,4.402869939804077,0.00782779110033971
3594,7189,3594,10783,4.408568859100342,0.008300204321130877
3598,7197,3598,10795,4.413088083267212,0.008684095088938193
3603,7207,3603,10810,4.418657064437866,0.00917096923490135
3607,7215,3607,10822,4.423407793045044,0.009565750927777117
3612,7225,3612,10837,4.429343938827515,0.010065391987041039
3617,7235,3617,10852,4.435171842575073,0.010571393609097868
3621,7243,3621,10864,4.439511775970459,0.010980422323541461
3626,7253,3626,10879,4.4451069831848145,0.011496551064396954
3630,7261,3630,10891,4.44962477684021,0.011912999433207005
3635,7271,3635,10906,4.455413103103638,0.012437547489412282
3639,7279,3639,10918,4.459909915924072,0.012860045166462442
3644,7289,3644,10933,4.465657949447632,0.013391295014343996
3648,7297,3648,10945,4.470308780670166,0.013818465236226984
3653,7307,3653,10960,4.476037979125977,0.014354694428220682
3658,7317,3658,10975,4.481836795806885,0.014892946917257177
3662,7325,3662,10987,4.486655950546265,0.015324650839261267
3667,7335,3667,11002,4.492396116256714,0.015865217581335855
3671,7343,3671,11014,4.496914863586426,0.016298095947604452
3676,7353,3676,11029,4.502892732620239,0.016839292915278747
3680,7361,3680,11041,4.507595062255859,0.017272012616331267
3685,7371,3685,11056,4.5135087966918945,0.017812194077805543
3689,7379,3689,11068,4.522937774658203,0.01824345692443785
3694,7389,3694,11083,4.529381990432739,0.01878102505907009
3699,7399,3699,11098,4.535445928573608,0.01931647030221484
3703,7407,3703,11110,4.540010929107666,0.019742983409855697
3708,7417,3708,11125,4.545757055282593,0.020273434794262357
3712,7425,3712,11137,4.550341844558716,0.02069536182614229
3717,7435,3717,11152,4.556116104125977,0.021219354329787166
3721,7443,3721,11164,4.56053900718689,0.021635541858586294
3726,7453,3726,11179,4.566209077835083,0.022151655217953703
3731,7463,3731,11194,4.572041034698486,0.022662791888251377
3735,7471,3735,11206,4.57706093788147,0.02306783514836752
3740,7481,3740,11221,4.583226919174194,0.023568957462998696
3744,7489,3744,11233,4.587682723999023,0.02396545356839397
3749,7499,3749,11248,4.593336820602417,0.024455230616126755
3753,7507,3753,11260,4.597933769226074,0.02484212780325379
3758,7517,3758,11275,4.603526830673218,0.02531926196149925
3762,7525,3762,11287,4.608072996139526,0.02569553686043946
3767,7535,3767,11302,4.613703966140747,0.02615876924312488
3772,7545,3772,11317,4.619338035583496,0.026613751526156193
3776,7553,3776,11329,4.623962879180908,0.02697155196233325
3781,7563,3781,11344,4.629780054092407,0.027410772460484623
3785,7571,3785,11356,4.634382963180542,0.02775550958438089
3790,7581,3790,11371,4.640069961547852,0.028177851313898827
3794,7589,3794,11383,4.644670009613037,0.028508659681619974
3799,7599,3799,11398,4.650478839874268,0.02891307794163822
3804,7609,3804,11413,4.656207799911499,0.029307115872597933
3808,7617,3808,11425,4.660664796829224,0.029614680602094268
3813,7627,3813,11440,4.6662819385528564,0.029989325690053192
3817,7635,3817,11452,4.670721769332886,0.030281030698347422
3822,7645,3822,11467,4.676459074020386,0.030635439424713695
3826,7653,3826,11479,4.681077003479004,0.030910640444062665
3831,7663,3831,11494,4.686809778213501,0.031244044255799963
3835,7671,3835,11506,4.6913957595825195,0.03150215463551831
3840,7681,3840,11521,4.6970908641815186,0.03181385365269307
3845,7691,3845,11536,4.7028419971466064,0.03211321500509712
3849,7699,3849,11548,4.707414865493774,0.032343694891437735
3854,7709,3854,11563,4.713059902191162,0.032620383062180736
3858,7717,3858,11575,4.717684030532837,0.032832497714252895
3863,7727,3863,11590,4.7236528396606445,0.03308595941621206
3867,7735,3867,11602,4.728827953338623,0.033279286835863786
3872,7745,3872,11617,4.734868049621582,0.03350902033048442
3876,7753,3876,11629,4.739430904388428,0.03368318004129378
3881,7763,3881,11644,4.7451090812683105,0.03388873670883186
3886,7773,3886,11659,4.750925779342651,0.034080688939639
3890,7781,3890,11671,4.75547194480896,0.03422438120298921
3895,7791,3895,11686,4.761180877685547,0.0343915757873674
3899,7799,3899,11698,4.7656049728393555,0.034515339309223236
3904,7809,3904,11713,4.771320819854736,0.0346574882596542
3908,7817,3908,11725,4.776141881942749,0.034761121915153126
3913,7827,3913,11740,4.7820470333099365,0.03487801191431572
3918,7837,3918,11755,4.787709951400757,0.034980806053454216
3922,7845,3922,11767,4.7922587394714355,0.03505287338737162
3927,7855,3927,11782,4.797987937927246,0.03513023494792833
3931,7863,3931,11794,4.802602052688599,0.03518194440266598
3936,7873,3936,11809,4.808336973190308,0.035233864248652935
3940,7881,3940,11821,4.812812805175781,0.03526523954133154
3945,7891,3945,11836,4.818547010421753,0.03529178469045746
3949,7899,3949,11848,4.823302984237671,0.035302908045423465
3954,7909,3954,11863,4.82926082611084,0.03530421508150994
3959,7919,3959,11878,4.835078954696655,0.03529158297158119
3963,7927,3963,11890,4.839572906494141,0.035271488385205885
3968,7937,3968,11905,4.845262765884399,0.035233950221368104
3972,7945,3972,11917,4.849900007247925,0.035194037607425344
3977,7955,3977,11932,4.855568885803223,0.03513187275348173
3981,7963,3981,11944,4.860028982162476,0.03507238424754178
3986,7973,3986,11959,4.8657097816467285,0.034985917882636386
3990,7981,3990,11971,4.87034797668457,0.034907131344198206
3995,7991,3995,11986,4.876342058181763,0.034796732940776565
4000,8001,4000,12001,4.882279872894287,0.03467321528466982
4004,8009,4004,12013,4.886948823928833,0.03456504660414339
4009,8019,4009,12028,4.89254093170166,0.03441826355901867
4013,8027,4013,12040,4.897027969360352,0.0342916743021533
4018,8037,4018,12055,4.902761936187744,0.03412211907175333
4022,8045,4022,12067,4.907330751419067,0.033977525570207945
4027,8055,4027,12082,4.912970066070557,0.03378574669466161
4032,8065,4032,12097,4.918720960617065,0.03358187965648085
4036,8073,4036,12109,4.923840045928955,0.03341021474727768
4041,8083,4041,12124,4.929879903793335,0.03318509268615344
4045,8091,4045,12136,4.934544801712036,0.03299669638158775
4050,8101,4050,12151,4.940047979354858,0.032751015220128465
4054,8109,4054,12163,4.944534778594971,0.03254646595155464
4059,8119,4059,12178,4.950243949890137,0.03228097442854505
4063,8127,4063,12190,4.95480489730835,0.032060890496040884
4068,8137,4068,12205,4.960470914840698,0.03177638374484104
4073,8147,4073,12220,4.966249942779541,0.03148167114795797
4077,8155,4077,12232,4.970946788787842,0.031238729519259323
4082,8165,4082,12247,4.977046012878418,0.030926312850738213
4086,8173,4086,12259,4.981997728347778,0.030669557302189787
4091,8183,4091,12274,4.987775087356567,0.030340316270212497
4095,8191,4095,12286,4.992316961288452,0.03007045993297197
4100,8201,4100,12301,4.998031854629517,0.02972529658916301
4105,8211,4105,12316,5.003523826599121,0.029371684492161876
4109,8219,4109,12328,5.008039951324463,0.029082904872211657
4114,8229,4114,12343,5.013797998428345,0.0287148119413132
4118,8237,4118,12355,5.018548011779785,0.028414826018320127
4123,8247,4123,12370,5.0245137214660645,0.028033203327140654
4127,8255,4127,12382,5.03088903427124,0.02772278011502749
4132,8265,4132,12397,5.036526918411255,0.02732859965226453
4136,8273,4136,12409,5.041043996810913,0.027008525713085874
4141,8283,4141,12424,5.0467369556427,0.026602782354189003
4146,8293,4146,12439,5.05239200592041,0.026191053906586603
4150,8301,4150,12451,5.056995868682861,0.02585757586894033
4155,8311,4155,12466,5.062658786773682,0.025435879895667313
4159,8319,4159,12478,5.067378997802734,0.025094847564673728
4164,8329,4164,12493,5.07336688041687,0.024664238831405783
4168,8337,4168,12505,5.078426837921143,0.024316504008879747
4173,8347,4173,12520,5.084453821182251,0.02387805600642423
4177,8355,4177,12532,5.08905291557312,0.023524483377514116
4182,8365,4182,12547,5.094682931900024,0.023079282667708867
4187,8375,4187,12562,5.100566864013672,0.022630802549770124
4191,8383,4191,12574,5.105597019195557,0.022269884123261363
4196,8393,4196,12589,5.111530065536499,0.02181635135673332
4200,8401,4200,12601,5.116055727005005,0.02145182715730698
4205,8411,4205,12616,5.121944904327393,0.02099433074033641
4209,8419,4209,12628,5.126662015914917,0.020627068621138278
4214,8429,4214,12643,5.133074998855591,0.020166688070958116
4219,8439,4219,12658,5.138661861419678,0.01970516706512626
4223,8447,4223,12670,5.143268823623657,0.019335348873710245
4228,8457,4228,12685,5.148940086364746,0.01887259715590517
4232,8465,4232,12697,5.153432846069336,0.018502213897022557
4237,8475,4237,12712,5.159105062484741,0.018039276753938793
4241,8483,4241,12724,5.163651943206787,0.017669159442334603
4246,8493,4246,12739,5.169305801391602,0.017207069517894524
4250,8501,4250,12751,5.1743550300598145,0.01683803967341646
4255,8511,4255,12766,5.180311918258667,0.016377818480464157
4260,8521,4260,12781,5.186117887496948,0.015919073096029024
4264,8529,4264,12793,5.19071102142334,0.01555334799047614
4269,8539,4269,12808,5.196444034576416,0.015098039866529689
4273,8547,4273,12820,5.201129913330078,0.014735463374108804
4278,8557,4278,12835,5.206787824630737,0.014284586093140206
4282,8565,4282,12847,5.211146116256714,0.013925947418783835
4287,8575,4287,12862,5.2168238162994385,0.013480479314694094
4291,8583,4291,12874,5.221527814865112,0.013126553645633976
4296,8593,4296,12889,5.227380990982056,0.012687452961017698
4301,8603,4301,12904,5.233222961425781,0.01225229457372734
4305,8611,4305,12916,5.237810850143433,0.01190719654618988
4310,8621,4310,12931,5.243499040603638,0.01147984320687101
4314,8629,4314,12943,5.248058795928955,0.011141345896589883
4319,8639,4319,12958,5.253619909286499,0.01072268009693289
4323,8647,4323,12970,5.258116960525513,0.010391475007395456
4328,8657,4328,12985,5.2637619972229,0.009982342365219665
4333,8667,4333,13000,5.2693798542022705,0.009578857165138288
4337,8675,4337,13012,5.274013996124268,0.009260298334083927
4342,8685,4342,13027,5.279994964599609,0.008867585183907067
4346,8693,4346,13039,5.284553050994873,0.008557946978271502
4351,8703,4351,13054,5.290333032608032,0.00817675369501103
4355,8711,4355,13066,5.294864892959595,0.007876619640342142
4360,8721,4360,13081,5.30068302154541,0.007507657633368581
4364,8729,4364,13093,5.305328845977783,0.0072175827406226745
4369,8739,4369,13108,5.31090784072876,0.00686152842536103
4374,8749,4374,13123,5.316529989242554,0.006512924695130096
4378,8757,4378,13135,5.321155786514282,0.006239535532017726
4383,8767,4383,13150,5.327126741409302,0.005904823294031303
4387,8775,4387,13162,5.331899881362915,0.0056427859788072965
4392,8785,4392,13177,5.337547063827515,0.005322552329403152
4396,8793,4396,13189,5.342095851898193,0.005072321557690884
4401,8803,4401,13204,5.347858905792236,0.004767115371350883
4406,8813,4406,13219,5.353478908538818,0.0044704798169732385
4410,8821,4410,13231,5.358019828796387,0.004239442674361271
4415,8831,4415,13246,5.363781929016113,0.0039586046394788355
4419,8839,4419,13258,5.368330955505371,0.003740384946922859
4424,8849,4424,13273,5.3740198612213135,0.0034757805157141775
4428,8857,4428,13285,5.378657102584839,0.0032707076237556976
4433,8867,4433,13300,5.3843019008636475,0.0030227235509983075
4437,8875,4437,13312,5.388844013214111,0.0028310866359788633
4442,8885,4442,13327,5.394654035568237,0.00260005890265802
4447,8895,4447,13342,5.400353908538818,0.00237857776699002
4451,8903,4451,13354,5.405027866363525,0.0022083200204860987
4456,8913,4456,13369,5.4106409549713135,0.002004217049830004
4460,8921,4460,13381,5.415151834487915,0.0018479501561614597
4465,8931,4465,13396,5.4213340282440186,0.001661433786125599
4469,8939,4469,13408,5.426390886306763,0.0015193056494808843
4474,8949,4474,13423,5.432598114013672,0.001350537845951294
4478,8957,4478,13435,5.4370808601379395,0.0012226601816109905
4483,8967,4483,13450,5.442764759063721,0.0010717588678517131
4488,8977,4488,13465,5.448657035827637,0.0009308188117529426
4492,8985,4492,13477,5.453467845916748,0.0008252501247625332
4497,8995,4497,13492,5.45907998085022,0.0007022769854074795
4501,9003,4501,13504,5.463624954223633,0.0006110910863981189
4506,9013,4506,13519,5.469280958175659,0.0005060974921207162
4510,9021,4510,13531,5.474126815795898,0.0004292882116487817
4515,9031,4515,13546,5.479684829711914,0.00034224589137465955
4520,9041,4520,13561,5.485306978225708,0.0002651488470064578
4524,9049,4524,13573,5.489876985549927,0.00021061248082787642
4529,9059,4529,13588,5.49551796913147,0.0001513383763267484
4533,9067,4533,13600,5.500058889389038,0.00011100935807917267
4538,9077,4538,13615,5.505795955657959,6.941884998923342e-05
4542,9085,4542,13627,5.510303020477295,4.316731974540744e-05
4547,9095,4547,13642,5.516205787658691,1.9074816236752667e-05
4551,9103,4551,13654,5.520921945571899,6.733567715855315e-06
4556,9113,4556,13669,5.527065992355347,9.337225037597818e-09


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0011000633239746094,2181.2938132599165
2002,2003,2002,4005,2.280527114868164,58.98939413564449
4004,4005,4004,8009,4.509216070175171,53.03643300809222
6006,6007,6006,12013,6.557736396789551,50.14448564934969
8008,8009,8008,16017,9.011595010757446,47.78238326053793
10010,10011,10010,20021,11.676583290100098,45.667972303392844
12012,12013,12012,24025,13.8959321975708,43.73827157437995
14014,14015,14014,28029,17.115005254745483,41.96421429747534
16016,16017,16016,32033,19.955968141555786,40.326626752231505
18018,18019,18018,36037,22.13455104827881,38.81085736169712
20020,20021,20020,40041,24.704042196273804,37.404696941323664
22022,22023,22022,44045,27.0596821308136,36.09739520430389
24024,24025,24024,48049,29.155108213424683,34.87920504021599
26026,26027,26026,52053,31.147736072540283,33.741197391877904
28028,28029,28028,56057,33.136481046676636,32.675202996515736
30030,30031,30030,60061,35.19402813911438,31.67380030947197
32032,32033,32032,64065,37.19806528091431,30.730308340338524
34034,34035,34034,68069,39.248173236846924,29.83876717643193
36036,36037,36036,72073,41.24838399887085,28.99390239063723
38038,38039,38038,76077,43.24014639854431,28.191075966046128
40040,40041,40040,80081,45.24280023574829,27.426228613720923
42042,42043,42042,84085,47.260823249816895,26.69581838396789
44044,44045,44044,88089,49.3740131855011,25.99675953070073
46046,46047,46046,92093,51.942129373550415,25.326364396208646
48048,48049,48048,96097,54.37241721153259,24.682289990762683
50050,50051,50050,100101,56.312294244766235,24.062490081422084
52052,52053,52052,104105,58.327967405319214,23.465172994981003
54054,54055,54054,108109,60.33034825325012,22.888764946980018
56056,56057,56056,112113,62.29389023780823,22.331878481869126
58058,58059,58058,116117,64.30425119400024,21.793285499888043
60060,60061,60060,120121,66.25876307487488,21.271894313895928
62062,62063,62062,124125,68.21049332618713,20.76673019411305
64064,64065,64064,128129,70.2581512928009,20.27691889943162
66066,66067,66066,132133,72.92543721199036,19.801672746742724
68068,68069,68068,136137,75.38293027877808,19.340278825864743
70070,70071,70070,140141,77.42764639854431,18.892089022114533
72072,72073,72072,144145,79.48442029953003,18.456511558652437
74074,74075,74074,148149,81.4573004245758,18.033094262313625
76076,76077,76076,152153,83.39859938621521,17.621252501791332
78078,78079,78078,156157,85.35580229759216,17.220515531400224
80080,80081,80080,160161,87.27231526374817,16.83045515125127
82082,82083,82082,164165,89.22171115875244,16.45067273713653
84084,84085,84084,168169,91.16441917419434,16.080795952795256
86086,86087,86086,172173,93.06998825073242,15.720475925140931
88088,88089,88088,176177,95.00507020950317,15.369384805435402
90090,90091,90090,180181,96.97749829292297,15.027213657072139
92092,92093,92092,184185,98.89448118209839,14.69367062078129
94094,94095,94094,188189,101.39060306549072,14.368479316052458
96096,96097,96096,192193,103.7192862033844,14.051377444162767
98098,98099,98098,196197,106.59745216369629,13.742115563676407
100100,100101,100100,200201,108.68919515609741,13.440456013834478
102102,102103,102102,204205,110.87200832366943,13.146171965067651
104104,104105,104104,208209,113.02520513534546,12.85904657902438
106106,106107,106106,212213,115.11272120475769,12.578872263163817
108108,108109,108108,216217,117.22778534889221,12.30545000719394
110110,110111,110110,220221,119.23177218437195,12.038588790493577
112112,112113,112112,224225,121.39110016822815,11.778105051239208
114114,114115,114114,228229,123.82145023345947,11.523822209284504
116116,116117,116116,232233,126.87766718864441,11.275570235959549
118118,118119,118118,236237,129.08838033676147,11.033185264917847
120120,120121,120120,240241,131.08825016021729,10.79650923896861
122122,122123,122122,244245,133.07888531684875,10.565389588519793
124124,124125,124124,248249,135.25730109214783,10.339678937857911
126126,126127,126126,252253,137.34092116355896,10.119234835991392
128128,128129,128128,256257,139.30051040649414,9.903919509231628
130130,130131,130130,260261,141.35481333732605,9.693599633051008
132132,132133,132132,264265,143.39034914970398,9.488146121100954
134134,134135,134134,268269,145.55514645576477,9.287433929541862
136136,136137,136136,272273,147.500794172287,9.091341875098124
138138,138139,138138,276277,149.50001215934753,8.899752465451002
140140,140141,140140,280281,151.48497009277344,8.71255174078658
142142,142143,142142,284285,153.50501823425293,8.529629125458314
144144,144145,144144,288289,155.49493718147278,8.350877288881179
146146,146147,146146,292293,157.45935535430908,8.176192014876847
148148,148149,148148,296297,159.41884422302246,8.005472078803791
150150,150151,150150,300301,161.35276627540588,7.838619131879341
152152,152153,152152,304305,163.26719737052917,7.675537592176283
154154,154155,154154,308309,165.20732736587524,7.516134541831548
156156,156157,156156,312313,167.14945816993713,7.36031963004632
158158,158159,158158,316317,169.07266306877136,7.208004981495151
160160,160161,160160,320321,171.03576135635376,7.0591051097869695
162162,162163,162162,324325,173.0136570930481,6.913536835643868
164164,164165,164164,328329,174.9808051586151,6.771219209477181
166166,166167,166166,332333,177.0032093524933,6.6320734380631166
168168,168169,168168,336337,179.2143042087555,6.496022815018591
170170,170171,170170,340341,181.37208223342896,6.362992654809773
172172,172173,172172,344345,183.30688738822937,6.23291023002173
174174,174175,174174,348349,185.1022481918335,6.1057047116416925
176176,176177,176176,352353,187.153626203537,5.981307112122522
178178,178179,178178,356357,189.83672332763672,5.859650231003798
180180,180181,180180,360361,192.7216193675995,5.740668602889286
182182,182183,182182,364365,195.54861903190613,5.624298447595493
184184,184185,184184,368369,200.29076409339905,5.510477622299618
186186,186187,186186,372373,204.16207718849182,5.399145575536409
188188,188189,188188,376377,207.190580368042,5.29024330290531
190190,190191,190190,380381,209.3960452079773,5.18371330436446
192192,192193,192192,384385,211.77341318130493,5.079499543003408
194194,194195,194194,388389,214.6214473247528,4.977547405196333
196196,196197,196196,392393,217.24164199829102,4.877803662050042
198198,198199,198198,396397,219.55877017974854,4.780216432071825
200200,200201,200200,400401,222.1956160068512,4.684735144986007
202202,202203,202202,404405,224.66296815872192,4.591310506644277
204204,204205,204204,408409,227.89457726478577,4.4998944649712485
206206,206207,206206,412413,230.519287109375,4.410440176899783
208208,208209,208208,416417,232.87555313110352,4.322901976254116
210210,210211,210210,420421,235.27060914039612,4.237235342538952
212212,212213,212212,424425,237.4436752796173,4.15339687060316
214214,214215,214214,428429,239.74439334869385,4.071344241143038
216216,216217,216216,432433,242.01642322540283,3.9910361920165087
218218,218219,218218,436437,244.2860233783722,3.912432490343349
220220,220221,220220,440441,246.9726321697235,3.835493905362455
222222,222223,222222,444445,249.60929107666016,3.7601821820259147
224224,224225,224224,448449,252.18155908584595,3.686460015306807
226226,226227,226226,452453,254.5910611152649,3.6142910251994635
228228,228229,228228,456457,256.90168499946594,3.543639732393899
230230,230231,230230,460461,259.2921531200409,3.474471534603026
232232,232233,232232,464465,261.60894322395325,3.406752683528225
234234,234235,234234,468469,264.0016140937805,3.3404502624438237
236236,236237,236236,472473,266.22930932044983,3.2755321643836623
238238,238239,238238,476477,268.5235741138458,3.2119670709150796
240240,240241,240240,480481,270.8299193382263,3.1497244314853106
242242,242243,242242,484485,273.05086731910706,3.0887744433214266
244244,244245,244244,488489,275.30400943756104,3.029088031875631
246246,246247,246246,492493,277.490745306015,2.9706368317948773
248248,248249,248248,496497,279.67144441604614,2.913393168406401
250250,250251,250250,500501,281.7946791648865,2.857330039702674
252252,252253,252252,504505,284.1916801929474,2.802421098813852
254254,254255,254254,508509,286.74918127059937,2.748640636953496
256256,256257,256256,512513,289.03922510147095,2.695963566828027
258258,258259,258258,516517,291.3203992843628,2.6443654064930797
260260,260261,260260,520521,293.5571184158325,2.5938222636509636
262262,262263,262262,524525,295.67409110069275,2.5443108203701286
264264,264265,264264,528529,297.7807421684265,2.495808318222089
266266,266267,266266,532533,299.9380271434784,2.448292543821026
268268,268269,268268,536537,302.1294152736664,2.401741814754587
270270,270271,270270,540541,304.3083493709564,2.356134965899514
272272,272273,272272,544545,306.53968715667725,2.311451336105165
274274,274275,274274,548549,308.7385711669922,2.2676707552419657
276276,276277,276276,552553,310.5774493217468,2.224773531599226
278278,278279,278278,556557,312.49559020996094,2.1827404396258316
280280,280281,280280,560561,314.4184892177582,2.1415527080039283
282282,282283,282282,564565,316.39019322395325,2.101192008044791
284284,284285,284284,568569,318.83321237564087,2.0616404424014263
286286,286287,286286,572573,321.46911215782166,2.022880534084493
288288,288289,288288,576577,324.10483026504517,1.9848952157772146
290290,290291,290290,580581,326.41622018814087,1.9476678194395163
292292,292293,292292,584585,328.7427752017975,1.911182066193419
294294,294295,294294,588589,331.26284742355347,1.8754220564800335
296296,296297,296296,592593,333.7288682460785,1.8403722604844006
298298,298299,298298,596597,336.25238132476807,1.8060175088176038
300300,300301,300300,600601,339.1867341995239,1.772342983450244
302302,302303,302302,604605,341.35476517677307,1.7393342088901136
304304,304305,304304,608609,344.01371121406555,1.7069770435959981
306306,306307,306306,612613,346.2194492816925,1.67525767162374
308308,308309,308308,616617,348.35729217529297,1.6441625944964926
310310,310311,310310,620621,350.61172318458557,1.613678623289843
312312,312313,312312,624625,352.7996280193329,1.5837928709333937
314314,314315,314314,628629,355.0008943080902,1.5544927447135706
316316,316317,316316,632633,357.20956110954285,1.5257659389803848
318318,318319,318318,636637,359.4140112400055,1.4976004280460984
320320,320321,320320,640641,361.53443217277527,1.469984459273178
322322,322323,322322,644645,363.851202249527,1.442906546347558
324324,324325,324324,648649,366.0624713897705,1.4163554627282338
326326,326327,326326,652653,368.3244574069977,1.39032023527227
328328,328329,328328,656657,370.55968618392944,1.3647901380272742
330330,330331,330330,660661,372.73890924453735,1.3397546861889396
332332,332333,332332,664665,374.89173221588135,1.3152036302162742
334334,334335,334334,668669,377.0877151489258,1.2911269501040579
336336,336337,336336,672673,379.3066921234131,1.2675148498030921
338338,338339,338338,676677,381.56870126724243,1.2443577517899485
340340,340341,340340,680681,383.8343753814697,1.2216462917768922
342342,342343,342342,684685,386.08393812179565,1.1993713135598227
344344,344345,344344,688689,388.22800731658936,1.1775238640028647
346346,346347,346346,692693,390.37486124038696,1.1560951881518804
348348,348349,348348,696697,392.5259392261505,1.1350767244754252
350350,350351,350350,700701,394.6692941188812,1.1144601002298486
352352,352353,352352,704705,396.9231712818146,1.0942371269436535
354354,354355,354354,708709,399.16297912597656,1.0743997960207707
356356,356357,356356,712713,401.39498019218445,1.0549402744535428
358358,358359,358358,716717,403.532594203949,1.035850900650189
360360,360361,360360,720721,405.68697023391724,1.0171241803682278
362362,362363,362362,724725,407.84594202041626,0.9987527827502163
364364,364365,364364,728729,409.9949543476105,0.9807295364646507
366366,366367,366366,732733,412.20164728164673,0.9630474259445236
368368,368369,368368,736737,414.411758184433,0.9456995877191048
370370,370371,370370,740741,416.6313850879669,0.9286793068434918
372372,372373,372372,744745,418.7895312309265,0.9119800134162688
374374,374375,374374,748749,420.93669724464417,0.8955952791862956
376376,376377,376376,752753,423.14165139198303,0.8795188142456709
378378,378379,378378,756757,425.2813892364502,0.8637444638062561
380380,380381,380380,760761,427.50364112854004,0.8482662050566887
382382,382383,382382,764765,429.9995450973511,0.8330781441009094
384384,384385,384384,768769,432.4473121166229,0.8181745129711544
386386,386387,386386,772773,434.88395643234253,0.8035496667167763
388388,388389,388388,776777,437.0434682369232,0.7891980805663934
390390,390391,390390,780781,439.2408893108368,0.7751143471609794
392392,392393,392392,784785,441.40874433517456,0.7612931738555062
394394,394395,394394,788789,443.7613422870636,0.7477293800875486
396396,396397,396396,792793,446.09405732154846,0.7344178948120543
398398,398399,398398,796797,448.4175581932068,0.7213537539995514
400400,400401,400400,800801,451.1283950805664,0.7085320981955192
402402,402403,402402,804805,453.3295621871948,0.6959481701414916
404404,404405,404404,808809,455.61966824531555,0.6835973124530028
406406,406407,406406,812813,458.6070191860199,0.6714749653556282
408408,408409,408408,816817,460.9824540615082,0.6595766644778678
410410,410411,410410,820821,463.8608922958374,0.6478980386950752
412412,412413,412412,824825,466.99742913246155,0.6364348080288664
414414,414415,414414,828829,469.372278213501,0.6251827815967772
416416,416417,416416,832833,472.1209032535553,0.6141378556114887
418418,418419,418418,836837,474.63309121131897,0.6032960114295065
420420,420421,420420,840841,477.5071883201599,0.592653313646224
422422,422423,422422,844845,480.06218338012695,0.5822059082381656
424424,424425,424424,848849,482.59731221199036,0.5719500207495685
426426,426427,426426,852853,484.87687611579895,0.561881954522164
428428,428429,428428,856857,487.1634781360626,0.5519980889691851
430430,430431,430430,860861,489.80267214775085,0.5422948778884802
432432,432433,432432,864865,492.63965010643005,0.5327688478187156
434434,434435,434434,868869,495.16024827957153,0.5234165964325257
436436,436437,436436,872873,497.38088512420654,0.514234790970022
438438,438439,438438,876877,499.71570205688477,0.5052201667078862
440440,440441,440440,880881,502.07758021354675,0.4963695254656386
442442,442443,442442,884885,504.41562700271606,0.4876797341486281
444444,444445,444444,888889,506.8121783733368,0.4791477233228534
446446,446447,446446,892893,509.7759323120117,0.4707704858262787
448448,448449,448448,896897,512.1807641983032,0.46254507541061685
450450,450451,450450,900901,514.4484901428223,0.4544686054163094
452452,452453,452452,904905,516.6929180622101,0.44653824747888393
454454,454455,454454,908909,520.1527051925659,0.43875123026509755
456456,456457,456456,912913,522.7159082889557,0.4311048382385252
458458,458459,458458,916917,526.3622181415558,0.4235964104550476
460460,460461,460460,920921,528.605954170227,0.41622333938380507
462462,462463,462462,924925,530.8338313102722,0.40898306975930154
464464,464465,464464,928929,533.2190222740173,0.4018730974578375
466466,466467,466466,932933,535.3428022861481,0.3948909684006594
468468,468469,468468,936937,537.5182473659515,0.3880342774820065
470470,470471,470470,940941,539.7465121746063,0.3813006675221686
472472,472473,472472,944945,542.7762553691864,0.3746878282454418
474474,474475,474474,948949,545.779871225357,0.3681934952804795
476476,476477,476476,952953,548.3522622585297,0.3618154491836094
478478,478479,478478,956957,550.8147630691528,0.35555151448670586
480480,480481,480480,960961,553.2092442512512,0.34939955876257045
482482,482483,482482,964965,555.5505821704865,0.34335749171657426
484484,484485,484484,968969,557.8801143169403,0.3374232642958077
486486,486487,486486,972973,560.1277832984924,0.33159486781914893
488488,488489,488488,976977,562.3495674133301,0.3258703331274546
490490,490491,490490,980981,564.6058423519135,0.32024772975341875
492492,492493,492492,984985,566.7961840629578,0.3147251651088254
494494,494495,494494,988989,569.0588612556458,0.30930078369181047
496496,496497,496496,992993,571.4414401054382,0.30397276631060777
498498,498499,498498,996997,573.6954801082611,0.2987393293255991
500501,500502,500501,1001003,576.0817263126373,0.29359617908278324
502503,502504,502503,1005007,578.6133742332458,0.2885467355815763
504505,504506,504505,1009011,580.9033694267273,0.28358672671083696
506507,506508,506507,1013015,583.148674249649,0.27871450380882834
508509,508510,508509,1017019,585.3261330127716,0.2739284502213195
510511,510512,510511,1021023,587.5307881832123,0.26922698064151973
512513,512514,512513,1025027,589.7034661769867,0.2646085404610403
514515,514516,514515,1029031,591.9396753311157,0.26007160513745475
516517,516518,516517,1033035,594.2188580036163,0.25561467957606965
518519,518520,518519,1037039,596.4036910533905,0.2512362975239739
520521,520522,520521,1041043,598.6829633712769,0.24693502097875353
522523,522524,522523,1045047,601.0072402954102,0.242709439608916
524525,524526,524525,1049051,603.2054162025452,0.23855817018852576
526527,526528,526527,1053055,605.3442471027374,0.23447985604343557
528529,528530,528529,1057059,607.664694070816,0.23047316650911398
530531,530532,530531,1061063,610.113908290863,0.22653679640177415
532533,532534,532533,1065067,612.3015501499176,0.22266946549984823
534535,534536,534535,1069071,614.5506553649902,0.21886991803648925
536537,536538,536537,1073075,616.7895321846008,0.2151369222053745
538539,538540,538539,1077079,618.9889574050903,0.2114692696743532
540541,540542,540541,1081083,621.1697402000427,0.20786577511080395
542543,542544,542543,1085087,623.3381969928741,0.20432527571858827
544545,544546,544545,1089091,625.5037953853607,0.2008466307826211
546547,546548,546547,1093095,627.6978192329407,0.1974287212251511
548549,548550,548549,1097099,631.7730123996735,0.1940704491702263
550551,550552,550551,1101103,635.4469921588898,0.19077073751941498
552553,552554,552553,1105107,638.7513401508331,0.18752852953400634
554555,554556,554555,1109111,641.6557660102844,0.18434278842835283
556557,556558,556557,1113115,644.653813123703,0.18121249697105668
558559,558560,558559,1117119,647.6599612236023,0.17813665709468296
560561,560562,560561,1121123,650.0309331417084,0.17511428951388552
562563,562564,562563,1125127,652.9414081573486,0.17214443335160468
564565,564566,564565,1129131,655.4789571762085,0.16922614577322292
566567,566568,566567,1133135,658.0934841632843,0.16635850162856514
568569,568570,568569,1137139,660.7127523422241,0.16354059310185676
570571,570572,570571,1141143,663.1169700622559,0.16077152936702532
572573,572574,572573,1145147,665.3642492294312,0.1580504362540296
574575,574576,574575,1149151,667.7867403030396,0.15537645591984983
576577,576578,576577,1153155,670.0775122642517,0.1527487465239119
578579,578580,578579,1157159,672.4831931591034,0.15016648191715376
580581,580582,580581,1161163,675.0320391654968,0.14762885133040982
582583,582584,582583,1165167,677.345516204834,0.14513505907359558
584585,584586,584585,1169171,680.6651730537415,0.14268432424034927
586587,586588,586587,1173175,683.5891242027283,0.14027588041824401
588589,588590,588589,1177179,687.1192502975464,0.13790897540491187
590591,590592,590591,1181183,689.9932742118835,0.13558287093098897
592593,592594,592593,1185187,692.5203251838684,0.133296842388404
594595,594596,594595,1189191,695.0658891201019,0.13105017856389622
596597,596598,596597,1193195,697.3772521018982,0.1288421813783316
598599,598600,598599,1197199,699.7898092269897,0.12667216563181682
600601,600602,600601,1201203,702.058158159256,0.12453945875347472
602603,602604,602603,1205207,704.1847453117371,0.12244340055735847
604605,604606,604605,1209211,706.4317293167114,0.12038334300086717
606607,606608,606607,1213215,708.5378880500793,0.11835864995236989
608609,608610,608609,1217219,710.6442742347717,0.11636869695905716
610611,610612,610611,1221223,712.6991612911224,0.1144128710232053
612613,612614,612613,1225227,714.8778781890869,0.11249057038048704
614615,614616,614615,1229231,717.8242073059082,0.11060120428396658
616617,616618,616617,1233235,720.0798079967499,0.10874419279309677
618619,618620,618619,1237239,722.4911532402039,0.10691896656533117
620621,620622,620621,1241243,725.1507792472839,0.10512496665330673
622623,622624,622623,1245247,727.6183743476868,0.10336164430600547
624625,624626,624625,1249251,729.9712052345276,0.10162846077366794
626627,626628,626627,1253255,732.2853412628174,0.0999248871155487
628629,628630,628629,1257259,734.4443602561951,0.09825040401517526
630631,630632,630631,1261263,736.6192932128906,0.09660450159412903
632633,632634,632633,1265267,738.7559270858765,0.0949866792341254
634635,634636,634635,1269271,740.8064341545105,0.09339644540068548
636637,636638,636637,1273275,742.8956632614136,0.09183331746964996
638639,638640,638639,1277279,744.9786150455475,0.09029682155903629
640641,640642,640641,1281283,747.8188033103943,0.08878649236351066
642643,642644,642643,1285287,750.380588054657,0.08730187299045156
644645,644646,644645,1289291,753.1330771446228,0.0858425148024935
646647,646648,646647,1293295,755.6508421897888,0.08440797726143501
648649,648650,648649,1297299,758.0724983215332,0.08299782777407927
650651,650652,650651,1301303,760.278626203537,0.08161164154398648
652653,652654,652653,1305307,762.526703119278,0.08024900142345359
654655,654656,654655,1309311,764.6561300754547,0.07890949777060996
656657,656658,656657,1313315,766.9492542743683,0.07759272830821828
658659,658660,658659,1317319,769.9158172607422,0.07629829798429455
660661,660662,660661,1321323,772.6503133773804,0.07502581883818493
662663,662664,662663,1325327,774.7968833446503,0.07377490986709745
664665,664666,664665,1329331,777.1520662307739,0.07254519689581684
666667,666668,666667,1333335,779.5232162475586,0.0713363124488069
668669,668670,668669,1337339,781.8077912330627,0.07014789562629176
670671,670672,670671,1341343,784.1723403930664,0.06897959197976888
672673,672674,672673,1345347,786.3725283145905,0.06783105339354734
674675,674676,674675,1349351,788.6038901805878,0.06670193796583135
676677,676678,676677,1353355,790.7531950473785,0.06559190989378294
678679,678680,678679,1357359,792.8319232463837,0.06450063935915296
680681,680682,680681,1361363,795.4258103370667,0.06342780241891433
682683,682684,682683,1365367,798.0314831733704,0.06237308089464477
684685,684686,684685,1369371,800.3602240085602,0.061336162266456995
686687,686688,686687,1373375,802.4398562908173,0.060316739568747835
688689,688690,688689,1377379,804.5168471336365,0.05931451128685694
690691,690692,690691,1381383,807.1927270889282,0.05832918125656761
692693,692694,692693,1385387,810.2920732498169,0.05736045856531291
694695,694696,694695,1389391,812.4362523555756,0.056408057455882954
696697,696698,696697,1393395,814.6637661457062,0.055471697230359496
698699,698700,698699,1397399,817.2813854217529,0.05455110215825698
700701,700702,700701,1401403,819.3962984085083,0.05364600138489095
702703,702704,702703,1405407,822.0847780704498,0.05275612884133807
704705,704706,704705,1409411,824.8512473106384,0.051881223156669876
706707,706708,706707,1413415,827.3357102870941,0.0510210275724603
708709,708710,708709,1417419,830.1340301036835,0.05017528985797526
710711,710712,710711,1421423,832.5101964473724,0.0493437622270676
712713,712714,712713,1425427,835.077977180481,0.04852620125723206
714715,714716,714715,1429431,837.7951462268829,0.04772236781025185
716717,716718,716717,1433435,840.676726102829,0.04693202695261789
718719,718720,718719,1437439,843.6999621391296,0.0461549478809502
720721,720722,720721,1441443,846.312328338623,0.04539090384514566
722723,722724,722723,1445447,848.7464911937714,0.044639672074822556
724725,724726,724725,1449451,851.1684243679047,0.04390103370781162
726727,726728,726727,1453455,853.6141083240509,0.043174773718305914
728729,728730,728729,1457459,856.7274880409241,0.04246068084739818
730731,730732,730731,1461463,858.9982330799103,0.0417585475352098
732733,732734,732733,1465467,861.2908091545105,0.04106816985313344
734735,734736,734735,1469471,863.7580642700195,0.04038934743869049
736737,736738,736737,1473475,866.2815833091736,0.039721883430729577
738739,738740,738739,1477479,868.5672721862793,0.039065584405989284
740741,740742,740741,1481483,871.1519622802734,0.0384202603175936
742743,742744,742743,1485487,873.3691310882568,0.03778572443320627
744745,744746,744745,1489491,875.7861602306366,0.037161793276141
746747,746748,746747,1493495,878.1556541919708,0.03654828656613063
748749,748750,748749,1497499,880.4102311134338,0.03594502716225634
750751,750752,750751,1501503,882.6596722602844,0.03535184100587685
752753,752754,752753,1505507,884.8993191719055,0.03476855706549031
754755,754756,754755,1509511,887.1186890602112,0.034195007283187806
756757,756758,756757,1513515,889.3675122261047,0.03363102651928784
758759,758760,758759,1517519,891.6070022583008,0.03307645250220048
760761,760762,760761,1521523,894.2188742160797,0.03253112577601769
762763,762764,762763,1525527,896.5224120616913,0.03199488964912689
764765,764766,764765,1529531,898.870599269867,0.03146759014748568
766767,766768,766767,1533535,901.828889131546,0.030949075962553252
768769,768770,768769,1537539,904.2061061859131,0.030439198407066215
770771,770772,770771,1541543,906.7617621421814,0.029937811365471134
772773,772774,772773,1545547,909.2577061653137,0.02944477124981404
774775,774776,774775,1549551,911.8690280914307,0.028959936953469878
776777,776778,776777,1553555,914.3366751670837,0.028483169808509956
778779,778780,778779,1557559,916.7592771053314,0.028014333540454572
780781,780782,780781,1561563,918.9011824131012,0.027553294227118386
782783,782784,782783,1565567,921.0057482719421,0.027099920256205223
784785,784786,784785,1569571,923.1587612628937,0.026654082284267133
786787,786788,786787,1573575,925.3511083126068,0.026215653197027677
788789,788790,788789,1577579,927.4370181560516,0.025784508068227296
790791,790792,790791,1581583,929.5456891059875,0.02536052412290246
792793,792794,792793,1585587,931.6995022296906,0.024943580698504775
794795,794796,794795,1589591,933.8020441532135,0.024533559206929567
796797,796798,796797,1593595,936.287611246109,0.024130343098022422
798799,798800,798799,1597599,938.7676253318787,0.023733817824677317
800801,800802,800801,1601603,941.7240424156189,0.023343870805661027
802803,802804,802803,1605607,944.3097610473633,0.02296039139275763
804805,804806,804805,1609611,946.9785442352295,0.022583270834957148
806807,806808,806807,1613615,949.6639621257782,0.02221240224628218
808809,808810,808809,1617619,952.3301951885223,0.02184768057270503
810811,810812,810811,1621623,954.9525442123413,0.021489002558837456
812813,812814,812813,1625627,957.5048551559448,0.021136266718031038
814815,814816,814815,1629631,959.7971813678741,0.020789373300203806
816817,816818,816817,1633635,962.9384210109711,0.0204482242610311
818819,818820,818819,1637639,965.2153122425079,0.020112723232841745
820821,820822,820821,1641643,967.9581742286682,0.019782775495286842
822823,822824,822823,1645647,970.2733671665192,0.019458287945099073
824825,824826,824825,1649651,972.6289422512054,0.01913916906880786
826827,826828,826827,1653655,975.061083316803,0.01882532891579558
828829,828830,828829,1657659,977.8074612617493,0.018516679068625308
830831,830832,830831,1661663,980.2935152053833,0.018213132618257077
832833,832834,832833,1665667,982.9183690547943,0.017914604136763046
834835,834836,834835,1669671,985.5453882217407,0.017621009651293207
836837,836838,836837,1673675,988.2239072322845,0.017332266619405345
838839,838840,838839,1677679,990.7405412197113,0.017048293903712874
840841,840842,840841,1681683,993.2250213623047,0.016769011746760043
842843,842844,842843,1685687,995.7901401519775,0.016494341748511943
844845,844846,844845,1689691,998.4864392280579,0.01622420684077497
846847,846848,846847,1693695,1000.9518871307373,0.015958531265710008
848849,848850,848849,1697699,1003.5630593299866,0.015697240551958203
850851,850852,850851,1701703,1006.6260132789612,0.01544026149315414
852853,852854,852853,1705707,1009.5331110954285,0.015187522124620045
854855,854856,854855,1709711,1012.6389412879944,0.014938951703470593
856857,856858,856857,1713715,1015.0803942680359,0.01469448068598922
858859,858860,858859,1717719,1017.1668684482574,0.014454040707278182
860861,860862,860861,1721723,1019.8613471984863,0.01421756456136336
862863,862864,862863,1725727,1021.8713982105255,0.01398498618073063
864865,864866,864865,1729731,1023.9511752128601,0.013756240615862225
866867,866868,866867,1733735,1026.0243122577667,0.013531264016819478
868869,868870,868869,1737739,1028.0646772384644,0.01330999361493923
870871,870872,870871,1741743,1030.25617313385,0.01309236770168809
872873,872874,872873,1745747,1032.66561627388,0.012878325612518893
874875,874876,874875,1749751,1035.0195252895355,0.012667807708339751
876877,876878,876877,1753755,1037.4585993289948,0.012460755357096787
878879,878880,878879,1757759,1040.189501285553,0.012257110917289538
880881,880882,880881,1761763,1042.7785501480103,0.0120568177203495
882883,882884,882883,1765767,1044.8989412784576,0.011859820053700787
884885,884886,884885,1769771,1047.0762922763824,0.011666063145298722
886887,886888,886887,1773775,1049.2554762363434,0.011475493146122062
888889,888890,888889,1777779,1051.5690841674805,0.011288057115052652
890891,890892,890891,1781783,1053.7508301734924,0.011103703003186638
892893,892894,892893,1785787,1056.0808942317963,0.01092237963871412
894895,894896,894895,1789791,1058.242612361908,0.010744036710889304
896897,896898,896897,1793795,1060.388503074646,0.01056862475638809
898899,898900,898899,1797799,1062.8307571411133,0.010396095143732964
900901,900902,900901,1801803,1065.183517217636,0.010226400060332708
902903,902904,902903,1805807,1067.4650371074677,0.010059492496907296
904905,904906,904905,1809811,1069.9576740264893,0.009895326234868662
906907,906908,906907,1813815,1072.115023136139,0.009733855832109839
908909,908910,908909,1817819,1074.2861912250519,0.009575036610385723
910911,910912,910911,1821823,1076.6954312324524,0.009418824640874845
912913,912914,912913,1825827,1078.9345662593842,0.009265176733379121
914915,914916,914915,1829831,1081.1637501716614,0.009114050422226683
916917,916918,916917,1833835,1083.4214141368866,0.008965403953538953
918919,918920,918919,1837839,1085.6101722717285,0.00881919627465777
920921,920922,920921,1841843,1087.8518080711365,0.008675387021071401
922923,922924,922923,1845847,1090.1127161979675,0.008533936504363737
924925,924926,924925,1849851,1092.2748003005981,0.008394805702209851
926927,926928,926927,1853855,1094.5097181797028,0.008257956244733577
928929,928930,928929,1857859,1096.676872253418,0.008123350405753627
930931,930932,930931,1861863,1098.8551461696625,0.007990951089709597
932933,932934,932933,1865867,1101.078092098236,0.007860721822680716
934935,934936,934935,1869871,1103.264434337616,0.007732626740789783
936937,936938,936937,1873875,1105.493455171585,0.007606630579971352
938939,938940,938939,1877879,1107.699901342392,0.007482698665626231
940941,940942,940941,1881883,1109.880618095398,0.0073607969032991605
942943,942944,942943,1885887,1112.0994591712952,0.007240891768105939
944945,944946,944945,1889891,1114.311867237091,0.007122950295070041
946947,946948,946947,1893895,1116.487262248993,0.007006940069800294
948949,948950,948949,1897899,1118.7396092414856,0.006892829219850682
950951,950952,950951,1901903,1120.981308221817,0.006780586403920097
952953,952954,952953,1905907,1123.355089187622,0.0066701808045763755
954955,954956,954955,1909911,1125.859590291977,0.006561582117683429
956957,956958,956957,1913915,1128.3449063301086,0.006454760545238969
958959,958960,958959,1917919,1130.6240193843842,0.006349686785711128
960961,960962,960961,1921923,1132.9203741550446,0.006246332026194068
962963,962964,962963,1925927,1135.2311441898346,0.006144667934108838
964965,964966,964965,1929931,1137.448587179184,0.006044666648790553
966967,966968,966967,1933935,1139.7379393577576,0.005946300773643998
968969,968970,968969,1937939,1142.1387922763824,0.005849543368071863
970971,970972,970971,1941943,1144.4334683418274,0.005754367940539851
972973,972974,972973,1945947,1146.7833292484283,0.005660748440163843
974975,974976,974975,1949951,1149.1001162528992,0.005568659248979202
976977,976978,976977,1953955,1151.2019410133362,0.005478075176256425
978979,978980,978979,1957959,1153.36696600914,0.005388971449406199
980981,980982,980981,1961963,1155.5345242023468,0.005301323707953998
982983,982984,982983,1965967,1157.7218461036682,0.005215107996605184
984985,984986,984985,1969971,1159.986251115799,0.005130300757855366
986987,986988,986987,1973975,1162.3003220558167,0.005046878825737622
988989,988990,988989,1977979,1164.5331263542175,0.004964819419001287
990991,990992,990991,1981983,1166.5959582328796,0.0048841001349728685
992993,992994,992993,1985987,1168.673971414566,0.004804698942507457
994995,994996,994995,1989991,1170.8736691474915,0.004726594176531762
996997,996998,996997,1993995,1173.3665699958801,0.0046497645313365865
998999,999000,998999,1997999,1175.6867713928223,0.004574189054778799
1001001,1001002,1001001,2002003,1177.774393081665,0.004499847142142244
1003003,1003004,1003003,2006007,1179.850726366043,0.004426718530226026
1005005,1005006,1005005,2010011,1181.9119024276733,0.004354783292228603
1007007,1007008,1007007,2014015,1183.971194267273,0.004284021831495011
1009009,1009010,1009009,2018019,1186.1942842006683,0.004214414875946204
1011011,1011012,1011011,2022023,1188.2506031990051,0.00414594347273578
1013013,1013014,1013013,2026027,1190.2954270839691,0.004078588983475129
1015015,1015016,1015015,2030031,1192.3620202541351,0.0040123330779806565
1017017,1017018,1017017,2034035,1194.4503452777863,0.003947157729840001
1019019,1019020,1019019,2038039,1196.5653183460236,0.003883045210614
1021021,1021022,1021021,2042043,1198.6140401363373,0.003819978085743969
1023023,1023024,1023023,2046047,1200.6841552257538,0.0037579392089810426
1025025,1025026,1025025,2050051,1202.7662951946259,0.0036969117178387023
1027027,1027028,1027027,2054055,1204.8290991783142,0.003636879028590556
1029029,1029030,1029029,2058059,1207.2673852443695,0.003577824831381804
1031031,1031032,1031031,2062063,1209.8429923057556,0.0035197330871596932
1033033,1033034,1033033,2066067,1212.3476321697235,0.003462588020624935
1035035,1035036,1035035,2070071,1214.930447101593,0.0034063741180716534
1037037,1037038,1037037,2074075,1217.236325263977,0.0033510761218167318
1039039,1039040,1039039,2078079,1219.4045813083649,0.0032966790261070855
1041041,1041042,1041041,2082083,1222.002221107483,0.003243168073140623
1043043,1043044,1043043,2086087,1224.4227221012115,0.003190528749200894
1045045,1045046,1045045,2090091,1226.647140264511,0.0031387467795411794
1047047,1047048,1047047,2094095,1229.685678243637,0.003087808125428637
1049049,1049050,1049049,2098099,1231.8885962963104,0.0030376989797105125
1051051,1051052,1051051,2102103,1233.9673600196838,0.002988405763062474
1053053,1053054,1053053,2106107,1236.0173292160034,0.002939915120009573
1055055,1055056,1055055,2110111,1238.3990151882172,0.002892213915743014
1057057,1057058,1057057,2114115,1240.9705312252045,0.0028452892318000522
1059059,1059060,1059059,2118119,1243.783529996872,0.002799128362880765
1061061,1061062,1061061,2122123,1246.8645193576813,0.0027537188126416368
1063063,1063064,1063063,2126127,1249.0577883720398,0.002709048291194449
1065065,1065066,1065065,2130131,1251.2715373039246,0.0026651047113546156
1067067,1067068,1067067,2134135,1253.43514919281,0.0026218761843210814
1069069,1069070,1069069,2138139,1255.6487910747528,0.002579351017971021
1071071,1071072,1071071,2142143,1257.7626621723175,0.002537517712198678
1073073,1073074,1073073,2146147,1260.868046283722,0.0024963649563005674
1075075,1075076,1075075,2150151,1263.2794790267944,0.002455881626133305
1077077,1077078,1077077,2154155,1265.409235239029,0.0024160567803619415
1079079,1079080,1079079,2158159,1267.5299272537231,0.0023768796578451656
1081081,1081082,1081081,2162163,1269.6797981262207,0.0023383396744520724
1083083,1083084,1083083,2166167,1271.8288624286652,0.0023004264204473657
1085085,1085086,1085085,2170171,1273.90585231781,0.0022631296569670667
1087087,1087088,1087087,2174175,1276.1896872520447,0.0022264393138584637
1089089,1089090,1089089,2178179,1278.3698601722717,0.0021903454861558203
1091091,1091092,1091091,2182183,1280.4737792015076,0.0021548384321476988
1093093,1093094,1093093,2186187,1282.6487562656403,0.002119908570421103
1095095,1095096,1095095,2190191,1284.8034722805023,0.0020855464765645593
1097097,1097098,1097097,2194195,1286.8998172283173,0.0020517428810080673
1099099,1099100,1099099,2198199,1289.0790011882782,0.0020184886672041102
1101101,1101102,1101101,2202203,1291.2192842960358,0.0019857748676486153
1103103,1103104,1103103,2206207,1293.330527305603,0.001953592662630399
1105105,1105106,1105105,2210211,1295.3929982185364,0.0019219333767068747
1107107,1107108,1107107,2214215,1297.5064051151276,0.0018907884775671846
1109109,1109110,1109109,2218219,1299.6047611236572,0.0018601495726215944
1111111,1111112,1111111,2222223,1301.7095732688904,0.0018300084070688172
1113113,1113114,1113113,2226227,1303.8632152080536,0.0018003568616222765
1115115,1115116,1115115,2230231,1305.973120212555,0.0017711869504637434
1117117,1117118,1117117,2234235,1308.7422363758087,0.0017424908182874788
1119119,1119120,1119119,2238239,1311.4054503440857,0.0017142607393907383
1121121,1121122,1121121,2242243,1314.1377391815186,0.0016864891141494809
1123123,1123124,1123123,2246247,1316.4774022102356,0.0016591684677678131
1125125,1125126,1125125,2250251,1319.4115703105927,0.001632291448459
1127127,1127128,1127127,2254255,1322.2251591682434,0.001605850824148547
1129129,1129130,1129129,2258259,1324.7641642093658,0.0015798394820194517
1131131,1131132,1131131,2262263,1327.4848561286926,0.0015542504260110945
1133133,1133134,1133133,2266267,1329.8284912109375,0.0015290767739770672
1135135,1135136,1135135,2270271,1331.92906332016,0.0015043117572304254
1137137,1137138,1137137,2274275,1334.0707740783691,0.0014799487171330838
1139139,1139140,1139139,2278279,1336.6770460605621,0.0014559811053231897
1141141,1141142,1141141,2282283,1339.3219583034515,0.0014324024797360835
1143143,1143144,1143143,2286287,1341.83047914505,0.0014092065043769253
1145145,1145146,1145145,2290291,1344.5716841220856,0.0013863869468195844
1147147,1147148,1147147,2294295,1347.0847663879395,0.0013639376765013367
1149149,1149150,1149149,2298299,1349.610433101654,0.0013418526635859962
1151151,1151152,1151151,2302303,1352.2749981880188,0.0013201259766901785
1153153,1153154,1153153,2306307,1355.02982711792,0.0012987517817464322
1155155,1155156,1155155,2310311,1357.370970249176,0.001277724339956876
1157157,1157158,1157157,2314315,1359.6908390522003,0.0012570380064289566
1159159,1159160,1159159,2318319,1362.0371870994568,0.0012366872286975195
1161161,1161162,1161161,2322323,1364.3398714065552,0.0012166665453605674
1163163,1163164,1163163,2326327,1366.8538250923157,0.001196970584032897
1165165,1165166,1165165,2330331,1369.5436911582947,0.0011775940604366042
1167167,1167168,1167167,2334335,1371.803655385971,0.001158531776241034
1169169,1169170,1169169,2338339,1374.1668872833252,0.0011397786189490944
1171171,1171172,1171171,2342343,1376.513501405716,0.00112132955848665
1173173,1173174,1173173,2346347,1378.9101071357727,0.0011031796485667655
1175175,1175176,1175175,2350351,1381.3461632728577,0.0010853240223696048
1177177,1177178,1177177,2354355,1383.7353904247284,0.0010677578929971787
1179179,1179180,1179179,2358359,1385.944708108902,0.0010504765523364767
1181181,1181182,1181181,2362363,1388.1594061851501,0.0010334753685583564
1183183,1183184,1183183,2366367,1390.7836751937866,0.001016749785662796
1185185,1185186,1185185,2370371,1392.8468582630157,0.0010002953225694
1187187,1187188,1187187,2374375,1395.0906312465668,0.0009841075706162883
1189189,1189190,1189189,2378379,1397.5147902965546,0.0009681821935600965
1191191,1191192,1191191,2382383,1399.7620811462402,0.000952514926098047
1193193,1193194,1193193,2386387,1401.903643131256,0.0009371015722763332
1195195,1195196,1195195,2390391,1404.7322239875793,0.0009219380049216852
1197197,1197198,1197197,2394395,1406.752248287201,0.0009070201640497544
1199199,1199200,1199199,2398399,1408.8260543346405,0.0008923440558419315
1201201,1201202,1201201,2402403,1410.9907641410828,0.0008779057521905997
1203203,1203204,1203203,2406407,1413.0556771755219,0.0008637013886527711
1205205,1205206,1205205,2410411,1415.1061372756958,0.0008497271636542791
1207207,1207208,1207207,2414415,1417.2387850284576,0.0008359793382624048
1209209,1209210,1209209,2418419,1419.52041721344,0.0008224542341395136
1211211,1211212,1211211,2422423,1421.6978843212128,0.0008091482330883082
1213213,1213214,1213213,2426427,1424.0260710716248,0.0007960577758012732
1215215,1215216,1215215,2430431,1426.1781241893768,0.0007831793614059279
1217217,1217218,1217217,2434435,1428.5249571800232,0.0007705095453047761
1219219,1219220,1219219,2438439,1431.0999352931976,0.0007580449401984879
1221221,1221222,1221221,2442443,1433.3085162639618,0.0007457822131300418
1223223,1223224,1223223,2446447,1436.1381351947784,0.0007337180857120984
1225225,1225226,1225225,2450451,1438.5207459926605,0.0007218493333311926
1227227,1227228,1227227,2454455,1440.6575272083282,0.0007101727833287441
1229229,1229230,1229229,2458459,1443.5975041389465,0.0006986853155694916
1231231,1231232,1231231,2462463,1445.9995551109314,0.0006873838600540694
1233233,1233234,1233233,2466467,1448.0356884002686,0.0006762653969190069
1235235,1235236,1235235,2470471,1450.1062741279602,0.0006653269560956687
1237237,1237238,1237237,2474475,1452.1511392593384,0.0006545656151502044
1239239,1239240,1239239,2478479,1454.1978542804718,0.0006439784997382958
1241241,1241242,1241241,2482483,1456.228104352951,0.000633562782354602
1243243,1243244,1243243,2486487,1458.300802230835,0.0006233156808548301
1245245,1245246,1245245,2490491,1460.3504803180695,0.0006132344594789174
1247247,1247248,1247247,2494495,1462.5428822040558,0.0006033164263499202
1249249,1249250,1249249,2498499,1464.6127643585205,0.0005935589334740143
1251251,1251252,1251251,2502503,1466.670684337616,0.0005839593761720607
1253253,1253254,1253253,2506507,1470.0493791103363,0.0005745151921701108
1255255,1255256,1255255,2510511,1472.3459503650665,0.0005652238604625381
1257257,1257258,1257257,2514515,1474.5605483055115,0.0005560829017667857
1259259,1259260,1259259,2518519,1476.823545217514,0.0005470898767043764
1261261,1261262,1261261,2522523,1479.0509622097015,0.0005382423858009133
1263263,1263264,1263263,2526527,1481.3452532291412,0.0005295380683492112
1265265,1265266,1265265,2530531,1483.5569252967834,0.0005209746025229833
1267267,1267268,1267267,2534535,1485.6987102031708,0.0005125497036715387
1269269,1269270,1269269,2538539,1487.8953912258148,0.0005042611252292772
1271271,1271272,1271271,2542543,1490.3106801509857,0.0004961066563282657
1273273,1273274,1273273,2546547,1492.5212581157684,0.00048808412225298525
1275275,1275276,1275275,2550551,1494.7605073451996,0.0004801913837582106
1277277,1277278,1277277,2554555,1497.0795540809631,0.0004724263367279491
1279279,1279280,1279279,2558559,1499.1460900306702,0.0004647869105838254
1281281,1281282,1281281,2562563,1501.0579822063446,0.0004572710688535153
1283283,1283284,1283283,2566567,1502.9112162590027,0.00044987680837493826
1285285,1285286,1285285,2570571,1504.7442910671234,0.00044260215815938864
1287287,1287288,1287287,2574575,1506.629809141159,0.00043544517939153593
1289289,1289290,1289289,2578579,1508.79945230484,0.0004284039647473037
1291291,1291292,1291291,2582583,1510.7311780452728,0.000421476638052809
1293293,1293294,1293293,2586587,1512.8236072063446,0.0004146613534885546
1295295,1295296,1295295,2590591,1515.0292873382568,0.0004079562952483684
1297297,1297298,1297297,2594595,1517.4373021125793,0.00040135967742571665
1299299,1299300,1299299,2598599,1519.9045441150665,0.00039486974242208817
1301301,1301302,1301301,2602603,1522.3494262695312,0.0003884847616291154
1303303,1303304,1303303,2606607,1524.687905073166,0.00038220303440539283
1305305,1305306,1305305,2610611,1527.1193704605103,0.0003760228880764771
1307307,1307308,1307307,2614615,1529.6985154151917,0.0003699426767980185
1309309,1309310,1309309,2618619,1532.3572952747345,0.0003639607814420742
1311311,1311312,1311311,2622623,1534.7233390808105,0.0003580756093697346
1313313,1313314,1313313,2626627,1537.0912082195282,0.00035228559374900215
1315315,1315316,1315315,2630631,1539.5750153064728,0.00034658919321373105
1317317,1317318,1317317,2634635,1542.2963662147522,0.0003409848914088798
1319319,1319320,1319319,2638639,1544.9848492145538,0.0003354711966494506
1321321,1321322,1321321,2642643,1547.9361851215363,0.00033004664112468163
1323323,1323324,1323323,2646647,1550.59761428833,0.00032470978158016806
1325325,1325326,1325325,2650651,1553.4033222198486,0.00031945919761255936
1327327,1327328,1327327,2654655,1555.9572632312775,0.00031429349201061996
1329329,1329330,1329329,2658659,1558.6016011238098,0.0003092112904141686
1331331,1331332,1331331,2662663,1560.8804302215576,0.00030421124051827064
1333333,1333334,1333333,2666667,1562.9870212078094,0.00029929201230061153
1335335,1335336,1335335,2670671,1565.1478819847107,0.0002944522968846286
1337337,1337338,1337337,2674675,1567.3077671527863,0.0002896908069942583
1339339,1339340,1339339,2678679,1569.8125212192535,0.00028500627638550213
1341341,1341342,1341341,2682683,1572.4234974384308,0.0002803974587095581
1343343,1343344,1343343,2686687,1575.6725702285767,0.0002758631286496893
1345345,1345346,1345345,2690691,1577.9861900806427,0.00027140208021592116
1347347,1347348,1347347,2694695,1580.406016111374,0.00026701312708610203
1349349,1349350,1349349,2698699,1582.9955923557281,0.0002626951022648427
1351351,1351352,1351351,2702703,1585.515729188919,0.00025844685785614274
1353353,1353354,1353353,2706707,1587.5506403446198,0.00025426726438126934
1355355,1355356,1355355,2710711,1589.4715282917023,0.0002501552103240101
1357357,1357358,1357357,2714715,1591.379295349121,0.0002461096032675414
1359359,1359360,1359359,2718719,1593.2415311336517,0.0002421293673933178
1361361,1361362,1361361,2722723,1595.0947132110596,0.0002382134449590012
1363363,1363364,1363363,2726727,1596.8882853984833,0.00023436079538896593
1365365,1365366,1365365,2730731,1598.7015211582184,0.00023057039425111725
1367367,1367368,1367367,2734735,1600.5233809947968,0.00022684123462113348
1369369,1369370,1369369,2738739,1602.3526620864868,0.00022317232560453704
1371371,1371372,1371371,2742743,1604.2465453147888,0.00021956269222300762
1373373,1373374,1373373,2746747,1606.0925283432007,0.00021601137564175588
1375375,1375376,1375375,2750751,1607.9399712085724,0.00021251743203265505
1377377,1377378,1377377,2754755,1609.70428109169,0.00020907993337004882
1379379,1379380,1379379,2758759,1611.5087523460388,0.00020569796629388293
1381381,1381382,1381381,2762763,1613.3511281013489,0.00020237063267813937
1383383,1383384,1383383,2766767,1615.2471103668213,0.00019909704883502854
1385385,1385386,1385385,2770771,1618.0580060482025,0.00019587634494655504
1387387,1387388,1387387,2774775,1619.8613412380219,0.0001927076658603255
1389389,1389390,1389389,2778779,1621.6037890911102,0.0001895901699526803
1391391,1391392,1391391,2782783,1623.5735292434692,0.0001865230295834408
1393393,1393394,1393393,2786787,1625.4161632061005,0.00018350542984535423
1395395,1395396,1395395,2790791,1627.5291702747345,0.00018053656992833567
1397397,1397398,1397397,2794795,1630.4436402320862,0.00017761566141416552
1399399,1399400,1399399,2798799,1633.034897327423,0.00017474192884492368
1401401,1401402,1401401,2802803,1635.3506972789764,0.00017191460915455536
1403403,1403404,1403403,2806807,1637.4393222332,0.00016913295178255794
1405405,1405406,1405405,2810811,1639.4759571552277,0.00016639621844660724
1407407,1407408,1407407,2814815,1641.528052330017,0.00016370368268781021
1409409,1409410,1409409,2818819,1643.5809993743896,0.00016105462987070496
1411411,1411412,1411411,2822823,1645.6447343826294,0.00015844835684220016
1413413,1413414,1413413,2826827,1647.747724056244,0.00015588417181788827
1415415,1415416,1415415,2830831,1650.1337983608246,0.00015336139449573238
1417417,1417418,1417417,2834835,1652.7635781764984,0.00015087935503288463
1419419,1419420,1419419,2838839,1655.4879863262177,0.00014843739506886777
1421421,1421422,1421421,2842843,1657.635371208191,0.0001460348665887068
1423423,1423424,1423423,2846847,1660.0935411453247,0.00014367113203661575
1425425,1425426,1425425,2850851,1662.505666255951,0.00014134556465705828
1427427,1427428,1427427,2854855,1664.8571512699127,0.00013905754690313188
1429429,1429430,1429429,2858859,1666.9413242340088,0.00013680647214187047
1431431,1431432,1431431,2862863,1668.987386226654,0.00013459174294894183
1433433,1433434,1433433,2866867,1671.021960258484,0.00013241277190445544
1435435,1435436,1435435,2870871,1673.0615322589874,0.00013026898136558884
1437437,1437438,1437437,2874875,1675.0829071998596,0.0001281598022160324
1439439,1439440,1439439,2878879,1677.081208229065,0.0001260846750028577
1441441,1441442,1441441,2882883,1679.0259373188019,0.00012404304982283065
1443443,1443444,1443443,2886887,1680.9149980545044,0.0001220343848444827
1445445,1445446,1445445,2890891,1683.0184733867645,0.00012005814755866595
1447447,1447448,1447447,2894895,1685.5044062137604,0.0001181138138690585
1449449,1449450,1449449,2898899,1687.8065302371979,0.00011620086797847762
1451451,1451452,1451451,2902903,1690.113754272461,0.00011431880307100073
1453453,1453454,1453453,2906907,1692.4521181583405,0.00011246711960666289
1455455,1455456,1455455,2910911,1694.5121850967407,0.00011064532714044617
1457457,1457458,1457457,2914915,1697.0491321086884,0.00010885294193485606
1459459,1459460,1459459,2918919,1699.1728911399841,0.00010708948968840559
1461461,1461462,1461461,2922923,1701.1586964130402,0.00010535450235238386
1463463,1463464,1463463,2926927,1703.230004310608,0.00010364752017721912
1465465,1465466,1465465,2930931,1705.4771211147308,0.00010196809046192357
1467467,1467468,1467467,2934935,1707.6564161777496,0.00010031576823621435
1469469,1469470,1469469,2938939,1710.2295260429382,9.869011569207942e-05
1471471,1471472,1471471,2942943,1712.0737221240997,9.709070161534328e-05
1473473,1473474,1473473,2946947,1714.0463581085205,9.551710195410124e-05
1475475,1475476,1475475,2950951,1716.1741650104523,9.396890015977988e-05
1477477,1477478,1477477,2954955,1718.2360210418701,9.244568582289503e-05
1479479,1479480,1479479,2958959,1720.2599790096283,9.094705490042543e-05
1481481,1481482,1481481,2962963,1722.273742198944,8.947261062530742e-05
1483483,1483484,1483483,2966967,1724.354097366333,8.80219620285061e-05
1485485,1485486,1485485,2970971,1727.161472082138,8.659472484850994e-05
1487487,1487488,1487487,2974975,1729.5509660243988,8.519052107658354e-05
1489489,1489490,1489489,2978979,1731.785696029663,8.380897838833334e-05
1491491,1491492,1491491,2982983,1734.4206492900848,8.244973082582874e-05
1493493,1493494,1493493,2986987,1737.3196663856506,8.111241834285465e-05
1495495,1495496,1495495,2990991,1739.5852732658386,7.979668646385107e-05
1497497,1497498,1497497,2994995,1741.703839302063,7.85021870797209e-05
1499499,1499500,1499499,2998999,1743.6919343471527,7.722857674252737e-05
1501502,1501503,1501502,3003005,1745.634693145752,7.597489752697584e-05
1503504,1503505,1503504,3007009,1748.4528892040253,7.474206904589664e-05
1505506,1505507,1505506,3011013,1750.8261213302612,7.352913394242933e-05
1507508,1507509,1507508,3015017,1753.1792314052582,7.233577071019681e-05
1509510,1509511,1509510,3019021,1755.3055233955383,7.11616631861034e-05
1511512,1511513,1511512,3023025,1757.4166300296783,7.000650055033475e-05
1513514,1513515,1513514,3027029,1759.7181980609894,6.886997709898424e-05
1515516,1515517,1515516,3031033,1762.4113693237305,6.77517915619319e-05
1517518,1517519,1517518,3035037,1764.5850553512573,6.665164778496546e-05
1519520,1519521,1519520,3039041,1766.7494382858276,6.55692548434672e-05
1521522,1521523,1521522,3043045,1768.9783790111542,6.45043254507982e-05
1523524,1523525,1523524,3047049,1771.5284931659698,6.345657811834826e-05
1525526,1525527,1525526,3051053,1774.1410291194916,6.242573510917282e-05
1527528,1527529,1527528,3055057,1777.491051197052,6.141152380223502e-05
1529530,1529531,1529530,3059061,1780.6108992099762,6.0413675214476825e-05
1531532,1531533,1531532,3063065,1783.2649822235107,5.943192559243471e-05
1533534,1533535,1533534,3067069,1785.8170611858368,5.846601482062397e-05
1535536,1535537,1535536,3071073,1788.3684341907501,5.751568710365973e-05
1537538,1537539,1537538,3075077,1790.8419442176819,5.658069107994379e-05
1539540,1539541,1539540,3079081,1793.5088651180267,5.566077868479624e-05
1541542,1541543,1541542,3083085,1796.2326772212982,5.475570708313171e-05
1543544,1543545,1543544,3087089,1798.9553401470184,5.3865236395722604e-05
1545546,1545547,1545546,3091093,1801.5745091438293,5.298913060869381e-05
1547548,1547549,1547548,3095097,1805.4417552947998,5.212715836933057e-05
1549550,1549551,1549550,3099101,1809.172503232956,5.1279091053402226e-05
1551552,1551553,1551552,3103105,1812.9658932685852,5.0444704470464785e-05
1553554,1553555,1553554,3107109,1816.8152551651,4.962377772699256e-05
1555556,1555557,1555556,3111113,1820.4010922908783,4.8816093567438656e-05
1557558,1557559,1557558,3115117,1823.9436581134796,4.8021437805800815e-05
1559560,1559561,1559560,3119121,1827.5003063678741,4.7239600803550275e-05
1561562,1561563,1561562,3123125,1830.5213131904602,4.647037519589503e-05
1563564,1563565,1563564,3127129,1832.3818311691284,4.571355748339556e-05
1565566,1565567,1565566,3131133,1834.352697134018,4.4968947690904315e-05
1567568,1567569,1567568,3135137,1836.5257182121277,4.423634834438417e-05
1569570,1569571,1569570,3139141,1838.8547751903534,4.3515565721463645e-05
1571572,1571573,1571572,3143145,1840.941976070404,4.280640939668956e-05
1573574,1573575,1573574,3147149,1843.2303140163422,4.210869144571916e-05
1575576,1575577,1575576,3151153,1846.2252180576324,4.142222712744115e-05
1577578,1577579,1577578,3155157,1848.6949744224548,4.074683488397568e-05
1579580,1579581,1579580,3159161,1850.9575061798096,4.0082336340674374e-05
1581582,1581583,1581582,3163165,1852.798572063446,3.942855528293876e-05
1583584,1583585,1583584,3167169,1854.688448190689,3.87853189067755e-05
1585586,1585587,1585586,3171173,1856.6810281276703,3.815245690930169e-05
1587588,1587589,1587588,3175177,1858.644525051117,3.7529802284552716e-05
1589590,1589591,1589590,3179181,1860.802555322647,3.6917189959240204e-05
1591592,1591593,1591592,3183185,1862.6173791885376,3.6314457815933565e-05
1593594,1593595,1593594,3187189,1864.6354081630707,3.5721446351999475e-05
1595596,1595597,1595596,3191193,1866.601565361023,3.513799913434923e-05
1597598,1597599,1597598,3195197,1868.5113162994385,3.456396143519669e-05
1599600,1599601,1599600,3199201,1870.4600882530212,3.3999181482613494e-05
1601602,1601603,1601602,3203205,1872.5083122253418,3.344350977840804e-05
1603604,1603605,1603604,3207209,1874.4601011276245,3.289679978024651e-05
1605606,1605607,1605606,3211213,1876.346577167511,3.2358906423723965e-05
1607608,1607609,1607608,3215217,1878.206199169159,3.182968794135377e-05
1609610,1609611,1609610,3219221,1880.0757644176483,3.130900370251766e-05
1611612,1611613,1611612,3223225,1881.970165014267,3.079671625982883e-05
1613614,1613615,1613614,3227229,1883.8153421878815,3.029269032595039e-05
1615616,1615617,1615616,3231233,1885.6860060691833,2.9796792546221695e-05
1617618,1617619,1617618,3235237,1887.5701911449432,2.9308891612345178e-05
1619620,1619621,1619620,3239241,1889.4650511741638,2.8828858489760023e-05
1621622,1621623,1621622,3243245,1891.4452941417694,2.8356566531329008e-05
1623624,1623625,1623624,3247249,1893.4140622615814,2.7891890454156965e-05
1625626,1625627,1625626,3251253,1895.366698026657,2.743470759014599e-05
1627628,1627629,1627628,3255257,1897.232880115509,2.6984897090187587e-05
1629630,1629631,1629630,3259261,1899.0768761634827,2.654233992416266e-05
1631632,1631633,1631632,3263265,1900.9224331378937,2.610691899462836e-05
1633634,1633635,1633634,3267269,1902.7820122241974,2.5678519250504905e-05
1635636,1635637,1635636,3271273,1904.739518404007,2.525702757338877e-05
1637638,1637639,1637638,3275277,1906.6861753463745,2.4842332209118467e-05
1639640,1639641,1639640,3279281,1908.6711752414703,2.4434323790956114e-05
1641642,1641643,1641642,3283285,1910.615079164505,2.4032894089032197e-05
1643644,1643645,1643644,3287289,1912.52614402771,2.3637937488274474e-05
1645646,1645647,1645646,3291293,1914.3797192573547,2.3249349055731727e-05
1647648,1647649,1647648,3295297,1916.2234580516815,2.2867026473250007e-05
1649650,1649651,1649650,3299301,1918.0870792865753,2.249086821848323e-05
1651652,1651653,1651652,3303305,1919.9768242835999,2.2120775270195736e-05
1653654,1653655,1653654,3307309,1921.8475341796875,2.1756649630333413e-05
1655656,1655657,1655656,3311313,1923.819895029068,2.139839500614471e-05
1657658,1657659,1657658,3315317,1925.774109363556,2.104591692386748e-05
1659660,1659661,1659660,3319321,1927.6749923229218,2.0699121478173765e-05
1661662,1661663,1661662,3323325,1929.5790331363678,2.0357917946967063e-05
1663664,1663665,1663664,3327329,1931.4817831516266,2.0022215494464035e-05
1665666,1665667,1665666,3331333,1933.4063034057617,1.9691925672304933e-05
1667668,1667669,1667668,3335337,1935.2010560035706,1.9366961168998387e-05
1669670,1669671,1669670,3339341,1937.0464770793915,1.9047235809921403e-05
1671672,1671673,1671672,3343345,1938.868833065033,1.873266546681407e-05
1673674,1673675,1673674,3347349,1940.8094232082367,1.8423166807224334e-05
1675676,1675677,1675676,3351353,1942.633530139923,1.8118658090315876e-05
1677678,1677679,1677678,3355357,1944.4654173851013,1.781905871212075e-05
1679680,1679681,1679680,3359361,1946.2377500534058,1.752428920553939e-05
1681682,1681683,1681682,3363365,1948.0849232673645,1.7234272604582657e-05
1683684,1683685,1683684,3367369,1949.9322481155396,1.6948931261140388e-05
1685686,1685687,1685686,3371373,1951.8331673145294,1.666819036927336e-05
1687688,1687689,1687688,3375377,1953.704602241516,1.639197546410287e-05
1689690,1689691,1689690,3379381,1955.5689914226532,1.6120213672365935e-05
1691692,1691693,1691692,3383385,1957.4447112083435,1.585283291660744e-05
1693694,1693695,1693694,3387389,1959.319253206253,1.558976305204851e-05
1695696,1695697,1695696,3391393,1961.1962661743164,1.5330933933910273e-05
1697698,1697699,1697698,3395397,1963.0417392253876,1.5076277691150608e-05
1699700,1699701,1699700,3399401,1964.873375415802,1.482572668010107e-05
1701702,1701703,1701702,3403405,1966.8039500713348,1.4579215076082619e-05
1703704,1703705,1703704,3407409,1969.4445323944092,1.4336677054416214e-05
1705706,1705707,1705706,3411413,1972.0321652889252,1.4098049405220081e-05
1707708,1707709,1707708,3415417,1974.3623502254486,1.386326835017826e-05
1709710,1709711,1709710,3419421,1976.557597398758,1.3632272157337866e-05
1711712,1711713,1711712,3423425,1978.7060720920563,1.3404999890553881e-05
1713714,1713715,1713714,3427429,1980.8700354099274,1.3181391182115476e-05
1715716,1715717,1715716,3431433,1982.9430310726166,1.2961387255927548e-05
1717718,1717719,1717718,3435437,1984.9495553970337,1.274493001801602e-05
1719720,1719721,1719720,3439441,1986.8413853645325,1.2531961942841008e-05
1721722,1721723,1721722,3443445,1988.769944190979,1.2322426869104675e-05
1723724,1723725,1723724,3447449,1990.5789651870728,1.2116269658690726e-05
1725726,1725727,1725726,3451453,1992.553304195404,1.1913435741917056e-05
1727728,1727729,1727728,3455457,1994.6934731006622,1.1713871117535746e-05
1729730,1729731,1729730,3459461,1996.5574142932892,1.1517523603288282e-05
1731732,1731733,1731732,3463465,1998.454291343689,1.1324341357976664e-05
1733734,1733735,1733734,3467469,2000.321393251419,1.1134272881463403e-05
1735736,1735737,1735736,3471473,2002.133599281311,1.0947268492600415e-05
1737738,1737739,1737738,3475477,2004.2353973388672,1.076327828286594e-05
1739740,1739741,1739740,3479481,2006.592785358429,1.0582253707980271e-05
1741742,1741743,1741742,3483485,2009.023389339447,1.0404147474218917e-05
1743744,1743745,1743744,3487489,2011.2386491298676,1.0228912060483708e-05
1745746,1745747,1745746,3491493,2013.3526504039764,1.0056501196231693e-05
1747748,1747749,1747748,3495497,2015.5162591934204,9.886869406727783e-06
1749750,1749751,1749750,3499501,2017.7110702991486,9.719971899357915e-06
1751752,1751753,1751752,3503505,2019.8375353813171,9.555764563629054e-06
1753754,1753755,1753754,3507509,2021.869430065155,9.394204198542866e-06
1755756,1755757,1755756,3511513,2024.2191181182861,9.235247603101016e-06
1757758,1757759,1757758,3515517,2026.0087022781372,9.078853622668248e-06
1759760,1759761,1759760,3519521,2027.906836271286,8.924980193114607e-06
1761762,1761763,1761762,3523525,2029.9431381225586,8.773587182986375e-06
1763764,1763765,1763764,3527529,2031.992567062378,8.624634119769325e-06
1765766,1765767,1765766,3531533,2033.9042212963104,8.47808189519128e-06
1767768,1767769,1767768,3535537,2035.8724331855774,8.333891855727416e-06
1769770,1769771,1769770,3539541,2037.7473771572113,8.192026143660769e-06
1771772,1771773,1771772,3543545,2039.6825802326202,8.052446787587542e-06
1773774,1773775,1773774,3547549,2041.6023533344269,7.915117180345987e-06
1775776,1775777,1775776,3551553,2043.4609372615814,7.780001055834873e-06
1777778,1777779,1777778,3555557,2045.3093492984772,7.647062830073992e-06
1779780,1779781,1779780,3559561,2047.1458129882812,7.51626726014365e-06
1781782,1781783,1781782,3563565,2049.0132281780243,7.387579557871504e-06
1783784,1783785,1783784,3567569,2050.8603451251984,7.260966185640427e-06
1785786,1785787,1785786,3571573,2052.768976211548,7.136393378459616e-06
1787788,1787789,1787788,3575577,2054.6828322410583,7.013828508206643e-06
1789790,1789791,1789790,3579581,2056.6280751228333,6.893238946759084e-06
1791792,1791793,1791792,3583585,2058.568966150284,6.774593089176051e-06
1793794,1793795,1793794,3587589,2060.4307692050934,6.657859330516658e-06
1795796,1795797,1795796,3591593,2062.2971770763397,6.54300697533472e-06
1797798,1797799,1797798,3595597,2064.2885291576385,6.430006010305078e-06
1799800,1799801,1799800,3599601,2066.1327612400055,6.318825967355224e-06
1801802,1801803,1801802,3603605,2067.9729363918304,6.2094378563415376e-06
1803804,1803805,1803804,3607609,2069.7562041282654,6.101812800807238e-06
1805806,1805807,1805806,3611613,2071.5303761959076,5.995922379042895e-06
1807808,1807809,1807808,3615617,2073.3151910305023,5.891738283025916e-06
1809810,1809811,1809810,3619621,2075.145938396454,5.789233455288922e-06
1811812,1811813,1811812,3623625,2076.965705394745,5.688380838364537e-06
1813814,1813815,1813814,3627629,2078.751083135605,5.589153374785383e-06
1815816,1815817,1815816,3631633,2080.5045642852783,5.4915250302656204e-06
1817818,1817819,1817818,3635637,2082.266384124756,5.3954704526404385e-06
1819820,1819821,1819820,3639641,2084.0162732601166,5.300963834997674e-06
1821822,1821823,1821822,3643645,2085.716944217682,5.207980166233028e-06
1823824,1823825,1823824,3647649,2087.3996522426605,5.116495003676391e-06
1825826,1825827,1825826,3651653,2089.0967993736267,5.026484473091841e-06
1827828,1827829,1827828,3655657,2090.8549041748047,4.937924245496106e-06
1829830,1829831,1829830,3659661,2092.6116983890533,4.850791469834803e-06
1831832,1831833,1831832,3663665,2094.3946533203125,4.7650630676798755e-06
1833834,1833835,1833834,3667669,2096.126430273056,4.6807159606032656e-06
1835836,1835837,1835836,3671673,2097.822911262512,4.597728207045293e-06
1837838,1837839,1837838,3675677,2099.5206611156464,4.516077979133115e-06
1839840,1839841,1839840,3679681,2101.2820003032684,4.435743676367565e-06
1841842,1841843,1841842,3683685,2103.1355521678925,4.356703811936313e-06
1843844,1843845,1843844,3687689,2105.0850973129272,4.27893792220857e-06
1845846,1845847,1845846,3691693,2106.966100215912,4.202425202493032e-06
1847848,1847849,1847848,3695697,2108.862169265747,4.127145530219423e-06
1849850,1849851,1849850,3699701,2110.5499591827393,4.053078896504303e-06
1851852,1851853,1851852,3703705,2112.2491822242737,3.980206088272098e-06
1853854,1853855,1853854,3707709,2114.051525115967,3.9085075513867196e-06
1855856,1855857,1855856,3711713,2115.8875272274017,3.837964413833106e-06
1857858,1857859,1857858,3715717,2117.7193484306335,3.7685581446567085e-06
1859860,1859861,1859860,3719721,2119.4642980098724,3.700270440276654e-06
1861862,1861863,1861862,3723725,2121.2356543540955,3.6330829971120693e-06
1863864,1863865,1863864,3727729,2122.9612152576447,3.566978421076783e-06
1865866,1865867,1865866,3731733,2124.65288233757,3.501939204397786e-06
1867868,1867869,1867868,3735737,2126.332998275757,3.4379479529889068e-06
1869870,1869871,1869870,3739741,2128.0520782470703,3.3749879548850004e-06
1871872,1871873,1871872,3743745,2129.7804222106934,3.3130424981209217e-06
1873874,1873875,1873874,3747749,2131.5558621883392,3.2520953254788765e-06
1875876,1875877,1875876,3751753,2133.301965236664,3.192130407114746e-06
1877878,1877879,1877878,3755757,2135.084784269333,3.1331317131844116e-06
1879880,1879881,1879880,3759761,2136.763393163681,3.075083782277943e-06
1881882,1881883,1881882,3763765,2138.4687070846558,3.0179713803590857e-06
1883884,1883885,1883884,3767769,2140.1770632267,2.961779159704747e-06
1885886,1885887,1885886,3771773,2141.8552281856537,2.906492568399699e-06
1887888,1887889,1887888,3775777,2143.5832302570343,2.8520968271550373e-06
1889890,1889891,1889890,3779781,2145.3363950252533,2.7985774977423716e-06
1891892,1891893,1891892,3783785,2147.121174097061,2.7459208240543376e-06
1893894,1893895,1893894,3787789,2148.8340673446655,2.69411259523622e-06
1895896,1895897,1895896,3791793,2150.5287911891937,2.6431393962411676e-06
1897898,1897899,1897898,3795797,2152.2158482074738,2.5929873572749784e-06
1899900,1899901,1899900,3799801,2153.9326951503754,2.5436434043513145e-06
1901902,1901903,1901902,3803805,2155.6022703647614,2.495094804544351e-06
1903904,1903905,1903904,3807809,2157.329725265503,2.44732848386775e-06
1905906,1905907,1905906,3811813,2159.0463490486145,2.4003318230825244e-06
1907908,1907909,1907908,3815817,2160.7503912448883,2.3540924303233624e-06
1909910,1909911,1909910,3819821,2162.505942106247,2.308598141098628e-06
1911912,1911913,1911912,3823825,2164.258505344391,2.26383701829036e-06
1913914,1913915,1913914,3827829,2165.956210374832,2.219797124780598e-06
1915916,1915917,1915916,3831833,2167.650395154953,2.1764669781987322e-06
1917918,1917919,1917918,3835837,2169.2945952415466,2.133834982487315e-06
1919920,1919921,1919920,3839841,2170.9742062091827,2.091890110023087e-06
1921922,1921923,1921922,3843845,2172.7679150104523,2.0506208784354385e-06
1923924,1923925,1923924,3847849,2174.5235781669617,2.0100167148484616e-06
1925926,1925927,1925926,3851853,2176.2663311958313,1.970066705325735e-06
1927928,1927929,1927928,3855857,2177.969206094742,1.9307605043650256e-06
1929930,1929931,1929930,3859861,2179.6455051898956,1.8920877664641012e-06
1931932,1931933,1931932,3863865,2181.3498392105103,1.854038146120729e-06
1933934,1933935,1933934,3867869,2183.050270318985,1.816601752580027e-06
1935936,1935937,1935936,3871873,2184.752712249756,1.7797683540266007e-06
1937938,1937939,1937938,3875877,2186.4471900463104,1.743528514452919e-06
1939940,1939941,1939940,3879881,2188.203058242798,1.707872684164613e-06
1941942,1941943,1941942,3883885,2189.932178258896,1.67279154084099e-06
1943944,1943945,1943944,3887889,2191.6336681842804,1.638275534787681e-06
1945946,1945947,1945946,3891893,2193.3277072906494,1.6043156847445061e-06
1947948,1947949,1947948,3895897,2195.041783094406,1.5709031231381232e-06
1949950,1949951,1949950,3899901,2196.7351381778717,1.5380287550215144e-06
1951952,1951953,1951952,3903905,2198.4211101531982,1.505684281255526e-06
1953954,1953955,1953954,3907909,2200.1235201358795,1.4738608342668158e-06
1955956,1955957,1955956,3911913,2201.808427095413,1.4425503422899055e-06
1957958,1957959,1957958,3915917,2203.4814841747284,1.411744278811966e-06
1959960,1959961,1959960,3919921,2205.2077622413635,1.3814345720675192e-06
1961962,1961963,1961962,3923925,2206.971328020096,1.3516131502910866e-06
1963964,1963965,1963964,3927929,2208.69366812706,1.3222722827777034e-06
1965966,1965967,1965966,3931933,2210.376985311508,1.2934042388224043e-06
1967968,1967969,1967968,3935937,2212.064583301544,1.2650012877202244e-06
1969970,1969971,1969970,3939941,2213.754531145096,1.2370561535135494e-06
1971972,1971973,1971972,3943945,2215.4443802833557,1.2095609918105765e-06
1973974,1973975,1973974,3947949,2217.152451276779,1.1825089814010425e-06
1975976,1975977,1975976,3951953,2218.838847398758,1.1558930737010087e-06
1977978,1977979,1977978,3955957,2220.533839225769,1.129705879066023e-06
1979980,1979981,1979980,3959961,2222.253467321396,1.1039404625989846e-06
1981982,1981983,1981982,3963965,2223.96085524559,1.0785903441501432e-06
1983984,1983985,1983984,3967969,2225.6381413936615,1.0536487025092356e-06
1985986,1985987,1985986,3971973,2227.341639280319,1.0291088301528362e-06
1987988,1987989,1987988,3975977,2229.3334143161774,1.0049644743048702e-06
1989990,1989991,1989990,3979981,2231.2624881267548,9.812091548155877e-07
1991992,1991993,1991992,3983985,2233.1158192157745,9.57836505222076e-07
1993994,1993995,1993994,3987989,2234.992618083954,9.348403864350985e-07
1995996,1995997,1995996,3991993,2236.679386138916,9.122148867390933e-07
1997998,1997999,1997998,3995997,2238.3879251480103,8.899539807316614e-07
2000000,2000001,2000000,4000001,2240.1321170330048,8.680516430104035e-07


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0005650520324707031,2181.2938132599165
1,4,4,8,0.0019378662109375,1650.9600894919724
2,6,6,12,0.0030868053436279297,786.9009567073322
3,8,8,16,0.004029989242553711,443.58608911943384
4,12,12,24,0.005432844161987305,300.56155646592265
5,20,20,40,0.007476091384887695,289.3974206603966
6,24,24,48,0.008771181106567383,223.69526839628975
7,32,32,64,0.010661840438842773,220.72167943146133
8,36,36,72,0.011862993240356445,183.69180242892548
9,44,44,88,0.014126062393188477,182.02986018160618
10,50,50,100,0.01618790626525879,181.17567132880208
11,56,56,112,0.018147945404052734,170.03638269693147
12,60,60,120,0.01933002471923828,148.57486999488424
13,64,64,128,0.020489931106567383,133.65412768561646
14,70,70,140,0.022565841674804688,109.77584992925767
15,72,72,144,0.02368903160095215,82.14485419750099
16,76,76,152,0.025273799896240234,80.83922421752368
17,80,80,160,0.026824951171875,78.96080307353009
18,88,88,176,0.029392004013061523,78.7719300343806
19,92,92,184,0.03115081787109375,75.49803880435866
20,96,96,192,0.032891035079956055,73.83934276444575
21,102,102,204,0.03518104553222656,73.37869766012068
22,106,106,212,0.036707162857055664,70.68360968449633
23,110,110,220,0.03832602500915527,69.18156561569117
24,116,116,232,0.04058504104614258,68.41646619118296
25,124,124,248,0.04332709312438965,68.3663813211524
26,128,128,256,0.044970035552978516,65.3897452770234
27,134,134,268,0.047178030014038086,64.9236398858518
28,138,138,276,0.04865312576293945,62.985472947437074
29,146,146,292,0.05112409591674805,62.95210477775822
30,150,150,300,0.052577972412109375,60.535359788497544
31,158,158,316,0.05451393127441406,60.50873240431133
32,162,162,324,0.0559239387512207,58.29827656607495
33,168,168,336,0.05773186683654785,57.92439847378023
34,172,172,344,0.05887198448181152,56.76619974948835
35,180,180,360,0.06115579605102539,56.754147744358306
36,184,184,368,0.06280875205993652,55.729978746412826
37,188,188,376,0.06395912170410156,55.19744382774138
38,196,196,392,0.06624889373779297,55.19050256349988
39,200,200,400,0.06739997863769531,54.64523022558342
40,208,208,416,0.06950712203979492,54.640314439927806
41,212,212,424,0.07103395462036133,54.108094140376124
42,220,220,440,0.07371020317077637,54.10375604936826
43,226,226,452,0.0758049488067627,53.877086292780405
44,234,234,468,0.07831001281738281,53.87330472012718
45,240,240,480,0.08030200004577637,53.49811888471481
46,248,248,496,0.0827641487121582,53.49460341009626
47,254,254,508,0.09033918380737305,52.9254795429415
48,262,262,524,0.09487295150756836,52.92221640965681
49,268,268,536,0.09690499305725098,52.26786738777196
50,276,276,552,0.09890580177307129,52.26485072563719
51,282,282,564,0.10049891471862793,51.44443076873904
52,290,290,580,0.10249495506286621,51.44147432892464
53,298,298,596,0.10501599311828613,51.438536470135205
54,306,306,612,0.10766386985778809,51.435615587362236
55,312,312,624,0.10930681228637695,49.7136069230437
56,320,320,640,0.1113119125366211,49.71073909746406
57,328,328,656,0.1140749454498291,49.70791406796411
58,336,336,672,0.11710000038146973,49.7051272194808
59,342,342,684,0.11895895004272461,47.47352121865515
60,350,350,700,0.1216888427734375,47.47091040218811
61,358,358,716,0.12419414520263672,47.468338978416114
62,366,366,732,0.1266341209411621,47.46580319891996
63,372,372,744,0.12841510772705078,44.90985403410468
64,380,380,760,0.13109779357910156,44.90739089077556
65,388,388,776,0.13387298583984375,44.90496943583321
66,396,396,792,0.13707709312438965,44.90258587415542
67,404,404,808,0.13986992835998535,44.90023677588715
68,410,410,820,0.14169907569885254,41.79387968652577
69,418,418,836,0.14455819129943848,41.79184236490073
70,424,424,848,0.1465449333190918,38.947228266797765
71,432,432,864,0.1487410068511963,38.94540290101531
72,440,440,880,0.15136003494262695,38.9435920282051
73,448,448,896,0.15386199951171875,38.941794501922686
74,454,454,908,0.15588998794555664,35.960261131487414
75,462,462,924,0.15852022171020508,35.95861437940107
76,468,468,936,0.160567045211792,33.287248377427886
77,476,476,952,0.16292095184326172,33.28577475992529
78,482,482,964,0.1645510196685791,30.539653791511455
79,488,488,976,0.16628098487854004,29.615008422158553
80,496,496,992,0.1684858798980713,29.61365911296957
81,502,502,1004,0.17035913467407227,27.041313078749454
82,510,510,1020,0.1724071502685547,27.040106249533892
83,516,516,1032,0.17441201210021973,24.651822871100194
84,524,524,1048,0.17693710327148438,24.650662686907026
85,530,530,1060,0.17895889282226562,21.926916595581133
86,538,538,1076,0.18155384063720703,21.925876387494327
87,544,544,1088,0.1838829517364502,19.38987887854023
88,552,552,1104,0.18660902976989746,19.388930271255276
89,558,558,1116,0.18898987770080566,16.608093985512596
90,566,566,1132,0.1918489933013916,16.60720854258807
91,572,572,1144,0.19408202171325684,14.340721007916954
92,580,580,1160,0.19652891159057617,14.339894160041126
93,586,586,1172,0.19814395904541016,12.296962068950279
94,594,594,1188,0.20064306259155273,12.29616325254949
95,600,600,1200,0.20230889320373535,10.510741953040451
96,608,608,1216,0.20458292961120605,10.510010324363634
97,614,614,1228,0.2061781883239746,9.014298594634283
98,622,622,1244,0.2081458568572998,9.013638444774529
99,630,630,1260,0.2100968360900879,9.01298080384538
100,638,638,1276,0.21232891082763672,9.012325589257216
101,644,644,1288,0.2139129638671875,7.780570310155326
102,652,652,1304,0.21584391593933105,7.779951526052514
103,658,658,1316,0.21737194061279297,6.819609936315487
104,666,666,1332,0.21929502487182617,6.819035208742889
105,674,674,1348,0.22133517265319824,6.818470923337259
106,682,682,1364,0.22345495223999023,6.817916235665393
107,688,688,1376,0.2255251407623291,5.9367486603406405
108,696,696,1392,0.22815585136413574,5.936211169413809
109,702,702,1404,0.2298288345336914,5.174314634658003
110,710,710,1420,0.23187994956970215,5.173815290662105
111,716,716,1432,0.23352813720703125,4.494302502301821
112,724,724,1448,0.23577284812927246,4.493820308759155
113,730,730,1460,0.23806285858154297,3.8866757925634374
114,738,738,1476,0.24089717864990234,3.8862466840530487
115,744,744,1488,0.24311399459838867,3.3576534065056194
116,752,752,1504,0.24571919441223145,3.357269581602168
117,758,758,1516,0.24735116958618164,2.880300846288719
118,766,766,1532,0.24935102462768555,2.8799550688476074
119,772,772,1544,0.25095391273498535,2.471740110092469
120,780,780,1560,0.2529909610748291,2.47143597397735
121,786,786,1572,0.25462794303894043,2.112352332036494
122,792,792,1584,0.25630688667297363,1.8133498744381313
123,798,798,1596,0.2578911781311035,1.4925185789629722
124,806,806,1612,0.259829044342041,1.4922642545719782
125,812,812,1624,0.2613718509674072,1.2760333677532572
126,820,820,1640,0.2639601230621338,1.2758055117387812
127,826,826,1652,0.26598095893859863,1.0747965742291399
128,834,834,1668,0.26834583282470703,1.0745936419660893
129,838,838,1676,0.26966094970703125,0.5794730414766036
130,846,846,1692,0.2723050117492676,0.5792765367091306
131,850,850,1700,0.27399516105651855,0.31190445181914583
132,858,858,1716,0.27664899826049805,0.3117665257838098
133,862,862,1724,0.278270959854126,0.16648912514040148
134,866,866,1732,0.27990293502807617,0.09332014461233484
135,872,872,1744,0.2821509838104248,0.0809951449637083
136,876,876,1752,0.28388404846191406,0.050160142572963196
137,880,880,1760,0.2853879928588867,0.032760873621782594
138,884,884,1768,0.28720998764038086,0.025375763368288062
139,888,888,1776,0.2887740135192871,0.021377153048092623
140,896,896,1792,0.29086995124816895,0.02133605104631897
141,900,900,1800,0.29208803176879883,0.016293070737106063
142,908,908,1816,0.2947530746459961,0.016264277908248914
143,912,912,1824,0.2962930202484131,0.012659173853762695
144,920,920,1840,0.29937005043029785,0.01263847739414814
145,924,924,1848,0.30092597007751465,0.009445123849559423
146,928,928,1856,0.30254483222961426,0.006891616261100353
147,936,936,1872,0.30533504486083984,0.0068789167659133454
148,940,940,1880,0.3071911334991455,0.0055435354696555805
149,948,948,1896,0.3099949359893799,0.00553332780089022
150,952,952,1904,0.3112339973449707,0.004343211079117282
151,960,960,1920,0.31325292587280273,0.0043347196871081906
152,964,964,1928,0.3144259452819824,0.0033238844248444366
153,970,970,1940,0.3169548511505127,0.003086398933987766
154,976,976,1952,0.31873393058776855,0.002892278228387113
155,980,980,1960,0.32044291496276855,0.0022202596724127943
156,988,988,1976,0.3235180377960205,0.0022151515900077356
157,992,992,1984,0.3251199722290039,0.0016091770994535182
158,1000,1000,2000,0.3271369934082031,0.0016054316405416102
159,1004,1004,2008,0.3290250301361084,0.0011430153840592538
160,1010,1010,2020,0.3312230110168457,0.001062806116806314
161,1014,1014,2028,0.33281898498535156,0.0007474035813856972
162,1020,1020,2040,0.33504486083984375,0.0006953956898314573
163,1024,1024,2048,0.33707189559936523,0.0005246692453511059
164,1030,1030,2060,0.33965110778808594,0.0004972708296691053
165,1034,1034,2068,0.34188389778137207,0.0003823883920404114
166,1042,1042,2084,0.3446199893951416,0.0003814495393044126
167,1046,1046,2092,0.3464689254760742,0.0002918856743008291
168,1052,1052,2104,0.34845900535583496,0.0002755629951707306
169,1058,1058,2116,0.3505978584289551,0.00026029314460629394
170,1062,1062,2124,0.35228705406188965,0.00019450272384347045
171,1068,1068,2136,0.3545229434967041,0.00018278977529462281
172,1074,1074,2148,0.35698699951171875,0.0001719445128856023
173,1078,1078,2156,0.35836195945739746,0.00013496233327714435
174,1084,1084,2168,0.36000895500183105,0.00012825582348341413
175,1088,1088,2176,0.36167311668395996,0.00010706492435019754
176,1094,1094,2188,0.36350202560424805,0.00010324783352189115
177,1098,1098,2196,0.36501502990722656,8.610767258687702e-05
178,1106,1106,2212,0.3678560256958008,8.592472920554428e-05
179,1110,1110,2220,0.36959290504455566,6.744613813225442e-05
180,1116,1116,2232,0.37186098098754883,6.424260652693192e-05
181,1120,1120,2240,0.3738870620727539,5.4416926218436856e-05
182,1126,1126,2252,0.37631702423095703,5.254078371308424e-05
183,1132,1132,2264,0.3785128593444824,5.0766687422765244e-05
184,1136,1136,2272,0.3802361488342285,4.44698126784715e-05
185,1140,1140,2280,0.38187599182128906,3.9589785956195556e-05
186,1148,1148,2296,0.3843238353729248,3.953774364617857e-05
187,1152,1152,2304,0.3861660957336426,3.3837318710538966e-05
188,1156,1156,2312,0.38814496994018555,2.9217035148576542e-05
189,1164,1164,2328,0.39218902587890625,2.9172171366553812e-05
190,1168,1168,2336,0.3940460681915283,2.4958050175882818e-05
191,1172,1172,2344,0.3957839012145996,2.0890831137876376e-05
192,1180,1180,2360,0.39831089973449707,2.085558344333549e-05
193,1184,1184,2368,0.3999481201171875,1.7467220004618866e-05
194,1192,1192,2384,0.40252017974853516,1.743914924645651e-05
195,1196,1196,2392,0.4037439823150635,1.3840700148648466e-05
196,1204,1204,2408,0.40649914741516113,1.381813206080551e-05
197,1208,1208,2416,0.40824389457702637,1.0393337561254157e-05
198,1216,1216,2432,0.41069793701171875,1.0377167541264498e-05
199,1220,1220,2440,0.41185688972473145,7.665222938157967e-06
200,1228,1228,2456,0.4138450622558594,7.651546525266895e-06
201,1232,1232,2464,0.4152719974517822,5.4896534038562095e-06
202,1240,1240,2480,0.417525053024292,5.48006596545747e-06
203,1244,1244,2488,0.41887497901916504,3.9288286188821075e-06
204,1252,1252,2504,0.42142391204833984,3.922081987184356e-06
205,1256,1256,2512,0.42308616638183594,2.8830952487624018e-06
206,1264,1264,2528,0.4250919818878174,2.878218651858333e-06
207,1268,1268,2536,0.42624497413635254,2.181166337322793e-06
208,1274,1274,2548,0.42781591415405273,2.059618964267429e-06
209,1278,1278,2556,0.4289522171020508,1.7095497923946823e-06
210,1286,1286,2572,0.43091678619384766,1.7063545101336786e-06
211,1290,1290,2580,0.4323158264160156,1.4161586250338587e-06
212,1296,1296,2592,0.4346041679382324,1.3648367485075141e-06
213,1302,1302,2604,0.437391996383667,1.3123968756190152e-06
214,1308,1308,2616,0.43955397605895996,1.2613271564987372e-06
215,1312,1312,2624,0.4408130645751953,1.0993429668815224e-06
216,1320,1320,2640,0.4428081512451172,1.0975418263114989e-06
217,1324,1324,2648,0.44460201263427734,9.043033060152084e-07
218,1332,1332,2664,0.4470038414001465,9.028540262079332e-07
219,1336,1336,2672,0.44831013679504395,7.182483159340336e-07
220,1344,1344,2688,0.4504368305206299,7.169280706875725e-07
221,1348,1348,2696,0.4518458843231201,5.373093472371693e-07
222,1352,1352,2704,0.45310282707214355,3.997984094894491e-07
223,1360,1360,2720,0.4551889896392822,3.9905967241793405e-07
224,1364,1364,2728,0.4566640853881836,2.8994077183597255e-07
225,1368,1368,2736,0.45785093307495117,1.970372522919206e-07
226,1376,1376,2752,0.4597897529602051,1.9649212390504545e-07
227,1380,1380,2760,0.46093010902404785,1.259768396266736e-07
228,1386,1386,2772,0.462507963180542,1.1362101304257521e-07
229,1392,1392,2784,0.4641149044036865,1.0229246072412934e-07
230,1398,1398,2796,0.4659850597381592,9.046414106705924e-08
231,1404,1404,2808,0.4677917957305908,7.983339855854865e-08
232,1410,1410,2820,0.469512939453125,6.987067990849027e-08
233,1416,1416,2832,0.47113990783691406,5.772221811639611e-08
234,1422,1422,2844,0.47311902046203613,4.715229806606658e-08
235,1426,1426,2852,0.4743349552154541,1.4687429938931018e-08
236,1434,1434,2868,0.4763360023498535,1.4476313481281977e-08
237,1438,1438,2876,0.47750210762023926,9.40292466111714e-09


==> plot_data/logistic_regression_problem_lambda_param10overN_data_namespambase/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0013971328735351562,2181.2938132599165
1,4,4,8,0.0028219223022460938,1650.9600894919724
2,6,6,12,0.00410914421081543,811.2562314125337
3,8,8,16,0.0052759647369384766,540.4289308351636
4,10,10,20,0.006644010543823242,340.4672839375705
5,12,12,24,0.007918834686279297,246.045559467972
6,14,14,28,0.009087085723876953,179.15645943945333
7,18,18,36,0.010715961456298828,176.09590819170626
8,22,22,44,0.012698888778686523,179.49204530230872
9,24,24,48,0.014139890670776367,132.26997085802282
10,26,26,52,0.01567816734313965,127.41736922878476
11,28,28,56,0.017106056213378906,131.37556663863074
12,32,32,64,0.019366025924682617,126.84435295539743
13,34,34,68,0.021001100540161133,106.30186430969206
14,36,36,72,0.023188114166259766,102.88115960850382
15,40,40,80,0.024930238723754883,102.47618365977314
16,44,44,88,0.026534080505371094,101.82312920170057
17,46,46,92,0.027615070343017578,97.15490589928982
18,50,50,100,0.029797077178955078,94.33019338730924
19,52,52,104,0.031145095825195312,80.4903442751745
20,54,54,108,0.03242802619934082,81.31254268609837
21,56,56,112,0.03369498252868652,81.88121702865942
22,58,58,116,0.03488326072692871,81.27086783594427
23,60,60,120,0.036536216735839844,76.74140494959192
24,62,62,124,0.037748098373413086,76.99510499544522
25,64,64,128,0.03890204429626465,74.5431711425615
26,66,66,132,0.04004526138305664,74.69278249642502
27,70,70,140,0.041754961013793945,74.56441781853619
28,72,72,144,0.04288220405578613,69.9782011093198
29,76,76,152,0.04479217529296875,69.91225327359734
30,78,78,156,0.0460970401763916,66.26838141079611
31,82,82,164,0.04790902137756348,66.27073562276814
32,84,84,168,0.049139976501464844,63.481344845964486
33,86,86,172,0.05089592933654785,63.7190912540359
34,88,88,176,0.05202007293701172,63.90336556497323
35,92,92,184,0.05359387397766113,63.807608879668805
36,94,94,188,0.05482196807861328,61.566793292530974
37,98,98,196,0.056558847427368164,61.52688100814953
38,100,100,200,0.05767107009887695,58.904292568147866
39,104,104,208,0.059439897537231445,58.88762163541469
40,106,106,212,0.06048011779785156,57.717888333730116
41,108,108,216,0.061654090881347656,57.62514878141383
42,110,110,220,0.06323695182800293,57.529530762268905
43,112,112,224,0.06441497802734375,57.41867547769448
44,116,116,232,0.06638288497924805,57.40215875999911
45,118,118,236,0.06744813919067383,56.81739714880291
46,120,120,240,0.06854510307312012,56.67589043198427
47,122,122,244,0.0696871280670166,56.457494112811446
48,126,126,252,0.0712900161743164,56.43205628063629
49,128,128,256,0.07230210304260254,55.982180017030714
50,132,132,264,0.07402706146240234,55.978461192982195
51,134,134,268,0.0751039981842041,54.69553390432793
52,138,138,276,0.07675719261169434,54.695983044795184
53,140,140,280,0.07784104347229004,54.45590175028951
54,144,144,288,0.07990217208862305,54.445062997060404
55,146,146,292,0.08104991912841797,53.8193328940863
56,150,150,300,0.08283305168151855,53.816132750525185
57,152,152,304,0.08396601676940918,53.525672145477074
58,156,156,312,0.08564519882202148,53.522790263717525
59,158,158,316,0.08673906326293945,53.34773220655529
60,162,162,324,0.08842921257019043,53.3207535877018
61,166,166,332,0.09010791778564453,53.25856436054846
62,170,170,340,0.09172201156616211,53.21180002390997
63,174,174,348,0.09336090087890625,53.17560667429029
64,176,176,352,0.09455108642578125,52.7891853756953
65,180,180,360,0.09660601615905762,52.77928969535628
66,182,182,364,0.09778308868408203,52.141518450020385
67,186,186,372,0.09964799880981445,52.1379852390578
68,188,188,376,0.10070419311523438,51.74794340898188
69,192,192,384,0.10232400894165039,51.745726125558804
70,194,194,388,0.10334300994873047,51.15281829385094
71,198,198,396,0.1049339771270752,51.139004666116534
72,200,200,400,0.10595011711120605,50.32606022315281
73,204,204,408,0.10756421089172363,50.33210907284115
74,206,206,412,0.1086130142211914,49.111912121295745
75,210,210,420,0.11024308204650879,49.106148589788745
76,212,212,424,0.11138415336608887,47.88341765867813
77,216,216,432,0.11345696449279785,47.873716808252766
78,220,220,440,0.11541199684143066,47.70529594795198
79,224,224,448,0.11733007431030273,47.56986665540762
80,228,228,456,0.11951112747192383,47.28607925363235
81,232,232,464,0.12119197845458984,47.21691307390756
82,240,240,480,0.12413406372070312,47.21483184032263
83,242,242,484,0.12527227401733398,45.974385723906835
84,246,246,492,0.12691116333007812,45.98467424968453
85,248,248,496,0.12813305854797363,44.98403881979198
86,252,252,504,0.1300640106201172,44.84044553590729
87,254,254,508,0.13176512718200684,43.57311045395045
88,256,256,512,0.1331479549407959,43.32134127210816
89,258,258,516,0.13443899154663086,42.342862578362656
90,262,262,524,0.1362619400024414,42.33275773240484
91,264,264,528,0.13752007484436035,42.11980298516801
92,268,268,536,0.13942885398864746,42.05487165395766
93,272,272,544,0.1410691738128662,41.98342412577972
94,276,276,552,0.1426830291748047,41.95492980523932
95,280,280,560,0.14431285858154297,41.998682712158825
96,284,284,568,0.1460728645324707,42.03792059843636
97,288,288,576,0.14788007736206055,42.06259545623175
98,290,290,580,0.14911103248596191,40.89056747301629
99,294,294,588,0.15101122856140137,40.87964705566492
100,296,296,592,0.15222406387329102,39.316257281756634
101,300,300,600,0.15388703346252441,39.274169876181304
102,302,302,604,0.15489506721496582,35.405214141751
103,306,306,612,0.15662407875061035,35.4526896313962
104,308,308,616,0.15768718719482422,34.17626727254515
105,312,312,624,0.15938591957092285,34.08729856638297
106,314,314,628,0.16045308113098145,32.95671528036314
107,318,318,636,0.16222500801086426,32.903598214128806
108,320,320,640,0.16338419914245605,32.15058893076093
109,324,324,648,0.16543126106262207,32.12697971344028
110,326,326,652,0.16662216186523438,29.92015578753194
111,330,330,660,0.16829919815063477,30.164880333014025
112,336,336,672,0.17041897773742676,30.182399399707037
113,340,340,680,0.17208409309387207,30.278798013638152
114,342,342,684,0.17313814163208008,29.63007955622834
115,346,346,692,0.17479991912841797,29.612355075034657
116,350,350,700,0.17661190032958984,29.630230023401282
117,352,352,704,0.17769908905029297,27.97622078695099
118,356,356,712,0.17951393127441406,28.03753285133712
119,358,358,716,0.18062400817871094,25.34843114369278
120,362,362,724,0.18231892585754395,25.453168551075578
121,366,366,732,0.18402314186096191,25.61177984731262
122,370,370,740,0.18565893173217773,25.78289374467704
123,372,372,744,0.18681716918945312,24.741572168414905
124,376,376,752,0.18849587440490723,24.835083425723724
125,378,378,756,0.1895618438720703,23.201882124629265
126,384,384,768,0.1917891502380371,23.195321246401818
127,390,390,780,0.19399094581604004,23.190550630701864
128,394,394,788,0.19556522369384766,23.23954731937738
129,396,396,792,0.19663119316101074,21.477107215243223
130,400,400,800,0.1981830596923828,21.570661583075434
131,402,402,804,0.1991729736328125,18.75149452098526
132,404,404,808,0.20022201538085938,20.331368843071232
133,410,410,820,0.2023160457611084,20.289049794597076
134,414,414,828,0.204024076461792,20.259360509390262
135,416,416,832,0.2050950527191162,19.527335682313606
136,420,420,840,0.2068009376525879,19.31077388472636
137,422,422,844,0.2079000473022461,17.956819459640883
138,426,426,852,0.2095041275024414,17.856707193638385
139,428,428,856,0.21053194999694824,14.142350177945218
140,432,432,864,0.2122809886932373,14.31766783192188
141,434,434,868,0.21345019340515137,13.324780552837069
142,438,438,876,0.2151482105255127,13.310923761402364
143,440,440,880,0.21629118919372559,11.853973581573541
144,444,444,888,0.2181541919708252,11.851520433455335
145,446,446,892,0.2195441722869873,11.008395336379749
146,450,450,900,0.22134804725646973,11.001379314050155
147,452,452,904,0.22255492210388184,10.008559577545952
148,458,458,916,0.2251279354095459,10.005290165935207
149,460,460,920,0.2263929843902588,9.572443249941443
150,464,464,928,0.22814488410949707,9.596939655818119
151,466,466,932,0.22922801971435547,9.501403702039966
152,470,470,940,0.23094987869262695,9.529918725749667
153,474,474,948,0.2328352928161621,9.546865253024748
154,478,478,956,0.23476696014404297,9.511269318368022
155,482,482,964,0.23661303520202637,9.435407092256355
156,486,486,972,0.2385101318359375,9.372193541336173
157,490,490,980,0.24045705795288086,9.34112863310213
158,492,492,984,0.2416400909423828,9.059318130712654
159,496,496,992,0.24331307411193848,9.067817113954902
160,498,498,996,0.24442410469055176,9.309412886534005
161,502,502,1004,0.24605393409729004,9.306294905412415
162,504,504,1008,0.24713397026062012,9.112889958891401
163,508,508,1016,0.2492051124572754,9.113831830920162
164,512,512,1024,0.25108909606933594,9.145918857784068
165,516,516,1032,0.25270724296569824,9.152418629197996
166,520,520,1040,0.25433826446533203,9.126671737871675
167,524,524,1048,0.2559840679168701,9.107646881023356
168,526,526,1052,0.2570970058441162,8.887666278525217
169,530,530,1060,0.258695125579834,8.888872054371518
170,532,532,1064,0.25972700119018555,8.831460499300647
171,536,536,1072,0.2614438533782959,8.831135469752098
172,538,538,1076,0.26259422302246094,8.806414540025685
173,542,542,1084,0.26430296897888184,8.804508373655949
174,546,546,1092,0.2661151885986328,8.809391401525659
175,550,550,1100,0.26778721809387207,8.81244743946877
176,554,554,1108,0.2695350646972656,8.781167101496862
177,558,558,1116,0.27118802070617676,8.758025714379869
178,562,562,1124,0.2728562355041504,8.744175941929825
179,566,566,1132,0.2745780944824219,8.727422997158556
180,570,570,1140,0.27627015113830566,8.71349668746609
181,572,572,1144,0.2776200771331787,8.559660649393322
182,576,576,1152,0.2792551517486572,8.556050719222526
183,578,578,1156,0.2803061008453369,8.120320403448432
184,582,582,1164,0.2818901538848877,8.118140655766751
185,586,586,1172,0.2835102081298828,8.097061699317692
186,588,588,1176,0.284534215927124,7.638968283079407
187,592,592,1184,0.2861809730529785,7.63701218152994
188,594,594,1188,0.28722596168518066,7.353176989130134
189,598,598,1196,0.28884100914001465,7.325656119624114
190,600,600,1200,0.289870023727417,7.107522423550449
191,604,604,1208,0.29145002365112305,7.079946429809297
192,608,608,1216,0.29299306869506836,7.035260657666413
193,612,612,1224,0.2945291996002197,6.951647145329503
194,614,614,1228,0.2955000400543213,6.525980611676346
195,618,618,1236,0.2970290184020996,6.523306809489782
196,620,620,1240,0.2981741428375244,6.498802229173634
197,624,624,1248,0.2998340129852295,6.469163069517094
198,628,628,1256,0.3015110492706299,6.40372465905466
199,630,630,1260,0.3026089668273926,6.186357278876812
200,634,634,1268,0.3043348789215088,6.184725097541332
201,638,638,1276,0.306016206741333,6.185192167299647
202,642,642,1284,0.3077688217163086,6.187958140872411
203,644,644,1288,0.30895304679870605,6.1556371626192
204,648,648,1296,0.3106980323791504,6.154659520064456
205,652,652,1304,0.3122990131378174,6.122803056083626
206,656,656,1312,0.3139619827270508,6.086306495836766
207,660,660,1320,0.315748929977417,6.053306006324647
208,664,664,1328,0.31756019592285156,6.025096303950022
209,666,666,1332,0.31868410110473633,5.798054297496378
210,670,670,1340,0.3203890323638916,5.797900965092822
211,672,672,1344,0.3214550018310547,5.602075518953484
212,676,676,1352,0.3231229782104492,5.57997056848501
213,680,680,1360,0.32476186752319336,5.538105909563342
214,682,682,1364,0.32584500312805176,5.3108229842841865
215,686,686,1372,0.32756996154785156,5.306829539099567
216,688,688,1376,0.3286271095275879,4.991279274022531
217,692,692,1384,0.3301961421966553,4.990579558520039
218,694,694,1388,0.33126091957092285,4.717796943624194
219,698,698,1396,0.3329010009765625,4.713725845544218
220,700,700,1400,0.33397889137268066,4.322210476406326
221,704,704,1408,0.33563804626464844,4.319442490166352
222,706,706,1412,0.3367161750793457,3.9093038090592245
223,710,710,1420,0.3384690284729004,3.9085605554630547
224,712,712,1424,0.3396000862121582,3.3354202805128352
225,716,716,1432,0.341292142868042,3.331588269776944
226,718,718,1436,0.3423490524291992,3.278931829186945
227,722,722,1444,0.3440840244293213,3.28295372409184
228,724,724,1448,0.3451499938964844,3.2680930311757947
229,728,728,1456,0.34676218032836914,3.2653658951552416
230,730,730,1460,0.34785914421081543,3.1596591317619414
231,734,734,1468,0.34949421882629395,3.1459867146380702
232,736,736,1472,0.35057711601257324,2.4502152909810775
233,740,740,1480,0.352154016494751,2.4552495830514545
234,746,746,1492,0.35443687438964844,2.456700108505629
235,748,748,1496,0.3555269241333008,2.019811086411096
236,752,752,1504,0.35715699195861816,2.0057954623284786
237,756,756,1512,0.35881924629211426,2.009358050776882
238,760,760,1520,0.3604700565338135,2.036791336063061
239,762,762,1524,0.36158013343811035,1.8439571018624292
240,766,766,1532,0.3632171154022217,1.8630425920786138
241,768,768,1536,0.36428308486938477,1.827822798031434
242,772,772,1544,0.366199254989624,1.8250014728048427
243,774,774,1548,0.36765027046203613,1.6477378561447722
244,778,778,1556,0.36964893341064453,1.6118088731888065
245,782,782,1564,0.3714790344238281,1.5812240359842917
246,784,784,1568,0.3726348876953125,1.290214586696834
247,788,788,1576,0.3745460510253906,1.2914685086590225
248,790,790,1580,0.37578415870666504,1.0163974565576837
249,794,794,1588,0.3776381015777588,1.017424727608386
250,796,796,1592,0.3787689208984375,0.7479697458059036
251,800,800,1600,0.3807680606842041,0.7096804343055965
252,804,804,1608,0.38249921798706055,0.6929855648535295
253,806,806,1612,0.38369011878967285,0.5517213756771753
254,810,810,1620,0.38541507720947266,0.5575003055440675
255,812,812,1624,0.38651204109191895,0.5673350545134781
256,816,816,1632,0.38815999031066895,0.5829821477813084
257,820,820,1640,0.38983726501464844,0.5492117036698119
258,822,822,1644,0.3909640312194824,0.5674136864449792
259,824,824,1648,0.3920910358428955,0.6022248134764823
260,828,828,1656,0.3937849998474121,0.6022857185520252
261,830,830,1660,0.39485597610473633,0.6029297948713292
262,834,834,1668,0.39661192893981934,0.6042666790599469
263,836,836,1672,0.3977930545806885,0.6037096523263017
264,840,840,1680,0.3994791507720947,0.6014428256117981
265,842,842,1684,0.4004960060119629,0.4955061188460377
266,846,846,1692,0.4021289348602295,0.49578811805201894
267,848,848,1696,0.4031980037689209,0.44338681278406966
268,852,852,1704,0.4050140380859375,0.4428736433408176
269,854,854,1708,0.40606021881103516,0.4044965840674877
270,858,858,1716,0.40769314765930176,0.40525008389533923
271,860,860,1720,0.40874814987182617,0.3835060524143046
272,864,864,1728,0.4104001522064209,0.3832871030462002
273,866,866,1732,0.4114861488342285,0.3740392699842232
274,870,870,1740,0.41320204734802246,0.37565488012990045
275,872,872,1744,0.41434407234191895,0.37932126942143896
276,874,874,1748,0.4154829978942871,0.37356102010255654
277,878,878,1756,0.41716504096984863,0.3732297696498108
278,880,880,1760,0.41829609870910645,0.33418124959405304
279,884,884,1768,0.42021703720092773,0.3327602733977528
280,886,886,1772,0.421550989151001,0.2798861456830082
281,890,890,1780,0.4233999252319336,0.2795847396685076
282,892,892,1784,0.42461705207824707,0.23199679874130652
283,896,896,1792,0.4265151023864746,0.23207750620747447
284,898,898,1796,0.42762207984924316,0.212408526532613
285,900,900,1800,0.4286980628967285,0.19286934914362064
286,902,902,1804,0.4297139644622803,0.17449745533690475
287,906,906,1812,0.4313790798187256,0.17456751069198617
288,908,908,1816,0.43244409561157227,0.16215965463322846
289,912,912,1824,0.434124231338501,0.1613955835964589
290,914,914,1828,0.43523216247558594,0.1493501761636935
291,918,918,1836,0.43691515922546387,0.1493805642537609
292,920,920,1840,0.43801212310791016,0.11171676347350967
293,924,924,1848,0.4397621154785156,0.1115529805516644
294,926,926,1852,0.4408590793609619,0.08162637693294528
295,928,928,1856,0.4418818950653076,0.0828565976568143
296,930,930,1860,0.44298291206359863,0.07206259370286716
297,934,934,1868,0.4447000026702881,0.07234785134426147
298,936,936,1872,0.44577693939208984,0.06168422863106571
299,940,940,1880,0.44738101959228516,0.06189443671325989
300,942,942,1884,0.4484832286834717,0.046178134508977564
301,946,946,1892,0.45012593269348145,0.04596172622905215
302,948,948,1896,0.4511990547180176,0.029541864734937917
303,952,952,1904,0.45286011695861816,0.029724443279405932
304,954,954,1908,0.4538919925689697,0.022532327907015315
305,958,958,1916,0.4556281566619873,0.022917943325410306
306,960,960,1920,0.4567420482635498,0.01926410588453109
307,964,964,1928,0.4583902359008789,0.01922022466942508
308,966,966,1932,0.4593989849090576,0.02156623313055661
309,970,970,1940,0.46103811264038086,0.02171415449288361
310,972,972,1944,0.4621269702911377,0.021410740155829444
311,976,976,1952,0.4639921188354492,0.021355873551556215
312,978,978,1956,0.46503710746765137,0.01983446218412155
313,982,982,1964,0.4667999744415283,0.019561435280706974
314,984,984,1968,0.46788525581359863,0.019240220238316397
315,988,988,1976,0.4695320129394531,0.019248891018833092
316,990,990,1980,0.4706110954284668,0.01825672119673527
317,994,994,1988,0.472182035446167,0.018251538474714835
318,996,996,1992,0.4732060432434082,0.01700770229376758
319,1000,1000,2000,0.47484707832336426,0.017006194679538567
320,1002,1002,2004,0.47594714164733887,0.01603262340756828
321,1006,1006,2012,0.47768306732177734,0.016032147362807336
322,1008,1008,2016,0.47876524925231934,0.01609032041108094
323,1012,1012,2024,0.48046302795410156,0.016117452411776867
324,1016,1016,2032,0.48215198516845703,0.016087364900272405
325,1018,1018,2036,0.48318004608154297,0.014296818934099065
326,1022,1022,2044,0.48485684394836426,0.014248860139446151
327,1024,1024,2048,0.48597097396850586,0.011040098057833347
328,1028,1028,2056,0.4875972270965576,0.01100542209167088
329,1030,1030,2060,0.48862218856811523,0.010542782407355844
330,1034,1034,2068,0.4902510643005371,0.010517195022430315
331,1036,1036,2072,0.4913311004638672,0.009299755029132939
332,1040,1040,2080,0.49298691749572754,0.009304263468493446
333,1042,1042,2084,0.493988037109375,0.009127783435928905
334,1046,1046,2092,0.4957289695739746,0.009081414456659331
335,1048,1048,2096,0.49688100814819336,0.00798224164691419
336,1052,1052,2104,0.4985480308532715,0.007938130389902653
337,1054,1054,2108,0.49959707260131836,0.0069563307821454146
338,1058,1058,2116,0.5011940002441406,0.006970629959710095
339,1060,1060,2120,0.5023181438446045,0.005672720931443109
340,1064,1064,2128,0.503960132598877,0.005666005518264683
341,1066,1066,2132,0.5051670074462891,0.004778024959932736
342,1070,1070,2140,0.5068199634552002,0.004720877503245902
343,1072,1072,2144,0.5080950260162354,0.003940335587685695
344,1076,1076,2152,0.5101230144500732,0.003920145292909183
345,1078,1078,2156,0.5113842487335205,0.003252791416571199
346,1082,1082,2164,0.5131778717041016,0.0032066053751123036
347,1084,1084,2168,0.5142779350280762,0.002060805143514699
348,1086,1086,2172,0.5153930187225342,0.0020762528387194834
349,1090,1090,2180,0.5170350074768066,0.002074150917565021
350,1092,1092,2184,0.5180270671844482,0.0016353320189637088
351,1096,1096,2192,0.5196502208709717,0.0016411882188549498
352,1098,1098,2196,0.5207481384277344,0.00140246701482738
353,1102,1102,2204,0.5225000381469727,0.0014011639553928035
354,1104,1104,2208,0.5235171318054199,0.0012840434646932408
355,1108,1108,2216,0.5252339839935303,0.0012698938805897342
356,1110,1110,2220,0.5263490676879883,0.0009335636337937103
357,1114,1114,2228,0.5281879901885986,0.000926087654534058
358,1116,1116,2232,0.5295040607452393,0.0004949704189129989
359,1120,1120,2240,0.5314939022064209,0.000491747709588708
360,1122,1122,2244,0.5329632759094238,0.00031222802385855175
361,1124,1124,2248,0.534217119216919,0.00029867265118355135
362,1126,1126,2252,0.5354142189025879,0.0002910417830435108
363,1128,1128,2256,0.5369000434875488,0.00031855913027811766
364,1130,1130,2260,0.5382061004638672,0.0003182371951879759
365,1134,1134,2268,0.5401911735534668,0.00031528889780929603
366,1136,1136,2272,0.5418350696563721,0.0002161586321562936
367,1140,1140,2280,0.5437378883361816,0.00021501508001620095
368,1142,1142,2284,0.5450069904327393,0.0001950005012076872
369,1146,1146,2292,0.5469472408294678,0.0001972571157011771
370,1148,1148,2296,0.5480620861053467,0.000199267083075938
371,1150,1150,2300,0.5490992069244385,0.00018486439364551188
372,1154,1154,2308,0.5509111881256104,0.0001845257603463324
373,1156,1156,2312,0.5522620677947998,0.00013986493524953403
374,1160,1160,2320,0.5544211864471436,0.0001391813964346511
375,1162,1162,2324,0.5560588836669922,0.0001190870791560883
376,1166,1166,2332,0.5577659606933594,0.00011815179539098608
377,1168,1168,2336,0.5588181018829346,0.00011121725003704341
378,1172,1172,2344,0.5604500770568848,0.00011156364223552373
379,1174,1174,2348,0.5617170333862305,0.00012034744838729239
380,1176,1176,2352,0.5630228519439697,0.00010178264938076609
381,1180,1180,2360,0.564716100692749,0.00010160878730403056
382,1182,1182,2364,0.5658929347991943,9.410487052718963e-05
383,1186,1186,2372,0.5676529407501221,9.411341716258903e-05
384,1188,1188,2376,0.5689601898193359,9.531269802209863e-05
385,1192,1192,2384,0.570742130279541,9.569605526849045e-05
386,1194,1194,2388,0.5719940662384033,0.00010350215222842962
387,1198,1198,2396,0.574038028717041,0.00010379710988672741
388,1200,1200,2400,0.5753281116485596,0.00011244544703004067
389,1204,1204,2408,0.5769801139831543,0.00011235226213557326
390,1206,1206,2412,0.5780930519104004,0.00010487260578884161
391,1210,1210,2420,0.5799980163574219,0.00010473333077243296
392,1214,1214,2428,0.5819389820098877,0.00010448377804550546
393,1216,1216,2432,0.5832860469818115,9.642943803100934e-05
394,1220,1220,2440,0.5850310325622559,9.66584063917253e-05
395,1222,1222,2444,0.5861730575561523,0.00010222293019523931
396,1226,1226,2452,0.5880279541015625,0.00010229895690372359
397,1228,1228,2456,0.5893731117248535,9.712099961234344e-05
398,1232,1232,2464,0.5913209915161133,9.709247365208284e-05
399,1234,1234,2468,0.5924282073974609,9.497492396803864e-05
400,1238,1238,2476,0.594202995300293,9.486244243817055e-05
401,1240,1240,2480,0.5955290794372559,9.316556213434524e-05
402,1244,1244,2488,0.5974302291870117,9.266903987281694e-05
403,1248,1248,2496,0.5991501808166504,9.192468712626578e-05
404,1250,1250,2500,0.6002869606018066,9.049078994394222e-05
405,1254,1254,2508,0.6019301414489746,9.051392487435805e-05
406,1256,1256,2512,0.6029400825500488,8.872369699020055e-05
407,1260,1260,2520,0.6046061515808105,8.868292786701204e-05
408,1262,1262,2524,0.6058609485626221,8.379445591799595e-05
409,1266,1266,2532,0.6078019142150879,8.372608749596111e-05
410,1268,1268,2536,0.6089141368865967,7.62700962013696e-05
411,1272,1272,2544,0.6106178760528564,7.620928124651982e-05
412,1274,1274,2548,0.6120378971099854,7.241388300371909e-05
413,1278,1278,2556,0.6138520240783691,7.240144964271167e-05
414,1280,1280,2560,0.6149570941925049,7.100073287347186e-05
415,1284,1284,2568,0.6166191101074219,7.137628438158572e-05
416,1288,1288,2576,0.6182689666748047,7.163369082263671e-05
417,1290,1290,2580,0.6193511486053467,7.038043213469791e-05
418,1294,1294,2588,0.6210000514984131,7.021803298812301e-05
419,1296,1296,2592,0.6220402717590332,7.00948013445668e-05
420,1300,1300,2600,0.623967170715332,7.00070338552905e-05
421,1302,1302,2604,0.625208854675293,6.884790320782486e-05
422,1306,1306,2612,0.6268520355224609,6.88379196844835e-05
423,1308,1308,2616,0.6279261112213135,6.5211362766604e-05
424,1312,1312,2624,0.6298189163208008,6.52715557407646e-05
425,1316,1316,2632,0.6315310001373291,6.547877808316116e-05
426,1318,1318,2636,0.6326169967651367,6.465522938015056e-05
427,1322,1322,2644,0.6342780590057373,6.46174287339818e-05
428,1324,1324,2648,0.6353280544281006,6.121993772012502e-05
429,1328,1328,2656,0.6369650363922119,6.111951825005235e-05
430,1330,1330,2660,0.6380281448364258,5.8583519262356276e-05
431,1334,1334,2668,0.6399250030517578,5.861908255155868e-05
432,1336,1336,2672,0.6413111686706543,5.739698303841578e-05
433,1340,1340,2680,0.643090009689331,5.7299880950267834e-05
434,1344,1344,2688,0.645205020904541,5.7125263765556156e-05
435,1346,1346,2692,0.6463680267333984,5.182343738852069e-05
436,1350,1350,2700,0.6482410430908203,5.1692963779714773e-05
437,1354,1354,2708,0.6501390933990479,5.1158379278604116e-05
438,1356,1356,2712,0.6514651775360107,4.739037046874728e-05
439,1360,1360,2720,0.6532449722290039,4.7183627202684875e-05
440,1364,1364,2728,0.6551141738891602,4.692515426540922e-05
441,1366,1366,2732,0.6564948558807373,4.4366618340063724e-05
442,1370,1370,2740,0.6582961082458496,4.4450283326114004e-05
443,1374,1374,2748,0.6599140167236328,4.4482193516159896e-05
444,1378,1378,2756,0.6618850231170654,4.4373274249664973e-05
445,1380,1380,2760,0.6631810665130615,4.067750273861748e-05
446,1384,1384,2768,0.6649959087371826,4.064291078975657e-05
447,1386,1386,2772,0.6662640571594238,3.774675224121893e-05
448,1388,1388,2776,0.6674580574035645,3.451606323778833e-05
449,1392,1392,2784,0.6693031787872314,3.4462799817447376e-05
450,1394,1394,2788,0.6706631183624268,2.8432274007172964e-05
451,1398,1398,2796,0.6724529266357422,2.838170598806755e-05
452,1400,1400,2800,0.6737251281738281,2.7917560487367155e-05
453,1404,1404,2808,0.67557692527771,2.799368962769222e-05
454,1406,1406,2812,0.6767439842224121,2.7524226993591583e-05
455,1410,1410,2820,0.6786360740661621,2.7576465640777315e-05
456,1414,1414,2828,0.6804540157318115,2.7570889642447582e-05
457,1416,1416,2832,0.6815590858459473,2.137369745014439e-05
458,1420,1420,2840,0.6833171844482422,2.1337815496735857e-05
459,1422,1422,2844,0.6843559741973877,1.9828219365081168e-05
460,1426,1426,2852,0.6860392093658447,1.9811542529168946e-05
461,1428,1428,2856,0.6871230602264404,2.0101483414691756e-05
462,1432,1432,2864,0.6890289783477783,2.0151911940047285e-05
463,1434,1434,2868,0.6902720928192139,1.994448155073769e-05
464,1438,1438,2876,0.6919710636138916,1.9983800029876875e-05
465,1440,1440,2880,0.6930551528930664,2.100303765928402e-05
466,1444,1444,2888,0.6950259208679199,2.0954252022420405e-05
467,1446,1446,2892,0.6963710784912109,1.8538703102422005e-05
468,1448,1448,2896,0.6974532604217529,1.4263347679843719e-05
469,1452,1452,2904,0.6992552280426025,1.4224318533706537e-05
470,1454,1454,2908,0.7003872394561768,8.322856956510805e-06
471,1458,1458,2916,0.7020831108093262,8.240959800787095e-06
472,1460,1460,2920,0.7031009197235107,4.159401441938826e-06
473,1462,1462,2924,0.7042140960693359,3.996809368800314e-06
474,1466,1466,2932,0.7061760425567627,3.9991510902837035e-06
475,1468,1468,2936,0.7074599266052246,2.073418500003754e-06
476,1472,1472,2944,0.7091710567474365,2.03850606794731e-06
477,1474,1474,2948,0.710219144821167,6.880076171000837e-07
478,1478,1478,2956,0.7122058868408203,6.513462267321302e-07
479,1480,1480,2960,0.7135241031646729,3.070175580432988e-07
480,1482,1482,2964,0.7145822048187256,9.288919500249904e-08
481,1486,1486,2972,0.7162730693817139,8.245660865213722e-08
482,1488,1488,2976,0.7173662185668945,2.145142161680269e-09


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.005098819732666016,7527.1682254052175
1001,2004,1002,3006,3.6467480659484863,16.497806269995635
2002,4006,2003,6009,7.238240957260132,8.493645480455598
3003,6008,3004,9012,10.868703842163086,5.458411064455504
4004,8010,4005,12015,14.944911003112793,4.0183071345327335
5005,10012,5006,15018,18.747506141662598,3.22679212312687
6006,12014,6007,18021,23.342329025268555,2.7412246159965434
7007,14016,7008,21024,28.049583911895752,2.4010585392661596
8008,16018,8009,24027,32.46620798110962,2.1473435429415986
9009,18020,9010,27030,36.59423875808716,1.9510757904063212
10010,20022,10011,30033,40.99786901473999,1.7860873272093158
11011,22024,11012,33036,44.91871500015259,1.6496502359241276
12012,24026,12013,36039,48.269286155700684,1.5356632292659924
13013,26028,13014,39042,53.206477880477905,1.4379722296016553
14014,28030,14015,42045,58.65890097618103,1.3520213924985
15015,30032,15016,45048,63.3932728767395,1.2742289145662653
16016,32034,16017,48051,66.61575698852539,1.207127379722806
17017,34036,17018,51054,70.00086998939514,1.146283669553668
18018,36038,18019,54057,74.22565603256226,1.0918120883015945
19019,38040,19020,57060,78.23007702827454,1.0424478336863103
20020,40042,20021,60063,81.88735604286194,0.9969560017580079
21021,42044,21022,63066,85.60669207572937,0.9558615275109332
22022,44046,22023,66069,89.36515092849731,0.9176484019026248
23023,46048,23024,69072,92.91565299034119,0.8819220992099872
24024,48050,24025,72075,96.25085091590881,0.8492827874051727
25025,50052,25026,75078,99.81518411636353,0.8197084285638994
26026,52054,26027,78081,103.37525296211243,0.7915118778582837
27027,54056,27028,81084,106.68792700767517,0.7649407176704699
28028,56058,28029,84087,109.89806199073792,0.7406526523391221
29029,58060,29030,87090,113.24599385261536,0.717516735978279
30030,60062,30031,90093,116.53232097625732,0.6960358251853904
31031,62064,31032,93096,119.81329298019409,0.6761034219180146
32032,64066,32033,96099,123.53746390342712,0.6566625917566853
33033,66068,33034,99102,127.02709794044495,0.6385920771299425
34034,68070,34035,102105,130.5686318874359,0.6213090652981919
35035,70072,35036,105108,133.9097719192505,0.6054368420846004
36036,72074,36037,108111,137.51473593711853,0.5899539575129893
37037,74076,37038,111114,140.93576383590698,0.575850874904063
38038,76078,38039,114117,144.5266411304474,0.5620418065409467
39039,78080,39040,117120,148.02537393569946,0.5489631221644231
40040,80082,40041,120123,151.34961700439453,0.5365798114016798
41041,82084,41042,123126,154.6927888393402,0.5247631347301649
42042,84086,42043,126129,158.01648998260498,0.5134134385461948
43043,86088,43044,129132,161.33764791488647,0.5022046245594538
44044,88090,44045,132135,164.70172691345215,0.4917957345551258
45045,90092,45046,135138,168.0752658843994,0.48152754926195485
46046,92094,46047,138141,173.13305377960205,0.47210523306603136
47047,94096,47048,141144,177.7668809890747,0.4630634162167553
48048,96098,48049,144147,182.45351481437683,0.45412089460296556
49049,98100,49050,147150,186.21646690368652,0.44561378928301565
50050,100102,50051,150153,189.73361086845398,0.43731890040362487
51051,102104,51052,153156,193.15243697166443,0.42939628356361936
52052,104106,52053,156159,196.5193920135498,0.421768821477599
53053,106108,53054,159162,199.83905696868896,0.41448086035052256
54054,108110,54055,162165,203.1999819278717,0.407511265570065
55055,110112,55056,165168,206.60861778259277,0.4005870653199963
56056,112114,56057,168171,209.92689394950867,0.393895394881838
57057,114116,57058,171174,213.25325894355774,0.38750695320595696
58058,116118,58059,174177,216.53420686721802,0.3814584564534016
59059,118120,59060,177180,219.7956600189209,0.3754735273141705
60060,120122,60061,180183,223.07716703414917,0.36974671455391217
61061,122124,61062,183186,226.45909190177917,0.36410737318692554
62062,124126,62063,186189,229.7380998134613,0.3586352511738369
63063,126128,63064,189192,233.04684901237488,0.3533858682058053
64064,128130,64065,192195,236.37164998054504,0.3483475837238075
65065,130132,65066,195198,239.5901539325714,0.34344225045606436
66066,132134,66067,198201,242.8056890964508,0.33863474435929675
67067,134136,67068,201204,246.01495790481567,0.3339623388565087
68068,136138,68069,204207,249.1772849559784,0.32942746442495263
69069,138140,69070,207210,252.3767011165619,0.32502469818791724
70070,140142,70071,210213,255.62268090248108,0.3207800291311287
71071,142144,71072,213216,258.807904958725,0.316658925908996
72072,144146,72073,216219,262.03289580345154,0.3124673175279895
73073,146148,73074,219222,265.2709319591522,0.30851173182782077
74074,148150,74075,222225,268.52366304397583,0.30464353173738346
75075,150152,75076,225228,271.7283990383148,0.3008890543515008
76076,152154,76077,228231,274.9656958580017,0.2972730325109296
77077,154156,77078,231234,278.1803369522095,0.29374264490434143
78078,156158,78079,234237,281.3559069633484,0.29019346320274053
79079,158160,79080,237240,284.6501941680908,0.28683214347802277
80080,160162,80081,240243,287.94939494132996,0.2835663693567767
81081,162164,81082,243246,291.13415002822876,0.28031315655607614
82082,164166,82083,246249,294.4020938873291,0.27707980180275626
83083,166168,83084,249252,297.5976128578186,0.27401483678659133
84084,168170,84085,252255,300.8032109737396,0.2710367277104524
85085,170172,85086,255258,303.970458984375,0.2680502941548184
86086,172174,86087,258261,307.20662808418274,0.2651336481958424
87087,174176,87088,261264,310.3590729236603,0.2623141853382549
88088,176178,88089,264267,313.5144839286804,0.2595501636806148
89089,178180,89090,267270,316.732253074646,0.2567464036401361
90090,180182,90091,270273,319.8972489833832,0.25406428346104803
91091,182184,91092,273276,323.1377079486847,0.2515219147080643
92092,184186,92093,276279,326.31721782684326,0.24902016379746783
93093,186188,93094,279282,329.65363097190857,0.24649716358726437
94094,188190,94095,282285,332.83149695396423,0.2439996516022802
95095,190192,95096,285288,336.0214488506317,0.24160324150398083
96096,192194,96097,288291,339.24643182754517,0.2392263167312194
97097,194196,97098,291294,342.4238488674164,0.23690407795038482
98098,196198,98099,294297,345.6061179637909,0.23467143730340467
99099,198200,99100,297300,348.8476028442383,0.23250848719362693
100100,200202,100101,300303,352.0409257411957,0.23028648278705077
101101,202204,101102,303306,355.26041316986084,0.228118407081638
102102,204206,102103,306309,358.4614100456238,0.2260358890016505
103103,206208,103104,309312,361.63514375686646,0.22399632231827127
104104,208210,104105,312315,364.84763407707214,0.2220149036620569
105105,210212,105106,315318,368.0416350364685,0.2200313745524909
106106,212214,106107,318321,371.2205328941345,0.21806712200850598
107107,214216,107108,321324,374.39325618743896,0.21616051192722807
108108,216218,108109,324327,377.6301329135895,0.21432161974189512
109109,218220,109110,327330,380.8391079902649,0.2125081885878899
110110,220222,110111,330333,384.05106806755066,0.2106970793720393
111111,222224,111112,333336,387.2442989349365,0.20893583075303468
112112,224226,112113,336339,390.4198808670044,0.20717976369996904
113113,226228,113114,339342,393.59871888160706,0.20549386142738513
114114,228230,114115,342345,396.78173089027405,0.2037603152293741
115115,230232,115116,345348,399.9455761909485,0.20212424049896072
116116,232234,116117,348351,403.13218092918396,0.20051385473016126
117117,234236,117118,351354,406.2981858253479,0.19894357516204764
118118,236238,118119,354357,409.52019596099854,0.19739563831899432
119119,238240,119120,357360,412.72762989997864,0.1958393422428344
120120,240242,120121,360363,415.89733600616455,0.1943071466866968
121121,242244,121122,363366,419.08821392059326,0.19279230246502266
122122,244246,122123,366369,422.25520610809326,0.19132446379262547
123123,246248,123124,369372,425.449257850647,0.1898995523715712
124124,248250,124125,372375,428.66551208496094,0.188462773552601
125125,250252,125126,375378,432.10064816474915,0.18705085916735698
126126,252254,126127,378381,435.4713649749756,0.18567268950937432
127127,254256,127128,381384,438.6673460006714,0.18433589931919414
128128,256258,128129,384387,441.8621621131897,0.18301034322576015
129129,258260,129130,387390,445.09716296195984,0.18167717431424535
130130,260262,130131,390393,448.28959703445435,0.18036237830892787
131131,262264,131132,393396,451.45953607559204,0.17907697554619517
132132,264266,132133,396399,454.70990204811096,0.1778225380294316
133133,266268,133134,399402,457.87704491615295,0.17658395933904103
134134,268270,134135,402405,461.1218979358673,0.17533394904421584
135135,270272,135136,405408,464.3357059955597,0.17413790986938693
136136,272274,136137,408411,467.4982359409332,0.17296563084528316
137137,274276,137138,411414,470.6668930053711,0.1718038296457962
138138,276278,138139,414417,473.841117143631,0.1706309357268765
139139,278280,139140,417420,477.0297088623047,0.1694840832387854
140140,280282,140141,420423,480.2375011444092,0.1683483669967245
141141,282284,141142,423426,483.41571283340454,0.1672327166688774
142142,284286,142143,426429,486.5437159538269,0.16613368243270088
143143,286288,143144,429432,489.69209384918213,0.16504226253346133
144144,288290,144145,432435,492.86531591415405,0.16398136337556934
145145,290292,145146,435438,496.05629992485046,0.16290896101418184
146146,292294,146147,438441,499.18534803390503,0.1618791703003808
147147,294296,147148,441444,502.3563549518585,0.1608572646655375
148148,296298,148149,444447,505.52002811431885,0.1598246188932535
149149,298300,149150,447450,508.7181248664856,0.1588046500182827
150150,300302,150151,450453,511.9009430408478,0.15781925526425766
151151,302304,151152,453456,515.1044819355011,0.15684078941740154
152152,304306,152153,456459,518.29065990448,0.15585675163492851
153153,306308,153154,459462,521.5037169456482,0.15492164332681568
154154,308310,154155,462465,524.6643087863922,0.15399009380962525
155155,310312,155156,465468,527.8446090221405,0.1530835003213724
156156,312314,156157,468471,531.0353388786316,0.1521651426119206
157157,314316,157158,471474,534.2558360099792,0.15124965226459608
158158,316318,158159,474477,537.4476919174194,0.15034279609426449
159159,318320,159160,477480,540.630481004715,0.14945472571707796
160160,320322,160161,480483,543.8682630062103,0.14857372365440824
161161,322324,161162,483486,547.2040810585022,0.14770831501300563
162162,324326,162163,486489,550.6126449108124,0.14685379122238373
163163,326328,163164,489492,554.0195429325104,0.1460215353017702
164164,328330,164165,492495,557.4643218517303,0.14519077583099715
165165,330332,165166,495498,560.8990938663483,0.14436370925795927
166166,332334,166167,498501,564.3367741107941,0.1435555053049029
167167,334336,167168,501504,567.77610206604,0.1427298386588518
168168,336338,168169,504507,571.1640181541443,0.14196044045274903
169169,338340,169170,507510,574.4781329631805,0.1411670707675512
170170,340342,170171,510513,577.6874988079071,0.14038354423792043
171171,342344,171172,513516,580.7995729446411,0.13961192019451119
172172,344346,172173,516519,583.9452850818634,0.13885429314905195
173173,346348,173174,519522,587.06369805336,0.13811171433189884
174174,348350,174175,522525,590.2492949962616,0.13735427009305567
175175,350352,175176,525528,593.428386926651,0.13662850934088056
176176,352354,176177,528531,596.5940027236938,0.13591056288714753
177177,354356,177178,531534,599.7376408576965,0.1351865487813484
178178,356358,178179,534537,602.8921618461609,0.13447545955204987
179179,358360,179180,537540,606.035441160202,0.1337655631123198
180180,360362,180181,540543,609.2303321361542,0.13307280397384602
181181,362364,181182,543546,612.4699728488922,0.13238329144041927
182182,364366,182183,546549,615.6785697937012,0.13170566990811494
183183,366368,183184,549552,618.8857898712158,0.1310416895776143
184184,368370,184185,552555,622.0636730194092,0.13036930579801265
185185,370372,185186,555558,625.2788639068604,0.12971068968545296
186186,372374,186187,558561,628.4346311092377,0.12905034065079235
187187,374376,187188,561564,631.6070199012756,0.12841976679374056
188188,376378,188189,564567,634.7437138557434,0.12779184837381763
189189,378380,189190,567570,637.8933091163635,0.1271694866427424
190190,380382,190191,570573,641.0608038902283,0.12654655516234925
191191,382384,191192,573576,644.237566947937,0.1259342502344225
192192,384386,192193,576579,647.38201379776,0.12532487717726326
193193,386388,193194,579582,650.531140089035,0.12470222717638535
194194,388390,194195,582585,653.9036450386047,0.12410089484183118
195195,390392,195196,585588,657.0541400909424,0.12350029504887061
196196,392394,196197,588591,660.1912980079651,0.12291293228372524
197197,394396,197198,591594,663.3209798336029,0.12231943448387028
198198,396398,198199,594597,666.4549510478973,0.12175190807647596
199199,398400,199200,597600,669.5998129844666,0.12118687697147834
200200,400402,200201,600603,672.7565670013428,0.12061233546410222
201201,402404,201202,603606,675.9349510669708,0.12004874657577602
202202,404406,202203,606609,679.0705268383026,0.11948765349734458
203203,406408,203204,609612,682.2094571590424,0.11894012164884771
204204,408410,204205,612615,685.3995339870453,0.1183956219592801
205205,410412,205206,615618,688.5217139720917,0.11785534625960281
206206,412414,206207,618621,691.6576619148254,0.11731828563097224
207207,414416,207208,621624,694.7807238101959,0.11678281152489944
208208,416418,208209,624627,697.9185147285461,0.11626146294292994
209209,418420,209210,627630,701.0755279064178,0.11574160594864225
210210,420422,210211,630633,704.2321040630341,0.11523256568943907
211211,422424,211212,633636,707.3968820571899,0.11472187432264036
212212,424426,212213,636639,710.5501358509064,0.11422107158250583
213213,426428,213214,639642,713.7352747917175,0.11371435881119396
214214,428430,214215,642645,716.9237909317017,0.11321671213590889
215215,430432,215216,645648,720.0480799674988,0.11272944273150642
216216,432434,216217,648651,723.1866850852966,0.11224269904414541
217217,434436,217218,651654,726.3152668476105,0.11175924310009577
218218,436438,218219,654657,729.4552800655365,0.1112829644298472
219219,438440,219220,657660,732.5716519355774,0.11081129226113262
220220,440442,220221,660663,735.7539701461792,0.11033430244788178
221221,442444,221222,663666,738.9620459079742,0.10985945648280904
222222,444446,222223,666669,742.1441488265991,0.10939786878043378
223223,446448,223224,669672,745.2741270065308,0.1089359788584261
224224,448450,224225,672675,748.4127910137177,0.10848241558960581
225225,450452,225226,675678,751.5352728366852,0.10803518534703471
226226,452454,226227,678681,754.6787188053131,0.10758411192000494
227227,454456,227228,681684,757.8724939823151,0.10714659151926753
228228,456458,228229,684687,761.0392611026764,0.10669520751616801
229229,458460,229230,687690,764.1762900352478,0.10626105517258111
230230,460462,230231,690693,767.3196640014648,0.10583009994843451
231231,462464,231232,693696,770.4563999176025,0.10540205221695942
232232,464466,232233,696699,773.6540987491608,0.10497622477305413
233233,466468,233234,699702,776.793182849884,0.10454209768977307
234234,468470,234235,702705,779.8808088302612,0.10412440362051711
235235,470472,235236,705708,783.0679867267609,0.10371492617196054
236236,472474,236237,708711,786.3616271018982,0.10330418657758855
237237,474476,237238,711714,789.488972902298,0.10289304848811298
238238,476478,238239,714717,792.5707049369812,0.1024892195546272
239239,478480,239240,717720,795.6998698711395,0.10209433690215519
240240,480482,240241,720723,798.8064379692078,0.1016947977059317
241241,482484,241242,723726,801.9685130119324,0.10128805645217653
242242,484486,242243,726729,805.1658160686493,0.10089610746217659
243243,486488,243244,729732,808.296709060669,0.10050745449370879
244244,488490,244245,732735,811.4073798656464,0.10011470221616037
245245,490492,245246,735738,814.5615110397339,0.09974203425008454
246246,492494,246247,738741,817.9421601295471,0.09935096413573774
247247,494496,247248,741744,821.1507251262665,0.09896969855253701
248248,496498,248249,744747,824.2744839191437,0.09859599244009587
249249,498500,249250,747750,827.4189789295197,0.0982161902320513
250250,500502,250251,750753,830.5472359657288,0.09785341511633305
251251,502504,251252,753756,833.7593369483948,0.09748814200611378
252252,504506,252253,756759,836.9172310829163,0.09709963740533567
253253,506508,253254,759762,840.0551159381866,0.0967417145948275
254254,508510,254255,762765,843.1779289245605,0.09638311707203684
255255,510512,255256,765768,846.334212064743,0.09602736738088424
256256,512514,256257,768771,849.474179983139,0.09567076871462632
257257,514516,257258,771774,852.6718518733978,0.09532250081429083
258258,516518,258259,774777,855.8559300899506,0.09497640523477457
259259,518520,259260,777780,858.9822278022766,0.09463343617062492
260260,520522,260261,780783,862.1382477283478,0.09429415298291133
261261,522524,261262,783786,865.3556168079376,0.09395859171672782
262262,524526,262263,786789,868.5151238441467,0.09361903066383093
263263,526528,263264,789792,871.6857960224152,0.09327822893101256
264264,528530,264265,792795,874.8217258453369,0.09294339048028633
265265,530532,265266,795798,877.9517290592194,0.09261626479928964
266266,532534,266267,798801,881.0879940986633,0.0922886057451251
267267,534536,267268,801804,884.2346091270447,0.0919639932053542
268268,536538,268269,804807,887.4438738822937,0.09163259724482486
269269,538540,269270,807810,890.5758669376373,0.09131221627285413
270270,540542,270271,810813,893.7761240005493,0.09099100371713575
271271,542544,271272,813816,896.9406960010529,0.09067776039228193
272272,544546,272273,816819,900.1109931468964,0.09035981666056614
273273,546548,273274,819822,903.3106389045715,0.09004430209279235
274274,548550,274275,822825,906.4885458946228,0.08973193009478564
275275,550552,275276,825828,909.6213209629059,0.08942181523525505
276276,552554,276277,828831,912.8073999881744,0.08911729145438585
277277,554556,277278,831834,915.9503200054169,0.08881903215115017
278278,556558,278279,834837,919.1320748329163,0.08851720266466145
279279,558560,279280,837840,922.2844667434692,0.08821582500240766
280280,560562,280281,840843,925.4756660461426,0.087919444687941
281281,562564,281282,843846,928.5954778194427,0.08761950703410548
282282,564566,282283,846849,931.8302681446075,0.08732924613650539
283283,566568,283284,849852,935.0987920761108,0.08703904316462285
284284,568570,284285,852855,938.2216219902039,0.08675181585203973
285285,570572,285286,855858,941.385605096817,0.08646448038052768
286286,572574,286287,858861,944.4996740818024,0.08618096503050765
287287,574576,287288,861864,948.0349569320679,0.08590201172228262
288288,576578,288289,864867,952.3668761253357,0.08561937550803123
289289,578580,289290,867870,957.4778048992157,0.08534126657286834
290290,580582,290291,870873,961.3578081130981,0.08506259887872147
291291,582584,291292,873876,964.6262040138245,0.08478989211107546
292292,584586,292293,876879,967.85888504982,0.08451946561035584
293293,586588,293294,879882,971.2927799224854,0.08424756777640141
294294,588590,294295,882885,974.7476987838745,0.08398369482893031
295295,590592,295296,885888,977.9843509197235,0.08370801241107984
296296,592594,296297,888891,981.133003950119,0.08343828658144048
297297,594596,297298,891894,984.3124058246613,0.08317414516386634
298298,596598,298299,894897,987.525074005127,0.08291341662516061
299299,598600,299300,897900,990.6627340316772,0.08265382449098979
300300,600602,300301,900903,993.7990419864655,0.0823981085941341
301301,602604,301302,903906,996.9474239349365,0.08214311643678229
302302,604606,302303,906909,1000.1062309741974,0.08188884889204928
303303,606608,303304,909912,1003.2295730113983,0.08163511414386448
304304,608610,304305,912915,1006.373685836792,0.08138010504808335
305305,610612,305306,915918,1009.4914600849152,0.08112451448869251
306306,612614,306307,918921,1012.7236630916595,0.08087314273325319
307307,614616,307308,921924,1015.8449268341064,0.0806254348535731
308308,616618,308309,924927,1019.0316488742828,0.08038052174197219
309309,618620,309310,927930,1022.1696648597717,0.08014079315034905
310310,620622,310311,930933,1025.32039809227,0.0798958136474539
311311,622624,311312,933936,1028.6442930698395,0.07965374562627403
312312,624626,312313,936939,1031.856763124466,0.07941650450811721
313313,626628,313314,939942,1035.0306799411774,0.07917364170862129
314314,628630,314315,942945,1038.2588820457458,0.07893356873864832
315315,630632,315316,945948,1041.408164024353,0.0786947631095245
316316,632634,316317,948951,1044.5740451812744,0.07845986047323095
317317,634636,317318,951954,1047.7258217334747,0.07822849031981605
318318,636638,318319,954957,1050.8688280582428,0.0779890043540945
319319,638640,319320,957960,1054.0289468765259,0.077759381290889
320320,640642,320321,960963,1057.1611387729645,0.07753257944204961
321321,642644,321322,963966,1060.3174169063568,0.07730391225413769
322322,644646,322323,966969,1063.4688119888306,0.07708046329935314
323323,646648,323324,969972,1066.61727309227,0.07685706888696586
324324,648650,324325,972975,1069.7187161445618,0.07663479043912957
325325,650652,325326,975978,1072.8897609710693,0.07641355826490326
326326,652654,326327,978981,1076.0706589221954,0.07619351641187677
327327,654656,327328,981984,1079.228903055191,0.07597313282894902
328328,656658,328329,984987,1082.3447289466858,0.07575552177695499
329329,658660,329330,987990,1085.5218570232391,0.07554059549511294
330330,660662,330331,990993,1088.660579919815,0.07532256937702186
331331,662664,331332,993996,1091.8191878795624,0.07511143944975629
332332,664666,332333,996999,1094.9780180454254,0.07489736709612771
333333,666668,333334,1000002,1098.1688838005066,0.07468470936328231
334334,668670,334335,1003005,1101.3640060424805,0.07447105111532437
335335,670672,335336,1006008,1104.5445611476898,0.07426070514884486
336336,672674,336337,1009011,1107.6880958080292,0.07404844286611478
337337,674676,337338,1012014,1110.8434658050537,0.07384173696118523
338338,676678,338339,1015017,1114.1088519096375,0.07363414524115797
339339,678680,339340,1018020,1117.3491039276123,0.07343024728106684
340340,680682,340341,1021023,1120.5147659778595,0.07322976654359081
341341,682684,341342,1024026,1123.6640198230743,0.07302279608848039
342342,684686,342343,1027029,1126.8021171092987,0.07282086288978462
343343,686688,343344,1030032,1129.951975107193,0.07262342461581284
344344,688690,344345,1033035,1133.1409430503845,0.07242868881257891
345345,690692,345346,1036038,1136.2924358844757,0.07223064821300795
346346,692694,346347,1039041,1139.4480559825897,0.07203473163099261
347347,694696,347348,1042044,1142.5617518424988,0.07183832311056904
348348,696698,348349,1045047,1145.7275018692017,0.07164758330873156
349349,698700,349350,1048050,1148.8503370285034,0.07145429295269423
350350,700702,350351,1051053,1151.9947879314423,0.0712635462587059
351351,702704,351352,1054056,1155.1176590919495,0.07107359631481813
352352,704706,352353,1057059,1158.3974869251251,0.07088419655701728
353353,706708,353354,1060062,1161.59099984169,0.0706947094622592
354354,708710,354355,1063065,1164.7735409736633,0.07050756635180733
355355,710712,355356,1066068,1167.8992140293121,0.0703207417154772
356356,712714,356357,1069071,1171.0375158786774,0.07013308282694197
357357,714716,357358,1072074,1174.2046599388123,0.06994539621518925
358358,716718,358359,1075077,1177.3646428585052,0.06976274001863203
359359,718720,359360,1078080,1180.4949469566345,0.06958119714181521
360360,720722,360361,1081083,1183.6241948604584,0.06939953422806866
361361,722724,361362,1084086,1186.7589139938354,0.06921925193455536
362362,724726,362363,1087089,1189.892410993576,0.06903808879542339
363363,726728,363364,1090092,1193.0656869411469,0.06886187490272278
364364,728730,364365,1093095,1196.2309129238129,0.06868252303502231
365365,730732,365366,1096098,1199.3492209911346,0.06850604022110929
366366,732734,366367,1099101,1202.5111229419708,0.06833199484026409
367367,734736,367368,1102104,1205.638504743576,0.068157335239448
368368,736738,368369,1105107,1208.7921650409698,0.06798055420767923
369369,738740,369370,1108110,1212.053109884262,0.06780760223591642
370370,740742,370371,1111113,1215.1984629631042,0.0676334252457309
371371,742744,371372,1114116,1218.3798689842224,0.06745809260974056
372372,744746,372373,1117119,1221.523586988449,0.06728626407311822
373373,746748,373374,1120122,1224.6928868293762,0.06711427075242682
374374,748750,374375,1123125,1227.8433787822723,0.06694299407718063
375375,750752,375376,1126128,1231.0147960186005,0.0667714860446722
376376,752754,376377,1129131,1234.1425108909607,0.06660223213839345
377377,754756,377378,1132134,1237.2790579795837,0.06643522535705415
378378,756758,378379,1135137,1240.4251279830933,0.06627135087182978
379379,758760,379380,1138140,1243.6027150154114,0.06610417648153089
380380,760762,380381,1141143,1246.746120929718,0.06594335816225794
381381,762764,381382,1144146,1249.9132409095764,0.06577952658335562
382382,764766,382383,1147149,1253.0877759456635,0.06561648188289837
383383,766768,383384,1150152,1256.2583458423615,0.06545250448471052
384384,768770,384385,1153155,1259.3971219062805,0.06529538741415308
385385,770772,385386,1156158,1262.5495109558105,0.06513237012222817
386386,772774,386387,1159161,1265.7043778896332,0.0649750957127253
387387,774776,387388,1162164,1268.8419868946075,0.06481972266374214
388388,776778,388389,1165167,1271.9635009765625,0.06465900004877767
389389,778780,389390,1168170,1275.1324877738953,0.06450198187485512
390390,780782,390391,1171173,1278.3456780910492,0.0643454819019098
391391,782784,391392,1174176,1281.5098719596863,0.06418672602376319
392392,784786,392393,1177179,1284.6665320396423,0.06403159612455056
393393,786788,393394,1180182,1287.8135669231415,0.06388071266883344
394394,788790,394395,1183185,1290.9587960243225,0.06372715586439881
395395,790792,395396,1186188,1294.0847549438477,0.06357453322561923
396396,792794,396397,1189191,1297.255756855011,0.06342363000658224
397397,794796,397398,1192194,1300.4047219753265,0.06327064707147656
398398,796798,398399,1195197,1303.5434629917145,0.06312170886849344
399399,798800,399400,1198200,1306.6934039592743,0.06297276787518058
400400,800802,400401,1201203,1309.8496308326721,0.06282351444315282
401401,802804,401402,1204206,1313.018019914627,0.06267517084597785
402402,804806,402403,1207209,1316.1373829841614,0.06252440000935167
403403,806808,403404,1210212,1319.2914869785309,0.062379969471294316
404404,808810,404405,1213215,1322.4530851840973,0.062234104161689174
405405,810812,405406,1216218,1325.585079908371,0.06209096334896458
406406,812814,406407,1219221,1328.7728979587555,0.06194253749708878
407407,814816,407408,1222224,1331.8665919303894,0.06179840485492605
408408,816818,408409,1225227,1335.0195748806,0.06165560378212831
409409,818820,409410,1228230,1338.168741941452,0.061514495904702926
410410,820822,410411,1231233,1341.3231389522552,0.06137498021053034
411411,822824,411412,1234236,1344.5648109912872,0.06123610360373277
412412,824826,412413,1237239,1347.7482688426971,0.06109562876918062
413413,826828,413414,1240242,1350.8960118293762,0.06095525485761755
414414,828830,414415,1243245,1354.0299980640411,0.06081667955004377
415415,830832,415416,1246248,1357.2066740989685,0.06067929220807855
416416,832834,416417,1249251,1360.3707330226898,0.06054175743884116
417417,834836,417418,1252254,1363.5078928470612,0.06040306264185347
418418,836838,418419,1255257,1366.6694560050964,0.06026871407630097
419419,838840,419420,1258260,1369.7905468940735,0.060132589233035105
420420,840842,420421,1261263,1372.954931974411,0.05999803644772328
421421,842844,421422,1264266,1376.1227538585663,0.05986405484327406
422422,844846,422423,1267269,1379.2579560279846,0.05972991670569172
423423,846848,423424,1270272,1382.3799679279327,0.059596150245852186
424424,848850,424425,1273275,1385.5554909706116,0.05946374485756678
425425,850852,425426,1276278,1388.7404849529266,0.05933206732515828
426426,852854,426427,1279281,1391.8855049610138,0.05919907424504345
427427,854856,427428,1282284,1395.0169899463654,0.05906868835882051
428428,856858,428429,1285287,1398.2213830947876,0.05893881947486079
429429,858860,429430,1288290,1401.3907208442688,0.0588066089530912
430430,860862,430431,1291293,1404.5791800022125,0.058678364806837635
431431,862864,431432,1294296,1407.767154932022,0.05854971923326957
432432,864866,432433,1297299,1410.9271049499512,0.058421492043635226
433433,866868,433434,1300302,1414.1489069461823,0.058294382941312506
434434,868870,434435,1303305,1417.3319220542908,0.058168406303593656
435435,870872,435436,1306308,1420.4515607357025,0.05804166982488823
436436,872874,436437,1309311,1423.5834748744965,0.05791795457844273
437437,874876,437438,1312314,1426.7358350753784,0.05779200810866314
438438,876878,438439,1315317,1429.844561100006,0.05766726786714571
439439,878880,439440,1318320,1433.0183520317078,0.05754391759910504
440440,880882,440441,1321323,1436.1316289901733,0.05741835710068699
441441,882884,441442,1324326,1439.2818179130554,0.057293671981824446
442442,884886,442443,1327329,1442.4150879383087,0.057172790215190616
443443,886888,443444,1330332,1445.5766909122467,0.05705300022418669
444444,888890,444445,1333335,1448.7415080070496,0.05693163285468472
445445,890892,445446,1336338,1451.9121367931366,0.05681374396044703
446446,892894,446447,1339341,1455.0398120880127,0.05669458049851528
447447,894896,447448,1342344,1458.198961019516,0.056576138915261254
448448,896898,448449,1345347,1461.32870388031,0.056457972974385484
449449,898900,449450,1348350,1464.5179629325867,0.05633830330771161
450450,900902,450451,1351353,1467.6450951099396,0.0562211262404162
451451,902904,451452,1354356,1470.9008359909058,0.056105323768861126
452452,904906,452453,1357359,1474.010354757309,0.05598744606686523
453453,906908,453454,1360362,1477.1540248394012,0.055871996311907424
454454,908910,454455,1363365,1480.300742149353,0.05575627851067111
455455,910912,455456,1366368,1483.421777009964,0.055639961998167564
456456,912914,456457,1369371,1486.5619759559631,0.055526395844935905
457457,914916,457458,1372374,1489.7044169902802,0.055411639623343945
458458,916918,458459,1375377,1492.8452908992767,0.05529790212676744
459459,918920,459460,1378380,1495.9965109825134,0.05518290323743713
460460,920922,460461,1381383,1499.2333381175995,0.05506938186044863
461461,922924,461462,1384386,1502.392716884613,0.05495822140619566
462462,924926,462463,1387389,1505.5476450920105,0.054844704227434704
463463,926928,463464,1390392,1508.7012090682983,0.05473243259257288
464464,928930,464465,1393395,1511.864578962326,0.05462007967435056
465465,930932,465466,1396398,1515.0244450569153,0.054511328489752486
466466,932934,466467,1399401,1518.1916131973267,0.054401612462243065
467467,934936,467468,1402404,1521.3799879550934,0.0542896384067717
468468,936938,468469,1405407,1524.5458080768585,0.05418094660853967
469469,938940,469470,1408410,1527.676080942154,0.054072229790108395
470470,940942,470471,1411413,1530.8868429660797,0.05396303886118403
471471,942944,471472,1414416,1534.0368402004242,0.053853469020396005
472472,944946,472473,1417419,1537.194760799408,0.053747301191833685
473473,946948,473474,1420422,1540.361130952835,0.053639915444364306
474474,948950,474475,1423425,1543.5116708278656,0.053533352469457895
475475,950952,475476,1426428,1546.630312204361,0.05342485800247232
476476,952954,476477,1429431,1549.8271751403809,0.05332076743616199
477477,954956,477478,1432434,1553.329232931137,0.053215817744785454
478478,956958,478479,1435437,1556.5475628376007,0.05310885204016813
479479,958960,479480,1438440,1559.668445110321,0.05300600652844878
480480,960962,480481,1441443,1562.8337488174438,0.052900794871675316
481481,962964,481482,1444446,1566.0634150505066,0.05279814907044056
482482,964966,482483,1447449,1569.2521698474884,0.05269305521687784
483483,966968,483484,1450452,1572.4843838214874,0.05259018527249282
484484,968970,484485,1453455,1575.718924999237,0.05248831227982009
485485,970972,485486,1456458,1578.9396629333496,0.052386169705641805
486486,972974,486487,1459461,1582.0803740024567,0.052283488354078145
487487,974976,487488,1462464,1585.2690658569336,0.052181147098963265
488488,976978,488489,1465467,1588.5091669559479,0.05207966296984523
489489,978980,489490,1468470,1591.748496055603,0.051980278207338415
490490,980982,490491,1471473,1594.8946959972382,0.051877976351534016
491491,982984,491492,1474476,1598.0711369514465,0.0517795587056753
492492,984986,492493,1477479,1601.2313709259033,0.05167965121290763
493493,986988,493494,1480482,1604.4182629585266,0.05158046599171939
494494,988990,494495,1483485,1607.6814849376678,0.05148222935349622
495495,990992,495496,1486488,1610.8185770511627,0.05138407037702564
496496,992994,496497,1489491,1613.998888015747,0.05128688516197144
497497,994996,497498,1492494,1617.1515748500824,0.05118980230508896
498498,996998,498499,1495497,1620.2715528011322,0.05109390031793737
499499,999000,499500,1498500,1623.4381759166718,0.050995432646232075
500501,1001004,500502,1501506,1626.583009004593,0.05090035688954231
501502,1003006,501503,1504509,1629.7402868270874,0.050805758639398846
502503,1005008,502504,1507512,1632.8726329803467,0.05071089473676693
503504,1007010,503505,1510515,1636.0216839313507,0.050615932341315784
504505,1009012,504506,1513518,1639.2338647842407,0.050521713827038184
505506,1011014,505507,1516521,1642.3657879829407,0.05042548369419819
506507,1013016,506508,1519524,1645.5556840896606,0.05033082427326008
507508,1015018,507509,1522527,1648.728436946869,0.05023666063607379
508509,1017020,508510,1525530,1651.8732669353485,0.05014328451215988
509510,1019022,509511,1528533,1655.0135951042175,0.05005090968552395
510511,1021024,510512,1531536,1658.1827890872955,0.049959424357439275
511512,1023026,511513,1534539,1661.31210398674,0.049867271964103566
512513,1025028,512514,1537542,1664.4548168182373,0.049773681414080784
513514,1027030,513515,1540545,1667.5774660110474,0.04968110229674494
514515,1029032,514516,1543548,1670.7137019634247,0.049589778822337394
515516,1031034,515517,1546551,1673.851751089096,0.04949589047100744
516517,1033036,516518,1549554,1677.0397238731384,0.04940552661719266
517518,1035038,517519,1552557,1680.1724331378937,0.049314870724629145
518519,1037040,518520,1555560,1683.3217520713806,0.04922398920825799
519520,1039042,519521,1558563,1686.452054977417,0.04913330849376507
520521,1041044,520522,1561566,1689.621505022049,0.049043751543649705
521522,1043046,521523,1564569,1692.8119859695435,0.0489543357216462
522523,1045048,522524,1567572,1695.9999539852142,0.04886592671937251
523524,1047050,523525,1570575,1699.155601978302,0.04877819638750225
524525,1049052,524526,1573578,1702.2986080646515,0.0486907016402256
525526,1051054,525527,1576581,1705.4767138957977,0.04860325131994614
526527,1053056,526528,1579584,1708.62118601799,0.04851394532852282
527528,1055058,527529,1582587,1711.7446508407593,0.04842633028783894
528529,1057060,528530,1585590,1714.8936820030212,0.04833868170862843
529530,1059062,529531,1588593,1718.072138786316,0.048251480924591306
530531,1061064,530532,1591596,1721.2370779514313,0.048163793258936494
531532,1063066,531533,1594599,1724.3970611095428,0.04807844823153573
532533,1065068,532534,1597602,1727.5854759216309,0.04799239403473621
533534,1067070,533535,1600605,1730.7109339237213,0.04790563487949839
534535,1069072,534536,1603608,1733.9016089439392,0.0478212656944379
535536,1071074,535537,1606611,1737.0146729946136,0.047737461207361775
536537,1073076,536538,1609614,1740.1617279052734,0.047654560577939264
537538,1075078,537539,1612617,1743.3033530712128,0.047569475282216445
538539,1077080,538540,1615620,1746.4674808979034,0.04748495266176178
539540,1079082,539541,1618623,1749.5907890796661,0.04740149079771072
540541,1081084,540542,1621626,1752.7552528381348,0.04731940388046496
541542,1083086,541543,1624629,1755.8993680477142,0.0472373421798693
542543,1085088,542544,1627632,1759.065689086914,0.04715322945776279
543544,1087090,543545,1630635,1762.1999127864838,0.047069958251086064
544545,1089092,544546,1633638,1765.362576007843,0.04698887720769562
545546,1091094,545547,1636641,1768.494961977005,0.046906223375117406
546547,1093096,546548,1639644,1771.6578459739685,0.046825318539049476
547548,1095098,547549,1642647,1775.227998971939,0.046742959562834585
548549,1097100,548550,1645650,1778.8756058216095,0.04666254513358581
549550,1099102,549551,1648653,1782.4012069702148,0.046581631675508106
550551,1101104,550552,1651656,1786.225327014923,0.04650192002009135
551552,1103106,551553,1654659,1789.835035085678,0.04642086829881009
552553,1105108,552554,1657662,1793.8439300060272,0.04634116964916757
553554,1107110,553555,1660665,1797.7989249229431,0.04626296538663155
554555,1109112,554556,1663668,1801.1518869400024,0.046185372442778316
555556,1111114,555557,1666671,1804.663337945938,0.046107495783871855
556557,1113116,556558,1669674,1808.100370168686,0.04603011263498047
557558,1115118,557559,1672677,1811.6722049713135,0.04595306099508889
558559,1117120,558560,1675680,1814.9623777866364,0.0458741017318971
559560,1119122,559561,1678683,1818.1772468090057,0.04579636055495939
560561,1121124,560562,1681686,1821.3694241046906,0.045718708366621286
561562,1123126,561563,1684689,1824.8428359031677,0.04564223754823615
562563,1125128,562564,1687692,1828.3851580619812,0.04556606764163007
563564,1127130,563565,1690695,1831.8375887870789,0.0454895422590198
564565,1129132,564566,1693698,1835.0059559345245,0.045412774130454636
565566,1131134,565567,1696701,1838.2205259799957,0.04533767696375435
566567,1133136,566568,1699704,1841.3831651210785,0.04526180666107393
567568,1135138,567569,1702707,1844.9258279800415,0.04518569262836536
568569,1137140,568570,1705710,1848.3076379299164,0.04511015470052371
569570,1139142,569571,1708713,1851.7804069519043,0.04503496786310279
570571,1141144,570572,1711716,1855.3732059001923,0.044959556576941395
571572,1143146,571573,1714719,1858.8313419818878,0.04488413905346533
572573,1145148,572574,1717722,1862.3637919425964,0.0448101383390167
573574,1147150,573575,1720725,1866.334076166153,0.04473666089506878
574575,1149152,574576,1723728,1870.2870519161224,0.04466009384850622
575576,1151154,575577,1726731,1874.3534178733826,0.044587020616745576
576577,1153156,576578,1729734,1878.1478769779205,0.04451414503819251
577578,1155158,577579,1732737,1881.9773280620575,0.04444091132245376
578579,1157160,578580,1735740,1885.3233659267426,0.04436869539131294
579580,1159162,579581,1738743,1888.5962400436401,0.04429689074822818
580581,1161164,580582,1741746,1891.8755869865417,0.04422357928160636
581582,1163166,581583,1744749,1895.4415469169617,0.04414986156371015
582583,1165168,582584,1747752,1898.611743927002,0.04407581319355813
583584,1167170,583585,1750755,1901.9417929649353,0.044004772847983986
584585,1169172,584586,1753758,1905.3456118106842,0.04393424596310069
585586,1171174,585587,1756761,1908.7309720516205,0.043862658416401246
586587,1173176,586588,1759764,1911.9918749332428,0.043793404369353084
587588,1175178,587589,1762767,1915.2745609283447,0.0437222551117884
588589,1177180,588590,1765770,1918.5419878959656,0.043650132005495834
589590,1179182,589591,1768773,1922.4201440811157,0.04358097710064612
590591,1181184,590592,1771776,1925.621423959732,0.04351138607125904
591592,1183186,591593,1774779,1928.8603188991547,0.043441357111078105
592593,1185188,592594,1777782,1932.5221920013428,0.04337170409417013
593594,1187190,593595,1780785,1936.6794199943542,0.043302403446432436
594595,1189192,594596,1783788,1941.9770851135254,0.04323324109282112
595596,1191194,595597,1786791,1948.2553520202637,0.04316388510778779
596597,1193196,596598,1789794,1955.093554019928,0.04309501779061975
597598,1195198,597599,1792797,1959.2258758544922,0.043026458381064
598599,1197200,598600,1795800,1963.5981090068817,0.04295820854531485
599600,1199202,599601,1798803,1968.2218689918518,0.042889869093414745
600601,1201204,600602,1801806,1972.311040878296,0.04282092554967676
601602,1203206,601603,1804809,1977.5238199234009,0.04275241000868846
602603,1205208,602604,1807812,1985.064659833908,0.04268527343265305
603604,1207210,603605,1810815,1991.0554311275482,0.04261758642496716
604605,1209212,604606,1813818,1997.0010690689087,0.04255037713301135
605606,1211214,605607,1816821,2003.3884608745575,0.04248414690846403
606607,1213216,606608,1819824,2007.9060881137848,0.042415345551489736
607608,1215218,607609,1822827,2012.2413218021393,0.04234929137965082
608609,1217220,608610,1825830,2015.62043094635,0.042283609795049415
609610,1219222,609611,1828833,2018.9647438526154,0.04221700195193989
610611,1221224,610612,1831836,2022.8233420848846,0.0421519214505679
611612,1223226,611613,1834839,2028.2265319824219,0.04208638289310329
612613,1225228,612614,1837842,2032.9879038333893,0.04202031037857523
613614,1227230,613615,1840845,2037.1618638038635,0.04195546826667851
614615,1229232,614616,1843848,2042.976124048233,0.04188987466477556
615616,1231234,615617,1846851,2048.7355608940125,0.04182607431539509
616617,1233236,616618,1849854,2054.129898786545,0.04176243709480332
617618,1235238,617619,1852857,2059.7739288806915,0.04169758628268028
618619,1237240,618620,1855860,2066.0419318675995,0.041635043040514574
619620,1239242,619621,1858863,2071.8875029087067,0.041571202125851414
620621,1241244,620622,1861866,2077.994777917862,0.04150764776204596
621622,1243246,621623,1864869,2084.0906269550323,0.04144455976529571
622623,1245248,622624,1867872,2089.212607860565,0.041379930669791065
623624,1247250,623625,1870875,2094.5463128089905,0.04131724388207658
624625,1249252,624626,1873878,2100.0910229682922,0.04125405273771321
625626,1251254,625627,1876881,2105.7901339530945,0.041191075797542
626627,1253256,626628,1879884,2111.277456998825,0.04112834275838395
627628,1255258,627629,1882887,2116.9726309776306,0.04106545570175513
628629,1257260,628630,1885890,2122.2987360954285,0.04100408538033662
629630,1259262,629631,1888893,2127.5815529823303,0.04094285784049134
630631,1261264,630632,1891896,2132.7739329338074,0.040880973521780106
631632,1263266,631633,1894899,2138.2709300518036,0.04081938163108134
632633,1265268,632634,1897902,2143.6012799739838,0.040758221462965594
633634,1267270,633635,1900905,2148.7185609340668,0.04069696935403044
634635,1269272,634636,1903908,2154.0890579223633,0.04063567369848897
635636,1271274,635637,1906911,2159.37774682045,0.04057409816959989
636637,1273276,636638,1909914,2164.5885627269745,0.04051328544301214
637638,1275278,637639,1912917,2169.7127211093903,0.04045297698030481
638639,1277280,638640,1915920,2175.095111131668,0.040392912771494593
639640,1279282,639641,1918923,2180.4443418979645,0.04033282272575889
640641,1281284,640642,1921926,2185.747433900833,0.040273815397085855
641642,1283286,641643,1924929,2191.419862985611,0.04021324417772121
642643,1285288,642644,1927932,2197.247104883194,0.04015354650255176
643644,1287290,643645,1930935,2202.5706741809845,0.04009462554677157
644645,1289292,644646,1933938,2207.7880580425262,0.04003443870533374
645646,1291294,645647,1936941,2213.2182669639587,0.039974716908545815
646647,1293296,646648,1939944,2218.617031097412,0.03991660761857929
647648,1295298,647649,1942947,2223.803519964218,0.03985788689351466
648649,1297300,648650,1945950,2229.237277030945,0.03979905945743667
649650,1299302,649651,1948953,2234.788936853409,0.03974067712260876
650651,1301304,650652,1951956,2240.141368865967,0.03968275122679188
651652,1303306,651653,1954959,2246.0997400283813,0.039624319100767025
652653,1305308,652654,1957962,2251.525661945343,0.03956645934158587
653654,1307310,653655,1960965,2257.1946709156036,0.0395078811179701
654655,1309312,654656,1963968,2264.332941055298,0.0394513010069204
655656,1311314,655657,1966971,2270.2472448349,0.039392405155012966
656657,1313316,656658,1969974,2275.903461933136,0.03933641526600695
657658,1315318,657659,1972977,2282.0164959430695,0.03927874493456329
658659,1317320,658660,1975980,2287.0984721183777,0.03922197036808939
659660,1319322,659661,1978983,2292.211678981781,0.03916570541150577
660661,1321324,660662,1981986,2297.267026901245,0.0391096770454169
661662,1323326,661663,1984989,2302.3890538215637,0.03905399721770664
662663,1325328,662664,1987992,2307.511715888977,0.03899830144291627
663664,1327330,663665,1990995,2312.5932998657227,0.03894232297534472
664665,1329332,664666,1993998,2317.6712868213654,0.0388862266754586
665666,1331334,665667,1997001,2322.7218039035797,0.03883053954450588
666667,1333336,666668,2000004,2327.828311920166,0.03877456749432895
667668,1335338,667669,2003007,4091.698336839676,0.03871932228321384
668669,1337340,668670,2006010,4099.084939956665,0.03866480605756806
669670,1339342,669671,2009013,4115.691527843475,0.03860982913101907
670671,1341344,670672,2012016,4139.026416063309,0.038555029375856975
671672,1343346,671673,2015019,4142.970368862152,0.038501210930917296
672673,1345348,672674,2018022,4146.455374956131,0.03844708491305937
673674,1347350,673675,2021025,4149.963955879211,0.038393645039832336
674675,1349352,674676,2024028,4153.836854934692,0.038339206021191785
675676,1351354,675677,2027031,4157.450986862183,0.03828540522954427
676677,1353356,676678,2030034,4161.239151000977,0.03823104801631416
677678,1355358,677679,2033037,4164.6348531246185,0.03817709151735471
678679,1357360,678680,2036040,4168.356494903564,0.03812284182095027
679680,1359362,679681,2039043,4171.726599931717,0.0380702406855562
680681,1361364,680682,2042046,4175.091633081436,0.03801742582800216
681682,1363366,681683,2045049,4178.780520915985,0.03796415519173024
682683,1365368,682684,2048052,4182.156746864319,0.03791121947506326
683684,1367370,683685,2051055,4185.515522003174,0.0378580127726309
684685,1369372,684686,2054058,4188.905415058136,0.037805041449246346
685686,1371374,685687,2057061,4192.562621831894,0.037752692680442124
686687,1373376,686688,2060064,4195.947293043137,0.03770106526098971
687688,1375378,687689,2063067,4199.137413978577,0.03764945925831853
688689,1377380,688690,2066070,4202.27200293541,0.03759599534532754
689690,1379382,689691,2069073,4205.992250919342,0.03754296102488297
690691,1381384,690692,2072076,4210.528977155685,0.03749097446416272
691692,1383386,691693,2075079,4215.187668800354,0.03743898047832772
692693,1385388,692694,2078082,4219.946036815643,0.03738743566827907
693694,1387390,693695,2081085,4223.696805000305,0.03733618166188535
694695,1389392,694696,2084088,4227.292818784714,0.03728485861392983
695696,1391394,695697,2087091,4231.148254871368,0.037233469729471835
696697,1393396,696698,2090094,4235.161218881607,0.03718269662203966
697698,1395398,697699,2093097,4238.718869924545,0.03713197352226416
698699,1397400,698700,2096100,4242.424997091293,0.03708065932369209
699700,1399402,699701,2099103,4246.540647983551,0.0370299874975899
700701,1401404,700702,2102106,4250.353470802307,0.03698010499647353
701702,1403406,701703,2105109,4254.4948699474335,0.03692995557867107
702703,1405408,702704,2108112,4258.967711925507,0.03688004927789734
703704,1407410,703705,2111115,4262.817600011826,0.036830290944635635
704705,1409412,704706,2114118,4267.033741950989,0.03678107391351659
705706,1411414,705707,2117121,4270.729420900345,0.036731516043801093
706707,1413416,706708,2120124,4274.544628858566,0.03668132059829077
707708,1415418,707709,2123127,4278.190690994263,0.036631594459322514
708709,1417420,708710,2126130,4282.122334957123,0.0365823926840676
709710,1419422,709711,2129133,4285.968441963196,0.03653395191213349
710711,1421424,710712,2132136,4290.232913970947,0.0364840890179039
711712,1423426,711713,2135139,4293.940696001053,0.03643541640849435
712713,1425428,712714,2138142,4297.519789934158,0.036386769426826504
713714,1427430,713715,2141145,4301.173377990723,0.03633834562606353
714715,1429432,714716,2144148,4304.812829017639,0.03629088347770448
715716,1431434,715717,2147151,4308.091698169708,0.03624298957220162
716717,1433436,716718,2150154,4312.041035890579,0.03619523824454518
717718,1435438,717719,2153157,4316.284625053406,0.036146624142929795
718719,1437440,718720,2156160,4320.174027919769,0.03609831373796624
719720,1439442,719721,2159163,4324.289486885071,0.03604966674538446
720721,1441444,720722,2162166,4328.527805089951,0.03600229898984253
721722,1443446,721723,2165169,4332.483278989792,0.03595412662616582
722723,1445448,722724,2168172,4336.397146940231,0.03590584421908716
723724,1447450,723725,2171175,4340.613430023193,0.03585837710306805
724725,1449452,724726,2174178,4344.800122022629,0.03581201867746131
725726,1451454,725727,2177181,4349.157467126846,0.03576470997359138
726727,1453456,726728,2180184,4352.994756937027,0.03571860784177261
727728,1455458,727729,2183187,4356.68745303154,0.035671457491844194
728729,1457460,728730,2186190,4360.579021930695,0.03562449936907797
729730,1459462,729731,2189193,4364.03465795517,0.03557748882667511
730731,1461464,730732,2192196,4367.6006100177765,0.03553088889566425
731732,1463466,731733,2195199,4371.755285978317,0.03548482366022654
732733,1465468,732734,2198202,4375.239307880402,0.0354382008772518
733734,1467470,733735,2201205,4379.271016120911,0.0353913798717258
734735,1469472,734736,2204208,4382.708813905716,0.03534572712669615
735736,1471474,735737,2207211,4385.886002063751,0.035300097420986276
736737,1473476,736738,2210214,4389.246035814285,0.035254299034932046
737738,1475478,737739,2213217,4392.560343980789,0.03520932006176736
738739,1477480,738740,2216220,4395.858367919922,0.03516398169085733
739740,1479482,739741,2219223,4399.202148914337,0.03511880136284162
740741,1481484,740742,2222226,4402.778849840164,0.03507275264200871
741742,1483486,741743,2225229,4406.3883509635925,0.035027042191359214
742743,1485488,742744,2228232,4410.389400005341,0.034981531938683474
743744,1487490,743745,2231235,4413.91626906395,0.03493698836427939
744745,1489492,744746,2234238,4417.088963031769,0.03489175106733455
745746,1491494,745747,2237241,4420.768791913986,0.034847662844185834
746747,1493496,746748,2240244,4423.96058678627,0.034803178792572
747748,1495498,747749,2243247,4427.193526029587,0.034758711204631254
748749,1497500,748750,2246250,4430.559084892273,0.03471424038798432
749750,1499502,749751,2249253,4434.830430984497,0.034669603393922444
750751,1501504,750752,2252256,4439.1307208538055,0.03462416969705373
751752,1503506,751753,2255259,4444.241780996323,0.034579417819259106
752753,1505508,752754,2258262,4449.22009396553,0.03453658034231921
753754,1507510,753755,2261265,4453.3006939888,0.03449279608321376
754755,1509512,754756,2264268,4458.001098871231,0.03444845521153184
755756,1511514,755757,2267271,4461.740766763687,0.03440501668410434
756757,1513516,756758,2270274,4465.388877868652,0.034362663063802756
757758,1515518,757759,2273277,4468.905707836151,0.034319789137953194
758759,1517520,758760,2276280,4472.3062398433685,0.03427602720330469
759760,1519522,759761,2279283,4475.762804985046,0.03423261836542224
760761,1521524,760762,2282286,4479.246771812439,0.03418961277930066
761762,1523526,761763,2285289,4482.66813993454,0.03414665835589403
762763,1525528,762764,2288292,4486.4732620716095,0.03410442505264655
763764,1527530,763765,2291295,4490.102833986282,0.03406161260136287
764765,1529532,764766,2294298,4493.757650136948,0.034019160661046044
765766,1531534,765767,2297301,4497.602061033249,0.03397746815608116
766767,1533536,766768,2300304,4501.4056391716,0.03393495422460546
767768,1535538,767769,2303307,4505.053637981415,0.03389227359184588
768769,1537540,768770,2306310,4508.750738859177,0.03384961175106582
769770,1539542,769771,2309313,4513.403367996216,0.03380806336281239
770771,1541544,770772,2312316,4517.763236045837,0.033766449540053145
771772,1543546,771773,2315319,4522.182215929031,0.033724763938153046
772773,1545548,772774,2318322,4526.025736808777,0.033683460769680096
773774,1547550,773775,2321325,4530.470230817795,0.03364172602232429
774775,1549552,774776,2324328,4534.898781776428,0.033599998056160985
775776,1551554,775777,2327331,4539.649871110916,0.0335584021104296
776777,1553556,776778,2330334,4544.470153808594,0.033517257137646084
777778,1555558,777779,2333337,4549.37979888916,0.03347643734377925
778779,1557560,778780,2336340,4554.1906089782715,0.03343526779462991
779780,1559562,779781,2339343,4558.6956288814545,0.03339471659819537
780781,1561564,780782,2342346,4562.211613893509,0.03335386601793289
781782,1563566,781783,2345349,4566.618706941605,0.033313104533590376
782783,1565568,782784,2348352,4570.546141862869,0.03327247619199625
783784,1567570,783785,2351355,4574.593616962433,0.033232224981475156
784785,1569572,784786,2354358,4578.544322967529,0.033192340004461585
785786,1571574,785787,2357361,4582.22572517395,0.033151528046801104
786787,1573576,786788,2360364,4585.520621061325,0.03311041713459417
787788,1575578,787789,2363367,4589.391371011734,0.03307095599666354
788789,1577580,788790,2366370,4592.958515882492,0.03303067898377776
789790,1579582,789791,2369373,4597.24237203598,0.03299129588231153
790791,1581584,790792,2372376,4600.510750770569,0.0329518017861119
791792,1583586,791793,2375379,4604.293848991394,0.03291252976850956
792793,1585588,792794,2378382,4608.062875032425,0.03287402156456665
793794,1587590,793795,2381385,4612.048408985138,0.03283395802100131
794795,1589592,794796,2384388,4615.508891105652,0.032795438206449035
795796,1591594,795797,2387391,4619.783047914505,0.032755821781393024
796797,1593596,796798,2390394,4623.007378816605,0.03271525218951865
797798,1595598,797799,2393397,4626.2900149822235,0.032676240287401015
798799,1597600,798800,2396400,4629.5637748241425,0.03263684814919543
799800,1599602,799801,2399403,4632.871695995331,0.032597626335700625
800801,1601604,800802,2402406,4636.373883962631,0.032558924927798216
801802,1603606,801803,2405409,4640.025093078613,0.032519601638341555
802803,1605608,802804,2408412,4643.816245794296,0.03248162298950774
803804,1607610,803805,2411415,4647.103326797485,0.032443141304611345
804805,1609612,804806,2414418,4650.2938940525055,0.03240454524893721
805806,1611614,805807,2417421,4653.539753913879,0.03236644182834425
806807,1613616,806808,2420424,4656.701565742493,0.03232829934131587
807808,1615618,807809,2423427,4660.016810894012,0.032289791975927074
808809,1617620,808810,2426430,4663.346800088882,0.03225160025067453
809810,1619622,809811,2429433,4666.582525014877,0.032214089267654344
810811,1621624,810812,2432436,4670.813022851944,0.032175778036616975
811812,1623626,811813,2435439,4674.429881095886,0.0321390231129044
812813,1625628,812814,2438442,4677.726385116577,0.032100406100653345
813814,1627630,813815,2441445,4681.018491029739,0.0320630025016726
814815,1629632,814816,2444448,4684.411664009094,0.03202519233309431
815816,1631634,815817,2447451,4687.647872924805,0.03198814424467855
816817,1633636,816818,2450454,4691.246066093445,0.03195124947524164
817818,1635638,817819,2453457,4694.548254966736,0.03191364057784085
818819,1637640,818820,2456460,4697.689256191254,0.03187679375332664
819820,1639642,819821,2459463,4700.970524072647,0.03183907057973556
820821,1641644,820822,2462466,4704.184775114059,0.03180179355695145
821822,1643646,821823,2465469,4707.555480957031,0.03176509848526621
822823,1645648,822824,2468472,4711.077173948288,0.03172879615340207
823824,1647650,823825,2471475,4714.901731014252,0.03169159653407405
824825,1649652,824826,2474478,4718.409392118454,0.031654371681725024
825826,1651654,825827,2477481,4722.380391120911,0.031617933373127016
826827,1653656,826828,2480484,4726.011096000671,0.031581702236508136
827828,1655658,827829,2483487,4729.288881063461,0.03154470658955688
828829,1657660,828830,2486490,4733.088234901428,0.03150773511879379
829830,1659662,829831,2489493,4737.078544139862,0.031471800484723644
830831,1661664,830832,2492496,4741.203775882721,0.03143545958118921
831832,1663666,831833,2495499,4744.547883987427,0.031399543542647734
832833,1665668,832834,2498502,4747.984932899475,0.03136315700430714
833834,1667670,833835,2501505,4751.371357917786,0.03132686094795645
834835,1669672,834836,2504508,4755.237520933151,0.03129095609074284
835836,1671674,835837,2507511,4758.935166835785,0.031255343315933715
836837,1673676,836838,2510514,4762.238480091095,0.031219599479300086
837838,1675678,837839,2513517,4765.484871149063,0.031183902519842377
838839,1677680,838840,2516520,4768.997900009155,0.03114803342759842
839840,1679682,839841,2519523,4772.540303945541,0.03111256327247247
840841,1681684,840842,2522526,4776.287311077118,0.031077125167939812
841842,1683686,841843,2525529,4780.122676849365,0.031042275073559722
842843,1685688,842844,2528532,4783.873647928238,0.031006753735709935
843844,1687690,843845,2531535,4787.852553844452,0.03097192180393904
844845,1689692,844846,2534538,4791.620132923126,0.030935997239794233
845846,1691694,845847,2537541,4795.152317047119,0.03090112885547569
846847,1693696,846848,2540544,4798.642001152039,0.030866403350955807
847848,1695698,847849,2543547,4802.349472999573,0.030832054626444005
848849,1697700,848850,2546550,4806.017889022827,0.03079660007824714
849850,1699702,849851,2549553,4809.739509820938,0.030761423760850448
850851,1701704,850852,2552556,4813.272099018097,0.03072729557788989
851852,1703706,851853,2555559,4817.237803936005,0.030693142069139867
852853,1705708,852854,2558562,4821.143630981445,0.030659198517241748
853854,1707710,853855,2561565,4825.088047027588,0.030624860501120565
854855,1709712,854856,2564568,4829.578109025955,0.030590744057917618
855856,1711714,855857,2567571,4834.420916795731,0.030556371528291493
856857,1713716,856858,2570574,4838.682142972946,0.030522578983436688
857858,1715718,857859,2573577,4843.063844919205,0.03048810725158546
858859,1717720,858860,2576580,4847.023699760437,0.030453990892056026
859860,1719722,859861,2579583,4850.397127151489,0.030420116816458176
860861,1721724,860862,2582586,4853.847176790237,0.03038651472161291
861862,1723726,861863,2585589,4857.14200592041,0.03035241820725787
862863,1725728,862864,2588592,4860.75612783432,0.03031901862777886
863864,1727730,863865,2591595,4864.114503145218,0.030285821374491206
864865,1729732,864866,2594598,4867.571174144745,0.03025216152491339
865866,1731734,865867,2597601,4871.000324964523,0.03021919363163761
866867,1733736,866868,2600604,4874.585211992264,0.03018562353645393
867868,1735738,867869,2603607,4878.970557928085,0.030152297469612677
868869,1737740,868870,2606610,4883.050940990448,0.030119596720396657
869870,1739742,869871,2609613,4887.415110111237,0.030085728130870848
870871,1741744,870872,2612616,4891.133594989777,0.030053000888074166
871872,1743746,871873,2615619,4894.926430940628,0.030019500361959217
872873,1745748,872874,2618622,4898.790283918381,0.029986421606736258
873874,1747750,873875,2621625,4902.595242977142,0.029953411200040136
874875,1749752,874876,2624628,4906.043792009354,0.02992070059553953
875876,1751754,875877,2627631,4909.304524898529,0.02988757572893519
876877,1753756,876878,2630634,4912.70180606842,0.029854832333512604
877878,1755758,877879,2633637,4916.000274181366,0.029822144668287365
878879,1757760,878880,2636640,4919.192974090576,0.029788771171297412
879880,1759762,879881,2639643,4922.645506858826,0.029755646672128933
880881,1761764,880882,2642646,4926.638334989548,0.02972325278642529
881882,1763766,881883,2645649,4930.629602909088,0.02969039900926873
882883,1765768,882884,2648652,4934.19583773613,0.02965827065963822
883884,1767770,883885,2651655,4937.6632759571075,0.029626119685417507
884885,1769772,884886,2654658,4941.138813734055,0.02959422837739112
885886,1771774,885887,2657661,4944.8299198150635,0.02956127459037816
886887,1773776,886888,2660664,4948.827579975128,0.029529615469073178
887888,1775778,887889,2663667,4952.210072994232,0.029497455796445138
888889,1777780,888890,2666670,4956.627835035324,0.029466116100593354
889890,1779782,889891,2669673,4960.03732585907,0.029434167181534576
890891,1781784,890892,2672676,4963.6160678863525,0.029402903041045647
891892,1783786,891893,2675679,4967.133340120316,0.02937107244906656
892893,1785788,892894,2678682,4970.79675412178,0.02933935275177646
893894,1787790,893895,2681685,4974.499418973923,0.029308029457752127
894895,1789792,894896,2684688,4978.276323080063,0.029276658033268177
895896,1791794,895897,2687691,4982.086149930954,0.029245277168229222
896897,1793796,896898,2690694,4985.691527843475,0.02921408079964749
897898,1795798,897899,2693697,4990.41171503067,0.02918310409222613
898899,1797800,898900,2696700,4995.1042239665985,0.029152423341656686
899900,1799802,899901,2699703,4999.972170829773,0.029120745462932973
900901,1801804,900902,2702706,5004.972925901413,0.029089889752867748
901902,1803806,901903,2705709,5009.674431800842,0.02905919281693059
902903,1805808,902904,2708712,5014.780626773834,0.02902849067322677
903904,1807810,903905,2711715,5019.504405975342,0.02899744144269789
904905,1809812,904906,2714718,5023.838215112686,0.028966995763767045
905906,1811814,905907,2717721,5027.703917980194,0.028935690175785567
906907,1813816,906908,2720724,5032.816445827484,0.028905024228151888
907908,1815818,907909,2723727,5037.032786130905,0.028873939025288564
908909,1817820,908910,2726730,5041.019506931305,0.028843062413216103
909910,1819822,909911,2729733,5045.392885923386,0.028812653026761836
910911,1821824,910912,2732736,5049.725791931152,0.028782113158740685
911912,1823826,911913,2735739,5054.0988137722015,0.028752115731549566
912913,1825828,912914,2738742,5058.239325761795,0.0287215346161247
913914,1827830,913915,2741745,5061.927144050598,0.0286915788128681
914915,1829832,914916,2744748,5065.9133858680725,0.02866078713122988
915916,1831834,915917,2747751,5069.776775121689,0.028630538579818676
916917,1833836,916918,2750754,5073.357801914215,0.028600612144145998
917918,1835838,917919,2753757,5076.794517993927,0.028571161084983032
918919,1837840,918920,2756760,5080.489871025085,0.0285411127970292
919920,1839842,919921,2759763,5084.144505977631,0.02851063468551729
920921,1841844,920922,2762766,5087.993330955505,0.028481110790380626
921922,1843846,921923,2765769,5091.740677118301,0.028451663374653435
922923,1845848,922924,2768772,5095.515827894211,0.028422044808394276
923924,1847850,923925,2771775,5099.532336950302,0.028392245980285225
924925,1849852,924926,2774778,5103.799822092056,0.02836262343225826
925926,1851854,925927,2777781,5107.682447910309,0.028332986248642555
926927,1853856,926928,2780784,5111.133094072342,0.028303642857281375
927928,1855858,927929,2783787,5114.9874448776245,0.028274421334572253
928929,1857860,928930,2786790,5118.735208749771,0.028245034223800758
929930,1859862,929931,2789793,5122.1567368507385,0.028216122886078665
930931,1861864,930932,2792796,5125.937621831894,0.028186402099890984
931932,1863866,931933,2795799,5130.151705026627,0.028157841501524672
932933,1865868,932934,2798802,5133.598215103149,0.028128996576924692
933934,1867870,933935,2801805,5137.055328845978,0.028100239693230833
934935,1869872,934936,2804808,5140.480310916901,0.028071228734916076
935936,1871874,935937,2807811,5144.828907966614,0.028042384305081214
936937,1873876,936938,2810814,5149.025298833847,0.028013755325446255
937938,1875878,937939,2813817,5152.712814092636,0.02798347389943956
938939,1877880,938940,2816820,5156.892079114914,0.027954690285696415
939940,1879882,939941,2819823,5160.875806808472,0.02792558804321743
940941,1881884,940942,2822826,5164.415240764618,0.027897375875909347
941942,1883886,941943,2825829,5168.497157096863,0.02786889989693009
942943,1885888,942944,2828832,5172.118111848831,0.027840701995955897
943944,1887890,943945,2831835,5175.662349939346,0.02781281352508813
944945,1889892,944946,2834838,5179.312213897705,0.02778388583283231
945946,1891894,945947,2837841,5183.339426994324,0.027755733230151236
946947,1893896,946948,2840844,5187.590912818909,0.02772779733459174
947948,1895898,947949,2843847,5192.227419137955,0.027699891033989843
948949,1897900,948950,2846850,5196.816307783127,0.02767230679455679
949950,1899902,949951,2849853,5201.191655158997,0.02764438150006754
950951,1901904,950952,2852856,5205.3339149951935,0.02761588063913223
951952,1903906,951953,2855859,5209.415547132492,0.027587947281062952
952953,1905908,952954,2858862,5213.032489776611,0.027560153686863487
953954,1907910,953955,2861865,5216.4420347213745,0.02753220568592951
954955,1909912,954956,2864868,5219.830653190613,0.02750450854000519
955956,1911914,955957,2867871,5223.474904060364,0.027477171661303146
956957,1913916,956958,2870874,5227.610511064529,0.027449873845398542
957958,1915918,957959,2873877,5231.658034801483,0.02742221693188185
958959,1917920,958960,2876880,5236.212136030197,0.027394678072596435
959960,1919922,959961,2879883,5240.1828100681305,0.027366760514269117
960961,1921924,960962,2882886,5244.601906776428,0.02733927430017502
961962,1923926,961963,2885889,5248.613600969315,0.027310930887324503
962963,1925928,962964,2888892,5252.506670951843,0.027284040668746457
963964,1927930,963965,2891895,5256.091553926468,0.027256460296484875
964965,1929932,964966,2894898,5259.645341157913,0.027229739702306688
965966,1931934,965967,2897901,5263.401695966721,0.027202205023058923
966967,1933936,966968,2900904,5267.032893896103,0.02717545553423406
967968,1935938,967969,2903907,5271.464231014252,0.027148316801685723
968969,1937940,968970,2906910,5276.753186941147,0.027121235867525684
969970,1939942,969971,2909913,5280.941751003265,0.027094575749288197
970971,1941944,970972,2912916,5285.699464797974,0.027067925462688436
971972,1943946,971973,2915919,5289.779031038284,0.027041320225180243
972973,1945948,972974,2918922,5294.023982048035,0.02701479605093482
973974,1947950,973975,2921925,5298.48277592659,0.026988092213287018
974975,1949952,974976,2924928,5302.789623975754,0.02696152322096168
975976,1951954,975977,2927931,5307.030978918076,0.02693498028384056
976977,1953956,976978,2930934,5312.0432250499725,0.0269079985555436
977978,1955958,977979,2933937,5316.7024738788605,0.026881365693043335
978979,1957960,978980,2936940,5320.38431596756,0.026854754205487552
979980,1959962,979981,2939943,5324.378356933594,0.026828830190424924
980981,1961964,980982,2942946,5328.16979598999,0.02680286422400968
981982,1963966,981983,2945949,5332.5676419734955,0.02677618648885982
982983,1965968,982984,2948952,5337.038569927216,0.026750973735033767
983984,1967970,983985,2951955,5341.830600738525,0.026724187275249278
984985,1969972,984986,2954958,5346.262991905212,0.0266975292324787
985986,1971974,985987,2957961,5350.712601900101,0.026671626230381662
986987,1973976,986988,2960964,5354.621773004532,0.026645260586519726
987988,1975978,987989,2963967,5358.698045015335,0.026619375119480537
988989,1977980,988990,2966970,5362.769677877426,0.02659372013840766
989990,1979982,989991,2969973,5366.420922994614,0.02656835868037888
990991,1981984,990992,2972976,5370.021301984787,0.026542259774942067
991992,1983986,991993,2975979,5373.730073928833,0.02651684874763305
992993,1985988,992994,2978982,5377.596878051758,0.026490979760637856
993994,1987990,993995,2981985,5381.801306962967,0.026465454793651588
994995,1989992,994996,2984988,5385.666743040085,0.026439945575475576
995996,1991994,995997,2987991,5389.418166875839,0.026414401523652487
996997,1993996,996998,2990994,5393.604700088501,0.026389493952592602
997998,1995998,997999,2993997,5398.450407981873,0.02636395296030969
998999,1998000,999000,2997000,5402.246125936508,0.026338771709561115
1000000,2000002,1000001,3000003,5406.496776819229,0.026313360594940605


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0026559829711914062,12064.709122577777
1001,2003,2002,4005,3.4950649738311768,12.835124349569014
2002,4005,4004,8009,6.758717060089111,11.944634412788218
3003,6007,6006,12013,10.094599962234497,11.148884621363322
4004,8009,8008,16017,13.44087290763855,10.435206510481294
5005,10011,10010,20021,16.938480138778687,9.793065177316748
6006,12013,12012,24025,20.515602111816406,9.213598608499524
7007,14015,14014,28029,23.948411226272583,8.689284992171451
8008,16017,16016,32033,27.571858882904053,8.213692023180556
9009,18019,18018,36037,30.72619891166687,7.781284697110095
10010,20021,20020,40041,33.880789041519165,7.387273657386686
11011,22023,22022,44045,37.06355810165405,7.0274945171859144
12012,24025,24024,48049,40.28280997276306,6.698310615191076
13013,26027,26026,52053,43.56460523605347,6.396533875067689
14014,28029,28028,56057,46.711780071258545,6.119359828790039
15015,30031,30030,60061,49.841068983078,5.864313836927977
16016,32033,32032,64065,53.03543210029602,5.629206242432701
17017,34035,34034,68069,56.18182396888733,5.412094713119586
18018,36037,36036,72073,59.378933906555176,5.211252415772833
19019,38039,38038,76077,62.53703022003174,5.025140957832264
20020,40041,40040,80081,65.71999502182007,4.852387255838039
21021,42043,42042,84085,68.95322394371033,4.691763661241566
22022,44045,44044,88089,72.13115692138672,4.54217080665876
23023,46047,46046,92093,75.29652905464172,4.402622738787613
24024,48049,48048,96097,78.45367217063904,4.272233984846025
25025,50051,50050,100101,81.62401103973389,4.150208263214154
26026,52053,52052,104105,84.79374194145203,4.035828599335218
27027,54055,54054,108109,87.96549391746521,3.928448648466656
28028,56057,56056,112113,91.10581016540527,3.8274850593079464
29029,58059,58058,116117,94.28150796890259,3.7324107388485572
30030,60061,60060,120121,97.44615387916565,3.6427489597372187
31031,62063,62062,124125,100.64060807228088,3.5580680003768066
32032,64065,64064,128129,103.80441808700562,3.4779763806545816
33033,66067,66066,132133,106.97126603126526,3.4021189303530264
34034,68069,68068,136137,110.12469911575317,3.330173004356766
35035,70071,70070,140141,113.37465000152588,3.261845197301227
36036,72073,72072,144145,116.55617618560791,3.196868415008794
37037,74075,74074,148149,119.75825500488281,3.134999261199482
38038,76077,76076,152153,122.90700197219849,3.0760157031345443
39039,78079,78078,156157,126.14792490005493,3.019714984460734
40040,80081,80080,160161,129.35842204093933,2.9659117573555704
41041,82083,82082,164165,132.52135109901428,2.9144364094536286
42042,84085,84084,168169,135.70116806030273,2.8651335640315665
43043,86087,86086,172173,138.98321723937988,2.817860734363421
44044,88089,88088,176177,142.3063349723816,2.7724871154441644
45045,90091,90090,180181,145.49201822280884,2.728892498254936
46046,92093,92092,184185,148.72013902664185,2.686966293324076
47047,94095,94094,188189,151.9368860721588,2.646606651966067
48048,96097,96096,192193,155.15496802330017,2.6077196748356073
49049,98099,98098,196197,158.39673805236816,2.570218698523604
50050,100101,100100,200201,161.65513706207275,2.5340236520896724
51051,102103,102102,204205,165.02342104911804,2.4990604762260773
52052,104105,104104,208209,168.24806809425354,2.4652605985138507
53053,106107,106106,212213,171.52575707435608,2.4325604590794683
54054,108109,108108,216217,174.77418494224548,2.4009010814006615
55055,110111,110110,220221,177.9986071586609,2.3702276837466343
56056,112113,112112,224225,181.1837830543518,2.340489327089017
57057,114115,114114,228229,184.3813018798828,2.3116385958164756
58058,116117,116116,232233,187.56935906410217,2.283631308006079
59059,118119,118118,236237,190.80045318603516,2.256426252261008
60060,120121,120120,240241,194.0019040107727,2.229984948551646
61061,122123,122122,244245,197.1868028640747,2.2042714306189737
62062,124125,124124,248249,200.38405799865723,2.1792520479211817
63063,126127,126126,252253,203.54104709625244,2.154895285159
64064,128129,128128,256257,206.7100269794464,2.1311716044274363
65065,130131,130130,260261,209.87272906303406,2.1080532828345895
66066,132133,132132,264265,213.11961793899536,2.085514271404463
67067,134135,134134,268269,216.2877230644226,2.0635300874073437
68068,136137,136136,272273,219.8714780807495,2.0420776913888403
69069,138139,138138,276277,223.0088551044464,2.0211353821541707
70070,140141,140140,280281,226.22470808029175,2.000682700532707
71071,142143,142142,284285,229.79627203941345,1.9807003410987818
72072,144145,144144,288289,233.03378295898438,1.9611700711611775
73073,146147,146146,292293,236.3176350593567,1.9420746563246212
74074,148149,148148,296297,239.5995969772339,1.9233977920503094
75075,150151,150150,300301,242.7890968322754,1.9051240406824945
76076,152153,152152,304305,245.9729609489441,1.887238773439094
77077,154155,154154,308309,249.51617407798767,1.869728116933402
78078,156157,156156,312313,252.71622109413147,1.8525789038649236
79079,158159,158158,316317,255.89196515083313,1.835778627450054
80080,160161,160160,320321,259.04586696624756,1.8193153993506712
81081,162163,162162,324325,262.25056409835815,1.8031779107404873
82082,164165,164164,328329,265.4277548789978,1.7873553962654114
83083,166167,166166,332333,268.905779838562,1.7718376006723702
84084,168169,168168,336337,272.1653790473938,1.756614747859203
85085,170171,170170,340341,275.33785700798035,1.741677512147362
86086,172173,172172,344345,278.5904519557953,1.7270169934363366
87087,174175,174174,348349,281.7684950828552,1.7126247108662938
88088,176177,176176,352353,284.9200351238251,1.6984925117903913
89089,178179,178178,356357,288.17061018943787,1.6846126237414865
90090,180181,180180,360361,291.47307109832764,1.670977608717294
91091,182183,182182,364365,294.66961002349854,1.657580344548478
92092,184185,184184,368369,297.83230686187744,1.6444140075036557
93093,186187,186186,372373,301.0050401687622,1.6314720560567366
94094,188189,188188,376377,304.19787406921387,1.6187482157110935
95095,190191,190190,380381,307.3924241065979,1.6062364648114453
96096,192193,192192,384385,310.7349691390991,1.5939310212797864
97097,194195,194194,388389,314.0838692188263,1.5818263301625848
98098,196197,196196,392393,317.4551730155945,1.5699170520074404
99099,198199,198198,396397,320.7851400375366,1.5581980519127683
100100,200201,200200,400401,324.1468458175659,1.5466643892923457
101101,202203,202202,404405,327.50811791419983,1.535311308240125
102102,204205,204204,408409,330.83103108406067,1.5241342284916755
103103,206207,206206,412413,334.1876459121704,1.5131287369113124
104104,208209,208208,416417,337.5370988845825,1.5022905794921826
105105,210211,210210,420421,340.91296792030334,1.4916156538165524
106106,212213,212212,424425,344.2813711166382,1.4811000019744824
107107,214215,214214,428429,347.65298986434937,1.4707398038408428
108108,216217,216216,432433,351.0458869934082,1.4605313707943424
109109,218219,218218,436437,354.3879339694977,1.4504711397494248
110110,220221,220220,440441,357.73757219314575,1.4405556675119442
111111,222223,222222,444445,361.11696195602417,1.4307816254950012
112112,224225,224224,448449,364.49558115005493,1.4211457946712471
113113,226227,226226,452453,367.8432331085205,1.4116450608235027
114114,228229,228228,456457,371.33100509643555,1.4022764100354834
115115,230231,230230,460461,374.70840215682983,1.3930369244499161
116116,232233,232232,464465,378.0592701435089,1.3839237782067357
117117,234235,234234,468469,381.40681505203247,1.3749342336286645
118118,236237,236236,472473,384.76181197166443,1.3660656375814142
119119,238239,238238,476477,388.10665488243103,1.3573154180212441
120120,240241,240240,480481,391.4586720466614,1.3486810807407892
121121,242243,242242,484485,394.80032205581665,1.3401602062367601
122122,244245,244244,488489,398.1534209251404,1.3317504467686376
123123,246247,246246,492493,401.53087615966797,1.3234495235356007
124124,248249,248248,496497,404.8978831768036,1.3152552240135265
125125,250251,250250,500501,408.2493019104004,1.3071653994102235
126126,252253,252252,504505,411.6285629272461,1.2991779622261674
127127,254255,254254,508509,414.98873710632324,1.2912908839571173
128128,256257,256256,512513,418.5522770881653,1.2835021928895003
129129,258259,258258,516517,422.00322818756104,1.2758099720067548
130130,260261,260260,520521,425.4120318889618,1.2682123569720716
131131,262263,262262,524525,428.82167506217957,1.2607075342330063
132132,264265,264264,528529,432.25367283821106,1.2532937391861196
133133,266267,266266,532533,435.60822916030884,1.2459692544434802
134134,268269,268268,536537,438.95588302612305,1.2387324081482802
135135,270271,270270,540541,442.3473961353302,1.231581572406867
136136,272273,272272,544545,445.66022181510925,1.2245151617444208
137137,274275,274274,548549,449.0396149158478,1.2175316316606768
138138,276277,276276,552553,452.4190709590912,1.210629477231123
139139,278279,278278,556557,455.80640721321106,1.203807234252963
140140,280281,280280,560561,459.22365617752075,1.1970634843455628
141141,282283,282282,564565,462.57851219177246,1.1903968195019843
142142,284285,284284,568569,465.9542200565338,1.183805880296859
143143,286287,286286,572573,469.28914308547974,1.1772893407342053
144144,288289,288288,576577,472.66038608551025,1.1708459071760444
145145,290291,290290,580581,476.03202295303345,1.1644743172982999
146146,292293,292292,584585,479.38637804985046,1.1581733390994486
147147,294295,294294,588589,482.7508201599121,1.1519417699346377
148148,296297,296296,592593,486.1625039577484,1.1457784356171032
149149,298299,298298,596597,489.549467086792,1.139682189517771
150150,300301,300300,600601,492.9353940486908,1.1336519117212447
151151,302303,302302,604605,496.2657699584961,1.1276865082163567
152152,304305,304304,608609,499.63904213905334,1.1217849101067259
153153,306307,306306,612613,503.0036988258362,1.115946072854058
154154,308309,308308,616617,506.3337049484253,1.1101689755687403
155155,310311,310310,620621,509.69115591049194,1.1044526202786074
156156,312313,312312,624625,513.0185780525208,1.098796031288657
157157,314315,314314,628629,516.3923871517181,1.0931982545134815
158158,316317,316316,632633,519.7780499458313,1.0876583568588103
159159,318319,318318,636637,523.1113500595093,1.0821754256157874
160160,320321,320320,640641,526.6372430324554,1.0767485678879893
161161,322323,322322,644645,530.2866480350494,1.0713769100166246
162162,324325,324324,648649,533.878231048584,1.0660595970548457
163163,326327,326326,652653,537.6256220340729,1.060795792242061
164164,328329,328328,656657,541.4047222137451,1.0555846765000751
165165,330331,330330,660661,545.1133921146393,1.0504254479437805
166166,332333,332332,664665,548.7627398967743,1.0453173214173148
167167,334335,334334,668669,552.4034941196442,1.0402595280393143
168168,336337,336336,672673,556.0032680034637,1.0352513147627178
169169,338339,338338,676677,559.6603090763092,1.0302919439618563
170170,340341,340340,680681,563.2963900566101,1.0253806930068095
171171,342343,342342,684685,567.0131320953369,1.0205168538759608
172172,344345,344344,688689,570.6321818828583,1.015699732788562
173173,346347,346346,692693,574.2754790782928,1.010928649802736
174174,348349,348348,696697,577.9002590179443,1.0062029384862399
175175,350351,350350,700701,581.7117428779602,1.0015219455617625
176176,352353,352352,704705,585.4709711074829,0.996885030557678
177177,354355,354354,708709,589.0779950618744,0.9922915655006364
178178,356357,356356,712713,592.5787830352783,0.987740934604517
179179,358359,358358,716717,595.9621629714966,0.9832325339393719
180180,360361,360360,720721,599.3490009307861,0.9787657711694919
181181,362363,362362,724725,602.7297511100769,0.9743400652423588
182182,364365,364364,728729,606.2850348949432,0.9699548461194354
183183,366367,366366,732733,609.7261140346527,0.9656095545160497
184184,368369,368368,736737,613.0896182060242,0.9613036416285468
185185,370371,370370,740741,616.4897201061249,0.957036568885087
186186,372373,372372,744745,619.8710510730743,0.9528078077019018
187187,374375,374374,748749,623.2484550476074,0.9486168392577383
188188,376377,376376,752753,626.6407558917999,0.9444631542228308
189189,378379,378378,756757,630.0046188831329,0.9403462525897339
190190,380381,380380,760761,633.3550472259521,0.9362656434132077
191191,382383,382382,764765,636.6993730068207,0.9322208446174045
192192,384385,384384,768769,640.3359401226044,0.9282113827885041
193193,386387,386386,772773,643.7729740142822,0.9242367929746251
194194,388389,388388,776777,647.1301369667053,0.9202966184930119
195195,390391,390390,780781,650.4735469818115,0.9163904107372218
196196,392393,392392,784785,653.8405690193176,0.9125177290006832
197197,394395,394394,788789,657.2041940689087,0.9086781402911583
198198,396397,396396,792793,660.7060961723328,0.9048712191724917
199199,398399,398398,796797,664.1229629516602,0.9010965475772537
200200,400401,400400,800801,667.507698059082,0.8973537146557646
201201,402403,402402,804805,670.9252579212189,0.8936423166214809
202202,404405,404404,808809,674.2963480949402,0.8899619565836474
203203,406407,406406,812813,677.6612520217896,0.88631224439996
204204,408409,408408,816817,681.0209541320801,0.882692796538322
205205,410411,410410,820821,684.391340970993,0.8791032359258679
206206,412413,412412,824825,687.7638339996338,0.8755431918143586
207207,414415,414414,828829,691.1254751682281,0.8720122996455757
208208,416417,416416,832833,694.4621019363403,0.8685102009185357
209209,418419,418418,836837,697.8485040664673,0.8650365430548845
210210,420421,420420,840841,701.2496249675751,0.8615909792915772
211211,422423,422422,844845,704.6236679553986,0.8581731685408158
212212,424425,424424,848849,707.9734320640564,0.8547827752809098
213213,426427,426426,852853,711.3267171382904,0.8514194694416801
214214,428429,428428,856857,714.6813411712646,0.8480829262825864
215215,430431,430430,860861,718.0193269252777,0.844772826303597
216216,432433,432432,864865,721.374655008316,0.8414888551142212
217217,434435,434434,868869,724.8528828620911,0.8382307033425604
218218,436437,436436,872873,728.2444851398468,0.8349980665370822
219219,438439,438438,876877,731.6246929168701,0.831790645052024
220220,440441,440440,880881,735.2273609638214,0.828608143970996
221221,442443,442442,884885,738.6914300918579,0.8254502729978412
222222,444445,444444,888889,742.071918964386,0.8223167463711434
223223,446447,446446,892893,745.4358310699463,0.8192072827696393
224224,448449,448448,896897,748.7924220561981,0.8161216052340023
225225,450451,450450,900901,752.1633489131927,0.8130594410704362
226226,452453,452452,904905,755.5266008377075,0.8100205217797338
227227,454455,454454,908909,758.9174199104309,0.8070045829590526
228228,456457,456456,912913,762.2965738773346,0.8040113642418873
229229,458459,458458,916917,765.6575651168823,0.8010406092053017
230230,460461,460460,920921,769.0280282497406,0.798092065298988
231231,462463,462462,924925,772.4061622619629,0.7951654837706883
232232,464465,464464,928929,776.0323550701141,0.7922606196116249
233233,466467,466466,932933,779.5280990600586,0.7893772314455418
234234,468469,468468,936937,782.934005022049,0.7865150815032393
235235,470471,470470,940941,786.3252739906311,0.783673935526167
236236,472473,472472,944945,789.7139010429382,0.7808535627118545
237237,474475,474474,948949,793.0507960319519,0.7780537356538844
238238,476477,476476,952953,796.4339051246643,0.7752742302673141
239239,478479,478478,956957,799.8545939922333,0.7725148257377441
240240,480481,480480,960961,803.2699508666992,0.769775304450377
241241,482483,482482,964965,806.603226184845,0.7670554519481811
242242,484485,484484,968969,809.969969034195,0.7643550568573119
243243,486487,486486,972973,813.3335962295532,0.7616739108398178
244244,488489,488488,976977,816.7069182395935,0.7590118085390714
245245,490491,490490,980981,820.069827079773,0.7563685475179227
246246,492493,492492,984985,823.4068689346313,0.7537439282223204
247247,494495,494494,988989,826.8085732460022,0.7511377539121895
248248,496497,496496,992993,830.1401269435883,0.748549830617776
249249,498499,498498,996997,833.4972290992737,0.74597996709781
250250,500501,500500,1001001,836.8569231033325,0.7434279747849359
251251,502503,502502,1005005,840.5072209835052,0.7408936677329621
252252,504505,504504,1009009,843.9825720787048,0.7383768625822995
253253,506507,506506,1013013,847.4141201972961,0.7358773785126687
254254,508509,508508,1017017,850.7863600254059,0.7333950371867104
255255,510511,510510,1021021,854.1509220600128,0.7309296627227013
256256,512513,512512,1025025,857.5424630641937,0.728481081643622
257257,514515,514514,1029029,860.9196321964264,0.7260491228407773
258258,516517,516516,1033033,864.3220951557159,0.7236336175210454
259259,518519,518518,1037037,867.7470850944519,0.7212343991923262
260260,520521,520520,1041041,871.1157691478729,0.7188513035907818
261261,522523,522522,1045045,874.4563910961151,0.7164841686735599
262262,524525,524524,1049049,877.8185470104218,0.714132834564225
263263,526527,526526,1053053,881.2118310928345,0.7117971435236541
264264,528529,528528,1057057,884.523276090622,0.7094769399063807
265265,530531,530530,1061061,887.9046928882599,0.7071720701314916
266266,532533,532532,1065065,891.2346270084381,0.7048823826535227
267267,534535,534534,1069069,894.6149108409882,0.702607727915165
268268,536537,536536,1073073,897.9661061763763,0.7003479583236185
269269,538539,538538,1077077,901.308473110199,0.6981029282214877
270270,540541,540540,1081081,904.6992540359497,0.695872493841307
271271,542543,542542,1085085,908.2305750846863,0.6936565150772367
272272,544545,544544,1089089,911.732106924057,0.69145485284389
273273,546547,546546,1093093,915.1183550357819,0.6892673660986475
274274,548549,548548,1097097,918.6996750831604,0.6870939183736482
275275,550551,550550,1101101,922.2091271877289,0.684934374947261
276276,552553,552552,1105105,925.6223840713501,0.6827886028167995
277277,554555,554554,1109109,928.9731011390686,0.6806564706785139
278278,556557,556556,1113113,932.3276772499084,0.6785378488893912
279279,558559,558558,1117117,935.700660943985,0.6764326094489661
280280,560561,560560,1121121,939.1026139259338,0.6743406259774929
281281,562563,562562,1125125,942.4821639060974,0.6722617736741086
282282,564565,564564,1129129,945.8599548339844,0.670195929309557
283283,566567,566566,1133133,949.2152800559998,0.66814297118799
284284,568569,568568,1137137,952.6197249889374,0.6661028262296895
285285,570571,570570,1141141,956.0046892166138,0.6640753303618112
286286,572573,572572,1145145,959.3911850452423,0.6620603643441427
287287,574575,574574,1149149,962.763631105423,0.6600578124071035
288288,576577,576576,1153153,966.1357228755951,0.6580675601999246
289289,578579,578578,1157157,969.6664550304413,0.6560894947760971
290290,580581,580580,1161161,973.099356174469,0.6541235045751819
291291,582583,582582,1165165,976.526504278183,0.6521694793882489
292292,584585,584584,1169169,980.1560461521149,0.6502273103469633
293293,586587,586586,1173173,983.5919020175934,0.6482968899035768
294294,588589,588588,1177177,987.0322108268738,0.6463781118072802
295295,590591,590590,1181181,990.3867492675781,0.6444708710805571
296296,592593,592592,1185185,993.8054051399231,0.642575076311914
297297,594595,594594,1189189,997.1776139736176,0.640690647485826
298298,596597,596596,1193193,1000.591185092926,0.6388174483072362
299299,598599,598598,1197197,1003.963583946228,0.6369553787262703
300300,600601,600600,1201201,1007.3335862159729,0.6351043398735783
301301,602603,602602,1205205,1010.7249929904938,0.6332642340585153
302302,604605,604604,1209209,1014.0856392383575,0.6314349647345807
303303,606607,606606,1213213,1017.4567999839783,0.6296164364957804
304304,608609,608608,1217217,1020.8205301761627,0.6278085550547985
305305,610611,610610,1221221,1024.2042899131775,0.626011227213894
306306,612613,612612,1225225,1027.6432240009308,0.6242243608703575
307307,614615,614614,1229229,1031.0600640773773,0.6224478649855882
308308,616617,616616,1233233,1034.4196569919586,0.6206816495796375
309309,618619,618618,1237237,1037.800148010254,0.6189256257039233
310310,620621,620620,1241241,1041.2755720615387,0.6171797054375929
311311,622623,622622,1245245,1044.7565970420837,0.6154438018693327
312312,624625,624624,1249249,1048.1521210670471,0.6137178290755401
313313,626627,626626,1253253,1051.5177121162415,0.6120017021166859
314314,628629,628628,1257257,1054.9014410972595,0.6102953370227624
315315,630631,630630,1261261,1058.3065609931946,0.6085986507696362
316316,632633,632632,1265265,1061.6930689811707,0.6069115612717724
317317,634635,634634,1269269,1065.08141207695,0.6052339873767778
318318,636637,636636,1273273,1068.5339801311493,0.6035658488362969
319319,638639,638638,1277277,1071.9323508739471,0.601907066304193
320320,640641,640640,1281281,1075.285269021988,0.600257561321996
321321,642643,642642,1285285,1078.618835926056,0.598617256309808
322322,644645,644644,1289289,1082.011085987091,0.5969860745371989
323323,646647,646646,1293293,1085.4230251312256,0.5953639401413966
324324,648649,648648,1297297,1088.8410642147064,0.5937507780836313
325325,650651,650650,1301301,1092.2596819400787,0.5921465141636872
326326,652653,652652,1305305,1095.597468137741,0.59055107498898
327327,654655,654654,1309309,1098.9957301616669,0.5889643879727373
328328,656657,656656,1313313,1102.391086101532,0.5873863813285425
329329,658659,658658,1317317,1105.7198450565338,0.5858169840430492
330330,660661,660660,1321321,1109.084200143814,0.5842561258796195
331331,662663,662662,1325325,1112.4535059928894,0.5827037373655912
332332,664665,664664,1329329,1115.8434429168701,0.5811597497722687
333333,666667,666666,1333333,1119.262332201004,0.579624096817497
334334,668669,668668,1337337,1122.6017799377441,0.5780967098526162
335335,670671,670670,1341341,1125.9576160907745,0.5765775220243086
336336,672673,672672,1345345,1129.3167350292206,0.5750664675160806
337337,674675,674674,1349349,1132.7102301120758,0.5735634812099306
338338,676677,676676,1353353,1136.0885019302368,0.5720684986827109
339339,678679,678678,1357357,1139.4493429660797,0.5705814561933948
340340,680681,680680,1361361,1142.8282051086426,0.5691022906794387
341341,682683,682682,1365365,1146.2347598075867,0.5676309397367731
342342,684685,684684,1369369,1149.6499891281128,0.5661673416252597
343343,686687,686686,1373373,1153.2633850574493,0.5647114352486824
344344,688689,688688,1377377,1156.700112104416,0.5632631601565663
345345,690691,690690,1381381,1160.0933949947357,0.561822456516893
346346,692693,692692,1385385,1163.651391029358,0.5603892651361093
347347,694695,694694,1389389,1167.113940000534,0.5589635274282045
348348,696697,696696,1393393,1170.505089044571,0.5575451854147104
349349,698699,698698,1397397,1173.8741590976715,0.5561341817137873
350350,700701,700700,1401401,1177.2280750274658,0.5547304595420428
351351,702703,702702,1405405,1180.6470310688019,0.5533339626927045
352352,704705,704704,1409409,1184.025645017624,0.5519446355392574
353353,706707,706706,1413413,1187.407263994217,0.5505624230263493
354354,708709,708708,1417417,1190.9242029190063,0.5491872706552385
355355,710711,710710,1421421,1194.3252770900726,0.5478191244856134
356356,712713,712712,1425425,1197.747689962387,0.546457931124678
357357,714715,714714,1429429,1201.155117034912,0.5451036377162382
358358,716717,716716,1433433,1204.535180091858,0.5437561919443397
359359,718719,718718,1437437,1207.9677481651306,0.5424155420096213
360360,720721,720720,1441441,1211.4043881893158,0.5410816366511426
361361,722723,722722,1445445,1214.7837669849396,0.5397544251045474
362362,724725,724724,1449449,1218.1864140033722,0.5384338571184344
363363,726727,726726,1453453,1221.5774099826813,0.5371198829452624
364364,728729,728728,1457457,1224.936005115509,0.5358124533304363
365365,730731,730730,1461461,1228.3306999206543,0.5345115195086692
366366,732733,732732,1465465,1231.7320351600647,0.5332170331967063
367367,734735,734734,1469469,1235.1118111610413,0.5319289465933252
368368,736737,736736,1473473,1238.5176088809967,0.5306472123538697
369369,738739,738738,1477477,1241.9018650054932,0.5293717836175347
370370,740741,740740,1481481,1245.311653137207,0.5281026139691676
371371,742743,742742,1485485,1248.7815110683441,0.5268396574556391
372372,744745,744744,1489489,1252.2536931037903,0.5255828685676533
373373,746747,746746,1493493,1255.6491861343384,0.5243322022361099
374374,748749,748748,1497497,1258.9972231388092,0.5230876138375606
375375,750751,750750,1501501,1262.3740680217743,0.5218490591742011
376376,752753,752752,1505505,1265.7638750076294,0.5206164944756893
377377,754755,754754,1509509,1269.1721048355103,0.5193898763991456
378378,756757,756756,1513513,1272.6650390625,0.5181691620091442
379379,758759,758758,1517517,1276.0815060138702,0.5169543087922648
380380,760761,760760,1521521,1279.4894251823425,0.5157452746316267
381381,762763,762762,1525525,1282.8786540031433,0.5145420178196218
382382,764765,764764,1529529,1286.265172958374,0.5133444970433629
383383,766767,766766,1533533,1289.6290171146393,0.5121526713846833
384384,768769,768768,1537537,1293.0072009563446,0.5109665003074042
385385,770771,770770,1541541,1296.3908989429474,0.5097859436627914
386386,772773,772772,1545545,1299.7843210697174,0.5086109616822796
387387,774775,774774,1549549,1303.1494460105896,0.5074415149701963
388388,776777,776776,1553553,1306.5282800197601,0.5062775644964859
389389,778779,778778,1557557,1309.9305529594421,0.5051190716003475
390390,780781,780780,1561561,1313.298245191574,0.5039659979847784
391391,782783,782782,1565565,1316.6457741260529,0.5028183057038405
392392,784785,784784,1569569,1320.0241179466248,0.5016759571699367
393393,786787,786786,1573573,1323.3949010372162,0.5005389151428972
394394,788789,788788,1577577,1326.8907070159912,0.4994071427208837
395395,790791,790790,1581581,1330.2834889888763,0.4982806033567613
396396,792793,792792,1585585,1333.6571769714355,0.4971592608235369
397397,794795,794794,1589589,1337.079801082611,0.4960430792380066
398398,796797,796796,1593593,1340.4579050540924,0.49493202304438455
399399,798799,798798,1597597,1343.820692062378,0.49382605701430293
400400,800801,800800,1601601,1347.1832721233368,0.49272514623226016
401401,802803,802802,1605605,1350.5456838607788,0.49162925610653474
402402,804805,804804,1609609,1353.9066090583801,0.49053835236372834
403403,806807,806806,1613613,1357.3299131393433,0.4894524010378518
404404,808809,808808,1617617,1360.708335161209,0.48837136846850626
405405,810811,810810,1621621,1364.08145403862,0.487295221297245
406406,812813,812812,1625625,1367.4637911319733,0.4862239264712116
407407,814815,814814,1629629,1370.8378620147705,0.48515745123586385
408408,816817,816816,1633633,1374.2190399169922,0.4840957631222409
409409,818819,818818,1637637,1377.5917942523956,0.48303882995787717
410410,820821,820820,1641641,1380.9593279361725,0.4819866198595264
411411,822823,822822,1645645,1384.3283610343933,0.4809391012222477
412412,824825,824824,1649649,1387.7027230262756,0.47989624272122455
413413,826827,826826,1653653,1391.1043419837952,0.4788580133172218
414414,828829,828828,1657657,1394.5759179592133,0.47782438223657664
415415,830831,830830,1661661,1398.1670560836792,0.47679531898756977
416416,832833,832832,1665665,1401.5765590667725,0.4757707933349593
417417,834835,834834,1669669,1404.94952917099,0.47475077531998977
418418,836837,836836,1673673,1408.333503961563,0.4737352352367452
419419,838839,838838,1677677,1411.88250207901,0.4727241436503391
420420,840841,840840,1681681,1415.2967541217804,0.47171747137326747
421421,842843,842842,1685685,1418.6966540813446,0.47071518947632285
422422,844845,844844,1689689,1422.0706779956818,0.4697172692813183
423423,846847,846846,1693693,1425.4447238445282,0.4687236823610874
424424,848849,848848,1697697,1428.8106470108032,0.4677344005303894
425425,850851,850850,1701701,1432.3180830478668,0.466749395849547
426426,852853,852852,1705705,1435.74964594841,0.4657686406208086
427427,854855,854854,1709709,1439.1310300827026,0.4647921073847101
428428,856857,856856,1713713,1442.5005822181702,0.4638197689109802
429429,858859,858858,1717717,1445.8947441577911,0.4628515982112731
430430,860861,860860,1721721,1449.3246488571167,0.46188756852461665
431431,862863,862862,1725725,1452.665402173996,0.4609276533155935
432432,864865,864864,1729729,1456.1401541233063,0.45997182627615985
433433,866867,866866,1733733,1459.7335422039032,0.45902006132564566
434434,868869,868868,1737737,1463.0926389694214,0.4580723325998406
435435,870871,870870,1741741,1466.4601788520813,0.45712861445099406
436436,872873,872872,1745745,1469.8692269325256,0.4561888814550912
437437,874875,874874,1749749,1473.2491850852966,0.45525310839548183
438438,876877,876876,1753753,1476.621304988861,0.45432127027197566
439439,878879,878878,1757757,1480.016680240631,0.4533933422899281
440440,880881,880880,1761761,1483.3832612037659,0.4524692998602404
441441,882883,882882,1765765,1486.7476551532745,0.4515491186102736
442442,884885,884884,1769769,1490.132167816162,0.45063277436020144
443443,886887,886886,1773773,1493.510525226593,0.4497202431321057
444444,888889,888888,1777777,1496.8557019233704,0.4488115011517948
445445,890891,890890,1781781,1500.2177908420563,0.4479065248378902
446446,892893,892892,1785785,1503.599837064743,0.44700529080182605
447447,894895,894894,1789789,1506.9877400398254,0.4461077758551255
448448,896897,896896,1793793,1510.3705899715424,0.44521395699484856
449449,898899,898898,1797797,1513.742301940918,0.4443238114090491
450450,900901,900900,1801801,1517.3394010066986,0.44343731646586093
451451,902903,902902,1805805,1520.8537871837616,0.44255444973350677
452452,904905,904904,1809809,1524.2098789215088,0.4416751889493753
453453,906907,906906,1813813,1527.5746638774872,0.4407995120345731
454454,908909,908908,1817817,1530.9773349761963,0.4399273970957438
455455,910911,910910,1821821,1534.3181371688843,0.43905882241051586
456456,912913,912912,1825825,1537.693589925766,0.4381937664365978
457457,914915,914914,1829829,1541.1089782714844,0.4373322078045021
458458,916917,916916,1833833,1544.4412100315094,0.43647412531572627
459459,918919,918918,1837837,1547.7976701259613,0.43561949794639077
460460,920921,920920,1841841,1551.3545660972595,0.43476830483268714
461461,922923,922922,1845845,1554.7896182537079,0.4339205252890679
462462,924925,924924,1849849,1558.1657631397247,0.4330761387864186
463463,926927,926926,1853853,1561.5341351032257,0.4322351249647909
464464,928929,928928,1857857,1564.9183349609375,0.4313974636261264
465465,930931,930930,1861861,1568.3503921031952,0.43056313472698093
466466,932933,932932,1865865,1571.7117512226105,0.4297321183948952
467467,934935,934934,1869869,1575.0979239940643,0.4289043948992912
468468,936937,936936,1873873,1578.5756721496582,0.4280799446769379
469469,938939,938938,1877877,1581.9469921588898,0.4272587483173993
470470,940941,940940,1881881,1585.3254890441895,0.42644078655757767
471471,942943,942942,1885885,1588.688971042633,0.4256260402926273
472472,944945,944944,1889889,1592.0791511535645,0.42481449056140264
473473,946947,946946,1893893,1595.430163860321,0.42400611855555326
474474,948949,948948,1897897,1598.8222980499268,0.4232009056122479
475475,950951,950950,1901901,1602.2013220787048,0.4223988332123554
476476,952953,952952,1905905,1605.5527811050415,0.4215998829822638
477477,954955,954954,1909909,1608.9235849380493,0.42080403669388033
478478,956957,956956,1913913,1612.2911150455475,0.42001127625553636
479479,958959,958958,1917917,1615.7177629470825,0.41922158371380647
480480,960961,960960,1921921,1619.217199087143,0.4184349477854994
481481,962963,962962,1925925,1622.626827955246,0.41765134872730414
482482,964965,964964,1929929,1625.9582540988922,0.416870764514897
483483,966967,966966,1933933,1629.4169840812683,0.4160931777423684
484484,968969,968968,1937937,1632.787768125534,0.41531857114023296
485485,970971,970970,1941941,1636.1376218795776,0.41454692757179146
486486,972973,972972,1945945,1639.5582990646362,0.413778230025855
487487,974975,974974,1949949,1642.981761932373,0.4130124616294779
488488,976977,976976,1953953,1646.4137270450592,0.41224960563158675
489489,978979,978978,1957957,1649.7780630588531,0.41148964540661837
490490,980981,980980,1961961,1653.1470499038696,0.41073256446361484
491491,982983,982982,1965965,1656.556146144867,0.40997834642803355
492492,984985,984984,1969969,1659.9266090393066,0.40922697505084216
493493,986987,986986,1973973,1663.2873899936676,0.4084784342085186
494494,988989,988988,1977977,1666.666246175766,0.4077327078957751
495495,990991,990990,1981981,1670.05025100708,0.4069897802291962
496496,992993,992992,1985985,1673.4470179080963,0.40624963543996273
497497,994995,994994,1989989,1677.0118010044098,0.40551225788294687
498498,996997,996996,1993993,1680.4127180576324,0.4047776320276171
499499,998999,998998,1997997,1683.7947421073914,0.40404574245985714
500501,1001003,1001002,2002005,1687.1817910671234,0.40331584678824584
501502,1003005,1003004,2006009,1690.5530202388763,0.4025893866964907
502503,1005007,1005006,2010013,1693.931361913681,0.4018656173157069
503504,1007009,1007008,2014017,1697.275573015213,0.4011445236774307
504505,1009011,1009010,2018021,1700.7595779895782,0.40042609093325154
505506,1011013,1011012,2022025,1704.159070968628,0.39971030433662236
506507,1013015,1013014,2026029,1707.5012340545654,0.3989971492537734
507508,1015017,1015016,2030033,1710.8516750335693,0.39828661115825525
508509,1017019,1017018,2034037,1714.2338600158691,0.397578675627301
509510,1019021,1019020,2038041,1717.5996358394623,0.39687332834910194
510511,1021023,1021022,2042045,1720.9947061538696,0.39617055510643695
511512,1023025,1023024,2046049,1724.4365780353546,0.39547034179668117
512513,1025027,1025026,2050053,1727.8214619159698,0.3947726744117972
513514,1027029,1027028,2054057,1731.1880459785461,0.39407753904743004
514515,1029031,1029030,2058061,1734.5438680648804,0.39338492190472607
515516,1031033,1031032,2062065,1737.890098810196,0.39269480927941913
516517,1033035,1033034,2066069,1741.23983502388,0.3920071875636495
517518,1035037,1035036,2070073,1744.6083459854126,0.3913220432586968
518519,1037039,1037038,2074077,1748.0133900642395,0.3906393629476952
519520,1039041,1039040,2078081,1751.3971590995789,0.3899591333247372
520521,1041043,1041042,2082085,1754.7799479961395,0.3892813411694078
521522,1043045,1043044,2086089,1758.1474349498749,0.3886059733613365
522523,1045047,1045046,2090093,1761.508173942566,0.38793301686928316
523524,1047049,1047048,2094097,1764.895262002945,0.38726245875841414
524525,1049051,1049050,2098101,1768.2391290664673,0.38659428618302627
525526,1051053,1051052,2102105,1771.6108231544495,0.3859284863956418
526527,1053055,1053054,2106109,1775.0224702358246,0.38526504672881856
527528,1055057,1055056,2110113,1778.4600219726562,0.38460395461333974
528529,1057059,1057058,2114117,1781.8041641712189,0.38394519756548107
529530,1059061,1059060,2118121,1785.1538980007172,0.3832887631870108
530531,1061063,1061062,2122125,1788.4889421463013,0.38263463917064655
531532,1063065,1063064,2126129,1791.859111070633,0.3819828132964176
532533,1065067,1065066,2130133,1795.2098460197449,0.3813332734280266
533534,1067069,1067068,2134137,1798.5597059726715,0.38068600751103077
534535,1069071,1069070,2138141,1801.920240163803,0.3800410035819368
535536,1071073,1071072,2142145,1805.2724740505219,0.379398249757287
536537,1073075,1073074,2146149,1808.8733191490173,0.378757734237297
537538,1075077,1075076,2150153,1812.2304000854492,0.3781194453022181
538539,1077079,1077078,2154157,1815.5827980041504,0.3774833713177941
539540,1079081,1079080,2158161,1818.9522202014923,0.3768495007225283
540541,1081083,1081082,2162165,1822.3107991218567,0.37621782204405463
541542,1083085,1083084,2166169,1825.6728081703186,0.3755883238845854
542543,1085087,1085086,2170173,1829.034420967102,0.3749609949281876
543544,1087089,1087088,2174177,1832.3787188529968,0.37433582393168763
544545,1089091,1089090,2178181,1835.7401220798492,0.3737127997319476
545546,1091093,1091092,2182185,1839.1343200206757,0.37309191124404606
546547,1093095,1093094,2186189,1842.5074679851532,0.3724731474540022
547548,1095097,1095096,2190193,1845.8994369506836,0.3718564974333276
548549,1097099,1097098,2194197,1849.2351830005646,0.37124195031537965
549550,1099101,1099100,2198201,1852.5999548435211,0.37062949531537015
550551,1101103,1101102,2202205,1856.098776102066,0.3700191217194515
551552,1103105,1103104,2206209,1859.6253590583801,0.3694108188901737
552553,1105107,1105106,2210213,1863.234887123108,0.36880457625738927
553554,1107109,1107108,2214217,1866.7449898719788,0.3682003833237104
554555,1109111,1109110,2218221,1870.1096940040588,0.36759822966450884
555556,1111113,1111112,2222225,1873.4557139873505,0.3669981049224589
556557,1113115,1113114,2226229,1876.8299272060394,0.36639999881299445
557558,1115117,1115116,2230233,1880.2174680233002,0.36580390112067107
558559,1117119,1117118,2234237,1883.6823971271515,0.36520980169734685
559560,1119121,1119120,2238241,1887.0877480506897,0.3646176904621825
560561,1121123,1121122,2242245,1890.4485051631927,0.3640275574016414
561562,1123125,1123124,2246249,1893.791172027588,0.3634393925731274
562563,1125127,1125126,2250253,1897.1706840991974,0.3628531860958901
563564,1127129,1127128,2254257,1900.5642449855804,0.3622689281583007
564565,1129131,1129130,2258261,1903.9287440776825,0.3616866090105759
565566,1131133,1131132,2262265,1907.2722401618958,0.3611062189684162
566567,1133135,1133134,2266269,1910.6520040035248,0.3605277484111866
567568,1135137,1135136,2270273,1914.0281131267548,0.3599511877873738
568569,1137139,1137138,2274277,1917.3933959007263,0.359376527603672
569570,1139141,1139140,2278281,1920.7192702293396,0.35880375842680223
570571,1141143,1141142,2282285,1924.134595155716,0.358232870892607
571572,1143145,1143144,2286289,1927.5581622123718,0.3576638556914986
572573,1145147,1145146,2290293,1930.923723936081,0.35709670357937284
573574,1147149,1147148,2294297,1934.2613968849182,0.3565314053739712
574575,1149151,1149150,2298301,1937.639820098877,0.3559679519457859
575576,1151153,1151152,2302305,1941.0033469200134,0.3554063342326117
576577,1153155,1153154,2306309,1944.3695652484894,0.35484654323227005
577578,1155157,1155156,2310313,1947.7161540985107,0.35428856998805713
578579,1157159,1157158,2314317,1951.0659592151642,0.35373240562148567
579580,1159161,1159160,2318321,1954.4286110401154,0.35317804129226715
580581,1161163,1161162,2322325,1957.7855741977692,0.3526254682274157
581582,1163165,1163164,2326329,1961.1701180934906,0.35207467771215306
582583,1165167,1165166,2330333,1964.5303490161896,0.3515256610880897
583584,1167169,1167168,2334337,1967.9034061431885,0.35097840974231076
584585,1169171,1169170,2338341,1971.279303073883,0.35043291512920405
585586,1171173,1171172,2342345,1974.6387860774994,0.34988916875227005
586587,1173175,1173174,2346349,1978.0740330219269,0.34934716216957895
587588,1175177,1175176,2350353,1981.588702917099,0.34880688699922757
588589,1177179,1177178,2354357,1984.9506101608276,0.3482683349029685
589590,1179181,1179180,2358361,1988.397912979126,0.3477314976043999
590591,1181183,1181182,2362365,1991.7318680286407,0.3471963668744138
591592,1183185,1183184,2366369,1995.0759191513062,0.3466629345421097
592593,1185187,1185186,2370373,1998.445270061493,0.34613119247842405
593594,1187189,1187188,2374377,2001.792839050293,0.3456011326161388
594595,1189191,1189190,2378381,2005.227833032608,0.3450727469371486
595596,1191193,1191192,2382385,2008.6343100070953,0.344546027468823
596597,1193195,1193194,2386389,2011.9763250350952,0.34402096629492007
597598,1195197,1195196,2390393,2015.3509600162506,0.34349755554467265
598599,1197199,1197198,2394397,2018.731775045395,0.3429757873964263
599600,1199201,1199200,2398401,2022.1155200004578,0.3424556540867343
600601,1201203,1201202,2402405,2025.4644401073456,0.3419371478885296
601602,1203205,1203204,2406409,2028.8533251285553,0.3414202611293149
602603,1205207,1205206,2410413,2032.3412871360779,0.34090498618570564
603604,1207209,1207208,2414417,2035.984040260315,0.34039131547979196
604605,1209211,1209210,2418421,2039.3360719680786,0.3398792414791387
605606,1211213,1211212,2422425,2042.8997418880463,0.33936875670224254
606607,1213215,1213214,2426429,2046.400285243988,0.3388598537130747
607608,1215217,1215216,2430433,2049.9058690071106,0.3383525251192623
608609,1217219,1217218,2434437,2053.5013670921326,0.33784676358118304
609610,1219221,1219220,2438441,2056.9407448768616,0.33734256179377553
610611,1221223,1221222,2442445,2060.284926891327,0.336839912501091
611612,1223225,1223224,2446449,2063.6505908966064,0.33633880850356945
612613,1225227,1225226,2450453,2067.0431730747223,0.33583924262529763
613614,1227229,1227228,2454457,2070.412915945053,0.335341207754027
614615,1229231,1229230,2458461,2073.779750108719,0.3348446968066128
615616,1231233,1231232,2462465,2077.14878988266,0.334349702749023
616617,1233235,1233234,2466469,2080.555762052536,0.3338562185981573
617618,1235237,1235236,2470473,2083.9463160037994,0.3333642374000192
618619,1237239,1237238,2474477,2087.267650127411,0.33287375224790594
619620,1239241,1239240,2478481,2090.6233110427856,0.3323847562824085
620621,1241243,1241242,2482485,2093.9820070266724,0.3318972426804976
621622,1243245,1243244,2486489,2097.339067220688,0.3314112046627997
622623,1245247,1245246,2490493,2100.678771018982,0.33092663548995915
623624,1247249,1247248,2494497,2104.021341085434,0.3304435284644569
624625,1249251,1249250,2498501,2107.419296979904,0.32996187692697276
625626,1251253,1251252,2502505,2110.7946910858154,0.32948167426366126
626627,1253255,1253254,2506509,2114.139986038208,0.32900291388978076
627628,1255257,1255256,2510513,2117.4896681308746,0.32852558927879727
628629,1257259,1257258,2514517,2121.024085044861,0.3280496939241857
629630,1259261,1259260,2518521,2124.465791940689,0.3275752213667147
630631,1261263,1261262,2522525,2127.860044002533,0.3271021651908086
631632,1263265,1263264,2526529,2131.213238954544,0.3266305190118146
632633,1265267,1265266,2530533,2134.566848039627,0.3261602764832787
633634,1267269,1267268,2534537,2137.8767850399017,0.3256914313042216
634635,1269271,1269270,2538541,2141.266860961914,0.32522397720276786
635636,1271273,1271272,2542545,2144.640009880066,0.3247579079470597
636637,1273275,1273274,2546549,2148.1144580841064,0.3242932173452573
637638,1275277,1275276,2550553,2151.4587371349335,0.32382989924008143
638639,1277279,1277278,2554557,2154.801856994629,0.3233679475088138
639640,1279281,1279280,2558561,2158.328602075577,0.32290735606875387
640641,1281283,1281282,2562565,2161.8712430000305,0.3224481188735808
641642,1283285,1283284,2566569,2165.250603914261,0.32199022990425874
642643,1285287,1285286,2570573,2168.695286989212,0.3215336831872264
643644,1287289,1287288,2574577,2172.0821759700775,0.32107847278166446
644645,1289291,1289290,2578581,2175.410719871521,0.3206245927776763
645646,1291293,1291292,2582585,2178.8270609378815,0.32017203730538313
646647,1293295,1293294,2586589,2182.17210316658,0.319720800522191
647648,1295297,1295296,2590593,2185.5873651504517,0.31927087662734266
648649,1297299,1297298,2594597,2188.9961841106415,0.31882225985100376
649650,1299301,1299300,2598601,2192.333983898163,0.3183749444579007
650651,1301303,1301302,2602605,2195.665757894516,0.31792892474004475
651652,1303305,1303304,2606609,2199.08566904068,0.3174841950312839
652653,1305307,1305306,2610613,2202.4744679927826,0.31704074969638896
653654,1307309,1307308,2614617,2205.8266520500183,0.3165985831274156
654655,1309311,1309310,2618621,2209.205556869507,0.3161576897564373
655656,1311313,1311312,2622625,2212.557543039322,0.31571806404099334
656657,1313315,1313314,2626629,2215.9236381053925,0.31527970047318377
657658,1315317,1315316,2630633,2219.254872083664,0.3148425935814885
658659,1317319,1317318,2634637,2222.6059839725494,0.3144067379180342
659660,1319321,1319320,2638641,2226.013684988022,0.31397212807314645
660661,1321323,1321322,2642645,2229.454020023346,0.3135387586626166
661662,1323325,1323324,2646649,2232.8413190841675,0.3131066243367968
662663,1325327,1325326,2650653,2236.157840013504,0.3126757197751431
663664,1327329,1327328,2654657,2239.506791114807,0.3122460396916722
664665,1329331,1329330,2658661,2242.912905931473,0.31181757882040984
665666,1331333,1331332,2662665,2246.2385201454163,0.31139033193539944
666667,1333335,1333334,2666669,2249.7143778800964,0.3109642938379693
667668,1335337,1335336,2670673,2253.204118013382,0.31053945935491356
668669,1337339,1337338,2674677,2256.5722510814667,0.31011582334940613
669670,1339341,1339340,2678681,2259.972468852997,0.3096933807100868
670671,1341343,1341342,2682685,2263.3332200050354,0.30927212634924217
671672,1343345,1343344,2686689,2266.697729110718,0.3088520552173577
672673,1345347,1345346,2690693,2270.0625789165497,0.30843316229038464
673674,1347349,1347348,2694697,2273.423803091049,0.3080154425679211
674675,1349351,1349350,2698701,2276.9188120365143,0.3075988910823071
675676,1351353,1351352,2702705,2280.2916688919067,0.3071835028949863
676677,1353355,1353354,2706709,2283.6352281570435,0.3067692730928684
677678,1355357,1355356,2710713,2287.0023560523987,0.3063561967865098
678679,1357359,1357358,2714717,2290.52419090271,0.3059442691210279
679680,1359361,1359360,2718721,2293.896686077118,0.30553348526336777
680681,1361363,1361362,2722725,2297.2694520950317,0.3051238404150354
681682,1363365,1363364,2726729,2300.633684873581,0.3047153297939076
682683,1365367,1365366,2730733,2303.9877190589905,0.30430794865242206
683684,1367369,1367368,2734737,2307.3513741493225,0.3039016922630253
684685,1369371,1369370,2738741,2310.707309961319,0.3034965559345437
685686,1371373,1371372,2742745,2314.0936958789825,0.3030925349867175
686687,1373375,1373374,2746749,2317.4495549201965,0.3026896247829427
687688,1375377,1375376,2750753,2320.869183063507,0.30228782069752924
688689,1377379,1377378,2754757,2324.212774038315,0.3018871181375289
689690,1379381,1379380,2758761,2327.5507140159607,0.30148751253182127
690691,1381383,1381382,2762765,2330.93310213089,0.30108899934020883
691692,1383385,1383384,2766769,2334.2760100364685,0.3006915740443219
692693,1385387,1385386,2770773,2337.6308290958405,0.3002952321457997
693694,1387389,1387388,2774777,2340.991136074066,0.2998999691753852
694695,1389391,1389390,2778781,2344.3373968601227,0.2995057806947443
695696,1391393,1391392,2782785,2347.712677001953,0.29911266227645683
696697,1393395,1393394,2786789,2351.0798461437225,0.2987206095276633
697698,1395397,1395396,2790793,2354.4177589416504,0.2983296180755133
698699,1397399,1397398,2794797,2357.7702808380127,0.297939683572622
699700,1399401,1399400,2798801,2361.131005048752,0.29755080169161374
700701,1401403,1401402,2802805,2364.4767541885376,0.2971629681360355
701702,1403405,1403404,2806809,2367.8547780513763,0.2967761786221672
702703,1405407,1405406,2810813,2371.204808950424,0.2963904288972117
703704,1407409,1407408,2814817,2374.5740809440613,0.2960057147338375
704705,1409411,1409410,2818821,2377.9120790958405,0.2956220319174463
705706,1411413,1411412,2822825,2381.3382320404053,0.29523937626800034
706707,1413415,1413414,2826829,2384.7183549404144,0.29485774361819495
707708,1415417,1415416,2830833,2388.0639169216156,0.29447712982619123
708709,1417419,1417418,2834837,2391.651927947998,0.29409753077925416
709710,1419421,1419420,2838841,2395.1327199935913,0.29371894237192464
710711,1421423,1421422,2842845,2398.5071761608124,0.29334136054058035
711712,1423425,1423424,2846849,2402.081199169159,0.29296478122341796
712713,1425427,1425426,2850853,2405.6084489822388,0.2925892003950139
713714,1427429,1427428,2854857,2409.0300059318542,0.29221461404631555
714715,1429431,1429430,2858861,2412.392151117325,0.28934317169296264
715716,1431433,1431432,2862865,2415.7891709804535,0.2889771243899304
716717,1433435,1433434,2866869,2419.216155052185,0.28861203355882026
717718,1435437,1435436,2870873,2422.610813856125,0.2882478954070393
718719,1437439,1437438,2874877,2425.969412088394,0.2878847061692795
719720,1439441,1439440,2878881,2429.3452010154724,0.2875224620984227
720721,1441443,1441442,2882885,2432.717878103256,0.28716115946917853
721722,1443445,1443444,2886889,2436.090409040451,0.28680079457262764
722723,1445447,1445446,2890893,2439.503361940384,0.2864413637216785
723724,1447449,1447448,2894897,2442.898943901062,0.28608286325106747
724725,1449451,1449450,2898901,2446.271213054657,0.28572528950462583
725726,1451453,1451452,2902905,2449.633125066757,0.2853686388571077
726727,1453455,1453454,2906909,2453.0142681598663,0.2850129076978192
727728,1455457,1455456,2910913,2456.3657462596893,0.2846580924306181
728729,1457459,1457458,2914917,2459.7601788043976,0.2843041894848284
729730,1459461,1459460,2918921,2463.1284441947937,0.28395119530432567
730731,1461463,1461462,2922925,2466.490084171295,0.28359910635481356
731732,1463465,1463464,2926929,2470.0240280628204,0.2832479191110906
732733,1465467,1465466,2930933,2473.6027760505676,0.28289763007705915
733734,1467469,1467468,2934937,2476.9943709373474,0.2825482357711735
734735,1469471,1469470,2938941,2480.340672016144,0.2821997327300778
735736,1471473,1471472,2942945,2483.7059800624847,0.2818521175049682
736737,1473475,1473474,2946949,2487.084962129593,0.2815053866652306
737738,1475477,1475476,2950953,2490.4406900405884,0.2811595368057169
738739,1477479,1477478,2954957,2493.7940349578857,0.2808145645303739
739740,1479481,1479480,2958961,2497.1569719314575,0.2804704664613382
740741,1481483,1481482,2962965,2500.5731461048126,0.28012723924075544
741742,1483485,1483484,2966969,2503.946943998337,0.27978487952896103
742743,1485487,1485486,2970973,2507.2911059856415,0.27944338399902335
743744,1487489,1487488,2974977,2510.685173034668,0.2791027493458387
744745,1489491,1489490,2978981,2514.080318927765,0.27876297227703617
745746,1491493,1491492,2982985,2517.6956651210785,0.2784240495184349
746747,1493495,1493494,2986989,2521.1871070861816,0.27808597781586286
747748,1495497,1495496,2990993,2524.6107420921326,0.2777487539242429
748749,1497499,1497498,2994997,2527.9800980091095,0.27741237462396384
749750,1499501,1499500,2999001,2531.3771991729736,0.27707683670269034
750751,1501503,1501502,3003005,2534.7858860492706,0.276742136971734
751752,1503505,1503504,3007009,2538.16086602211,0.2764082722533203
752753,1505507,1505506,3011013,2541.553727865219,0.2760752393896837
753754,1507509,1507508,3015017,2545.0043001174927,0.27574303523942945
754755,1509511,1509510,3019021,2548.383980035782,0.27541165666480083
755756,1511513,1511512,3023025,2552.0661318302155,0.2750811005662399
756757,1513515,1513514,3027029,2555.7843730449677,0.27475136384236976
757758,1515517,1515516,3031033,2559.533720970154,0.2744224434118223
758759,1517519,1517518,3035037,2563.157033920288,0.27409433620778145
759760,1519521,1519520,3039041,2566.7588169574738,0.27376703918162093
760761,1521523,1521522,3043045,2570.3411650657654,0.2734405493010854
761762,1523525,1523524,3047049,2573.9864749908447,0.2731148635430145
762763,1525527,1525526,3051053,2577.5588459968567,0.2727899789042567
763764,1527529,1527528,3055057,2581.1544020175934,0.27246589239439345
764765,1529531,1529530,3059061,2584.8474581241608,0.27214260103937704
765766,1531533,1531532,3063065,2588.482245206833,0.27182010187789274
766767,1533535,1533534,3067069,2592.0653080940247,0.2714983919668157
767768,1535537,1535536,3071073,2595.622400045395,0.271177468372116
768769,1537539,1537538,3075077,2599.2273259162903,0.2708573281815916
769770,1539541,1539540,3079081,2602.817052125931,0.2705379684921354
770771,1541543,1541542,3083085,2606.3905210494995,0.2702193864133733
771772,1543545,1543544,3087089,2609.959550857544,0.2699015790785779
772773,1545547,1545546,3091093,2613.535094022751,0.269584543622841
773774,1547549,1547548,3095097,2617.1148788928986,0.26926827719944413
774775,1549551,1549550,3099101,2620.513969182968,0.2689527769853157
775776,1551553,1551552,3103105,2624.1668961048126,0.26863804015920323
776777,1553555,1553554,3107109,2627.6366720199585,0.268324063912587
777778,1555557,1555556,3111113,2631.012889146805,0.26801084546423226
778779,1557559,1557558,3115117,2634.414423942566,0.2676983820329042
779780,1559561,1559560,3119121,2637.798586130142,0.26738667086101486
780781,1561563,1561562,3123125,2641.1510379314423,0.2670757091946143
781782,1563565,1563564,3127129,2644.6304800510406,0.2667654943015805
782783,1565567,1565566,3131133,2648.093371152878,0.2664560234588862
783784,1567569,1567568,3135137,2651.4855558872223,0.26614729395623726
784785,1569571,1569570,3139141,2654.877767801285,0.2658393030978914
785786,1571573,1571572,3143145,2658.2160880565643,0.26553204820629617
786787,1573575,1573574,3147149,2661.5844221115112,0.2652255266020802
787788,1575577,1575576,3151153,2664.9734477996826,0.26491973563861393
788789,1577579,1577578,3155157,2668.321923971176,0.26461467266562977
789790,1579581,1579580,3159161,2671.6683492660522,0.26431033505286905
790791,1581583,1581582,3163165,2675.041624069214,0.264006720186444
791792,1583585,1583584,3167169,2678.453145980835,0.26370382545064786
792793,1585587,1585586,3171173,2681.886066198349,0.26340164826251566
793794,1587589,1587588,3175177,2685.2425808906555,0.2631001860390825
794795,1589591,1589590,3179181,2688.6257140636444,0.2627994362064783
795796,1591593,1591592,3183185,2691.992795228958,0.26249939621447993
796797,1593595,1593594,3187189,2695.3476898670197,0.2622000635146833
797798,1595597,1595596,3191193,2698.742287158966,0.26190143557869305
798799,1597599,1597598,3195197,2702.1220898628235,0.26160350988175196
799800,1599601,1599600,3199201,2705.5115308761597,0.26130628392274957
800801,1601603,1601602,3203205,2709.114045858383,0.26100975520239444
801802,1603605,1603604,3207209,2712.5057520866394,0.26071392123776604
802803,1605607,1605606,3211213,2715.9632561206818,0.26041877955867676
803804,1607609,1607608,3215217,2719.510101079941,0.26012432770039595
804805,1609611,1609610,3219221,2722.8868222236633,0.25983056321638287
805806,1611613,1611612,3223225,2726.254946947098,0.2595374836728297
806807,1613615,1613614,3227229,2729.62198805809,0.2592450866395666
807808,1615617,1615616,3231233,2732.9595189094543,0.2589533697046136
808809,1617619,1617618,3235237,2736.3227529525757,0.25866233046872367
809810,1619621,1619620,3239241,2739.7530510425568,0.2583719665362878
810811,1621623,1621622,3243245,2743.119817018509,0.25808227552624885
811812,1623625,1623624,3247249,2746.495525121689,0.2577932550721016
812813,1625627,1625626,3251253,2749.864701271057,0.25750490282007377
813814,1627629,1627628,3255257,2753.2695829868317,0.25721721641457407
814815,1629631,1629630,3259261,2756.6644401550293,0.25693019353093405
815816,1631633,1631632,3263265,2760.0347290039062,0.2566438318353903
816817,1633635,1633634,3267269,2763.4291739463806,0.2563581290178263
817818,1635637,1635636,3271273,2766.778920173645,0.2560730827790394
818819,1637639,1637638,3275277,2770.243138074875,0.25578869081800804
819820,1639641,1639640,3279281,2773.596997022629,0.25550495085917646
820821,1641643,1641642,3283285,2776.974799156189,0.2552218606324459
821822,1643645,1643644,3287289,2780.536544084549,0.2549394178768125
822823,1645647,1645646,3291293,2784.2056272029877,0.25465762033854844
823824,1647649,1647648,3295297,2787.771963119507,0.2543764657857537
824825,1649651,1649650,3299301,2791.3208181858063,0.25409595198107127
825826,1651653,1651652,3303305,2794.877569913864,0.2538160767107911
826827,1653655,1653654,3307309,2798.4840519428253,0.25353683776666003
827828,1655657,1655656,3311313,2802.053514957428,0.2532582329495199
828829,1657659,1657658,3315317,2805.7568719387054,0.2529802600693074
829830,1659661,1659660,3319321,2809.335478067398,0.25270291695233027
830831,1661663,1661662,3323325,2812.935727119446,0.2524262014285341
831832,1663665,1663664,3327329,2816.4685518741608,0.2521501113387785
832833,1665667,1665666,3331333,2820.0489361286163,0.251874644536656
833834,1667669,1667668,3335337,2823.6223850250244,0.25159979888485395
834835,1669671,1669670,3339341,2827.18758392334,0.25132557224969787
835836,1671673,1671672,3343345,2830.84211397171,0.251051962522979
836837,1673675,1673674,3347349,2834.39319896698,0.2507789675855747
837838,1675677,1675676,3351353,2837.9633798599243,0.2505065853438282
838839,1677679,1677678,3355357,2841.5120120048523,0.2502348137059016
839840,1679681,1679680,3359361,2845.074695110321,0.24996365058905212
840841,1681683,1681682,3363365,2848.455286026001,0.24969309393054573
841842,1683685,1683684,3367369,2851.840231180191,0.24942314166401047
842843,1685687,1685686,3371373,2855.2074699401855,0.24915379173216934
843844,1687689,1687688,3375377,2858.903932094574,0.24888504210321116
844845,1689691,1689690,3379381,2862.35196518898,0.2486168907398678
845846,1691693,1691692,3383385,2865.7138521671295,0.24834933561214712
846847,1693695,1693694,3387389,2869.087804079056,0.24808237471188477
847848,1695697,1695696,3391393,2872.4946789741516,0.24781600603091647
848849,1697699,1697698,3395397,2875.876361846924,0.24755022757381084
849850,1699701,1699700,3399401,2879.227727174759,0.24728503735241247
850851,1701703,1701702,3403405,2882.6669738292694,0.2470204333840229
851852,1703705,1703704,3407409,2886.10262799263,0.2467564137041336
852853,1705707,1705706,3411413,2889.508544921875,0.24649297634823597
853854,1707709,1707708,3415417,2892.8544108867645,0.2462301193663734
854855,1709711,1709710,3419421,2896.2153131961823,0.24596784081222722
855856,1711713,1711712,3423425,2899.5756368637085,0.2457061387522117
856857,1713715,1713714,3427429,2902.9609389305115,0.24544501126001705
857858,1715717,1715716,3431433,2906.4732961654663,0.24518445642206643
858859,1717719,1717718,3435437,2910.158936023712,0.244924472322964
859860,1719721,1719720,3439441,2913.565801858902,0.2446650570655038
860861,1721723,1721722,3443445,2916.9705350399017,0.24440620875611785
861862,1723725,1723724,3447449,2920.649252176285,0.24414792551579012
862863,1725727,1725726,3451453,2924.299450159073,0.24389020546186657
863864,1727729,1727728,3455457,2927.7765159606934,0.24363304673534003
864865,1729731,1729730,3459461,2931.1547708511353,0.24337644746992737
865866,1731733,1731732,3463465,2934.577708005905,0.24312040582117334
866867,1733735,1733734,3467469,2938.113774061203,0.24286491994280368
867868,1735737,1735736,3471473,2941.6182289123535,0.24260998800673406
868869,1737739,1737738,3475477,2944.964996099472,0.24235560818124213
869870,1739741,1739740,3479481,2948.381824016571,0.2421017786473385
870871,1741743,1741742,3483485,2951.7802770137787,0.2418484976005857
871872,1743745,1743744,3487489,2955.1686398983,0.2415957632347272
872873,1745747,1745746,3491493,2958.513554096222,0.24134357376169646
873874,1747749,1747748,3495497,2961.9157350063324,0.24109192738433194
874875,1749751,1749750,3499501,2965.2595829963684,0.24084082233639492
875876,1751753,1751752,3503505,2968.6483080387115,0.24059025684255175
876877,1753755,1753754,3507509,2972.0087530612946,0.24034022913474473
877878,1755757,1755756,3511513,2975.343014240265,0.24009073746674403
878879,1757759,1757758,3515517,2978.744162082672,0.23984178008504387
879880,1759761,1759760,3519521,2982.1257650852203,0.23959335525432834
880881,1761763,1761762,3523525,2985.4951322078705,0.23934546123928158
881882,1763765,1763764,3527529,2988.860116004944,0.2390980963155016
882883,1765767,1765766,3531533,2992.2203409671783,0.23885125876950042
883884,1767769,1767768,3535537,2995.6163198947906,0.238604946885971
884885,1769771,1769770,3539541,2999.009019136429,0.23835915896779625
885886,1771773,1771772,3543545,3002.3643629550934,0.23811389331785904
886887,1773775,1773774,3547549,3005.7057461738586,0.23786914824631822
887888,1775777,1775776,3551553,3009.138664960861,0.23762492207788455
888889,1777779,1777778,3555557,3012.528477191925,0.2373812131354498
889890,1779781,1779780,3559561,3015.891725063324,0.23713801975463866
890891,1781783,1781782,3563565,3019.220498085022,0.2368953402765328
891892,1783785,1783784,3567569,3022.587347984314,0.23665317305312783
892893,1785787,1785786,3571573,3025.9815311431885,0.23641151643641933
893894,1787789,1787788,3575577,3029.3529160022736,0.23617036878931685
894895,1789791,1789790,3579581,3032.712224960327,0.23592972848200588
895896,1791793,1791792,3583585,3036.057865858078,0.23568959389194788
896897,1793795,1793794,3587589,3039.463362932205,0.23544996340569924
897898,1795797,1795796,3591593,3042.8477540016174,0.23521083540799737
898899,1797799,1797798,3595597,3046.3736460208893,0.23497220830176957
899900,1799801,1799800,3599601,3049.8093209266663,0.23473408048630517
900901,1801803,1801802,3603605,3053.1747801303864,0.2344964503772644
901902,1803805,1803804,3607609,3056.5394620895386,0.2342593163903075
902903,1805807,1805806,3611613,3059.944967985153,0.23402267695018963
903904,1807809,1807808,3615617,3063.2847821712494,0.23378653048894193
904905,1809811,1809810,3619621,3066.6354229450226,0.2335508754476905
905906,1811813,1811812,3623625,3070.1548578739166,0.2333157102639234
906907,1813815,1813814,3627629,3073.540121078491,0.23308103339695663
907908,1815817,1815816,3631633,3076.9200870990753,0.2328468432988302
908909,1817819,1817818,3635637,3080.251261949539,0.23261313843613607
909910,1819821,1819820,3639641,3083.6423161029816,0.2323799172809231
910911,1821823,1821822,3643645,3087.1383221149445,0.2321471783088782
911912,1823825,1823824,3647649,3090.7086141109467,0.2319149200029642
912913,1825827,1825826,3651653,3094.0689730644226,0.2316831408552389
913914,1827829,1827828,3655657,3097.4375212192535,0.23145183936139802
914915,1829831,1829830,3659661,3100.83478808403,0.2312210140262323
915916,1831833,1831832,3663665,3104.2272429466248,0.23099066335817042
916917,1833835,1833834,3667669,3107.609139919281,0.23076078586927906
917918,1835837,1835836,3671673,3110.962013244629,0.23053138008253882
918919,1837839,1837838,3675677,3114.331378221512,0.23030244452638726
919920,1839841,1839840,3679681,3117.9142651557922,0.23007397773835692
920921,1841843,1841842,3683685,3121.3513531684875,0.2298459782541613
921922,1843845,1843844,3687689,3124.7688291072845,0.2296184446204279
922923,1845847,1845846,3691693,3128.118273973465,0.22939137538924115
923924,1847849,1847848,3695697,3131.5618538856506,0.2291647691217804
924925,1849851,1849850,3699701,3134.918431997299,0.22893862437740609
925926,1851853,1851852,3703705,3138.370385169983,0.22871293973184947
926927,1853855,1853854,3707709,3141.775608062744,0.2284877137572039
927928,1855857,1855856,3711713,3145.139678955078,0.22826294504011457
928929,1857859,1857858,3715717,3148.491338968277,0.22803863216358877
929930,1859861,1859860,3719721,3151.94731426239,0.22781477372336667
930931,1861863,1861862,3723725,3155.3844521045685,0.22759136831700744
931932,1863865,1863864,3727729,3158.8422582149506,0.22736841455662216
932933,1865867,1865866,3731733,3162.407623052597,0.22714591104522697
933934,1867869,1867868,3735737,3165.8304691314697,0.2269238564040279
934935,1869871,1869870,3739741,3169.202308177948,0.22670224925604998
935936,1871873,1871872,3743745,3172.5799281597137,0.2264810882279562
936937,1873875,1873874,3747749,3175.9571919441223,0.22626037195368554
937938,1875877,1875876,3751753,3179.3137781620026,0.2260400990726339
938939,1877879,1877878,3755757,3182.6905930042267,0.22582026823147316
939940,1879881,1879880,3759761,3186.057844877243,0.22560087807869422
940941,1881883,1881882,3763765,3189.4725620746613,0.22538192727370188
941942,1883885,1883884,3767769,3192.829383134842,0.22516341447590094
942943,1885887,1885886,3771773,3196.190205812454,0.22494533835197217
943944,1887889,1887888,3775777,3199.5729641914368,0.2247276975758723
944945,1889891,1889890,3779781,3202.9171121120453,0.22451049082519603
945946,1891893,1891892,3783785,3206.2884800434113,0.22429371678299503
946947,1893895,1893894,3787789,3209.6302630901337,0.22407737413777795
947948,1895897,1895896,3791793,3213.1376209259033,0.2238614615835104
948949,1897899,1897898,3795797,3216.5382339954376,0.22364597782143392
949950,1899901,1899900,3799801,3219.885540008545,0.2234309215509711
950951,1901903,1901902,3803805,3223.2454750537872,0.22321629148791544
951952,1903905,1903904,3807809,3226.6568369865417,0.2230020863498794
952953,1905907,1905906,3811813,3230.033149957657,0.22278830484719947
953954,1907909,1907908,3815817,3233.4755251407623,0.22257494571204006
954955,1909911,1909910,3819821,3236.980283021927,0.22236200767656555
955956,1911913,1911912,3823825,3240.3493859767914,0.22214948947112134
956957,1913915,1913914,3827829,3243.696568965912,0.22193738983878575
957958,1915917,1915916,3831833,3247.0573019981384,0.22172570752627507
958959,1917919,1917918,3835837,3250.4922029972076,0.2215144412857626
959960,1919921,1919920,3839841,3253.862202167511,0.22130358987305954
960961,1921923,1921922,3843845,3257.199594974518,0.22109315204397717
961962,1923925,1923924,3847849,3260.647348880768,0.22088312656887865
962963,1925927,1925926,3851853,3264.041425228119,0.22067351221812714
963964,1927929,1927928,3855857,3267.3921089172363,0.22046430776936177
964965,1929931,1929930,3859861,3270.7364590168,0.22025551200022164
965966,1931933,1931932,3863865,3274.103410243988,0.22004712369744084
966967,1933935,1933934,3867869,3277.4797308444977,0.2198391416513914
967968,1935937,1935936,3871873,3280.911952018738,0.21963156465790235
968969,1937939,1937938,3875877,3284.2707710266113,0.21942439151644066
969970,1939941,1939940,3879881,3287.655741214752,0.21921762103011133
970971,1941943,1941942,3883885,3291.02024102211,0.21901125200929528
971972,1943945,1943944,3887889,3294.388871908188,0.2188052832698304
972973,1945947,1945946,3891893,3297.903604030609,0.21859971363119257
973974,1947949,1947948,3895897,3301.3627030849457,0.21839454191285768
974975,1949951,1949950,3899901,3304.72096991539,0.2181897669488535
975976,1951953,1951952,3903905,3308.1044149398804,0.21798538756956987
976977,1953955,1953954,3907909,3311.5009689331055,0.21778140261085355
977978,1955957,1955956,3911913,3314.882644891739,0.21757781091582729
978979,1957959,1957958,3915917,3318.2991049289703,0.2173746113312518
979980,1959961,1959960,3919921,3321.702966928482,0.21717180270934477
980981,1961963,1961962,3923925,3325.0656559467316,0.2169693839041429
981982,1963965,1963964,3927929,3328.4125230312347,0.21676735377877776
982983,1965967,1965966,3931933,3331.7745089530945,0.21656571119274304
983984,1967969,1967968,3935937,3335.1324331760406,0.21636445502190327
984985,1969971,1969970,3939941,3338.50740814209,0.21616358413666603
985986,1971973,1971972,3943945,3341.8888082504272,0.21596309741289588
986987,1973975,1973974,3947949,3345.242119073868,0.21576299373191432
987988,1975977,1975976,3951953,3348.6237099170685,0.2155632719877758
988989,1977979,1977978,3955957,3351.9927201271057,0.21536393106725882
989990,1979981,1979980,3959961,3355.4347681999207,0.2151649698644178
990991,1981983,1981982,3963965,3359.0268342494965,0.21496638727876416
991992,1983985,1983984,3967969,3362.434376001358,0.21476818222072325
992993,1985987,1985986,3971973,3365.8001849651337,0.21457035358980647
993994,1987989,1987988,3975977,3369.1948342323303,0.21437290030553413
994995,1989991,1989990,3979981,3372.5652000904083,0.21417582128196955
995996,1991993,1991992,3983985,3375.9365379810333,0.21397911543499504
996997,1993995,1993994,3987989,3379.316915035248,0.2137827816986828
997998,1995997,1995996,3991993,3382.652661085129,0.21358681899619114
998999,1997999,1997998,3995997,3385.994081020355,0.21339122626341123
1000000,2000001,2000000,4000001,3389.333256006241,0.21319600243805326


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0027458667755126953,12064.709122577777
1001,2003,2002,4005,3.6115479469299316,65.54308581374062
2002,4005,4004,8009,7.196931838989258,42.36125675350013
3003,6007,6006,12013,10.735725164413452,34.03888935166469
4004,8009,8008,16017,14.49898099899292,28.9736744604088
5005,10011,10010,20021,18.256932020187378,25.347796528210893
6006,12013,12012,24025,22.094247102737427,22.541154451162583
7007,14015,14014,28029,25.44001603126526,20.266618657631625
8008,16017,16016,32033,28.789549827575684,18.369066826699054
9009,18019,18018,36037,32.211326122283936,16.75518334221306
10010,20021,20020,40041,35.59293293952942,15.363866328221775
11011,22023,22022,44045,39.035109996795654,14.152344435575287
12012,24025,24024,48049,42.55358123779297,13.089117171617545
13013,26027,26026,52053,46.08311414718628,12.150095046214119
14014,28029,28028,56057,49.516438007354736,11.316336767915345
15015,30031,30030,60061,52.99904203414917,10.572633315323401
16016,32033,32032,64065,56.371178150177,9.906575041453834
17017,34035,34034,68069,59.71449899673462,9.30790492201595
18018,36037,36036,72073,63.01842379570007,8.768053615920508
19019,38039,38038,76077,66.41734886169434,8.279796333541526
20020,40041,40040,80081,69.74904108047485,7.83699363989399
21021,42043,42042,84085,73.06229400634766,7.434391921489805
22022,44045,44044,88089,76.45601320266724,7.0674677593142405
23023,46047,46046,92093,79.86075496673584,6.732304990688135
24024,48049,48048,96097,83.18646001815796,6.425496532749094
25025,50051,50050,100101,86.52707099914551,6.144065203598075
26026,52053,52052,104105,89.86694502830505,5.885399280419733
27027,54055,54054,108109,93.20168399810791,5.647199603103218
28028,56057,56056,112113,96.58000111579895,5.42743580638853
29029,58059,58058,116117,99.95947599411011,5.224309832568906
30030,60061,60060,120121,103.30021214485168,5.036225299478247
31031,62063,62062,124125,106.6273250579834,4.861761615753494
32032,64065,64064,128129,109.949383020401,4.699651975070083
33033,66067,66066,132133,113.29242396354675,4.5487645438679465
34034,68069,68068,136137,116.62531900405884,4.408086297122281
35035,70071,70070,140141,119.94893288612366,4.276709065070463
36036,72073,72072,144145,123.2637460231781,4.153817437863836
37037,74075,74074,148149,126.88334703445435,4.038678240984154
38038,76077,76076,152153,130.3403868675232,3.9306313461856917
39039,78079,78078,156157,133.66798901557922,3.829081623838647
40040,80081,80080,160161,137.01576709747314,3.7334918754459068
41041,82083,82082,164165,140.35639786720276,3.643376690981313
42042,84085,84084,168169,143.7153570652008,3.5582967863683734
43043,86087,86086,172173,147.20238590240479,3.4778541834857606
44044,88089,88088,176177,150.5920910835266,3.4016880430081073
45045,90091,90090,180181,153.91083407402039,3.3294707772256515
46046,92093,92092,184185,157.3594582080841,3.2609046608413337
47047,94095,94094,188189,160.69124603271484,3.1957188153337484
48048,96097,96096,192193,164.0047812461853,3.1336665222806914
49049,98099,98098,196197,167.33908200263977,3.0745228269388463
50050,100101,100100,200201,170.66259479522705,3.018082398313709
51051,102103,102102,204205,173.99177503585815,2.96415761627577
52052,104105,104104,208209,177.49394011497498,2.912576859982437
53053,106107,106106,212213,180.93330693244934,2.8631829749247117
54054,108109,108108,216217,184.28635001182556,2.8158318987552775
55055,110111,110110,220221,187.62109899520874,2.7703914283592894
56056,112113,112112,224225,190.93987202644348,2.726740112721018
57057,114115,114114,228229,194.25598120689392,2.6847662579166354
58058,116117,116116,232233,197.5934500694275,2.6443670321714308
59059,118119,118118,236237,201.05178713798523,2.6054476602639625
60060,120121,120120,240241,204.36580300331116,2.5679206978093134
61061,122123,122122,244245,207.69349694252014,2.531705376924947
62062,124125,124124,248249,210.9986629486084,2.4967270159067994
63063,126127,126126,252253,214.33691000938416,2.462916486127142
64064,128129,128128,256257,217.92963314056396,2.430209730318893
65065,130131,130130,260261,221.2511329650879,2.3985473269094655
66066,132133,132132,264265,224.5895709991455,2.3678740957093396
67067,134135,134134,268269,227.93601894378662,2.338138740768045
68068,136137,136136,272273,231.25413584709167,2.309293526604961
69069,138139,138138,276277,234.591126203537,2.281293984502554
70070,140141,140140,280281,237.9416139125824,2.2540986458207044
71071,142143,142142,284285,241.27411484718323,2.227668799694584
72072,144145,144144,288289,244.57360291481018,2.2019682726804604
73073,146147,146146,292293,247.926029920578,2.1769632282048406
74074,148149,148148,296297,251.27779006958008,2.15262198390883
75075,150151,150150,300301,254.58129906654358,2.1289148527066573
76076,152153,152152,304305,257.9308590888977,2.1058139750857663
77077,154155,154154,308309,261.25280117988586,2.0832931818367797
78078,156157,156156,312313,264.592472076416,2.061327881379839
79079,158159,158158,316317,268.0914239883423,2.039894936457131
80080,160161,160160,320321,271.58864402770996,2.018972557998495
81081,162163,162162,324325,274.91818499565125,1.998540207881888
82082,164165,164164,328329,278.2998969554901,1.9785785097737971
83083,166167,166166,332333,281.6118631362915,1.9590691673110996
84084,168169,168168,336337,284.9523799419403,1.9399948889404186
85085,170171,170170,340341,288.28871297836304,1.9213393188474583
86086,172173,172172,344345,291.6226840019226,1.9030869733906002
87087,174175,174174,348349,294.9464840888977,1.8852231825749186
88088,176177,176176,352353,298.2528610229492,1.8677340361209644
89089,178179,178178,356357,301.5746760368347,1.8506063337190426
90090,180181,180180,360361,304.8728840351105,1.8338275390888157
91091,182183,182182,364365,308.23843908309937,1.817385737575023
92092,184185,184184,368369,311.5676119327545,1.8012695968864136
93093,186187,186186,372373,314.8887288570404,1.785468330806907
94094,188189,188188,376377,318.22092604637146,1.7699716655552038
95095,190191,190190,380381,321.6007330417633,1.7547698086145829
96096,192193,192192,384385,325.2059290409088,1.739853419818246
97097,194195,194194,388389,328.62334394454956,1.7252135934522812
98098,196197,196196,392393,331.9477400779724,1.7108418227326183
99099,198199,198198,396397,335.30570101737976,1.6967299528078001
100100,200201,200200,400401,338.6727252006531,1.6828702026996325
101101,202203,202202,404405,341.98027205467224,1.669255127055294
102102,204205,204204,408409,345.3311839103699,1.6558775974026503
103103,206207,206206,412413,348.69270610809326,1.642730784647938
104104,208209,208208,416417,352.08227491378784,1.6298081427630677
105105,210211,210210,420421,355.4292480945587,1.6171033935170271
106106,212213,212212,424425,358.74741411209106,1.6046105122277368
107107,214215,214214,428429,362.11046409606934,1.59232371440703
108108,216217,216216,432433,365.4399619102478,1.5802374432769284
109109,218219,218218,436437,368.7953109741211,1.5683463580535317
110110,220221,220220,440441,372.1017942428589,1.556645322982149
111111,222223,222222,444445,375.4348828792572,1.5451293970290862
112112,224225,224224,448449,378.8297791481018,1.533793824222812
113113,226227,226226,452453,382.1812801361084,1.5226340245644678
114114,228229,228228,456457,385.5349860191345,1.5116455854858941
115115,230231,230230,460461,388.8596041202545,1.5008242538187915
116116,232233,232232,464465,392.1724669933319,1.490165928233182
117117,234235,234234,468469,395.7134358882904,1.479666652103333
118118,236237,236236,472473,399.17777705192566,1.4693226068011427
119119,238239,238238,476477,402.5410759449005,1.4591301053660573
120120,240241,240240,480481,405.878201007843,1.4490855865096819
121121,242243,242242,484485,409.20735001564026,1.4391856089932844
122122,244245,244244,488489,412.55543780326843,1.4294268462854234
123123,246247,246246,492493,415.8822720050812,1.4198060815215285
124124,248249,248248,496497,419.19719314575195,1.4103202027345105
125125,250251,250250,500501,422.6311550140381,1.4009661983382102
126126,252253,252252,504505,426.11056113243103,1.3917411528709636
127127,254255,254254,508509,429.5118041038513,1.3826422429174272
128128,256257,256256,512513,432.86035418510437,1.3736667332977959
129129,258259,258258,516517,436.1562850475311,1.3648119734116335
130130,260261,260260,520521,439.476930141449,1.3560753937872505
131131,262263,262262,524525,443.0320370197296,1.3474545027966087
132132,264265,264264,528529,446.453556060791,1.3389468835503067
133133,266267,266266,532533,449.80646896362305,1.3305501909198938
134134,268269,268268,536537,453.10089087486267,1.3222621487366268
135135,270271,270270,540541,456.54367899894714,1.3140805471084605
136136,272273,272272,544545,459.9613130092621,1.306003239860729
137137,274275,274274,548549,463.29757595062256,1.298028142120529
138138,276277,276276,552553,466.65905809402466,1.2901532279938692
139139,278279,278278,556557,469.9887840747833,1.2823765283756074
140140,280281,280280,560561,473.3273561000824,1.2746961288285092
141141,282283,282282,564565,476.66826915740967,1.2671101675914542
142142,284285,284284,568569,480.01656103134155,1.2596168336549454
143143,286287,286286,572573,483.364511013031,1.2522143649566715
144144,288289,288288,576577,486.73221802711487,1.2449010466061736
145145,290291,290290,580581,490.1623661518097,1.2376752092404786
146146,292293,292292,584585,493.6927111148834,1.2305352274124743
147147,294295,294294,588589,496.9171669483185,1.2234795180866058
148148,296297,296296,592593,500.12242698669434,1.2165065391636745
149149,298299,298298,596597,503.3312110900879,1.2096147880965873
150150,300301,300300,600601,506.55142307281494,1.2028028043223458
151151,302303,302302,604605,509.74848794937134,1.1960691691729153
152152,304305,304304,608609,512.9500560760498,1.1894124782338622
153153,306307,306306,612613,516.4713459014893,1.1828313743353647
154154,308309,308308,616617,519.7609858512878,1.1763245337078843
155155,310311,310310,620621,523.055046081543,1.1698906649071432
156156,312313,312312,624625,526.2859840393066,1.1635285077663866
157157,314315,314314,628629,529.5528709888458,1.157236832412309
158158,316317,316316,632633,532.7953858375549,1.1510144383028091
159159,318319,318318,636637,536.0421772003174,1.1448601533138572
160160,320321,320320,640641,539.3095922470093,1.1387728328445519
161161,322323,322322,644645,542.549586057663,1.1327513589876617
162162,324325,324324,648649,545.8652429580688,1.1267946397001651
163163,326327,326326,652653,549.1072850227356,1.1209016080265428
164164,328329,328328,656657,552.3695530891418,1.1150712213402585
165165,330331,330330,660661,555.5514221191406,1.1093024606143445
166166,332333,332332,664665,558.7142670154572,1.1035943297374615
167167,334335,334334,668669,561.8681931495667,1.097945854824502
168168,336337,336336,672673,565.0409061908722,1.0923560835744865
169169,338339,338338,676677,568.2156939506531,1.0868240846521076
170170,340341,340340,680681,571.3433890342712,1.081348947069273
171171,342343,342342,684685,574.474879026413,1.0759297796266765
172172,344345,344344,688689,577.7494280338287,1.0705657103389967
173173,346347,346346,692693,580.9045510292053,1.0652558858946577
174174,348349,348348,696697,584.0928280353546,1.0599994711446925
175175,350351,350350,700701,587.446527004242,1.0547956485916075
176176,352353,352352,704705,590.6675798892975,1.0496436179073498
177177,354355,354354,708709,593.8532218933105,1.0445425954712846
178178,356357,356356,712713,597.040491104126,1.039491813895438
179179,358359,358358,716717,600.2323830127716,1.0344905216134066
180180,360361,360360,720721,603.40469622612,1.0295379824492557
181181,362363,362362,724725,606.5847351551056,1.0246334751936956
182182,364365,364364,728729,609.7925200462341,1.0197762932348269
183183,366367,366366,732733,613.0582580566406,1.014965744156143
184184,368369,368368,736737,616.3752660751343,1.0102011493727332
185185,370371,370370,740741,619.5536730289459,1.005481843776579
186186,372373,372372,744745,622.7067139148712,1.0008071753909462
187187,374375,374374,748749,625.838446855545,0.9961765050302347
188188,376377,376376,752753,629.0214080810547,0.9915892059816542
189189,378379,378378,756757,632.3122670650482,0.9870446636869019
190190,380381,380380,760761,635.5990869998932,0.9825422754347528
191191,382383,382382,764765,638.8089511394501,0.9780814500791166
192192,384385,384384,768769,642.5077829360962,0.9736616077352664
193193,386387,386386,772773,645.7466490268707,0.9692821795251803
194194,388389,388388,776777,648.9055140018463,0.9649426072846836
195195,390391,390390,780781,652.6495079994202,0.9606423433233431
196196,392393,392392,784785,655.7805562019348,0.9563808501588937
197197,394395,394394,788789,658.9455320835114,0.9521576002844085
198198,396397,396396,792793,662.1219940185547,0.9479720759136399
199199,398399,398398,796797,665.3484590053558,0.9438237687681976
200200,400401,400400,800801,668.5847098827362,0.9397121798483568
201201,402403,402402,804805,671.998370885849,0.9356368192056834
202202,404405,404404,808809,675.6364891529083,0.9315972057484032
203203,406407,406406,812813,679.2813808917999,0.9275928670176654
204204,408409,408408,816817,682.8770830631256,0.923623339014739
205205,410411,410410,820821,686.5120389461517,0.9196881659772771
206206,412413,412412,824825,690.1731789112091,0.9157869002174266
207207,414415,414414,828829,693.7825491428375,0.9119191019217396
208208,416417,416416,832833,697.4097290039062,0.9080843389820075
209209,418419,418418,836837,701.0849230289459,0.9042821868206374
210210,420421,420420,840841,704.7403750419617,0.900512228228763
211211,422423,422422,844845,708.2710890769958,0.8967740531879826
212212,424425,424424,848849,711.6555879116058,0.8930672587339359
213213,426427,426426,852853,715.0450599193573,0.8893914487725851
214214,428429,428428,856857,718.4124600887299,0.8857462339674385
215215,430431,430430,860861,721.7871551513672,0.8821312315576506
216216,432433,432432,864865,725.2795331478119,0.8785460652397887
217217,434435,434434,868869,728.7489638328552,0.8749903650132183
218218,436437,436436,872873,732.162034034729,0.8714637670618686
219219,438439,438438,876877,735.5371630191803,0.8679659136068949
220220,440441,440440,880881,738.9014959335327,0.864496452788444
221221,442443,442442,884885,742.3597829341888,0.8610550385401439
222222,444445,444444,888889,745.7370221614838,0.8576413304654125
223223,446447,446446,892893,749.1372859477997,0.8542549937228614
224224,448449,448448,896897,752.6482629776001,0.8508956989026046
225225,450451,450450,900901,756.0742311477661,0.8475631219280331
226226,452453,452452,904905,759.5109450817108,0.8442569439303043
227227,454455,454454,908909,762.9657161235809,0.8409768511610309
228228,456457,456456,912913,766.3406639099121,0.8377225348667707
229229,458459,458458,916917,769.7556009292603,0.8344936912017147
230230,460461,460460,920921,773.1973671913147,0.8312900211312808
231231,462463,462462,924925,776.5642919540405,0.8281112303247937
232232,464465,464464,928929,779.9815609455109,0.8249570290663542
233233,466467,466466,932933,783.4262778759003,0.8218271321657085
234234,468469,468468,936937,786.8488590717316,0.8187212588654802
235235,470471,470470,940941,790.271586894989,0.8156391327556776
236236,472473,472472,944945,793.6467130184174,0.81258048169002
237237,474475,474474,948949,797.0499222278595,0.8095450376949884
238238,476477,476476,952953,800.4667541980743,0.8065325369007041
239239,478479,478478,956957,803.9899048805237,0.8035427194517979
240240,480481,480480,960961,807.4905638694763,0.8005753294364695
241241,482483,482482,964965,810.8975381851196,0.7976301148009952
242242,484485,484484,968969,814.2920110225677,0.7947068272915203
243243,486487,486486,972973,817.7078800201416,0.7918052223703853
244244,488489,488488,976977,821.1208200454712,0.7889250591488235
245245,490491,490490,980981,824.4939091205597,0.7860661003123823
246246,492493,492492,984985,827.8624970912933,0.7832281120736297
247247,494495,494494,988989,831.3651919364929,0.7804108640757477
248248,496497,496496,992993,834.8811340332031,0.7776141293597902
249249,498499,498498,996997,838.3510000705719,0.7748376842810103
250250,500501,500500,1001001,841.9991068840027,0.7720813084488327
251251,502503,502502,1005005,845.4920961856842,0.7693447846813797
252252,504505,504504,1009009,848.8632941246033,0.7666278989308921
253253,506507,506506,1013013,852.2363610267639,0.763930440236436
254254,508509,508508,1017017,855.6353099346161,0.7612522006638756
255255,510511,510510,1021021,859.0238389968872,0.7585929752513039
256256,512513,512512,1025025,862.389769077301,0.7559525619562919
257257,514515,514514,1029029,866.0402891635895,0.7533307616049569
258258,516517,516516,1033033,869.4684629440308,0.7507273778392118
259259,518519,518518,1037037,872.8657150268555,0.7481422170640144
260260,520521,520520,1041041,876.2912058830261,0.7455750883982546
261261,522523,522522,1045045,879.7592189311981,0.7430258036383748
262262,524525,524524,1049049,883.134360074997,0.7404941771965241
263263,526527,526526,1053053,886.511265039444,0.7379800260605407
264264,528529,528528,1057057,889.960294008255,0.7354831697502959
265265,530531,530530,1061061,893.6581389904022,0.7330034302722197
266266,532533,532532,1065065,897.2671382427216,0.7305406320756447
267267,534535,534534,1069069,900.6978042125702,0.7280946020146075
268268,536537,536536,1073073,904.0962510108948,0.7256651692987361
269269,538539,538538,1077077,907.5549640655518,0.723252165458689
270270,540541,540540,1081081,910.9708528518677,0.7208554243061371
271271,542543,542542,1085085,914.3955221176147,0.7184747819010227
272272,544545,544544,1089089,917.840667963028,0.7161100764933508
273273,546547,546546,1093093,921.2866830825806,0.7137611485068192
274274,548549,548548,1097097,924.6662180423737,0.711427840495162
275275,550551,550550,1101101,928.0584621429443,0.7091099971075892
276276,552553,552552,1105105,931.504096031189,0.7068074650469498
277277,554555,554554,1109109,934.9576258659363,0.7045200930479041
278278,556557,556556,1113113,938.3366038799286,0.7022477318314486
279279,558559,558558,1117117,941.7191770076752,0.6999902340776316
280280,560561,560560,1121121,945.0752568244934,0.697747454396449
281281,562563,562562,1125125,948.4369850158691,0.6955192492878268
282282,564565,564564,1129129,951.7694611549377,0.6933054793025804
283283,566567,566566,1133133,955.1079289913177,0.691106004809626
284284,568569,568568,1137137,958.4317462444305,0.6889206854284566
285285,570571,570570,1141141,961.8354041576385,0.6867493849331368
286286,572573,572572,1145145,965.1882529258728,0.6845919688494178
287287,574575,574574,1149149,968.5334990024567,0.68244830441472
288288,576577,576576,1153153,971.9027719497681,0.6803182605690381
289289,578579,578578,1157157,975.2426450252533,0.6782017078985518
290290,580581,580580,1161161,978.568706035614,0.6760985186410835
291291,582583,582582,1165165,981.9179878234863,0.6740085666351661
292292,584585,584584,1169169,985.235239982605,0.6719317273091292
293293,586587,586586,1173173,988.5746409893036,0.6698678776519955
294294,588589,588588,1177177,991.9277892112732,0.6678168983071373
295295,590591,590590,1181181,995.3125970363617,0.6657787141703011
296296,592593,592592,1185185,998.7930729389191,0.6637531594824395
297297,594595,594594,1189189,1002.3182020187378,0.6617401172316022
298298,596597,596596,1193193,1005.7436108589172,0.6597394718501164
299299,598599,598598,1197197,1009.0787000656128,0.657751109196397
300300,600601,600600,1201201,1012.4099810123444,0.6557749165203859
301301,602603,602602,1205205,1015.7497491836548,0.6538107824580948
302302,604605,604604,1209209,1019.2070200443268,0.6518585969934065
303303,606607,606606,1213213,1022.6190841197968,0.6499182514544373
304304,608609,608608,1217217,1026.019133090973,0.6479896384771564
305305,610611,610610,1221221,1029.344228029251,0.6460726519944728
306306,612613,612612,1225225,1032.7197000980377,0.644167187219864
307307,614615,614614,1229229,1036.0940589904785,0.6422731568873132
308308,616617,616616,1233233,1039.5050129890442,0.640390473196021
309309,618619,618618,1237237,1043.018481016159,0.6385190040255111
310310,620621,620620,1241241,1046.3672170639038,0.6366586494896183
311311,622623,622622,1245245,1049.7305731773376,0.6348093108972535
312312,624625,624624,1249249,1053.0961339473724,0.6329708907196618
313313,626627,626626,1253253,1056.4675650596619,0.6311432925867848
314314,628629,628628,1257257,1059.874668121338,0.6293264212454233
315315,630631,630630,1261261,1063.2511188983917,0.6275201825737895
316316,632633,632632,1265265,1066.580050945282,0.6257244835323945
317317,634635,634634,1269269,1069.9690079689026,0.6239392321804189
318318,636637,636636,1273273,1073.3535199165344,0.6221643376284192
319319,638639,638638,1277277,1076.7227339744568,0.6203997100510605
320320,640641,640640,1281281,1080.0645530223846,0.6186452606507373
321321,642643,642642,1285285,1083.3890488147736,0.6169009016557538
322322,644645,644644,1289289,1086.766359090805,0.6151665462966776
323323,646647,646646,1293293,1090.1095099449158,0.6134421088008821
324324,648649,648648,1297297,1093.5041711330414,0.6117275043689006
325325,650651,650650,1301301,1096.87619805336,0.6100226491689682
326326,652653,652652,1305305,1100.248962879181,0.6083274603170139
327327,654655,654654,1309309,1103.6225020885468,0.606641855865746
328328,656657,656656,1313313,1106.965805053711,0.6049657547991956
329329,658659,658658,1317317,1110.3094611167908,0.6032990769963362
330330,660661,660660,1321321,1113.660024881363,0.6016417432419985
331331,662663,662662,1325325,1117.216826915741,0.5999936752177746
332332,664665,664664,1329329,1120.5926520824432,0.5983547954583628
333333,666667,666666,1333333,1123.954663991928,0.5967250273733953
334334,668669,668668,1337337,1127.2945129871368,0.5951042952128773
335335,670671,670670,1341341,1130.6222269535065,0.5934925240671873
336336,672673,672672,1345345,1133.9703178405762,0.5918896398543438
337337,674675,674674,1349349,1137.5168640613556,0.5902955693036347
338338,676677,676676,1353353,1140.9837429523468,0.5887102399447031
339339,678679,678678,1357357,1144.3260049819946,0.5871335801057285
340340,680681,680680,1361361,1147.7395160198212,0.5855655188934179
341341,682683,682682,1365365,1151.2611169815063,0.5840059861820919
342342,684685,684684,1369369,1154.6709089279175,0.5824549126082275
343343,686687,686686,1373373,1158.3702569007874,0.5809122295595444
344344,688689,688688,1377377,1161.9739410877228,0.5793778711395134
345345,690691,690690,1381381,1165.5708141326904,0.5778517682447273
346346,692693,692692,1385385,1169.1811769008636,0.5763338544093131
347347,694695,694694,1389389,1172.7778041362762,0.5748240639222786
348348,696697,696696,1393393,1176.422446012497,0.5733223317729426
349349,698699,698698,1397397,1180.0047919750214,0.5718285936382017
350350,700701,700700,1401401,1183.1609799861908,0.5703427858770738
351351,702703,702702,1405405,1186.3101570606232,0.5688648455270595
352352,704705,704704,1409409,1189.4931061267853,0.5673947102804959
353353,706707,706706,1413413,1192.6500759124756,0.5659323184972891
354354,708709,708708,1417417,1195.8117730617523,0.5644776091758104
355355,710711,710710,1421421,1198.9464600086212,0.5630305219583533
356356,712713,712712,1425425,1202.1192150115967,0.561590997111125
357357,714715,714714,1429429,1205.2685639858246,0.5601589755297027
358358,716717,716716,1433433,1208.4606401920319,0.5587343987208442
359359,718719,718718,1437437,1211.6057801246643,0.5573172087915736
360360,720721,720720,1441441,1214.707925081253,0.5559073484546388
361361,722723,722722,1445445,1217.8486790657043,0.5545047610121401
362362,724725,724724,1449449,1221.059063911438,0.5531093903446163
363363,726727,726726,1453453,1224.3586010932922,0.5517211809110449
364364,728729,728728,1457457,1227.6056220531464,0.5503400777397474
365365,730731,730730,1461461,1230.749393939972,0.5489660264156555
366366,732733,732732,1465465,1233.924565076828,0.5475989730821311
367367,734735,734734,1469469,1237.08429813385,0.5462388644245948
368368,736737,736736,1473473,1240.2210109233856,0.5448856476723449
369369,738739,738738,1477477,1243.2904238700867,0.5435392705821869
370370,740741,740740,1481481,1246.3863871097565,0.5421996814420709
371371,742743,742742,1485485,1249.584510087967,0.5408668290601781
372372,744745,744744,1489489,1252.6912741661072,0.5395406627503689
373373,746747,746746,1493493,1255.7679319381714,0.5382211323412776
374374,748749,748748,1497497,1258.8746881484985,0.5369081881544844
375375,750751,750750,1501501,1262.0022959709167,0.5356017810172489
376376,752753,752752,1505505,1265.1338398456573,0.5343018622279487
377377,754755,754754,1509509,1268.3101079463959,0.5330083835815458
378378,756757,756756,1513513,1271.6724948883057,0.5317212973423011
379379,758759,758758,1517517,1274.8845739364624,0.530440556247413
380380,760761,760760,1521521,1278.024444103241,0.5291661134906462
381381,762763,762762,1525525,1281.2477090358734,0.5278979227368836
382382,764765,764764,1529529,1284.4703559875488,0.5266359380930226
383383,766767,766766,1533533,1287.5914840698242,0.5253801141225267
384384,768769,768768,1537537,1290.7622230052948,0.5241304058199603
385385,770771,770770,1541541,1293.9105942249298,0.5228867686255398
386386,772773,772772,1545545,1297.0769171714783,0.5216491584124014
387387,774775,774774,1549549,1300.24662399292,0.5204175314684107
388388,776777,776776,1553553,1303.366641998291,0.5191918445161718
389389,778779,778778,1557557,1306.4572291374207,0.5179720546821045
390390,780781,780780,1561561,1309.6176452636719,0.516758119510996
391391,782783,782782,1565565,1312.7488470077515,0.5155499969532684
392392,784785,784784,1569569,1315.8861429691315,0.5143476453595213
393393,786787,786786,1573573,1319.0464689731598,0.5131510234750749
394394,788789,788788,1577577,1322.1617789268494,0.5119600904381514
395395,790791,790790,1581581,1325.2983701229095,0.5107748057780555
396396,792793,792792,1585585,1328.4767649173737,0.5095951293951657
397397,794795,794794,1589589,1331.61021900177,0.5084210215845815
398398,796797,796796,1593593,1334.7305591106415,0.5072524430033809
399399,798799,798798,1597597,1337.8480360507965,0.5060893546760781
400400,800801,800800,1601601,1340.9693357944489,0.5049317180018988
401401,802803,802802,1605605,1344.0920150279999,0.503779494732953
402402,804805,804804,1609609,1347.1904101371765,0.5026326469778724
403403,806807,806806,1613613,1350.2925221920013,0.5014911372054485
404404,808809,808808,1617617,1353.429370880127,0.500354928220986
405405,810811,810810,1621621,1356.5733149051666,0.4992239831844927
406406,812813,812812,1625625,1359.730456829071,0.4980982655870321
407407,814815,814814,1629629,1362.8380460739136,0.4969777392670949
408408,816817,816816,1633633,1365.9621279239655,0.4958623683814949
409409,818819,818818,1637637,1369.0772199630737,0.4947521174290159
410410,820821,820820,1641641,1372.217148065567,0.49364695122494595
411411,822823,822822,1645645,1375.3320710659027,0.49254683490653406
412412,824825,824824,1649649,1378.455905199051,0.49145173393299046
413413,826827,826826,1653653,1381.5749070644379,0.4903616140709346
414414,828829,828828,1657657,1384.6991591453552,0.48927644140349
415415,830831,830830,1661661,1387.8254261016846,0.4881961823157326
416416,832833,832832,1665665,1391.0018730163574,0.4871208035019663
417417,834835,834834,1669669,1394.125610113144,0.4860502719475335
418418,836837,836836,1673673,1397.2281548976898,0.48498455494518566
419419,838839,838838,1677677,1400.3499081134796,0.48392362006961775
420420,840841,840840,1681681,1403.5775151252747,0.4828674351938389
421421,842843,842842,1685685,1406.8717341423035,0.4818159684746206
422422,844845,844844,1689689,1410.022915840149,0.4807691883524967
423423,846847,846846,1693693,1413.173063993454,0.47972706354448746
424424,848849,848848,1697697,1416.3342821598053,0.4786895630550134
425425,850851,850850,1701701,1419.4821479320526,0.47765665614861064
426426,852853,852852,1705705,1422.6253290176392,0.4766283123735775
427427,854855,854854,1709709,1425.7580380439758,0.4756045015401469
428428,856857,856856,1713713,1428.9753711223602,0.4745851937295811
429429,858859,858858,1717717,1432.1455261707306,0.47357035927052493
430430,860861,860860,1721721,1435.2793319225311,0.47255996877174766
431431,862863,862862,1725725,1438.4169759750366,0.4715539930821251
432432,864865,864864,1729729,1441.5286779403687,0.4705524033142865
433433,866867,866866,1733733,1444.734009027481,0.46955517082642473
434434,868869,868868,1737737,1447.8961281776428,0.4685622672259342
435435,870871,870870,1741741,1451.029901266098,0.46757366436941084
436436,872873,872872,1745745,1454.1878108978271,0.4665893343517382
437437,874875,874874,1749749,1457.3082041740417,0.4656092495115445
438438,876877,876876,1753753,1460.491811990738,0.4646333824239264
439439,878879,878878,1757757,1463.6077950000763,0.4636617058986303
440440,880881,880880,1761761,1466.7307970523834,0.4626941929800523
441441,882883,882882,1765765,1469.821758031845,0.4617308169417811
442442,884885,884884,1769769,1472.9597120285034,0.46077155128296
443443,886887,886886,1773773,1476.084702014923,0.45981636973556306
444444,888889,888888,1777777,1479.2342631816864,0.4588652462425671
445445,890891,890890,1781781,1482.4565830230713,0.4579181549761415
446446,892893,892892,1785785,1485.5780189037323,0.45697507033037255
447447,894895,894894,1789789,1488.6904730796814,0.45603596690125414
448448,896897,896896,1793793,1491.7945051193237,0.45510081951397297
449449,898899,898898,1797797,1494.9414868354797,0.4541696031956235
450450,900901,900900,1801801,1498.1076259613037,0.45324229318612197
451451,902903,902902,1805805,1501.2376940250397,0.45231886492911144
452452,904905,904904,1809809,1504.375195980072,0.45139929407923773
453453,906907,906906,1813813,1507.563043832779,0.4504835564894165
454454,908909,908908,1817817,1510.6869552135468,0.4495716282126523
455455,910911,910910,1821821,1513.8116879463196,0.44866348550567636
456456,912913,912912,1825825,1516.9490780830383,0.44775910481257597
457457,914915,914914,1829829,1520.098128080368,0.44685846277752717
458458,916917,916916,1833833,1523.3485720157623,0.44596153624479484
459459,918919,918918,1837837,1526.6128568649292,0.44506830223508587
460460,920921,920920,1841841,1529.7845079898834,0.44417873796373897
461461,922923,922922,1845845,1532.9357159137726,0.44329282083890575
462462,924925,924924,1849849,1536.0722179412842,0.44241052844154183
463463,926927,926926,1853853,1539.2427039146423,0.44153183854541567
464464,928929,928928,1857857,1542.538264989853,0.44065672909891873
465465,930931,930930,1861861,1545.7185559272766,0.4397851782359794
466466,932933,932932,1865865,1548.7998979091644,0.43891716425969207
467467,934935,934934,1869869,1551.9651679992676,0.4380526656532311
468468,936937,936936,1873873,1555.0831520557404,0.43719166107621277
469469,938939,938938,1877877,1558.230463027954,0.43633412935923843
470470,940941,940940,1881881,1561.4068810939789,0.43548004949298047
471471,942943,942942,1885885,1564.5454709529877,0.4346294006536482
472472,944945,944944,1889889,1567.8896470069885,0.433782162173884
473473,946947,946946,1893893,1571.1389141082764,0.4329383135482203
474474,948949,948948,1897897,1574.2778351306915,0.43209783444399363
475475,950951,950950,1901901,1577.4018378257751,0.43126070468861144
476476,952953,952952,1905905,1580.53178191185,0.43042690426409536
477477,954955,954954,1909909,1583.6582968235016,0.42959641331435705
478478,956957,956956,1913913,1586.779145002365,0.42876921214519825
479479,958959,958958,1917917,1589.8959000110626,0.42794528120975883
480480,960961,960960,1921921,1593.0997321605682,0.4271246011212497
481481,962963,962962,1925925,1596.254832983017,0.426307152642039
482482,964965,964964,1929929,1599.399167060852,0.42549291668728983
483483,966967,966966,1933933,1602.5744888782501,0.42468187432314153
484484,968969,968968,1937937,1605.7575500011444,0.42387400676125253
485485,970971,970970,1941941,1608.8805751800537,0.42306929535698146
486486,972973,972972,1945945,1612.014477968216,0.42226772162212
487487,974975,974974,1949949,1615.1437380313873,0.4214692671994271
488488,976977,976976,1953953,1618.282154083252,0.42067391388263786
489489,978979,978978,1957957,1621.4354000091553,0.4198816436019115
490490,980981,980980,1961961,1624.5485861301422,0.41909243843110744
491491,982983,982982,1965965,1627.669986963272,0.41830628873140085
492492,984985,984984,1969969,1630.7920169830322,0.41752317151804164
493493,986987,986986,1973973,1633.9336550235748,0.41674306641834846
494494,988989,988988,1977977,1637.059382200241,0.4159659560518776
495495,990991,990990,1981981,1640.1830830574036,0.4151918231709715
496496,992993,992992,1985985,1643.5108890533447,0.4144206506516639
497497,994995,994994,1989989,1646.7800180912018,0.41365242151005077
498498,996997,996996,1993993,1649.9586489200592,0.4128871188895573
499499,998999,998998,1997997,1653.0769369602203,0.4121247260573
500501,1001003,1001002,2002005,1656.284439086914,0.41136446911150415
501502,1003005,1003004,2006009,1659.4209570884705,0.4106078490440268
502503,1005007,1005006,2010013,1662.6401789188385,0.40985408931555867
503504,1007009,1007008,2014017,1665.880213022232,0.40910317369889526
504505,1009011,1009010,2018021,1669.012097120285,0.4083550860905234
505506,1011013,1011012,2022025,1672.1195549964905,0.40760981049788825
506507,1013015,1013014,2026029,1675.240730047226,0.4068673310612212
507508,1015017,1015016,2030033,1678.386167049408,0.406127632029893
508509,1017019,1017018,2034037,1681.5109939575195,0.4053906977733277
509510,1019021,1019020,2038041,1684.6169791221619,0.4046565127810027
510511,1021023,1021022,2042045,1687.7972960472107,0.4039250616569916
511512,1023025,1023024,2046049,1690.9412989616394,0.4031963291163265
512513,1025027,1025026,2050053,1694.0589439868927,0.4024702999886358
513514,1027029,1027028,2054057,1697.2396922111511,0.4017469592163252
514515,1029031,1029030,2058061,1700.4065759181976,0.4010262918545777
515516,1031033,1031032,2062065,1703.5231919288635,0.4003082830695348
516517,1033035,1033034,2066069,1706.6259360313416,0.39959291813283926
517518,1035037,1035036,2070073,1709.7793979644775,0.39888018242345424
518519,1037039,1037038,2074077,1712.8950560092926,0.3981700614331203
519520,1039041,1039040,2078081,1716.0563850402832,0.3974625407572603
520521,1041043,1041042,2082085,1719.1881470680237,0.39675760609497956
521522,1043045,1043044,2086089,1722.3586361408234,0.3960552432527038
522523,1045047,1045046,2090093,1725.4819960594177,0.3953554381387221
523524,1047049,1047048,2094097,1728.6162419319153,0.39465817675954895
524525,1049051,1049050,2098101,1731.7088010311127,0.39396344523265725
525526,1051053,1051052,2102105,1734.879277229309,0.3932712297682883
526527,1053055,1053054,2106109,1738.0274698734283,0.3925815166785469
527528,1055057,1055056,2110113,1741.1445000171661,0.39189429237558215
528529,1057059,1057058,2114117,1744.260754108429,0.39120954336976865
529530,1059061,1059060,2118121,1747.4505760669708,0.39052725626424944
530531,1061063,1061062,2122125,1750.57945394516,0.389847417762212
531532,1063065,1063064,2126129,1753.7238399982452,0.3891700146614312
532533,1065067,1065066,2130133,1756.8565032482147,0.3884950338560884
533534,1067069,1067068,2134137,1759.9954450130463,0.3878224623276765
534535,1069071,1069070,2138141,1763.111664056778,0.38715228715773264
535536,1071073,1071072,2142145,1766.2569580078125,0.38648449551510566
536537,1073075,1073074,2146149,1769.4203989505768,0.38581907466323173
537538,1075077,1075076,2150153,1772.5440452098846,0.38515601195103955
538539,1077079,1077078,2154157,1775.675409078598,0.38449529482022626
539540,1079081,1079080,2158161,1778.7942957878113,0.3838369108070765
540541,1081083,1081082,2162165,1781.955978155136,0.3831808475188154
541542,1083085,1083084,2166169,1785.230796098709,0.38252709266998863
542543,1085087,1085086,2170173,1788.5393319129944,0.3818756340442633
543544,1087089,1087088,2174177,1791.6827220916748,0.38122645952535095
544545,1089091,1089090,2178181,1794.7995479106903,0.3805795570697228
545546,1091093,1091092,2182185,1797.9232971668243,0.3799349147302564
546547,1093095,1093094,2186189,1801.0389430522919,0.379292520632589
547548,1095097,1095096,2190193,1804.1647939682007,0.3786523629896692
548549,1097099,1097098,2194197,1807.3196589946747,0.3780144300944812
549550,1099101,1099100,2198201,1810.5179960727692,0.37737871032550174
550551,1101103,1101102,2202205,1813.6635301113129,0.37674519213760504
551552,1103105,1103104,2206209,1816.8117461204529,0.3761138640638819
552553,1105107,1105106,2210213,1819.9421031475067,0.37548471472655365
553554,1107109,1107108,2214217,1823.0652329921722,0.37485773281332513
554555,1109111,1109110,2218221,1826.231498003006,0.37423290709739376
555556,1111113,1111112,2222225,1829.380441904068,0.3736102264301735
556557,1113115,1113114,2226229,1832.5903708934784,0.37298967973583785
557558,1115117,1115116,2230233,1835.746726989746,0.37237125601131993
558559,1117119,1117118,2234237,1838.8692932128906,0.37175494433722633
559560,1119121,1119120,2238241,1842.026883840561,0.37114073386510427
560561,1121123,1121122,2242245,1845.1260170936584,0.3705286138174415
561562,1123125,1123124,2246249,1848.3123281002045,0.3699185734931234
562563,1125127,1125126,2250253,1851.4391491413116,0.3693106022619759
563564,1127129,1127128,2254257,1854.6136400699615,0.3687046895702224
564565,1129131,1129130,2258261,1857.759437084198,0.3681008249277511
565566,1131133,1131132,2262265,1860.8816771507263,0.3674989979226666
566567,1133135,1133134,2266269,1864.003713130951,0.3668991982103762
567568,1135137,1135136,2270273,1867.1561181545258,0.36630141551540873
568569,1137139,1137138,2274277,1870.2904450893402,0.36570563963141467
569570,1139141,1139140,2278281,1873.4177911281586,0.36511186042116606
570571,1141143,1141142,2282285,1876.5319900512695,0.36452006781655655
571572,1143145,1143144,2286289,1879.6743738651276,0.3639302518149634
572573,1145147,1145146,2290293,1882.9006159305573,0.36334240248106653
573574,1147149,1147148,2294297,1886.1595721244812,0.3627565099468484
574575,1149151,1149150,2298301,1889.3576400279999,0.3621725644061371
575576,1151153,1151152,2302305,1892.4875979423523,0.3615905561218824
576577,1153155,1153154,2306309,1895.6466541290283,0.3610104754243366
577578,1155157,1155156,2310313,1898.7334659099579,0.36043231269832177
578579,1157159,1157158,2314317,1901.9162690639496,0.3598560584050574
579580,1159161,1159160,2318321,1905.0359802246094,0.35928170305305684
580581,1161163,1161162,2322325,1908.1982719898224,0.3587092372290499
581582,1163165,1163164,2326329,1911.4130189418793,0.35813865157069813
582583,1165167,1165166,2330333,1914.573634147644,0.35756993678296567
583584,1167169,1167168,2334337,1917.692223072052,0.35700308362902433
584585,1169171,1169170,2338341,1920.8162529468536,0.35643808293934853
585586,1171173,1171172,2342345,1923.9656689167023,0.35587492558806844
586587,1173175,1173174,2346349,1927.1689660549164,0.35531360252571176
587588,1175177,1175176,2350353,1930.2921659946442,0.3547541047537379
588589,1177179,1177178,2354357,1933.4266510009766,0.354196423335452
589590,1179181,1179180,2358361,1936.567710161209,0.3536405493887287
590591,1181183,1181182,2362365,1939.7808530330658,0.3530864740914694
591592,1183185,1183184,2366369,1942.9930069446564,0.35253418867978326
592593,1185187,1185186,2370373,1946.1632809638977,0.35198368444071093
593594,1187189,1187188,2374377,1949.3129959106445,0.3514349527285958
594595,1189191,1189190,2378381,1952.4529581069946,0.350887984943256
595596,1191193,1191192,2382385,1955.6330041885376,0.3503427725372603
596597,1193195,1193194,2386389,1958.8973350524902,0.3497993070304801
597598,1195197,1195196,2390393,1962.0493819713593,0.34925757999189955
598599,1197199,1197198,2394397,1965.1541020870209,0.34871758303597744
599600,1199201,1199200,2398401,1968.2661159038544,0.34817930784629425
600601,1201203,1201202,2402405,1971.4339048862457,0.3476427461482672
601602,1203205,1203204,2406409,1974.565680027008,0.3471078897200641
602603,1205207,1205206,2410413,1977.7154169082642,0.34657473039806064
603604,1207209,1207208,2414417,1980.8863849639893,0.346043260067745
604605,1209211,1209210,2418421,1984.0054650306702,0.34551347066553717
605606,1211213,1211212,2422425,1987.176884174347,0.34498535418060783
606607,1213215,1213214,2426429,1990.2835211753845,0.34445890264942136
607608,1215217,1215216,2430433,1993.4371128082275,0.34393410816301184
608609,1217219,1217218,2434437,1996.5836019515991,0.3434109628578881
609610,1219221,1219220,2438441,1999.757719039917,0.3428894589233096
610611,1221223,1221222,2442445,2002.9930489063263,0.34236958859764854
611612,1223225,1223224,2446449,2006.2955479621887,0.34185134416475194
612613,1225227,1225226,2450453,2009.4958741664886,0.3413347179593984
613614,1227229,1227228,2454457,2012.7490890026093,0.3408197023672983
614615,1229231,1229230,2458461,2016.1362390518188,0.34030628981417976
615616,1231233,1231232,2462465,2019.2929091453552,0.3397944727803406
616617,1233235,1233234,2466469,2022.4767761230469,0.3392842437897343
617618,1235237,1235236,2470473,2025.6299121379852,0.33877559540997026
618619,1237239,1237238,2474477,2028.7320120334625,0.3382685202595894
619620,1239241,1239240,2478481,2031.8635761737823,0.33776301099896955
620621,1241243,1241242,2482485,2034.9988720417023,0.3372590603412391
621622,1243245,1243244,2486489,2038.11989402771,0.3367566610304493
622623,1245247,1245246,2490493,2041.282516002655,0.33625580587431614
623624,1247249,1247248,2494497,2044.4289638996124,0.3357564877060213
624625,1249251,1249250,2498501,2047.5937149524689,0.3352586994169542
625626,1251253,1251252,2502505,2050.7111802101135,0.334762433936703
626627,1253255,1253254,2506509,2053.8790969848633,0.33426768423487374
627628,1255257,1255256,2510513,2056.9948949813843,0.333774443330185
628629,1257259,1257258,2514517,2060.130650997162,0.3332827042831923
629630,1259261,1259260,2518521,2063.2598621845245,0.33279246018901176
630631,1261263,1261262,2522525,2066.415102958679,0.33230370419551036
631632,1263265,1263264,2526529,2069.5454030036926,0.3318164294887538
632633,1265267,1265266,2530533,2072.6637489795685,0.3313306292893685
633634,1267269,1267268,2534537,2075.805119037628,0.33084629687255074
634635,1269271,1269270,2538541,2078.925341129303,0.33036342554078146
635636,1271273,1271272,2542545,2082.076539039612,0.3298820086456544
636637,1273275,1273274,2546549,2085.2640058994293,0.32940203957514314
637638,1275277,1275276,2550553,2088.375237941742,0.3289235117572389
638639,1277279,1277278,2554557,2091.4781110286713,0.3284464186617697
639640,1279281,1279280,2558561,2094.629280090332,0.3279707537985814
640641,1281283,1281282,2562565,2097.7560770511627,0.32749651070844266
641642,1283285,1283284,2566569,2100.853175878525,0.32702368298305373
642643,1285287,1285286,2570573,2103.9923000335693,0.3265522642413998
643644,1287289,1287288,2574577,2107.1477031707764,0.32608224814975983
644645,1289291,1289290,2578581,2110.319983959198,0.32561362840715447
645646,1291293,1291292,2582585,2113.4114830493927,0.3251463987489842
646647,1293295,1293294,2586589,2116.542226076126,0.32468055295066733
647648,1295297,1295296,2590593,2119.7070281505585,0.3242160848240019
648649,1297299,1297298,2594597,2122.8501031398773,0.3237529882171657
649650,1299301,1299300,2598601,2125.941927909851,0.3232912570165354
650651,1301303,1301302,2602605,2129.06333899498,0.32283088514304836
651652,1303305,1303304,2606609,2132.233170032501,0.32237186655220285
652653,1305307,1305306,2610613,2135.416501045227,0.3219141952376958
653654,1307309,1307308,2614617,2138.5707879066467,0.3214578652259661
654655,1309311,1309310,2618621,2141.7341310977936,0.3210028705852892
655656,1311313,1311312,2622625,2145.0452921390533,0.32054920540940657
656657,1313315,1313314,2626629,2148.3026168346405,0.32009686383389635
657658,1315317,1315316,2630633,2151.407438993454,0.31964584001980256
658659,1317319,1317318,2634637,2154.5390980243683,0.31919612817546295
659660,1319321,1319320,2638641,2157.6689450740814,0.3187477225346811
660661,1321323,1321322,2642645,2160.794415950775,0.3183006173640024
661662,1323325,1323324,2646649,2163.9211840629578,0.31785480696999
662663,1325327,1325326,2650653,2167.088392972946,0.317410285682854
663664,1327329,1327328,2654657,2170.3101241588593,0.31696704787282215
664665,1329331,1329330,2658661,2173.4371869564056,0.31652508794286405
665666,1331333,1331332,2662665,2176.5390520095825,0.31608440032323415
666667,1333335,1333334,2666669,2179.6888139247894,0.3156449794805667
667668,1335337,1335336,2670673,2182.820550918579,0.3152068199142377
668669,1337339,1337338,2674677,2185.945657014847,0.3147699161545461
669670,1339341,1339340,2678681,2189.0639810562134,0.3143342627554375
670671,1341343,1341342,2682685,2192.1908481121063,0.3138998543181515
671672,1343345,1343344,2686689,2195.321835041046,0.3134666854602983
672673,1345347,1345346,2690693,2198.493592262268,0.31303475083950616
673674,1347349,1347348,2694697,2201.66530585289,0.312604045135231
674675,1349351,1349350,2698701,2204.8179070949554,0.3121745630669466
675676,1351353,1351352,2702705,2207.977371931076,0.31174629937777354
676677,1353355,1353354,2706709,2211.0657300949097,0.3113192488453933
677678,1355357,1355356,2710713,2214.1845037937164,0.31089340627113415
678679,1357359,1357358,2714717,2217.3177769184113,0.31046876649452315
679680,1359361,1359360,2718721,2220.464648962021,0.31004532437509624
680681,1361363,1361362,2722725,2223.5903010368347,0.30962307481058815
681682,1363365,1363364,2726729,2226.7808232307434,0.3092020127187425
682683,1365367,1365366,2730733,2229.898520231247,0.30878213305186364
683684,1367369,1367368,2734737,2233.034812927246,0.3083634307877219
684685,1369371,1369370,2738741,2236.164892911911,0.30794590093864826
685686,1371373,1371372,2742745,2239.3342118263245,0.30752953853334475
686687,1373375,1373374,2746749,2242.447783946991,0.30711433863871207
687688,1375377,1375376,2750753,2245.888589859009,0.3067002963489358
688689,1377379,1377378,2754757,2249.1608130931854,0.3062874067818484
689690,1379381,1379380,2758761,2252.282473087311,0.30587566508256714
690691,1381383,1381382,2762765,2255.4674570560455,0.30546506642167515
691692,1383385,1383384,2766769,2258.616019964218,0.30505560600613535
692693,1385387,1385386,2770773,2261.777065038681,0.3046472790574626
693694,1387389,1387388,2774777,2264.988615989685,0.3042400808317325
694695,1389391,1389390,2778781,2268.172660112381,0.30383400660684856
695696,1391393,1391392,2782785,2271.3075029850006,0.30342905169345613
696697,1393395,1393394,2786789,2274.4245131015778,0.3030252114240284
697698,1395397,1395396,2790793,2277.5784668922424,0.3026224811528664
698699,1397399,1397398,2794797,2280.7039802074432,0.302220856268832
699700,1399401,1399400,2798801,2283.8259930610657,0.30182033217352
700701,1401403,1401402,2802805,2287.0144279003143,0.30142090431218094
701702,1403405,1403404,2806809,2290.160742998123,0.3010225681373413
702703,1405407,1405406,2810813,2293.262759923935,0.30062531913790735
703704,1407409,1407408,2814817,2296.3882989883423,0.3002291528227943
704705,1409411,1409410,2818821,2299.4864132404327,0.2998340647263831
705706,1411413,1411412,2822825,2302.668058872223,0.29944005040488264
706707,1413415,1413414,2826829,2305.7834901809692,0.2990471054454247
707708,1415417,1415416,2830833,2308.922350883484,0.29865522545878775
708709,1417419,1417418,2834837,2312.036199092865,0.29826440606848337
709710,1419421,1419420,2838841,2315.1882750988007,0.2978746429325838
710711,1421423,1421422,2842845,2318.3429760932922,0.29748593173462723
711712,1423425,1423424,2846849,2321.5268528461456,0.2970982681708847
712713,1425427,1425426,2850853,2324.6794440746307,0.29671164797400706
713714,1427429,1427428,2854857,2327.8286349773407,0.29632606688574015
714715,1429431,1429430,2858861,2330.9466400146484,0.29594152068239055
715716,1431433,1431432,2862865,2334.0895750522614,0.2955580051566358
716717,1433435,1433434,2866869,2337.2434589862823,0.29517551613025717
717718,1435437,1435436,2870873,2340.357619047165,0.29479404944140697
718719,1437439,1437438,2874877,2343.5122530460358,0.2944136009500653
719720,1439441,1439440,2878881,2346.6705610752106,0.2940341665453161
720721,1441443,1441442,2882885,2349.8194279670715,0.29365574213079526
721722,1443445,1443444,2886889,2352.9435868263245,0.29327832363560447
722723,1445447,1445446,2890893,2356.0795509815216,0.2929019070143113
723724,1447449,1447448,2894897,2359.1982412338257,0.2925264882378542
724725,1449451,1449450,2898901,2362.349165916443,0.2921520632971806
725726,1451453,1451452,2902905,2365.4747710227966,0.29177862843789626
726727,1453455,1453454,2906909,2368.6388082504272,0.2914061795709131
727728,1455457,1455456,2910913,2371.774528026581,0.2910347126507986
728729,1457459,1457458,2914917,2374.9204199314117,0.29066422376126866
729730,1459461,1459460,2918921,2378.0538079738617,0.290294708995134
730731,1461463,1461462,2922925,2381.216304063797,0.2899261644761282
731732,1463465,1463464,2926929,2384.370092153549,0.2895585863479937
732733,1465467,1465466,2930933,2387.672618150711,0.28919197076538694
733734,1467469,1467468,2934937,2390.8832421302795,0.28882631391388713
734735,1469471,1469470,2938941,2394.005537033081,0.2884616119972634
735736,1471473,1471472,2942945,2397.126242160797,0.28809786123019876
736737,1473475,1473474,2946949,2400.2531809806824,0.2877350578619371
737738,1475477,1475476,2950953,2403.3699259757996,0.2873731981489982
738739,1477479,1477478,2954957,2406.5326709747314,0.2870122783770057
739740,1479481,1479480,2958961,2409.702203989029,0.2866522948424972
740741,1481483,1481482,2962965,2412.903831243515,0.2862932438674761
741742,1483485,1483484,2966969,2416.0326538085938,0.28593512179031677
742743,1485487,1485486,2970973,2419.1554231643677,0.2855779249694024
743744,1487489,1487488,2974977,2422.2840139865875,0.28522164978312503
744745,1489491,1489490,2978981,2425.423793077469,0.28486629262806673
745746,1491493,1491492,2982985,2428.5716800689697,0.28451184991718037
746747,1493495,1493494,2986989,2431.7404561042786,0.2841583180870657
747748,1495497,1495496,2990993,2434.9427359104156,0.2838056935888744
748749,1497499,1497498,2994997,2438.1269631385803,0.2834539728901291
749750,1499501,1499500,2999001,2441.265424013138,0.28310315248199913
750751,1501503,1501502,3003005,2444.41659617424,0.2827532288720249
751752,1503505,1503504,3007009,2447.529319047928,0.2824041985841177
752753,1505507,1505506,3011013,2450.68238902092,0.2820560581640166
753754,1507509,1507508,3015017,2453.8245849609375,0.2817088041701936
754755,1509511,1509510,3019021,2456.9661571979523,0.28136243317931076
755756,1511513,1511512,3023025,2460.11749792099,0.2810169417934958
756757,1513515,1513514,3027029,2463.2386140823364,0.2806723266185145
757758,1515517,1515516,3031033,2466.382683992386,0.28032858429105545
758759,1517519,1517518,3035037,2469.504660129547,0.2799857114569022
759760,1519521,1519520,3039041,2472.6445360183716,0.2796437047818472
760761,1521523,1521522,3043045,2475.794676065445,0.2793025609516917
761762,1523525,1523524,3047049,2478.90354013443,0.278962276659513
762763,1525527,1525526,3051053,2482.067677974701,0.27862284862203524
763764,1527529,1527528,3055057,2485.189106941223,0.27828427357962937
764765,1529531,1529530,3059061,2488.312432050705,0.2779465482726664
765766,1531533,1531532,3063065,2491.4400589466095,0.27760966947244015
766767,1533535,1533534,3067069,2494.5412380695343,0.27727363396115834
767768,1535537,1535536,3071073,2497.6977360248566,0.27693843853376165
768769,1537539,1537538,3075077,2500.7906761169434,0.2766040800088376
769770,1539541,1539540,3079081,2503.979259967804,0.2762705552158877
770771,1541543,1541542,3083085,2507.1164441108704,0.27593786099896533
771772,1543545,1543544,3087089,2510.24178314209,0.27560599423122767
772773,1545547,1545546,3091093,2513.3728709220886,0.275274951776737
773774,1547549,1547548,3095097,2516.530506134033,0.27494473053775437
774775,1549551,1549550,3099101,2519.6567120552063,0.27461532742745476
775776,1551553,1551552,3103105,2522.781137943268,0.2742867393644701
776777,1553555,1553554,3107109,2526.125235080719,0.27395896329107927
777778,1555557,1555556,3111113,2529.426398038864,0.2736319961659319
778779,1557559,1557558,3115117,2532.5576169490814,0.27330583495677274
779780,1559561,1559560,3119121,2535.7424330711365,0.27298047665499325
780781,1561563,1561562,3123125,2538.8794651031494,0.27265591825562296
781782,1563565,1563564,3127129,2542.06085896492,0.2723321567809762
782783,1565567,1565566,3131133,2545.177093029022,0.2720091892606433
783784,1567569,1567568,3135137,2548.3196680545807,0.2716870127351285
784785,1569571,1569570,3139141,2551.4955899715424,0.2713656242740399
785786,1571573,1571572,3143145,2554.6601390838623,0.2710450209433475
786787,1573575,1573574,3147149,2557.8105590343475,0.27072519984176324
787788,1575577,1575576,3151153,2560.9534780979156,0.27040615806618007
788789,1577579,1577578,3155157,2564.0952401161194,0.27008789273713774
789790,1579581,1579580,3159161,2567.245115995407,0.26977040098972793
790791,1581583,1581582,3163165,2570.394743204117,0.2694536799663183
791792,1583585,1583584,3167169,2573.5445079803467,0.2691377268292854
792793,1585587,1585586,3171173,2576.7340371608734,0.2688225387555576
793794,1587589,1587588,3175177,2579.952406167984,0.2685081129293394
794795,1589591,1589590,3179181,2583.0732519626617,0.26819444655484403
795796,1591593,1591592,3183185,2586.26127910614,0.2678815368508367
796797,1593595,1593594,3187189,2589.405543088913,0.2675693810433586
797798,1595597,1595596,3191193,2592.536509990692,0.26725797637482174
798799,1597599,1597598,3195197,2595.6550171375275,0.2669473201058281
799800,1599601,1599600,3199201,2598.7627971172333,0.26663740950243664
800801,1601603,1601602,3203205,2601.9204380512238,0.26632824184889614
801802,1603605,1603604,3207209,2605.3009791374207,0.26601981444582634
802803,1605607,1605606,3211213,2608.55672621727,0.26571212459384697
803804,1607609,1607608,3215217,2611.701003074646,0.26540516962268157
804805,1609611,1609610,3219221,2614.8715641498566,0.2650989468656917
805806,1611613,1611612,3223225,2618.038733959198,0.2647934536689718
806807,1613615,1613614,3227229,2621.2504642009735,0.2644886874004442
807808,1615617,1615616,3231233,2624.4814291000366,0.26418464542621223
808809,1617619,1617618,3235237,2627.6138050556183,0.2638813251378451
809810,1619621,1619620,3239241,2630.7219960689545,0.26357872393236903
810811,1621623,1621622,3243245,2633.8733241558075,0.263276839223181
811812,1623625,1623624,3247249,2636.985948085785,0.2629756684345921
812813,1625627,1625626,3251253,2640.1370561122894,0.2626752090000082
813814,1627629,1627628,3255257,2643.2748959064484,0.26237545836920617
814815,1629631,1629630,3259261,2646.4392552375793,0.2620764140065148
815816,1631633,1631632,3263265,2649.5352940559387,0.2617780733817199
816817,1633635,1633634,3267269,2652.6658141613007,0.261480433980978
817818,1635637,1635636,3271273,2655.7987110614777,0.2611834933013597
818819,1637639,1637638,3275277,2658.9482851028442,0.26088724885448755
819820,1639641,1639640,3279281,2662.095563173294,0.26059169815926
820821,1641643,1641642,3283285,2665.5040459632874,0.26029683874548937
821822,1643645,1643644,3287289,2668.7300679683685,0.260002668161178
822823,1645647,1645646,3291293,2671.8082242012024,0.25970918395978515
823824,1647649,1647648,3295297,2674.960009098053,0.25941638371295994
824825,1649651,1649650,3299301,2678.1148500442505,0.2591242649996275
825826,1651653,1651652,3303305,2681.239593029022,0.25883282540416985
826827,1653655,1653654,3307309,2684.413675069809,0.25854206253643497
827828,1655657,1655656,3311313,2687.528727054596,0.25825197400627076
828829,1657659,1657658,3315317,2690.726443052292,0.25796255743807706
829830,1659661,1659660,3319321,2693.889322042465,0.2576738104708056
830831,1661663,1661662,3323325,2696.993621110916,0.2573857307434082
831832,1663665,1663664,3327329,2700.1247730255127,0.2570983159203024
832833,1665667,1665666,3331333,2703.2572298049927,0.25681156366954383
833834,1667669,1667668,3335337,2706.4227850437164,0.256525471670102
834835,1669671,1669670,3339341,2709.54309797287,0.2562400376118603
835836,1671673,1671672,3343345,2712.819538116455,0.2559552591974352
836837,1673675,1673674,3347349,2716.185425043106,0.25567113413853804
837838,1675677,1675676,3351353,2719.398089170456,0.255387660157794
838839,1677679,1677678,3355357,2722.52449798584,0.25510483499056136
839840,1679681,1679680,3359361,2725.6684172153473,0.2548226563776552
840841,1681683,1681682,3363365,2728.776460170746,0.2545411220744427
841842,1683685,1683684,3367369,2731.898810863495,0.25426022985084273
842843,1685687,1685686,3371373,2735.242849111557,0.2539799774731364
843844,1687689,1687688,3375377,2738.481708049774,0.2537003627312515
844845,1689691,1689690,3379381,2741.617441177368,0.25342138342239195
845846,1691693,1691692,3383385,2744.753441095352,0.2531430373492185
846847,1693695,1693694,3387389,2747.9112989902496,0.25286532233440084
847848,1695697,1695696,3391393,2751.0471000671387,0.2525882361951517
848849,1697699,1697698,3395397,2754.2194278240204,0.2523117767759686
849850,1699701,1699700,3399401,2757.3616411685944,0.2520359419140732
850851,1701703,1701702,3403405,2760.548420906067,0.2517607294739719
851852,1703705,1703704,3407409,2763.718403816223,0.25148613731471414
852853,1705707,1705706,3411413,2766.892637014389,0.2512121633189963
853854,1707709,1707708,3415417,2769.9895498752594,0.25093880536405777
854855,1709711,1709710,3419421,2773.154402256012,0.2506660613526037
855856,1711713,1711712,3423425,2776.2506268024445,0.2503939291818824
856857,1713715,1713714,3427429,2779.4572830200195,0.25012240677097
857858,1715717,1715716,3431433,2782.6283128261566,0.2498514920425805
858859,1717719,1717718,3435437,2785.777922153473,0.24958118293034204
859860,1719721,1719720,3439441,2788.9110720157623,0.24931147737333959
860861,1721723,1721722,3443445,2792.0710339546204,0.24904237332884804
861862,1723725,1723724,3447449,2795.184536933899,0.2487738687541423
862863,1725727,1725726,3451453,2798.345316886902,0.2485059616228682
863864,1727729,1727728,3455457,2801.46950006485,0.2482386499104905
864865,1729731,1729730,3459461,2804.7553770542145,0.24797193160520692
865866,1731733,1731732,3463465,2808.0416860580444,0.2477058047097671
866867,1733735,1733734,3467469,2811.1813700199127,0.24744026723055867
867868,1735737,1735736,3471473,2814.3051459789276,0.2471753171794262
868869,1737739,1737738,3475477,2817.434007167816,0.24691095258276619
869870,1739741,1739740,3479481,2820.565299987793,0.24664717147607007
870871,1741743,1741742,3483485,2823.7294840812683,0.24638397190210526
871872,1743745,1743744,3487489,2826.894401073456,0.24612135190727713
872873,1745747,1745746,3491493,2830.108241081238,0.24585930955618096
873874,1747749,1747748,3495497,2833.2601039409637,0.24559784291705
874875,1749751,1749750,3499501,2836.408117055893,0.24533695006357448
875876,1751753,1751752,3503505,2839.5480301380157,0.2450766290858155
876877,1753755,1753754,3507509,2842.6724710464478,0.2448168780774722
877878,1755757,1755756,3511513,2845.800358057022,0.24455769513951964
878879,1757759,1757758,3515517,2848.9573760032654,0.24429907838566578
879880,1759761,1759760,3519521,2852.0851500034332,0.2440410259332566
880881,1761763,1761762,3523525,2855.210900068283,0.243783535912371
881882,1763765,1763764,3527529,2858.3726329803467,0.24352660645854485
882883,1765767,1765766,3531533,2861.4872410297394,0.24327023571640893
883884,1767769,1767768,3535537,2864.6749992370605,0.243014421841508
884885,1769771,1769770,3539541,2867.7640199661255,0.24275916298938682
885886,1771773,1771772,3543545,2870.9114830493927,0.242504457335599
886887,1773775,1773774,3547549,2874.0208480358124,0.2422503030520602
887888,1775777,1775776,3551553,2877.1455430984497,0.24199669832887594
888889,1777779,1777778,3555557,2880.2685861587524,0.2417436413543328
889890,1779781,1779780,3559561,2883.421200990677,0.2414911303367262
890891,1781783,1781782,3563565,2886.6207571029663,0.24123916347707564
891892,1783785,1783784,3567569,2889.7640120983124,0.24098773899822845
892893,1785787,1785786,3571573,2893.0581908226013,0.240736855121213
893894,1787789,1787788,3575577,2896.3701169490814,0.24048651008342858
894895,1789791,1789790,3579581,2899.5963048934937,0.24023670212045545
895896,1791793,1791792,3583585,2902.740494966507,0.2399874294824258
896897,1793795,1793794,3587589,2905.8592689037323,0.23973869042674778
897898,1795797,1795796,3591593,2909.003231048584,0.23949048321264854
898899,1797799,1797798,3595597,2912.1081070899963,0.23924280611572613
899900,1799801,1799800,3599601,2915.3624358177185,0.2389956574097596
900901,1801803,1801802,3603605,2918.6244370937347,0.2387490353848989
901902,1803805,1803804,3607609,2921.8278641700745,0.23850293833311298
902903,1805807,1805806,3611613,2924.9723269939423,0.23825736455182778
903904,1807809,1807808,3615617,2928.1134610176086,0.23801231235302112
904905,1809811,1809810,3619621,2931.224671125412,0.2377677800523088
905906,1811813,1811812,3623625,2934.3796820640564,0.23752376596894464
906907,1813815,1813814,3627629,2937.540514230728,0.23728026843673433
907908,1815817,1815816,3631633,2940.694048166275,0.23703728579130257
908909,1817819,1817818,3635637,2943.867718935013,0.23679481637918798
909910,1819821,1819820,3639641,2947.060217857361,0.2365528585451102
910911,1821823,1821822,3643645,2950.1815440654755,0.23631141065561678
911912,1823825,1823824,3647649,2953.3035731315613,0.23607047107179824
912913,1825827,1825826,3651653,2956.447986125946,0.23583003816747805
913914,1827829,1827828,3655657,2959.6224360466003,0.23559011032193666
914915,1829831,1829830,3659661,2962.7672760486603,0.23535068592354946
915916,1831833,1831832,3663665,2965.8940761089325,0.23511176336432982
916917,1833835,1833834,3667669,2969.257822036743,0.23487334104356705
917918,1835837,1835836,3671673,2972.4134001731873,0.23463541736964544
918919,1837839,1837838,3675677,2975.5912668704987,0.23439799075640622
919920,1839841,1839840,3679681,2978.707733154297,0.23416105962496658
920921,1841843,1841842,3683685,2981.835058927536,0.2339246224019007
921922,1843845,1843844,3687689,2985.03227186203,0.2336886775210587
922923,1845847,1845846,3691693,2988.20494389534,0.23345322342720465
923924,1847849,1847848,3695697,2991.2994079589844,0.23321825855964562
924925,1849851,1849850,3699701,2994.4383850097656,0.23298378137951659
925926,1851853,1851852,3703705,2997.5458691120148,0.23274979034613352
926927,1853855,1853854,3707709,3000.7041029930115,0.23251628392608836
927928,1855857,1855856,3711713,3003.853234052658,0.23228326058961102
928929,1857859,1857858,3715717,3007.077802181244,0.23205071882148331
929930,1859861,1859860,3719721,3010.1696860790253,0.2318186571028491
930931,1861863,1861862,3723725,3013.2959520816803,0.23158707393304212
931932,1863865,1863864,3727729,3016.5216131210327,0.23135596780775813
932933,1865867,1865866,3731733,3019.86638712883,0.23112533722814987
933934,1867869,1867868,3735737,3023.081181049347,0.23089518071174098
934935,1869871,1869870,3739741,3026.241136074066,0.23066549677787407
935936,1871873,1871872,3743745,3029.3889269828796,0.23043628394589177
936937,1873875,1873874,3747749,3032.5254559516907,0.23020754074605065
937938,1875877,1875876,3751753,3035.7653279304504,0.2299792657195212
938939,1877879,1877878,3755757,3038.8831429481506,0.22975145740019798
939940,1879881,1879880,3759761,3042.043555021286,0.22952411434562237
940941,1881883,1881882,3763765,3045.3150169849396,0.2292972351078788
941942,1883885,1883884,3767769,3048.4541771411896,0.22907081824814668
942943,1885887,1885886,3771773,3051.5835371017456,0.22884486233124335
943944,1887889,1887888,3775777,3054.7131128311157,0.22861936592926213
944945,1889891,1889890,3779781,3057.852516889572,0.22839432762521028
945946,1891893,1891892,3783785,3060.971694946289,0.22816974599845707
946947,1893895,1893894,3787789,3064.081295967102,0.22794561963928572
947948,1895897,1895896,3791793,3067.271776199341,0.22772194714889338
948949,1897899,1897898,3795797,3070.438849210739,0.2274987271248392
949950,1899901,1899900,3799801,3073.578472137451,0.22727595817559632
950951,1901903,1901902,3803805,3076.7565310001373,0.22705363891691377
951952,1903905,1903904,3807809,3080.0741641521454,0.22683176796635962
952953,1905907,1905906,3811813,3083.260200023651,0.22661034395059687
953954,1907909,1907908,3815817,3086.4427120685577,0.22638936549628852
954955,1909911,1909910,3819821,3089.5866298675537,0.22616883124464948
955956,1911913,1911912,3823825,3092.7177970409393,0.2259487398332567
956957,1913915,1913914,3827829,3095.9360988140106,0.22572908991060103
957958,1915917,1915916,3831833,3099.1507160663605,0.22550988013063034
958959,1917919,1917918,3835837,3102.347825050354,0.22529110914911143
959960,1919921,1919920,3839841,3105.5874769687653,0.2250727756345441
960961,1921923,1921922,3843845,3109.056415081024,0.22485487825179007
961962,1923925,1923924,3847849,3112.246376991272,0.22463741568026308
962963,1925927,1925926,3851853,3115.3837389945984,0.22442038659573882
963964,1927929,1927928,3855857,3118.502692937851,0.22420378968490695
964965,1929931,1929930,3859861,3121.6567089557648,0.2239876236399141
965966,1931933,1931932,3863865,3124.7923011779785,0.22377188715836382
966967,1933935,1933934,3867869,3127.9908318519592,0.22355657893604075
967968,1935937,1935936,3871873,3131.1776089668274,0.22334169768510037
968969,1937939,1937938,3875877,3134.302939891815,0.2231272421158792
969970,1939941,1939940,3879881,3137.4310171604156,0.2229132109459897
970971,1941943,1941942,3883885,3140.598300933838,0.22269960289668234
971972,1943945,1943944,3887889,3143.8412630558014,0.2224864166964835
972973,1945947,1945946,3891893,3147.134532928467,0.22227365107937658
973974,1947949,1947948,3895897,3150.242141008377,0.22206130477934494
974975,1949951,1949950,3899901,3153.499256849289,0.22184937654492387
975976,1951953,1951952,3903905,3156.7019867897034,0.2216378651191917
976977,1953955,1953954,3907909,3159.8160421848297,0.2214267692543217
977978,1955957,1955956,3911913,3163.0062930583954,0.22121608771522006
978979,1957959,1957958,3915917,3166.122011899948,0.221005819259517
979980,1959961,1959960,3919921,3169.2861409187317,0.22079596265211876
980981,1961963,1961962,3923925,3172.404706954956,0.2205865166743024
981982,1963965,1963964,3927929,3175.546851873398,0.2203774800982501
982983,1965967,1965966,3931933,3178.6548340320587,0.2201688517088769
983984,1967969,1967968,3935937,3181.795439004898,0.21996063028927892
984985,1969971,1969970,3939941,3184.9175820350647,0.21975281463892316
985986,1971973,1971972,3943945,3188.098969936371,0.21954540355000063
986987,1973975,1973974,3947949,3191.246320962906,0.21933839582561632
987988,1975977,1975976,3951953,3194.400829076767,0.21913179027251317
988989,1977979,1977978,3955957,3197.487025976181,0.2189255857028911
989990,1979981,1979980,3959961,3200.64662194252,0.21871978093076905
990991,1981983,1981982,3963965,3203.85978102684,0.21851437477926083
991992,1983985,1983984,3967969,3207.151419878006,0.21830936607329932
992993,1985987,1985986,3971973,3210.3389620780945,0.2181047536432743
993994,1987989,1987988,3975977,3213.5356738567352,0.2179005363232136
994995,1989991,1989990,3979981,3216.726588010788,0.21769671295260196
995996,1991993,1991992,3983985,3219.8757379055023,0.2174932823763811
996997,1993995,1993994,3987989,3223.101881980896,0.21729024344313075
997998,1995997,1995996,3991993,3226.2371332645416,0.2170875950014306
998999,1997999,1997998,3995997,3229.360999107361,0.21688533591441228
1000000,2000001,2000000,4000001,3232.502713918686,0.2166834650452074


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0029349327087402344,12064.709122577777
1001,2003,1001,3004,3.814255714416504,1.081112418198245
2002,4005,2002,6007,7.438738822937012,0.23651446568328538
3003,6007,3003,9010,11.312902688980103,0.1033214599101484
4004,8009,4004,12013,15.392501831054688,0.05736764844004938
5005,10011,5005,15016,19.37235188484192,0.03677323784904729
6006,12013,6006,18019,23.76543092727661,0.026102900248588412
7007,14015,7007,21022,27.416931867599487,0.019222093715143274
8008,16017,8008,24025,31.04142689704895,0.014864625576592516
9009,18019,9009,27028,34.61112594604492,0.011805651212853263
10010,20021,10010,30031,38.26709985733032,0.009544548203848535
11011,22023,11011,33034,41.95066690444946,0.007896683888247935
12012,24025,12012,36037,45.69839000701904,0.00659135574096581
13013,26027,13013,39040,49.17533588409424,0.0055896630001370795
14014,28029,14014,42043,52.33380699157715,0.004792524105141638
15015,30031,15015,45046,55.53766393661499,0.00414137494226452
16016,32033,16016,48049,58.72829270362854,0.0036119735123065766
17017,34035,17017,51052,61.91007995605469,0.003173069149852381
18018,36037,18018,54055,65.07790780067444,0.0028111199808336096
19019,38039,19019,57058,68.23487091064453,0.0025028508498508018
20020,40041,20020,60061,71.38699698448181,0.002241971844341606
21021,42043,21021,63064,74.56941795349121,0.0020186352958262432
22022,44045,22022,66067,77.75248980522156,0.0018273158493684605
23023,46047,23023,69070,81.33155608177185,0.0016630015616101446
24024,48049,24024,72073,84.46893286705017,0.001516828224339406
25025,50051,25025,75076,87.64894890785217,0.001391092575431685
26026,52053,26026,78079,90.76573204994202,0.0012795733364328044
27027,54055,27027,81082,93.92856788635254,0.0011810493560915347
28028,56057,28028,84085,97.03047704696655,0.001094615952752065
29029,58059,29029,87088,100.59425973892212,0.001015768211800605
30030,60061,30030,90091,103.72895193099976,0.0009469393517065328
31031,62063,31031,93094,107.10560894012451,0.0008845652610034449
32032,64065,32032,96097,110.34594202041626,0.0008282670551125193
33033,66067,33033,99100,113.45813870429993,0.0007780286869092379
34034,68069,34034,102103,116.61467480659485,0.0007316113315027906
35035,70071,35035,105106,120.15351486206055,0.0006906106282258406
36036,72073,36036,108109,123.32692670822144,0.0006527325913339155
37037,74075,37037,111112,126.45845603942871,0.0006181628468766576
38038,76077,38038,114115,129.59396195411682,0.0005869194174010772
39039,78079,39039,117118,132.80724382400513,0.0005577117262873799
40040,80081,40040,120121,136.04245781898499,0.0005314653353707399
41041,82083,41041,123124,139.56394791603088,0.0005068210066383472
42042,84085,42042,126127,142.7154097557068,0.0004841958561883075
43043,86087,43043,129130,145.84037590026855,0.0004633940479834564
44044,88089,44044,132133,149.01714992523193,0.00044364019595377613
45045,90091,45045,135136,152.22818565368652,0.0004259109864506172
46046,92093,46046,138139,155.35653686523438,0.0004090492693649139
47047,94095,47047,141142,158.5482497215271,0.00039354062573693227
48048,96097,48048,144145,161.74791598320007,0.0003790990340348799
49049,98099,49049,147148,164.9419538974762,0.00036568315226759296
50050,100101,50050,150151,168.03075289726257,0.00035356161060917657
51051,102103,51051,153154,171.18036603927612,0.0003419875865802169
52052,104105,52052,156157,174.31843495368958,0.0003315274152555503
53053,106107,53053,159160,177.4928686618805,0.00032163729156309273
54054,108109,54054,162163,180.80200386047363,0.00031195291740004905
55055,110111,55055,165166,184.16376972198486,0.00030303633684525266
56056,112113,56056,168169,187.50724697113037,0.00029428337620629463
57057,114115,57057,171172,190.840922832489,0.0002860368258552626
58058,116117,58058,174175,194.18677687644958,0.00027807352307718247
59059,118119,59059,177178,197.55430793762207,0.0002701857392821694
60060,120121,60060,180181,200.8835198879242,0.0002628112088132184
61061,122123,61061,183184,204.2026298046112,0.00025547312725393567
62062,124125,62062,186187,207.6540768146515,0.0002485995792085305
63063,126127,63063,189190,211.1269018650055,0.00024188053248508368
64064,128129,64064,192193,214.45727682113647,0.00023525397409684956
65065,130131,65065,195196,217.8007128238678,0.00022901087868376635
66066,132133,66066,198199,221.1649148464203,0.0002227404202130856
67067,134135,67067,201202,224.49698567390442,0.00021670449314115103
68068,136137,68068,204205,227.9295196533203,0.00021082127204863355
69069,138139,69069,207208,231.30770683288574,0.0002050726816378301
70070,140141,70070,210211,234.6520698070526,0.00019969312415923923
71071,142143,71071,213214,238.00091171264648,0.000194501235455391
72072,144145,72072,216217,241.3759458065033,0.00018948895194625948
73073,146147,73073,219220,244.75707697868347,0.00018453031589160673
74074,148149,74074,222223,248.10691285133362,0.00017973863577935845
75075,150151,75075,225226,251.42265582084656,0.00017511609621578828
76076,152153,76076,228229,254.79598474502563,0.0001703733159956755
77077,154155,77077,231232,258.14615178108215,0.00016573125503782649
78078,156157,78078,234235,261.49320578575134,0.00016107034934975673
79079,158159,79079,237238,264.83274579048157,0.00015636643183825072
80080,160161,80080,240241,268.1673209667206,0.00015177652494458016
81081,162163,81081,243244,271.58967900276184,0.0001470652441639686
82082,164165,82082,246247,274.89964985847473,0.00014241270764614455
83083,166167,83083,249250,278.25491094589233,0.00013771186604571994
84084,168169,84084,252253,281.6021807193756,0.00013294586642587092
85085,170171,85085,255256,284.97570991516113,0.00012838259135605767
86086,172173,86086,258259,288.2978847026825,0.00012396969032124616
87087,174175,87087,261262,291.6038718223572,0.0001199091893795412
88088,176177,88088,264265,294.94205474853516,0.00011582251863728743
89089,178179,89089,267268,298.3127727508545,0.0001116852381528588
90090,180181,90090,270271,301.6616897583008,0.00010794173613248859
91091,182183,91091,273274,304.99639892578125,0.00010416499026177917
92092,184185,92092,276277,308.30326795578003,0.00010040933193522505
93093,186187,93093,279280,311.67064690589905,9.660917021392379e-05
94094,188189,94094,282283,315.0936577320099,9.30845199036412e-05
95095,190191,95095,285286,318.4010429382324,8.960674313129857e-05
96096,192193,96096,288289,321.7499167919159,8.611644989287015e-05
97097,194195,97097,291292,325.05195903778076,8.262146366178058e-05
98098,196197,98098,294295,328.4229817390442,7.912145338195842e-05
99099,198199,99099,297298,331.7641179561615,7.559852929261979e-05
100100,200201,100100,300301,335.07679200172424,7.205719703051727e-05
101101,202203,101101,303304,338.3998749256134,6.842176298960112e-05
102102,204205,102102,306307,341.78729581832886,6.477458373410627e-05
103103,206207,103103,309310,345.1681399345398,6.125335858087055e-05
104104,208209,104104,312313,348.64675092697144,5.774228884547483e-05
105105,210211,105105,315316,352.035612821579,5.4209758673096076e-05
106106,212213,106106,318319,355.3739969730377,5.0599051974131726e-05
107107,214215,107107,321322,358.70293498039246,4.697754229709972e-05
108108,216217,108108,324325,362.06733107566833,4.3422898670542054e-05
109109,218219,109109,327328,365.39985179901123,4.0078059100778773e-05
110110,220221,110110,330331,368.7344298362732,3.748267590708565e-05
111111,222223,111111,333334,372.1106958389282,3.537140219123103e-05
112112,224225,112112,336337,375.5574028491974,3.357582500029821e-05
113113,226227,113113,339340,378.8812258243561,3.1772888178238645e-05
114114,228229,114114,342343,382.2576549053192,2.9990122129675e-05
115115,230231,115115,345346,385.59646677970886,2.8210008167661726e-05
116116,232233,116116,348349,388.90149688720703,2.6607442123349756e-05
117117,234235,117117,351352,392.3258008956909,2.5210547391907312e-05
118118,236237,118118,354355,395.6301758289337,2.4026487153605558e-05
119119,238239,119119,357358,398.98450994491577,2.2831371097709052e-05
120120,240241,120120,360361,402.29383277893066,2.160562689823564e-05
121121,242243,121121,363364,405.6561598777771,2.0328161554061808e-05
122122,244245,122122,366367,408.99699783325195,1.904594319057651e-05
123123,246247,123123,369370,412.30432987213135,1.7725013094604947e-05
124124,248249,124124,372373,415.6840078830719,1.6412392142228782e-05
125125,250251,125125,375376,419.01412868499756,1.5090223314473405e-05
126126,252253,126126,378379,422.38878202438354,1.3727494660997763e-05
127127,254255,127127,381382,425.708438873291,1.2336744475760497e-05
128128,256257,128128,384385,429.0252888202667,1.0928586561931297e-05
129129,258259,129129,387388,432.36354875564575,1.0320472938474268e-05
130130,260261,130130,390391,435.7038109302521,1.0474112059455365e-05
131131,262263,131131,393394,439.0241367816925,1.0559393558651209e-05
132132,264265,132132,396397,442.36266684532166,1.0672009011614136e-05
133133,266267,133133,399400,445.68483781814575,1.0802243195939809e-05
134134,268269,134134,402403,449.02320408821106,1.0829622624441981e-05
135135,270271,135135,405406,452.3699357509613,1.086459269572515e-05
136136,272273,136136,408409,455.72707986831665,1.0883411960094236e-05
137137,274275,137137,411412,459.08720993995667,1.0955009202007204e-05
138138,276277,138138,414415,462.4105839729309,1.1034875569748692e-05
139139,278279,139139,417418,465.9713110923767,1.1150621503475122e-05
140140,280281,140140,420421,469.3424618244171,1.1223884939681739e-05
141141,282283,141141,423424,472.69530177116394,1.1599138815654442e-05
142142,284285,142142,426427,476.0490050315857,1.1976573659921996e-05
143143,286287,143143,429430,479.40621995925903,1.2380098269204609e-05
144144,288289,144144,432433,482.79568099975586,1.2766464351443574e-05
145145,290291,145145,435436,486.1354479789734,1.3119279174134135e-05
146146,292293,146146,438439,489.4423348903656,1.3451714039547369e-05
147147,294295,147147,441442,492.7888607978821,1.3696615496883169e-05
148148,296297,148148,444445,496.11070585250854,1.3847000445821323e-05
149149,298299,149149,447448,499.47171783447266,1.3993787433719262e-05
150150,300301,150150,450451,502.8089747428894,1.4115632438915782e-05
151151,302303,151151,453454,506.15341687202454,1.4210754670784809e-05
152152,304305,152152,456457,509.59619975090027,1.4354545783135109e-05
153153,306307,153153,459460,512.9294037818909,1.4484479834209196e-05
154154,308309,154154,462463,516.2736339569092,1.4583352822228335e-05
155155,310311,155155,465466,519.617429971695,1.4637349522672594e-05
156156,312313,156156,468469,523.0572509765625,1.4653125617769547e-05
157157,314315,157157,471472,526.7601459026337,1.4636614650953561e-05
158158,316317,158158,474475,530.2126529216766,1.4575163731933571e-05
159159,318319,159159,477478,533.6957569122314,1.4486724467133172e-05
160160,320321,160160,480481,537.2894577980042,1.4357654436025769e-05
161161,322323,161161,483484,540.6742849349976,1.4269962775870226e-05
162162,324325,162162,486487,544.0044898986816,1.4257257134886459e-05
163163,326327,163163,489490,547.3764758110046,1.4179584468365647e-05
164164,328329,164164,492493,550.6997907161713,1.4053466657060198e-05
165165,330331,165165,495496,554.0121078491211,1.3907894754083827e-05
166166,332333,166166,498499,557.3871648311615,1.377645821776241e-05
167167,334335,167167,501502,560.7088539600372,1.364433228445705e-05
168168,336337,168168,504505,564.0494267940521,1.3492142898030579e-05
169169,338339,169169,507508,567.3824338912964,1.3317734556039795e-05
170170,340341,170170,510511,570.7157878875732,1.312246240559034e-05
171171,342343,171171,513514,574.06112408638,1.2983542546862736e-05
172172,344345,172172,516517,577.411367893219,1.2859434718848206e-05
173173,346347,173173,519520,580.7428948879242,1.272346344194375e-05
174174,348349,174174,522523,584.1290926933289,1.2572952982736751e-05
175175,350351,175175,525526,587.5089237689972,1.2476049960241653e-05
176176,352353,176176,528529,590.9020719528198,1.2432832591002807e-05
177177,354355,177177,531532,594.2229979038239,1.2351960322121158e-05
178178,356357,178178,534535,597.5662467479706,1.224707011715509e-05
179179,358359,179179,537538,600.9158546924591,1.2188620530650951e-05
180180,360361,180180,540541,604.3209338188171,1.212014103657566e-05
181181,362363,181181,543544,607.8925149440765,1.2015820175292902e-05
182182,364365,182182,546547,611.5372858047485,1.2069956937921233e-05
183183,366367,183183,549550,614.9840829372406,1.2110856914659962e-05
184184,368369,184184,552553,618.2901418209076,1.2129296010243706e-05
185185,370371,185185,555556,621.6284708976746,1.2110966054024175e-05
186186,372373,186186,558559,624.9476528167725,1.2064434486092068e-05
187187,374375,187187,561562,628.3228468894958,1.2021759175695479e-05
188188,376377,188188,564565,631.7325277328491,1.1993388397968374e-05
189189,378379,189189,567568,635.1056518554688,1.1950985935982317e-05
190190,380381,190190,570571,638.4269580841064,1.1862079190905206e-05
191191,382383,191191,573574,641.7528870105743,1.173504460894037e-05
192192,384385,192192,576577,645.1538717746735,1.1593821909627877e-05
193193,386387,193193,579580,648.4800839424133,1.1523246939759701e-05
194194,388389,194194,582583,651.8114159107208,1.1469845048850402e-05
195195,390391,195195,585586,655.1387858390808,1.1459602319519036e-05
196196,392393,196196,588589,658.6610469818115,1.1395313777029514e-05
197197,394395,197197,591592,662.3081579208374,1.1274125427007675e-05
198198,396397,198198,594595,665.6531209945679,1.1095880836364813e-05
199199,398399,199199,597598,669.0092267990112,1.0954718163702637e-05
200200,400401,200200,600601,672.3306539058685,1.0793333785841241e-05
201201,402403,201201,603604,675.7038760185242,1.0594234481686726e-05
202202,404405,202202,606607,679.0326566696167,1.0328327334718779e-05
203203,406407,203203,609610,682.3896179199219,1.0044968803413212e-05
204204,408409,204204,612613,685.7092978954315,9.769933967618272e-06
205205,410411,205205,615616,689.0650098323822,9.577008313499391e-06
206206,412413,206206,618619,692.4045879840851,9.36941069085151e-06
207207,414415,207207,621622,695.7768688201904,9.169636541628279e-06
208208,416417,208208,624625,699.1443419456482,9.167442840407602e-06
209209,418419,209209,627628,702.4342188835144,9.144721843767911e-06
210210,420421,210210,630631,705.7912459373474,9.269573638448492e-06
211211,422423,211211,633634,709.1162009239197,9.479865184403025e-06
212212,424425,212212,636637,712.467033624649,9.657325790612958e-06
213213,426427,213213,639640,715.7965228557587,9.824527296586893e-06
214214,428429,214214,642643,719.1251540184021,9.948824299499393e-06
215215,430431,215215,645646,722.5003917217255,1.0038198524853215e-05
216216,432433,216216,648649,725.9528429508209,1.0118543286807835e-05
217217,434435,217217,651652,729.4012620449066,1.0160847523366101e-05
218218,436437,218218,654655,732.7392299175262,1.0173929695156403e-05
219219,438439,219219,657658,736.0814008712769,1.0182093319599517e-05
220220,440441,220220,660661,739.4111688137054,1.0162881153519265e-05
221221,442443,221221,663664,742.8036968708038,1.0115567420143634e-05
222222,444445,222222,666667,746.1364059448242,1.005233389150817e-05
223223,446447,223223,669670,749.505735874176,1.0034797014668584e-05
224224,448449,224224,672673,752.9181706905365,9.999335816246457e-06
225225,450451,225225,675676,756.2699477672577,9.981815310311504e-06
226226,452453,226226,678679,759.6034557819366,9.946337740984745e-06
227227,454455,227227,681682,762.9045088291168,9.913868780131452e-06
228228,456457,228228,684685,766.2734699249268,9.851315553532913e-06
229229,458459,229229,687688,769.6029009819031,9.769606549525633e-06
230230,460461,230230,690691,772.9707777500153,9.652023436501622e-06
231231,462463,231231,693694,776.2916059494019,9.528990631224588e-06
232232,464465,232232,696697,779.6078717708588,9.395289453095756e-06
233233,466467,233233,699700,782.9761078357697,9.233734090230428e-06
234234,468469,234234,702703,786.4788358211517,9.044029866345227e-06
235235,470471,235235,705706,790.063622713089,8.881406756700017e-06
236236,472473,236236,708709,793.4085297584534,8.8175820565084e-06
237237,474475,237237,711712,796.7687909603119,8.766035534790717e-06
238238,476477,238238,714715,800.0891649723053,8.702108971192501e-06
239239,478479,239239,717718,803.6825699806213,8.605853508925065e-06
240240,480481,240240,720721,807.1729388237,8.473409252474084e-06
241241,482483,241241,723724,810.5188808441162,8.423858162132092e-06
242242,484485,242242,726727,813.8676588535309,8.39754102344159e-06
243243,486487,243243,729730,817.2206358909607,8.34877573652193e-06
244244,488489,244244,732733,820.5577960014343,8.273405910586007e-06
245245,490491,245245,735736,823.8717539310455,8.198960131267086e-06
246246,492493,246246,738739,827.2304680347443,8.104163498501293e-06
247247,494495,247247,741742,830.5810668468475,7.997790817171335e-06
248248,496497,248248,744745,833.913899898529,7.887101673986763e-06
249249,498499,249249,747748,837.2460289001465,7.77301102061756e-06
250250,500501,250250,750751,840.5897529125214,7.641227057320066e-06
251251,502503,251251,753754,843.970901966095,7.485370588256046e-06
252252,504505,252252,756757,847.2884979248047,7.390346581814811e-06
253253,506507,253253,759760,850.6402926445007,7.32052831153851e-06
254254,508509,254254,762763,853.9739739894867,7.249809641507454e-06
255255,510511,255255,765766,857.3537290096283,7.184977221186273e-06
256256,512513,256256,768769,860.7015027999878,7.0972819230519235e-06
257257,514515,257257,771772,864.0465288162231,6.9711786636617035e-06
258258,516517,258258,774775,867.6080360412598,6.8284807639429346e-06
259259,518519,259259,777778,871.0444247722626,6.651449439232238e-06
260260,520521,260260,780781,874.3662960529327,6.481550371972844e-06
261261,522523,261261,783784,877.7107787132263,6.362381100188941e-06
262262,524525,262262,786787,881.1603009700775,6.189329724293202e-06
263263,526527,263263,789790,884.5851838588715,6.0123493312858045e-06
264264,528529,264264,792793,887.8922898769379,5.834255716763437e-06
265265,530531,265265,795796,891.2272658348083,5.663012416334823e-06
266266,532533,266266,798799,894.5707256793976,5.5310301831923425e-06
267267,534535,267267,801802,897.8928470611572,5.467592927743681e-06
268268,536537,268268,804805,901.1927788257599,5.3929106798022985e-06
269269,538539,269269,807808,904.5846607685089,5.2999275794718415e-06
270270,540541,270270,810811,908.0076367855072,5.212314135860652e-06
271271,542543,271271,813814,911.3812079429626,5.119109118822962e-06
272272,544545,272272,816817,914.8058207035065,5.031963155488484e-06
273273,546547,273273,819820,918.2219467163086,4.958632416673936e-06
274274,548549,274274,822823,921.6386480331421,4.895338861388154e-06
275275,550551,275275,825826,925.0344197750092,4.835595973418094e-06
276276,552553,276276,828829,928.4277009963989,4.796809662366286e-06
277277,554555,277277,831832,931.923907995224,4.7560370148858055e-06
278278,556557,278278,834835,935.4918987751007,4.683135557570495e-06
279279,558559,279279,837838,938.9420049190521,4.5607375795952976e-06
280280,560561,280280,840841,942.3253428936005,4.4021235225955024e-06
281281,562563,281281,843844,945.744827747345,4.341678504715674e-06
282282,564565,282282,846847,949.1093847751617,4.2766405385918915e-06
283283,566567,283283,849850,952.477324962616,4.174371497356333e-06
284284,568569,284284,852853,955.8420269489288,4.017383616883308e-06
285285,570571,285285,855856,959.2673966884613,3.848637788905762e-06
286286,572573,286286,858859,962.694531917572,3.7437639548443258e-06
287287,574575,287287,861862,966.0308678150177,3.624089004006237e-06
288288,576577,288288,864865,969.3539979457855,3.4889872040366754e-06
289289,578579,289289,867868,972.7194306850433,3.3229298423975706e-06
290290,580581,290290,870871,976.0718877315521,3.1422132451552898e-06
291291,582583,291291,873874,979.4537718296051,2.949536792584695e-06
292292,584585,292292,876877,982.7865519523621,2.725329977693036e-06
293293,586587,293293,879880,986.1787629127502,2.5238059606635943e-06
294294,588589,294294,882883,989.5125260353088,2.3968968889676034e-06
295295,590591,295295,885886,992.9529099464417,2.2871900000609457e-06
296296,592593,296296,888889,996.4254419803619,2.1858813852304593e-06
297297,594595,297297,891892,999.7711389064789,2.1874620870221406e-06
298298,596597,298298,894895,1003.1137657165527,2.1570813260041177e-06
299299,598599,299299,897898,1006.4760687351227,2.110265995725058e-06
300300,600601,300300,900901,1009.9053559303284,2.233306076959707e-06
301301,602603,301301,903904,1013.3038928508759,2.469563696649857e-06
302302,604605,302302,906907,1016.6757309436798,2.771812432911247e-06
303303,606607,303303,909910,1020.011109828949,3.0406226869672537e-06
304304,608609,304304,912913,1023.3969779014587,3.2796724553918466e-06
305305,610611,305305,915916,1026.752457857132,3.4826334740500897e-06
306306,612613,306306,918919,1030.1110787391663,3.6382243706611916e-06
307307,614615,307307,921922,1033.468223810196,3.814613592112437e-06
308308,616617,308308,924925,1036.7991547584534,3.969178578699939e-06
309309,618619,309309,927928,1040.1444590091705,4.089159119757824e-06
310310,620621,310310,930931,1043.504737854004,4.1845141822705045e-06
311311,622623,311311,933934,1046.8516509532928,4.2293977458029985e-06
312312,624625,312312,936937,1050.2060840129852,4.250014171702787e-06
313313,626627,313313,939940,1053.54052400589,4.241168426233344e-06
314314,628629,314314,942943,1056.8740289211273,4.188181264908053e-06
315315,630631,315315,945946,1060.2295258045197,4.1021812648978084e-06
316316,632633,316316,948949,1063.5809168815613,4.009960321127437e-06
317317,634635,317317,951952,1066.9521598815918,3.8939124351600185e-06
318318,636637,318318,954955,1070.2808697223663,3.7397439882624894e-06
319319,638639,319319,957958,1073.6043338775635,3.535209543770179e-06
320320,640641,320320,960961,1076.9896550178528,3.3147316571557894e-06
321321,642643,321321,963964,1080.3130569458008,3.083461706410162e-06
322322,644645,322322,966967,1083.6907629966736,2.81617212749552e-06
323323,646647,323323,969970,1087.0480890274048,2.537301043048501e-06
324324,648649,324324,972973,1090.408846616745,2.2167023416841403e-06
325325,650651,325325,975976,1093.7741348743439,1.8671689758775756e-06
326326,652653,326326,978979,1097.1228637695312,1.5037512639537454e-06
327327,654655,327327,981982,1100.4728167057037,1.1532720236573368e-06
328328,656657,328328,984985,1103.8202607631683,8.763690857449546e-07
329329,658659,329329,987988,1107.1961357593536,7.159287633839995e-07
330330,660661,330330,990991,1110.5384650230408,6.59683792036958e-07
331331,662663,331331,993994,1113.9083659648895,7.533944881288335e-07
332332,664665,332332,996997,1117.2786588668823,8.688311936566606e-07
333333,666667,333333,1000000,1120.6150126457214,1.0025778465205804e-06
334334,668669,334334,1003003,1123.951416015625,1.1639422154985368e-06
335335,670671,335335,1006006,1127.3154170513153,1.3204553397372365e-06
336336,672673,336336,1009009,1130.793212890625,1.4539291441906244e-06
337337,674675,337337,1012012,1134.2515850067139,1.5897858247626573e-06
338338,676677,338338,1015015,1137.622044801712,1.7138590919785202e-06
339339,678679,339339,1018018,1140.9750108718872,1.8533355614636093e-06
340340,680681,340340,1021021,1144.346629858017,1.959233486559242e-06
341341,682683,341341,1024024,1147.6610589027405,2.0517945813480765e-06
342342,684685,342342,1027027,1151.0197548866272,2.1340347302611917e-06
343343,686687,343343,1030030,1154.4215247631073,2.2115436877356842e-06
344344,688689,344344,1033033,1158.0482659339905,2.293598299729638e-06
345345,690691,345345,1036036,1161.587035894394,2.3623033484909683e-06
346346,692693,346346,1039039,1164.9686629772186,2.4093733372865245e-06
347347,694695,347347,1042042,1168.2979168891907,2.4502351152477786e-06
348348,696697,348348,1045045,1171.7239909172058,2.4703222152311355e-06
349349,698699,349349,1048048,1175.207018852234,2.4765195121290162e-06
350350,700701,350350,1051051,1178.5377168655396,2.485039658495225e-06
351351,702703,351351,1054054,1181.8910439014435,2.5610315788071603e-06
352352,704705,352352,1057057,1185.328992843628,2.6949292077915743e-06
353353,706707,353353,1060060,1188.6668729782104,2.8116555768065155e-06
354354,708709,354354,1063063,1192.0462279319763,2.8918057068949565e-06
355355,710711,355355,1066066,1195.4120199680328,2.9452894523274153e-06
356356,712713,356356,1069069,1198.7705657482147,2.9837647161912173e-06
357357,714715,357357,1072072,1202.151743888855,3.0224600777728483e-06
358358,716717,358358,1075075,1205.5277779102325,3.027787897735834e-06
359359,718719,359359,1078078,1208.8678257465363,3.0140236049192026e-06
360360,720721,360360,1081081,1212.2227199077606,3.0133542168186978e-06
361361,722723,361361,1084084,1215.625593662262,2.9917700885562226e-06
362362,724725,362362,1087087,1218.9781448841095,2.9467737476807088e-06
363363,726727,363363,1090090,1222.3312418460846,2.945664164144546e-06
364364,728729,364364,1093093,1225.6973958015442,2.94938035949599e-06
365365,730731,365365,1096096,1229.030357837677,2.9307684599189088e-06
366366,732733,366366,1099099,1232.3928067684174,2.9243001335998997e-06
367367,734735,367367,1102102,1235.7583448886871,2.994120222865604e-06
368368,736737,368368,1105105,1239.1040897369385,3.0471510399365798e-06
369369,738739,369369,1108108,1242.4618048667908,3.0915944080334157e-06
370370,740741,370370,1111111,1245.821303844452,3.115628715022467e-06
371371,742743,371371,1114114,1249.1858177185059,3.1134677556110546e-06
372372,744745,372372,1117117,1252.652923822403,3.1332947401097044e-06
373373,746747,373373,1120120,1256.108426809311,3.1225554266711697e-06
374374,748749,374374,1123123,1259.5330867767334,3.074070264119655e-06
375375,750751,375375,1126126,1263.0479888916016,3.00070496450644e-06
376376,752753,376376,1129129,1266.419133901596,2.8865106287412345e-06
377377,754755,377377,1132132,1269.7808020114899,2.7965143090113997e-06
378378,756757,378378,1135135,1273.1297907829285,2.677992597455159e-06
379379,758759,379379,1138138,1276.5130288600922,2.5500994524918497e-06
380380,760761,380380,1141141,1279.8554828166962,2.4359687813557684e-06
381381,762763,381381,1144144,1283.2226297855377,2.3961765691637993e-06
382382,764765,382382,1147147,1286.5506927967072,2.3273278202395886e-06
383383,766767,383383,1150150,1289.8936018943787,2.247985321446322e-06
384384,768769,384384,1153153,1293.234939813614,2.170521838706918e-06
385385,770771,385385,1156156,1296.5831289291382,2.063832653220743e-06
386386,772773,386386,1159159,1299.9253160953522,1.9462549971649423e-06
387387,774775,387387,1162162,1303.2607579231262,1.8174432625528425e-06
388388,776777,388388,1165165,1306.6335418224335,1.7261427274206653e-06
389389,778779,389389,1168168,1309.9993467330933,1.6256071830866858e-06
390390,780781,390390,1171171,1313.3997519016266,1.5638997865607962e-06
391391,782783,391391,1174174,1316.741133928299,1.503300154581666e-06
392392,784785,392392,1177177,1320.0930478572845,1.4173911040415987e-06
393393,786787,393393,1180180,1323.4775638580322,1.319504008279182e-06
394394,788789,394394,1183183,1326.8288009166718,1.189375325338915e-06
395395,790791,395395,1186186,1330.1814818382263,1.075808540917933e-06
396396,792793,396396,1189189,1333.5122528076172,9.248433343600482e-07
397397,794795,397397,1192192,1336.883817911148,9.066170605365187e-07
398398,796797,398398,1195195,1340.2487318515778,1.033664375427179e-06
399399,798799,399399,1198198,1343.5914816856384,1.249947672476992e-06
400400,800801,400400,1201201,1346.979084968567,1.5053101378725842e-06
401401,802803,401401,1204204,1350.3491559028625,1.7325746739516035e-06
402402,804805,402402,1207207,1353.9483749866486,1.932068698806688e-06
403403,806807,403403,1210210,1357.3750829696655,2.092370777972974e-06
404404,808809,404404,1213213,1360.7178709506989,2.2465374058810994e-06
405405,810811,405405,1216216,1364.1132097244263,2.3605352907907218e-06
406406,812813,406406,1219219,1367.6514286994934,2.4354067136300728e-06
407407,814815,407407,1222222,1370.9678928852081,2.4825549189699814e-06
408408,816817,408408,1225225,1374.4283456802368,2.5080917112063617e-06
409409,818819,409409,1228228,1377.9031789302826,2.497043169569224e-06
410410,820821,410410,1231231,1381.289393901825,2.4591117835370824e-06
411411,822823,411411,1234234,1384.6841378211975,2.4030050553847104e-06
412412,824825,412412,1237237,1388.036409854889,2.3115480871638283e-06
413413,826827,413413,1240240,1391.4858758449554,2.217371729784645e-06
414414,828829,414414,1243243,1394.960828781128,2.120159479090944e-06
415415,830831,415415,1246246,1398.3132190704346,1.9803428585873917e-06
416416,832833,416416,1249249,1401.6560637950897,1.8595055735204369e-06
417417,834835,417417,1252252,1404.9977159500122,1.787253495422192e-06
418418,836837,418418,1255255,1408.3680157661438,1.6923204384511337e-06
419419,838839,419419,1258258,1411.7155678272247,1.5642672224203125e-06
420420,840841,420420,1261261,1415.0672907829285,1.4160177670419216e-06
421421,842843,421421,1264264,1418.4186789989471,1.2300843081902713e-06
422422,844845,422422,1267267,1421.7534277439117,1.0174280760111287e-06
423423,846847,423423,1270270,1425.1149706840515,9.150171536020935e-07
424424,848849,424424,1273273,1428.4694797992706,8.341703505720943e-07
425425,850851,425425,1276276,1431.803748846054,8.79475919646211e-07
426426,852853,426426,1279279,1435.1791727542877,9.35486241360195e-07
427427,854855,427427,1282282,1438.5126807689667,9.944833436748013e-07
428428,856857,428428,1285285,1441.8691837787628,1.024516677716747e-06
429429,858859,429429,1288288,1445.258241891861,1.0420444596093148e-06
430430,860861,430430,1291291,1448.6020889282227,1.0496169124962762e-06
431431,862863,431431,1294294,1451.930547952652,1.0582298273220658e-06
432432,864865,432432,1297297,1455.3351616859436,1.0364547051722184e-06
433433,866867,433433,1300300,1458.6876528263092,1.0507901606615633e-06
434434,868869,434434,1303303,1462.1555578708649,1.0903713700827211e-06
435435,870871,435435,1306306,1465.7338407039642,1.1330957931932062e-06
436436,872873,436436,1309309,1469.1101558208466,1.1501379049150273e-06
437437,874875,437437,1312312,1472.6928486824036,1.2226300896145403e-06
438438,876877,438438,1315315,1476.0992786884308,1.3042226782999933e-06
439439,878879,439439,1318318,1479.4394388198853,1.3615353964269161e-06
440440,880881,440440,1321321,1482.8049018383026,1.3968874554848298e-06
441441,882883,441441,1324324,1486.1920669078827,1.4527868188451976e-06
442442,884885,442442,1327327,1489.5469827651978,1.5028854249976575e-06
443443,886887,443443,1330330,1492.9009437561035,1.538326614536345e-06
444444,888889,444444,1333333,1496.337611913681,1.5755013009766117e-06
445445,890891,445445,1336336,1499.738872051239,1.6295616660499945e-06
446446,892893,446446,1339339,1503.139102935791,1.6479007172165439e-06
447447,894895,447447,1342342,1506.4594478607178,1.6463563952129334e-06
448448,896897,448448,1345345,1509.7914378643036,1.6522444639122114e-06
449449,898899,449449,1348348,1513.1633007526398,1.6330050129909068e-06
450450,900901,450450,1351351,1516.538115978241,1.6610028978902847e-06
451451,902903,451451,1354354,1520.0267970561981,1.6698722902219743e-06
452452,904905,452452,1357357,1523.4486148357391,1.68760925589595e-06
453453,906907,453453,1360360,1526.8397817611694,1.688105840003118e-06
454454,908909,454454,1363363,1530.5248308181763,1.6890717233764008e-06
455455,910911,455455,1366366,1533.8186378479004,1.73511216416955e-06
456456,912913,456456,1369369,1537.1591737270355,1.7539259715704247e-06
457457,914915,457457,1372372,1540.495284795761,1.7374295566696674e-06
458458,916917,458458,1375375,1543.8501498699188,1.6869907994987443e-06
459459,918919,459459,1378378,1547.3053867816925,1.6128433344420046e-06
460460,920921,460460,1381381,1550.649300813675,1.5148543752729893e-06
461461,922923,461461,1384384,1554.0779089927673,1.4555680536432192e-06
462462,924925,462462,1387387,1557.6713976860046,1.3882909115636721e-06
463463,926927,463463,1390390,1561.057196855545,1.3177868822822347e-06
464464,928929,464464,1393393,1564.4337408542633,1.279382559005171e-06
465465,930931,465465,1396396,1567.786212682724,1.2828932085540146e-06
466466,932933,466466,1399399,1571.1953828334808,1.2964119378011674e-06
467467,934935,467467,1402402,1574.935798883438,1.2888285709777847e-06
468468,936937,468468,1405405,1578.4480979442596,1.2931322999065742e-06
469469,938939,469469,1408408,1581.8742547035217,1.3040680642006919e-06
470470,940941,470470,1411411,1585.4478168487549,1.3001390470890328e-06
471471,942943,471471,1414414,1589.0360298156738,1.2508844520198181e-06
472472,944945,472472,1417417,1592.5759608745575,1.1698830348905176e-06
473473,946947,473473,1420420,1596.2191317081451,1.066371623892337e-06
474474,948949,474474,1423423,1599.8163468837738,1.0172898328164592e-06
475475,950951,475475,1426426,1603.4016058444977,9.76524461293593e-07
476476,952953,476476,1429429,1606.9812037944794,9.487393981544301e-07
477477,954955,477477,1432432,1610.5790567398071,9.210234566126019e-07
478478,956957,478478,1435435,1614.1448156833649,9.104660421144217e-07
479479,958959,479479,1438438,1617.7227058410645,8.906517905415967e-07
480480,960961,480480,1441441,1621.2713210582733,8.648676157463342e-07
481481,962963,481481,1444444,1624.9001598358154,8.145907486323267e-07
482482,964965,482482,1447447,1628.4777839183807,7.615763024659827e-07
483483,966967,483483,1450450,1632.0169169902802,6.94213667884469e-07
484484,968969,484484,1453453,1635.6428399085999,6.419904821086675e-07
485485,970971,485485,1456456,1639.2199668884277,5.709298420697451e-07
486486,972973,486486,1459459,1642.7874038219452,5.238525773165748e-07
487487,974975,487487,1462462,1646.3371849060059,5.879574018763378e-07
488488,976977,488488,1465465,1649.8282296657562,7.245089364005253e-07
489489,978979,489489,1468468,1653.210031747818,9.51731635723263e-07
490490,980981,490490,1471471,1656.7757649421692,1.1303254723316059e-06
491491,982983,491491,1474474,1660.2323739528656,1.2946984497830272e-06
492492,984985,492492,1477477,1663.5812227725983,1.4227844076231122e-06
493493,986987,493493,1480480,1666.976727962494,1.4949982869438827e-06
494494,988989,494494,1483483,1670.3101286888123,1.5264686226146296e-06
495495,990991,495495,1486486,1673.6454010009766,1.5633449947927147e-06
496496,992993,496496,1489489,1676.9914937019348,1.5772657206980512e-06
497497,994995,497497,1492492,1680.3583657741547,1.5534842532360926e-06
498498,996997,498498,1495495,1683.7450287342072,1.4919114619260654e-06
499499,998999,499499,1498498,1687.1049647331238,1.3830449461238459e-06
500501,1001003,500501,1501504,1690.440439939499,1.2711061572190374e-06
501502,1003005,501502,1504507,1693.8102598190308,1.1860283848363906e-06
502503,1005007,502503,1507510,1697.1986408233643,1.0752573871286586e-06
503504,1007009,503504,1510513,1700.5076637268066,9.182240319205448e-07
504505,1009011,504505,1513516,1703.829598903656,8.20789864519611e-07
505506,1011013,505506,1516519,1707.2152798175812,7.458565960405394e-07
506507,1013015,506507,1519522,1710.5520839691162,6.44828105578199e-07
507508,1015017,507508,1522525,1713.868754863739,6.762347766198218e-07
508509,1017019,508509,1525528,1717.2132139205933,6.831705832155421e-07
509510,1019021,509510,1528531,1720.5662808418274,6.578811735380441e-07
510511,1021023,510511,1531534,1723.892669916153,6.90424712956883e-07
511512,1023025,511512,1534537,1727.2690598964691,7.355902198469266e-07
512513,1025027,512513,1537540,1730.6333377361298,7.776143320370466e-07
513514,1027029,513514,1540543,1734.3563289642334,8.332299330504611e-07
514515,1029031,514515,1543546,1737.8736219406128,8.971583156380802e-07
515516,1031033,515516,1546549,1741.22256398201,1.0056628525489941e-06
516517,1033035,516517,1549552,1744.5801467895508,1.099255314329639e-06
517518,1035037,517518,1552555,1747.9335627555847,1.1458741937531158e-06
518519,1037039,518519,1555558,1751.258365869522,1.1448737495811656e-06
519520,1039041,519520,1558561,1754.6519610881805,1.1624888429651037e-06
520521,1041043,520521,1561564,1758.034278869629,1.1759348126361147e-06
521522,1043045,521522,1564567,1761.462001800537,1.1601950973272324e-06
522523,1045047,522523,1567570,1764.7983937263489,1.1760603229049593e-06
523524,1047049,523524,1570573,1768.1620609760284,1.2184082152089104e-06
524525,1049051,524525,1573576,1771.5116307735443,1.2701002560788766e-06
525526,1051053,525526,1576579,1774.851173877716,1.2830896594095975e-06
526527,1053055,526527,1579582,1778.1896660327911,1.273350790143013e-06
527528,1055057,527528,1582585,1781.5296638011932,1.3168191799195483e-06
528529,1057059,528529,1585588,1785.0137708187103,1.339338268735446e-06
529530,1059061,529530,1588591,1788.3502707481384,1.337015419267118e-06
530531,1061063,530531,1591594,1791.6910157203674,1.340364178759046e-06
531532,1063065,531532,1594597,1795.0262808799744,1.3240241969469935e-06
532533,1065067,532533,1597600,1798.3706529140472,1.2683176464634016e-06
533534,1067069,533534,1600603,1801.708378791809,1.2682576198130846e-06
534535,1069071,534535,1603606,1805.0695569515228,1.3152202882338315e-06
535536,1071073,535536,1606609,1808.4268736839294,1.3295793905854225e-06
536537,1073075,536537,1609612,1811.7360796928406,1.3324479368748143e-06
537538,1075077,537538,1612615,1815.096028804779,1.3270146155264229e-06
538539,1077079,538539,1615618,1818.4342877864838,1.3184926501708105e-06
539540,1079081,539540,1618621,1821.7534849643707,1.2881209840998054e-06
540541,1081083,540541,1621624,1825.1447138786316,1.2450182111933827e-06
541542,1083085,541542,1624627,1829.0308198928833,1.2111941032344475e-06
542543,1085087,542543,1627630,1832.7048797607422,1.175376382889226e-06
543544,1087089,543544,1630633,1836.2744498252869,1.1344127415213734e-06
544545,1089091,544545,1633636,1839.8244128227234,1.1037591320928186e-06
545546,1091093,545546,1636639,1843.4225678443909,1.0659023246262223e-06
546547,1093095,546547,1639642,1847.0046017169952,9.839059202931821e-07
547548,1095097,547548,1642645,1850.5912828445435,9.251343726646155e-07
548549,1097099,548549,1645648,1854.244045972824,9.044761100085452e-07
549550,1099101,549550,1648651,1857.969765663147,8.611823432147503e-07
550551,1101103,550551,1651654,1861.547415971756,8.710612746654078e-07
551552,1103105,551552,1654657,1865.3772447109222,8.560582500649616e-07
552553,1105107,552553,1657660,1868.9707119464874,8.199131116271019e-07
553554,1107109,553554,1660663,1872.5500128269196,8.013648766791448e-07
554555,1109111,554555,1663666,1876.1348519325256,7.747639756416902e-07
555556,1111113,555556,1666669,1879.697401046753,7.14740963303484e-07
556557,1113115,556557,1669672,1883.291358947754,6.37686753179878e-07
557558,1115117,557558,1672675,1886.9000680446625,5.446763680083677e-07
558559,1117119,558559,1675678,1890.3446078300476,5.183101166039705e-07
559560,1119121,559560,1678681,1893.7146890163422,5.141864676261321e-07
560561,1121123,560561,1681684,1897.173444032669,5.020574462832883e-07
561562,1123125,561562,1684687,1900.756313085556,4.869471013080329e-07
562563,1125127,562563,1687690,1904.097263097763,4.428657121025026e-07
563564,1127129,563564,1690693,1907.4749329090118,4.98417648486793e-07
564565,1129131,564565,1693696,1910.8147559165955,5.234105628915131e-07
565566,1131133,565566,1696699,1914.1497430801392,5.412111931946129e-07
566567,1133135,566567,1699702,1917.51784491539,6.340833351714537e-07
567568,1135137,567568,1702705,1920.8426847457886,7.214894139906392e-07
568569,1137139,568569,1705708,1924.2038819789886,8.507049642503262e-07
569570,1139141,569570,1708711,1927.579905986786,9.48479282669723e-07
570571,1141143,570571,1711714,1930.9487400054932,1.018011971609667e-06
571572,1143145,571572,1714717,1934.3264276981354,1.045267708832398e-06
572573,1145147,572573,1717720,1937.6658809185028,1.032871296047233e-06
573574,1147149,573574,1720723,1941.0026726722717,9.72519046626985e-07
574575,1149151,574575,1723726,1944.3320617675781,9.008035704027861e-07
575576,1151153,575576,1726729,1947.7047128677368,8.477181836497039e-07
576577,1153155,576577,1729732,1951.0311708450317,7.683192961849272e-07
577578,1155157,577578,1732735,1954.5950639247894,6.268983270274475e-07
578579,1157159,578579,1735738,1957.9829769134521,4.4504668039735407e-07
579580,1159161,579580,1738741,1961.3110547065735,3.2257776183541864e-07
580581,1161163,580581,1741744,1964.6881167888641,2.6166890165768564e-07
581582,1163165,581582,1744747,1968.0011239051819,2.2870153770782053e-07
582583,1165167,582583,1747750,1971.3148567676544,2.673841663636267e-07
583584,1167169,583584,1750753,1974.6394879817963,3.3941250876523554e-07
584585,1169171,584585,1753756,1978.027109861374,3.7853715184610337e-07
585586,1171173,585586,1756759,1981.4550697803497,4.101457307115197e-07
586587,1173175,586587,1759762,1984.7994177341461,4.509183781920001e-07
587588,1175177,587588,1762765,1988.1504759788513,4.7907633415889e-07
588589,1177179,588589,1765768,1991.5143349170685,5.483452696353197e-07
589590,1179181,589590,1768771,1994.942905664444,5.967067409073934e-07
590591,1181183,590591,1771774,1998.2802398204803,6.780664989491925e-07
591592,1183185,591592,1774777,2001.5883839130402,7.216749509098008e-07
592593,1185187,592593,1777780,2004.9305768013,7.320286385947838e-07
593594,1187189,593594,1780783,2008.2615759372711,7.4403578764759e-07
594595,1189191,594595,1783786,2011.6285009384155,7.88759280112572e-07
595596,1191193,595596,1786789,2014.9456560611725,8.446386345895007e-07
596597,1193195,596597,1789792,2018.260764837265,8.803999662632123e-07
597598,1195197,597598,1792795,2021.599946975708,8.796250767773017e-07
598599,1197199,598599,1795798,2024.9433488845825,8.670522220199928e-07
599600,1199201,599600,1798801,2028.308394908905,8.6460386228282e-07
600601,1201203,600601,1801804,2031.641394853592,8.518982212990522e-07
601602,1203205,601602,1804807,2034.988823890686,8.109691407298669e-07
602603,1205207,602603,1807810,2038.3352718353271,8.249280654126778e-07
603604,1207209,603604,1810813,2041.771726846695,8.443494152743369e-07
604605,1209211,604605,1813816,2045.381008863449,8.95224729902111e-07
605606,1211213,605606,1816819,2048.7229387760162,9.099931048694998e-07
606607,1213215,606607,1819822,2052.042243003845,8.894676284398884e-07
607608,1215217,607608,1822825,2055.415969848633,8.541574061382562e-07
608609,1217219,608609,1825828,2058.7351579666138,8.271508704638109e-07
609610,1219221,609610,1828831,2062.032935857773,7.951493898872286e-07
610611,1221223,610611,1831834,2065.365784883499,7.813487172825262e-07
611612,1223225,611612,1834837,2068.7058668136597,7.571597961941734e-07
612613,1225227,612613,1837840,2072.052840948105,7.063936209306121e-07
613614,1227229,613614,1840843,2075.3719708919525,6.742320692865178e-07
614615,1229231,614615,1843846,2078.6560349464417,6.420614226954058e-07
615616,1231233,615616,1846849,2082.004513025284,5.945457814959809e-07
616617,1233235,616617,1849852,2085.365634918213,5.893525667488575e-07
617618,1235237,617618,1852855,2088.9370748996735,5.682413757313043e-07
618619,1237239,618619,1855858,2092.4977288246155,5.526453605853021e-07
619620,1239241,619620,1858861,2095.9586188793182,5.079327820567414e-07
620621,1241243,620621,1861864,2099.3011240959167,4.6135392040014267e-07
621622,1243245,621622,1864867,2102.622116804123,4.467456165002659e-07
622623,1245247,622623,1867870,2106.0446088314056,4.3051659304182976e-07
623624,1247249,623624,1870873,2109.457669734955,3.889545041602105e-07
624625,1249251,624625,1873876,2112.8323278427124,3.5802804632112384e-07
625626,1251253,625626,1876879,2116.2068729400635,4.2787723941728473e-07
626627,1253255,626627,1879882,2119.541455745697,4.604426067089662e-07
627628,1255257,627628,1882885,2122.8630146980286,4.89906597067602e-07
628629,1257259,628629,1885888,2126.2545619010925,5.902020348003134e-07
629630,1259261,629630,1888891,2129.602150917053,6.847458280390128e-07
630631,1261263,630631,1891894,2132.9243268966675,7.307571650017053e-07
631632,1263265,631632,1894897,2136.2358498573303,7.634771463926882e-07
632633,1265267,632633,1897900,2139.533787727356,7.980834197951481e-07
633634,1267269,633634,1900903,2142.8726167678833,8.451552275801077e-07
634635,1269271,634635,1903906,2146.2274668216705,8.447113941656426e-07
635636,1271273,635636,1906909,2149.5538418293,8.411152521148324e-07
636637,1273275,636637,1909912,2152.878762960434,8.049701136769727e-07
637638,1275277,637638,1912915,2156.2196159362793,7.35328285372816e-07
638639,1277279,638639,1915918,2159.568431854248,6.643003871431574e-07
639640,1279281,639640,1918921,2162.909513950348,5.662022886099294e-07
640641,1281283,640641,1921924,2166.2527170181274,4.7268986236304045e-07
641642,1283285,641642,1924927,2169.620609998703,3.8729012885596603e-07
642643,1285287,642643,1927930,2172.985394716263,2.9898365028202534e-07
643644,1287289,643644,1930933,2176.3782167434692,2.3853135644458234e-07
644645,1289291,644645,1933936,2179.7315118312836,2.9460898076649755e-07
645646,1291293,645646,1936939,2183.029653787613,3.13548298436217e-07
646647,1293295,646647,1939942,2186.6036999225616,3.949917299905792e-07
647648,1295297,647648,1942945,2190.029095888138,4.6936111175455153e-07
648649,1297299,648649,1945948,2193.344050884247,5.307374522089958e-07
649650,1299301,649650,1948951,2196.6825518608093,6.056252459529787e-07
650651,1301303,650651,1951954,2199.997492790222,6.76422132528387e-07
651652,1303305,651652,1954957,2203.3046309947968,7.171238394221291e-07
652653,1305307,652653,1957960,2206.645674943924,7.327544153667986e-07
653654,1307309,653654,1960963,2210.00697183609,7.698599802097306e-07
654655,1309311,654655,1963966,2213.5097007751465,7.973740139277652e-07
655656,1311313,655656,1966969,2216.827816963196,7.994185580173507e-07
656657,1313315,656657,1969972,2220.149223804474,7.907965482445434e-07
657658,1315317,657658,1972975,2223.479085922241,7.759426807751879e-07
658659,1317319,658659,1975978,2226.8665347099304,7.44352291803807e-07
659660,1319321,659660,1978981,2230.226181745529,7.138460205169395e-07
660661,1321323,660661,1981984,2233.534094810486,7.291055226232857e-07
661662,1323325,661662,1984987,2236.9321868419647,7.61110641178675e-07
662663,1325327,662663,1987990,2240.28164601326,7.91455022408627e-07
663664,1327329,663664,1990993,2243.59157705307,8.0551762948744e-07
664665,1329331,664665,1993996,2247.0810039043427,8.038277883315459e-07
665666,1331333,665666,1996999,2250.5114607810974,7.969410944497213e-07
666667,1333335,666667,2000002,2253.85564994812,7.727376214461401e-07
667668,1335337,667668,2003005,2257.1991329193115,7.222133717732504e-07
668669,1337339,668669,2006008,2260.517646074295,6.737918738508597e-07
669670,1339341,669670,2009011,2263.864778995514,6.061200110707432e-07
670671,1341343,670671,2012014,2267.3847358226776,5.328693077899516e-07
671672,1343345,671672,2015017,2270.7351427078247,4.440607881406322e-07
672673,1345347,672673,2018020,2274.1889657974243,4.326011548982933e-07
673674,1347349,673674,2021023,2277.5143480300903,4.314661055104807e-07
674675,1349351,674675,2024026,2280.8719437122345,4.2762076191138476e-07
675676,1351353,675676,2027029,2284.242688894272,4.061475920025259e-07
676677,1353355,676677,2030032,2287.615129709244,3.7505742511712015e-07
677678,1355357,677678,2033035,2290.9381947517395,3.4119329939130694e-07
678679,1357359,678679,2036038,2294.276841878891,2.8307294996920973e-07
679680,1359361,679680,2039041,2297.666302919388,2.322267391718924e-07
680681,1361363,680681,2042044,2301.0023186206818,2.4695691536180675e-07
681682,1363365,681682,2045047,2304.3514099121094,2.692122507141903e-07
682683,1365367,682683,2048050,2307.685874938965,3.189616109011695e-07
683684,1367369,683684,2051053,2310.994111776352,4.0827944758348167e-07
684685,1369371,684685,2054056,2314.373694896698,5.268902896204963e-07
685686,1371373,685686,2057059,2317.7792880535126,6.099726306274533e-07
686687,1373375,686687,2060062,2321.0816848278046,6.597656465601176e-07
687688,1375377,687688,2063065,2324.4388148784637,6.900027074152604e-07
688689,1377379,688689,2066068,2327.7587130069733,6.85486156726256e-07
689690,1379381,689690,2069071,2331.095268011093,6.573573045898229e-07
690691,1381383,690691,2072074,2334.4736618995667,5.813108145957813e-07
691692,1383385,691692,2075077,2337.789163827896,4.841585905523971e-07
692693,1385387,692693,2078080,2341.347208738327,3.7790596252307296e-07
693694,1387389,693694,2081083,2344.9890048503876,3.080058377236128e-07
694695,1389391,694695,2084086,2348.592976808548,2.9839247872587293e-07
695696,1391393,695696,2087089,2352.1773447990417,2.6539055397734046e-07
696697,1393395,696697,2090092,2355.801466703415,2.3361280909739435e-07
697698,1395397,697698,2093095,2359.3661799430847,2.1744017431046814e-07
698699,1397399,698699,2096098,2362.9468488693237,2.4857945390976965e-07
699700,1399401,699700,2099101,2366.4984328746796,2.7363603294361383e-07
700701,1401403,700701,2102104,2370.1990377902985,2.8847716748714447e-07
701702,1403405,701702,2105107,2373.863328933716,3.0795308703090996e-07
702703,1405407,702703,2108110,2377.567544937134,3.2571188057772815e-07
703704,1407409,703704,2111113,2381.115528821945,3.40343831339851e-07
704705,1409411,704705,2114116,2384.7564747333527,4.107369022676721e-07
705706,1411413,705706,2117119,2388.3053879737854,4.5329215936362743e-07
706707,1413415,706707,2120122,2391.856246948242,4.985831765225157e-07
707708,1415417,707708,2123125,2395.433230638504,5.283909558784217e-07
708709,1417419,708709,2126128,2399.0514726638794,5.481815605890006e-07
709710,1419421,709710,2129131,2402.6496958732605,5.704805516870692e-07
710711,1421423,710711,2132134,2406.1587777137756,5.88577677262947e-07
711712,1423425,711712,2135137,2409.637622833252,5.873098416486755e-07
712713,1425427,712713,2138140,2413.189351797104,5.749134288635105e-07
713714,1427429,713714,2141143,2416.6089310646057,5.486836016643792e-07
714715,1429431,714715,2144146,2419.9526178836823,5.769215931650251e-07
715716,1431433,715716,2147149,2423.306659936905,5.843430699314922e-07
716717,1433435,716717,2150152,2426.68963766098,5.795500328531489e-07
717718,1435437,717718,2153155,2430.0826349258423,5.680158210452646e-07
718719,1437439,718719,2156158,2433.4022829532623,5.42187990504317e-07
719720,1439441,719720,2159161,2436.7531130313873,5.33800630364567e-07
720721,1441443,720721,2162164,2440.0932598114014,5.055590008851141e-07
721722,1443445,721722,2165167,2443.451955795288,4.699904820881784e-07
722723,1445447,722723,2168170,2446.8207290172577,4.664652806241065e-07
723724,1447449,723724,2171173,2450.1726336479187,4.6810055209789425e-07
724725,1449451,724725,2174176,2453.498039960861,4.526318662101403e-07
725726,1451453,725726,2177179,2456.8234329223633,4.074881871929392e-07
726727,1453455,726727,2180182,2460.188845872879,3.810491762124002e-07
727728,1455457,727728,2183185,2463.5431518554688,3.5266930353827775e-07
728729,1457459,728729,2186188,2466.9590740203857,3.020359145011753e-07
729730,1459461,729730,2189191,2470.4060158729553,2.2588574211113155e-07
730731,1461463,730731,2192194,2473.7648968696594,2.2697531676385552e-07
731732,1463465,731732,2195197,2477.188153028488,2.4579094315413386e-07
732733,1465467,732733,2198200,2480.8320128917694,2.3497887013945729e-07
733734,1467469,733734,2201203,2484.2185728549957,2.1999949240125716e-07
734735,1469471,734735,2204206,2487.6290810108185,2.855504135368392e-07
735736,1471473,735736,2207209,2491.0138998031616,3.2210664357990026e-07
736737,1473475,736737,2210212,2494.5857939720154,3.3036121749319136e-07
737738,1475477,737738,2213215,2498.1590209007263,3.4348704502917826e-07
738739,1477479,738739,2216218,2501.733561038971,4.427547537488863e-07
739740,1479481,739740,2219221,2505.1456248760223,5.080764822196215e-07
740741,1481483,740741,2222224,2508.498571872711,5.477486411109567e-07
741742,1483485,741742,2225227,2511.822506904602,5.692563718184829e-07
742743,1485487,742743,2228230,2515.196133852005,5.830443114973605e-07
743744,1487489,743744,2231233,2518.573725938797,5.574074748437852e-07
744745,1489491,744745,2234236,2521.9184839725494,4.911689757136628e-07
745746,1491493,745746,2237239,2525.2881088256836,3.792847564909607e-07
746747,1493495,746747,2240242,2528.6429579257965,2.95500285574235e-07
747748,1495497,747748,2243245,2531.9719128608704,2.591677912278101e-07
748749,1497499,748749,2246248,2535.3872780799866,2.267843228764832e-07
749750,1499501,749750,2249251,2538.7295129299164,2.213655534433201e-07
750751,1501503,750751,2252254,2542.118523836136,2.2252061171457171e-07
751752,1503505,751752,2255257,2545.4833788871765,2.4698420020285994e-07
752753,1505507,752753,2258260,2549.056109905243,2.520482667023316e-07
753754,1507509,753754,2261263,2552.5197789669037,2.7890928322449327e-07
754755,1509511,754755,2264266,2555.8569688796997,3.052027750527486e-07
755756,1511513,755756,2267269,2559.1965548992157,3.32052877638489e-07
756757,1513515,756757,2270272,2562.572772026062,3.7790960050188005e-07
757758,1515517,757758,2273275,2565.943960905075,4.3613363231997937e-07
758759,1517519,758759,2276278,2569.3141486644745,4.6215791371650994e-07
759760,1519521,759760,2279281,2572.659614801407,4.99227098771371e-07
760761,1521523,760761,2282284,2576.081696987152,5.138244887348264e-07
761762,1523525,761762,2285287,2579.446893930435,5.147267074789852e-07
762763,1525527,762763,2288290,2582.78342795372,5.22057234775275e-07
763764,1527529,763764,2291293,2586.246752977371,5.240763130132109e-07
764765,1529531,764765,2294296,2589.790513753891,5.371948645915836e-07
765766,1531533,765766,2297299,2593.1739089488983,5.743422661907971e-07
766767,1533535,766767,2300302,2596.573703765869,5.723086360376328e-07
767768,1535537,767768,2303305,2599.939079761505,5.547735781874508e-07
768769,1537539,768769,2306308,2603.3062777519226,5.602469173027202e-07
769770,1539541,769770,2309311,2606.6534008979797,5.415658961283043e-07
770771,1541543,770771,2312314,2609.986853837967,5.032852641306818e-07
771772,1543545,771772,2315317,2613.345346927643,5.159236025065184e-07
772773,1545547,772773,2318320,2616.6866879463196,4.989396984456107e-07
773774,1547549,773774,2321323,2620.0179347991943,4.822086339117959e-07
774775,1549551,774775,2324326,2623.37238073349,4.726280167233199e-07
775776,1551553,775776,2327329,2626.776696920395,4.7640605771448463e-07
776777,1553555,776777,2330332,2630.10737490654,4.4343505578581244e-07
777778,1555557,777778,2333335,2633.485723733902,3.9537917473353446e-07
778779,1557559,778779,2336338,2636.8037028312683,3.616751200752333e-07
779780,1559561,779780,2339341,2640.2582218647003,3.718669177033007e-07
780781,1561563,780781,2342344,2643.7216498851776,3.4513686841819435e-07
781782,1563565,781782,2345347,2647.112049818039,3.333771019242704e-07
782783,1565567,782783,2348350,2650.4609427452087,3.182722139172256e-07
783784,1567569,783784,2351353,2653.8015580177307,2.9480725061148405e-07
784785,1569571,784785,2354356,2657.1919298171997,2.6485940907150507e-07
785786,1571573,785786,2357359,2660.558469772339,2.3603206500411034e-07
786787,1573575,786787,2360362,2663.9235787391663,2.421038516331464e-07
787788,1575577,787788,2363365,2667.382682800293,2.842698449967429e-07
788789,1577579,788789,2366368,2670.7651257514954,3.236782504245639e-07
789790,1579581,789790,2369371,2674.127415895462,3.4125332604162395e-07
790791,1581583,790791,2372374,2677.5025577545166,4.0368104237131774e-07
791792,1583585,791792,2375377,2680.83575963974,4.77926732855849e-07
792793,1585587,792793,2378380,2684.1878519058228,4.928369889967144e-07
793794,1587589,793794,2381383,2687.59303689003,5.038546078139916e-07
794795,1589591,794795,2384386,2690.973785638809,4.834382707485929e-07
795796,1591593,795796,2387389,2694.3182888031006,4.309513315092772e-07
796797,1593595,796797,2390392,2697.6306517124176,3.98553311242722e-07
797798,1595597,797798,2393395,2700.968964099884,3.5352968552615494e-07
798799,1597599,798799,2396398,2704.3045728206635,3.1273339118342847e-07
799800,1599601,799800,2399401,2707.690342903137,2.6143970899283886e-07
800801,1601603,800801,2402404,2711.057580947876,2.1404412109404802e-07
801802,1603605,801802,2405407,2714.455258846283,1.6667581803631037e-07
802803,1605607,802803,2408410,2718.0116958618164,1.250937202712521e-07
803804,1607609,803804,2411413,2721.404397010803,1.73185981111601e-07
804805,1609611,804805,2414416,2724.828003883362,2.430078893667087e-07
805806,1611613,805806,2417419,2728.3803420066833,2.868946467060596e-07
806807,1613615,806807,2420422,2731.7950489521027,3.166969690937549e-07
807808,1615617,807808,2423425,2735.1294298171997,3.275981725892052e-07
808809,1617619,808809,2426428,2738.482890844345,3.313216438982636e-07
809810,1619621,809810,2429431,2741.8304028511047,3.459317667875439e-07
810811,1621623,810811,2432434,2745.1932756900787,3.7838981370441616e-07
811812,1623625,811812,2435437,2748.5431637763977,4.2545070755295455e-07
812813,1625627,812813,2438440,2751.9575958251953,4.42723830929026e-07
813814,1627629,813814,2441443,2755.334326982498,4.3546606320887804e-07
814815,1629631,814815,2444446,2758.6826667785645,4.366975190350786e-07
815816,1631633,815816,2447449,2762.0093936920166,4.309858923079446e-07
816817,1633635,816817,2450452,2765.399605989456,4.0371742215938866e-07
817818,1635637,817818,2453455,2768.9500148296356,4.407484084367752e-07
818819,1637639,818819,2456458,2772.336045026779,4.38598362961784e-07
819820,1639641,819820,2459461,2775.7244367599487,4.457215254660696e-07
820821,1641643,820821,2462464,2779.0312576293945,4.366393113741651e-07
821822,1643645,821822,2465467,2782.399475812912,3.951026883441955e-07
822823,1645647,822823,2468470,2785.7665598392487,3.5291850508656353e-07
823824,1647649,823824,2471473,2789.116938829422,3.429013304412365e-07
824825,1649651,824825,2474476,2792.523750782013,3.488203219603747e-07
825826,1651653,825826,2477479,2795.931133747101,3.575351001927629e-07
826827,1653655,826827,2480482,2799.2977378368378,3.5506127460394055e-07
827828,1655657,827828,2483485,2802.658113002777,3.313780325697735e-07
828829,1657659,828829,2486488,2806.0331819057465,3.0059527489356697e-07
829830,1659661,829830,2489491,2809.3653450012207,2.546385076129809e-07
830831,1661663,830831,2492494,2812.7127289772034,2.62436515185982e-07
831832,1663665,831832,2495497,2816.0646529197693,2.417909854557365e-07
832833,1665667,832833,2498500,2819.402941942215,2.2098720364738256e-07
833834,1667669,833834,2501503,2822.7412757873535,1.9639628590084612e-07
834835,1669671,834835,2504506,2826.1210889816284,1.5691330190747976e-07
835836,1671673,835836,2507509,2829.462189912796,1.4309625839814544e-07
836837,1673675,836837,2510512,2832.972541809082,1.666376192588359e-07
837838,1675677,837838,2513515,2836.4899230003357,1.9352046365384012e-07
838839,1677679,838839,2516518,2839.8408739566803,2.3762731871102005e-07
839840,1679681,839840,2519521,2843.169455051422,2.75349520961754e-07
840841,1681683,840841,2522524,2846.535467863083,3.270633897045627e-07
841842,1683685,841842,2525527,2849.8867378234863,3.582645149435848e-07
842843,1685687,842843,2528530,2853.3397579193115,3.6044730222783983e-07
843844,1687689,843844,2531533,2856.7247507572174,3.4501863410696387e-07
844845,1689691,844845,2534536,2860.082932949066,3.260502126067877e-07
845846,1691693,845846,2537539,2863.446703672409,3.0581941246055067e-07
846847,1693695,846847,2540542,2866.7999918460846,2.5199915398843586e-07
847848,1695697,847848,2543545,2870.14604473114,2.2792482923250645e-07
848849,1697699,848849,2546548,2873.4950358867645,1.961889211088419e-07
849850,1699701,849850,2549551,2876.8115010261536,1.490570866735652e-07
850851,1701703,850851,2552554,2880.178748846054,1.1418887879699469e-07
851852,1703705,851852,2555557,2883.631045818329,1.136340870289132e-07
852853,1705707,852853,2558560,2887.0137248039246,1.4170473150443286e-07
853854,1707709,853854,2561563,2890.4934458732605,1.9376420823391527e-07
854855,1709711,854855,2564566,2894.0333647727966,2.2726271708961576e-07
855856,1711713,855856,2567569,2897.4057557582855,2.285451046191156e-07
856857,1713715,856857,2570572,2900.769302845001,2.3287248041015118e-07
857858,1715717,857858,2573575,2904.0975608825684,2.753276930889115e-07
858859,1717719,858859,2576578,2907.7439296245575,3.1017771107144654e-07
859860,1719721,859860,2579581,2911.196954727173,3.4653385228011757e-07
860861,1721723,860861,2582584,2914.53271484375,3.601217031246051e-07
861862,1723725,861862,2585587,2917.9525718688965,3.431032382650301e-07
862863,1725727,862863,2588590,2921.30867767334,3.333061613375321e-07
863864,1727729,863864,2591593,2924.6771008968353,3.3754440664779395e-07
864865,1729731,864865,2594596,2928.0406687259674,3.631557774497196e-07
865866,1731733,865866,2597599,2931.3724689483643,3.770783223444596e-07
866867,1733735,866867,2600602,2934.8189659118652,3.6369783629197627e-07
867868,1735737,867868,2603605,2938.1824939250946,3.317109076306224e-07
868869,1737739,868869,2606608,2941.5234138965607,3.0756746127735823e-07
869870,1739741,869870,2609611,2944.8628237247467,3.1139279599301517e-07
870871,1741743,870871,2612614,2948.222597837448,3.346303856233135e-07
871872,1743745,871872,2615617,2951.5836358070374,3.399945853743702e-07
872873,1745747,872873,2618620,2954.952749967575,3.353961801622063e-07
873874,1747749,873874,2621623,2958.3097746372223,3.0366936698555946e-07
874875,1749751,874875,2624626,2961.6502487659454,2.603028406156227e-07
875876,1751753,875876,2627629,2964.981602907181,2.579909050837159e-07
876877,1753755,876877,2630632,2968.336993932724,2.505057636881247e-07
877878,1755757,877878,2633635,2971.702888727188,2.3379834601655602e-07
878879,1757759,878879,2636638,2975.0580348968506,2.045107976300642e-07
879880,1759761,879880,2639641,2978.381778717041,1.6668309399392456e-07
880881,1761763,880881,2642644,2981.7144918441772,1.3501266948878765e-07
881882,1763765,881882,2645647,2985.137753009796,1.4763827493879944e-07
882883,1765767,882883,2648650,2988.4792668819427,2.0093102648388594e-07
883884,1767769,883884,2651653,2991.803330898285,2.3217762645799667e-07
884885,1769771,884885,2654656,2995.149104833603,2.3726897779852152e-07
885886,1771773,885886,2657659,2998.560354948044,2.659744495758787e-07
886887,1773775,886887,2660662,3001.959501028061,2.899978426285088e-07
887888,1775777,887888,2663665,3005.3619499206543,3.1584750104229897e-07
888889,1777779,888889,2666668,3008.703655719757,3.462882887106389e-07
889890,1779781,889890,2669671,3012.0400519371033,3.3883407013490796e-07
890891,1781783,890891,2672674,3015.4167239665985,3.098975867033005e-07
891892,1783785,891892,2675677,3018.723645925522,2.8955946618225425e-07
892893,1785787,892893,2678680,3022.10085773468,2.505257725715637e-07
893894,1787789,893894,2681683,3025.602516889572,2.275737642776221e-07
894895,1789791,894895,2684686,3028.9553320407867,1.8968239601235837e-07
895896,1791793,895896,2687689,3032.293907880783,1.7853017197921872e-07
896897,1793795,896897,2690692,3035.6256239414215,1.5821387933101505e-07
897898,1795797,897898,2693695,3038.9762217998505,1.5248951967805624e-07
898899,1797799,898899,2696698,3042.29354596138,1.9299295672681183e-07
899900,1799801,899900,2699701,3045.8574788570404,1.961179805221036e-07
900901,1801803,900901,2702704,3049.252091884613,2.3546635929960757e-07
901902,1803805,901902,2705707,3052.595841884613,2.7532587409950793e-07
902903,1805807,902903,2708710,3055.948115825653,2.7866735763382167e-07
903904,1807809,903904,2711713,3059.298274040222,3.0880619306117296e-07
904905,1809811,904905,2714716,3062.6125848293304,3.1686249712947756e-07
905906,1811813,905906,2717719,3065.9662158489227,3.1932540878187865e-07
906907,1813815,906907,2720722,3069.3295137882233,3.3487958717159927e-07
907908,1815817,907908,2723725,3072.7683777809143,3.1546551326755434e-07
908909,1817819,908909,2726728,3076.184080839157,3.385466698091477e-07
909910,1819821,909910,2729731,3079.7368218898773,3.393597580725327e-07
910911,1821823,910911,2732734,3083.285616874695,3.271306923124939e-07
911912,1823825,911912,2735737,3086.7788898944855,3.4044387575704604e-07
912913,1825827,912913,2738740,3090.3413166999817,3.310487954877317e-07
913914,1827829,913914,2741743,3093.8978548049927,3.101595211774111e-07
914915,1829831,914915,2744746,3097.4406628608704,3.198947524651885e-07
915916,1831833,915916,2747749,3100.988464832306,3.250825102441013e-07
916917,1833835,916917,2750752,3104.53076505661,3.16464138450101e-07
917918,1835837,917918,2753755,3108.1133749485016,3.0164119380060583e-07
918919,1837839,918919,2756758,3111.6317517757416,2.802444214466959e-07
919920,1839841,919920,2759761,3115.1493589878082,2.590059011708945e-07
920921,1841843,920921,2762764,3118.6722779273987,2.3258871806319803e-07
921922,1843845,921922,2765767,3122.1966960430145,2.0388506527524441e-07
922923,1845847,922923,2768770,3125.7525837421417,1.5461228031199425e-07
923924,1847849,923924,2771773,3129.2367708683014,1.1314659786876291e-07
924925,1849851,924925,2774776,3132.7631437778473,1.5072873793542385e-07
925926,1851853,925926,2777779,3136.544819831848,1.8017817637883127e-07
926927,1853855,926927,2780782,3140.119395971298,1.9045182853005826e-07
927928,1855857,927928,2783785,3143.4628326892853,2.1717460185755044e-07
928929,1857859,928929,2786788,3146.815757036209,2.2177664504852146e-07
929930,1859861,929930,2789791,3150.180845975876,2.1206506062299013e-07
930931,1861863,930931,2792794,3153.50567984581,2.5179542717523873e-07
931932,1863865,931932,2795797,3156.848834991455,2.9376860766205937e-07
932933,1865867,932933,2798800,3160.2191178798676,3.0903538572601974e-07
933934,1867869,933934,2801803,3163.922610759735,3.0839692044537514e-07
934935,1869871,934935,2804806,3167.437198638916,2.699853212106973e-07
935936,1871873,935936,2807809,3170.781240940094,2.296401362400502e-07
936937,1873875,936937,2810812,3174.1401529312134,2.2062522475607693e-07
937938,1875877,937938,2813815,3177.4584419727325,1.8323225958738476e-07
938939,1877879,938939,2816818,3180.7974169254303,1.685057213762775e-07
939940,1879881,939940,2819821,3184.132519721985,1.4436591300182045e-07
940941,1881883,940941,2822824,3187.496976852417,1.3246608432382345e-07
941942,1883885,941942,2825827,3190.845478773117,1.517419150331989e-07
942943,1885887,942943,2828830,3194.1714799404144,1.5691330190747976e-07
943944,1887889,943944,2831833,3197.556802034378,1.7155252862721682e-07
944945,1889891,944945,2834836,3200.863602876663,1.8687751435209066e-07
945946,1891893,945946,2837839,3204.192484855652,2.1764753910247236e-07
946947,1893895,946947,2840842,3207.537854909897,2.3135544324759394e-07
947948,1895897,947948,2843845,3210.864778995514,2.4248583940789104e-07
948949,1897899,948949,2846848,3214.2110798358917,2.592205419205129e-07
949950,1899901,949950,2849851,3217.529653787613,2.587003109510988e-07
950951,1901903,950951,2852854,3220.935975790024,2.600936568342149e-07
951952,1903905,951952,2855857,3224.4365496635437,2.6375164452474564e-07
952953,1905907,952953,2858860,3227.763368844986,2.5536610337439924e-07
953954,1907909,953954,2861863,3231.332232952118,2.6638554118108004e-07
954955,1909911,954955,2864866,3234.71488571167,2.9003604140598327e-07
955956,1911913,955956,2867869,3237.9009346961975,2.8636168281082064e-07
956957,1913915,956957,2870872,3241.0342268943787,2.9691000236198306e-07
957958,1915917,957958,2873875,3244.1298489570618,2.905089786509052e-07
958959,1917919,958959,2876878,3247.3357439041138,2.6062662072945386e-07
959960,1919921,959960,2879881,3251.1923367977142,2.3292523110285401e-07
960961,1921923,960961,2882884,3254.4287190437317,2.3619213607162237e-07
961962,1923925,961962,2885887,3257.905884742737,2.2354288375936449e-07
962963,1925927,962963,2888890,3262.3448498249054,1.951775630004704e-07
963964,1927929,963964,2891893,3268.1463720798492,1.775133569026366e-07
964965,1929931,964965,2894896,3273.026039838791,1.5540172171313316e-07
965966,1931933,965966,2897899,3277.053373813629,1.1267366062384099e-07
966967,1933935,966967,2900902,3281.3801758289337,8.802453521639109e-08
967968,1935937,967968,2903905,3285.6122159957886,8.866481948643923e-08
968969,1937939,968969,2906908,3289.753588914871,7.958078640513122e-08
969970,1939941,969970,2909911,3294.256540775299,1.2703640095423907e-07
970971,1941943,970971,2912914,3297.9290838241577,1.4981742424424738e-07
971972,1943945,971972,2915917,3301.7234978675842,1.782282197382301e-07
972973,1945947,972973,2918920,3305.2544119358063,2.1333471522666514e-07
973974,1947949,973974,2921923,3309.1423938274384,2.2198764781933278e-07
974975,1949951,974975,2924926,3312.9348180294037,2.520791895221919e-07
975976,1951953,975976,2927929,3316.8008377552032,2.5289591576438397e-07
976977,1953955,976977,2930932,3320.454509973526,2.6283123588655144e-07
977978,1955957,977978,2933935,3324.095536708832,2.249398676212877e-07
978979,1957959,978979,2936938,3327.9381999969482,2.2216408979147673e-07
979980,1959961,979980,2939941,3331.585175037384,2.075139491353184e-07
980981,1961963,980981,2942944,3335.5409858226776,1.8570972315501422e-07
981982,1963965,981982,2945947,3339.3902127742767,1.704411261016503e-07
982983,1965967,982983,2948950,3343.1723136901855,1.2574673746712506e-07
983984,1967969,983984,2951953,3346.7480187416077,7.755625119898468e-08
984985,1969971,984985,2954956,3350.2226927280426,8.520146366208792e-08
985986,1971973,985986,2957959,3353.805943965912,1.128009898820892e-07
986987,1973975,986987,2960962,3357.6238539218903,1.334356056759134e-07
987988,1975977,987988,2963965,3361.109556913376,1.5796103980392218e-07
988989,1977979,988989,2966968,3365.4896879196167,1.6153353499248624e-07
989990,1979981,989990,2969971,3369.824367761612,1.554435584694147e-07
990991,1981983,990991,2972974,3374.2988719940186,1.7871752788778394e-07
991992,1983985,991992,2975977,3377.9148190021515,2.1089908841531724e-07
992993,1985987,992993,2978980,3381.945502758026,2.387914719292894e-07
993994,1987989,993994,2981983,3385.275140762329,2.537417458370328e-07
994995,1989991,994995,2984986,3388.5555629730225,2.6130874175578356e-07
995996,1991993,995996,2987989,3392.094361782074,2.7021815185435116e-07
996997,1993995,996997,2990992,3395.7904148101807,2.747656253632158e-07
997998,1995997,997998,2993995,3399.44744181633,2.6434281608089805e-07
998999,1997999,998999,2996998,3403.761720895767,2.6790075935423374e-07
1000000,2000001,1000000,3000001,3407.6098589897156,2.7104761102236807e-07


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002299785614013672,12064.709122577777
2002,2003,2002,4005,4.75390100479126,60.67671186811822
4004,4005,4004,8009,9.179544925689697,40.02609617545022
6006,6007,6006,12013,13.806530952453613,32.13797708286802
8008,8009,8008,16017,18.536274909973145,27.246786066505592
10010,10011,10010,20021,23.83765196800232,23.723299817738734
12012,12013,12012,24025,28.585903882980347,20.989859030964
14014,14015,14014,28029,32.98323893547058,18.776198956609733
16016,16017,16016,32033,37.389081954956055,16.934860506264158
18018,18019,18018,36037,41.90768313407898,15.375758415093514
20020,20021,20020,40041,46.458094120025635,14.038860967322762
22022,22023,22022,44045,50.93951988220215,12.881498903649117
24024,24025,24024,48049,55.376060962677,11.871907541533801
26026,26027,26026,52053,59.79984092712402,10.98564499834174
28028,28029,28028,56057,64.16934204101562,10.20344186195689
30030,30031,30030,60061,68.58322882652283,9.509827417139604
32032,32033,32032,64065,73.0224277973175,8.89219817101548
34034,34035,34034,68069,77.4310851097107,8.340162209044138
36036,36037,36036,72073,81.85543990135193,7.845063883871262
38038,38039,38038,76077,86.2601227760315,7.399629918034407
40040,40041,40040,80081,90.88143110275269,6.997701481135664
42042,42043,42042,84085,95.27119588851929,6.634028092285007
44044,44045,44044,88089,99.68200707435608,6.304106939418489
46046,46047,46046,92093,104.10074591636658,6.004056088931975
48048,48049,48048,96097,108.60720896720886,5.730513324713684
50050,50051,50050,100101,113.03764796257019,5.480554602134362
52052,52053,52052,104105,117.41631197929382,5.251627681196624
54054,54055,54054,108109,121.85888314247131,5.041497629967125
56056,56057,56056,112113,126.2500491142273,4.848201704922758
58058,58059,58058,116117,130.64207792282104,4.670011710717517
60060,60061,60060,120121,135.01412796974182,4.505402381795648
62062,62063,62062,124125,139.41858577728271,4.353024655658373
64064,64065,64064,128129,143.82268595695496,4.211682953255149
66066,66067,66066,132133,148.24550604820251,4.080315767972934
68068,68069,68068,136137,152.6328158378601,3.9579790064890403
70070,70071,70070,140141,156.9849009513855,3.8438316339797893
72072,72073,72072,144145,161.39062309265137,3.7371232607620186
74074,74075,74074,148149,165.78386688232422,3.637183463866677
76076,76077,76076,152153,170.35667991638184,3.5434122191090864
78078,78079,78078,156157,174.70426988601685,3.455271782277123
80080,80081,80080,160161,179.05490684509277,3.372279685723697
82082,82083,82082,164165,183.42714285850525,3.2940024048857595
84084,84085,84084,168169,187.81218886375427,3.2200498701367906
86086,86087,86086,172173,192.23461890220642,3.1500706432252628
88088,88089,88088,176177,196.61578702926636,3.0837476713004435
90090,90091,90090,180181,201.02780175209045,3.0207945441597985
92092,92093,92092,184185,205.39346408843994,2.960952190687749
94094,94095,94094,188189,209.76182103157043,2.903985959379497
96096,96097,96096,192193,214.1278998851776,2.849683035279668
98098,98099,98098,196197,218.48798394203186,2.7978501520228747
100100,100101,100100,200201,222.96164512634277,2.7483115630911925
102102,102103,102102,204205,227.35588788986206,2.7009072410255612
104104,104105,104104,208209,231.71004009246826,2.6554912774245167
106106,106107,106106,212213,236.0722680091858,2.61193045985965
108108,108109,108108,216217,240.47041988372803,2.5701030049676774
110110,110111,110110,220221,244.8715558052063,2.5298974294582877
112112,112113,112112,224225,249.3859510421753,2.49121154308159
114114,114115,114114,228229,253.93149590492249,2.453951549479825
116116,116117,116116,232233,258.3166968822479,2.4180312426651653
118118,118119,118118,236237,262.70561480522156,2.3833712882224063
120120,120121,120120,240241,267.083379983902,2.34989857967048
122122,122123,122122,244245,271.49806094169617,2.3175456616263546
124124,124125,124124,248249,275.97581481933594,2.286250212287996
126126,126127,126126,252253,280.36494398117065,2.2559545787007664
128128,128129,128128,256257,284.8008179664612,2.2266053590283263
130130,130131,130130,260261,289.2810549736023,2.198153026674845
132132,132133,132132,264265,293.66827297210693,2.17055159175834
134134,134135,134134,268269,298.0662851333618,2.143758295880616
136136,136137,136136,272273,302.45581102371216,2.1177333513569465
138138,138139,138138,276277,306.82402300834656,2.092439649719381
140140,140141,140140,280281,311.2592279911041,2.0678425762762345
142142,142143,142142,284285,315.6270411014557,2.0439097965718247
144144,144145,144144,288289,320.04482793807983,2.02061107002919
146146,146147,146146,292293,324.4516439437866,1.9979180825139338
148148,148149,148148,296297,328.8220191001892,1.9758042942758038
150150,150151,150150,300301,333.22871804237366,1.9542448017436982
152152,152153,152152,304305,337.60684084892273,1.9332162117461849
154154,154155,154154,308309,342.0134038925171,1.9126965269679204
156156,156157,156156,312313,346.3915808200836,1.8926650414832693
158158,158159,158158,316317,350.782488822937,1.8731022454157937
160160,160161,160160,320321,355.13146805763245,1.8539897377941088
162162,162163,162162,324325,359.52449679374695,1.835310146883785
164164,164165,164164,328329,363.8648729324341,1.8170470572022168
166166,166167,166166,332333,368.22841691970825,1.7991849426452973
168168,168169,168168,336337,372.6263380050659,1.7817091051256284
170170,170171,170170,340341,377.02136874198914,1.7646056182147731
172172,172173,172172,344345,381.43832182884216,1.747861275312971
174174,174175,174174,348349,385.8674638271332,1.7314635419861588
176176,176177,176176,352353,390.5388789176941,1.715400538443646
178178,178179,178178,356357,394.9487929344177,1.6996609200305102
180180,180181,180180,360361,399.36937403678894,1.6842339163158613
182182,182183,182182,364365,403.7784860134125,1.6691092750515963
184184,184185,184184,368369,408.2091820240021,1.6542772278389748
186186,186187,186186,372373,412.6572849750519,1.6397284605573077
188188,188189,188188,376377,417.09700298309326,1.6254540859663393
190190,190191,190190,380381,421.4944038391113,1.6114456182913273
192192,192193,192192,384385,425.86330914497375,1.5976949496543966
194194,194195,194194,388389,430.2623689174652,1.5841943281520798
196196,196197,196196,392393,434.6337699890137,1.5709363374971872
198198,198199,198198,396397,439.03688406944275,1.5579138780340145
200200,200201,200200,400401,443.4321959018707,1.5451201491068787
202202,202203,202202,404405,448.0033800601959,1.532548632572798
204204,204205,204204,408409,452.5551071166992,1.5201930774546781
206206,206207,206206,412413,456.92317605018616,1.5080474855803914
208208,208209,208208,416417,461.32906198501587,1.496106098198652
210210,210211,210210,420421,465.7057468891144,1.484363383417076
212212,212213,212212,424425,470.16528391838074,1.4728140244824317
214214,214215,214214,428429,474.63135385513306,1.4614529087866686
216216,216217,216216,432433,479.0395667552948,1.4502751175496087
218218,218219,218218,436437,483.4170660972595,1.4392759161673894
220220,220221,220220,440441,487.7992398738861,1.4284507451247919
222222,222223,222222,444445,492.18144488334656,1.4177952114714572
224224,224225,224224,448449,496.53914403915405,1.4073050808110565
226226,226227,226226,452453,501.00561475753784,1.3969762697433907
228228,228229,228228,456457,505.4425790309906,1.386804838793978
230230,230231,230230,460461,509.88569712638855,1.3767869856928883
232232,232233,232232,464465,514.2478201389313,1.3669190390992298
234234,234235,234234,468469,518.5970029830933,1.357197452622131
236236,236237,236236,472473,523.0150117874146,1.347618799249176
238238,238239,238238,476477,527.5157949924469,1.338179766002213
240240,240241,240240,480481,532.0613729953766,1.3288771489569626
242242,242243,242242,484485,536.4400818347931,1.3197078484918165
244244,244245,244244,488489,540.8856220245361,1.310668864809486
246246,246247,246246,492493,545.3025758266449,1.3017572936932993
248248,248249,248248,496497,549.7405200004578,1.2929703224872355
250250,250251,250250,500501,554.094349861145,1.2843052262815036
252252,252253,252252,504505,558.4840829372406,1.2757593643164
254254,254255,254254,508509,562.8595368862152,1.2673301765316864
256256,256257,256256,512513,567.2532279491425,1.2590151803233312
258258,258259,258258,516517,571.6063737869263,1.2508119674639602
260260,260261,260260,520521,576.010244846344,1.2427182011360856
262262,262263,262262,524525,580.5504689216614,1.2347316131745174
264264,264265,264264,528529,584.9281978607178,1.2268500013851735
266266,266267,266266,532533,589.3509769439697,1.219071227022141
268268,268269,268268,536537,593.7068119049072,1.2113932123829727
270270,270271,270270,540541,598.0449941158295,1.203813939850079
272272,272273,272272,544545,602.4472188949585,1.1963314624736086
274274,274275,274274,548549,606.8187148571014,1.1889438553316722
276276,276277,276276,552553,611.2700209617615,1.1816492630023276
278278,278279,278278,556557,615.6358017921448,1.1744458806606417
280280,280281,280280,560561,619.9970149993896,1.1673319522542442
282282,282283,282282,564565,624.3961217403412,1.160305768786202
284284,284285,284284,568569,628.7423319816589,1.1533656666488241
286286,286287,286286,572573,633.1303060054779,1.1465100260484178
288288,288289,288288,576577,637.516704082489,1.1397372694882506
290290,290291,290290,580581,641.9389131069183,1.1330458603260922
292292,292293,292292,584585,646.311420917511,1.1264343013790494
294294,294295,294294,588589,650.7278399467468,1.1199011336175317
296296,296297,296296,592593,655.0723321437836,1.11344493487195
298298,298299,298298,596597,659.4302468299866,1.1070643186194502
300300,300301,300300,600601,663.7925679683685,1.1007579328252177
302302,302303,302302,604605,668.1835100650787,1.0945244588256173
304304,304305,304304,608609,672.5390751361847,1.0883626102331618
306306,306307,306306,612613,676.9105489253998,1.082271131921516
308308,308309,308308,616617,681.3031768798828,1.076248799030509
310310,310311,310310,620621,685.7174229621887,1.0702944160275365
312312,312313,312312,624625,690.1975729465485,1.0644068157689617
314314,314315,314314,628629,694.5925409793854,1.0585848586415523
316316,316317,316316,632633,699.0168449878693,1.0528274317221076
318318,318319,318318,636637,703.3981809616089,1.0471334479461802
320320,320321,320320,640641,707.9090218544006,1.0415018453422817
322322,322323,322322,644645,712.4492938518524,1.0359315862733638
324324,324325,324324,648649,716.7220408916473,1.0304216567219555
326326,326327,326326,652653,721.0660517215729,1.0249710655825766
328328,328329,328328,656657,725.426558971405,1.019578844003263
330330,330331,330330,660661,729.764307975769,1.0142440447234549
332332,332333,332332,664665,734.167888879776,1.0089657414646354
334334,334335,334334,668669,738.5385699272156,1.0037430283264257
336336,336337,336336,672673,742.945562839508,0.9985750192026899
338338,338339,338338,676677,747.3908109664917,0.9934608472267428
340340,340341,340340,680681,751.7743430137634,0.9883996642292914
342342,342343,342342,684685,756.1731939315796,0.9833906402254797
344344,344345,344344,688689,760.5867321491241,0.9784329629019339
346346,346347,346346,692693,765.0272047519684,0.9735258371438249
348348,348349,348348,696697,769.4548099040985,0.9686684845528362
350350,350351,350350,700701,773.8356747627258,0.9638601430033304
352352,352353,352352,704705,778.2111659049988,0.9591000662076112
354354,354355,354354,708709,782.5542118549347,0.9543875232830032
356356,356357,356356,712713,786.9037868976593,0.9497217983534938
358358,358359,358358,716717,791.3318519592285,0.9451021901440981
360360,360361,360360,720721,795.8266377449036,0.9405280116079666
362362,362363,362362,724725,800.5788087844849,0.9359985895553109
364364,364365,364364,728729,805.0265128612518,0.9315132642823301
366366,366367,366366,732733,809.4183518886566,0.9270713892492495
368368,368369,368368,736737,813.8071219921112,0.922672330712885
370370,370371,370370,740741,818.1642508506775,0.9183154674301477
372372,372373,372372,744745,822.6156969070435,0.9140001903324446
374374,374375,374374,748749,827.1003530025482,0.9097259022128128
376376,376377,376376,752753,831.5335049629211,0.9054920174439758
378378,378379,378378,756757,835.9024798870087,0.9012979616836674
380380,380381,380380,760761,840.3295738697052,0.8971431715981453
382382,382383,382382,764765,844.7072830200195,0.8930270945929806
384384,384385,384384,768769,849.0909860134125,0.8889491885511234
386386,386387,386386,772773,853.5131499767303,0.8849089215855201
388388,388389,388388,776777,857.9231760501862,0.8809057717880933
390390,390391,390390,780781,862.267523765564,0.8769392269859964
392392,392393,392392,784785,866.8803699016571,0.8730087845233356
394394,394395,394394,788789,871.3310639858246,0.8691139510210633
396396,396397,396396,792793,875.7284290790558,0.8652542421750695
398398,398399,398398,796797,880.1474330425262,0.8614291825306282
400400,400401,400400,800801,884.6075329780579,0.8576383052841265
402402,402403,402402,804805,889.002434015274,0.8538811520793388
404404,404405,404404,808809,893.3629169464111,0.8501572728164319
406406,406407,406406,812813,897.7352600097656,0.846466225462791
408408,408409,408408,816817,902.1206867694855,0.8428075758638442
410410,410411,410410,820821,906.4962041378021,0.8391808975757158
412412,412413,412412,824825,910.9148721694946,0.8355857716796891
414414,414415,414414,828829,915.3261828422546,0.8320217866221356
416416,416417,416416,832833,919.6794791221619,0.8284885380508058
418418,418419,418418,836837,924.1404778957367,0.8249856286402064
420420,420421,420420,840841,928.5249898433685,0.8215126679679088
422422,422423,422422,844845,932.904953956604,0.8180692723235552
424424,424425,424424,848849,937.2769160270691,0.8146550645979005
426426,426427,426426,852853,941.6724629402161,0.811269674115465
428428,428429,428428,856857,946.0248458385468,0.8079127365126624
430430,430431,430430,860861,950.4559328556061,0.8045838935813663
432432,432433,432432,864865,954.8530869483948,0.8012827931615902
434434,434435,434434,868869,959.2228689193726,0.7980090889923304
436436,436437,436436,872873,963.5849158763885,0.7947624406006071
438438,438439,438438,876877,967.9454128742218,0.7915425131723168
440440,440441,440440,880881,972.6091477870941,0.7883489774321788
442442,442443,442442,884885,977.0028448104858,0.7851815095327765
444444,444445,444444,888889,981.4284858703613,0.7820397909363237
446446,446447,446446,892893,985.8608529567719,0.7789235083146195
448448,448449,448448,896897,990.2463150024414,0.7758323534308147
450450,450451,450450,900901,994.6684308052063,0.7727660230393667
452452,452453,452452,904905,999.0369300842285,0.7697242187823576
454454,454455,454454,908909,1003.4034371376038,0.7667066470985446
456456,456457,456456,912913,1007.7725598812103,0.7637130191124015
458458,458459,458458,916917,1012.226814031601,0.7607430505486263
460460,460461,460460,920921,1016.5578548908234,0.7577964616448298
462462,462463,462462,924925,1020.9164500236511,0.7548729770442151
464464,464465,464464,928929,1025.2912409305573,0.7519723257282749
466466,466467,466466,932933,1029.6885449886322,0.7490942409167474
468468,468469,468468,936937,1034.0666999816895,0.7462384599875804
470470,470471,470470,940941,1038.4337029457092,0.7434047244023532
472472,472473,472472,944945,1042.779042005539,0.7405927796171454
474474,474475,474474,948949,1047.1462180614471,0.7378023750097782
476476,476477,476476,952953,1051.4985411167145,0.7350332637979591
478478,478479,478478,956957,1055.8904139995575,0.7322852029774367
480480,480481,480480,960961,1060.2620449066162,0.7295579532365082
482482,482483,482482,964965,1064.6203830242157,0.7268512788923545
484484,484485,484484,968969,1069.0078389644623,0.7241649478219188
486486,486487,486486,972973,1073.3649060726166,0.721498731390966
488488,488489,488488,976977,1077.7545139789581,0.718852404395875
490490,490491,490490,980981,1082.1159839630127,0.7162257449817844
492492,492493,492492,984985,1086.5132038593292,0.7136185345989361
494494,494495,494494,988989,1090.8888368606567,0.7110305579390115
496496,496497,496496,992993,1095.2396659851074,0.7084616028569144
498498,498499,498498,996997,1099.6360340118408,0.7059114603343914
500501,500502,500501,1001003,1104.0058579444885,0.7033786645224609
502503,502504,502503,1005007,1108.6708171367645,0.7008655413810629
504505,504506,504505,1009011,1113.2286758422852,0.698370621768845
506507,506508,506507,1013015,1117.5976388454437,0.6958937085728394
508509,508510,508509,1017019,1122.0014321804047,0.6934346094440116
510511,510512,510511,1021023,1126.367660999298,0.6909931340996991
512513,512514,512513,1025027,1130.7462258338928,0.6885690906437958
514515,514516,514515,1029031,1135.1936049461365,0.6861622930264275
516517,516518,516517,1033035,1139.5439591407776,0.6837725578443496
518519,518520,518519,1037039,1143.8742830753326,0.6813997042936535
520521,520522,520521,1041043,1148.23859500885,0.6790435541115585
522523,522524,522523,1045047,1152.6129958629608,0.6767039315491274
524525,524526,524525,1049051,1156.9944698810577,0.6743806633166969
526527,526528,526527,1053055,1161.3789761066437,0.6720735785365832
528529,528530,528529,1057059,1165.7357399463654,0.669782508717617
530531,530532,530531,1061063,1170.1701860427856,0.6675072972830094
532533,532534,532533,1065067,1174.5388419628143,0.6652478156047437
534535,534536,534535,1069071,1178.9089329242706,0.6630038568546297
536537,536538,536537,1073075,1183.2834270000458,0.660775261638264
538539,538540,538539,1077079,1187.6624789237976,0.6585618727294786
540541,540542,540541,1081083,1192.0618679523468,0.6563635350485129
542543,542544,542543,1085087,1196.4292569160461,0.6541800956256338
544545,544546,544545,1089091,1200.7837891578674,0.6520114035502047
546547,546548,546547,1093095,1205.1719739437103,0.6498573099524947
548549,548550,548549,1097099,1209.5859270095825,0.6477176679600234
550551,550552,550551,1101103,1213.9447770118713,0.645592332661181
552553,552554,552553,1105107,1218.3348009586334,0.6434811610834004
554555,554556,554555,1109111,1222.7140500545502,0.641384050657507
556557,556558,556557,1113115,1227.0945069789886,0.6393008372069744
558559,558560,558559,1117119,1231.469489812851,0.6372313694701006
560561,560562,560561,1121123,1235.829579114914,0.6351755118867004
562563,562564,562563,1125127,1240.3838000297546,0.6331331306719221
564565,564566,564565,1129131,1244.9850597381592,0.6311040937907819
566567,566568,566567,1133135,1249.380611896515,0.6290882709363359
568569,568570,568569,1137139,1253.7494831085205,0.6270855334842054
570571,570572,570571,1141143,1258.1112897396088,0.6250957544816629
572573,572574,572573,1145147,1262.5059950351715,0.6231188086057955
574575,574576,574575,1149151,1266.9867429733276,0.6211545721525908
576577,576578,576577,1153155,1271.3877518177032,0.6192029229987384
578579,578580,578579,1157159,1275.746307849884,0.6172637405852583
580581,580582,580581,1161163,1280.1639938354492,0.6153369058829412
582583,582584,582583,1165167,1284.5965769290924,0.6134223013759765
584585,584586,584585,1169171,1288.9590537548065,0.6115198110346682
586587,586588,586587,1173175,1293.3305490016937,0.6096293202881498
588589,588590,588589,1177179,1297.777816772461,0.6077507160152891
590591,590592,590591,1181183,1302.184534072876,0.605883886504671
592593,592594,592593,1185187,1306.5871269702911,0.604028721440045
594595,594596,594595,1189191,1311.0308511257172,0.602185111885774
596597,596598,596597,1193195,1315.408226966858,0.6003529502468155
598599,598600,598599,1197199,1319.7524948120117,0.5985321302723605
600601,600602,600601,1201203,1324.1073579788208,0.5967225470121775
602603,602604,602603,1205207,1328.4634220600128,0.5949240968111553
604605,604606,604605,1209211,1332.8606309890747,0.5931366772874753
606607,606608,606607,1213215,1337.2196538448334,0.5913601873016887
608609,608610,608609,1217219,1341.6508297920227,0.5895945269530785
610611,610612,610611,1221223,1346.0214099884033,0.5878395975560124
612613,612614,612613,1225227,1350.3691778182983,0.5860953016144776
614615,614616,614615,1229231,1354.7234609127045,0.5843615428111661
616617,616618,616617,1233235,1359.1204509735107,0.5826382259892853
618619,618620,618619,1237239,1363.5468831062317,0.5809252571380057
620621,620622,620621,1241243,1367.9033877849579,0.5792225455388689
622623,622624,622623,1245247,1372.5382778644562,0.577529997264719
624625,624626,624625,1249251,1376.9811918735504,0.5758475215661747
626627,626628,626627,1253255,1381.3409268856049,0.574175028827085
628629,628630,628629,1257259,1385.7185978889465,0.5725124304917699
630631,630632,630631,1261263,1390.1185417175293,0.5708596390486491
632633,632634,632633,1265267,1394.5526599884033,0.5692165680084145
634635,634636,634635,1269271,1398.9809758663177,0.5675831319022109
636637,636638,636637,1273275,1403.3548319339752,0.5659592462616274
638639,638640,638639,1277279,1407.799416065216,0.5643448275877745
640641,640642,640641,1281283,1412.1770079135895,0.5627397933694738
642643,642644,642643,1285287,1416.5217578411102,0.5611440620377834
644645,644646,644645,1289291,1420.9389340877533,0.5595575529787311
646647,646648,646647,1293295,1425.3216669559479,0.5579801864878391
648649,648650,648649,1297299,1429.7438879013062,0.5564118837937713
650651,650652,650651,1301303,1434.1217958927155,0.5548525670128583
652653,652654,652653,1305307,1438.5035359859467,0.5533021591636498
654655,654656,654655,1309311,1442.872858762741,0.551760584132353
656657,656658,656657,1313315,1447.2286260128021,0.5502277666673763
658659,658660,658659,1317319,1451.6428859233856,0.5487036323720531
660661,660662,660661,1321323,1456.0320110321045,0.5471881076937279
662663,662664,662663,1325327,1460.4066519737244,0.5456811199001095
664665,664666,664665,1329331,1464.8020799160004,0.5441825970774516
666667,666668,666667,1333335,1469.3749659061432,0.5426924681178207
668669,668670,668669,1337339,1473.8567340373993,0.5412106627063622
670671,670672,670671,1341343,1478.2321519851685,0.5397371113103873
672673,672674,672673,1345347,1482.7938740253448,0.5382717451684584
674675,674676,674675,1349351,1487.2798857688904,0.5368144962794759
676677,676678,676677,1353355,1491.7140591144562,0.5353652973935823
678679,678680,678679,1357359,1496.1529867649078,0.5339240820012492
680681,680682,680681,1361363,1500.5382008552551,0.5324907843241817
682683,682684,682683,1365367,1504.9430658817291,0.531065339297129
684685,684686,684685,1369371,1509.3504168987274,0.5296476825787977
686687,686688,686687,1373375,1513.7250900268555,0.5282377505081968
688689,688690,688689,1377379,1518.0743608474731,0.5268354801355599
690691,690692,690691,1381383,1522.5876870155334,0.525440809180509
692693,692694,692693,1385387,1526.9418680667877,0.5240536760393297
694695,694696,694695,1389391,1531.308021068573,0.5226740197667823
696697,696698,696697,1393395,1535.6677498817444,0.5213017800833768
698699,698700,698699,1397399,1540.1057019233704,0.5199368973389937
700701,700702,700701,1401403,1544.4970099925995,0.5185793125310738
702703,702704,702703,1405407,1548.8951890468597,0.5172289672882471
704705,704706,704705,1409411,1553.337699174881,0.515885803852143
706707,706708,706707,1413415,1557.6636190414429,0.5145497650737525
708709,708710,708709,1417419,1562.0651679039001,0.5132207944225229
710711,710712,710711,1421423,1566.4321410655975,0.5118988359481591
712713,712714,712713,1425427,1570.8261890411377,0.5105838342933566
714715,714716,714715,1429431,1575.1920149326324,0.5092757346847065
716717,716718,716717,1433435,1579.6368079185486,0.5079744829217816
718719,718720,718719,1437439,1584.1811828613281,0.5066800253625843
720721,720722,720721,1441443,1588.6598799228668,0.5053923089308228
722723,722724,722723,1445447,1593.130649805069,0.5041112810940831
724725,724726,724725,1449451,1597.662713766098,0.5028368898692861
726727,726728,726727,1453455,1602.3099429607391,0.5015690838063165
728729,728730,728729,1457459,1606.8094189167023,0.5003078119880229
730731,730732,730731,1461463,1611.2958278656006,0.4990530240138469
732733,732734,732733,1465467,1615.6742680072784,0.497804670010737
734735,734736,734735,1469471,1620.081717967987,0.49656270060040697
736737,736738,736737,1473475,1624.7277419567108,0.49532706692116335
738739,738740,738739,1477479,1629.0904560089111,0.49409772059880197
740741,740742,740741,1481483,1633.6739859580994,0.49287461375206476
742743,742744,742743,1485487,1638.0895738601685,0.4916576989890018
744745,744746,744745,1489491,1642.487725019455,0.4904469293887814
746747,746748,746747,1493495,1646.8583800792694,0.4892422585035092
748749,748750,748749,1497499,1651.2044007778168,0.488043640356409
750751,750752,750751,1501503,1655.604327917099,0.486851029427271
752753,752754,752753,1505507,1660.0034430027008,0.48566438065063267
754755,754756,754755,1509511,1664.416827917099,0.48448364940850297
756757,756758,756757,1513515,1668.8520488739014,0.4833087915303622
758759,758760,758759,1517519,1673.3600919246674,0.4821397632786102
760761,760762,760761,1521523,1677.7542719841003,0.48097652135402313
762763,762764,762763,1525527,1682.1441159248352,0.4798190228812018
764765,764766,764765,1529531,1686.5347797870636,0.4786672254012956
766767,766768,766767,1533535,1691.3563997745514,0.4775210868810973
768769,768770,768769,1537539,1695.7457089424133,0.47638056569485343
770771,770772,770771,1541543,1700.1193528175354,0.47524562062244513
772773,772774,772773,1545547,1704.4762449264526,0.47411621085120714
774775,774776,774775,1549551,1708.8082230091095,0.4729922959541
776777,776778,776777,1553555,1713.2858889102936,0.4718738359042618
778779,778780,778779,1557559,1717.6606941223145,0.47076079106227553
780781,780782,780781,1561563,1722.0833847522736,0.4696531221652549
782783,782784,782783,1565567,1726.517585992813,0.4685507903341204
784785,784786,784785,1569571,1731.06516289711,0.46745375706086634
786787,786788,786787,1573575,1735.547639131546,0.4663619842085609
788789,788790,788789,1577579,1739.9209899902344,0.46527543399679416
790791,790792,790791,1581583,1744.3436107635498,0.46419406901441107
792793,792794,792793,1585587,1748.8934841156006,0.4631178522049595
794795,794796,794795,1589591,1753.5992147922516,0.4620467468575953
796797,796798,796797,1593595,1758.260078907013,0.46098071661617723
798799,798800,798799,1597599,1763.1429529190063,0.4599197254592582
800801,800802,800801,1601603,1767.9065458774567,0.45886373771463695
802803,802804,802803,1605607,1772.5968379974365,0.4578127180393494
804805,804806,804805,1609611,1777.393846988678,0.45676663142148755
806807,806808,806807,1613615,1782.0800189971924,0.45572544318019936
808809,808810,808809,1617619,1786.8008739948273,0.45468911895659403
810811,810812,810811,1621623,1791.469691991806,0.45365762471010385
812813,812814,812813,1625627,1796.1205570697784,0.45263092671666527
814815,814816,814815,1629631,1800.8108959197998,0.4516089915723569
816817,816818,816817,1633635,1805.4786818027496,0.4505917861661146
818819,818820,818819,1637639,1810.192883014679,0.44957927770883543
820821,820822,820821,1641643,1814.945235967636,0.44857143370245467
822823,822824,822823,1645647,1819.5894100666046,0.44756822195449786
824825,824826,824825,1649651,1824.4976539611816,0.44656961056352884
826827,826828,826827,1653655,1829.80979514122,0.4455755679136928
828829,828830,828829,1657659,1834.9299640655518,0.4445860626947251
830831,830832,830831,1661663,1839.9719660282135,0.44360106386193365
832833,832834,832833,1665667,1845.0595610141754,0.44262054066530254
834835,834836,834835,1669671,1850.2210838794708,0.4416444626294833
836837,836838,836837,1673675,1855.3132998943329,0.4406727995501569
838839,838840,838839,1677679,1860.3463160991669,0.4397055215031287
840841,840842,840841,1681683,1865.4161548614502,0.4387425988279574
842843,842844,842843,1685687,1870.7591760158539,0.4377840021334123
844845,844846,844845,1689691,1875.8480257987976,0.43682970228837803
846847,846848,846847,1693695,1880.8763778209686,0.4358796704236738
848849,848850,848849,1697699,1885.9697709083557,0.4349338779320533
850851,850852,850851,1701703,1891.0928120613098,0.43399229645365267
852853,852854,852853,1705707,1895.8034009933472,0.4330548978814477
854855,854856,854855,1709711,1900.5568089485168,0.4321216543612536
856857,856858,856857,1713715,1905.2848467826843,0.43119253828444926
858859,858860,858859,1717719,1910.0397498607635,0.4302675222807011
860861,860862,860861,1721723,1914.7195620536804,0.4293465792252391
862863,862864,862863,1725727,1919.4182889461517,0.42842968223158095
864865,864866,864865,1729731,1924.1014878749847,0.42751680464971287
866867,866868,866867,1733735,1928.7843420505524,0.4266079200551758
868869,868870,868869,1737739,1933.50346493721,0.42570300226361724
870871,870872,870871,1741743,1938.1910347938538,0.4248020253107825
872873,872874,872873,1745747,1942.881817817688,0.42390496346342843
874875,874876,874875,1749751,1947.562933921814,0.4230117912102287
876877,876878,876877,1753755,1952.262830734253,0.4221224832563166
878879,878880,878879,1757759,1956.9463539123535,0.4212370145305613
880881,880882,880881,1761763,1961.6541068553925,0.42035536017465347
882883,882884,882883,1765767,1966.3610088825226,0.41947749554128677
884885,884886,884885,1769771,1971.0672459602356,0.41860340019411524
886887,886888,886887,1773775,1975.7960529327393,0.4177330541169795
888889,888890,888889,1777779,1980.5624949932098,0.4168664250519214
890891,890892,890891,1781783,1985.5647978782654,0.4160034891865507
892893,892894,892893,1785787,1990.3143239021301,0.415144222906747
894895,894896,894895,1789791,1994.9784851074219,0.41428860280393565
896897,896898,896897,1793795,1999.684541940689,0.4134366056714498
898899,898900,898899,1797799,2004.3187210559845,0.41258820848997857
900901,900902,900901,1801803,2008.9944970607758,0.4117433884348429
902903,902904,902903,1805807,2013.9119749069214,0.41090212288327166
904905,904906,904905,1809811,2018.6840720176697,0.4100643893907545
906907,906908,906907,1813815,2023.3778638839722,0.4092301657055941
908909,908910,908909,1817819,2028.0818219184875,0.408399429763449
910911,910912,910911,1821823,2032.7787539958954,0.40757215968551463
912913,912914,912913,1825827,2037.4935607910156,0.40674833376579045
914915,914916,914915,1829831,2042.2788848876953,0.4059279304910888
916917,916918,916917,1833835,2046.9315347671509,0.40511092851556896
918919,918920,918919,1837839,2051.616791009903,0.4042973066771083
920921,920922,920921,1841843,2056.313155889511,0.403487043986388
922923,922924,922923,1845847,2060.970543861389,0.4026801196287124
924925,924926,924925,1849851,2065.6327748298645,0.4018765129512758
926927,926928,926927,1853855,2070.3272998332977,0.4010762034849904
928929,928930,928929,1857859,2075.0031187534332,0.40027917091902054
930931,930932,930931,1861863,2079.7023627758026,0.3994853951080586
932933,932934,932933,1865867,2084.4229698181152,0.3986948560741439
934935,934936,934935,1869871,2089.1024038791656,0.3979075340066629
936937,936938,936937,1873875,2093.827845811844,0.3971234092459781
938939,938940,938939,1877879,2098.511207818985,0.3963424622979801
940941,940942,940941,1881883,2103.3977789878845,0.3955646738213545
942943,942944,942943,1885887,2108.2381739616394,0.3947900246403151
944945,944946,944945,1889891,2112.9546189308167,0.3940184957227757
946947,946948,946947,1893895,2117.643194913864,0.39325006819490227
948949,948950,948949,1897899,2122.30738902092,0.39248472333565587
950951,950952,950951,1901903,2127.1207768917084,0.3917224425713357
952953,952954,952953,1905907,2132.0061688423157,0.3909632074773981
954955,954956,954955,1909911,2136.697731733322,0.39020699977481854
956957,956958,956957,1913915,2141.361454963684,0.38945380133191065
958959,958960,958959,1917919,2146.1392769813538,0.3887035941625072
960961,960962,960961,1921923,2151.0563180446625,0.3879563604186842
962963,962964,962963,1925927,2155.7242550849915,0.3872120823980367
964965,964966,964965,1929931,2160.4131338596344,0.3864707425382221
966967,966968,966967,1933935,2165.0967218875885,0.3857323234060459
968969,968970,968969,1937939,2169.8053550720215,0.3849968077174708
970971,970972,970971,1941943,2174.507383108139,0.3842641783230647
972973,972974,972973,1945947,2179.205271959305,0.3835344181970868
974975,974976,974975,1949951,2183.8901040554047,0.3828075104574964
976977,976978,976977,1953955,2188.549073934555,0.38208343834958214
978979,978980,978979,1957959,2193.2205817699432,0.38136218525141885
980981,980982,980981,1961963,2197.9202387332916,0.38064373466477264
982983,982984,982983,1965967,2202.61794090271,0.3799280702278338
984985,984986,984985,1969971,2207.3218579292297,0.379215175702484
986987,986988,986987,1973975,2212.0614359378815,0.378505034972477
988989,988990,988989,1977979,2216.7893240451813,0.37779763204707706
990991,990992,990991,1981983,2221.462965965271,0.37709295106105856
992993,992994,992993,1985987,2226.1190259456635,0.3763909762728872
994995,994996,994995,1989991,2230.815659046173,0.37569169205380604
996997,996998,996997,1993995,2235.4539799690247,0.37499508290238737
998999,999000,998999,1997999,2240.1443209648132,0.3743011334354378
1001001,1001002,1001001,2002003,2244.7954709529877,0.3736098283825413
1003003,1003004,1003003,2006007,2249.4604148864746,0.37292115259333514
1005005,1005006,1005005,2010011,2254.11598277092,0.3722350910284149
1007007,1007008,1007007,2014015,2258.780173063278,0.3715516287684295
1009009,1009010,1009009,2018019,2263.4820940494537,0.3708707509977103
1011011,1011012,1011011,2022023,2268.135239839554,0.37019244302791776
1013013,1013014,1013013,2026027,2273.036563873291,0.369516690267119
1015015,1015016,1015015,2030031,2277.7032351493835,0.36884347823797725
1017017,1017018,1017017,2034035,2282.5632030963898,0.3681727925722953
1019019,1019020,1019019,2038039,2287.449527978897,0.3675046190091962
1021021,1021022,1021021,2042043,2292.193529844284,0.36683894339694234
1023023,1023024,1023023,2046047,2296.966068983078,0.36617575168565963
1025025,1025026,1025025,2050051,2301.6921758651733,0.36551502993461327
1027027,1027028,1027027,2054055,2306.3716638088226,0.36485676430311287
1029029,1029030,1029029,2058059,2311.019096851349,0.3642009410523315
1031031,1031032,1031031,2062063,2315.691209077835,0.3635475465471245
1033033,1033034,1033033,2066067,2320.4287729263306,0.3628965672614868
1035035,1035036,1035035,2070071,2325.102350950241,0.3622479897530866
1037037,1037038,1037037,2074075,2329.771618127823,0.36160180069600756
1039039,1039040,1039039,2078079,2334.480568885803,0.36095798684254987
1041041,1041042,1041041,2082083,2339.1411368846893,0.360316535063248
1043043,1043044,1043043,2086087,2343.80446100235,0.359677432310491
1045045,1045046,1045045,2090091,2348.5228538513184,0.3590406656403502
1047047,1047048,1047047,2094095,2353.1760199069977,0.35840622219620855
1049049,1049050,1049049,2098099,2357.8504209518433,0.35777408922331233
1051051,1051052,1051051,2102103,2362.484783887863,0.35714425405603833
1053053,1053054,1053053,2106107,2367.3237178325653,0.3565167041178938
1055055,1055056,1055055,2110111,2372.1727969646454,0.3558914269269735
1057057,1057058,1057057,2114115,2376.8310730457306,0.35526841009414056
1059059,1059060,1059059,2118119,2381.688153743744,0.35464764131393167
1061061,1061062,1061061,2122123,2386.3560090065002,0.354029108371833
1063063,1063064,1063063,2126127,2391.0675909519196,0.3534127991479181
1065065,1065066,1065065,2130131,2395.8287649154663,0.35279870159683924
1067067,1067068,1067067,2134135,2400.5197970867157,0.3521868037732929
1069069,1069070,1069069,2138139,2405.1640689373016,0.3515770938083733
1071071,1071072,1071071,2142143,2409.8303220272064,0.3509695599186671
1073073,1073074,1073073,2146147,2414.515843153,0.3503641904080723
1075075,1075076,1075075,2150151,2419.5764169692993,0.3497609736641607
1077077,1077078,1077077,2154155,2424.298017978668,0.3491598981545394
1079079,1079080,1079079,2158159,2428.9926538467407,0.3485609524359461
1081081,1081082,1081081,2162163,2433.87162399292,0.34796412513060204
1083083,1083084,1083083,2166167,2438.5234088897705,0.347369404957135
1085085,1085086,1085085,2170171,2443.2390677928925,0.3467767807051132
1087087,1087088,1087087,2174175,2447.912488937378,0.3461862412514165
1089089,1089090,1089089,2178179,2452.6133120059967,0.3455977755384083
1091091,1091092,1091091,2182183,2457.397511959076,0.3450113726012205
1093093,1093094,1093093,2186187,2462.047341108322,0.3444270215368306
1095095,1095096,1095095,2190191,2466.716356754303,0.34384471153134655
1097097,1097098,1097097,2194195,2471.4094920158386,0.343264431838179
1099099,1099100,1099099,2198199,2476.0799679756165,0.3426861717925931
1101101,1101102,1101101,2202203,2480.7985780239105,0.3421099207971565
1103103,1103104,1103103,2206207,2485.6412448883057,0.3415356683344726
1105105,1105106,1105105,2210211,2490.5547120571136,0.34096340395444713
1107107,1107108,1107107,2214215,2495.5837218761444,0.3403931172833836
1109109,1109110,1109109,2218219,2500.3340990543365,0.3398247980148881
1111111,1111112,1111111,2222223,2505.040694952011,0.33925843592624005
1113113,1113114,1113113,2226227,2509.776885032654,0.3386940208474698
1115115,1115116,1115115,2230231,2514.5077970027924,0.33813154269410006
1117117,1117118,1117117,2234235,2519.194296836853,0.33757099143804226
1119119,1119120,1119119,2238239,2523.895805835724,0.33701235713124333
1121121,1121122,1121121,2242243,2528.5691509246826,0.3364556298874959
1123123,1123124,1123123,2246247,2533.295350074768,0.33590079988607613
1125125,1125126,1125125,2250251,2537.9424130916595,0.3353478573844768
1127127,1127128,1127127,2254255,2542.630198955536,0.3347967926929414
1129129,1129130,1129129,2258259,2547.4213309288025,0.33424759619447286
1131131,1131132,1131131,2262263,2552.0888998508453,0.3337002583393769
1133133,1133134,1133133,2266267,2556.74719786644,0.33315476963798574
1135135,1135136,1135135,2270271,2561.4713368415833,0.3326111206697533
1137137,1137138,1137137,2274275,2566.1185009479523,0.3320693020723411
1139139,1139140,1139139,2278279,2570.7656078338623,0.3315293045507133
1141141,1141142,1141141,2282283,2575.504630088806,0.33099111887167965
1143143,1143144,1143143,2286287,2580.1620709896088,0.33045473586207663
1145145,1145146,1145145,2290291,2584.7994129657745,0.3299201464160433
1147147,1147148,1147147,2294295,2589.6476271152496,0.32938734147865034
1149149,1149150,1149149,2298299,2594.5234088897705,0.32885631206590915
1151151,1151152,1151151,2302303,2599.2061638832092,0.3283270492502197
1153153,1153154,1153153,2306307,2603.879212141037,0.3277995441585517
1155155,1155156,1155155,2310311,2608.562306165695,0.3272737879851775
1157157,1157158,1157157,2314315,2613.226611852646,0.32674977198075794
1159159,1159160,1159159,2318319,2617.908819913864,0.3262274874487048
1161161,1161162,1161161,2322323,2622.5998950004578,0.3257069257560943
1163163,1163164,1163163,2326327,2627.248820066452,0.3251880783227534
1165165,1165166,1165165,2330331,2631.9566509723663,0.3246709366339928
1167167,1167168,1167167,2334335,2636.600373983383,0.32415549221514084
1169169,1169170,1169169,2338339,2641.299989938736,0.32364173666246643
1171171,1171172,1171171,2342343,2645.991768836975,0.32312966162317025
1173173,1173174,1173173,2346347,2650.8339278697968,0.32261925879538467
1175175,1175176,1175175,2350351,2655.6050288677216,0.3221105199354497
1177177,1177178,1177177,2354355,2660.241914987564,0.32160343685245607
1179179,1179180,1179179,2358359,2664.8952779769897,0.32109800141006417
1181181,1181182,1181181,2362363,2669.572736978531,0.3205942055228661
1183183,1183184,1183183,2366367,2674.2630457878113,0.32009204116002365
1185185,1185186,1185185,2370371,2679.150027990341,0.3195915003434493
1187187,1187188,1187187,2374375,2683.8980510234833,0.3190925751441682
1189189,1189190,1189189,2378379,2688.554510831833,0.3185952576877753
1191191,1191192,1191191,2382383,2693.2914760112762,0.3180995401489781
1193193,1193194,1193193,2386387,2697.9451761245728,0.317605414749778
1195195,1195196,1195195,2390391,2702.6462478637695,0.3171128737685649
1197197,1197198,1197197,2394395,2707.3527870178223,0.31662190953284153
1199199,1199200,1199199,2398399,2712.084737062454,0.3161325144155853
1201201,1201202,1201201,2402403,2716.72616815567,0.3156446808407054
1203203,1203204,1203203,2406407,2721.4417259693146,0.31515840127940464
1205205,1205206,1205205,2410411,2726.066589832306,0.3146736682519986
1207207,1207208,1207207,2414415,2730.7309041023254,0.31419047433155356
1209209,1209210,1209209,2418419,2735.363065958023,0.31370881212933455
1211211,1211212,1211211,2422423,2740.0465359687805,0.3132286743093573
1213213,1213214,1213213,2426427,2744.7232551574707,0.3127500535792933
1215215,1215216,1215215,2430431,2749.404057741165,0.31227294269774575
1217217,1217218,1217217,2434435,2754.0871658325195,0.31179733446697355
1219219,1219220,1219219,2438439,2758.7597119808197,0.3113232217328914
1221221,1221222,1221221,2442443,2763.4213650226593,0.3108505973887077
1223223,1223224,1223223,2446447,2768.101241827011,0.31037945437128656
1225225,1225226,1225225,2450451,2772.8004517555237,0.3099097856611479
1227227,1227228,1227227,2454455,2777.461770057678,0.30944158428610535
1229229,1229230,1229229,2458459,2782.3608677387238,0.30897484331944725
1231231,1231232,1231231,2462463,2787.0641779899597,0.30850955586902273
1233233,1233234,1233233,2466467,2791.7194299697876,0.30804571509361267
1235235,1235236,1235235,2470471,2796.3644721508026,0.30758331419383467
1237237,1237238,1237237,2474475,2801.163707971573,0.3071223464085051
1239239,1239240,1239239,2478479,2805.9328248500824,0.3066628050255531
1241241,1241242,1241241,2482483,2810.8022499084473,0.30620468336746853
1243243,1243244,1243243,2486487,2815.7039799690247,0.30574797480585403
1245245,1245246,1245245,2490491,2820.3837399482727,0.305292672743235
1247247,1247248,1247247,2494495,2825.0937299728394,0.3048387706348876
1249249,1249250,1249249,2498499,2829.76824092865,0.3043862619651918
1251251,1251252,1251251,2502503,2834.552358865738,0.3039351402694592
1253253,1253254,1253253,2506507,2839.252716064453,0.30348539911574335
1255255,1255256,1255255,2510511,2843.937597990036,0.3030370321121154
1257257,1257258,1257257,2514515,2848.602110862732,0.3025900329084834
1259259,1259260,1259259,2518519,2853.2733449935913,0.3021443951947731
1261261,1261262,1261261,2522523,2857.9474968910217,0.30170011269365204
1263263,1263264,1263263,2526527,2862.6413209438324,0.30125717917690054
1265265,1265266,1265265,2530531,2867.3355820178986,0.3008155884381267
1267267,1267268,1267267,2534535,2872.04269695282,0.3003753343291464
1269269,1269270,1269269,2538539,2876.694761991501,0.29993641071996535
1271271,1271272,1271271,2542543,2881.4028627872467,0.2994988115315209
1273273,1273274,1273273,2546547,2886.0747079849243,0.29906253071385436
1275275,1275276,1275275,2550551,2890.767447948456,0.2986275622588437
1277277,1277278,1277277,2554555,2895.45529794693,0.2981939001911087
1279279,1279280,1279279,2558559,2900.102098941803,0.297761538575287
1281281,1281282,1281281,2562563,2904.7720110416412,0.29733047150511993
1283283,1283284,1283283,2566567,2909.633908033371,0.2969006931198237
1285285,1285286,1285285,2570571,2914.3858649730682,0.2964721975804423
1287287,1287288,1287287,2574575,2919.048696756363,0.29604497909895144
1289289,1289290,1289289,2578579,2923.728653907776,0.29561903190915473
1291291,1291292,1291291,2582583,2928.3825039863586,0.2951943502866925
1293293,1293294,1293293,2586587,2933.1167948246,0.2947709285399469
1295295,1295296,1295295,2590591,2937.8470978736877,0.2943487610118609
1297297,1297298,1297297,2594595,2942.500830888748,0.2939278420763003
1299299,1299300,1299299,2598599,2947.1847789287567,0.2935081661416916
1301301,1301302,1301301,2602603,2952.007917165756,0.29308972765102226
1303303,1303304,1303303,2606607,2956.6729769706726,0.2926725210782024
1305305,1305306,1305305,2610611,2961.365859746933,0.29225654093352205
1307307,1307308,1307307,2614615,2966.0274579524994,0.29184178193099797
1309309,1309310,1309309,2618619,2970.7801349163055,0.2914282386609557
1311311,1311312,1311311,2622623,2975.620250940323,0.2910159055409167
1313313,1313314,1313313,2626627,2980.556179046631,0.29060477720486233
1315315,1315316,1315315,2630631,2985.455636024475,0.29019484832315356
1317317,1317318,1317317,2634635,2990.3747520446777,0.28978611358797934
1319319,1319320,1319319,2638639,2995.195606946945,0.2893785677424603
1321321,1321322,1321321,2642643,2999.8764810562134,0.28897220554063097
1323323,1323324,1323323,2646647,3004.528100967407,0.2885670217801817
1325325,1325326,1325325,2650651,3009.332254886627,0.2881630112788116
1327327,1327328,1327327,2654655,3014.0587871074677,0.2877601688978757
1329329,1329330,1329329,2658659,3018.738410949707,0.2873584895150998
1331331,1331332,1331331,2662663,3023.4072258472443,0.2869579680445895
1333333,1333334,1333333,2666667,3028.129590988159,0.2865585994313733
1335335,1335336,1335335,2670671,3032.781080722809,0.28616037864776445
1337337,1337338,1337337,2674675,3037.4412820339203,0.28576330069699907
1339339,1339340,1339339,2678679,3042.166531085968,0.28536736060414114
1341341,1341342,1341341,2682683,3046.8368439674377,0.2849725534360914
1343343,1343344,1343343,2686687,3051.7030398845673,0.2845788742724835
1345345,1345346,1345345,2690691,3056.46381688118,0.2841863182384259
1347347,1347348,1347347,2694695,3061.1354517936707,0.28379488046994084
1349349,1349350,1349349,2698699,3065.8078808784485,0.28340455614852544
1351351,1351352,1351351,2702703,3070.4948279857635,0.2830153404684097
1353353,1353354,1353353,2706707,3075.2694039344788,0.2826272286565654
1355355,1355356,1355355,2710711,3080.037871837616,0.2822402159708872
1357357,1357358,1357357,2714715,3084.705682992935,0.2818542976929166
1359359,1359360,1359359,2718719,3089.442691087723,0.28146946913329884
1361361,1361362,1361361,2722723,3094.1208069324493,0.2810857256226882
1363363,1363364,1363363,2726727,3098.8579359054565,0.2807030625299376
1365365,1365366,1365365,2730731,3103.970855951309,0.28032147524208995
1367367,1367368,1367367,2734735,3109.000277042389,0.27994095917347295
1369369,1369370,1369369,2738739,3114.042366027832,0.27956150976569916
1371371,1371372,1371371,2742743,3119.0915138721466,0.279183122484028
1373373,1373374,1373373,2746747,3124.13329410553,0.2788057928210037
1375375,1375376,1375375,2750751,3129.2043809890747,0.2784295163000934
1377377,1377378,1377377,2754755,3134.242365837097,0.278054288459316
1379379,1379380,1379379,2758759,3139.2661440372467,0.2776801048694324
1381381,1381382,1381381,2762763,3144.286814928055,0.2773069611230312
1383383,1383384,1383383,2766767,3149.5890049934387,0.276934852838167
1385385,1385386,1385385,2770771,3154.7654490470886,0.2765637756601791
1387387,1387388,1387387,2774775,3159.7844009399414,0.27619372525441577
1389389,1389390,1389389,2778779,3164.821939945221,0.2758246973116911
1391391,1391392,1391391,2782783,3169.5306990146637,0.27545668754646613
1393393,1393394,1393393,2786787,3174.3348758220673,0.27508969170230557
1395395,1395396,1395395,2790791,3179.0360078811646,0.27472370554278314
1397397,1397398,1397397,2794795,3183.702610015869,0.2743587248478434
1399399,1399400,1399399,2798799,3188.430755853653,0.27399474543744873
1401401,1401402,1401401,2802803,3193.07675075531,0.2736317631370184
1403403,1403404,1403403,2806807,3197.7282240390778,0.2732697738083516
1405405,1405406,1405405,2810811,3202.4282608032227,0.2729087733277993
1407407,1407408,1407407,2814815,3207.0730240345,0.2725487575989973
1409409,1409410,1409409,2818819,3211.7446699142456,0.27218972254922846
1411411,1411412,1411411,2822823,3216.459836959839,0.2718316641239653
1413413,1413414,1413413,2826827,3221.1639969348907,0.27147457829232735
1415415,1415416,1415415,2830831,3225.8525619506836,0.27111846104526194
1417417,1417418,1417417,2834835,3230.738133907318,0.27076330840282026
1419419,1419420,1419419,2838839,3235.6006758213043,0.27040911639414844
1421421,1421422,1421421,2842843,3240.2724969387054,0.27005588107931544
1423423,1423424,1423423,2846847,3244.923999071121,0.2697035985402181
1425425,1425426,1425425,2850851,3249.6518337726593,0.2693522648733051
1427427,1427428,1427427,2854855,3254.2746369838715,0.2690018762041291
1429429,1429430,1429429,2858859,3258.952008008957,0.2686524286691565
1431431,1431432,1431431,2862863,3263.6208879947662,0.2683039184394147
1433433,1433434,1433433,2866867,3268.2649998664856,0.2679563417004829
1435435,1435436,1435435,2870871,3272.906965970993,0.2676096946524922
1437437,1437438,1437437,2874875,3277.699469804764,0.2672639735210396
1439439,1439440,1439439,2878879,3282.5502038002014,0.26691917455900693
1441441,1441442,1441441,2882883,3287.202742099762,0.26657529403019
1443443,1443444,1443443,2886887,3291.8500678539276,0.26623232822021237
1445445,1445446,1445445,2890891,3296.574812889099,0.2658902734383446
1447447,1447448,1447447,2894895,3301.258059024811,0.2655491260084091
1449449,1449450,1449449,2898899,3305.8874781131744,0.2652088822796941
1451451,1451452,1451451,2902903,3310.621230840683,0.26486953861967777
1453453,1453454,1453453,2906907,3315.292135953903,0.2645310914122092
1455455,1455456,1455455,2910911,3319.9601669311523,0.26419353705932735
1457457,1457458,1457457,2914915,3325.0481259822845,0.263856871993994
1459459,1459460,1459459,2918919,3329.7574529647827,0.2635210926509899
1461461,1461462,1461461,2922923,3334.439983844757,0.2631861954960186
1463463,1463464,1463463,2926927,3339.1146397590637,0.2628521770129737
1465465,1465466,1465465,2930931,3343.901160955429,0.2625190336966625
1467467,1467468,1467467,2934935,3348.583643913269,0.2621867620746343
1469469,1469470,1469469,2938939,3353.3184950351715,0.26185535867261933
1471471,1471472,1471471,2942943,3358.0109388828278,0.2615248200527276
1473473,1473474,1473473,2946947,3363.052706003189,0.26119514278980205
1475475,1475476,1475475,2950951,3368.084100961685,0.26086632347323757
1477477,1477478,1477477,2954955,3373.1125209331512,0.2605383587106189
1479479,1479480,1479479,2958959,3378.1479120254517,0.2602112451349967
1481481,1481482,1481481,2962963,3383.199937105179,0.2598849793866975
1483483,1483484,1483483,2966967,3388.3025028705597,0.25955955813333276
1485485,1485486,1485485,2970971,3393.3505008220673,0.2592349780516088
1487487,1487488,1487487,2974975,3398.3764810562134,0.2589112358436978
1489489,1489490,1489489,2978979,3403.4805879592896,0.25858832822268596
1491491,1491492,1491491,2982983,3408.7395210266113,0.2582662519198493
1493493,1493494,1493493,2986987,3413.855443954468,0.2579450036864728
1495495,1495496,1495495,2990991,3418.871097803116,0.25762458029203117
1497497,1497498,1497497,2994995,3424.0630910396576,0.25730497851691325
1499499,1499500,1499499,2998999,3428.9117918014526,0.2569861951578787
1501502,1501503,1501502,3003005,3433.710983991623,0.25666806841582
1503504,1503505,1503504,3007009,3438.465229034424,0.25635091277035826
1505506,1505507,1505506,3011013,3443.2849700450897,0.2560345660440362
1507508,1507509,1507508,3015017,3448.039760828018,0.25571902510273503
1509510,1509511,1509510,3019021,3453.014402151108,0.255404286826888
1511512,1511513,1511512,3023025,3457.7467629909515,0.2550903481169371
1513514,1513515,1513514,3027029,3462.430862903595,0.25477720588787633
1515516,1515517,1515516,3031033,3467.1307320594788,0.2544648570692516
1517518,1517519,1517518,3035037,3472.116180896759,0.25415329860697966
1519520,1519521,1519520,3039041,3476.912863969803,0.25384252746334823
1521522,1521523,1521522,3043045,3481.6567130088806,0.2535325406151969
1523524,1523525,1523524,3047049,3486.5130639076233,0.25322333505755523
1525526,1525527,1525526,3051053,3491.4442160129547,0.2529149077945476
1527528,1527529,1527528,3055057,3496.296814918518,0.2526072558557644
1529530,1529531,1529530,3059061,3501.0419569015503,0.2523003762762528
1531532,1531533,1531532,3063065,3505.784564971924,0.251994266112888
1533534,1533535,1533534,3067069,3510.4725110530853,0.2516889224298211
1535536,1535537,1535536,3071073,3515.183121919632,0.2513843423148501
1537538,1537539,1537538,3075077,3519.872658967972,0.2510805228703248
1539540,1539541,1539540,3079081,3524.543086051941,0.2507774612022331
1541542,1541543,1541542,3083085,3529.237979888916,0.2504751544420287
1543544,1543545,1543544,3087089,3533.9092059135437,0.2501735997320793
1545546,1545547,1545546,3091093,3538.556384086609,0.24987279422930442
1547548,1547549,1547548,3095097,3543.264643907547,0.24957273510699451
1549550,1549551,1549550,3099101,3547.965348958969,0.24927341955299198
1551552,1551553,1551552,3103105,3552.765748977661,0.24897484476059617
1553554,1553555,1553554,3107109,3557.7359340190887,0.24867700794857228
1555556,1555557,1555556,3111113,3562.406221151352,0.24837990634296148
1557558,1557559,1557558,3115117,3567.210849046707,0.2480835371898138
1559560,1559561,1559560,3119121,3572.0120408535004,0.24778789773699827
1561562,1561563,1561562,3123125,3576.707619190216,0.24749298526330676
1563564,1563565,1563564,3127129,3581.4506709575653,0.24719879704753112
1565566,1565567,1565566,3131133,3586.112761735916,0.24690533038665308
1567568,1567569,1567568,3135137,3590.7488629817963,0.2466125825922063
1569570,1569571,1569570,3139141,3595.549824953079,0.24632055098481942
1571572,1571573,1571572,3143145,3600.2223460674286,0.2460292329033109
1573574,1573575,1573574,3147149,3604.898456096649,0.24573862569923222
1575576,1575577,1575576,3151153,3609.6666860580444,0.24544872673686768
1577578,1577579,1577578,3155157,3614.3241081237793,0.24515953338959662
1579580,1579581,1579580,3159161,3619.013447999954,0.24487104304716922
1581582,1581583,1581582,3163165,3623.731173992157,0.2445832531157066
1583584,1583585,1583584,3167169,3628.3918840885162,0.24429616100860585
1585586,1585587,1585586,3171173,3633.0837240219116,0.24400976415199693
1587588,1587589,1587588,3175177,3637.7886850833893,0.24372405998656177
1589590,1589591,1589590,3179181,3642.4841599464417,0.24343904596935317
1591592,1591593,1591592,3183185,3647.13281583786,0.24315471956469992
1593594,1593595,1593594,3187189,3651.805421113968,0.2428710782496637
1595596,1595597,1595596,3191193,3656.466673851013,0.24258811951585812
1597598,1597599,1597598,3195197,3661.0804579257965,0.24230584086399176
1599600,1599601,1599600,3199201,3665.69780087471,0.24202423981478205
1601602,1601603,1601602,3203205,3670.318193912506,0.24174331388894643
1603604,1603605,1603604,3207209,3675.0031628608704,0.2414630606308492
1605606,1605607,1605606,3211213,3679.689822912216,0.24118347759031167
1607608,1607609,1607608,3215217,3684.3719370365143,0.240904562329888
1609610,1609611,1609610,3219221,3689.0434980392456,0.24062631242486532
1611612,1611613,1611612,3223225,3693.7424080371857,0.2403487254632637
1613614,1613615,1613614,3227229,3698.4767060279846,0.2400717990421981
1615616,1615617,1615616,3231233,3703.154624938965,0.23979553077515448
1617618,1617619,1617618,3235237,3707.907753944397,0.23951991828289465
1619620,1619621,1619620,3239241,3712.7496540546417,0.23924495919709443
1621622,1621623,1621622,3243245,3717.4213609695435,0.23897065116398153
1623624,1623625,1623624,3247249,3722.0534908771515,0.2386969918388786
1625626,1625627,1625626,3251253,3726.7508709430695,0.23842397888984124
1627628,1627629,1627628,3255257,3731.555704832077,0.23815160999583895
1629630,1629631,1629630,3259261,3736.2191219329834,0.2378798828467552
1631632,1631633,1631632,3263265,3740.9119050502777,0.2376087951433874
1633634,1633635,1633634,3267269,3745.636512041092,0.23733834459562786
1635636,1635637,1635636,3271273,3750.3324389457703,0.23706852893337782
1637638,1637639,1637638,3275277,3755.468142747879,0.23679934588108154
1639640,1639641,1639640,3279281,3760.260015964508,0.2365307931922871
1641642,1641643,1641642,3283285,3764.9836349487305,0.2362628686150856
1643644,1643645,1643644,3287289,3769.64817404747,0.23599556991939608
1645646,1645647,1645646,3291293,3774.3424429893494,0.23572889488423243
1647648,1647649,1647648,3295297,3779.0381088256836,0.2354628412904276
1649650,1649651,1649650,3299301,3783.669203042984,0.23519740694246138
1651652,1651653,1651652,3303305,3788.311989068985,0.23493258964845154
1653654,1653655,1653654,3307309,3793.0172939300537,0.2346683872219728
1655656,1655657,1655656,3311313,3797.6796929836273,0.23440479749478982
1657658,1657659,1657658,3315317,3802.3631360530853,0.23414181830594316
1659660,1659661,1659660,3319321,3807.169729948044,0.23387944750720635
1661662,1661663,1661662,3323325,3812.030844926834,0.23361768295580987
1663664,1663665,1663664,3327329,3816.6970250606537,0.23335652252353611
1665666,1665667,1665666,3331333,3821.385466814041,0.23309596408762445
1667668,1667669,1667668,3335337,3826.0270009040833,0.23283600553986616
1669670,1669671,1669670,3339341,3830.7997250556946,0.2325766447775095
1671672,1671673,1671672,3343345,3835.526741027832,0.2323178797159926
1673674,1673675,1673674,3347349,3840.183662891388,0.23205970826711564
1675676,1675677,1675676,3351353,3844.8350129127502,0.23180212836632563
1677678,1677679,1677678,3355357,3849.5743827819824,0.23154513794725062
1679680,1679681,1679680,3359361,3854.226826906204,0.23128873496170854
1681682,1681683,1681682,3363365,3858.861790895462,0.2310329173651553
1683684,1683685,1683684,3367369,3863.5773499011993,0.23077768312759872
1685686,1685687,1685686,3371373,3868.219352722168,0.2305230302245036
1687688,1687689,1687688,3375377,3872.881635904312,0.23026895664406766
1689690,1689691,1689690,3379381,3877.5698449611664,0.2300154603781266
1691692,1691693,1691692,3383385,3882.3573899269104,0.229762539436706
1693694,1693695,1693694,3387389,3887.0518209934235,0.22951019182983146
1695696,1695697,1695696,3391393,3891.7508301734924,0.2292584155820805
1697698,1697699,1697698,3395397,3896.468204975128,0.22900720872712554
1699700,1699701,1699700,3399401,3901.126708984375,0.22875656930409605
1701702,1701703,1701702,3403405,3905.800817966461,0.2285064953703113
1703704,1703705,1703704,3407409,3910.522572994232,0.2282569849758147
1705706,1705707,1705706,3411413,3915.2328720092773,0.22800803619247745
1707708,1707709,1707708,3415417,3919.8839790821075,0.2277596471049037
1709710,1709711,1709710,3419421,3924.599598169327,0.2275118157886027
1711712,1711713,1711712,3423425,3929.252079963684,0.22726454034273047
1713714,1713715,1713714,3427429,3933.9570429325104,0.22701781887553807
1715716,1715717,1715716,3431433,3938.6161358356476,0.2267716494952765
1717718,1717719,1717718,3435437,3943.3141570091248,0.22652603032292973
1719720,1719721,1719720,3439441,3947.957039833069,0.22628095948675764
1721722,1721723,1721722,3443445,3952.7170419692993,0.22603643512957206
1723724,1723725,1723724,3447449,3957.400239944458,0.2257924553923658
1725726,1725727,1725726,3451453,3962.038656949997,0.2255490184361406
1727728,1727729,1727728,3455457,3966.697462081909,0.2253061224200792
1729730,1729731,1729730,3459461,3971.6015717983246,0.22506376551791618
1731732,1731733,1731732,3463465,3976.333306789398,0.2248219459052052
1733734,1733735,1733734,3467469,3981.046956062317,0.2245806617775088
1735736,1735737,1735736,3471473,3985.7273559570312,0.22433991132675146
1737738,1737739,1737738,3475477,3990.391832113266,0.22409969275940966
1739740,1739741,1739740,3479481,3995.1142070293427,0.22386000428741681
1741742,1741743,1741742,3483485,3999.88302898407,0.22362084413180128
1743744,1743745,1743744,3487489,4004.5222549438477,0.22338221052086737
1745746,1745747,1745746,3491493,4009.1868238449097,0.22314410169201437
1747748,1747749,1747748,3495497,4013.8536677360535,0.22290651588627952
1749750,1749751,1749750,3499501,4018.5074520111084,0.22266945136470895
1751752,1751753,1751752,3503505,4023.3496038913727,0.22243290638107283
1753754,1753755,1753754,3507509,4028.0807271003723,0.22219687920187425
1755756,1755757,1755756,3511513,4032.770171880722,0.22196136810998723
1757758,1757759,1757758,3515517,4037.4397099018097,0.2217263713846478
1759760,1759761,1759760,3519521,4042.1206290721893,0.22149188731964387
1761762,1761763,1761762,3523525,4046.809666156769,0.22125791421058238
1763764,1763765,1763764,3527529,4051.4538300037384,0.22102445036398422
1765766,1765767,1765766,3531533,4056.1152789592743,0.22079149409728416
1767768,1767769,1767768,3535537,4060.791626930237,0.220559043729736
1769770,1769771,1769770,3539541,4065.5643589496613,0.2203270975896885
1771772,1771773,1771772,3543545,4070.2930018901825,0.2200956540145853
1773774,1773775,1773774,3547549,4075.1848998069763,0.2198647113473271
1775776,1775777,1775776,3551553,4080.05402803421,0.21963426794172847
1777778,1777779,1777778,3555557,4084.74085688591,0.21940432215342298
1779780,1779781,1779780,3559561,4089.409698009491,0.21917487235077715
1781782,1781783,1781782,3563565,4094.0908937454224,0.21894591690215748
1783784,1783785,1783784,3567569,4098.739641904831,0.2187174541886634
1785786,1785787,1785786,3571573,4103.4259259700775,0.21848948260048928
1787788,1787789,1787788,3575577,4108.252830982208,0.2182620005296485
1789790,1789791,1789790,3579581,4113.006599903107,0.21803500638088735
1791792,1791793,1791792,3583585,4117.672245979309,0.21780849855531415
1793794,1793795,1793794,3587589,4122.356248140335,0.21758247547404608
1795796,1795797,1795796,3591593,4127.001603841782,0.21735693555456237
1797798,1797799,1797798,3595597,4131.651002883911,0.21713187723071314
1799800,1799801,1799800,3599601,4136.503235816956,0.21690729893452954
1801802,1801803,1801802,3603605,4141.153810977936,0.2166831991107756
1803804,1803805,1803804,3607609,4145.800557136536,0.21645957621149137
1805806,1805807,1805806,3611613,4150.504482984543,0.21623642868871684
1807808,1807809,1807808,3615617,4155.449547052383,0.21601375500540598
1809810,1809811,1809810,3619621,4160.150623083115,0.2157915536336077
1811812,1811813,1811812,3623625,4164.804616928101,0.21556982304900885
1813814,1813815,1813814,3627629,4169.437786817551,0.2153485617309343
1815816,1815817,1815816,3631633,4174.099541902542,0.21512776817507984
1817818,1817819,1817818,3635637,4178.832950115204,0.2149074408753222
1819820,1819821,1819820,3639641,4183.813017845154,0.2146875783273572
1821822,1821823,1821822,3643645,4188.497878074646,0.2144681790505274
1823824,1823825,1823824,3647649,4193.147068977356,0.21424924155144254
1825826,1825827,1825826,3651653,4197.8661477565765,0.21403076435854018
1827828,1827829,1827828,3655657,4202.515860080719,0.2138127459984389
1829830,1829831,1829830,3659661,4207.185415029526,0.21359518500321428
1831832,1831833,1831832,3663665,4211.89159989357,0.2133780799122178
1833834,1833835,1833834,3667669,4216.709192037582,0.2131614292757149
1835836,1835837,1835836,3671673,4221.423552036285,0.21294523164579005
1837838,1837839,1837838,3675677,4226.142035961151,0.2127294855818036
1839840,1839841,1839840,3679681,4230.801050901413,0.21251418965039193
1841842,1841843,1841842,3683685,4235.468526124954,0.21229934242001036
1843844,1843845,1843844,3687689,4240.193270921707,0.21208494247184717
1845846,1845847,1845846,3691693,4244.95007109642,0.2118709883889096
1847848,1847849,1847848,3695697,4249.662735939026,0.2116574787578429
1849850,1849851,1849850,3699701,4254.392082929611,0.21144441217984422
1851852,1851853,1851852,3703705,4259.056733846664,0.2112317872524727
1853854,1853855,1853854,3707709,4263.722405910492,0.2110196025823825
1855856,1855857,1855856,3711713,4268.415844917297,0.21080785678896063
1857858,1857859,1857858,3715717,4273.0724539756775,0.21059655436511093
1859860,1859861,1859860,3719721,4277.717505931854,0.21038568840231164
1861862,1861863,1861862,3723725,4282.416085958481,0.2101752571761608
1863864,1863865,1863864,3727729,4287.1167249679565,0.20996525932605437
1865866,1865867,1865866,3731733,4291.745219945908,0.20975569349138823
1867868,1867869,1867868,3735737,4296.499185800552,0.2095465583188343
1869870,1869871,1869870,3739741,4301.280739068985,0.20933785246597836
1871872,1871873,1871872,3743745,4305.938288927078,0.20912957459040626
1873874,1873875,1873874,3747749,4310.604646921158,0.2089217233551608
1875876,1875877,1875876,3751753,4315.227801799774,0.20871429743601766
1877878,1877879,1877878,3755757,4319.886115074158,0.2085072955051146
1879880,1879881,1879880,3759761,4324.575672864914,0.20830071624732227
1881882,1881883,1881882,3763765,4329.2517030239105,0.20809455834933033
1883884,1883885,1883884,3767769,4333.947895050049,0.20788882050510438
1885886,1885887,1885886,3771773,4338.611768007278,0.20768350141042902
1887888,1887889,1887888,3775777,4343.573312997818,0.20747859977200278
1889890,1889891,1889890,3779781,4348.251757144928,0.2072741142965242
1891892,1891893,1891892,3783785,4352.928771018982,0.20707004369796778
1893894,1893895,1893894,3787789,4357.627857923508,0.20686638669940294
1895896,1895897,1895896,3791793,4362.298276901245,0.20666314202571812
1897898,1897899,1897898,3795797,4367.0987668037415,0.20646030840543972
1899900,1899901,1899900,3799801,4371.757230758667,0.2062578845761891
1901902,1901903,1901902,3803805,4376.429517745972,0.2060558692774066
1903904,1903905,1903904,3807809,4381.099759817123,0.2058542612576275
1905906,1905907,1905906,3811813,4385.783899784088,0.20565305926356814
1907908,1907909,1907908,3815817,4390.499851942062,0.2054522620564967
1909910,1909911,1909910,3819821,4395.198893070221,0.2052518683976814
1911912,1911913,1911912,3823825,4400.242692947388,0.20505187705020944
1913914,1913915,1913914,3827829,4404.961562871933,0.20485228678990097
1915916,1915917,1915916,3831833,4409.6803431510925,0.20465309638893814
1917918,1917919,1917918,3835837,4414.3159601688385,0.20445430463223602
1919920,1919921,1919920,3839841,4418.963288068771,0.20425591031198564
1921922,1921923,1921922,3843845,4423.663072109222,0.20405791220946412
1923924,1923925,1923924,3847849,4428.311846971512,0.2038603091295954
1925926,1925927,1925926,3851853,4433.019514799118,0.20366309986820852
1927928,1927929,1927928,3855857,4437.749998807907,0.2034662832338654
1929930,1929931,1929930,3859861,4442.397401809692,0.20326985804240394
1931932,1931933,1931932,3863865,4447.083482980728,0.20307382310420508
1933934,1933935,1933934,3867869,4451.794034004211,0.20287817724056367
1935936,1935937,1935936,3871873,4456.420534133911,0.20268291928005056
1937938,1937939,1937938,3875877,4461.360008955002,0.20248804805669351
1939940,1939941,1939940,3879881,4466.075471878052,0.2022935623972444
1941942,1941943,1941942,3883885,4470.728209972382,0.2020994611466449
1943944,1943945,1943944,3887889,4475.394414901733,0.2019057431480178
1945946,1945947,1945946,3891893,4480.171870946884,0.20171240725358075
1947948,1947949,1947948,3895897,4484.8787751197815,0.20151945231737045
1949950,1949951,1949950,3899901,4489.547554016113,0.20132687719342357
1951952,1951953,1951952,3903905,4494.194893121719,0.20113468074669072
1953954,1953955,1953954,3907909,4499.22262597084,0.20094286185121746
1955956,1955957,1955956,3911913,4504.0372059345245,0.2007514193701354
1957958,1957959,1957958,3915917,4508.732905864716,0.20056035218840407
1959960,1959961,1959960,3919921,4513.391453027725,0.20036965918188798
1961962,1961963,1961962,3923925,4518.073987722397,0.20017933923918463
1963964,1963965,1963964,3927929,4522.7506980896,0.19998939124889148
1965966,1965967,1965966,3931933,4527.478595018387,0.19979981410870096
1967968,1967969,1967968,3935937,4532.302670955658,0.1996106067126675
1969970,1969971,1969970,3939941,4536.935380935669,0.19942176797121647
1971972,1971973,1971972,3943945,4541.64004778862,0.19923329678567825
1973974,1973975,1973974,3947949,4546.294841766357,0.19904519207375415
1975976,1975977,1975976,3951953,4550.921060800552,0.1988574527495075
1977978,1977979,1977978,3955957,4555.73059797287,0.19867007773609657
1979980,1979981,1979980,3959961,4560.4220678806305,0.19848306595849863
1981982,1981983,1981982,3963965,4565.210164070129,0.19829641634169093
1983984,1983985,1983984,3967969,4569.902776002884,0.19811012782520265
1985986,1985987,1985986,3971973,4574.543251037598,0.19792419934128702
1987988,1987989,1987988,3975977,4579.247550010681,0.19773862983674917
1989990,1989991,1989990,3979981,4583.955366849899,0.19755341825839423
1991992,1991993,1991992,3983985,4588.607778072357,0.19736856355484633
1993994,1993995,1993994,3987989,4593.2763459682465,0.19718406468018657
1995996,1995997,1995996,3991993,4597.934273958206,0.196999920593953
1997998,1997999,1997998,3995997,4602.866447925568,0.19681613025932165
2000000,2000001,2000000,4000001,4607.572920799255,0.19663269264310657


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0058441162109375,12064.709122577777
1001,7464,7464,14928,22.337682962417603,0.20711947713971313
2002,15168,15168,30336,47.1640510559082,0.033931367774130194
3003,22980,22980,45960,74.1202540397644,0.023931723146233708
4004,30900,30900,61800,98.12813019752502,0.02163328727874614
5005,38802,38802,77604,122.24070906639099,0.021135450318979565
6006,46722,46722,93444,149.71453189849854,0.019952024764279486
7007,54656,54656,109312,176.52278113365173,0.01942558198243205
8008,62520,62520,125040,202.8719141483307,0.013227093633759068
9009,70474,70474,140948,226.82937002182007,0.013088619421978365
10010,78444,78444,156888,252.5719211101532,0.013014944728638511
11011,86268,86268,172536,278.30533504486084,0.00910960692090157
12012,94212,94212,188424,303.17382621765137,0.009079115157874185
13013,102154,102154,204308,327.07973408699036,0.008891416662663687
14014,110116,110116,220232,354.2395250797272,0.0088567284947203
15015,118072,118072,236144,378.66551518440247,0.008771253462327877
16016,126014,126014,252028,402.6845588684082,0.008301757843582891
17017,134008,134008,268016,427.63274598121643,0.008296194935610401
18018,141994,141994,283988,452.1954550743103,0.00825646351040632
19019,149980,149980,299960,478.6927869319916,0.00824022644519573
20020,157980,157980,315960,508.8689911365509,0.00823686442890903
21021,165978,165978,331956,537.063001871109,0.008231528809119482
22022,173842,173842,347684,565.1250171661377,0.003059662985833711
23023,181778,181778,363556,591.4076581001282,0.0030518880776071455
24024,189766,189766,379532,623.3845510482788,0.0030502662193612196
25025,197746,197746,395492,654.3624951839447,0.003047534855795675
26026,205726,205726,411452,684.2512891292572,0.0030448771358351223
27027,213648,213648,427296,713.8214380741119,0.0029866077293263515
28028,221624,221624,443248,743.979325056076,0.002983521453643334
29029,229606,229606,459212,771.7895171642303,0.002976289730213466
30030,237598,237598,475196,795.9876282215118,0.0029756170224572998
31031,245592,245592,491184,817.7576432228088,0.0029742751776211662
32032,253566,253566,507132,842.6080420017242,0.002952171238575829
33033,261534,261534,523068,866.9546940326691,0.0029472911410266533
34034,269530,269530,539060,890.9341552257538,0.002946503491330077
35035,277450,277450,554900,913.1285500526428,0.0027701464114215923
36036,285406,285406,570812,935.3121140003204,0.0027650704632833367
37037,293398,293398,586796,957.6555359363556,0.0027645146765280515
38038,301392,301392,602784,982.9666221141815,0.002764008646408911
39039,309348,309348,618696,1006.1300270557404,0.002746056323303492
40040,317334,317334,634668,1030.9737720489502,0.0027442900300229667
41041,325330,325330,650660,1054.8438701629639,0.0027437515473138774
42042,333324,333324,666648,1080.2317471504211,0.0027417949713708367
43043,341312,341312,682624,1104.2962839603424,0.0027409733993408736
44044,349308,349308,698616,1128.6539101600647,0.0027404856937209843
45045,357286,357286,714572,1152.5920209884644,0.002666634472916485
46046,365266,365266,730532,1177.6816930770874,0.002660747422851273
47047,373258,373258,746516,1201.565187215805,0.002660300373463542
48048,381252,381252,762504,1225.7138919830322,0.0026597569940349786
49049,389248,389248,778496,1249.7344059944153,0.0026593696256895782
50050,397240,397240,794480,1276.0980360507965,0.002658844958205009
51051,405222,405222,810444,1301.758424282074,0.0026359743296779925
52052,413200,413200,826400,1327.5116219520569,0.002632535255543189
53053,421188,421188,842376,1352.4250042438507,0.0026309112363378517
54054,429174,429174,858348,1377.1334071159363,0.0026292307666153647
55055,437168,437168,874336,1399.9464468955994,0.0026283010538463714
56056,445166,445166,890332,1422.2358238697052,0.002627841902722139
57057,453162,453162,906324,1444.6103119850159,0.002627398291224381
58058,461150,461150,922300,1466.9689311981201,0.0026252891093463404
59059,469142,469142,938284,1490.849583864212,0.0026248204776493367
60060,477132,477132,954264,1514.1772480010986,0.002624125465445104
61061,485114,485114,970228,1536.1522760391235,0.002603795901450212
62062,493108,493108,986216,1560.341313123703,0.0026032918322016485
63063,500986,500986,1001972,1585.4233832359314,0.002417935987978126
64064,508964,508964,1017928,1608.239193201065,0.002414960423266166
65065,516956,516956,1033912,1632.0857031345367,0.002414373846477247
66066,524938,524938,1049876,1654.6326229572296,0.0024099243000819115
67067,532934,532934,1065868,1677.8712179660797,0.002409630435067811
68068,540924,540924,1081848,1703.0935702323914,0.0024081805549940327
69069,548900,548900,1097800,1729.0901908874512,0.00240120117632614
70070,556884,556884,1113768,1753.0372860431671,0.00240033851514454
71071,564880,564880,1129760,1777.5402040481567,0.002399970106125693
72072,572800,572800,1145600,1801.3743340969086,0.0019959337914770003
73073,580760,580760,1161520,1824.775689125061,0.001992120876820991
74074,588746,588746,1177492,1848.7652418613434,0.0019917241879738867
75075,596740,596740,1193480,1872.3026061058044,0.0019912867046514293
76076,604734,604734,1209468,1894.961818933487,0.001991030387216597
77077,612726,612726,1225452,1919.8111009597778,0.0019898096379620256
78078,620722,620722,1241444,1943.0842580795288,0.0019895689401892014
79079,628716,628716,1257432,1965.8287591934204,0.001987739306059666
80080,636710,636710,1273420,1990.144373178482,0.001987221907256753
81081,644704,644704,1289408,2013.9782040119171,0.0019867615919793025
82082,652702,652702,1305404,2037.0974140167236,0.0019864651549141854
83083,660698,660698,1321396,2060.0347430706024,0.0019862440967699513
84084,668690,668690,1337380,2083.563383102417,0.0019841727680613985
85085,676686,676686,1353372,2107.808867931366,0.001983876085432712
86086,684682,684682,1369364,2132.569904088974,0.0019835199127555825
87087,692678,692678,1385356,2157.094587087631,0.0019832608377328143
88088,700664,700664,1401328,2181.844507932663,0.001978168438654393
89089,708662,708662,1417324,2205.641222000122,0.0019779500689764973
90090,716662,716662,1433324,2229.423267841339,0.0019775579621637007
91091,724664,724664,1449328,2253.670328140259,0.001977226547751343
92092,732660,732660,1465320,2277.9142060279846,0.001976900235604262
93093,740660,740660,1481320,2301.8443660736084,0.0019761713811021764
94094,748584,748584,1497168,2326.0803599357605,0.0005695894033124205
95095,756536,756536,1513072,2354.1624541282654,0.0005692783524864353
96096,764504,764504,1529008,2377.632511138916,0.0005688375676982105
97097,772500,772500,1545000,2400.4199590682983,0.0005688203364115907
98098,780500,780500,1561000,2424.519322872162,0.0005687448556273011
99099,788502,788502,1577004,2451.025153160095,0.0005686506519850809
100100,796500,796500,1593000,2477.57874417305,0.0005686257682100404
101101,804504,804504,1609008,2504.214476108551,0.0005686202639481053
102102,812502,812502,1625004,2530.931116104126,0.0005684430834662635
103103,820506,820506,1641012,2557.4734239578247,0.0005684193947672611
104104,828512,828512,1657024,2584.210594177246,0.0005684121115336893
105105,836518,836518,1673036,2617.5389552116394,0.0005683998097083531
106106,844520,844520,1689040,2646.881462097168,0.0005682248647644883
107107,852526,852526,1705052,2675.8297820091248,0.0005682202317984775
108108,860534,860534,1721068,2703.630844116211,0.0005682188439095626
109109,868540,868540,1737080,2732.0390820503235,0.0005682114060618915
110110,876548,876548,1753096,2763.0561010837555,0.0005682100181729766
111111,884554,884554,1769108,2791.4667870998383,0.0005682048795279115
112112,892562,892562,1785124,2820.4862921237946,0.0005682034898200072
113113,900566,900566,1801132,2848.78120303154,0.0005681140737578971
114114,908570,908570,1817140,2876.8844799995422,0.0005681019192707026
115115,916578,916578,1833156,2905.012498140335,0.0005681005332007771
116116,924582,924582,1849164,2934.2260439395905,0.0005680553858837811
117117,932586,932586,1865172,2962.71617102623,0.0005680477170244558
118118,940592,940592,1881184,2992.7264568805695,0.0005680418616975658
119119,948598,948598,1897196,3021.7596759796143,0.0005680257909261854
120120,956602,956602,1913204,3052.4582240581512,0.0005678149791492615
121121,964608,964608,1929216,3082.073147058487,0.0005678122925019125
122122,972614,972614,1945228,3112.058802127838,0.0005677955214196118
123123,980622,980622,1961244,3141.5514481067657,0.0005677941353496863
124124,988630,988630,1977260,3166.665544986725,0.0005677927510987502
125125,996638,996638,1993276,3194.68412399292,0.0005677913650288247
126126,1004644,1004644,2009288,3220.6929202079773,0.0005677715653291671
127127,1012652,1012652,2025304,3246.373591184616,0.0005677701792592416
128128,1020660,1020660,2041320,3271.727741956711,0.0005677687986462843
129129,1028666,1028666,2057332,3297.027976036072,0.0005677574390574591
130130,1036674,1036674,2073348,3322.268846988678,0.000567756054806523
131131,1044680,1044680,2089360,3347.5940461158752,0.0005676971813954879
132132,1052686,1052686,2105372,3372.6982321739197,0.000567695820791414
133133,1060694,1060694,2121388,3397.84614109993,0.0005676944365404779
134134,1068700,1068700,2137400,3422.963176012039,0.0005676761647919193
135135,1076706,1076706,2153412,3447.835060119629,0.00056767405840219
136136,1084714,1084714,2169428,3474.4516801834106,0.0005676726759702433
137137,1092720,1092720,2185440,3499.1978681087494,0.0005676524342561606
138138,1100726,1100726,2201452,3523.3239572048187,0.000567645760384039
139139,1108728,1108728,2217456,3547.232848882675,0.0005674083622579928
140140,1116736,1116736,2233472,3570.8574459552765,0.0005674069780070568
141141,1124742,1124742,2249484,3596.150938987732,0.0005673942487192107
142142,1132750,1132750,2265500,3619.6438381671906,0.000567392866287264
143143,1140758,1140758,2281516,3642.6859040260315,0.0005673914856743068
144144,1148764,1148764,2297528,3666.386463165283,0.000567361872526817
145145,1156770,1156770,2313540,3689.3496820926666,0.000567358865737333
146146,1164778,1164778,2329556,3712.741259098053,0.0005673574833053863
147147,1172784,1172784,2345568,3733.976589202881,0.0005673465384461451
148148,1180792,1180792,2361584,3754.8233318328857,0.0005673451560141984
149149,1188800,1188800,2377600,3778.5467960834503,0.0005673437735822517
150150,1196804,1196804,2393608,3801.7301251888275,0.0005673123559972737
151151,1204812,1204812,2409624,3826.8367400169373,0.000567310973565327
152152,1212820,1212820,2425640,3848.095158100128,0.0005673095929523697
153153,1220826,1220826,2441652,3869.286994934082,0.0005672511288139503
154154,1228832,1228832,2457664,3891.2339441776276,0.0005672473707818426
155155,1236840,1236840,2473680,3913.3077211380005,0.0005672459901688853
156156,1244846,1244846,2489692,3936.647040128708,0.000567186421903898
157157,1252854,1252854,2505708,3958.8262951374054,0.0005671850412909407
158158,1260862,1260862,2521724,3982.6432111263275,0.000567183658858994
159159,1268868,1268868,2537736,4007.194077014923,0.0005671322978741955
160160,1276876,1276876,2553752,4027.814261198044,0.0005671309172612382
161161,1284884,1284884,2569768,4048.779294013977,0.0005671295348292915
162162,1292888,1292888,2585776,4069.826940059662,0.0005671121234627208
163163,1300896,1300896,2601792,4090.9408688545227,0.0005671107410307741
164164,1308902,1308902,2617804,4112.266324043274,0.0005670899572578492
165165,1316910,1316910,2633820,4134.589154243469,0.0005670885748259025
166166,1324916,1324916,2649832,4158.47119307518,0.000567084520298522
167167,1332924,1332924,2665848,4179.91784620285,0.0005670831415045541
168168,1340930,1340930,2681860,4201.0581929683685,0.0005670798527717125
169169,1348938,1348938,2697876,4221.712688922882,0.0005670784703397658
170170,1356942,1356942,2713884,4244.009602069855,0.0005667703007929958
171171,1364950,1364950,2729900,4266.016750097275,0.0005667689183610491
172172,1372958,1372958,2745916,4288.282329082489,0.0005667675395670813
173173,1380966,1380966,2761932,4310.413254976273,0.0005667661607731134
174174,1388974,1388974,2777948,4332.553112268448,0.0005667647801601561
175175,1396980,1396980,2793960,4354.184633016586,0.0005667526384058874
176176,1404988,1404988,2809976,4375.371755123138,0.0005667512596119195
177177,1412996,1412996,2825992,4396.3765251636505,0.0005667498789989622
178178,1421002,1421002,2842004,4418.18977689743,0.000566614111448871
179179,1429010,1429010,2858020,4440.97998714447,0.0005666127308359137
180180,1437016,1437016,2874032,4462.494589090347,0.0005666067136189668
181181,1445024,1445024,2890048,4486.635045051575,0.0005666053348249989
182182,1453030,1453030,2906060,4511.745404958725,0.0005666018769261427
183183,1461036,1461036,2922072,4534.3164529800415,0.0005665987155225594
184184,1469042,1469042,2938084,4556.850037097931,0.0005664396685460815
185185,1477050,1477050,2954100,4579.1990921497345,0.0005664382933900924
186186,1485058,1485058,2970116,4601.487809181213,0.0005664369145961246
187187,1493066,1493066,2986132,4624.48209810257,0.0005664355339831673
188188,1501070,1501070,3002140,4648.682251214981,0.0005664225136570167
189189,1509078,1509078,3018156,4672.025053977966,0.0005664211348630488
190190,1517084,1517084,3034168,4695.335026025772,0.0005662480107275769
191191,1525092,1525092,3050184,4718.503251075745,0.0005662466355715878
192192,1533100,1533100,3066200,4741.107465028763,0.0005662452567776199
193193,1541106,1541106,3082212,4763.603976011276,0.0005662399962602649
194194,1549114,1549114,3098228,4786.138295173645,0.000566238617466297
195195,1557122,1557122,3114244,4808.520071029663,0.0005662372404913185
196196,1565130,1565130,3130260,4831.007629156113,0.00056623586351634
197197,1573136,1573136,3146272,4853.614758014679,0.0005662338953698054
198198,1581132,1581132,3162264,4876.04208111763,0.0005662275161739672
199199,1589140,1589140,3178280,4901.701044082642,0.0005662261555698933
200200,1597142,1597142,3194284,4930.377199888229,0.0005662192852469161
201201,1605148,1605148,3210296,4956.6792368888855,0.0005662100138579262
202202,1613156,1613156,3226312,4980.367117166519,0.0005662086550728418
203203,1621162,1621162,3242324,5004.1297471523285,0.0005661912018695148
204204,1629170,1629170,3258340,5027.5749771595,0.0005661898394464515
205205,1637176,1637176,3274352,5051.8860721588135,0.0005661787763528991
206206,1645184,1645184,3290368,5075.889643192291,0.0005661774157488253
207207,1653192,1653192,3306384,5099.489905118942,0.0005661760551447514
208208,1661198,1661198,3322396,5124.082407951355,0.0005661677932948805
209209,1669204,1669204,3338408,5149.380733013153,0.0005660827810061164
210210,1677212,1677212,3354424,5172.20019698143,0.0005660814204020426
211211,1685220,1685220,3370440,5192.611859083176,0.0005660800579789793
212212,1693226,1693226,3386452,5213.143200159073,0.0005659485341311665
213213,1701232,1701232,3402464,5234.301270008087,0.0005659454636770533
214214,1709240,1709240,3418480,5255.361251115799,0.0005659441012539901
215215,1717244,1717244,3434488,5276.372796058655,0.0005659038288285956
216216,1725252,1725252,3450504,5297.24125123024,0.0005659024664055323
217217,1733256,1733256,3466512,5319.0141389369965,0.0005658281243086094
218218,1741264,1741264,3482528,5340.107956171036,0.0005658267637045356
219219,1749270,1749270,3498540,5361.114171028137,0.0005658240534103243
220220,1757276,1757276,3514552,5382.113888025284,0.0005658132813550765
221221,1765284,1765284,3530568,5403.02276301384,0.000565811922569992
222222,1773290,1773290,3546580,5423.978103160858,0.0005657461006194353
223223,1781298,1781298,3562596,5444.905484199524,0.0005657447400153615
224224,1789306,1789306,3578612,5465.845276117325,0.000565743381230277
225225,1797314,1797314,3594628,5488.3710770606995,0.0005657420206262032
226226,1805320,1805320,3610640,5509.84517788887,0.0005657396377500845
227227,1813326,1813326,3626652,5530.620509147644,0.000565734762858483
228228,1821334,1821334,3642668,5551.247160196304,0.0005657334040733986
229229,1829340,1829340,3658680,5571.712069988251,0.0005657140045514097
230230,1837348,1837348,3674696,5592.338613033295,0.0005657126457663253
231231,1845354,1845354,3690708,5612.901819944382,0.000565707077839761
232232,1853362,1853362,3706724,5633.5920259952545,0.0005657057190546766
233233,1861368,1861368,3722736,5654.233741044998,0.000565699026992661
234234,1869376,1869376,3738752,5674.875977039337,0.0005656976663885871
235235,1877384,1877384,3754768,5695.446798086166,0.0005656963076035026
236236,1885390,1885390,3770780,5716.10719704628,0.000565683345485013
237237,1893398,1893398,3786796,5736.778636217117,0.0005656819885189179
238238,1901404,1901404,3802808,5757.505645275116,0.0005656717330566607
239239,1909412,1909412,3818824,5778.162847995758,0.0005656703742715763
240240,1917418,1917418,3834836,5798.85259103775,0.0005656388784700539
241241,1925426,1925426,3850852,5819.507427215576,0.00056563751786598
242242,1933432,1933432,3866864,5840.096019029617,0.0005655207223753678
243243,1941438,1941438,3882876,5857.76264500618,0.0005655187833326636
244244,1949446,1949446,3898892,5879.055466175079,0.0005655174263665685
245245,1957454,1957454,3914908,5900.095008134842,0.0005655160694004735
246246,1965460,1965460,3930920,5921.498637199402,0.0005655043678416405
247247,1973468,1973468,3946936,5942.250168085098,0.000565503009056556
248248,1981474,1981474,3962948,5962.930149078369,0.0005654526994476328
249249,1989480,1989480,3978960,5983.541618108749,0.0005654494871123461
250250,1997488,1997488,3994976,6004.076382160187,0.0005654481283272617
251251,2005494,2005494,4010988,6024.742300033569,0.00056530424990342
252252,2013500,2013500,4027000,6045.443649053574,0.0005653033913404215
253253,2021506,2021506,4043012,6066.0743932724,0.0005652899872075068
254254,2029514,2029514,4059028,6086.699536085129,0.0005652886284224223
255255,2037520,2037520,4075040,6107.283169031143,0.0005652867785101989
256256,2045528,2045528,4091056,6127.9766709804535,0.0005652854215441039
257257,2053534,2053534,4107068,6148.609053134918,0.0005652444469887996
258258,2061542,2061542,4123084,6169.252559900284,0.0005652430882037152
259259,2069548,2069548,4139096,6189.855684041977,0.0005652411418850534
260260,2077554,2077554,4155108,6210.476763963699,0.0005652316049236106
261261,2085562,2085562,4171124,6231.2409591674805,0.0005652302479575155
262262,2093568,2093568,4187136,6251.942668199539,0.0005652166582876816
263263,2101576,2101576,4203152,6272.612960100174,0.0005652153013215866
264264,2109584,2109584,4219168,6293.17991900444,0.0005652139425365021
265265,2117586,2117586,4235172,6313.799061059952,0.0005651870942529058
266266,2125594,2125594,4251188,6334.42304110527,0.0005651857391058002
267267,2133602,2133602,4267204,6355.224102973938,0.0005651843803207157
268268,2141608,2141608,4283216,6375.884599208832,0.0005651778883475345
269269,2149612,2149612,4299224,6396.444129228592,0.0005651612555084284
270270,2157620,2157620,4315240,6417.06275510788,0.0005651598985423334
271271,2165628,2165628,4331256,6437.775857925415,0.0005651585433952278
272272,2173632,2173632,4347264,6458.384489059448,0.0005651420269714436
273273,2181640,2181640,4363280,6478.942873954773,0.0005651406700053485
274274,2189646,2189646,4379292,6499.599645137787,0.0005651354676956544
275275,2197654,2197654,4395308,6520.268285989761,0.0005651341107295593
276276,2205658,2205658,4411316,6540.888388872147,0.0005651022202073364
277277,2213666,2213666,4427332,6561.451878070831,0.0005651008614222519
278278,2221668,2221668,4443336,6582.071696996689,0.0005648253754770849
279279,2229676,2229676,4459352,6602.713777065277,0.0005648240203299792
280280,2237684,2237684,4475368,6623.282380104065,0.0005648226651828736
281281,2245690,2245690,4491380,6643.880268096924,0.0005647924808727112
282282,2253698,2253698,4507396,6664.731768846512,0.0005647911257256055
283283,2261704,2261704,4523408,6685.491815090179,0.00056477308862668
284284,2269712,2269712,4539424,6706.046773195267,0.0005647717316605849
285285,2277718,2277718,4555436,6726.807579040527,0.0005647648358717561
286286,2285726,2285726,4571452,6747.359434127808,0.0005647634807246504
287287,2293732,2293732,4587464,6767.980943918228,0.0005647029702231521
288288,2301740,2301740,4603480,6788.726116895676,0.0005647016150760464
289289,2309748,2309748,4619496,6809.262233972549,0.0005647002617479302
290290,2317754,2317754,4635508,6829.717559099197,0.0005646908375638304
291291,2325760,2325760,4651520,6850.236218929291,0.0005646903318847762
292292,2333768,2333768,4667536,6870.821587085724,0.00056468897855666
293293,2341772,2341772,4683544,6891.3764860630035,0.0005646302943205228
294294,2349780,2349780,4699560,6911.931612968445,0.0005646289391734172
295295,2357788,2357788,4715576,6932.420398235321,0.0005646275840263115
296296,2365794,2365794,4731588,6952.943372249603,0.0005646169120154809
297297,2373802,2373802,4747604,6973.583778142929,0.0005646155550493859
298298,2381808,2381808,4763616,6994.187992095947,0.0005645589080813807
299299,2389816,2389816,4779632,7014.749624967575,0.000564557552934275
300300,2397824,2397824,4795648,7035.394721031189,0.0005645561996061588
301301,2405830,2405830,4811660,7055.954744100571,0.0005645527908200165
302302,2413838,2413838,4827676,7076.608287096024,0.0005645514374919003
303303,2421844,2421844,4843688,7097.158687114716,0.0005645471646857914
304304,2429848,2429848,4859696,7117.787431001663,0.0005643997901643161
305305,2437856,2437856,4875712,7138.3312022686005,0.0005643984350172104
306306,2445860,2445860,4891720,7158.850932121277,0.0005643746026180452
307307,2453868,2453868,4907736,7179.4967041015625,0.0005643732492899289
308308,2461876,2461876,4923752,7200.033607959747,0.0005643718977808021
309309,2469882,2469882,4939764,7220.562490940094,0.0005643481508741388
310310,2477890,2477890,4955780,7241.159598112106,0.0005643467975460226
311311,2485896,2485896,4971792,7261.704280138016,0.0005643426102324156
312312,2493904,2493904,4987808,7282.334745168686,0.0005643412587232888
313313,2501910,2501910,5003820,7303.010097980499,0.0005643362837872701
314314,2509918,2509918,5019836,7323.838016033173,0.0005643349304591538
315315,2517924,2517924,5035848,7344.561548233032,0.0005643209678964922
316316,2525932,2525932,5051864,7365.107692241669,0.0005643196127493866
317317,2533938,2533938,5067876,7385.793061971664,0.0005642875203193398
318318,2541946,2541946,5083892,7406.547893047333,0.000564286168810213
319319,2549954,2549954,5099908,7427.2323751449585,0.0005642848136631073
320320,2557960,2557960,5115920,7447.93826508522,0.0005640449726342922
321321,2565968,2565968,5131936,7468.4375739097595,0.0005640436174871866
322322,2573976,2573976,5147952,7489.006042957306,0.0005640422659780597
323323,2581982,2581982,5163964,7509.769611120224,0.0005640337421937147
324324,2589988,2589988,5179976,7530.4888870716095,0.000564027712243842
325325,2597996,2597996,5195992,7551.274117946625,0.0005640263607347151
326326,2606002,2606002,5212004,7571.93235707283,0.0005640212493744912
327327,2614010,2614010,5228020,7592.691522121429,0.0005640198960463749
328328,2622016,2622016,5244032,7613.267067909241,0.0005640100553137017
329329,2630024,2630024,5260048,7634.0729858875275,0.0005640087019855855
330330,2638030,2638030,5276060,7654.832286119461,0.0005639983410219429
331331,2646038,2646038,5292076,7675.437909126282,0.0005639969876938267
332332,2654044,2654044,5308088,7696.011377096176,0.0005638675484078703
333333,2662050,2662050,5324100,7716.63884806633,0.0005638633429043693
334334,2670056,2670056,5340112,7737.155470132828,0.000563849611353362
335335,2678064,2678064,5356128,7757.698152065277,0.0005638482616632245
336336,2686072,2686072,5372144,7778.369131088257,0.0005638469083351083
337337,2694078,2694078,5388156,7799.153198957443,0.0005638131242449163
338338,2702086,2702086,5404172,7819.810503959656,0.0005638117727357894
339339,2710094,2710094,5420188,7840.509802103043,0.0005638104212266626
340340,2718102,2718102,5436204,7861.3307909965515,0.0005638090678985463
341341,2726108,2726108,5452216,7881.912598133087,0.0005637887588818558
342342,2734116,2734116,5468232,7902.653048992157,0.0005637874073727289
343343,2742122,2742122,5484244,7923.298772096634,0.0005636641708406387
344344,2750128,2750128,5500256,7943.902936220169,0.00056365907403233
345345,2758136,2758136,5516272,7964.612082958221,0.0005636577225232031
346346,2766144,2766144,5532288,7985.245465993881,0.0005636563728330657
347347,2774150,2774150,5548300,8005.910399198532,0.0005636216701532248
348348,2782158,2782158,5564316,8026.545550107956,0.000563620318644098
349349,2790166,2790166,5580332,8047.114464044571,0.0005636189671349712
350350,2798172,2798172,5596344,8067.856323957443,0.0005636049336317228
351351,2806180,2806180,5612360,8088.5998520851135,0.0005636035839415854
352352,2814188,2814188,5628376,8109.37863612175,0.000563602234251448
353353,2822194,2822194,5644388,8129.992166996002,0.0005635958914353978
354354,2830200,2830200,5660400,8151.099533081055,0.0005635507059196243
355355,2838208,2838208,5676416,8172.016019105911,0.0005635493525915081
356356,2846216,2846216,5692432,8192.600439071655,0.0005635480029013706
357357,2854222,2854222,5708444,8213.260824203491,0.0005635186553263338
358358,2862230,2862230,5724460,8233.959081172943,0.0005635173056361964
359359,2870236,2870236,5740472,8254.598976135254,0.0005634988156089094
360360,2878244,2878244,5756488,8275.302379131317,0.0005634974659187719
361361,2886252,2886252,5772504,8296.08767914772,0.0005634961162286345
362362,2894260,2894260,5788520,8316.829713106155,0.0005634947647195077
363363,2902266,2902266,5804532,8337.55402302742,0.0005634852404909907
364364,2910274,2910274,5820548,8358.34604024887,0.0005634838908008533
365365,2918280,2918280,5836560,8378.978207111359,0.0005634793396893656
366366,2926286,2926286,5852572,8399.710623025894,0.0005634483459289186
367367,2934294,2934294,5868588,8420.566068172455,0.0005634469962387811
368368,2942302,2942302,5884604,8441.367510080338,0.0005634456447296543
369369,2950310,2950310,5900620,8462.136611938477,0.0005634442950395169
370370,2958316,2958316,5916632,8482.926120996475,0.0005634255812765332
371371,2966324,2966324,5932648,8503.63237786293,0.0005634242315863958
372372,2974332,2974332,5948664,8524.462369203568,0.0005634228800772689
373373,2982340,2982340,5964680,8545.360725164413,0.0005634215303871315
374374,2990344,2990344,5980688,8566.049612045288,0.0005633787422993919
375375,2998350,2998350,5996700,8586.804931163788,0.0005633766613755142
376376,3006356,3006356,6012712,8607.580316066742,0.0005633724122162675
377377,3014364,3014364,6028728,8628.436479091644,0.0005633710643451195
378378,3022372,3022372,6044744,8649.100317001343,0.0005633697128359927
379379,3030378,3030378,6060756,8669.967625141144,0.0005633389264403377
380380,3038386,3038386,6076772,8690.765652179718,0.0005633375767502002
381381,3046392,3046392,6092784,8711.411629199982,0.0005633293876599055
382382,3054400,3054400,6108800,8732.146775245667,0.000563328037969768
383383,3062406,3062406,6124812,8752.920537948608,0.0005633178807329386
384384,3070414,3070414,6140828,8773.742444038391,0.0005633165328617906
385385,3078422,3078422,6156844,8794.55757021904,0.0005633151813526638
386386,3086428,3086428,6172856,8815.308266162872,0.0005633054024656303
387387,3094436,3094436,6188872,8836.163085222244,0.0005633040564134717
388388,3102442,3102442,6204884,8856.983174085617,0.0005632794618577464
389389,3110448,3110448,6220896,8877.720340013504,0.0005632806933135726
390390,3118456,3118456,6236912,8898.450602054596,0.0005632793436234351
391391,3126462,3126462,6252924,8919.286942005157,0.0005632732318190392
392392,3134466,3134466,6268932,8940.009218215942,0.0005632477495964849
393393,3142474,3142474,6284948,8960.733129024506,0.0005632464017253369
394394,3150482,3150482,6300964,8981.618305206299,0.0005632450520351995
395395,3158486,3158486,6316972,9002.373094081879,0.0005632220818370115
396396,3166492,3166492,6332984,9023.16002202034,0.0005632154679915402
397397,3174498,3174498,6348996,9043.907086133957,0.0005631703952531097
398398,3182506,3182506,6365012,9064.711126089096,0.0005631690455629723
399399,3190514,3190514,6381028,9085.560026884079,0.0005631676995108137
400400,3198518,3198518,6397036,9106.444093942642,0.0005631502826872747
401401,3206526,3206526,6413052,9127.39488697052,0.0005631489329971373
402402,3214534,3214534,6429068,9148.219474077225,0.0005631475869449787
403403,3222540,3222540,6445080,9169.052791118622,0.0005631357744277921
404404,3230548,3230548,6461096,9189.873336076736,0.000563134426556644
405405,3238556,3238556,6477112,9210.677649974823,0.000563133078685496
406406,3246562,3246562,6493124,9231.45320725441,0.00056312815650017
407407,3254566,3254566,6509132,9252.29223895073,0.0005631043877656339
408408,3262574,3262574,6525148,9273.161142110825,0.0005631030380754964
409409,3270582,3270582,6541164,9293.951397895813,0.0005631016902043484
410410,3278588,3278588,6557176,9314.948965072632,0.0005630931991618127
411411,3286594,3286594,6573188,9335.7416369915,0.0005630895375361433
412412,3294602,3294602,6589204,9356.540503263474,0.0005630881878460059
413413,3302608,3302608,6605216,9377.68516421318,0.0005630285977531457
414414,3310616,3310616,6621232,9398.469249248505,0.0005630272517009871
415415,3318624,3318624,6637248,9419.33256816864,0.0005630259020108497
416416,3326630,3326630,6653260,9440.181385040283,0.0005630067626043456
417417,3334638,3334638,6669276,9461.209028959274,0.0005630054147331975
418418,3342646,3342646,6685292,9482.25679397583,0.0005630040668620495
419419,3350652,3350652,6701304,9503.251097917557,0.0005629979350487702
420420,3358660,3358660,6717320,9524.496133089066,0.0005629965871776221
421421,3366666,3366666,6733332,9545.649058103561,0.0005629845600196859
422422,3374674,3374674,6749348,9566.84807896614,0.0005629832121485379
423423,3382680,3382680,6765360,9587.275381088257,0.0005629612405755324
424424,3390688,3390688,6781376,9606.88846898079,0.0005629598927043844
425425,3398696,3398696,6797392,9629.188691139221,0.0005629585448332364
426426,3406702,3406702,6813404,9650.551132917404,0.0005629419156321092
427427,3414710,3414710,6829420,9671.425671100616,0.0005629405677609611
428428,3422716,3422716,6845432,9692.332818031311,0.0005629380484606372
429429,3430722,3430722,6861444,9713.248514175415,0.0005629264651361154
430430,3438730,3438730,6877460,9734.209495067596,0.0005629251190839568
431431,3446738,3446738,6893476,9755.272083044052,0.0005629237693938194
432432,3454744,3454744,6909488,9776.162467241287,0.00056284603124368
433433,3462752,3462752,6925504,9797.162575006485,0.0005628446870105108
434434,3470760,3470760,6941520,9818.204169988632,0.0005628433391393628
435435,3478766,3478766,6957532,9839.193947076797,0.0005628274884657003
436436,3486774,3486774,6973548,9860.475395917892,0.0005628261424135417
437437,3494778,3494778,6989556,9881.565455913544,0.0005628192011499777
438438,3502784,3502784,7005568,9902.727405071259,0.0005628057679132326
439439,3510792,3510792,7021584,9923.626680850983,0.0005628044182230951
440440,3518798,3518798,7037596,9944.845586061478,0.0005627856589853764
441441,3526806,3526806,7053612,9966.236128091812,0.0005627843129332177
442442,3534812,3534812,7069624,9987.581003189087,0.0005627813516184688
443443,3542816,3542816,7085632,10009.205966949463,0.0005627258888125652
444444,3550824,3550824,7101648,10030.659003019333,0.0005627245427604066
445445,3558830,3558830,7117660,10052.107459068298,0.0005627026621368714
446446,3566838,3566838,7133676,10073.550169229507,0.0005627013160847127
447447,3574846,3574846,7149692,10095.043091058731,0.0005626999682135647
448448,3582852,3582852,7165704,10116.672071933746,0.0005626953006867552
449449,3590860,3590860,7181720,10138.133357048035,0.0005626939546345966
450450,3598866,3598866,7197732,10159.545530080795,0.0005626689562632237
451451,3606874,3606874,7213748,10180.990136146545,0.000562667610211065
452452,3614882,3614882,7229764,10202.479233026505,0.000562666262339917
453453,3622884,3622884,7245768,10223.95714211464,0.000562560759135522
454454,3630892,3630892,7261784,10245.500194072723,0.0005625594130833633
455455,3638898,3638898,7277796,10266.980715036392,0.0005625530575343873
456456,3646906,3646906,7293812,10288.439663887024,0.0005625517096632393
457457,3654912,3654912,7309824,10309.892590284348,0.0005625363392027793
458458,3662920,3662920,7325840,10331.451454162598,0.0005625349931506207
459459,3670926,3670926,7341852,10353.17220902443,0.0005625310113828164
460460,3678934,3678934,7357868,10374.801097154617,0.0005625296671496471
461461,3686942,3686942,7373884,10396.279328107834,0.0005625283210974885
462462,3694948,3694948,7389896,10417.805104970932,0.0005625009544019122
463463,3702956,3702956,7405912,10439.365703105927,0.0005624996065307641
464464,3710962,3710962,7421924,10460.90938091278,0.0005624982677545631
465465,3718968,3718968,7437936,10482.450543880463,0.0005621694854198722
466466,3726976,3726976,7453952,10503.938844919205,0.000562168141186703
467467,3734984,3734984,7469968,10525.445977210999,0.0005621667987725232
468468,3742990,3742990,7485980,10547.042939901352,0.0005621577292913571
469469,3750998,3750998,7501996,10568.452178001404,0.0005621563850581879
470470,3759004,3759004,7518008,10589.9208111763,0.0005621457275992725
471471,3767012,3767012,7534024,10611.417490959167,0.0005621443833661033
472472,3775020,3775020,7550040,10632.832554101944,0.0005621430409519235
473473,3783028,3783028,7566056,10654.363636016846,0.0005621416948997648
474474,3791032,3791032,7582064,10675.801774978638,0.0005621218224405311
475475,3799040,3799040,7598080,10697.082909107208,0.0005621204763883725
476476,3807048,3807048,7614096,10718.52734708786,0.0005621191339741927
477477,3815054,3815054,7630108,10739.901991128922,0.0005621008385787718
478478,3823062,3823062,7646124,10761.292985916138,0.0005620994943456026
479479,3831070,3831070,7662140,10782.89301109314,0.0005620981501124334
480480,3839076,3839076,7678152,10804.32765507698,0.0005620841984637082
481481,3847084,3847084,7694168,10825.937088012695,0.0005620828542305389
482482,3855092,3855092,7710184,10847.322094917297,0.0005620815099973697
483483,3863098,3863098,7726196,10868.60473394394,0.0005620576757792151
484484,3871104,3871104,7742208,10889.85111618042,0.0005620581723633222
485485,3879112,3879112,7758224,10911.066288948059,0.000562056828130153
486486,3887118,3887118,7774236,10932.757343053818,0.0005620480806101114
487487,3895126,3895126,7790252,10954.123821258545,0.0005620467345579527
488488,3903132,3903132,7806264,10975.496818065643,0.0005620437332254369
489489,3911140,3911140,7822280,10996.799674034119,0.0005620423908112571
490490,3919146,3919146,7838292,11018.171192884445,0.0005620392130367691
491491,3927152,3927152,7854304,11039.366791963577,0.0005618439117824892
492492,3935160,3935160,7870320,11061.052654266357,0.0005618425693683093
493493,3943168,3943168,7886336,11082.461766958237,0.0005618412269541295
494494,3951176,3951176,7902352,11103.80333185196,0.0005618398845399497
495495,3959182,3959182,7918364,11125.102840900421,0.0005617595907096984
496496,3967190,3967190,7934380,11146.527306079865,0.0005617582482955186
497497,3975196,3975196,7950392,11167.82062125206,0.0005617517672362737
498498,3983204,3983204,7966408,11189.111525058746,0.0005617504266410833
499499,3991212,3991212,7982424,11210.372292041779,0.0005617490842269035
500501,3999224,3999224,7998448,11231.841430187225,0.0005617329461529152
501502,4007232,4007232,8014464,11253.183224916458,0.0005617316037387354
502503,4015238,4015238,8030476,11274.4611389637,0.0005617260922008427
503504,4023246,4023246,8046492,11295.911082029343,0.0005617247497866629
504505,4031248,4031248,8062496,11317.11208987236,0.00056136358580261
505506,4039256,4039256,8078512,11338.40824007988,0.0005613622433884302
506507,4047264,4047264,8094528,11359.715872049332,0.0005613609009742504
507508,4055270,4055270,8110540,11381.094637155533,0.0005612913610093528
508509,4063276,4063276,8126552,11399.857031106949,0.0005612881195702357
509510,4071284,4071284,8142568,11422.287331104279,0.0005612867789750453
510511,4079290,4079290,8158580,11445.53048825264,0.0005612601053144317
511512,4087298,4087298,8174596,11468.127820253372,0.0005612587665382307
512513,4095306,4095306,8190612,11490.234763145447,0.0005612574259430403
513514,4103312,4103312,8206624,11511.510840177536,0.0005612462027784204
514515,4111320,4111320,8222640,11532.961646080017,0.0005612448640022194
515516,4119326,4119326,8238652,11554.434489011765,0.0005612417826341698
516517,4127334,4127334,8254668,11575.817409038544,0.0005612404420389794
517518,4135340,4135340,8270680,11597.093523979187,0.0005612219301838195
518519,4143348,4143348,8286696,11618.368176937103,0.0005612205877696397
519520,4151356,4151356,8302712,11639.781184196472,0.0005612192471744493
520521,4159362,4159362,8318724,11660.980385065079,0.0005611602537101135
521522,4167368,4167368,8334736,11682.427980184555,0.0005611601591226645
522523,4175376,4175376,8350752,11703.757355213165,0.0005611588167084847
523524,4183382,4183382,8366764,11725.047538995743,0.0005610773714579409
524525,4191390,4191390,8382780,11746.4162940979,0.0005610760290437611
525526,4199396,4199396,8398792,11767.747257947922,0.0005610741682176013
526527,4207404,4207404,8414808,11789.23582291603,0.0005610728312603896
527528,4215410,4215410,8430820,11810.639725208282,0.0005610107364191208
528529,4223416,4223416,8446832,11832.023885250092,0.0005610077969322447
529530,4231424,4231424,8462848,11853.264413118362,0.0005610064563370543
530531,4239430,4239430,8478860,11874.557282209396,0.0005609936251858016
531532,4247438,4247438,8494876,11895.838522911072,0.0005609922845906112
532533,4255446,4255446,8510892,11917.157343149185,0.0005609909458144102
533534,4263452,4263452,8526904,11938.521901130676,0.0005609831896435935
534535,4271460,4271460,8542920,11959.762629032135,0.0005609818508673925
535536,4279466,4279466,8558932,11981.096887111664,0.0005609771415038267
536537,4287474,4287474,8574948,12002.359333992004,0.0005609758009086363
537538,4295480,4295480,8590960,12023.681371927261,0.0005608401934296126
538539,4303488,4303488,8606976,12045.090053081512,0.0005608388546534115
539540,4311496,4311496,8622992,12066.4121260643,0.0005608375158772105
540541,4319502,4319502,8639004,12087.74651813507,0.0005607834118563915
541542,4327510,4327510,8655020,12109.199151039124,0.0005607820730801905
542543,4335518,4335518,8671036,12130.518923044205,0.000560780732485
543544,4343524,4343524,8687048,12151.864795923233,0.0005606239810731495
544545,4351532,4351532,8703064,12173.32005405426,0.0005606226441159379
545546,4359540,4359540,8719080,12194.651724100113,0.0005606213053397369
546547,4367548,4367548,8735096,12215.9110622406,0.0005606199665635359
547548,4375554,4375554,8751108,12237.210144042969,0.0005606141567113809
548549,4383562,4383562,8767124,12258.491587162018,0.0005606128197541693
549550,4391564,4391564,8783128,12279.764876127243,0.000560502587177325
550551,4399572,4399572,8799144,12301.197077035904,0.0005605012520391028
551552,4407576,4407576,8815152,12322.77767109871,0.0005603355857601855
552553,4415582,4415582,8831164,12344.07598900795,0.0005603323970717611
553554,4423588,4423588,8847176,12365.446748971939,0.0005603315257758368
554555,4431594,4431594,8863188,12386.632560968399,0.0005603237259492744
555556,4439602,4439602,8879204,12407.959826946259,0.0005603223871730734
556557,4447610,4447610,8895220,12429.299633026123,0.0005603210538538406
557558,4455616,4455616,8911232,12450.561123132706,0.0005603067202173406
558559,4463622,4463622,8927244,12471.873590230942,0.0005603043809969677
559560,4471630,4471630,8943260,12493.07649898529,0.0005603030440397561
560561,4479636,4479636,8959272,12514.45606303215,0.0005602896635537036
561562,4487642,4487642,8975284,12535.823823928833,0.0005602243272733176
562563,4495650,4495650,8991300,12557.088521003723,0.0005602229921350954
563564,4503658,4503658,9007316,12578.504533052444,0.0005602216569968732
564565,4511662,4511662,9023324,12599.887963056564,0.0005602073579211719
565566,4519670,4519670,9039340,12621.229504108429,0.0005602060227829497
566567,4527674,4527674,9055348,12642.468924045563,0.000560185140784597
567568,4535682,4535682,9071364,12663.802961111069,0.0005601838056463748
568569,4543688,4543688,9087376,12684.981273889542,0.0005601744069281267
569570,4551696,4551696,9103392,12706.424822092056,0.0005601730699709151
570571,4559702,4559702,9119404,12727.622583150864,0.0005600345721177291
571572,4567708,4567708,9135416,12749.000848054886,0.0005600328968284884
572573,4575714,4575714,9151428,12770.278100013733,0.000560030406631995
573574,4583720,4583720,9167440,12791.512635946274,0.0005600219319603639
574575,4591728,4591728,9183456,12813.001858234406,0.0005600205968221417
575576,4599736,4599736,9199472,12834.43815112114,0.0005600192616839195
576577,4607742,4607742,9215484,12855.695513248444,0.000559996122319717
577578,4615750,4615750,9231500,12877.161375045776,0.0005599947853625054
578579,4623756,4623756,9247512,12898.439366102219,0.0005599892429017927
579580,4631764,4631764,9263528,12919.802469968796,0.00055998790958256
580581,4639772,4639772,9279544,12941.164256095886,0.0005599865726253483
581582,4647778,4647778,9295556,12962.510823011398,0.0005599792875727871
582583,4655786,4655786,9311572,12983.738310098648,0.0005599779524345649
583584,4663792,4663792,9327584,13005.048226118088,0.0005599721462203888
584585,4671798,4671798,9343596,13026.253761053085,0.0005599674714176217
585586,4679806,4679806,9359612,13047.688110113144,0.0005599661362793995
586587,4687812,4687812,9375624,13069.068948030472,0.0005599290143436519
587588,4695818,4695818,9391636,13090.476264953613,0.0005599250034720171
588589,4703826,4703826,9407652,13111.884290218353,0.0005599236701527843
589590,4711832,4711832,9423664,13133.579442024231,0.0005599163068836788
590591,4719840,4719840,9439680,13154.823230028152,0.0005599149699264672
591592,4727846,4727846,9455692,13173.011266231537,0.0005597823437710758
592593,4735854,4735854,9471708,13195.591982841492,0.0005597810086328536
593594,4743862,4743862,9487724,13217.416893959045,0.0005597796734946314
594595,4751868,4751868,9503736,13238.957117080688,0.0005595965903921751
595596,4759876,4759876,9519752,13260.142861127853,0.0005595952570729423
596597,4767882,4767882,9535764,13281.372469186783,0.0005595932325377362
597598,4775890,4775890,9551780,13302.585571289062,0.0005595918992185034
598599,4783896,4783896,9567792,13323.627796173096,0.0005595660313701956
599600,4791904,4791904,9583808,13344.771263122559,0.0005595646998699522
600601,4799912,4799912,9599824,13365.790666103363,0.0005595633665507194
601602,4807916,4807916,9615832,13386.90235209465,0.0005595565053226892
602603,4815922,4815922,9631844,13407.945425987244,0.0005594964804913616
603604,4823928,4823928,9647856,13429.060635089874,0.0005594944395852508
604605,4831932,4831932,9663864,13450.309802055359,0.0005594316244241782
605606,4839940,4839940,9679880,13471.486496210098,0.0005594302911049454
606607,4847946,4847946,9695892,13492.533714056015,0.0005594078629655996
607608,4855952,4855952,9711904,13513.737240076065,0.0005594047051999951
608609,4863960,4863960,9727920,13534.873008012772,0.0005594033718807623
609610,4871968,4871968,9743936,13555.956153869629,0.0005594020403805189
610611,4879974,4879974,9759948,13576.794688224792,0.000559339521714719
611612,4887982,4887982,9775964,13597.364100933075,0.0005593381865764968
612613,4895990,4895990,9791980,13617.796627998352,0.0005593368568952428
613614,4903998,4903998,9807996,13639.44474196434,0.00055933552357601
614615,4912002,4912002,9824004,13660.816217899323,0.0005593205733021023
615616,4920008,4920008,9840016,13682.158870220184,0.0005593179866991704
616617,4928014,4928014,9856028,13703.021155834198,0.0005593026326096151
617618,4936022,4936022,9872044,13723.430058002472,0.0005593013011093717
618619,4944030,4944030,9888060,13744.030080080032,0.0005592999696091283
619620,4952036,4952036,9904072,13764.411366939545,0.0005592915767920204
620621,4960044,4960044,9920088,13784.818148851395,0.0005592902434727876
621622,4968050,4968050,9936100,13805.315579891205,0.0005592851503024576
622623,4976058,4976058,9952116,13825.75672006607,0.0005592838188022142
623624,4984064,4984064,9968128,13846.225525140762,0.0005592741217697039
624625,4992072,4992072,9984144,13866.7356569767,0.0005592727884504711
625626,5000078,5000078,10000156,13887.282598018646,0.0005592566685663769
626627,5008086,5008086,10016172,13907.662052869797,0.0005592553370661335
627628,5016092,5016092,10032184,13928.176677942276,0.0005591731678578071
628629,5024100,5024100,10048200,13948.77150797844,0.0005591718363575637
629630,5032108,5032108,10064216,13969.206111192703,0.0005591705048573203
630631,5040114,5040114,10080228,13989.659476041794,0.0005591633780568372
631632,5048122,5048122,10096244,14010.235561132431,0.0005591620483755833
632633,5056128,5056128,10112256,14030.874912023544,0.000559141280973563
633634,5064134,5064134,10128268,14051.417819023132,0.0005591419139818754
634635,5072138,5072138,10144276,14071.893651008606,0.0005591302870016079
635636,5080146,5080146,10160292,14092.565999031067,0.0005591289555013645
636637,5088152,5088152,10176304,14113.090158939362,0.0005591258868662408
637638,5096158,5096158,10192316,14133.746115207672,0.00055901591804286
638639,5104166,5104166,10208332,14154.371490240097,0.0005590145865426166
639640,5112174,5112174,10224348,14174.85908317566,0.0005590132568613626
640641,5120182,5120182,10240364,14195.509521961212,0.0005590119253611192
641642,5128188,5128188,10256376,14216.059953927994,0.0005589267384493724
642643,5136196,5136196,10272392,14236.624608039856,0.0005589254087681184
643644,5144204,5144204,10288408,14257.157771110535,0.0005589240790868644
644645,5152210,5152210,10304420,14277.805923938751,0.0005589169868471799
645646,5160218,5160218,10320436,14298.307552099228,0.000558915657165926
646647,5168224,5168224,10336448,14318.86450791359,0.0005589073480223306
647648,5176232,5176232,10352464,14339.547157049179,0.0005589060183410766
648649,5184238,5184238,10368476,14360.054161071777,0.000558821504455409
649650,5192246,5192246,10384492,14380.83562207222,0.0005588201729551656
650651,5200254,5200254,10400508,14401.305294275284,0.0005588188432739116
651652,5208260,5208260,10416520,14421.794394016266,0.0005588088934018742
652653,5216266,5216266,10432532,14442.285388231277,0.0005588071799138561
653654,5224274,5224274,10448548,14462.763463020325,0.0005588058520515915
654655,5232280,5232280,10464560,14483.345108032227,0.0005587576979451114
655656,5240284,5240284,10480568,14503.715146064758,0.0005587536106759217
656657,5248292,5248292,10496584,14524.064434051514,0.0005587522809946677
657658,5256296,5256296,10512592,14544.653272151947,0.0005587319483311148
658659,5264300,5264300,10528600,14564.991044998169,0.0005586818188021425
659660,5272306,5272306,10544612,14585.318509101868,0.0005586142233369173
660661,5280312,5280312,10560624,14605.822670221329,0.0005586097086052177
661662,5288320,5288320,10576640,14626.23633813858,0.0005586083789239638
662663,5296328,5296328,10592656,14646.641669988632,0.0005586070474237204
663664,5304334,5304334,10608668,14667.232101917267,0.0005584726241067983
664665,5312342,5312342,10624684,14687.86184501648,0.0005584712962445337
665666,5320350,5320350,10640700,14708.504195213318,0.0005584699665632797
666667,5328356,5328356,10656712,14729.133609056473,0.0005584644222835777
667668,5336364,5336364,10672728,14749.680835962296,0.0005584630944213131
668669,5344372,5344372,10688744,14770.18403506279,0.0005584617665590486
669670,5352378,5352378,10704756,14790.76926112175,0.0005584355712926481
670671,5360386,5360386,10720772,14811.249592065811,0.0005584342416113941
671672,5368394,5368394,10736788,14831.894275903702,0.0005584329137491295
672673,5376402,5376402,10752804,14852.387320280075,0.0005584315840678755
673674,5384408,5384408,10768816,14872.890808105469,0.0005584151549555827
674675,5392414,5392414,10784828,14893.598590135574,0.000558414480110514
675676,5400420,5400420,10800840,14914.273628950119,0.000558404653929756
676677,5408428,5408428,10816856,14934.915385961533,0.0005584033260674914
677678,5416434,5416434,10832868,14955.568056106567,0.0005583968541031936
678679,5424442,5424442,10848884,14976.215747117996,0.000558395526240929
679680,5432450,5432450,10864900,14996.843131065369,0.000558394196559675
680681,5440454,5440454,10880908,15017.506839036942,0.000558320931304479
681682,5448462,5448462,10896924,15038.153373003006,0.0005583196052612038
682683,5456470,5456470,10912940,15058.777483224869,0.0005583182737609604
683684,5464476,5464476,10928952,15079.273673057556,0.0005583068304986227
684685,5472484,5472484,10944968,15099.863915205002,0.0005583055026363581
685686,5480490,5480490,10960980,15120.416965007782,0.0005582861667789984
686687,5488498,5488498,10976996,15140.931945085526,0.0005582848389167339
687688,5496506,5496506,10993012,15161.523687124252,0.0005582835110544693
688689,5504512,5504512,11009024,15182.150949001312,0.0005582783851423301
689690,5512520,5512520,11025040,15203.324906110764,0.0005582770554610761
690691,5520526,5520526,11041052,15224.176483154297,0.0005582616231549764
691692,5528532,5528532,11057064,15245.336535215378,0.0005582597259490285
692693,5536538,5536538,11073076,15266.578313112259,0.0005582468911597971
693694,5544546,5544546,11089092,15287.189496278763,0.0005582455614785431
694695,5552552,5552552,11105104,15307.804573059082,0.0005582408157351892
695696,5560560,5560560,11121120,15328.451105117798,0.0005582394878729247
696697,5568564,5568564,11137128,15349.272562980652,0.0005578256241278723
697698,5576568,5576568,11153136,15369.96224117279,0.0005578205546044046
698699,5584574,5584574,11169148,15390.697673082352,0.0005578172040259233
699700,5592580,5592580,11185160,15411.396875143051,0.0005577977262873901
700701,5600588,5600588,11201176,15431.837321043015,0.0005577964002441149
701702,5608596,5608596,11217192,15452.208405017853,0.0005577950760198291
702703,5616604,5616604,11233208,15472.64096403122,0.0005577937481575646
703704,5624608,5624608,11249216,15493.12213730812,0.0005577486099355156
704705,5632616,5632616,11265232,15511.89135813713,0.0005577472838922404
705706,5640624,5640624,11281248,15527.664354085922,0.0005577459578489652
706707,5648630,5648630,11297260,15550.043952941895,0.0005577311821980402
707708,5656636,5656636,11313272,15572.780029058456,0.0005577282699960051
708709,5664644,5664644,11329288,15594.524927139282,0.0005577269457717193
709710,5672650,5672650,11345300,15615.79426407814,0.0005577057290793164
710711,5680658,5680658,11361316,15637.141057014465,0.0005577044030360412
711712,5688666,5688666,11377332,15658.492670059204,0.000557703076992766
712713,5696672,5696672,11393344,15679.889575004578,0.0005576617350016022
713714,5704680,5704680,11409360,15701.207649230957,0.0005576604107773164
714715,5712688,5712688,11425376,15722.677951097488,0.0005576590829150518
715716,5720694,5720694,11441388,15743.926876068115,0.0005576571893470827
716717,5728698,5728698,11457396,15765.298175096512,0.0005576087023655418
717718,5736706,5736706,11473412,15786.687290906906,0.0005576073799602455
718719,5744712,5744712,11489424,15808.077404022217,0.0005575991799560143
719720,5752720,5752720,11505440,15829.378722190857,0.0005575978557317285
720721,5760728,5760728,11521456,15850.593445062637,0.0005575965296884533
721722,5768732,5768732,11537464,15871.956283092499,0.0005575611903623212
722723,5776740,5776740,11553480,15893.237607002258,0.0005575598661380354
723724,5784746,5784746,11569492,15914.652022123337,0.0005575544346356764
724725,5792754,5792754,11585508,15936.113762140274,0.0005575531085924013
725726,5800760,5800760,11601520,15957.457408189774,0.0005575445993599715
726727,5808764,5808764,11617528,15978.636646986008,0.0005573916387220379
727728,5816772,5816772,11633544,15999.818164110184,0.0005573903163167415
728729,5824778,5824778,11649556,16021.066152095795,0.0005573890739469789
729730,5832786,5832786,11665572,16042.289735078812,0.0005573877497226931
730731,5840792,5840792,11681584,16063.770280122757,0.0005573384805757087
731732,5848800,5848800,11697600,16085.058717012405,0.0005573371581704123
732733,5856808,5856808,11713616,16106.349082946777,0.0005573358357651159
733734,5864814,5864814,11729628,16127.455997943878,0.0005573336766246939
734735,5872822,5872822,11745644,16148.704091072083,0.0005573323542193975
735736,5880826,5880826,11761652,16170.038275957108,0.0005573084545176243
736737,5888832,5888832,11777664,16191.165157079697,0.0005572927602770505
737738,5896840,5896840,11793680,16212.343975067139,0.0005572914378717542
738739,5904846,5904846,11809692,16233.725379228592,0.0005572555764956633
739740,5912854,5912854,11825708,16255.15961098671,0.0005572542522713775
740741,5920862,5920862,11841724,16276.287459850311,0.0005572529298660811
741742,5928870,5928870,11857740,16297.542417049408,0.0005572516056417953
742743,5936876,5936876,11873752,16318.75981593132,0.0005572379050136078
743744,5944884,5944884,11889768,16340.08085513115,0.000557236580789322
744745,5952892,5952892,11905784,16361.291890144348,0.0005572352583840257
745746,5960898,5960898,11921796,16382.568854093552,0.0005572181544266641
746747,5968906,5968906,11937812,16403.775913000107,0.0005572168320213677
747748,5976912,5976912,11953824,16424.897862911224,0.0005572154950641561
748749,5984918,5984918,11969836,16446.240364074707,0.0005571862511715153
749750,5992924,5992924,11985848,16467.395046949387,0.0005571833698923001
750751,6000932,6000932,12001864,16488.619663000107,0.0005571820474870037
751752,6008938,6008938,12017876,16509.92524600029,0.0005571706515183905
752753,6016946,6016946,12033892,16531.159344911575,0.0005571693254751153
753754,6024952,6024952,12049904,16552.459181070328,0.0005571658857661532
754755,6032958,6032958,12065916,16573.733319997787,0.0005570422745222459
755756,6040966,6040966,12081932,16594.933836221695,0.0005570409502979601
756757,6048974,6048974,12097948,16616.139981269836,0.0005570396278926637
757758,6056980,6056980,12113960,16637.46855211258,0.0005570201556110987
758759,6064988,6064988,12129976,16658.69846200943,0.0005570188332058024
759760,6072996,6072996,12145992,16679.93086218834,0.000557017510800506
760761,6081002,6081002,12162004,16701.43485403061,0.0005570089451794047
761762,6089010,6089010,12178020,16722.71132016182,0.0005570076209551189
762763,6097014,6097014,12194028,16743.90589904785,0.0005569740860664751
763764,6105022,6105022,12210044,16765.21029806137,0.0005569727618421894
764765,6113028,6113028,12226056,16786.42991709709,0.0005569682853092672
765766,6121034,6121034,12242068,16807.58034014702,0.0005569373661273858
766767,6129042,6129042,12258084,16828.621850013733,0.0005569360419031
767768,6137050,6137050,12274100,16849.77022600174,0.000556934721316793
768769,6145056,6145056,12290112,16870.798574209213,0.0005569290024141083
769770,6153064,6153064,12306128,16891.997928142548,0.0005569276818278013
770771,6161068,6161068,12322136,16913.086729049683,0.0005568466822296614
771772,6169076,6169076,12338152,16934.137411117554,0.000556845359824365
772773,6177080,6177080,12354160,16955.14033317566,0.0005568313245021272
773774,6185088,6185088,12370176,16976.122009277344,0.0005568300039158203
774775,6193096,6193096,12386192,16997.18113708496,0.0005568286815105239
775776,6201102,6201102,12402204,17018.283600091934,0.0005568140695686452
776777,6209108,6209108,12418216,17039.35489320755,0.0005568102333199931
777778,6217114,6217114,12434228,17060.447122097015,0.0005567687476286665
778779,6225122,6225122,12450244,17081.631301879883,0.0005567674270423595
779780,6233130,6233130,12466260,17102.780472278595,0.0005567661046370631
780781,6241136,6241136,12482272,17124.123250961304,0.0005567638218053617
781782,6249142,6249142,12498284,17145.56823825836,0.0005567505922954297
782783,6257150,6257150,12514300,17167.23612189293,0.0005567492717091227
783784,6265156,6265156,12530312,17188.942546129227,0.0005567328316828934
784785,6273164,6273164,12546328,17210.36348605156,0.0005567315110965865
785786,6281172,6281172,12562344,17231.495561122894,0.0005567301905102795
786787,6289178,6289178,12578356,17253.454246997833,0.0005561807029152988
787788,6297186,6297186,12594372,17274.824746131897,0.0005561793841479812
788789,6305192,6305192,12610384,17290.9161632061,0.000556177972612204
789790,6313200,6313200,12626400,17306.368052005768,0.0005561766538448865
790791,6321206,6321206,12642412,17318.491291999817,0.0005561460966418963
791792,6329214,6329214,12658428,17330.762777090073,0.0005561447778745787
792793,6337222,6337222,12674444,17343.15977191925,0.0005561434591072612
793794,6345230,6345230,12690460,17355.70130109787,0.000556142142158933
794795,6353234,6353234,12706468,17368.33209991455,0.0005561310281336773
795796,6361240,6361240,12722480,17380.62472987175,0.0005561279504036065
796797,6369248,6369248,12738496,17393.144222974777,0.0005561266334552784
797798,6377252,6377252,12754504,17405.18899011612,0.0005560983281611698
798799,6385260,6385260,12770520,17417.147152900696,0.0005560970093938522
799800,6393266,6393266,12786532,17428.829843997955,0.0005560855588555569
800801,6401274,6401274,12802548,17441.312152147293,0.0005560842419072287
801802,6409280,6409280,12818560,17453.578601121902,0.0005560763347602915
802803,6417288,6417288,12834576,17465.342890024185,0.0005560750159929739
803804,6425294,6425294,12850588,17477.726615190506,0.000556052555111819
804805,6433302,6433302,12866604,17489.924482107162,0.000556051234525512
805806,6441310,6441310,12882620,17502.24098587036,0.0005560499175771838
806807,6449316,6449316,12898632,17514.779225111008,0.0005560442805290222
807808,6457322,6457322,12914644,17526.567630290985,0.0005560371300816769
808809,6465330,6465330,12930660,17538.632921934128,0.0005560358131333487
809810,6473336,6473336,12946672,17550.340750217438,0.000555938573597814
810811,6481344,6481344,12962688,17562.344917058945,0.0005559372566494858
811812,6489350,6489350,12978700,17574.39560198784,0.0005559363526117522
812813,6497356,6497356,12994712,17586.093092918396,0.0005557765234698309
813814,6505362,6505362,13010724,17598.385416030884,0.0005557716503972188
814815,6513370,6513370,13026740,17609.8071539402,0.0005557703334488906
815816,6521376,6521376,13042752,17621.254554986954,0.0005557541226153262
816817,6529384,6529384,13058768,17632.540198087692,0.000555752805666998
817818,6537390,6537390,13074780,17643.992000102997,0.0005556050327868434
818819,6545396,6545396,13090792,17655.514099121094,0.0005556014821195276
819820,6553404,6553404,13106808,17666.969194173813,0.0005556001651711995
820821,6561410,6561410,13122820,17678.336776018143,0.000555593122044229
821822,6569418,6569418,13138836,17689.607117176056,0.0005555918050959008
822823,6577426,6577426,13154852,17701.429347276688,0.0005555904881475726
823824,6585432,6585432,13170864,17713.054222106934,0.0005555648021982051
824825,6593440,6593440,13186880,17725.06784105301,0.0005555634870688664
825826,6601446,6601446,13202892,17736.464740037918,0.0005555573989113327
826827,6609454,6609454,13218908,17748.00027823448,0.000555556083781994
827828,6617460,6617460,13234920,17759.435483932495,0.0005555396892304998
828829,6625468,6625468,13250936,17771.095196962357,0.0005555383722821716
829830,6633476,6633476,13266952,17782.587115049362,0.0005555370553338435
830831,6641482,6641482,13282964,17794.024673223495,0.0005555306852329522
831832,6649488,6649488,13298976,17805.554134130478,0.0005555217921937583
832833,6657496,6657496,13314992,17817.061470985413,0.0005555204752454301
833834,6665504,6665504,13331008,17828.58925819397,0.000555519158297102
834835,6673510,6673510,13347020,17840.115514993668,0.0005554956514970399
835836,6681518,6681518,13363036,17851.65559196472,0.0005554943345487118
836837,6689524,6689524,13379048,17863.33158302307,0.0005554920189752011
837838,6697532,6697532,13395064,17874.597514152527,0.0005554907020268729
838839,6705538,6705538,13411076,17886.416830062866,0.0005554700674110791
839840,6713546,6713546,13427092,17897.85351204872,0.0005554687504627509
840841,6721554,6721554,13443108,17909.290267944336,0.0005554674335144227
841842,6729558,6729558,13459116,17920.69682407379,0.0005554519684665138
842843,6737564,6737564,13475128,17932.125281095505,0.0005554420768021373
843844,6745570,6745570,13491140,17943.651118278503,0.0005553559785766993
844845,6753578,6753578,13507156,17955.478218078613,0.0005553546634473605
845846,6761586,6761586,13523172,17967.187999010086,0.0005553533464990323
846847,6769592,6769592,13539184,17978.539119005203,0.0005553509272431256
847848,6777600,6777600,13555200,17990.023260116577,0.0005553496102947975
848849,6785606,6785606,13571212,18001.578545093536,0.0005553253831749316
849850,6793614,6793614,13587228,18013.472353219986,0.0005553240698645823
850851,6801620,6801620,13603240,18025.187457084656,0.000555319398699794
851852,6809628,6809628,13619256,18037.04953813553,0.0005553180835704552
852853,6817634,6817634,13635268,18048.33174109459,0.0005552991678996477
853854,6825640,6825640,13651280,18059.73415827751,0.0005552950460696593
854855,6833648,6833648,13667296,18071.140693187714,0.0005552937309403205
855856,6841654,6841654,13683308,18082.99304819107,0.0005552833590627415
856857,6849662,6849662,13699324,18094.428932905197,0.0005552820439334027
857858,6857668,6857668,13715336,18105.906336069107,0.0005552659131353721
858859,6865676,6865676,13731352,18117.280122995377,0.0005552645998250227
859860,6873682,6873682,13747364,18128.769176244736,0.0005552626680582762
860861,6881688,6881688,13763376,18140.468168973923,0.0005552427519432968
861862,6889696,6889696,13779392,18152.27138018608,0.0005552414349949686
862863,6897702,6897702,13795404,18163.676030158997,0.0005552359471039381
863864,6905708,6905708,13811416,18175.03445315361,0.0005551565245696111
864865,6913716,6913716,13827432,18186.648525238037,0.0005551552112592617
865866,6921724,6921724,13843448,18198.22676205635,0.0005551538943109335
866867,6929732,6929732,13859464,18209.710942983627,0.0005551525810005842
867868,6937738,6937738,13875476,18221.229598999023,0.000555140297365142
868869,6945746,6945746,13891492,18232.629016160965,0.0005551389840547927
869870,6953754,6953754,13907508,18244.076596021652,0.0005551376707444433
870871,6961760,6961760,13923520,18255.743447065353,0.0005551226931856945
871872,6969768,6969768,13939536,18267.255923986435,0.0005551213798753452
872873,6977774,6977774,13955548,18278.814776182175,0.0005551132180698914
873874,6985782,6985782,13971564,18290.1755259037,0.0005551119047595421
874875,6993790,6993790,13987580,18301.550868988037,0.0005551105896302033
875876,7001796,7001796,14003592,18312.949996232986,0.0005550840014620917
876877,7009802,7009802,14019604,18324.33189892769,0.0005550821497308789
877878,7017810,7017810,14035620,18335.667320251465,0.0005550808346015401
878879,7025816,7025816,14051632,18347.15996813774,0.0005550562673306558
879880,7033824,7033824,14067648,18358.580141067505,0.0005550549522013171
880881,7041832,7041832,14083664,18369.973778009415,0.0005550536388909677
881882,7049838,7049838,14099676,18381.732229948044,0.0005550494042836362
882883,7057844,7057844,14115688,18393.154477119446,0.0005550029454752803
883884,7065850,7065850,14131700,18404.79231595993,0.0005550056503125234
884885,7073858,7073858,14147716,18416.112869024277,0.000555004337002174
885886,7081864,7081864,14163728,18427.44180417061,0.0005549893285206053
886887,7089872,7089872,14179744,18438.81906914711,0.0005549880133912666
887888,7097880,7097880,14195760,18450.1294028759,0.0005549867000809172
888889,7105886,7105886,14211772,18461.550096035004,0.0005549699926632456
889890,7113894,7113894,14227788,18472.976634025574,0.0005549686793528963
890891,7121898,7121898,14243796,18484.480657100677,0.0005549055749725085
891892,7129904,7129904,14259808,18496.272314071655,0.0005549030047404813
892893,7137910,7137910,14275820,18507.750138044357,0.0005548914341488853
893894,7145918,7145918,14291836,18519.427008152008,0.000554890120838536
894895,7153924,7153924,14307848,18530.766279935837,0.0005548842909774976
895896,7161932,7161932,14323864,18542.175452947617,0.0005548829776671482
896897,7169940,7169940,14339880,18553.7858440876,0.0005548816643567989
897898,7177944,7177944,14355888,18565.322286128998,0.0005548598692257656
898899,7185952,7185952,14371904,18576.96498799324,0.0005548585559154162
899900,7193958,7193958,14387916,18588.30326604843,0.0005548564386117505
900901,7201964,7201964,14403928,18599.721262931824,0.0005547118980757659
901902,7209972,7209972,14419944,18611.198255062103,0.0005547105847654166
902903,7217978,7217978,14435956,18622.538051843643,0.0005546697193494765
903904,7225986,7225986,14451972,18634.13712000847,0.0005546684060391271
904905,7233994,7233994,14467988,18646.05605697632,0.0005546670945477672
905906,7242000,7242000,14484000,18657.641555070877,0.0005546411630348302
906907,7250008,7250008,14500016,18669.035091161728,0.0005546398515434703
907908,7258016,7258016,14516032,18680.448533058167,0.0005546385382331209
908909,7266022,7266022,14532044,18691.748095035553,0.0005546292431972688
909910,7274030,7274030,14548060,18703.10394001007,0.0005546279317059088
910911,7282036,7282036,14564072,18714.562381267548,0.0005546231150219683
911912,7290044,7290044,14580088,18726.00936102867,0.0005546218035306083
912913,7298050,7298050,14596100,18737.408664226532,0.0005544441937672673
913914,7306058,7306058,14612116,18748.710274219513,0.0005544428822759073
914915,7314066,7314066,14628132,18760.027292966843,0.0005544415707845474
915916,7322072,7322072,14644144,18771.66737794876,0.0005544312261918094
916917,7330080,7330080,14660160,18783.23081088066,0.00055442991288146
917918,7338086,7338086,14676172,18794.79917407036,0.0005544277337321546
918919,7346094,7346094,14692188,18806.101351976395,0.000554426424059784
919920,7354100,7354100,14708200,18817.567160844803,0.0005544114756048657
920921,7362108,7362108,14724216,18829.009583950043,0.0005544101622945163
921922,7370112,7370112,14740224,18840.58359003067,0.0005542009512282675
922923,7378120,7378120,14756240,18852.132174253464,0.0005541996397369076
923924,7386128,7386128,14772256,18863.53776907921,0.000554198330064537
924925,7394134,7394134,14788268,18875.2746591568,0.0005541949249163736
925926,7402140,7402140,14804280,18886.684490203857,0.0005541668160731206
926927,7410148,7410148,14820296,18897.9823949337,0.0005541655045817606
927928,7418156,7418156,14836312,18909.381816148758,0.0005541641949093901
928929,7426162,7426162,14852324,18920.80085515976,0.0005541529371839715
929930,7434170,7434170,14868340,18932.307261943817,0.0005541516238736222
930931,7442176,7442176,14884352,18944.218766212463,0.0005541435748455115
931932,7450184,7450184,14900368,18956.120840072632,0.0005541422633541515
932933,7458190,7458190,14916380,18968.17236804962,0.0005541366499528522
933934,7466198,7466198,14932396,18980.121285915375,0.0005541353402804816
934935,7474206,7474206,14948412,18992.179656982422,0.0005541340306081111
935936,7482212,7482212,14964424,19004.26588511467,0.0005541155442188028
936937,7490220,7490220,14980440,19015.74630999565,0.0005541142327274429
937938,7498222,7498222,14996444,19027.233483076096,0.0005540417332667857
938939,7506230,7506230,15012460,19039.002902030945,0.0005540404254134046
939940,7514238,7514238,15028476,19050.441384077072,0.0005540391175600234
940941,7522246,7522246,15044492,19062.097890138626,0.0005540378060686635
941942,7530252,7530252,15060504,19074.526039123535,0.0005540302208828507
942943,7538258,7538258,15076516,19086.71080994606,0.0005540284637390869
943944,7546264,7546264,15092528,19098.62997317314,0.0005539775502256816
944945,7554272,7554272,15108544,19111.162976026535,0.0005539762423723005
945946,7562280,7562280,15124560,19123.267846107483,0.0005539749308809405
946947,7570286,7570286,15140572,19135.241762161255,0.0005539562553167343
947948,7578292,7578292,15156584,19147.80711889267,0.0005539556113944855
948949,7586298,7586298,15172596,19159.17620897293,0.0005538589575735386
949950,7594306,7594306,15188612,19170.257687091827,0.0005538576479011681
950951,7602314,7602314,15204628,19181.135100126266,0.0005538563364098081
951952,7610320,7610320,15220640,19191.881246089935,0.0005538536479434697
952953,7618326,7618326,15236652,19202.487357139587,0.00055383562357747
953954,7626334,7626334,15252668,19213.242748975754,0.00055383431208611
954955,7634342,7634342,15268684,19224.154766082764,0.0005538330042327289
955956,7642348,7642348,15284696,19235.64248895645,0.0005538253080885625
956957,7650356,7650356,15300712,19247.65472793579,0.0005538240002351813
957958,7658364,7658364,15316728,19259.135328054428,0.0005538226887438213
958959,7666366,7666366,15332732,19271.047002077103,0.0005537589586310787
959960,7674374,7674374,15348748,19282.187783002853,0.0005537576489587082
960961,7682382,7682382,15364764,19293.46390414238,0.000553756341105327
961962,7690388,7690388,15380776,19304.471920967102,0.0005537532833841396
962963,7698394,7698394,15396788,19315.768384218216,0.000553739821043564
963964,7706402,7706402,15412804,19326.971466064453,0.0005537385150091723
964965,7714410,7714410,15428820,19337.802368164062,0.0005537372035178123
965966,7722416,7722416,15444832,19348.767367124557,0.0005537278066185536
966967,7730424,7730424,15460848,19359.7031519413,0.000553726496946183
967968,7738430,7738430,15476860,19370.833254098892,0.0005535030431929044
968969,7746438,7746438,15492876,19381.881833076477,0.0005535017371585127
969970,7754446,7754446,15508892,19392.897832155228,0.0005535004293051315
970971,7762450,7762450,15524900,19403.873665094376,0.0005534965166589245
971972,7770458,7770458,15540916,19414.557794094086,0.0005534952088055434
972973,7778464,7778464,15556928,19425.282449007034,0.0005534352349059191
973974,7786470,7786470,15572940,19435.834894180298,0.0005534363826882327
974975,7794478,7794478,15588956,19446.47182917595,0.0005534350748348515
975976,7802486,7802486,15604972,19457.105219125748,0.0005534337669814704
976977,7810492,7810492,15620984,19467.71969103813,0.000553239964574459
977978,7818498,7818498,15636996,19478.3276822567,0.0005532365321414545
978979,7826506,7826506,15653012,19489.123991250992,0.0005532352261070628
979980,7834514,7834514,15669028,19499.799411058426,0.0005532339182536816
980981,7842520,7842520,15685040,19510.621809005737,0.0005532312861760147
981982,7850528,7850528,15701056,19521.590136051178,0.0005532299801416229
982983,7858534,7858534,15717068,19532.174680233,0.0005532146587938769
983984,7866542,7866542,15733084,19543.643908023834,0.0005532133527594851
984985,7874550,7874550,15749100,19554.463207006454,0.000553212044906104
985986,7882556,7882556,15765112,19565.257491111755,0.0005531844963115873
986987,7890564,7890564,15781128,19576.205094099045,0.0005531831902771955
987988,7898572,7898572,15797144,19587.152179002762,0.0005531818842428038
988989,7906578,7906578,15813156,19598.38582611084,0.000553135818336159
989990,7914586,7914586,15829172,19609.08522415161,0.0005531345123017672
990991,7922592,7922592,15845184,19619.979506969452,0.0005531311562663177
991992,7930600,7930600,15861200,19631.12739419937,0.000553129850231926
992993,7938606,7938606,15877212,19641.927596092224,0.0005531251881620847
993994,7946612,7946612,15893224,19653.068011045456,0.0005531082206289284
994995,7954620,7954620,15909240,19663.896962165833,0.000553106916413526
995996,7962628,7962628,15925256,19675.12880706787,0.0005531056085601449
996997,7970634,7970634,15941268,19686.151942014694,0.0005531026472453959
997998,7978640,7978640,15957280,19697.09569501877,0.00055309757226496
998999,7986646,7986646,15973292,19707.815543174744,0.0005530855705728754
1000000,7994654,7994654,15989308,19718.463359117508,0.0005530842627194943


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namea9a/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.03370094299316406,12064.709122577777
1001,3744,3744,7488,24.570235013961792,0.1510504415291507
2002,7736,7736,15472,49.48080587387085,0.013294467175001046
3003,11916,11916,23832,75.53520393371582,0.004405298595884233
4004,15908,15908,31816,101.01627397537231,0.0007309857865038794
5005,20050,20050,40100,126.56784105300903,0.0005847362608619733
6006,24640,24640,49280,154.9280309677124,0.000517089221830247
7007,29176,29176,58352,182.63866996765137,0.0005145269660715712
8008,33434,33434,66868,208.81292486190796,0.000395150447729975
9009,38974,38974,77948,241.5090959072113,0.0003945950302295387
10010,46578,46578,93156,284.647038936615,0.00039447286690119654
11011,53052,53052,106104,322.9363238811493,0.000389044846087927
12012,59502,59502,119004,362.36348605155945,0.000388112119253492
13013,64786,64786,129572,395.8347849845886,0.0003517358400131343
14014,70386,70386,140772,429.0076129436493,0.00035001113792532124
15015,78042,78042,156084,472.1558930873871,0.0003497763882478466
16016,85172,85172,170344,511.93689489364624,0.00034545769267424475
17017,91700,91700,183400,547.4451830387115,0.00034386813240416814
18018,99454,99454,198908,588.505609035492,0.00034371587753412314
19019,107258,107258,214516,631.1718430519104,0.0003436467195570003
20020,114154,114154,228308,670.3175601959229,0.00033932807309611235
21021,121984,121984,243968,712.5952031612396,0.00033928822267625947
22022,129354,129354,258708,751.2601149082184,0.00033439869548601564
23023,134600,134600,269200,781.5855128765106,0.0003256054205849068
24024,142500,142500,285000,824.2899069786072,0.0003255189149058424
25025,150388,150388,300776,865.334371805191,0.00032547817136219237
26026,157174,157174,314348,902.3457779884338,0.0003108118053205544
27027,164622,164622,329244,942.4063968658447,0.00031069875512912404
28028,172290,172290,344580,982.5411729812622,0.0003105367886746535
29029,177950,177950,355900,1016.2306320667267,0.00023654973847442307
30030,183888,183888,367776,1051.3777160644531,0.00023641393272555433
31031,191862,191862,383724,1093.8815088272095,0.0002364025785936974
32032,199852,199852,399704,1132.814083814621,0.00023639086430193856
33033,207844,207844,415688,1170.989816904068,0.00023638605125597678
34034,215842,215842,431684,1209.6943891048431,0.00023638254060642794
35035,223298,223298,446596,1246.281741142273,0.0002329058279428864
36036,231164,231164,462328,1285.2384457588196,0.0002328642876818776
37037,239160,239160,478320,1327.4551508426666,0.0002328611990378704
38038,247158,247158,494316,1372.9769008159637,0.00023285733186639845
39039,255144,255144,510288,1416.3611640930176,0.00023283911286853254
40040,263146,263146,526292,1458.8248829841614,0.00023283669361262582
41041,271146,271146,542292,1505.4257040023804,0.00023283476912183687
42042,279144,279144,558288,1548.9402058124542,0.00023283105838345364
43043,287142,287142,574284,1589.1929709911346,0.00023282845540961716
44044,295134,295134,590268,1625.5218119621277,0.00023282286019821186
45045,303130,303130,606260,1658.487459897995,0.0002328199643670814
46046,310462,310462,620924,1687.56454205513,0.0002294297555636149
47047,318432,318432,636864,1720.8271689414978,0.00022942101350054145
48048,326424,326424,652848,1755.4392981529236,0.00022941479801374953
49049,334424,334424,668848,1793.0070128440857,0.0002294119585712906
50050,342420,342420,684840,1827.5726201534271,0.00022940793678571936
51051,350410,350410,700820,1862.482922077179,0.00022940135204407852
52052,358406,358406,716812,1899.3222908973694,0.00022939711197977886
53053,366404,366404,732808,1934.7543618679047,0.0002293895886396058
54054,374400,374400,748800,1966.746001958847,0.00022938516303838696
55055,382392,382392,764784,2003.0047628879547,0.00022938034453545697
56056,390392,390392,780784,2042.3198509216309,0.00022937747780815698
57057,398390,398390,796780,2083.792552947998,0.00022937446738069411
58058,406186,406186,812372,2116.5271739959717,0.00022752280528948177
59059,413654,413654,827308,2148.911017894745,0.00022740377426089253
60060,421608,421608,843216,2184.2568259239197,0.0002273705122206593
61061,429594,429594,859188,2222.064164876938,0.00022736206483386923
62062,437580,437580,875160,2257.978492975235,0.00022735560742148664
63063,445578,445578,891156,2294.018215894699,0.00022735144193575252
64064,453568,453568,907136,2339.6987159252167,0.0002273464106110623
65065,461568,461568,923136,2380.095151901245,0.00022734387493983377
66066,469554,469554,939108,2420.5389120578766,0.00022732974139216822
67067,477548,477548,955096,2455.735311985016,0.00022732636716682464
68068,485540,485540,971080,2489.6733119487762,0.0002273211630381411
69069,493536,493536,987072,2519.494947910309,0.0002273172194691142
70070,501538,501538,1003076,2544.7791318893433,0.00022731373792339582
71071,509534,509534,1019068,2570.4060339927673,0.00022731130047759507
72072,517496,517496,1034992,2595.2097527980804,0.00022700486442772672
73073,525478,525478,1050956,2620.546282052994,0.00022699927831126843
74074,533374,533374,1066748,2645.2544469833374,0.00022683046699967235
75075,541356,541356,1082712,2671.7022149562836,0.00022682297276332974
76076,549346,549346,1098692,2697.5187599658966,0.00022681942027702462
77077,557338,557338,1114676,2722.9032320976257,0.00022681451628159266
78078,565336,565336,1130672,2751.0731978416443,0.000226808126171818
79079,573332,573332,1146664,2776.5863728523254,0.00022680457004753407
80080,581316,581316,1162632,2801.134136915207,0.00022679908761347178
81081,589120,589120,1178240,2825.9595239162445,0.00022651914332527667
82082,597108,597108,1194216,2851.0717639923096,0.00022651173640042543
83083,605034,605034,1210068,2877.315779209137,0.00022641810755885672
84084,613020,613020,1226040,2904.294902086258,0.0002264099439344136
85085,621014,621014,1242028,2930.4323511123657,0.0002264047652715817
86086,628992,628992,1257984,2955.569155931473,0.00022637344591203146
87087,636982,636982,1273964,2983.0813360214233,0.0002263388978462899
88088,644982,644982,1289964,3009.477791070938,0.00022633708613284398
89089,652980,652980,1305960,3035.3698630332947,0.00022633497428614646
90090,659988,659988,1319976,3061.910552740097,0.00021260894754959736
91091,666550,666550,1333100,3082.974928855896,0.00021252491205814295
92092,674422,674422,1348844,3106.5318768024445,0.00021248089979053475
93093,682414,682414,1364828,3132.529401779175,0.00021247828954074066
94094,690406,690406,1380812,3156.875715970993,0.00021247541735647246
95095,698382,698382,1396764,3180.883882045746,0.00021246663345664274
96096,706380,706380,1412760,3203.3221859931946,0.0002124616366927512
97097,714222,714222,1428444,3225.229383945465,0.00021225445561867673
98098,722198,722198,1444396,3247.148458003998,0.000212247727176873
99099,730180,730180,1460360,3268.9125208854675,0.0002122202695318265
100100,738176,738176,1476352,3291.2116339206696,0.00021221728457021527
101101,746172,746172,1492344,3314.845472097397,0.000212212631595321
102102,754168,754168,1508336,3339.2325451374054,0.00021220853705017362
103103,762162,762162,1524324,3361.511691093445,0.000212204729905352
104104,770160,770160,1540320,3383.2873480319977,0.00021220034250291064
105105,778158,778158,1556316,3405.085837125778,0.00021219773225311656
106106,786148,786148,1572296,3427.2405047416687,0.00021219387235760223
107107,794144,794144,1588288,3449.23069190979,0.00021218976144155022
108108,802142,802142,1604284,3470.649158000946,0.00021218616348051
109109,810146,810146,1620292,3492.6417520046234,0.0002121838078892324
110110,818132,818132,1636264,3516.1608798503876,0.00021214416301518213
111111,826124,826124,1652248,3535.0470700263977,0.00021213692889432423
112112,834118,834118,1668236,3546.9941897392273,0.00021213425679889042
113113,842114,842114,1684228,3558.896024942398,0.0002121300985891139
114114,850118,850118,1700236,3570.377990961075,0.00021212718456808943
115115,858114,858114,1716228,3581.8843977451324,0.00021212387036939617
116116,866110,866110,1732220,3593.4034729003906,0.00021211938110354822
117117,874108,874108,1748216,3604.8283970355988,0.00021211616694927216
118118,882098,882098,1764196,3616.2749099731445,0.0002121120851370506
119119,887784,887784,1775568,3625.1378738880157,0.00012878716916020494
120120,895692,895692,1791384,3636.7137200832367,0.00012876090477220714
121121,903646,903646,1807292,3648.867218017578,0.00012873057676188182
122122,911632,911632,1823264,3660.2262370586395,0.00012872759907622822
123123,919622,919622,1839244,3671.6866149902344,0.00012872150909970514
124124,927616,927616,1855232,3685.695802927017,0.00012871750732301734
125125,935616,935616,1871232,3700.687515974045,0.0001287147151742829
126126,943616,943616,1887232,3717.2433109283447,0.00012871183207607828
127127,951614,951614,1903228,3733.0330379009247,0.00012870947102783248
128128,959616,959616,1919232,3747.420691013336,0.0001287082504859427
129129,967618,967618,1935236,3762.912610054016,0.0001287063532799948
130130,975618,975618,1951236,3781.1386399269104,0.00012870479076809715
131131,983618,983618,1967236,3795.9526600837708,0.0001287015365960542
132132,991620,991620,1983240,3810.3910558223724,0.00012869987767771818
133133,999622,999622,1999244,3823.1089940071106,0.0001286979913857067
134134,1007620,1007620,2015240,3834.569680929184,0.00012869426973338705
135135,1015622,1015622,2031244,3846.331226825714,0.00012869211423094384
136136,1023620,1023620,2047240,3857.901059150696,0.00012868945304944646
137137,1031616,1031616,2063232,3869.54248714447,0.00012868628618889488
138138,1039616,1039616,2079232,3880.936819076538,0.00012868367048213258
139139,1047618,1047618,2095236,3892.4136798381805,0.00012868180419900455
140140,1055608,1055608,2111216,3903.828374147415,0.0001286555616388796
141141,1063610,1063610,2127220,3915.238378047943,0.00012865052667621057
142142,1071612,1071612,2143224,3926.7469000816345,0.00012864957716374192
143143,1079614,1079614,2159228,3938.0702180862427,0.00012864775453635957
144144,1087614,1087614,2175228,3949.3470029830933,0.00012864447853644378
145145,1095610,1095610,2191220,3960.817620038986,0.00012863859956269152
146146,1103610,1103610,2207220,3972.1446809768677,0.00012863606571045239
147147,1111612,1111612,2223224,3983.5570800304413,0.0001286321257794043
148148,1119604,1119604,2239208,3994.8636429309845,0.00012856915600423235
149149,1126932,1126932,2253864,4005.4253561496735,0.00012851599240093492
150150,1134922,1134922,2269844,4016.926246881485,0.00012851386418333277
151151,1142914,1142914,2285828,4028.1593108177185,0.00012851139763370156
152152,1150914,1150914,2301828,4039.8310449123383,0.0001285092112084385
153153,1158910,1158910,2317820,4051.3211929798126,0.00012850600433012005
154154,1166912,1166912,2333824,4062.580992937088,0.00012850409075326752
155155,1174912,1174912,2349824,4074.086574792862,0.00012850273196818307
156156,1182912,1182912,2365824,4085.668756008148,0.00012850061102653854
157157,1190910,1190910,2381820,4098.488373994827,0.0001284989557461813
158158,1198910,1198910,2397820,4110.498142004013,0.0001284961344936164
159159,1206912,1206912,2413824,4122.488536119461,0.00012849414451920893
160160,1214914,1214914,2429828,4134.26748085022,0.0001284931058762595
161161,1222916,1222916,2445832,4146.327313899994,0.00012849149788962677
162162,1230916,1230916,2461832,4158.29457783699,0.00012848852566094138
163163,1238918,1238918,2477836,4170.734170913696,0.00012848769983975217
164164,1246916,1246916,2493832,4182.645689964294,0.00012848285768995993
165165,1254920,1254920,2509840,4195.120733976364,0.00012848159531131387
166166,1262922,1262922,2525844,4207.078237056732,0.00012847992729803082
167167,1270920,1270920,2541840,4219.505419969559,0.00012847747711930424
168168,1278922,1278922,2557844,4232.2941699028015,0.00012847541256633122
169169,1286926,1286926,2573852,4244.087624073029,0.00012847403195337392
170170,1294926,1294926,2589852,4255.841005086899,0.00012846994832216296
171171,1302928,1302928,2605856,4268.012058973312,0.00012846823301515542
172172,1310928,1310928,2621856,4280.049883842468,0.00012846276331401896
173173,1318932,1318932,2637864,4291.755327939987,0.00012846141362388153
174174,1326936,1326936,2653872,4303.303432941437,0.00012846064964833204
175175,1334936,1334936,2669872,4317.851277112961,0.00012845788660342805
176176,1342938,1342938,2685876,4333.194609880447,0.00012845625133195426
177177,1350940,1350940,2701880,4346.961420059204,0.00012845458513766062
178178,1358940,1358940,2717880,4360.093638896942,0.00012845305172959343
179179,1366942,1366942,2733884,4372.969460964203,0.00012845122910221107
180180,1374944,1374944,2749888,4384.588947057724,0.00012844900811614934
181181,1382948,1382948,2765896,4396.164185762405,0.00012844756383856293
182182,1390950,1390950,2781900,4407.838757991791,0.00012844561933889054
183183,1398952,1398952,2797904,4419.305959939957,0.0001284433928958606
184184,1406956,1406956,2813912,4430.8508207798,0.00012844218690588605
185185,1414958,1414958,2829916,4442.5232310295105,0.00012844003867940046
186186,1422962,1422962,2845924,4454.0750641822815,0.00012843849071941804
187187,1430964,1430964,2861928,4465.65437912941,0.00012843712829635479
188188,1438966,1438966,2877932,4477.528153896332,0.00012843505282944534
189189,1446964,1446964,2893928,4489.243874073029,0.00012842859905504156
190190,1454966,1454966,2909932,4500.71951007843,0.0001284265108552063
191191,1462968,1462968,2925936,4512.281453847885,0.0001284246191062266
192192,1470970,1470970,2941940,4523.6219210624695,0.0001284231293539051
193193,1478970,1478970,2957940,4539.338864803314,0.0001284201534872409
194194,1486970,1486970,2973940,4554.9510180950165,0.00012841774696426
195195,1494970,1494970,2989940,4567.416013002396,0.0001284138907067245
196196,1502970,1502970,3005940,4578.896003007889,0.00012841254647355527
197197,1510968,1510968,3021936,4590.3297238349915,0.00012840982526540756
198198,1518970,1518970,3037940,4601.934168100357,0.00012840795534430072
199199,1526972,1526972,3053944,4613.60711979866,0.0001284047721128445
200200,1534974,1534974,3069948,4625.188829898834,0.00012840047202189453
201201,1542978,1542978,3085956,4637.025455951691,0.000128399897221243
202202,1550982,1550982,3101964,4648.79921579361,0.0001283980927837547
203203,1558982,1558982,3117964,4660.691928863525,0.00012839336886827368
204204,1566986,1566986,3133972,4672.444634914398,0.00012839252121921163
205205,1574988,1574988,3149976,4684.362588882446,0.00012838898328482173
206206,1582994,1582994,3165988,4696.561088085175,0.00012838817747251596
207207,1590996,1590996,3181992,4708.355170726776,0.00012838451220886782
208208,1598996,1598996,3197992,4720.089191913605,0.00012838324073527474
209209,1607000,1607000,3214000,4731.900423049927,0.00012838048860430717
210210,1615004,1615004,3230008,4743.635693788528,0.000128379275338375
211211,1623008,1623008,3246016,4755.384136915207,0.00012837714530178346
212212,1631012,1631012,3262024,4767.552789926529,0.0001283759829675546
213213,1639014,1639014,3278028,4780.019968032837,0.00012837325994041748
214214,1647018,1647018,3294036,4792.289016962051,0.0001283719320781529
215215,1655020,1655020,3310040,4804.5820479393005,0.00012837007852795068
216216,1663024,1663024,3326048,4816.9277057647705,0.00012836889436584897
217217,1671024,1671024,3342048,4829.313600063324,0.00012836713358410634
218218,1679020,1679020,3358040,4841.686496973038,0.00012836178575525992
219219,1687022,1687022,3374044,4853.968790054321,0.00012835995585191995
220220,1695026,1695026,3390052,4866.220376968384,0.000128357927678735
221221,1703028,1703028,3406056,4878.467287063599,0.000128355673950864
222222,1711032,1711032,3422064,4890.719105005264,0.0001283539259020472
223223,1719034,1719034,3438068,4903.061386108398,0.0001283519268326927
224224,1727036,1727036,3454072,4915.44403886795,0.0001283484434679849
225225,1735040,1735040,3470080,4927.763195991516,0.0001283471610804554
226226,1743038,1743038,3486076,4940.134296178818,0.00012834499284508638
227227,1751042,1751042,3502084,4952.420919179916,0.00012834359222324565
228228,1759042,1759042,3518084,4964.739177942276,0.00012834104381909128
229229,1767046,1767046,3534092,4977.020128965378,0.0001283391520701116
230230,1775048,1775048,3550096,4989.585595846176,0.00012833759319619276
231231,1783052,1783052,3566104,5002.128290176392,0.00012833604341722094
232232,1791054,1791054,3582108,5014.485070943832,0.0001283334058825858
233233,1799056,1799056,3598112,5026.758986949921,0.00012833218715968542
234234,1807056,1807056,3614112,5039.004461050034,0.0001283289948332822
235235,1815058,1815058,3630116,5051.275520086288,0.0001283269502891926
236236,1823060,1823060,3646120,5063.5558989048,0.00012832567517762072
237237,1831060,1831060,3662120,5076.000226736069,0.00012832257198169827
238238,1839062,1839062,3678124,5088.358386039734,0.00012832138236262836
239239,1847064,1847064,3694128,5100.754555940628,0.0001283196579606738
240240,1855066,1855066,3710132,5113.060527801514,0.00012831715685024392
241241,1863068,1863068,3726136,5125.411423921585,0.00012831531785195693
242242,1871066,1871066,3742132,5137.749664068222,0.0001283121218875749
243243,1879072,1879072,3758144,5150.103564977646,0.00012831120693590492
244244,1887072,1887072,3774144,5162.317451953888,0.00012830872219637968
245245,1895074,1895074,3790148,5174.580306053162,0.00012830659397877753
246246,1903076,1903076,3806152,5186.827437162399,0.00012830340710934252
247247,1911078,1911078,3822156,5199.2992651462555,0.0001283025831071427
248248,1919076,1919076,3838152,5211.683309793472,0.0001282990433537634
249249,1927078,1927078,3854156,5223.939905166626,0.00012829779552703258
250250,1935080,1935080,3870160,5236.198469877243,0.00012829625302401837
251251,1943080,1943080,3886160,5248.506452083588,0.0001282945777347777
252252,1951084,1951084,3902168,5260.841114997864,0.00012829168190364726
253253,1959086,1959086,3918172,5273.230198144913,0.00012828745457227342
254254,1967086,1967086,3934172,5285.477291107178,0.00012828490071115084
255255,1975088,1975088,3950176,5298.250988006592,0.00012828230137529317
256256,1983092,1983092,3966184,5313.202978134155,0.00012827981299778912
257257,1991096,1991096,3982192,5324.8506371974945,0.00012827758473576978
258258,1998802,1998802,3997604,5337.541549921036,0.0001252429519809084
259259,2006802,2006802,4013604,5349.650938987732,0.00012524130215751939
260260,2014802,2014802,4029604,5362.020940065384,0.00012523893201432656
261261,2022804,2022804,4045608,5374.491523981094,0.00012523654731921852
262262,2030806,2030806,4061612,5386.9840540885925,0.00012523523582785856
263263,2038812,2038812,4077624,5399.540489912033,0.0001252342826774111
264264,2046814,2046814,4093628,5412.232903003693,0.00012523234181571752
265265,2054814,2054814,4109628,5426.435230016708,0.00012522936594905332
266266,2062812,2062812,4125624,5437.735954999924,0.00012522668112069368
267267,2070814,2070814,4141628,5448.926114082336,0.00012522395445557777
268268,2078818,2078818,4157636,5460.291704893112,0.00012522278120741248
269269,2086822,2086822,4173644,5471.503994941711,0.00012522153883764986
270270,2094824,2094824,4189648,5483.1088671684265,0.00012521970165835228
271271,2102828,2102828,4205656,5495.996042966843,0.0001252185356861446
272272,2110828,2110828,4221656,5507.194375991821,0.00012521582721092273
273273,2118830,2118830,4237660,5518.6162350177765,0.00012521346434368752
274274,2126670,2126670,4253340,5530.4660930633545,0.00012521127609943505
275275,2134188,2134188,4268376,5541.6887810230255,0.0001252032943739323
276276,2142184,2142184,4284368,5554.421329975128,0.0001252005204150919
277277,2150186,2150186,4300372,5568.799757003784,0.00012519931442511734
278278,2158184,2158184,4316368,5584.357756853104,0.00012519720985437743
279279,2166184,2166184,4332368,5603.60191488266,0.00012519377196440473
280280,2174188,2174188,4348376,5621.260301113129,0.00012519061419880018
281281,2182190,2182190,4364380,5637.624014854431,0.00012518890071078204
282282,2190194,2190194,4380388,5653.164602994919,0.00012518808580352925
283283,2198192,2198192,4396384,5668.542858123779,0.0001251835928997025
284284,2206194,2206194,4412388,5683.79052400589,0.00012518140101747122
285285,2214198,2214198,4428396,5699.943472862244,0.00012517889263108373
286286,2222200,2222200,4444400,5715.262746810913,0.00012517765753727872
287287,2230204,2230204,4460408,5729.080220937729,0.00012517541290435474
288288,2238208,2238208,4476416,5740.52348279953,0.00012517447430582251
289289,2246210,2246210,4492420,5751.92795085907,0.00012517197683337145
290290,2254212,2254212,4508424,5765.444638967514,0.00012517027244030032
291291,2262214,2262214,4524428,5778.417139053345,0.00012516890274127945
292292,2270218,2270218,4540436,5791.729398012161,0.00012516760580183472
293293,2278220,2278220,4556440,5804.88260102272,0.0001251647754543228
294294,2286222,2286222,4572444,5817.881295919418,0.00012516312199295498
295295,2294224,2294224,4588448,5831.8684849739075,0.00012516165770648513
296296,2302222,2302222,4604444,5845.4414529800415,0.00012515865455497988
297297,2310224,2310224,4620448,5858.954015016556,0.0001251567136932863
298298,2318224,2318224,4636448,5872.146395921707,0.0001251538942597108
299299,2326224,2326224,4652448,5883.985730171204,0.00012515260459622368
300300,2334226,2334226,4668452,5896.1515510082245,0.00012514955415099394
301301,2342230,2342230,4684460,5908.569751024246,0.00012514847730926704
302302,2350230,2350230,4700460,5920.020653963089,0.00012514657828432973
303303,2358232,2358232,4716464,5931.856449127197,0.0001251429675903637
304304,2366236,2366236,4732472,5943.795552015305,0.00012514151785580907
305305,2374234,2374234,4748468,5955.154008865356,0.00012513777801359538
306306,2382238,2382238,4764476,5966.435963869095,0.00012513661567936651
307307,2390240,2390240,4780480,5977.806407928467,0.00012513549154391512
308308,2398240,2398240,4796480,5989.247911930084,0.0001251337926078122
309309,2406238,2406238,4812476,6000.830489873886,0.00012513072942965664
310310,2414242,2414242,4828484,6013.073851823807,0.00012512945613707416
311311,2422242,2422242,4844484,6030.538470983505,0.00012512736066128127
312312,2430246,2430246,4860492,6043.975510120392,0.0001251259836863028
313313,2438246,2438246,4876492,6056.071017980576,0.00012512305693235248
314314,2446248,2446248,4892496,6068.395761966705,0.00012512084322224837
315315,2454250,2454250,4908500,6080.677345991135,0.00012511885142885149
316316,2462252,2462252,4924504,6092.623369932175,0.00012511621753219515
317317,2470256,2470256,4940512,6104.379503965378,0.00012511513887147885
318318,2478256,2478256,4956512,6116.763386964798,0.00012511242312029935
319319,2486258,2486258,4972516,6128.660869836807,0.00012511019849625882
320320,2494260,2494260,4988520,6140.503742933273,0.00012510738451965153
321321,2502262,2502262,5004524,6152.5683851242065,0.00012510546184785198
322322,2510264,2510264,5020528,6164.5177528858185,0.00012510292617662344
323323,2518266,2518266,5036532,6176.655643939972,0.00012510113083408214
324324,2526268,2526268,5052536,6194.67565703392,0.00012509242696978617
325325,2534274,2534274,5068548,6207.944283008575,0.00012509158113971353
326326,2542278,2542278,5084556,6219.951514959335,0.00012509097177826334
327327,2550282,2550282,5100564,6231.6118631362915,0.00012508974032243714
328328,2558286,2558286,5116572,6244.47140789032,0.00012508814324974082
329329,2566290,2566290,5132580,6255.6332359313965,0.00012508656072895974
330330,2574286,2574286,5148572,6267.773761987686,0.00012508307736425195
331331,2582290,2582290,5164580,6279.043306112289,0.0001250823352165753
332332,2590294,2590294,5180588,6292.3280119895935,0.00012508080362749752
333333,2598298,2598298,5196596,6305.864173173904,0.00012507923929661047
334334,2606300,2606300,5212600,6317.9916639328,0.00012507663268479519
335335,2614304,2614304,5228608,6330.468508005142,0.0001250747955054976
336336,2622306,2622306,5244612,6342.582706928253,0.00012507328210631385
337337,2630312,2630312,5260624,6355.472275018692,0.00012507225619629025
338338,2638312,2638312,5276624,6367.330697059631,0.00012506887469498906
339339,2646314,2646314,5292628,6382.596949100494,0.0001250673994945828
340340,2654318,2654318,5308636,6398.684818029404,0.00012506577877502423
341341,2662324,2662324,5324648,6411.5422258377075,0.00012506522398325615
342342,2670328,2670328,5340656,6423.605112075806,0.00012506255006883293
343343,2678328,2678328,5356656,6435.580946922302,0.00012506103666964918
344344,2686330,2686330,5372660,6447.407645940781,0.00012505865197454114
345345,2694330,2694330,5388660,6459.097005844116,0.00012505477752711158
346346,2702334,2702334,5404668,6470.741888046265,0.00012505394806794357
347347,2710334,2710334,5420668,6482.883458137512,0.00012505177983257454
348348,2718336,2718336,5436672,6494.868124008179,0.00012504988626460545
349349,2726340,2726340,5452680,6506.836760759354,0.00012504829282988794
350350,2734342,2734342,5468684,6519.70134305954,0.00012504597725637723
351351,2742346,2742346,5484692,6530.873027086258,0.0001250444784091087
352352,2750348,2750348,5500696,6542.14056801796,0.00012504372716648504
353353,2758348,2758348,5516696,6554.865004062653,0.00012504122059908696
354354,2766352,2766352,5532704,6567.168065071106,0.00012503982725320384
355355,2774354,2774354,5548708,6580.040006875992,0.0001250366240128642
356356,2782358,2782358,5564716,6592.5682418346405,0.00012503475954872556
357357,2790358,2790358,5580716,6605.594779968262,0.00012503294783527963
358358,2798362,2798362,5596724,6618.735512018204,0.00012503089419624303
359359,2806362,2806362,5612724,6630.167984962463,0.00012502897516242228
360360,2814366,2814366,5628732,6641.644560813904,0.00012502756180765573
361361,2822368,2822368,5644736,6653.638688087463,0.00012502642857725732
362362,2830372,2830372,5660744,6665.934872150421,0.00012502485878940206
363363,2838372,2838372,5676744,6679.76530790329,0.00012502073514042422
364364,2846372,2846372,5692744,6692.8518679142,0.0001250192926818272
365365,2854372,2854372,5708744,6706.292948007584,0.00012501627315941732
366366,2862374,2862374,5724748,6719.344580888748,0.00012501433957368135
367367,2870376,2870376,5740752,6732.678937911987,0.00012501197124947794
368368,2878378,2878378,5756756,6744.900636911392,0.0001250085697392933
369369,2886382,2886382,5772764,6758.11622095108,0.0001250066125066951
370370,2894386,2894386,5788772,6770.7238709926605,0.00012500578304752707
371371,2902388,2902388,5804776,6783.242136955261,0.000125003285575076
372372,2910390,2910390,5820780,6795.534957885742,0.0001250017903657863
373373,2918392,2918392,5836784,6807.97528886795,0.00012499962031142786
374374,2926392,2926392,5852784,6819.581696033478,0.00012499638614826836
375375,2934392,2934392,5868784,6832.616817951202,0.00012499453077907674
376376,2942396,2942396,5884792,6846.03028512001,0.00012499241893237922
377377,2950400,2950400,5900800,6858.176805973053,0.00012499095646489877
378378,2958402,2958402,5916804,6870.874392747879,0.00012498800970206503
379379,2966404,2966404,5932808,6883.1028008461,0.00012498657451942563
380380,2974400,2974400,5948800,6895.187607049942,0.00012497580974013545
381381,2982406,2982406,5964812,6907.423002958298,0.0001249746019311715
382382,2990406,2990406,5980812,6920.233165740967,0.0001249716242455179
383383,2998408,2998408,5996816,6932.956657886505,0.00012497041097958572
384384,3006410,3006410,6012820,6945.411376953125,0.00012496884301071987
385385,3014410,3014410,6028820,6958.144511938095,0.00012496544695750345
386386,3022410,3022410,6044820,6970.164781808853,0.00012496349336288404
387387,3030414,3030414,6060828,6982.766247034073,0.0001249617362191202
388388,3038418,3038418,6076836,6995.960958957672,0.00012496058661781717
389389,3046418,3046418,6092836,7008.350476026535,0.00012495902956288774
390390,3054420,3054420,6108840,7020.360216140747,0.00012495722330641001
391391,3062422,3062422,6124844,7032.614036083221,0.0001249549131898675
392392,3070424,3070424,6140848,7045.47666478157,0.00012495267765189055
393393,3078428,3078428,6156856,7057.614020824432,0.00012495148075686302
394394,3086432,3086432,6172864,7070.628415107727,0.00012494985821831506
395395,3094430,3094430,6188860,7082.365241765976,0.00012494742804847192
396396,3102432,3102432,6204864,7093.864673137665,0.00012494619477365632
397397,3110436,3110436,6220872,7105.319988965988,0.00012494389011408202
398398,3118438,3118438,6236876,7116.599404096603,0.00012494318434619345
399399,3126440,3126440,6252880,7127.848965883255,0.00012494145812524948
400400,3134444,3134444,6268888,7139.223310947418,0.00012494045950006694
401401,3142444,3142444,6284888,7150.870596885681,0.00012493719441408757
402402,3150446,3150446,6300892,7162.381810903549,0.0001249357155757025
403403,3158014,3158014,6316028,7174.680063962936,0.00010959440623992123
404404,3165892,3165892,6331784,7187.240710020065,0.00010959029532386921
405405,3173892,3173892,6347784,7199.995045900345,0.00010958868369925767
406406,3181894,3181894,6363788,7212.686920881271,0.00010958656275761314
407407,3189898,3189898,6379796,7225.7264268398285,0.00010958576785924379
408408,3197900,3197900,6395800,7238.345395088196,0.0001095834668376483
409409,3205902,3205902,6411804,7251.639906167984,0.0001095811567211058
410410,3213904,3213904,6427808,7263.866077899933,0.00010957959057122935
411411,3221908,3221908,6443816,7276.611510038376,0.00010957802442135289
412412,3229912,3229912,6459824,7289.589246034622,0.00010957631820929237
413413,3237912,3237912,6475824,7301.855880975723,0.00010957275662804022
414414,3245916,3245916,6491832,7314.181037902832,0.00010957144331769086
415415,3253918,3253918,6507836,7326.046238899231,0.00010956824735330883
416416,3261920,3261920,6523840,7338.6136248111725,0.0001095664320018841
417417,3269924,3269924,6539848,7351.382882118225,0.00010956491496472154
418418,3277928,3277928,6555856,7364.3281490802765,0.00010956393271044362
419419,3285932,3285932,6571864,7376.870957136154,0.00010956302685372066
420420,3293934,3293934,6587868,7389.599715948105,0.00010956184632959776
421421,3301936,3301936,6603872,7402.2928919792175,0.00010955993820971344
422422,3309936,3309936,6619872,7415.195160865784,0.00010955756988551002
423423,3317938,3317938,6635876,7426.832075119019,0.00010955580728477798
424424,3325940,3325940,6651880,7439.722184896469,0.00010955433754133992
425425,3333942,3333942,6667884,7452.085119962692,0.00010955214202112984
426426,3341946,3341946,6683892,7465.505810022354,0.00010955067227769177
427427,3349950,3349950,6699900,7479.051707983017,0.00010954901517834514
428428,3357952,3357952,6715904,7490.9896059036255,0.0001095470433938317
429429,3365956,3365956,6731912,7503.865708112717,0.00010954557183140423
430430,3373960,3373960,6747920,7516.778349876404,0.00010954450226563495
431431,3381964,3381964,6763928,7529.343622922897,0.0001095436546165729
432432,3389968,3389968,6779936,7542.358554840088,0.00010954241588478908
433433,3397964,3397964,6795928,7554.412557125092,0.0001095399657060625
434434,3405968,3405968,6811936,7566.601452112198,0.00010953826676995959
435435,3413966,3413966,6827932,7579.318102121353,0.00010953491255349945
436436,3421968,3421968,6843936,7592.3171210289,0.00010953338824037928
437437,3429970,3429970,6859940,7604.620557069778,0.0001095318602892803
438438,3437972,3437972,6875944,7616.636275053024,0.00010953029959637206
439439,3445976,3445976,6891952,7628.108855009079,0.00010952836055366788
440440,3453976,3453976,6907952,7641.320461034775,0.00010952650336548686
441441,3461982,3461982,6923964,7654.079284906387,0.0001095262668968644
442442,3469966,3469966,6939932,7665.964652061462,0.00010952610136882868
443443,3477802,3477802,6955604,7678.510760068893,0.00010952576849376783
444444,3484800,3484800,6969600,7689.956108093262,9.331427827419247e-05
445445,3492780,3492780,6985560,7702.12292098999,9.33101346163312e-05
446446,3500766,3500766,7001532,7715.421035051346,9.330525426776148e-05
447447,3508758,3508758,7017516,7727.2190709114075,9.329622844234109e-05
448448,3516758,3516758,7033516,7739.302773952484,9.329357999376953e-05
449449,3524142,3524142,7048284,7751.205189943314,9.32848433876643e-05
450450,3531926,3531926,7063852,7763.112648010254,9.327789848612156e-05
451451,3539908,3539908,7079816,7776.368840932846,9.327565021521877e-05
452452,3547898,3547898,7095796,7788.299333810806,9.326638246420771e-05
453453,3555896,3555896,7111792,7800.243298768997,9.326481267635245e-05
454454,3563896,3563896,7127792,7812.622358083725,9.32636085053673e-05
455455,3571894,3571894,7143788,7824.803128004074,9.326185136160348e-05
456456,3579894,3579894,7159788,7838.015746116638,9.325787141278852e-05
457457,3587890,3587890,7175780,7851.329700946808,9.325564133177977e-05
458458,3595890,3595890,7191780,7864.760426998138,9.325376413471531e-05
459459,3603892,3603892,7207784,7877.570760011673,9.32511902647093e-05
460460,3611890,3611890,7223780,7889.782081127167,9.324963684775867e-05
461461,3619892,3619892,7239784,7902.575755119324,9.324804705101997e-05
462462,3627896,3627896,7255792,7915.021718978882,9.32469865801977e-05
463463,3635898,3635898,7271796,7927.207176923752,9.324567508883774e-05
464464,3643898,3643898,7287796,7939.758256912231,9.324465463578235e-05
465465,3651900,3651900,7303800,7953.7641248703,9.324337588623166e-05
466466,3659904,3659904,7319808,7965.389960050583,9.324146776634734e-05
467467,3667906,3667906,7335812,7976.912811040878,9.323909216618631e-05
468468,3675910,3675910,7351820,7988.763071060181,9.323812810180243e-05
469469,3683914,3683914,7367828,8000.462677001953,9.323732410848606e-05
470470,3691916,3691916,7383832,8012.727912902832,9.323614722234197e-05
471471,3699920,3699920,7399840,8024.564216852188,9.32351886149263e-05
472472,3707922,3707922,7415844,8036.464766025543,9.323424819740467e-05
473473,3715926,3715926,7431852,8048.344675779343,9.32328257476911e-05
474474,3723928,3723928,7447856,8060.349511861801,9.323191443399992e-05
475475,3731932,3731932,7463864,8072.104546070099,9.323110498371534e-05
476476,3739936,3739936,7479872,8083.538738965988,9.322996265836991e-05
477477,3747936,3747936,7495872,8095.040255069733,9.322870755568147e-05
478478,3755936,3755936,7511872,8106.432404994965,9.322444202553015e-05
479479,3763940,3763940,7527880,8118.080888748169,9.322333426098339e-05
480480,3771946,3771946,7543892,8129.671411991119,9.322275764134247e-05
481481,3779948,3779948,7559896,8141.188038825989,9.322082951257471e-05
482482,3787952,3787952,7575904,8152.7881190776825,9.321957440988626e-05
483483,3795956,3795956,7591912,8164.237859964371,9.321847028331831e-05
484484,3803958,3803958,7607916,8175.593590974808,9.321612560597714e-05
485485,3811962,3811962,7623924,8187.124344110489,9.321563265984878e-05
486486,3819966,3819966,7639932,8200.554944992065,9.321493234892841e-05
487487,3827970,3827970,7655940,8213.730453968048,9.321399011241738e-05
488488,3835954,3835954,7671908,8227.371016979218,9.310379755333997e-05
489489,3843956,3843956,7687912,8239.517596960068,9.310275527241174e-05
490490,3851960,3851960,7703920,8251.235055923462,9.310152199759614e-05
491491,3859962,3859962,7719924,8262.69276189804,9.309989945904817e-05
492492,3867964,3867964,7735928,8275.806792974472,9.309884080721531e-05
493493,3875966,3875966,7751932,8288.074819803238,9.309794404543936e-05
494494,3883970,3883970,7767940,8300.369486808777,9.309297638537828e-05
495495,3891974,3891974,7783948,8312.145826101303,9.309220513387118e-05
496496,3899974,3899974,7799948,8326.291639089584,9.309015695180278e-05
497497,3907980,3907980,7815960,8338.73748087883,9.308921653428115e-05
498498,3915982,3915982,7831964,8350.725409030914,9.308669541496783e-05
499499,3923988,3923988,7847976,8362.926189899445,9.308609696745407e-05
500501,3931996,3931996,7863992,8375.878509759903,9.30839050852228e-05
501502,3939998,3939998,7879996,8389.091576099396,9.308329936175141e-05
502503,3948000,3948000,7896000,8401.820761919022,9.308116386819165e-05
503504,3956002,3956002,7912004,8414.116397857666,9.307700020144694e-05
504505,3964006,3964006,7928012,8426.638839006424,9.307589425588958e-05
505506,3972008,3972008,7944016,8438.018276929855,9.307480468123686e-05
506507,3980014,3980014,7960028,8449.595999956131,9.307383334089536e-05
507508,3988018,3988018,7976036,8461.069015979767,9.307281834480818e-05
508509,3996018,3996018,7992036,8472.493729114532,9.307177606387995e-05
509510,4004022,4004022,8008044,8484.18180513382,9.306993160862476e-05
510511,4012024,4012024,8024048,8495.849211931229,9.306932588515338e-05
511512,4020026,4020026,8040052,8507.608264923096,9.306861284130719e-05
512513,4028028,4028028,8056056,8520.143522024155,9.306618812843226e-05
513514,4036034,4036034,8072068,8531.95577287674,9.306608444603626e-05
514515,4044038,4044038,8088076,8544.568274021149,9.306440006184857e-05
515516,4052042,4052042,8104084,8556.474166154861,9.30635433178395e-05
516517,4060046,4060046,8120092,8568.518056869507,9.306250649387948e-05
517518,4068046,4068046,8136092,8580.012729883194,9.305941784987226e-05
518519,4076048,4076048,8152096,8592.345742940903,9.305717321694829e-05
519520,4084048,4084048,8168096,8604.35098695755,9.305583444074728e-05
520521,4092052,4092052,8184104,8617.085340976715,9.305496314482298e-05
521522,4100058,4100058,8200116,8628.92749118805,9.305354979005642e-05
522523,4108062,4108062,8216124,8640.487235069275,9.305300045525655e-05
523524,4116064,4116064,8232128,8652.296590805054,9.305216553912032e-05
524525,4124070,4124070,8248140,8664.14608001709,9.305135063186754e-05
525526,4132072,4132072,8264144,8676.16763496399,9.304971354140434e-05
526527,4140076,4140076,8280152,8690.493170976639,9.30482037801994e-05
527528,4148078,4148078,8296156,8702.46970295906,9.304621016781311e-05
528529,4156084,4156084,8312168,8715.192216157913,9.304567902290728e-05
529530,4164086,4164086,8328172,8727.687076807022,9.304438754043076e-05
530531,4172088,4172088,8344176,8738.781017780304,9.304236846219283e-05
531532,4180092,4180092,8360184,8750.087146043777,9.303996193921193e-05
532533,4188094,4188094,8376188,8761.90893793106,9.303955812356435e-05
533534,4196094,4196094,8392188,8773.515941858292,9.303741353505757e-05
534535,4204096,4204096,8408192,8785.30028295517,9.303617844125256e-05
535536,4212100,4212100,8424200,8797.418647050858,9.303465230914298e-05
536537,4220102,4220102,8440204,8809.02745294571,9.303359183832072e-05
537538,4228106,4228106,8456212,8820.906100034714,9.303246770286933e-05
538539,4236106,4236106,8472212,8832.24810910225,9.303154911322054e-05
539540,4244108,4244108,8488216,8844.100095033646,9.303028491558507e-05
540541,4252110,4252110,8504220,8855.823643922806,9.30292753764661e-05
541542,4260114,4260114,8520228,8867.317800998688,9.302834041591268e-05
542543,4268118,4268118,8536236,8879.337297916412,9.302734542870894e-05
543544,4276118,4276118,8552236,8892.006641864777,9.302567195845768e-05
544545,4284122,4284122,8568244,8903.657879114151,9.302274156652857e-05
545546,4292126,4292126,8584252,8915.200784921646,9.302154285251163e-05
546547,4300128,4300128,8600256,8927.12379693985,9.302033868152648e-05
547548,4308134,4308134,8616268,8939.898137807846,9.30199385038577e-05
548549,4316138,4316138,8632276,8952.366358995438,9.301948921347503e-05
549550,4324140,4324140,8648280,8964.040583848953,9.301753743784502e-05
550551,4332144,4332144,8664288,8975.338287830353,9.301594946009573e-05
551552,4340146,4340146,8680292,8986.493261814117,9.301428508479148e-05
552553,4348150,4348150,8696300,8997.917036056519,9.301300269726198e-05
553554,4356150,4356150,8712300,9009.360985994339,9.301067984779365e-05
554555,4364154,4364154,8728308,9021.158399105072,9.300997589889448e-05
555556,4372156,4372156,8744312,9032.728719949722,9.300760575570166e-05
556557,4380158,4380158,8760316,9044.252444982529,9.300633792008739e-05
557558,4388162,4388162,8776324,9055.62809920311,9.300486635765992e-05
558559,4396164,4396164,8792328,9069.715762853622,9.300371857534628e-05
559560,4404168,4404168,8808336,9083.132019996643,9.299959492636845e-05
560561,4412172,4412172,8824344,9097.204033136368,9.299864359491039e-05
561562,4420176,4420176,8840352,9108.964668989182,9.299753401137423e-05
562563,4428178,4428178,8856356,9120.870739936829,9.2996802777634e-05
563564,4436178,4436178,8872356,9132.944772958755,9.299369776272215e-05
564565,4444180,4444180,8888360,9147.402414798737,9.299247722083237e-05
565566,4452184,4452184,8904368,9159.865628004074,9.299191151512787e-05
566567,4460184,4460184,8920368,9172.669539928436,9.297786527895369e-05
567568,4468184,4468184,8936368,9184.846221923828,9.297553879150655e-05
568569,4476188,4476188,8952376,9197.15489578247,9.297444012190681e-05
569570,4484194,4484194,8968388,9209.215960741043,9.297396718466189e-05
570571,4492196,4492196,8984392,9222.009803056717,9.297277574660257e-05
571572,4500202,4500202,9000404,9233.969883918762,9.29715133679565e-05
572573,4507662,4507662,9015324,9245.714777946472,4.8176270865951665e-05
573574,4515622,4515622,9031244,9257.929999828339,4.817403714696411e-05
574575,4523616,4523616,9047232,9270.128941059113,4.8172505557886325e-05
575576,4531614,4531614,9063228,9282.448985815048,4.817110311705619e-05
576577,4539616,4539616,9079232,9294.967912912369,4.816964974452276e-05
577578,4547620,4547620,9095240,9307.761698007584,4.8168838475248776e-05
578579,4555622,4555622,9111244,9319.646728038788,4.816767614101991e-05
579580,4563626,4563626,9127252,9332.970612049103,4.816683940589428e-05
580581,4571628,4571628,9143256,9345.460038900375,4.816522778128274e-05
581582,4579628,4579628,9159256,9358.031720876694,4.8164056352106854e-05
582583,4587630,4587630,9175260,9371.18741106987,4.816251566808205e-05
583584,4595636,4595636,9191272,9383.659312009811,4.816140790353529e-05
584585,4603638,4603638,9207276,9396.575572013855,4.815865213458892e-05
585586,4611642,4611642,9223284,9407.89815402031,4.8157737182918936e-05
586587,4619648,4619648,9239296,9419.292406082153,4.8157342462218367e-05
587588,4627654,4627654,9255308,9430.898927927017,4.8155725380638614e-05
588589,4635656,4635656,9271312,9442.289084911346,4.815300417249091e-05
589590,4643660,4643660,9287320,9454.825087070465,4.8152247472899035e-05
590591,4651662,4651662,9303324,9466.337843894958,4.815159445570316e-05
591592,4659664,4659664,9319328,9478.207419872284,4.815058127860539e-05
592593,4667666,4667666,9335332,9490.523386955261,4.814886415260844e-05
593594,4675672,4675672,9351344,9502.565751075745,4.814832027477678e-05
594595,4683676,4683676,9367352,9514.53267788887,4.814743260794785e-05
595596,4691682,4691682,9383364,9526.580249786377,4.814589919988066e-05
596597,4699686,4699686,9399372,9538.920305013657,4.8144234824576415e-05
597598,4707694,4707694,9415388,9551.408746957779,4.8144111133296974e-05
598599,4715698,4715698,9431396,9564.133141040802,4.814279418496881e-05
599600,4723704,4723704,9447408,9577.139149188995,4.814233579963911e-05
600601,4731710,4731710,9463420,9589.55125784874,4.814201020053588e-05
601602,4739712,4739712,9479424,9602.02046585083,4.813949271920137e-05
602603,4747718,4747718,9495436,9615.50515294075,4.813863961317111e-05
603604,4755720,4755720,9511440,9628.117332935333,4.813809209736064e-05
604605,4763724,4763724,9527448,9641.702644109726,4.813597479369491e-05
605606,4771730,4771730,9543460,9654.045153141022,4.813275700144004e-05
606607,4779736,4779736,9559472,9666.422271966934,4.813237137568649e-05
607608,4787742,4787742,9575484,9678.515363931656,4.8131882067536935e-05
608609,4795748,4795748,9591496,9691.074465990067,4.813087980437558e-05
609610,4803750,4803750,9607500,9703.952887058258,4.812935549125541e-05
610611,4811756,4811756,9623512,9716.62767291069,4.8128655180335045e-05
611612,4819760,4819760,9639520,9728.967235088348,4.812797124031931e-05
612613,4827762,4827762,9655524,9742.684159994125,4.812401130038779e-05
613614,4835768,4835768,9671536,9754.84210896492,4.812340921489522e-05
614615,4843774,4843774,9687548,9766.688544988632,4.811994222109206e-05
615616,4851780,4851780,9703560,9779.015278816223,4.811945836991072e-05
616617,4859782,4859782,9719564,9791.074779987335,4.8117841288330965e-05
617618,4867786,4867786,9735572,9804.311798095703,4.8113819502759725e-05
618619,4875792,4875792,9751584,9815.737643957138,4.811343751498498e-05
619620,4883792,4883792,9767584,9827.515342950821,4.8111623982549645e-05
620621,4891796,4891796,9783592,9840.064710855484,4.811002690985333e-05
621622,4899800,4899800,9799600,9853.050737857819,4.8109664930962026e-05
622623,4907804,4907804,9815608,9867.77434706688,4.8107935072039254e-05
623624,4915808,4915808,9831616,9880.79858994484,4.810676728084218e-05
624625,4923812,4923812,9847624,9894.015525817871,4.810495192941744e-05
625626,4931816,4931816,9863632,9908.20220899582,4.8103775043273345e-05
626627,4939820,4939820,9879640,9921.329432964325,4.8100841013365425e-05
627628,4947824,4947824,9895648,9933.83042883873,4.810060818272177e-05
628629,4955826,4955826,9911652,9947.765688180923,4.809844176634215e-05
629630,4963832,4963832,9927664,9959.724628925323,4.809497477253899e-05
630631,4971838,4971838,9943676,9971.735690116882,4.809445090359077e-05
631632,4979842,4979842,9959684,9984.18023610115,4.809403617400676e-05
632633,4987846,4987846,9975692,9997.60100197792,4.809228266822174e-05
633634,4995854,4995854,9991708,10010.004081010818,4.809216261492111e-05
634635,5003856,5003856,10007712,10022.337241888046,4.809085112356115e-05
635636,5011860,5011860,10023720,10034.962509155273,4.809022539120633e-05
636637,5019862,5019862,10039724,10049.69403386116,4.808710036741104e-05
637638,5027868,5027868,10055736,10062.690940856934,4.8084830268635415e-05
638639,5035870,5035870,10071740,10076.460229873657,4.80836442875443e-05
639640,5043874,5043874,10087748,10090.313735961914,4.808209814655129e-05
640641,5051880,5051880,10103760,10103.056557178497,4.808185622096062e-05
641642,5059884,5059884,10119768,10114.799787044525,4.808013000001665e-05
642643,5067884,5067884,10135768,10127.604351043701,4.80788221466355e-05
643644,5075890,5075890,10151780,10139.585155963898,4.80761009384878e-05
644645,5083894,5083894,10167788,10151.546803951263,4.807567711395677e-05
645646,5091896,5091896,10183792,10165.186940908432,4.807386903848965e-05
646647,5099902,5099902,10199804,10177.915655851364,4.807206641999073e-05
647648,5107906,5107906,10215812,10190.212120056152,4.807131517736707e-05
648649,5115908,5115908,10231816,10202.41528391838,4.8069732656585984e-05
649650,5123914,5123914,10247828,10213.978256940842,4.806924880540464e-05
650651,5131916,5131916,10263832,10225.440024852753,4.8067071475088596e-05
651652,5139920,5139920,10279840,10237.002223968506,4.8066367526189424e-05
652653,5147926,5147926,10295852,10248.948096036911,4.8065865485114045e-05
653654,5155930,5155930,10311860,10260.54241681099,4.806418473890517e-05
654655,5163932,5163932,10327864,10272.007558822632,4.8060643166536465e-05
655656,5171938,5171938,10343876,10283.404302835464,4.8057723688543774e-05
656657,5179946,5179946,10359892,10295.13494515419,4.805759817827493e-05
657658,5187948,5187948,10375896,10306.85745382309,4.805463686352596e-05
658659,5195954,5195954,10391908,10318.169606924057,4.8054133003461175e-05
659660,5203960,5203960,10407920,10329.642491817474,4.8050973418867216e-05
660661,5211964,5211964,10423928,10342.053047180176,4.805018215847667e-05
661662,5219970,5219970,10439940,10355.102109909058,4.804994932783302e-05
662663,5227972,5227972,10455944,10368.625874042511,4.8049361794255674e-05
663664,5235242,5235242,10470484,10380.006292104721,4.785737291967962e-05
664665,5243236,5243236,10486472,10392.492612838745,4.785667078976985e-05
665666,5251238,5251238,10502476,10405.086639881134,4.785606142831966e-05
666667,5259236,5259236,10518472,10416.587924957275,4.785514647664968e-05
667668,5267240,5267240,10534480,10428.32358288765,4.785450983035844e-05
668669,5275240,5275240,10550480,10440.38830280304,4.785342389368452e-05
669670,5283246,5283246,10566492,10453.45567893982,4.785311466548592e-05
670671,5291250,5291250,10582500,10466.931813955307,4.7851886847638525e-05
671672,5299254,5299254,10598508,10479.614068984985,4.78517195006134e-05
672673,5307258,5307258,10614516,10491.78339099884,4.785102646565065e-05
673674,5315260,5315260,10630520,10504.245143175125,4.784829434356652e-05
674675,5323262,5323262,10646524,10516.511357069016,4.784764860232826e-05
675676,5331266,5331266,10662532,10528.734397888184,4.784660632140003e-05
676677,5339268,5339268,10678536,10541.593277931213,4.784544580616057e-05
677678,5347274,5347274,10694548,10554.355508089066,4.784531301993411e-05
678679,5355278,5355278,10710556,10566.836457967758,4.784456905326806e-05
679680,5363284,5363284,10726568,10579.287019968033,4.78439233120298e-05
680681,5371290,5371290,10742580,10592.574565887451,4.784359589393716e-05
681682,5379296,5379296,10758592,10605.007993936539,4.7842228013905697e-05
682683,5387302,5387302,10774604,10618.326171875,4.7841929699643515e-05
683684,5395304,5395304,10790608,10630.940546989441,4.784082921105437e-05
684685,5403310,5403310,10806620,10644.06333398819,4.784042903338559e-05
685686,5411312,5411312,10822624,10656.065248012543,4.783993608725723e-05
686687,5419316,5419316,10838632,10668.493372917175,4.7838564569246955e-05
687688,5427320,5427320,10854640,10680.878556013107,4.7837775127845816e-05
688689,5435322,5435322,10870644,10693.317858934402,4.7837056627031416e-05
689690,5443324,5443324,10886648,10705.729650974274,4.783639087690972e-05
690691,5451326,5451326,10902652,10719.116044044495,4.783586518897209e-05
691692,5459330,5459330,10918660,10732.285477876663,4.7835399527684785e-05
692693,5467332,5467332,10934664,10744.91076207161,4.7833829739829525e-05
693694,5475336,5475336,10950672,10757.913442850113,4.783312397194095e-05
694695,5483342,5483342,10966684,10769.572745084763,4.7832767450017855e-05
695696,5491348,5491348,10982696,10781.531282901764,4.783236545335967e-05
696697,5499352,5499352,10998704,10793.63192820549,4.78317124361638e-05
697698,5507356,5507356,11014712,10806.358540058136,4.783075019076932e-05
698699,5515362,5515362,11030724,10818.911438941956,4.78303281852277e-05
699700,5523364,5523364,11046728,10832.092458963394,4.782959513249807e-05
700701,5531368,5531368,11062736,10845.898658752441,4.782903124578297e-05
701702,5539372,5539372,11078744,10860.12159705162,4.782723954122048e-05
702703,5547374,5547374,11094748,10872.064903974533,4.782674295711331e-05
703704,5555380,5555380,11110760,10884.715074062347,4.782627001986839e-05
704705,5563384,5563384,11126768,10896.848695993423,4.782577889272943e-05
705706,5571390,5571390,11142780,10909.136403083801,4.782431096828077e-05
706707,5579396,5579396,11158792,10921.555417776108,4.782402720593382e-05
707708,5587402,5587402,11174804,10934.279505968094,4.7822759370319545e-05
708709,5595408,5595408,11190816,10946.919122934341,4.782264295499772e-05
709710,5603410,5603410,11206820,10958.833219051361,4.78205292893108e-05
710711,5611412,5611412,11222824,10971.079831123352,4.781991992786061e-05
711712,5619412,5619412,11238824,10983.755379915237,4.781688221555669e-05
712713,5627416,5627416,11254832,10996.278589010239,4.781659117725212e-05
713714,5635420,5635420,11270840,11008.594157934189,4.781525240105111e-05
714715,5643428,5643428,11286856,11021.198805093765,4.781517600349616e-05
715716,5651424,5651424,11302848,11033.865684986115,4.780938797921408e-05
716717,5659430,5659430,11318860,11046.696181058884,4.78089878015453e-05
717718,5667432,5667432,11334864,11061.011116981506,4.780832750839181e-05
718719,5675436,5675436,11350872,11073.200289964676,4.780658855452202e-05
719720,5683440,5683440,11366880,11085.766306877136,4.7806410293560475e-05
720721,5691446,5691446,11382892,11098.257323026657,4.780597191711422e-05
721722,5699450,5699450,11398900,11110.888752937317,4.780500603374094e-05
722723,5707454,5707454,11414908,11122.976371049881,4.78040637972299e-05
723724,5715460,5715460,11430920,11135.825340032578,4.7803589040995575e-05
724725,5723462,5723462,11446924,11148.2471139431,4.780275048688054e-05
725726,5731468,5731468,11462936,11160.279664993286,4.780213021149393e-05
726727,5739470,5739470,11478940,11173.962476015091,4.780132439918816e-05
727728,5747474,5747474,11494948,11189.050549983978,4.77993435197277e-05
728729,5755480,5755480,11510960,11202.177257061005,4.779927621711977e-05
729730,5763484,5763484,11526968,11214.847149133682,4.779697883350309e-05
730731,5771490,5771490,11542980,11227.723116159439,4.779663686349522e-05
731732,5779498,5779498,11558996,11238.93217587471,4.7796560465940274e-05
732733,5787498,5787498,11574996,11250.166974067688,4.7795309001230635e-05
733734,5795506,5795506,11591012,11262.054144144058,4.779523442266509e-05
734735,5803510,5803510,11607020,11273.665156841278,4.7794816055102274e-05
735736,5811516,5811516,11623032,11285.241919994354,4.7794032070669346e-05
736737,5819520,5819520,11639040,11296.802202939987,4.779391747433692e-05
737738,5827524,5827524,11655048,11308.57255101204,4.779110167874023e-05
738739,5835528,5835528,11671056,11321.52963399887,4.7790723328944296e-05
739740,5843534,5843534,11687068,11333.626747846603,4.7790148528292775e-05
740741,5851540,5851540,11703080,11347.607811927795,4.778982111020014e-05
741742,5859544,5859544,11719088,11360.292216062546,4.778920265380293e-05
742743,5867550,5867550,11735100,11373.597379207611,4.7788460506126285e-05
743744,5875552,5875552,11751104,11386.352909088135,4.7787871153559536e-05
744745,5883558,5883558,11767116,11399.350744962692,4.778678703587502e-05
745746,5891562,5891562,11783124,11411.982241153717,4.778640141012147e-05
746747,5899564,5899564,11799128,11424.559586763382,4.778568836627528e-05
747748,5907566,5907566,11815132,11438.705055952072,4.778476977662649e-05
748749,5915572,5915572,11831144,11452.11277604103,4.778365655511152e-05
749750,5923576,5923576,11847152,11465.306929826736,4.7783049012650736e-05
750751,5931578,5931578,11863156,11477.798770904541,4.778214679390658e-05
751752,5939582,5939582,11879164,11489.69396519661,4.7781535613466986e-05
752753,5947586,5947586,11895172,11501.652084112167,4.778132824867498e-05
753754,5955588,5955588,11911176,11513.816824913025,4.7780627937754616e-05
754755,5963592,5963592,11927184,11527.826241016388,4.7778898078831844e-05
755756,5971596,5971596,11943192,11539.723148107529,4.777869617100805e-05
756757,5979600,5979600,11959200,11552.129284858704,4.777796311827842e-05
757758,5987602,5987602,11975204,11563.963531017303,4.777680442202836e-05
758759,5995606,5995606,11991212,11577.24056816101,4.777631693286821e-05
759760,6003612,6003612,12007224,11590.163790941238,4.777578214998357e-05
760761,6011614,6011614,12023228,11603.050202846527,4.7774661652510986e-05
761762,6019620,6019620,12039240,11615.134126901627,4.7773881306056865e-05
762763,6027626,6027626,12055252,11627.955046892166,4.777308458869811e-05
763764,6035630,6035630,12071260,11640.224630117416,4.7772629841347225e-05
764765,6043636,6043636,12087272,11652.376775979996,4.777260073751677e-05
765766,6051642,6051642,12103284,11664.545330047607,4.777257527166512e-05
766767,6059646,6059646,12119292,11678.037868022919,4.777057620231062e-05
767768,6067650,6067650,12135300,11690.42997097969,4.7769988668733276e-05
768769,6075652,6075652,12151304,11702.850441932678,4.776951391249895e-05
769770,6083656,6083656,12167312,11716.030636072159,4.776684545504395e-05
770771,6091660,6091660,12183320,11728.68485403061,4.776650166604668e-05
771772,6099664,6099664,12199328,11742.335248947144,4.776566493092105e-05
772773,6107668,6107668,12215336,11754.792183160782,4.776495916303247e-05
773774,6115674,6115674,12231348,11768.23114991188,4.776475361722987e-05
774775,6123678,6123678,12247356,11781.476903915405,4.776332752953749e-05
775776,6131684,6131684,12263368,11793.535983800888,4.776309469889384e-05
776777,6139690,6139690,12279380,11805.85387301445,4.7762328904354945e-05
777778,6147696,6147696,12295392,11818.382637023926,4.776198147737887e-05
778779,6155700,6155700,12311400,11831.308364152908,4.776138666784391e-05
779780,6163702,6163702,12327404,11842.950328826904,4.776079731527716e-05
780781,6171708,6171708,12343416,11854.945634126663,4.7760040615685284e-05
781782,6179712,6179712,12359424,11866.953306913376,4.775966044689994e-05
782783,6187712,6187712,12375424,11879.385663986206,4.7758732762304135e-05
783784,6195720,6195720,12391440,11891.862858057022,4.7758656364749186e-05
784785,6203446,6203446,12406892,11904.108717918396,4.3524112697923556e-05
785786,6211450,6211450,12422900,11917.143632888794,4.3523634303710423e-05
786787,6219454,6219454,12438908,11929.784616947174,4.3522968553588726e-05
787788,6227460,6227460,12454920,11941.910083055496,4.352061478130054e-05
788789,6235466,6235466,12470932,11954.158799886703,4.352051837486215e-05
789790,6243470,6243470,12486940,11966.320015907288,4.352004179963842e-05
790791,6251476,6251476,12502952,11978.297960996628,4.3518259190022945e-05
791792,6259480,6259480,12518960,11992.404437065125,4.3517802623682655e-05
792793,6267484,6267484,12534968,12004.691654920578,4.3515765355550684e-05
793794,6275490,6275490,12550980,12016.869148015976,4.35155689046951e-05
794795,6283494,6283494,12566988,12028.902195930481,4.351429015514441e-05
795796,6291498,6291498,12582996,12040.913276910782,4.351368988864124e-05
796797,6299504,6299504,12599008,12052.899644851685,4.351353163656313e-05
797798,6307506,6307506,12615012,12064.247332811356,4.351075040176511e-05
798799,6315508,6315508,12631016,12076.0521941185,4.3510020987014286e-05
799800,6323512,6323512,12647024,12088.375960826874,4.350902418082114e-05
800801,6331518,6331518,12663036,12101.415224075317,4.350853669166099e-05
801802,6339524,6339524,12679048,12114.004008054733,4.3505639041541144e-05
802803,6347526,6347526,12695052,12126.874216079712,4.350494600657839e-05
803804,6355532,6355532,12711064,12140.80870294571,4.350473318481818e-05
804805,6363534,6363534,12727068,12154.307427883148,4.3503525375854224e-05
805806,6371538,6371538,12743076,12168.269876003265,4.3502879634615965e-05
806807,6379542,6379542,12759084,12181.800481081009,4.350252856966108e-05
807808,6387548,6387548,12775096,12195.031320095062,4.3501560867298394e-05
808809,6395552,6395552,12791104,12208.1079890728,4.3500258470885456e-05
809810,6403554,6403554,12807108,12221.078359127045,4.3499057937879115e-05
810811,6411560,6411560,12823120,12233.868082046509,4.349834671302233e-05
811812,6419564,6419564,12839128,12246.700219869614,4.3498021113919094e-05
812813,6427564,6427564,12855128,12259.243822813034,4.3494286728673615e-05
813814,6435570,6435570,12871140,12272.015914916992,4.3493953853612766e-05
814815,6443572,6443572,12887144,12285.48195695877,4.349326809460763e-05
815816,6451580,6451580,12903160,12298.2425699234,4.349319169705268e-05
816817,6459582,6459582,12919164,12310.46561908722,4.3492496843100525e-05
817818,6467588,6467588,12935176,12322.87373805046,4.349172559159342e-05
818819,6475592,6475592,12951184,12335.196906089783,4.3491158066899516e-05
819820,6483596,6483596,12967192,12348.866146802902,4.3490701500559226e-05
820821,6491602,6491602,12983204,12362.335932016373,4.349042137619108e-05
821822,6499606,6499606,12999212,12374.57818698883,4.3489941162988544e-05
822823,6507610,6507610,13015220,12386.952405929565,4.348959919298068e-05
823824,6515618,6515618,13031236,12398.722290039062,4.348952279542573e-05
824825,6523620,6523620,13047240,12411.196585893631,4.348830225353595e-05
825826,6531624,6531624,13063248,12423.392183065414,4.348687616584357e-05
826827,6539628,6539628,13079256,12435.598186016083,4.3486377762747e-05
827828,6547634,6547634,13095268,12449.042984962463,4.3486119466251694e-05
828829,6555634,6555634,13111268,12461.746957063675,4.3484258640091866e-05
829830,6563640,6563640,13127280,12474.119660139084,4.348403490439523e-05
830831,6571642,6571642,13143284,12487.06882095337,4.348327456682455e-05
831832,6579648,6579648,13159296,12500.166156053543,4.348292532085907e-05
832833,6587652,6587652,13175304,12512.510522842407,4.348144830146339e-05
833834,6595658,6595658,13191316,12525.820997953415,4.348007860244252e-05
834835,6603662,6603662,13207324,12538.977834939957,4.3479436499183066e-05
835836,6611670,6611670,13223340,12550.928814888,4.347936010162812e-05
836837,6619676,6619676,13239352,12562.88616490364,4.3478876250446774e-05
837838,6627680,6627680,13255360,12575.34111905098,4.347888352640439e-05
838839,6635682,6635682,13271364,12589.308527946472,4.347871981735807e-05
839840,6643688,6643688,13287376,12602.417680978775,4.3478697989485227e-05
840841,6651692,6651692,13303384,12615.108706951141,4.3478743464220315e-05
841842,6659696,6659696,13319392,12628.59992980957,4.347606409282889e-05
842843,6667700,6667700,13335400,12641.096162080765,4.347471440269146e-05
843844,6675706,6675706,13351412,12653.823755025864,4.3474423364386894e-05
844845,6683712,6683712,13367424,12665.706953048706,4.3473957703099586e-05
845846,6691716,6691716,13383432,12677.312358856201,4.347335379861761e-05
846847,6699718,6699718,13399436,12689.356693029404,4.3472458855831064e-05
847848,6707722,6707722,13415444,12701.132019042969,4.3471731260069646e-05
848849,6715728,6715728,13431456,12714.162924051285,4.3471514800330624e-05
849850,6723732,6723732,13447464,12725.623893022537,4.34701178164687e-05
850851,6731738,6731738,13463476,12737.190071105957,4.346972309576813e-05
851852,6739744,6739744,13479488,12748.949939966202,4.346933747001458e-05
852853,6747746,6747746,13495492,12760.993965148926,4.346847163105849e-05
853854,6755750,6755750,13511500,12772.81253695488,4.346780224295799e-05
854855,6763754,6763754,13527508,12784.358081102371,4.346716741565615e-05
855856,6771758,6771758,13543516,12797.334072828293,4.346615787653718e-05
856857,6779764,6779764,13559528,12811.377378940582,4.3465801354614086e-05
857858,6787768,6787768,13575536,12824.06705212593,4.346559762780089e-05
858859,6795770,6795770,13591540,12837.458355903625,4.346461719251238e-05
859860,6803776,6803776,13607552,12849.781985998154,4.346211972006131e-05
860861,6811776,6811776,13623552,12862.22312092781,4.346189780335408e-05
861862,6819778,6819778,13639556,12874.413198947906,4.3459787775645964e-05
862863,6827782,6827782,13655564,12887.127958059311,4.34596004197374e-05
863864,6835788,6835788,13671576,12899.912195205688,4.345890920376405e-05
864865,6843792,6843792,13687584,12912.574253797531,4.345832348917611e-05
865866,6851796,6851796,13703592,12926.434584140778,4.345684283180162e-05
866867,6859800,6859800,13719600,12939.212681055069,4.3456551793497056e-05
867868,6867804,6867804,13735608,12951.740791082382,4.345454726717435e-05
868869,6875806,6875806,13751612,12964.312457084656,4.345342131273355e-05
869870,6883808,6883808,13767616,12977.069447040558,4.345296474639326e-05
870871,6891812,6891812,13783624,12989.222445964813,4.3452073441585526e-05
871872,6899812,6899812,13799624,13001.835490942001,4.3449590521049686e-05
872873,6907818,6907818,13815636,13014.25734090805,4.344926310295705e-05
873874,6915826,6915826,13831652,13026.708012104034,4.34491867054021e-05
874875,6923832,6923832,13847664,13039.280030965805,4.344746230344754e-05
875876,6931836,6931836,13863672,13051.748080015182,4.344695480540395e-05
876877,6939844,6939844,13879688,13064.317367076874,4.3446882045827806e-05
877878,6947844,6947844,13895688,13077.26681303978,4.3444486436783336e-05
878879,6955846,6955846,13911692,13091.039024829865,4.344324588601012e-05
879880,6963850,6963850,13927700,13104.440226078033,4.344277112977579e-05
880881,6971856,6971856,13943712,13117.640795946121,4.344244734966196e-05
881882,6979860,6979860,13959720,13129.946136951447,4.3441797970444895e-05
882883,6987868,6987868,13975736,13142.037905931473,4.344172339187935e-05
883884,6995872,6995872,13991744,13154.97809100151,4.344040098658297e-05
884885,7003876,7003876,14007752,13167.525307893753,4.344029366620816e-05
885886,7011878,7011878,14023756,13180.471816062927,4.3439238652354106e-05
886887,7019884,7019884,14039768,13194.218608856201,4.343909859017003e-05
887888,7027884,7027884,14055768,13206.680840015411,4.3432810343801975e-05
888889,7035884,7035884,14071768,13219.063599824905,4.3431091398815624e-05
889890,7043890,7043890,14087780,13231.363952875137,4.343075488577597e-05
890891,7051892,7051892,14103784,13244.174374818802,4.3429747165646404e-05
891892,7059898,7059898,14119796,13256.614900112152,4.342919601185713e-05
892893,7067904,7067904,14135808,13268.954445838928,4.342886131780688e-05
893894,7075910,7075910,14151820,13280.849478960037,4.3428224671515636e-05
894895,7083914,7083914,14167828,13292.840643167496,4.34278463217197e-05
895896,7091918,7091918,14183836,13306.400995969772,4.342745342000853e-05
896897,7099922,7099922,14199844,13318.250848054886,4.342642750998493e-05
897898,7107924,7107924,14215848,13331.432574987411,4.34256908192765e-05
898899,7115930,7115930,14231860,13344.23004078865,4.3425387048046105e-05
899900,7123932,7123932,14247864,13355.893873929977,4.342313150118571e-05
900901,7131934,7131934,14263868,13368.544867753983,4.3422196540632285e-05
901902,7139938,7139938,14279876,13380.904015779495,4.342147076386027e-05
902903,7147944,7147944,14295888,13392.054584741592,4.342104512033984e-05
903904,7155948,7155948,14311896,13403.773056983948,4.342050124250818e-05
904905,7163952,7163952,14327904,13415.876689910889,4.3419411667855456e-05
905906,7171954,7171954,14343908,13428.41902589798,4.3417498091002926e-05
906907,7179960,7179960,14359920,13441.07817697525,4.341720159573015e-05
907908,7187964,7187964,14375928,13453.278559923172,4.341647945693694e-05
908909,7195968,7195968,14391936,13466.205044984818,4.341570820542984e-05
909910,7203974,7203974,14407948,13479.697678804398,4.341542626207229e-05
910911,7211982,7211982,14423964,13491.603130817413,4.341534622653853e-05
911912,7219984,7219984,14439968,13504.393987894058,4.341442581790034e-05
912913,7227992,7227992,14455984,13519.857613801956,4.341434942034539e-05
913914,7235392,7235392,14470784,13531.592653751373,4.341268868301995e-05
914915,7243386,7243386,14486772,13544.37918996811,4.341220483183861e-05
915916,7251384,7251384,14502768,13555.975635051727,4.341181193012744e-05
916917,7259386,7259386,14518772,13567.494168758392,4.3411388105596416e-05
917918,7267390,7267390,14534780,13580.286394834518,4.3410227590356953e-05
918919,7275394,7275394,14550788,13592.625545024872,4.340974737715442e-05
919920,7283392,7283392,14566784,13604.369197845459,4.340895429777447e-05
920921,7291398,7291398,14582796,13615.99936580658,4.3408719648141414e-05
921922,7299402,7299402,14598804,13628.24512887001,4.340808118286077e-05
922923,7307408,7307408,14614816,13641.845431089401,4.3407853809185326e-05
923924,7315414,7315414,14630828,13655.43402504921,4.340761915955227e-05
924925,7323418,7323418,14646836,13668.406026124954,4.340759005572181e-05
925926,7331420,7331420,14662840,13679.977890729904,4.340715895523317e-05
926927,7339420,7339420,14678840,13692.455008983612,4.340629493526649e-05
927928,7347420,7347420,14694840,13704.591820001602,4.340558734838851e-05
928929,7355420,7355420,14710840,13716.922101020813,4.34049670730019e-05
929930,7363422,7363422,14726844,13728.77842593193,4.340454870543908e-05
930931,7371426,7371426,14742852,13740.805862903595,4.3404328607721254e-05
931932,7379428,7379428,14758856,13752.169239997864,4.3403651943663135e-05
932933,7387432,7387432,14774864,13763.51307797432,4.34034282079665e-05
933934,7395434,7395434,14790868,13776.763675928116,4.340294799476396e-05
934935,7403440,7403440,14806880,13789.88859295845,4.340272607805673e-05
935936,7411440,7411440,14822880,13803.600567102432,4.340180930739734e-05
936937,7419444,7419444,14838888,13816.309986829758,4.3401430957601406e-05
937938,7427446,7427446,14854892,13828.083345890045,4.3401219954830594e-05
938939,7435452,7435452,14870904,13839.338204860687,4.34010162280174e-05
939940,7443456,7443456,14886912,13851.715706825256,4.3400748836575076e-05
940941,7451460,7451460,14902920,13863.348667860031,4.340025952842552e-05
941942,7459466,7459466,14918932,13876.380854129791,4.339964289101772e-05
942943,7467470,7467470,14934940,13889.137466907501,4.3399297283031046e-05
943944,7475474,7475474,14950948,13901.654238939285,4.339815677667502e-05
944945,7483476,7483476,14966952,13914.627781867981,4.3397758417995647e-05
945946,7491480,7491480,14982960,13927.069828987122,4.3397218178142793e-05
946947,7499482,7499482,14998964,13940.782978057861,4.3396561522968113e-05
947948,7507488,7507488,15014976,13952.792669057846,4.339647421147674e-05
948949,7515490,7515490,15030980,13965.299055814743,4.339569204603322e-05
949950,7523498,7523498,15046996,13978.885556936264,4.339564293331932e-05
950951,7531494,7531494,15062988,13994.516617059708,4.3393658415880054e-05
951952,7539496,7539496,15078992,14006.626850128174,4.339333463576622e-05
952953,7547504,7547504,15095008,14018.874220132828,4.339328734204173e-05
953954,7555504,7555504,15111008,14031.349503040314,4.339151564636268e-05
954955,7563506,7563506,15127012,14044.78676199913,4.3389492930145934e-05
955956,7571510,7571510,15143020,14056.324828863144,4.338900907896459e-05
956957,7579516,7579516,15159032,14067.857383012772,4.338887447374873e-05
957958,7587520,7587520,15175040,14080.759607076645,4.3388616177253425e-05
958959,7595524,7595524,15191048,14092.575716972351,4.338777580414899e-05
959960,7603530,7603530,15207060,14105.393985033035,4.338774306233972e-05
960961,7611534,7611534,15223068,14118.302013874054,4.338723010732792e-05
961962,7619538,7619538,15239076,14130.832818984985,4.338685539551079e-05
962963,7627540,7627540,15255080,14143.54448390007,4.3386435208958574e-05
963964,7635544,7635544,15271088,14155.870110034943,4.338620783528313e-05
964965,7643548,7643548,15287096,14167.52370095253,4.338529106462374e-05
965966,7651552,7651552,15303104,14180.279592037201,4.3385118260630406e-05
966967,7659558,7659558,15319116,14193.734405994415,4.338457256380934e-05
967968,7667560,7667560,15335120,14205.359507083893,4.338372127676848e-05
968969,7675564,7675564,15351128,14217.451033830643,4.338369035394862e-05
969970,7683570,7683570,15367140,14229.88090801239,4.3383455704315566e-05
970971,7691570,7691570,15383140,14242.750043869019,4.338202779763378e-05
971972,7699572,7699572,15399144,14256.297116041183,4.3380192437325604e-05
972973,7707576,7707576,15415152,14269.222537994385,4.338005601312034e-05
973974,7715578,7715578,15431156,14282.917984008789,4.337889913585968e-05
974975,7723582,7723582,15447164,14294.878370761871,4.337825521361083e-05
975976,7731586,7731586,15463172,14308.45861005783,4.3378058762755245e-05
976977,7739588,7739588,15479176,14320.889060974121,4.337755854066927e-05
977978,7747590,7747590,15495180,14333.10948586464,4.337716927693691e-05
978979,7755592,7755592,15511184,14345.908413887024,4.3376658140914515e-05
979980,7763304,7763304,15526608,14359.862401008606,3.829822162515484e-05
980981,7771302,7771302,15542604,14373.060348033905,3.829777233477216e-05
981982,7779304,7779304,15558608,14386.333557128906,3.829737761407159e-05
982983,7787306,7787306,15574612,14398.906306028366,3.829709748970345e-05
983984,7795308,7795308,15590616,14411.830615997314,3.8296573620755225e-05
984985,7803312,7803312,15606624,14423.778312921524,3.829605338978581e-05
985986,7811316,7811316,15622632,14436.628542900085,3.829554952972103e-05
986987,7819320,7819320,15638640,14449.16763806343,3.8295285776257515e-05
987988,7827324,7827324,15654648,14461.559640169144,3.829488377959933e-05
988989,7835328,7835328,15670656,14474.140588998795,3.8293726902338676e-05
989990,7843332,7843332,15686664,14486.581846952438,3.829323759418912e-05
990991,7851338,7851338,15702676,14499.4039208889,3.829315937764477e-05
991992,7859334,7859334,15718668,14511.509483098984,3.8290150769171305e-05
992993,7867338,7867338,15734676,14523.539192914963,3.828949593298603e-05
993994,7875344,7875344,15750688,14535.310198068619,3.828935950878076e-05
994995,7883344,7883344,15766688,14547.280365943909,3.828837907349225e-05
995996,7891352,7891352,15782704,14559.146865844727,3.828833359875716e-05
996997,7899356,7899356,15798712,14571.26872086525,3.8287493225652725e-05
997998,7907362,7907362,15814724,14583.39840888977,3.828737135336269e-05
998999,7915352,7915352,15830704,14596.655728816986,3.827371801889967e-05
1000000,7923356,7923356,15846712,14609.249511003494,3.827304135484155e-05


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/adaptive_proximal_gradient.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,2,1,3,0.0007541179656982422,848.1427353403399
28,58,29,87,0.027872085571289062,62.9785207281368
55,112,56,168,0.0475161075592041,54.08712962900722
83,168,84,252,0.0693511962890625,50.44031887741676
111,224,112,336,0.08897113800048828,47.81801451262527
139,280,140,420,0.10674524307250977,45.73767180609639
166,334,167,501,0.125413179397583,43.01569059937947
194,390,195,585,0.14530301094055176,41.32841072373549
222,446,223,669,0.16881918907165527,39.63842301050522
249,500,250,750,0.19244003295898438,37.43437196943228
277,556,278,834,0.21297812461853027,36.02296302893592
305,612,306,918,0.23708319664001465,34.663163670765925
332,666,333,999,0.2603950500488281,33.35483586732539
360,722,361,1083,0.2879030704498291,32.112270620477375
388,778,389,1167,0.31032228469848633,31.14301324740495
416,834,417,1251,0.3396260738372803,29.9049479763205
443,888,444,1332,0.3611431121826172,29.110408485795915
471,944,472,1416,0.387911319732666,28.168331680457413
499,1000,500,1500,0.41123104095458984,27.293755769228483
526,1054,527,1581,0.4339640140533447,26.56888695102839
554,1110,555,1665,0.45282816886901855,25.81195523052247
582,1166,583,1749,0.4752650260925293,25.01229219333368
610,1222,611,1833,0.4978921413421631,24.278415489758117
637,1276,638,1914,0.517747163772583,23.710236182238532
665,1332,666,1998,0.5412211418151855,22.869710564221123
693,1388,694,2082,0.562333345413208,22.296544512702212
720,1442,721,2163,0.5876290798187256,21.741147679447977
748,1498,749,2247,0.6129472255706787,21.125168196835602
776,1554,777,2331,0.6397240161895752,20.58861788311674
803,1608,804,2412,0.6614241600036621,20.1106513522991
831,1664,832,2496,0.691115140914917,19.478609929034747
859,1720,860,2580,0.7135300636291504,19.086483057199075
887,1776,888,2664,0.7416760921478271,18.59882410197565
914,1830,915,2745,0.7599589824676514,18.09824517795232
942,1886,943,2829,0.7899692058563232,17.656307852144664
970,1942,971,2913,0.8138501644134521,17.21000513088393
997,1996,998,2994,0.8396971225738525,16.830750287960882
1025,2052,1026,3078,0.8605010509490967,16.370067496020056
1053,2108,1054,3162,0.8853302001953125,15.914391900723672
1080,2162,1081,3243,0.9048969745635986,15.586359335893121
1108,2218,1109,3327,0.9290130138397217,15.123075582424804
1136,2274,1137,3411,0.9534091949462891,14.759768984733682
1164,2330,1165,3495,0.9793891906738281,14.391866584223067
1191,2384,1192,3576,1.0035440921783447,14.055229421168406
1219,2440,1220,3660,1.0293681621551514,13.666414132949285
1247,2496,1248,3744,1.05134916305542,13.338787395585655
1274,2550,1275,3825,1.072033166885376,12.97936002973779
1302,2606,1303,3909,1.096764326095581,12.69275364453415
1330,2662,1331,3993,1.118096113204956,12.39773409934537
1358,2718,1359,4077,1.1422131061553955,12.100561865667942
1385,2772,1386,4158,1.161945104598999,11.763971178456472
1413,2828,1414,4242,1.1851892471313477,11.493092600531327
1441,2884,1442,4326,1.2156710624694824,11.18170053347069
1468,2938,1469,4407,1.241936206817627,10.938399802216736
1496,2994,1497,4491,1.2624702453613281,10.690158432390035
1524,3050,1525,4575,1.28999924659729,10.406784462091537
1551,3104,1552,4656,1.3100993633270264,10.16194930722395
1579,3160,1580,4740,1.3384771347045898,9.922262942234738
1607,3216,1608,4824,1.3609051704406738,9.671782730840278
1635,3272,1636,4908,1.3822941780090332,9.489333558555245
1662,3326,1663,4989,1.4068472385406494,9.26062684169608
1690,3382,1691,5073,1.4354681968688965,9.046359510964976
1718,3438,1719,5157,1.4568822383880615,8.795828827192963
1745,3492,1746,5238,1.4759411811828613,8.587777290410486
1773,3548,1774,5322,1.4987640380859375,8.365397199631957
1801,3604,1802,5406,1.5181550979614258,8.171766451319854
1829,3660,1830,5490,1.5394291877746582,7.961504883600128
1856,3714,1857,5571,1.557967185974121,7.772093108553008
1884,3770,1885,5655,1.5758731365203857,7.604615363180187
1912,3826,1913,5739,1.5979411602020264,7.451451584378333
1939,3880,1940,5820,1.6171209812164307,7.27314990262812
1967,3936,1968,5904,1.6408910751342773,7.083838351395798
1995,3992,1996,5988,1.6602232456207275,6.940368190290997
2022,4046,2023,6069,1.679152250289917,6.7936718899459265
2050,4102,2051,6153,1.7029411792755127,6.642920606674579
2078,4158,2079,6237,1.7283201217651367,6.489029000869209
2106,4214,2107,6321,1.7579162120819092,6.360667965209359
2133,4268,2134,6402,1.7862040996551514,6.216809083711951
2161,4324,2162,6486,1.8117141723632812,6.043094573864096
2189,4380,2190,6570,1.8402869701385498,5.916810670858922
2216,4434,2217,6651,1.8651020526885986,5.768203951020723
2244,4490,2245,6735,1.889336109161377,5.648015565805849
2272,4546,2273,6819,1.912363052368164,5.51768675875303
2299,4600,2300,6900,1.9360101222991943,5.388995710716131
2327,4656,2328,6984,1.9595072269439697,5.27248492617332
2355,4712,2356,7068,1.9828600883483887,5.161338424568612
2383,4768,2384,7152,2.003826141357422,5.036150162889953
2410,4822,2411,7233,2.0267152786254883,4.928494558631428
2438,4878,2439,7317,2.0496041774749756,4.821204667270763
2466,4934,2467,7401,2.069819211959839,4.714834846503322
2493,4988,2494,7482,2.0919251441955566,4.604259396444718
2521,5044,2522,7566,2.1168551445007324,4.505424804495988
2549,5100,2550,7650,2.143430233001709,4.374935722466262
2577,5156,2578,7734,2.165928363800049,4.278392448825571
2604,5210,2605,7815,2.1917293071746826,4.19288551206273
2632,5266,2633,7899,2.2177860736846924,4.103881519381503
2660,5322,2661,7983,2.242631196975708,4.005607600030771
2687,5376,2688,8064,2.259593963623047,3.925759419023734
2715,5432,2716,8148,2.2858030796051025,3.843844862392416
2743,5488,2744,8232,2.3113882541656494,3.74975078780642
2770,5542,2771,8313,2.3364832401275635,3.6724037756241614
2798,5598,2799,8397,2.35707426071167,3.5987788214595184
2826,5654,2827,8481,2.3781871795654297,3.5154606424553094
2854,5710,2855,8565,2.4029953479766846,3.4500955670428084
2881,5764,2882,8646,2.426405191421509,3.36528787235045
2909,5820,2910,8730,2.452336072921753,3.279679178230367
2937,5876,2938,8814,2.473421096801758,3.191057992460742
2964,5930,2965,8895,2.494589328765869,3.124343806610682
2992,5986,2993,8979,2.5171780586242676,3.046801280378645
3020,6042,3021,9063,2.54404616355896,2.9785401346276785
3048,6098,3049,9147,2.5676021575927734,2.918059458103812
3075,6152,3076,9228,2.5958609580993652,2.852750058508377
3103,6208,3104,9312,2.6198971271514893,2.796880845954547
3131,6264,3132,9396,2.646818161010742,2.731537533055757
3158,6318,3159,9477,2.667677164077759,2.6757269538330775
3186,6374,3187,9561,2.6947813034057617,2.6149809638875467
3214,6430,3215,9645,2.7159311771392822,2.5604816274740188
3241,6484,3242,9726,2.7406063079833984,2.496592492695754
3269,6540,3270,9810,2.7714290618896484,2.4400812695192826
3297,6596,3298,9894,2.795133352279663,2.38986884892347
3325,6652,3326,9978,2.818082094192505,2.340611723425468
3352,6706,3353,10059,2.843513250350952,2.293429170645254
3380,6762,3381,10143,2.865770101547241,2.2476892737659
3408,6818,3409,10227,2.8919801712036133,2.2013732748529264
3435,6872,3436,10308,2.914130210876465,2.161049728314879
3463,6928,3464,10392,2.937425136566162,2.112691846804182
3491,6984,3492,10476,2.9662342071533203,2.0670714791787077
3518,7038,3519,10557,2.9923250675201416,2.01704351806427
3546,7094,3547,10641,3.016613245010376,1.9799226080664312
3574,7150,3575,10725,3.04260516166687,1.931849975170394
3602,7206,3603,10809,3.066373109817505,1.8995391219154953
3629,7260,3630,10890,3.0908942222595215,1.861644925508699
3657,7316,3658,10974,3.1124751567840576,1.8175810471751674
3685,7372,3686,11058,3.138500213623047,1.781051397787337
3712,7426,3713,11139,3.161234140396118,1.7481321899771274
3740,7482,3741,11223,3.18624210357666,1.714150949594
3768,7538,3769,11307,3.207332134246826,1.6771094496625665
3796,7594,3797,11391,3.2335453033447266,1.6430176179939053
3823,7648,3824,11472,3.2517030239105225,1.6122366601410931
3851,7704,3852,11556,3.273480176925659,1.5657950181331444
3879,7760,3880,11640,3.295208215713501,1.5344477636540432
3906,7814,3907,11721,3.316620111465454,1.4926852773064638
3934,7870,3935,11805,3.340567111968994,1.4633175988759604
3962,7926,3963,11889,3.362133026123047,1.4331852166893668
3989,7980,3990,11970,3.3862762451171875,1.4037953376362111
4017,8036,4018,12054,3.41154408454895,1.3819495653198146
4045,8092,4046,12138,3.43974232673645,1.3511405421105565
4073,8148,4074,12222,3.4674339294433594,1.3191313449184463
4100,8202,4101,12303,3.4952480792999268,1.2931968569864694
4128,8258,4129,12387,3.5296173095703125,1.2695835780074276
4156,8314,4157,12471,3.5610973834991455,1.233425365253197
4183,8368,4184,12552,3.5961501598358154,1.2089709635509962
4211,8424,4212,12636,3.6360931396484375,1.1838466426237346
4239,8480,4240,12720,3.6751911640167236,1.15748345786983
4267,8536,4268,12804,3.7121100425720215,1.1380132238612077
4294,8590,4295,12885,3.749972343444824,1.110501750980461
4322,8646,4323,12969,3.7891101837158203,1.085870126916916
4350,8702,4351,13053,3.8266661167144775,1.0619125173186603
4377,8756,4378,13134,3.868129014968872,1.039679957549538
4405,8812,4406,13218,3.9334051609039307,1.018579682026484
4433,8868,4434,13302,3.997619152069092,0.9979220562618139
4460,8922,4461,13383,4.0366621017456055,0.9758771161091317
4488,8978,4489,13467,4.066941261291504,0.9565635480043966
4516,9034,4517,13551,4.099197149276733,0.9366270217748252
4544,9090,4545,13635,4.141613006591797,0.9153423845207271
4571,9144,4572,13716,4.172988176345825,0.8986206988797676
4599,9200,4600,13800,4.208719253540039,0.8800657217118442
4627,9256,4628,13884,4.240479946136475,0.8618623049831058
4654,9310,4655,13965,4.269463062286377,0.8461200866669287
4682,9366,4683,14049,4.300256967544556,0.8266359372789793
4710,9422,4711,14133,4.331299066543579,0.810359869730064
4738,9478,4739,14217,4.38027811050415,0.792284592380156
4765,9532,4766,14298,4.4127891063690186,0.7786977914543058
4793,9588,4794,14382,4.444561243057251,0.7604912154821477
4821,9644,4822,14466,4.477039098739624,0.7447394254977553
4848,9698,4849,14547,4.508830308914185,0.7308812422052142
4876,9754,4877,14631,4.542116165161133,0.7152780298853259
4904,9810,4905,14715,4.57656717300415,0.7018370061218775
4931,9864,4932,14796,4.606893062591553,0.690227642382979
4959,9920,4960,14880,4.640318155288696,0.6759268617292946
4987,9976,4988,14964,4.671295404434204,0.6618985247292812
5015,10032,5016,15048,4.70070219039917,0.6496330033709228
5042,10086,5043,15129,4.724452257156372,0.6364550819042734
5070,10142,5071,15213,4.748804092407227,0.6240414297269581
5098,10198,5099,15297,4.7733540534973145,0.6101240118297255
5125,10252,5126,15378,4.799408197402954,0.5989210909486928
5153,10308,5154,15462,4.825534343719482,0.5850987584852874
5181,10364,5182,15546,4.850808143615723,0.5733277946044382
5208,10418,5209,15627,4.877289295196533,0.5590503633524122
5236,10474,5237,15711,4.904937267303467,0.5479305739246456
5264,10530,5265,15795,4.928648233413696,0.536087058150656
5292,10586,5293,15879,4.954827070236206,0.525386760375909
5319,10640,5320,15960,4.985384225845337,0.5148848336472156
5347,10696,5348,16044,5.014208078384399,0.5036473356539091
5375,10752,5376,16128,5.041919946670532,0.4946276680042274
5402,10806,5403,16209,5.067045211791992,0.48440321439943546
5430,10862,5431,16293,5.098858118057251,0.47387671302351464
5458,10918,5459,16377,5.130134105682373,0.4651176334843967
5486,10974,5487,16461,5.156344175338745,0.45564570950944017
5513,11028,5514,16542,5.1850481033325195,0.44844240394741064
5541,11084,5542,16626,5.217642068862915,0.4387525107675856
5569,11140,5570,16710,5.249446153640747,0.43051012389344123
5596,11194,5597,16791,5.2780983448028564,0.4211646141760639
5624,11250,5625,16875,5.308264255523682,0.41306499670702124
5652,11306,5653,16959,5.3343541622161865,0.4056583221963592
5679,11360,5680,17040,5.358744144439697,0.3981244934186634
5707,11416,5708,17124,5.387263298034668,0.38943822054693555
5735,11472,5736,17208,5.410082101821899,0.3816753974523408
5763,11528,5764,17292,5.438868999481201,0.37309997066711276
5790,11582,5791,17373,5.467315196990967,0.36701250745102243
5818,11638,5819,17457,5.49651312828064,0.3593452125899148
5846,11694,5847,17541,5.526661157608032,0.3522645034369134
5873,11748,5874,17622,5.553770065307617,0.3449312239298479
5901,11804,5902,17706,5.584686040878296,0.33876234077433764
5929,11860,5930,17790,5.608465194702148,0.33210397992741036
5957,11916,5958,17874,5.632411241531372,0.3243177599701994
5984,11970,5985,17955,5.658111333847046,0.3181306990752546
6012,12026,6013,18039,5.687489986419678,0.3114557632957258
6040,12082,6041,18123,5.716582298278809,0.3079543799773319
6067,12136,6068,18204,5.74631404876709,0.2994189916317964
6095,12192,6096,18288,5.773771047592163,0.29377831832175616
6123,12248,6124,18372,5.802634954452515,0.28807808652436506
6150,12302,6151,18453,5.823675155639648,0.28248756085395144
6178,12358,6179,18537,5.851465225219727,0.2765581061329385
6206,12414,6207,18621,5.877790927886963,0.27078235426631636
6234,12470,6235,18705,5.903419256210327,0.2656082016322898
6261,12524,6262,18786,5.932351350784302,0.2601573828879964
6289,12580,6290,18870,5.958473205566406,0.2552990384087934
6317,12636,6318,18954,5.989652395248413,0.2508066023339097
6344,12690,6345,19035,6.01829719543457,0.24572889525632036
6372,12746,6373,19119,6.049241065979004,0.24154529231157085
6400,12802,6401,19203,6.080609083175659,0.23635272679314312
6427,12856,6428,19284,6.109547138214111,0.23208876855778726
6455,12912,6456,19368,6.140810966491699,0.22746106789509213
6483,12968,6484,19452,6.183608055114746,0.22340052596246096
6511,13024,6512,19536,6.2145020961761475,0.21942967463053265
6538,13078,6539,19617,6.239042043685913,0.21515663927038986
6566,13134,6567,19701,6.2668352127075195,0.21120681794150187
6594,13190,6595,19785,6.2920050621032715,0.20740848820025803
6621,13244,6622,19866,6.319305181503296,0.20395381664422985
6649,13300,6650,19950,6.346409320831299,0.1997843792007643
6677,13356,6678,20034,6.373592138290405,0.19594407864497043
6705,13412,6706,20118,6.409592151641846,0.19109108514135187
6732,13466,6733,20199,6.43633508682251,0.18735237862426857
6760,13522,6761,20283,6.46246337890625,0.18369031109784828
6788,13578,6789,20367,6.49076509475708,0.1798549543173067
6815,13632,6816,20448,6.515305995941162,0.17683639075130486
6843,13688,6844,20532,6.542750358581543,0.17300320881338394
6871,13744,6872,20616,6.57021427154541,0.1698205252663456
6898,13798,6899,20697,6.596320152282715,0.16690578694488067
6926,13854,6927,20781,6.624206066131592,0.16373416980025013
6954,13910,6955,20865,6.651098251342773,0.1605137436519044
6982,13966,6983,20949,6.681046009063721,0.1570411992083791
7009,14020,7010,21030,6.706024169921875,0.15434707572637762
7037,14076,7038,21114,6.734183311462402,0.151199855663549
7065,14132,7066,21198,6.7605881690979,0.14852957772518494
7092,14186,7093,21279,6.7877702713012695,0.14569002082691895
7120,14242,7121,21363,6.815388202667236,0.1426262043544284
7148,14298,7149,21447,6.842389106750488,0.13997194191074414
7176,14354,7177,21531,6.87074613571167,0.1372196775273551
7203,14408,7204,21612,6.89624810218811,0.13493119195470626
7231,14464,7232,21696,6.924584150314331,0.13199867928722142
7259,14520,7260,21780,6.952178239822388,0.1295167494653242
7286,14574,7287,21861,6.981628179550171,0.1270616236965907
7314,14630,7315,21945,7.008795261383057,0.12466572475000248
7342,14686,7343,22029,7.037944078445435,0.12239162012338056
7369,14740,7370,22110,7.065275192260742,0.11980869808485295
7397,14796,7398,22194,7.09419322013855,0.11800736456962113
7425,14852,7426,22278,7.1249840259552,0.11566989816708428
7453,14908,7454,22362,7.149729013442993,0.11305555183014349
7480,14962,7481,22443,7.177881240844727,0.1110453024537037
7508,15018,7509,22527,7.204951047897339,0.10905818604680917
7536,15074,7537,22611,7.237300395965576,0.10699033915545897
7563,15128,7564,22692,7.264734268188477,0.10544569393596248
7591,15184,7592,22776,7.290753126144409,0.10321443973941768
7619,15240,7620,22860,7.31657600402832,0.10104472410307608
7646,15294,7647,22941,7.339034080505371,0.09935963413727222
7674,15350,7675,23025,7.365571022033691,0.0971814264224804
7702,15406,7703,23109,7.39338231086731,0.09527506298240951
7730,15462,7731,23193,7.417602062225342,0.09346428158391973
7757,15516,7758,23274,7.444220304489136,0.09178086915312633
7785,15572,7786,23358,7.473144054412842,0.090005409327091
7813,15628,7814,23442,7.4991700649261475,0.08800690269231382
7840,15682,7841,23523,7.5270631313323975,0.08646001056069963
7868,15738,7869,23607,7.555288076400757,0.08496733832669179
7896,15794,7897,23691,7.582757234573364,0.08331016120826007
7924,15850,7925,23775,7.610968112945557,0.08158628218313879
7951,15904,7952,23856,7.638467073440552,0.08006013939586865
7979,15960,7980,23940,7.667974233627319,0.07851072892935917
8007,16016,8008,24024,7.698706150054932,0.07687027742667851
8034,16070,8035,24105,7.728804111480713,0.07564242095895679
8062,16126,8063,24189,7.7567222118377686,0.07423216284291811
8090,16182,8091,24273,7.784558057785034,0.07276935545792185
8117,16236,8118,24354,7.812218189239502,0.0714859897855149
8145,16292,8146,24438,7.841609954833984,0.07009680877320079
8173,16348,8174,24522,7.868368148803711,0.06864930902963806
8201,16404,8202,24606,7.900987148284912,0.06734459178346697
8228,16458,8229,24687,7.940467357635498,0.06617213769527552
8256,16514,8257,24771,7.966590166091919,0.06489445725424048
8284,16570,8285,24855,7.996625185012817,0.06383517718336407
8311,16624,8312,24936,8.024496078491211,0.06259848684692315
8339,16680,8340,25020,8.051894187927246,0.06141564735889915
8367,16736,8368,25104,8.080941200256348,0.060269989042126326
8395,16792,8396,25188,8.107566118240356,0.05909873027201229
8422,16846,8423,25269,8.143607139587402,0.057873103584825
8450,16902,8451,25353,8.171893119812012,0.0568134611099822
8478,16958,8479,25437,8.200618028640747,0.0557904156830773
8505,17012,8506,25518,8.229648113250732,0.054704573688013625
8533,17068,8534,25602,8.258805990219116,0.05368323502318617
8561,17124,8562,25686,8.287060260772705,0.05270092253351777
8588,17178,8589,25767,8.315822124481201,0.05180789837561406
8616,17234,8617,25851,8.345954179763794,0.05081672515404989
8644,17290,8645,25935,8.373959302902222,0.05026483001518045
8672,17346,8673,26019,8.40185022354126,0.0489143769424345
8699,17400,8700,26100,8.431100130081177,0.047978939613017246
8727,17456,8728,26184,8.458436250686646,0.04711416331474538
8755,17512,8756,26268,8.485572099685669,0.04625088183524895
8782,17566,8783,26349,8.514223098754883,0.04547922164579177
8810,17622,8811,26433,8.540209293365479,0.04460048487851509
8838,17678,8839,26517,8.56876516342163,0.04377063290667138
8866,17734,8867,26601,8.593563079833984,0.042953574163561825
8893,17788,8894,26682,8.618652105331421,0.042175552225785395
8921,17844,8922,26766,8.645879030227661,0.041457580181827325
8949,17900,8950,26850,8.673803091049194,0.04064700420781264
8976,17954,8977,26931,8.700744152069092,0.03983878457790979
9004,18010,9005,27015,8.730082035064697,0.039097795582279105
9032,18066,9033,27099,8.758937120437622,0.03841230515854477
9059,18120,9060,27180,8.780961990356445,0.037656009157103654
9087,18176,9088,27264,8.809125185012817,0.03691393659460118
9115,18232,9116,27348,8.8353111743927,0.03624804182152275
9143,18288,9144,27432,8.861115217208862,0.03550422795160557
9170,18342,9171,27513,8.887612104415894,0.03489837335007451
9198,18398,9199,27597,8.914819240570068,0.03421070959461758
9226,18454,9227,27681,8.941171169281006,0.03354449749929245
9253,18508,9254,27762,8.964392185211182,0.03292670596408698
9281,18564,9282,27846,8.99210810661316,0.03232874685511433
9309,18620,9310,27930,9.020501136779785,0.03177889001551648
9336,18674,9337,28011,9.048687219619751,0.0311238437755037
9364,18730,9365,28095,9.078456163406372,0.030493538557720967
9392,18786,9393,28179,9.107745170593262,0.029905441075356975
9420,18842,9421,28263,9.135643243789673,0.029218273140600104
9447,18896,9448,28344,9.16053819656372,0.028668189959716983
9475,18952,9476,28428,9.188784122467041,0.028141415776303802
9503,19008,9504,28512,9.213098049163818,0.02762516075745225
9530,19062,9531,28593,9.23681926727295,0.0271185895534245
9558,19118,9559,28677,9.265273094177246,0.02667414999416451
9586,19174,9587,28761,9.289067029953003,0.026147805754703768
9614,19230,9615,28845,9.315514087677002,0.025659909137402792
9641,19284,9642,28926,9.341468334197998,0.025251208634472277
9669,19340,9670,29010,9.366173267364502,0.02476047120342173
9697,19396,9698,29094,9.394100189208984,0.02442449007310188
9724,19450,9725,29175,9.422119140625,0.02389037826446838
9752,19506,9753,29259,9.450075149536133,0.023387890877870632
9780,19562,9781,29343,9.478881120681763,0.02292294312951526
9807,19616,9808,29424,9.503732204437256,0.022549758771674533
9835,19672,9836,29508,9.53240418434143,0.022138989673408105
9863,19728,9864,29592,9.559676170349121,0.021688310679564893
9891,19784,9892,29676,9.588720083236694,0.02132692581540141
9918,19838,9919,29757,9.61478328704834,0.02090360022691584
9946,19894,9947,29841,9.651864051818848,0.020544179296962284
9974,19950,9975,29925,9.679033041000366,0.020107732270730594
10001,20004,10002,30006,9.703642129898071,0.019755908447109505
10029,20060,10030,30090,9.731635332107544,0.019413764479168094
10057,20116,10058,30174,9.758392095565796,0.019093379691526025
10085,20172,10086,30258,9.786338090896606,0.01875741010701404
10112,20226,10113,30339,9.811901330947876,0.018421848884713654
10140,20282,10141,30423,9.845861196517944,0.018070071138595267
10168,20338,10169,30507,9.871158123016357,0.017703016593259235
10195,20392,10196,30588,9.897144079208374,0.017374468407183485
10223,20448,10224,30672,9.92430830001831,0.01701516574280504
10251,20504,10252,30756,9.94895625114441,0.016716161219733294
10278,20558,10279,30837,9.973603248596191,0.01641897920330848
10306,20614,10307,30921,9.99888825416565,0.016114547697043236
10334,20670,10335,31005,10.025790214538574,0.015795907587857982
10362,20726,10363,31089,10.048740148544312,0.015525675678418338
10389,20780,10390,31170,10.075391292572021,0.015267412898992916
10417,20836,10418,31254,10.102866172790527,0.014985340917064605
10445,20892,10446,31338,10.12938904762268,0.01467682628856437
10472,20946,10473,31419,10.152947187423706,0.014445921836113484
10500,21002,10501,31503,10.178368091583252,0.014165557303613241
10528,21058,10529,31587,10.200932264328003,0.013877459398941028
10555,21112,10556,31668,10.224419116973877,0.013642928307717739
10583,21168,10584,31752,10.247849941253662,0.013388561149895395
10611,21224,10612,31836,10.273009300231934,0.013209073472808086
10639,21280,10640,31920,10.296837091445923,0.01287383510998552
10666,21334,10667,32001,10.320914268493652,0.012653237335598533
10694,21390,10695,32085,10.348509311676025,0.012355745248100902
10722,21446,10723,32169,10.378191232681274,0.0121398840016127
10749,21500,10750,32250,10.403655290603638,0.01188898523230364
10777,21556,10778,32334,10.431331157684326,0.011685010835890353
10805,21612,10806,32418,10.456984043121338,0.011438412213465199
10833,21668,10834,32502,10.484262228012085,0.011233861897267161
10860,21722,10861,32583,10.506540060043335,0.011058411448971128
10888,21778,10889,32667,10.532646179199219,0.01081197981011428
10916,21834,10917,32751,10.556749105453491,0.010623916814097356
10943,21888,10944,32832,10.578893184661865,0.010443653739002912
10971,21944,10972,32916,10.604942083358765,0.010244831408272148
10999,22000,11000,33000,10.629993200302124,0.010011277839453214
11026,22054,11027,33081,10.652830362319946,0.009855904899268353
11054,22110,11055,33165,10.681917190551758,0.009678328848281126
11082,22166,11083,33249,10.709084272384644,0.009473877031723532
11110,22222,11111,33333,10.736906051635742,0.009283286975460214
11137,22276,11138,33414,10.763917207717896,0.00910568989274907
11165,22332,11166,33498,10.789997100830078,0.00893972595190462
11193,22388,11194,33582,10.814517974853516,0.0087984648374686
11220,22442,11221,33663,10.83947229385376,0.00862347187432988
11248,22498,11249,33747,10.865342378616333,0.008497609230971648
11276,22554,11277,33831,10.893601179122925,0.008283114295977612
11304,22610,11305,33915,10.918837070465088,0.008132351279073191
11331,22664,11332,33996,10.941429138183594,0.007971428318569451
11359,22720,11360,34080,10.966848134994507,0.007812770838768301
11387,22776,11388,34164,10.99337911605835,0.007674038366417335
11414,22830,11415,34245,11.019044160842896,0.00754855530635723
11442,22886,11443,34329,11.043788194656372,0.007413091637772595
11470,22942,11471,34413,11.067917108535767,0.00727898224602086
11497,22996,11498,34494,11.092756986618042,0.007160927448808252
11525,23052,11526,34578,11.117375373840332,0.007032522906229133
11553,23108,11554,34662,11.142545223236084,0.006904779421802232
11581,23164,11582,34746,11.168327331542969,0.006775902129561473
11608,23218,11609,34827,11.194935083389282,0.0066569392217843415
11636,23274,11637,34911,11.221460342407227,0.0065467100157547975
11664,23330,11665,34995,11.248265266418457,0.0064196003361303156
11691,23384,11692,35076,11.276602268218994,0.006297978671341298
11719,23440,11720,35160,11.310823202133179,0.006191364328287818
11747,23496,11748,35244,11.33568525314331,0.0060705555248432574
11774,23550,11775,35325,11.35779619216919,0.005960226465390406
11802,23606,11803,35409,11.384268045425415,0.0058568297181409434
11830,23662,11831,35493,11.408149003982544,0.005758636874588774
11858,23718,11859,35577,11.430946111679077,0.005654514479942918
11885,23772,11886,35658,11.451589107513428,0.005563314650089524
11913,23828,11914,35742,11.47514820098877,0.0054494514615726075
11941,23884,11942,35826,11.507597208023071,0.005348808073335931
11968,23938,11969,35907,11.535240173339844,0.005251911181403557
11996,23994,11997,35991,11.558746099472046,0.005163814566117253
12024,24050,12025,36075,11.584134101867676,0.005069562366543323
12052,24106,12053,36159,11.607579231262207,0.004967620350271318
12079,24160,12080,36240,11.631842136383057,0.004882100674649337
12107,24216,12108,36324,11.654685258865356,0.004789003208884424
12135,24272,12136,36408,11.679461240768433,0.004698945644804553
12162,24326,12163,36489,11.705031156539917,0.004616364123535277
12190,24382,12191,36573,11.72990894317627,0.0045332488632539025
12218,24438,12219,36657,11.756989240646362,0.004443347414735399
12245,24492,12246,36738,11.779288053512573,0.004366560649373241
12273,24548,12274,36822,11.802694082260132,0.0042939918532738375
12301,24604,12302,36906,11.825706958770752,0.004212064109424318
12329,24660,12330,36990,11.850353240966797,0.004132697908630689
12356,24714,12357,37071,11.87250018119812,0.004036077957039197
12384,24770,12385,37155,11.895758152008057,0.003958004649007307
12412,24826,12413,37239,11.923527240753174,0.0038876010769399727
12439,24880,12440,37320,11.947973251342773,0.003825655805144379
12467,24936,12468,37404,11.971924304962158,0.0037558427980002307
12495,24992,12496,37488,11.994056224822998,0.0036709502185203746
12523,25048,12524,37572,12.018509149551392,0.0036105520399587476
12550,25102,12551,37653,12.041122198104858,0.0035393836483308405
12578,25158,12579,37737,12.06562614440918,0.0034676026832585194
12606,25214,12607,37821,12.090470314025879,0.00339601040332127
12633,25268,12634,37902,12.114280223846436,0.0033338178875510494
12661,25324,12662,37986,12.13633108139038,0.003276454419960828
12689,25380,12690,38070,12.162108182907104,0.003214816239051288
12716,25434,12717,38151,12.185348272323608,0.0031567245235919472
12744,25490,12745,38235,12.210783004760742,0.0030997021721077544
12772,25546,12773,38319,12.23725414276123,0.0030490006378158796
12800,25602,12801,38403,12.264141082763672,0.0029917293669541323
12827,25656,12828,38484,12.290761947631836,0.0029304064084954007
12855,25712,12856,38568,12.31675124168396,0.002874927488960566
12883,25768,12884,38652,12.343955278396606,0.0028258496824946633
12910,25822,12911,38733,12.369264125823975,0.0027694442304664335
12938,25878,12939,38817,12.393898010253906,0.002723388045978936
12966,25934,12967,38901,12.420905351638794,0.002668742191531237
12994,25990,12995,38985,12.44691514968872,0.0026186688728557783
13021,26044,13022,39066,12.472209215164185,0.002574014473339048
13049,26100,13050,39150,12.499651193618774,0.002526244023442814
13077,26156,13078,39234,12.530351161956787,0.0024774910524456573
13104,26210,13105,39315,12.5553719997406,0.0024304486629489475
13132,26266,13133,39399,12.582417249679565,0.002393707117107624
13160,26322,13161,39483,12.610626220703125,0.0023459241484715676
13187,26376,13188,39564,12.635544061660767,0.0023036644219018854
13215,26432,13216,39648,12.66070818901062,0.0022639191830648997
13243,26488,13244,39732,12.686697244644165,0.002219672678961615
13271,26544,13272,39816,12.710216283798218,0.00217924358230448
13298,26598,13299,39897,12.734861135482788,0.0021449375406064064
13326,26654,13327,39981,12.76098108291626,0.002106374964114366
13354,26710,13355,40065,12.787257194519043,0.00206645669095451
13381,26764,13382,40146,12.811132192611694,0.002027527276368346
13409,26820,13410,40230,12.835801124572754,0.0019944218361160893
13437,26876,13438,40314,12.861021280288696,0.0019532263021346807
13464,26930,13465,40395,12.885723114013672,0.0019104986214415476
13492,26986,13493,40479,12.912604331970215,0.0018767463180893174
13520,27042,13521,40563,12.940264225006104,0.0018402836817585921
13548,27098,13549,40647,12.966398239135742,0.0018067761798192805
13575,27152,13576,40728,12.991663217544556,0.0017780421857196416
13603,27208,13604,40812,13.01641321182251,0.0017485735629634291
13631,27264,13632,40896,13.042967081069946,0.0017152663759816278
13658,27318,13659,40977,13.066840171813965,0.0016851465219360762
13686,27374,13687,41061,13.092332124710083,0.001657230416526545
13714,27430,13715,41145,13.11628532409668,0.0016266376159137508
13742,27486,13743,41229,13.143638134002686,0.0015964460636723743
13769,27540,13770,41310,13.174851179122925,0.0015678414488320414
13797,27596,13798,41394,13.20388126373291,0.0015416983395653006
13825,27652,13826,41478,13.226733207702637,0.0015116369460201895
13852,27706,13853,41559,13.250425100326538,0.0014851728416260812
13880,27762,13881,41643,13.274453163146973,0.0014594762537853967
13908,27818,13909,41727,13.295915126800537,0.0014351020624872035
13935,27872,13936,41808,13.317694187164307,0.0014096987363245717
13963,27928,13964,41892,13.33971619606018,0.0013755214714592512
13991,27984,13992,41976,13.36734414100647,0.0013512886259832158
14019,28040,14020,42060,13.39046335220337,0.0013168687778488675
14046,28094,14047,42141,13.411140203475952,0.001294988670906605
14074,28150,14075,42225,13.433037042617798,0.0012716812769895114
14102,28206,14103,42309,13.455631256103516,0.0012486190275922127
14129,28260,14130,42390,13.478150129318237,0.0012286917807386999
14157,28316,14158,42474,13.499829053878784,0.0012070105300381329
14185,28372,14186,42558,13.522906064987183,0.0011843878164654598
14213,28428,14214,42642,13.549633026123047,0.0011613923302320472
14240,28482,14241,42723,13.574531078338623,0.0011435828200774267
14268,28538,14269,42807,13.595169067382812,0.0011227528149220234
14296,28594,14297,42891,13.619397163391113,0.0011004806584651305
14323,28648,14324,42972,13.640095949172974,0.0010817919135206466
14351,28704,14352,43056,13.66241717338562,0.001060374639564543
14379,28760,14380,43140,13.685225248336792,0.0010410932975446485
14406,28814,14407,43221,13.704789161682129,0.0010235986590032553
14434,28870,14435,43305,13.726202249526978,0.0010051432640239
14462,28926,14463,43389,13.746289253234863,0.0009855017866584603
14490,28982,14491,43473,13.7680082321167,0.0009672105151139476
14517,29036,14518,43554,13.790014266967773,0.0009511109362847492
14545,29092,14546,43638,13.81280517578125,0.0009338924860458064
14573,29148,14574,43722,13.833069086074829,0.000916850794851598
14600,29202,14601,43803,13.851853132247925,0.0009016335189926394
14628,29258,14629,43887,13.877360105514526,0.0008815848635777002
14656,29314,14657,43971,13.897704362869263,0.0008648051273212332
14683,29368,14684,44052,13.92150616645813,0.0008494681767388101
14711,29424,14712,44136,13.943263053894043,0.000826369348260414
14739,29480,14740,44220,13.965784072875977,0.0008135907077075899
14767,29536,14768,44304,13.9880952835083,0.0007996155671889937
14794,29590,14795,44385,14.009329319000244,0.0007826018423884307
14822,29646,14823,44469,14.033300399780273,0.0007665089603960951
14850,29702,14851,44553,14.05745816230774,0.0007537257497460814
14877,29756,14878,44634,14.077330350875854,0.0007398570594432385
14905,29812,14906,44718,14.106863260269165,0.0007287284091717083
14933,29868,14934,44802,14.128763198852539,0.0007141684625366906
14961,29924,14962,44886,14.148128986358643,0.0007015723402901131
14988,29978,14989,44967,14.171683073043823,0.0006881973185954848
15016,30034,15017,45051,14.192183017730713,0.000675962314858225
15044,30090,15045,45135,14.215455055236816,0.0006613414670937345
15071,30144,15072,45216,14.234999179840088,0.0006492997870282124
15099,30200,15100,45300,14.263405084609985,0.000636319382124384
15127,30256,15128,45384,14.290868997573853,0.0006243787599942152
15154,30310,15155,45465,14.31221604347229,0.0006124074163835758
15182,30366,15183,45549,14.336841344833374,0.0006014546444248481
15210,30422,15211,45633,14.36016321182251,0.0005914830447864006
15238,30478,15239,45717,14.380365133285522,0.0005784404133919452
15265,30532,15266,45798,14.40210509300232,0.0005678405314029078
15293,30588,15294,45882,14.423915147781372,0.0005591269418800948
15321,30644,15322,45966,14.445572137832642,0.0005482029148424772
15348,30698,15349,46047,14.466154098510742,0.0005395258012867998
15376,30754,15377,46131,14.489819288253784,0.0005279487626239643
15404,30810,15405,46215,14.513472080230713,0.0005189078412968229
15432,30866,15433,46299,14.537757158279419,0.0005086703595225117
15459,30920,15460,46380,14.558234214782715,0.0005007111896020433
15487,30976,15488,46464,14.584810018539429,0.0004910240469371274
15515,31032,15516,46548,14.609713315963745,0.00048190439099471405
15542,31086,15543,46629,14.631912231445312,0.0004727724016220236
15570,31142,15571,46713,14.655231952667236,0.0004643354735662797
15598,31198,15599,46797,14.68007516860962,0.00045566651465378527
15625,31252,15626,46878,14.702394247055054,0.0004485513120471296
15653,31308,15654,46962,14.728318214416504,0.00044041345392997755
15681,31364,15682,47046,14.752803087234497,0.0004314531396403254
15709,31420,15710,47130,14.78127408027649,0.00042542648736798583
15736,31474,15737,47211,14.806275129318237,0.00041734906596957444
15764,31530,15765,47295,14.834227323532104,0.0004095927257594667
15792,31586,15793,47379,14.858636140823364,0.0004018921235910966
15819,31640,15820,47460,14.881899118423462,0.000395204226720125
15847,31696,15848,47544,14.903694152832031,0.0003884546925974064
15875,31752,15876,47628,14.92784833908081,0.00038072075085437973
15903,31808,15904,47712,14.9531409740448,0.0003730760987536996
15930,31862,15931,47793,14.973373174667358,0.0003655193271470125
15958,31918,15959,47877,14.998674154281616,0.00035898505677778303
15986,31974,15987,47961,15.021287202835083,0.000352443790234247
16013,32028,16014,48042,15.043866157531738,0.0003468781342235161
16041,32084,16042,48126,15.064213991165161,0.0003404867391054722
16069,32140,16070,48210,15.088024139404297,0.0003333976424073626
16096,32194,16097,48291,15.109080076217651,0.0003280582847082769
16124,32250,16125,48375,15.128584146499634,0.00032111427287873084
16152,32306,16153,48459,15.154659032821655,0.00031515538876192295
16180,32362,16181,48543,15.17943811416626,0.00030843103468214395
16207,32416,16208,48624,15.204667091369629,0.00030305202869840286
16235,32472,16236,48708,15.233350276947021,0.00029672105699773965
16263,32528,16264,48792,15.26200819015503,0.00029047666089354607
16290,32582,16291,48873,15.291398286819458,0.0002848388630809495
16318,32638,16319,48957,15.317901134490967,0.00027859000556418323
16346,32694,16347,49041,15.3475501537323,0.00027371309113277675
16373,32748,16374,49122,15.37631106376648,0.00026901523540345806
16401,32804,16402,49206,15.41103720664978,0.0002640534275997197
16429,32860,16430,49290,15.450969219207764,0.0002595150784827638
16457,32916,16458,49374,15.493372201919556,0.00025526081947191415
16484,32970,16485,49455,15.531009197235107,0.00025128252536887885
16512,33026,16513,49539,15.56016206741333,0.0002457615137245739
16540,33082,16541,49623,15.583781242370605,0.0002414439941276214
16567,33136,16568,49704,15.607931137084961,0.0002367552314126442
16595,33192,16596,49788,15.635333061218262,0.00023238732023855846
16623,33248,16624,49872,15.662265062332153,0.00022821400011707738
16651,33304,16652,49956,15.68855619430542,0.00022434989625708113
16678,33358,16679,50037,15.712406158447266,0.00021991537880694523
16706,33414,16707,50121,15.737910032272339,0.00021626551313147502
16734,33470,16735,50205,15.761220216751099,0.00021199039247221663
16761,33524,16762,50286,15.785994052886963,0.00020773199764789751
16789,33580,16790,50370,15.809305191040039,0.00020421541364612494
16817,33636,16818,50454,15.836794137954712,0.00020097410936159577
16844,33690,16845,50535,15.85940408706665,0.0001971231002926288
16872,33746,16873,50619,15.885891199111938,0.00019312454878672725
16900,33802,16901,50703,15.911293268203735,0.00018991466583884176
16928,33858,16929,50787,15.940332174301147,0.00018626984376624023
16955,33912,16956,50868,15.969178199768066,0.00018287112334292033
16983,33968,16984,50952,15.999344110488892,0.00017977028267068818
17011,34024,17012,51036,16.02697491645813,0.00017654048110671283
17038,34078,17039,51117,16.05499815940857,0.0001729915060195708
17066,34134,17067,51201,16.09232997894287,0.00017010790213589644
17094,34190,17095,51285,16.122716188430786,0.0001671110563847833
17122,34246,17123,51369,16.155351161956787,0.00016437946965197625
17149,34300,17150,51450,16.18497109413147,0.00016117055042741413
17177,34356,17178,51534,16.206690073013306,0.00015824710862943903
17205,34412,17206,51618,16.22945213317871,0.0001551849175029929
17232,34466,17233,51699,16.250972270965576,0.00015276999374691513
17260,34522,17261,51783,16.270840167999268,0.000150019786019584
17288,34578,17289,51867,16.2953200340271,0.00014680797528399125
17315,34632,17316,51948,16.31498122215271,0.00014449199670707458
17343,34688,17344,52032,16.337212324142456,0.0001418210860038016
17371,34744,17372,52116,16.358834266662598,0.00013939280461272574
17399,34800,17400,52200,16.38262128829956,0.0001363943305250359
17426,34854,17427,52281,16.403253078460693,0.00013421365406429686
17454,34910,17455,52365,16.42362332344055,0.00013217691957834177
17482,34966,17483,52449,16.448291063308716,0.00012918421646190836
17509,35020,17510,52530,16.467221975326538,0.0001267870975425467
17537,35076,17538,52614,16.49146318435669,0.00012485064155498549
17565,35132,17566,52698,16.513527154922485,0.0001219681331576794
17592,35186,17593,52779,16.534902095794678,0.00011988882715741056
17620,35242,17621,52863,16.55510711669922,0.00011753482533549686
17648,35298,17649,52947,16.576682090759277,0.000115515549509837
17676,35354,17677,53031,16.599945306777954,0.00011306521321330365
17703,35408,17704,53112,16.619155168533325,0.00011120169824607729
17731,35464,17732,53196,16.64199924468994,0.00010918967984707706
17759,35520,17760,53280,16.664066076278687,0.00010714316181292816
17786,35574,17787,53361,16.686105251312256,0.00010536588797549484
17814,35630,17815,53445,16.707059144973755,0.00010358388908571214
17842,35686,17843,53529,16.72948122024536,0.00010145428825580893
17870,35742,17871,53613,16.752455234527588,9.939313235918235e-05
17897,35796,17898,53694,16.7773859500885,9.764440937942709e-05
17925,35852,17926,53778,16.806846380233765,9.585132158917986e-05
17953,35908,17954,53862,16.83027195930481,9.41474797855335e-05
17980,35962,17981,53943,16.85122513771057,9.259061982902494e-05
18008,36018,18009,54027,16.877024173736572,9.083993347758224e-05
18036,36074,18037,54111,16.89958119392395,8.91626165184789e-05
18063,36128,18064,54192,16.92099094390869,8.771070895363664e-05
18091,36184,18092,54276,16.944321155548096,8.609217798039026e-05
18119,36240,18120,54360,17.03759527206421,8.446861602351419e-05
18147,36296,18148,54444,17.059890270233154,8.270004582300317e-05
18174,36350,18175,54525,17.07925295829773,8.144528896991687e-05
18202,36406,18203,54609,17.100958347320557,7.999300453320757e-05
18230,36462,18231,54693,17.119803190231323,7.844937908885186e-05
18257,36516,18258,54774,17.13989233970642,7.71947121620542e-05
18285,36572,18286,54858,17.160617351531982,7.555681827398075e-05
18313,36628,18314,54942,17.1807701587677,7.390646067051421e-05
18341,36684,18342,55026,17.200085163116455,7.254420506797032e-05
18368,36738,18369,55107,17.218356370925903,7.125431704935181e-05
18396,36794,18397,55191,17.24160099029541,7.033172789761011e-05
18424,36850,18425,55275,17.260990381240845,6.874086079733388e-05
18451,36904,18452,55356,17.283583402633667,6.745865630364278e-05
18479,36960,18480,55440,17.305256366729736,6.616018117711064e-05
18507,37016,18508,55524,17.327458143234253,6.481920740952773e-05
18534,37070,18535,55605,17.348226070404053,6.353203616527026e-05
18562,37126,18563,55689,17.36776113510132,6.2375406969295e-05
18590,37182,18591,55773,17.391239166259766,6.129492396667047e-05
18618,37238,18619,55857,17.412877082824707,6.021782030529721e-05
18645,37292,18646,55938,17.43406915664673,5.9017326179855445e-05
18673,37348,18674,56022,17.45603108406067,5.7675523180478194e-05
18701,37404,18702,56106,17.477459192276,5.671579492627643e-05
18728,37458,18729,56187,17.49916124343872,5.561318448599195e-05
18756,37514,18757,56271,17.520507097244263,5.441081736989872e-05
18784,37570,18785,56355,17.544991970062256,5.336737581274065e-05
18811,37624,18812,56436,17.565855979919434,5.2403360768948914e-05
18839,37680,18840,56520,17.59119415283203,5.143566374954389e-05
18867,37736,18868,56604,17.610488176345825,5.050450101862225e-05
18895,37792,18896,56688,17.633098125457764,4.951173866629688e-05
18922,37846,18923,56769,17.652668237686157,4.873654302173236e-05
18950,37902,18951,56853,17.67254614830017,4.781592497238307e-05
18978,37958,18979,56937,17.695624351501465,4.686658280661504e-05
19005,38012,19006,57018,17.714227199554443,4.614131489688589e-05
19033,38068,19034,57102,17.734788179397583,4.5351707399277075e-05
19061,38124,19062,57186,17.753865242004395,4.4553717316375696e-05
19089,38180,19090,57270,17.772517204284668,4.373292529180617e-05
19116,38234,19117,57351,17.794178009033203,4.2998175672437355e-05
19144,38290,19145,57435,17.814305067062378,4.224437645916623e-05
19172,38346,19173,57519,17.835864067077637,4.1320122363686096e-05
19199,38400,19200,57600,17.857025146484375,4.063301844325906e-05
19227,38456,19228,57684,17.878644943237305,3.956099862989504e-05
19255,38512,19256,57768,17.899935007095337,3.8906461554688576e-05
19282,38566,19283,57849,17.918339014053345,3.816365165221214e-05
19310,38622,19311,57933,17.93884515762329,3.7512362951019895e-05
19338,38678,19339,58017,17.958896160125732,3.643594732238853e-05
19366,38734,19367,58101,17.981353282928467,3.580665338631661e-05
19393,38788,19394,58182,18.00074601173401,3.518697235449508e-05
19421,38844,19422,58266,18.022192239761353,3.454984573636466e-05
19449,38900,19450,58350,18.044355154037476,3.399990578145662e-05
19476,38954,19477,58431,18.06330418586731,3.342804859585158e-05
19504,39010,19505,58515,18.084084272384644,3.2799817859086033e-05
19532,39066,19533,58599,18.103824138641357,3.21748198075511e-05
19560,39122,19561,58683,18.123342037200928,3.157387868668593e-05
19587,39176,19588,58764,18.145576238632202,3.106290159848868e-05
19615,39232,19616,58848,18.167498111724854,3.046230801828642e-05
19643,39288,19644,58932,18.19278621673584,2.9915203640484833e-05
19670,39342,19671,59013,18.2138192653656,2.9444276947288017e-05
19698,39398,19699,59097,18.23986506462097,2.892571274060174e-05
19726,39454,19727,59181,18.261413097381592,2.839296507772815e-05
19753,39508,19754,59262,18.285269021987915,2.78912730209413e-05
19781,39564,19782,59346,18.306682109832764,2.7345707735548785e-05
19809,39620,19810,59430,18.329870223999023,2.6917774448520504e-05
19837,39676,19838,59514,18.354345321655273,2.6356369744462427e-05
19864,39730,19865,59595,18.376697063446045,2.587898734418559e-05
19892,39786,19893,59679,18.400330066680908,2.5460000301791297e-05
19920,39842,19921,59763,18.424073219299316,2.4971999664558098e-05
19947,39896,19948,59844,18.446746110916138,2.4516197754564928e-05
19975,39952,19976,59928,18.46800923347473,2.4061977796918654e-05
20003,40008,20004,60012,18.49190616607666,2.366276839893544e-05
20031,40064,20032,60096,18.51272439956665,2.3268588847713545e-05
20058,40118,20059,60177,18.535322189331055,2.280571561641409e-05
20086,40174,20087,60261,18.55672597885132,2.2372660055225424e-05
20114,40230,20115,60345,18.579366207122803,2.18888919789606e-05
20141,40284,20142,60426,18.60024118423462,2.151325270460802e-05
20169,40340,20170,60510,18.623353242874146,2.116476446190063e-05
20197,40396,20198,60594,18.645437240600586,2.076949795082328e-05
20224,40450,20225,60675,18.668039321899414,2.038305729001877e-05
20252,40506,20253,60759,18.693255186080933,2.0001176494588435e-05
20280,40562,20281,60843,18.71615719795227,1.958947927960253e-05
20308,40618,20309,60927,18.738429307937622,1.9168227481713984e-05
20335,40672,20336,61008,18.76139211654663,1.8838174128177343e-05
20363,40728,20364,61092,18.784212350845337,1.8424779341330577e-05
20391,40784,20392,61176,18.804254293441772,1.8094327401740884e-05
20418,40838,20419,61257,18.823647022247314,1.782031017683039e-05
20446,40894,20447,61341,18.844423294067383,1.7443009483031346e-05
20474,40950,20475,61425,18.866457223892212,1.7136960195784923e-05
20501,41004,20502,61506,18.887078285217285,1.6852812677825568e-05
20529,41060,20530,61590,18.911709308624268,1.651885622777627e-05
20557,41116,20558,61674,18.936569213867188,1.6207103158194514e-05
20585,41172,20586,61758,18.959107160568237,1.5894245962044806e-05
20612,41226,20613,61839,19.03662109375,1.5586390645694337e-05
20640,41282,20641,61923,19.071868181228638,1.532786529878649e-05
20668,41338,20669,62007,19.095790147781372,1.5055243693495868e-05
20695,41392,20696,62088,19.11725425720215,1.490363843004161e-05
20723,41448,20724,62172,19.138249158859253,1.4451106267188152e-05
20751,41504,20752,62256,19.158860206604004,1.4175433648233593e-05
20779,41560,20780,62340,19.179696083068848,1.3900928706789273e-05
20806,41614,20807,62421,19.1996111869812,1.3678119671567401e-05
20834,41670,20835,62505,19.220736980438232,1.3411400459517608e-05
20862,41726,20863,62589,19.244043111801147,1.3140315104465117e-05
20889,41780,20890,62670,19.263323307037354,1.293959519443888e-05
20917,41836,20918,62754,19.285704135894775,1.268692858502618e-05
20945,41892,20946,62838,19.306133031845093,1.2467431020013464e-05
20972,41946,20973,62919,19.326436042785645,1.2257028856765828e-05
21000,42002,21001,63003,19.3478901386261,1.2025349064970214e-05
21028,42058,21029,63087,19.36734414100647,1.1804127325376612e-05
21056,42114,21057,63171,19.39073920249939,1.1576594715734245e-05
21083,42168,21084,63252,19.40908718109131,1.1314332709844166e-05
21111,42224,21112,63336,19.430596113204956,1.1117403914795432e-05
21139,42280,21140,63420,19.451919078826904,1.0933238058896677e-05
21166,42334,21167,63501,19.470147132873535,1.0753521792139509e-05
21194,42390,21195,63585,19.490941286087036,1.0542645895839087e-05
21222,42446,21223,63669,19.510687112808228,1.0351013656872965e-05
21250,42502,21251,63753,19.53142499923706,1.017925546875631e-05
21277,42556,21278,63834,19.549975156784058,9.995575283028302e-06
21305,42612,21306,63918,19.569111108779907,9.803191687751678e-06
21333,42668,21334,64002,19.59092617034912,9.595087703928584e-06
21360,42722,21361,64083,19.609430074691772,9.434793696527777e-06
21388,42778,21389,64167,19.630467176437378,9.250071002497862e-06
21416,42834,21417,64251,19.660685062408447,9.089655804928043e-06
21443,42888,21444,64332,19.684868097305298,8.923213272282737e-06
21471,42944,21472,64416,19.70859122276306,8.771624266046274e-06
21499,43000,21500,64500,19.731942176818848,8.596329962529126e-06
21527,43056,21528,64584,19.755104064941406,8.439138127869228e-06
21554,43110,21555,64665,19.776244163513184,8.300383910864184e-06
21582,43166,21583,64749,19.796136140823364,8.140651971189072e-06
21610,43222,21611,64833,19.815309047698975,7.986729087861022e-06
21637,43276,21638,64914,19.840618133544922,7.833631912035344e-06
21665,43332,21666,64998,19.869929313659668,7.684920092287939e-06
21693,43388,21694,65082,19.90418815612793,7.538177555943548e-06
21720,43442,21721,65163,19.93033719062805,7.3998558036691975e-06
21748,43498,21749,65247,19.953477144241333,7.2706512810327695e-06
21776,43554,21777,65331,19.979318141937256,7.14130510459654e-06
21804,43610,21805,65415,20.0085871219635,7.0173973654164e-06
21831,43664,21832,65496,20.037707090377808,6.8922679474781035e-06
21859,43720,21860,65580,20.065237998962402,6.747534598616767e-06
21887,43776,21888,65664,20.092122077941895,6.6342644231554004e-06
21914,43830,21915,65745,20.114522218704224,6.503494773824059e-06
21942,43886,21943,65829,20.13832116127014,6.385905408023973e-06
21970,43942,21971,65913,20.1588191986084,6.266907234930841e-06
21998,43998,21999,65997,20.180113315582275,6.129268854238035e-06
22025,44052,22026,66078,20.20172119140625,6.032995997884427e-06
22053,44108,22054,66162,20.222175121307373,5.909618380428583e-06
22081,44164,22082,66246,20.247762203216553,5.811124879073759e-06
22108,44218,22109,66327,20.26716637611389,5.6954286264954135e-06
22136,44274,22137,66411,20.290878295898438,5.586522206613154e-06
22164,44330,22165,66495,20.311838150024414,5.491110300681612e-06
22191,44384,22192,66576,20.333884239196777,5.383754114518524e-06
22219,44440,22220,66660,20.35724902153015,5.287417366162117e-06
22247,44496,22248,66744,20.378576278686523,5.197323957872868e-06
22275,44552,22276,66828,20.402085065841675,5.090239142191422e-06
22302,44606,22303,66909,20.42308521270752,4.996816528546333e-06
22330,44662,22331,66993,20.44649910926819,4.90639149575145e-06
22358,44718,22359,67077,20.466233253479004,4.815032298211008e-06
22385,44772,22386,67158,20.48797106742859,4.719687240140047e-06
22413,44828,22414,67242,20.507166147232056,4.6395874733207165e-06
22441,44884,22442,67326,20.52649426460266,4.528533509073895e-06
22469,44940,22470,67410,20.55652618408203,4.460878699319437e-06
22496,44994,22497,67491,20.58320713043213,4.377905838737206e-06
22524,45050,22525,67575,20.602959156036377,4.287634396860085e-06
22552,45106,22553,67659,20.625761032104492,4.209962526147137e-06
22579,45160,22580,67740,20.646667003631592,4.133726747568289e-06
22607,45216,22608,67824,20.665995121002197,4.052953954669647e-06
22635,45272,22636,67908,20.68818712234497,3.982810198976949e-06
22662,45326,22663,67989,20.708990335464478,3.900672822965134e-06
22690,45382,22691,68073,20.73417019844055,3.822268354269909e-06
22718,45438,22719,68157,20.75531315803528,3.748897711375321e-06
22746,45494,22747,68241,20.788517236709595,3.679128553812916e-06
22773,45548,22774,68322,20.808711290359497,3.622400186031882e-06
22801,45604,22802,68406,20.836037158966064,3.5445102639641846e-06
22829,45660,22830,68490,20.8565571308136,3.490911240078276e-06
22856,45714,22857,68571,20.878221035003662,3.413610329516814e-06
22884,45770,22885,68655,20.900418043136597,3.3514880897200783e-06
22912,45826,22913,68739,20.92010521888733,3.290509880571335e-06
22939,45880,22940,68820,20.94679617881775,3.2253407198368222e-06
22967,45936,22968,68904,20.969382286071777,3.1635827326681465e-06
22995,45992,22996,68988,21.00130033493042,3.1025379030324984e-06
23023,46048,23024,69072,21.021065950393677,3.0475114272121573e-06
23050,46102,23051,69153,21.04791808128357,2.9965548264954123e-06
23078,46158,23079,69237,21.07033109664917,2.936366058747808e-06
23106,46214,23107,69321,21.100560188293457,2.8853811500084703e-06
23133,46268,23134,69402,21.12225914001465,2.829694039974129e-06
23161,46324,23162,69486,21.14666223526001,2.778377961476508e-06
23189,46380,23190,69570,21.16882610321045,2.7243669364906964e-06
23217,46436,23218,69654,21.198824167251587,2.672836785677646e-06
23244,46490,23245,69735,21.217530250549316,2.6136460746783996e-06
23272,46546,23273,69819,21.24640417098999,2.5664184022389236e-06
23300,46602,23301,69903,21.267471075057983,2.517653797440289e-06
23327,46656,23328,69984,21.28837013244629,2.472761593708128e-06
23355,46712,23356,70068,21.307223081588745,2.418976578155707e-06
23383,46768,23384,70152,21.333214282989502,2.3749340698486776e-06
23410,46822,23411,70233,21.355006217956543,2.3342446411334095e-06
23438,46878,23439,70317,21.378380060195923,2.2840954443381634e-06
23466,46934,23467,70401,21.40373134613037,2.2400678290068754e-06
23494,46990,23495,70485,21.423359394073486,2.1994309236106346e-06
23521,47044,23522,70566,21.451011180877686,2.155086235688941e-06
23549,47100,23550,70650,21.470518112182617,2.1073957441331004e-06
23577,47156,23578,70734,21.494027137756348,2.068896151286026e-06
23604,47210,23605,70815,21.513630151748657,2.030544692388503e-06
23632,47266,23633,70899,21.536607027053833,1.9908954982383875e-06
23660,47322,23661,70983,21.557760000228882,1.957468043656263e-06
23688,47378,23689,71067,21.578994274139404,1.9142058818033547e-06
23715,47432,23716,71148,21.59985113143921,1.876380679277645e-06
23743,47488,23744,71232,21.619001150131226,1.83714462309581e-06
23771,47544,23772,71316,21.65002703666687,1.8028047179541318e-06
23798,47598,23799,71397,21.668360233306885,1.7617506955502904e-06
23826,47654,23827,71481,21.70004916191101,1.7320246570307063e-06
23854,47710,23855,71565,21.72639012336731,1.696181925581186e-06
23881,47764,23882,71646,21.747079133987427,1.66506083587592e-06
23909,47820,23910,71730,21.76650905609131,1.6287967810058035e-06
23937,47876,23938,71814,21.78846311569214,1.5976602298906073e-06
23965,47932,23966,71898,21.808138132095337,1.560801479172369e-06
23992,47986,23993,71979,21.838760137557983,1.5343898667197209e-06
24020,48042,24021,72063,21.859254121780396,1.4988157772677368e-06
24048,48098,24049,72147,21.890302181243896,1.4670516748083173e-06
24075,48152,24076,72228,21.91069531440735,1.4390788010132383e-06
24103,48208,24104,72312,21.937729120254517,1.4069631788515835e-06
24131,48264,24132,72396,21.95745301246643,1.379764398734551e-06
24159,48320,24160,72480,21.977827072143555,1.351008563688083e-06
24186,48374,24187,72561,22.00026535987854,1.3263465916679706e-06
24214,48430,24215,72645,22.0195951461792,1.2989352171643986e-06
24242,48486,24243,72729,22.044079065322876,1.2731193237414118e-06
24269,48540,24270,72810,22.06304931640625,1.2508345434980583e-06
24297,48596,24298,72894,22.096562147140503,1.2245232028362807e-06
24325,48652,24326,72978,22.115764379501343,1.1988752248726087e-06
24352,48706,24353,73059,22.138880014419556,1.177443209599005e-06
24380,48762,24381,73143,22.158903121948242,1.1532148391779629e-06
24408,48818,24409,73227,22.179235219955444,1.1272898063907633e-06
24436,48874,24437,73311,22.203140258789062,1.104793000195059e-06
24463,48928,24464,73392,22.223124980926514,1.0849369118659524e-06
24491,48984,24492,73476,22.246652126312256,1.063354943653394e-06
24519,49040,24520,73560,22.268081188201904,1.0420319540571654e-06
24546,49094,24547,73641,22.300719261169434,1.0212714869339834e-06
24574,49150,24575,73725,22.320056200027466,9.982962865251466e-07
24602,49206,24603,73809,22.347124338150024,9.714804036775604e-07
24629,49260,24630,73890,22.366733074188232,9.535970093565993e-07
24657,49316,24658,73974,22.386763095855713,9.309056849815533e-07
24685,49372,24686,74058,22.405622005462646,9.131551905738888e-07
24713,49428,24714,74142,22.424840211868286,8.935774076235248e-07
24740,49482,24741,74223,22.442711114883423,8.779844620221411e-07
24768,49538,24769,74307,22.46216917037964,8.555845170121756e-07
24796,49594,24797,74391,22.483342170715332,8.39458607515553e-07
24823,49648,24824,74472,22.502527952194214,8.211877684516367e-07
24851,49704,24852,74556,22.521119117736816,8.068566330621252e-07
24879,49760,24880,74640,22.54176115989685,7.876420795582817e-07
24907,49816,24908,74724,22.56036615371704,7.692217423027614e-07
24934,49870,24935,74805,22.581789255142212,7.547147333752946e-07
24962,49926,24963,74889,22.60028910636902,7.372403842964559e-07
24990,49982,24991,74973,22.62061905860901,7.19064928489388e-07
25017,50036,25018,75054,22.638657093048096,7.026999355730368e-07
25045,50092,25046,75138,22.657097339630127,6.873002575957798e-07
25073,50148,25074,75222,22.675401210784912,6.719066050209221e-07
25100,50202,25101,75303,22.693665027618408,6.598195341211976e-07
25128,50258,25129,75387,22.71160912513733,6.428946335290675e-07
25156,50314,25157,75471,22.73012614250183,6.284421942837071e-07
25184,50370,25185,75555,22.748688220977783,6.135030616860604e-07
25211,50424,25212,75636,22.766526222229004,6.019149623170961e-07
25239,50480,25240,75720,22.788652181625366,5.884105576114962e-07
25267,50536,25268,75804,22.807037353515625,5.771768201157101e-07
25294,50590,25295,75885,22.828202962875366,5.630882924378966e-07
25322,50646,25323,75969,22.850134134292603,5.492082664204645e-07
25350,50702,25351,76053,22.869577169418335,5.341120186130865e-07
25378,50758,25379,76137,22.893025159835815,5.220271077632788e-07
25405,50812,25406,76218,22.912606239318848,5.058610668129404e-07
25433,50868,25434,76302,22.932220220565796,4.912858457828406e-07
25461,50924,25462,76386,22.952024221420288,4.812744691662374e-07
25488,50978,25489,76467,22.971140146255493,4.6726472646696493e-07
25516,51034,25517,76551,22.992119073867798,4.5633487388840877e-07
25544,51090,25545,76635,23.0102322101593,4.456192073121201e-07
25571,51144,25572,76716,23.02943205833435,4.3300678953528404e-07
25599,51200,25600,76800,23.048673152923584,4.238079327478772e-07
25627,51256,25628,76884,23.06871509552002,4.1130931549560046e-07
25655,51312,25656,76968,23.08830428123474,4.016386583316489e-07
25682,51366,25683,77049,23.10685896873474,3.9256212858163053e-07
25710,51422,25711,77133,23.12608003616333,3.825081194008817e-07
25738,51478,25739,77217,23.14479899406433,3.7295956190064317e-07
25765,51532,25766,77298,23.16411805152893,3.6412745885172626e-07
25793,51588,25794,77382,23.18424916267395,3.540733359841397e-07
25821,51644,25822,77466,23.206477165222168,3.4470178889023373e-07
25848,51698,25849,77547,23.227795362472534,3.370844297023723e-07
25876,51754,25877,77631,23.248380184173584,3.2892103263293393e-07
25904,51810,25905,77715,23.270203113555908,3.1959564239514293e-07
25932,51866,25933,77799,23.29250717163086,3.111078967776848e-07
25959,51920,25960,77880,23.31305432319641,3.0354260616149986e-07
25987,51976,25988,77964,23.331570148468018,2.954379851871636e-07
26015,52032,26016,78048,23.349744081497192,2.872377535823034e-07
26042,52086,26043,78129,23.36848521232605,2.8089766601624433e-07
26070,52142,26071,78213,23.391951084136963,2.7139140001963824e-07
26098,52198,26099,78297,23.41035532951355,2.6442012313054875e-07
26126,52254,26127,78381,23.4289231300354,2.568542640801752e-07
26153,52308,26154,78462,23.449515104293823,2.4909127205319237e-07
26181,52364,26182,78546,23.468569040298462,2.430972472211579e-07
26209,52420,26210,78630,23.49342632293701,2.3573375074192882e-07
26236,52474,26237,78711,23.512142181396484,2.2941230781725608e-07
26264,52530,26265,78795,23.530887126922607,2.2131439436634537e-07
26292,52586,26293,78879,23.550523281097412,2.151747366951895e-07
26319,52640,26320,78960,23.570176124572754,2.0812228740396677e-07
26347,52696,26348,79044,23.594755172729492,2.0041863990627462e-07
26375,52752,26376,79128,23.613352298736572,1.948430963238934e-07
26403,52808,26404,79212,23.635149002075195,1.8890386854764074e-07
26430,52862,26431,79293,23.65655517578125,1.8350272057432448e-07
26458,52918,26459,79377,23.676483154296875,1.7683885289443424e-07
26486,52974,26487,79461,23.698671102523804,1.7130059859482571e-07
26513,53028,26514,79542,23.71691918373108,1.6483738818351412e-07
26541,53084,26542,79626,23.73634934425354,1.5944965525704902e-07
26569,53140,26570,79710,23.75484323501587,1.5368084405054105e-07
26597,53196,26598,79794,23.77335023880005,1.4803890735493042e-07
26624,53250,26625,79875,23.793626070022583,1.4355327948578633e-07
26652,53306,26653,79959,23.81164312362671,1.384504457746516e-07
26680,53362,26681,80043,23.831847190856934,1.3337501059140777e-07
26707,53416,26708,80124,23.851325273513794,1.2908367352792993e-07
26735,53472,26736,80208,23.86991834640503,1.2422924555721693e-07
26763,53528,26764,80292,23.889081239700317,1.197071242131642e-07
26790,53582,26791,80373,23.90705108642578,1.1509837349876761e-07
26818,53638,26819,80457,23.92680335044861,1.1063161764468532e-07
26846,53694,26847,80541,23.945966243743896,1.06514448816597e-07
26874,53750,26875,80625,23.964279174804688,1.0119697435584385e-07
26901,53804,26902,80706,23.984554052352905,9.871507700154325e-08
26929,53860,26930,80790,24.002838134765625,9.255427357857116e-08
26957,53916,26958,80874,24.021290063858032,8.82423591974657e-08
26984,53970,26985,80955,24.039764165878296,8.43772340886062e-08
27012,54026,27013,81039,24.059559106826782,7.987227945704944e-08
27040,54082,27041,81123,24.08005404472351,7.610992724949028e-08
27067,54136,27068,81204,24.099643230438232,7.19066974852467e-08
27095,54192,27096,81288,24.11896324157715,6.788070550101111e-08
27123,54248,27124,81372,24.14459800720215,6.379400474543218e-08
27151,54304,27152,81456,24.16301417350769,5.991171292407671e-08
27178,54358,27179,81537,24.18171215057373,5.627305199595867e-08
27206,54414,27207,81621,24.201255321502686,5.284073267830536e-08
27234,54470,27235,81705,24.219962120056152,4.88716977997683e-08
27261,54524,27262,81786,24.240989208221436,4.5746446630801074e-08
27289,54580,27290,81870,24.262890100479126,4.2601982386258896e-08
27317,54636,27318,81954,24.29202103614807,3.9315182220889255e-08
27345,54692,27346,82038,24.31822633743286,3.584307251003338e-08
27372,54746,27373,82119,24.343953132629395,3.309992280264851e-08
27400,54802,27401,82203,24.37060523033142,2.9627244657604024e-08
27428,54858,27429,82287,24.398126125335693,2.585966285550967e-08
27455,54912,27456,82368,24.417197227478027,2.3124016479414422e-08
27483,54968,27484,82452,24.439725160598755,1.9924755179090425e-08
27511,55024,27512,82536,24.458341121673584,1.6909666555875447e-08
27538,55078,27539,82617,24.47724223136902,1.4345232557388954e-08
27566,55134,27567,82701,24.497626066207886,1.1582187653402798e-08
27594,55190,27595,82785,24.516467332839966,8.494907888234593e-09
27622,55246,27623,82869,24.53535509109497,5.682295523001812e-09
27649,55300,27650,82950,24.55495810508728,2.7974920158158056e-09
27677,55356,27678,83034,24.57558298110962,3.7971403799019754e-11


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012929439544677734,2181.4194943796983
1001,2003,2002,4005,2.083881139755249,35.469008324394736
2002,4005,4004,8009,3.7600128650665283,34.40807984936259
3003,6007,6006,12013,5.381834030151367,33.40915906251007
4004,8009,8008,16017,6.823575973510742,32.46649241354112
5005,10011,10010,20021,8.367573022842407,31.574817185092343
6006,12013,12012,24025,10.655004978179932,30.729356494634658
7007,14015,14014,28029,13.033334016799927,29.925806080461598
8008,16017,16016,32033,14.922853946685791,29.160312226378892
9009,18019,18018,36037,17.020570993423462,28.429442473491918
10010,20021,20020,40041,18.604860067367554,27.730151575056198
11011,22023,22022,44045,20.18110489845276,27.05974513210731
12012,24025,24024,48049,21.71625304222107,26.415842942091558
13013,26027,26026,52053,23.18020987510681,25.796343564906238
14014,28029,28028,56057,24.672911882400513,25.199391102974914
15015,30031,30030,60061,26.131555795669556,24.62334476796559
16016,32033,32032,64065,27.623703956604004,24.066751484178212
17017,34035,34034,68069,29.105128049850464,23.528321551468252
18018,36037,36036,72073,30.58879804611206,23.00690724257811
19019,38039,38038,76077,32.114301919937134,22.501484122476768
20020,40041,40040,80081,33.72951793670654,22.011134833710912
21021,42043,42042,84085,35.22915315628052,21.53503507780397
22022,44045,44044,88089,36.72470784187317,21.07244152781209
23023,46047,46046,92093,38.18768119812012,20.622681423360746
24024,48049,48048,96097,39.694260120391846,20.18514362154656
25025,50051,50050,100101,41.20482683181763,19.759270901450236
26026,52053,52052,104105,42.723315954208374,19.344553344373935
27027,54055,54054,108109,44.233383893966675,18.94052263505432
28028,56057,56056,112113,45.79564189910889,18.546747150268857
29029,58059,58058,116117,47.311460971832275,18.16283425082861
30030,60061,60060,120121,48.81859302520752,17.788409349263247
31031,62063,62062,124125,50.32033395767212,17.42312502340951
32032,64065,64064,128129,51.78358197212219,17.066659395597753
33033,66067,66066,132133,53.26893186569214,16.718711055442327
34034,68069,68068,136137,54.753591775894165,16.378996975641485
35035,70071,70070,140141,56.22053575515747,16.047250692088596
36036,72073,72072,144145,57.750038146972656,15.723220711224826
37037,74075,74074,148149,59.27613091468811,15.406669113086082
38038,76077,76076,152153,60.7823760509491,15.097370323150471
39039,78079,78078,156157,62.327457904815674,14.795110030047113
40040,80081,80080,160161,63.81347990036011,14.499684229522131
41041,82083,82082,164165,65.2956600189209,14.210898377900776
42042,84085,84084,168169,66.79907393455505,13.928566640679605
43043,86087,86086,172173,68.30095076560974,13.652511223918623
44044,88089,88088,176177,69.80014085769653,13.382561777846263
45045,90091,90090,180181,71.35210800170898,13.118554863542954
46046,92093,92092,184185,72.86093282699585,12.860333474838967
47047,94095,94094,188189,74.35861301422119,12.607746608625234
48048,96097,96096,192193,75.85052704811096,12.360648877686799
49049,98099,98098,196197,77.35159087181091,12.118900160955377
50050,100101,100100,200201,78.83917713165283,11.882365286744289
51051,102103,102102,204205,80.308434009552,11.65091374510655
52052,104105,104104,208209,81.79112887382507,11.424419425951896
53053,106107,106106,212213,83.31579494476318,11.202760379985875
54054,108109,108108,216217,84.82643795013428,10.985818599903496
55055,110111,110110,220221,86.52674698829651,10.773479819588829
56056,112113,112112,224225,88.25576210021973,10.565633329353773
57057,114115,114114,228229,89.87662601470947,10.362171805483285
58058,116117,116116,232233,91.5476450920105,10.162991152574818
59059,118119,118118,236237,93.23581385612488,9.96799035733693
60060,120121,120120,240241,94.82266616821289,9.777071352677467
61061,122123,122122,244245,96.33524990081787,9.59013889105222
62062,124125,124124,248249,97.79210710525513,9.407100426173315
63063,126127,126126,252253,99.27154111862183,9.227866002281985
64064,128129,128128,256257,100.75854897499084,9.052348150292346
65065,130131,130130,260261,102.22938990592957,8.880461790195795
66066,132133,132132,264265,103.87586688995361,8.71212413919261
67067,134135,134134,268269,105.56757998466492,8.547254625079518
68068,136137,136136,272273,107.23592495918274,8.385774804486573
69069,138139,138138,276277,108.9399528503418,8.227608285596375
70070,140141,140140,280281,111.11850094795227,8.072680655033082
71071,142143,142142,284285,113.05877208709717,7.920919408630425
72072,144145,144144,288289,114.5725519657135,7.772253885831674
73073,146147,146146,292293,116.02846002578735,7.626615207490545
74074,148149,148148,296297,117.48810982704163,7.483936216864095
75075,150151,150150,300301,118.9675281047821,7.344151423606263
76076,152153,152152,304305,120.4232349395752,7.207196950584375
77077,154155,154154,308309,121.91765594482422,7.07301048334466
78078,156157,156156,312313,123.36713409423828,6.941531222071831
79079,158159,158158,316317,124.82455205917358,6.812699835883905
80080,160161,160160,320321,126.3263030052185,6.686458419317773
81081,162163,162162,324325,127.78291320800781,6.562750450860449
82082,164165,164164,328329,129.29141211509705,6.441520753393206
83083,166167,166166,332333,130.75920796394348,6.322715456413903
84084,168169,168168,336337,132.22711086273193,6.206281959916623
85085,170171,170170,340341,133.69375705718994,6.092168899808144
86086,172173,172172,344345,135.20442390441895,5.980326114754462
87087,174175,174174,348349,136.66602206230164,5.870704614348256
88088,176177,176176,352353,138.15738987922668,5.763256548507343
89089,178179,178178,356357,139.6510307788849,5.65793517801319
90090,180181,180180,360361,141.17385601997375,5.554694846107395
91091,182183,182182,364365,142.70920515060425,5.453490951075423
92092,184185,184184,368369,144.49027681350708,5.354279919749274
93093,186187,186186,372373,146.2180609703064,5.257019181869168
94094,188189,188188,376377,147.8789598941803,5.161667145250817
95095,190191,190190,380381,149.55553603172302,5.0681831717073464
96096,192193,192192,384385,151.38532400131226,4.976527553688356
97097,194195,194194,388389,152.936940908432,4.886661491588143
98098,196197,196196,392393,154.8321931362152,4.798547071696703
99099,198199,198198,396397,156.51292991638184,4.712147244757261
100100,200201,200200,400401,158.12949681282043,4.627425805103599
101101,202203,202202,404405,159.7592761516571,4.544347370351716
102102,204205,204204,408409,161.38389587402344,4.462877361623441
103103,206207,206206,412413,162.9303059577942,4.382981984279695
104104,208209,208208,416417,164.49662899971008,4.304628209147609
105105,210211,210210,420421,166.30677890777588,4.227783754217853
106106,212213,212212,424425,168.0950129032135,4.152417066806038
107107,214215,214214,428429,169.67587113380432,4.078497306154077
108108,216217,216216,432433,171.26953601837158,4.005994326462201
109109,218219,218218,436437,172.9979898929596,3.9348786603396775
110110,220221,220220,440441,174.49671292304993,3.8651215026609407
111111,222223,222222,444445,176.18326210975647,3.7966946948155282
112112,224225,224224,448449,177.72758507728577,3.729570709342397
113113,226227,226226,452453,179.26203083992004,3.6637226349374714
114114,228229,228228,456457,180.74593901634216,3.599124161827376
115115,230231,230230,460461,182.2393307685852,3.535749567495145
116116,232233,232232,464465,183.91442394256592,3.4735737027557434
117117,234235,234234,468469,185.79115295410156,3.4125719781663975
118118,236237,236236,472473,187.85199284553528,3.3527203507696868
119119,238239,238238,476477,189.4576530456543,3.293995311154731
120120,240241,240240,480481,191.7632598876953,3.2363738708371557
121121,242243,242242,484485,194.07678604125977,3.1798335499411223
122122,244245,244244,488489,196.22145700454712,3.1243523651841087
123123,246247,246246,492493,198.05195093154907,3.069908818152385
124124,248249,248248,496497,199.80928707122803,3.01648188386298
125125,250251,250250,500501,201.94151210784912,2.964050999602705
126126,252253,252252,504505,203.71742391586304,2.912596054041387
127127,254255,254254,508509,205.3281009197235,2.862097376609313
128128,256257,256256,512513,206.99701404571533,2.8125357271352414
129129,258259,258258,516517,208.6107521057129,2.7638922857354373
130130,260261,260260,520521,211.1240200996399,2.7161486429528168
131131,262263,262262,524525,214.37007808685303,2.6692867901351747
132132,264265,264264,528529,216.9112949371338,2.623289110049768
133133,266267,266266,532533,219.82853198051453,2.578138367727661
134134,268269,268268,536537,222.14451098442078,2.53381770153203
135135,270271,270270,540541,223.9102349281311,2.490310614445548
136136,272273,272272,544545,225.42290687561035,2.4476009655709277
137137,274275,274274,548549,226.90721011161804,2.4056729618411055
138138,276277,276276,552553,228.39407086372375,2.3645111499299674
139139,278279,278278,556557,229.8681070804596,2.3241004083648704
140140,280281,280280,560561,231.41905808448792,2.2844259398290205
141141,282283,282282,564565,232.87300419807434,2.245473263654958
142142,284285,284284,568569,234.48126602172852,2.2072282085010784
143143,286287,286286,572573,236.04758310317993,2.169676905206984
144144,288289,288288,576577,237.60983514785767,2.1328057798257305
145145,290291,290290,580581,239.11916613578796,2.096601546823649
146146,292293,292292,584585,240.60955595970154,2.061051202449221
147147,294295,294294,588589,242.11716103553772,2.026142018263158
148148,296297,296296,592593,243.6458351612091,1.9918615348259436
149149,298299,298298,596597,245.10939192771912,1.9581975555402096
150150,300301,300300,600601,246.59456181526184,1.9251381406446626
151151,302303,302302,604605,248.13989305496216,1.8926716013512532
152152,304305,304304,608609,249.82379388809204,1.8607864941290018
153153,306307,306306,612613,251.38520002365112,1.8294716151234525
154154,308309,308308,616617,253.03842902183533,1.7987159947157352
155155,310311,310310,620621,254.65541005134583,1.7685088922096384
156156,312313,312312,624625,256.1574580669403,1.7388397906520368
157157,314315,314314,628629,257.8459348678589,1.7096983917748503
158158,316317,316316,632633,259.8594970703125,1.6810746110627406
159159,318319,318318,636637,262.4168908596039,1.6529585729392693
160160,320321,320320,640641,264.20900106430054,1.6253406060684483
161161,322323,322322,644645,265.8316287994385,1.5982112387703182
162162,324325,324324,648649,267.3621199131012,1.5715611945486216
163163,326327,326326,652653,268.9387140274048,1.5453813877238645
164164,328329,328328,656657,270.51087284088135,1.5196629191732427
165165,330331,330330,660661,272.05711698532104,1.4943970721715232
166166,332333,332332,664665,273.59478998184204,1.469575308333674
167167,334335,334334,668669,275.25572299957275,1.4451892636521961
168168,336337,336336,672673,276.768404006958,1.421230744632112
169169,338339,338338,676677,278.3619258403778,1.3976917245158802
170170,340341,340340,680681,279.9427740573883,1.3745643396001697
171171,342343,342342,684685,281.5807189941406,1.35184088563949
172172,344345,344344,688689,283.1321179866791,1.3295138143355416
173173,346347,346346,692693,284.67947816848755,1.307575729910809
174174,348349,348348,696697,286.19439601898193,1.286019385761847
175175,350351,350350,700701,287.8056569099426,1.2648376811933986
176176,352353,352352,704705,289.3196039199829,1.2440236582299349
177177,354355,354354,708709,290.8781158924103,1.223570498499953
178178,356357,356356,712713,292.39645290374756,1.203471520197354
179179,358359,358358,716717,293.94718194007874,1.1837201751116027
180180,360361,360360,720721,295.5593099594116,1.1643100457295077
181181,362363,362362,724725,297.2651951313019,1.1452348424038519
182182,364365,364364,728729,298.9030411243439,1.1264884005884142
183183,366367,366366,732733,300.4367370605469,1.1080646781384758
184184,368369,368368,736737,301.9581341743469,1.0899577526743087
185185,370371,370370,740741,303.6370198726654,1.0721618190052595
186186,372373,372372,744745,305.2214081287384,1.0546711866140868
187187,374375,374374,748749,306.9389970302582,1.0374802772009843
188188,376377,376376,752753,308.9530141353607,1.0205836222824018
189189,378379,378378,756757,310.5337691307068,1.0039758608479588
190190,380381,380380,760761,312.1881408691406,0.9876517370696547
191191,382383,382382,764765,313.7639980316162,0.9716060980638304
192192,384385,384384,768769,315.88754200935364,0.9558338917067886
193193,386387,386386,772773,317.484158039093,0.9403301644989597
194194,388389,388388,776777,319.1244819164276,0.9250900594778386
195195,390391,390390,780781,320.65000796318054,0.9101088141801483
196196,392393,392392,784785,322.64821887016296,0.8953817586490231
197197,394395,394394,788789,324.6876459121704,0.8809043134890544
198198,396397,396396,792793,326.2199378013611,0.8666719879626044
199199,398399,398398,796797,327.6965398788452,0.8526803781318222
200200,400401,400400,800801,329.62812089920044,0.8389251650427241
201201,402403,402402,804805,331.33516907691956,0.8254021129483817
202202,404405,404404,808809,332.8357560634613,0.8121070675754254
203203,406407,406406,812813,334.3291931152344,0.7990359544268131
204204,408409,408408,816817,335.8507647514343,0.7861847771252997
205205,410411,410410,820821,337.3313009738922,0.7735496157919215
206206,412413,412412,824825,338.82484579086304,0.761126625463362
207207,414415,414414,828829,340.3615849018097,0.7489120345429683
208208,416417,416416,832833,341.8581988811493,0.7369021432870113
209209,418419,418418,836837,343.3538899421692,0.7250933223252787
210210,420421,420420,840841,344.8160619735718,0.713482011213614
211211,422423,422422,844845,346.3023750782013,0.7020647170203347
212212,424425,424424,848849,348.04337215423584,0.6908380129425495
213213,426427,426426,852853,349.99447894096375,0.6797985369532853
214214,428429,428428,856857,351.9109888076782,0.6689429904805593
215215,430431,430430,860861,353.71790075302124,0.6582681371128274
216216,432433,432432,864865,356.5361649990082,0.6477708013349002
217217,434435,434434,868869,358.2806899547577,0.6374478672912574
218218,436437,436436,872873,360.2280559539795,0.6272962775761926
219219,438439,438438,876877,362.0223979949951,0.6173130320518112
220220,440441,440440,880881,363.74486088752747,0.607495186689448
221221,442443,442442,884885,365.25109100341797,0.5978398524393924
222222,444445,444444,888889,366.710923910141,0.5883441941230103
223223,446447,446446,892893,368.2026119232178,0.5790054293506728
224224,448449,448448,896897,370.1302638053894,0.569820827461399
225225,450451,450450,900901,371.91219902038574,0.5607877084875099
226226,452453,452452,904905,373.77894401550293,0.5519034421406559
227227,454455,454454,908909,375.4575660228729,0.5431654468193301
228228,456457,456456,912913,377.06607389450073,0.5345711886394611
229229,458459,458458,916917,378.7015690803528,0.5261181804845592
230230,460461,460460,920921,380.2967960834503,0.5178039810754171
231231,462463,462462,924925,381.84259581565857,0.5096261940634577
232232,464465,464464,928929,383.364688873291,0.5015824671393148
233233,466467,466466,932933,384.86215686798096,0.4936704911626748
234234,468469,468468,936937,386.41525888442993,0.4858879993108758
235235,470471,470470,940941,388.03363490104675,0.4782327662450143
236236,472473,472472,944945,389.6580581665039,0.47070260729321944
237237,474475,474474,948949,391.2225959300995,0.4632953776534805
238238,476477,476476,952953,392.8113408088684,0.4560089716103448
239239,478479,478478,956957,394.3230941295624,0.4488413217715106
240240,480481,480480,960961,395.95538902282715,0.44179039831760747
241241,482483,482482,964965,397.5481140613556,0.43485420826868904
242242,484485,484484,968969,399.0875668525696,0.42803079476937
243243,486487,486486,972973,400.70999789237976,0.42131823638351307
244244,488489,488488,976977,402.2746651172638,0.4147146464074467
245245,490491,490490,980981,403.83442282676697,0.4082181721961433
246246,492493,492492,984985,405.37931990623474,0.4018269945048587
247247,494495,494494,988989,406.9428598880768,0.3955393268425951
248248,496497,496496,992993,408.57129979133606,0.38935341484113906
249249,498499,498498,996997,410.0449938774109,0.38326753563535476
250250,500501,500500,1001001,411.6105990409851,0.377279997257574
251251,502503,502502,1005005,413.19141578674316,0.3713891380440373
252252,504505,504504,1009009,415.08250999450684,0.3655933260541815
253253,506507,506506,1013013,416.6780707836151,0.3598909585007277
254254,508509,508508,1017017,418.58472204208374,0.354280461193639
255255,510511,510510,1021021,421.5215120315552,0.3487602879926044
256256,512513,512512,1025025,424.4566390514374,0.3433289202733931
257257,514515,514514,1029029,426.69137501716614,0.3379848664050087
258258,516517,516516,1033033,428.72213411331177,0.33272666123446015
259259,518519,518518,1037037,430.313688993454,0.3275528655871085
260260,520521,520520,1041041,431.8591899871826,0.3224620657719015
261261,522523,522522,1045045,433.4155170917511,0.317452873101729
262262,524525,524524,1049049,435.04981899261475,0.31252392341923496
263263,526527,526526,1053053,436.6104609966278,0.30767387663502177
264264,528529,528528,1057057,438.4976189136505,0.3029014162742669
265265,530531,530530,1061061,440.9537398815155,0.2982052490330034
266266,532533,532532,1065065,443.45016598701477,0.29358410434213056
267267,534535,534534,1069069,446.4544520378113,0.2890367339416571
268268,536537,536536,1073073,449.74092292785645,0.28456191146301535
269269,538539,538538,1077077,451.83477210998535,0.28015843201978896
270270,540541,540540,1081081,453.4889061450958,0.2758251118067392
271271,542543,542542,1085085,455.7225890159607,0.2715607877058801
272272,544545,544544,1089089,457.82564997673035,0.2673643169026718
273273,546547,546546,1093093,459.91726183891296,0.263234576507557
274274,548549,548548,1097097,461.8300449848175,0.2591704631865923
275275,550551,550550,1101101,463.48366808891296,0.25517089279890115
276276,552553,552552,1105105,465.9145748615265,0.25123480004083376
277277,554555,554554,1109109,467.5399158000946,0.24736113809854032
278278,556557,556556,1113113,469.0089180469513,0.24354887830588723
279279,558559,558558,1117117,470.5237190723419,0.2397970098102178
280280,560561,560560,1121121,472.0708839893341,0.23610453924470676
281281,562563,562562,1125125,473.55119585990906,0.23247049040617185
282282,564565,564564,1129129,475.07728481292725,0.228893903940957
283283,566567,566566,1133133,476.5823268890381,0.22537383703445357
284284,568569,568568,1137137,478.12467789649963,0.2219093631100577
285285,570571,570570,1141141,479.92449283599854,0.2184995715307423
286286,572573,572572,1145145,481.5176680088043,0.21514356730881445
287287,574575,574574,1149149,483.3350429534912,0.21184047082056168
288288,576577,576576,1153153,485.599986076355,0.20858941752567262
289289,578579,578578,1157157,487.2259101867676,0.20538955769404765
290290,580581,580580,1161161,488.81172585487366,0.20224005613511054
291291,582583,582582,1165165,490.5898859500885,0.1991400919357602
292292,584585,584584,1169169,492.1198990345001,0.19608885820093747
293293,586587,586586,1173173,493.63612508773804,0.1930855617998759
294294,588589,588588,1177177,495.3560960292816,0.19012942311724146
295295,590591,590590,1181181,496.8751058578491,0.18721967580995624
296296,592593,592592,1185185,498.4121811389923,0.1843555665667509
297297,594595,594594,1189189,499.9608430862427,0.18153635487510655
298298,596597,596596,1193193,501.57096004486084,0.17876131278967478
299299,598599,598598,1197197,503.14889788627625,0.17602972470774603
300300,600601,600600,1201201,504.7812650203705,0.17334088714687823
301301,602603,602602,1205205,506.4297261238098,0.1706941085286644
302302,604605,604604,1209209,508.0949478149414,0.16808870896534245
303303,606607,606606,1213213,509.6425061225891,0.16552402005106615
304304,608609,608608,1217217,511.1891348361969,0.16299938465726882
305305,610611,610610,1221221,512.8450100421906,0.16051415673064184
306306,612613,612612,1225225,514.4998970031738,0.15806770109702484
307307,614615,614614,1229229,516.3061451911926,0.15565939326802436
308308,616617,616616,1233233,518.0048940181732,0.15328861925036108
309309,618619,618618,1237237,519.5243759155273,0.1509547753599918
310310,620621,620620,1241241,521.0237319469452,0.1486572680403242
311311,622623,622622,1245245,522.5365388393402,0.1463955136820232
312312,624625,624624,1249249,524.0075490474701,0.14416893844759215
313313,626627,626626,1253253,525.6239619255066,0.14197697809879628
314314,628629,628628,1257257,527.2467138767242,0.1398190778273829
315315,630631,630630,1261261,528.7908849716187,0.137694692088985
316316,632633,632632,1265265,530.2969009876251,0.13560328444066272
317317,634635,634634,1269269,531.8795638084412,0.13354432737992283
318318,636637,636636,1273273,533.373025894165,0.13151730218851299
319319,638639,638638,1277277,534.9211468696594,0.1295216987787171
320320,640641,640640,1281281,536.562490940094,0.12755701554124244
321321,642643,642642,1285285,538.1881458759308,0.12562275919799504
322322,644645,644644,1289289,539.8302171230316,0.12371844465587856
323323,646647,646646,1293293,541.3767008781433,0.12184359486400353
324324,648649,648648,1297297,542.8505659103394,0.11999774067339786
325325,650651,650650,1301301,544.5142171382904,0.11818042070001411
326326,652653,652652,1305305,546.2323958873749,0.11639118118921488
327327,654655,654654,1309309,548.1695868968964,0.11462957588253175
328328,656657,656656,1313313,549.9125699996948,0.11289516588919923
329329,658659,658658,1317317,552.0765039920807,0.11118751955677908
330330,660661,660660,1321321,554.0630779266357,0.10950621234724167
331331,662663,662662,1325325,556.079626083374,0.10785082671236523
332332,664665,664664,1329329,558.4239959716797,0.10622095197425097
333333,666667,666666,1333333,560.658059835434,0.10461618420583818
334334,668669,668668,1337337,563.3796119689941,0.10303612611539847
335335,670671,670670,1341341,566.2039530277252,0.10148038693137096
336336,672673,672672,1345345,568.0788481235504,0.0999485822906081
337337,674675,674674,1349349,570.6535220146179,0.09844033412775843
338338,676677,676676,1353353,573.0854439735413,0.09695527056794617
339339,678679,678678,1357357,574.6968479156494,0.09549302581979191
340340,680681,680680,1361361,579.6232509613037,0.09405324007127547
341341,682683,682682,1365365,582.2939369678497,0.09263555938821355
342342,684685,684684,1369369,585.5080149173737,0.09123963561239634
343343,686687,686686,1373373,587.3019030094147,0.08986512626404419
344344,688689,688688,1377377,590.3649439811707,0.08851169444415063
345345,690691,690690,1381381,593.5418682098389,0.08717900873978124
346346,692693,692692,1385385,595.8186140060425,0.08586674313039566
347347,694695,694694,1389389,597.7735619544983,0.08457457689621606
348348,696697,696696,1393393,599.3062291145325,0.08330219452761867
349349,698699,698698,1397397,601.1020638942719,0.0820492856380497
350350,700701,700700,1401401,603.4389388561249,0.0808155448752359
351351,702703,702702,1405405,606.8552379608154,0.07960067183717001
352352,704705,704704,1409409,609.7155301570892,0.07840437098786879
353353,706707,706706,1413413,612.4791588783264,0.07722635157472268
354354,708709,708708,1417417,615.2498669624329,0.07606632754857401
355355,710711,710710,1421421,617.4275019168854,0.07492401748299926
356356,712713,712712,1425425,619.0401768684387,0.07379914449768421
357357,714715,714714,1429429,620.838241815567,0.07269143618088947
358358,716717,716716,1433433,622.3816299438477,0.07160062451453086
359359,718719,718718,1437437,623.7922661304474,0.07052644579994194
360360,720721,720720,1441441,625.8118290901184,0.06946864058602387
361361,722723,722722,1445445,627.6198899745941,0.06842695359739537
362362,724725,724724,1449449,629.5348088741302,0.06740113366390688
363363,726727,726726,1453453,631.3125720024109,0.06639093365288318
364364,728729,728728,1457457,633.2668948173523,0.065396110401025
365365,730731,730730,1461461,634.9822328090668,0.06441642464744746
366366,732733,732732,1465465,636.7290461063385,0.06345164096933331
367367,734735,734734,1469469,638.830276966095,0.06250152771713147
368368,736737,736736,1473473,640.5057799816132,0.061565856952483955
369369,738739,738738,1477477,642.1734538078308,0.06064440438535712
370370,740741,740740,1481481,644.1469750404358,0.05973694931390128
371371,742743,742742,1485485,645.8243868350983,0.05884327456453775
372372,744745,744744,1489489,647.2769720554352,0.057963166432955404
373373,746747,746746,1493493,648.9276819229126,0.05709641462772197
374374,748749,748748,1497497,650.8939108848572,0.05624281221162164
375375,750751,750750,1501501,652.9153180122375,0.055402155548222254
376376,752753,752752,1505505,654.4899549484253,0.05457424424537294
377377,754755,754754,1509509,655.9602048397064,0.053758881102453415
378378,756757,756756,1513513,657.474662065506,0.05295587205750962
379379,758759,758758,1517517,659.0079698562622,0.052165026134844084
380380,760761,760760,1521521,660.5581789016724,0.05138615539510738
381381,762763,762762,1525525,662.0801811218262,0.050619074884025395
382382,764765,764764,1529529,663.6221551895142,0.049863602583513966
383383,766767,766766,1533533,665.2602179050446,0.049119559364157794
384384,768769,768768,1537537,666.8516569137573,0.048386768936097724
385385,770771,770770,1541541,668.4445359706879,0.04766505780355601
386386,772773,772772,1545545,670.2754330635071,0.046954255219361585
387387,774775,774774,1549549,672.1788399219513,0.04625419313765633
388388,776777,776776,1553553,673.7409899234772,0.04556470617171726
389389,778779,778778,1557557,675.3825340270996,0.04488563154939129
390390,780781,780780,1561561,676.9084801673889,0.04421680907080372
391391,782783,782782,1565565,678.462819814682,0.04355808106504355
392392,784785,784784,1569569,680.061821937561,0.04290929235105523
393393,786787,786786,1573573,681.6637001037598,0.0422702901937555
394394,788789,788788,1577577,684.1441879272461,0.0416409242671989
395395,790791,790790,1581581,685.8457140922546,0.04102104661365047
396396,792793,792792,1585585,688.4269239902496,0.04041051160470488
397397,794795,794794,1589589,690.9165678024292,0.039809175904565564
398398,796797,796796,1593593,692.7332179546356,0.039216898431618574
399399,798799,798798,1597597,694.3697049617767,0.038633540322393856
400400,800801,800800,1601601,696.0239808559418,0.03805896489495808
401401,802803,802802,1605605,697.5905921459198,0.03749303761412648
402402,804805,804804,1609609,699.180716753006,0.03693562605610623
403403,806807,806806,1613613,700.8056309223175,0.03638659987439041
404404,808809,808808,1617617,702.3442749977112,0.03584583076622039
405405,810811,810810,1621621,703.8180329799652,0.03531319243916187
406406,812813,812812,1625625,705.4626219272614,0.03478856057881785
407407,814815,814814,1629629,707.0664420127869,0.03427181281733738
408408,816817,816816,1633633,708.7188141345978,0.033762828700105274
409409,818819,818818,1637637,710.2664699554443,0.03326148965754783
410410,820821,820820,1641641,711.7947678565979,0.032767678972163594
411411,822823,822822,1645645,713.373703956604,0.03228128175044276
412412,824825,824824,1649649,714.8350191116333,0.031802184892740115
413413,826827,826826,1653653,716.4481670856476,0.031330277063716494
414414,828829,828828,1657657,718.087563753128,0.03086544866573604
415415,830831,830830,1661661,719.5986020565033,0.03040759180908026
416416,832833,832832,1665665,721.0676691532135,0.029956600285345303
417417,834835,834834,1669669,722.5775728225708,0.029512369540384498
418418,836837,836836,1673673,724.3216478824615,0.029074796647819312
419419,838839,838838,1677677,726.0019710063934,0.02864378028266401
420420,840841,840840,1681681,727.6663110256195,0.028219220695518743
421421,842843,842842,1685685,729.7207469940186,0.027801019688240558
422422,844845,844844,1689689,731.2978367805481,0.027389080587681747
423423,846847,846846,1693693,733.4269268512726,0.0269833082227251
424424,848849,848848,1697697,736.7841098308563,0.026583608899272804
425425,850851,850850,1701701,739.3764219284058,0.02618989037694064
426426,852853,852852,1705705,741.6490890979767,0.025802061845752178
427427,854855,854854,1709709,744.1863691806793,0.025420033903856165
428428,856857,856856,1713713,746.2378540039062,0.02504371853410703
429429,858859,858858,1717717,747.9747169017792,0.02467302908291913
430430,860861,860860,1721721,749.6189799308777,0.02430788023787045
431431,862863,862862,1725725,751.1734759807587,0.023948188007011595
432432,864865,864864,1729729,752.7681059837341,0.023593869696696856
433433,866867,866866,1733733,754.2743828296661,0.02324484389259851
434434,868869,868868,1737737,755.7419819831848,0.022901030438106318
435435,870871,870870,1741741,757.239599943161,0.022562350414659704
436436,872873,872872,1745745,759.0637068748474,0.022228726121966247
437437,874875,874874,1749749,760.9606280326843,0.021900081059357035
438438,876877,876876,1753753,762.6018781661987,0.02157633990634622
439439,878879,878878,1757757,764.5117998123169,0.021257428502849507
440440,880881,880880,1761761,766.5312139987946,0.02094327383304062
441441,882883,882882,1765765,768.3320798873901,0.0206338040055698
442442,884885,884884,1769769,769.8804459571838,0.02032894823605602
443443,886887,886886,1773773,771.3542490005493,0.02002863683014766
444444,888889,888888,1777777,772.9983351230621,0.019732801165673663
445445,890891,890890,1781781,774.5590941905975,0.01944137367604526
446446,892893,892892,1785785,776.1016359329224,0.01915428783331663
447447,894895,894894,1789789,777.5996849536896,0.018871478132496122
448448,896897,896896,1793793,779.0565729141235,0.018592880074493223
449449,898899,898898,1797797,780.6422238349915,0.018318430150884524
450450,900901,900900,1801801,782.1979489326477,0.01804806582811125
451451,902903,902902,1805805,783.8035228252411,0.01778172553213153
452452,904905,904904,1809809,785.3429498672485,0.017519348633527443
453453,906907,906906,1813813,786.8189399242401,0.017260875432384637
454454,908909,908908,1817817,788.304477930069,0.017006247143513065
455455,910911,910910,1821821,789.8129739761353,0.0167554058832593
456456,912913,912912,1825825,791.343444108963,0.016508294653135636
457457,914915,914914,1829829,792.9946839809418,0.016264857328565085
458458,916917,916916,1833833,794.5882499217987,0.01602503864285154
459459,918919,918918,1837837,796.2825980186462,0.015788784175242654
460460,920921,920920,1841841,798.0063519477844,0.015556040337855848
461461,922923,922922,1845845,800.505469083786,0.015326754360444284
462462,924925,924924,1849849,802.2385580539703,0.015100874280392418
463463,926927,926926,1853853,804.3967199325562,0.01487834892839146
464464,928929,928928,1857857,805.987212896347,0.01465912791672963
465465,930931,930930,1861861,807.6101651191711,0.014443161626559231
466466,932933,932932,1865865,809.3756580352783,0.014230401196073217
467467,934935,934934,1869869,811.1825728416443,0.014020798509363885
468468,936937,936936,1873873,812.7694659233093,0.013814306183576264
469469,938939,938938,1877877,814.3181698322296,0.013610877558562606
470470,940941,940940,1881881,815.892914056778,0.013410466684945277
471471,942943,942942,1885885,817.6385819911957,0.013213028313202813
472472,944945,944944,1889889,819.5301997661591,0.013018517883097047
473473,946947,946946,1893893,821.7420098781586,0.012826891512759175
474474,948949,948948,1897897,824.0959408283234,0.012638105987775816
475475,950951,950950,1901901,826.1199538707733,0.012452118750957197
476476,952953,952952,1905905,827.9618000984192,0.012268887892901148
477477,954955,954954,1909909,829.7815268039703,0.012088372140738102
478478,956957,956956,1913913,832.0713858604431,0.011910530849263523
479479,958959,958958,1917917,833.9903299808502,0.011735323990478719
480480,960961,960960,1921921,837.0897009372711,0.011562712143927456
481481,962963,962962,1925925,839.1562850475311,0.01139265648851051
482482,964965,964964,1929929,841.0239889621735,0.011225118792140165
483483,966967,966966,1933933,843.1007080078125,0.01106006140196314
484484,968969,968968,1937937,845.1555318832397,0.010897447236970947
485485,970971,970970,1941941,847.4159939289093,0.010737239778450203
486486,972973,972972,1945945,849.4353170394897,0.010579403061001358
487487,974975,974974,1949949,851.4134228229523,0.010423901664353252
488488,976977,976976,1953953,853.3664228916168,0.010270700704609226
489489,978979,978978,1957957,855.2427349090576,0.010119765826516414
490490,980981,980980,1961961,857.2877569198608,0.009971063194484486
491491,982983,982982,1965965,859.3593330383301,0.009824559485423379
492492,984985,984984,1969969,861.252995967865,0.009680221880444151
493493,986987,986986,1973973,863.0996398925781,0.00953801805690091
494494,988989,988988,1977977,864.794037103653,0.009397916180660104
495495,990991,990990,1981981,867.1613368988037,0.009259884899961435
496496,992993,992992,1985985,869.2286639213562,0.009123893335072353
497497,994995,994994,1989989,871.4325180053711,0.008989911074650081
498498,996997,996996,1993993,873.0712480545044,0.008857908165282424
499499,998999,998998,1997997,874.6091821193695,0.008727855106940297
500501,1001003,1001002,2002005,876.9717299938202,0.00859959579054248
501502,1003005,1003004,2006009,878.5755898952484,0.008473357582261087
502503,1005007,1005006,2010013,880.2785937786102,0.008348983339942606
503504,1007009,1007008,2014017,882.4516260623932,0.008226445303876062
504505,1009011,1009010,2018021,884.4257628917694,0.008105716133513852
505506,1011013,1011012,2022025,886.3976330757141,0.00798676889996841
506507,1013015,1013014,2026029,888.3215570449829,0.007869577080214185
507508,1015017,1015016,2030033,891.1111009120941,0.007754114551175917
508509,1017019,1017018,2034037,893.396087884903,0.007640355583134806
509510,1019021,1019020,2038041,895.3021910190582,0.007528274833589421
510511,1021023,1021022,2042045,897.3537061214447,0.0074178473416850466
511512,1023025,1023024,2046049,899.8741579055786,0.007309048522643025
512513,1025027,1025026,2050053,902.4229238033295,0.00720185416082586
513514,1027029,1027028,2054057,904.3198537826538,0.007096240405644494
514515,1029031,1029030,2058061,906.84565782547,0.006992183764850779
515516,1031033,1031032,2062065,908.5179579257965,0.006889661099080513
516517,1033035,1033034,2066069,910.1490440368652,0.006788649617419651
517518,1035037,1035036,2070073,912.3793859481812,0.0066891268711515295
518519,1037039,1037038,2074077,914.4166448116302,0.006591070748640959
519520,1039041,1039040,2078081,916.6821398735046,0.006494459470559377
520521,1041043,1041042,2082085,918.3181049823761,0.0063992715848826265
521522,1043045,1043044,2086089,920.5580580234528,0.006305485961206614
522523,1045047,1045046,2090093,922.4653630256653,0.006213081786540897
523524,1047049,1047048,2094097,924.6560459136963,0.00612203855973803
524525,1049051,1049050,2098101,926.5708329677582,0.006032336087855583
525526,1051053,1051052,2102105,928.8300700187683,0.005943954480585489
526527,1053055,1053054,2106109,930.5555238723755,0.005856874145592883
527528,1055057,1055056,2110113,932.2247791290283,0.005771075784991808
528529,1057059,1057058,2114117,933.9365799427032,0.005686540388865069
529530,1059061,1059060,2118121,935.6209769248962,0.005603249233217866
530531,1061063,1061062,2122125,937.5695340633392,0.00552118387452083
531532,1063065,1063064,2126129,939.382443189621,0.00544032614459411
532533,1065067,1065066,2130133,941.1519770622253,0.005360658148447328
533534,1067069,1067068,2134137,942.9054238796234,0.005282162258026801
534535,1069071,1069070,2138141,945.208655834198,0.0052048211096007435
535536,1071073,1071072,2142145,947.0988628864288,0.005128617599552854
536537,1073075,1073074,2146149,949.147971868515,0.005053534879380095
537538,1075077,1075076,2150153,950.88294506073,0.004979556353191583
538539,1077079,1077078,2154157,952.6901121139526,0.004906665672933741
539540,1079081,1079080,2158161,954.5809559822083,0.004834846735207066
540541,1081083,1081082,2162165,956.5117309093475,0.00476408367728709
541542,1083085,1083084,2166169,958.1338467597961,0.004694360873259029
542543,1085087,1085086,2170173,960.5444979667664,0.004625662930948238
543544,1087089,1087088,2174177,962.6839168071747,0.0045579746880548555
544545,1089091,1089090,2178181,964.8709740638733,0.004491281208629516
545546,1091093,1091092,2182185,966.7732150554657,0.004425567780003803
546547,1093095,1093094,2186189,968.9131798744202,0.004360819908697522
547548,1095097,1095096,2190193,970.8889639377594,0.004297023317917592
548549,1097099,1097098,2194197,972.931834936142,0.004234163943806379
549550,1099101,1099100,2198201,974.9159018993378,0.004172227932485839
550551,1101103,1101102,2202205,976.7013189792633,0.00411120163630585
551552,1103105,1103104,2206209,978.6761898994446,0.004051071611684165
552553,1105107,1105106,2210213,981.1528720855713,0.003991824615127371
553554,1107109,1107108,2214217,983.2041611671448,0.003933447600616091
554555,1109111,1109110,2218221,985.0454449653625,0.003875927716762817
555556,1111113,1111112,2222225,986.8987939357758,0.003819252303628673
556557,1113115,1113114,2226229,988.7714738845825,0.003763408889653874
557558,1115117,1115116,2230233,990.6970720291138,0.003708385189497676
558559,1117119,1117118,2234237,993.1144127845764,0.003654169100400395
559560,1119121,1119120,2238241,995.26713514328,0.0036007486999096727
560561,1121123,1121122,2242245,997.9448490142822,0.0035481122433793644
561562,1123125,1123124,2246249,999.8556339740753,0.0034962481604452478
562563,1125127,1125126,2250253,1001.9260160923004,0.003445145053547094
563564,1127129,1127128,2254257,1003.772962808609,0.003394791693949628
564565,1129131,1129130,2258261,1005.371297121048,0.0033451770207193476
565566,1131133,1131132,2262265,1007.2165961265564,0.0032962901374276043
566567,1133135,1133134,2266269,1009.1328480243683,0.003248120308739999
567568,1135137,1135136,2270273,1011.0434677600861,0.003200656959961634
568569,1137139,1137138,2274277,1012.6643040180206,0.0031538896731717614
569570,1139141,1139140,2278281,1014.333172082901,0.0031078081859732265
570571,1141143,1141142,2282285,1015.9527750015259,0.003062402386717622
571572,1143145,1143144,2286289,1017.7954609394073,0.003017662316096903
572573,1145147,1145146,2290293,1020.7842938899994,0.002973578161459045
573574,1147149,1147148,2294297,1022.477698802948,0.002930140256580671
574575,1149151,1149150,2298301,1024.1235001087189,0.002887339078029072
575576,1151153,1151152,2302305,1026.1263377666473,0.002845165244366399
576577,1153155,1153154,2306309,1027.66081905365,0.002803609513648553
577578,1155157,1155156,2310313,1029.2135691642761,0.0027626627802419534
578579,1157159,1157158,2314317,1031.6785538196564,0.002722316074596165
579580,1159161,1159160,2318321,1033.9846711158752,0.0026825605596059177
580581,1161163,1161162,2322325,1035.5047571659088,0.002643387529587926
581582,1163165,1163164,2326329,1036.9898898601532,0.0026047884078934658
582583,1165167,1165166,2330333,1038.4939589500427,0.0025667547449756967
583584,1167169,1167168,2334337,1039.967668056488,0.0025292782169117345
584585,1169171,1169170,2338341,1041.6126170158386,0.0024923506227878534
585586,1171173,1171172,2342345,1043.1584689617157,0.0024559638834489306
586587,1173175,1173174,2346349,1044.6671209335327,0.0024201100396794573
587588,1175177,1175176,2350353,1046.163341999054,0.0023847812500434884
588589,1177179,1177178,2354357,1047.6545929908752,0.0023499697889519666
589590,1179181,1179180,2358361,1049.1608378887177,0.002315668046207975
590591,1181183,1181182,2362365,1050.6289110183716,0.0022818685231413838
591592,1183185,1183184,2366369,1052.1176459789276,0.0022485638329499125
592593,1185187,1185186,2370373,1053.60014295578,0.002215746698084331
593594,1187189,1187188,2374377,1055.084142923355,0.0021834099487705316
594595,1189191,1189190,2378381,1056.5601181983948,0.0021515465210768525
595596,1191193,1191192,2382385,1058.040647983551,0.002120149455890896
596597,1193195,1193194,2386389,1059.5090000629425,0.0020892118969868534
597598,1195197,1195196,2390393,1060.9876430034637,0.0020587270898886345
598599,1197199,1197198,2394397,1062.471673965454,0.002028688379596133
599600,1199201,1199200,2398401,1063.960350036621,0.0019990892099031043
600601,1201203,1201202,2402405,1065.4211149215698,0.001969923121123429
601602,1203205,1203204,2406409,1066.9044160842896,0.0019411837497500528
602603,1205207,1205206,2410413,1068.3845839500427,0.0019128648261812486
603604,1207209,1207208,2414417,1069.8677451610565,0.0018849601733563759
604605,1209211,1209210,2418421,1071.3730299472809,0.0018574637050505771
605606,1211213,1211212,2422425,1072.8705749511719,0.001830369425988465
606607,1213215,1213214,2426429,1074.383271932602,0.0018036714290019518
607608,1215217,1215216,2430433,1075.850989818573,0.0017773638942344405
608609,1217219,1217218,2434437,1077.3372559547424,0.0017514410874355235
609610,1219221,1219220,2438441,1078.777979850769,0.0017258973599609817
610611,1221223,1221222,2442445,1080.077645778656,0.001700727145930614
611612,1223225,1223224,2446449,1081.3844170570374,0.0016759249615461158
612613,1225227,1225226,2450453,1082.6279110908508,0.0016514854047500194
613614,1227229,1227228,2454457,1084.3220229148865,0.0016274031526108956
614615,1229231,1229230,2458461,1086.0358619689941,0.0016036729606412337
615616,1231233,1231232,2462465,1087.6390800476074,0.00158028966245638
616617,1233235,1233234,2466469,1089.2484109401703,0.0015572481673871152
617618,1235237,1235236,2470473,1090.8872079849243,0.0015345434600249064
618619,1237239,1237238,2474477,1092.4597730636597,0.0015121705989713519
619620,1239241,1239240,2478481,1094.8574759960175,0.0014901247160423736
620621,1241243,1241242,2482485,1096.791396856308,0.0014684010139944803
621622,1243245,1243244,2486489,1098.4171109199524,0.001446994767434262
622623,1245247,1245246,2490493,1100.1244518756866,0.00142590132031728
623624,1247249,1247248,2494497,1101.8116188049316,0.0014051160846975108
624625,1249251,1249250,2498501,1103.3087661266327,0.0013846345407273475
625626,1251253,1251252,2502505,1104.780993938446,0.0013644522352933564
626627,1253255,1253254,2506509,1106.317270040512,0.0013445647808794092
627628,1255257,1255256,2510513,1107.7915210723877,0.001324967854429815
628629,1257259,1257258,2514517,1109.3613109588623,0.0013056571966671981
629630,1259261,1259260,2518521,1110.9052579402924,0.0012866286112966918
630631,1261263,1261262,2522525,1112.4609949588776,0.0012678779638690685
631632,1263265,1263264,2526529,1113.932373046875,0.0012494011803028116
632633,1265267,1265266,2530533,1115.4272768497467,0.0012311942472251758
633634,1267269,1267268,2534537,1116.9079189300537,0.001213253210039511
634635,1269271,1269270,2538541,1118.3680970668793,0.0011955741720157675
635636,1271273,1271272,2542545,1119.904606103897,0.001178153294972617
636637,1273275,1273274,2546549,1121.3769309520721,0.001160986796094221
637638,1275277,1275276,2550553,1122.8546059131622,0.0011440709483849787
638639,1277279,1277278,2554557,1124.3504309654236,0.0011274020805558393
639640,1279281,1279280,2558561,1125.8294730186462,0.0011109765745231925
640641,1281283,1281282,2562565,1127.3055770397186,0.0010947908657499283
641642,1283285,1283284,2566569,1128.8044650554657,0.0010788414422222559
642643,1285287,1285286,2570573,1130.2579538822174,0.0010631248436538954
643644,1287289,1287288,2574577,1131.7844140529633,0.0010476376598944626
644645,1289291,1289290,2578581,1133.2597961425781,0.0010323765325210843
645646,1291293,1291292,2582585,1134.7624979019165,0.0010173381512004198
646647,1293295,1293294,2586589,1136.231286764145,0.001002519254825529
647648,1295297,1295296,2590593,1137.7213609218597,0.0009879166298105702
648649,1297299,1297298,2594597,1139.1755480766296,0.0009735271106592336
649650,1299301,1299300,2598601,1140.6670908927917,0.0009593475776910054
650651,1301303,1301302,2602605,1142.148628950119,0.000945374957268541
651652,1303305,1303304,2606609,1143.6043128967285,0.000931606221115544
652653,1305307,1305306,2610613,1145.0676350593567,0.0009180383852935847
653654,1307309,1307308,2614617,1146.5252950191498,0.0009046685099747265
654655,1309311,1309310,2618621,1147.9916639328003,0.0008914936981909705
655656,1311313,1311312,2622625,1149.4833180904388,0.0008785110958342557
656657,1313315,1313314,2626629,1150.9694731235504,0.0008657178906332774
657658,1315317,1315316,2630633,1152.4259819984436,0.0008531113114713662
658659,1317319,1317318,2634637,1153.9009108543396,0.0008406886283864878
659660,1319321,1319320,2638641,1155.4164538383484,0.0008284471512070013
660661,1321323,1321322,2642645,1156.9141600131989,0.0008163842288695378
661662,1323325,1323324,2646649,1158.369174003601,0.0008044972502148084
662663,1325327,1325326,2650653,1159.8423500061035,0.0007927836417138678
663664,1327329,1327328,2654657,1161.3172209262848,0.0007812408679228611
664665,1329331,1329330,2658661,1162.8587930202484,0.0007698664305735292
665666,1331333,1331332,2662665,1164.353096961975,0.0007586578680047751
666667,1333335,1333334,2666669,1165.8622069358826,0.0007476127547079159
667668,1335337,1335336,2670673,1167.29869389534,0.000736728700758249
668669,1337339,1337338,2674677,1168.7741258144379,0.0007260033514739916
669670,1339341,1339340,2678681,1170.2696499824524,0.0007154343868478463
670671,1341343,1341342,2682685,1171.7576739788055,0.0007050195201827592
671672,1343345,1343344,2686689,1173.2124750614166,0.0006947564993424749
672673,1345347,1345346,2690693,1174.6972448825836,0.0006846431045914869
673674,1347349,1347348,2694697,1176.1436760425568,0.0006746771488224113
674675,1349351,1349350,2698701,1177.6081931591034,0.0006648564775559862
675676,1351353,1351352,2702705,1179.1008431911469,0.0006551789667810226
676677,1353355,1353354,2706709,1180.5615129470825,0.0006456425251144537
677678,1355357,1355356,2710713,1182.0388538837433,0.0006362450906181039
678679,1357359,1357358,2714717,1183.5355851650238,0.0006269846320492434
679680,1359361,1359360,2718721,1185.030529975891,0.0006178591481784679
680681,1361363,1361362,2722725,1186.483638048172,0.0006088666668802034
681682,1363365,1363364,2726729,1187.9643337726593,0.0006000052451327065
682683,1365367,1365366,2730733,1189.4364838600159,0.0005912729679948825
683684,1367369,1367368,2734737,1190.9025061130524,0.0005826679490610331
684685,1369371,1369370,2738741,1192.405996799469,0.000574188329323988
685686,1371373,1371372,2742745,1194.081160068512,0.0005658322767203572
686687,1373375,1373374,2746749,1195.9119699001312,0.0005575979870400261
687688,1375377,1375376,2750753,1198.0495479106903,0.0005494836814250448
688689,1377379,1377378,2754757,1199.7810430526733,0.0005414876078475572
689690,1379381,1379380,2758761,1201.4741787910461,0.0005336080395181853
690691,1381383,1381382,2762765,1203.3126118183136,0.0005258432749997155
691692,1383385,1383384,2766769,1205.2339000701904,0.0005181916379797258
692693,1385387,1385386,2770773,1207.1239268779755,0.000510651476588464
693694,1387389,1387388,2774777,1208.818778038025,0.0005032211631714745
694695,1389391,1389390,2778781,1210.8859779834747,0.0004958990938348506
695696,1391393,1391392,2782785,1212.629059791565,0.0004886836883315482
696697,1393395,1393394,2786789,1214.7946310043335,0.00048157338937926397
697698,1395397,1395396,2790793,1216.9837248325348,0.00047456666277412296
698699,1397399,1397398,2794797,1219.1485919952393,0.0004676619963674966
699700,1399401,1399400,2798801,1221.7541148662567,0.00046085790074812394
700701,1401403,1401402,2802805,1224.3597960472107,0.00045415290765049576
701702,1403405,1403404,2806809,1226.1448090076447,0.00044754557063697575
702703,1405407,1405406,2810813,1228.007661819458,0.0004410344647567399
703704,1407409,1407408,2814817,1230.1437249183655,0.0004346181851815345
704705,1409411,1409410,2818821,1232.020499944687,0.0004282953484562313
705706,1411413,1411412,2822825,1234.4600939750671,0.00042206459045246447
706707,1413415,1413414,2826829,1236.2216238975525,0.00041592456818762
707708,1415417,1415416,2830833,1238.0804388523102,0.0004098739569826648
708709,1417419,1417418,2834837,1239.7527210712433,0.00040391145296325703
709710,1419421,1419420,2838841,1241.5778200626373,0.00039803577010388835
710711,1421423,1421422,2842845,1243.5030410289764,0.00039224564193318656
711712,1423425,1423424,2846849,1245.3506209850311,0.00038653982005598664
712713,1425427,1425426,2850853,1247.0711069107056,0.0003809170749491386
713714,1427429,1427428,2854857,1248.8661918640137,0.00037537619448357873
714715,1429431,1429430,2858861,1250.6152169704437,0.00036991598449276353
715716,1431433,1431432,2862865,1252.3947370052338,0.00036453526820423576
716717,1433435,1433434,2866869,1254.1048710346222,0.0003592328863533112
717718,1435437,1435436,2870873,1255.7681379318237,0.000354007696159897
718719,1437439,1437438,2874877,1257.6842529773712,0.0003488585717832393
719720,1439441,1439440,2878881,1259.401687860489,0.0003437844042082361
720721,1441443,1441442,2882885,1261.1539878845215,0.0003387840999948821
721722,1443445,1443444,2886889,1263.241196155548,0.00033385658207407687
722723,1445447,1445446,2890893,1264.8056960105896,0.00032900078883812967
723724,1447449,1447448,2894897,1266.3042788505554,0.00032421567459550715
724725,1449451,1449450,2898901,1267.8601460456848,0.0003195002088887122
725726,1451453,1451452,2902905,1269.3553721904755,0.00031485337603953667
726727,1453455,1453454,2906909,1270.8700859546661,0.00031027417526274803
727728,1455457,1455456,2910913,1272.4684660434723,0.00030576162089346326
728729,1457459,1457458,2914917,1273.9979348182678,0.00030131474090921984
729730,1459461,1459460,2918921,1275.4946780204773,0.00029693257783947047
730731,1461463,1461462,2922925,1276.983680009842,0.0002926141887655831
731732,1463465,1463464,2926929,1278.6192059516907,0.00028835864316079096
732733,1465467,1465466,2930933,1280.2253148555756,0.0002841650260734241
733734,1467469,1467468,2934937,1281.7300369739532,0.0002800324336931226
734735,1469471,1469470,2938941,1283.217406988144,0.00027595997721618915
735736,1471473,1471472,2942945,1284.7103779315948,0.00027194677988973126
736737,1473475,1473474,2946949,1286.1972959041595,0.0002679919781485296
737738,1475477,1475476,2950953,1287.9405121803284,0.00026409472093291697
738739,1477479,1477478,2954957,1289.525321006775,0.00026025416934771783
739740,1479481,1479480,2958961,1291.0595290660858,0.0002564694973443693
740741,1481483,1481482,2962965,1292.5289280414581,0.0002527398905840528
741742,1483485,1483484,2966969,1294.0035500526428,0.0002490645463240071
742743,1485487,1485486,2970973,1295.614806175232,0.00024544267421333643
743744,1487489,1487488,2974977,1297.308376789093,0.00024187349481508136
744745,1489491,1489490,2978981,1299.35098195076,0.00023835624062940042
745746,1491493,1491492,2982985,1300.9177868366241,0.0002348901548430149
746747,1493495,1493494,2986989,1302.589998960495,0.0002314744921250167
747748,1495497,1495496,2990993,1304.1508538722992,0.00022810851783106045
748749,1497499,1497498,2994997,1305.730689048767,0.00022479150788967672
749750,1499501,1499500,2999001,1307.5523359775543,0.0002215227492570193
750751,1501503,1501502,3003005,1309.305125951767,0.00021830153877999692
751752,1503505,1503504,3007009,1310.8703918457031,0.00021512718365102046
752753,1505507,1505506,3011013,1312.700756072998,0.00021199900186275045
753754,1507509,1507508,3015017,1314.3228991031647,0.00020891632038910757
754755,1509511,1509510,3019021,1315.9773478507996,0.00020587847677688842
755756,1511513,1511512,3023025,1317.4515228271484,0.00020288481755414978
756757,1513515,1513514,3027029,1318.9692900180817,0.00019993469959445065
757758,1515517,1515516,3031033,1320.5043759346008,0.0001970274884115497
758759,1517519,1517518,3035037,1321.9696309566498,0.00019416255929627368
759760,1519521,1519520,3039041,1323.4395008087158,0.00019133929640702263
760761,1521523,1521522,3043045,1324.9675879478455,0.0001885570928834568
761762,1523525,1523524,3047049,1327.054015159607,0.00018581535084649659
762763,1525527,1525526,3051053,1328.58455991745,0.0001831134810572621
763764,1527529,1527528,3055057,1330.0781960487366,0.0001804509029170731
764765,1529531,1529530,3059061,1331.5608370304108,0.00017782704424007534
765766,1531533,1531532,3063065,1333.1238911151886,0.0001752413411395537
766767,1533535,1533534,3067069,1334.6973600387573,0.00017269323825530591
767768,1535537,1535536,3071073,1336.2416388988495,0.00017018218807152152
768769,1537539,1537538,3075077,1337.9591670036316,0.0001677076510304687
769770,1539541,1539540,3079081,1339.7335150241852,0.00016526909530512057
770771,1541543,1541542,3083085,1341.6031160354614,0.00016286599748127628
771772,1543545,1543544,3087089,1343.2406568527222,0.00016049784107963205
772773,1545547,1545546,3091093,1344.7744960784912,0.00015816411735158908
773774,1547549,1547548,3095097,1346.2995069026947,0.00015586432527925353
774775,1549551,1549550,3099101,1347.7879610061646,0.00015359797066594183
775776,1551553,1551552,3103105,1349.3402349948883,0.00015136456670461484
776777,1553555,1553554,3107109,1350.8788800239563,0.00014916363420525158
777778,1555557,1555556,3111113,1352.3724389076233,0.00014699470000323345
778779,1557559,1557558,3115117,1353.8494579792023,0.00014485729855095997
779780,1559561,1559560,3119121,1355.3235857486725,0.00014275097078098042
780781,1561563,1561562,3123125,1356.8142659664154,0.00014067526444705436
781782,1563565,1563564,3127129,1358.2862060070038,0.00013862973401046474
782783,1565567,1565566,3131133,1359.7849490642548,0.00013661394007158378
783784,1567569,1567568,3135137,1361.2767519950867,0.0001346274499383071
784785,1569571,1569570,3139141,1362.7690551280975,0.0001326698370576196
785786,1571573,1571572,3143145,1364.2494418621063,0.000130740681242969
786787,1573575,1573574,3147149,1365.765552997589,0.0001288395682195187
787788,1575577,1575576,3151153,1367.2521770000458,0.00012696609019258176
788789,1577579,1577578,3155157,1368.7487120628357,0.00012511984448337898
789790,1579581,1579580,3159161,1370.2330009937286,0.00012330043568908877
790791,1581583,1581582,3163165,1371.7150721549988,0.00012150747215855517
791792,1583585,1583584,3167169,1373.2070689201355,0.00011974057031238772
792793,1585587,1585586,3171173,1374.7159719467163,0.00011799934986811422
793794,1587589,1587588,3175177,1376.255264043808,0.00011628343759184645
794795,1589591,1589590,3179181,1377.7171819210052,0.00011459246536560386
795796,1591593,1591592,3183185,1379.2202739715576,0.0001129260701873136
796797,1593595,1593594,3187189,1380.7130959033966,0.00011128389451187104
797798,1595597,1595596,3191193,1382.213355064392,0.0001096655857963924
798799,1597599,1597598,3195197,1383.710401058197,0.00010807079695496213
799800,1599601,1599600,3199201,1385.1981270313263,0.00010649918567651184
800801,1601603,1601602,3203205,1386.6637499332428,0.00010495041499325453
801802,1603605,1603604,3207209,1388.1383697986603,0.00010342415259856352
802803,1605607,1605606,3211213,1389.6362178325653,0.0001019200710743462
803804,1607609,1607608,3215217,1391.1277358531952,0.0001004378472089229
804805,1609611,1609610,3219221,1392.461769104004,9.89771638160164e-05
805806,1611613,1611612,3223225,1393.83758187294,9.753770711995458e-05
806807,1613615,1613614,3227229,1395.1213698387146,9.611916834728618e-05
807808,1615617,1615616,3231233,1396.4075741767883,9.47212433857203e-05
808809,1617619,1617618,3235237,1397.673283815384,9.334363244306587e-05
809810,1619621,1619620,3239241,1398.9189131259918,9.198603970617114e-05
810811,1621623,1621622,3243245,1400.2110919952393,9.064817447779205e-05
811812,1623625,1623624,3247249,1401.9012858867645,8.932974958497653e-05
812813,1625627,1625626,3251253,1403.4575598239899,8.803048206118547e-05
813814,1627629,1627628,3255257,1404.974997997284,8.675009382841381e-05
814815,1629631,1629630,3259261,1406.488399028778,8.548830965082743e-05
815816,1631633,1631632,3263265,1408.0382328033447,8.424485952218674e-05
816817,1633635,1633634,3267269,1409.6905591487885,8.301947650579677e-05
817818,1635637,1635636,3271273,1411.312332868576,8.181189775768871e-05
818819,1637639,1637638,3275277,1412.8594398498535,8.062186464030674e-05
819820,1639641,1639640,3279281,1414.4943478107452,7.944912215407385e-05
820821,1641643,1641642,3283285,1416.2201948165894,7.829341825527081e-05
821822,1643645,1643644,3287289,1417.916630744934,7.715450556133874e-05
822823,1645647,1645646,3291293,1419.5568799972534,7.603214010032389e-05
823824,1647649,1647648,3295297,1421.9481489658356,7.492608062875661e-05
824825,1649651,1649650,3299301,1424.9580838680267,7.38360905643276e-05
825826,1651653,1651652,3303305,1427.4926180839539,7.276193605321168e-05
826827,1653655,1653654,3307309,1431.4553129673004,7.17033869932493e-05
827828,1655657,1655656,3311313,1434.4900560379028,7.066021623813867e-05
828829,1657659,1657658,3315317,1437.1507759094238,6.963220039324369e-05
829830,1659661,1659660,3319321,1439.3630888462067,6.861911890609917e-05
830831,1661663,1661662,3323325,1441.3990769386292,6.762075497590558e-05
831832,1663665,1663664,3327329,1442.957545042038,6.663689430297381e-05
832833,1665667,1665666,3331333,1444.9156019687653,6.566732622559357e-05
833834,1667669,1667668,3335337,1447.1766159534454,6.471184281053866e-05
834835,1669671,1669670,3339341,1449.433270931244,6.377023930781434e-05
835836,1671673,1671672,3343345,1451.7362129688263,6.284231403697049e-05
836837,1673675,1673674,3347349,1453.6466779708862,6.192786804604111e-05
837838,1675677,1675676,3351353,1455.6601338386536,6.10267054526048e-05
838839,1677679,1677678,3355357,1457.4025838375092,6.013863298903743e-05
839840,1679681,1679680,3359361,1459.399132013321,5.926346034357266e-05
840841,1681683,1681682,3363365,1460.9141509532928,5.840100050136243e-05
841842,1683685,1683684,3367369,1462.4378628730774,5.7551068039174424e-05
842843,1685687,1685686,3371373,1464.0003778934479,5.671348117175512e-05
843844,1687689,1687688,3375377,1465.949858903885,5.5888060501274595e-05
844845,1689691,1689690,3379381,1467.9850549697876,5.507462878995284e-05
845846,1691693,1691692,3383385,1469.7522897720337,5.427301221061498e-05
846847,1693695,1693694,3387389,1471.8649649620056,5.348303886876238e-05
847848,1695697,1695696,3391393,1473.4828927516937,5.2704539598380507e-05
848849,1697699,1697698,3395397,1475.8232789039612,5.193734739350475e-05
849850,1699701,1699700,3399401,1477.946534872055,5.118129809034144e-05
850851,1701703,1701702,3403405,1480.182512998581,5.043622968514683e-05
851852,1703705,1703704,3407409,1482.3532729148865,4.9701982561600744e-05
852853,1705707,1705706,3411413,1484.322496175766,4.897839960449346e-05
853854,1707709,1707708,3415417,1486.23433303833,4.826532551760465e-05
854855,1709711,1709710,3419421,1488.2088038921356,4.756260784688493e-05
855856,1711713,1711712,3423425,1490.0609829425812,4.687009584358748e-05
856857,1713715,1713714,3427429,1491.9202148914337,4.618764148744958e-05
857858,1715717,1715716,3431433,1493.7153811454773,4.5515098463511094e-05
858859,1717719,1717718,3435437,1495.5194280147552,4.4852322616861784e-05
859860,1719721,1719720,3439441,1497.2207729816437,4.419917218001501e-05
860861,1721723,1721722,3443445,1498.889818906784,4.3555507090786705e-05
861862,1723725,1723724,3447449,1500.71089220047,4.292118978810322e-05
862863,1725727,1725726,3451453,1502.4309980869293,4.229608384775929e-05
863864,1727729,1727728,3455457,1504.1096861362457,4.168005614246795e-05
864865,1729731,1729730,3459461,1505.8451888561249,4.107297445443692e-05
865866,1731733,1731732,3463465,1507.8136332035065,4.047470861223701e-05
866867,1733735,1733734,3467469,1510.0362861156464,3.9885130831862625e-05
867868,1735737,1735736,3471473,1512.0821089744568,3.930411446617654e-05
868869,1737739,1737738,3475477,1514.055408000946,3.8731535710212484e-05
869870,1739741,1739740,3479481,1516.0485620498657,3.816727121375152e-05
870871,1741743,1741742,3483485,1518.4001939296722,3.76112005824325e-05
871872,1743745,1743744,3487489,1520.4131951332092,3.706320489982318e-05
872873,1745747,1745746,3491493,1522.45693898201,3.65231665000465e-05
873874,1747749,1747748,3495497,1524.5003941059113,3.599097010464902e-05
874875,1749751,1749750,3499501,1526.508798122406,3.546650168573251e-05
875876,1751753,1751752,3503505,1528.6743409633636,3.494964857964078e-05
876877,1753755,1753754,3507509,1530.8451590538025,3.444030051014124e-05
877878,1755757,1755756,3511513,1532.9218399524689,3.39383486789302e-05
878879,1757759,1757758,3515517,1534.5282011032104,3.344368496982497e-05
879880,1759761,1759760,3519521,1536.0749080181122,3.295620388144016e-05
880881,1761763,1761762,3523525,1537.6527349948883,3.2475801049258735e-05
881882,1763765,1763764,3527529,1539.2162990570068,3.2002373700379394e-05
882883,1765767,1765766,3531533,1540.7616519927979,3.153582042614289e-05
883884,1767769,1767768,3535537,1542.2781729698181,3.107604118213203e-05
884885,1769771,1769770,3539541,1543.7680039405823,3.062293774291902e-05
885886,1771773,1771772,3543545,1545.2808630466461,3.0176413247318123e-05
886887,1773775,1773774,3547549,1546.7944300174713,2.9736371971011977e-05
887888,1775777,1775776,3551553,1548.713536977768,2.930271955392527e-05
888889,1777779,1777778,3555557,1550.956955909729,2.8875363341285265e-05
889890,1779781,1779780,3559561,1552.588143825531,2.8454212156248104e-05
890891,1781783,1781782,3563565,1554.23175573349,2.8039175276717287e-05
891892,1783785,1783784,3567569,1555.8303561210632,2.7630164481706743e-05
892893,1785787,1785786,3571573,1557.4215638637543,2.722709189129091e-05
893894,1787789,1787788,3575577,1559.0495371818542,2.6829871217159962e-05
894895,1789791,1789790,3579581,1560.5685079097748,2.6438417535246117e-05
895896,1791793,1791792,3583585,1562.0602388381958,2.605264739941049e-05
896897,1793795,1793794,3587589,1563.5916140079498,2.5672477590887866e-05
897898,1795797,1795796,3591593,1565.5371007919312,2.5297827278336626e-05
898899,1797799,1797798,3595597,1567.2068359851837,2.4928615971475665e-05
899900,1799801,1799800,3599601,1569.040277004242,2.456476488532644e-05
900901,1801803,1801802,3603605,1570.5874419212341,2.4206196144405112e-05
901902,1803805,1803804,3607609,1572.7006359100342,2.385283289640938e-05
902903,1805807,1805806,3611613,1574.3484728336334,2.3504599880652677e-05
903904,1807809,1807808,3615617,1575.9580459594727,2.31614220638221e-05
904905,1809811,1809810,3619621,1577.4998998641968,2.2823226458967838e-05
905906,1811813,1811812,3623625,1579.318463087082,2.2489940306513745e-05
906907,1813815,1813814,3627629,1581.0266258716583,2.2161492665873084e-05
907908,1815817,1815816,3631633,1583.3741540908813,2.183781293751963e-05
908909,1817819,1817818,3635637,1584.885351896286,2.1518832113542885e-05
909910,1819821,1819820,3639641,1586.3469741344452,2.1204482095527055e-05
910911,1821823,1821822,3643645,1587.8667171001434,2.0894695126116858e-05
911912,1823825,1823824,3647649,1589.328775882721,2.058940549432009e-05
912913,1825827,1825826,3651653,1591.0559067726135,2.0288547602831386e-05
913914,1827829,1827828,3655657,1592.7813138961792,1.999205687752692e-05
914915,1829831,1829830,3659661,1594.3326921463013,1.9699870222211757e-05
915916,1831833,1831832,3663665,1595.8432919979095,1.9411924995438312e-05
916917,1833835,1833834,3667669,1597.3114178180695,1.9128159806314216e-05
917918,1835837,1835836,3671673,1598.9234960079193,1.8848513491320773e-05
918919,1837839,1837838,3675677,1600.384677886963,1.8572926705928694e-05
919920,1839841,1839840,3679681,1601.8462080955505,1.8301340332982363e-05
920921,1841843,1841842,3683685,1603.3594880104065,1.8033696164820867e-05
921922,1843845,1843844,3687689,1604.9359550476074,1.776993713065167e-05
922923,1845847,1845846,3691693,1607.0012230873108,1.7510006614429585e-05
923924,1847849,1847848,3695697,1608.4964399337769,1.7253849136977806e-05
924925,1849851,1849850,3699701,1609.9689939022064,1.7001410128614225e-05
925926,1851853,1851852,3703705,1612.1955008506775,1.6752635133343574e-05
926927,1853855,1853854,3707709,1614.1737768650055,1.6507471173099475e-05
927928,1855857,1855856,3711713,1615.5876460075378,1.6265865838249738e-05
928929,1857859,1857858,3715717,1616.8650479316711,1.6027767514970037e-05
929930,1859861,1859860,3719721,1619.315311908722,1.5793125157870236e-05
930931,1861863,1861862,3723725,1620.9788229465485,1.5561888403681223e-05
931932,1863865,1863864,3727729,1622.6626379489899,1.533400825337594e-05
932933,1865867,1865866,3731733,1626.1250689029694,1.510943582161417e-05
933934,1867869,1867868,3735737,1627.811075925827,1.4888122791489877e-05
934935,1869871,1869870,3739741,1629.485948085785,1.4670022096652247e-05
935936,1871873,1871872,3743745,1631.3667759895325,1.4455087011810974e-05
936937,1873875,1873874,3747749,1633.2183909416199,1.4243271721170458e-05
937938,1875877,1875876,3751753,1634.9651079177856,1.4034530636308773e-05
938939,1877879,1877878,3755757,1637.5993139743805,1.382881919198553e-05
939940,1879881,1879880,3759761,1639.7569789886475,1.3626093846141885e-05
940941,1881883,1881882,3763765,1641.572278022766,1.3426310601971636e-05
941942,1883885,1883884,3767769,1643.250303030014,1.3229427054284315e-05
942943,1885887,1885886,3771773,1644.8329319953918,1.3035401025263127e-05
943944,1887889,1887888,3775777,1646.373820066452,1.2844191132899141e-05
944945,1889891,1889890,3779781,1647.886962890625,1.2655756449930777e-05
945946,1891893,1891892,3783785,1649.5157661437988,1.2470056617530645e-05
946947,1893895,1893894,3787789,1651.0491700172424,1.2287052072679217e-05
947948,1895897,1895896,3791793,1652.5844161510468,1.2106703366043803e-05
948949,1897899,1897898,3795797,1654.073117017746,1.192897229884693e-05
949950,1899901,1899900,3799801,1655.6435749530792,1.1753820672311122e-05
950951,1901903,1901902,3803805,1657.0885059833527,1.1581211197153607e-05
951952,1903905,1903904,3807809,1658.5575828552246,1.1411106925152126e-05
952953,1905907,1905906,3811813,1660.0255570411682,1.1243471249144932e-05
953954,1907909,1907908,3815817,1661.4697279930115,1.107826847146498e-05
954955,1909911,1909910,3819821,1663.0807089805603,1.091546323550574e-05
955956,1911913,1911912,3823825,1664.622614145279,1.0755020866781706e-05
956957,1913915,1913914,3827829,1666.2312641143799,1.0596907145554724e-05
957958,1915917,1915916,3831833,1667.7876827716827,1.0441087965773477e-05
958959,1917919,1917918,3835837,1669.6672129631042,1.0287530244568188e-05
959960,1919921,1919920,3839841,1671.1684329509735,1.0136200899069081e-05
960961,1921923,1921922,3843845,1672.624459028244,9.987067983274756e-06
961962,1923925,1923924,3847849,1674.2891669273376,9.840099096436461e-06
962963,1925927,1925926,3851853,1675.7717578411102,9.695263543108013e-06
963964,1927929,1927928,3855857,1677.271973848343,9.55252937728801e-06
964965,1929931,1929930,3859861,1679.755931854248,9.41186692671181e-06
965966,1931933,1931932,3863865,1681.7612388134003,9.273245609620062e-06
966967,1933935,1933934,3867869,1683.2586650848389,9.136636322182312e-06
967968,1935937,1935936,3871873,1684.7193858623505,9.002009505820752e-06
968969,1937939,1937938,3875877,1686.1767120361328,8.869336056704924e-06
969970,1939941,1939940,3879881,1687.6339769363403,8.738588348933263e-06
970971,1941943,1941942,3883885,1690.0143508911133,8.6097378471095e-06
971972,1943945,1943944,3887889,1691.876741886139,8.48275738007942e-06
972973,1945947,1945946,3891893,1693.9625718593597,8.357619435628294e-06
973974,1947949,1947948,3895897,1695.7516210079193,8.234297524722933e-06
974975,1949951,1949950,3899901,1697.6294569969177,8.112765385703824e-06
975976,1951953,1951952,3903905,1699.9072489738464,7.99299687059829e-06
976977,1953955,1953954,3907909,1701.574786901474,7.874966172494169e-06
977978,1955957,1955956,3911913,1703.2171568870544,7.758648393974e-06
978979,1957959,1957958,3915917,1704.7270810604095,7.64401863762032e-06
979980,1959961,1959960,3919921,1706.6277949810028,7.531052233389346e-06
980981,1961963,1961962,3923925,1708.228462934494,7.41972507967148e-06
981982,1963965,1963964,3927929,1710.057797908783,7.310013756978151e-06
982983,1965967,1965966,3931933,1712.4082930088043,7.2018942773866e-06
983984,1967969,1967968,3935937,1714.6061577796936,7.095343676155608e-06
984985,1969971,1969970,3939941,1716.0885798931122,6.990339329604467e-06
985986,1971973,1971972,3943945,1718.0037610530853,6.886858614052471e-06
986987,1973975,1973974,3947949,1719.6641418933868,6.784879815313616e-06
987988,1975977,1975976,3951953,1721.338320016861,6.684380423394032e-06
988989,1977979,1977978,3955957,1722.928689956665,6.585339633602416e-06
989990,1979981,1979980,3959961,1724.5073020458221,6.487735959126439e-06
990991,1981983,1981982,3963965,1726.0778620243073,6.391548481587961e-06
991992,1983985,1983984,3967969,1727.799901008606,6.296756964729866e-06
992993,1985987,1985986,3971973,1729.3629240989685,6.2033407175476896e-06
993994,1987989,1987988,3975977,1730.9545149803162,6.111280185905343e-06
994995,1989991,1989990,3979981,1732.6308498382568,6.020555474606226e-06
995996,1991993,1991992,3983985,1734.2629129886627,5.931147370574763e-06
996997,1993995,1993994,3987989,1735.896164894104,5.843036319674866e-06
997998,1995997,1995996,3991993,1737.560971736908,5.756203904638824e-06
998999,1997999,1997998,3995997,1739.0456221103668,5.67063148082525e-06
1000000,2000001,2000000,4000001,1740.5057470798492,5.58630085834011e-06


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0010797977447509766,2181.4194943796983
1001,2003,2002,4005,1.7322759628295898,60.32343774180572
2002,4005,4004,8009,3.436156988143921,53.8499366883982
3003,6007,6006,12013,5.12670111656189,50.99186825038555
4004,8009,8008,16017,6.967211008071899,48.752759392813005
5005,10011,10010,20021,8.713039875030518,46.758201211835285
6006,12013,12012,24025,10.542521953582764,44.93193088011094
7007,14015,14014,28029,12.3138587474823,43.244418145702184
8008,16017,16016,32033,14.05112886428833,41.67791649327205
9009,18019,18018,36037,15.774017095565796,40.219524300277726
10010,20021,20020,40041,17.488980054855347,38.85890210790262
11011,22023,22022,44045,19.48236083984375,37.58720739053888
12012,24025,24024,48049,21.045321941375732,36.39654519750411
13013,26027,26026,52053,22.687103986740112,35.27969401642213
14014,28029,28028,56057,24.253175020217896,34.229983159542144
15015,30031,30030,60061,25.87743592262268,33.24124787055848
16016,32033,32032,64065,27.68208909034729,32.30781785900831
17017,34035,34034,68069,29.286262035369873,31.424514341854547
18018,36037,36036,72073,30.84328293800354,30.586643297693854
19019,38039,38038,76077,32.451483964920044,29.789980392475854
20020,40041,40040,80081,34.00261688232422,29.030747349822832
21021,42043,42042,84085,35.51441311836243,28.30558157639757
22022,44045,44044,88089,37.08456778526306,27.61150150678054
23023,46047,46046,92093,38.65678906440735,26.945870036554425
24024,48049,48048,96097,40.437087059020996,26.306357978694678
25025,50051,50050,100101,41.981207847595215,25.69090895068757
26026,52053,52052,104105,43.678956031799316,25.09770660584445
27027,54055,54054,108109,45.30334115028381,24.52514471664108
28028,56057,56056,112113,46.770617961883545,23.971800313401673
29029,58059,58058,116117,48.33151698112488,23.436409869876798
30030,60061,60060,120121,49.86950993537903,22.917848391327652
31031,62063,62062,124125,51.71391797065735,22.415111182313467
32032,64065,64064,128129,53.72916889190674,21.92729803387965
33033,66067,66066,132133,55.447169065475464,21.45359955994786
34034,68069,68068,136137,57.34312987327576,20.993285420167922
35035,70071,70070,140141,59.047394037246704,20.545694184102103
36036,72073,72072,144145,60.51428985595703,20.110224614280924
37037,74075,74074,148149,61.963146924972534,19.686328170149636
38038,76077,76076,152153,63.38620400428772,19.27350255917554
39039,78079,78078,156157,64.84578204154968,18.871286184204337
40040,80081,80080,160161,66.27766680717468,18.479253356940035
41041,82083,82082,164165,67.70236396789551,18.097018269415912
42042,84085,84084,168169,69.13035297393799,17.724207800410795
43043,86087,86086,172173,70.611496925354,17.36048033181214
44044,88089,88088,176177,72.0864610671997,17.005517709993683
45045,90091,90090,180181,73.59081101417542,16.659021865107206
46046,92093,92092,184185,75.19619107246399,16.320712775821903
47047,94095,94094,188189,76.85569596290588,15.990326691478117
48048,96097,96096,192193,78.4301528930664,15.667614575622565
49049,98099,98098,196197,79.9661009311676,15.35234074024629
50050,100101,100100,200201,81.73948812484741,15.04428164456101
51051,102103,102102,204205,83.44010305404663,14.743224836003606
52052,104105,104104,208209,84.96208906173706,14.448968014390289
53053,106107,106106,212213,86.52702283859253,14.161318202901498
54054,108109,108108,216217,88.09581589698792,13.880091011916534
55055,110111,110110,220221,89.69855284690857,13.605109983691818
56056,112113,112112,224225,91.22568202018738,13.336206007555916
57057,114115,114114,228229,92.76970386505127,13.073216796736347
58058,116117,116116,232233,94.44235801696777,12.815986419143883
59059,118119,118118,236237,96.17238688468933,12.564364875481033
60060,120121,120120,240241,97.62502408027649,12.318207718933081
61061,122123,122122,244245,99.17944002151489,12.07737571146265
62062,124125,124124,248249,100.89015889167786,11.841734512372796
63063,126127,126126,252253,102.48617196083069,11.611154395377412
64064,128129,128128,256257,104.11504697799683,11.38550999088909
65065,130131,130130,260261,105.81780791282654,11.164680050656784
66066,132133,132132,264265,107.56823301315308,10.948547232246938
67067,134135,134134,268269,109.26113891601562,10.736997901167115
68068,136137,136136,272273,110.99563598632812,10.529921948711717
69069,138139,138138,276277,112.70289206504822,10.327212623838022
70070,140141,140140,280281,114.56143379211426,10.128766377590182
71071,142143,142142,284285,115.99800491333008,9.93448271876639
72072,144145,144144,288289,117.48617815971375,9.744264079690652
73073,146147,146146,292293,119.2016749382019,9.558015691076093
74074,148149,148148,296297,120.78351497650146,9.375645465104412
75075,150151,150150,300301,122.33246397972107,9.197063885941361
76076,152153,152152,304305,123.70971083641052,9.022183907010799
77077,154155,154154,308309,125.13052487373352,8.850920854432843
78078,156157,156156,312313,126.47548484802246,8.683192336101342
79079,158159,158158,316317,127.83176875114441,8.518918155943197
80080,160161,160160,320321,129.17073011398315,8.358020232960826
81081,162163,162162,324325,130.49153995513916,8.200422524697615
82082,164165,164164,328329,131.99801301956177,8.046050954820885
83083,166167,166166,332333,133.59094619750977,7.894833344540302
84084,168169,168168,336337,135.0182249546051,7.746699347615731
85085,170171,170170,340341,136.77029514312744,7.601580388726575
86086,172173,172172,344345,138.58396077156067,7.459409605000246
87087,174175,174174,348349,140.23649287223816,7.320121790511962
88088,176177,176176,352353,141.78791308403015,7.183653343569858
89089,178179,178178,356357,143.33162808418274,7.0499422166299155
90090,180181,180180,360361,145.12626194953918,6.918927868669698
91091,182183,182182,364365,147.12427806854248,6.790551219876079
92092,184185,184184,368369,148.90420579910278,6.664754608496992
93093,186187,186186,372373,150.76070404052734,6.54148174971499
94094,188189,188188,376377,152.99188089370728,6.420677696409257
95095,190191,190190,380381,154.6596338748932,6.302288801675672
96096,192193,192192,384385,156.37361311912537,6.186262682982374
97097,194195,194194,388389,158.0727949142456,6.072548187842131
98098,196197,196196,392393,159.73547291755676,5.961095360895797
99099,198199,198198,396397,161.3861608505249,5.851855412302029
100100,200201,200200,400401,162.9097499847412,5.744780687337993
101101,202203,202202,404405,164.58627891540527,5.639824637129436
102102,204205,204204,408409,166.17558979988098,5.5369417904232705
103103,206207,206206,412413,167.80450582504272,5.436087726335927
104104,208209,208208,416417,169.47753190994263,5.337219048009047
105105,210211,210210,420421,171.2418909072876,5.240293357116116
106106,212213,212212,424425,172.97698092460632,5.145269229163546
107107,214215,214214,428429,174.4481749534607,5.052106189540837
108108,216217,216216,432433,175.86870789527893,4.960764690277983
109109,218219,218218,436437,177.31137800216675,4.871206087469091
110110,220221,220220,440441,178.80704593658447,4.783392619330357
111111,222223,222222,444445,180.22077012062073,4.69728738486026
112112,224225,224224,448449,181.71382308006287,4.612854323075112
113113,226227,226226,452453,183.16911005973816,4.53005819279565
114114,228229,228228,456457,184.7056269645691,4.4488645529600035
115115,230231,230230,460461,186.13558197021484,4.3692397434441546
116116,232233,232232,464465,187.60770106315613,4.291150866371822
117117,234235,234234,468469,189.01887106895447,4.21456576789592
118118,236237,236236,472473,190.56363201141357,4.139453020433166
119119,238239,238238,476477,192.0859830379486,4.065781905345943
120120,240241,240240,480481,193.64076280593872,3.9935223960445683
121121,242243,242242,484485,195.3561737537384,3.9226451415119072
122122,244245,244244,488489,197.02102398872375,3.853121450227036
123123,246247,246246,492493,198.68611788749695,3.784923274483276
124124,248249,248248,496497,200.40835213661194,3.7180231950885627
125125,250251,250250,500501,201.93067383766174,3.6523944064375655
126126,252253,252252,504505,203.46500396728516,3.5880107019460183
127127,254255,254254,508509,204.95498299598694,3.524846459839523
128128,256257,256256,512513,206.463800907135,3.4628766292865976
129129,258259,258258,516517,208.0123360157013,3.4020767168683506
130130,260261,260260,520521,209.43351292610168,3.342422773377166
131131,262263,262262,524525,210.88280296325684,3.283891380934051
132132,264265,264264,528529,212.32262992858887,3.22645964042124
133133,266267,266266,532533,213.7566740512848,3.1701051592176555
134134,268269,268268,536537,215.1654908657074,3.1148060392353045
135135,270271,270270,540541,216.59967279434204,3.0605408652443202
136136,272273,272272,544545,218.12200498580933,3.007288693483474
137137,274275,274274,548549,219.5482850074768,2.955029040548652
138138,276277,276276,552553,220.99099707603455,2.90374187255145
139139,278279,278278,556557,222.43630695343018,2.853407594542432
140140,280281,280280,560561,223.89934992790222,2.804007040193028
141141,282283,282282,564565,225.34400010108948,2.7555214617298134
142142,284285,284284,568569,226.80340886116028,2.7079325201143547
143143,286287,286286,572573,228.28753113746643,2.6612222754635013
144144,288289,288288,576577,229.72203397750854,2.6153731777041003
145145,290291,290290,580581,231.2172770500183,2.5703680574572445
146146,292293,292292,584585,232.7512469291687,2.5261901171438694
147147,294295,294294,588589,234.2582437992096,2.4828229223113567
148148,296297,296296,592593,235.76648497581482,2.440250393169663
149149,298299,298298,596597,237.32105612754822,2.3984567963369727
150150,300301,300300,600601,238.811350107193,2.357426736786465
151151,302303,302302,604605,240.25778484344482,2.317145149990779
152152,304305,304304,608609,241.70306205749512,2.2775972942599765
153153,306307,306306,612613,243.16847705841064,2.2387687432658367
154154,308309,308308,616617,244.66359090805054,2.2006453787498685
155155,310311,310310,620621,246.16386008262634,2.1632133834108345
156156,312313,312312,624625,247.6495499610901,2.126459233964624
157157,314315,314314,628629,249.3806929588318,2.0903696943755676
158158,316317,316316,632633,250.90651607513428,2.0549318092529347
159159,318319,318318,636637,252.366632938385,2.020132897408189
160160,320321,320320,640641,253.81283688545227,1.9859605455708333
161161,322323,322322,644645,255.2459421157837,1.952402602256825
162162,324325,324324,648649,256.6880919933319,1.9194471717870556
163163,326327,326326,652653,258.12754106521606,1.8870826084518058
164164,328329,328328,656657,259.6324019432068,1.855297510817195
165165,330331,330330,660661,261.1683750152588,1.8240807161696466
166166,332333,332332,664665,262.75125193595886,1.793421295097005
167167,334335,334334,668669,264.4774489402771,1.7633085462001645
168168,336337,336336,672673,266.2025330066681,1.7337319909333928
169169,338339,338338,676677,267.8260519504547,1.7046813685698226
170170,340341,340340,680681,269.4344849586487,1.6761466312890434
171171,342343,342342,684685,271.05233001708984,1.6481179393834964
172172,344345,344344,688689,272.4718699455261,1.6205856565803742
173173,346347,346346,692693,273.92745995521545,1.5935403454776633
174174,348349,348348,696697,275.3689799308777,1.5669727630886428
175175,350351,350350,700701,276.8403158187866,1.5408738564954092
176176,352353,352352,704705,278.2819619178772,1.515234758605743
177177,354355,354354,708709,279.69067907333374,1.4900467840113834
178178,356357,356356,712713,281.1738669872284,1.4653014249485068
179179,358359,358358,716717,282.7337670326233,1.4409903473512031
180180,360361,360360,720721,284.28206396102905,1.4171053870035166
181181,362363,362362,724725,285.9685320854187,1.3936385457786855
182182,364365,364364,728729,287.4524779319763,1.370581987972514
183183,366367,366366,732733,288.9851019382477,1.347928036722351
184184,368369,368368,736737,290.4384949207306,1.325669170509741
185185,370371,370370,740741,291.84865498542786,1.3037980197493653
186186,372373,372372,744745,293.33456897735596,1.2823073634563116
187187,374375,374374,748749,294.76203179359436,1.261190125993835
188188,376377,376376,752753,296.2577769756317,1.2404393738961517
189189,378379,378378,756757,297.7465190887451,1.2200483127692223
190190,380381,380380,760761,299.23288893699646,1.200010284261566
191191,382383,382382,764765,300.7024619579315,1.1803187631088576
192192,384385,384384,768769,302.14919686317444,1.1609673542459404
193193,386387,386386,772773,303.6593849658966,1.1419497899877342
194194,388389,388388,776777,305.13542199134827,1.1232599272769903
195195,390391,390390,780781,306.689838886261,1.1048917449935516
196196,392393,392392,784785,308.15411400794983,1.0868393413301192
197197,394395,394394,788789,309.5803861618042,1.069096931226909
198198,396397,396396,792793,311.0343277454376,1.051658843865539
199199,398399,398398,796797,312.49370098114014,1.0345195202236255
200200,400401,400400,800801,313.945405960083,1.017673510683153
201201,402403,402402,804805,315.41670083999634,1.0011154726970517
202202,404405,404404,808809,316.8891599178314,0.9848401685069348
203203,406407,406406,812813,318.341383934021,0.9688424629160863
204204,408409,408408,816817,319.77430987358093,0.9531173211120176
205205,410411,410410,820821,321.21938490867615,0.9376598065392727
206206,412413,412412,824825,322.6912567615509,0.9224650788221425
207207,414415,414414,828829,324.12787890434265,0.9075283917339902
208208,416417,416416,832833,325.5614469051361,0.8928450912128483
209209,418419,418418,836837,327.03112983703613,0.878410613423739
210210,420421,420420,840841,328.51766085624695,0.8642204828635158
211211,422423,422422,844845,330.005872964859,0.8502703105094724
212212,424425,424424,848849,331.43304991722107,0.8365557920106994
213213,426427,426426,852853,332.8832359313965,0.8230727059193441
214214,428429,428428,856857,334.31148076057434,0.8098169119622298
215215,430431,430430,860861,335.74777603149414,0.7967843493526061
216216,432433,432432,864865,337.23565793037415,0.7839710351377107
217217,434435,434434,868869,339.89169216156006,0.7713730625855533
218218,436437,436436,872873,341.644366979599,0.7589865996083063
219219,438439,438438,876877,343.31804299354553,0.7468078872178694
220220,440441,440440,880881,345.0448188781738,0.734833238020542
221221,442443,442442,884885,346.804456949234,0.7230590347403449
222222,444445,444444,888889,348.3226659297943,0.7114817287806545
223223,446447,446446,892893,349.80082297325134,0.70009783881369
224224,448449,448448,896897,351.28832387924194,0.6889039494025155
225225,450451,450450,900901,352.7531988620758,0.6778967096552151
226226,452453,452452,904905,354.2611541748047,0.6670728319063528
227227,454455,454454,908909,355.7190499305725,0.6564290904298105
228228,456457,456456,912913,357.24599504470825,0.6459623201781142
229229,458459,458458,916917,358.847247838974,0.635669415551547
230230,460461,460460,920921,360.50407886505127,0.6255473291923863
231231,462463,462462,924925,362.07214283943176,0.6155930708072219
232232,464465,464464,928929,363.76761388778687,0.605803706013603
233233,466467,466466,932933,365.3004820346832,0.5961763552134016
234234,468469,468468,936937,366.7652518749237,0.5867081924897093
235235,470471,470470,940941,368.2267589569092,0.5773964445279489
236236,472473,472472,944945,369.66329407691956,0.5682383895614294
237237,474475,474474,948949,371.135812997818,0.5592313563379321
238238,476477,476476,952953,372.6351261138916,0.5503727231103994
239239,478479,478478,956957,374.08500480651855,0.5416599166485412
240240,480481,480480,960961,375.56579208374023,0.5330904112734061
241241,482483,482482,964965,377.03762006759644,0.5246617279086649
242242,484485,484484,968969,378.5284900665283,0.5163714331580422
243243,486487,486486,972973,380.033714056015,0.5082171383980949
244244,488489,488488,976977,381.529226064682,0.5001964988923646
245245,490491,490490,980981,382.97447776794434,0.4923072129238335
246246,492493,492492,984985,384.45708179473877,0.48454702094670665
247247,494495,494494,988989,385.8790400028229,0.4769137047555887
248248,496497,496496,992993,387.3605749607086,0.4694050866728503
249249,498499,498498,996997,388.83515977859497,0.4620190287519108
250250,500501,500500,1001001,390.2911560535431,0.4547534320003024
251251,502503,502502,1005005,391.7824649810791,0.447606235615126
252252,504505,504504,1009009,393.25491309165955,0.44057541623965335
253253,506507,506506,1013013,394.7461578845978,0.4336589872299328
254254,508509,508508,1017017,396.2552800178528,0.4268549979428826
255255,510511,510510,1021021,397.7375659942627,0.4201615330347295
256256,512513,512512,1025025,399.1716060638428,0.4135767117747946
257257,514515,514514,1029029,400.67915391921997,0.40709868737701527
258258,516517,516516,1033033,402.17130398750305,0.40072564634090213
259259,518519,518518,1037037,403.6134867668152,0.3944558078093223
260260,520521,520520,1041041,405.09507417678833,0.3882874229391291
261261,522523,522522,1045045,406.5473837852478,0.38221877428429707
262262,524525,524524,1049049,408.0195851325989,0.3762481751917903
263263,526527,526526,1053053,409.5424358844757,0.37037396921073196
264264,528529,528528,1057057,411.02641201019287,0.3645945295132833
265265,530531,530530,1061061,412.51233291625977,0.358908258327574
266266,532533,532532,1065065,413.9544668197632,0.3533135863821144
267267,534535,534534,1069069,415.4346499443054,0.3478089723625999
268268,536537,536536,1073073,416.9812397956848,0.34239290237871955
269269,538539,538538,1077077,418.4554901123047,0.33706388944222
270270,540541,540540,1081081,419.916512966156,0.33182047295645134
271271,542543,542542,1085085,421.4290599822998,0.326661218214781
272272,544545,544544,1089089,423.05970001220703,0.32158471591139914
273273,546547,546546,1093093,424.7674341201782,0.31658958166065077
274274,548549,548548,1097097,426.3863959312439,0.3116744555255764
275275,550551,550550,1101101,428.09225702285767,0.3068380015574803
276276,552553,552552,1105105,429.7419879436493,0.30207890734493503
277277,554555,554554,1109109,431.21353697776794,0.2973958835701751
278278,556557,556556,1113113,432.7625768184662,0.29278766357583663
279279,558559,558558,1117117,434.280394077301,0.2882530029409054
280280,560561,560560,1121121,435.7316617965698,0.2837906790635998
281281,562563,562562,1125125,437.23168110847473,0.2793994907533488
282282,564565,564564,1129129,438.7042498588562,0.275078257832547
283283,566567,566566,1133133,440.22297406196594,0.27082582074319816
284284,568569,568568,1137137,441.7988369464874,0.26664104016435886
285285,570571,570570,1141141,443.3304579257965,0.2625227966349257
286286,572573,572572,1145145,444.8818829059601,0.2584699901865406
287287,574575,574574,1149149,446.32426500320435,0.2544815399805884
288288,576577,576576,1153153,447.8227159976959,0.250556383955427
289289,578579,578578,1157157,449.3005998134613,0.24669347847896006
290290,580581,580580,1161161,450.8010540008545,0.24289179800825877
291291,582583,582582,1165165,452.37873005867004,0.23915033475645942
292292,584585,584584,1169169,453.9415509700775,0.2354680983654589
293293,586587,586586,1173173,455.44157791137695,0.23184411558656848
294294,588589,588588,1177177,456.92967891693115,0.22827742996514644
295295,590591,590590,1181181,458.4190630912781,0.22476710153387103
296296,592593,592592,1185185,459.8805019855499,0.22131220651010608
297297,594595,594594,1189189,461.33191299438477,0.2179118370006563
298298,596597,596596,1193193,462.85971212387085,0.2145651007114111
299299,598599,598598,1197197,464.34163308143616,0.21127112066255904
300300,600601,600600,1201201,465.84709310531616,0.20802903491016878
301301,602603,602602,1205205,467.30771112442017,0.2048379962729996
302302,604605,604604,1209209,468.83738708496094,0.20169717206340465
303303,606607,606606,1213213,470.32841300964355,0.1986057438257376
304304,608609,608608,1217217,471.8052570819855,0.19556290707782864
305305,610611,610610,1221221,473.3081250190735,0.19256787105769035
306306,612613,612612,1225225,474.7487139701843,0.18961985847715823
307307,614615,614614,1229229,476.1932260990143,0.18671810527735033
308308,616617,616616,1233233,477.7047109603882,0.18386186039026597
309309,618619,618618,1237237,479.17032980918884,0.18105038550640984
310310,620621,620620,1241241,480.65046310424805,0.17828295484412138
311311,622623,622622,1245245,482.1480348110199,0.1755588549250433
312312,624625,624624,1249249,483.6084408760071,0.17287738435334177
313313,626627,626626,1253253,485.9599859714508,0.1702378535999287
314314,628629,628628,1257257,488.04223895072937,0.16763958478964014
315315,630631,630630,1261261,490.30247616767883,0.16508191149330287
316316,632633,632632,1265265,492.00120997428894,0.16256417852355298
317317,634635,634634,1269269,493.6886570453644,0.1600857417338375
318318,636637,636636,1273273,495.20043897628784,0.15764596782310036
319319,638639,638638,1277277,496.6652569770813,0.15524423414240118
320320,640641,640640,1281281,498.15423583984375,0.1528799285055129
321321,642643,642642,1285285,499.63140892982483,0.15055244900327125
322322,644645,644644,1289289,501.106892824173,0.1482612038228126
323323,646647,646646,1293293,502.5863161087036,0.14600561106726673
324324,648649,648648,1297297,504.0683741569519,0.1437850985815885
325325,650651,650650,1301301,505.6792447566986,0.14159910378020868
326326,652653,652652,1305305,507.25518703460693,0.1394470734786637
327327,654655,654654,1309309,508.78602600097656,0.13732846372772656
328328,656657,656656,1313313,510.1982400417328,0.13524273965106204
329329,658659,658658,1317317,511.60401487350464,0.1331893752862925
330330,660661,660660,1321321,513.0901520252228,0.1311678534272005
331331,662663,662662,1325325,514.5436398983002,0.12917766547218434
332332,664665,664664,1329329,516.0252590179443,0.127218311272145
333333,666667,666666,1333333,517.5166819095612,0.1252892989832617
334334,668669,668668,1337337,519.0003719329834,0.12339014492147271
335335,670671,670670,1341341,520.4618229866028,0.12152037342150379
336336,672673,672672,1345345,521.915543794632,0.11967951669475951
337337,674675,674674,1349349,523.4082100391388,0.11786711469414968
338338,676677,676676,1353353,524.8848600387573,0.11608271497880196
339339,678679,678678,1357357,526.3465888500214,0.11432587258150306
340340,680681,680680,1361361,527.8110649585724,0.11259614988000521
341341,682683,682682,1365365,529.3258938789368,0.11089311646821898
342342,684685,684684,1369369,530.7794749736786,0.1092163490332041
343343,686687,686686,1373373,532.2405819892883,0.10756543123102347
344344,688689,688688,1377377,533.712397813797,0.10593995356623509
345345,690691,690690,1381381,535.1796629428864,0.10433951327536306
346346,692693,692692,1385385,536.6775329113007,0.10276371420843589
347347,694695,694694,1389389,538.1994519233704,0.10121216671711863
348348,696697,696696,1393393,539.7711389064789,0.09968448754170822
349349,698699,698698,1397397,541.3140339851379,0.09818029970210773
350350,700701,700700,1401401,542.89031291008,0.09669923238857336
351351,702703,702702,1405405,544.4553301334381,0.0952409208583731
352352,704705,704704,1409409,546.0297379493713,0.09380500632926214
353353,706707,706706,1413413,547.549712896347,0.09239113587864267
354354,708709,708708,1417417,549.0540778636932,0.09099896234386051
355355,710711,710710,1421421,550.5440468788147,0.08962814422284282
356356,712713,712712,1425425,552.1855938434601,0.08827834557780534
357357,714715,714714,1429429,553.8580429553986,0.08694923594055126
358358,716717,716716,1433433,555.4758768081665,0.08564049021970277
359359,718719,718718,1437437,557.1337821483612,0.08435178860804626
360360,720721,720720,1441441,558.8825299739838,0.08308281649419769
361361,722723,722722,1445445,560.4138140678406,0.08183326437278993
362362,724725,724724,1449449,562.0019431114197,0.08060282775966243
363363,726727,726726,1453453,563.4827699661255,0.0793912071047771
364364,728729,728728,1457457,564.9641218185425,0.07819810771093216
365365,730731,730730,1461461,566.4269378185272,0.07702323964929292
366366,732733,732732,1465465,567.8761098384857,0.07586631768037932
367367,734735,734734,1469469,569.3799619674683,0.07472706117493999
368368,736737,736736,1473473,570.945271730423,0.07360519403493981
369369,738739,738738,1477477,572.5459339618683,0.07250044461875405
370370,740741,740740,1481481,574.0724430084229,0.07141254566511179
371371,742743,742742,1485485,575.5712070465088,0.07034123421942695
372372,744745,744744,1489489,577.0665819644928,0.06928625156228918
373373,746747,746746,1493493,578.5458879470825,0.06824734313750014
374374,748749,748748,1497497,580.0982868671417,0.06722425848215607
375375,750751,750750,1501501,581.6805589199066,0.06621675115945891
376376,752753,752752,1505505,583.233628988266,0.06522457868925358
377377,754755,754754,1509509,584.8020029067993,0.06424750248322653
378378,756757,756756,1513513,586.335037946701,0.06328528777999054
379379,758759,758758,1517517,587.8197247982025,0.06233770358005586
380380,760761,760760,1521521,589.2855889797211,0.061404522583984544
381381,762763,762762,1525525,590.7487728595734,0.06048552113043115
382382,764765,764764,1529529,592.2732779979706,0.05958047913543396
383383,766767,766766,1533533,593.7790191173553,0.058689180033752564
384384,768769,768768,1537537,595.2876617908478,0.0578114107189549
385385,770771,770770,1541541,596.7942979335785,0.05694696148680123
386386,772773,772772,1545545,598.2710690498352,0.05609562597851436
387387,774775,774774,1549549,599.7713627815247,0.05525720112586896
388388,776777,776776,1553553,601.2876689434052,0.05443148709628076
389389,778779,778778,1557557,602.8011977672577,0.05361828723857798
390390,780781,780780,1561561,604.2381660938263,0.05281740803161483
391391,782783,782782,1565565,605.7485239505768,0.05202865903163456
392392,784785,784784,1569569,607.2071650028229,0.0512518528222472
393393,786787,786786,1573573,608.6321380138397,0.050486804963270515
394394,788789,788788,1577577,610.1330718994141,0.04973333394298152
395395,790791,790790,1581581,611.7045459747314,0.04899126112911745
396396,792793,792792,1585585,613.2296578884125,0.04826041072158205
397397,794795,794794,1589589,614.7116639614105,0.047540609705947645
398398,796797,796796,1593593,616.2493598461151,0.046831687807980416
399399,798799,798798,1597597,617.8353769779205,0.046133477448279336
400400,800801,800800,1601601,619.3808720111847,0.04544581369759726
401401,802803,802802,1605605,620.8971540927887,0.04476853423466309
402402,804805,804804,1609609,622.3888440132141,0.044101479302298685
403403,806807,806806,1613613,623.8628528118134,0.043444491666264184
404404,808809,808808,1617617,625.2984688282013,0.04279741657308023
405405,810811,810810,1621621,626.7712068557739,0.0421601017105786
406406,812813,812812,1625625,628.2984998226166,0.041532397167088675
407407,814815,814814,1629629,629.845116853714,0.040914155393238616
408408,816817,816816,1633633,631.3794040679932,0.04030523116193763
409409,818819,818818,1637637,632.8831548690796,0.03970548153256459
410410,820821,820820,1641641,634.4005830287933,0.0391147658118598
411411,822823,822822,1645645,635.8793301582336,0.03853294551822728
412412,824825,824824,1649649,637.3277997970581,0.0379598843463782
413413,826827,826826,1653653,638.8237929344177,0.037395448130496334
414414,828829,828828,1657657,640.3080861568451,0.03683950481092779
415415,830831,830830,1661661,641.7435998916626,0.03629192439882445
416416,832833,832832,1665665,643.2663550376892,0.03575257894362949
417417,834835,834834,1669669,644.8045120239258,0.03522134249953979
418418,836837,836836,1673673,646.3415579795837,0.034698091093218864
419419,838839,838838,1677677,647.8439049720764,0.034182702691396116
420420,840841,840840,1681681,649.454393863678,0.03367505717028507
421421,842843,842842,1685685,651.1244060993195,0.03317503628443319
422422,844845,844844,1689689,652.8183870315552,0.03268252363579904
423423,846847,846846,1693693,654.7130579948425,0.03219740464498955
424424,848849,848848,1697697,656.4030609130859,0.03171956652147401
425425,850851,850850,1701701,658.0776147842407,0.031248898234480293
426426,852853,852852,1705705,659.755735874176,0.030785290485368932
427427,854855,854854,1709709,661.4606919288635,0.03032863567852928
428428,856857,856856,1713713,663.0412800312042,0.02987882789602736
429429,858859,858858,1717717,664.5531878471375,0.02943576286827465
430430,860861,860860,1721721,666.4320797920227,0.028999337949471737
431431,862863,862862,1725725,668.4071130752563,0.028569452090664527
432432,864865,864864,1729729,670.383584022522,0.028146005814278396
433433,866867,866866,1733733,672.0726108551025,0.02772890118910709
434434,868869,868868,1737737,673.7473969459534,0.027318041805074245
435435,870871,870870,1741741,675.4432330131531,0.02691333274981389
436436,872873,872872,1745745,677.2095067501068,0.026514680583659356
437437,874875,874874,1749749,678.8389718532562,0.0261219933169059
438438,876877,876876,1753753,680.4062080383301,0.02573518038639122
439439,878879,878878,1757757,682.0567481517792,0.025354152632417026
440440,880881,880880,1761761,683.7107689380646,0.024978822276921164
441441,882883,882882,1765765,685.532408952713,0.024609102901081314
442442,884885,884884,1769769,687.267865896225,0.024244909423941863
443443,886887,886886,1773773,689.097158908844,0.02388615808047234
444444,888889,888888,1777777,690.962338924408,0.02353276640178592
445445,890891,890890,1781781,692.8013670444489,0.023184653193197846
446446,892893,892892,1785785,694.5102317333221,0.02284173851523974
447447,894895,894894,1789789,696.3210351467133,0.022503943662286474
448448,896897,896896,1793793,698.2095670700073,0.022171191144707336
449449,898899,898898,1797797,699.916296005249,0.0218434046684024
450450,900901,900900,1801801,701.7748739719391,0.02152050911581682
451451,902903,902902,1805805,703.4400231838226,0.021202430527523575
452452,904905,904904,1809809,705.2298419475555,0.02088909608482936
453453,906907,906906,1813813,706.9768998622894,0.020580434089652044
454454,908909,908908,1817817,708.8334670066833,0.020276373949059234
455455,910911,910910,1821821,710.6101140975952,0.01997684615628259
456456,912913,912912,1825825,712.3135240077972,0.01968178227377848
457457,914915,914914,1829829,714.1039538383484,0.019391114917311825
458458,916917,916916,1833833,715.8606789112091,0.019104777737652512
459459,918919,918918,1837837,717.3649401664734,0.01882270540625086
460460,920921,920920,1841841,719.0159969329834,0.018544833597502475
461461,922923,922922,1845845,720.5794818401337,0.018271098973286826
462462,924925,924924,1849849,722.246376991272,0.018001439168756406
463463,926927,926926,1853853,723.8177070617676,0.017735792775056325
464464,928929,928928,1857857,725.457878112793,0.017474099325227144
465465,930931,930930,1861861,727.0818729400635,0.017216299279766645
466466,932933,932932,1865865,728.6424770355225,0.016962334011509483
467467,934935,934934,1869869,730.1618609428406,0.01671214579153002
468468,936937,936936,1873873,731.7685859203339,0.016465677774590404
469469,938939,938938,1877877,733.4346377849579,0.016222873986066588
470470,940941,940940,1881881,735.1072220802307,0.015983679308078536
471471,942943,942942,1885885,736.9537401199341,0.015748039465165675
472472,944945,944944,1889889,738.5482559204102,0.015515901012349786
473473,946947,946946,1893893,740.1973130702972,0.015287211321606264
474474,948949,948948,1897897,741.7431490421295,0.015061918568790134
475475,950951,950950,1901901,743.2382380962372,0.01483997172135787
476476,952953,952952,1905905,744.7396008968353,0.014621320526543968
477477,954955,954954,1909909,746.2202010154724,0.014405915497832211
478478,956957,956956,1913913,747.747918844223,0.014193707904269104
479479,958959,958958,1917917,749.2732839584351,0.013984649757958323
480480,960961,960960,1921921,750.7625830173492,0.013778693803033093
481481,962963,962962,1925925,752.2312951087952,0.013575793503378009
482482,964965,964964,1929929,753.7182538509369,0.013375903032624592
483483,966967,966966,1933933,755.3131878376007,0.013178977261532054
484484,968969,968968,1937937,757.0639309883118,0.012984971749119723
485485,970971,970970,1941941,758.7160258293152,0.012793842729820426
486486,972973,972972,1945945,760.2002239227295,0.012605547104612924
487487,974975,974974,1949949,761.678297996521,0.012420042429994282
488488,976977,976976,1953953,763.1602110862732,0.01223728690763437
489489,978979,978978,1957957,764.6522459983826,0.01205723937471248
490490,980981,980980,1961961,766.1437468528748,0.011879859294253947
491491,982983,982982,1965965,767.803328037262,0.01170510674421621
492492,984985,984984,1969969,769.4421379566193,0.011532942409871794
493493,986987,986986,1973973,771.1369931697845,0.011363327572325943
494494,988989,988988,1977977,773.0053551197052,0.01119622410124066
495495,990991,990990,1981981,774.4782328605652,0.011031594444489201
496496,992993,992992,1985985,776.4361329078674,0.010869401618833763
497497,994995,994994,1989989,778.109983921051,0.01070960920287689
498498,996997,996996,1993993,779.5952739715576,0.010552181326261234
499499,998999,998998,1997997,781.0977988243103,0.010397082662734647
500501,1001003,1001002,2002005,782.5744640827179,0.010244126905263329
501502,1003005,1003004,2006009,784.046854019165,0.010093585062236343
502503,1005007,1005006,2010013,785.5575790405273,0.009945269597551487
503504,1007009,1007008,2014017,787.0387651920319,0.009799147277021802
504505,1009011,1009010,2018021,788.4889831542969,0.00965518536872878
505506,1011013,1011012,2022025,789.9944620132446,0.009513351636655898
506507,1013015,1013014,2026029,791.462954044342,0.009373614331138924
507508,1015017,1015016,2030033,793.0488448143005,0.009235942183636325
508509,1017019,1017018,2034037,794.5511958599091,0.00910030439717957
509510,1019021,1019020,2038041,796.0280809402466,0.00896667064068879
510511,1021023,1021022,2042045,797.5344920158386,0.008835011040901009
511512,1023025,1023024,2046049,799.2263128757477,0.008705296175776311
512513,1025027,1025026,2050053,800.8709619045258,0.008577497067108197
513514,1027029,1027028,2054057,802.9871439933777,0.008451585174157117
514515,1029031,1029030,2058061,805.3350610733032,0.008327532387170322
515516,1031033,1031032,2062065,806.9185070991516,0.008205311019651162
516517,1033035,1033034,2066069,808.5448060035706,0.00808489380312949
517518,1035037,1035036,2070073,810.2785699367523,0.007966253879772012
518519,1037039,1037038,2074077,811.8565320968628,0.007849364796811642
519520,1039041,1039040,2078081,813.4349269866943,0.007734200499612598
520521,1041043,1041042,2082085,814.9993648529053,0.007620735326554495
521522,1043045,1043044,2086089,816.4991519451141,0.007508944002097451
522523,1045047,1045046,2090093,817.9761028289795,0.00739880163109774
523524,1047049,1047048,2094097,819.4275860786438,0.007290283693237143
524525,1049051,1049050,2098101,821.0453441143036,0.007183366037111227
525526,1051053,1051052,2102105,822.6748390197754,0.007078024874431321
526527,1053055,1053054,2106109,824.3424100875854,0.006974236775135978
527528,1055057,1055056,2110113,826.2070019245148,0.006871978660910827
528529,1057059,1057058,2114117,828.1467900276184,0.006771227800527413
529530,1059061,1059060,2118121,830.0747127532959,0.006671961804158855
530531,1061063,1061062,2122125,831.5190920829773,0.006574158618604997
531532,1063065,1063064,2126129,832.9437928199768,0.006477796521949131
532533,1065067,1065066,2130133,834.2630391120911,0.006382854118328396
533534,1067069,1067068,2134137,835.8341541290283,0.00628931033270419
534535,1069071,1069070,2138141,837.86381483078,0.006197144406996813
535536,1071073,1071072,2142145,839.2682979106903,0.006106335893832693
536537,1073075,1073074,2146149,841.0829849243164,0.006016864653588527
537538,1075077,1075076,2150153,842.7000329494476,0.005928710847570073
538539,1077079,1077078,2154157,844.2881460189819,0.005841854935624724
539540,1079081,1079080,2158161,846.1957819461823,0.005756277669547671
540541,1081083,1081082,2162165,848.0591077804565,0.005671960090239736
541542,1083085,1083084,2166169,849.9270570278168,0.005588883522364085
542543,1085087,1085086,2170173,851.7650408744812,0.005507029570821942
543544,1087089,1087088,2174177,853.6063580513,0.005426380115181928
544545,1089091,1089090,2178181,855.4732229709625,0.005346917307065269
545546,1091093,1091092,2182185,857.9143707752228,0.00526862356480251
546547,1093095,1093094,2186189,860.0232651233673,0.005191481570250289
547548,1095097,1095096,2190193,861.6965479850769,0.005115474264130171
548549,1097099,1097098,2194197,863.5933787822723,0.005040584842845419
549550,1099101,1099100,2198201,865.1754109859467,0.004966796753251401
550551,1101103,1101102,2202205,866.7000961303711,0.004894093690609225
551552,1103105,1103104,2206209,868.4977300167084,0.004822459593242456
552553,1105107,1105106,2210213,870.0587389469147,0.004751878640149698
553554,1107109,1107108,2214217,871.6329071521759,0.004682335246229741
554555,1109111,1109110,2218221,873.3363621234894,0.0046138140595530786
555556,1111113,1111112,2222225,875.943363904953,0.004546299957610245
556557,1113115,1113114,2226229,877.7469170093536,0.0044797780434464585
557558,1115117,1115116,2230233,879.4946990013123,0.0044142336424783934
558559,1117119,1117118,2234237,881.2018330097198,0.004349652299652007
559560,1119121,1119120,2238241,882.6666588783264,0.0042860197751224405
560561,1121123,1121122,2242245,884.3041749000549,0.004223322041980282
561562,1123125,1123124,2246249,885.7905209064484,0.004161545282386214
562563,1125127,1125126,2250253,887.5806488990784,0.0041006758842740965
563564,1127129,1127128,2254257,889.2402718067169,0.004040700439304601
564565,1129131,1129130,2258261,890.9704530239105,0.003981605738545113
565566,1131133,1131132,2262265,892.5709478855133,0.003923378770082309
566567,1133135,1133134,2266269,894.297111749649,0.003866006715838921
567568,1135137,1135136,2270273,896.0486319065094,0.0038094769489589453
568569,1137139,1137138,2274277,897.5153558254242,0.0037537770305107188
569570,1139141,1139140,2278281,899.2181899547577,0.003698894707213185
570571,1141143,1141142,2282285,900.8570377826691,0.003644817907570541
571572,1143145,1143144,2286289,902.4495370388031,0.0035915347405079956
572573,1145147,1145146,2290293,904.1365718841553,0.003539033492188537
573574,1147149,1147148,2294297,905.963082075119,0.0034873026218065206
574575,1149151,1149150,2298301,907.6398739814758,0.003436330761815043
575576,1151153,1151152,2302305,909.7453498840332,0.003386106712810033
576577,1153155,1153154,2306309,911.6182370185852,0.0033366194425070717
577578,1155157,1155156,2310313,913.1316568851471,0.003287858082785533
578579,1157159,1157158,2314317,914.6124799251556,0.0032398119265053538
579580,1159161,1159160,2318321,916.3030619621277,0.0031924704262564774
580581,1161163,1161162,2322325,917.8790040016174,0.0031458231916303703
581582,1163165,1163164,2326329,919.7460589408875,0.003099859986150477
582583,1165167,1165166,2330333,921.4826231002808,0.003054570725225858
583584,1167169,1167168,2334337,923.1619420051575,0.0030099454751280064
584585,1169171,1169170,2338341,924.6416320800781,0.0029659744487844364
585586,1171173,1171172,2342345,926.1776449680328,0.002922648004982875
586587,1173175,1173174,2346349,927.7181389331818,0.002879956645074344
587588,1175177,1175176,2350353,929.2710249423981,0.002837891012632099
588589,1177179,1177178,2354357,930.9037389755249,0.002796441888449408
589590,1179181,1179180,2358361,932.4396188259125,0.0027556001919037953
590591,1181183,1181182,2362365,934.1366589069366,0.0027153569758411322
591592,1183185,1183184,2366369,935.8880920410156,0.0026757034264619506
592593,1185187,1185186,2370373,937.7557578086853,0.002636630860479272
593594,1187189,1187188,2374377,939.3010330200195,0.002598130723754366
594595,1189191,1189190,2378381,940.8032341003418,0.0025601945885682653
595596,1191193,1191192,2382385,942.4042398929596,0.0025228141528259584
596597,1193195,1193194,2386389,944.2511160373688,0.002485981236304724
597598,1195197,1195196,2390393,945.9084610939026,0.0024496877815636253
598599,1197199,1197198,2394397,947.392040014267,0.0024139258495097238
599600,1199201,1199200,2398401,948.8999161720276,0.002378687619284392
600601,1201203,1201202,2402405,950.7193479537964,0.002343965385193769
601602,1203205,1203204,2406409,952.6626598834991,0.0023097515565950744
602603,1205207,1205206,2410413,954.2807040214539,0.0022760386549407485
603604,1207209,1207208,2414417,956.69824385643,0.0022428193118457784
604605,1209211,1209210,2418421,958.3663277626038,0.0022100862692013834
605606,1211213,1211212,2422425,959.9464011192322,0.002177832375309663
606607,1213215,1213214,2426429,961.7352290153503,0.0021460505847699096
607608,1215217,1215216,2430433,964.0117909908295,0.00211473395665962
608609,1217219,1217218,2434437,966.1336989402771,0.002083875652374445
609610,1219221,1219220,2438441,968.4321579933167,0.002053468934718694
610611,1221223,1221222,2442445,969.992527961731,0.0020235071662000337
611612,1223225,1223224,2446449,971.6475117206573,0.001993983807551558
612613,1225227,1225226,2450453,973.3309121131897,0.0019648924157991132
613614,1227229,1227228,2454457,974.8359789848328,0.0019362266441476095
614615,1229231,1229230,2458461,976.2766809463501,0.0019079802386841038
615616,1231233,1231232,2462465,977.7100870609283,0.0018801470383777996
616617,1233235,1233234,2466469,979.1681208610535,0.001852720973374744
617618,1235237,1235236,2470473,980.5889270305634,0.0018256960635198993
618619,1237239,1237238,2474477,982.0731310844421,0.0017990664168792136
619620,1239241,1239240,2478481,984.168536901474,0.0017728262284890661
620621,1241243,1241242,2482485,985.773185968399,0.0017469697795604588
621622,1243245,1243244,2486489,987.3502731323242,0.0017214914354326538
622623,1245247,1245246,2490493,988.9595017433167,0.0016963856446636782
623624,1247249,1247248,2494497,990.5476899147034,0.0016716469381208299
624625,1249251,1249250,2498501,992.0244839191437,0.0016472699272753744
625626,1251253,1251252,2502505,993.4502620697021,0.00162324930295199
626627,1253255,1253254,2506509,995.1702148914337,0.0015995798344192735
627628,1255257,1255256,2510513,997.043613910675,0.0015762563684802444
628629,1257259,1257258,2514517,998.5925760269165,0.0015532738277670433
629630,1259261,1259260,2518521,1000.5119171142578,0.0015306272097177498
630631,1261263,1261262,2522525,1002.4872369766235,0.001508311585894262
631632,1263265,1263264,2526529,1004.0923368930817,0.0014863221001633065
632633,1265267,1265266,2530533,1005.5577340126038,0.0014646539682416915
633634,1267269,1267268,2534537,1006.9987337589264,0.001443302476786812
634635,1269271,1269270,2538541,1008.4286789894104,0.0014222629813502863
635636,1271273,1271272,2542545,1010.1057560443878,0.0014015309063779569
636637,1273275,1273274,2546549,1012.0740239620209,0.0013811017438456474
637638,1275277,1275276,2550553,1013.5565891265869,0.0013609710513264872
638639,1277279,1277278,2554557,1014.9991140365601,0.0013411344533551528
639640,1279281,1279280,2558561,1016.4421629905701,0.0013215876375625157
640641,1281283,1281282,2562565,1017.892077922821,0.0013023263561535714
641642,1283285,1283284,2566569,1019.3163850307465,0.001283346423065268
642643,1285287,1285286,2570573,1020.7520678043365,0.0012646437147623146
643644,1287289,1287288,2574577,1022.1861929893494,0.0012462141679634442
644645,1289291,1289290,2578581,1023.6366090774536,0.0012280537793003532
645646,1291293,1291292,2582585,1025.241261959076,0.0012101586044082069
646647,1293295,1293294,2586589,1027.3831679821014,0.0011925247569024577
647648,1295297,1295296,2590593,1029.571171760559,0.001175148408037785
648649,1297299,1297298,2594597,1031.4095890522003,0.0011580257847754183
649650,1299301,1299300,2598601,1033.346519947052,0.001141153170351572
650651,1301303,1301302,2602605,1035.5646359920502,0.001124526902344769
651652,1303305,1303304,2606609,1037.245770931244,0.0011081433718800326
652653,1305307,1305306,2610613,1039.1778330802917,0.001091999024197321
653654,1307309,1307308,2614617,1041.272570848465,0.001076090355809356
654655,1309311,1309310,2618621,1042.9917469024658,0.001060413915524805
655656,1311313,1311312,2622625,1045.5265259742737,0.001044966302629291
656657,1313315,1313314,2626629,1048.2789950370789,0.001029744165862212
657658,1315317,1315316,2630633,1050.3971688747406,0.001014744204667295
658659,1317319,1317318,2634637,1052.6813640594482,0.000999963165668305
659660,1319321,1319320,2638641,1054.5118107795715,0.0009853978441469735
660661,1321323,1321322,2642645,1056.7115659713745,0.0009710450823376959
661662,1323325,1323324,2646649,1058.6534888744354,0.0009569017686317238
662663,1325327,1325326,2650653,1060.462984085083,0.0009429648373497912
663664,1327329,1327328,2654657,1062.1243209838867,0.0009292312679463066
664665,1329331,1329330,2658661,1063.5991480350494,0.000915698084440919
665666,1331333,1331332,2662665,1065.3962440490723,0.0009023623542816495
666667,1333335,1333334,2666669,1067.1662590503693,0.0008892211878901435
667668,1335337,1335336,2670673,1068.7050340175629,0.0008762717386616714
668669,1337339,1337338,2674677,1071.1616761684418,0.0008635112014871993
669670,1339341,1339340,2678681,1073.4426908493042,0.0008509368126397021
670671,1341343,1341342,2682685,1075.5292029380798,0.0008385458487509823
671672,1343345,1343344,2686689,1077.5852711200714,0.0008263356266979827
672673,1345347,1345346,2690693,1079.1722569465637,0.0008143035025796053
673674,1347349,1347348,2694697,1081.691181898117,0.0008024468716030242
674675,1349351,1349350,2698701,1083.7391498088837,0.0007907631669468174
675676,1351353,1351352,2702705,1085.5600938796997,0.0007792498596472797
676677,1353355,1353354,2706709,1087.017364025116,0.0007679044579163019
677678,1355357,1355356,2710713,1088.4610459804535,0.0007567245064592498
678679,1357359,1357358,2714717,1089.8849878311157,0.0007457075855654693
679680,1359361,1359360,2718721,1091.356279850006,0.0007348513125862155
680681,1361363,1361362,2722725,1092.8142569065094,0.0007241533373871789
681682,1363365,1363364,2726729,1094.6545639038086,0.0007136113467822724
682683,1365367,1365366,2730733,1096.5398950576782,0.0007032230599861578
683684,1367369,1367368,2734737,1098.0755751132965,0.0006929862304332346
684685,1369371,1369370,2738741,1099.623454093933,0.0006828986441860252
685686,1371373,1371372,2742745,1101.1473181247711,0.0006729581197078005
686687,1373375,1373374,2746749,1102.6718690395355,0.0006631625076352066
687688,1375377,1375376,2750753,1104.3801510334015,0.000653509690437204
688689,1377379,1377378,2754757,1106.0763850212097,0.0006439975811645127
689690,1379381,1379380,2758761,1107.6301510334015,0.0006346241234496119
690691,1381383,1381382,2762765,1109.0525670051575,0.0006253872916204273
691692,1383385,1383384,2766769,1110.4306559562683,0.0006162850889950278
692693,1385387,1385386,2770773,1111.927206993103,0.0006073155491321813
693694,1387389,1387388,2774777,1113.424516916275,0.0005984767331028706
694695,1389391,1389390,2778781,1114.9093000888824,0.0005897667318777167
695696,1391393,1391392,2782785,1116.3957509994507,0.0005811836633711209
696697,1393395,1393394,2786789,1117.7999801635742,0.0005727256732370734
697698,1395397,1395396,2790793,1119.5309598445892,0.0005643909346417786
698699,1397399,1397398,2794797,1121.0053000450134,0.0005561776474678481
699700,1399401,1399400,2798801,1122.8722059726715,0.0005480840375184926
700701,1401403,1401402,2802805,1124.49413895607,0.000540108357427016
701702,1403405,1403404,2806809,1125.9315819740295,0.0005322488847241402
702703,1405407,1405406,2810813,1127.3644020557404,0.0005245039226338122
703704,1407409,1407408,2814817,1128.7881071567535,0.0005168717984815885
704705,1409411,1409410,2818821,1130.2519299983978,0.0005093508653999379
705706,1411413,1411412,2822825,1131.7044439315796,0.0005019394993723836
706707,1413415,1413414,2826829,1133.1309299468994,0.0004946361009388056
707708,1415417,1415416,2830833,1134.5472478866577,0.0004874390936038253
708709,1417419,1417418,2834837,1135.9643149375916,0.00048034692429155257
709710,1419421,1419420,2838841,1137.3681480884552,0.0004733580626634648
710711,1421423,1421422,2842845,1138.8042500019073,0.00046647100066365965
711712,1423425,1423424,2846849,1140.2450950145721,0.0004596842521777944
712713,1425427,1425426,2850853,1141.6861598491669,0.0004529963531467729
713714,1427429,1427428,2854857,1143.1551780700684,0.0004464058607709376
714715,1429431,1429430,2858861,1144.871325969696,0.00043991135339638276
715716,1431433,1431432,2862865,1147.2256870269775,0.0004335114302875809
716717,1433435,1433434,2866869,1149.66739487648,0.00042720471151369566
717718,1435437,1435436,2870873,1151.5468270778656,0.0004209898360159059
718719,1437439,1437438,2874877,1153.3593699932098,0.0004148654644495764
719720,1439441,1439440,2878881,1154.913264989853,0.00040883027611471334
720721,1441443,1441442,2882885,1157.3571968078613,0.00040288296941071167
721722,1443445,1443444,2886889,1158.8832530975342,0.00039702226217741554
722723,1445447,1445446,2890893,1160.3093769550323,0.00039124689124037104
723724,1447449,1447448,2894897,1161.7526700496674,0.00038555561150133144
724725,1449451,1449450,2898901,1163.190724849701,0.00037994719605194405
725726,1451453,1451452,2902905,1164.6314477920532,0.00037442043628743704
726727,1453455,1453454,2906909,1166.235605955124,0.0003689741411108116
727728,1455457,1455456,2910913,1168.1514067649841,0.00036360713659178145
728729,1457459,1457458,2914917,1169.950807094574,0.0003583182664215201
729730,1459461,1459460,2918921,1171.7484760284424,0.00035310639111685305
730731,1461463,1461462,2922925,1174.130187034607,0.0003479703874518236
731732,1463465,1463464,2926929,1176.795361995697,0.0003429091490261271
732733,1465467,1465466,2930933,1179.9477808475494,0.0003379215853556161
733734,1467469,1467468,2934937,1181.9571678638458,0.0003330066223270478
734735,1469471,1469470,2938941,1183.8940110206604,0.0003281632009475288
735736,1471473,1471472,2942945,1185.5775508880615,0.0003233902782540099
736737,1473475,1473474,2946949,1187.1736969947815,0.0003186868261764175
737738,1475477,1475476,2950953,1188.6410839557648,0.0003140518317650276
738739,1477479,1477478,2954957,1190.4225940704346,0.0003094842970767786
739740,1479481,1479480,2958961,1192.0803139209747,0.00030498323849315057
740741,1481483,1481482,2962965,1193.79185795784,0.0003005476864927914
741742,1483485,1483484,2966969,1195.4364948272705,0.00029617668667469843
742743,1485487,1485486,2970973,1197.1051001548767,0.0002918692977118553
743744,1487489,1487488,2974977,1198.6495769023895,0.0002876245923744136
744745,1489491,1489490,2978981,1200.085685968399,0.0002834416568475717
745746,1491493,1491492,2982985,1201.5461828708649,0.00027931959073157486
746747,1493495,1493494,2986989,1203.0169160366058,0.000275257507155402
747748,1495497,1495496,2990993,1204.6615591049194,0.0002712545316398973
748749,1497499,1497498,2994997,1207.5599009990692,0.0002673098025525178
749750,1499501,1499500,2999001,1209.9944639205933,0.00026342247110733297
750751,1501503,1501502,3003005,1211.637521982193,0.0002595917009102777
751752,1503505,1503504,3007009,1213.1824069023132,0.00025581666761809174
752753,1505507,1505506,3011013,1214.6191487312317,0.0002520965589383195
753754,1507509,1507508,3015017,1216.0929391384125,0.0002484305746293103
754755,1509511,1509510,3019021,1218.7580659389496,0.000244817925931784
755756,1511513,1511512,3023025,1220.4812240600586,0.00024125783556883107
756757,1513515,1513514,3027029,1222.384771823883,0.00023774953797328635
757758,1515517,1515516,3031033,1223.8714129924774,0.00023429227826454735
758759,1517519,1517518,3035037,1225.3699159622192,0.00023088531315806904
759760,1519521,1519520,3039041,1226.8446128368378,0.00022752790948743495
760761,1521523,1521522,3043045,1228.3347840309143,0.00022421934556859924
761762,1523525,1523524,3047049,1229.961847782135,0.00022095890994933143
762763,1525527,1525526,3051053,1232.1049118041992,0.0002177459009544691
763764,1527529,1527528,3055057,1233.5631098747253,0.0002145796281638468
764765,1529531,1529530,3059061,1235.0505318641663,0.0002114594108206802
765766,1531533,1531532,3063065,1236.5525550842285,0.00020838457783156628
766767,1533535,1533534,3067069,1237.9998090267181,0.00020535446810754365
767768,1535537,1535536,3071073,1239.4516711235046,0.0002023684305640927
768769,1537539,1537538,3075077,1240.9308009147644,0.00019942582298426714
769770,1539541,1539540,3079081,1242.371710062027,0.00019652601292818872
770771,1541543,1541542,3083085,1243.821130990982,0.00019366837693723937
771772,1543545,1543544,3087089,1245.3101079463959,0.00019085230121618224
772773,1545547,1545546,3091093,1246.849191904068,0.00018807718004154594
773774,1547549,1547548,3095097,1248.7584431171417,0.00018534241723955347
774775,1549551,1549550,3099101,1250.661152124405,0.00018264742516294064
775776,1551553,1551552,3103105,1253.6561510562897,0.00017999162457726925
776777,1553555,1553554,3107109,1255.8487408161163,0.00017737444454724027
777778,1555557,1555556,3111113,1257.867651939392,0.00017479532311881485
778779,1557559,1557558,3115117,1259.9674389362335,0.0001722537058412854
779780,1559561,1559560,3119121,1262.216343164444,0.00016974904690414405
780781,1561563,1561562,3123125,1263.7680430412292,0.000167280808113901
781782,1563565,1563564,3127129,1265.4487318992615,0.00016484845900777145
782783,1565567,1565566,3131133,1266.9740197658539,0.00016245147742210975
783784,1567569,1567568,3135137,1268.4492769241333,0.00016008934812816733
784785,1569571,1569570,3139141,1269.933261871338,0.00015776156374158745
785786,1571573,1571572,3143145,1271.7954769134521,0.00015546762472240516
786787,1573575,1573574,3147149,1273.4597570896149,0.00015320703766974475
787788,1575577,1575576,3151153,1275.460753917694,0.00015097931770924333
788789,1577579,1577578,3155157,1276.9854378700256,0.00014878398610562726
789790,1579581,1579580,3159161,1278.9876370429993,0.0001466205713995805
790791,1581583,1581582,3163165,1280.8545730113983,0.00014448860906668415
791792,1583585,1583584,3167169,1282.9901950359344,0.0001423876414037295
792793,1585587,1585586,3171173,1284.7167041301727,0.00014031721696028399
793794,1587589,1587588,3175177,1286.4948060512543,0.00013827689156187262
794795,1589591,1589590,3179181,1288.0851910114288,0.00013626622694573598
795796,1591593,1591592,3183185,1289.6382880210876,0.0001342847913292644
796797,1593595,1593594,3187189,1291.2355918884277,0.00013233215952368482
797798,1595597,1595596,3191193,1292.8392269611359,0.00013040791247931338
798799,1597599,1597598,3195197,1294.2799067497253,0.00012851163683080813
799800,1599601,1599600,3199201,1296.082939863205,0.00012664292546560318
800801,1601603,1601602,3203205,1297.8041207790375,0.0001248013774102219
801802,1603605,1603604,3207209,1299.490285873413,0.00012298659748921636
802803,1605607,1605606,3211213,1300.843894958496,0.00012119819587042002
803804,1607609,1607608,3215217,1302.1300508975983,0.0001194357889744424
804805,1609611,1609610,3219221,1303.41064286232,0.00011769899867886124
805806,1611613,1611612,3223225,1304.6834330558777,0.00011598745209084882
806807,1613615,1613614,3227229,1306.010528087616,0.00011430078166085877
807808,1615617,1615616,3231233,1307.2360100746155,0.00011263862586474715
808809,1617619,1617618,3235237,1308.5837798118591,0.00011100062783953035
809810,1619621,1619620,3239241,1310.2418110370636,0.0001093864359518193
810811,1621623,1621622,3243245,1311.7654631137848,0.00010779570413887996
811812,1623625,1623624,3247249,1313.4040100574493,0.0001062280911128255
812813,1625627,1625626,3251253,1314.8889181613922,0.00010468326024692942
813814,1627629,1627628,3255257,1316.6662259101868,0.00010316088025774661
814815,1629631,1629630,3259261,1318.5431439876556,0.0001016606245229923
815816,1631633,1631632,3263265,1320.3697528839111,0.00010018217130891571
816817,1633635,1633634,3267269,1321.9765288829803,9.872520320186595e-05
817818,1635637,1635636,3271273,1324.105045080185,9.728940790409979e-05
818819,1637639,1637638,3275277,1326.5505819320679,9.587447766534751e-05
819820,1639641,1639640,3279281,1328.4951119422913,9.448010848700505e-05
820821,1641643,1641642,3283285,1330.0965898036957,9.31060013726892e-05
821822,1643645,1643644,3287289,1331.6584918498993,9.175186187349027e-05
822823,1645647,1645646,3291293,1333.7076649665833,9.041739940585103e-05
823824,1647649,1647648,3295297,1335.306442975998,8.91023277063141e-05
824825,1649651,1649650,3299301,1336.9385941028595,8.78063647178351e-05
825826,1651653,1651652,3303305,1338.3825738430023,8.652923304452997e-05
826827,1653655,1653654,3307309,1339.825660943985,8.52706580189988e-05
827828,1655657,1655656,3311313,1341.2753601074219,8.403037043080985e-05
828829,1657659,1657658,3315317,1342.7804398536682,8.280810379801551e-05
829830,1659661,1659660,3319321,1344.2090899944305,8.160359641351533e-05
830831,1661663,1661662,3323325,1345.669333934784,8.041658975344035e-05
831832,1663665,1663664,3327329,1347.172306060791,7.924682950033457e-05
832833,1665667,1665666,3331333,1348.6322371959686,7.809406486103398e-05
833834,1667669,1667668,3335337,1350.060935974121,7.695804856666655e-05
834835,1669671,1669670,3339341,1351.5069661140442,7.583853732739954e-05
835836,1671673,1671672,3343345,1352.9432640075684,7.473529058188433e-05
836837,1673675,1673674,3347349,1354.3863549232483,7.364807242993265e-05
837838,1675677,1675676,3351353,1355.8538451194763,7.257664947246667e-05
838839,1677679,1677678,3355357,1357.34526014328,7.152079217576102e-05
839840,1679681,1679680,3359361,1358.9298470020294,7.048027418932179e-05
840841,1681683,1681682,3363365,1361.345006942749,6.945487234588654e-05
841842,1683685,1683684,3367369,1362.777794122696,6.844436734354531e-05
842843,1685687,1685686,3371373,1364.1905720233917,6.744854181306437e-05
843844,1687689,1687688,3375377,1365.6363110542297,6.64671829326835e-05
844845,1689691,1689690,3379381,1367.0761020183563,6.550008015437925e-05
845846,1691693,1691692,3383385,1368.5285849571228,6.454702611335961e-05
846847,1693695,1693694,3387389,1369.9638719558716,6.36078168554377e-05
847848,1695697,1695696,3391393,1371.4037969112396,6.268225115491077e-05
848849,1697699,1697698,3395397,1372.8603358268738,6.177013017349964e-05
849850,1699701,1699700,3399401,1374.265380859375,6.087125882459077e-05
850851,1701703,1701702,3403405,1375.707107782364,5.9985444408994226e-05
851852,1703705,1703704,3407409,1377.1429278850555,5.911249706969102e-05
852853,1705707,1705706,3411413,1378.6206600666046,5.8252229905519926e-05
853854,1707709,1707708,3415417,1380.7583701610565,5.740445840274333e-05
854855,1709711,1709710,3419421,1382.2608878612518,5.656900100348139e-05
855856,1711713,1711712,3423425,1384.1217198371887,5.574567887833837e-05
856857,1713715,1713714,3427429,1385.5966160297394,5.493431558534212e-05
857858,1715717,1715716,3431433,1387.1120147705078,5.413473695625726e-05
858859,1717719,1717718,3435437,1388.578127861023,5.334677177870617e-05
859860,1719721,1719720,3439441,1389.986188173294,5.257025179616903e-05
860861,1721723,1721722,3443445,1391.3913369178772,5.180500988899439e-05
861862,1723725,1723724,3447449,1392.827898979187,5.105088268919644e-05
862863,1725727,1725726,3451453,1394.2103779315948,5.0307708534091944e-05
863864,1727729,1727728,3455457,1395.6028280258179,4.957532814842125e-05
864865,1729731,1729730,3459461,1397.0287408828735,4.885358441697463e-05
865866,1731733,1731732,3463465,1398.4267678260803,4.8142323294086964e-05
866867,1733735,1733734,3467469,1399.8315689563751,4.744139198464836e-05
867868,1735737,1735736,3471473,1401.216532945633,4.675064030834619e-05
868869,1737739,1737738,3475477,1402.6124629974365,4.6069920927038766e-05
869870,1739741,1739740,3479481,1404.0305919647217,4.539908763945277e-05
870871,1741743,1741742,3483485,1405.465735912323,4.473799651805166e-05
871872,1743745,1743744,3487489,1406.8583891391754,4.4086506363782973e-05
872873,1745747,1745746,3491493,1408.7082979679108,4.3444477455523156e-05
873874,1747749,1747748,3495497,1410.3694729804993,4.281177245957224e-05
874875,1749751,1749750,3499501,1412.0073580741882,4.218825574753282e-05
875876,1751753,1751752,3503505,1414.3403890132904,4.157379385105742e-05
876877,1753755,1753754,3507509,1415.8155500888824,4.096825523447478e-05
877878,1755757,1755756,3511513,1417.347289800644,4.0371510181103076e-05
878879,1757759,1757758,3515517,1418.9426469802856,3.978343102062354e-05
879880,1759761,1759760,3519521,1420.4990510940552,3.9203891674333136e-05
880881,1761763,1761762,3523525,1422.0538659095764,3.863276788251824e-05
881882,1763765,1763764,3527529,1423.5880270004272,3.806993765920197e-05
882883,1765767,1765766,3531533,1425.1315319538116,3.751528072371002e-05
883884,1767769,1767768,3535537,1426.594822883606,3.6968677704862785e-05
884885,1769771,1769770,3539541,1428.0607380867004,3.6430012073651596e-05
885886,1771773,1771772,3543545,1429.6865649223328,3.589916843793617e-05
886887,1773775,1773774,3547549,1431.139524936676,3.537603265613143e-05
887888,1775777,1775776,3551553,1433.4550170898438,3.4860493542510085e-05
888889,1777779,1777778,3555557,1435.6456699371338,3.435244013871852e-05
889890,1779781,1779780,3559561,1437.1976449489594,3.385176387382671e-05
890891,1781783,1781782,3563565,1438.6784269809723,3.335835742745985e-05
891892,1783785,1783784,3567569,1440.1013638973236,3.287211529823253e-05
892893,1785787,1785786,3571573,1441.5928950309753,3.2392933462688234e-05
893894,1787789,1787788,3575577,1443.1632578372955,3.192070937529934e-05
894895,1789791,1789790,3579581,1444.5966439247131,3.1455341741093434e-05
895896,1791793,1791792,3583585,1446.1437258720398,3.0996730970400677e-05
896897,1793795,1793794,3587589,1447.5688889026642,3.0544779292540625e-05
897898,1795797,1795796,3591593,1448.9882318973541,3.009938927789335e-05
898899,1797799,1797798,3595597,1450.5030081272125,2.966046645269671e-05
899900,1799801,1799800,3599601,1452.0898530483246,2.9227916229501716e-05
900901,1801803,1801802,3603605,1453.5944588184357,2.88016461809093e-05
901902,1803805,1803804,3607609,1455.035588979721,2.8381565130075614e-05
902903,1805807,1805806,3611613,1456.5041527748108,2.7967583150712017e-05
903904,1807809,1807808,3615617,1457.9271039962769,2.7559611567085085e-05
904905,1809811,1809810,3619621,1459.3696138858795,2.7157563295077125e-05
905906,1811813,1811812,3623625,1460.8158888816833,2.6761352160065144e-05
906907,1813815,1813814,3627629,1462.2652847766876,2.637089346535504e-05
907908,1815817,1815816,3631633,1463.711175918579,2.598610331006057e-05
908909,1817819,1817818,3635637,1465.1557960510254,2.5606899725971743e-05
909910,1819821,1819820,3639641,1466.5611209869385,2.5233201313312748e-05
910911,1821823,1821822,3643645,1468.0094101428986,2.486492837761034e-05
911912,1823825,1823824,3647649,1469.4035799503326,2.450200213388598e-05
912913,1825827,1825826,3651653,1470.8023040294647,2.4144344479282154e-05
913914,1827829,1827828,3655657,1472.1884939670563,2.379187901624391e-05
914915,1829831,1829830,3659661,1473.6023218631744,2.3444530825145193e-05
915916,1831833,1831832,3663665,1475.0183029174805,2.310222510004678e-05
916917,1833835,1833834,3667669,1476.4033198356628,2.2764888853998855e-05
917918,1835837,1835836,3671673,1477.8114278316498,2.2432449668485788e-05
918919,1837839,1837838,3675677,1479.2414989471436,2.210483660292084e-05
919920,1839841,1839840,3679681,1480.6794929504395,2.178197951252514e-05
920921,1841843,1841842,3683685,1482.0884218215942,2.1463809162014513e-05
921922,1843845,1843844,3687689,1483.5384199619293,2.1150257794033678e-05
922923,1845847,1845846,3691693,1484.95734500885,2.084125821966154e-05
923924,1847849,1847848,3695697,1486.3815550804138,2.053674415947171e-05
924925,1849851,1849850,3699701,1488.2281138896942,2.0236650357219332e-05
925926,1851853,1851852,3703705,1489.690724849701,1.994091337564896e-05
926927,1853855,1853854,3707709,1491.090471982956,1.9649468981697282e-05
927928,1855857,1855856,3711713,1492.3949179649353,1.936225555709825e-05
928929,1857859,1857858,3715717,1493.6897749900818,1.9079211256212147e-05
929930,1859861,1859860,3719721,1495.0089528560638,1.8800275597641303e-05
930931,1861863,1861862,3723725,1496.8992431163788,1.852538900948275e-05
931932,1863865,1863864,3727729,1498.9405510425568,1.8254492601954553e-05
932933,1865867,1865866,3731733,1500.9283239841461,1.798752839476947e-05
933934,1867869,1867868,3735737,1502.78240275383,1.772443954450864e-05
934935,1869871,1869870,3739741,1505.236014842987,1.746516943512688e-05
935936,1871873,1871872,3743745,1509.102061033249,1.720966281482106e-05
936937,1873875,1873874,3747749,1511.9758749008179,1.6957865113909065e-05
937938,1875877,1875876,3751753,1514.3516409397125,1.6709722217456147e-05
938939,1877879,1877878,3755757,1516.035474061966,1.6465181261082762e-05
939940,1879881,1879880,3759761,1517.5780098438263,1.6224189721469884e-05
940941,1881883,1881882,3763765,1519.1111340522766,1.5986696212166862e-05
941942,1883885,1883884,3767769,1521.0358669757843,1.5752650028844073e-05
942943,1885887,1885886,3771773,1522.976313829422,1.552200103560608e-05
943944,1887889,1887888,3775777,1524.777498960495,1.5294699778678478e-05
944945,1889891,1889890,3779781,1526.5182268619537,1.5070697713781556e-05
945946,1891893,1891892,3783785,1528.284462928772,1.4849947092443472e-05
946947,1893895,1893894,3787789,1529.9761190414429,1.4632400393566058e-05
947948,1895897,1895896,3791793,1531.7075290679932,1.4418011346606363e-05
948949,1897899,1897898,3795797,1533.5085229873657,1.4206734249455621e-05
949950,1899901,1899900,3799801,1535.9629938602448,1.3998523513691907e-05
950951,1901903,1901902,3803805,1537.7166409492493,1.3793334801448509e-05
951952,1903905,1903904,3807809,1539.5263550281525,1.3591124343292904e-05
952953,1905907,1905906,3811813,1541.2057979106903,1.3391848597166245e-05
953954,1907909,1907908,3815817,1542.9289529323578,1.3195465157878061e-05
954955,1909911,1909910,3819821,1544.4528048038483,1.3001932188672072e-05
955956,1911913,1911912,3823825,1546.0394780635834,1.281120808016567e-05
956957,1913915,1913914,3827829,1547.5620911121368,1.2623252018784115e-05
957958,1915917,1915916,3831833,1549.1743078231812,1.2438023986760527e-05
958959,1917919,1917918,3835837,1550.9116070270538,1.2255484307388542e-05
959960,1919921,1919920,3839841,1552.3922340869904,1.2075593872395984e-05
960961,1921923,1921922,3843845,1554.1627299785614,1.1898314369318541e-05
961962,1923925,1923924,3847849,1556.019613981247,1.1723607713065576e-05
962963,1925927,1925926,3851853,1557.9082930088043,1.1551436728041153e-05
963964,1927929,1927928,3855857,1559.764002084732,1.1381764352336177e-05
964965,1929931,1929930,3859861,1561.4870820045471,1.1214554547223088e-05
965966,1931933,1931932,3863865,1563.1352100372314,1.1049771501348005e-05
966967,1933935,1933934,3867869,1564.7423770427704,1.0887379858104396e-05
967968,1935937,1935936,3871873,1566.3812589645386,1.0727345170380431e-05
968969,1937939,1937938,3875877,1568.0906569957733,1.0569632991064282e-05
969970,1939941,1939940,3879881,1569.6975438594818,1.0414209555165144e-05
970971,1941943,1941942,3883885,1571.3745849132538,1.0261041893500078e-05
971972,1943945,1943944,3887889,1573.0231239795685,1.011009726425982e-05
972973,1945947,1945946,3891893,1574.5717010498047,9.961342925635108e-06
973974,1947949,1947948,3895897,1576.1535251140594,9.814747613745567e-06
974975,1949951,1949950,3899901,1577.8078479766846,9.670279609963472e-06
975976,1951953,1951952,3903905,1579.4008059501648,9.527908332529478e-06
976977,1953955,1953954,3907909,1580.9208879470825,9.387603085997398e-06
977978,1955957,1955956,3911913,1582.6012680530548,9.24933408441575e-06
978979,1957959,1957958,3915917,1584.1288588047028,9.113071541833051e-06
979980,1959961,1959960,3919921,1585.6806101799011,8.978786695479357e-06
980981,1961963,1961962,3923925,1587.19633102417,8.846450441524212e-06
981982,1963965,1963964,3927929,1588.6943061351776,8.71603458563186e-06
982983,1965967,1965966,3931933,1590.2179729938507,8.587511388213898e-06
983984,1967969,1967968,3935937,1591.8512148857117,8.460853450742434e-06
984985,1969971,1969970,3939941,1593.7313389778137,8.336033488376415e-06
985986,1971973,1971972,3943945,1595.4004549980164,8.213024898395815e-06
986987,1973975,1973974,3947949,1597.0232520103455,8.091801305454283e-06
987988,1975977,1975976,3951953,1598.54838681221,7.972337016326492e-06
988989,1977979,1977978,3955957,1600.2609839439392,7.85460622410028e-06
989990,1979981,1979980,3959961,1601.7771809101105,7.738584031358187e-06
990991,1981983,1981982,3963965,1603.2682361602783,7.624245313309075e-06
991992,1983985,1983984,3967969,1604.7794539928436,7.51156585465651e-06
992993,1985987,1985986,3971973,1606.2584137916565,7.400521667477733e-06
993994,1987989,1987988,3975977,1607.764769077301,7.291088763849984e-06
994995,1989991,1989990,3979981,1609.2649910449982,7.183243951658369e-06
995996,1991993,1991992,3983985,1610.845862865448,7.076964038787992e-06
996997,1993995,1993994,3987989,1612.3757519721985,6.972226401558146e-06
997998,1995997,1995996,3991993,1613.9875819683075,6.8690086436618e-06
998999,1997999,1997998,3995997,1615.5079889297485,6.767288482478762e-06
1000000,2000001,2000000,4000001,1617.0725541114807,6.667044658570376e-06


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/fista.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0005440711975097656,2181.4194943796983
6,13,6,19,0.007731914520263672,475.341262047961
11,23,11,34,0.010568857192993164,269.2215147773172
17,35,17,52,0.01370382308959961,172.6347767136524
23,47,23,70,0.016872882843017578,128.11197162982648
28,57,28,85,0.020776987075805664,106.89745497453373
34,69,34,103,0.024498939514160156,90.89703659674024
40,81,40,121,0.02764582633972168,80.92403487595084
45,91,45,136,0.03040170669555664,75.4055646350912
51,103,51,154,0.03370189666748047,70.59612599936463
57,115,57,172,0.03753185272216797,66.93782025427026
62,125,62,187,0.041838884353637695,64.47695869392714
68,137,68,205,0.04690384864807129,61.961100934910974
74,149,74,223,0.0506739616394043,59.79211566003187
79,159,79,238,0.05553102493286133,58.27456052332968
85,171,85,256,0.06010603904724121,56.817651051392886
91,183,91,274,0.06392383575439453,55.698538093732395
96,193,96,289,0.06809878349304199,54.97578033758964
102,205,102,307,0.07251882553100586,54.3028992537229
108,217,108,325,0.07663893699645996,53.771986065378314
113,227,113,340,0.08077287673950195,53.38235354402559
119,239,119,358,0.08438587188720703,52.91742223202027
125,251,125,376,0.08962273597717285,52.420336897666175
130,261,130,391,0.09491896629333496,51.976409549316486
136,273,136,409,0.10164189338684082,51.4138911828868
142,285,142,427,0.10776972770690918,50.82463187679514
147,295,147,442,0.11311078071594238,50.313647586099705
153,307,153,460,0.11950087547302246,49.67584367919994
159,319,159,478,0.12598586082458496,49.013822643435105
164,329,164,493,0.13228487968444824,48.448419797262886
170,341,170,511,0.13894081115722656,47.76069773511426
176,353,176,529,0.1454300880432129,47.071279177080896
181,363,181,544,0.15088987350463867,46.501659813889546
187,375,187,562,0.15744686126708984,45.82923394258728
193,387,193,580,0.16385388374328613,45.17017766097433
198,397,198,595,0.1692488193511963,44.62920787606731
204,409,204,613,0.17518281936645508,43.986387521197
210,421,210,631,0.18125486373901367,43.34752713411194
215,431,215,646,0.18689370155334473,42.81677530070351
221,443,221,664,0.1933457851409912,42.18067175063857
227,455,227,682,0.19996285438537598,41.544299002584694
232,465,232,697,0.2057507038116455,41.01296983235011
238,477,238,715,0.21248984336853027,40.373331254076675
244,489,244,733,0.21991872787475586,39.73091391887783
249,499,249,748,0.22577166557312012,39.19349236949347
255,511,255,766,0.2325887680053711,38.54700590607035
261,523,261,784,0.24370789527893066,37.90074619447046
266,533,266,799,0.250180721282959,37.364304631269306
272,545,272,817,0.2567780017852783,36.72540542416391
278,557,278,835,0.263136625289917,36.09364836150303
283,567,283,850,0.26839494705200195,35.573402046420824
289,579,289,868,0.2745048999786377,34.9567192049567
295,591,295,886,0.27955198287963867,34.347982827107444
300,601,300,901,0.28418469429016113,33.84638733393899
306,613,306,919,0.2910647392272949,33.25098235494329
312,625,312,937,0.2984657287597656,32.66263774734762
317,635,317,952,0.3040149211883545,32.17784895510931
323,647,323,970,0.31056785583496094,31.60276804819955
329,659,329,988,0.3167150020599365,31.03477969934579
334,669,334,1003,0.32224488258361816,30.566562423337018
340,681,340,1021,0.3292880058288574,30.01039981665076
346,693,346,1039,0.3351738452911377,29.46014041681792
351,703,351,1054,0.34009289741516113,29.00606429400159
357,715,357,1072,0.34528493881225586,28.466746744174543
363,727,363,1090,0.35013365745544434,27.933892811922988
368,737,368,1105,0.3542928695678711,27.49507989429958
374,749,374,1123,0.3592708110809326,26.975013326032013
380,761,380,1141,0.3634927272796631,26.462100865233197
385,771,385,1156,0.3676338195800781,26.040056772065782
391,783,391,1174,0.372891902923584,25.539889789674362
397,795,397,1192,0.3770596981048584,25.046390408381512
402,805,402,1207,0.38036298751831055,24.640110517797666
408,817,408,1225,0.3843200206756592,24.15839965899181
414,829,414,1243,0.3895597457885742,23.682868847367445
419,839,419,1258,0.39310169219970703,23.291151371228807
425,851,425,1276,0.3969838619232178,22.826339244835253
431,863,431,1294,0.4013667106628418,22.36701887484537
436,873,436,1309,0.40535569190979004,21.988300915081936
442,885,442,1327,0.408998966217041,21.538585978154288
448,897,448,1345,0.41275787353515625,21.093995066514026
453,907,453,1360,0.41579484939575195,20.72741019113687
459,919,459,1378,0.42005467414855957,20.292208956889226
465,931,465,1396,0.4249238967895508,19.86215245143694
470,941,470,1411,0.4287757873535156,19.507716659674543
476,953,476,1429,0.43329477310180664,19.087157602947855
481,963,481,1444,0.4374568462371826,18.740689152243704
487,975,487,1462,0.4411137104034424,18.329768891379672
493,987,493,1480,0.44492173194885254,17.924171738842688
498,997,498,1495,0.4485907554626465,17.590249950868838
504,1009,504,1513,0.4525127410888672,17.1944061482086
510,1021,510,1531,0.45656490325927734,16.80379327116043
515,1031,515,1546,0.45957088470458984,16.482204696050303
521,1043,521,1564,0.46330976486206055,16.100918961261186
527,1055,527,1582,0.46698975563049316,15.724605862734165
532,1065,532,1597,0.4704866409301758,15.414783296224186
538,1077,538,1615,0.47431492805480957,15.047514537390043
544,1089,544,1633,0.4781978130340576,14.68517580920934
549,1099,549,1648,0.48145580291748047,14.386988987590826
555,1111,555,1666,0.48535776138305664,14.033663733000708
561,1123,561,1684,0.48972177505493164,13.685224530902701
566,1133,566,1699,0.49289870262145996,13.398581526181943
572,1145,572,1717,0.49721503257751465,13.059088023725508
578,1157,578,1735,0.5022919178009033,12.724519621129161
583,1167,583,1750,0.5061948299407959,12.44952057377327
589,1179,589,1768,0.510887861251831,12.124150586568817
595,1191,595,1786,0.5147106647491455,11.80388221502335
600,1201,600,1801,0.517838716506958,11.540910947418297
606,1213,606,1819,0.5228378772735596,11.230049713581252
612,1225,612,1837,0.5278947353363037,10.924298972420047
617,1235,617,1852,0.5320818424224854,10.67338263016677
623,1247,623,1870,0.537545919418335,10.376892522634193
629,1259,629,1888,0.5428659915924072,10.085381824844944
634,1269,634,1903,0.5468659400939941,9.846222424750636
640,1281,640,1921,0.5514466762542725,9.563709244205029
646,1293,646,1939,0.5564818382263184,9.286045545250659
651,1303,651,1954,0.5604188442230225,9.058346946772986
657,1315,657,1972,0.5653576850891113,8.78953022904443
663,1327,663,1990,0.5694777965545654,8.525549732458103
668,1337,668,2005,0.5727348327636719,8.309278538963213
674,1349,674,2023,0.5764029026031494,8.054233742906149
680,1361,680,2041,0.5802018642425537,7.804101062697555
685,1371,685,2056,0.5833728313446045,7.599421422482351
691,1383,691,2074,0.5872838497161865,7.3583273740800905
697,1395,697,2092,0.5912008285522461,7.122160295334993
702,1405,702,2107,0.5953218936920166,6.929106981734662
708,1417,708,2125,0.6001129150390625,6.701924687167548
714,1429,714,2143,0.6053357124328613,6.479598803353042
719,1439,719,2158,0.6090118885040283,6.2980049166205845
725,1451,725,2176,0.6128168106079102,6.084458962200529
731,1463,731,2194,0.616506814956665,5.875620319128075
736,1473,736,2209,0.6205887794494629,5.705140189091139
742,1485,742,2227,0.6245718002319336,5.504777573497904
748,1497,748,2245,0.6281819343566895,5.308965880839878
753,1507,753,2260,0.6312687397003174,5.149237685339131
759,1519,759,2278,0.6352968215942383,4.9616754885820455
765,1531,765,2296,0.63997483253479,4.7785757988169735
770,1541,770,2311,0.6443099975585938,4.629385879071378
776,1553,776,2329,0.6494338512420654,4.4544102802829
782,1565,782,2347,0.6545238494873047,4.283830655161751
787,1575,787,2362,0.6580088138580322,4.145016092211449
793,1587,793,2380,0.6627316474914551,3.982407066873975
799,1599,799,2398,0.6679549217224121,3.82408343004613
804,1609,804,2413,0.6722538471221924,3.69538260176364
810,1621,810,2431,0.6765038967132568,3.544774672094036
816,1633,816,2449,0.6801390647888184,3.398292497876014
821,1643,821,2464,0.6835830211639404,3.2793335991316326
827,1655,827,2482,0.6877167224884033,3.140266180550725
833,1667,833,2500,0.6926147937774658,3.0051670831868478
838,1677,838,2515,0.6967990398406982,2.8955793576420774
844,1689,844,2533,0.7015879154205322,2.7676247078436518
850,1701,850,2551,0.7056987285614014,2.6434954373243045
855,1711,855,2566,0.7097606658935547,2.542938441501633
861,1723,861,2584,0.7140789031982422,2.4256830560151457
867,1735,867,2602,0.7193608283996582,2.312096565554384
872,1745,872,2617,0.7246789932250977,2.2202010318935663
878,1757,878,2635,0.7303988933563232,2.1131860523051955
884,1769,884,2653,0.7353019714355469,2.0096699361462242
889,1779,889,2668,0.7407538890838623,1.9260359985871673
895,1791,895,2686,0.745589017868042,1.828779811967138
901,1803,901,2704,0.750450849533081,1.7348563830371404
906,1813,906,2719,0.7539608478546143,1.6590924118647763
912,1825,912,2737,0.7584378719329834,1.5711345173907603
918,1837,918,2755,0.7628350257873535,1.4863518506724631
923,1847,923,2770,0.7659709453582764,1.418083716848514
929,1859,929,2788,0.7710559368133545,1.3389707350016806
935,1871,935,2806,0.7760787010192871,1.2628619244673018
940,1881,940,2821,0.77927565574646,1.2016848340036859
946,1893,946,2839,0.7830069065093994,1.1309090599932006
952,1905,952,2857,0.7879040241241455,1.0629436315472276
957,1915,957,2872,0.7912540435791016,1.0084022270319792
963,1927,963,2890,0.7949337959289551,0.9454093353905364
969,1939,969,2908,0.7986979484558105,0.8850352092281355
974,1949,974,2923,0.8019378185272217,0.8366798778869224
980,1961,980,2941,0.805635929107666,0.7809524359079205
986,1973,986,2959,0.8091819286346436,0.7276838573562827
991,1983,991,2974,0.8120729923248291,0.6851364191112452
997,1995,997,2992,0.8156406879425049,0.6362501446617443
1003,2007,1003,3010,0.820462703704834,0.5896866142137469
1008,2017,1008,3025,0.8248238563537598,0.5526218643780112
1014,2029,1014,3043,0.8293278217315674,0.5101837473280284
1020,2041,1020,3061,0.8346817493438721,0.4699168103146576
1025,2051,1025,3076,0.838864803314209,0.437976414298646
1031,2063,1031,3094,0.8427069187164307,0.4015330653944602
1037,2075,1037,3112,0.8479747772216797,0.36708770415407344
1042,2085,1042,3127,0.852092981338501,0.3398654149243612
1048,2097,1048,3145,0.8568768501281738,0.30892596724277155
1054,2109,1054,3163,0.8619101047515869,0.2798168999183872
1059,2119,1059,3178,0.8658719062805176,0.2569176800502646
1065,2131,1065,3196,0.8709368705749512,0.23102189993198863
1071,2143,1071,3214,0.8762288093566895,0.20680280875762946
1076,2153,1076,3229,0.8799617290496826,0.18786230104217339
1082,2165,1082,3247,0.8836917877197266,0.16657733202760028
1088,2177,1088,3265,0.8886868953704834,0.14681613265611304
1093,2187,1093,3280,0.8918569087982178,0.1314740567128183
1099,2199,1099,3298,0.896636962890625,0.11437005606308048
1105,2211,1105,3316,0.9017088413238525,0.09864617512778295
1110,2221,1110,3331,0.9053938388824463,0.08656536141086235
1116,2233,1116,3349,0.9103586673736572,0.0732602155587756
1122,2245,1122,3367,0.9152719974517822,0.061219436036935804
1127,2255,1127,3382,0.9188597202301025,0.052124674606034205
1133,2267,1133,3400,0.9233818054199219,0.042305593202740965
1139,2279,1139,3418,0.9285078048706055,0.03364339379618286
1144,2289,1144,3433,0.9318568706512451,0.027278246529590433
1150,2301,1150,3451,0.9368588924407959,0.02062519452726974
1156,2313,1156,3469,0.9417927265167236,0.015002335992335247
1161,2323,1161,3484,0.9484298229217529,0.011068859713645907
1167,2335,1167,3502,0.9561569690704346,0.007209945105614679
1173,2347,1173,3520,0.9596529006958008,0.004246828049531359
1178,2357,1178,3535,0.9640567302703857,0.0024300832934613936
1184,2369,1184,3553,0.9676029682159424,0.000997285498669953
1190,2381,1190,3571,0.9719419479370117,0.00034322595229241415
1195,2391,1195,3586,0.9748988151550293,0.00036662368302131654
1201,2403,1201,3604,0.9784839153289795,0.0010463694802638202
1207,2415,1207,3622,0.9830238819122314,0.0024045645272963156
1212,2425,1212,3637,0.9866230487823486,0.004030210173709747
1218,2437,1218,3655,0.990257978439331,0.006544712336221892
1224,2449,1224,3673,0.9936697483062744,0.009643552251873189
1229,2459,1229,3688,0.9964509010314941,0.012649790377508907
1235,2471,1235,3706,0.9998879432678223,0.016740331918413176
1241,2483,1241,3724,1.0043740272521973,0.02133148617497227
1246,2493,1246,3739,1.0078368186950684,0.02552064030578549
1252,2505,1252,3757,1.0128929615020752,0.0309610062114416
1258,2517,1258,3775,1.0167179107666016,0.036827797099704185
1263,2527,1263,3790,1.0210368633270264,0.04202331250712632
1269,2539,1269,3808,1.0255277156829834,0.04860178540855031
1275,2551,1275,3826,1.029686689376831,0.05552824007338586
1280,2561,1280,3841,1.032829999923706,0.061544928005218935
1286,2573,1286,3859,1.03653883934021,0.06903309992958384
1292,2585,1292,3877,1.040024757385254,0.07678674774444971
1297,2595,1297,3892,1.042815923690796,0.08343117715241988
1303,2607,1303,3910,1.0464558601379395,0.0916019416878271
1309,2619,1309,3928,1.0507347583770752,0.09996551352878669
1314,2629,1314,3943,1.0538609027862549,0.1070662321525333
1320,2641,1320,3961,1.0583808422088623,0.11572593531707298
1326,2653,1326,3979,1.0628418922424316,0.12451772208135026
1331,2663,1331,3994,1.0661499500274658,0.13193071234468334
1337,2675,1337,4012,1.070112705230713,0.14091334880879458
1343,2687,1343,4030,1.0748538970947266,0.14997342698188731
1348,2697,1348,4045,1.0786628723144531,0.15756999850066222
1354,2709,1354,4063,1.0823979377746582,0.166727590408982
1360,2721,1360,4081,1.0862059593200684,0.175916464622901
1365,2731,1365,4096,1.089829921722412,0.18358758291890354
1371,2743,1371,4114,1.0945789813995361,0.1927976747450657
1377,2755,1377,4132,1.0988380908966064,0.2020002188048693
1382,2765,1382,4147,1.102529764175415,0.20965327004364553
1388,2777,1388,4165,1.1065196990966797,0.21880558841314723
1394,2789,1394,4183,1.1118638515472412,0.22790960893405554
1399,2799,1399,4198,1.116379976272583,0.23544842610749583
1405,2811,1405,4216,1.1211740970611572,0.24442449664365995
1411,2823,1411,4234,1.130378007888794,0.253309911456995
1416,2833,1416,4249,1.134917974472046,0.2606353044284333
1422,2845,1422,4267,1.1392309665679932,0.26931994930134806
1427,2855,1427,4282,1.1433937549591064,0.2764611726322528
1433,2867,1433,4300,1.1484129428863525,0.284906390634319
1439,2879,1439,4318,1.1524627208709717,0.29320696937236335
1444,2889,1444,4333,1.1555976867675781,0.3000071325926683
1450,2901,1450,4351,1.1593496799468994,0.30801958085987735
1456,2913,1456,4369,1.1639199256896973,0.3158632185133001
1461,2923,1461,4384,1.1678197383880615,0.3222651017172211
1467,2935,1467,4402,1.1722118854522705,0.32977977424116034
1473,2947,1473,4420,1.175710916519165,0.3371053673233746
1478,2957,1478,4435,1.1786696910858154,0.3430611987856764
1484,2969,1484,4453,1.1821858882904053,0.35002476714009845
1490,2981,1490,4471,1.1859078407287598,0.3567833283063919
1495,2991,1495,4486,1.189194917678833,0.3622552924636011
1501,3003,1501,4504,1.194443702697754,0.36862528292465413
1507,3015,1507,4522,1.199828863143921,0.37477657701163025
1512,3025,1512,4537,1.2041599750518799,0.37973222035998333
1518,3037,1518,4555,1.2082078456878662,0.38547053065099135
1524,3049,1524,4573,1.2122178077697754,0.3909773454995502
1529,3059,1529,4588,1.2150869369506836,0.39538662589552587
1535,3071,1535,4606,1.2187058925628662,0.4004589457858856
1541,3083,1541,4624,1.2222228050231934,0.4052895161538572
1546,3093,1546,4639,1.225172996520996,0.40912826097542165
1552,3105,1552,4657,1.229360818862915,0.4135084936272051
1558,3117,1558,4675,1.234252691268921,0.41763979133304474
1563,3127,1563,4690,1.2372608184814453,0.42089097512723583
1569,3139,1569,4708,1.2418959140777588,0.4245611218764225
1575,3151,1575,4726,1.246783971786499,0.427977836910145
1580,3161,1580,4741,1.2509467601776123,0.4306309819875196
1586,3173,1586,4759,1.254300832748413,0.43358166098403217
1592,3185,1592,4777,1.259023904800415,0.4362784002086073
1597,3195,1597,4792,1.2627599239349365,0.43833229304198085
1603,3207,1603,4810,1.2671058177947998,0.4405659122724046
1609,3219,1609,4828,1.271101951599121,0.4425487737360072
1614,3229,1614,4843,1.2742557525634766,0.4440106479522683
1620,3241,1620,4861,1.277923822402954,0.44553751675391595
1626,3253,1626,4879,1.2817208766937256,0.44681762898062516
1631,3263,1631,4894,1.284836769104004,0.44769686224333327
1637,3275,1637,4912,1.289078712463379,0.4485280938940832
1643,3287,1643,4930,1.2945926189422607,0.44911651120139595
1648,3297,1648,4945,1.2990920543670654,0.44942254139846227
1654,3309,1654,4963,1.303602933883667,0.4495701660190434
1660,3321,1660,4981,1.3074288368225098,0.4494801325458866
1665,3331,1665,4996,1.3105196952819824,0.44922518278497137
1671,3343,1671,5014,1.3141648769378662,0.448705490384782
1677,3355,1677,5032,1.317884922027588,0.4479552075176798
1682,3365,1682,5047,1.320863962173462,0.4471560073557157
1688,3377,1688,5065,1.3258037567138672,0.44599110310844026
1694,3389,1694,5083,1.330934762954712,0.44460509263490167
1699,3399,1699,5098,1.3339908123016357,0.44328405832141016
1705,3411,1705,5116,1.3381667137145996,0.44150327190197913
1711,3423,1711,5134,1.3416857719421387,0.43951335852079865
1716,3433,1716,5149,1.3455078601837158,0.43769860819418227
1722,3445,1722,5167,1.3500618934631348,0.43533701652950185
1728,3457,1728,5185,1.3548898696899414,0.4327789755636786
1733,3467,1733,5200,1.3583228588104248,0.43050030024551234
1739,3479,1739,5218,1.3625867366790771,0.42759313923886566
1745,3491,1745,5236,1.367527961730957,0.42450143365022086
1750,3501,1750,5251,1.3705778121948242,0.4217870603794154
1756,3513,1756,5269,1.374189853668213,0.41836800829855747
1762,3525,1762,5287,1.3775157928466797,0.4147767079901996
1767,3535,1767,5302,1.3811709880828857,0.411655794559465
1773,3547,1773,5320,1.3856678009033203,0.40776119196539184
1779,3559,1779,5338,1.3905177116394043,0.403708345338714
1784,3569,1784,5353,1.3940708637237549,0.4002138953311487
1790,3581,1790,5371,1.3988637924194336,0.3958847067347051
1796,3593,1796,5389,1.4027929306030273,0.39141244534062025
1801,3603,1801,5404,1.4063596725463867,0.3875802176938805
1807,3615,1807,5422,1.410017728805542,0.3828599107185937
1813,3627,1813,5440,1.4138257503509521,0.37801216824107087
1818,3637,1818,5455,1.4170408248901367,0.37387907836045997
1824,3649,1824,5473,1.4223120212554932,0.3688122727917289
1830,3661,1830,5491,1.4264919757843018,0.3636339317737338
1835,3671,1835,5506,1.429844856262207,0.35923746110870525
1841,3683,1841,5524,1.4338576793670654,0.35386902264269793
1847,3695,1847,5542,1.4393069744110107,0.34840458228052285
1852,3705,1852,5557,1.4445037841796875,0.34378138475119613
1858,3717,1858,5575,1.4492697715759277,0.33815471246794004
1864,3729,1864,5593,1.4534318447113037,0.33244700867328447
1869,3739,1869,5608,1.456618070602417,0.32763251302651497
1875,3751,1875,5626,1.4603238105773926,0.32179007652450764
1881,3763,1881,5644,1.4643938541412354,0.3158818374429302
1886,3773,1886,5659,1.4684388637542725,0.31091202788252303
1892,3785,1892,5677,1.4735949039459229,0.30489755668941143
1898,3797,1898,5695,1.4774746894836426,0.29883306833664847
1903,3807,1903,5710,1.4811408519744873,0.2937451574141505
1909,3819,1909,5728,1.4852197170257568,0.28760348180105666
1915,3831,1915,5746,1.488846778869629,0.2814275665000423
1920,3841,1920,5761,1.49208402633667,0.27625879503625583
1926,3853,1926,5779,1.4967317581176758,0.2700344211857555
1932,3865,1932,5797,1.5021939277648926,0.26379139633309023
1937,3875,1937,5812,1.5060639381408691,0.258578572209899
1943,3887,1943,5830,1.5096838474273682,0.2523155106827062
1949,3899,1949,5848,1.5132768154144287,0.24604911612368596
1954,3909,1954,5863,1.5161778926849365,0.24082833478371413
1960,3921,1960,5881,1.519709825515747,0.23456922592708906
1966,3933,1966,5899,1.523310899734497,0.2283210718818509
1971,3943,1971,5914,1.5261309146881104,0.22312602967190287
1977,3955,1977,5932,1.5306098461151123,0.21691000328007704
1983,3967,1983,5950,1.5350987911224365,0.2107177992504603
1988,3977,1988,5965,1.5382459163665771,0.2055789484717252
1994,3989,1994,5983,1.5419847965240479,0.19944162272258836
2000,4001,2000,6001,1.545644760131836,0.19334029930109864
2005,4011,2005,6016,1.5486578941345215,0.1882864623776186
2011,4023,2011,6034,1.5525016784667969,0.18226230799098175
2017,4035,2017,6052,1.5564789772033691,0.17628635874746124
2022,4045,2022,6067,1.5604338645935059,0.17134633577006753
2028,4057,2028,6085,1.5651500225067139,0.1654699446532959
2034,4069,2034,6103,1.5694808959960938,0.15965390004714664
2039,4079,2039,6118,1.5731489658355713,0.15485632357206214
2045,4091,2045,6136,1.577807903289795,0.14916175549444688
2051,4103,2051,6154,1.581355094909668,0.1435391977169047
2056,4113,2056,6169,1.585007905960083,0.13891155800570232
2062,4125,2062,6187,1.5906996726989746,0.13343102298108533
2068,4137,2068,6205,1.5948598384857178,0.12803307778244744
2073,4147,2073,6220,1.5993778705596924,0.12360028887974295
2079,4159,2079,6238,1.6041288375854492,0.11836222552392428
2085,4171,2085,6256,1.6093077659606934,0.11321553733898782
2090,4181,2090,6271,1.6135568618774414,0.1089983405233852
2096,4193,2096,6289,1.6178698539733887,0.10402587943303843
2102,4205,2102,6307,1.6216089725494385,0.09915178015296533
2107,4215,2107,6322,1.6246058940887451,0.09516674916972079
2113,4227,2113,6340,1.6281678676605225,0.09047860659836715
2119,4239,2119,6358,1.6317768096923828,0.08589485052505097
2124,4249,2124,6373,1.6347310543060303,0.08215626738012816
2130,4261,2130,6391,1.639375925064087,0.07776917138983208
2136,4273,2136,6409,1.644331693649292,0.07349217725845847
2141,4283,2141,6424,1.6483206748962402,0.07001353104283226
2147,4295,2147,6442,1.6531789302825928,0.06594342417270127
2153,4307,2153,6460,1.6582117080688477,0.06198880736587853
2158,4317,2158,6475,1.6621358394622803,0.05878279550051957
2164,4329,2164,6493,1.6670947074890137,0.05504444463372238
2170,4341,2170,6511,1.6718809604644775,0.05142634698722759
2175,4351,2175,6526,1.675527811050415,0.048504177454560704
2181,4363,2181,6544,1.679926872253418,0.04511019619974377
2187,4375,2187,6562,1.6840567588806152,0.041840133214009256
2192,4385,2192,6577,1.687356948852539,0.03921040552222621
2198,4397,2198,6595,1.69144868850708,0.03616972611689562
2204,4409,2204,6613,1.6950819492340088,0.033254936146363434
2209,4419,2209,6628,1.697948932647705,0.030922293237154008
2215,4431,2215,6646,1.701962947845459,0.028238783010237967
2221,4443,2221,6664,1.7060978412628174,0.025681329893586735
2226,4453,2226,6679,1.7091188430786133,0.023646224027174867
2232,4465,2232,6697,1.7134289741516113,0.021319103555924812
2238,4477,2238,6715,1.717862844467163,0.01911702429720208
2243,4487,2243,6730,1.7209968566894531,0.017377118653030266
2249,4499,2249,6748,1.725822925567627,0.015402964736949798
2255,4511,2255,6766,1.7307178974151611,0.013552356158811563
2260,4521,2260,6781,1.7348217964172363,0.012104137211167654
2266,4533,2266,6799,1.739583969116211,0.010478490181185407
2272,4545,2272,6817,1.744743824005127,0.008974643672559068
2277,4555,2277,6832,1.7483856678009033,0.007813971022983424
2283,4567,2283,6850,1.7537908554077148,0.006531527414608718
2289,4579,2289,6868,1.7582688331604004,0.005368650859509216
2294,4589,2294,6883,1.7621729373931885,0.004490205376896483
2300,4601,2300,6901,1.7677688598632812,0.0035438267567542425
2306,4613,2306,6919,1.772655725479126,0.00271377039825893
2311,4623,2311,6934,1.7771847248077393,0.0021098546393432116
2317,4635,2317,6952,1.7830207347869873,0.001489090122390735
2323,4647,2323,6970,1.7883226871490479,0.0009799993745218671
2328,4657,2328,6985,1.792536735534668,0.0006396558499091043
2334,4669,2334,7003,1.7973499298095703,0.00033012678090926784
2340,4681,2340,7021,1.8028678894042969,0.00012642321905786957
2345,4691,2345,7036,1.8069970607757568,3.589972232020955e-05
2351,4703,2351,7054,1.8116238117218018,2.037836975432583e-05
2357,4715,2357,7072,1.8151679039001465,0.00010425693722027063
2362,4725,2362,7087,1.8192389011383057,0.00024841752338033984
2368,4737,2368,7105,1.8244118690490723,0.0005085125500272625
2373,4747,2373,7120,1.8281407356262207,0.0007962580372122829
2379,4759,2379,7138,1.8334169387817383,0.001224716594038
2385,4771,2385,7156,1.8385059833526611,0.0017416561430536603
2390,4781,2390,7171,1.8432199954986572,0.0022382925137662824
2396,4793,2396,7189,1.8478548526763916,0.0029111602113971458
2402,4805,2402,7207,1.8542699813842773,0.003665560910462773
2407,4815,2407,7222,1.8587899208068848,0.004354662892296801
2413,4827,2413,7240,1.8631079196929932,0.005251828917948842
2419,4839,2419,7258,1.8685297966003418,0.006223066541906519
2424,4849,2424,7273,1.8731939792633057,0.007087004847676326
2430,4861,2430,7291,1.8783879280090332,0.008186741156919197
2436,4873,2436,7309,1.8826618194580078,0.009352445627200723
2441,4883,2441,7324,1.8864319324493408,0.010372100473318824
2447,4895,2447,7342,1.8913118839263916,0.011650937863805666
2453,4907,2453,7360,1.896528959274292,0.012987151618744974
2458,4917,2458,7375,1.9006948471069336,0.014142267165539124
2464,4929,2464,7393,1.9053997993469238,0.015575657566614609
2470,4941,2470,7411,1.9105148315429688,0.017057685773238518
2475,4951,2475,7426,1.9142930507659912,0.018327650542005358
2481,4963,2481,7444,1.919205904006958,0.019890899489041658
2487,4975,2487,7462,1.9244239330291748,0.021494154980132407
2492,4985,2492,7477,1.9289138317108154,0.02285859667040313
2498,4997,2498,7495,1.932804822921753,0.024527425117639723
2504,5009,2504,7513,1.937195062637329,0.02622782869434559
2509,5019,2509,7528,1.9411919116973877,0.027666838571690278
2515,5031,2515,7546,1.9462947845458984,0.029417539673886495
2521,5043,2521,7564,1.9507789611816406,0.0311915665321294
2526,5053,2526,7579,1.9540948867797852,0.03268565596999906
2532,5065,2532,7597,1.9578378200531006,0.03449494269000297
2538,5077,2538,7615,1.9614858627319336,0.03631936458793916
2543,5087,2543,7630,1.9644370079040527,0.03784918434951123
2549,5099,2549,7648,1.968371868133545,0.03969381133720162
2555,5111,2555,7666,1.9727427959442139,0.0415453353242583
2560,5121,2560,7681,1.9758408069610596,0.04309144328783532
2566,5133,2566,7699,1.9808228015899658,0.04494807584717364
2572,5145,2572,7717,1.9856319427490234,0.04680342777703572
2577,5155,2577,7732,1.9888968467712402,0.04834654175340347
2583,5167,2583,7750,1.9927308559417725,0.05019227046705055
2589,5179,2589,7768,1.9973487854003906,0.052028898094704346
2594,5189,2594,7783,2.001643657684326,0.053550575835060954
2600,5201,2600,7801,2.0069339275360107,0.055363773809176564
2606,5213,2606,7819,2.011302947998047,0.05716066985894486
2611,5223,2611,7834,2.0148868560791016,0.058643914364211014
2617,5235,2617,7852,2.019150733947754,0.06040481437287326
2623,5247,2623,7870,2.0233378410339355,0.062142890567884024
2628,5257,2628,7885,2.0280656814575195,0.06357228914157531
2634,5269,2634,7903,2.0332558155059814,0.06526293988872567
2640,5281,2640,7921,2.0386297702789307,0.06692477006708941
2645,5291,2645,7936,2.043071985244751,0.06828614564426516
2651,5303,2651,7954,2.04724383354187,0.06988988466343926
2657,5315,2657,7972,2.051076889038086,0.07145913371698498
2662,5325,2662,7987,2.0554356575012207,0.07273909945922696
2668,5337,2668,8005,2.0606307983398438,0.07424013108823146
2674,5349,2674,8023,2.0657737255096436,0.07570132448745426
2679,5359,2679,8038,2.069429636001587,0.07688727206243584
2685,5371,2685,8056,2.074436902999878,0.07827088013095818
2691,5383,2691,8074,2.0785698890686035,0.07960983980399305
2696,5393,2696,8089,2.081829786300659,0.0806904318199031
2702,5405,2702,8107,2.0857737064361572,0.08194365617555377
2708,5417,2708,8125,2.089550733566284,0.08314818609483154
2713,5427,2713,8140,2.093369722366333,0.08411387313276464
2719,5439,2719,8158,2.098228931427002,0.08522600536673508
2725,5451,2725,8176,2.10257887840271,0.08628620847514412
2730,5461,2730,8191,2.106235980987549,0.08712934207107992
2736,5473,2736,8209,2.110140800476074,0.08809188391012412
2742,5485,2742,8227,2.1138477325439453,0.08899995151318763
2747,5495,2747,8242,2.118285894393921,0.0897145088989646
2753,5507,2753,8260,2.123807907104492,0.09052076614284488
2759,5519,2759,8278,2.128626823425293,0.09127054141697499
2764,5529,2764,8293,2.1324098110198975,0.09185177802180533
2770,5541,2770,8311,2.1369497776031494,0.09249650564993317
2776,5553,2776,8329,2.1405649185180664,0.09308323319896772
2781,5563,2781,8344,2.1434340476989746,0.0935275717862396
2787,5575,2787,8362,2.1468379497528076,0.09400696501529637
2793,5587,2793,8380,2.1501970291137695,0.09442740741963007
2798,5597,2798,8395,2.153775930404663,0.0947326120830212
2804,5609,2804,8413,2.1586058139801025,0.09504457384139187
2810,5621,2810,8431,2.1633107662200928,0.0952973006250204
2815,5631,2815,8446,2.1662516593933105,0.09546270194437056
2821,5643,2821,8464,2.1705589294433594,0.09560706172771916
2827,5655,2827,8482,2.175520658493042,0.0956925876527066
2832,5665,2832,8497,2.178727865219116,0.09571912704780061
2838,5677,2838,8515,2.1842780113220215,0.09569760927990956
2844,5689,2844,8533,2.1895999908447266,0.09561828032622088
2849,5699,2849,8548,2.1936798095703125,0.09550836467440149
2855,5711,2855,8566,2.1987369060516357,0.09532437154814488
2861,5723,2861,8584,2.2052717208862305,0.09508412036927893
2866,5733,2866,8599,2.209697723388672,0.09484141042344163
2872,5745,2872,8617,2.2137038707733154,0.0944997716879925
2878,5757,2878,8635,2.2178759574890137,0.0941038826156273
2883,5767,2883,8650,2.2215628623962402,0.09373311540298346
2889,5779,2889,8668,2.226670742034912,0.09323990293057705
2895,5791,2895,8686,2.232050895690918,0.09269486094490276
2900,5801,2900,8701,2.2357540130615234,0.09220175172470135
2906,5813,2906,8719,2.239763021469116,0.09156419468740751
2912,5825,2912,8737,2.2438149452209473,0.09087763287755024
2917,5835,2917,8752,2.247361660003662,0.09026885112746186
2923,5847,2923,8770,2.2513248920440674,0.08949532256747261
2929,5859,2929,8788,2.2559847831726074,0.08867601448014284
2934,5869,2934,8803,2.2600629329681396,0.08795917296197331
2940,5881,2940,8821,2.2648227214813232,0.0870591609781286
2946,5893,2946,8839,2.268847942352295,0.08611696553737147
2951,5903,2951,8854,2.2724149227142334,0.08530054964683131
2957,5915,2957,8872,2.2759907245635986,0.08428454082820735
2963,5927,2963,8890,2.279719829559326,0.08323025287563723
2968,5937,2968,8905,2.282801866531372,0.08232347501154891
2974,5949,2974,8923,2.2871549129486084,0.08120276184286013
2980,5961,2980,8941,2.292247772216797,0.08004790986603894
2985,5971,2985,8956,2.2959706783294678,0.0790605412333889
2991,5983,2991,8974,2.299452781677246,0.07784702928120169
2997,5995,2997,8992,2.3029699325561523,0.07660370000280636
3002,6005,3002,9007,2.306337833404541,0.07554594167959294
3008,6017,3008,9025,2.3102898597717285,0.07425201755700073
3014,6029,3014,9043,2.3144309520721436,0.07293274760615986
3019,6039,3019,9058,2.318459987640381,0.07181515518027481
3025,6051,3025,9076,2.323943853378296,0.07045360737731698
3031,6063,3031,9094,2.3289709091186523,0.06907130667661932
3036,6073,3036,9109,2.3332178592681885,0.06790471983219959
3042,6085,3042,9127,2.3383827209472656,0.06648863605028055
3048,6097,3048,9145,2.343411922454834,0.06505645594381804
3053,6107,3053,9160,2.3477530479431152,0.06385186182399138
3059,6119,3059,9178,2.3535947799682617,0.06239443254366961
3065,6131,3065,9196,2.357408046722412,0.060925539865706924
3070,6141,3070,9211,2.360585927963257,0.05969387129050574
3076,6153,3076,9229,2.3644628524780273,0.05820814662752127
3082,6165,3082,9247,2.3686039447784424,0.056715498254447994
3087,6175,3087,9262,2.371896743774414,0.05546747304208566
3093,6187,3093,9280,2.376110792160034,0.053966215243690385
3099,6199,3099,9298,2.3865418434143066,0.052462467173768346
3104,6209,3104,9313,2.3911118507385254,0.051208555219886875
3110,6221,3110,9331,2.395443916320801,0.04970424288876529
3116,6233,3116,9349,2.400852918624878,0.04820178741260861
3121,6243,3121,9364,2.404021739959717,0.0469522526819901
3127,6255,3127,9382,2.407867908477783,0.04545712640231159
3133,6267,3133,9400,2.411773920059204,0.0439681145898021
3138,6277,3138,9415,2.4156908988952637,0.042733005200375374
3144,6289,3144,9433,2.420224666595459,0.04125901262523257
3150,6301,3150,9451,2.4237759113311768,0.039795248448399434
3155,6311,3155,9466,2.4267988204956055,0.03858427019042665
3161,6323,3161,9484,2.430764675140381,0.03714287335174049
3167,6335,3167,9502,2.4356019496917725,0.03571558560156518
3172,6345,3172,9517,2.439866781234741,0.03453789409445562
3178,6357,3178,9535,2.443643808364868,0.033139811831802035
3184,6369,3184,9553,2.4477996826171875,0.03175940331186666
3189,6379,3189,9568,2.451427698135376,0.03062341230815946
3195,6391,3195,9586,2.457300901412964,0.029278424622702914
3201,6403,3201,9604,2.4616546630859375,0.02795432641653406
3206,6413,3206,9619,2.465686798095703,0.026867631184359198
3212,6425,3212,9637,2.4700658321380615,0.025584544682942578
3218,6437,3218,9655,2.474616765975952,0.024325242632585287
3223,6447,3223,9670,2.4783918857574463,0.023294683415088002
3229,6459,3229,9688,2.4827957153320312,0.022081446269908156
3235,6471,3235,9706,2.4866509437561035,0.02089462247931806
3240,6481,3240,9721,2.489694833755493,0.019926408733681455
3246,6493,3246,9739,2.4938907623291016,0.018790249685935123
3252,6505,3252,9757,2.4975688457489014,0.017682891954223123
3257,6515,3257,9772,2.5011839866638184,0.016782658498755154
3263,6527,3263,9790,2.505558729171753,0.015730100823702742
3269,6539,3269,9808,2.5094406604766846,0.014708451320075255
3274,6549,3274,9823,2.512807846069336,0.01388116502948833
3280,6561,3280,9841,2.5166878700256348,0.012917859578919888
3286,6573,3286,9859,2.5206117630004883,0.01198720099671391
3291,6583,3291,9874,2.523859977722168,0.011236961207941931
3297,6595,3297,9892,2.527784824371338,0.010367442523602222
3302,6605,3302,9907,2.531038999557495,0.009668762398405306
3308,6617,3308,9925,2.53562593460083,0.008861760592822066
3314,6629,3314,9943,2.540776014328003,0.00808932326856393
3319,6639,3319,9958,2.5448808670043945,0.007472222641808912
3325,6651,3325,9976,2.5497989654541016,0.006763815356066516
3331,6663,3331,9994,2.5549299716949463,0.006090620847089667
3336,6673,3336,10009,2.5589959621429443,0.005556638531288627
3342,6685,3342,10027,2.5630080699920654,0.004948386595287957
3348,6697,3348,10045,2.5722408294677734,0.004375713050080776
3353,6707,3353,10060,2.57696270942688,0.003925716409867164
3359,6719,3359,10078,2.581561803817749,0.003418438169092042
3365,6731,3365,10096,2.5857458114624023,0.002946868369463118
3370,6741,3370,10111,2.589148998260498,0.0025811617073259185
3376,6753,3376,10129,2.5932717323303223,0.002174994949768916
3382,6765,3382,10147,2.597637891769409,0.0018044007805428919
3387,6775,3387,10162,2.6014928817749023,0.0015226569905735232
3393,6787,3393,10180,2.6063339710235596,0.0012169222235343113
3399,6799,3399,10198,2.6112818717956543,0.0009462876288353073
3404,6809,3404,10213,2.6146318912506104,0.000747387859405535
3410,6821,3410,10231,2.618853807449341,0.0005404037165135378
3416,6833,3416,10249,2.6231889724731445,0.0003676726254298046
3421,6843,3421,10264,2.626617908477783,0.0002496197829486846
3427,6855,3427,10282,2.6304218769073486,0.00013866028530173935
3433,6867,3433,10300,2.6346168518066406,6.0766838828385517e-05
3438,6877,3438,10315,2.63875675201416,2.0765610997841577e-05
3444,6889,3444,10333,2.643904685974121,2.2143251499073813e-06
3450,6901,3450,10351,2.649513006210327,1.5286457824004174e-05
3455,6911,3455,10366,2.653184652328491,4.9937377411879424e-05
3461,6923,3461,10384,2.6569418907165527,0.00011953221849125839
3467,6935,3467,10402,2.660738706588745,0.00021913105717885628
3472,6945,3472,10417,2.663595676422119,0.00032461336081723857
3478,6957,3478,10435,2.667147636413574,0.00047763398038114246
3484,6969,3484,10453,2.6705617904663086,0.0006588970068150957
3489,6979,3489,10468,2.674393892288208,0.0008310501272035253
3495,6991,3495,10486,2.678931951522827,0.0010623693798379463
3501,7003,3501,10504,2.6827309131622314,0.0013200143965832467
3506,7013,3506,10519,2.685945749282837,0.0015543100410013722
3512,7025,3512,10537,2.6906518936157227,0.0018583320462539632
3518,7037,3518,10555,2.694788932800293,0.0021865765295387973
3523,7047,3523,10570,2.6979968547821045,0.002478047658655669
3529,7059,3529,10588,2.7023048400878906,0.002848630814924036
3535,7071,3535,10606,2.7066256999969482,0.003241136880319573
3540,7081,3540,10621,2.709696054458618,0.0035843568956579475
3546,7093,3546,10639,2.713873863220215,0.004014826004436145
3552,7105,3552,10657,2.71765398979187,0.004464756905122158
3557,7115,3557,10672,2.7208006381988525,0.004853920711866522
3563,7127,3563,10690,2.7245707511901855,0.005337201686984372
3569,7139,3569,10708,2.728085994720459,0.005837390448846236
3574,7149,3574,10723,2.731001853942871,0.0062664737433806295
3580,7161,3580,10741,2.7345447540283203,0.006795297001986
3586,7173,3586,10759,2.738496780395508,0.007338450993529477
3591,7183,3591,10774,2.7422468662261963,0.007801372194421674
3597,7195,3597,10792,2.746882677078247,0.008368446006556951
3603,7207,3603,10810,2.7516119480133057,0.008947287318051167
3608,7217,3608,10825,2.754859685897827,0.009437993507617648
3614,7229,3614,10843,2.758737802505493,0.010036065988742848
3620,7241,3620,10861,2.7625060081481934,0.010643348474786762
3625,7251,3625,10876,2.7662978172302246,0.011155798521485849
3631,7263,3631,10894,2.7715189456939697,0.011777608051147581
3637,7275,3637,10912,2.775796890258789,0.01240604816450741
3642,7285,3642,10927,2.7789628505706787,0.01293415142606591
3648,7297,3648,10945,2.782700777053833,0.013572363030220913
3654,7309,3654,10963,2.787834882736206,0.014214601608841804
3659,7319,3659,10978,2.7912588119506836,0.014752214536201791
3665,7331,3665,10996,2.7962608337402344,0.015399456877617013
3671,7343,3671,11014,2.800881862640381,0.016048143282546334
3676,7353,3676,11029,2.805027723312378,0.016589173371244215
3682,7365,3682,11047,2.8086798191070557,0.01723819687776995
3688,7377,3688,11065,2.813509941101074,0.01788617168233486
3693,7387,3693,11080,2.817206859588623,0.018424737513555556
3699,7399,3699,11098,2.821347713470459,0.01906860173039604
3705,7411,3705,11116,2.825002908706665,0.01970906431381536
3710,7421,3710,11131,2.828089714050293,0.020239610553289822
3716,7433,3716,11149,2.8317530155181885,0.020871784210044098
3722,7445,3722,11167,2.8358919620513916,0.021498346674434288
3727,7455,3727,11182,2.8391387462615967,0.022015653585981454
3733,7467,3733,11200,2.8438258171081543,0.02262998764592794
3739,7479,3739,11218,2.848256826400757,0.023236614730990368
3744,7489,3744,11233,2.851942777633667,0.023735731846727504
3750,7501,3750,11251,2.8563358783721924,0.02432637308845642
3756,7513,3756,11269,2.860527753829956,0.024907302589554092
3761,7523,3761,11284,2.863489866256714,0.025383497709299263
3767,7535,3767,11302,2.8667778968811035,0.0259448557134192
3773,7547,3773,11320,2.8703670501708984,0.02649460326335884
3778,7557,3778,11335,2.8733277320861816,0.02694339754179964
3784,7569,3784,11353,2.8767240047454834,0.02747022271057631
3790,7581,3790,11371,2.8801119327545166,0.02798369334095696
3795,7591,3795,11386,2.8829777240753174,0.028400973144698582
3801,7603,3801,11404,2.887425661087036,0.028888503444363778
3807,7615,3807,11422,2.891528844833374,0.02936113989687783
3812,7625,3812,11437,2.894526958465576,0.0297432725053568
3818,7637,3818,11455,2.8981807231903076,0.030187353096948755
3824,7649,3824,11473,2.9020938873291016,0.030615226047189026
3829,7659,3829,11488,2.906111001968384,0.03095910796514545
3835,7671,3835,11506,2.9110107421875,0.03135621452315718
3841,7683,3841,11524,2.9155118465423584,0.03173600871502913
3846,7693,3846,11539,2.9185478687286377,0.032039028445296935
3852,7705,3852,11557,2.922144651412964,0.032386197446157894
3858,7717,3858,11575,2.925794839859009,0.03271512306616842
3863,7727,3863,11590,2.928741931915283,0.032975080232859
3869,7739,3869,11608,2.9322450160980225,0.03326981286852515
3875,7751,3875,11626,2.9360337257385254,0.03354552037274061
3880,7761,3880,11641,2.9401397705078125,0.03376056969500496
3886,7773,3886,11659,2.9440059661865234,0.03400078869663048
3892,7785,3892,11677,2.9474518299102783,0.03422135596724729
3897,7795,3897,11692,2.9504168033599854,0.034390020734576865
3903,7807,3903,11710,2.9540839195251465,0.034574114044517046
3909,7819,3909,11728,2.957509756088257,0.03473811564026619
3914,7829,3914,11743,2.961482048034668,0.034859359866345585
3920,7841,3920,11761,2.966207981109619,0.03498627685144129
3926,7853,3926,11779,2.9701788425445557,0.03509288136081068
3931,7863,3931,11794,2.9732208251953125,0.03516618452363218
3937,7875,3937,11812,2.976801872253418,0.035235509915992225
3943,7887,3943,11830,2.9809489250183105,0.03528452938758164
3948,7897,3948,11845,2.9839558601379395,0.035309904862856456
3954,7909,3954,11863,2.9880318641662598,0.0353218511305613
3960,7921,3960,11881,2.992910861968994,0.03531370121152122
3965,7931,3965,11896,2.9964659214019775,0.03529164070278057
3971,7943,3971,11914,3.0000157356262207,0.03524695964847524
3977,7955,3977,11932,3.0036377906799316,0.03518255510232393
3982,7965,3982,11947,3.006647825241089,0.035113936056973216
3988,7977,3988,11965,3.010326862335205,0.03501380961961331
3994,7989,3994,11983,3.013953685760498,0.03489446600224255
3999,7999,3999,11998,3.017443895339966,0.03478048371891873
4005,8011,4005,12016,3.0219669342041016,0.03462646437606054
4011,8023,4011,12034,3.0259227752685547,0.03445386524492733
4016,8033,4016,12049,3.0290067195892334,0.03429602627159056
4022,8045,4022,12067,3.0326600074768066,0.03409005180787972
4028,8057,4028,12085,3.0363218784332275,0.03386628349073817
4033,8067,4033,12100,3.0401060581207275,0.033666444883238
4039,8079,4039,12118,3.0447397232055664,0.033410890755249056
4045,8091,4045,12136,3.048365831375122,0.03313849230437427
4050,8101,4050,12151,3.0513370037078857,0.03289889545385449
4056,8113,4056,12169,3.054921865463257,0.032596599865883036
4062,8125,4062,12187,3.0594067573547363,0.03227856620219427
4067,8135,4067,12202,3.0626020431518555,0.03200182045213751
4073,8147,4073,12220,3.0662498474121094,0.03165604137529954
4079,8159,4079,12238,3.071013927459717,0.031295756672420794
4084,8169,4084,12253,3.0747668743133545,0.030984768704229282
4090,8181,4090,12271,3.0782899856567383,0.03059908611908213
4096,8193,4096,12289,3.0819168090820312,0.030200218525806122
4101,8203,4101,12304,3.0855507850646973,0.029858104290269694
4107,8215,4107,12322,3.0898618698120117,0.02943632037113275
4113,8227,4113,12340,3.094564914703369,0.02900273451234625
4118,8237,4118,12355,3.0983498096466064,0.02863275921811237
4124,8249,4124,12373,3.1020009517669678,0.028178844359899813
4130,8261,4130,12391,3.106370687484741,0.02771456788877913
4135,8271,4135,12406,3.1095588207244873,0.02732013301988445
4141,8283,4141,12424,3.1134417057037354,0.026838225558321938
4147,8295,4147,12442,3.1175248622894287,0.02634746129524501
4152,8305,4152,12457,3.1205198764801025,0.025932120186666907
4158,8317,4158,12475,3.1242527961730957,0.025426546285416407
4164,8329,4164,12493,3.1278889179229736,0.02491368754181167
4169,8339,4169,12508,3.1310060024261475,0.02448115053971378
4175,8351,4175,12526,3.135075807571411,0.02395641718760544
4181,8363,4181,12544,3.139512777328491,0.02342602331600574
4186,8373,4186,12559,3.1427078247070312,0.022980122953640603
4192,8385,4192,12577,3.147185802459717,0.0224408591448082
4198,8397,4198,12595,3.1521248817443848,0.021897580243944503
4203,8407,4203,12610,3.1555399894714355,0.021442198675117652
4209,8419,4209,12628,3.1596360206604004,0.02089306098775978
4215,8431,4215,12646,3.1634130477905273,0.020341541073889857
4220,8441,4220,12661,3.1667206287384033,0.019880531969874937
4226,8453,4226,12679,3.1704137325286865,0.019326118930393932
4232,8465,4232,12697,3.1739587783813477,0.018770923649867655
4237,8475,4237,12712,3.176950693130493,0.01830806462885448
4243,8487,4243,12730,3.181818962097168,0.01775287628345268
4248,8497,4248,12745,3.1853268146514893,0.01729079389644994
4254,8509,4254,12763,3.1893489360809326,0.016737456575469878
4260,8521,4260,12781,3.1930649280548096,0.01618589821362093
4265,8531,4265,12796,3.196337938308716,0.01572801380848432
4271,8543,4271,12814,3.2013509273529053,0.015181112789491635
4277,8555,4277,12832,3.205812931060791,0.014637506120834587
4282,8565,4282,12847,3.2098758220672607,0.014187396623015047
4288,8577,4288,12865,3.2136118412017822,0.013651190827090431
4294,8589,4294,12883,3.2172658443450928,0.013119752114334915
4299,8599,4299,12898,3.221101760864258,0.012680892551429679
4305,8611,4305,12916,3.225944757461548,0.012159497591142099
4311,8623,4311,12934,3.230376958847046,0.0116442735649116
4316,8633,4316,12949,3.2344930171966553,0.011219976364372997
4322,8645,4322,12967,3.238710641860962,0.01071728726924448
4328,8657,4328,12985,3.2435479164123535,0.01022207823973531
4333,8667,4333,13000,3.247519016265869,0.00981543337900348
4339,8679,4339,13018,3.252466917037964,0.009335061983279047
4345,8691,4345,13036,3.2563509941101074,0.008863372671839898
4350,8701,4350,13051,3.260329008102417,0.008477218513121443
4356,8713,4356,13069,3.2653257846832275,0.008022472999414276
4362,8725,4362,13087,3.270509719848633,0.007577506752227237
4367,8735,4367,13102,3.274622917175293,0.007214434482989418
4373,8747,4373,13120,3.2789759635925293,0.006788332490827997
4379,8759,4379,13138,3.2829158306121826,0.006373008588980156
4384,8769,4384,13153,3.2868738174438477,0.006035376451109187
4390,8781,4390,13171,3.292343854904175,0.005640658098741369
4396,8793,4396,13189,3.2966928482055664,0.005257616901644724
4401,8803,4401,13204,3.3003528118133545,0.004947546575635897
4407,8815,4407,13222,3.3047149181365967,0.004586659499864254
4413,8827,4413,13240,3.308605909347534,0.004238235963725856
4418,8837,4418,13255,3.3126018047332764,0.003957582650059521
4424,8849,4424,13273,3.317612886428833,0.003632638797967047
4430,8861,4430,13291,3.3227200508117676,0.0033208143811407353
4435,8871,4435,13306,3.326955795288086,0.0030711256808899634
4441,8883,4441,13324,3.3323488235473633,0.0027838540509037557
4447,8895,4447,13342,3.3372249603271484,0.002510215134293503
4452,8905,4452,13357,3.340566635131836,0.0022927029532411325
4458,8917,4458,13375,3.3442089557647705,0.0020444257113467756
4464,8929,4464,13393,3.347660779953003,0.0018101516646993332
4469,8939,4469,13408,3.3505258560180664,0.0016256916135262145
4475,8951,4475,13426,3.354966640472412,0.001417333948893429
4481,8963,4481,13444,3.3583178520202637,0.0012232169453909592
4486,8973,4486,13459,3.3614258766174316,0.0010723707215447575
4492,8985,4492,13477,3.365504741668701,0.0009044921824852281
4498,8997,4498,13495,3.369243860244751,0.0007509703523282951
4503,9007,4503,13510,3.3722777366638184,0.0006340123932204733
4509,9019,4509,13528,3.3759360313415527,0.0005068350915280462
4515,9031,4515,13546,3.3795058727264404,0.0003940142172496053
4520,9041,4520,13561,3.3825669288635254,0.0003109434870793848
4526,9053,4526,13579,3.387018918991089,0.0002243578343268382
4532,9065,4532,13597,3.392305850982666,0.00015200788618585648
4537,9075,4537,13612,3.3956658840179443,0.00010253858306441543
4543,9087,4543,13630,3.3996009826660156,5.608597587070108e-05
4549,9099,4549,13648,3.4035398960113525,2.3619416765541246e-05
4554,9109,4554,13663,3.4072399139404297,7.1617057528783334e-06
4560,9121,4560,13681,3.411757707595825,1.2792838788300287e-08
4566,9133,4566,13699,3.4170868396759033,6.467403295573604e-06
4571,9143,4571,13714,3.4207608699798584,2.2118684228189522e-05
4577,9155,4577,13732,3.4253509044647217,5.307158517098287e-05
4583,9167,4583,13750,3.428985834121704,9.711956613500661e-05
4588,9177,4588,13765,3.431896686553955,0.00014368075733273145
4594,9189,4594,13783,3.4360718727111816,0.00021119059829288744
4600,9201,4600,13801,3.4407260417938232,0.0002911775748088985
4605,9211,4605,13816,3.4448108673095703,0.00036719115917094314
4611,9223,4611,13834,3.4488818645477295,0.00046941980087922275
4617,9235,4617,13852,3.4526238441467285,0.0005834158771449438
4622,9245,4622,13867,3.4556517601013184,0.000687207087025854
4628,9257,4628,13885,3.460399866104126,0.0008220683614581503
4634,9269,4634,13903,3.4654018878936768,0.0009679066148464699
4639,9279,4639,13918,3.4692628383636475,0.0010976092947885263
4645,9291,4645,13936,3.473435878753662,0.0012627921606735981
4651,9303,4651,13954,3.477186679840088,0.0014380836996679136
4656,9313,4656,13969,3.480353832244873,0.001591647684108466
4662,9325,4662,13987,3.484280824661255,0.0017846207373395373
4668,9337,4668,14005,3.488302707672119,0.0019867569494635973
4673,9347,4673,14020,3.4927470684051514,0.002161950225399778
4679,9359,4679,14038,3.4983737468719482,0.002379966947160028
4685,9371,4685,14056,3.503335952758789,0.002606129768992105
4690,9381,4690,14071,3.507678985595703,0.0028005520493934455
4696,9393,4696,14089,3.5126919746398926,0.003040673856730791
4702,9405,4702,14107,3.517544984817505,0.003287866212986046
4707,9415,4707,14122,3.521829843521118,0.0034989794130524388
4713,9427,4713,14140,3.5257248878479004,0.00375811712660834
4719,9439,4719,14158,3.529228687286377,0.00402320796206368
4724,9449,4724,14173,3.5321168899536133,0.004248374918461195
4730,9461,4730,14191,3.535653829574585,0.004523334854525274
4736,9473,4736,14209,3.5393826961517334,0.004803103081030713
4741,9483,4741,14224,3.542491912841797,0.005039621527203053
4747,9495,4747,14242,3.5463168621063232,0.005327142361238657
4753,9507,4753,14260,3.550618886947632,0.005618309261080867
4758,9517,4758,14275,3.5544447898864746,0.005863435673290951
4764,9529,4764,14293,3.5585858821868896,0.0061602140037848585
4770,9541,4770,14311,3.563408851623535,0.006459466595515551
4775,9551,4775,14326,3.5669188499450684,0.006710434970727874
4781,9563,4781,14344,3.5709009170532227,0.0070131481987800726
4787,9575,4787,14362,3.575065851211548,0.007317163611332944
4792,9585,4792,14377,3.5791707038879395,0.007571207561227311
4798,9597,4798,14395,3.5842769145965576,0.007876542966300804
4804,9609,4804,14413,3.588216781616211,0.008182020363506126
4809,9619,4809,14428,3.5918469429016113,0.008436401643052704
4815,9631,4815,14446,3.597054958343506,0.008741092310629028
4821,9643,4821,14464,3.6013519763946533,0.009044789741324166
4826,9653,4826,14479,3.604412794113159,0.00929682885987404
4832,9665,4832,14497,3.6080589294433594,0.009597689325460124
4838,9677,4838,14515,3.6118390560150146,0.009896457240074596
4843,9687,4843,14530,3.6149868965148926,0.010143559207904218
4849,9699,4849,14548,3.6194097995758057,0.010437513342935745
4855,9711,4855,14566,3.6237120628356934,0.010728319118129548
4860,9721,4860,14581,3.627912998199463,0.010967991520487885
4866,9733,4866,14599,3.632593870162964,0.011252091923893204
4872,9745,4872,14617,3.6371519565582275,0.01153203758883592
4877,9755,4877,14632,3.641366720199585,0.011761904840795978
4883,9767,4883,14650,3.6452159881591797,0.012033350270712617
4889,9779,4889,14668,3.6489927768707275,0.0122996912484723
4894,9789,4894,14683,3.654110908508301,0.012517511801206638
4900,9801,4900,14701,3.6587977409362793,0.012773670178489738
4906,9813,4906,14719,3.662522792816162,0.013023840999267122
4911,9823,4911,14734,3.665560722351074,0.013227530672452303
4917,9835,4917,14752,3.669839859008789,0.0134659688277452
4923,9847,4923,14770,3.6739447116851807,0.013697613884914972
4928,9857,4928,14785,3.678175926208496,0.013885271412391376
4934,9869,4934,14803,3.681964874267578,0.01410378450339067
4940,9881,4940,14821,3.686004877090454,0.014314784891553245
4945,9891,4945,14836,3.689506769180298,0.014484711479326506
4951,9903,4951,14854,3.693849802017212,0.014681342332778513
4957,9915,4957,14872,3.6984798908233643,0.014869830221073244
4962,9925,4962,14887,3.702256917953491,0.015020537687291835
4968,9937,4968,14905,3.706721782684326,0.015193582314395826
4974,9949,4974,14923,3.710463047027588,0.015357942627474586
4979,9959,4979,14938,3.7139737606048584,0.015488152734974392
4985,9971,4985,14956,3.7188286781311035,0.015636158295137648
4991,9983,4991,14974,3.723594903945923,0.01577502676821041
4996,9993,4996,14989,3.7273528575897217,0.0158836707272485
5002,10005,5002,15007,3.731639862060547,0.016005437345938844
5008,10017,5008,15025,3.7353549003601074,0.016117705795863912
5013,10027,5013,15040,3.739396810531616,0.01620393160033018
5019,10039,5019,15058,3.743673801422119,0.016298524622015975
5025,10051,5025,15076,3.7473318576812744,0.01638335639268007
5030,10061,5030,15091,3.7505197525024414,0.016446543369966093
5036,10073,5036,15109,3.7554688453674316,0.016513311614289705
5042,10085,5042,15127,3.759190082550049,0.016570159155207875
5047,10095,5047,15142,3.7622170448303223,0.016609930880349566
5053,10107,5053,15160,3.7658748626708984,0.01664851868383721
5059,10119,5059,15178,3.7697160243988037,0.01667713058850495
5064,10129,5064,15193,3.7728519439697266,0.016693356262180714
5070,10141,5070,15211,3.776319980621338,0.01670369938847216
5076,10153,5076,15229,3.779855728149414,0.01670411016198159
5081,10163,5081,15244,3.782853841781616,0.016696891864967256
5087,10175,5087,15262,3.7869210243225098,0.01667919813030494
5093,10187,5093,15280,3.7921578884124756,0.016651705800541095
5098,10197,5098,15295,3.7966208457946777,0.016621358786096607
5104,10209,5104,15313,3.802114725112915,0.01657608472339689
5110,10221,5110,15331,3.80721378326416,0.016521229450972896
5115,10231,5115,15346,3.8111648559570312,0.016468266856008995
5121,10243,5121,15364,3.8155438899993896,0.01639610331324093
5127,10255,5127,15382,3.8207647800445557,0.016314657812017686
5132,10265,5132,15397,3.8243799209594727,0.01623978636416723
5138,10277,5138,15415,3.828091859817505,0.01614165731336925
5144,10289,5144,15433,3.8332359790802,0.01603462898935959
5149,10299,5149,15448,3.8402607440948486,0.015938752296278835
5155,10311,5155,15466,3.845564842224121,0.015815819105114315
5161,10323,5161,15484,3.851515769958496,0.015684452957543726
5166,10333,5166,15499,3.8555798530578613,0.015568671602068207
5172,10345,5172,15517,3.859318733215332,0.015422329025227555
5178,10357,5178,15535,3.863086700439453,0.01526809803613105
5183,10367,5183,15550,3.866826057434082,0.015133696782527295
5189,10379,5189,15568,3.8721227645874023,0.01496555173730485
5194,10389,5194,15583,3.876710891723633,0.014819862368312897
5200,10401,5200,15601,3.882380723953247,0.014638550861718613
5206,10413,5206,15619,3.8882148265838623,0.014450387070155557
5211,10423,5211,15634,3.8937389850616455,0.014288522437368556
5217,10435,5217,15652,3.8986849784851074,0.014088422990653271
5223,10447,5223,15670,3.903984785079956,0.013882164416031628
5228,10457,5228,15685,3.9141178131103516,0.013705760561265379
5234,10469,5234,15703,3.920747756958008,0.013488873554706515
5240,10481,5240,15721,3.9265449047088623,0.013266559350881835
5245,10491,5245,15736,3.9306087493896484,0.013077344254725176
5251,10503,5251,15754,3.934400796890259,0.012845776930134889
5257,10515,5257,15772,3.939410924911499,0.012609550449724338
5262,10525,5262,15787,3.9428718090057373,0.012409337364488238
5268,10537,5268,15805,3.9474239349365234,0.012165297456590451
5274,10549,5274,15823,3.9527578353881836,0.011917400009906487
5279,10559,5279,15838,3.956540822982788,0.01170808109304744
5285,10571,5285,15856,3.960723876953125,0.011453866424858461
5291,10583,5291,15874,3.964874029159546,0.011196622688316893
5296,10593,5296,15889,3.96828293800354,0.010980153068544496
5302,10605,5302,15907,3.9731216430664062,0.010718127673726485
5308,10617,5308,15925,3.97705078125,0.010453916898654825
5313,10627,5313,15940,3.9814348220825195,0.010232287497615289
5319,10639,5319,15958,3.9870259761810303,0.009964846236130143
5325,10651,5325,15976,3.991255760192871,0.009696065270190957
5330,10661,5330,15991,3.9943089485168457,0.009471271948655158
5336,10673,5336,16009,3.9982337951660156,0.009200804825695741
5342,10685,5342,16027,4.00248384475708,0.008929835215553794
5347,10695,5347,16042,4.006337881088257,0.0087038542665141
5353,10707,5353,16060,4.010167837142944,0.008432721064764337
5359,10719,5359,16078,4.013608932495117,0.00816190824491514
5364,10729,5364,16093,4.016513824462891,0.007936682302556619
5370,10741,5370,16111,4.020924806594849,0.007667198932949759
5376,10753,5376,16129,4.025547742843628,0.007398841106464715
5381,10763,5381,16144,4.028719902038574,0.007176270887839564
5387,10775,5387,16162,4.032788991928101,0.0069106995107404146
5393,10787,5393,16180,4.037771701812744,0.006647036604022105
5398,10797,5398,16195,4.041881799697876,0.006428970039905835
5404,10809,5404,16213,4.045869827270508,0.006169503375303975
5410,10821,5410,16231,4.050508737564087,0.005912698113661463
5415,10831,5415,16246,4.054194927215576,0.005700912128645541
5421,10843,5421,16264,4.05922794342041,0.005449649025763392
5427,10855,5427,16282,4.064428806304932,0.0052017604316461075
5432,10865,5432,16297,4.067728757858276,0.004997938012706982
5438,10877,5438,16315,4.0727598667144775,0.00475685592039099
5444,10889,5444,16333,4.077784776687622,0.004519812894614006
5449,10899,5449,16348,4.082028865814209,0.0043255227143390584
5455,10911,5455,16366,4.086347818374634,0.004096455980175051
5461,10923,5461,16384,4.090022802352905,0.0038720391876267968
5466,10933,5466,16399,4.0937769412994385,0.003688723469508659
5472,10945,5472,16417,4.098735809326172,0.003473352283094755
5478,10957,5478,16435,4.10838770866394,0.003263186553908781
5483,10967,5483,16450,4.113448858261108,0.003092156895490916
5489,10979,5489,16468,4.118034839630127,0.00289200409224577
5495,10991,5495,16486,4.121826887130737,0.002697556233897558
5500,11001,5500,16501,4.124915838241577,0.002539991790854401
5506,11013,5506,16519,4.128843069076538,0.002356419821808231
5512,11025,5512,16537,4.13310170173645,0.002178993881216229
5517,11035,5517,16552,4.136580944061279,0.002035935684261858
5523,11047,5523,16570,4.141037702560425,0.0018701374527836379
5529,11059,5529,16588,4.146277904510498,0.001710863016114672
5534,11069,5534,16603,4.1504967212677,0.0015832025208055711
5540,11081,5540,16621,4.154892683029175,0.0014361861414045052
5546,11093,5546,16639,4.158456802368164,0.0012960022625065903
5551,11103,5551,16654,4.161316871643066,0.0011844680415151743
5557,11115,5557,16672,4.164738893508911,0.0010570418891120426
5563,11127,5563,16690,4.168421745300293,0.0009366842078861737
5568,11137,5568,16705,4.172483921051025,0.00084183343631139
5574,11149,5574,16723,4.176301717758179,0.0007345991617739855
5580,11161,5580,16741,4.180548906326294,0.0006345967956349341
5585,11171,5585,16756,4.184522867202759,0.0005568156583422024
5591,11183,5591,16774,4.188246726989746,0.00047017203496579896
5597,11195,5597,16792,4.191778898239136,0.0003908545322701684
5602,11205,5602,16807,4.194828748703003,0.00033036579372947017
5608,11217,5608,16825,4.198507785797119,0.0002645190594421365
5614,11229,5614,16843,4.202810764312744,0.0002060270926449448
5619,11239,5619,16858,4.2058937549591064,0.00016289851646433817
5625,11251,5625,16876,4.210831880569458,0.00011787108962835191
5631,11263,5631,16894,4.215737819671631,8.016300455437886e-05
5636,11273,5636,16909,4.219132900238037,5.4310857080963615e-05
5642,11285,5642,16927,4.222700834274292,2.9943128538434394e-05
5648,11297,5648,16945,4.22621488571167,1.2794346389455313e-05
5653,11307,5653,16960,4.229109048843384,3.981476197623124e-06
5659,11319,5659,16978,4.2325828075408936,7.15007217877428e-09


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.001032114028930664,2181.4194943796983
2002,2003,2002,4005,2.966780185699463,59.063444236102214
4004,4005,4004,8009,5.555600166320801,53.10730164883603
6006,6007,6006,12013,7.849394083023071,50.21336123158744
8008,8009,8008,16017,10.164947032928467,47.8494876308398
10010,10011,10010,20021,12.66627812385559,45.73338437039615
12012,12013,12012,24025,15.117233276367188,43.80213242083164
14014,14015,14014,28029,17.606956005096436,42.02663547953284
16016,16017,16016,32033,20.53499126434326,40.38770314813041
18018,18019,18018,36037,22.705068111419678,38.870672513610316
20020,20021,20020,40041,25.33299708366394,37.46332494316175
22022,22023,22022,44045,27.550679206848145,36.15490131437582
24024,24025,24024,48049,29.69358801841736,34.935646044907344
26026,26027,26026,52053,31.895568132400513,33.79662211954178
28028,28029,28028,56057,34.087729930877686,32.72965306120659
30030,30031,30030,60061,36.28276205062866,31.727311024429582
32032,32033,32032,64065,38.48111319541931,30.78290970167336
34034,34035,34034,68069,40.65879702568054,29.890484826944885
36036,36037,36036,72073,42.76422309875488,29.044758501028582
38038,38039,38038,76077,45.023120164871216,28.24108999942746
40040,40041,40040,80081,47.22663712501526,27.475417962206166
42042,42043,42042,84085,49.494938135147095,26.74419888149555
44044,44045,44044,88089,51.70404624938965,26.044345854958692
46046,46047,46046,92093,53.87692904472351,25.373170376284634
48048,48049,48048,96097,56.020230293273926,24.728328837686604
50050,50051,50050,100101,58.1987841129303,24.10777455747234
52052,52053,52052,104105,60.37129497528076,23.50971553548061
54054,54055,54054,108109,62.64399790763855,22.932577745933713
56056,56057,56056,112113,64.84451627731323,22.374973550532786
58058,58059,58058,116117,67.07564330101013,21.83567470537514
60060,60061,60060,120121,69.24432325363159,21.313589403281412
62062,62063,62062,124125,71.40091109275818,20.807742808159674
64064,64065,64064,128129,73.55668306350708,20.317260579029607
66066,66067,66066,132133,75.66166615486145,19.841354934348146
68068,68069,68068,136137,77.8868260383606,19.379312863610267
70070,70071,70070,140141,80.0694031715393,18.930486147815373
72072,72073,72072,144145,82.2739908695221,18.49428290057699
74074,74075,74074,148149,84.44458293914795,18.070169126264545
76076,76077,76076,152153,86.5980532169342,17.657637363636468
78078,78079,78078,156157,88.7101981639862,17.25622437570769
80080,80081,80080,160161,90.87451219558716,16.865501709786486
82082,82083,82082,164165,93.01063013076782,16.485070475632256
84084,84085,84084,168169,95.23677802085876,16.114558070234352
86086,86087,86086,172173,97.42873501777649,15.75361535636614
88088,88089,88088,176177,99.59606504440308,15.401914225278233
90090,90091,90090,180181,101.73148012161255,15.059145485233444
92092,92093,92092,184185,103.86776494979858,14.72501702701561
94094,94095,94094,188189,106.0079140663147,14.399252225397959
96096,96097,96096,192193,108.18506026268005,14.081588542074883
98098,98099,98098,196197,110.60195827484131,13.771776300995953
100100,100101,100100,200201,113.03631591796875,13.469577611585123
102102,102103,102102,204205,115.44395399093628,13.17476541907979
104104,104105,104104,208209,117.67642903327942,12.88712266440541
106106,106107,106106,212213,119.83737111091614,12.606441538636886
108108,108109,108108,216217,121.98102307319641,12.332522819321525
110110,110111,110110,220221,124.1361391544342,12.06517527780477
112112,112113,112112,224225,126.59023904800415,11.804215148270714
114114,114115,114114,228229,128.91676497459412,11.54946565053956
116116,116117,116116,232233,131.60820198059082,11.300756559786805
118118,118119,118118,236237,133.79722905158997,11.057923817308279
120120,120121,120120,240241,136.0001220703125,10.820809177260571
122122,122123,122122,244245,138.7726891040802,10.589259885006186
124124,124125,124124,248249,141.38688015937805,10.363128383281264
126126,126127,126126,252253,143.83098602294922,10.14227204291933
128128,128129,128128,256257,146.89123106002808,9.926552915296725
130130,130131,130130,260261,149.60768508911133,9.715837504048181
132132,132133,132132,264265,152.0485360622406,9.509996553932865
134134,134135,134134,268269,154.80645608901978,9.308904855007881
136136,136137,136136,272273,157.39810729026794,9.112441060522656
138138,138139,138138,276277,160.0643870830536,8.920487517157426
140140,140141,140140,280281,162.4995629787445,8.732930106419076
142142,142143,142142,284285,165.007404088974,8.54965809616749
144144,144145,144144,288289,167.21952509880066,8.37056400138431
146146,146147,146146,292293,169.60943698883057,8.195543453415553
148148,148149,148148,296297,172.25153994560242,8.024495077019651
150150,150151,150150,300301,175.16075491905212,7.857320374633105
152152,152153,152152,304305,177.3848729133606,7.693923617337191
154154,154155,154154,308309,179.61347723007202,7.534211742061757
156156,156157,156156,312313,181.94244003295898,7.378094254606026
158158,158159,158158,316317,184.35407900810242,7.225483138091022
160160,160161,160160,320321,186.59959197044373,7.076292766483675
162162,162163,162162,324325,189.09044194221497,6.930439822854623
164164,164165,164164,328329,192.03437328338623,6.78784322204433
166166,166167,166166,332333,194.2692151069641,6.648424037434552
168168,168169,168168,336337,196.50883889198303,6.512105431524105
170170,170171,170170,340341,198.75022530555725,6.378812590034045
172172,172173,172172,344345,202.32450795173645,6.248472659269169
174174,174175,174174,348349,204.89441013336182,6.121014686484273
176176,176177,176176,352353,208.41334295272827,5.996369563019698
178178,178179,178178,356357,210.52745509147644,5.874469969982442
180180,180181,180180,360361,212.75950813293457,5.755250326269106
182182,182183,182182,364365,215.12861609458923,5.638646738749344
184184,184185,184184,368369,217.24889492988586,5.524596954430876
186186,186187,186186,372373,219.44216012954712,5.413040314465661
188188,188189,188188,376377,221.654620885849,5.30391770984977
190190,190191,190190,380381,224.8390121459961,5.197171538702719
192192,192193,192192,384385,227.77209901809692,5.092745665014263
194194,194195,194194,388389,230.26854014396667,4.990585378763285
196196,196197,196196,392393,232.76904821395874,4.890637357326
198198,198199,198198,396397,235.11821699142456,4.7928496280947
200200,200201,200200,400401,237.4797420501709,4.697171532244624
202202,202203,202202,404405,239.7732961177826,4.603553689585397
204204,204205,204204,408409,242.01655101776123,4.511947964449178
206206,206207,206206,412413,244.24516201019287,4.422307432564139
208208,208209,208208,416417,246.48767518997192,4.3345863488736995
210210,210211,210210,420421,248.69043517112732,4.24874011626207
212212,212213,212212,424425,250.94519209861755,4.16472525515303
214214,214215,214214,428429,253.33358216285706,4.082499373947712
216216,216217,216216,432433,255.5663559436798,4.002021140275247
218218,218219,218218,436437,258.05944204330444,3.9232502530285274
220220,220221,220220,440441,260.4791522026062,3.846147415157816
222222,222223,222222,444445,262.77548122406006,3.7706743072042173
224224,224225,224224,448449,265.01763820648193,3.6967935615456327
226226,226227,226226,452453,267.1816201210022,3.624468737338475
228228,228229,228228,456457,269.40205001831055,3.5536642961332063
230230,230231,230230,460461,271.57134318351746,3.484345578146417
232232,232233,232232,464465,273.80611419677734,3.416478779171598
234234,234235,234234,468469,276.0877401828766,3.3500309281097316
236236,236237,236236,472473,278.25258016586304,3.284969865105836
238238,238239,238238,476477,280.52464413642883,3.221264220272815
240240,240241,240240,480481,282.8376500606537,3.158883392989651
242242,242243,242242,484485,285.02022314071655,3.0977975317556457
244244,244245,244244,488489,287.16080808639526,3.037977514591148
246246,246247,246246,492493,289.50498509407043,2.9793949299631777
248248,248249,248248,496497,291.9288709163666,2.9220220582307093
250250,250251,250250,500501,294.11228919029236,2.865831853589043
252252,252253,252252,504505,296.36933398246765,2.8107979265035965
254254,254255,254254,508509,298.60532999038696,2.7568945266195897
256256,256257,256256,512513,300.79305601119995,2.704096526134549
258258,258259,258258,516517,302.974246263504,2.6523794036222625
260260,260261,260260,520521,305.16347908973694,2.6017192282943142
262262,262263,262262,524525,307.31700921058655,2.552092644690674
264264,264265,264264,528529,309.5170922279358,2.50347685778479
266266,266267,266266,532533,313.76140117645264,2.455849618493744
268268,268269,268268,536537,317.36070919036865,2.4091892095813137
270270,270271,270270,540541,320.5915882587433,2.3634744319451784
272272,272273,272272,544545,323.517117023468,2.31868459127611
274274,274275,274274,548549,326.5876512527466,2.274799485079825
276276,276277,276276,552553,329.4556291103363,2.2317993900502415
278278,278279,278278,556557,331.85805106163025,2.1896650497884593
280280,280281,280280,560561,334.7219588756561,2.14837766285234
282282,282283,282282,564565,337.25730991363525,2.10791887113146
284284,284285,284284,568569,339.8537690639496,2.0682707485382252
286286,286287,286286,572573,342.5423891544342,2.029415790004464
288288,288289,288288,576577,344.88647508621216,1.9913369007770143
290290,290291,290290,580581,347.1361060142517,1.9540173860015102
292292,292293,292292,584585,349.54904413223267,1.9174409405923143
294294,294295,294294,588589,351.8588001728058,1.8815916393691623
296296,296297,296296,592593,354.25594902038574,1.846453927468474
298298,298299,298298,596597,356.78024196624756,1.8120126110067076
300300,300301,300300,600601,359.0993900299072,1.7782528479995108
302302,302303,302302,604605,362.50561809539795,1.7451601395231364
304304,304305,304304,608609,365.50804829597473,1.7127203211159667
306306,306307,306306,612613,368.8825442790985,1.6809195544086606
308308,308309,308308,616617,371.7179400920868,1.649744318980197
310310,310311,310310,620621,374.2357749938965,1.6191814044321973
312312,312313,312312,624625,376.7801320552826,1.589217902676296
314314,314315,314314,628629,379.1017951965332,1.5598412004251259
316316,316317,316316,632633,381.4930970668793,1.5310389718870283
318318,318319,318318,636637,383.7626540660858,1.5027991716531233
320320,320321,320320,640641,385.8909361362457,1.4751100277748037
322322,322323,322322,644645,388.1316111087799,1.4479600350260853
324324,324325,324324,648649,390.23581409454346,1.421337948342284
326326,326327,326326,652653,392.3359749317169,1.3952327764362735
328328,328329,328328,656657,394.387332201004,1.3696337755795867
330330,330331,330330,660661,396.56231927871704,1.3445304435513208
332332,332333,332332,664665,399.5133922100067,1.3199125137450665
334334,334335,334334,668669,401.75457406044006,1.295769949431019
336336,336337,336336,672673,404.1871690750122,1.2720929381697488
338338,338339,338338,676677,406.8348820209503,1.2488718863706936
340340,340341,340340,680681,409.29335927963257,1.226097413996854
342342,342343,342342,684685,411.64442706108093,1.203760349403865
344344,344345,344344,688689,413.97056698799133,1.1818517243169708
346346,346347,346346,692693,416.10920119285583,1.1603627689365794
348348,348349,348348,696697,418.27911710739136,1.1392849071742148
350350,350351,350350,700701,420.4157431125641,1.1186097520084104
352352,352353,352352,704705,422.46865725517273,1.0983291009639515
354354,354355,354354,708709,424.5550420284271,1.0784349317071928
356356,356357,356356,712713,426.6414852142334,1.0589193977549485
358358,358359,358358,716717,429.53977131843567,1.039774824293545
360360,360361,360360,720721,432.0335569381714,1.0209937041072408
362362,362363,362362,724725,434.79177713394165,1.0025686936089642
364364,364365,364364,728729,437.32297921180725,0.9844926089753017
366366,366367,366366,732733,439.71326518058777,0.966758422377552
368368,368369,368368,736737,441.91686511039734,0.9493592583115742
370370,370371,370370,740741,444.1623430252075,0.9322883900197212
372372,372373,372372,744745,446.28526520729065,0.9155392360046335
374374,374375,374374,748749,448.57410526275635,0.8991053566307983
376376,376377,376376,752753,451.5341761112213,0.8829804508133066
378378,378379,378378,756757,454.25962805747986,0.8671583527881239
380380,380381,380380,760761,456.40905117988586,0.8516330289678535
382382,382383,382382,764765,458.76431703567505,0.8363985748720779
384384,384385,384384,768769,461.1304440498352,0.8214492121387593
386386,386387,386386,772773,463.4117000102997,0.8067792856083997
388388,388389,388388,776777,465.77326226234436,0.7923832604818699
390390,390391,390390,780781,467.96668910980225,0.7782557195492927
392392,392393,392392,784785,470.1970839500427,0.7643913604886166
394394,394395,394394,788789,472.3408451080322,0.7507849932305817
396396,396397,396396,792793,474.4171509742737,0.7374315373888294
398398,398399,398398,796797,477.0116720199585,0.7243260197553809
400400,400401,400400,800801,479.5989282131195,0.711463571857621
402402,402403,402402,804805,481.9451861381531,0.698839427573148
404404,404405,404404,808809,484.015013217926,0.6864489208076066
406406,406407,406406,812813,486.096009016037,0.6742874832262942
408408,408409,408408,816817,488.66506695747375,0.6623506420430658
410410,410411,410410,820821,491.86006808280945,0.6506340178628989
412412,412413,412412,824825,494.0011692047119,0.6391333225776634
414414,414415,414414,828829,496.2203571796417,0.6278443573118011
416416,416417,416416,832833,498.839182138443,0.6167630104214368
418418,418419,418418,836837,500.94674825668335,0.6058852555371459
420420,420421,420420,840841,503.62285113334656,0.5952071496592453
422422,422423,422422,844845,506.3993110656738,0.5847248312956026
424424,424425,424424,848849,508.78658723831177,0.5744345186463988
426426,426427,426426,852853,511.61372208595276,0.5643325078312955
428428,428429,428428,856857,514.0317921638489,0.5544151711605991
430430,430431,430430,860861,516.6100301742554,0.5446789554475799
432432,432433,432432,864865,519.3004331588745,0.5351203803604676
434434,434435,434434,868869,522.1640419960022,0.5257360368148056
436436,436437,436436,872873,525.1935660839081,0.5165225854032087
438438,438439,438438,876877,527.81982421875,0.5074767548641148
440440,440441,440440,880881,530.2431533336639,0.4985953405853252
442442,442443,442442,884885,532.6692931652069,0.4898752031440381
444444,444445,444444,888889,535.0900390148163,0.4813132668813296
446446,446447,446446,892893,538.1379721164703,0.47290651850994436
448448,448449,448448,896897,540.496856212616,0.46465200575494237
450450,450451,450450,900901,542.7915141582489,0.45654683602754176
452452,452453,452452,904905,545.2565350532532,0.44858817512783844
454454,454455,454454,908909,547.6703312397003,0.44077324598094947
456456,456457,456456,912913,550.0684130191803,0.43309932739941814
458458,458459,458458,916917,552.6427421569824,0.4255637528784746
460460,460461,460460,920921,554.847540140152,0.4181639094148295
462462,462463,462462,924925,557.2431969642639,0.41089723635650444
464464,464465,464464,928929,559.6153690814972,0.40376122427846894
466466,466467,466466,932933,561.9007701873779,0.3967534138831752
468468,468469,468468,936937,564.1356780529022,0.3898713949286048
470470,470471,470470,940941,566.3571252822876,0.3831128051790529
472472,472473,472472,944945,568.5638320446014,0.37647532938092354
474474,474475,474474,948949,570.7859442234039,0.3699566982629676
476476,476477,476476,952953,573.0472812652588,0.3635546875578939
478478,478479,478478,956957,575.5159711837769,0.3572671170476269
480480,480481,480480,960961,577.9671061038971,0.3510918496294835
482482,482483,482482,964965,580.2509713172913,0.3450267904050861
484484,484485,484484,968969,583.2527549266815,0.3390698857879215
486486,486487,486486,972973,585.6153380870819,0.3332191226335226
488488,488489,488488,976977,588.2054400444031,0.3274725273877266
490490,490491,490490,980981,590.6776719093323,0.3218281652547148
492492,492493,492492,984985,593.2686469554901,0.3162841393842655
494494,494495,494494,988989,595.7541880607605,0.310838590076969
496496,496497,496496,992993,598.1670432090759,0.30548969400774695
498498,498499,498498,996997,600.2722702026367,0.3002356634659691
500501,500502,500501,1001003,602.4144051074982,0.29507219071115287
502503,502504,502503,1005007,604.568253993988,0.29000271208440154
504505,504506,504505,1009011,606.7222011089325,0.2850229413691068
506507,506508,506507,1013015,608.8292701244354,0.2801312260719442
508509,508510,508509,1017019,610.9498591423035,0.2753259457655304
510511,510512,510511,1021023,613.08837723732,0.27060551142528766
512513,512514,512513,1025027,615.2021141052246,0.26596836478120167
514515,514516,514515,1029031,617.5813410282135,0.2614129776837899
516517,516518,516517,1033035,620.1208620071411,0.2569378514847358
518519,518520,518519,1037039,622.9683611392975,0.2525415164303695
520521,520522,520521,1041043,625.6705989837646,0.24822253106935932
522523,522524,522523,1045047,628.2865490913391,0.24397948167222694
524525,524526,524525,1049051,630.8839681148529,0.23981098166598258
526527,526528,526527,1053055,633.6639602184296,0.23571567107740066
528529,528530,528529,1057059,636.2872068881989,0.23169221599289358
530531,530532,530531,1061063,638.8301079273224,0.2277393080261163
532533,532534,532533,1065067,641.1171400547028,0.22385566380046384
534535,534536,534535,1069071,643.8871450424194,0.2200400244408911
536537,536538,536537,1073075,646.5402691364288,0.2162911550769877
538539,538540,538539,1077079,649.180822134018,0.21260784435798996
540541,540542,540541,1081083,651.5867280960083,0.20898890397711511
542543,542544,542543,1085087,653.8452880382538,0.20543316820624113
544545,544546,544545,1089091,656.3239450454712,0.2019394934416141
546547,546548,546547,1093095,658.9532012939453,0.1985067577584232
548549,548550,548549,1097099,661.4691121578217,0.19513386047560743
550551,550552,550551,1101103,664.1425778865814,0.19181972172827955
552553,552554,552553,1105107,666.8064570426941,0.18856328205367845
554555,554556,554555,1109111,669.3785312175751,0.1853635019797366
556557,556558,556557,1113115,671.9685711860657,0.18221936162785823
558559,558560,558559,1117119,674.4244260787964,0.17912986032138178
560561,560562,560561,1121123,677.02783203125,0.17609401620313747
562563,562564,562563,1125127,679.674751996994,0.1731108658610765
564565,564566,564565,1129131,682.1251521110535,0.17017946396197203
566567,566568,566567,1133135,684.7328860759735,0.16729888289319206
568569,568570,568569,1137139,687.8198232650757,0.1644682124101564
570571,570572,570571,1141143,690.5205190181732,0.1616865592945942
572573,572574,572573,1145147,693.7662301063538,0.1589530470172349
574575,574576,574575,1149151,696.3028430938721,0.1562668154089124
576577,576578,576577,1153155,698.3969120979309,0.153627020337467
578579,578580,578579,1157159,701.1206951141357,0.1510328333929465
580581,580582,580581,1161163,703.1323680877686,0.14848344157883275
582583,582584,582583,1165167,705.1990909576416,0.14597804700827055
584585,584586,584585,1169171,707.2402591705322,0.14351586660961857
586587,586588,586587,1173175,709.2788002490997,0.1410961318357522
588589,588590,588589,1177179,711.4976511001587,0.13871808837905064
590591,590592,590591,1181183,713.8107891082764,0.13638099589547892
592593,592594,592593,1185187,716.1574981212616,0.13408412773117107
594595,594596,594595,1189191,718.6747169494629,0.13182677065503867
596597,596598,596597,1193195,721.1525082588196,0.1296082245995649
598599,598600,598599,1197199,723.9155530929565,0.12742780240364482
600601,600602,600601,1201203,726.1070892810822,0.12528482956338394
602603,602604,602603,1205207,728.2534899711609,0.12317864398551137
604605,604606,604605,1209211,730.4537391662598,0.12110859574852384
606607,606608,606607,1213215,732.6578271389008,0.1190740468664444
608609,608610,608609,1217219,734.8751220703125,0.11707437105951612
610611,610612,610611,1221223,737.2151391506195,0.115108953526601
612613,612614,612613,1225227,739.4285209178925,0.11317719072712862
614615,614616,614615,1229231,741.552402973175,0.11127849016156688
616617,616618,616617,1233235,743.8576619625092,0.10941227016076027
618619,618620,618619,1237239,746.3246359825134,0.10757795967845141
620621,620622,620621,1241243,748.6019721031189,0.10577499808687207
622623,622624,622623,1245247,751.0790269374847,0.10400283497756391
624625,624626,624625,1249251,753.2712881565094,0.10226092996595071
626627,626628,626627,1253255,755.4270551204681,0.10054875250079931
628629,628630,628629,1257259,757.788407087326,0.09886578167493099
630631,630632,630631,1261263,760.0445330142975,0.0972115060434362
632633,632634,632633,1265267,762.2954759597778,0.09558542344188936
634635,634636,634635,1269271,764.518590927124,0.09398704081081632
636637,636638,636637,1273275,766.7221939563751,0.09241587402289042
638639,638640,638639,1277279,768.9942591190338,0.09087144771331168
640641,640642,640641,1281283,771.2260801792145,0.08935329511405143
642643,642644,642643,1285287,773.3898251056671,0.08786095789014325
644645,644646,644645,1289291,775.5959720611572,0.08639398598188563
646647,646648,646647,1293295,777.776976108551,0.0849519374474994
648649,648650,648649,1297299,779.9323709011078,0.08353437831055999
650651,650652,650651,1301303,782.1461429595947,0.08214088240924866
652653,652654,652653,1305307,784.327455997467,0.08077103124969653
654655,654656,654655,1309311,786.6046900749207,0.07942441386273913
656657,656658,656657,1313315,788.7806122303009,0.07810062666055728
658659,658660,658659,1317319,790.9917030334473,0.07679927330048031
660661,660662,660661,1321323,793.1728811264038,0.07551996454719756
662663,662664,662663,1325327,795.3470332622528,0.07426231814110906
664665,664666,664665,1329331,797.5549912452698,0.0730259586672446
666667,666668,666667,1333335,799.7429940700531,0.07181051742782074
668669,668670,668669,1337339,801.9985952377319,0.07061563231673063
670671,670672,670671,1341343,804.3244171142578,0.06944094769573894
672673,672674,672673,1345347,806.8258621692657,0.06828611427590658
674675,674676,674675,1349351,809.315446138382,0.06715078899776472
676677,676678,676677,1353355,811.6431400775909,0.06603463491660477
678679,678680,678679,1357359,813.9129521846771,0.06493732108799577
680681,680682,680681,1361363,816.2440309524536,0.06385852245773549
682683,682684,682683,1365367,818.4847590923309,0.06279791975134685
684685,684686,684685,1369371,820.7031071186066,0.061755199368121794
686687,686688,686687,1373375,823.0979270935059,0.06073005327596093
688689,688690,688689,1377379,825.4712841510773,0.05972217890791853
690691,690692,690691,1381383,827.7605950832367,0.05873127906215814
692693,692694,692693,1385387,830.1328990459442,0.05775706180236284
694695,694696,694695,1389391,832.234708070755,0.056799240361328884
696697,696698,696697,1393395,834.3588349819183,0.05585753304501395
698699,698700,698699,1397399,836.5266120433807,0.05493166314010978
700701,700702,700701,1401403,838.6907730102539,0.05402135882229686
702703,702704,702703,1405407,840.9185132980347,0.05312635306597713
704705,704706,704705,1409411,843.2238771915436,0.05224638355684874
706707,706708,706707,1413415,845.5249762535095,0.05138119260584517
708709,708710,708709,1417419,847.5926380157471,0.05053052706375638
710711,710712,710711,1421423,849.6791019439697,0.04969413823857849
712713,712714,712713,1425427,851.8270599842072,0.048871781814114
714715,714716,714715,1429431,853.9907221794128,0.04806321777004996
716717,716718,716717,1433435,856.6775801181793,0.047268210303855085
718719,718720,718719,1437439,858.7679522037506,0.046486527753245355
720721,720722,720721,1441443,860.8425831794739,0.04571794252160544
722723,722724,722723,1445447,862.8837549686432,0.044962231003751185
724725,724726,724725,1449451,864.9471220970154,0.04421917351328375
726727,726728,726727,1453455,867.0846221446991,0.0434885542115353
728729,728730,728729,1457459,869.2284271717072,0.042770161037537946
730731,730732,730731,1461463,871.2465662956238,0.042063785640038986
732733,732734,732733,1465467,873.3330292701721,0.041369223310084635
734735,734736,734735,1469471,875.4164271354675,0.04068627291496796
736737,736738,736737,1473475,877.5082471370697,0.04001473683342738
738739,738740,738739,1477479,879.5951859951019,0.03935442089289154
740741,740742,740741,1481483,881.6303060054779,0.03870513430661049
742743,742744,742743,1485487,883.7168691158295,0.03806668961271953
744745,744746,744745,1489491,885.775876045227,0.037438902614781
746747,746748,746747,1493495,887.9950411319733,0.03682159232198501
748749,748750,748749,1497499,890.612909078598,0.036214580892647064
750751,750752,750751,1501503,893.141948223114,0.03561769357679623
752753,752754,752753,1505507,895.727203130722,0.035030758661150685
754755,754756,754755,1509511,898.098776102066,0.03445360741409331
756757,756758,756757,1513515,900.2966148853302,0.033886074032693614
758759,758760,758759,1517519,902.5962901115417,0.03332799558984334
760761,760762,760761,1521523,905.2670841217041,0.03277921198287004
762763,762764,762763,1525527,907.5089871883392,0.03223956588351484
764765,764766,764765,1529531,909.860472202301,0.03170890268734183
766767,766768,766767,1533535,912.618674993515,0.031187070465989564
768769,768770,768769,1537539,914.8732950687408,0.03067391991896784
770771,770772,770771,1541543,916.9125740528107,0.03016930432670506
772773,772774,772773,1545547,919.0380811691284,0.029673079504732414
774775,774776,774775,1549551,921.8588643074036,0.029185103758777586
776777,776778,776777,1553555,924.4153161048889,0.028705237839858455
778779,778780,778779,1557559,927.3115820884705,0.028233344901195778
780781,780782,780781,1561563,929.8621001243591,0.027769290455125883
782783,782784,782783,1565567,932.0543532371521,0.027312942332628154
784785,784786,784785,1569571,934.2613971233368,0.026864170639328222
786787,786788,786787,1573575,936.4692580699921,0.026422847718208686
788789,788790,788789,1577579,938.6023008823395,0.025988848108113416
790791,790792,790791,1581583,941.0866980552673,0.02556204850566246
792793,792794,792793,1585587,944.0780611038208,0.02514232772671221
794795,794796,794795,1589591,946.26806807518,0.024729566668838743
796797,796798,796797,1593595,948.3858041763306,0.024323648274503284
798799,798800,798799,1597599,950.5385799407959,0.023924457495695606
800801,800802,800801,1601603,952.6523950099945,0.023531881257554232
802803,802804,802803,1605607,954.7293410301208,0.023145808423805647
804805,804806,804805,1609611,956.9053182601929,0.022766129762885612
806807,806808,806807,1613615,959.1583271026611,0.022392737914174177
808809,808810,808809,1617619,961.3118810653687,0.022025527355367558
810811,810812,810811,1621623,963.4311311244965,0.021664394369167894
812813,812814,812813,1625627,965.5568602085114,0.02130923701292886
814815,814816,814815,1629631,967.7257039546967,0.020959955086823356
816817,816818,816817,1633635,969.8346750736237,0.020616450102806994
818819,818820,818819,1637639,971.9858272075653,0.020278625255627958
820821,820822,820821,1641643,974.0967121124268,0.01994638539213156
822823,822824,822823,1645647,976.1666638851166,0.019619636983406963
824825,824826,824825,1649651,978.2901451587677,0.01929828809556966
826827,826828,826827,1653655,980.3721480369568,0.018982248362362952
828829,828830,828829,1657659,982.4853398799896,0.01867142895730467
830831,830832,830831,1661663,984.5959103107452,0.018365742567084453
832833,832834,832833,1665667,986.6680619716644,0.018065103365302093
834835,834836,834835,1669671,989.3436269760132,0.017769426986092185
836837,836838,836837,1673675,991.9849779605865,0.017478630498430903
838839,838840,838839,1677679,994.5866351127625,0.017192632381920703
840841,840842,840841,1681683,997.1054179668427,0.01691135250212028
842843,842844,842843,1685687,999.6857581138611,0.016634712085192405
844845,844846,844845,1689691,1002.609503030777,0.01636263369596236
846847,846848,846847,1693695,1005.2246861457825,0.01609504121313421
848849,848850,848849,1697699,1008.1062841415405,0.015831859807803994
850851,850852,850851,1701703,1010.4697751998901,0.0155730159194718
852853,852854,852853,1705707,1012.6467342376709,0.015318437235691817
854855,854856,854855,1709711,1014.7478630542755,0.015068052669107601
856857,856858,856857,1713715,1017.048201084137,0.014821792336761064
858859,858860,858859,1717719,1019.8612680435181,0.014579587538833039
860861,860862,860861,1721723,1022.4068241119385,0.014341370739316517
862863,862864,862863,1725727,1024.963278055191,0.014107075544075087
864865,864866,864865,1729731,1027.6632270812988,0.013876636682539356
866867,866868,866867,1733735,1030.1756439208984,0.013649989987357003
868869,868870,868869,1737739,1032.759693145752,0.0134270723760892
870871,870872,870871,1741743,1035.3606631755829,0.013207821831883848
872873,872874,872873,1745747,1038.0130739212036,0.012992177385171999
874875,874876,874875,1749751,1040.3194539546967,0.012780079095932706
876877,876878,876877,1753755,1042.6850340366364,0.012571468035730504
878879,878880,878879,1757759,1044.961207151413,0.012366286269866578
880881,880882,880881,1761763,1047.1586701869965,0.01216447684078048
882883,882884,882883,1765767,1049.973295211792,0.011965983751338172
884885,884886,884885,1769771,1052.3949902057648,0.011770751948006364
886887,886888,886887,1773775,1054.671019077301,0.011578727304140557
888889,888890,888889,1777779,1057.156939983368,0.01138985660486469
890891,890892,890891,1781783,1059.5092091560364,0.01120408753126867
892893,892894,892893,1785787,1061.933737039566,0.011021368644833274
894895,894896,894895,1789791,1064.3290202617645,0.010841649371513995
896897,896898,896897,1793795,1066.5822882652283,0.0106648799891218
898899,898900,898899,1797799,1068.6624991893768,0.010491011610042733
900901,900902,900901,1801803,1071.4331421852112,0.010319996168391299
902903,902904,902903,1805807,1073.4621441364288,0.010151786406481733
904905,904906,904905,1809811,1075.6359889507294,0.00998633585936659
906907,906908,906907,1813815,1077.9658529758453,0.009823598842672254
908909,908910,908909,1817819,1080.3561401367188,0.009663530438274393
910911,910912,910911,1821823,1082.4761989116669,0.009506086481678722
912913,912914,912913,1825827,1085.3722989559174,0.009351223549288079
914915,914916,914915,1829831,1087.3967821598053,0.009198898945442124
916917,916918,916917,1833835,1089.4103980064392,0.009049070689911787
918919,918920,918919,1837839,1091.630527973175,0.008901697505962147
920921,920922,920921,1841843,1093.6706221103668,0.0087567388077332
922923,922924,922923,1845847,1095.7313861846924,0.008614154689894349
924925,924926,924925,1849851,1097.8299350738525,0.008473905914115676
926927,926928,926927,1853855,1099.9027903079987,0.008335953899404558
928929,928930,928929,1857859,1102.2150809764862,0.008200260709372742
930931,930932,930931,1861863,1104.4630799293518,0.008066789042914024
932933,932934,932933,1865867,1106.6975700855255,0.007935502221812385
934935,934936,934935,1869871,1109.0215220451355,0.00780636418130598
936937,936938,936937,1873875,1111.5220999717712,0.00767933945905952
938939,938940,938939,1877879,1113.8647191524506,0.0075543931851598245
940941,940942,940941,1881883,1116.0137732028961,0.007431491071770324
942943,942944,942943,1885887,1118.8539080619812,0.00731059940335399
944945,944946,944945,1889891,1121.2118940353394,0.007191685027692074
946947,946948,946947,1893895,1123.3735501766205,0.007074715344742799
948949,948950,948949,1897899,1126.5753030776978,0.006959658298910654
950951,950952,950951,1901903,1128.6262440681458,0.00684648236870089
952953,952954,952953,1905907,1130.6459510326385,0.006735156558647759
954955,954956,954955,1909911,1132.7285141944885,0.006625650388741633
956957,956958,956957,1913915,1134.7637960910797,0.006517933887948857
958959,958960,958959,1917919,1136.8002281188965,0.0064119775837525594
960961,960962,960961,1921923,1138.848158121109,0.006307752494763008
962963,962964,962963,1925927,1140.8907310962677,0.006205230121736349
964965,964966,964965,1929931,1143.015242099762,0.006104382439616529
966967,966968,966967,1933935,1145.1637082099915,0.00600518189014565
968969,968970,968969,1937939,1147.2032051086426,0.005907601372996396
970971,970972,970971,1941943,1149.9513700008392,0.00581161423872345
972973,972974,972973,1945947,1152.768984079361,0.0057171942808054155
974975,974976,974975,1949951,1155.0117061138153,0.005624315728368856
976977,976978,976977,1953955,1157.2159821987152,0.005532953238684968
978979,978980,978979,1957959,1159.4809970855713,0.005443081890120993
980981,980982,980981,1961963,1161.7263522148132,0.005354677174750577
982983,982984,982983,1965967,1164.0095889568329,0.005267714991873618
984985,984986,984985,1969971,1166.1841390132904,0.0051821716406266205
986987,986988,986987,1973975,1168.3558061122894,0.005098023813388863
988989,988990,988989,1977979,1170.5532901287079,0.005015248589643306
990991,990992,990991,1981983,1172.9630541801453,0.004933823428473261
992993,992994,992993,1985987,1175.1814489364624,0.004853726163332794
994995,994996,994995,1989991,1177.3744111061096,0.004774934995111835
996997,996998,996997,1993995,1179.6609971523285,0.004697428485314958
998999,999000,998999,1997999,1181.6047801971436,0.004621185551741291
1001001,1001002,1001001,2002003,1183.5157392024994,0.004546185460981178
1003003,1003004,1003003,2006007,1185.340496301651,0.0044724078228455255
1005005,1005006,1005005,2010011,1187.2339231967926,0.0043998325852498965
1007007,1007008,1007007,2014015,1189.1552951335907,0.0043284400276206725
1009009,1009010,1009009,2018019,1191.2916412353516,0.004258210756574954
1011011,1011012,1011011,2022023,1193.3903329372406,0.0041891256985309155
1013013,1013014,1013013,2026027,1195.2974500656128,0.004121166096751949
1015015,1015016,1015015,2030031,1197.7315571308136,0.004054313503615958
1017017,1017018,1017017,2034035,1200.1696121692657,0.00398854977731844
1019019,1019020,1019019,2038039,1202.6566331386566,0.003923857075960768
1021021,1021022,1021021,2042043,1205.022227048874,0.0038602178519795416
1023023,1023024,1023023,2046047,1207.3571710586548,0.003797614848849662
1025025,1025026,1025025,2050051,1209.8896052837372,0.003736031094035752
1027027,1027028,1027027,2054055,1212.6847710609436,0.0036754498963773585
1029029,1029030,1029029,2058059,1215.0187120437622,0.0036158548399498613
1031031,1031032,1031031,2062063,1217.3819670677185,0.0035572297796306884
1033033,1033034,1033033,2066067,1219.8088471889496,0.0034995588374613362
1035035,1035036,1035035,2070071,1222.4615380764008,0.003442826396849341
1037037,1037038,1037037,2074075,1225.1922051906586,0.0033870170997261084
1039039,1039040,1039039,2078079,1227.6991019248962,0.0033321158408625706
1041041,1041042,1041041,2082083,1230.6856219768524,0.003278107764572269
1043043,1043044,1043043,2086087,1233.4131741523743,0.0032249782598228194
1045045,1045046,1045045,2090091,1235.9054369926453,0.003172712956711621
1047047,1047048,1047047,2094095,1238.5850670337677,0.003121297722259442
1049049,1049050,1049049,2098099,1241.214122056961,0.0030707186563176947
1051051,1051052,1051051,2102103,1243.3861062526703,0.003020962088271517
1053053,1053054,1053053,2106107,1245.5323462486267,0.0029720145716964907
1055055,1055056,1055055,2110111,1247.7214159965515,0.002923862883108086
1057057,1057058,1057057,2114115,1249.7591590881348,0.002876494015595199
1059059,1059060,1059059,2118119,1252.5128371715546,0.00282989517745591
1061061,1061062,1061061,2122123,1255.5332350730896,0.002784053786626828
1063063,1063064,1063063,2126127,1258.1603379249573,0.0027389574689777874
1065065,1065066,1065065,2130131,1260.5847690105438,0.002694594053309629
1067067,1067068,1067067,2134135,1263.3566489219666,0.0026509515695352093
1069069,1069070,1069069,2138139,1265.791412115097,0.0026080182436771793
1071071,1071072,1071071,2142143,1267.9555730819702,0.002565782496048996
1073073,1073074,1073073,2146147,1269.9847249984741,0.0025242329371621963
1075075,1075076,1075075,2150151,1271.866698026657,0.0024833583651115987
1077077,1077078,1077077,2154155,1273.7627351284027,0.0024431477613688912
1079079,1079080,1079079,2158159,1275.6432461738586,0.002403590289645763
1081081,1081082,1081081,2162163,1277.4503211975098,0.0023646752906643087
1083083,1083084,1083083,2166167,1279.265370130539,0.002326392281133849
1085085,1085086,1085085,2170171,1281.0787541866302,0.002288730949771889
1087087,1087088,1087087,2174175,1282.9125530719757,0.002251681154234575
1089089,1089090,1089089,2178179,1284.7311480045319,0.0022152329194113918
1091091,1091092,1091091,2182183,1286.6131739616394,0.002179376433446123
1093093,1093094,1093093,2186187,1288.4539949893951,0.002144102046372609
1095095,1095096,1095095,2190191,1290.3001770973206,0.0021094002656809607
1097097,1097098,1097097,2194195,1292.0672430992126,0.0020752617551806907
1099099,1099100,1099099,2198199,1293.8752300739288,0.002041677331817482
1101101,1101102,1101101,2202203,1295.730278968811,0.002008637963626825
1103103,1103104,1103103,2206207,1298.1344242095947,0.0019761347659823514
1105105,1105106,1105105,2210211,1300.4348340034485,0.0019441590003452802
1107107,1107108,1107107,2214215,1302.2194011211395,0.0019127020719906795
1109109,1109110,1109109,2218219,1303.9917130470276,0.0018817555265968622
1111111,1111112,1111111,2222223,1305.9912042617798,0.001851311048540083
1113113,1113114,1113113,2226227,1307.9268670082092,0.0018213604582797416
1115115,1115116,1115115,2230231,1310.1452841758728,0.001791895711221514
1117117,1117118,1117117,2234235,1313.171308040619,0.001762908893738313
1119119,1119120,1119119,2238239,1315.751795053482,0.0017343922221471075
1121121,1121122,1121121,2242243,1317.8700122833252,0.0017063380403214978
1123123,1123124,1123123,2246247,1319.918004989624,0.0016787388176453533
1125125,1125126,1125125,2250251,1321.9880390167236,0.0016515871465117016
1127127,1127128,1127127,2254255,1324.0240271091461,0.0016248757409584869
1129129,1129130,1129129,2258259,1326.0927131175995,0.0015985974345085197
1131131,1131132,1131131,2262263,1328.169809103012,0.0015727451770999323
1133133,1133134,1133133,2266267,1330.2834491729736,0.0015473120353135528
1135135,1135136,1135135,2270271,1332.8699781894684,0.0015222911881664913
1137137,1137138,1137137,2274275,1335.5171530246735,0.0014976759268847673
1139139,1139140,1139139,2278279,1338.0107090473175,0.0014734596522885113
1141141,1141142,1141141,2282283,1340.1270589828491,0.0014496358734277237
1143143,1143144,1143143,2286287,1342.7565121650696,0.001426198204967477
1145145,1145146,1145145,2290291,1345.3038930892944,0.001403140366505795
1147147,1147148,1147147,2294295,1347.3820350170135,0.0013804561800725423
1149149,1149150,1149149,2298299,1349.4589531421661,0.0013581395691062426
1151151,1151152,1151151,2302303,1351.4581639766693,0.0013361845556119079
1153153,1153154,1153153,2306307,1353.5106310844421,0.0013145852605020991
1155155,1155156,1155155,2310311,1355.5326342582703,0.0012933358997315736
1157157,1157158,1157157,2314315,1357.540560245514,0.001272430784183598
1159159,1159160,1159159,2318319,1359.520622253418,0.0012518643175098987
1161161,1161162,1161161,2322323,1361.4573891162872,0.0012316309954485405
1163163,1163164,1163163,2326327,1363.323430299759,0.001211725402868069
1165165,1165166,1165165,2330331,1365.7264111042023,0.0011921422135401372
1167167,1167168,1167167,2334335,1368.0269210338593,0.0011728761882068284
1169169,1169170,1169169,2338339,1370.4897379875183,0.0011539221728753546
1171171,1171172,1171171,2342343,1372.653668165207,0.001135275098135935
1173173,1173174,1173173,2346347,1374.886393070221,0.0011169299771154328
1175175,1175176,1175175,2350351,1377.100203037262,0.0010988819043404874
1177177,1177178,1177177,2354355,1379.562586069107,0.0010811260543732715
1179179,1179180,1179179,2358359,1381.5869960784912,0.0010636576804472497
1181181,1181182,1181181,2362363,1383.5565462112427,0.0010464721140124311
1183183,1183184,1183183,2366367,1385.9393322467804,0.0010295647616658243
1185185,1185186,1185185,2370371,1387.9052081108093,0.0010129311053788115
1187187,1187188,1187187,2374375,1390.4403421878815,0.0009965667013602797
1189189,1189190,1189189,2378379,1392.6259450912476,0.0009804671771007634
1191191,1191192,1191191,2382383,1394.4861340522766,0.0009646282325093125
1193193,1193194,1193193,2386387,1396.5204501152039,0.0009490456371850087
1195195,1195196,1195195,2390391,1398.6646091938019,0.0009337152297348439
1197197,1197198,1197197,2394395,1400.7015731334686,0.0009186329165231655
1199199,1199200,1199199,2398399,1402.6781430244446,0.000903794670989555
1201201,1201202,1201201,2402403,1404.6853721141815,0.0008891965314887784
1203203,1203204,1203203,2406407,1407.1318790912628,0.0008748346023139675
1205205,1205206,1205205,2410411,1409.740956068039,0.0008607050494902069
1207207,1207208,1207207,2414415,1412.1557381153107,0.0008468041031619578
1209209,1209210,1209209,2418419,1414.4761452674866,0.0008331280537277053
1211211,1211212,1211211,2422423,1417.4806442260742,0.0008196732524083927
1213213,1213214,1213213,2426427,1419.9104719161987,0.0008064361101105533
1215215,1215216,1215215,2430431,1422.1335980892181,0.0007934130959483809
1217217,1217218,1217217,2434435,1424.153109073639,0.0007806007367889833
1219219,1219220,1219219,2438439,1426.132805109024,0.0007679956154333922
1221221,1221222,1221221,2442443,1428.6929259300232,0.0007555943712986846
1223223,1223224,1223223,2446447,1431.076425075531,0.000743393697916872
1225225,1225226,1225225,2450451,1433.488251209259,0.0007313903423664669
1227227,1227228,1227227,2454455,1435.740462064743,0.0007195811056135426
1229229,1229230,1229229,2458459,1437.798131942749,0.0007079628397832494
1231231,1231232,1231231,2462463,1439.955194234848,0.0006965324486145619
1233233,1233234,1233233,2466467,1442.4599533081055,0.0006852868864370976
1235235,1235236,1235235,2470471,1445.0056929588318,0.0006742231569205615
1237237,1237238,1237237,2474475,1447.1464450359344,0.0006633383122789382
1239239,1239240,1239239,2478479,1449.317491054535,0.000652629453497866
1241241,1241242,1241241,2482483,1451.6800022125244,0.0006420937273787786
1243243,1243244,1243243,2486487,1454.2637162208557,0.0006317283283578945
1245245,1245246,1245245,2490491,1457.1297662258148,0.0006215304958914203
1247247,1247248,1247247,2494495,1460.5593321323395,0.0006114975149102975
1249249,1249250,1249249,2498499,1463.4443171024323,0.0006016267138875264
1251251,1251252,1251251,2502503,1465.9618821144104,0.0005919154646107927
1253253,1253254,1253253,2506507,1468.5548601150513,0.0005823611825235275
1255255,1255256,1255255,2510511,1470.9908080101013,0.0005729613238827369
1257257,1257258,1257257,2514515,1473.650547027588,0.0005637133876916778
1259259,1259260,1259259,2518519,1476.2907168865204,0.0005546149124029398
1261261,1261262,1261261,2522523,1479.096692085266,0.0005456634769416269
1263263,1263264,1263263,2526527,1481.6561350822449,0.0005368566996821755
1265265,1265266,1265265,2530531,1484.8823070526123,0.0005281922375388604
1267267,1267268,1267267,2534535,1488.736060142517,0.000519667785852107
1269269,1269270,1269269,2538539,1492.231593132019,0.0005112810767968767
1271271,1271272,1271271,2542543,1496.312870979309,0.0005030298797237265
1273273,1273274,1273273,2546547,1499.941209077835,0.0004949120005903751
1275275,1275276,1275275,2550551,1503.53977394104,0.0004869252803700874
1277277,1277278,1277277,2554555,1507.130790233612,0.00047906759527904796
1279279,1279280,1279279,2558559,1510.557501077652,0.00047133685643530043
1281281,1281282,1281281,2562563,1512.94762301445,0.0004637310083808188
1283283,1283284,1283283,2566567,1514.7950241565704,0.0004562480293088811
1285285,1285286,1285285,2570571,1516.8727922439575,0.00044888593038194813
1287287,1287288,1287287,2574575,1519.2123410701752,0.00044164275448110857
1289289,1289290,1289289,2578579,1521.3456063270569,0.00043451657677451294
1291291,1291292,1291291,2582583,1523.487514257431,0.0004275055035805053
1293293,1293294,1293293,2586587,1526.6383502483368,0.00042060767225393647
1295295,1295296,1295295,2590591,1528.9351201057434,0.0004138212492534876
1297297,1297298,1297297,2594595,1531.3333220481873,0.00040714443252909405
1299299,1299300,1299299,2598599,1533.3683211803436,0.00040057544788396626
1301301,1301302,1301301,2602603,1535.2226121425629,0.0003941125504525189
1303303,1303304,1303303,2606607,1537.1441452503204,0.0003877540235635024
1305305,1305306,1305305,2610611,1539.1349470615387,0.0003814981783989424
1307307,1307308,1307307,2614615,1541.4024152755737,0.00037534335399413976
1309309,1309310,1309309,2618619,1543.1655659675598,0.00036928791575974174
1311311,1311312,1311311,2622623,1545.0904519557953,0.0003633302554817419
1313313,1313314,1313313,2626627,1547.074443101883,0.00035746879200360127
1315315,1315316,1315315,2630631,1549.0447742938995,0.0003517019687251377
1317317,1317318,1317317,2634635,1550.9635801315308,0.00034602825473939447
1319319,1319320,1319319,2638639,1552.968299150467,0.0003404461443778928
1321321,1321322,1321321,2642643,1554.9546301364899,0.00033495415584638977
1323323,1323324,1323323,2646647,1556.8416271209717,0.00032955083133856533
1325325,1325326,1325325,2650651,1558.7157802581787,0.00032423473680864845
1327327,1327328,1327327,2654655,1560.5555310249329,0.000319004462085104
1329329,1329330,1329329,2658659,1562.416393995285,0.00031385861893795663
1331331,1331332,1331331,2662663,1564.299203157425,0.00030879584232934576
1333333,1333334,1333333,2666667,1566.170662164688,0.00030381478848084953
1335335,1335336,1335335,2670671,1568.0013031959534,0.0002989141363514136
1337337,1337338,1337337,2674675,1569.883073091507,0.0002940925860457355
1339339,1339340,1339339,2678679,1571.8309881687164,0.00028934885858689086
1341341,1341342,1341341,2682683,1573.80921292305,0.0002846816953478992
1343343,1343344,1343343,2686687,1575.7740380764008,0.0002800898591885925
1345345,1345346,1345345,2690691,1577.6954560279846,0.0002755721319545046
1347347,1347348,1347347,2694695,1579.5538539886475,0.0002711273156137395
1349349,1349350,1349349,2698699,1581.3833620548248,0.00026675423180222424
1351351,1351352,1351351,2702703,1583.2195510864258,0.0002624517209142141
1353353,1353354,1353353,2706707,1585.134080171585,0.0002582186421022925
1355355,1355356,1355355,2710711,1587.0947360992432,0.0002540538730499975
1357357,1357358,1357357,2714715,1589.0346670150757,0.00024995631008550845
1359359,1359360,1359359,2718719,1590.9991512298584,0.0002459248668174041
1361361,1361362,1361361,2722723,1592.944435119629,0.00024195847481678356
1363363,1363364,1363363,2726727,1594.824098110199,0.00023805608259408473
1365365,1365366,1365365,2730731,1596.6850440502167,0.00023421665594014485
1367367,1367368,1367367,2734735,1598.5709431171417,0.00023043917747145315
1369369,1369370,1369369,2738739,1600.43705701828,0.00022672264640277717
1371371,1371372,1371371,2742743,1602.334319114685,0.00022306607741029438
1373373,1373374,1373373,2746747,1604.2360870838165,0.00021946850210952107
1375375,1375376,1375375,2750751,1606.2062451839447,0.00021592896700894926
1377377,1377378,1377377,2754755,1608.1424100399017,0.0002124465346469151
1379379,1379380,1379379,2758759,1610.0925822257996,0.00020902028234104364
1381381,1381382,1381381,2762763,1611.9563891887665,0.00020564930252930935
1383383,1383384,1383383,2766767,1613.869649887085,0.00020233270220160193
1385385,1385386,1385385,2770771,1615.7416172027588,0.00019906960312709998
1387387,1387388,1387387,2774775,1617.5641112327576,0.0001958591406037158
1389389,1389390,1389389,2778779,1619.4010319709778,0.00019270046504971106
1391391,1391392,1391391,2782783,1621.2066750526428,0.00018959273950258648
1393393,1393394,1393393,2786787,1623.1523940563202,0.00018653514109701064
1395395,1395396,1395395,2790791,1624.9776961803436,0.0001835268602690121
1397397,1397398,1397397,2794795,1626.7848770618439,0.0001805671005286058
1399399,1399400,1399399,2798799,1628.5825831890106,0.0001776550781187325
1401401,1401402,1401401,2802803,1630.4095571041107,0.00017479002212894557
1403403,1403404,1403403,2806807,1632.297255039215,0.00017197117426803743
1405405,1405406,1405405,2810811,1634.1866040229797,0.00016919778795454476
1407407,1407408,1407407,2814815,1636.0602900981903,0.00016646912922624324
1409409,1409410,1409409,2818819,1637.9185512065887,0.00016378447605802648
1411411,1411412,1411411,2822823,1639.8131351470947,0.00016114311756609823
1413413,1413414,1413413,2826827,1641.6922161579132,0.000158544354917467
1415415,1415416,1415415,2830831,1643.5560100078583,0.00015598750007939088
1417417,1417418,1417417,2834835,1645.3810820579529,0.00015347187650149863
1419419,1419420,1419419,2838839,1647.3131079673767,0.00015099681854735536
1421421,1421422,1421421,2842843,1649.6598629951477,0.00014856167126708897
1423423,1423424,1423423,2846847,1652.0357172489166,0.00014616579051107692
1425425,1425426,1425425,2850851,1654.6069450378418,0.00014380854190676473
1427427,1427428,1427427,2854855,1656.9496068954468,0.000141489302222908
1429429,1429430,1429429,2858859,1659.1131241321564,0.00013920745777795673
1431431,1431432,1431431,2862863,1661.1856272220612,0.0001369624048948026
1433433,1433434,1433433,2866867,1663.3521621227264,0.00013475354944603168
1435435,1435436,1435435,2870871,1665.267344236374,0.00013258030764973228
1437437,1437438,1437437,2874875,1667.2851440906525,0.00013044210402313183
1439439,1439440,1439439,2878879,1669.2208790779114,0.00012833837354264688
1441441,1441442,1441441,2882883,1671.0847821235657,0.00012626855937014625
1443443,1443444,1443443,2886887,1672.9313452243805,0.00012423211455825367
1445445,1445446,1445445,2890891,1675.135411977768,0.00012222850034504518
1447447,1447448,1447447,2894895,1677.0224840641022,0.00012025718683617015
1449449,1449450,1449449,2898899,1678.9199900627136,0.00011831765255010396
1451451,1451452,1451451,2902903,1680.8232100009918,0.00011640938498658215
1453453,1453454,1453453,2906907,1682.6538219451904,0.00011453187937604525
1455455,1455456,1455455,2910911,1684.4577751159668,0.00011268463936175976
1457457,1457458,1457457,2914915,1686.7152781486511,0.00011086717654507083
1459459,1459460,1459459,2918919,1689.408224105835,0.00010907901037171541
1461461,1461462,1461461,2922923,1691.4993040561676,0.00010731966813182225
1463463,1463464,1463463,2926927,1693.7255229949951,0.00010558868495991192
1465465,1465466,1465465,2930931,1695.792729139328,0.00010388560281171522
1467467,1467468,1467467,2934935,1697.9294950962067,0.00010220997194210213
1469469,1469470,1469469,2938939,1700.1132690906525,0.00010056134919977922
1471471,1471472,1471471,2942943,1702.2895741462708,9.893929893678433e-05
1473473,1473474,1473473,2946947,1704.5258991718292,9.734339221267874e-05
1475475,1475476,1475475,2950951,1706.5620801448822,9.577320759035501e-05
1477477,1477478,1477477,2954955,1708.3390681743622,9.42283298854818e-05
1479479,1479480,1479479,2958959,1710.267864227295,9.2708350734938e-05
1481481,1481482,1481481,2962963,1712.363652229309,9.121286882418644e-05
1483483,1483484,1483483,2966967,1714.3536930084229,8.974148852303188e-05
1485485,1485486,1485485,2970971,1716.29203414917,8.82938213635498e-05
1487487,1487488,1487487,2974975,1718.2264409065247,8.686948478953127e-05
1489489,1489490,1489489,2978979,1720.1347572803497,8.54681023838566e-05
1491491,1491492,1491491,2982983,1722.128007888794,8.408930386849534e-05
1493493,1493494,1493493,2986987,1723.9576289653778,8.27327249908194e-05
1495495,1495496,1495495,2990991,1725.8029201030731,8.139800752360316e-05
1497497,1497498,1497497,2994995,1727.6315081119537,8.00847985829023e-05
1499499,1499500,1499499,2998999,1729.4859070777893,7.879275131017494e-05
1501502,1501503,1501502,3003005,1731.3466711044312,7.75208947061401e-05
1503504,1503505,1503504,3007009,1733.230901002884,7.627016259448283e-05
1505506,1505507,1505506,3011013,1735.1465611457825,7.503958477173e-05
1507508,1507509,1507508,3015017,1737.055741071701,7.382883575246524e-05
1509510,1509511,1509510,3019021,1739.0073459148407,7.26375963040482e-05
1511512,1511513,1511512,3023025,1740.9127700328827,7.146555105919106e-05
1513514,1513515,1513514,3027029,1742.7490320205688,7.031239135812939e-05
1515516,1515517,1515516,3031033,1744.6073200702667,6.917781195170392e-05
1517518,1517519,1517518,3035037,1746.6158781051636,6.806151361615775e-05
1519520,1519521,1519520,3039041,1748.454534292221,6.696320110677334e-05
1521522,1521523,1521522,3043045,1750.2806012630463,6.588258509054867e-05
1523524,1523525,1523524,3047049,1752.0678470134735,6.481937964508688e-05
1525526,1525527,1525526,3051053,1753.8262810707092,6.377330407758564e-05
1527528,1527529,1527528,3055057,1755.6373000144958,6.274408258377662e-05
1529530,1529531,1529530,3059061,1757.4572591781616,6.173144288368348e-05
1531532,1531533,1531532,3063065,1759.2958941459656,6.073511804061127e-05
1533534,1533535,1533534,3067069,1761.0507640838623,5.9754844755843806e-05
1535536,1535537,1535536,3071073,1762.8137900829315,5.879036427813844e-05
1537538,1537539,1537538,3075077,1764.5597620010376,5.7841422062665515e-05
1539540,1539541,1539540,3079081,1766.2850601673126,5.690776765732153e-05
1541542,1541543,1541542,3083085,1767.9826109409332,5.598915402060811e-05
1543544,1543545,1543544,3087089,1769.676743030548,5.5085339567995106e-05
1545546,1545547,1545546,3091093,1771.3953459262848,5.419608487500227e-05
1547548,1547549,1547548,3095097,1773.14306807518,5.3321155860430736e-05
1549550,1549551,1549550,3099101,1774.913027048111,5.246032117156574e-05
1551552,1551553,1551552,3103105,1776.6656761169434,5.161335411685286e-05
1553554,1553555,1553554,3107109,1778.4031801223755,5.078003039216128e-05
1555556,1555557,1555556,3111113,1780.102133989334,4.996013069558103e-05
1557558,1557559,1557558,3115117,1781.7964470386505,4.9153438112625736e-05
1559560,1559561,1559560,3119121,1783.5907320976257,4.83597401625957e-05
1561562,1561563,1561562,3123125,1785.493222951889,4.757882720696216e-05
1563564,1563565,1563564,3127129,1787.4214479923248,4.681049313148833e-05
1565566,1565567,1565566,3131133,1789.334801197052,4.6054535459916224e-05
1567568,1567569,1567568,3135137,1791.1408400535583,4.531075421709829e-05
1569570,1569571,1569570,3139141,1792.793632030487,4.457895352061314e-05
1571572,1571573,1571572,3143145,1794.567548274994,4.38589399891498e-05
1573574,1573575,1573574,3147149,1796.3512959480286,4.315052399306296e-05
1575576,1575577,1575576,3151153,1798.1909050941467,4.2453518403817725e-05
1577578,1577579,1577578,3155157,1800.0123262405396,4.17677393897975e-05
1579580,1579581,1579580,3159161,1801.7844061851501,4.109300584786979e-05
1581582,1581583,1581582,3163165,1803.5241532325745,4.042913974444673e-05
1583584,1583585,1583584,3167169,1805.23423910141,3.977596611548506e-05
1585586,1585587,1585586,3171173,1806.914008140564,3.91333126117388e-05
1587588,1587589,1587588,3175177,1808.6122949123383,3.850100961244607e-05
1589590,1589591,1589590,3179181,1810.3421189785004,3.787889045270276e-05
1591592,1591593,1591592,3183185,1812.0812029838562,3.726679074134154e-05
1593594,1593595,1593594,3187189,1813.8287312984467,3.666454938411334e-05
1595596,1595597,1595596,3191193,1815.6049921512604,3.607200721944537e-05
1597598,1597599,1597598,3195197,1817.3472571372986,3.5489007927935745e-05
1599600,1599601,1599600,3199201,1819.0345001220703,3.491539791866671e-05
1601602,1601603,1601602,3203205,1820.7425711154938,3.4351025760770426e-05
1603604,1603605,1603604,3207209,1822.4176692962646,3.3795742751863145e-05
1605606,1605607,1605606,3211213,1824.1272552013397,3.3249402349611046e-05
1607608,1607609,1607608,3215217,1825.8535470962524,3.271186028541706e-05
1609610,1609611,1609610,3219221,1827.6474959850311,3.2182975019168225e-05
1611612,1611613,1611612,3223225,1829.404410123825,3.166260694342782e-05
1613614,1613615,1613614,3227229,1831.1017112731934,3.115061872449587e-05
1615616,1615617,1615616,3231233,1832.792890071869,3.0646875643469684e-05
1617618,1617619,1617618,3235237,1834.4942321777344,3.0151244686749124e-05
1619620,1619621,1619620,3239241,1836.1857540607452,2.966359500078397e-05
1621622,1621623,1621622,3243245,1837.874029159546,2.918379823313444e-05
1623624,1623625,1623624,3247249,1839.5972542762756,2.8711727736663306e-05
1625626,1625627,1625626,3251253,1841.3152530193329,2.824725879690959e-05
1627628,1627629,1627628,3255257,1843.0491580963135,2.779026942789642e-05
1629630,1629631,1629630,3259261,1844.7992839813232,2.7340638780515292e-05
1631632,1631633,1631632,3263265,1846.5282020568848,2.6898248393081303e-05
1633634,1633635,1633634,3267269,1848.2147750854492,2.6462981509212113e-05
1635636,1635637,1635636,3271273,1849.9000430107117,2.6034723646262137e-05
1637638,1637639,1637638,3275277,1851.556617975235,2.561336168582784e-05
1639640,1639641,1639640,3279281,1853.269368171692,2.5198784442181932e-05
1641642,1641643,1641642,3283285,1855.0564670562744,2.47908827759602e-05
1643644,1643645,1643644,3287289,1856.803015947342,2.4389549139414157e-05
1645646,1645647,1645646,3291293,1858.5488300323486,2.3994677690097888e-05
1647648,1647649,1647648,3295297,1860.2362110614777,2.3606164290868037e-05
1649650,1649651,1649650,3299301,1861.9211020469666,2.3223906509883818e-05
1651652,1651653,1651652,3303305,1863.6131551265717,2.284780362060701e-05
1653654,1653655,1653654,3307309,1865.326042175293,2.247775637442828e-05
1655656,1655657,1655656,3311313,1867.0220029354095,2.211366756910138e-05
1657658,1657659,1657658,3315317,1868.743940114975,2.1755440684501082e-05
1659660,1659661,1659660,3319321,1870.4870150089264,2.140298158792575e-05
1661662,1661663,1661662,3323325,1872.2034821510315,2.105619751091581e-05
1663664,1663665,1663664,3327329,1873.9001641273499,2.071499682188005e-05
1665666,1665667,1665666,3331333,1875.6092751026154,2.0379289480843e-05
1667668,1667669,1667668,3335337,1877.3090119361877,2.0048987380505423e-05
1669670,1669671,1669670,3339341,1879.0019690990448,1.9724003095689113e-05
1671672,1671673,1671672,3343345,1880.6930932998657,1.940425124757894e-05
1673674,1673675,1673674,3347349,1882.3705191612244,1.908964736685448e-05
1675676,1675677,1675676,3351353,1884.0783760547638,1.878010846212419e-05
1677678,1677679,1677678,3355357,1885.7469861507416,1.847555336098594e-05
1679680,1679681,1679680,3359361,1887.5016250610352,1.8175901118411275e-05
1681682,1681683,1681682,3363365,1889.249655008316,1.788107351785584e-05
1683684,1683685,1683684,3367369,1890.9518358707428,1.7590992456462118e-05
1685686,1685687,1685686,3371373,1892.636875152588,1.7305581422988325e-05
1687688,1687689,1687688,3375377,1894.3198790550232,1.7024765270434727e-05
1689690,1689691,1689690,3379381,1896.002748966217,1.6748470102356805e-05
1691692,1691693,1691692,3383385,1897.7161102294922,1.647662293180474e-05
1693694,1693695,1693694,3387389,1899.41011095047,1.620915213607077e-05
1695696,1695697,1695696,3391393,1901.101585149765,1.594598757037602e-05
1697698,1697699,1697698,3395397,1902.823055267334,1.5687059431002126e-05
1699700,1699701,1699700,3399401,1904.5100951194763,1.543229984690697e-05
1701702,1701703,1701702,3403405,1906.2021670341492,1.5181641515482625e-05
1703704,1703705,1703704,3407409,1907.9070799350739,1.4935018043615855e-05
1705706,1705707,1705706,3411413,1909.7510251998901,1.4692365084556513e-05
1707708,1707709,1707708,3415417,1911.7060952186584,1.4453618405241286e-05
1709710,1709711,1709710,3419421,1913.5638799667358,1.4218715023162076e-05
1711712,1711713,1711712,3423425,1915.4454991817474,1.3987593433739676e-05
1713714,1713715,1713714,3427429,1917.2445030212402,1.376019201870804e-05
1715716,1715717,1715716,3431433,1918.9384372234344,1.3536451547224715e-05
1717718,1717719,1717718,3435437,1920.6666922569275,1.3316312561073573e-05
1719720,1719721,1719720,3439441,1922.3649642467499,1.3099717307341052e-05
1721722,1721723,1721722,3443445,1923.9156880378723,1.288660894260829e-05
1723724,1723725,1723724,3447449,1925.5111560821533,1.2676930850830104e-05
1725726,1725727,1725726,3451453,1927.052983045578,1.247062823495071e-05
1727728,1727729,1727728,3455457,1928.63183426857,1.2267646525288e-05
1729730,1729731,1729730,3459461,1930.2177731990814,1.2067932175341411e-05
1731732,1731733,1731732,3463465,1931.746865272522,1.1871432434418239e-05
1733734,1733735,1733734,3467469,1933.3133072853088,1.1678096143441508e-05
1735736,1735737,1735736,3471473,1934.8658530712128,1.1487871688586893e-05
1737738,1737739,1737738,3475477,1936.4007360935211,1.130070938870631e-05
1739740,1739741,1739740,3479481,1938.0282711982727,1.1116559790025349e-05
1741742,1741743,1741742,3483485,1939.5831460952759,1.0935374234577466e-05
1743744,1743745,1743744,3487489,1941.4293291568756,1.0757105314951332e-05
1745746,1745747,1745746,3491493,1943.1087260246277,1.0581705737422453e-05
1747748,1747749,1747748,3495497,1944.7847859859467,1.0409129572508391e-05
1749750,1749751,1749750,3499501,1946.5242931842804,1.0239331345474056e-05
1751752,1751753,1751752,3503505,1948.3348460197449,1.0072265922644874e-05
1753754,1753755,1753754,3507509,1950.3266413211823,9.907889761961997e-06
1755756,1755757,1755756,3511513,1952.278911113739,9.746159435053414e-06
1757758,1757759,1757758,3515517,1953.9673871994019,9.587032423041819e-06
1759760,1759761,1759760,3519521,1955.65731716156,9.430466548110417e-06
1761762,1761763,1761762,3523525,1957.3401200771332,9.276420882997627e-06
1763764,1763765,1763764,3527529,1959.0521800518036,9.124854614128708e-06
1765766,1765767,1765766,3531533,1960.7854690551758,8.975727723736782e-06
1767768,1767769,1767768,3535537,1962.54261302948,8.829001444610185e-06
1769770,1769771,1769770,3539541,1964.368819952011,8.684636441103066e-06
1771772,1771773,1771772,3543545,1966.1872911453247,8.542595310245815e-06
1773774,1773775,1773774,3547549,1967.9393780231476,8.402840308008308e-06
1775776,1775777,1775776,3551553,1969.6801249980927,8.265334827228799e-06
1777778,1777779,1777778,3555557,1971.399343252182,8.130042488119216e-06
1779780,1779781,1779780,3559561,1973.1371490955353,7.996927479325677e-06
1781782,1781783,1781782,3563565,1975.085372209549,7.865955126362678e-06
1783784,1783785,1783784,3567569,1976.9234380722046,7.737090868431551e-06
1785786,1785787,1785786,3571573,1978.6699361801147,7.610300372107304e-06
1787788,1787789,1787788,3575577,1980.2973420619965,7.485550895580673e-06
1789790,1789791,1789790,3579581,1981.9010429382324,7.362809014921368e-06
1791792,1791793,1791792,3583585,1983.5347311496735,7.242042670441151e-06
1793794,1793795,1793794,3587589,1985.345558166504,7.123220029825461e-06
1795796,1795797,1795796,3591593,1987.0462222099304,7.006309715507086e-06
1797798,1797799,1797798,3595597,1988.9636631011963,6.89128114572668e-06
1799800,1799801,1799800,3599601,1990.9319820404053,6.778103625038057e-06
1801802,1801803,1801802,3603605,1992.834834098816,6.666747935923922e-06
1803804,1803805,1803804,3607609,1994.64133310318,6.557184406119632e-06
1805806,1805807,1805806,3611613,1996.4504640102386,6.449383931794728e-06
1807808,1807809,1807808,3615617,1998.1544930934906,6.343318659673969e-06
1809810,1809811,1809810,3619621,1999.8049499988556,6.2389603954216e-06
1811812,1811813,1811812,3623625,2001.3793451786041,6.1362816268228926e-06
1813814,1813815,1813814,3627629,2002.8955101966858,6.035255523784144e-06
1815816,1815817,1815816,3631633,2004.4107971191406,5.93585491515114e-06
1817818,1817819,1817818,3635637,2005.9221260547638,5.838054448759067e-06
1819820,1819821,1819820,3639641,2007.5356140136719,5.741827862948412e-06
1821822,1821823,1821822,3643645,2009.120796918869,5.647149805554363e-06
1823824,1823825,1823824,3647649,2010.7496840953827,5.553995606533135e-06
1825826,1825827,1825826,3651653,2012.3402812480927,5.462340482154104e-06
1827828,1827829,1827828,3655657,2013.9522140026093,5.372160330807674e-06
1829830,1829831,1829830,3659661,2015.521371126175,5.283431619318435e-06
1831832,1831833,1831832,3663665,2017.1281189918518,5.19613081451098e-06
1833834,1833835,1833834,3667669,2018.6850531101227,5.11023483795725e-06
1835836,1835837,1835836,3671673,2020.261836051941,5.025721293350216e-06
1837838,1837839,1837838,3675677,2021.8524222373962,4.942567898069683e-06
1839840,1839841,1839840,3679681,2023.44389295578,4.860752824242809e-06
1841842,1841843,1841842,3683685,2025.145387172699,4.780254357683589e-06
1843844,1843845,1843844,3687689,2026.8694820404053,4.701051238953369e-06
1845846,1845847,1845846,3691693,2028.4387941360474,4.6231227770476835e-06
1847848,1847849,1847848,3695697,2030.0026559829712,4.546448394648905e-06
1849850,1849851,1849850,3699701,2031.5526101589203,4.471008082873595e-06
1851852,1851853,1851852,3703705,2033.130112171173,4.396781605464639e-06
1853854,1853855,1853854,3707709,2034.701523065567,4.323749635659624e-06
1855856,1855857,1855856,3711713,2036.2653810977936,4.251892960382975e-06
1857858,1857859,1857858,3715717,2037.8988432884216,4.18119270761963e-06
1859860,1859861,1859860,3719721,2039.585594177246,4.111630232728203e-06
1861862,1861863,1861862,3723725,2041.223974943161,4.043187118440983e-06
1863864,1863865,1863864,3727729,2042.7847411632538,3.975845515924448e-06
1865866,1865867,1865866,3731733,2044.3540170192719,3.909587576345075e-06
1867868,1867869,1867868,3735737,2045.9130601882935,3.8443957919298555e-06
1869870,1869871,1869870,3739741,2047.4742331504822,3.780253223339969e-06
1871872,1871873,1871872,3743745,2049.041595220566,3.717142703862919e-06
1873874,1873875,1873874,3747749,2050.6147241592407,3.655047976280912e-06
1875876,1875877,1875876,3751753,2052.11971616745,3.593952328628802e-06
1877878,1877879,1877878,3755757,2053.6467850208282,3.533839844749309e-06
1879880,1879881,1879880,3759761,2055.2140889167786,3.474694835858827e-06
1881882,1881883,1881882,3763765,2056.7668731212616,3.416501272113237e-06
1883884,1883885,1883884,3767769,2058.3022091388702,3.3592443742236355e-06
1885886,1885887,1885886,3771773,2059.8407130241394,3.3029089081537677e-06
1887888,1887889,1887888,3775777,2061.3731651306152,3.247479980927892e-06
1889890,1889891,1889890,3779781,2062.848610162735,3.1929429269439424e-06
1891892,1891893,1891892,3783785,2064.322375059128,3.1392835353472037e-06
1893894,1893895,1893894,3787789,2065.8313541412354,3.0864875952829607e-06
1895896,1895897,1895896,3791793,2067.0076870918274,3.0345411232701736e-06
1897898,1897899,1897898,3795797,2068.156907081604,2.9834305905751535e-06
1899900,1899901,1899900,3799801,2069.3307390213013,2.9331425821510493e-06
1901902,1901903,1901902,3803805,2070.44411110878,2.8836637966378476e-06
1903904,1903905,1903904,3807809,2071.5464050769806,2.8349811600492103e-06
1905906,1905907,1905906,3811813,2072.6082060337067,2.787081825772475e-06
1907908,1907909,1907908,3815817,2073.6773750782013,2.73995340194233e-06
1909910,1909911,1909910,3819821,2074.726521253586,2.6935831556329504e-06
1911912,1911913,1911912,3823825,2075.783523082733,2.647959263413213e-06
1913914,1913915,1913914,3827829,2076.8744311332703,2.6030694471046445e-06
1915916,1915917,1915916,3831833,2078.1220610141754,2.558901996962959e-06
1917918,1917919,1917918,3835837,2079.645839214325,2.5154450895570335e-06
1919920,1919921,1919920,3839841,2081.208747148514,2.472687697263609e-06
1921922,1921923,1921922,3843845,2082.8361310958862,2.4306182240252383e-06
1923924,1923925,1923924,3847849,2084.442432165146,2.389225642218662e-06
1925926,1925927,1925926,3851853,2086.036999940872,2.348499037907459e-06
1927928,1927929,1927928,3855857,2087.6058270931244,2.308427838215721e-06
1929930,1929931,1929930,3859861,2089.1367700099945,2.26900147026754e-06
1931932,1931933,1931932,3863865,2090.660045146942,2.2302094748738455e-06
1933934,1933935,1933934,3867869,2092.212503194809,2.1920417339060805e-06
1935936,1935937,1935936,3871873,2093.7899510860443,2.15448801554885e-06
1937938,1937939,1937938,3875877,2095.419631242752,2.117538883794623e-06
1939940,1939941,1939940,3879881,2097.2959492206573,2.081183879454329e-06
1941942,1941943,1941942,3883885,2098.9404590129852,2.045414134954626e-06
1943944,1943945,1943944,3887889,2100.4371662139893,2.0102196458537946e-06
1945946,1945947,1945946,3891893,2101.916139125824,1.9755917719521676e-06
1947948,1947949,1947948,3895897,2103.4321250915527,1.941520849868539e-06
1949950,1949951,1949950,3899901,2104.9783141613007,1.907998353090079e-06
1951952,1951953,1951952,3903905,2106.5621631145477,1.8750149592960952e-06
1953954,1953955,1953954,3907909,2108.2790122032166,1.8425627104079467e-06
1955956,1955957,1955956,3911913,2110.070247888565,1.8106323977917782e-06
1957958,1957959,1957958,3915917,2111.641347169876,1.7792156086215982e-06
1959960,1959961,1959960,3919921,2113.223520040512,1.7483047258792794e-06
1961962,1961963,1961962,3923925,2115.1428632736206,1.7178909956783173e-06
1963964,1963965,1963964,3927929,2116.8896420001984,1.6879668010005844e-06
1965966,1965967,1965966,3931933,2118.4526829719543,1.658523842706927e-06
1967968,1967969,1967968,3935937,2119.8803782463074,1.629554958526569e-06
1969970,1969971,1969970,3939941,2121.397181034088,1.601051963007194e-06
1971972,1971973,1971972,3943945,2122.812366247177,1.573007580191188e-06
1973974,1973975,1973974,3947949,2124.5056982040405,1.5454144204340992e-06
1975976,1975977,1975976,3951953,2126.112965106964,1.518265321465151e-06
1977978,1977979,1977978,3955957,2127.463401079178,1.4915528936398914e-06
1979980,1979981,1979980,3959961,2128.877253293991,1.4652705431217328e-06
1981982,1981983,1981982,3963965,2130.407905101776,1.4394109939530608e-06
1983984,1983985,1983984,3967969,2131.7334191799164,1.41396753861045e-06
1985986,1985987,1985986,3971973,2133.2756972312927,1.388933355883637e-06
1987988,1987989,1987988,3975977,2134.526848077774,1.364301851936034e-06
1989990,1989991,1989990,3979981,2135.7392740249634,1.3400668876784039e-06
1991992,1991993,1991992,3983985,2136.889461040497,1.316221869274159e-06
1993994,1993995,1993994,3987989,2137.967408180237,1.2927604302603868e-06
1995996,1995997,1995996,3991993,2138.9909381866455,1.269676545234688e-06
1997998,1997999,1997998,3995997,2140.039754152298,1.2469638477341505e-06
2000000,2000001,2000000,4000001,2141.0965712070465,1.2246168807905633e-06


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/proxflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0008759498596191406,2181.4194943796983
1,4,4,8,0.0025529861450195312,1651.0810025948942
2,6,6,12,0.004111766815185547,787.0138414872515
3,8,8,16,0.005583047866821289,443.6895532228107
4,12,12,24,0.007873058319091797,300.66016246667004
5,20,20,40,0.01164388656616211,289.49557450497423
6,24,24,48,0.01399993896484375,223.78623088754762
7,32,32,64,0.018385887145996094,220.81261182620847
8,36,36,72,0.02080988883972168,183.77908068817942
9,44,44,88,0.02485203742980957,182.1170983560105
10,50,50,100,0.027957916259765625,181.27504299099633
11,56,56,112,0.031132936477661133,170.13408406175336
12,60,60,120,0.03370094299316406,148.65325821818533
13,64,64,128,0.03749895095825195,133.7311705141201
14,70,70,140,0.042738914489746094,109.91007130056119
15,72,72,144,0.04452991485595703,82.23078898851077
16,76,76,152,0.04692888259887695,80.91936398800976
17,80,80,160,0.04934287071228027,79.04529536254631
18,88,88,176,0.05314517021179199,78.85624657588028
19,92,92,184,0.05566596984863281,75.58327398235679
20,96,96,192,0.05786395072937012,73.92414756257904
21,102,102,204,0.06100893020629883,73.46183075002295
22,106,106,212,0.06332206726074219,70.76717652738853
23,110,110,220,0.06579780578613281,69.26330237974526
24,116,116,232,0.06909489631652832,68.49817273290205
25,124,124,248,0.07320284843444824,68.44794841411067
26,128,128,256,0.07548117637634277,65.47411002685817
27,134,134,268,0.07845497131347656,65.00800772888533
28,138,138,276,0.08075594902038574,63.04930993963785
29,146,146,292,0.08486819267272949,63.01626689073737
30,150,150,300,0.0878760814666748,60.585296799987645
31,158,158,316,0.09429192543029785,60.558948448604724
32,162,162,324,0.09705090522766113,58.35275952431084
33,168,168,336,0.10044288635253906,57.9806696844048
34,172,172,344,0.10273575782775879,56.84317694752394
35,180,180,360,0.10667181015014648,56.83095757162528
36,184,184,368,0.10909700393676758,55.80233445900785
37,188,188,376,0.11155414581298828,55.26741500557728
38,196,196,392,0.11548495292663574,55.260526121163366
39,200,200,400,0.1177821159362793,54.71731502524608
40,208,208,416,0.12210202217102051,54.71238647379096
41,212,212,424,0.12491393089294434,54.182335491579806
42,220,220,440,0.12903404235839844,54.178004291141406
43,226,226,452,0.1326918601989746,53.95350490107603
44,234,234,468,0.1372988224029541,53.949722585297195
45,240,240,480,0.14156794548034668,53.58659410904352
46,248,248,496,0.14683103561401367,53.58308064107223
47,254,254,508,0.15015101432800293,53.02376492425742
48,262,262,524,0.15372896194458008,53.020486627652645
49,268,268,536,0.15672707557678223,52.363445531572324
50,276,276,552,0.16040396690368652,52.36040531387562
51,282,282,564,0.16334795951843262,51.534811430448826
52,290,290,580,0.1678609848022461,51.53184572684222
53,298,298,596,0.17274999618530273,51.52889704564018
54,306,306,612,0.17676281929016113,51.52596401722826
55,314,314,628,0.18097996711730957,51.523045408566986
56,320,320,640,0.18393397331237793,49.70963317137989
57,328,328,656,0.1880970001220703,49.70675919202199
58,336,336,672,0.19238495826721191,49.70392743917978
59,344,344,688,0.19648408889770508,49.70113320769474
60,350,350,700,0.19957399368286133,47.28948443135232
61,358,358,716,0.2033989429473877,47.28695536312193
62,366,366,732,0.20725607872009277,47.284457457507415
63,374,374,748,0.21102380752563477,47.28198773234476
64,380,380,760,0.21399974822998047,44.50139544548506
65,388,388,776,0.21788787841796875,44.49901055163082
66,396,396,792,0.22166895866394043,44.49666438437498
67,402,402,804,0.22466206550598145,41.628758446245456
68,410,410,820,0.22832894325256348,41.62652138665749
69,418,418,836,0.23200488090515137,41.62432679554627
70,426,426,852,0.23574495315551758,41.62216970167037
71,432,432,864,0.2389380931854248,38.47845638222566
72,440,440,880,0.24344491958618164,38.4764978048629
73,446,446,892,0.24777603149414062,35.605241254758994
74,454,454,908,0.251964807510376,35.603498638495694
75,460,460,920,0.2549409866333008,32.79745501433467
76,468,468,936,0.2587740421295166,32.79595320932981
77,474,474,948,0.2617659568786621,30.281377828350514
78,482,482,964,0.2657759189605713,30.280015378572898
79,488,488,976,0.2702641487121582,27.96866530868556
80,496,496,992,0.2741730213165283,27.967421028228046
81,502,502,1004,0.2773277759552002,25.31751598934352
82,510,510,1020,0.2813849449157715,25.316356268892605
83,516,516,1032,0.28475499153137207,22.79057474097681
84,524,524,1048,0.2895689010620117,22.789515262186114
85,530,530,1060,0.2928040027618408,20.195509882466013
86,538,538,1076,0.29683995246887207,20.1945174394441
87,546,546,1092,0.30082201957702637,20.193532850744305
88,552,552,1104,0.30373501777648926,18.196492665958885
89,560,560,1120,0.3074958324432373,18.19557843901748
90,568,568,1136,0.31119203567504883,18.194674315126576
91,576,576,1152,0.31499695777893066,18.19377921116984
92,582,582,1164,0.3179929256439209,15.855835403595961
93,590,590,1180,0.321727991104126,15.854996069153913
94,596,596,1192,0.3247079849243164,13.63403399250251
95,604,604,1208,0.3285040855407715,13.633220217886446
96,610,610,1220,0.3314077854156494,11.559610759062593
97,618,618,1236,0.3350369930267334,11.558905750267627
98,624,624,1248,0.3383979797363281,9.875058336087818
99,632,632,1264,0.342897891998291,9.874432987100136
100,638,638,1276,0.3462231159210205,8.450791633237714
101,646,646,1292,0.35015201568603516,8.450220112861643
102,654,654,1308,0.3537750244140625,8.449653610203882
103,660,660,1320,0.3567831516265869,7.287453598091474
104,668,668,1336,0.36051297187805176,7.2869027186224
105,676,676,1352,0.36424899101257324,7.28635734374177
106,684,684,1368,0.36819887161254883,7.285817055112943
107,692,692,1384,0.37193894386291504,7.285281478272395
108,700,700,1400,0.375715970993042,7.284750277743683
109,708,708,1416,0.37961602210998535,7.284223152710297
110,712,712,1424,0.38193583488464355,7.112176431706416
111,720,720,1440,0.3856377601623535,7.11169473953953
112,724,724,1448,0.38825082778930664,6.996298979986932
113,732,732,1464,0.3926379680633545,6.9958610614829695
114,736,736,1472,0.3952169418334961,6.895541195452211
115,744,744,1488,0.3997528553009033,6.895200796451377
116,750,750,1500,0.40306997299194336,6.8524637146970235
117,758,758,1516,0.40709710121154785,6.8521624695990795
118,764,764,1528,0.4103727340698242,6.78937145325699
119,772,772,1544,0.41417813301086426,6.78909277828086
120,778,778,1556,0.41724586486816406,6.70426366562765
121,786,786,1572,0.42114996910095215,6.704004095999835
122,792,792,1584,0.4247889518737793,6.619096416169782
123,800,800,1600,0.4285738468170166,6.618859003474313
124,806,806,1612,0.43161702156066895,6.531396723279158
125,812,812,1624,0.4346790313720703,6.444216556788206
126,820,820,1640,0.43909287452697754,6.444001119788936
127,828,828,1656,0.4441089630126953,6.443787795403637
128,834,834,1668,0.44785308837890625,6.341279464076251
129,842,842,1684,0.4521169662475586,6.341071465569371
130,848,848,1696,0.4554009437561035,6.226331071003756
131,856,856,1712,0.45934319496154785,6.226126738472544
132,862,862,1724,0.4623119831085205,6.106090354097773
133,870,870,1740,0.46617603302001953,6.105892757609013
134,878,878,1756,0.4700300693511963,6.1056966709778635
135,886,886,1772,0.4739818572998047,6.10550197386317
136,894,894,1788,0.4779369831085205,6.105308558801539
137,902,902,1804,0.48174309730529785,6.10511632970713
138,910,910,1820,0.4858839511871338,6.10492520055675
139,918,918,1836,0.4902048110961914,6.104735094229909
140,926,926,1852,0.49434399604797363,6.104545941489732
141,932,932,1864,0.4979689121246338,6.050129058606558
142,940,940,1880,0.5021259784698486,6.04994914112217
143,946,946,1892,0.5053088665008545,5.977639815893326
144,954,954,1908,0.5090360641479492,5.977468607945525
145,960,960,1920,0.5126168727874756,5.906851342289201
146,966,966,1932,0.515949010848999,5.831078057195782
147,974,974,1948,0.520359992980957,5.830926949525406
148,982,982,1964,0.5242187976837158,5.830776880698295
149,990,990,1980,0.5278909206390381,5.830627787165099
150,998,998,1996,0.5315699577331543,5.830479611450755
151,1006,1006,2012,0.5353059768676758,5.830332301483736
152,1014,1014,2028,0.5400240421295166,5.830185810001922
153,1022,1022,2044,0.5500359535217285,5.830040094029528
154,1030,1030,2060,0.553900957107544,5.829895114411897
155,1038,1038,2076,0.5576009750366211,5.829750835405321
156,1046,1046,2092,0.5613808631896973,5.829607224313804
157,1054,1054,2108,0.5651628971099854,5.829464251165518
158,1062,1062,2124,0.5689640045166016,5.829321888429149
159,1070,1070,2140,0.5725619792938232,5.829180110758784
160,1078,1078,2156,0.5763630867004395,5.829038894770406
161,1086,1086,2172,0.5802288055419922,5.828898218842028
162,1094,1094,2188,0.5839369297027588,5.828758062936913
163,1102,1102,2204,0.5878851413726807,5.828618408445095
164,1110,1110,2220,0.5925719738006592,5.828479238044679
165,1118,1118,2236,0.5988919734954834,5.828340535576444
166,1126,1126,2252,0.6035089492797852,5.828202285932889
167,1134,1134,2268,0.6076958179473877,5.828064474958978
168,1142,1142,2284,0.6130139827728271,5.827927089364721
169,1150,1150,2300,0.6172580718994141,5.827790116645815
170,1158,1158,2316,0.6215219497680664,5.827653545013277
171,1166,1166,2332,0.6263108253479004,5.827517363330458
172,1174,1174,2348,0.6328141689300537,5.827381561057109
173,1180,1180,2360,0.6361939907073975,5.795390582761115
174,1188,1188,2376,0.6406688690185547,5.795260712016898
175,1196,1196,2392,0.6489050388336182,5.795131316634638
176,1204,1204,2408,0.6528158187866211,5.795002367832012
177,1212,1212,2424,0.6566300392150879,5.794873840011064
178,1220,1220,2440,0.6614358425140381,5.794745710334382
179,1228,1228,2456,0.6665210723876953,5.794617958359254
180,1236,1236,2472,0.6708638668060303,5.794490565725255
181,1244,1244,2488,0.6756839752197266,5.794363515883219
182,1252,1252,2504,0.6794209480285645,5.79423679386332
183,1260,1260,2520,0.6830499172210693,5.7941103860741805
184,1268,1268,2536,0.6874518394470215,5.79398428013053
185,1276,1276,2552,0.6922769546508789,5.793858464704158
186,1282,1282,2564,0.6957497596740723,5.757370221176188
187,1290,1290,2580,0.6994428634643555,5.757248045425172
188,1298,1298,2596,0.703434944152832,5.757126287913479
189,1306,1306,2612,0.7072157859802246,5.757004921382418
190,1314,1314,2628,0.7111649513244629,5.756883921255167
191,1322,1322,2644,0.7148599624633789,5.756763265335621
192,1330,1330,2660,0.7186880111694336,5.756642933541798
193,1338,1338,2676,0.7227258682250977,5.7565229076702735
194,1344,1344,2688,0.7259159088134766,5.734999213158403
195,1352,1352,2704,0.7296760082244873,5.7348820557074305
196,1360,1360,2720,0.7334861755371094,5.734765199734511
197,1368,1368,2736,0.738274097442627,5.734648625522027
198,1376,1376,2752,0.743211030960083,5.7345323153745085
199,1384,1384,2768,0.7478699684143066,5.734416253374093
200,1392,1392,2784,0.7518389225006104,5.734300425164861
201,1400,1400,2800,0.7559189796447754,5.734184817765822
202,1406,1406,2812,0.7590231895446777,5.6933271837418715
203,1414,1414,2828,0.7627241611480713,5.693213156221759
204,1422,1422,2844,0.7665069103240967,5.693099426483968
205,1430,1430,2860,0.7703428268432617,5.6929859734493675
206,1438,1438,2876,0.7741508483886719,5.692872778115429
207,1446,1446,2892,0.7779510021209717,5.692759823323058
208,1454,1454,2908,0.7816798686981201,5.692647093551614
209,1462,1462,2924,0.785679817199707,5.6925345747368965
210,1470,1470,2940,0.789849042892456,5.692422254111534
211,1478,1478,2956,0.794701099395752,5.692310120064576
212,1486,1486,2972,0.7995009422302246,5.692198162014279
213,1494,1494,2988,0.8038830757141113,5.692086370299194
214,1502,1502,3004,0.8078210353851318,5.69197473608051
215,1510,1510,3020,0.8120989799499512,5.691863251253835
216,1518,1518,3036,0.8164310455322266,5.691751908374954
217,1526,1526,3052,0.8227200508117676,5.691640700589346
218,1534,1534,3068,0.8288140296936035,5.691529621573977
219,1542,1542,3084,0.832988977432251,5.691418665482729
220,1550,1550,3100,0.8387918472290039,5.691307826899106
221,1558,1558,3116,0.8446259498596191,5.691197100794739
222,1562,1562,3124,0.8473730087280273,5.641108237551293
223,1570,1570,3140,0.8512489795684814,5.6409997384630515
224,1578,1578,3156,0.8551139831542969,5.640891420515345
225,1586,1586,3172,0.858922004699707,5.640783267834308
226,1594,1594,3188,0.8628840446472168,5.640675266372114
227,1602,1602,3204,0.8668410778045654,5.640567403673117
228,1610,1610,3220,0.8706738948822021,5.640459668671383
229,1618,1618,3236,0.874413013458252,5.640352051516061
230,1626,1626,3252,0.8781261444091797,5.640244543418703
231,1632,1632,3264,0.8812868595123291,5.488862212086701
232,1640,1640,3280,0.8849730491638184,5.488756904219258
233,1648,1648,3296,0.8901598453521729,5.488651790106928
234,1654,1654,3308,0.8936169147491455,4.897993398479002
235,1662,1662,3324,0.8976671695709229,4.897891023196848
236,1670,1670,3340,0.9015250205993652,4.897789446025172
237,1678,1678,3356,0.9052858352661133,4.8976885814823845
238,1686,1686,3372,0.9090008735656738,4.897588353914671
239,1694,1694,3388,0.9126651287078857,4.89748869633172
240,1702,1702,3404,0.9163100719451904,4.897389549384002
241,1710,1710,3420,0.9201018810272217,4.897290860461453
242,1718,1718,3436,0.9240379333496094,4.897192582902903
243,1726,1726,3452,0.9277739524841309,4.897094675298149
244,1732,1732,3464,0.9306769371032715,4.800094329690182
245,1740,1740,3480,0.9345238208770752,4.799998451898318
246,1748,1748,3496,0.9385101795196533,4.799903085759183
247,1756,1756,3512,0.9421718120574951,4.799808188153747
248,1764,1764,3528,0.9459898471832275,4.799713720221575
249,1772,1772,3544,0.949836015701294,4.7996196468981225
250,1780,1780,3560,0.9537520408630371,4.7995259365037555
251,1788,1788,3576,0.9575281143188477,4.799432560379728
252,1796,1796,3592,0.9615108966827393,4.799339492568265
253,1804,1804,3608,0.9653539657592773,4.799246709526187
254,1812,1812,3624,0.969092845916748,4.799154189872411
255,1820,1820,3640,0.9730329513549805,4.799061914164781
256,1828,1828,3656,0.9767968654632568,4.7989698647005525
257,1836,1836,3672,0.9805259704589844,4.798878025339263
258,1844,1844,3688,0.9842729568481445,4.798786381344939
259,1852,1852,3704,0.988523006439209,4.798694919247623
260,1860,1860,3720,0.9925839900970459,4.798603626717181
261,1868,1868,3736,0.9966180324554443,4.79851249245246
262,1876,1876,3752,1.0002028942108154,4.798421506082491
263,1884,1884,3768,1.0039830207824707,4.798330658076679
264,1892,1892,3784,1.0077481269836426,4.798239939666814
265,1900,1900,3800,1.0115368366241455,4.798149342774536
266,1906,1906,3812,1.0146009922027588,4.711683660194353
267,1914,1914,3828,1.0183501243591309,4.711593663658618
268,1922,1922,3844,1.0221529006958008,4.711503872069102
269,1930,1930,3860,1.0261640548706055,4.7114142727996295
270,1938,1938,3876,1.0298569202423096,4.7113248541694475
271,1946,1946,3892,1.0337328910827637,4.7112356053603435
272,1954,1954,3908,1.037672996520996,4.7111465163415005
273,1962,1962,3924,1.0413718223571777,4.711057577803331
274,1970,1970,3940,1.0452289581298828,4.710968781094834
275,1978,1978,3956,1.049185037612915,4.710880118169598
276,1986,1986,3972,1.0529170036315918,4.7107915815358865
277,1994,1994,3988,1.0566110610961914,4.710703164211395
278,2002,2002,4004,1.060256004333496,4.710614859682551
279,2010,2010,4020,1.0640549659729004,4.710526661866879
280,2018,2018,4036,1.0678200721740723,4.710438565080267
281,2026,2026,4052,1.0716969966888428,4.710350564004784
282,2028,2028,4056,1.0730280876159668,4.710262653662539
283,2036,2036,4072,1.0767669677734375,4.710174829388734
284,2044,2044,4088,1.0804119110107422,4.710087086808585
285,2052,2052,4104,1.0841789245605469,4.709999421817429
286,2060,2060,4120,1.0879099369049072,4.709911830559008
287,2068,2068,4136,1.0918028354644775,4.7098243094101235
288,2076,2076,4152,1.0957129001617432,4.709736854961534
289,2084,2084,4168,1.0997178554534912,4.70964946400602
290,2092,2092,4184,1.1034679412841797,4.70956213352224
291,2100,2100,4200,1.1072289943695068,4.709474860662908
292,2108,2108,4216,1.1109728813171387,4.709387642742854
293,2116,2116,4232,1.1147761344909668,4.709300477228908
294,2124,2124,4248,1.1184790134429932,4.709213361729439
295,2132,2132,4264,1.122297763824463,4.709126293985037
296,2140,2140,4280,1.1263999938964844,4.7090392718604335
297,2146,2146,4292,1.1294457912445068,4.675862713420884
298,2154,2154,4308,1.13326096534729,4.675776550498199
299,2162,2162,4324,1.1372449398040771,4.675690435673573
300,2170,2170,4340,1.1439049243927002,4.675604366564812
301,2178,2178,4356,1.1491940021514893,4.6755183409405845
302,2186,2186,4372,1.153012990951538,4.675432356708143
303,2192,2192,4384,1.1562178134918213,4.527601693628867
304,2200,2200,4400,1.16025710105896,4.5275177741079915
305,2206,2206,4412,1.1632771492004395,3.882447474365449
306,2214,2214,4428,1.167382001876831,3.882371247395554
307,2220,2220,4440,1.1712419986724854,3.3491916022717305
308,2228,2228,4456,1.175199031829834,3.349117732645709
309,2236,2236,4472,1.17976975440979,3.3490444067174394
310,2244,2244,4488,1.183473825454712,3.3489715612086
311,2252,2252,4504,1.1878700256347656,3.348899141685365
312,2260,2260,4520,1.192141056060791,3.3488271012596442
313,2268,2268,4536,1.1963510513305664,3.3487553994849577
314,2276,2276,4552,1.200251817703247,3.3486840014147674
315,2284,2284,4568,1.204190969467163,3.348612876803145
316,2292,2292,4584,1.2079689502716064,3.3485419994226504
317,2300,2300,4600,1.211899995803833,3.3484713464831657
318,2308,2308,4616,1.2158048152923584,3.348400898138493
319,2316,2316,4632,1.219757080078125,3.3483306370646915
320,2324,2324,4648,1.2238819599151611,3.348260548100029
321,2332,2332,4664,1.2280199527740479,3.3481906179405314
322,2340,2340,4680,1.2317240238189697,3.3481208348783866
323,2346,2346,4692,1.2348270416259766,3.3055820497268087
324,2354,2354,4708,1.2393641471862793,3.3055140823302054
325,2362,2362,4724,1.2439429759979248,3.3054463679944774
326,2370,2370,4740,1.2481269836425781,3.3053788908223396
327,2378,2378,4756,1.2519888877868652,3.3053116363471418
328,2386,2386,4772,1.256108045578003,3.3052445913743895
329,2394,2394,4788,1.2600760459899902,3.3051777438450927
330,2402,2402,4804,1.2638120651245117,3.305111082712756
331,2410,2410,4820,1.267807960510254,3.305044597835945
332,2414,2414,4828,1.2702860832214355,3.232720765495287
333,2422,2422,4844,1.2741179466247559,3.2326584950266124
334,2430,2430,4860,1.278235912322998,3.2325964086380736
335,2438,2438,4876,1.282020092010498,3.2325344925438912
336,2446,2446,4892,1.2860119342803955,3.2324727344467874
337,2454,2454,4908,1.2906429767608643,3.2324111233428994
338,2462,2462,4924,1.295365810394287,3.2323496493545463
339,2470,2470,4940,1.2994911670684814,3.2322883035870973
340,2478,2478,4956,1.3035809993743896,3.23222707800403
341,2486,2486,4972,1.307508945465088,3.2321659653219967
342,2494,2494,4988,1.3116600513458252,3.2321049589190807
343,2502,2502,5004,1.3155567646026611,3.232044052754759
344,2510,2510,5020,1.3195829391479492,3.231983241302828
345,2518,2518,5036,1.3239097595214844,3.2319225194918317
346,2526,2526,5052,1.327974796295166,3.231861882655153
347,2534,2534,5068,1.3316638469696045,3.231801326484856
348,2542,2542,5084,1.3354339599609375,3.2317408469943985
349,2550,2550,5100,1.3398430347442627,3.231680440485775
350,2554,2554,5108,1.3421919345855713,3.1801732424349893
351,2562,2562,5124,1.3460590839385986,3.1801140483861445
352,2570,2570,5140,1.34993314743042,3.180054949414398
353,2578,2578,5156,1.3539340496063232,3.1799959404460196
354,2586,2586,5172,1.3578288555145264,3.1799370167918823
355,2594,2594,5188,1.3620390892028809,3.1798781741056246
356,2602,2602,5204,1.3659420013427734,3.1798194083532962
357,2610,2610,5220,1.3698759078979492,3.1797607157822085
358,2618,2618,5236,1.3737537860870361,3.1797020928950133
359,2626,2626,5252,1.3779568672180176,3.179643536427079
360,2634,2634,5268,1.3818371295928955,3.1795850433248916
361,2642,2642,5284,1.3856770992279053,3.179526610728317
362,2650,2650,5300,1.3901660442352295,3.1794682359540047
363,2658,2658,5316,1.3947398662567139,3.1794099164804948
364,2666,2666,5332,1.3991401195526123,3.179351649934688
365,2674,2674,5348,1.402918815612793,3.1792934340817283
366,2682,2682,5364,1.4067468643188477,3.1792352668118156
367,2690,2690,5380,1.4107341766357422,3.1791771461330427
368,2698,2698,5396,1.4145910739898682,3.1791190701607093
369,2706,2706,5412,1.41914701461792,3.1790610371116372
370,2714,2714,5428,1.4236679077148438,3.1790030452949622
371,2722,2722,5444,1.427968978881836,3.178945093107245
372,2730,2730,5460,1.4319407939910889,3.178887179025878
373,2738,2738,5476,1.436100959777832,3.1788293016040825
374,2746,2746,5492,1.4408760070800781,3.178771459465679
375,2754,2754,5508,1.4453179836273193,3.178713651301223
376,2762,2762,5524,1.4495389461517334,3.178655875862887
377,2770,2770,5540,1.4534988403320312,3.178598131962076
378,2778,2778,5556,1.4572811126708984,3.178540418464763
379,2786,2786,5572,1.461426019668579,3.178482734288764
380,2794,2794,5588,1.4651970863342285,3.178425078401574
381,2800,2800,5600,1.4697940349578857,3.166429272537016
382,2808,2808,5616,1.4740631580352783,3.166371896210194
383,2816,2816,5632,1.4784231185913086,3.1663145671587927
384,2824,2824,5648,1.4823291301727295,3.166257281689923
385,2832,2832,5664,1.4869718551635742,3.1662000365274707
386,2840,2840,5680,1.4912750720977783,3.1661428287588933
387,2848,2848,5696,1.4957098960876465,3.1660856557878105
388,2856,2856,5712,1.499722957611084,3.166028515292851
389,2864,2864,5728,1.5040669441223145,3.165971405194
390,2872,2872,5744,1.5077917575836182,3.1659143236209957
391,2880,2880,5760,1.5117249488830566,3.165857268888658
392,2888,2888,5776,1.515528917312622,3.16580023947256
393,2894,2894,5788,1.518707036972046,3.113935064784414
394,2902,2902,5804,1.5233888626098633,3.1138787139341275
395,2910,2910,5820,1.5298559665679932,3.1138224269103603
396,2918,2918,5836,1.5349807739257812,3.113766199331394
397,2926,2926,5852,1.5404038429260254,3.1137100272004545
398,2934,2934,5868,1.5465238094329834,3.113653906867853
399,2942,2942,5884,1.5505390167236328,3.113597834996426
400,2950,2950,5900,1.5543479919433594,3.113541808531295
401,2958,2958,5916,1.5581440925598145,3.1134858246726935
402,2966,2966,5932,1.5621769428253174,3.1134298808508447
403,2974,2974,5948,1.5661430358886719,3.113373974704473
404,2982,2982,5964,1.570105791091919,3.1133181040606814
405,2990,2990,5980,1.5739829540252686,3.1132622669179
406,2998,2998,5996,1.5779430866241455,3.113206461429172
407,3006,3006,6012,1.581852912902832,3.1131506858888542
408,3008,3008,6016,1.5832159519195557,3.113094938718632
409,3016,3016,6032,1.587697982788086,3.1130392184569473
410,3024,3024,6048,1.5918688774108887,3.1129835237477437
411,3032,3032,6064,1.5962340831756592,3.1129278533322804
412,3040,3040,6080,1.600496768951416,3.112872206039242
413,3046,3046,6092,1.6036529541015625,3.074804226109336
414,3054,3054,6108,1.607522964477539,3.0747487386947796
415,3062,3062,6124,1.6117382049560547,3.0746933529158014
416,3070,3070,6140,1.6157989501953125,3.07463805789007
417,3078,3078,6156,1.6197729110717773,3.0745828441081358
418,3086,3086,6172,1.6236400604248047,3.0745277032492595
419,3094,3094,6188,1.6277339458465576,3.074472628023045
420,3102,3102,6204,1.6317839622497559,3.074417612032903
421,3110,3110,6220,1.6359727382659912,3.074362649657246
422,3116,3116,6232,1.6393249034881592,2.978436393499919
423,3124,3124,6248,1.6439170837402344,2.9783822745130237
424,3132,3132,6264,1.6480379104614258,2.9783282441412666
425,3140,3140,6280,1.6518568992614746,2.9782742956309676
426,3148,3148,6296,1.655815839767456,2.978220422944787
427,3154,3154,6308,1.659193754196167,2.5448435682088757
428,3162,3162,6324,1.6631689071655273,2.5447940644098708
429,3168,3168,6336,1.6661708354949951,2.184483480129188
430,3176,3176,6352,1.670255184173584,2.1844399969406822
431,3184,3184,6368,1.6740880012512207,2.1843966594497033
432,3192,3192,6384,1.678375005722046,2.184353455793371
433,3200,3200,6400,1.682286024093628,2.184310375268524
434,3208,3208,6416,1.6863460540771484,2.184267408206324
435,3216,3216,6432,1.690551996231079,2.184224545861184
436,3224,3224,6448,1.694648027420044,2.1841817803152708
437,3232,3232,6464,1.6986029148101807,2.1841391043893736
438,3240,3240,6480,1.7025988101959229,2.1840965115671906
439,3248,3248,6496,1.7067310810089111,2.184053995925865
440,3256,3256,6512,1.7110750675201416,2.1840115520761856
441,3264,3264,6528,1.7149569988250732,2.1839691751067676
442,3272,3272,6544,1.7189090251922607,2.1839268605378948
443,3276,3276,6552,1.7213099002838135,2.174849106264901
444,3284,3284,6568,1.7253599166870117,2.1748071879737836
445,3292,3292,6584,1.7293498516082764,2.174765393677035
446,3300,3300,6600,1.7332520484924316,2.1747237096078607
447,3308,3308,6616,1.7373580932617188,2.1746821237686618
448,3316,3316,6632,1.7417619228363037,2.1746406256921773
449,3324,3324,6648,1.745988130569458,2.1745992062350297
450,3332,3332,6664,1.7499058246612549,2.1745578573987814
451,3340,3340,6680,1.7538628578186035,2.174516572177822
452,3348,3348,6696,1.757962942123413,2.174475344426355
453,3356,3356,6712,1.7621140480041504,2.174434168744824
454,3364,3364,6728,1.7660329341888428,2.1743930403820286
455,3372,3372,6744,1.769974946975708,2.1743519551491772
456,3380,3380,6760,1.7738280296325684,2.174310909347696
457,3388,3388,6776,1.7780940532684326,2.1742698997051093
458,3396,3396,6792,1.781933069229126,2.174228923320584
459,3398,3398,6796,1.7833280563354492,2.1112894876903283
460,3406,3406,6812,1.7876977920532227,2.1112498494900365
461,3414,3414,6828,1.7918028831481934,2.11121029632352
462,3422,3422,6844,1.7963268756866455,2.111170822235408
463,3430,3430,6860,1.8004770278930664,2.11113142188492
464,3438,3438,6876,1.8050360679626465,2.111092090473562
465,3446,3446,6892,1.8093299865722656,2.111052823681348
466,3454,3454,6908,1.8134520053863525,2.111013617612116
467,3462,3462,6924,1.817375898361206,2.1109744687446437
468,3470,3470,6940,1.821775197982788,2.1109353738899017
469,3474,3474,6948,1.824397087097168,2.0963996713381903
470,3482,3482,6964,1.828446865081787,2.096361783427824
471,3490,3490,6980,1.8324148654937744,2.0963239551522292
472,3498,3498,6996,1.8363828659057617,2.0962861824713173
473,3506,3506,7012,1.841252088546753,2.096248461727214
474,3514,3514,7028,1.8452370166778564,2.096210789603788
475,3522,3522,7044,1.8494231700897217,2.0961731630881104
476,3530,3530,7060,1.853430986404419,2.0961355794383962
477,3538,3538,7076,1.8573970794677734,2.096098036155581
478,3546,3546,7092,1.8615858554840088,2.0960605309569473
479,3552,3552,7104,1.8647239208221436,2.0899037671180167
480,3560,3560,7120,1.8691258430480957,2.0898666740324643
481,3568,3568,7136,1.8734550476074219,2.089829616348993
482,3576,3576,7152,1.8787100315093994,2.089792591733385
483,3584,3584,7168,1.8830101490020752,2.0897555980794777
484,3592,3592,7184,1.89090895652771,2.0897186334808566
485,3600,3600,7200,1.8963508605957031,2.08968169621005
486,3608,3608,7216,1.9004950523376465,2.0896447846961337
487,3614,3614,7228,1.9038798809051514,2.0703473468723814
488,3622,3622,7244,1.907667875289917,2.070310947635221
489,3630,3630,7260,1.9119648933410645,2.0702745815672188
490,3638,3638,7276,1.916287899017334,2.0702382465680103
491,3646,3646,7292,1.9210739135742188,2.0702019407178796
492,3654,3654,7308,1.9257118701934814,2.070165662259342
493,3662,3662,7324,1.9305038452148438,2.0701294095794083
494,3670,3670,7340,1.9345951080322266,2.0700931811956025
495,3676,3676,7352,1.9388439655303955,2.039311624333777
496,3684,3684,7368,1.9446449279785156,2.039275715802887
497,3690,3690,7380,1.948564052581787,1.7835434920621083
498,3698,3698,7396,1.9526710510253906,1.7835082414787848
499,3704,3704,7408,1.9561238288879395,1.5789441239281814
500,3712,3712,7424,1.9600918292999268,1.5789103737700998
501,3720,3720,7440,1.96400785446167,1.5788766799233827
502,3728,3728,7456,1.9681169986724854,1.5788430403407574
503,3736,3736,7472,1.9728519916534424,1.5788094530989838
504,3744,3744,7488,1.977543830871582,1.5787759163885084
505,3752,3752,7504,1.9816739559173584,1.5787424285040288
506,3760,3760,7520,1.9862210750579834,1.5787089878360803
507,3768,3768,7536,1.9907970428466797,1.578675592863533
508,3776,3776,7552,1.995445966720581,1.5786422421477937
509,3784,3784,7568,1.9995930194854736,1.5786089343255298
510,3792,3792,7584,2.0035579204559326,1.5785756681036673
511,3798,3798,7596,2.0067219734191895,1.571874385888691
512,3806,3806,7612,2.0104639530181885,1.571842090012069
513,3814,3814,7628,2.0142641067504883,1.5718098630030681
514,3820,3820,7640,2.0174551010131836,1.5246449807913223
515,3828,3828,7656,2.0216310024261475,1.5246138101326778
516,3834,3834,7668,2.024852991104126,1.4831982288235395
517,3842,3842,7684,2.028873920440674,1.483167675652453
518,3850,3850,7700,2.0328400135040283,1.483137284508075
519,3858,3858,7716,2.0368540287017822,1.4831070447789898
520,3866,3866,7732,2.040958881378174,1.4830769469620009
521,3874,3874,7748,2.0448389053344727,1.483046982524229
522,3882,3882,7764,2.048875093460083,1.4830171437852187
523,3890,3890,7780,2.0528159141540527,1.482987423812915
524,3898,3898,7796,2.0568881034851074,1.4829578163329415
525,3906,3906,7812,2.060642957687378,1.4829283156525435
526,3914,3914,7828,2.064656972885132,1.4828989165904432
527,3922,3922,7844,2.06850004196167,1.4828696144193145
528,3930,3930,7860,2.0723907947540283,1.4828404048134871
529,3938,3938,7876,2.0764269828796387,1.4828112838043808
530,3946,3946,7892,2.08062481880188,1.4827822477400332
531,3954,3954,7908,2.0848608016967773,1.4827532932523582
532,3962,3962,7924,2.088939905166626,1.4827244172257679
533,3970,3970,7940,2.093045949935913,1.482695616770343
534,3976,3976,7952,2.096118927001953,1.4842243044622592
535,3984,3984,7968,2.100098133087158,1.4841958248538276
536,3992,3992,7984,2.103945016860962,1.4841674357721786
537,4000,4000,8000,2.107631206512451,1.4841391320326238
538,4008,4008,8016,2.1115729808807373,1.4841109089151132
539,4016,4016,8032,2.115300178527832,1.4840827621139852
540,4024,4024,8048,2.1192891597747803,1.4840546876921508
541,4032,4032,8064,2.123185873031616,1.4840266820419856
542,4040,4040,8080,2.1270320415496826,1.4839987418505416
543,4048,4048,8096,2.1309239864349365,1.483970864068624
544,4056,4056,8112,2.1347639560699463,1.4839430458846437
545,4064,4064,8128,2.1387388706207275,1.4839152846996058
546,4072,4072,8144,2.142573118209839,1.4838875781072147
547,4080,4080,8160,2.1466000080108643,1.483859923875002
548,4088,4088,8176,2.150580883026123,1.4838323199273873
549,4096,4096,8192,2.154489755630493,1.4838047643314667
550,4104,4104,8208,2.1583759784698486,1.4837772552835986
551,4112,4112,8224,2.162341833114624,1.483749791098262
552,4120,4120,8240,2.1662089824676514,1.4837223701970288
553,4128,4128,8256,2.1700520515441895,1.4836949910999238
554,4136,4136,8272,2.173845052719116,1.4836676524167842
555,4144,4144,8288,2.1776628494262695,1.4836403528391884
556,4152,4152,8304,2.181691884994507,1.4836130911352257
557,4160,4160,8320,2.185534954071045,1.4835858661416523
558,4168,4168,8336,2.1896021366119385,1.4835586767601399
559,4174,4174,8348,2.192857027053833,1.4722450910305724
560,4182,4182,8364,2.197115898132324,1.4722184157868696
561,4190,4190,8380,2.2010769844055176,1.4721918023575427
562,4198,4198,8396,2.204986810684204,1.4721652472857159
563,4206,4206,8412,2.2088451385498047,1.4721387474219227
564,4214,4214,8428,2.2128689289093018,1.4721122998910232
565,4222,4222,8444,2.2167208194732666,1.4720859020625312
566,4230,4230,8460,2.2205958366394043,1.4720595515238983
567,4238,4238,8476,2.22448992729187,1.4720332460584586
568,4246,4246,8492,2.22837495803833,1.4720069836236007
569,4254,4254,8508,2.2321391105651855,1.4719807623343968
570,4262,4262,8524,2.2361669540405273,1.4719545804456402
571,4270,4270,8540,2.2401280403137207,1.4719284363395673
572,4278,4278,8556,2.2441327571868896,1.4719023285124422
573,4286,4286,8572,2.2481698989868164,1.4718762555630747
574,4294,4294,8588,2.2520289421081543,1.471850216183043
575,4302,4302,8604,2.255880832672119,1.4718242091490765
576,4310,4310,8620,2.2597548961639404,1.4717982333133932
577,4318,4318,8636,2.2635908126831055,1.4717722875983554
578,4326,4326,8652,2.2675881385803223,1.471746370988967
579,4334,4334,8668,2.2714791297912598,1.471720482527985
580,4342,4342,8684,2.275416135787964,1.4716946213117126
581,4348,4348,8696,2.2785470485687256,1.4602378381679273
582,4356,4356,8712,2.2822468280792236,1.4602120626759643
583,4364,4364,8728,2.2860841751098633,1.4601863507401731
584,4372,4372,8744,2.290191173553467,1.4601606976659696
585,4380,4380,8760,2.2940621376037598,1.460135099230797
586,4388,4388,8776,2.298082113265991,1.4601095516283067
587,4396,4396,8792,2.3022239208221436,1.46008405142004
588,4404,4404,8808,2.306360960006714,1.4600585954938197
589,4412,4412,8824,2.3102290630340576,1.4600331810262333
590,4420,4420,8840,2.314257860183716,1.4600078054513688
591,4428,4428,8856,2.31830096244812,1.459982466430688
592,4436,4436,8872,2.322673797607422,1.4599571618299478
593,4444,4444,8888,2.326586961746216,1.4599318896971454
594,4446,4446,8892,2.327997922897339,1.459906648241713
595,4454,4454,8908,2.331822156906128,1.459881435819625
596,4462,4462,8924,2.335783004760742,1.4598562509169142
597,4470,4470,8940,2.3402087688446045,1.459831092137506
598,4478,4478,8956,2.3439769744873047,1.4598059581906
599,4486,4486,8972,2.3480660915374756,1.4597808478816887
600,4494,4494,8988,2.352146863937378,1.4597557601015296
601,4502,4502,9004,2.3558878898620605,1.4597306938195516
602,4508,4508,9016,2.3590359687805176,1.4545977700599906
603,4516,4516,9032,2.3631279468536377,1.4545728384761105
604,4524,4524,9048,2.3670480251312256,1.4545479341312557
605,4532,4532,9064,2.3709628582000732,1.45452305513777
606,4540,4540,9080,2.3748910427093506,1.4544981997946707
607,4548,4548,9096,2.3787992000579834,1.4544733665654803
608,4554,4554,9108,2.3818750381469727,1.4364713888861615
609,4562,4562,9124,2.385650873184204,1.4364467315895126
610,4570,4570,9140,2.389538049697876,1.4364221138307585
611,4578,4578,9156,2.3945138454437256,1.4363975325039746
612,4586,4586,9172,2.398697853088379,1.4363729848014373
613,4594,4594,9188,2.402662992477417,1.4363484681808814
614,4602,4602,9204,2.4065558910369873,1.4363239803378747
615,4610,4610,9220,2.410433053970337,1.4362995191822847
616,4618,4618,9236,2.414318084716797,1.4362750828146318
617,4626,4626,9252,2.418116807937622,1.4362506695078991
618,4634,4634,9268,2.422122001647949,1.4362262776885473
619,4642,4642,9284,2.425989866256714,1.4362019059225304
620,4650,4650,9300,2.42996883392334,1.4361775528996077
621,4656,4656,9312,2.4330220222473145,1.4171495382875037
622,4664,4664,9328,2.4368820190429688,1.4171254353237828
623,4672,4672,9344,2.4409079551696777,1.4171013570972946
624,4678,4678,9356,2.4442391395568848,1.1890238143164424
625,4686,4686,9372,2.448815107345581,1.1890012344119896
626,4692,4692,9384,2.452026844024658,0.9977350904274545
627,4698,4698,9396,2.455118179321289,0.8365107641935765
628,4706,4706,9412,2.4589481353759766,0.8364922607819381
629,4710,4710,9420,2.461195945739746,0.43763535231778405
630,4718,4718,9436,2.4651551246643066,0.4376183455743785
631,4724,4724,9448,2.4681758880615234,0.3671899368976028
632,4732,4732,9464,2.471879005432129,0.36717510184746516
633,4738,4738,9476,2.4749979972839355,0.30653764755231805
634,4746,4746,9492,2.4789559841156006,0.3065240748676388
635,4752,4752,9504,2.4820311069488525,0.2562917124166688
636,4758,4758,9516,2.485083818435669,0.21365881537110454
637,4766,4766,9532,2.489886999130249,0.21364769382796567
638,4770,4770,9540,2.4931390285491943,0.11018171739283389
639,4776,4776,9552,2.4966888427734375,0.09265626177682407
640,4782,4782,9564,2.4997730255126953,0.07267670700059625
641,4788,4788,9576,2.502908945083618,0.06037062448240249
642,4794,4794,9588,2.5059797763824463,0.0508112176605664
643,4800,4800,9600,2.509174108505249,0.04311152230150128
644,4808,4808,9616,2.5131289958953857,0.043105276225105627
645,4812,4812,9624,2.515428066253662,0.023532723595849347
646,4820,4820,9640,2.5192859172821045,0.023528284134044952
647,4824,4824,9648,2.521665096282959,0.01296340566489107
648,4832,4832,9664,2.525930881500244,0.01295975675157024
649,4838,4838,9676,2.5291168689727783,0.011123589837779946
650,4844,4844,9688,2.532418966293335,0.009593391951625563
651,4852,4852,9704,2.5363829135894775,0.009590317314064123
652,4856,4856,9712,2.5386929512023926,0.005422181105359414
653,4864,4864,9728,2.542746067047119,0.005419527534286317
654,4868,4868,9736,2.5454840660095215,0.003123863559608253
655,4876,4876,9752,2.5500738620758057,0.0031217839089094923
656,4880,4880,9760,2.552438974380493,0.0018710307707578977
657,4884,4884,9768,2.5549428462982178,0.0012102509300575548
658,4892,4892,9784,2.559061050415039,0.0012091206184550174
659,4896,4896,9792,2.5614709854125977,0.0008252528043612983
660,4904,4904,9808,2.5657711029052734,0.000824426313783988
661,4908,4908,9816,2.568753957748413,0.0005876671955320489
662,4916,4916,9832,2.573817014694214,0.0005869586824474027
663,4920,4920,9840,2.576528787612915,0.00042886974608791206
664,4928,4928,9856,2.5817079544067383,0.00042832090935007727
665,4932,4932,9864,2.5846099853515625,0.0003171531765246982
666,4936,4936,9872,2.587815999984741,0.0002492295660658783
667,4944,4944,9888,2.5930328369140625,0.00024881111039576354
668,4948,4948,9896,2.5957419872283936,0.00019086109864474565
669,4954,4954,9908,2.599421977996826,0.00017982852466502663
670,4962,4962,9924,2.6035521030426025,0.00017953416954696877
671,4966,4966,9932,2.6063270568847656,0.00013753296832419437
672,4974,4974,9948,2.610403060913086,0.00013732904540120217
673,4978,4978,9956,2.6128180027008057,0.00010768005472527875
674,4986,4986,9972,2.617086887359619,0.00010753105300409516
675,4990,4990,9980,2.619792938232422,8.69035918640293e-05
676,4998,4998,9996,2.623887062072754,8.679715642756491e-05
677,5004,5004,10008,2.627142906188965,8.107928078970872e-05
678,5010,5010,10020,2.630445957183838,7.558949300801032e-05
679,5016,5016,10032,2.6337029933929443,7.079197905568435e-05
680,5024,5024,10048,2.637809991836548,7.070447566093208e-05
681,5028,5028,10056,2.640316963195801,5.304549461015995e-05
682,5036,5036,10072,2.6444480419158936,5.297910809076711e-05
683,5040,5040,10080,2.64711594581604,4.0218869798991363e-05
684,5048,5048,10096,2.6512019634246826,4.0170136799133616e-05
685,5052,5052,10104,2.6535229682922363,3.135934207421087e-05
686,5060,5060,10120,2.6575019359588623,3.1319979825639166e-05
687,5064,5064,10128,2.6598620414733887,2.4009507569644484e-05
688,5072,5072,10144,2.6638598442077637,2.3974464511411497e-05
689,5076,5076,10152,2.6662800312042236,1.752195453263994e-05
690,5084,5084,10168,2.6703829765319824,1.7497752537565248e-05
691,5088,5088,10176,2.6729750633239746,1.2511766271927627e-05
692,5096,5096,10192,2.677109956741333,1.2491399616010312e-05
693,5100,5100,10200,2.679450035095215,8.90570345291053e-06
694,5108,5108,10216,2.6839969158172607,8.890541039363598e-06
695,5112,5112,10224,2.686990976333618,6.352883815452515e-06
696,5118,5118,10236,2.6917219161987305,5.918186047892959e-06
697,5122,5122,10244,2.6949269771575928,4.37242135831184e-06
698,5130,5130,10260,2.698970079421997,4.364135179457662e-06
699,5134,5134,10268,2.70121693611145,3.1005122309579747e-06
700,5140,5140,10280,2.7042739391326904,2.8815994710384985e-06
701,5144,5144,10288,2.7065658569335938,2.145240273421223e-06
702,5152,5152,10304,2.7105488777160645,2.140489527846512e-06
703,5156,5156,10312,2.7128188610076904,1.5130729025258915e-06
704,5162,5162,10324,2.7158939838409424,1.4051680636839592e-06
705,5166,5166,10332,2.7182159423828125,1.0610763183649397e-06
706,5172,5172,10344,2.721359968185425,1.000877091428265e-06
707,5176,5176,10352,2.723615884780884,7.703553137616836e-07
708,5182,5182,10364,2.72672700881958,7.301526920855395e-07
709,5186,5186,10372,2.7291109561920166,5.743983138017938e-07
710,5194,5194,10388,2.7330498695373535,5.732119916501688e-07
711,5198,5198,10396,2.7353458404541016,4.5602348563988926e-07
712,5206,5206,10412,2.7394609451293945,4.551878873826354e-07
713,5210,5210,10420,2.7430739402770996,3.5632297112897504e-07
714,5218,5218,10436,2.7486979961395264,3.5571349599194946e-07
715,5222,5222,10444,2.7509818077087402,2.659055553522194e-07
716,5230,5230,10460,2.755126953125,2.654522859302233e-07
717,5234,5234,10468,2.7575418949127197,1.9895367131539388e-07
718,5240,5240,10480,2.761183023452759,1.8749449282040587e-07
719,5246,5246,10492,2.7645139694213867,1.7561990262038307e-07
720,5252,5252,10504,2.7677690982818604,1.6517890344402986e-07
721,5256,5256,10512,2.770352840423584,1.298193410548265e-07
722,5264,5264,10528,2.7744901180267334,1.2958355455339188e-07
723,5268,5268,10536,2.7769179344177246,9.678626611275831e-08
724,5276,5276,10552,2.780996799468994,9.662028332968475e-08
725,5280,5280,10560,2.783247947692871,7.09484311300912e-08
726,5284,5284,10568,2.785487174987793,4.861499292019289e-08
727,5292,5292,10584,2.790328025817871,4.84919837617781e-08
728,5296,5296,10592,2.792768955230713,2.924150521721458e-08
729,5302,5302,10604,2.7962570190429688,2.5634790290496312e-08
730,5308,5308,10616,2.7995588779449463,2.245201358164195e-08
731,5312,5312,10624,2.802121877670288,1.2066720955772325e-08
732,5316,5316,10632,2.8047239780426025,4.67684913019184e-09
733,5324,5324,10648,2.8091189861297607,4.629555405699648e-09
734,5328,5328,10656,2.8116071224212646,1.8530954548623413e-09


==> plot_data/logistic_regression_problem_lambda_param1overN_data_namespambase/proxflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0011909008026123047,2181.4194943796983
1,4,4,8,0.005404949188232422,1651.0810025948942
2,6,6,12,0.006912946701049805,811.3696513540854
3,8,8,16,0.008089780807495117,540.5334161789265
4,10,10,20,0.009407997131347656,340.5664798776347
5,12,12,24,0.010545015335083008,246.140754933793
6,14,14,28,0.011706829071044922,179.24733065039914
7,18,18,36,0.013952970504760742,176.1873394977806
8,22,22,44,0.016134023666381836,179.58271494054793
9,24,24,48,0.017527103424072266,132.35720100719527
10,26,26,52,0.01906895637512207,127.5058312975259
11,28,28,56,0.020360946655273438,131.4658535876756
12,32,32,64,0.022569894790649414,126.9273311629006
13,34,34,68,0.0243380069732666,106.38123453026947
14,36,36,72,0.026174068450927734,102.97302140781767
15,40,40,80,0.028110027313232422,102.56973292267685
16,44,44,88,0.030094146728515625,101.90902027413154
17,46,46,92,0.03180122375488281,97.10644598258204
18,50,50,100,0.03448200225830078,93.96666929492062
19,52,52,104,0.03574800491333008,80.51470788221422
20,54,54,108,0.03700089454650879,81.38939433846622
21,56,56,112,0.03817915916442871,82.00616609540543
22,58,58,116,0.039652109146118164,81.40809900282443
23,60,60,120,0.04092001914978027,77.27750404624817
24,62,62,124,0.04237484931945801,77.41682296761519
25,64,64,128,0.043810129165649414,77.29127669344939
26,66,66,132,0.04514884948730469,75.38269629840511
27,68,68,136,0.04643106460571289,74.57344655132124
28,70,70,140,0.047791242599487305,74.45491375690153
29,72,72,144,0.050438880920410156,72.89565423677095
30,76,76,152,0.05244016647338867,72.83600996361133
31,78,78,156,0.05365395545959473,70.95660971649431
32,82,82,164,0.05543875694274902,70.8559514329113
33,84,84,168,0.05681419372558594,66.7040948524666
34,88,88,176,0.05882596969604492,66.70628838848688
35,90,90,180,0.0600588321685791,64.6110555713069
36,94,94,188,0.06197619438171387,64.62213936484864
37,96,96,192,0.06398582458496094,61.35867357934194
38,98,98,196,0.06548690795898438,61.38600898506115
39,100,100,200,0.06685209274291992,59.51669595146177
40,102,102,204,0.06798291206359863,58.8749888722914
41,104,104,208,0.0691530704498291,58.44336644526447
42,108,108,216,0.07172894477844238,58.4360573106178
43,110,110,220,0.07315516471862793,56.43453445098294
44,112,112,224,0.07435393333435059,56.551864421448954
45,114,114,228,0.07572102546691895,56.620124460127045
46,118,118,236,0.07779097557067871,56.49773390423138
47,120,120,240,0.07900810241699219,56.26668731028121
48,124,124,248,0.0812528133392334,56.26031895604524
49,126,126,252,0.08301591873168945,55.34762315016383
50,128,128,256,0.08427119255065918,55.35964365627274
51,130,130,260,0.08552908897399902,55.135816007733865
52,134,134,268,0.08737993240356445,55.11996700146119
53,136,136,272,0.08849215507507324,54.47187253877382
54,140,140,280,0.09038805961608887,54.460106571777715
55,142,142,284,0.09173989295959473,53.995674247524676
56,146,146,292,0.09503316879272461,53.98969323174424
57,148,148,296,0.09651780128479004,53.54799543413492
58,152,152,304,0.1009979248046875,53.547729439598015
59,154,154,308,0.10247206687927246,53.297972867992485
60,158,158,316,0.10521912574768066,53.28910465196236
61,160,160,320,0.1068730354309082,52.98907781832577
62,164,164,328,0.11747503280639648,52.97954489768176
63,168,168,336,0.12012004852294922,52.90770113835151
64,172,172,344,0.12801408767700195,52.83963764705277
65,176,176,352,0.1328749656677246,52.78713789992162
66,178,178,356,0.14022493362426758,52.25327558316644
67,182,182,364,0.14376187324523926,52.248644915350724
68,184,184,368,0.1462268829345703,51.77790444441848
69,188,188,376,0.15604496002197266,51.7729651594334
70,190,190,380,0.15787506103515625,51.1308652608252
71,194,194,388,0.16051411628723145,51.144042207439725
72,198,198,396,0.16318106651306152,51.14235790919838
73,200,200,400,0.16576099395751953,50.19738391472356
74,204,204,408,0.17054104804992676,50.18790358401748
75,206,206,412,0.17378783226013184,49.01987311435073
76,210,210,420,0.1770789623260498,49.0151181990102
77,214,214,428,0.18018412590026855,48.813888695023934
78,218,218,436,0.186323881149292,48.45078280481425
79,222,222,444,0.18867802619934082,48.25445844813794
80,226,226,452,0.19124412536621094,48.12914163925393
81,228,228,456,0.1943039894104004,47.78043202340723
82,232,232,464,0.20229887962341309,47.803659177300005
83,236,236,472,0.20585203170776367,47.74127696793107
84,238,238,476,0.20785093307495117,46.6917099609675
85,242,242,484,0.21006202697753906,46.68986907280987
86,246,246,492,0.21241188049316406,46.5350640111194
87,250,250,500,0.2186739444732666,46.43962633016986
88,254,254,508,0.22170495986938477,46.36275224338169
89,256,256,512,0.2232041358947754,44.603278747423474
90,260,260,520,0.2252979278564453,44.61722790112458
91,264,264,528,0.22761797904968262,44.55255070294106
92,266,266,532,0.22904491424560547,44.202186014393874
93,270,270,540,0.231428861618042,44.16553095498216
94,274,274,548,0.23483610153198242,43.956234997552656
95,276,276,552,0.23643708229064941,41.3888165030487
96,280,280,560,0.2387678623199463,41.412520489006056
97,282,282,564,0.24010396003723145,38.53731514314245
98,288,288,576,0.2429518699645996,38.52108653706773
99,292,292,584,0.24497103691101074,38.32462242309771
100,294,294,588,0.24639487266540527,36.3725934846027
101,298,298,596,0.25074195861816406,35.45290479418327
102,302,302,604,0.25292110443115234,35.145798198275315
103,304,304,608,0.25431084632873535,34.43120198338033
104,306,306,612,0.255810022354126,33.8112297347966
105,310,310,620,0.25812697410583496,33.82724564697105
106,312,312,624,0.25946998596191406,33.55399990068668
107,316,316,632,0.2614309787750244,33.11477046947175
108,318,318,636,0.2647511959075928,30.245051758503678
109,322,322,644,0.2672121524810791,30.405262184572166
110,326,326,652,0.26905298233032227,30.561979020608305
111,328,328,656,0.27028799057006836,29.94582935692324
112,332,332,664,0.27252197265625,29.9901192699499
113,336,336,672,0.2747070789337158,30.01721787064048
114,340,340,680,0.27681493759155273,29.85000213716512
115,344,344,688,0.27961301803588867,29.571844819323132
116,348,348,696,0.28217196464538574,29.05370405994654
117,352,352,704,0.28421878814697266,28.50284601506405
118,356,356,712,0.286578893661499,27.94759427352824
119,360,360,720,0.28884100914001465,27.48897837057939
120,362,362,724,0.29035401344299316,25.13154886062148
121,366,366,732,0.292496919631958,24.935208757318378
122,370,370,740,0.2957329750061035,24.73677631097712
123,372,372,744,0.2974419593811035,22.762698919210834
124,376,376,752,0.30011796951293945,22.799630572042815
125,380,380,760,0.30266404151916504,22.959608318923983
126,382,382,764,0.30402302742004395,23.85094554175248
127,386,386,772,0.30598878860473633,23.869656402449436
128,388,388,776,0.30730199813842773,23.124501286195255
129,392,392,784,0.3099820613861084,23.149328377794518
130,396,396,792,0.3151359558105469,23.215561523934184
131,398,398,796,0.3172469139099121,22.85033307290678
132,400,400,800,0.320904016494751,22.734638782003458
133,402,402,804,0.3227870464324951,22.034492601362444
134,406,406,812,0.32555198669433594,22.03470805771167
135,408,408,816,0.3272829055786133,20.267372641775182
136,412,412,824,0.33960914611816406,20.246939110776793
137,414,414,828,0.34471702575683594,18.621050064706424
138,420,420,840,0.34987401962280273,18.62050186296915
139,424,424,848,0.35263991355895996,18.604731339084537
140,426,426,852,0.35439205169677734,18.28569076951044
141,430,430,860,0.3566930294036865,18.25929530312601
142,432,432,864,0.3581809997558594,16.073354066111847
143,436,436,872,0.3607628345489502,16.054788212609992
144,440,440,880,0.3644380569458008,16.000858459471374
145,444,444,888,0.36811184883117676,15.940291716132265
146,446,446,892,0.3699531555175781,15.121231866329708
147,450,450,900,0.3729829788208008,15.143674407780168
148,452,452,904,0.37450098991394043,13.586876436336752
149,456,456,912,0.3766050338745117,13.677500722518971
150,458,458,916,0.37886810302734375,13.36653466168832
151,462,462,924,0.3895859718322754,13.329561554868746
152,466,466,932,0.39307284355163574,13.356639302294184
153,468,468,936,0.3955409526824951,12.929975249683594
154,472,472,944,0.39837217330932617,12.953606236539827
155,476,476,952,0.40097689628601074,12.9863600374822
156,480,480,960,0.40569186210632324,13.012764427370143
157,484,484,968,0.40807199478149414,12.968375152335739
158,488,488,976,0.4102029800415039,12.944639389041527
159,490,490,980,0.41189098358154297,11.18712633352493
160,494,494,988,0.41433191299438477,11.228704895451074
161,498,498,996,0.41758108139038086,10.857200179936626
162,502,502,1004,0.42369699478149414,10.65782094159033
163,510,510,1020,0.4278299808502197,10.657483168600834
164,512,512,1024,0.4290812015533447,9.245447615018406
165,520,520,1040,0.4330408573150635,9.245136022170414
166,522,522,1044,0.43439793586730957,8.429720695927472
167,526,526,1052,0.43653297424316406,8.507294381690713
168,528,528,1056,0.4380300045013428,8.531101657455224
169,532,532,1064,0.4404029846191406,8.560325653437303
170,534,534,1068,0.44237208366394043,7.589703500604628
171,536,536,1072,0.4436819553375244,7.953682581923545
172,540,540,1080,0.44567298889160156,7.616555722885778
173,544,544,1088,0.44800305366516113,7.574580517953905
174,548,548,1096,0.45029616355895996,7.566321619887049
175,550,550,1100,0.4515509605407715,7.243394234190646
176,554,554,1108,0.4535679817199707,7.268056553781435
177,558,558,1116,0.45540308952331543,7.298242213413232
178,560,560,1120,0.4564979076385498,7.187162948870196
179,564,564,1128,0.45810985565185547,7.1205426126261955
180,568,568,1136,0.45970702171325684,7.074956299939231
181,570,570,1140,0.46080589294433594,7.087459260031892
182,574,574,1148,0.4627799987792969,7.071548680202682
183,576,576,1152,0.46448588371276855,6.821196601189399
184,580,580,1160,0.4669339656829834,6.796033939556196
185,582,582,1164,0.46891117095947266,6.228855834697129
186,588,588,1176,0.47176194190979004,6.236601937179216
187,592,592,1184,0.4733920097351074,6.293919745173412
188,596,596,1192,0.47500181198120117,6.359442289687877
189,598,598,1196,0.47607922554016113,6.521003829996403
190,602,602,1204,0.4776730537414551,6.512558077328322
191,604,604,1208,0.478740930557251,5.847446609088593
192,608,608,1216,0.4807591438293457,5.859913015601478
193,610,610,1220,0.4831380844116211,5.659978771089527
194,614,614,1228,0.48526597023010254,5.670019739357372
195,616,616,1232,0.4866499900817871,5.64224090566438
196,620,620,1240,0.48880887031555176,5.63404288730635
197,624,624,1248,0.4906949996948242,5.602492974419761
198,628,628,1256,0.4923529624938965,5.580511403290075
199,632,632,1264,0.49403810501098633,5.56938012108867
200,634,634,1268,0.49517297744750977,5.435562679775217
201,638,638,1276,0.497204065322876,5.434873864739302
202,640,640,1280,0.498582124710083,4.837847624007281
203,644,644,1288,0.5004730224609375,4.840673819508538
204,646,646,1292,0.5016047954559326,4.6435275391570485
205,650,650,1300,0.5033071041107178,4.640981651519041
206,652,652,1304,0.5044758319854736,4.5142310480180186
207,656,656,1312,0.5067300796508789,4.538011176606119
208,660,660,1320,0.508734941482544,4.560935305809608
209,662,662,1324,0.5100281238555908,4.723550369520581
210,666,666,1332,0.5123240947723389,4.730616050704498
211,668,668,1336,0.5136079788208008,4.556358233995866
212,672,672,1344,0.5158898830413818,4.552716025382665
213,674,674,1348,0.5176410675048828,4.466320291599004
214,678,678,1356,0.5200231075286865,4.465891799332553
215,680,680,1360,0.5214018821716309,4.373901208883922
216,684,684,1368,0.5231490135192871,4.36580800993238
217,688,688,1376,0.5248351097106934,4.3559591903201635
218,692,692,1384,0.5264871120452881,4.358085663279894
219,696,696,1392,0.5281460285186768,4.359842055745048
220,700,700,1400,0.5303390026092529,4.36682935590909
221,704,704,1408,0.5323441028594971,4.374100823418985
222,708,708,1416,0.5342929363250732,4.348138084984157
223,712,712,1424,0.536067008972168,4.326429468286619
224,714,714,1428,0.5372779369354248,4.266774030251781
225,718,718,1436,0.5390090942382812,4.265184141984264
226,722,722,1444,0.5408360958099365,4.253302605378963
227,726,726,1452,0.5426030158996582,4.220596798062843
228,730,730,1460,0.5445849895477295,4.188952159157338
229,734,734,1468,0.5464498996734619,4.1584766482944815
230,738,738,1476,0.5487618446350098,4.112089669454235
231,740,740,1480,0.5501160621643066,3.713281204803934
232,744,744,1488,0.5518798828125,3.7107961217249112
233,748,748,1496,0.5537769794464111,3.676816040407175
234,752,752,1504,0.5554838180541992,3.6187146551633305
235,754,754,1508,0.5565829277038574,3.366097906214236
236,758,758,1516,0.5582818984985352,3.3627573009764546
237,760,760,1520,0.5593969821929932,3.011416037967706
238,764,764,1528,0.5611240863800049,3.0254132918505547
239,768,768,1536,0.5630500316619873,3.046265884426248
240,770,770,1540,0.5647039413452148,2.97333372435844
241,774,774,1548,0.5667760372161865,2.963158100698706
242,776,776,1552,0.5678179264068604,2.422341959974915
243,780,780,1560,0.5695140361785889,2.4165503498222733
244,782,782,1564,0.5706570148468018,2.171991077868256
245,786,786,1572,0.5723409652709961,2.1787124557118887
246,790,790,1580,0.5739881992340088,2.1902494847363414
247,794,794,1588,0.5755839347839355,2.18428848031499
248,798,798,1596,0.5772249698638916,2.170407507663981
249,802,802,1604,0.5789289474487305,2.137938621803869
250,806,806,1612,0.5810308456420898,2.072429053774272
251,810,810,1620,0.5828959941864014,2.0129492395110447
252,812,812,1624,0.5840280055999756,1.677308643836227
253,816,816,1632,0.5857200622558594,1.6788453760448192
254,818,818,1636,0.5869178771972656,1.6505786667931943
255,822,822,1644,0.5885748863220215,1.6396601297292364
256,824,824,1648,0.5896730422973633,1.5488360872138855
257,828,828,1656,0.5913238525390625,1.5434853379498463
258,830,830,1660,0.5923640727996826,1.2276104195492508
259,834,834,1668,0.593925952911377,1.2249832041452464
260,836,836,1672,0.5950069427490234,1.0827841567438554
261,840,840,1680,0.5970518589019775,1.0996045005945234
262,842,842,1684,0.5983932018280029,1.1144954862855911
263,844,844,1688,0.599513053894043,1.0900817375234055
264,848,848,1696,0.6012380123138428,1.0722291506041302
265,850,850,1700,0.6023070812225342,0.99418177011853
266,854,854,1708,0.603909969329834,0.976142243436243
267,858,858,1716,0.605522871017456,0.9476558397360577
268,860,860,1720,0.6065590381622314,0.8263356761838168
269,864,864,1728,0.6083030700683594,0.8079683856437896
270,866,866,1732,0.6093780994415283,0.7607931042946348
271,868,868,1736,0.6104462146759033,0.7045481816105621
272,870,870,1740,0.6116108894348145,0.7676323867150359
273,872,872,1744,0.6129648685455322,0.625838136807829
274,876,876,1752,0.6151230335235596,0.61745450774049
275,878,878,1756,0.6162729263305664,0.5900308022642093
276,882,882,1764,0.6179399490356445,0.5814758852825435
277,886,886,1772,0.6195950508117676,0.5714492992512987
278,888,888,1776,0.6207160949707031,0.5121740816555302
279,892,892,1784,0.6223509311676025,0.5061323176248607
280,894,894,1788,0.62335205078125,0.4765180821003696
281,898,898,1796,0.6249768733978271,0.4783328322671423
282,902,902,1804,0.6267180442810059,0.4803574623863369
283,904,904,1808,0.6278390884399414,0.50668309455898
284,906,906,1812,0.6288940906524658,0.50447473107522
285,908,908,1816,0.6301259994506836,0.5066514735162855
286,912,912,1824,0.6333670616149902,0.5035911119769025
287,914,914,1828,0.6346859931945801,0.45878260016809236
288,918,918,1836,0.636660099029541,0.4581787625598963
289,920,920,1840,0.6380019187927246,0.42717602566710866
290,924,924,1848,0.6404399871826172,0.4284628797956884
291,926,926,1852,0.6419680118560791,0.3554739890212204
292,930,930,1860,0.6438388824462891,0.35553685513548317
293,932,932,1864,0.6448891162872314,0.2735203277270557
294,936,936,1872,0.646895170211792,0.2768641062310735
295,938,938,1876,0.648252010345459,0.23847275312130023
296,942,942,1884,0.6503801345825195,0.23460966792379168
297,944,944,1888,0.6517481803894043,0.14435280310271992
298,948,948,1896,0.6538088321685791,0.14328032700018412
299,950,950,1900,0.6557040214538574,0.10942330235332065
300,956,956,1912,0.659555196762085,0.10897390629600068
301,958,958,1916,0.6608471870422363,0.09676745776368989
302,962,962,1924,0.6630358695983887,0.09838578806363785
303,964,964,1928,0.6645801067352295,0.0918062154682957
304,968,968,1936,0.6668510437011719,0.09128369003144599
305,970,970,1940,0.6681890487670898,0.08183384591143295
306,974,974,1948,0.6701979637145996,0.08201369090261323
307,976,976,1952,0.671489953994751,0.0950657021276129
308,980,980,1960,0.673353910446167,0.09546193218864119
309,982,982,1964,0.6746060848236084,0.09421461155989164
310,986,986,1972,0.6766080856323242,0.0933677534853814
311,990,990,1980,0.678455114364624,0.09274384950822423
312,992,992,1984,0.6798160076141357,0.09158487132481241
313,996,996,1992,0.6825339794158936,0.09163068108841799
314,998,998,1996,0.683908224105835,0.08409951380826897
315,1002,1002,2004,0.6859021186828613,0.08377055567984826
316,1004,1004,2008,0.6871590614318848,0.06372367439109894
317,1008,1008,2016,0.6891510486602783,0.06319521949183127
318,1010,1010,2020,0.690446138381958,0.05119802426645492
319,1014,1014,2028,0.6925630569458008,0.05119415893841506
320,1016,1016,2032,0.6936681270599365,0.0478339415640221
321,1020,1020,2040,0.6954779624938965,0.04780319042481551
322,1022,1022,2044,0.6968650817871094,0.0441973877698274
323,1026,1026,2052,0.6991591453552246,0.04489069923340594
324,1030,1030,2060,0.7011258602142334,0.0456954275445014
325,1032,1032,2064,0.702570915222168,0.03758258398192993
326,1036,1036,2072,0.7047469615936279,0.037391458993738524
327,1038,1038,2076,0.7058498859405518,0.030924722081408618
328,1042,1042,2084,0.7075049877166748,0.030542568484634103
329,1044,1044,2088,0.7086961269378662,0.02568381401033548
330,1048,1048,2096,0.7106540203094482,0.025620221678195776
331,1050,1050,2100,0.7119858264923096,0.01917237687666784
332,1054,1054,2108,0.7140820026397705,0.019686785330804923
333,1056,1056,2112,0.7154591083526611,0.020558709244255624
334,1060,1060,2120,0.7172729969024658,0.02031906664296912
335,1062,1062,2124,0.7186229228973389,0.017501860238667177
336,1066,1066,2132,0.7203230857849121,0.0175582601559654
337,1068,1068,2136,0.721444845199585,0.01601047412373191
338,1072,1072,2144,0.723228931427002,0.01600514837218725
339,1074,1074,2148,0.7243578433990479,0.016048765076789095
340,1078,1078,2156,0.7260470390319824,0.016033443105015976
341,1082,1082,2164,0.7277250289916992,0.015720385292411265
342,1084,1084,2168,0.7289071083068848,0.012734328836700115
343,1088,1088,2176,0.7313930988311768,0.012814544578645837
344,1090,1090,2180,0.7326569557189941,0.01309871109458527
345,1094,1094,2188,0.7342679500579834,0.013056761511620607
346,1096,1096,2192,0.7353060245513916,0.010825750192225314
347,1100,1100,2200,0.7369489669799805,0.010743819134404475
348,1102,1102,2204,0.7380399703979492,0.005123215733988218
349,1104,1104,2208,0.7390918731689453,0.005297060616726412
350,1106,1106,2212,0.7402172088623047,0.006753163238386151
351,1108,1108,2216,0.7413508892059326,0.005406084588457816
352,1110,1110,2220,0.7424759864807129,0.005402350168765224
353,1112,1112,2224,0.7436020374298096,0.0044947352013196
354,1116,1116,2232,0.7452480792999268,0.004399154975203601
355,1118,1118,2236,0.7464351654052734,0.004133567514600145
356,1120,1120,2240,0.7479250431060791,0.003955842519417274
357,1122,1122,2244,0.74959397315979,0.003510233288238851
358,1126,1126,2252,0.7515981197357178,0.003495331839872051
359,1128,1128,2256,0.7531259059906006,0.003068597704213971
360,1132,1132,2264,0.7553191184997559,0.0030402714103274775
361,1134,1134,2268,0.7566540241241455,0.002170877033904617
362,1138,1138,2276,0.7585489749908447,0.0021628295966138467
363,1140,1140,2280,0.7596521377563477,0.001617727236293831
364,1144,1144,2288,0.7614390850067139,0.0015950655538290448
365,1146,1146,2292,0.7626690864562988,0.001230847769193133
366,1150,1150,2300,0.7651729583740234,0.001217942083599155
367,1152,1152,2304,0.7666089534759521,0.0007826954067695624
368,1156,1156,2312,0.7684259414672852,0.0007627611745419927
369,1158,1158,2316,0.769665002822876,0.0006341938913010381
370,1160,1160,2320,0.7708280086517334,0.0005550962341658305
371,1164,1164,2328,0.7728838920593262,0.0005526757203142552
372,1166,1166,2332,0.7742750644683838,0.0005202491499858297
373,1168,1168,2336,0.7754471302032471,0.00029142001176296617
374,1172,1172,2344,0.7773098945617676,0.0002874642310644049
375,1174,1174,2348,0.7786810398101807,0.00020180802493996453
376,1178,1178,2356,0.7807409763336182,0.00019240123754116212
377,1180,1180,2360,0.7823030948638916,0.00013825711596382462
378,1184,1184,2368,0.7840659618377686,0.00013772645536391792
379,1186,1186,2372,0.7852039337158203,0.00013240588020835276
380,1190,1190,2380,0.7869389057159424,0.00013480029815582384
381,1192,1192,2384,0.7879409790039062,0.00014746661690878682
382,1196,1196,2392,0.7896928787231445,0.0001468657636678472
383,1198,1198,2396,0.7908527851104736,0.00010960520580738375
384,1200,1200,2400,0.7918908596038818,0.00013297390216848726
385,1204,1204,2408,0.7935450077056885,0.0001338348527042399
386,1206,1206,2412,0.7946078777313232,5.7178381211997475e-05
387,1210,1210,2420,0.7966568470001221,5.45742254871584e-05
388,1212,1212,2424,0.7981979846954346,3.300166235931101e-05
389,1216,1216,2432,0.8001930713653564,3.298585681932309e-05
390,1218,1218,2436,0.8012599945068359,2.5327511821160442e-05
391,1222,1222,2444,0.8029289245605469,2.517205723506777e-05
392,1224,1224,2448,0.8040928840637207,2.1975171875965316e-05
393,1228,1228,2456,0.8060758113861084,2.134618978288927e-05
394,1230,1230,2460,0.8071050643920898,1.9876769783877535e-05
395,1234,1234,2468,0.808945894241333,1.9999223354716378e-05
396,1236,1236,2472,0.8100669384002686,1.8451926393936446e-05
397,1240,1240,2480,0.8118879795074463,1.8110386918124277e-05
398,1242,1242,2484,0.8131568431854248,1.3605173080577515e-05
399,1244,1244,2488,0.8146061897277832,1.2448575034795795e-05
400,1248,1248,2496,0.81675124168396,1.2452739952095726e-05
401,1250,1250,2500,0.8180418014526367,1.982117464649491e-05
402,1252,1252,2504,0.8192918300628662,2.1884840180064202e-05
403,1254,1254,2508,0.8204360008239746,1.9758361645472178e-05
404,1258,1258,2516,0.8222699165344238,1.9769432242355833e-05
405,1260,1260,2520,0.8237020969390869,2.5000072014336183e-05
406,1264,1264,2528,0.8257720470428467,2.4924918875512958e-05
407,1266,1266,2532,0.8269808292388916,2.4043991970756906e-05
408,1270,1270,2540,0.829010009765625,2.436320335164055e-05
409,1272,1272,2544,0.8315021991729736,2.6029244963865494e-05
410,1276,1276,2552,0.8337719440460205,2.6009704811258416e-05
411,1278,1278,2556,0.8352019786834717,2.5176859026032616e-05
412,1280,1280,2560,0.8366029262542725,2.3615653844899498e-05
413,1284,1284,2568,0.8385531902313232,2.341657761917304e-05
414,1286,1286,2572,0.8396549224853516,1.8670598024073115e-05
415,1290,1290,2580,0.8415579795837402,1.8595581423141994e-05
416,1292,1292,2584,0.8427920341491699,1.6297840488732618e-05
417,1296,1296,2592,0.8445398807525635,1.6314718664034444e-05
418,1298,1298,2596,0.8457939624786377,1.5316657140829193e-05
419,1302,1302,2604,0.8479681015014648,1.512813912540878e-05
420,1304,1304,2608,0.8493180274963379,1.4231123032004689e-05
421,1308,1308,2616,0.8511600494384766,1.4111672498984262e-05
422,1310,1310,2620,0.8532638549804688,1.3261920457807719e-05
423,1312,1312,2624,0.8544361591339111,1.2610547400981886e-05
424,1316,1316,2632,0.8561100959777832,1.260642113720678e-05
425,1318,1318,2636,0.8572020530700684,1.2034275755468116e-05
426,1322,1322,2644,0.8590221405029297,1.2013871128147002e-05
427,1324,1324,2648,0.8603899478912354,1.1890473160747206e-05
428,1328,1328,2656,0.8622331619262695,1.1883923889399739e-05
429,1330,1330,2660,0.8634939193725586,1.1481146771075146e-05
430,1332,1332,2664,0.8656589984893799,1.0954465437862382e-05
431,1336,1336,2672,0.8674030303955078,1.094808305879269e-05
432,1338,1338,2676,0.8685188293457031,1.0447021622894681e-05
433,1342,1342,2684,0.8701679706573486,1.0448139164509485e-05
434,1346,1346,2692,0.8718400001525879,1.0448844022903359e-05
435,1350,1350,2700,0.8734688758850098,1.0431756663820124e-05
436,1352,1352,2704,0.8745169639587402,9.911056849887245e-06
437,1356,1356,2712,0.8762218952178955,9.90433136394131e-06
438,1358,1358,2716,0.877331018447876,9.243488193533267e-06
439,1362,1362,2724,0.8790898323059082,9.218531204169267e-06
440,1364,1364,2728,0.8803520202636719,8.988491003947274e-06
441,1368,1368,2736,0.882472038269043,8.989656976154947e-06
442,1370,1370,2740,0.8836081027984619,8.44459486870619e-06
443,1374,1374,2748,0.8854410648345947,8.435916356575035e-06
444,1376,1376,2752,0.8865799903869629,7.982856004673522e-06
445,1380,1380,2760,0.8883659839630127,7.973290394147625e-06
446,1382,1382,2764,0.8895390033721924,7.880529892645427e-06
447,1386,1386,2772,0.8914060592651367,7.884352726250654e-06
448,1388,1388,2776,0.8925471305847168,7.84526878305769e-06
449,1392,1392,2784,0.894158124923706,7.797284979460528e-06
450,1396,1396,2792,0.8959228992462158,7.737118266959442e-06
451,1400,1400,2800,0.8981518745422363,7.66444736655103e-06
452,1404,1404,2808,0.899946928024292,7.602708137710579e-06
453,1406,1406,2812,0.9010140895843506,7.489072800126451e-06
454,1410,1410,2820,0.9031198024749756,7.498381592085934e-06
455,1414,1414,2828,0.9048409461975098,7.506919814659341e-06
456,1418,1418,2836,0.9065289497375488,7.457811307176598e-06
457,1422,1422,2844,0.9082350730895996,7.4281680326748756e-06
458,1426,1426,2852,0.9099111557006836,7.410294301735121e-06
459,1430,1430,2860,0.9115819931030273,7.4020729243784444e-06
460,1434,1434,2868,0.9138779640197754,7.3928442816395545e-06
461,1438,1438,2876,0.9162280559539795,7.3751491527218604e-06
462,1440,1440,2880,0.917396068572998,6.929242999831331e-06
463,1444,1444,2888,0.9191110134124756,6.926831133569067e-06
464,1446,1446,2892,0.9201788902282715,6.692016654596955e-06
465,1450,1450,2900,0.9218349456787109,6.6896168391394895e-06
466,1452,1452,2904,0.9230170249938965,6.525480898744718e-06
467,1456,1456,2912,0.9247369766235352,6.51730647405202e-06
468,1460,1460,2920,0.9263401031494141,6.489570978374104e-06
469,1464,1464,2928,0.9280431270599365,6.391764145519119e-06
470,1468,1468,2936,0.9299421310424805,6.321135970210889e-06
471,1472,1472,2944,0.9322569370269775,6.219894316927821e-06
472,1476,1476,2952,0.9339351654052734,6.143801329017151e-06
473,1480,1480,2960,0.9355881214141846,6.079730269448191e-06
474,1484,1484,2968,0.9371850490570068,6.0174381815158995e-06
475,1488,1488,2976,0.9387750625610352,5.973606562292844e-06
476,1490,1490,2980,0.9398400783538818,5.859031716681784e-06
477,1494,1494,2988,0.9414529800415039,5.863496426172787e-06
478,1498,1498,2996,0.9431369304656982,5.872451879440632e-06
479,1502,1502,3004,0.9446988105773926,5.867059940101171e-06
480,1506,1506,3012,0.9468848705291748,5.86030682825367e-06
481,1510,1510,3020,0.9489119052886963,5.858115969203936e-06
482,1512,1512,3024,0.9499950408935547,5.8957964483852265e-06
483,1516,1516,3032,0.9516549110412598,5.8951590062861214e-06
484,1518,1518,3036,0.9527370929718018,5.72976364310307e-06
485,1522,1522,3044,0.9543848037719727,5.728558221562707e-06
486,1526,1526,3052,0.9559919834136963,5.702584985556314e-06
487,1528,1528,3056,0.9570209980010986,5.5485326129200985e-06
488,1532,1532,3064,0.9587130546569824,5.546452484850306e-06
489,1536,1536,3072,0.9603400230407715,5.4966028528724564e-06
490,1540,1540,3080,0.9618968963623047,5.452190976029669e-06
491,1542,1542,3084,0.9631638526916504,5.067843858341803e-06
492,1546,1546,3092,0.9652318954467773,5.043633450441121e-06
493,1550,1550,3100,0.9669549465179443,4.98698727824376e-06
494,1552,1552,3104,0.9680368900299072,4.733235186904494e-06
495,1556,1556,3112,0.9695339202880859,4.6918680709495675e-06
496,1560,1560,3120,0.9711089134216309,4.611756253325439e-06
497,1562,1562,3124,0.9721858501434326,4.146200126342592e-06
498,1566,1566,3132,0.9738020896911621,4.117093112654402e-06
499,1568,1568,3136,0.974761962890625,3.5987890214528306e-06
500,1572,1572,3144,0.9766170978546143,3.5856343174600624e-06
501,1574,1574,3148,0.9777657985687256,3.5802620459435275e-06
502,1578,1578,3156,0.9795620441436768,3.5837737186739105e-06
503,1580,1580,3160,0.9809510707855225,3.1865929486230016e-06
504,1584,1584,3168,0.9827671051025391,3.1754062774780323e-06
505,1586,1586,3172,0.9839270114898682,2.8346939870971255e-06
506,1590,1590,3180,0.985572099685669,2.8257300073164515e-06
507,1592,1592,3184,0.9866609573364258,2.036787122960959e-06
508,1596,1596,3192,0.9882349967956543,2.0317785356382956e-06
509,1598,1598,3196,0.9892690181732178,1.7320904817097471e-06
510,1602,1602,3204,0.9909839630126953,1.7211274325745762e-06
511,1604,1604,3208,0.9920687675476074,1.1732245184248313e-06
512,1608,1608,3216,0.9937009811401367,1.171197027360904e-06
513,1610,1610,3220,0.9949660301208496,1.016456394609122e-06
514,1614,1614,3228,0.9972469806671143,9.841462542681256e-07
515,1616,1616,3232,0.9987211227416992,6.118057171988767e-07
516,1620,1620,3240,1.0005629062652588,6.121798605818185e-07
517,1622,1622,3244,1.001749038696289,3.861464392684866e-07
518,1626,1626,3252,1.0038468837738037,3.821398877335014e-07
519,1628,1628,3256,1.0050098896026611,2.5592157726350706e-07
520,1632,1632,3264,1.006875991821289,2.536371539463289e-07
521,1634,1634,3268,1.0082809925079346,1.1618408279900905e-07
522,1638,1638,3276,1.0103991031646729,1.2089321899111383e-07
523,1640,1640,3280,1.0116548538208008,1.424417632733821e-07
524,1644,1644,3288,1.014059066772461,1.3934629805589793e-07
525,1646,1646,3292,1.015429973602295,1.3984288216306595e-07
526,1650,1650,3300,1.0174601078033447,1.404511067448766e-07
527,1652,1652,3304,1.0187220573425293,1.1906502095371252e-07
528,1656,1656,3312,1.0206248760223389,1.1417637324484531e-07
529,1658,1658,3316,1.0218369960784912,5.6224394029413816e-08
530,1662,1662,3324,1.0238609313964844,5.542824510484934e-08
531,1664,1664,3328,1.0250828266143799,6.547566044901032e-08
532,1668,1668,3336,1.0269849300384521,6.871277946629561e-08
533,1670,1670,3340,1.0281879901885986,1.0020244189945515e-07
534,1674,1674,3348,1.0310349464416504,1.0007477158069378e-07
535,1676,1676,3352,1.0326159000396729,6.496418336610077e-08
536,1680,1680,3360,1.034553050994873,6.200218649610179e-08
537,1682,1682,3364,1.0357909202575684,3.257468961237464e-09


==> plot_data/quadratic_minimax_problem_n20_alpha0/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,8.392333984375e-05,4.387061074692293
200,201,200,401,0.00596308708190918,0.1842133593717011
400,401,400,801,0.013149023056030273,0.08950090778682597
601,602,601,1203,0.019085168838500977,0.0640727904903761
801,802,801,1603,0.026002883911132812,0.05368010844351703
1001,1002,1001,2003,0.03272700309753418,0.04784400270691025
1201,1202,1201,2403,0.038706064224243164,0.043962346568317545
1401,1402,1401,2803,0.04642510414123535,0.040170424392327105
1602,1603,1602,3205,0.05220603942871094,0.0378297155531487
1802,1803,1802,3605,0.05798912048339844,0.03500764031340371
2002,2003,2002,4005,0.06401896476745605,0.033218977387609094
2202,2203,2202,4405,0.07025623321533203,0.031712977453885745
2402,2403,2402,4805,0.07633113861083984,0.030488556797115297
2603,2604,2603,5207,0.08235502243041992,0.029160518425359824
2803,2804,2803,5607,0.08842611312866211,0.02808380132600252
3003,3004,3003,6007,0.09497809410095215,0.027439038899275816
3203,3204,3203,6407,0.10264921188354492,0.02695027946362406
3403,3404,3403,6807,0.11031413078308105,0.026584533343648
3604,3605,3604,7209,0.11766409873962402,0.02608917186135332
3804,3805,3804,7609,0.12536191940307617,0.029376093689549996
4004,4005,4004,8009,0.13289308547973633,0.025416334225533774
4204,4205,4204,8409,0.14143109321594238,0.024972310198149255
4404,4405,4404,8809,0.14855098724365234,0.024715147719762857
4605,4606,4605,9211,0.15561914443969727,0.024591685184676682
4805,4806,4805,9611,0.16398906707763672,0.02880578201952542
5005,5006,5005,10011,0.1708831787109375,0.02474827063384724
5205,5206,5205,10411,0.17736601829528809,0.02527854875902983
5405,5406,5405,10811,0.18422198295593262,0.027694679864959045
5606,5607,5606,11213,0.19057607650756836,0.02795125230114081
5806,5807,5806,11613,0.19726204872131348,0.023608594264080074
6006,6007,6006,12013,0.20487403869628906,0.023527162933789102
6206,6207,6206,12413,0.21230220794677734,0.023341135626410606
6406,6407,6406,12813,0.21848511695861816,0.02310628117723416
6607,6608,6607,13215,0.22456598281860352,0.023122723586407712
6807,6808,6807,13615,0.23079395294189453,0.02377070920682427
7007,7008,7007,14015,0.2368299961090088,0.022869241994367823
7207,7208,7207,14415,0.24302101135253906,0.022819616348137704
7407,7408,7407,14815,0.2491300106048584,0.022491314432376227
7608,7609,7608,15217,0.25562500953674316,0.02251223999144792
7808,7809,7808,15617,0.26163411140441895,0.022361100974653488
8008,8009,8008,16017,0.2675960063934326,0.022206739994266353
8208,8209,8208,16417,0.2734389305114746,0.022090115079058198
8408,8409,8408,16817,0.27960801124572754,0.02201226857961251
8609,8610,8609,17219,0.28551197052001953,0.02206761219570357
8809,8810,8809,17619,0.291409969329834,0.02532542037528179
9009,9010,9009,18019,0.2972989082336426,0.02170092808990991
9209,9210,9209,18419,0.3033599853515625,0.021560398210116696
9409,9410,9409,18819,0.3095860481262207,0.021370971442305983
9610,9611,9610,19221,0.3158071041107178,0.023018260673251138
9810,9811,9810,19621,0.32196617126464844,0.022092837094809345
10010,10011,10010,20021,0.32786989212036133,0.021082136954524492
10210,10211,10210,20421,0.3337540626525879,0.02105114947261687
10410,10411,10410,20821,0.3396790027618408,0.02104825035317345
10611,10612,10611,21223,0.34578514099121094,0.020883696401520716
10811,10812,10811,21623,0.35199689865112305,0.02103615413548143
11011,11012,11011,22023,0.3580470085144043,0.020849232031725236
11211,11212,11211,22423,0.3639209270477295,0.020621427912150585
11411,11412,11411,22823,0.36974406242370605,0.020507565956851187
11612,11613,11612,23225,0.37547898292541504,0.020163599691971262
11812,11813,11812,23625,0.38126325607299805,0.020357944259584922
12012,12013,12012,24025,0.3872079849243164,0.02329837724243542
12212,12213,12212,24425,0.39293909072875977,0.02006217064033194
12412,12413,12412,24825,0.3987252712249756,0.019968714368819664
12613,12614,12613,25227,0.4045541286468506,0.019621998615492634
12813,12814,12813,25627,0.4103271961212158,0.019899776004216118
13013,13014,13013,26027,0.4161970615386963,0.01993662452670902
13213,13214,13213,26427,0.42197394371032715,0.019652571174822473
13413,13414,13413,26827,0.4277491569519043,0.022252880702721165
13614,13615,13614,27229,0.4342200756072998,0.01925047727339765
13814,13815,13814,27629,0.4399750232696533,0.019169855049710513
14014,14015,14014,28029,0.44704198837280273,0.0236484376452837
14214,14215,14214,28429,0.45429515838623047,0.019161913414835825
14414,14415,14414,28829,0.4602701663970947,0.020047409941289892
14615,14616,14615,29231,0.46623706817626953,0.018652850296161528
14815,14816,14815,29631,0.472365140914917,0.020111290038272937
15015,15016,15015,30031,0.4783952236175537,0.018503485751028174
15215,15216,15215,30431,0.4847140312194824,0.022785686975259425
15415,15416,15415,30831,0.4907369613647461,0.022488827658294897
15616,15617,15616,31233,0.49677324295043945,0.022505017714190806
15816,15817,15816,31633,0.5029451847076416,0.01821839774626749
16016,16017,16016,32033,0.5090959072113037,0.01805512329677396
16216,16217,16216,32433,0.5150740146636963,0.02059380622184377
16416,16417,16416,32833,0.5211362838745117,0.017892965512531923
16617,16618,16617,33235,0.5271739959716797,0.017968702738862623
16817,16818,16817,33635,0.5330660343170166,0.017881281551843195
17017,17018,17017,34035,0.5392539501190186,0.017607733741237874
17217,17218,17217,34435,0.5454950332641602,0.01844185460455576
17417,17418,17417,34835,0.5514712333679199,0.020809148761590388
17618,17619,17618,35237,0.5574369430541992,0.017501993938133356
17818,17819,17818,35637,0.5638132095336914,0.017329461393972474
18018,18019,18018,36037,0.5704550743103027,0.017220536921859684
18218,18219,18218,36437,0.5777370929718018,0.017163429339517384
18418,18419,18418,36837,0.5841779708862305,0.017427318626169475
18619,18620,18619,37239,0.5908281803131104,0.020523368668403007
18819,18820,18819,37639,0.5973050594329834,0.01685197121953309
19019,19020,19019,38039,0.6035699844360352,0.021856660079918353
19219,19220,19219,38439,0.6097431182861328,0.016747392759050222
19419,19420,19419,38839,0.6163280010223389,0.016581568709277673
19620,19621,19620,39241,0.6232771873474121,0.016589931914777367
19820,19821,19820,39641,0.6302900314331055,0.016499111602322994
20020,20021,20020,40041,0.6365640163421631,0.02035303289088751
20220,20221,20220,40441,0.6427550315856934,0.017184700367162003
20420,20421,20420,40841,0.64906907081604,0.01626664845034462
20621,20622,20621,41243,0.6552200317382812,0.018844066069117336
20821,20822,20821,41643,0.66121506690979,0.015877683449230566
21021,21022,21021,42043,0.6673181056976318,0.016889381576759756
21221,21222,21221,42443,0.673382043838501,0.018468896118016307
21421,21422,21421,42843,0.679440975189209,0.015771494062805747
21622,21623,21622,43245,0.6859970092773438,0.01583270682596724
21822,21823,21822,43645,0.6922240257263184,0.015595182074509889
22022,22023,22022,44045,0.698371171951294,0.0155996405448533
22222,22223,22222,44445,0.7045419216156006,0.015460291942131082
22422,22423,22422,44845,0.7106409072875977,0.015551359833280098
22623,22624,22623,45247,0.7167580127716064,0.015364964758678212
22823,22824,22823,45647,0.722999095916748,0.015259065297969962
23023,23024,23023,46047,0.7290802001953125,0.0151621643664495
23223,23224,23223,46447,0.7351911067962646,0.015133444717631216
23423,23424,23423,46847,0.7414772510528564,0.015979810705922953
23624,23625,23624,47249,0.7476301193237305,0.01722911183769795
23824,23825,23824,47649,0.7537322044372559,0.014810854232805483
24024,24025,24024,48049,0.7597920894622803,0.015275523085091556
24224,24225,24224,48449,0.765869140625,0.014709586575179127
24424,24425,24424,48849,0.772284984588623,0.01681523933371397
24625,24626,24625,49251,0.7784140110015869,0.015242620309582471
24825,24826,24825,49651,0.7844760417938232,0.014505814625316516
25025,25026,25025,50051,0.790524959564209,0.014420089579536171
25225,25226,25225,50451,0.7966358661651611,0.014477080655222387
25425,25426,25425,50851,0.8027269840240479,0.014348836205393123
25626,25627,25626,51253,0.8088440895080566,0.014235110793421385
25826,25827,25826,51653,0.8148989677429199,0.014241671170314437
26026,26027,26026,52053,0.8209578990936279,0.013992561867390996
26226,26227,26226,52453,0.8270111083984375,0.01398753211140654
26426,26427,26426,52853,0.8330380916595459,0.014147185056737423
26627,26628,26627,53255,0.8391051292419434,0.015957573560474694
26827,26828,26827,53655,0.845142126083374,0.013737339576572749
27027,27028,27027,54055,0.8511919975280762,0.013618643265642823
27227,27228,27227,54455,0.85725998878479,0.015659829778024274
27427,27428,27427,54855,0.8637239933013916,0.013505103169415852
27628,27629,27628,55257,0.8697431087493896,0.01349951621601422
27828,27829,27828,55657,0.875669002532959,0.01342429139348619
28028,28029,28028,56057,0.8817222118377686,0.014339094300417046
28228,28229,28228,56457,0.8878011703491211,0.013366143462820135
28428,28429,28428,56857,0.8939299583435059,0.014336431517761884
28629,28630,28629,57259,0.9001600742340088,0.013252705114974263
28829,28830,28829,57659,0.9063811302185059,0.013181256507363083
29029,29030,29029,58059,0.9125480651855469,0.013063788847197983
29229,29230,29229,58459,0.9187159538269043,0.015745701304893764
29429,29430,29429,58859,0.9248089790344238,0.014587684914652909
29630,29631,29630,59261,0.9310240745544434,0.013654264398053444
29830,29831,29830,59661,0.9372920989990234,0.012745491950715875
30030,30031,30030,60061,0.9433979988098145,0.013995564545420065
30230,30231,30230,60461,0.9497780799865723,0.012629157072454248
30430,30431,30430,60861,0.9561190605163574,0.012609507220559986
30631,30632,30631,61263,0.9625170230865479,0.012486798200242248
30831,30832,30831,61663,0.9694032669067383,0.012429828369275824
31031,31032,31031,62063,0.9757640361785889,0.01233793456389007
31231,31232,31231,62463,0.9817290306091309,0.012273760072572065
31431,31432,31431,62863,0.9877619743347168,0.013390922066411737
31632,31633,31632,63265,0.9939792156219482,0.014677482178872719
31832,31833,31832,63665,0.9999749660491943,0.012135463319280044
32032,32033,32032,64065,1.0069389343261719,0.01538484873071717
32232,32233,32232,64465,1.0131299495697021,0.014984331008584479
32432,32433,32432,64865,1.0202341079711914,0.011938306999697378
32633,32634,32633,65267,1.026522159576416,0.01210897758471628
32833,32834,32833,65667,1.0324649810791016,0.012529778225425831
33033,33034,33033,66067,1.0384151935577393,0.011662466355523291
33233,33234,33233,66467,1.044335126876831,0.015335092939516353
33433,33434,33433,66867,1.0502829551696777,0.011658389270715408
33634,33635,33634,67269,1.0562701225280762,0.011550851084817532
33834,33835,33834,67669,1.0625770092010498,0.011442153251707577
34034,34035,34034,68069,1.0685770511627197,0.011533268032610506
34234,34235,34234,68469,1.074627161026001,0.011402700849156738
34434,34435,34434,68869,1.0809710025787354,0.011323583234960395
34635,34636,34635,69271,1.087151050567627,0.011367177427921291
34835,34836,34835,69671,1.0939030647277832,0.011344341238345696
35035,35036,35035,70071,1.10001802444458,0.011161932342710287
35235,35236,35235,70471,1.1061089038848877,0.01355887504151913
35435,35436,35435,70871,1.1121799945831299,0.013314579110700196
35636,35637,35636,71273,1.1182451248168945,0.01294219570337818
35836,35837,35836,71673,1.1242640018463135,0.01097024139430618
36036,36037,36036,72073,1.1303081512451172,0.010965834461048063
36236,36237,36236,72473,1.136348009109497,0.011888154741444171
36436,36437,36436,72873,1.142388105392456,0.010759902989858027
36637,36638,36637,73275,1.148463249206543,0.010689466699165125
36837,36838,36837,73675,1.154466152191162,0.010703263173325608
37037,37038,37037,74075,1.1604831218719482,0.010691816212449455
37237,37238,37237,74475,1.1664690971374512,0.011457087115894497
37437,37438,37437,74875,1.1723041534423828,0.01057078430266816
37638,37639,37638,75277,1.1780641078948975,0.011290875105509196
37838,37839,37838,75677,1.183912992477417,0.010352720637895257
38038,38039,38038,76077,1.1897921562194824,0.011165393564655403
38238,38239,38238,76477,1.1956291198730469,0.010250936751035156
38438,38439,38438,76877,1.2014999389648438,0.010291781271826337
38639,38640,38639,77279,1.2076449394226074,0.010090867243373346
38839,38840,38839,77679,1.2135770320892334,0.01016562891382518
39039,39040,39039,78079,1.2226932048797607,0.011701398280788219
39239,39240,39239,78479,1.2294721603393555,0.010245664140523265
39439,39440,39439,78879,1.2353920936584473,0.00996534469500198
39640,39641,39640,79281,1.2437961101531982,0.009948367557898762
39840,39841,39840,79681,1.2500810623168945,0.009903463810679662
40040,40041,40040,80081,1.2582800388336182,0.00980710031279822
40240,40241,40240,80481,1.2649180889129639,0.01203257202896133
40440,40441,40440,80881,1.2708699703216553,0.009729798017285693
40641,40642,40641,81283,1.2779450416564941,0.009982092153465481
40841,40842,40841,81683,1.2844059467315674,0.009637874136854494
41041,41042,41041,82083,1.29062819480896,0.009570404293112096
41241,41242,41241,82483,1.2967901229858398,0.011148533065216506
41441,41442,41441,82883,1.3029050827026367,0.009481025770236252
41642,41643,41642,83285,1.309061050415039,0.009456963085172672
41842,41843,41842,83685,1.315237045288086,0.009382659323967259
42042,42043,42042,84085,1.3218450546264648,0.011448509340062174
42242,42243,42242,84485,1.3279650211334229,0.009345144855758401
42442,42443,42442,84885,1.3344430923461914,0.009217754436636354
42643,42644,42643,85287,1.3404102325439453,0.009161943486176372
42843,42844,42843,85687,1.3468642234802246,0.009142820677727653
43043,43044,43043,86087,1.3528120517730713,0.010143596241899824
43243,43244,43243,86487,1.3587861061096191,0.008994178343671163
43443,43444,43443,86887,1.3646860122680664,0.009304369683762009
43644,43645,43644,87289,1.3706350326538086,0.008937245085437973
43844,43845,43844,87689,1.3765439987182617,0.009320026988471586
44044,44045,44044,88089,1.3830931186676025,0.008890415276702616
44244,44245,44244,88489,1.3890140056610107,0.008850883211299286
44444,44445,44444,88889,1.3949570655822754,0.009008247036694872
44645,44646,44645,89291,1.4009530544281006,0.008828107987199702
44845,44846,44845,89691,1.4069430828094482,0.010151020588288909
45045,45046,45045,90091,1.4128341674804688,0.008798780492575323
45245,45246,45245,90491,1.4187588691711426,0.008542407031617629
45445,45446,45445,90891,1.4246909618377686,0.008587599773307487
45646,45647,45646,91293,1.430643081665039,0.008585586616359712
45846,45847,45846,91693,1.4365298748016357,0.00856437548795065
46046,46047,46046,92093,1.4426629543304443,0.00847780016859289
46246,46247,46246,92493,1.4487922191619873,0.008436203431380664
46446,46447,46446,92893,1.454787015914917,0.008400786679596282
46647,46648,46647,93295,1.460726022720337,0.009022651241716079
46847,46848,46847,93695,1.4666450023651123,0.00828299455687527
47047,47048,47047,94095,1.472594976425171,0.008653361338931865
47247,47248,47247,94495,1.4783082008361816,0.008244454831417556
47447,47448,47447,94895,1.4840140342712402,0.008443839618910955
47648,47649,47648,95297,1.4897000789642334,0.008097907247944947
47848,47849,47848,95697,1.4957571029663086,0.008118665054317456
48048,48049,48048,96097,1.5032310485839844,0.00818648728571346
48248,48249,48248,96497,1.5106351375579834,0.00829676985019953
48448,48449,48448,96897,1.517035961151123,0.0081780990262309
48649,48650,48649,97299,1.5230610370635986,0.007949077293283629
48849,48850,48849,97699,1.5288410186767578,0.007814239057312032
49049,49050,49049,98099,1.5346181392669678,0.0077974849276984965
49249,49250,49249,98499,1.5407471656799316,0.007809645299363575
49449,49450,49449,98899,1.547408103942871,0.007773459803747118
49650,49651,49650,99301,1.5532801151275635,0.00783703922826673
49850,49851,49850,99701,1.5591180324554443,0.0076902340014995
50050,50051,50050,100101,1.564958095550537,0.007579996032670245
50250,50251,50250,100501,1.5708842277526855,0.00930518785887562
50450,50451,50450,100901,1.5768399238586426,0.0077449079115948635
50651,50652,50651,101303,1.5828521251678467,0.007485673990440684
50851,50852,50851,101703,1.5888011455535889,0.007436660587515145
51051,51052,51051,102103,1.594763994216919,0.007484348524433028
51251,51252,51251,102503,1.6007380485534668,0.007416223104808162
51451,51452,51451,102903,1.6066820621490479,0.007329371516299548
51652,51653,51652,103305,1.6126511096954346,0.007593209689607612
51852,51853,51852,103705,1.618588924407959,0.007262764164795382
52052,52053,52052,104105,1.6245100498199463,0.007295176720471927
52252,52253,52252,104505,1.6304352283477783,0.007174263478162078
52452,52453,52452,104905,1.6363589763641357,0.0071672415049468296
52653,52654,52653,105307,1.6423921585083008,0.007147963595512411
52853,52854,52853,105707,1.6483421325683594,0.007123158366932032
53053,53054,53053,106107,1.6544718742370605,0.007760234507233116
53253,53254,53253,106507,1.6604039669036865,0.007040737099156903
53453,53454,53453,106907,1.6663439273834229,0.006941576805611954
53654,53655,53654,107309,1.67215895652771,0.00855396703792472
53854,53855,53854,107709,1.6778161525726318,0.006918943363875176
54054,54055,54054,108109,1.683495044708252,0.006907321159691736
54254,54255,54254,108509,1.689338207244873,0.006919407245725566
54454,54455,54454,108909,1.695418119430542,0.006905896520878805
54655,54656,54655,109311,1.701267957687378,0.006774720413557326
54855,54856,54855,109711,1.7071502208709717,0.006966943424937531
55055,55056,55055,110111,1.7129158973693848,0.008284943342452038
55255,55256,55255,110511,1.7186739444732666,0.006675640675454933
55455,55456,55455,110911,1.7244360446929932,0.006887294746810684
55656,55657,55656,111313,1.730757236480713,0.006665509007886521
55856,55857,55856,111713,1.7365729808807373,0.006671097530787778
56056,56057,56056,112113,1.742692232131958,0.0065286326538250145
56256,56257,56256,112513,1.7490081787109375,0.006512178681099781
56456,56457,56456,112913,1.7550148963928223,0.007170814998733508
56657,56658,56657,113315,1.7607841491699219,0.007036975323387839
56857,56858,56857,113715,1.7665510177612305,0.006628510898732772
57057,57058,57057,114115,1.7722859382629395,0.006411856692851152
57257,57258,57257,114515,1.7780930995941162,0.006427970010303372
57457,57458,57457,114915,1.783865213394165,0.006296796937530491
57658,57659,57658,115317,1.7897169589996338,0.0065113234634079685
57858,57859,57858,115717,1.7956559658050537,0.006223892145659718
58058,58059,58058,116117,1.8014731407165527,0.006238527342008057
58258,58259,58258,116517,1.8072659969329834,0.006934188763934251
58458,58459,58458,116917,1.8131258487701416,0.006191489784595947
58659,58660,58659,117319,1.819025993347168,0.006129301607581325
58859,58860,58859,117719,1.8248131275177002,0.006128510236352602
59059,59060,59059,118119,1.8306171894073486,0.006012974400067028
59259,59260,59259,118519,1.8365230560302734,0.006503450496967767
59459,59460,59459,118919,1.842345952987671,0.006969063310439132
59660,59661,59660,119321,1.848282814025879,0.005955188446155179
59860,59861,59860,119721,1.8541979789733887,0.005944758400561272
60060,60061,60060,120121,1.8600919246673584,0.005954715249174598
60260,60261,60260,120521,1.8658618927001953,0.005929704913928896
60460,60461,60460,120921,1.8716650009155273,0.005874443116280285
60661,60662,60661,121323,1.878913164138794,0.006368864791791769
60861,60862,60861,121723,1.8869860172271729,0.005843942343254285
61061,61062,61061,122123,1.8939540386199951,0.00573028977690027
61261,61262,61261,122523,1.9010372161865234,0.005761455181750258
61461,61462,61461,122923,1.9074602127075195,0.0056893122943081405
61662,61663,61662,123325,1.9132869243621826,0.005716393864227136
61862,61863,61862,123725,1.9191172122955322,0.005763568976174787
62062,62063,62062,124125,1.924957036972046,0.006830292075994993
62262,62263,62262,124525,1.930811882019043,0.005639443525685054
62462,62463,62462,124925,1.936629056930542,0.006354217891780564
62663,62664,62663,125327,1.9428942203521729,0.005649345742346727
62863,62864,62863,125727,1.949002981185913,0.005922099622513662
63063,63064,63063,126127,1.9551770687103271,0.00549446712282669
63263,63264,63263,126527,1.960773229598999,0.005404755339666591
63463,63464,63463,126927,1.966426134109497,0.005448619248934733
63664,63665,63664,127329,1.9722869396209717,0.00539733937481982
63864,63865,63864,127729,1.9781520366668701,0.006329431523668227
64064,64065,64064,128129,1.9840080738067627,0.006071161406448663
64264,64265,64264,128529,1.9898529052734375,0.005378177169698621
64464,64465,64464,128929,1.9957730770111084,0.006297521759131589
64665,64666,64665,129331,2.001701831817627,0.005499432729780842
64865,64866,64865,129731,2.0076041221618652,0.005206590121344269
65065,65066,65065,130131,2.013468027114868,0.005165210976184468
65265,65266,65265,130531,2.019310235977173,0.005186362543535456
65465,65466,65465,130931,2.0251970291137695,0.0051491589271982436
65666,65667,65666,131333,2.0310862064361572,0.005094684891638816
65866,65867,65866,131733,2.0369300842285156,0.005089414485359224
66066,66067,66066,132133,2.042809247970581,0.005084373667053362
66266,66267,66266,132533,2.0486888885498047,0.005019498584227978
66466,66467,66466,132933,2.054676055908203,0.0057519883578847535
66667,66668,66667,133335,2.060727119445801,0.0059973431784928494
66867,66868,66867,133735,2.066754102706909,0.005198702771323449
67067,67068,67067,134135,2.072866201400757,0.00495725920870504
67267,67268,67267,134535,2.078994035720825,0.004967827608209544
67467,67468,67467,134935,2.085029125213623,0.004912304888524369
67668,67669,67668,135337,2.0911848545074463,0.004907585766098389
67868,67869,67868,135737,2.0972900390625,0.004821251958755352
68068,68069,68068,136137,2.1034791469573975,0.004916036586098999
68268,68269,68268,136537,2.1096949577331543,0.004777763562331958
68468,68469,68468,136937,2.115812063217163,0.0056909401098151815
68669,68670,68669,137339,2.122056007385254,0.004751102848833676
68869,68870,68869,137739,2.1282291412353516,0.004708817096448989
69069,69070,69069,138139,2.1342568397521973,0.004740308783840497
69269,69270,69269,138539,2.1404459476470947,0.00471294447544304
69469,69470,69469,138939,2.146618127822876,0.0046557639966246945
69670,69671,69670,139341,2.1528570652008057,0.005438587423022217
69870,69871,69870,139741,2.159011125564575,0.004620582415964322
70070,70071,70070,140141,2.1652369499206543,0.00467691717402689
70270,70271,70270,140541,2.1713950634002686,0.004633310967836424
70470,70471,70470,140941,2.178497076034546,0.005135959582836533
70671,70672,70671,141343,2.184680938720703,0.004818497442031835
70871,70872,70871,141743,2.190891981124878,0.004537664851487004
71071,71072,71071,142143,2.1971330642700195,0.004478370570521063
71271,71272,71271,142543,2.203507900238037,0.0044380542917019416
71471,71472,71471,142943,2.2098512649536133,0.00550553512503129
71672,71673,71672,143345,2.2163431644439697,0.004418308941482875
71872,71873,71872,143745,2.2228901386260986,0.0044010790322850345
72072,72073,72072,144145,2.2295732498168945,0.004550585163954764
72272,72273,72272,144545,2.2354471683502197,0.004336360023473361
72472,72473,72472,144945,2.2421350479125977,0.004386385452943663
72673,72674,72673,145347,2.2483861446380615,0.004266148950698774
72873,72874,72873,145747,2.2545549869537354,0.004306013271173263
73073,73074,73073,146147,2.260401964187622,0.004368505208174496
73273,73274,73273,146547,2.2671220302581787,0.004220452475308665
73473,73474,73473,146947,2.2731690406799316,0.004232532645310114
73674,73675,73674,147349,2.27935528755188,0.00420454142805173
73874,73875,73874,147749,2.2855072021484375,0.0041778686714670525
74074,74075,74074,148149,2.29158091545105,0.0041492419813747
74274,74275,74274,148549,2.297776937484741,0.0049413642641980594
74474,74475,74474,148949,2.3039159774780273,0.004094237889205395
74675,74676,74675,149351,2.3100149631500244,0.004347989379374318
74875,74876,74875,149751,2.3160719871520996,0.004352237742207087
75075,75076,75075,150151,2.3221099376678467,0.004111572405706692
75275,75276,75275,150551,2.328226089477539,0.004016017647812896
75475,75476,75475,150951,2.3343141078948975,0.003967689654041947
75676,75677,75676,151353,2.340445041656494,0.0039585771005068125
75876,75877,75876,151753,2.3465962409973145,0.004016242266465073
76076,76077,76076,152153,2.3527119159698486,0.003922439245840739
76276,76277,76276,152553,2.3587920665740967,0.0039232251695556376
76476,76477,76476,152953,2.365058183670044,0.003927968373853759
76677,76678,76677,153355,2.37115216255188,0.0039155854501979346
76877,76878,76877,153755,2.377155065536499,0.0038379269602644914
77077,77078,77077,154155,2.3830771446228027,0.004017083666070026
77277,77278,77277,154555,2.388982057571411,0.00380998928413208
77477,77478,77477,154955,2.394925117492676,0.004253593401453428
77678,77679,77678,155357,2.4008991718292236,0.004505435811539767
77878,77879,77878,155757,2.4071109294891357,0.003796784374044313
78078,78079,78078,156157,2.4129929542541504,0.003761760084559125
78278,78279,78278,156557,2.418830156326294,0.003752619746253092
78478,78479,78478,156957,2.4246721267700195,0.004442957393857844
78679,78680,78679,157359,2.4305460453033447,0.0037194109519679826
78879,78880,78879,157759,2.4364190101623535,0.004289927016560843
79079,79080,79079,158159,2.442671060562134,0.0036335026142721603
79279,79280,79279,158559,2.4497642517089844,0.0036619962806652235
79479,79480,79479,158959,2.455785036087036,0.003637455317627421
79680,79681,79680,159361,2.4616808891296387,0.0036215236095768003
79880,79881,79880,159761,2.467574119567871,0.0035811287507339614
80080,80081,80080,160161,2.473362922668457,0.003549600837316861
80280,80281,80280,160561,2.4792211055755615,0.003525268798222221
80480,80481,80480,160961,2.484923839569092,0.003530853858326753
80681,80682,80681,161363,2.4906370639801025,0.0035012477240758816
80881,80882,80881,161763,2.496381998062134,0.0035396966291925324
81081,81082,81081,162163,2.502146005630493,0.0034937515058734423
81281,81282,81281,162563,2.5079381465911865,0.0034794799775795236
81481,81482,81481,162963,2.5136141777038574,0.0034531336162571284
81682,81683,81682,163365,2.51933217048645,0.0035234022151713327
81882,81883,81882,163765,2.525048017501831,0.003391207761783828
82082,82083,82082,164165,2.530730962753296,0.00342141062564471
82282,82283,82282,164565,2.536450147628784,0.0033739122836171555
82482,82483,82482,164965,2.542114019393921,0.003362924229011136
82683,82684,82683,165367,2.547842025756836,0.003337813068802138
82883,82884,82883,165767,2.5535471439361572,0.00333957901680127
83083,83084,83083,166167,2.559235095977783,0.003308847359710524
83283,83284,83283,166567,2.5649170875549316,0.0032614769889697487
83483,83484,83483,166967,2.57066011428833,0.0032901329092645953
83684,83685,83684,167369,2.5762760639190674,0.0032522562928965267
83884,83885,83884,167769,2.5819830894470215,0.003430670210142134
84084,84085,84084,168169,2.587728977203369,0.0032498172627532704
84284,84285,84284,168569,2.5934841632843018,0.0032878764332279478
84484,84485,84484,168969,2.5991880893707275,0.003178506228619986
84685,84686,84685,169371,2.605015993118286,0.0031827645694890837
84885,84886,84885,169771,2.6107521057128906,0.003153012815661423
85085,85086,85085,170171,2.6165740489959717,0.003131743231737187
85285,85286,85285,170571,2.6222851276397705,0.0038548792050088483
85485,85486,85485,170971,2.6281180381774902,0.0031241580021964623
85686,85687,85686,171373,2.6347761154174805,0.00309213250228823
85886,85887,85886,171773,2.640895128250122,0.003653988181409942
86086,86087,86086,172173,2.6471450328826904,0.0030565048907959962
86286,86287,86286,172573,2.6534039974212646,0.0030133734220454582
86486,86487,86486,172973,2.6596450805664062,0.003035299043922183
86687,86688,86687,173375,2.6660962104797363,0.0034117501226775294
86887,86888,86887,173775,2.672119140625,0.0029837631199694696
87087,87088,87087,174175,2.6783318519592285,0.0029793056537222285
87287,87288,87287,174575,2.6846542358398438,0.003472783261981378
87487,87488,87487,174975,2.6917810440063477,0.0034719139830723294
87688,87689,87688,175377,2.6986539363861084,0.0029383688664977115
87888,87889,87888,175777,2.7064080238342285,0.0029286020786804426
88088,88089,88088,176177,2.7125189304351807,0.002890123528292857
88288,88289,88288,176577,2.7185258865356445,0.003254860081970538
88488,88489,88488,176977,2.7245709896087646,0.0028831670632926687
88689,88690,88689,177379,2.730557918548584,0.0028617709267257417
88889,88890,88889,177779,2.736582040786743,0.0028787458454369707
89089,89090,89089,178179,2.7438299655914307,0.002854293197406956
89289,89290,89289,178579,2.7501399517059326,0.0028335521645838557
89489,89490,89489,178979,2.756319046020508,0.0027986226215475658
89690,89691,89690,179381,2.7623910903930664,0.002797017562184415
89890,89891,89890,179781,2.768386125564575,0.0028771675413115853
90090,90091,90090,180181,2.774447202682495,0.0027601793921146586
90290,90291,90290,180581,2.780560255050659,0.0027510336896191382
90490,90491,90490,180981,2.7874722480773926,0.0027328906662145115
90691,90692,90691,181383,2.7946600914001465,0.002765741384548856
90891,90892,90891,181783,2.8012499809265137,0.0027078023550482838
91091,91092,91091,182183,2.808372974395752,0.0026857046355221828
91291,91292,91291,182583,2.8166069984436035,0.0027055606298255503
91491,91492,91491,182983,2.824234962463379,0.0029223895109068325
91692,91693,91692,183385,2.8326730728149414,0.0030508969340298
91892,91893,91892,183785,2.8407440185546875,0.002642757492388949
92092,92093,92092,184185,2.848912239074707,0.002747672159544797
92292,92293,92292,184585,2.8567261695861816,0.002632957874924081
92492,92493,92492,184985,2.8642420768737793,0.002662579054659466
92693,92694,92693,185387,2.8719630241394043,0.002595387658751011
92893,92894,92893,185787,2.8790111541748047,0.002602040684684526
93093,93094,93093,186187,2.8853180408477783,0.002546957466465552
93293,93294,93293,186587,2.891637086868286,0.0025601583943741673
93493,93494,93493,186987,2.898045063018799,0.0025336463686294664
93694,93695,93694,187389,2.904486894607544,0.0025248093091717414
93894,93895,93894,187789,2.9108500480651855,0.0025017686748316716
94094,94095,94094,188189,2.9174411296844482,0.002482368142545164
94294,94295,94294,188589,2.923586130142212,0.002484588387495414
94494,94495,94494,188989,2.9296951293945312,0.002484490234709274
94695,94696,94695,189391,2.9358069896698,0.0024628206096987603
94895,94896,94895,189791,2.9423019886016846,0.002445507890017871
95095,95096,95095,190191,2.949517011642456,0.002421010781207876
95295,95296,95295,190591,2.9557950496673584,0.002797926268710221
95495,95496,95495,190991,2.9620649814605713,0.0024683017547263387
95696,95697,95696,191393,2.968714952468872,0.002819048677648437
95896,95897,95896,191793,2.9756102561950684,0.0023796505504858297
96096,96097,96096,192193,2.982501983642578,0.002366768593489598
96296,96297,96296,192593,2.989962100982666,0.00234162770136808
96496,96497,96496,192993,2.997338056564331,0.0023410311782760284
96697,96698,96697,193395,3.0042402744293213,0.0023317232604085276
96897,96898,96897,193795,3.010906934738159,0.002315832830699188
97097,97098,97097,194195,3.016913890838623,0.0023151788170183716
97297,97298,97297,194595,3.023452043533325,0.002327021936142518
97497,97498,97497,194995,3.0296928882598877,0.002345124183046016
97698,97699,97698,195397,3.0362401008605957,0.002273092235491242
97898,97899,97898,195797,3.0429370403289795,0.0022919999418918166
98098,98099,98098,196197,3.0491230487823486,0.002267009526085826
98298,98299,98298,196597,3.0556600093841553,0.002257641773356471
98498,98499,98498,196997,3.0620250701904297,0.0022360462938346252
98699,98700,98699,197399,3.068444013595581,0.002236744638619309
98899,98900,98899,197799,3.0745880603790283,0.0022276731004945796
99099,99100,99099,198199,3.080963134765625,0.002186273404782907
99299,99300,99299,198599,3.0873401165008545,0.002199848622595925
99499,99500,99499,198999,3.093677043914795,0.002172153627115488
99700,99701,99700,199401,3.0999109745025635,0.0021663422529639357
99900,99901,99900,199801,3.106419086456299,0.0021586298501468882
100100,100101,100100,200201,3.112997055053711,0.0021607337677454173
100300,100301,100300,200601,3.121328830718994,0.0021265191688241984
100501,100502,100501,201003,3.1273579597473145,0.002477897831871667
100701,100702,100701,201403,3.1336541175842285,0.0021588591862794523
100901,100902,100901,201803,3.139907121658325,0.002097600059635112
101101,101102,101101,202203,3.146394968032837,0.0020934499449136437
101301,101302,101301,202603,3.1525208950042725,0.002078212015683252
101502,101503,101502,203005,3.1586930751800537,0.002135682411642782
101702,101703,101702,203405,3.1647841930389404,0.0020467714399281024
101902,101903,101902,203805,3.1708521842956543,0.0020564319544325205
102102,102103,102102,204205,3.176826238632202,0.0020544327762940595
102302,102303,102302,204605,3.1827900409698486,0.002025394241734383
102503,102504,102503,205007,3.188847064971924,0.002013846267478056
102703,102704,102703,205407,3.194821834564209,0.0019795264523525453
102903,102904,102903,205807,3.2008020877838135,0.0020271959647076006
103103,103104,103103,206207,3.2068421840667725,0.0020624523265620727
103303,103304,103303,206607,3.2129290103912354,0.002365685617369958
103504,103505,103504,207009,3.2192740440368652,0.0019512594178104565
103704,103705,103704,207409,3.225306272506714,0.001959356593229385
103904,103905,103904,207809,3.2313220500946045,0.0019266817791848475
104104,104105,104104,208209,3.237375020980835,0.0023203157803093175
104304,104305,104304,208609,3.2437450885772705,0.0024666992166183788
104505,104506,104505,209011,3.249797821044922,0.0019104162862166017
104705,104706,104705,209411,3.2557880878448486,0.0019150513659901653
104905,104906,104905,209811,3.2617599964141846,0.0019035008963317218
105105,105106,105105,210211,3.267735004425049,0.001878819774269109
105305,105306,105305,210611,3.27384090423584,0.0018628549165607459
105506,105507,105506,211013,3.279711961746216,0.0018434927025985327
105706,105707,105706,211413,3.2856481075286865,0.00186391662555715
105906,105907,105906,211813,3.2915608882904053,0.0018314255923566186
106106,106107,106106,212213,3.2972910404205322,0.0018231154342759294
106306,106307,106306,212613,3.3029990196228027,0.0018303941707185757
106507,106508,106507,213015,3.3087520599365234,0.0019020799693027308
106707,106708,106707,213415,3.3144619464874268,0.0018242506477508273
106907,106908,106907,213815,3.3201658725738525,0.0018116413887355855
107107,107108,107107,214215,3.325888156890869,0.001794353317253482
107307,107308,107307,214615,3.331618070602417,0.001770503820076475
107508,107509,107508,215017,3.3373360633850098,0.0017688444047526436
107708,107709,107708,215417,3.3431789875030518,0.0017633297263442487
107908,107909,107908,215817,3.348910093307495,0.00175689116111394
108108,108109,108108,216217,3.354748010635376,0.0017505104472458285
108308,108309,108308,216617,3.360464096069336,0.0017336300323418958
108509,108510,108509,217019,3.3662359714508057,0.0017570439491589017
108709,108710,108709,217419,3.3719420433044434,0.001771568470308674
108909,108910,108909,217819,3.3774871826171875,0.0017184764659409298
109109,109110,109109,218219,3.3831369876861572,0.001690736181115698
109309,109310,109309,218619,3.388843059539795,0.001685560043985458
109510,109511,109510,219021,3.394631862640381,0.0020503060785849563
109710,109711,109710,219421,3.401560068130493,0.0017933072858361137
109910,109911,109910,219821,3.407201051712036,0.0016670729948234423
110110,110111,110110,220221,3.413037061691284,0.0016720652008267666
110310,110311,110310,220621,3.41866397857666,0.0016681153537302523
110511,110512,110511,221023,3.424373149871826,0.0017043666700417043
110711,110712,110711,221423,3.4300100803375244,0.001630730147572345
110911,110912,110911,221823,3.435783863067627,0.0016462189922318785
111111,111112,111111,222223,3.441925048828125,0.0016272382822902238
111311,111312,111311,222623,3.447645902633667,0.001630860545235837
111512,111513,111512,223025,3.453498125076294,0.001973421864346481
111712,111713,111712,223425,3.4594061374664307,0.0016497760140332248
111912,111913,111912,223825,3.465385913848877,0.0016509893443243599
112112,112113,112112,224225,3.471330165863037,0.0015922264368267536
112312,112313,112312,224625,3.4773151874542236,0.001866095632571293
112513,112514,112513,225027,3.483408212661743,0.0015679692610233965
112713,112714,112713,225427,3.49135422706604,0.0015570706777178992
112913,112914,112913,225827,3.497330904006958,0.0017688504923033003
113113,113114,113113,226227,3.503391981124878,0.0015306489640070085
113313,113314,113313,226627,3.509456157684326,0.0018244976674517558
113514,113515,113514,227029,3.5155200958251953,0.0015950948368420189
113714,113715,113714,227429,3.521696090698242,0.001514327481886504
113914,113915,113914,227829,3.527379035949707,0.0015037345010464015
114114,114115,114114,228229,3.5330350399017334,0.0014906765327306873
114314,114315,114314,228629,3.5387442111968994,0.001492603407971611
114515,114516,114515,229031,3.5449442863464355,0.001572575354195766
114715,114716,114715,229431,3.5506060123443604,0.0016918182829638556
114915,114916,114915,229831,3.55627703666687,0.0015894605538221043
115115,115116,115115,230231,3.5619959831237793,0.0014511839250585102
115315,115316,115315,230631,3.5677571296691895,0.0014447147318500412
115516,115517,115516,231033,3.5734710693359375,0.0014290836295854491
115716,115717,115716,231433,3.579155921936035,0.0014220382512299898
115916,115917,115916,231833,3.584869146347046,0.0015123753057512438
116116,116117,116116,232233,3.5907561779022217,0.0014527219363455234
116316,116317,116316,232633,3.5965209007263184,0.0014317939071454746
116517,116518,116517,233035,3.6023061275482178,0.001397616744222485
116717,116718,116717,233435,3.6081840991973877,0.001729923687399927
116917,116918,116917,233835,3.61393404006958,0.0014060680161308318
117117,117118,117117,234235,3.6196930408477783,0.0013829640546094008
117317,117318,117317,234635,3.6254470348358154,0.0013658441305125168
117518,117519,117518,235037,3.63128399848938,0.0013741863874188968
117718,117719,117718,235437,3.6370790004730225,0.0013616081073660167
117918,117919,117918,235837,3.642910957336426,0.0013478107742836423
118118,118119,118118,236237,3.6486852169036865,0.0013481359131859551
118318,118319,118318,236637,3.654442071914673,0.001333985521968418
118519,118520,118519,237039,3.6602728366851807,0.001351580207503543
118719,118720,118719,237439,3.6660261154174805,0.0013623949920032797
118919,118920,118919,237839,3.6717939376831055,0.0016236333137807136
119119,119120,119119,238239,3.677556037902832,0.0013440041576175774
119319,119320,119319,238639,3.683351993560791,0.0013031999390708008
119520,119521,119520,239041,3.689303159713745,0.001299802838990786
119720,119721,119720,239441,3.6947929859161377,0.0012936138090681559
119920,119921,119920,239841,3.700490951538086,0.001280803175899679
120120,120121,120120,240241,3.7061381340026855,0.0012915421528494654
120320,120321,120320,240641,3.711609125137329,0.0015741380128025107
120521,120522,120521,241043,3.7179951667785645,0.0012574759024699162
120721,120722,120721,241443,3.723543167114258,0.0012584205682553118
120921,120922,120921,241843,3.7291011810302734,0.0012628521176559918
121121,121122,121121,242243,3.734652042388916,0.0012605110390395647
121321,121322,121321,242643,3.740784168243408,0.0012520548309660488
121522,121523,121522,243045,3.746443033218384,0.0012370507540522637
121722,121723,121722,243445,3.75209903717041,0.001233221417735528
121922,121923,121922,243845,3.757869005203247,0.0012620581211772945
122122,122123,122122,244245,3.763512134552002,0.001396477825447388
122322,122323,122322,244645,3.769150972366333,0.0012068895063344009
122523,122524,122523,245047,3.7749099731445312,0.0012076667823499904
122723,122724,122723,245447,3.780634880065918,0.0012093911294735976
122923,122924,122923,245847,3.7863521575927734,0.001193351806952085
123123,123124,123123,246247,3.792379856109619,0.0013862279925165386
123323,123324,123323,246647,3.79809308052063,0.001192049627098032
123524,123525,123524,247049,3.8038480281829834,0.0011871920101064234
123724,123725,123724,247449,3.8095500469207764,0.001171623254379103
123924,123925,123924,247849,3.815338134765625,0.0011733665565287024
124124,124125,124124,248249,3.8210980892181396,0.0011496159962049329
124324,124325,124324,248649,3.826862096786499,0.0011759479773421648
124525,124526,124525,249051,3.832611083984375,0.0011452044261821117
124725,124726,124725,249451,3.8383100032806396,0.0011360195480188888
124925,124926,124925,249851,3.8440871238708496,0.0011979675754439376
125125,125126,125125,250251,3.849799871444702,0.0011257432005647137
125325,125326,125325,250651,3.855563163757324,0.0014572170404162624
125526,125527,125526,251053,3.861307144165039,0.0011143353716482124
125726,125727,125726,251453,3.8670551776885986,0.001344827512584897
125926,125927,125926,251853,3.8728342056274414,0.0011916298614509518
126126,126127,126126,252253,3.878615140914917,0.001334492990883916
126326,126327,126326,252653,3.8843789100646973,0.0010970876455032254
126527,126528,126527,253055,3.8901638984680176,0.001087715043927725
126727,126728,126727,253455,3.898062229156494,0.0010786454520220771
126927,126928,126927,253855,3.9039130210876465,0.0010753172322552566
127127,127128,127127,254255,3.909770965576172,0.001080036759620222
127327,127328,127327,254655,3.9154438972473145,0.0010720323463715993
127528,127529,127528,255057,3.921091079711914,0.0010617718705357366
127728,127729,127728,255457,3.926607131958008,0.001064745852923373
127928,127929,127928,255857,3.932122230529785,0.0011163869088877953
128128,128129,128128,256257,3.9377641677856445,0.0011684356160127569
128328,128329,128328,256657,3.9432928562164307,0.0011079505507777484
128529,128530,128529,257059,3.9488840103149414,0.001036137601422121
128729,128730,128729,257459,3.9546561241149902,0.001029208300109196
128929,128930,128929,257859,3.960767984390259,0.0010151670591419212
129129,129130,129129,258259,3.9664809703826904,0.001160114270210304
129329,129330,129329,258659,3.972261905670166,0.0010118230418512438
129530,129531,129530,259061,3.977795124053955,0.0010108026739660723
129730,129731,129730,259461,3.9833080768585205,0.0010040421387750834
129930,129931,129930,259861,3.988878011703491,0.0009964625398363467
130130,130131,130130,260261,3.99446702003479,0.000995443159684135
130330,130331,130330,260661,4.000014066696167,0.0011963462071715252
130531,130532,130531,261063,4.0056610107421875,0.0009893129355422823
130731,130732,130731,261463,4.011348009109497,0.0009740912169129199
130931,130932,130931,261863,4.016903877258301,0.0009832487700799225
131131,131132,131131,262263,4.024167060852051,0.0009675248846267337
131331,131332,131331,262663,4.029836177825928,0.0012085797639784857
131532,131533,131532,263065,4.035996913909912,0.0009561088254208913
131732,131733,131732,263465,4.04387092590332,0.0011324472505581471
131932,131933,131932,263865,4.050867080688477,0.0009488652833244813
132132,132133,132132,264265,4.058872222900391,0.0009416677131564679
132332,132333,132332,264665,4.0671820640563965,0.0010474106550642805
132533,132534,132533,265067,4.074672222137451,0.0009391527990270324
132733,132734,132733,265467,4.081303119659424,0.0009346015618101989
132933,132934,132933,265867,4.087646007537842,0.0009252652448546309
133133,133134,133133,266267,4.094093084335327,0.0009282484550835479
133333,133334,133333,266667,4.100348949432373,0.0009107167911038078
133534,133535,133534,267069,4.1074910163879395,0.0009229251679655787
133734,133735,133734,267469,4.113518238067627,0.0009053848049808773
133934,133935,133934,267869,4.1195409297943115,0.0009046697339533317
134134,134135,134134,268269,4.125558137893677,0.0011015384923384905
134334,134335,134334,268669,4.131557941436768,0.000892351678143847
134535,134536,134535,269071,4.137609004974365,0.0008835631272666769
134735,134736,134735,269471,4.143641233444214,0.0008824844498494463
134935,134936,134935,269871,4.149658203125,0.0008814480288405924
135135,135136,135135,270271,4.15588903427124,0.0008664775752209806
135335,135336,135335,270671,4.162125110626221,0.0011121516441556652
135536,135537,135536,271073,4.168336868286133,0.0008716514274627282
135736,135737,135736,271473,4.174356937408447,0.0008718763087799703
135936,135937,135936,271873,4.1803882122039795,0.0008701320144015297
136136,136137,136136,272273,4.186373233795166,0.0008633270653788447
136336,136337,136336,272673,4.192474126815796,0.0008428195950073837
136537,136538,136537,273075,4.198529005050659,0.0009622815812748764
136737,136738,136737,273475,4.204576015472412,0.0008453180415168806
136937,136938,136937,273875,4.210543155670166,0.0008691796185143435
137137,137138,137137,274275,4.216644048690796,0.0008621890132352567
137337,137338,137337,274675,4.222623109817505,0.0009724587126406361
137538,137539,137538,275077,4.228631019592285,0.0008225407993310344
137738,137739,137738,275477,4.234624147415161,0.0008178716715195934
137938,137939,137938,275877,4.2406580448150635,0.0008719273092150432
138138,138139,138138,276277,4.2466700077056885,0.0008076750692895464
138338,138339,138338,276677,4.252785921096802,0.0008072514943052438
138539,138540,138539,277079,4.259169101715088,0.0008037699328223744
138739,138740,138739,277479,4.265147924423218,0.0007962183868394575
138939,138940,138939,277879,4.2710959911346436,0.0008370568078086618
139139,139140,139139,278279,4.276912212371826,0.000798955002818312
139339,139340,139339,278679,4.2827630043029785,0.0008179378083061257
139540,139541,139540,279081,4.28889012336731,0.0007808744853122916
139740,139741,139740,279481,4.295107126235962,0.0007715505045615191
139940,139941,139940,279881,4.301197052001953,0.0007701095901389206
140140,140141,140140,280281,4.307244062423706,0.0008829414118405274
140340,140341,140340,280681,4.313421010971069,0.0007681930363129683
140541,140542,140541,281083,4.320026874542236,0.0007602449461354242
140741,140742,140741,281483,4.325862884521484,0.0007524530035653965
140941,140942,140941,281883,4.334167003631592,0.0007591521167983261
141141,141142,141141,282283,4.340939044952393,0.0007489894230189703
141341,141342,141341,282683,4.347537040710449,0.0007513495897013959
141542,141543,141542,283085,4.355116128921509,0.0007486385834564896
141742,141743,141742,283485,4.362594127655029,0.0009191136660090752
141942,141943,141942,283885,4.369481086730957,0.0007363847392440774
142142,142143,142142,284285,4.37546706199646,0.0007266661033785641
142342,142343,142342,284685,4.381401062011719,0.0007287518830309675
142543,142544,142543,285087,4.387360095977783,0.000721231495867403
142743,142744,142743,285487,4.39601993560791,0.0007272428029268289
142943,142944,142943,285887,4.4020280838012695,0.0007196440344845118
143143,143144,143143,286287,4.40802788734436,0.0007177238235414018
143343,143344,143343,286687,4.413977146148682,0.0007090762179392175
143544,143545,143544,287089,4.419948101043701,0.0007504219890605997
143744,143745,143744,287489,4.426149845123291,0.0007511017002516375
143944,143945,143944,287889,4.43210506439209,0.0006953815426757991
144144,144145,144144,288289,4.438138246536255,0.0007866793868530316
144344,144345,144344,288689,4.4446611404418945,0.0006941051463635806
144545,144546,144545,289091,4.451077938079834,0.0006886556749827547
144745,144746,144745,289491,4.45818018913269,0.0006930992297283054
144945,144946,144945,289891,4.4647932052612305,0.0007290451122745437
145145,145146,145145,290291,4.47192907333374,0.0006757342744131555
145345,145346,145345,290691,4.478311061859131,0.0006800463279515547
145546,145547,145546,291093,4.484546184539795,0.0006726292077813969
145746,145747,145746,291493,4.490753173828125,0.0006735967903033116
145946,145947,145946,291893,4.496976852416992,0.0006696160115679304
146146,146147,146146,292293,4.503147125244141,0.0006550809927905331
146346,146347,146346,292693,4.509557008743286,0.0006579191183080772
146547,146548,146547,293095,4.515882968902588,0.0007588485683847496
146747,146748,146747,293495,4.522067070007324,0.000654859091435867
146947,146948,146947,293895,4.52822208404541,0.0007626097930480924
147147,147148,147147,294295,4.534364938735962,0.0006539400142594591
147347,147348,147347,294695,4.5405189990997314,0.0006398937594515995
147548,147549,147548,295097,4.546767234802246,0.0006309352394024798
147748,147749,147748,295497,4.552958965301514,0.0006301908264619116
147948,147949,147948,295897,4.559099912643433,0.0006341250734221485
148148,148149,148148,296297,4.565240144729614,0.0007294904541625422
148348,148349,148348,296697,4.571562051773071,0.0006199280915566175
148549,148550,148549,297099,4.577552080154419,0.0006215067286359311
148749,148750,148749,297499,4.583526849746704,0.0006234459301208046
148949,148950,148949,297899,4.589659929275513,0.0006187376467107481
149149,149150,149149,298299,4.59571099281311,0.0007240656962584647
149349,149350,149349,298699,4.601701259613037,0.00063522301640395
149550,149551,149550,299101,4.607801198959351,0.0006084015211351991
149750,149751,149750,299501,4.613699197769165,0.0006300910072013121
149950,149951,149950,299901,4.619568824768066,0.0006000672268320527
150150,150151,150150,300301,4.62552809715271,0.0006053260583021621
150350,150351,150350,300701,4.631399869918823,0.0005989790327182159
150551,150552,150551,301103,4.637290000915527,0.0005889145124479104
150751,150752,150751,301503,4.643148183822632,0.0005919802959962046
150951,150952,150951,301903,4.649040937423706,0.000583767641232543
151151,151152,151151,302303,4.655080080032349,0.0006896638590626267
151351,151352,151351,302703,4.661136865615845,0.0005898321416545478
151552,151553,151552,303105,4.667191028594971,0.0005738304089787259
151752,151753,151752,303505,4.673123121261597,0.0006553232276423368
151952,151953,151952,303905,4.678899049758911,0.0005689630868226012
152152,152153,152152,304305,4.68464994430542,0.000616742827320846
152352,152353,152352,304705,4.690564155578613,0.0005695178016930882
152553,152554,152553,305107,4.697937965393066,0.0005579720652972241
152753,152754,152753,305507,4.704041004180908,0.0005609425282615424
152953,152954,152953,305907,4.710277080535889,0.000556402154053537
153153,153154,153153,306307,4.716645240783691,0.0005649123186464199
153353,153354,153353,306707,4.72368597984314,0.0005497716367166829
153554,153555,153554,307109,4.730372190475464,0.0005478378911291875
153754,153755,153754,307509,4.736592054367065,0.0006257059473216982
153954,153955,153954,307909,4.742831230163574,0.0006138146603546427
154154,154155,154154,308309,4.750833988189697,0.0005549644384654061
154354,154355,154354,308709,4.75726318359375,0.0005435916514393337
154555,154556,154555,309111,4.763485908508301,0.0005348504324938715
154755,154756,154755,309511,4.770111083984375,0.0005411296592752773
154955,154956,154955,309911,4.776684045791626,0.0005279530502752121
155155,155156,155155,310311,4.784116983413696,0.000523160911245305
155355,155356,155355,310711,4.791898965835571,0.0005206017490215979
155556,155557,155556,311113,4.799359083175659,0.0005175400273136614
155756,155757,155756,311513,4.805708169937134,0.0005187604407791742
155956,155957,155956,311913,4.811750888824463,0.0005205375817327428
156156,156157,156156,312313,4.818008184432983,0.0005434485371678235
156356,156357,156356,312713,4.82404899597168,0.000514362858967838
156557,156558,156557,313115,4.83056902885437,0.000531503515378153
156757,156758,156757,313515,4.836606025695801,0.00057676372530731
156957,156958,156957,313915,4.843160152435303,0.0005039868974430141
157157,157158,157157,314315,4.849131107330322,0.0005012883830006463
157357,157358,157357,314715,4.85510516166687,0.0005928086847497647
157558,157559,157558,315117,4.861465215682983,0.0004978901243677881
157758,157759,157758,315517,4.867424011230469,0.0004908455438178869
157958,157959,157958,315917,4.873827219009399,0.0004901962280133639
158158,158159,158158,316317,4.879883050918579,0.0004846508601206442
158358,158359,158358,316717,4.885889053344727,0.0004855767662551454
158559,158560,158559,317119,4.892207145690918,0.00048366702073812933
158759,158760,158759,317519,4.898288249969482,0.0004794584849106455
158959,158960,158959,317919,4.904277086257935,0.0004761610829343989
159159,159160,159159,318319,4.910499095916748,0.0004748427246493994
159359,159360,159359,318719,4.916738033294678,0.0004718117556958178
159560,159561,159560,319121,4.922813892364502,0.000464894777586666
159760,159761,159760,319521,4.9287049770355225,0.0004678210733110973
159960,159961,159960,319921,4.934571981430054,0.0004809036131793822
160160,160161,160160,320321,4.940781116485596,0.00047188082456982056
160360,160361,160360,320721,4.946885108947754,0.00046582920277660504
160561,160562,160561,321123,4.956192970275879,0.00045901124193607046
160761,160762,160761,321523,4.962559938430786,0.00045460726639254745
160961,160962,160961,321923,4.96855616569519,0.00045444083074762414
161161,161162,161161,322323,4.974496126174927,0.00045391411570882493
161361,161362,161361,322723,4.980443954467773,0.00045258913913899995
161562,161563,161562,323125,4.986407995223999,0.0004442577053349836
161762,161763,161762,323525,4.99234414100647,0.00044226038666085864
161962,161963,161962,323925,4.9983720779418945,0.00048539236280799883
162162,162163,162162,324325,5.004338026046753,0.000545605697776332
162362,162363,162362,324725,5.010426044464111,0.00044052363286115845
162563,162564,162563,325127,5.016526222229004,0.0005304419123240473
162763,162764,162763,325527,5.022649049758911,0.0005014111847095812
162963,162964,162963,325927,5.02888298034668,0.00043146831832868883
163163,163164,163163,326327,5.035049915313721,0.00042593209832637305
163363,163364,163363,326727,5.041283130645752,0.0004243638517011122
163564,163565,163564,327129,5.047581911087036,0.0004248246144064964
163764,163765,163764,327529,5.054059028625488,0.00042310731021801484
163964,163965,163964,327929,5.060664176940918,0.0004188423977482823
164164,164165,164164,328329,5.066979169845581,0.0004191934786234894
164364,164365,164364,328729,5.073336124420166,0.000416931293971408
164565,164566,164565,329131,5.079945087432861,0.0004134096319817943
164765,164766,164765,329531,5.086087942123413,0.0004072371329818886
164965,164966,164965,329931,5.092339992523193,0.00040694825483742874
165165,165166,165165,330331,5.098221063613892,0.00040675735506080606
165365,165366,165365,330731,5.104362964630127,0.000434841169707032
165566,165567,165566,331133,5.110666036605835,0.0004005913771831611
165766,165767,165766,331533,5.116876125335693,0.0004018425750016604
165966,165967,165966,331933,5.1231749057769775,0.0004274617659233051
166166,166167,166166,332333,5.129440069198608,0.0003960376922236419
166366,166367,166366,332733,5.1357262134552,0.00039738053076470673
166567,166568,166567,333135,5.141992092132568,0.0003953172411127106
166767,166768,166767,333535,5.147974014282227,0.00038838694427199095
166967,166968,166967,333935,5.15397310256958,0.00039058822737542066
167167,167168,167167,334335,5.159934043884277,0.0003845160311542035
167367,167368,167367,334735,5.165893077850342,0.0003943911909553938
167568,167569,167568,335137,5.17189621925354,0.00043361647743507
167768,167769,167768,335537,5.177868127822876,0.0004854314432980932
167968,167969,167968,335937,5.183833122253418,0.0003792898388876672
168168,168169,168168,336337,5.189929008483887,0.000388295054301492
168368,168369,168368,336737,5.196310997009277,0.00046268618192321545
168569,168570,168569,337139,5.20226788520813,0.00036954529346390914
168769,168770,168769,337539,5.208165884017944,0.00037281932380677223
168969,168970,168969,337939,5.214069128036499,0.0003714898094938882
169169,169170,169169,338339,5.219969987869263,0.0003673734146756985
169369,169370,169369,338739,5.2260191440582275,0.0003695138056925279
169570,169571,169570,339141,5.231956958770752,0.00036386070551619904
169770,169771,169770,339541,5.238887071609497,0.0003597263154288514
169970,169971,169970,339941,5.2451090812683105,0.0003637617085146127
170170,170171,170170,340341,5.251421928405762,0.00035672227513760613
170370,170371,170370,340741,5.257649898529053,0.0003549410851476745
170571,170572,170571,341143,5.264033079147339,0.0003557734288630801
170771,170772,170771,341543,5.270365953445435,0.00036003794816088917
170971,170972,170971,341943,5.276633024215698,0.00036259572969769973
171171,171172,171171,342343,5.282819032669067,0.00043387044140503496
171371,171372,171371,342743,5.2891130447387695,0.0003526685205801025
171572,171573,171572,343145,5.295519113540649,0.0003542319320621289
171772,171773,171772,343545,5.3015429973602295,0.0003477255963992194
171972,171973,171972,343945,5.3077099323272705,0.0003639883817650026
172172,172173,172172,344345,5.3138439655303955,0.0003903290118092034
172372,172373,172372,344745,5.319900035858154,0.000338185814128999
172573,172574,172573,345147,5.325945138931274,0.00035036308243509707
172773,172774,172773,345547,5.332123041152954,0.0003352636019525433
172973,172974,172973,345947,5.337990045547485,0.0003353930970071596
173173,173174,173173,346347,5.3438720703125,0.00039730535750351245
173373,173374,173373,346747,5.349778890609741,0.0003336561320582976
173574,173575,173574,347149,5.355725049972534,0.0003953041197756024
173774,173775,173774,347549,5.361598014831543,0.00032699604239713856
173974,173975,173974,347949,5.367469072341919,0.00032448678119324
174174,174175,174174,348349,5.373390197753906,0.00032240336553091947
174374,174375,174374,348749,5.37935996055603,0.0003218876315850002
174575,174576,174575,349151,5.385490894317627,0.00031892126444114043
174775,174776,174775,349551,5.391595125198364,0.00031780933279829007
174975,174976,174975,349951,5.397444248199463,0.00031767658614543034
175175,175176,175175,350351,5.403226137161255,0.0003170290253647121
175375,175376,175375,350751,5.409119129180908,0.00031574794127072945
175576,175577,175576,351153,5.414889097213745,0.000313341181104001
175776,175777,175776,351553,5.420750141143799,0.0003112425959706701
175976,175977,175976,351953,5.426484107971191,0.0003089204095466061
176176,176177,176176,352353,5.432289123535156,0.0003602665614480855
176376,176377,176376,352753,5.438261032104492,0.0003847424523713432
176577,176578,176577,353155,5.444620132446289,0.0003026051251339166
176777,176778,176777,353555,5.450724124908447,0.00030218129240591095
176977,176978,176977,353955,5.456570148468018,0.0003868828761804963
177177,177178,177177,354355,5.462739944458008,0.0003286602758874009
177377,177378,177377,354755,5.4686689376831055,0.00029683848061824513
177578,177579,177578,355157,5.474549055099487,0.0003381156672813502
177778,177779,177778,355557,5.480371952056885,0.00029485843449589375
177978,177979,177978,355957,5.486234188079834,0.0002959516010246236
178178,178179,178178,356357,5.4921650886535645,0.00029379591406455735
178378,178379,178378,356757,5.498064279556274,0.00033033504433212956
178579,178580,178579,357159,5.504678964614868,0.0002940531678635279
178779,178780,178779,357559,5.510596036911011,0.0002883188176822511
178979,178980,178979,357959,5.516426086425781,0.0003401817459499014
179179,179180,179179,358359,5.523452997207642,0.00028767645134080956
179379,179380,179379,358759,5.529356002807617,0.0002841154628224168
179580,179581,179580,359161,5.535557985305786,0.00028273230785779666
179780,179781,179780,359561,5.541690111160278,0.0002813915890793804
179980,179981,179980,359961,5.547508001327515,0.000292933446136171
180180,180181,180180,360361,5.553593158721924,0.000279122320265064
180380,180381,180380,360761,5.5601890087127686,0.00029625684403312454
180581,180582,180581,361163,5.568521022796631,0.00027568675540764185
180781,180782,180781,361563,5.5745580196380615,0.00027311049069369956
180981,180982,180981,361963,5.580512046813965,0.0002724797902356959
181181,181182,181181,362363,5.586742162704468,0.0003110329297033935
181381,181382,181381,362763,5.592849969863892,0.00026923465257679374
181582,181583,181582,363165,5.598818063735962,0.0002875842521175985
181782,181783,181782,363565,5.604816913604736,0.00030832610270207193
181982,181983,181982,363965,5.61084508895874,0.0003021819723720803
182182,182183,182182,364365,5.616818904876709,0.00027387796156166277
182382,182383,182382,364765,5.622966051101685,0.00027520710625293817
182583,182584,182583,365167,5.629870176315308,0.0002585944338142107
182783,182784,182783,365567,5.63630485534668,0.00026409072355995986
182983,182984,182983,365967,5.642567873001099,0.0002593932311743648
183183,183184,183183,366367,5.648600101470947,0.00030421101746746306
183383,183384,183383,366767,5.654539108276367,0.0002548493891848503
183584,183585,183584,367169,5.660656929016113,0.0002557005498134259
183784,183785,183784,367569,5.6666481494903564,0.0002661511832057892
183984,183985,183984,367969,5.6726861000061035,0.00025127229110594683
184184,184185,184184,368369,5.678584098815918,0.00025066394799333307
184384,184385,184384,368769,5.684732913970947,0.0002482721286143449
184585,184586,184585,369171,5.690938234329224,0.0002480101237386213
184785,184786,184785,369571,5.697250127792358,0.00024531213783366015
184985,184986,184985,369971,5.7031848430633545,0.00024512924252334046
185185,185186,185185,370371,5.7093939781188965,0.00024357394991545757
185385,185386,185385,370771,5.715309143066406,0.00024182026139709983
185586,185587,185586,371173,5.721649885177612,0.00025008617682130885
185786,185787,185786,371573,5.7278220653533936,0.00029011158199657183
185986,185987,185986,371973,5.734095096588135,0.00027486539654629667
186186,186187,186186,372373,5.740170001983643,0.0002384808034714095
186386,186387,186386,372773,5.7470619678497314,0.00023471671119783806
186587,186588,186587,373175,5.753270149230957,0.0002745534899662632
186787,186788,186787,373575,5.75948691368103,0.0002335043870584064
186987,186988,186987,373975,5.765733957290649,0.0002672833787622686
187187,187188,187187,374375,5.77222204208374,0.0002729668310545426
187387,187388,187387,374775,5.7784881591796875,0.00023221335571923073
187588,187589,187588,375177,5.784893989562988,0.00023113189685331054
187788,187789,187788,375577,5.7915730476379395,0.00022854059922586156
187988,187989,187988,375977,5.797904968261719,0.00022714517783529927
188188,188189,188188,376377,5.804168939590454,0.00027250520513978226
188388,188389,188388,376777,5.8103320598602295,0.00022363630717678538
188589,188590,188589,377179,5.817324161529541,0.0002262462250111337
188789,188790,188789,377579,5.82368803024292,0.00022363248477573375
188989,188990,188989,377979,5.830142021179199,0.00022172403201245187
189189,189190,189189,378379,5.8369081020355225,0.00021977923851245195
189389,189390,189389,378779,5.843222141265869,0.00025900164191725033
189590,189591,189590,379181,5.849500894546509,0.000228038030296149
189790,189791,189790,379581,5.855754137039185,0.0002167964599494826
189990,189991,189990,379981,5.861678123474121,0.00021501620074210377
190190,190191,190190,380381,5.867967128753662,0.00021694122131495864
190390,190391,190390,380781,5.874185085296631,0.0002120389590269198
190591,190592,190591,381183,5.8803629875183105,0.00029827212924373115
190791,190792,190791,381583,5.886468172073364,0.00021094661318686933
190991,190992,190991,381983,5.892568111419678,0.00021161005061647844
191191,191192,191191,382383,5.898640155792236,0.00021767600259413612
191391,191392,191391,382783,5.9046831130981445,0.00020912774266787623
191592,191593,191592,383185,5.910820245742798,0.00020745164122263843
191792,191793,191792,383585,5.916913986206055,0.00025870781041512607
191992,191993,191992,383985,5.922997951507568,0.0002040953535588511
192192,192193,192192,384385,5.929072856903076,0.0002062000658832997
192392,192393,192392,384785,5.935148000717163,0.00020395440604012034
192593,192594,192593,385187,5.941354036331177,0.00020086218581682626
192793,192794,192793,385587,5.947381973266602,0.00020051696255671272
192993,192994,192993,385987,5.953437089920044,0.00023976091373831225
193193,193194,193193,386387,5.95947003364563,0.00019963382807135316
193393,193394,193393,386787,5.965485095977783,0.00020119134891362798
193594,193595,193594,387189,5.971453905105591,0.00022944715013016178
193794,193795,193794,387589,5.977291107177734,0.00020197763413767192
193994,193995,193994,387989,5.983159065246582,0.0001944407344532303
194194,194195,194194,388389,5.988994121551514,0.00019336009155058683
194394,194395,194394,388789,5.99533486366272,0.00019279448643281675
194595,194596,194595,389191,6.001224994659424,0.00019022000634029974
194795,194796,194795,389591,6.007076025009155,0.00019256913859278893
194995,194996,194995,389991,6.012937068939209,0.00018934059880832842
195195,195196,195195,390391,6.019092082977295,0.0001884795232287495
195395,195396,195395,390791,6.025193929672241,0.00018597517864970165
195596,195597,195596,391193,6.031227111816406,0.00021023132681399247
195796,195797,195796,391593,6.037191867828369,0.00018585019699536958
195996,195997,195996,391993,6.043178081512451,0.00018461738845802867
196196,196197,196196,392393,6.049242258071899,0.0001827993903157307
196396,196397,196396,392793,6.055253982543945,0.00018326277535487675
196597,196598,196597,393195,6.061342000961304,0.00018275301994597515
196797,196798,196797,393595,6.068274974822998,0.00018143382325329667
196997,196998,196997,393995,6.075947999954224,0.00018059143169079893
197197,197198,197197,394395,6.084223031997681,0.000181073413260446
197397,197398,197397,394795,6.092506170272827,0.00017729309811006128
197598,197599,197598,395197,6.100609064102173,0.0001757924055001007
197798,197799,197798,395597,6.108780145645142,0.00021093220848104804
197998,197999,197998,395997,6.1170759201049805,0.00017556605811814644
198198,198199,198198,396397,6.125242233276367,0.00017340960413312844
198398,198399,198398,396797,6.1336400508880615,0.00017251911235031944
198599,198600,198599,397199,6.142135143280029,0.00017324527596625252
198799,198800,198799,397599,6.15003228187561,0.00017514524245488788
198999,199000,198999,397999,6.157486200332642,0.00020136233979246203
199199,199200,199199,398399,6.164865016937256,0.00017015670715026703
199399,199400,199399,398799,6.1718809604644775,0.0001708085984260323
199600,199601,199600,399201,6.177896976470947,0.00016842327097694456
199800,199801,199800,399601,6.183763027191162,0.00016932244511551553
200000,200001,200000,400001,6.189651966094971,0.00020154354922429128


==> plot_data/quadratic_minimax_problem_n20_alpha0/eag-c.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,8.20159912109375e-05,4.387061074692293
100,201,0,201,0.0046558380126953125,1.0673545918633924
200,401,0,401,0.010454177856445312,0.4049021910637366
300,601,0,601,0.015111923217773438,0.3042707958389895
400,801,0,801,0.01993393898010254,0.21271367149175655
501,1003,0,1003,0.024610042572021484,0.1717728895974256
601,1203,0,1203,0.030383825302124023,0.14972243764114768
701,1403,0,1403,0.03548598289489746,0.1217329166933894
801,1603,0,1603,0.04034686088562012,0.10203790309631597
901,1803,0,1803,0.04562997817993164,0.08933779537451116
1001,2003,0,2003,0.050582170486450195,0.08265066885959595
1101,2203,0,2203,0.05531191825866699,0.08230505365279778
1201,2403,0,2403,0.0604090690612793,0.06176758946000925
1301,2603,0,2603,0.06524300575256348,0.0695209338266348
1401,2803,0,2803,0.06975412368774414,0.0589485050023372
1502,3005,0,3005,0.0746009349822998,0.0627481296261858
1602,3205,0,3205,0.07983589172363281,0.05293675918341365
1702,3405,0,3405,0.0847630500793457,0.04722635532851449
1802,3605,0,3605,0.09051108360290527,0.05093361305164786
1902,3805,0,3805,0.09790396690368652,0.04504451194371095
2002,4005,0,4005,0.1035451889038086,0.04177796728718847
2102,4205,0,4205,0.10905718803405762,0.04067682130710717
2202,4405,0,4405,0.11379504203796387,0.03842459003575901
2302,4605,0,4605,0.11889314651489258,0.04007450093735216
2402,4805,0,4805,0.12466907501220703,0.03627332959248263
2503,5007,0,5007,0.12936615943908691,0.034346849076908
2603,5207,0,5207,0.13394403457641602,0.03365380370352932
2703,5407,0,5407,0.1384119987487793,0.03299723751354892
2803,5607,0,5607,0.1430220603942871,0.03135474476718378
2903,5807,0,5807,0.14801788330078125,0.026535319435883005
3003,6007,0,6007,0.15320706367492676,0.029390797885835523
3103,6207,0,6207,0.15788006782531738,0.02612188985375729
3203,6407,0,6407,0.1625521183013916,0.02748500625159133
3303,6607,0,6607,0.16750383377075195,0.02424581732098491
3403,6807,0,6807,0.17211008071899414,0.024008143925917536
3504,7009,0,7009,0.17679119110107422,0.025162460325511227
3604,7209,0,7209,0.18116092681884766,0.022578718206167147
3704,7409,0,7409,0.18564891815185547,0.021494259299025112
3804,7609,0,7609,0.190155029296875,0.02043875890666776
3904,7809,0,7809,0.19461607933044434,0.01987993616688908
4004,8009,0,8009,0.19915127754211426,0.02015308122435684
4104,8209,0,8209,0.2035839557647705,0.017455340496693332
4204,8409,0,8409,0.20844221115112305,0.018193517796546033
4304,8609,0,8609,0.21246004104614258,0.017525793056724182
4404,8809,0,8809,0.21614694595336914,0.018550087622006765
4505,9011,0,9011,0.21981215476989746,0.016164363810323944
4605,9211,0,9211,0.22364401817321777,0.01611030940457769
4705,9411,0,9411,0.22757816314697266,0.01611548503031052
4805,9611,0,9611,0.2311859130859375,0.01538845563391613
4905,9811,0,9811,0.2348320484161377,0.014905501717866506
5005,10011,0,10011,0.2384331226348877,0.01366056757129582
5105,10211,0,10211,0.24202609062194824,0.014068546361759207
5205,10411,0,10411,0.24564719200134277,0.014925184532832122
5305,10611,0,10611,0.24953413009643555,0.013640662268505044
5405,10811,0,10811,0.2531242370605469,0.01386276237210343
5506,11013,0,11013,0.2567439079284668,0.013639937871897831
5606,11213,0,11213,0.26033592224121094,0.014041214092744102
5706,11413,0,11413,0.2639482021331787,0.013441807764246163
5806,11613,0,11613,0.26752686500549316,0.012562686014286216
5906,11813,0,11813,0.27134013175964355,0.012706676435404613
6006,12013,0,12013,0.2749161720275879,0.012894773898899512
6106,12213,0,12213,0.2784910202026367,0.012936444587394073
6206,12413,0,12413,0.2820770740509033,0.012225834205619113
6306,12613,0,12613,0.28563785552978516,0.012636036977946803
6406,12813,0,12813,0.28920912742614746,0.013037047529582194
6507,13015,0,13015,0.29280900955200195,0.012716971695537092
6607,13215,0,13215,0.2963690757751465,0.012510088247604023
6707,13415,0,13415,0.3000919818878174,0.01191296661983371
6807,13615,0,13615,0.3036532402038574,0.01228381496683447
6907,13815,0,13815,0.30721521377563477,0.012154934084562058
7007,14015,0,14015,0.3107719421386719,0.01143366202513963
7107,14215,0,14215,0.31433606147766113,0.011593119488544449
7207,14415,0,14415,0.31784605979919434,0.0116494057725054
7307,14615,0,14615,0.3213231563568115,0.011910279317454647
7407,14815,0,14815,0.3248021602630615,0.011463874642140671
7508,15017,0,15017,0.3284599781036377,0.011237794855793343
7608,15217,0,15217,0.33194494247436523,0.011236355233733394
7708,15417,0,15417,0.3354299068450928,0.011160862470629666
7808,15617,0,15617,0.3388960361480713,0.010678561032865207
7908,15817,0,15817,0.34237003326416016,0.01012244253562772
8008,16017,0,16017,0.34584712982177734,0.010267321945978992
8108,16217,0,16217,0.3493199348449707,0.010258392149599074
8208,16417,0,16417,0.3528120517730713,0.009970428254309695
8308,16617,0,16617,0.3562769889831543,0.009805773793440862
8408,16817,0,16817,0.35987210273742676,0.009612290022200577
8509,17019,0,17019,0.36338114738464355,0.009843928341412143
8609,17219,0,17219,0.36684703826904297,0.009394042355870174
8709,17419,0,17419,0.37032413482666016,0.00887133103669788
8809,17619,0,17619,0.37380099296569824,0.008724093024721866
8909,17819,0,17819,0.37726712226867676,0.008641432623350877
9009,18019,0,18019,0.38073301315307617,0.008447788572745304
9109,18219,0,18219,0.3843100070953369,0.00807796240372097
9209,18419,0,18419,0.3878591060638428,0.00802890122705077
9309,18619,0,18619,0.3914680480957031,0.008202690218464951
9409,18819,0,18819,0.39497923851013184,0.008147570997580322
9510,19021,0,19021,0.3985931873321533,0.007813795330105162
9610,19221,0,19221,0.40212416648864746,0.0075448511345763206
9710,19421,0,19421,0.4056510925292969,0.007657580682796772
9810,19621,0,19621,0.40918612480163574,0.007423646563510711
9910,19821,0,19821,0.41271209716796875,0.007125141438191955
10010,20021,0,20021,0.4161369800567627,0.006979110647953697
10110,20221,0,20221,0.41951704025268555,0.007072047529712677
10210,20421,0,20421,0.42281508445739746,0.007306044548107694
10310,20621,0,20621,0.4261031150817871,0.007122484668401108
10410,20821,0,20821,0.43041110038757324,0.007054476557523793
10511,21023,0,21023,0.43421101570129395,0.007197522422412029
10611,21223,0,21223,0.43970799446105957,0.007217110692236581
10711,21423,0,21423,0.44394803047180176,0.007034724766388607
10811,21623,0,21623,0.44763708114624023,0.006801956835663474
10911,21823,0,21823,0.452099084854126,0.006853774568441507
11011,22023,0,22023,0.4561789035797119,0.0069720348285935785
11111,22223,0,22223,0.4595949649810791,0.006963776379840413
11211,22423,0,22423,0.46294617652893066,0.00688826026740812
11311,22623,0,22623,0.4663100242614746,0.00701225189075417
11411,22823,0,22823,0.46984410285949707,0.007227540837921803
11512,23025,0,23025,0.4733011722564697,0.0071371224056349675
11612,23225,0,23225,0.4767942428588867,0.007007994851043972
11712,23425,0,23425,0.48030710220336914,0.006932453786308687
11812,23625,0,23625,0.4838709831237793,0.006963093971099112
11912,23825,0,23825,0.4876730442047119,0.006931159863468218
12012,24025,0,24025,0.4912550449371338,0.006748001210483645
12112,24225,0,24225,0.4946420192718506,0.0067614090825382014
12212,24425,0,24425,0.4989020824432373,0.0069063461046462655
12312,24625,0,24625,0.5027320384979248,0.006933862111952244
12412,24825,0,24825,0.506472110748291,0.006831744835719266
12513,25027,0,25027,0.5100760459899902,0.006736872446141184
12613,25227,0,25227,0.5136499404907227,0.006740973300526169
12713,25427,0,25427,0.5182862281799316,0.006652254223970815
12813,25627,0,25627,0.5219011306762695,0.006446150083099497
12913,25827,0,25827,0.5254449844360352,0.006256808269584062
13013,26027,0,26027,0.5289821624755859,0.006266652863865043
13113,26227,0,26227,0.5325100421905518,0.006284665353945361
13213,26427,0,26427,0.5363509654998779,0.006161205162714325
13313,26627,0,26627,0.5398960113525391,0.006084193536884966
13413,26827,0,26827,0.5434141159057617,0.006070544577842459
13514,27029,0,27029,0.5471451282501221,0.006049756629090452
13614,27229,0,27229,0.5507619380950928,0.005883855083628956
13714,27429,0,27429,0.5542910099029541,0.005630819649733052
13814,27629,0,27629,0.5578229427337646,0.005534136269399937
13914,27829,0,27829,0.561378002166748,0.005484136694319016
14014,28029,0,28029,0.5649011135101318,0.005359328750633811
14114,28229,0,28229,0.568479061126709,0.005226611260802524
14214,28429,0,28429,0.572045087814331,0.005221411119496696
14314,28629,0,28629,0.575645923614502,0.005284486990020055
14414,28829,0,28829,0.5791559219360352,0.005238478021754753
14515,29031,0,29031,0.5826930999755859,0.005094542465507088
14615,29231,0,29231,0.5862460136413574,0.004986087068140045
14715,29431,0,29431,0.5897510051727295,0.004970757367798045
14815,29631,0,29631,0.5932741165161133,0.0048753573432271475
14915,29831,0,29831,0.5969328880310059,0.0047153357472845365
15015,30031,0,30031,0.6004810333251953,0.004681158358388621
15115,30231,0,30231,0.6039800643920898,0.004753516654410479
15215,30431,0,30431,0.607867956161499,0.004824672478728818
15315,30631,0,30631,0.6113669872283936,0.004803612360299999
15415,30831,0,30831,0.6151151657104492,0.004785380106719047
15516,31033,0,31033,0.6187341213226318,0.004852157638110348
15616,31233,0,31233,0.6221351623535156,0.004856474899261709
15716,31433,0,31433,0.6255390644073486,0.004759914324156903
15816,31633,0,31633,0.6289422512054443,0.00467911114166003
15916,31833,0,31833,0.6323671340942383,0.004710220906360681
16016,32033,0,32033,0.6371688842773438,0.004771719012250733
16116,32233,0,32233,0.6427431106567383,0.004783929100922037
16216,32433,0,32433,0.6463611125946045,0.00479909611065722
16316,32633,0,32633,0.6498630046844482,0.00488299111987913
16416,32833,0,32833,0.6537039279937744,0.0049767506537911725
16517,33035,0,33035,0.6573150157928467,0.0049572996567738255
16617,33235,0,33235,0.6608982086181641,0.004886877152238715
16717,33435,0,33435,0.6643378734588623,0.004869768005565191
16817,33635,0,33635,0.6678421497344971,0.004871100810860564
16917,33835,0,33835,0.672476053237915,0.004841582355329571
17017,34035,0,34035,0.6767139434814453,0.004788829128157551
17117,34235,0,34235,0.681481122970581,0.004806423949449826
17217,34435,0,34435,0.6853160858154297,0.004882998782845022
17317,34635,0,34635,0.6897449493408203,0.004901780150849659
17417,34835,0,34835,0.6946251392364502,0.004855225454750469
17518,35037,0,35037,0.6992430686950684,0.004816319531499973
17618,35237,0,35237,0.7039849758148193,0.004797525307041281
17718,35437,0,35437,0.7088472843170166,0.004730441596576756
17818,35637,0,35637,0.713468074798584,0.004613402370356125
17918,35837,0,35837,0.7179470062255859,0.004527855825744497
18018,36037,0,36037,0.7225990295410156,0.004516580614556767
18118,36237,0,36237,0.7273080348968506,0.0045147033825063965
18218,36437,0,36437,0.7318761348724365,0.004461157724276734
18318,36637,0,36637,0.7363431453704834,0.0044181650949096886
18418,36837,0,36837,0.7409069538116455,0.004410184870183538
18519,37039,0,37039,0.745373010635376,0.004368532686871857
18619,37239,0,37239,0.7493700981140137,0.0042590714074018056
18719,37439,0,37439,0.7533791065216064,0.004126576417163519
18819,37639,0,37639,0.7572841644287109,0.004049446008025196
18919,37839,0,37839,0.7610828876495361,0.004002818432140154
19019,38039,0,38039,0.764815092086792,0.003928673885354569
19119,38239,0,38239,0.7684831619262695,0.00386619047830315
19219,38439,0,38439,0.7726211547851562,0.00386803342265996
19319,38639,0,38639,0.7762649059295654,0.003889534286485661
19419,38839,0,38839,0.779853105545044,0.003854552340424131
19520,39041,0,39041,0.7835211753845215,0.003775596866220422
19620,39241,0,39241,0.7871758937835693,0.0037153477204209524
19720,39441,0,39441,0.7907800674438477,0.003678904356854645
19820,39641,0,39641,0.7943990230560303,0.003616669886075913
19920,39841,0,39841,0.7979919910430908,0.0035381985450971707
20020,40041,0,40041,0.8015921115875244,0.003526437686351484
20120,40241,0,40241,0.8051819801330566,0.003575674516521372
20220,40441,0,40441,0.8088772296905518,0.0036133678409468843
20320,40641,0,40641,0.8125109672546387,0.0036186268317476857
20420,40841,0,40841,0.8161280155181885,0.003627340671491457
20521,41043,0,41043,0.8197300434112549,0.003656158071737758
20621,41243,0,41243,0.8235070705413818,0.003653164365296124
20721,41443,0,41443,0.8278841972351074,0.003602992153220731
20821,41643,0,41643,0.8314781188964844,0.003569686309565726
20921,41843,0,41843,0.8351991176605225,0.0035921667269177902
21021,42043,0,42043,0.8388440608978271,0.003631074678563314
21121,42243,0,42243,0.84328293800354,0.0036535544170685896
21221,42443,0,42443,0.8468780517578125,0.003686664727612707
21321,42643,0,42643,0.850776195526123,0.0037470837426399127
21421,42843,0,42843,0.8544168472290039,0.0037963152073887817
21522,43045,0,43045,0.8595478534698486,0.00379166801913963
21622,43245,0,43245,0.8637840747833252,0.0037589148665859804
21722,43445,0,43445,0.8679649829864502,0.0037478345902089353
21822,43645,0,43645,0.8723700046539307,0.003745491355419233
21922,43845,0,43845,0.8776042461395264,0.003726830686026307
22022,44045,0,44045,0.8819730281829834,0.0037120395408280107
22122,44245,0,44245,0.8863308429718018,0.003733454809577551
22222,44445,0,44445,0.8907780647277832,0.0037757134425443414
22322,44645,0,44645,0.8952891826629639,0.0037885982486271655
22422,44845,0,44845,0.8994729518890381,0.003766394419145786
22523,45047,0,45047,0.9033010005950928,0.0037422645456167036
22623,45247,0,45247,0.9070920944213867,0.0037181432689013046
22723,45447,0,45447,0.9110012054443359,0.003665817263423618
22823,45647,0,45647,0.9146749973297119,0.0035931714449502408
22923,45847,0,45847,0.9183430671691895,0.0035439321086579508
23023,46047,0,46047,0.9224488735198975,0.00353070734188824
23123,46247,0,46247,0.9265532493591309,0.0035213418232610933
23223,46447,0,46447,0.9308590888977051,0.0034937777095578573
23323,46647,0,46647,0.9349651336669922,0.003468387443767022
23423,46847,0,46847,0.9393291473388672,0.00345312519873274
23524,47049,0,47049,0.9433281421661377,0.0034126824227102186
23624,47249,0,47249,0.947066068649292,0.0033339798472745608
23724,47449,0,47449,0.9506881237030029,0.0032494506430725766
23824,47649,0,47649,0.9543271064758301,0.003190818179037223
23924,47849,0,47849,0.9579782485961914,0.00314816800225836
24024,48049,0,48049,0.9617102146148682,0.003101494128553399
24124,48249,0,48249,0.9653260707855225,0.0030686659149796983
24224,48449,0,48449,0.9689531326293945,0.0030686960000341702
24324,48649,0,48649,0.972559928894043,0.003073462535060667
24424,48849,0,48849,0.9766771793365479,0.0030464672044980138
24525,49051,0,49051,0.980463981628418,0.0029965700214453542
24625,49251,0,49251,0.9840729236602783,0.0029544012890565475
24725,49451,0,49451,0.9876821041107178,0.002918925108141795
24825,49651,0,49651,0.9920220375061035,0.0028742019167119453
24925,49851,0,49851,0.9958631992340088,0.0028337408024300937
25025,50051,0,50051,0.9994900226593018,0.002832319380721873
25125,50251,0,50251,1.0031192302703857,0.0028648651626167034
25225,50451,0,50451,1.0071282386779785,0.00289237084146579
25325,50651,0,50651,1.011199951171875,0.0029046182394376102
25425,50851,0,50851,1.0148711204528809,0.002918167177645575
25526,51053,0,51053,1.0184969902038574,0.002932861464379709
25626,51253,0,51253,1.0225720405578613,0.0029270260384629786
25726,51453,0,51453,1.0283551216125488,0.002900882643863504
25826,51653,0,51653,1.032628059387207,0.0028876571036222935
25926,51853,0,51853,1.038682222366333,0.002905310701126534
26026,52053,0,52053,1.04355788230896,0.0029345608700795
26126,52253,0,52253,1.0484910011291504,0.0029607131939564076
26226,52453,0,52453,1.0530781745910645,0.0029950039188995333
26326,52653,0,52653,1.0579121112823486,0.003039302832940597
26426,52853,0,52853,1.0627760887145996,0.00306967821135482
26527,53055,0,53055,1.0672650337219238,0.003069426646637729
26627,53255,0,53255,1.0717320442199707,0.0030538434962603376
26727,53455,0,53455,1.0761878490447998,0.003045823841038101
26827,53655,0,53655,1.0806221961975098,0.0030421477618152817
26927,53855,0,53855,1.0850801467895508,0.003033339287844165
27027,54055,0,54055,1.0895402431488037,0.003032260331735814
27127,54255,0,54255,1.09425687789917,0.0030519622958326384
27227,54455,0,54455,1.098656177520752,0.0030783286808199815
27327,54655,0,54655,1.1027462482452393,0.003086780736451006
27427,54855,0,54855,1.1067121028900146,0.003074839446928304
27528,55057,0,55057,1.1103579998016357,0.0030563605640995
27628,55257,0,55257,1.1139678955078125,0.003031795773763916
27728,55457,0,55457,1.117522954940796,0.0029907482973340824
27828,55657,0,55657,1.1210429668426514,0.002942111915777855
27928,55857,0,55857,1.1246089935302734,0.0029094092781719663
28028,56057,0,56057,1.1281201839447021,0.0028967349611878856
28128,56257,0,56257,1.131636142730713,0.0028865494460537625
28228,56457,0,56457,1.1352698802947998,0.002869306967611539
28328,56657,0,56657,1.1391749382019043,0.0028516527401632073
28428,56857,0,56857,1.1428852081298828,0.0028328620082355973
28529,57059,0,57059,1.1467058658599854,0.0027957228795076634
28629,57259,0,57259,1.1503009796142578,0.002736760860113118
28729,57459,0,57459,1.1539888381958008,0.002675925385800521
28829,57659,0,57659,1.1575109958648682,0.0026297566770034017
28929,57859,0,57859,1.161041021347046,0.0025938837059872786
29029,58059,0,58059,1.1645541191101074,0.002562142342374719
29129,58259,0,58259,1.1680688858032227,0.0025430374654775065
29229,58459,0,58459,1.1716029644012451,0.0025409813493694903
29329,58659,0,58659,1.1751110553741455,0.0025383157864291646
29429,58859,0,58859,1.1786088943481445,0.0025167910720348056
29530,59061,0,59061,1.1821389198303223,0.002481681851320229
29630,59261,0,59261,1.1856489181518555,0.002448782228785596
29730,59461,0,59461,1.1893320083618164,0.0024182065431847906
29830,59661,0,59661,1.1929900646209717,0.0023861388914979487
29930,59861,0,59861,1.196531057357788,0.002364104747120316
30030,60061,0,60061,1.2000770568847656,0.002367698564722654
30130,60261,0,60261,1.2035839557647705,0.0023909315353088955
30230,60461,0,60461,1.207103967666626,0.0024129709734338383
30330,60661,0,60661,1.2105998992919922,0.0024270664134750757
30430,60861,0,60861,1.2140958309173584,0.0024395367695122525
30531,61063,0,61063,1.217829942703247,0.0024478946063307074
30631,61263,0,61263,1.2213060855865479,0.002442747059705675
30731,61463,0,61463,1.2248010635375977,0.0024290991694118982
30831,61663,0,61663,1.2286128997802734,0.0024256606886608996
30931,61863,0,61863,1.2321019172668457,0.0024409120402841857
31031,62063,0,62063,1.2355949878692627,0.0024653568860609257
31131,62263,0,62263,1.2399611473083496,0.002491638587731647
31231,62463,0,62463,1.2435331344604492,0.0025228999495527805
31331,62663,0,62663,1.2473008632659912,0.002556152224293601
31431,62863,0,62863,1.2510159015655518,0.0025770961227783084
31532,63065,0,63065,1.25474214553833,0.002578710047573433
31632,63265,0,63265,1.2583510875701904,0.0025708250686072823
31732,63465,0,63465,1.26192307472229,0.002565260237147976
31832,63665,0,63665,1.2654900550842285,0.002562116239532298
31932,63865,0,63865,1.269050121307373,0.0025593424183206273
32032,64065,0,64065,1.272723913192749,0.002564000987120601
32132,64265,0,64265,1.2762250900268555,0.0025805201565868947
32232,64465,0,64465,1.2797009944915771,0.002598429086823534
32332,64665,0,64665,1.2831859588623047,0.002604072588794919
32432,64865,0,64865,1.286729097366333,0.0025961199015487597
32533,65067,0,65067,1.2902662754058838,0.002580434899538899
32633,65267,0,65267,1.2937862873077393,0.002557471529815911
32733,65467,0,65467,1.2973110675811768,0.0025247817938927066
32833,65667,0,65667,1.3008430004119873,0.0024901144690407944
32933,65867,0,65867,1.3043429851531982,0.002466397793160908
33033,66067,0,66067,1.3078391551971436,0.002454819228397141
33133,66267,0,66267,1.311337947845459,0.0024454603410924477
33233,66467,0,66467,1.3148281574249268,0.002432846910746171
33333,66667,0,66667,1.3183350563049316,0.0024182556688892467
33433,66867,0,66867,1.321835994720459,0.0023985743866934794
33534,67069,0,67069,1.325364112854004,0.0023651400529902753
33634,67269,0,67269,1.328861951828003,0.002318907170465284
33734,67469,0,67469,1.3326680660247803,0.0022721500895469464
33834,67669,0,67669,1.3362791538238525,0.0022346662565864697
33934,67869,0,67869,1.3408279418945312,0.0022053767897853935
34034,68069,0,68069,1.3447020053863525,0.0021825933955287717
34134,68269,0,68269,1.348315954208374,0.0021700126169286126
34234,68469,0,68469,1.3518390655517578,0.0021665415103854974
34334,68669,0,68669,1.3553731441497803,0.0021606134371208647
34434,68869,0,68869,1.3588778972625732,0.0021427101809933643
34535,69071,0,69071,1.362403154373169,0.0021159631283091864
34635,69271,0,69271,1.3659000396728516,0.0020891404026423706
34735,69471,0,69471,1.3699140548706055,0.002063793360179333
34835,69671,0,69671,1.3734431266784668,0.002040907189189321
34935,69871,0,69871,1.3769550323486328,0.002028770954314745
35035,70071,0,70071,1.3804481029510498,0.002034549152724416
35135,70271,0,70271,1.3839600086212158,0.002052669323688617
35235,70471,0,70471,1.3877341747283936,0.0020709974722026158
35335,70671,0,70671,1.391254186630249,0.0020846801539058457
35435,70871,0,70871,1.3947761058807373,0.0020951716392265227
35536,71073,0,71073,1.398324966430664,0.002100399054862868
35636,71273,0,71273,1.4018280506134033,0.002096974938302714
35736,71473,0,71473,1.4053308963775635,0.0020904186106610804
35836,71673,0,71673,1.4088411331176758,0.002092034359565157
35936,71873,0,71873,1.4125499725341797,0.0021061480100324262
36036,72073,0,72073,1.4160749912261963,0.002127761501764157
36136,72273,0,72273,1.4195771217346191,0.002152533196306687
36236,72473,0,72473,1.4230751991271973,0.0021798869320937574
36336,72673,0,72673,1.4265830516815186,0.002205586639121379
36436,72873,0,72873,1.430105209350586,0.002221102722655808
36537,73075,0,73075,1.4336450099945068,0.002223570722706126
36637,73275,0,73275,1.4371531009674072,0.0022194318393253683
36737,73475,0,73475,1.4406630992889404,0.0022157487507988042
36837,73675,0,73675,1.4442508220672607,0.0022139257771392118
36937,73875,0,73875,1.4478249549865723,0.002214604506085151
37037,74075,0,74075,1.4514482021331787,0.0022215017775233836
37137,74275,0,74275,1.454962968826294,0.002235081247068343
37237,74475,0,74475,1.4584519863128662,0.002247825420073512
37337,74675,0,74675,1.4619290828704834,0.002251518604418499
37437,74875,0,74875,1.465433120727539,0.002245042937601857
37538,75077,0,75077,1.4689691066741943,0.002231014346963123
37638,75277,0,75277,1.4724669456481934,0.0022103529675977047
37738,75477,0,75477,1.4759650230407715,0.0021838873123087507
37838,75677,0,75677,1.4794659614562988,0.0021578568792885956
37938,75877,0,75877,1.4829812049865723,0.0021396246368093025
38038,76077,0,76077,1.486480951309204,0.002129259708038191
38138,76277,0,76277,1.4899981021881104,0.00212081880499033
38238,76477,0,76477,1.4934980869293213,0.0021104087864917166
38338,76677,0,76677,1.4971141815185547,0.002097047679753491
38438,76877,0,76877,1.5006420612335205,0.0020776336726437273
38539,77079,0,77079,1.5041768550872803,0.002047804554149655
38639,77279,0,77279,1.5076720714569092,0.002010141474435998
38739,77479,0,77479,1.5111701488494873,0.001972672241692261
38839,77679,0,77679,1.5146830081939697,0.0019417435881117022
38939,77879,0,77879,1.518315076828003,0.00191788715728436
39039,78079,0,78079,1.5221729278564453,0.0019008010596479048
39139,78279,0,78279,1.5255250930786133,0.001891489312936453
39239,78479,0,78479,1.5288619995117188,0.0018871085664988573
39339,78679,0,78679,1.53218412399292,0.0018798460438502528
39439,78879,0,78879,1.5355899333953857,0.001864446560580227
39540,79081,0,79081,1.539039134979248,0.0018428981672343637
39640,79281,0,79281,1.542375087738037,0.0018206565068441588
39740,79481,0,79481,1.545835018157959,0.0018000411650954675
39840,79681,0,79681,1.549149990081787,0.001783742000643617
39940,79881,0,79881,1.5526468753814697,0.001777376958453249
40040,80081,0,80081,1.5559659004211426,0.0017840396158051786
40140,80281,0,80281,1.5592799186706543,0.0017990672649556576
40240,80481,0,80481,1.5625998973846436,0.0018146615456116344
40340,80681,0,80681,1.5659940242767334,0.0018270402166984331
40440,80881,0,80881,1.5693728923797607,0.001835746855021983
40541,81083,0,81083,1.572732925415039,0.0018394784187885458
40641,81283,0,81283,1.576186180114746,0.0018377815219774848
40741,81483,0,81483,1.5795142650604248,0.00183555560134167
40841,81683,0,81683,1.5828440189361572,0.0018399645519211777
40941,81883,0,81883,1.5862071514129639,0.00185344131589539
41041,82083,0,82083,1.5895459651947021,0.00187306880101494
41141,82283,0,82283,1.5929689407348633,0.0018957201759200815
41241,82483,0,82483,1.596365213394165,0.0019193069247216187
41341,82683,0,82683,1.5997068881988525,0.0019397285607861035
41441,82883,0,82883,1.6030750274658203,0.0019518075881724579
41542,83085,0,83085,1.6064488887786865,0.0019546000724135013
41642,83285,0,83285,1.609762191772461,0.0019525026496811885
41742,83485,0,83485,1.613145112991333,0.0019502839928196548
41842,83685,0,83685,1.616481065750122,0.0019498322230946388
41942,83885,0,83885,1.619854211807251,0.0019524621463306805
42042,84085,0,84085,1.6232750415802002,0.0019599428528215656
42142,84285,0,84285,1.6266450881958008,0.0019710879937284175
42242,84485,0,84485,1.63002610206604,0.0019803854505259792
42342,84685,0,84685,1.6334199905395508,0.00198255989837258
42442,84885,0,84885,1.6370229721069336,0.0019765870262380405
42543,85087,0,85087,1.6404950618743896,0.001963759587821181
42643,85287,0,85287,1.6438210010528564,0.0019454469354159318
42743,85487,0,85487,1.6471660137176514,0.0019236817275325418
42843,85687,0,85687,1.6506929397583008,0.001903304448633611
42943,85887,0,85887,1.6540250778198242,0.001888684005523003
43043,86087,0,86087,1.6582798957824707,0.0018794421717620684
43143,86287,0,86287,1.6615900993347168,0.0018716928282145036
43243,86487,0,86487,1.6649038791656494,0.0018623299520830734
43343,86687,0,86687,1.668360948562622,0.0018495533259617865
43443,86887,0,86887,1.6716768741607666,0.0018308946169432092
43544,87089,0,87089,1.675034999847412,0.001804305349139528
43644,87289,0,87289,1.6783461570739746,0.00177275944832017
43744,87489,0,87489,1.6816561222076416,0.001741861222188358
43844,87689,0,87689,1.685028076171875,0.001716075882038835
43944,87889,0,87889,1.689070224761963,0.0016965063759835366
44044,88089,0,88089,1.6925499439239502,0.0016831551437075628
44144,88289,0,88289,1.6958909034729004,0.0016755953064798953
44244,88489,0,88489,1.6992390155792236,0.0016706572997871952
44344,88689,0,88689,1.702639102935791,0.001662943041747961
44444,88889,0,88889,1.7059688568115234,0.0016493942336650478
44545,89091,0,89091,1.709522008895874,0.001631404133151033
44645,89291,0,89291,1.7128551006317139,0.0016128391603971583
44745,89491,0,89491,1.7162270545959473,0.001596276118128307
44845,89691,0,89691,1.7197661399841309,0.0015847302278729437
44945,89891,0,89891,1.7231628894805908,0.0015819193136072374
45045,90091,0,90091,1.7265658378601074,0.0015888856592116217
45145,90291,0,90291,1.7299671173095703,0.0016018155797608274
45245,90491,0,90491,1.73335599899292,0.0016152686111808672
45345,90691,0,90691,1.7367520332336426,0.0016261502889058426
45445,90891,0,90891,1.7401630878448486,0.0016334445515196866
45546,91093,0,91093,1.7435970306396484,0.0016365424923272182
45646,91293,0,91293,1.7470111846923828,0.0016363215071425394
45746,91493,0,91493,1.750411033630371,0.0016368719445404487
45846,91693,0,91693,1.7539000511169434,0.001642922858312116
45946,91893,0,91893,1.7573041915893555,0.0016559245946463973
46046,92093,0,92093,1.7606990337371826,0.001673934619050464
46146,92293,0,92293,1.7641081809997559,0.0016943532655905075
46246,92493,0,92493,1.7675058841705322,0.0017146210662758554
46346,92693,0,92693,1.7708978652954102,0.0017312309762592898
46446,92893,0,92893,1.7744920253753662,0.00174098146307194
46547,93095,0,93095,1.777940034866333,0.0017438341999876249
46647,93295,0,93295,1.7814340591430664,0.0017429755020846177
46747,93495,0,93495,1.784877061843872,0.001741921796825721
46847,93695,0,93695,1.7883782386779785,0.001742610907538379
46947,93895,0,93895,1.7919402122497559,0.001746297346197491
47047,94095,0,94095,1.795409917831421,0.0017535961114787015
47147,94295,0,94295,1.7988171577453613,0.0017627427130379565
47247,94495,0,94495,1.8022501468658447,0.0017695842377897883
47347,94695,0,94695,1.8056461811065674,0.0017705243217322978
47447,94895,0,94895,1.8090450763702393,0.0017646910755345162
47548,95097,0,95097,1.8124611377716064,0.001752873039526044
47648,95297,0,95297,1.8158762454986572,0.001736709332267942
47748,95497,0,95497,1.8192791938781738,0.0017185381453621042
47848,95697,0,95697,1.8226020336151123,0.0017020556367588222
47948,95897,0,95897,1.825937032699585,0.0016899421372710982
48048,96097,0,96097,1.8294620513916016,0.0016816394361211457
48148,96297,0,96297,1.832787036895752,0.0016743529732910726
48248,96497,0,96497,1.836143970489502,0.001665476250721223
48348,96697,0,96697,1.8396549224853516,0.0016530795894744753
48448,96897,0,96897,1.842972993850708,0.0016353771220881086
48549,97099,0,97099,1.846325159072876,0.001611599123157771
48649,97299,0,97299,1.8496901988983154,0.0015846500058269701
48749,97499,0,97499,1.8530702590942383,0.0015586584171250505
48849,97699,0,97699,1.8564071655273438,0.0015369674553322628
48949,97899,0,97899,1.859910011291504,0.0015207396250883228
49049,98099,0,98099,1.8632361888885498,0.0015099043845301888
49149,98299,0,98299,1.866569995880127,0.001503347659574665
49249,98499,0,98499,1.8699510097503662,0.0014980979783085903
49349,98699,0,98699,1.8733620643615723,0.001490344674723202
49449,98899,0,98899,1.8772571086883545,0.0014782526788620924
49550,99101,0,99101,1.8806910514831543,0.0014629201228826235
49650,99301,0,99301,1.884155035018921,0.0014473930755653677
49750,99501,0,99501,1.887679100036621,0.0014342099814929612
49850,99701,0,99701,1.8911731243133545,0.001426143531259742
49950,99901,0,99901,1.8946659564971924,0.0014256056501998754
50050,100101,0,100101,1.8982181549072266,0.0014325955599946872
50150,100301,0,100301,1.9017689228057861,0.001443964823865616
50250,100501,0,100501,1.9053690433502197,0.00145567188038496
50350,100701,0,100701,1.908884048461914,0.00146515598749627
50450,100901,0,100901,1.9125089645385742,0.001471392692476386
50551,101103,0,101103,1.916067123413086,0.0014743001787036042
50651,101303,0,101303,1.9196979999542236,0.0014752831662834588
50751,101503,0,101503,1.9232730865478516,0.0014776801378005996
50851,101703,0,101703,1.9268090724945068,0.0014847256112442478
50951,101903,0,101903,1.930413007736206,0.0014972804382558545
51051,102103,0,102103,1.9339990615844727,0.0015138549507893954
51151,102303,0,102303,1.9375932216644287,0.0015321431250083664
51251,102503,0,102503,1.9411580562591553,0.0015495912978981258
51351,102703,0,102703,1.94482421875,0.001563358806754074
51451,102903,0,102903,1.9484329223632812,0.0015714482131111915
51552,103105,0,103105,1.952120065689087,0.0015742496757250536
51652,103305,0,103305,1.955714225769043,0.0015742132430969882
51752,103505,0,103505,1.9593260288238525,0.0015740859340015211
51852,103705,0,103705,1.9628591537475586,0.0015756322334849514
51952,103905,0,103905,1.9664452075958252,0.0015798242092214393
52052,104105,0,104105,1.9700119495391846,0.00158660307348652
52152,104305,0,104305,1.9736452102661133,0.001594092872228056
52252,104505,0,104505,1.9772560596466064,0.0015990904973808282
52352,104705,0,104705,1.980794906616211,0.0015990256360576252
52452,104905,0,104905,1.9844181537628174,0.001593220942615384
52553,105107,0,105107,1.9880499839782715,0.0015823085725213055
52653,105307,0,105307,1.9917278289794922,0.0015680283698008043
52753,105507,0,105507,1.995365858078003,0.0015526400410521425
52853,105707,0,105707,1.9989981651306152,0.0015389546135519798
52953,105907,0,105907,2.0031850337982178,0.0015286469364750711
53053,106107,0,106107,2.0068180561065674,0.0015210830926291688
53153,106307,0,106307,2.0109829902648926,0.001514087654483631
53253,106507,0,106507,2.014400005340576,0.0015054371893267224
53353,106707,0,106707,2.0181918144226074,0.0014933736354768282
53453,106907,0,106907,2.021656036376953,0.0014766919303561717
53554,107109,0,107109,2.0251641273498535,0.0014553321310045483
53654,107309,0,107309,2.0286290645599365,0.001431978129637149
53754,107509,0,107509,2.0320918560028076,0.0014098005328303052
53854,107709,0,107709,2.0356149673461914,0.0013913938383567056
53954,107909,0,107909,2.0404410362243652,0.0013777651422495036
54054,108109,0,108109,2.0439019203186035,0.001368674712736372
54154,108309,0,108309,2.0474109649658203,0.0013627332153544128
54254,108509,0,108509,2.050922155380249,0.0013573385267385061
54354,108709,0,108709,2.054392099380493,0.0013497499870769975
54454,108909,0,108909,2.0578551292419434,0.0013388685261992274
54555,109111,0,109111,2.061483144760132,0.0013256575137909697
54655,109311,0,109311,2.065088987350464,0.0013126796004695681
54755,109511,0,109511,2.0685372352600098,0.0013022792481171162
54855,109711,0,109711,2.072007894515991,0.001296798391623782
54955,109911,0,109911,2.0756711959838867,0.0012977533953724629
55055,110111,0,110111,2.079303026199341,0.0013046169334038893
55155,110311,0,110311,2.083024024963379,0.001314747113687327
55255,110511,0,110511,2.08660888671875,0.0013250041709871683
55355,110711,0,110711,2.0900821685791016,0.0013332857111948589
55455,110911,0,110911,2.0935401916503906,0.001338756528243636
55556,111113,0,111113,2.0980610847473145,0.0013416946855590904
55656,111313,0,111313,2.101519823074341,0.0013436433226989945
55756,111513,0,111513,2.104964256286621,0.0013473029313144638
55856,111713,0,111713,2.108415126800537,0.0013549428453512148
55956,111913,0,111913,2.111846923828125,0.0013670299464661575
56056,112113,0,112113,2.1153111457824707,0.0013822859606987328
56156,112313,0,112313,2.118833065032959,0.0013986276495806529
56256,112513,0,112513,2.122354030609131,0.0014137135899817091
56356,112713,0,112713,2.125887155532837,0.0014253041260339978
56456,112913,0,112913,2.129401206970215,0.0014321617427647832
56557,113115,0,113115,2.132951021194458,0.001434877803544759
56657,113315,0,113315,2.136521100997925,0.0014354256210066564
56757,113515,0,113515,2.1401240825653076,0.0014360229291114713
56857,113715,0,113715,2.1436550617218018,0.0014381689783241978
56957,113915,0,113915,2.1472229957580566,0.0014425229720969805
57057,114115,0,114115,2.150745153427124,0.0014486468343088718
57157,114315,0,114315,2.1542890071868896,0.0014547473271161297
57257,114515,0,114515,2.1578140258789062,0.0014583069703305832
57357,114715,0,114715,2.1613481044769287,0.0014574324940890948
57457,114915,0,114915,2.164865016937256,0.0014516483723575394
57558,115117,0,115117,2.168416976928711,0.0014415642444502198
57658,115317,0,115317,2.171950101852417,0.0014289046131346177
57758,115517,0,115517,2.1755049228668213,0.001415699521821569
57858,115717,0,115717,2.179046869277954,0.0014040874652643553
57958,115917,0,115917,2.1826581954956055,0.0013951133704164019
58058,116117,0,116117,2.1868669986724854,0.0013881101410605037
58158,116317,0,116317,2.190425157546997,0.0013812903671307703
58258,116517,0,116517,2.1943271160125732,0.0013727584629237572
58358,116717,0,116717,2.197892904281616,0.001361034835554449
58458,116917,0,116917,2.2017669677734375,0.0013453705796312573
58559,117119,0,117119,2.2054340839385986,0.001326097236770188
58659,117319,0,117319,2.2089879512786865,0.0013056419979946352
58759,117519,0,117519,2.2125749588012695,0.0012865137995573131
58859,117719,0,117719,2.2161669731140137,0.0012707579701460867
58959,117919,0,117919,2.2197110652923584,0.0012591564610793036
59059,118119,0,118119,2.2232539653778076,0.0012513118157479498
59159,118319,0,118319,2.226792097091675,0.0012457782827354135
59259,118519,0,118519,2.2305381298065186,0.0012403512366213174
59359,118719,0,118719,2.234490156173706,0.0012330350489255998
59459,118919,0,118919,2.238278865814209,0.001223204105869211
59560,119121,0,119121,2.2423551082611084,0.0012117644303724217
59660,119321,0,119321,2.24596905708313,0.0012009442503621134
59760,119521,0,119521,2.24949312210083,0.0011928230134014698
59860,119721,0,119721,2.2531981468200684,0.001189288274385339
59960,119921,0,119921,2.2567949295043945,0.001191239292838619
60060,120121,0,120121,2.2603650093078613,0.0011978910627687836
60160,120321,0,120321,2.2639801502227783,0.0012069953109918629
60260,120521,0,120521,2.267529010772705,0.0012160416406080858
60360,120721,0,120721,2.271031141281128,0.0012233289727530394
60460,120921,0,120921,2.2746970653533936,0.0012282581349603644
60561,121123,0,121123,2.2782840728759766,0.0012313321069720839
60661,121323,0,121323,2.28183913230896,0.0012340492612210427
60761,121523,0,121523,2.2853949069976807,0.0012385862275623662
60861,121723,0,121723,2.2889840602874756,0.0012465550501840653
60961,121923,0,121923,2.2925660610198975,0.0012581417940070547
61061,122123,0,122123,2.2961370944976807,0.0012721759013534003
61161,122323,0,122323,2.2997052669525146,0.0012867770811281246
61261,122523,0,122523,2.303274154663086,0.0012998905564955393
61361,122723,0,122723,2.306823968887329,0.0013097779899204935
61461,122923,0,122923,2.3103859424591064,0.0013156965635649413
61562,123125,0,123125,2.3139760494232178,0.0013183268886036094
61662,123325,0,123325,2.317549228668213,0.0013193081901889466
61762,123525,0,123525,2.321101188659668,0.0013204583064103268
61862,123725,0,123725,2.3246610164642334,0.0013229926965235045
61962,123925,0,123925,2.3282251358032227,0.001327294607374821
62062,124125,0,124125,2.331808090209961,0.0013327255067515278
62162,124325,0,124325,2.335353136062622,0.0013376491374219816
62262,124525,0,124525,2.3389031887054443,0.0013400594333804524
62362,124725,0,124725,2.342466115951538,0.0013385416414368352
62462,124925,0,124925,2.3460280895233154,0.0013328070640767876
62563,125127,0,125127,2.350684881210327,0.001323481762663548
62663,125327,0,125327,2.354182004928589,0.0013122055010089079
62763,125527,0,125527,2.357678174972534,0.001300734676191776
62863,125727,0,125727,2.3611881732940674,0.0012906962131568177
62963,125927,0,125927,2.364698886871338,0.0012827227509193122
63063,126127,0,126127,2.3682188987731934,0.0012761361411390132
63163,126327,0,126327,2.3717150688171387,0.0012694212515995242
63263,126527,0,126527,2.37520694732666,0.0012609750828942302
63363,126727,0,126727,2.3787100315093994,0.0012496128339744
63463,126927,0,126927,2.382205009460449,0.001234930306391453
63564,127129,0,127129,2.385767936706543,0.001217469957805779
63664,127329,0,127329,2.3893609046936035,0.0011994065953910115
63764,127529,0,127529,2.392911911010742,0.0011827644365060613
63864,127729,0,127729,2.3964061737060547,0.0011691608259753834
63964,127929,0,127929,2.39990496635437,0.0011591500512954734
64064,128129,0,128129,2.4035580158233643,0.0011522205255517085
64164,128329,0,128329,2.407111883163452,0.001146982188772943
64264,128529,0,128529,2.410668134689331,0.0011416009200992106
64364,128729,0,128729,2.414216995239258,0.0011346175558625768
64464,128929,0,128929,2.417710065841675,0.0011257272052057057
64565,129131,0,129131,2.4211652278900146,0.001115808639143752
64665,129331,0,129331,2.424527883529663,0.0011068243116640866
64765,129531,0,129531,2.427888870239258,0.001100567830344454
64865,129731,0,129731,2.4312479496002197,0.00109851252859559
64965,129931,0,129931,2.4346508979797363,0.001101130304909402
65065,130131,0,130131,2.438149929046631,0.0011075219812861166
65165,130331,0,130331,2.4415621757507324,0.001115755643891863
65265,130531,0,130531,2.4449520111083984,0.0011237911960981048
65365,130731,0,130731,2.449080228805542,0.001130274921076301
65465,130931,0,130931,2.4525229930877686,0.001134828826836185
65566,131133,0,131133,2.4559781551361084,0.0011380825563218396
65666,131333,0,131333,2.459439277648926,0.0011414079735422653
65766,131533,0,131533,2.4628028869628906,0.0011465554335009156
65866,131733,0,131733,2.466235876083374,0.0011546681539989963
65966,131933,0,131933,2.4696269035339355,0.001165726350479626
66066,132133,0,132133,2.4729971885681152,0.0011786288192106341
66166,132333,0,132333,2.4763588905334473,0.001191690770077236
66266,132533,0,132533,2.4797089099884033,0.0012031546966401784
66366,132733,0,132733,2.4830620288848877,0.0012116872205620423
66466,132933,0,132933,2.4864580631256104,0.0012168758669294545
66567,133135,0,133135,2.4898860454559326,0.0012194317193560643
66667,133335,0,133335,2.4932281970977783,0.0012207407797331406
66767,133535,0,133535,2.4965720176696777,0.0012222991794524135
66867,133735,0,133735,2.499958038330078,0.0012250560419659654
66967,133935,0,133935,2.5033512115478516,0.0012291736107488877
67067,134135,0,134135,2.5066990852355957,0.0012339206869557088
67167,134335,0,134335,2.5102789402008057,0.0012378394893487123
67267,134535,0,134535,2.5136289596557617,0.0012393177079660135
67367,134735,0,134735,2.5170440673828125,0.001237296667797865
67467,134935,0,134935,2.5207512378692627,0.0012316485220151459
67568,135137,0,135137,2.52414608001709,0.001223016155154614
67668,135337,0,135337,2.527517080307007,0.0012129176072889238
67768,135537,0,135537,2.530879020690918,0.0012028394107488792
67868,135737,0,135737,2.535799026489258,0.0011940161635542708
67968,135937,0,135937,2.5394740104675293,0.0011868012363774071
68068,136137,0,136137,2.5428380966186523,0.0011805212034008876
68168,136337,0,136337,2.5462231636047363,0.0011738724413281761
68268,136537,0,136537,2.550309896469116,0.001165514426206311
68368,136737,0,136737,2.5537970066070557,0.0011545350063868374
68468,136937,0,136937,2.557539224624634,0.0011407845371504465
68569,137139,0,137139,2.560987949371338,0.0011249117431240384
68669,137339,0,137339,2.5651650428771973,0.0011088563688309893
68769,137539,0,137539,2.568681001663208,0.0010942690903759655
68869,137739,0,137739,2.5720388889312744,0.001082422994812133
68969,137939,0,137939,2.575618028640747,0.0010736708217486185
69069,138139,0,138139,2.5796051025390625,0.0010674326315821324
69169,138339,0,138339,2.5830330848693848,0.001062427913293851
69269,138539,0,138539,2.5864830017089844,0.001057148788560264
69369,138739,0,138739,2.5903899669647217,0.0010505338237381976
69469,138939,0,138939,2.595863103866577,0.0010425026912944588
69570,139141,0,139141,2.599390983581543,0.0010339126606182904
69670,139341,0,139341,2.6028249263763428,0.001026495450055356
69770,139541,0,139541,2.606271982192993,0.0010217661391864405
69870,139741,0,139741,2.611877202987671,0.001020843501182434
69970,139941,0,139941,2.6156911849975586,0.00102390269709295
70070,140141,0,140141,2.6199162006378174,0.0010300095649300647
70170,140341,0,140341,2.6240949630737305,0.0010374949610785222
70270,140541,0,140541,2.628316879272461,0.0010446884701483068
70370,140741,0,140741,2.634481906890869,0.0010505317433506447
70470,140941,0,140941,2.639354944229126,0.0010548314352339418
70571,141143,0,141143,2.643930196762085,0.0010582760176608638
70671,141343,0,141343,2.648426055908203,0.001062079422990922
70771,141543,0,141543,2.6531269550323486,0.001067644585432602
70871,141743,0,141743,2.657792091369629,0.0010757683914840797
70971,141943,0,141943,2.662247896194458,0.001086280161536596
71071,142143,0,142143,2.666651964187622,0.001098138340525941
71171,142343,0,142343,2.67108416557312,0.0011098464311664297
71271,142543,0,142543,2.675725221633911,0.0011199259105610653
71371,142743,0,142743,2.6803150177001953,0.0011273660513241653
71471,142943,0,142943,2.6847779750823975,0.001131979012644588
71572,143145,0,143145,2.6895790100097656,0.0011344729888931018
71672,143345,0,143345,2.6940760612487793,0.0011360291941346357
71772,143545,0,143545,2.6985931396484375,0.0011378759739134109
71872,143745,0,143745,2.70304799079895,0.0011407285274978249
71972,143945,0,143945,2.7076261043548584,0.001144581882564306
72072,144145,0,144145,2.712111234664917,0.0011486769909599388
72172,144345,0,144345,2.7166459560394287,0.0011517331373246031
72272,144545,0,144545,2.7208681106567383,0.0011524496331047787
72372,144745,0,144745,2.7247021198272705,0.0011500418924641545
72472,144945,0,144945,2.7283971309661865,0.0011445132817639889
72573,145147,0,145147,2.732077121734619,0.0011365109185042838
72673,145347,0,145347,2.735759973526001,0.001127414905486295
72773,145547,0,145547,2.7395730018615723,0.001118465039975015
72873,145747,0,145747,2.7432940006256104,0.0011105922646403718
72973,145947,0,145947,2.747101068496704,0.0011039565284082827
73073,146147,0,146147,2.7506871223449707,0.0010979021646176223
73173,146347,0,146347,2.7544500827789307,0.0010913023810353642
73273,146547,0,146547,2.7581520080566406,0.0010830501191108903
73373,146747,0,146747,2.7620890140533447,0.0010724700576519703
73473,146947,0,146947,2.7656900882720947,0.0010595972327050896
73574,147149,0,147149,2.769379138946533,0.0010451243864532133
73674,147349,0,147349,2.773400068283081,0.0010307764571610273
73774,147549,0,147549,2.7770261764526367,0.0010179050433600494
73874,147749,0,147749,2.7806320190429688,0.0010075025947601035
73974,147949,0,147949,2.784230947494507,0.000999755940570069
74074,148149,0,148149,2.7878479957580566,0.0009940549924147145
74174,148349,0,148349,2.791781187057495,0.0009892509704428464
74274,148549,0,148549,2.7954869270324707,0.0009841161546772458
74374,148749,0,148749,2.7991838455200195,0.0009778906604127285
74474,148949,0,148949,2.8028790950775146,0.0009706534699824129
74575,149151,0,149151,2.8067851066589355,0.000963235322718374
74675,149351,0,149351,2.8104560375213623,0.0009571588910445978
74775,149551,0,149551,2.8141701221466064,0.0009536822883274291
74875,149751,0,149751,2.817946195602417,0.0009536305562602861
74975,149951,0,149951,2.822200059890747,0.0009569733320912373
75075,150151,0,150151,2.825923204421997,0.0009627865947572978
75175,150351,0,150351,2.829524040222168,0.0009696252805129255
75275,150551,0,150551,2.833138942718506,0.0009761192061184185
75375,150751,0,150751,2.8372390270233154,0.0009814569153328478
75475,150951,0,150951,2.841132164001465,0.000985589195091962
75576,151153,0,151153,2.8447301387786865,0.0009892179249460424
75676,151353,0,151353,2.848677158355713,0.000993392577900434
75776,151553,0,151553,2.853555917739868,0.0009992315010242854
75876,151753,0,151753,2.85771107673645,0.0010072697187388814
75976,151953,0,151953,2.8614389896392822,0.0010172283249528437
76076,152153,0,152153,2.8650949001312256,0.001028126651325982
76176,152353,0,152353,2.868774890899658,0.001038646622963756
76276,152553,0,152553,2.8726680278778076,0.0010475591321412114
76376,152753,0,152753,2.8764820098876953,0.0010541089416690136
76476,152953,0,152953,2.8800342082977295,0.0010582622461742708
76577,153155,0,153155,2.8836240768432617,0.0010607040932872844
76677,153355,0,153355,2.887326955795288,0.0010624423897540266
76777,153555,0,153555,2.8910861015319824,0.0010644792284496484
76877,153755,0,153755,2.895432949066162,0.0010673323349624038
76977,153955,0,153955,2.898948907852173,0.0010708756407884438
77077,154155,0,154155,2.9024908542633057,0.0010743610897160404
77177,154355,0,154355,2.9062180519104004,0.0010766741907691337
77277,154555,0,154555,2.9107091426849365,0.001076766172798292
77377,154755,0,154755,2.9143290519714355,0.0010740675802313
77477,154955,0,154955,2.9179630279541016,0.0010686840101889498
77578,155157,0,155157,2.9216930866241455,0.0010612520454229123
77678,155357,0,155357,2.9260900020599365,0.0010530103474834815
77778,155557,0,155557,2.929650068283081,0.0010449812440112172
77878,155757,0,155757,2.933237075805664,0.0010378588910046292
77978,155957,0,155957,2.936803102493286,0.0010316681549368664
78078,156157,0,156157,2.94096302986145,0.0010257819239320035
78178,156357,0,156357,2.944582939147949,0.0010192278131191368
78278,156557,0,156557,2.948184013366699,0.0010111040246629243
78378,156757,0,156757,2.9517860412597656,0.0010009338801809779
78478,156957,0,156957,2.9559099674224854,0.000988883896991085
78579,157159,0,157159,2.959567070007324,0.0009756528945409037
78679,157359,0,157359,2.9631760120391846,0.000962770786885982
78779,157559,0,157559,2.966797113418579,0.0009513435271498311
78879,157759,0,157759,2.9705841541290283,0.000942134118170347
78979,157959,0,157959,2.9742720127105713,0.0009351994843797639
79079,158159,0,158159,2.977879047393799,0.0009299282455535872
79179,158359,0,158359,2.9831809997558594,0.0009253084871290601
79279,158559,0,158559,2.9869260787963867,0.0009203502965556831
79379,158759,0,158759,2.9907588958740234,0.0009145258799706488
79479,158959,0,158959,2.9943530559539795,0.0009080264991396564
79580,159161,0,159161,2.9980008602142334,0.0009016478581305168
79680,159361,0,159361,3.0015950202941895,0.000896720479762326
79780,159561,0,159561,3.005255937576294,0.0008942730757924846
79880,159761,0,159761,3.008970022201538,0.000894892054526377
79980,159961,0,159961,3.012559175491333,0.000898406278121127
80080,160161,0,160161,3.0161211490631104,0.0009039281050257195
80180,160361,0,160361,3.0196261405944824,0.0009102070487694014
80280,160561,0,160561,3.023428201675415,0.0009161213339080752
80380,160761,0,160761,3.0269949436187744,0.0009210627257674832
80480,160961,0,160961,3.0305700302124023,0.0009250889085619462
80581,161163,0,161163,3.0341591835021973,0.0009288855001947785
80681,161363,0,161363,3.037943124771118,0.0009333430672882763
80781,161563,0,161563,3.041501998901367,0.0009393457209627499
80881,161763,0,161763,3.0449979305267334,0.000947227954407332
80981,161963,0,161963,3.0485000610351562,0.0009566364992142678
81081,162163,0,162163,3.0519859790802,0.0009666556808162054
81181,162363,0,162363,3.0557498931884766,0.0009761334800950727
81281,162563,0,162563,3.0593390464782715,0.000984057923238766
81381,162763,0,162763,3.062840223312378,0.0009898753841833911
81481,162963,0,162963,3.0663528442382812,0.0009936572447954426
81582,163165,0,163165,3.0699379444122314,0.000996052643186995
81682,163365,0,163365,3.0736582279205322,0.0009979188030616651
81782,163565,0,163565,3.0772180557250977,0.00100006586852164
81882,163765,0,163765,3.08076810836792,0.0010028493010776991
81982,163965,0,163965,3.0843241214752197,0.0010060591730787088
82082,164165,0,164165,3.0881130695343018,0.0010089813913014317
82182,164365,0,164365,3.0916481018066406,0.0010106534682368252
82282,164565,0,164565,3.095255136489868,0.0010102333151440046
82382,164765,0,164765,3.0987861156463623,0.001007321848753464
82482,164965,0,164965,3.1024110317230225,0.0010021007930145808
82583,165167,0,165167,3.1062259674072266,0.0009951833618913296
82683,165367,0,165367,3.1097640991210938,0.0009876707091756424
82783,165567,0,165567,3.113284111022949,0.0009803972486307473
82883,165767,0,165767,3.1167800426483154,0.0009738716515537823
82983,165967,0,165967,3.12054705619812,0.0009680251008316155
83083,166167,0,166167,3.1241350173950195,0.0009622674978916743
83183,166367,0,166367,3.127635955810547,0.0009557641521839236
83283,166567,0,166567,3.1311402320861816,0.0009477917322843659
83383,166767,0,166767,3.134683847427368,0.0009380364695932248
83483,166967,0,166967,3.138427972793579,0.0009267560803420624
83584,167169,0,167169,3.1423659324645996,0.0009146319587977128
83684,167369,0,167369,3.146127223968506,0.0009030174031439471
83784,167569,0,167569,3.1496479511260986,0.0008928135405595049
83884,167769,0,167769,3.153323173522949,0.000884596317954252
83984,167969,0,167969,3.15708589553833,0.0008783251616144327
84084,168169,0,168169,3.160644054412842,0.000873407874743729
84184,168369,0,168369,3.164292097091675,0.0008689655711052333
84284,168569,0,168569,3.1679091453552246,0.0008642089964452994
84384,168769,0,168769,3.171663999557495,0.0008587904249607236
84484,168969,0,168969,3.1751749515533447,0.000852978107370054
84585,169171,0,169171,3.1790311336517334,0.00084752432169788
84685,169371,0,169371,3.1825249195098877,0.0008435828867218076
84785,169571,0,169571,3.1860039234161377,0.0008419820779379084
84885,169771,0,169771,3.1911139488220215,0.000843117064672766
84985,169971,0,169971,3.194791078567505,0.0008467226248128713
85085,170171,0,170171,3.198374032974243,0.0008519626875088011
85185,170371,0,170371,3.202700138092041,0.0008577575277262221
85285,170571,0,170571,3.2079219818115234,0.0008631927728393921
85385,170771,0,170771,3.2114319801330566,0.0008678251250297845
85485,170971,0,170971,3.2149388790130615,0.0008717876261863695
85586,171173,0,171173,3.218487024307251,0.0008757308410332178
85686,171373,0,171373,3.2222111225128174,0.0008803975726308011
85786,171573,0,171573,3.226487159729004,0.0008864785712112553
85886,171773,0,171773,3.2299678325653076,0.0008941541631040388
85986,171973,0,171973,3.2334530353546143,0.0009030236132339664
86086,172173,0,172173,3.237173080444336,0.0009122398475144123
86186,172373,0,172373,3.2423360347747803,0.0009208029937222869
86286,172573,0,172573,3.245877981185913,0.0009278871317429346
86386,172773,0,172773,3.249380111694336,0.0009330972104073045
86486,172973,0,172973,3.2528951168060303,0.0009365749854052516
86587,173175,0,173175,3.2572450637817383,0.0009389256965602678
86687,173375,0,173375,3.2608048915863037,0.0009408738110536373
86787,173575,0,173575,3.2643678188323975,0.0009430668705487247
86887,173775,0,173775,3.268019914627075,0.0009457297563372018
86987,173975,0,173975,3.272245168685913,0.0009485978005525292
87087,174175,0,174175,3.2761752605438232,0.0009510039896589251
87187,174375,0,174375,3.279932975769043,0.0009521228972955541
87287,174575,0,174575,3.283474922180176,0.0009512835600976517
87387,174775,0,174775,3.287317991256714,0.0009482220234699681
87487,174975,0,174975,3.2915141582489014,0.0009431738001132771
87588,175177,0,175177,3.295168161392212,0.0009367190248346826
87688,175377,0,175377,3.2989261150360107,0.0009298293871590868
87788,175577,0,175577,3.3026230335235596,0.0009231788541380415
87888,175777,0,175777,3.306917190551758,0.0009171306367946925
87988,175977,0,175977,3.3104441165924072,0.0009115525521134318
88088,176177,0,176177,3.314249038696289,0.0009058976204110063
88188,176377,0,176377,3.3180339336395264,0.000899454848901086
88288,176577,0,176577,3.3483850955963135,0.0008916545532991943
88388,176777,0,176777,3.3699910640716553,0.0008823143472637314
88488,176977,0,176977,3.3758552074432373,0.0008717526528191332
88589,177179,0,177179,3.3809049129486084,0.0008606188648109262
88689,177379,0,177379,3.3858072757720947,0.0008501066459656683
88789,177579,0,177579,3.3908050060272217,0.0008409450479955734
88889,177779,0,177779,3.39578914642334,0.0008335584689124669
88989,177979,0,177979,3.4024641513824463,0.000827836304251596
89089,178179,0,178179,3.407876968383789,0.0008232192833545158
89189,178379,0,178379,3.4231371879577637,0.0008189531924501059
89289,178579,0,178579,3.4282398223876953,0.0008144174185373537
89389,178779,0,178779,3.4337339401245117,0.000809404162514606
89489,178979,0,178979,3.438847064971924,0.0008042315951174141
89590,179181,0,179181,3.4442861080169678,0.0007996018393932136
89690,179381,0,179381,3.4491569995880127,0.0007965070918047374
89790,179581,0,179581,3.4542860984802246,0.0007956031503644702
89890,179781,0,179781,3.459423065185547,0.0007971336884171355
89990,179981,0,179981,3.4643101692199707,0.0008007734895635716
90090,180181,0,180181,3.4691169261932373,0.0008057464206869393
90190,180381,0,180381,3.4743869304656982,0.0008111233436595108
90290,180581,0,180581,3.4792661666870117,0.000816163577950558
90390,180781,0,180781,3.4840471744537354,0.0008205558831743719
90490,180981,0,180981,3.488896131515503,0.0008244831050824066
90591,181183,0,181183,3.4939231872558594,0.0008285494418414911
90691,181383,0,181383,3.4987399578094482,0.0008333633743347014
90791,181583,0,181583,3.5032429695129395,0.0008394559346877494
90891,181783,0,181783,3.5082719326019287,0.0008468893408817444
90991,181983,0,181983,3.513010025024414,0.0008552365358413432
91091,182183,0,182183,3.5174720287323,0.0008637209964976449
91191,182383,0,182383,3.5218911170959473,0.0008714804862890933
91291,182583,0,182583,3.5272090435028076,0.0008778468552083648
91391,182783,0,182783,3.5316529273986816,0.0008825492118494932
91491,182983,0,182983,3.5360829830169678,0.0008857743363477003
91592,183185,0,183185,3.5413761138916016,0.000888078899176781
91692,183385,0,183385,3.5457961559295654,0.0008900699096325926
91792,183585,0,183585,3.55013108253479,0.0008922577659147486
91892,183785,0,183785,3.5546162128448486,0.0008947641844294143
91992,183985,0,183985,3.5591139793395996,0.0008972920815997399
92092,184185,0,184185,3.563408851623535,0.0008992284103945579
92192,184385,0,184385,3.5672829151153564,0.0008998702672839234
92292,184585,0,184585,3.5713300704956055,0.0008986890341270558
92392,184785,0,184785,3.574937105178833,0.0008955275128232423
92492,184985,0,184985,3.5785129070281982,0.0008906565533221694
92593,185187,0,185187,3.5821280479431152,0.0008846166159663174
92693,185387,0,185387,3.585875988006592,0.000878260034818713
92793,185587,0,185587,3.5897490978240967,0.0008721249110783372
92893,185787,0,185787,3.593717098236084,0.0008664606690127524
92993,185987,0,185987,3.5973682403564453,0.0008610943982780624
93093,186187,0,186187,3.601130962371826,0.0008555261481078117
93193,186387,0,186387,3.6049420833587646,0.0008491560470077379
93293,186587,0,186587,3.6086480617523193,0.0008415455333584331
93393,186787,0,186787,3.6123032569885254,0.0008326166216676273
93493,186987,0,186987,3.616245985031128,0.0008227253420393627
93594,187189,0,187189,3.6200110912323,0.0008124802718371369
93694,187389,0,187389,3.623756170272827,0.000802931143436931
93794,187589,0,187589,3.627552032470703,0.000794662113098775
93894,187789,0,187789,3.6315081119537354,0.0007879758349172392
93994,187989,0,187989,3.6352031230926514,0.0007827141134753449
94094,188189,0,188189,3.638916254043579,0.0007783592113028995
94194,188389,0,188389,3.6430931091308594,0.0007742711600968495
94294,188589,0,188589,3.64690899848938,0.0007699705472040792
94394,188789,0,188789,3.6505138874053955,0.0007653578326524802
94494,188989,0,188989,3.654366970062256,0.0007607801791359441
94595,189191,0,189191,3.6581919193267822,0.0007568849673641497
94695,189391,0,189391,3.6620049476623535,0.0007545176678981245
94795,189591,0,189591,3.665663957595825,0.0007541874035616835
94895,189791,0,189791,3.669290065765381,0.0007560192327353153
94995,189991,0,189991,3.6730690002441406,0.0007596530200392278
95095,190191,0,190191,3.677060842514038,0.0007643765134928485
95195,190391,0,190391,3.6806721687316895,0.0007693934798117416
95295,190591,0,190591,3.6843130588531494,0.0007741085895051778
95395,190791,0,190791,3.6880509853363037,0.0007783148567584336
95495,190991,0,190991,3.692629098892212,0.0007822248145111499
95596,191193,0,191193,3.696319103240967,0.0007863901271057027
95696,191393,0,191393,3.699997901916504,0.0007912990200015061
95796,191593,0,191593,3.70408296585083,0.0007973508190031904
95896,191793,0,191793,3.7078709602355957,0.0008045181797518771
95996,191993,0,191993,3.7116639614105225,0.0008123640812578168
96096,192193,0,192193,3.71527099609375,0.0008201826783622205
96196,192393,0,192393,3.719097137451172,0.0008272349627148337
96296,192593,0,192593,3.722944974899292,0.0008329855468372971
96396,192793,0,192793,3.726785182952881,0.0008372600970994839
96496,192993,0,192993,3.730323076248169,0.0008402717264357288
96597,193195,0,193195,3.7341508865356445,0.0008425262976018672
96697,193395,0,193395,3.738075017929077,0.0008445270207044877
96797,193595,0,193595,3.741772174835205,0.0008466693057664391
96897,193795,0,193795,3.74531626701355,0.0008489948638913945
96997,193995,0,193995,3.7488510608673096,0.0008511910529386722
97097,194195,0,194195,3.7524330615997314,0.0008527016737781329
97197,194395,0,194395,3.7562949657440186,0.0008529326600357097
97297,194595,0,194595,3.7603719234466553,0.0008514739423800917
97397,194795,0,194795,3.7638840675354004,0.0008482519684506491
97497,194995,0,194995,3.767380952835083,0.0008435580921917654
97598,195197,0,195197,3.771170139312744,0.0008378891808847192
97698,195397,0,195397,3.774707078933716,0.0008319891550956358
97798,195597,0,195597,3.778409957885742,0.0008262818387742534
97898,195797,0,195797,3.782233238220215,0.0008209282039933645
97998,195997,0,195997,3.785723924636841,0.0008157316669440638
98098,196197,0,196197,3.7894668579101562,0.0008102412984337118
98198,196397,0,196397,3.7933170795440674,0.0008039566797691744
98298,196597,0,196597,3.7972350120544434,0.0007965502411254371
98398,196797,0,196797,3.8007209300994873,0.0007880257015586181
98498,196997,0,196997,3.804518938064575,0.0007787592225022795
98599,197199,0,197199,3.8080739974975586,0.0007693136027286702
98699,197399,0,197399,3.811836004257202,0.0007606092228967299
98799,197599,0,197599,3.815371036529541,0.0007531083759723326
98899,197799,0,197799,3.8189902305603027,0.0007470169310039487
98999,197999,0,197999,3.822650194168091,0.0007421469632506081
99099,198199,0,198199,3.826956033706665,0.0007380270677818757
99199,198399,0,198399,3.830493927001953,0.0007341203675572351
99299,198599,0,198599,3.834023952484131,0.0007300651489868317
99399,198799,0,198799,3.8377699851989746,0.0007258447735270744
99499,198999,0,198999,3.8417880535125732,0.000721819252360302
99600,199201,0,199201,3.8455049991607666,0.000718578735194168
99700,199401,0,199401,3.849048137664795,0.0007168365414369836
99800,199601,0,199601,3.8526060581207275,0.0007169783094077633
99900,199801,0,199801,3.8568131923675537,0.0007190374731894531
100000,200001,0,200001,3.8604700565338135,0.0007226374491856396


==> plot_data/quadratic_minimax_problem_n20_alpha0/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.224082946777344e-05,4.387061074692293
100,201,200,401,0.0042340755462646484,0.24400872360835765
200,401,400,801,0.008651971817016602,0.11396482179674887
300,601,600,1201,0.013067007064819336,0.07772603596230616
400,801,800,1601,0.01716923713684082,0.06190660644187962
501,1003,1002,2005,0.021404266357421875,0.05363210938132448
601,1203,1202,2405,0.025474071502685547,0.04854289708923014
701,1403,1402,2805,0.029764175415039062,0.044811894255043366
801,1603,1602,3205,0.03382611274719238,0.04179654400397964
901,1803,1802,3605,0.037937164306640625,0.03924971924554778
1001,2003,2002,4005,0.04191422462463379,0.03706348955839846
1101,2203,2202,4405,0.045882225036621094,0.035178785925197326
1201,2403,2402,4805,0.049880027770996094,0.03355453267398762
1301,2603,2602,5205,0.05383610725402832,0.03215726348792642
1401,2803,2802,5605,0.05793619155883789,0.03095767199648659
1502,3005,3004,6009,0.06195712089538574,0.02991998323202208
1602,3205,3204,6409,0.06588602066040039,0.029040939320774044
1702,3405,3404,6809,0.06990790367126465,0.02828835829650628
1802,3605,3604,7209,0.0738520622253418,0.027643543602227788
1902,3805,3804,7609,0.0777430534362793,0.027090075263709473
2002,4005,4004,8009,0.08164715766906738,0.02661366298608146
2102,4205,4204,8409,0.0855553150177002,0.026201975227758096
2202,4405,4404,8809,0.08989405632019043,0.0258444527270099
2302,4605,4604,9209,0.09481215476989746,0.02553211595577548
2402,4805,4804,9609,0.09883308410644531,0.02525737490279822
2503,5007,5006,10013,0.1029660701751709,0.025011551173271675
2603,5207,5206,10413,0.10695910453796387,0.02479413074736284
2703,5407,5406,10813,0.11099910736083984,0.024598087482034042
2803,5607,5606,11213,0.1149911880493164,0.02441972624861084
2903,5807,5806,11613,0.11914205551147461,0.024255984393149754
3003,6007,6006,12013,0.12314605712890625,0.02410432926149394
3103,6207,6206,12413,0.12713122367858887,0.023962670451067175
3203,6407,6406,12813,0.13113808631896973,0.02382928529238106
3303,6607,6606,13213,0.1352701187133789,0.023702755993531773
3403,6807,6806,13613,0.13924026489257812,0.023581916916485614
3504,7009,7008,14017,0.1432480812072754,0.023464670603200708
3604,7209,7208,14417,0.1472160816192627,0.023352546952781245
3704,7409,7408,14817,0.1515500545501709,0.02324371933040331
3804,7609,7608,15217,0.1555020809173584,0.02313765993724719
3904,7809,7808,15617,0.15942597389221191,0.023033936061227892
4004,8009,8008,16017,0.16335606575012207,0.02293219301852367
4104,8209,8208,16417,0.1672811508178711,0.022832140115381733
4204,8409,8408,16817,0.1717979907989502,0.02273353910866042
4304,8609,8608,17217,0.1758420467376709,0.022636194729250055
4404,8809,8808,17617,0.17992901802062988,0.02253994690559794
4505,9011,9010,18021,0.18398308753967285,0.022443716054252546
4605,9211,9210,18421,0.18813323974609375,0.022349299282451357
4705,9411,9410,18821,0.19263100624084473,0.022255651010420593
4805,9611,9610,19221,0.19651508331298828,0.022162698835552937
4905,9811,9810,19621,0.20040297508239746,0.022070383260160423
5005,10011,10010,20021,0.20429611206054688,0.02197865534524145
5105,10211,10210,20421,0.20817303657531738,0.02188747479025684
5205,10411,10410,20821,0.21209001541137695,0.021796808361813313
5305,10611,10610,21221,0.21645903587341309,0.021706628608024154
5405,10811,10810,21621,0.22035717964172363,0.021616912806721164
5506,11013,11012,22025,0.2243189811706543,0.02152675159037204
5606,11213,11212,22425,0.22822308540344238,0.02143791452511929
5706,11413,11412,22825,0.23304009437561035,0.021349493655195773
5806,11613,11612,23225,0.23719120025634766,0.021261478021364178
5906,11813,11812,23625,0.24240899085998535,0.021173858394926075
6006,12013,12012,24025,0.2477099895477295,0.0210866269634385
6106,12213,12212,24425,0.2525019645690918,0.02099977707368877
6206,12413,12412,24825,0.2570030689239502,0.020913303021499314
6306,12613,12612,25225,0.2615621089935303,0.020827199879831903
6406,12813,12812,25625,0.26665401458740234,0.02074146335821519
6507,13015,13014,26029,0.2707061767578125,0.020655237771859597
6607,13215,13214,26429,0.2746002674102783,0.020570227190828582
6707,13415,13414,26829,0.2787151336669922,0.020485573100828172
6807,13615,13614,27229,0.2826039791107178,0.02040127280177237
6907,13815,13814,27629,0.28647398948669434,0.020317323829549257
7007,14015,14014,28029,0.29040002822875977,0.020233723914058508
7107,14215,14214,28429,0.29442501068115234,0.020150470944893955
7207,14415,14414,28829,0.29851794242858887,0.020067562943277894
7307,14615,14614,29229,0.30258917808532715,0.019984998039106475
7407,14815,14814,29629,0.30667591094970703,0.019902774452176045
7508,15017,15016,30033,0.31112122535705566,0.019820073346504125
7608,15217,15216,30433,0.31519103050231934,0.019738530710620945
7708,15417,15416,30833,0.3192932605743408,0.019657324434985902
7808,15617,15616,31233,0.3233621120452881,0.019576452971328227
7908,15817,15816,31633,0.32742905616760254,0.0194959148077385
8008,16017,16016,32033,0.33158206939697266,0.01941570846305175
8108,16217,16216,32433,0.3356630802154541,0.019335832482250178
8208,16417,16416,32833,0.33975815773010254,0.01925628543269952
8308,16617,16616,33233,0.3438279628753662,0.019177065901067873
8408,16817,16816,33633,0.3481781482696533,0.019098172490801885
8509,17019,17018,34037,0.3522531986236572,0.01901881976864435
8609,17219,17218,34437,0.35626697540283203,0.018940577695431893
8709,17419,17418,34837,0.3607921600341797,0.0188626576221969
8809,17619,17618,35237,0.3652820587158203,0.018785058202323093
8909,17819,17818,35637,0.36936402320861816,0.018707778098734175
9009,18019,18018,36037,0.3736100196838379,0.018630815983125406
9109,18219,18218,36437,0.3777179718017578,0.01855417053533105
9209,18419,18418,36837,0.3817882537841797,0.018477840442803484
9309,18619,18618,37237,0.3858602046966553,0.018401824400183057
9409,18819,18818,37637,0.3899199962615967,0.018326121108942536
9510,19021,19020,38041,0.39412927627563477,0.01824997692728853
9610,19221,19220,38441,0.3981759548187256,0.01817489836439712
9710,19421,19420,38841,0.40213823318481445,0.018100128682825716
9810,19621,19620,39241,0.40610504150390625,0.018025666608942708
9910,19821,19820,39641,0.41005802154541016,0.01795151087488961
10010,20021,20020,40041,0.41402316093444824,0.017877660218460007
10110,20221,20220,40441,0.4181392192840576,0.017804113382996836
10210,20421,20420,40841,0.4221010208129883,0.01773086911730443
10310,20621,20620,41241,0.4261600971221924,0.017657926175572894
10410,20821,20820,41641,0.4301149845123291,0.01758528331731253
10511,21023,21022,42045,0.4341120719909668,0.017512217372213767
10611,21223,21222,42445,0.43808507919311523,0.01744017395041506
10711,21423,21422,42845,0.44231510162353516,0.017368426909774835
10811,21623,21622,43245,0.4463019371032715,0.01729697503062207
10911,21823,21822,43645,0.4502692222595215,0.0172258170983744
11011,22023,22022,44045,0.45433712005615234,0.01715495190350446
11111,22223,22222,44445,0.4583280086517334,0.017084378241508134
11211,22423,22422,44845,0.4622809886932373,0.017014094912875637
11311,22623,22622,45245,0.46623730659484863,0.016944100723063484
11411,22823,22822,45645,0.47032904624938965,0.01687439448246843
11512,23025,23024,46049,0.4743030071258545,0.016804282255806782
11612,23225,23224,46449,0.4782378673553467,0.016735151214378838
11712,23425,23424,46849,0.4823112487792969,0.016666304571029123
11812,23625,23624,47249,0.4862809181213379,0.01659774115572194
11912,23825,23824,47649,0.49027514457702637,0.01652945980324449
12012,24025,24024,48049,0.4945690631866455,0.016461459353185378
12112,24225,24224,48449,0.4983370304107666,0.016393738649913198
12212,24425,24424,48849,0.5020861625671387,0.016326296542556084
12312,24625,24624,49249,0.5058190822601318,0.016259131884980845
12412,24825,24824,49649,0.5095071792602539,0.016192243535772873
12513,25027,25026,50053,0.513343095779419,0.016124965612223152
12613,25227,25226,50453,0.5171399116516113,0.016058629208975092
12713,25427,25426,50853,0.5208921432495117,0.015992565706711873
12813,25627,25626,51253,0.5246310234069824,0.015926773982740765
12913,25827,25826,51653,0.5284171104431152,0.015861252918988957
13013,26027,26026,52053,0.5322270393371582,0.01579600140198428
13113,26227,26226,52453,0.5359642505645752,0.015731018322836098
13213,26427,26426,52853,0.5398991107940674,0.01566630257721642
13313,26627,26626,53253,0.5440230369567871,0.015601853065340806
13413,26827,26826,53653,0.5489370822906494,0.015537668691949714
13514,27029,27028,54057,0.5541501045227051,0.015473110492795109
13614,27229,27228,54457,0.5587470531463623,0.015409455752744657
13714,27429,27428,54857,0.5633211135864258,0.015346062881567299
13814,27629,27628,55257,0.568317174911499,0.015282930801961206
13914,27829,27828,55657,0.572749137878418,0.015220058441056731
14014,28029,28028,56057,0.5778090953826904,0.015157444730397951
14114,28229,28228,56457,0.5818061828613281,0.015095088605924645
14214,28429,28428,56857,0.5859382152557373,0.015032989007954085
14314,28629,28628,57257,0.5903000831604004,0.014971144881162992
14414,28829,28828,57657,0.5946240425109863,0.014909555174569671
14515,29031,29030,58061,0.5987870693206787,0.014847606754191575
14615,29231,29230,58461,0.602849006652832,0.014786525270388241
14715,29431,29430,58861,0.6068291664123535,0.014725695069349514
14815,29631,29630,59261,0.6108050346374512,0.014665115117324604
14915,29831,29830,59661,0.6151680946350098,0.014604784384815403
15015,30031,30030,60061,0.6191501617431641,0.014544701846559078
15115,30231,30230,60461,0.6232509613037109,0.01448486648151075
15215,30431,30430,60861,0.6275300979614258,0.014425277272825825
15315,30631,30630,61261,0.6314842700958252,0.014365933207843056
15415,30831,30830,61661,0.6356039047241211,0.014306833278067182
15516,31033,31032,62065,0.6396870613098145,0.01424738913558572
15616,31233,31232,62465,0.6436700820922852,0.01418877688358528
15716,31433,31432,62865,0.648705005645752,0.014130405756190456
15816,31633,31632,63265,0.6532611846923828,0.014072274761440025
15916,31833,31832,63665,0.6572730541229248,0.014014382911453726
16016,32033,32032,64065,0.6614441871643066,0.0139567292224153
16116,32233,32232,64465,0.665600061416626,0.013899312714555747
16216,32433,32432,64865,0.6696760654449463,0.013842132412136788
16316,32633,32632,65265,0.6737301349639893,0.013785187343434193
16416,32833,32832,65665,0.677731990814209,0.013728476540721377
16517,33035,33034,66069,0.6817142963409424,0.013671435440173726
16617,33235,33234,66469,0.6857509613037109,0.013615192600759746
16717,33435,33434,66869,0.6897521018981934,0.013559181138438509
16817,33635,33634,67269,0.6936790943145752,0.01350340010134909
16917,33835,33834,67669,0.6976170539855957,0.013447848541546467
17017,34035,34034,68069,0.7015552520751953,0.013392525514985343
17117,34235,34234,68469,0.7056329250335693,0.013337430081504184
17217,34435,34434,68869,0.7095701694488525,0.013282561304809058
17317,34635,34634,69269,0.7135601043701172,0.013227918252457985
17417,34835,34834,69669,0.7174949645996094,0.01317349999584482
17518,35037,35036,70073,0.7214810848236084,0.013118764793756114
17618,35237,35236,70473,0.7254080772399902,0.013064795582927223
17718,35437,35436,70873,0.7296030521392822,0.01301104839572354
17818,35637,35636,71273,0.7335391044616699,0.012957522318763317
17918,35837,35836,71673,0.73750901222229,0.012904216442422432
18018,36037,36036,72073,0.7415122985839844,0.012851129860818794
18118,36237,36236,72473,0.7454450130462646,0.01279826167179707
18218,36437,36436,72873,0.7493631839752197,0.012745610976913279
18318,36637,36636,73273,0.7532899379730225,0.012693176881419535
18418,36837,36836,73673,0.7572453022003174,0.012640958494248851
18519,37039,37038,74077,0.7613260746002197,0.012588435974189925
18619,37239,37238,74477,0.7652568817138672,0.012536648480033455
18719,37439,37438,74877,0.769366979598999,0.012485074034150523
18819,37639,37638,75277,0.773292064666748,0.012433711760083094
18919,37839,37838,75677,0.7772190570831299,0.012382560784978723
19019,38039,38038,76077,0.7811520099639893,0.012331620239575868
19119,38239,38238,76477,0.7850711345672607,0.01228088925818896
19219,38439,38438,76877,0.7892191410064697,0.012230366978693818
19319,38639,38638,77277,0.793126106262207,0.012180052542512906
19419,38839,38838,77677,0.7969589233398438,0.012129945094600848
19520,39041,39040,78081,0.8008460998535156,0.012079545808436398
19620,39241,39240,78481,0.8046901226043701,0.01202985183459805
19720,39441,39440,78881,0.8085460662841797,0.011980362296512089
19820,39641,39640,79281,0.8124451637268066,0.011931076353151427
19920,39841,39840,79681,0.8164150714874268,0.011881993166948941
20020,40041,40040,80081,0.8202581405639648,0.01183311190378311
20120,40241,40240,80481,0.8241310119628906,0.011784431732963906
20220,40441,40440,80881,0.8279950618743896,0.011735951827218701
20320,40641,40640,81281,0.8320162296295166,0.011687671362678157
20420,40841,40840,81681,0.8359780311584473,0.011639589518862252
20521,41043,41042,82085,0.8400139808654785,0.011591227634416544
20621,41243,41242,82485,0.8439500331878662,0.011543542549898145
20721,41443,41442,82885,0.8480823040008545,0.011496053636773956
20821,41643,41642,83285,0.8520209789276123,0.011448760088015549
20921,41843,41842,83685,0.8559520244598389,0.011401661099914676
21021,42043,42042,84085,0.8598682880401611,0.011354755872069319
21121,42243,42242,84485,0.8639211654663086,0.011308043607370302
21221,42443,42442,84885,0.8678140640258789,0.011261523511987627
21321,42643,42642,85285,0.871757984161377,0.0112151947953571
21421,42843,42842,85685,0.8756351470947266,0.011169056670166717
21522,43045,43044,86089,0.879734992980957,0.01112264982504777
21622,43245,43244,86489,0.8839521408081055,0.011076892420077013
21722,43445,43444,86889,0.8878650665283203,0.011031323256230713
21822,43645,43644,87289,0.8918561935424805,0.010985941559104768
21922,43845,43844,87689,0.8956599235534668,0.010940746557480913
22022,44045,44044,88089,0.8994722366333008,0.010895737483313583
22122,44245,44244,88489,0.9032208919525146,0.010850913571716898
22222,44445,44444,88889,0.9069671630859375,0.010806274060951618
22322,44645,44644,89289,0.9107160568237305,0.010761818192412247
22422,44845,44844,89689,0.9145369529724121,0.010717545210614084
22523,45047,45046,90093,0.9183211326599121,0.010673014371946841
22623,45247,45246,90493,0.9220809936523438,0.010629106719673554
22723,45447,45446,90893,0.9258322715759277,0.010585379698837745
22823,45647,45646,91293,0.9296250343322754,0.010541832566340786
22923,45847,45846,91693,0.9333739280700684,0.010498464582141067
23023,46047,46046,92093,0.937265157699585,0.010455275009241429
23123,46247,46246,92493,0.9410390853881836,0.010412263113676686
23223,46447,46446,92893,0.9453420639038086,0.010369428164501055
23323,46647,46646,93293,0.949099063873291,0.010326769433775803
23423,46847,46846,93693,0.9528682231903076,0.010284286196556858
23524,47049,47048,94097,0.9566593170166016,0.010241555526386868
23624,47249,47248,94497,0.9607012271881104,0.010199422850170116
23724,47449,47448,94897,0.9647140502929688,0.010157463503327056
23824,47649,47648,95297,0.9686059951782227,0.010115676772798968
23924,47849,47848,95697,0.9726309776306152,0.010074061948460666
24024,48049,48048,96097,0.9764940738677979,0.010032618323108216
24124,48249,48248,96497,0.9807159900665283,0.009991345192447064
24224,48449,48448,96897,0.984647274017334,0.00995024185508015
24324,48649,48648,97297,0.988490104675293,0.009909307612495753
24424,48849,48848,97697,0.9929032325744629,0.009868541769055873
24525,49051,49050,98101,0.9975769519805908,0.009827538495193936
24625,49251,49250,98501,1.0013749599456787,0.009787109041254165
24725,49451,49450,98901,1.0055480003356934,0.009746845909811806
24825,49651,49650,99301,1.0096821784973145,0.009706748416633661
24925,49851,49850,99701,1.0153982639312744,0.009666815880301487
25025,50051,50050,100101,1.0196411609649658,0.009627047622200218
25125,50251,50250,100501,1.0234911441802979,0.009587442966506592
25225,50451,50450,100901,1.0276331901550293,0.009548001240177635
25325,50651,50650,101301,1.0314500331878662,0.009508721772939172
25425,50851,50850,101701,1.0354349613189697,0.009469603897274465
25526,51053,51052,102105,1.0395619869232178,0.009430258189362294
25626,51253,51252,102505,1.0438709259033203,0.009391463104581561
25726,51453,51452,102905,1.0482978820800781,0.009352827618676379
25826,51653,51652,103305,1.0532422065734863,0.009314351075073826
25926,51853,51852,103705,1.0578601360321045,0.009276032819902103
26026,52053,52052,104105,1.062164068222046,0.00923787220197936
26126,52253,52252,104505,1.066918134689331,0.009199868572802628
26226,52453,52452,104905,1.071547031402588,0.009162021286536771
26326,52653,52652,105305,1.0760669708251953,0.009124329700003632
26426,52853,52852,105705,1.0801610946655273,0.009086793172670976
26527,53055,53054,106109,1.0842421054840088,0.009049038023257273
26627,53255,53254,106509,1.0890002250671387,0.009011811237919354
26727,53455,53454,106909,1.0932800769805908,0.008974737599638951
26827,53655,53654,107309,1.0972881317138672,0.008937816478385275
26927,53855,53854,107709,1.101464033126831,0.008901047246719404
27027,54055,54054,108109,1.1054801940917969,0.008864429279783642
27127,54255,54254,108509,1.1096251010894775,0.008827961955290868
27227,54455,54454,108909,1.1138370037078857,0.008791644653514006
27327,54655,54654,109309,1.1180031299591064,0.008755476757275497
27427,54855,54854,109709,1.1226401329040527,0.008719457651936706
27528,55057,55056,110113,1.126812219619751,0.008683228762360428
27628,55257,55256,110513,1.1310851573944092,0.008647506877631283
27728,55457,55456,110913,1.1350481510162354,0.00861193194895774
27828,55657,55656,111313,1.1389849185943604,0.008576503371778088
27928,55857,55856,111713,1.143226146697998,0.008541220544017788
28028,56057,56056,112113,1.1476221084594727,0.00850608286607914
28128,56257,56256,112513,1.1526870727539062,0.008471089740831111
28228,56457,56456,112913,1.157310962677002,0.008436240573599233
28328,56657,56656,113313,1.1618170738220215,0.008401534772155474
28428,56857,56856,113713,1.1664760112762451,0.008366971746708104
28529,57059,57058,114117,1.1721351146697998,0.008332207417595033
28629,57259,57258,114517,1.1775360107421875,0.008297929597551771
28729,57459,57458,114917,1.1830260753631592,0.008263792792834741
28829,57659,57658,115317,1.1884031295776367,0.008229796423321747
28929,57859,57858,115717,1.1939740180969238,0.008195939911277242
29029,58059,58058,116117,1.1993741989135742,0.008162222681342373
29129,58259,58258,116517,1.2045209407806396,0.008128644160525297
29229,58459,58458,116917,1.209618091583252,0.008095203778191359
29329,58659,58658,117317,1.214677095413208,0.00806190096605345
29429,58859,58858,117717,1.2195031642913818,0.008028735158162345
29530,59061,59060,118121,1.2237060070037842,0.007995376184348438
29630,59261,59260,118521,1.227769136428833,0.007962484052373132
29730,59461,59460,118921,1.23183012008667,0.007929727235149852
29830,59661,59660,119321,1.2358620166778564,0.007897105176008062
29930,59861,59860,119721,1.2398719787597656,0.007864617320567235
30030,60061,60060,120121,1.2440011501312256,0.007832263116727552
30130,60261,60260,120521,1.248466968536377,0.007800042014660447
30230,60461,60460,120921,1.2526161670684814,0.007767953466799313
30330,60661,60660,121321,1.256519079208374,0.007735996927830199
30430,60861,60860,121721,1.2606582641601562,0.007704171854682442
30531,61063,61062,122125,1.2650041580200195,0.007672161424384856
30631,61263,61262,122525,1.2694041728973389,0.0076405989637465845
30731,61463,61462,122925,1.273772954940796,0.007609166347733111
30831,61663,61662,123325,1.2784199714660645,0.0075778630421773656
30931,61863,61862,123725,1.2823750972747803,0.0075466885151098265
31031,62063,62062,124125,1.2866101264953613,0.007515642236749418
31131,62263,62262,124525,1.2905709743499756,0.007484723679494517
31231,62463,62462,124925,1.2947142124176025,0.007453932317913985
31331,62663,62662,125325,1.298706293106079,0.007423267628738286
31431,62863,62862,125725,1.3027739524841309,0.007392729090850528
31532,63065,63064,126129,1.3072528839111328,0.007362012688914633
31632,63265,63264,126529,1.3116331100463867,0.007331726147370554
31732,63465,63464,126929,1.3157880306243896,0.007301564201455097
31832,63665,63664,127329,1.320909023284912,0.007271526338594972
31932,63865,63864,127729,1.3253450393676758,0.007241612048325651
32032,64065,64064,128129,1.3304932117462158,0.007211820822282571
32132,64265,64264,128529,1.335482120513916,0.007182152154192482
32232,64465,64464,128929,1.3404242992401123,0.007152605539864971
32332,64665,64664,129329,1.345487117767334,0.007123180477183726
32432,64865,64864,129729,1.350135087966919,0.007093876466098154
32533,65067,65066,130133,1.3543200492858887,0.007064401781155894
32633,65267,65266,130533,1.35843825340271,0.007035339579408933
32733,65467,65466,130933,1.3631842136383057,0.007006396936486132
32833,65667,65666,131333,1.3674860000610352,0.0069775733605351295
32933,65867,65866,131733,1.3714392185211182,0.006948868361727015
33033,66067,66066,132133,1.3754560947418213,0.006920281452247954
33133,66267,66266,132533,1.3797800540924072,0.006891812146290943
33233,66467,66466,132933,1.3843541145324707,0.006863459960047532
33333,66667,66666,133333,1.388416051864624,0.006835224411699583
33433,66867,66866,133733,1.3926060199737549,0.006807105021411168
33534,67069,67068,134137,1.397078037261963,0.006778821856792532
33634,67269,67268,134537,1.401266098022461,0.006750934500649469
33734,67469,67468,134937,1.405649185180664,0.00672316187014001
33834,67669,67668,135337,1.4102470874786377,0.006695503493295036
33934,67869,67868,135737,1.4148521423339844,0.006667958900087056
34034,68069,68068,136137,1.4191012382507324,0.006640527622422218
34134,68269,68268,136537,1.4235708713531494,0.006613209194132384
34234,68469,68468,136937,1.427860975265503,0.006586003150967135
34334,68669,68668,137337,1.4323320388793945,0.006558909030585957
34434,68869,68868,137737,1.4367852210998535,0.00653192637255039
34535,69071,69070,138141,1.4409420490264893,0.006504786560796256
34635,69271,69270,138541,1.4451451301574707,0.006478026556877027
34735,69471,69470,138941,1.4503579139709473,0.006451376640783591
34835,69671,69670,139341,1.454531192779541,0.006424836359626273
34935,69871,69870,139741,1.4586851596832275,0.0063984052623785575
35035,70071,70070,140141,1.4633700847625732,0.0063720828998694015
35135,70271,70270,140541,1.4675321578979492,0.0063458688247755345
35235,70471,70470,140941,1.4717559814453125,0.006319762591614038
35335,70671,70670,141341,1.4758851528167725,0.006293763756734599
35435,70871,70870,141741,1.4801380634307861,0.006267871878312006
35536,71073,71072,142145,1.484264850616455,0.006241829199142931
35636,71273,71272,142545,1.4884510040283203,0.006216150973997304
35736,71473,71472,142945,1.492661952972412,0.006190578386354045
35836,71673,71672,143345,1.4967260360717773,0.006165111001631597
35936,71873,71872,143745,1.5008361339569092,0.006139748387036292
36036,72073,72072,144145,1.504967212677002,0.006114490111554905
36136,72273,72272,144545,1.5090980529785156,0.0060893357459473624
36236,72473,72472,144945,1.5131499767303467,0.006064284862739422
36336,72673,72672,145345,1.517212152481079,0.0060393370362154435
36436,72873,72872,145745,1.5212771892547607,0.006014491842411115
36537,73075,73074,146149,1.525362253189087,0.005989501944012134
36637,73275,73274,146549,1.5295469760894775,0.005964861766506236
36737,73475,73474,146949,1.5337352752685547,0.005940322956084465
36837,73675,73674,147349,1.5377681255340576,0.005915885095733384
36937,73875,73874,147749,1.5418212413787842,0.0058915477701550695
37037,74075,74074,148149,1.545882225036621,0.005867310565760089
37137,74275,74274,148549,1.55000901222229,0.0058431730706605236
37237,74475,74474,148949,1.5542190074920654,0.005819134874662815
37337,74675,74674,149349,1.5583479404449463,0.005795195569261004
37437,74875,74874,149749,1.562596082687378,0.005771354747629617
37538,75077,75076,150153,1.5668652057647705,0.0057473750711171815
37638,75277,75276,150553,1.5710961818695068,0.005723730977957329
37738,75477,75476,150953,1.575301170349121,0.005700184154095967
37838,75677,75676,151353,1.5795261859893799,0.005676734199377498
37938,75877,75876,151753,1.5837931632995605,0.005653380715292511
38038,76077,76076,152153,1.5879302024841309,0.005630123304971026
38138,76277,76276,152553,1.5922322273254395,0.005606961573175729
38238,76477,76476,152953,1.5964231491088867,0.005583895126295303
38338,76677,76676,153353,1.6006519794464111,0.005560923572337659
38438,76877,76876,153753,1.6048979759216309,0.005538046520923362
38539,77079,77078,154157,1.6090753078460693,0.005515036227865703
38639,77279,77278,154557,1.6133301258087158,0.005492347952133196
38739,77479,77478,154957,1.6174850463867188,0.005469753013567384
38839,77679,77678,155357,1.621725082397461,0.005447251028189034
38939,77879,77878,155757,1.6259970664978027,0.0054248416135985736
39039,78079,78078,156157,1.630958080291748,0.005402524388969544
39139,78279,78278,156557,1.635099172592163,0.005380298975042232
39239,78479,78478,156957,1.6393489837646484,0.005358164994117084
39339,78679,78678,157357,1.6435890197753906,0.0053361220700484215
39439,78879,78878,157757,1.6478462219238281,0.005314169828237971
39540,79081,79080,158161,1.65214204788208,0.005292089731105537
39640,79281,79280,158561,1.6563019752502441,0.005270318633680339
39740,79481,79480,158961,1.6604421138763428,0.0052486371002472615
39840,79681,79680,159361,1.6646831035614014,0.005227044762349522
39940,79881,79880,159761,1.6689331531524658,0.005205541253046146
40040,80081,80080,160161,1.6730711460113525,0.005184126206905686
40140,80281,80280,160561,1.6772222518920898,0.005162799260000051
40240,80481,80480,160961,1.681467056274414,0.005141560049898295
40340,80681,80680,161361,1.6856372356414795,0.005120408215660488
40440,80881,80880,161761,1.6897892951965332,0.005099343397831577
40541,81083,81082,162165,1.6940820217132568,0.0050781558932589165
40641,81283,81282,162565,1.698256254196167,0.005057264897015461
40741,81483,81482,162965,1.7024362087249756,0.00503645984412097
40841,81683,81682,163365,1.7067761421203613,0.005015740381013602
40941,81883,81882,163765,1.7110099792480469,0.0049951061555860285
41041,82083,82082,164165,1.7152140140533447,0.004974556817179435
41141,82283,82282,164565,1.719468116760254,0.004954092016577594
41241,82483,82482,164965,1.723667860031128,0.004933711406000938
41341,82683,82682,165365,1.7278079986572266,0.004913414639100601
41441,82883,82882,165765,1.7320561408996582,0.004893201370952563
41542,83085,83084,166169,1.7363619804382324,0.004872870375698116
41642,83285,83284,166569,1.7405319213867188,0.004852823902361474
41742,83485,83484,166969,1.7446610927581787,0.004832859898095875
41842,83685,83684,167369,1.7488722801208496,0.004812978023632288
41942,83885,83884,167769,1.7531170845031738,0.004793177941097396
42042,84085,84084,168169,1.7573418617248535,0.004773459314007856
42142,84285,84284,168569,1.7614710330963135,0.004753821807264584
42242,84485,84484,168969,1.765606164932251,0.0047342650871470575
42342,84685,84684,169369,1.7697980403900146,0.004714788821307638
42442,84885,84884,169769,1.7740490436553955,0.004695392678765937
42543,85087,85086,170173,1.7784221172332764,0.004675883568260828
42643,85287,85286,170573,1.7826790809631348,0.004656647477815262
42743,85487,85486,170973,1.7869250774383545,0.004637490522611249
42843,85687,85686,171373,1.7911641597747803,0.004618412377094773
42943,85887,85886,171773,1.7953600883483887,0.004599412717051115
43043,86087,86086,172173,1.799626111984253,0.004580491219599321
43143,86287,86286,172573,1.8038020133972168,0.004561647563186797
43243,86487,86486,172973,1.8079442977905273,0.004542881427583712
43343,86687,86686,173373,1.8121490478515625,0.004524192493877646
43443,86887,86886,173773,1.8163912296295166,0.004505580444468188
43544,87089,87088,174177,1.8205952644348145,0.004486859993848942
43644,87289,87288,174577,1.8247590065002441,0.004468401526396055
43744,87489,87488,174977,1.8291351795196533,0.004450018995125976
43844,87689,87688,175377,1.8333990573883057,0.004431712087645273
43944,87889,87888,175777,1.8381991386413574,0.004413480492845678
44044,88089,88088,176177,1.8424110412597656,0.004395323900898777
44144,88289,88288,176577,1.8466742038726807,0.0043772420032507885
44244,88489,88488,176977,1.8504791259765625,0.004359234492617242
44344,88689,88688,177377,1.854259967803955,0.004341301062977856
44444,88889,88888,177777,1.858546257019043,0.004323441409571246
44545,89091,89090,178181,1.8623402118682861,0.004305477737096482
44645,89291,89290,178581,1.8678321838378906,0.004287765457063616
44745,89491,89490,178981,1.8718981742858887,0.004270126043477431
44845,89691,89690,179381,1.875899076461792,0.00425255919657306
44945,89891,89890,179781,1.8798582553863525,0.00423506461781887
45045,90091,90090,180181,1.8836300373077393,0.00421764200991132
45145,90291,90290,180581,1.8874211311340332,0.004200291076769972
45245,90491,90490,180981,1.8913002014160156,0.004183011523532391
45345,90691,90690,181381,1.895211935043335,0.004165803056549231
45445,90891,90890,181781,1.8990600109100342,0.004148665383379156
45546,91093,91092,182185,1.9031410217285156,0.0041314278961336074
45646,91293,91292,182585,1.9073431491851807,0.004114431638737725
45746,91493,91492,182985,1.9114181995391846,0.004097505302147127
45846,91693,91692,183385,1.916445255279541,0.004080648598715015
45946,91893,91892,183785,1.921093225479126,0.0040638612419779405
46046,92093,92092,184185,1.9253759384155273,0.0040471429466509235
46146,92293,92292,184585,1.9297599792480469,0.004030493428622653
46246,92493,92492,184985,1.933933973312378,0.0040139124049505676
46346,92693,92692,185385,1.93784499168396,0.003997399593856141
46446,92893,92892,185785,1.9418540000915527,0.003980954714720053
46547,93095,93094,186189,1.9458322525024414,0.003964414056513435
46647,93295,93294,186589,1.9497380256652832,0.003948104876389191
46747,93495,93494,186989,1.9538002014160156,0.00393186279050701
46847,93695,93694,187389,1.9580039978027344,0.003915687522848269
46947,93895,93894,187789,1.962663173675537,0.003899578798529858
47047,94095,94094,188189,1.967353105545044,0.003883536343799519
47147,94295,94294,188589,1.9725430011749268,0.003867559886031196
47247,94495,94494,188989,1.9767701625823975,0.0038516491537203333
47347,94695,94694,189389,1.9814090728759766,0.003835803876479375
47447,94895,94894,189789,1.9858360290527344,0.0038200237850330694
47548,95097,95096,190193,1.9898622035980225,0.0038041517864052616
47648,95297,95296,190593,1.9938008785247803,0.0037885019083097856
47748,95497,95496,190993,1.9977970123291016,0.0037729164121575445
47848,95697,95696,191393,2.001753091812134,0.0037573950330880546
47948,95897,95896,191793,2.005697011947632,0.003741937507330403
48048,96097,96096,192193,2.0096471309661865,0.003726543572198825
48148,96297,96296,192593,2.0136210918426514,0.0037112129660882044
48248,96497,96496,192993,2.018357038497925,0.0036959454284696516
48348,96697,96696,193393,2.0224449634552,0.0036807406998860446
48448,96897,96896,193793,2.026492118835449,0.0036655985219476842
48549,97099,97098,194197,2.0305590629577637,0.0036503681521949135
48649,97299,97298,194597,2.0346779823303223,0.0036353509237053447
48749,97499,97498,194997,2.038794994354248,0.003620395474505458
48849,97699,97698,195397,2.042757034301758,0.003605501550441781
48949,97899,97898,195797,2.0467541217803955,0.003590668898406413
49049,98099,98098,196197,2.050711154937744,0.0035758972663327026
49149,98299,98298,196597,2.054669141769409,0.0035611864031910023
49249,98499,98498,196997,2.058642864227295,0.0035465360589843316
49349,98699,98698,197397,2.0625970363616943,0.0035319459847442335
49449,98899,98898,197797,2.067305088043213,0.0035174159325263876
49550,99101,99100,198201,2.0714008808135986,0.003502801253666727
49650,99301,99300,198601,2.0754711627960205,0.003488391099789987
49750,99501,99500,199001,2.0795161724090576,0.003474040227762176
49850,99701,99700,199401,2.08347487449646,0.00345974839370404
49950,99901,99900,199801,2.087563991546631,0.003445515354739607
50050,100101,100100,200201,2.091517925262451,0.003431340868992097
50150,100301,100300,200601,2.0954182147979736,0.0034172246955797496
50250,100501,100500,201001,2.0992770195007324,0.003403166594611812
50350,100701,100700,201401,2.103113889694214,0.0033891663271843615
50450,100901,100900,201801,2.10695219039917,0.003375223655376346
50551,101103,101102,202205,2.110896110534668,0.003361199777976271
50651,101303,101302,202605,2.114927053451538,0.00334737215759376
50751,101503,101502,203005,2.1188101768493652,0.00333360142257898
50851,101703,101702,203405,2.1227121353149414,0.0033198873389115777
50951,101903,101902,203805,2.1266181468963623,0.003306229673533883
51051,102103,102102,204205,2.1305010318756104,0.003292628194347024
51151,102303,102302,204605,2.134335994720459,0.0032790826702069516
51251,102503,102502,205005,2.138216257095337,0.0032655928709205283
51351,102703,102702,205405,2.1420531272888184,0.0032521585672415864
51451,102903,102902,205805,2.145983934402466,0.003238779530867077
51552,103105,103104,206209,2.1498641967773438,0.0032253225716536013
51652,103305,103304,206609,2.153797149658203,0.003212053935726564
51752,103505,103504,207009,2.1580002307891846,0.0031988398855643464
51852,103705,103704,207409,2.1624629497528076,0.003185680196606894
51952,103905,103904,207809,2.166996955871582,0.003172574645217944
52052,104105,104104,208209,2.170894145965576,0.0031595230086812944
52152,104305,104304,208609,2.174776077270508,0.003146525065196907
52252,104505,104504,209009,2.178746223449707,0.0031335805938772707
52352,104705,104704,209409,2.1825919151306152,0.003120689374743531
52452,104905,104904,209809,2.1865899562835693,0.0031078511887218507
52553,105107,105106,210213,2.1904749870300293,0.0030949382299083083
52653,105307,105306,210613,2.19441294670105,0.003082205981372849
52753,105507,105506,211013,2.19850492477417,0.0030695261119612276
52853,105707,105706,211413,2.202594041824341,0.003056898406191248
52953,105907,105906,211813,2.2067770957946777,0.003044322649467209
53053,106107,106106,212213,2.210813283920288,0.003031798628076219
53153,106307,106306,212613,2.215015172958374,0.0030193261291846262
53253,106507,106506,213013,2.2189621925354004,0.0030069049408342867
53353,106707,106706,213413,2.222851037979126,0.0029945348519390645
53453,106907,106906,213813,2.226912021636963,0.0029822156522812003
53554,107109,107108,214217,2.230988025665283,0.002969824702537307
53654,107309,107308,214617,2.23488712310791,0.002957607157820564
53754,107509,107508,215017,2.238758087158203,0.002945439874790568
53854,107709,107708,215417,2.2426531314849854,0.002933322646676077
53954,107909,107908,215817,2.24652099609375,0.0029212552675564546
54054,108109,108108,216217,2.250386953353882,0.002909237532358191
54154,108309,108308,216617,2.2543039321899414,0.002897269236851446
54254,108509,108508,217017,2.2581632137298584,0.0028853501776465677
54354,108709,108708,217417,2.262083053588867,0.0028734801521906176
54454,108909,108908,217817,2.2659902572631836,0.0028616589587639393
54555,109111,109110,218221,2.2698869705200195,0.0028497689157634975
54655,109311,109310,218621,2.2737619876861572,0.0028380452678556027
54755,109511,109510,219021,2.277714967727661,0.002826369849795231
54855,109711,109710,219421,2.2816290855407715,0.002814742463169884
54955,109911,109910,219821,2.285494089126587,0.002803162910383327
55055,110111,110110,220221,2.2893600463867188,0.0027916309946521838
55155,110311,110310,220621,2.2932002544403076,0.0027801465200026636
55255,110511,110510,221021,2.297118902206421,0.002768709291267182
55355,110711,110710,221421,2.300899028778076,0.002757319114081033
55455,110911,110910,221821,2.304965019226074,0.0027459757948791255
55556,111113,111112,222225,2.3094210624694824,0.00273456640936194
55656,111313,111312,222625,2.313225030899048,0.0027233166923807577
55756,111513,111512,223025,2.317125082015991,0.0027121132555454016
55856,111713,111712,223425,2.3209149837493896,0.002700955908464218
55956,111913,111912,223825,2.3246772289276123,0.0026898444615288527
56056,112113,112112,224225,2.328550100326538,0.002678778725910949
56156,112313,112312,224625,2.3323190212249756,0.0026677585135589927
56256,112513,112512,225025,2.3361918926239014,0.002656783637195071
56356,112713,112712,225425,2.3400800228118896,0.0026458539103117354
56456,112913,112912,225825,2.3440821170806885,0.002634969147168808
56557,113115,113114,226229,2.348036050796509,0.0026240209884552273
56657,113315,113314,226629,2.3518362045288086,0.0026132260436435933
56757,113515,113514,227029,2.355675220489502,0.0026024755080931777
56857,113715,113714,227429,2.359462261199951,0.002591769199108963
56957,113915,113914,227829,2.3634631633758545,0.0025811069347475447
57057,114115,114114,228229,2.3676280975341797,0.002570488533813974
57157,114315,114314,228629,2.3718321323394775,0.002559913815858767
57257,114515,114514,229029,2.375697135925293,0.002549382601174776
57357,114715,114714,229429,2.3795711994171143,0.0025388947107941365
57457,114915,114914,229829,2.3834311962127686,0.0025284499664852606
57558,115117,115116,230233,2.3873112201690674,0.002517944389384992
57658,115317,115316,230633,2.391184091567993,0.002507585832482533
57758,115517,115516,231033,2.394991159439087,0.002497269889587577
57858,115717,115716,231433,2.3988568782806396,0.002486996385390603
57958,115917,115916,231833,2.4027771949768066,0.002476765145303307
58058,116117,116116,232233,2.4065699577331543,0.0024665759954555846
58158,116317,116316,232633,2.410529136657715,0.002456428762692665
58258,116517,116516,233033,2.414454936981201,0.002446323274572094
58358,116717,116716,233433,2.4183762073516846,0.0024362593593608246
58458,116917,116916,233833,2.4222850799560547,0.00242623684603231
58559,117119,117118,234237,2.4262380599975586,0.0024161559590907575
58659,117319,117318,234637,2.430109977722168,0.0024062161490246686
58759,117519,117518,235037,2.434115171432495,0.0023963172302858896
58859,117719,117718,235437,2.437952995300293,0.0023864590346518114
58959,117919,117918,235837,2.4417781829833984,0.0023766413945919148
59059,118119,118118,236237,2.445823907852173,0.0023668641432648277
59159,118319,118318,236637,2.4496071338653564,0.0023571271145156024
59259,118519,118518,237037,2.453782081604004,0.0023474301428727863
59359,118719,118718,237437,2.4576821327209473,0.002337773063545691
59459,118919,118918,237837,2.461740016937256,0.0023281557124215464
59560,119121,119120,238241,2.465588092803955,0.0023184823474499345
59660,119321,119320,238641,2.469618082046509,0.002308944356291497
59760,119521,119520,239041,2.4734740257263184,0.0022994456034198755
59860,119721,119720,239441,2.477555990219116,0.002289985927412913
59960,119921,119920,239841,2.481586217880249,0.0022805651675125134
60060,120121,120120,240241,2.4854190349578857,0.0022711831636219463
60160,120321,120320,240641,2.4894251823425293,0.0022618397563030795
60260,120521,120520,241041,2.4934372901916504,0.0022525347867736975
60360,120721,120720,241441,2.4985709190368652,0.0022432680969048063
60460,120921,120920,241841,2.5028669834136963,0.0022340395292179192
60561,121123,121122,242245,2.5074622631073,0.002224757212055106
60661,121323,121322,242645,2.512153148651123,0.0022156047961906537
60761,121523,121522,243045,2.516890048980713,0.0022064900323970297
60861,121723,121722,243445,2.522747039794922,0.0021974127657776177
60961,121923,121922,243845,2.527501106262207,0.002188372842073003
61061,122123,122122,244245,2.5315771102905273,0.002179370107658379
61161,122323,122322,244645,2.5355210304260254,0.0021704044095409553
61261,122523,122522,245045,2.5393800735473633,0.002161475595357307
61361,122723,122722,245445,2.5432300567626953,0.002152583513370839
61461,122923,122922,245845,2.5470991134643555,0.002143728012469163
61562,123125,123124,246249,2.5509960651397705,0.002134820934925411
61662,123325,123324,246649,2.555021047592163,0.002126038507392765
61762,123525,123524,247049,2.5590810775756836,0.002117292209838103
61862,123725,123724,247449,2.563133955001831,0.002108581893626524
61962,123925,123924,247849,2.5672309398651123,0.0020999074107345707
62062,124125,124124,248249,2.571460008621216,0.0020912686137477534
62162,124325,124324,248649,2.575634241104126,0.0020826653558580453
62262,124525,124524,249049,2.579768180847168,0.0020740974908613615
62362,124725,124724,249449,2.583954095840454,0.0020655648731550767
62462,124925,124924,249849,2.588083267211914,0.002057067357735554
62563,125127,125126,250253,2.592586040496826,0.002048520350670511
62663,125327,125326,250653,2.596724033355713,0.002040092954613752
62763,125527,125526,251053,2.600939989089966,0.0020317002279730155
62863,125727,125726,251453,2.6050732135772705,0.002023342028122002
62963,125927,125926,251853,2.6092379093170166,0.002015018213021156
63063,126127,126126,252253,2.613415241241455,0.0020067286412152655
63163,126327,126326,252653,2.6175670623779297,0.0019984731718310084
63263,126527,126526,253053,2.621795177459717,0.001990251664574641
63363,126727,126726,253453,2.626000165939331,0.0019820639797295697
63463,126927,126926,253853,2.6300289630889893,0.001973909978153963
63564,127129,127128,254257,2.6340630054473877,0.0019657084856429846
63664,127329,127328,254657,2.6381640434265137,0.0019576217688401843
63764,127529,127528,255057,2.6421329975128174,0.0019495683199349915
63864,127729,127728,255457,2.6462361812591553,0.001941548002066804
63964,127929,127928,255857,2.6502010822296143,0.001933560678938055
64064,128129,128128,256257,2.6541781425476074,0.0019256062148118587
64164,128329,128328,256657,2.6581192016601562,0.0019176844745097572
64264,128529,128528,257057,2.662067174911499,0.001909795323409397
64364,128729,128728,257457,2.666079044342041,0.0019019386274422444
64464,128929,128928,257857,2.670044183731079,0.0018941142530913338
64565,129131,129130,258261,2.6740641593933105,0.0018862443076360902
64665,129331,129330,258661,2.6780130863189697,0.0018784844980569133
64765,129531,129530,259061,2.6819770336151123,0.0018707566115136087
64865,129731,129730,259461,2.6859281063079834,0.0018630605166781858
64965,129931,129930,259861,2.6899912357330322,0.001855396082762924
65065,130131,130130,260261,2.6941370964050293,0.00184776317951815
65165,130331,130330,260661,2.697991132736206,0.0018401616772300232
65265,130531,130530,261061,2.701833963394165,0.001832591446718308
65365,130731,130730,261461,2.705677032470703,0.0018250523593342407
65465,130931,130930,261861,2.7095091342926025,0.0018175442869582783
65566,131133,131132,262265,2.713608980178833,0.001809992485699441
65666,131333,131332,262665,2.717433214187622,0.0018025463680507784
65766,131533,131532,263065,2.7212741374969482,0.001795130882942572
65866,131733,131732,263465,2.7250969409942627,0.0017877459043557924
65966,131933,131932,263865,2.7289059162139893,0.0017803913067898248
66066,132133,132132,264265,2.732745885848999,0.0017730669652603658
66166,132333,132332,264665,2.7365639209747314,0.0017657727552972784
66266,132533,132532,265065,2.7403719425201416,0.0017585085529425069
66366,132733,132732,265465,2.7442259788513184,0.0017512742347479118
66466,132933,132932,265865,2.7480759620666504,0.0017440696777732204
66567,133135,133134,266269,2.751953125,0.001736823159664914
66667,133335,133334,266669,2.755751132965088,0.0017296780528846538
66767,133535,133534,267069,2.759554147720337,0.0017225623403179775
66867,133735,133734,267469,2.7634270191192627,0.0017154759010401923
66967,133935,133934,267869,2.7672481536865234,0.0017084186146240808
67067,134135,134134,268269,2.771076202392578,0.0017013903611378695
67167,134335,134334,268669,2.7749061584472656,0.001694391021143133
67267,134535,134534,269069,2.778722047805786,0.0016874204756928367
67367,134735,134734,269469,2.7825331687927246,0.0016804786063292691
67467,134935,134934,269869,2.7863340377807617,0.0016735652950820312
67568,135137,135136,270273,2.790178060531616,0.001666611718988814
67668,135337,135336,270673,2.7940380573272705,0.0016597554546494539
67768,135537,135536,271073,2.798145055770874,0.0016529273962564194
67868,135737,135736,271473,2.8029732704162598,0.001646127427773425
67968,135937,135936,271873,2.8073770999908447,0.0016393554336415486
68068,136137,136136,272273,2.8113012313842773,0.001632611298777284
68168,136337,136336,272673,2.815762996673584,0.0016258949085705442
68268,136537,136536,273073,2.81977915763855,0.001619206148882733
68368,136737,136736,273473,2.8243091106414795,0.001612544906044839
68468,136937,136936,273873,2.8283021450042725,0.0016059110668554268
68569,137139,137138,274277,2.8325490951538086,0.0015992385905348953
68669,137339,137338,274677,2.8366241455078125,0.0015926594921201371
68769,137539,137538,275077,2.8404250144958496,0.0015861074594204127
68869,137739,137738,275477,2.8442962169647217,0.0015795823810902084
68969,137939,137938,275877,2.848341941833496,0.0015730841462421178
69069,138139,138138,276277,2.852306842803955,0.0015666126444448963
69169,138339,138338,276677,2.8561041355133057,0.0015601677657215997
69269,138539,138538,277077,2.8598179817199707,0.0015537494005477077
69369,138739,138738,277477,2.8635692596435547,0.0015473574398492983
69469,138939,138938,277877,2.8674070835113525,0.0015409917750011423
69570,139141,139140,278281,2.8713600635528564,0.0015345890349359838
69670,139341,139340,278681,2.875135898590088,0.0015282758979551663
69770,139541,139540,279081,2.8791401386260986,0.001521988732552163
69870,139741,139740,279481,2.883018970489502,0.0015157274318826548
69970,139941,139940,279881,2.886850118637085,0.0015094918895418635
70070,140141,140140,280281,2.8908801078796387,0.0015032819995627511
70170,140341,140340,280681,2.894803047180176,0.0014970976564141962
70270,140541,140540,281081,2.898698091506958,0.001490938754999273
70370,140741,140740,281481,2.903381109237671,0.0014848051906533562
70470,140941,140940,281881,2.907392978668213,0.0014786968591424235
70571,141143,141142,282285,2.911487102508545,0.0014725529511879349
70671,141343,141342,282685,2.9155020713806152,0.0014664950240942938
70771,141543,141542,283085,2.9197349548339844,0.0014604620186719783
70871,141743,141742,283485,2.923704147338867,0.001454453832395876
70971,141943,141942,283885,2.927739143371582,0.00144847036316264
71071,142143,142142,284285,2.9316470623016357,0.0014425115092889865
71171,142343,142342,284685,2.9355452060699463,0.0014365771695099103
71271,142543,142542,285085,2.939439058303833,0.0014306672429770244
71371,142743,142742,285485,2.9433772563934326,0.0014247816292568235
71471,142943,142942,285885,2.9474339485168457,0.0014189202283289575
71572,143145,143144,286289,2.951399087905884,0.0014130246891427183
71672,143345,143344,286689,2.955310106277466,0.0014072116550229877
71772,143545,143544,287089,2.959230899810791,0.001401422535110811
71872,143745,143744,287489,2.9632692337036133,0.001395657231025652
71972,143945,143944,287889,2.9673142433166504,0.0013899156447917012
72072,144145,144144,288289,2.971369981765747,0.0013841976788362704
72172,144345,144344,288689,2.975304126739502,0.0013785032359880003
72272,144545,144544,289089,2.97920298576355,0.001372832219475324
72372,144745,144744,289489,2.983100175857544,0.001367184532924772
72472,144945,144944,289889,2.986973285675049,0.001361560080359351
72573,145147,145146,290293,2.9908900260925293,0.0013559028695818089
72673,145347,145346,290693,2.994753122329712,0.0013503248285861524
72773,145547,145546,291093,2.9985899925231934,0.0013447697350611769
72873,145747,145746,291493,3.002389907836914,0.001339237494603421
72973,145947,145946,291893,3.006186008453369,0.001333728013197769
73073,146147,146146,292293,3.0100090503692627,0.0013282411972158998
73173,146347,146346,292693,3.0140249729156494,0.0013227769534146663
73273,146547,146546,293093,3.0180561542510986,0.0013173351889344982
73373,146747,146746,293493,3.0222089290618896,0.0013119158112978406
73473,146947,146946,293893,3.026095151901245,0.0013065187284075806
73574,147149,147148,294297,3.030019998550415,0.0013010902115628044
73674,147349,147348,294697,3.0338852405548096,0.0012957376640448696
73774,147549,147548,295097,3.0377700328826904,0.0012904071363412947
73874,147749,147748,295497,3.0417861938476562,0.0012850985378648904
73974,147949,147948,295897,3.045875310897827,0.0012798117784011552
74074,148149,148148,296297,3.049718141555786,0.0012745467681066836
74174,148349,148348,296697,3.0543291568756104,0.001269303417507698
74274,148549,148548,297097,3.0584890842437744,0.0012640816374985138
74374,148749,148748,297497,3.062343120574951,0.0012588813393399842
74474,148949,148948,297897,3.066356897354126,0.0012537024346580565
74575,149151,149150,298301,3.0701942443847656,0.001248493366745823
74675,149351,149350,298701,3.074120283126831,0.0012433571970844517
74775,149551,149550,299101,3.0780138969421387,0.0012382421570818233
74875,149751,149750,299501,3.081794023513794,0.0012331481598127723
74975,149951,149950,299901,3.08559513092041,0.0012280751187097034
75075,150151,150150,300301,3.089437246322632,0.0012230229475611747
75175,150351,150350,300701,3.0932552814483643,0.0012179915605103951
75275,150551,150550,301101,3.0971219539642334,0.001212980872053783
75375,150751,150750,301501,3.1011099815368652,0.0012079907970395229
75475,150951,150950,301901,3.105386972427368,0.0012030212506660963
75576,151153,151152,302305,3.109337091445923,0.0011980227604172593
75676,151353,151352,302705,3.113215923309326,0.0011930942214922022
75776,151553,151552,303105,3.117711067199707,0.0011881859580550004
75876,151753,151752,303505,3.121809244155884,0.001183297886694451
75976,151953,151952,303905,3.1259021759033203,0.001178429924342487
76076,152153,152152,304305,3.1297600269317627,0.0011735819882727528
76176,152353,152352,304705,3.133815050125122,0.0011687539960992717
76276,152553,152552,305105,3.137727975845337,0.0011639458657749313
76376,152753,152752,305505,3.141606092453003,0.0011591575155902255
76476,152953,152952,305905,3.1455280780792236,0.001154388864171719
76577,153155,153154,306309,3.1495091915130615,0.0011495924389400586
76677,153355,153354,306709,3.1533710956573486,0.001144863137235229
76777,153555,153554,307109,3.157231092453003,0.001140153291377413
76877,153755,153754,307509,3.161393165588379,0.0011354628213273007
76977,153955,153954,307909,3.165436267852783,0.0011307916473748854
77077,154155,154154,308309,3.1693811416625977,0.0011261396901380532
77177,154355,154354,308709,3.1732993125915527,0.0011215068705612604
77277,154555,154554,309109,3.1772470474243164,0.0011168931099141952
77377,154755,154754,309509,3.181220054626465,0.0011122983297904595
77477,154955,154954,309909,3.185124158859253,0.0011077224521061743
77578,155157,155156,310313,3.1890621185302734,0.0011031199233709635
77678,155357,155356,310713,3.192978858947754,0.0010985818046799188
77778,155557,155556,311113,3.1969780921936035,0.0010940623553291973
77878,155757,155756,311513,3.2009332180023193,0.0010895614985150842
77978,155957,155956,311913,3.2048420906066895,0.0010850791577498718
78078,156157,156156,312313,3.208735942840576,0.001080615256860472
78178,156357,156356,312713,3.2127292156219482,0.0010761697199872051
78278,156557,156556,313113,3.216768980026245,0.0010717424715824412
78378,156757,156756,313513,3.2207159996032715,0.0010673334364093585
78478,156957,156956,313913,3.224621057510376,0.0010629425395406503
78579,157159,157158,314317,3.22855806350708,0.0010585260689953125
78679,157359,157358,314717,3.2325351238250732,0.001054171404704609
78779,157559,157558,315117,3.2364320755004883,0.0010498346550422174
78879,157759,157758,315517,3.2403481006622314,0.0010455157463092463
78979,157959,157958,315917,3.244263172149658,0.0010412146051100048
79079,158159,158158,316317,3.248152017593384,0.0010369311583507488
79179,158359,158358,316717,3.253278970718384,0.0010326653332384033
79279,158559,158558,317117,3.2571940422058105,0.0010284170572793824
79379,158759,158758,317517,3.26117205619812,0.0010241862582783293
79479,158959,158958,317917,3.265075922012329,0.0010199728643369079
79580,159161,159160,318321,3.2691729068756104,0.0010157349305401128
79680,159361,159360,318721,3.2731881141662598,0.0010115563044671315
79780,159561,159560,319121,3.2770941257476807,0.0010073948688198546
79880,159761,159760,319521,3.2810120582580566,0.0010032505528786693
79980,159961,159960,319921,3.284907102584839,0.000999123286214956
80080,160161,160160,320321,3.288804054260254,0.0009950129986897663
80180,160361,160360,320721,3.292694091796875,0.0009909196204527177
80280,160561,160560,321121,3.2966341972351074,0.0009868430819407832
80380,160761,160760,321521,3.3004138469696045,0.0009827833138771347
80480,160961,160960,321921,3.3043088912963867,0.0009787402472699015
80581,161163,161162,322325,3.308115005493164,0.0009746736328361112
80681,161363,161362,322725,3.311941146850586,0.0009706639285989526
80781,161563,161562,323125,3.3159570693969727,0.0009666707198609293
80881,161763,161762,323525,3.319808006286621,0.0009626939387612899
80981,161963,161962,323925,3.3237900733947754,0.0009587335177184958
81081,162163,162162,324325,3.3278450965881348,0.0009547893894289958
81181,162363,162362,324725,3.3321480751037598,0.0009508614868661091
81281,162563,162562,325125,3.335961103439331,0.0009469497432789391
81381,162763,162762,325525,3.3400120735168457,0.0009430540921911496
81481,162963,162962,325925,3.3438169956207275,0.0009391744673998846
81582,163165,163164,326329,3.347633123397827,0.000935272246707893
81682,163365,163364,326729,3.3514840602874756,0.0009314246356059012
81782,163565,163564,327129,3.3555991649627686,0.0009275928531690238
81882,163765,163764,327529,3.3594858646392822,0.0009237768342798167
81982,163965,163964,327929,3.3632829189300537,0.0009199765140887116
82082,164165,164164,328329,3.3671321868896484,0.0009161918280129229
82182,164365,164364,328729,3.3708841800689697,0.0009124227117353531
82282,164565,164564,329129,3.374678134918213,0.0009086691012035014
82382,164765,164764,329529,3.378476142883301,0.0009049309326283809
82482,164965,164964,329929,3.3822362422943115,0.0009012081424833965
82583,165167,165166,330333,3.386070966720581,0.0008974636698816971
82683,165367,165366,330733,3.3898510932922363,0.0008937715992658582
82783,165567,165566,331133,3.3936691284179688,0.0008900947174380366
82883,165767,165766,331533,3.3974599838256836,0.0008864329619131639
82983,165967,165966,331933,3.4012279510498047,0.000882786270463232
83083,166167,166166,332333,3.4050040245056152,0.0008791545811162163
83183,166367,166366,332733,3.4087889194488525,0.0008755378321550661
83283,166567,166566,333133,3.412574052810669,0.0008719359621165982
83383,166767,166766,333533,3.416714906692505,0.0008683489097905232
83483,166967,166966,333933,3.4206111431121826,0.0008647766142183077
83584,167169,167168,334337,3.424520969390869,0.0008611835127072635
83684,167369,167368,334737,3.4283089637756348,0.000857640694820799
83784,167569,167568,335137,3.4320502281188965,0.0008541124517124077
83884,167769,167768,335537,3.435857057571411,0.0008505987234229927
83984,167969,167968,335937,3.4396331310272217,0.0008470994502401269
84084,168169,168168,336337,3.4434852600097656,0.0008436145726970179
84184,168369,168368,336737,3.4472970962524414,0.0008401440315715475
84284,168569,168568,337137,3.4510631561279297,0.0008366877678851835
84384,168769,168768,337537,3.4548189640045166,0.0008332457229020795
84484,168969,168968,337937,3.4586281776428223,0.0008298178381279802
84585,169171,169170,338341,3.462549924850464,0.0008263699884994855
84685,169371,169370,338741,3.4667229652404785,0.000822970389769486
84785,169571,169570,339141,3.4706239700317383,0.0008195847766291025
84885,169771,169770,339541,3.4745142459869385,0.0008162130915430944
84985,169971,169970,339941,3.4783971309661865,0.0008128552772129153
85085,170171,170170,340341,3.4822280406951904,0.0008095112765757376
85185,170371,170370,340741,3.486030101776123,0.0008061810328035038
85285,170571,170570,341141,3.4898340702056885,0.0008028644893019075
85385,170771,170770,341541,3.4936671257019043,0.0007995615897095013
85485,170971,170970,341941,3.497497081756592,0.0007962722778966719
85586,171173,171172,342345,3.501399040222168,0.0007929638083128772
85686,171373,171372,342745,3.5052971839904785,0.000789701639074892
85786,171573,171572,343145,3.5091309547424316,0.0007864528900561255
85886,171773,171772,343545,3.512953042984009,0.0007832175060472207
85986,171973,171972,343945,3.5167312622070312,0.0007799954320659252
86086,172173,172172,344345,3.5205721855163574,0.0007767866133561951
86186,172373,172372,344745,3.5244300365448,0.0007735909953872531
86286,172573,172572,345145,3.5283620357513428,0.0007704085238526242
86386,172773,172772,345545,3.532210111618042,0.0007672391446693147
86486,172973,172972,345945,3.536079168319702,0.0007640828039767418
86587,173175,173174,346349,3.539933919906616,0.0007609080799701154
86687,173375,173374,346749,3.5438551902770996,0.0007577777846080904
86787,173575,173574,347149,3.547760248184204,0.000754660366950111
86887,173775,173774,347549,3.5516090393066406,0.0007515557740186439
86987,173975,173974,347949,3.5554749965667725,0.0007484639530541494
87087,174175,174174,348349,3.559433937072754,0.0007453848515140839
87187,174375,174374,348749,3.563720941543579,0.0007423184170720906
87287,174575,174574,349149,3.5676732063293457,0.0007392645976170561
87387,174775,174774,349549,3.571605920791626,0.0007362233412522726
87487,174975,174974,349949,3.5754411220550537,0.0007331945962945061
87588,175177,175176,350353,3.579324245452881,0.0007301482111720159
87688,175377,175376,350753,3.5834429264068604,0.0007271444586568655
87788,175577,175576,351153,3.5880539417266846,0.0007241530632618487
87888,175777,175776,351553,3.5920162200927734,0.0007211739741510998
87988,175977,175976,351953,3.5959041118621826,0.0007182071406978532
88088,176177,176176,352353,3.599799156188965,0.0007152525124836574
88188,176377,176376,352753,3.6037650108337402,0.0007123100392974267
88288,176577,176576,353153,3.607771158218384,0.0007093796711346646
88388,176777,176776,353553,3.6116371154785156,0.000706461358196588
88488,176977,176976,353953,3.6154990196228027,0.0007035550508892803
88589,177179,177178,354357,3.6198551654815674,0.0007006318165245928
88689,177379,177378,354757,3.6238150596618652,0.0006977494913351491
88789,177579,177578,355157,3.6277291774749756,0.0006948790237266729
88889,177779,177778,355557,3.6315839290618896,0.0006920203649183336
88989,177979,177978,355957,3.6363582611083984,0.0006891734663299825
89089,178179,178178,356357,3.640247106552124,0.0006863382795813204
89189,178379,178378,356757,3.6442041397094727,0.0006835147564910646
89289,178579,178578,357157,3.6482129096984863,0.0006807028490761866
89389,178779,178778,357557,3.6521410942077637,0.0006779025095509966
89489,178979,178978,357957,3.656219244003296,0.0006751136903264208
89590,179181,179180,358361,3.6601130962371826,0.0006723086283243344
89690,179381,179380,358761,3.663987874984741,0.0006695428217354923
89790,179581,179580,359161,3.667983055114746,0.0006667883933824186
89890,179781,179780,359561,3.671999931335449,0.0006640452964562696
89990,179981,179980,359961,3.6758809089660645,0.000661313484340747
90090,180181,180180,360361,3.6797430515289307,0.0006585929106113304
90190,180381,180380,360761,3.683608055114746,0.0006558835290344818
90290,180581,180580,361161,3.687519073486328,0.0006531852935668883
90390,180781,180780,361561,3.691534996032715,0.0006504981583546004
90490,180981,180980,361961,3.695482015609741,0.0006478220777323728
90591,181183,181182,362365,3.6993792057037354,0.0006451304109503172
90691,181383,181382,362765,3.7032649517059326,0.0006424764126731859
90791,181583,181582,363165,3.707130193710327,0.0006398333326642635
90891,181783,181782,363565,3.7110509872436523,0.000637201126006946
90991,181983,181982,363965,3.7149670124053955,0.0006345797479694101
91091,182183,182182,364365,3.7188479900360107,0.0006319691540038736
91191,182383,182382,364765,3.722745180130005,0.0006293692997457922
91291,182583,182582,365165,3.7266879081726074,0.0006267801410131619
91391,182783,182782,365565,3.7306201457977295,0.0006242016338056925
91491,182983,182982,365965,3.7345762252807617,0.0006216337343041626
91592,183185,183184,366369,3.738535165786743,0.0006190508787165712
91692,183385,183384,366769,3.742434024810791,0.000616504168876702
91792,183585,183584,367169,3.746457099914551,0.0006139679359317464
91892,183785,183784,367569,3.7504281997680664,0.0006114421367808764
91992,183985,183984,367969,3.75433611869812,0.0006089267285005744
92092,184185,184184,368369,3.7582719326019287,0.0006064216683438989
92192,184385,184384,368769,3.76225209236145,0.0006039269137397423
92292,184585,184584,369169,3.7662670612335205,0.0006014424222921702
92392,184785,184784,369569,3.7702388763427734,0.0005989681517796376
92492,184985,184984,369969,3.774260997772217,0.0005965040601543032
92593,185187,185186,370373,3.778351068496704,0.0005940256170458203
92693,185387,185386,370773,3.7823071479797363,0.0005915818584856152
92793,185587,185586,371173,3.7862610816955566,0.0005891481532896432
92893,185787,185786,371573,3.7902321815490723,0.0005867244600994535
92993,185987,185986,371973,3.7942070960998535,0.0005843107377267003
93093,186187,186186,372373,3.7981250286102295,0.0005819069451524923
93193,186387,186386,372773,3.802006959915161,0.0005795130415266957
93293,186587,186586,373173,3.8059849739074707,0.0005771289861672234
93393,186787,186786,373573,3.810091018676758,0.0005747547385593525
93493,186987,186986,373973,3.8140430450439453,0.0005723902583550136
93594,187189,187188,374377,3.818120241165161,0.0005700120068292604
93694,187389,187388,374777,3.822064161300659,0.0005676670377216321
93794,187589,187588,375177,3.8261680603027344,0.0005653317155688939
93894,187789,187788,375577,3.830095052719116,0.0005630060006845002
93994,187989,187988,375977,3.8340320587158203,0.0005606898535451493
94094,188189,188188,376377,3.838024139404297,0.0005583832347901581
94194,188389,188388,376777,3.842036008834839,0.0005560861052207555
94294,188589,188588,377177,3.846261978149414,0.0005537984257994406
94394,188789,188788,377577,3.850346088409424,0.0005515201576493039
94494,188989,188988,377977,3.854344129562378,0.000549251262053377
94595,189191,189190,378381,3.858315944671631,0.0005469691518445876
94695,189391,189390,378781,3.8622519969940186,0.0005447189786051994
94795,189591,189590,379181,3.866274118423462,0.0005424780623405207
94895,189791,189790,379581,3.8702311515808105,0.0005402463649683385
94995,189991,189990,379981,3.8741941452026367,0.0005380238485631097
95095,190191,190190,380381,3.87813401222229,0.0005358104753552924
95195,190391,190390,380781,3.882075071334839,0.0005336062077307536
95295,190591,190590,381181,3.886025905609131,0.0005314110082300831
95395,190791,190790,381581,3.8899550437927246,0.0005292248395479789
95495,190991,190990,381981,3.893908977508545,0.0005270476645326075
95596,191193,191192,382385,3.897879123687744,0.0005248578091078595
95696,191393,191392,382785,3.9018101692199707,0.0005226985995938372
95796,191593,191592,383185,3.905750036239624,0.0005205482728393725
95896,191793,191792,383585,3.909684896469116,0.0005184067923017403
95996,191993,191992,383985,3.9136171340942383,0.0005162741215885456
96096,192193,192192,384385,3.9175710678100586,0.0005141502244571144
96196,192393,192392,384785,3.9215240478515625,0.0005120350648138418
96296,192593,192592,385185,3.9254910945892334,0.0005099286067136191
96396,192793,192792,385585,3.9294891357421875,0.0005078308143592323
96496,192993,192992,385985,3.9334330558776855,0.0005057416521007108
96597,193195,193194,386389,3.9374051094055176,0.0005036403220410416
96697,193395,193394,386789,3.9413859844207764,0.0005015683990246994
96797,193595,193594,387189,3.945505142211914,0.0004995049996805148
96897,193795,193794,387589,3.9494619369506836,0.0004974500889429897
96997,193995,193994,387989,3.9535531997680664,0.0004954036318908944
97097,194195,194194,388389,3.9575071334838867,0.0004933655937466648
97197,194395,194394,388789,3.9615988731384277,0.0004913359398757927
97297,194595,194594,389189,3.965451955795288,0.0004893146357862796
97397,194795,194794,389589,3.969343900680542,0.000487301647128011
97497,194995,194994,389989,3.9731712341308594,0.0004852969396921588
97598,195197,195196,390393,3.9771602153778076,0.00048328055634108214
97698,195397,195396,390793,3.981372117996216,0.00048129239124743264
97798,195597,195596,391193,3.985795021057129,0.00047931240525470335
97898,195797,195796,391593,3.9898180961608887,0.00047734056471492676
97998,195997,195996,391993,3.9946539402008057,0.0004753768361185795
98098,196197,196196,392393,3.998885154724121,0.000473421186093979
98198,196397,196396,392793,4.003031015396118,0.0004714735814067335
98298,196597,196596,393193,4.006967067718506,0.00046953398895918826
98398,196797,196796,393593,4.011446952819824,0.0004676023757898199
98498,196997,196996,393993,4.016211986541748,0.00046567870907273816
98599,197199,197198,394397,4.0201661586761475,0.0004637438384417335
98699,197399,197398,394797,4.024298906326294,0.0004618360453391859
98799,197599,197598,395197,4.028473138809204,0.00045993610069567774
98899,197799,197798,395597,4.032583236694336,0.0004580439722234852
98999,197999,197998,395997,4.0366621017456055,0.0004561596277677057
99099,198199,198198,396397,4.0413312911987305,0.00045428303530572464
99199,198399,198398,396797,4.045583009719849,0.000452414162946645
99299,198599,198598,397197,4.05014705657959,0.000450552978930778
99399,198799,198798,397597,4.0540242195129395,0.0004486994516291035
99499,198999,198998,397997,4.058033227920532,0.0004468535495427096
99600,199201,199200,398401,4.0619330406188965,0.000444996896462976
99700,199401,199400,398801,4.065977096557617,0.00044316622629691983
99800,199601,199600,399201,4.070139169692993,0.00044134308731430094
99900,199801,199800,399601,4.074229955673218,0.00043952744853262976
100000,200001,200000,400001,4.078203201293945,0.00043771927909687125


==> plot_data/quadratic_minimax_problem_n20_alpha0/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.605552673339844e-05,4.387061074692293
100,201,200,401,0.004263162612915039,0.24400872360835765
200,401,400,801,0.008306264877319336,0.11396482179674887
300,601,600,1201,0.012281179428100586,0.07772603596230616
400,801,800,1601,0.01627802848815918,0.06190660644187962
501,1003,1002,2005,0.020492076873779297,0.05363210938132448
601,1203,1202,2405,0.02526116371154785,0.04854289708923014
701,1403,1402,2805,0.029702186584472656,0.044811894255043366
801,1603,1602,3205,0.033898115158081055,0.04179654400397964
901,1803,1802,3605,0.03812718391418457,0.03924971924554778
1001,2003,2002,4005,0.0424041748046875,0.03706348955839846
1101,2203,2202,4405,0.04651594161987305,0.035178785925197326
1201,2403,2402,4805,0.05059099197387695,0.03355453267398762
1301,2603,2602,5205,0.05438995361328125,0.03215726348792642
1401,2803,2802,5605,0.05789899826049805,0.03095767199648659
1502,3005,3004,6009,0.06125020980834961,0.02991998323202208
1602,3205,3204,6409,0.0645749568939209,0.029040939320774044
1702,3405,3404,6809,0.06790399551391602,0.02828835829650628
1802,3605,3604,7209,0.07123708724975586,0.027643543602227788
1902,3805,3804,7609,0.07462024688720703,0.027090075263709473
2002,4005,4004,8009,0.11212515830993652,0.02661366298608146
2102,4205,4204,8409,0.12381100654602051,0.026201975227758096
2202,4405,4404,8809,0.12827420234680176,0.0258444527270099
2302,4605,4604,9209,0.13292431831359863,0.02553211595577548
2402,4805,4804,9609,0.13739490509033203,0.02525737490279822
2503,5007,5006,10013,0.14232921600341797,0.025011551173271675
2603,5207,5206,10413,0.14678621292114258,0.02479413074736284
2703,5407,5406,10813,0.15110015869140625,0.024598087482034042
2803,5607,5606,11213,0.15563106536865234,0.02441972624861084
2903,5807,5806,11613,0.15998625755310059,0.024255984393149754
3003,6007,6006,12013,0.16427111625671387,0.02410432926149394
3103,6207,6206,12413,0.1685020923614502,0.023962670451067175
3203,6407,6406,12813,0.17255115509033203,0.02382928529238106
3303,6607,6606,13213,0.1769249439239502,0.023702755993531773
3403,6807,6806,13613,0.18070411682128906,0.023581916916485614
3504,7009,7008,14017,0.18414998054504395,0.023464670603200708
3604,7209,7208,14417,0.18747806549072266,0.023352546952781245
3704,7409,7408,14817,0.19103217124938965,0.02324371933040331
3804,7609,7608,15217,0.1943531036376953,0.02313765993724719
3904,7809,7808,15617,0.19768309593200684,0.023033936061227892
4004,8009,8008,16017,0.20102715492248535,0.02293219301852367
4104,8209,8208,16417,0.2043609619140625,0.022832140115381733
4204,8409,8408,16817,0.20786404609680176,0.02273353910866042
4304,8609,8608,17217,0.2112131118774414,0.022636194729250055
4404,8809,8808,17617,0.21453595161437988,0.02253994690559794
4505,9011,9010,18021,0.21788907051086426,0.022443716054252546
4605,9211,9210,18421,0.2212049961090088,0.022349299282451357
4705,9411,9410,18821,0.2248539924621582,0.022255651010420593
4805,9611,9610,19221,0.22821712493896484,0.022162698835552937
4905,9811,9810,19621,0.23160910606384277,0.022070383260160423
5005,10011,10010,20021,0.23498916625976562,0.02197865534524145
5105,10211,10210,20421,0.2382831573486328,0.02188747479025684
5205,10411,10410,20821,0.24213504791259766,0.021796808361813313
5305,10611,10610,21221,0.24554228782653809,0.021706628608024154
5405,10811,10810,21621,0.24889326095581055,0.021616912806721164
5506,11013,11012,22025,0.2523651123046875,0.02152675159037204
5606,11213,11212,22425,0.2556171417236328,0.02143791452511929
5706,11413,11412,22825,0.2591691017150879,0.021349493655195773
5806,11613,11612,23225,0.2623932361602783,0.021261478021364178
5906,11813,11812,23625,0.26566410064697266,0.021173858394926075
6006,12013,12012,24025,0.26892518997192383,0.0210866269634385
6106,12213,12212,24425,0.27220821380615234,0.02099977707368877
6206,12413,12412,24825,0.27573394775390625,0.020913303021499314
6306,12613,12612,25225,0.2790231704711914,0.020827199879831903
6406,12813,12812,25625,0.2823061943054199,0.02074146335821519
6507,13015,13014,26029,0.2856571674346924,0.020655237771859597
6607,13215,13214,26429,0.2891991138458252,0.020570227190828582
6707,13415,13414,26829,0.2930910587310791,0.020485573100828172
6807,13615,13614,27229,0.29640698432922363,0.02040127280177237
6907,13815,13814,27629,0.29978013038635254,0.020317323829549257
7007,14015,14014,28029,0.3030431270599365,0.020233723914058508
7107,14215,14214,28429,0.3071732521057129,0.020150470944893955
7207,14415,14414,28829,0.3110010623931885,0.020067562943277894
7307,14615,14614,29229,0.3144261837005615,0.019984998039106475
7407,14815,14814,29629,0.3178219795227051,0.019902774452176045
7508,15017,15016,30033,0.3214411735534668,0.019820073346504125
7608,15217,15216,30433,0.3250579833984375,0.019738530710620945
7708,15417,15416,30833,0.32834410667419434,0.019657324434985902
7808,15617,15616,31233,0.33159804344177246,0.019576452971328227
7908,15817,15816,31633,0.3348522186279297,0.0194959148077385
8008,16017,16016,32033,0.3380851745605469,0.01941570846305175
8108,16217,16216,32433,0.3417370319366455,0.019335832482250178
8208,16417,16416,32833,0.34501028060913086,0.01925628543269952
8308,16617,16616,33233,0.34827423095703125,0.019177065901067873
8408,16817,16816,33633,0.3517723083496094,0.019098172490801885
8509,17019,17018,34037,0.3550431728363037,0.01901881976864435
8609,17219,17218,34437,0.3586270809173584,0.018940577695431893
8709,17419,17418,34837,0.3618910312652588,0.0188626576221969
8809,17619,17618,35237,0.3651261329650879,0.018785058202323093
8909,17819,17818,35637,0.3683600425720215,0.018707778098734175
9009,18019,18018,36037,0.37159299850463867,0.018630815983125406
9109,18219,18218,36437,0.3750760555267334,0.01855417053533105
9209,18419,18418,36837,0.37830615043640137,0.018477840442803484
9309,18619,18618,37237,0.3815422058105469,0.018401824400183057
9409,18819,18818,37637,0.3847620487213135,0.018326121108942536
9510,19021,19020,38041,0.3881661891937256,0.01824997692728853
9610,19221,19220,38441,0.39229321479797363,0.01817489836439712
9710,19421,19420,38841,0.39588499069213867,0.018100128682825716
9810,19621,19620,39241,0.3991522789001465,0.018025666608942708
9910,19821,19820,39641,0.4024052619934082,0.01795151087488961
10010,20021,20020,40041,0.4063541889190674,0.017877660218460007
10110,20221,20220,40441,0.4104161262512207,0.017804113382996836
10210,20421,20420,40841,0.41390514373779297,0.01773086911730443
10310,20621,20620,41241,0.4175240993499756,0.017657926175572894
10410,20821,20820,41641,0.4208393096923828,0.01758528331731253
10511,21023,21022,42045,0.42496418952941895,0.017512217372213767
10611,21223,21222,42445,0.42899298667907715,0.01744017395041506
10711,21423,21422,42845,0.43228912353515625,0.017368426909774835
10811,21623,21622,43245,0.4360771179199219,0.01729697503062207
10911,21823,21822,43645,0.4401721954345703,0.0172258170983744
11011,22023,22022,44045,0.44382429122924805,0.01715495190350446
11111,22223,22222,44445,0.44739317893981934,0.017084378241508134
11211,22423,22422,44845,0.4509623050689697,0.017014094912875637
11311,22623,22622,45245,0.45455002784729004,0.016944100723063484
11411,22823,22822,45645,0.45807528495788574,0.01687439448246843
11512,23025,23024,46049,0.4616272449493408,0.016804282255806782
11612,23225,23224,46449,0.4649841785430908,0.016735151214378838
11712,23425,23424,46849,0.4683411121368408,0.016666304571029123
11812,23625,23624,47249,0.47170209884643555,0.01659774115572194
11912,23825,23824,47649,0.47530221939086914,0.01652945980324449
12012,24025,24024,48049,0.47863292694091797,0.016461459353185378
12112,24225,24224,48449,0.4819209575653076,0.016393738649913198
12212,24425,24424,48849,0.4852161407470703,0.016326296542556084
12312,24625,24624,49249,0.4885270595550537,0.016259131884980845
12412,24825,24824,49649,0.4926478862762451,0.016192243535772873
12513,25027,25026,50053,0.4960823059082031,0.016124965612223152
12613,25227,25226,50453,0.4994239807128906,0.016058629208975092
12713,25427,25426,50853,0.5027570724487305,0.015992565706711873
12813,25627,25626,51253,0.5068180561065674,0.015926773982740765
12913,25827,25826,51653,0.510181188583374,0.015861252918988957
13013,26027,26026,52053,0.5135371685028076,0.01579600140198428
13113,26227,26226,52453,0.5168631076812744,0.015731018322836098
13213,26427,26426,52853,0.5201821327209473,0.01566630257721642
13313,26627,26626,53253,0.5236811637878418,0.015601853065340806
13413,26827,26826,53653,0.527076244354248,0.015537668691949714
13514,27029,27028,54057,0.5305280685424805,0.015473110492795109
13614,27229,27228,54457,0.5339250564575195,0.015409455752744657
13714,27429,27428,54857,0.5373172760009766,0.015346062881567299
13814,27629,27628,55257,0.5407631397247314,0.015282930801961206
13914,27829,27828,55657,0.5443511009216309,0.015220058441056731
14014,28029,28028,56057,0.5476820468902588,0.015157444730397951
14114,28229,28228,56457,0.5510151386260986,0.015095088605924645
14214,28429,28428,56857,0.5543591976165771,0.015032989007954085
14314,28629,28628,57257,0.5578272342681885,0.014971144881162992
14414,28829,28828,57657,0.5611703395843506,0.014909555174569671
14515,29031,29030,58061,0.5645041465759277,0.014847606754191575
14615,29231,29230,58461,0.5678131580352783,0.014786525270388241
14715,29431,29430,58861,0.5711159706115723,0.014725695069349514
14815,29631,29630,59261,0.5745720863342285,0.014665115117324604
14915,29831,29830,59661,0.5780589580535889,0.014604784384815403
15015,30031,30030,60061,0.5813860893249512,0.014544701846559078
15115,30231,30230,60461,0.5847113132476807,0.01448486648151075
15215,30431,30430,60861,0.5881342887878418,0.014425277272825825
15315,30631,30630,61261,0.591569185256958,0.014365933207843056
15415,30831,30830,61661,0.5948810577392578,0.014306833278067182
15516,31033,31032,62065,0.5982100963592529,0.01424738913558572
15616,31233,31232,62465,0.6015141010284424,0.01418877688358528
15716,31433,31432,62865,0.6048200130462646,0.014130405756190456
15816,31633,31632,63265,0.6083130836486816,0.014072274761440025
15916,31833,31832,63665,0.6116669178009033,0.014014382911453726
16016,32033,32032,64065,0.6149942874908447,0.0139567292224153
16116,32233,32232,64465,0.6183161735534668,0.013899312714555747
16216,32433,32432,64865,0.6216230392456055,0.013842132412136788
16316,32633,32632,65265,0.6254041194915771,0.013785187343434193
16416,32833,32832,65665,0.62888503074646,0.013728476540721377
16517,33035,33034,66069,0.6323990821838379,0.013671435440173726
16617,33235,33234,66469,0.6357481479644775,0.013615192600759746
16717,33435,33434,66869,0.6392760276794434,0.013559181138438509
16817,33635,33634,67269,0.642951250076294,0.01350340010134909
16917,33835,33834,67669,0.6463322639465332,0.013447848541546467
17017,34035,34034,68069,0.649691104888916,0.013392525514985343
17117,34235,34234,68469,0.6531691551208496,0.013337430081504184
17217,34435,34434,68869,0.6566059589385986,0.013282561304809058
17317,34635,34634,69269,0.6598761081695557,0.013227918252457985
17417,34835,34834,69669,0.6631491184234619,0.01317349999584482
17518,35037,35036,70073,0.6664121150970459,0.013118764793756114
17618,35237,35236,70473,0.6696791648864746,0.013064795582927223
17718,35437,35436,70873,0.6730802059173584,0.01301104839572354
17818,35637,35636,71273,0.6766142845153809,0.012957522318763317
17918,35837,35836,71673,0.6798861026763916,0.012904216442422432
18018,36037,36036,72073,0.683131217956543,0.012851129860818794
18118,36237,36236,72473,0.6863648891448975,0.01279826167179707
18218,36437,36436,72873,0.6899609565734863,0.012745610976913279
18318,36637,36636,73273,0.6935510635375977,0.012693176881419535
18418,36837,36836,73673,0.6968340873718262,0.012640958494248851
18519,37039,37038,74077,0.7001900672912598,0.012588435974189925
18619,37239,37238,74477,0.7034852504730225,0.012536648480033455
18719,37439,37438,74877,0.7074329853057861,0.012485074034150523
18819,37639,37638,75277,0.7107691764831543,0.012433711760083094
18919,37839,37838,75677,0.7140452861785889,0.012382560784978723
19019,38039,38038,76077,0.7173402309417725,0.012331620239575868
19119,38239,38238,76477,0.7206110954284668,0.01228088925818896
19219,38439,38438,76877,0.724013090133667,0.012230366978693818
19319,38639,38638,77277,0.7274312973022461,0.012180052542512906
19419,38839,38838,77677,0.7307100296020508,0.012129945094600848
19520,39041,39040,78081,0.7341761589050293,0.012079545808436398
19620,39241,39240,78481,0.7374720573425293,0.01202985183459805
19720,39441,39440,78881,0.7409861087799072,0.011980362296512089
19820,39641,39640,79281,0.7442638874053955,0.011931076353151427
19920,39841,39840,79681,0.7475481033325195,0.011881993166948941
20020,40041,40040,80081,0.7508599758148193,0.01183311190378311
20120,40241,40240,80481,0.7541511058807373,0.011784431732963906
20220,40441,40440,80881,0.7576830387115479,0.011735951827218701
20320,40641,40640,81281,0.7609663009643555,0.011687671362678157
20420,40841,40840,81681,0.7642569541931152,0.011639589518862252
20521,41043,41042,82085,0.7676081657409668,0.011591227634416544
20621,41243,41242,82485,0.7710020542144775,0.011543542549898145
20721,41443,41442,82885,0.7748911380767822,0.011496053636773956
20821,41643,41642,83285,0.7781713008880615,0.011448760088015549
20921,41843,41842,83685,0.7814791202545166,0.011401661099914676
21021,42043,42042,84085,0.7847769260406494,0.011354755872069319
21121,42243,42242,84485,0.7880520820617676,0.011308043607370302
21221,42443,42442,84885,0.7917649745941162,0.011261523511987627
21321,42643,42642,85285,0.795051097869873,0.0112151947953571
21421,42843,42842,85685,0.7983119487762451,0.011169056670166717
21522,43045,43044,86089,0.8016431331634521,0.01112264982504777
21622,43245,43244,86489,0.8049640655517578,0.011076892420077013
21722,43445,43444,86889,0.8089599609375,0.011031323256230713
21822,43645,43644,87289,0.8122670650482178,0.010985941559104768
21922,43845,43844,87689,0.8156599998474121,0.010940746557480913
22022,44045,44044,88089,0.8190860748291016,0.010895737483313583
22122,44245,44244,88489,0.8232932090759277,0.010850913571716898
22222,44445,44444,88889,0.8267161846160889,0.010806274060951618
22322,44645,44644,89289,0.8299791812896729,0.010761818192412247
22422,44845,44844,89689,0.8335270881652832,0.010717545210614084
22523,45047,45046,90093,0.83685302734375,0.010673014371946841
22623,45247,45246,90493,0.8403279781341553,0.010629106719673554
22723,45447,45446,90893,0.8437702655792236,0.010585379698837745
22823,45647,45646,91293,0.8470070362091064,0.010541832566340786
22923,45847,45846,91693,0.8502500057220459,0.010498464582141067
23023,46047,46046,92093,0.8534872531890869,0.010455275009241429
23123,46247,46246,92493,0.8572039604187012,0.010412263113676686
23223,46447,46446,92893,0.8606619834899902,0.010369428164501055
23323,46647,46646,93293,0.8639049530029297,0.010326769433775803
23423,46847,46846,93693,0.8671972751617432,0.010284286196556858
23524,47049,47048,94097,0.8704659938812256,0.010241555526386868
23624,47249,47248,94497,0.8737242221832275,0.010199422850170116
23724,47449,47448,94897,0.8773071765899658,0.010157463503327056
23824,47649,47648,95297,0.8805890083312988,0.010115676772798968
23924,47849,47848,95697,0.8838472366333008,0.010074061948460666
24024,48049,48048,96097,0.8871171474456787,0.010032618323108216
24124,48249,48248,96497,0.8904011249542236,0.009991345192447064
24224,48449,48448,96897,0.8939011096954346,0.00995024185508015
24324,48649,48648,97297,0.8972022533416748,0.009909307612495753
24424,48849,48848,97697,0.9007790088653564,0.009868541769055873
24525,49051,49050,98101,0.9042141437530518,0.009827538495193936
24625,49251,49250,98501,0.9075078964233398,0.009787109041254165
24725,49451,49450,98901,0.9107611179351807,0.009746845909811806
24825,49651,49650,99301,0.9141221046447754,0.009706748416633661
24925,49851,49850,99701,0.9179441928863525,0.009666815880301487
25025,50051,50050,100101,0.9225962162017822,0.009627047622200218
25125,50251,50250,100501,0.9266631603240967,0.009587442966506592
25225,50451,50450,100901,0.930164098739624,0.009548001240177635
25325,50651,50650,101301,0.933969259262085,0.009508721772939172
25425,50851,50850,101701,0.9380879402160645,0.009469603897274465
25526,51053,51052,102105,0.9415731430053711,0.009430258189362294
25626,51253,51252,102505,0.9448461532592773,0.009391463104581561
25726,51453,51452,102905,0.9481470584869385,0.009352827618676379
25826,51653,51652,103305,0.9514749050140381,0.009314351075073826
25926,51853,51852,103705,0.9547860622406006,0.009276032819902103
26026,52053,52052,104105,0.9580972194671631,0.00923787220197936
26126,52253,52252,104505,0.9614551067352295,0.009199868572802628
26226,52453,52452,104905,0.9647622108459473,0.009162021286536771
26326,52653,52652,105305,0.9680671691894531,0.009124329700003632
26426,52853,52852,105705,0.9713761806488037,0.009086793172670976
26527,53055,53054,106109,0.9747161865234375,0.009049038023257273
26627,53255,53254,106509,0.9780302047729492,0.009011811237919354
26727,53455,53454,106909,0.9813282489776611,0.008974737599638951
26827,53655,53654,107309,0.9847631454467773,0.008937816478385275
26927,53855,53854,107709,0.9880781173706055,0.008901047246719404
27027,54055,54054,108109,0.9913783073425293,0.008864429279783642
27127,54255,54254,108509,0.9946801662445068,0.008827961955290868
27227,54455,54454,108909,0.9979982376098633,0.008791644653514006
27327,54655,54654,109309,1.0013060569763184,0.008755476757275497
27427,54855,54854,109709,1.004992961883545,0.008719457651936706
27528,55057,55056,110113,1.0083389282226562,0.008683228762360428
27628,55257,55256,110513,1.0116453170776367,0.008647506877631283
27728,55457,55456,110913,1.0149621963500977,0.00861193194895774
27828,55657,55656,111313,1.018273115158081,0.008576503371778088
27928,55857,55856,111713,1.0215752124786377,0.008541220544017788
28028,56057,56056,112113,1.0248920917510986,0.00850608286607914
28128,56257,56256,112513,1.028196096420288,0.008471089740831111
28228,56457,56456,112913,1.0315170288085938,0.008436240573599233
28328,56657,56656,113313,1.0348231792449951,0.008401534772155474
28428,56857,56856,113713,1.0381231307983398,0.008366971746708104
28529,57059,57058,114117,1.0414509773254395,0.008332207417595033
28629,57259,57258,114517,1.0447502136230469,0.008297929597551771
28729,57459,57458,114917,1.0480539798736572,0.008263792792834741
28829,57659,57658,115317,1.051281213760376,0.008229796423321747
28929,57859,57858,115717,1.0546891689300537,0.008195939911277242
29029,58059,58058,116117,1.057819128036499,0.008162222681342373
29129,58259,58258,116517,1.0609452724456787,0.008128644160525297
29229,58459,58458,116917,1.0640971660614014,0.008095203778191359
29329,58659,58658,117317,1.0672392845153809,0.00806190096605345
29429,58859,58858,117717,1.070406198501587,0.008028735158162345
29530,59061,59060,118121,1.0735690593719482,0.007995376184348438
29630,59261,59260,118521,1.076709270477295,0.007962484052373132
29730,59461,59460,118921,1.0798752307891846,0.007929727235149852
29830,59661,59660,119321,1.0830662250518799,0.007897105176008062
29930,59861,59860,119721,1.0862131118774414,0.007864617320567235
30030,60061,60060,120121,1.0904719829559326,0.007832263116727552
30130,60261,60260,120521,1.0948641300201416,0.007800042014660447
30230,60461,60460,120921,1.099095106124878,0.007767953466799313
30330,60661,60660,121321,1.1027240753173828,0.007735996927830199
30430,60861,60860,121721,1.1061370372772217,0.007704171854682442
30531,61063,61062,122125,1.1096701622009277,0.007672161424384856
30631,61263,61262,122525,1.1133100986480713,0.0076405989637465845
30731,61463,61462,122925,1.1171820163726807,0.007609166347733111
30831,61663,61662,123325,1.1211252212524414,0.0075778630421773656
30931,61863,61862,123725,1.1252861022949219,0.0075466885151098265
31031,62063,62062,124125,1.1290769577026367,0.007515642236749418
31131,62263,62262,124525,1.133155107498169,0.007484723679494517
31231,62463,62462,124925,1.1370460987091064,0.007453932317913985
31331,62663,62662,125325,1.1405901908874512,0.007423267628738286
31431,62863,62862,125725,1.1446471214294434,0.007392729090850528
31532,63065,63064,126129,1.1482820510864258,0.007362012688914633
31632,63265,63264,126529,1.1515991687774658,0.007331726147370554
31732,63465,63464,126929,1.1552770137786865,0.007301564201455097
31832,63665,63664,127329,1.158674955368042,0.007271526338594972
31932,63865,63864,127729,1.1624341011047363,0.007241612048325651
32032,64065,64064,128129,1.166274070739746,0.007211820822282571
32132,64265,64264,128529,1.1697862148284912,0.007182152154192482
32232,64465,64464,128929,1.1733272075653076,0.007152605539864971
32332,64665,64664,129329,1.1766910552978516,0.007123180477183726
32432,64865,64864,129729,1.1800761222839355,0.007093876466098154
32533,65067,65066,130133,1.1834602355957031,0.007064401781155894
32633,65267,65266,130533,1.1868250370025635,0.007035339579408933
32733,65467,65466,130933,1.1901700496673584,0.007006396936486132
32833,65667,65666,131333,1.193526029586792,0.0069775733605351295
32933,65867,65866,131733,1.1968603134155273,0.006948868361727015
33033,66067,66066,132133,1.200242280960083,0.006920281452247954
33133,66267,66266,132533,1.2036030292510986,0.006891812146290943
33233,66467,66466,132933,1.2069621086120605,0.006863459960047532
33333,66667,66666,133333,1.2103612422943115,0.006835224411699583
33433,66867,66866,133733,1.2136969566345215,0.006807105021411168
33534,67069,67068,134137,1.2171361446380615,0.006778821856792532
33634,67269,67268,134537,1.2206902503967285,0.006750934500649469
33734,67469,67468,134937,1.2241201400756836,0.00672316187014001
33834,67669,67668,135337,1.2275891304016113,0.006695503493295036
33934,67869,67868,135737,1.2309739589691162,0.006667958900087056
34034,68069,68068,136137,1.2344810962677002,0.006640527622422218
34134,68269,68268,136537,1.2378230094909668,0.006613209194132384
34234,68469,68468,136937,1.241157054901123,0.006586003150967135
34334,68669,68668,137337,1.2445251941680908,0.006558909030585957
34434,68869,68868,137737,1.2478430271148682,0.00653192637255039
34535,69071,69070,138141,1.2512471675872803,0.006504786560796256
34635,69271,69270,138541,1.2545831203460693,0.006478026556877027
34735,69471,69470,138941,1.258249044418335,0.006451376640783591
34835,69671,69670,139341,1.261620044708252,0.006424836359626273
34935,69871,69870,139741,1.265002965927124,0.0063984052623785575
35035,70071,70070,140141,1.2682969570159912,0.0063720828998694015
35135,70271,70270,140541,1.2715840339660645,0.0063458688247755345
35235,70471,70470,140941,1.2750191688537598,0.006319762591614038
35335,70671,70670,141341,1.2783501148223877,0.006293763756734599
35435,70871,70870,141741,1.2816822528839111,0.006267871878312006
35536,71073,71072,142145,1.2851309776306152,0.006241829199142931
35636,71273,71272,142545,1.2885680198669434,0.006216150973997304
35736,71473,71472,142945,1.2918701171875,0.006190578386354045
35836,71673,71672,143345,1.295177936553955,0.006165111001631597
35936,71873,71872,143745,1.2984881401062012,0.006139748387036292
36036,72073,72072,144145,1.301919937133789,0.006114490111554905
36136,72273,72272,144545,1.3052332401275635,0.0060893357459473624
36236,72473,72472,144945,1.308535099029541,0.006064284862739422
36336,72673,72672,145345,1.3118321895599365,0.0060393370362154435
36436,72873,72872,145745,1.315134048461914,0.006014491842411115
36537,73075,73074,146149,1.3186571598052979,0.005989501944012134
36637,73275,73274,146549,1.3220269680023193,0.005964861766506236
36737,73475,73474,146949,1.3253529071807861,0.005940322956084465
36837,73675,73674,147349,1.3286809921264648,0.005915885095733384
36937,73875,73874,147749,1.3320331573486328,0.0058915477701550695
37037,74075,74074,148149,1.3353610038757324,0.005867310565760089
37137,74275,74274,148549,1.338691234588623,0.0058431730706605236
37237,74475,74474,148949,1.3420040607452393,0.005819134874662815
37337,74675,74674,149349,1.3453280925750732,0.005795195569261004
37437,74875,74874,149749,1.3487141132354736,0.005771354747629617
37538,75077,75076,150153,1.3519511222839355,0.0057473750711171815
37638,75277,75276,150553,1.3551180362701416,0.005723730977957329
37738,75477,75476,150953,1.3582971096038818,0.005700184154095967
37838,75677,75676,151353,1.3614740371704102,0.005676734199377498
37938,75877,75876,151753,1.3646681308746338,0.005653380715292511
38038,76077,76076,152153,1.3680620193481445,0.005630123304971026
38138,76277,76276,152553,1.3712382316589355,0.005606961573175729
38238,76477,76476,152953,1.3744561672210693,0.005583895126295303
38338,76677,76676,153353,1.3776400089263916,0.005560923572337659
38438,76877,76876,153753,1.3810203075408936,0.005538046520923362
38539,77079,77078,154157,1.3846280574798584,0.005515036227865703
38639,77279,77278,154557,1.3885712623596191,0.005492347952133196
38739,77479,77478,154957,1.392137050628662,0.005469753013567384
38839,77679,77678,155357,1.3966059684753418,0.005447251028189034
38939,77879,77878,155757,1.4002571105957031,0.0054248416135985736
39039,78079,78078,156157,1.4042060375213623,0.005402524388969544
39139,78279,78278,156557,1.4077770709991455,0.005380298975042232
39239,78479,78478,156957,1.411161184310913,0.005358164994117084
39339,78679,78678,157357,1.414586067199707,0.0053361220700484215
39439,78879,78878,157757,1.4182310104370117,0.005314169828237971
39540,79081,79080,158161,1.4215459823608398,0.005292089731105537
39640,79281,79280,158561,1.4247190952301025,0.005270318633680339
39740,79481,79480,158961,1.4280610084533691,0.0052486371002472615
39840,79681,79680,159361,1.43123197555542,0.005227044762349522
39940,79881,79880,159761,1.4344761371612549,0.005205541253046146
40040,80081,80080,160161,1.4376540184020996,0.005184126206905686
40140,80281,80280,160561,1.4409122467041016,0.005162799260000051
40240,80481,80480,160961,1.444087028503418,0.005141560049898295
40340,80681,80680,161361,1.4472720623016357,0.005120408215660488
40440,80881,80880,161761,1.4506349563598633,0.005099343397831577
40541,81083,81082,162165,1.4539179801940918,0.0050781558932589165
40641,81283,81282,162565,1.4571552276611328,0.005057264897015461
40741,81483,81482,162965,1.46038818359375,0.00503645984412097
40841,81683,81682,163365,1.4636249542236328,0.005015740381013602
40941,81883,81882,163765,1.4668631553649902,0.0049951061555860285
41041,82083,82082,164165,1.4701659679412842,0.004974556817179435
41141,82283,82282,164565,1.4734022617340088,0.004954092016577594
41241,82483,82482,164965,1.4766321182250977,0.004933711406000938
41341,82683,82682,165365,1.4798781871795654,0.004913414639100601
41441,82883,82882,165765,1.4831910133361816,0.004893201370952563
41542,83085,83084,166169,1.4866302013397217,0.004872870375698116
41642,83285,83284,166569,1.489866018295288,0.004852823902361474
41742,83485,83484,166969,1.4940290451049805,0.004832859898095875
41842,83685,83684,167369,1.4972460269927979,0.004812978023632288
41942,83885,83884,167769,1.5006589889526367,0.004793177941097396
42042,84085,84084,168169,1.504014015197754,0.004773459314007856
42142,84285,84284,168569,1.507349967956543,0.004753821807264584
42242,84485,84484,168969,1.5106632709503174,0.0047342650871470575
42342,84685,84684,169369,1.5139760971069336,0.004714788821307638
42442,84885,84884,169769,1.5173041820526123,0.004695392678765937
42543,85087,85086,170173,1.5208730697631836,0.004675883568260828
42643,85287,85286,170573,1.5241661071777344,0.004656647477815262
42743,85487,85486,170973,1.527440071105957,0.004637490522611249
42843,85687,85686,171373,1.5307278633117676,0.004618412377094773
42943,85887,85886,171773,1.534024953842163,0.004599412717051115
43043,86087,86086,172173,1.5373282432556152,0.004580491219599321
43143,86287,86286,172573,1.5406122207641602,0.004561647563186797
43243,86487,86486,172973,1.54398512840271,0.004542881427583712
43343,86687,86686,173373,1.5474650859832764,0.004524192493877646
43443,86887,86886,173773,1.5507981777191162,0.004505580444468188
43544,87089,87088,174177,1.5541441440582275,0.004486859993848942
43644,87289,87288,174577,1.5574321746826172,0.004468401526396055
43744,87489,87488,174977,1.5607280731201172,0.004450018995125976
43844,87689,87688,175377,1.5640339851379395,0.004431712087645273
43944,87889,87888,175777,1.5681800842285156,0.004413480492845678
44044,88089,88088,176177,1.5715179443359375,0.004395323900898777
44144,88289,88288,176577,1.5748679637908936,0.0043772420032507885
44244,88489,88488,176977,1.578179121017456,0.004359234492617242
44344,88689,88688,177377,1.5814809799194336,0.004341301062977856
44444,88889,88888,177777,1.584873914718628,0.004323441409571246
44545,89091,89090,178181,1.5885560512542725,0.004305477737096482
44645,89291,89290,178581,1.5918331146240234,0.004287765457063616
44745,89491,89490,178981,1.595184087753296,0.004270126043477431
44845,89691,89690,179381,1.598757266998291,0.00425255919657306
44945,89891,89890,179781,1.6022179126739502,0.00423506461781887
45045,90091,90090,180181,1.6055080890655518,0.00421764200991132
45145,90291,90290,180581,1.6092312335968018,0.004200291076769972
45245,90491,90490,180981,1.6130640506744385,0.004183011523532391
45345,90691,90690,181381,1.6163051128387451,0.004165803056549231
45445,90891,90890,181781,1.6196632385253906,0.004148665383379156
45546,91093,91092,182185,1.6229650974273682,0.0041314278961336074
45646,91293,91292,182585,1.6262671947479248,0.004114431638737725
45746,91493,91492,182985,1.6295502185821533,0.004097505302147127
45846,91693,91692,183385,1.6329452991485596,0.004080648598715015
45946,91893,91892,183785,1.6362502574920654,0.0040638612419779405
46046,92093,92092,184185,1.6396021842956543,0.0040471429466509235
46146,92293,92292,184585,1.6430940628051758,0.004030493428622653
46246,92493,92492,184985,1.6464550495147705,0.0040139124049505676
46346,92693,92692,185385,1.6500091552734375,0.003997399593856141
46446,92893,92892,185785,1.6533701419830322,0.003980954714720053
46547,93095,93094,186189,1.657137155532837,0.003964414056513435
46647,93295,93294,186589,1.6603782176971436,0.003948104876389191
46747,93495,93494,186989,1.663661003112793,0.00393186279050701
46847,93695,93694,187389,1.6672420501708984,0.003915687522848269
46947,93895,93894,187789,1.670553207397461,0.003899578798529858
47047,94095,94094,188189,1.6737961769104004,0.003883536343799519
47147,94295,94294,188589,1.6770381927490234,0.003867559886031196
47247,94495,94494,188989,1.6802639961242676,0.0038516491537203333
47347,94695,94694,189389,1.6835331916809082,0.003835803876479375
47447,94895,94894,189789,1.6869261264801025,0.0038200237850330694
47548,95097,95096,190193,1.6902611255645752,0.0038041517864052616
47648,95297,95296,190593,1.6935410499572754,0.0037885019083097856
47748,95497,95496,190993,1.6967942714691162,0.0037729164121575445
47848,95697,95696,191393,1.7000420093536377,0.0037573950330880546
47948,95897,95896,191793,1.7035491466522217,0.003741937507330403
48048,96097,96096,192193,1.7067639827728271,0.003726543572198825
48148,96297,96296,192593,1.7100021839141846,0.0037112129660882044
48248,96497,96496,192993,1.713327169418335,0.0036959454284696516
48348,96697,96696,193393,1.7165660858154297,0.0036807406998860446
48448,96897,96896,193793,1.7200090885162354,0.0036655985219476842
48549,97099,97098,194197,1.723426103591919,0.0036503681521949135
48649,97299,97298,194597,1.7267682552337646,0.0036353509237053447
48749,97499,97498,194997,1.7300441265106201,0.003620395474505458
48849,97699,97698,195397,1.7337872982025146,0.003605501550441781
48949,97899,97898,195797,1.7370612621307373,0.003590668898406413
49049,98099,98098,196197,1.7415440082550049,0.0035758972663327026
49149,98299,98298,196597,1.7449510097503662,0.0035611864031910023
49249,98499,98498,196997,1.7482361793518066,0.0035465360589843316
49349,98699,98698,197397,1.7518901824951172,0.0035319459847442335
49449,98899,98898,197797,1.7574551105499268,0.0035174159325263876
49550,99101,99100,198201,1.7624292373657227,0.003502801253666727
49650,99301,99300,198601,1.7662270069122314,0.003488391099789987
49750,99501,99500,199001,1.7705159187316895,0.003474040227762176
49850,99701,99700,199401,1.7761149406433105,0.00345974839370404
49950,99901,99900,199801,1.7812259197235107,0.003445515354739607
50050,100101,100100,200201,1.785677194595337,0.003431340868992097
50150,100301,100300,200601,1.7898952960968018,0.0034172246955797496
50250,100501,100500,201001,1.7945899963378906,0.003403166594611812
50350,100701,100700,201401,1.7993590831756592,0.0033891663271843615
50450,100901,100900,201801,1.8038651943206787,0.003375223655376346
50551,101103,101102,202205,1.8083691596984863,0.003361199777976271
50651,101303,101302,202605,1.812788963317871,0.00334737215759376
50751,101503,101502,203005,1.817121982574463,0.00333360142257898
50851,101703,101702,203405,1.8215911388397217,0.0033198873389115777
50951,101903,101902,203805,1.825890064239502,0.003306229673533883
51051,102103,102102,204205,1.830143928527832,0.003292628194347024
51151,102303,102302,204605,1.8345370292663574,0.0032790826702069516
51251,102503,102502,205005,1.8387541770935059,0.0032655928709205283
51351,102703,102702,205405,1.842900037765503,0.0032521585672415864
51451,102903,102902,205805,1.8476181030273438,0.003238779530867077
51552,103105,103104,206209,1.8518431186676025,0.0032253225716536013
51652,103305,103304,206609,1.856018304824829,0.003212053935726564
51752,103505,103504,207009,1.8598980903625488,0.0031988398855643464
51852,103705,103704,207409,1.8634212017059326,0.003185680196606894
51952,103905,103904,207809,1.866833209991455,0.003172574645217944
52052,104105,104104,208209,1.870253086090088,0.0031595230086812944
52152,104305,104304,208609,1.8736591339111328,0.003146525065196907
52252,104505,104504,209009,1.8770999908447266,0.0031335805938772707
52352,104705,104704,209409,1.880511999130249,0.003120689374743531
52452,104905,104904,209809,1.8839740753173828,0.0031078511887218507
52553,105107,105106,210213,1.8875839710235596,0.0030949382299083083
52653,105307,105306,210613,1.8910772800445557,0.003082205981372849
52753,105507,105506,211013,1.8946812152862549,0.0030695261119612276
52853,105707,105706,211413,1.8980810642242432,0.003056898406191248
52953,105907,105906,211813,1.9014461040496826,0.003044322649467209
53053,106107,106106,212213,1.9048182964324951,0.003031798628076219
53153,106307,106306,212613,1.908346176147461,0.0030193261291846262
53253,106507,106506,213013,1.9123361110687256,0.0030069049408342867
53353,106707,106706,213413,1.91566801071167,0.0029945348519390645
53453,106907,106906,213813,1.9190089702606201,0.0029822156522812003
53554,107109,107108,214217,1.922386884689331,0.002969824702537307
53654,107309,107308,214617,1.9258952140808105,0.002957607157820564
53754,107509,107508,215017,1.92946195602417,0.002945439874790568
53854,107709,107708,215417,1.9331791400909424,0.002933322646676077
53954,107909,107908,215817,1.9367790222167969,0.0029212552675564546
54054,108109,108108,216217,1.9405491352081299,0.002909237532358191
54154,108309,108308,216617,1.9439001083374023,0.002897269236851446
54254,108509,108508,217017,1.9481201171875,0.0028853501776465677
54354,108709,108708,217417,1.9516632556915283,0.0028734801521906176
54454,108909,108908,217817,1.9552791118621826,0.0028616589587639393
54555,109111,109110,218221,1.959618091583252,0.0028497689157634975
54655,109311,109310,218621,1.9631149768829346,0.0028380452678556027
54755,109511,109510,219021,1.967061996459961,0.002826369849795231
54855,109711,109710,219421,1.9708402156829834,0.002814742463169884
54955,109911,109910,219821,1.9745569229125977,0.002803162910383327
55055,110111,110110,220221,1.9780240058898926,0.0027916309946521838
55155,110311,110310,220621,1.9821200370788574,0.0027801465200026636
55255,110511,110510,221021,1.9857470989227295,0.002768709291267182
55355,110711,110710,221421,1.9899482727050781,0.002757319114081033
55455,110911,110910,221821,1.9941010475158691,0.0027459757948791255
55556,111113,111112,222225,2.0013041496276855,0.00273456640936194
55656,111313,111312,222625,2.005862236022949,0.0027233166923807577
55756,111513,111512,223025,2.0100719928741455,0.0027121132555454016
55856,111713,111712,223425,2.0153143405914307,0.002700955908464218
55956,111913,111912,223825,2.019813060760498,0.0026898444615288527
56056,112113,112112,224225,2.024792194366455,0.002678778725910949
56156,112313,112312,224625,2.029158115386963,0.0026677585135589927
56256,112513,112512,225025,2.0339109897613525,0.002656783637195071
56356,112713,112712,225425,2.0382111072540283,0.0026458539103117354
56456,112913,112912,225825,2.0431690216064453,0.002634969147168808
56557,113115,113114,226229,2.0473852157592773,0.0026240209884552273
56657,113315,113314,226629,2.052417039871216,0.0026132260436435933
56757,113515,113514,227029,2.0580930709838867,0.0026024755080931777
56857,113715,113714,227429,2.06246018409729,0.002591769199108963
56957,113915,113914,227829,2.067472219467163,0.0025811069347475447
57057,114115,114114,228229,2.0722429752349854,0.002570488533813974
57157,114315,114314,228629,2.0774521827697754,0.002559913815858767
57257,114515,114514,229029,2.082533121109009,0.002549382601174776
57357,114715,114714,229429,2.088052988052368,0.0025388947107941365
57457,114915,114914,229829,2.093203067779541,0.0025284499664852606
57558,115117,115116,230233,2.098886251449585,0.002517944389384992
57658,115317,115316,230633,2.103379011154175,0.002507585832482533
57758,115517,115516,231033,2.1084799766540527,0.002497269889587577
57858,115717,115716,231433,2.112950086593628,0.002486996385390603
57958,115917,115916,231833,2.1177260875701904,0.002476765145303307
58058,116117,116116,232233,2.121906280517578,0.0024665759954555846
58158,116317,116316,232633,2.1262261867523193,0.002456428762692665
58258,116517,116516,233033,2.130425214767456,0.002446323274572094
58358,116717,116716,233433,2.1346209049224854,0.0024362593593608246
58458,116917,116916,233833,2.1389319896698,0.00242623684603231
58559,117119,117118,234237,2.143961191177368,0.0024161559590907575
58659,117319,117318,234637,2.148271083831787,0.0024062161490246686
58759,117519,117518,235037,2.152677059173584,0.0023963172302858896
58859,117719,117718,235437,2.1570801734924316,0.0023864590346518114
58959,117919,117918,235837,2.161283016204834,0.0023766413945919148
59059,118119,118118,236237,2.165497064590454,0.0023668641432648277
59159,118319,118318,236637,2.169724225997925,0.0023571271145156024
59259,118519,118518,237037,2.174208164215088,0.0023474301428727863
59359,118719,118718,237437,2.1784660816192627,0.002337773063545691
59459,118919,118918,237837,2.1825451850891113,0.0023281557124215464
59560,119121,119120,238241,2.1863012313842773,0.0023184823474499345
59660,119321,119320,238641,2.1897451877593994,0.002308944356291497
59760,119521,119520,239041,2.1931309700012207,0.0022994456034198755
59860,119721,119720,239441,2.1969032287597656,0.002289985927412913
59960,119921,119920,239841,2.200469970703125,0.0022805651675125134
60060,120121,120120,240241,2.2039191722869873,0.0022711831636219463
60160,120321,120320,240641,2.207259178161621,0.0022618397563030795
60260,120521,120520,241041,2.2105820178985596,0.0022525347867736975
60360,120721,120720,241441,2.2141501903533936,0.0022432680969048063
60460,120921,120920,241841,2.2175660133361816,0.0022340395292179192
60561,121123,121122,242245,2.220975160598755,0.002224757212055106
60661,121323,121322,242645,2.224339008331299,0.0022156047961906537
60761,121523,121522,243045,2.227703094482422,0.0022064900323970297
60861,121723,121722,243445,2.2316291332244873,0.0021974127657776177
60961,121923,121922,243845,2.2350571155548096,0.002188372842073003
61061,122123,122122,244245,2.2385010719299316,0.002179370107658379
61161,122323,122322,244645,2.2418339252471924,0.0021704044095409553
61261,122523,122522,245045,2.2451388835906982,0.002161475595357307
61361,122723,122722,245445,2.2484662532806396,0.002152583513370839
61461,122923,122922,245845,2.2519149780273438,0.002143728012469163
61562,123125,123124,246249,2.2553012371063232,0.002134820934925411
61662,123325,123324,246649,2.2586512565612793,0.002126038507392765
61762,123525,123524,247049,2.262040138244629,0.002117292209838103
61862,123725,123724,247449,2.265519142150879,0.002108581893626524
61962,123925,123924,247849,2.269213914871216,0.0020999074107345707
62062,124125,124124,248249,2.2726690769195557,0.0020912686137477534
62162,124325,124324,248649,2.276052951812744,0.0020826653558580453
62262,124525,124524,249049,2.279412031173706,0.0020740974908613615
62362,124725,124724,249449,2.282963991165161,0.0020655648731550767
62462,124925,124924,249849,2.2864298820495605,0.002057067357735554
62563,125127,125126,250253,2.2908661365509033,0.002048520350670511
62663,125327,125326,250653,2.294239044189453,0.002040092954613752
62763,125527,125526,251053,2.2976021766662598,0.0020317002279730155
62863,125727,125726,251453,2.301054000854492,0.002023342028122002
62963,125927,125926,251853,2.304435968399048,0.002015018213021156
63063,126127,126126,252253,2.3078153133392334,0.0020067286412152655
63163,126327,126326,252653,2.3112142086029053,0.0019984731718310084
63263,126527,126526,253053,2.3145651817321777,0.001990251664574641
63363,126727,126726,253453,2.3179168701171875,0.0019820639797295697
63463,126927,126926,253853,2.321321964263916,0.001973909978153963
63564,127129,127128,254257,2.3248131275177,0.0019657084856429846
63664,127329,127328,254657,2.328119993209839,0.0019576217688401843
63764,127529,127528,255057,2.3314261436462402,0.0019495683199349915
63864,127729,127728,255457,2.334721088409424,0.001941548002066804
63964,127929,127928,255857,2.3380191326141357,0.001933560678938055
64064,128129,128128,256257,2.3413331508636475,0.0019256062148118587
64164,128329,128328,256657,2.3446362018585205,0.0019176844745097572
64264,128529,128528,257057,2.3479490280151367,0.001909795323409397
64364,128729,128728,257457,2.351149082183838,0.0019019386274422444
64464,128929,128928,257857,2.3543570041656494,0.0018941142530913338
64565,129131,129130,258261,2.3576080799102783,0.0018862443076360902
64665,129331,129330,258661,2.360812187194824,0.0018784844980569133
64765,129531,129530,259061,2.3640151023864746,0.0018707566115136087
64865,129731,129730,259461,2.3672173023223877,0.0018630605166781858
64965,129931,129930,259861,2.370413064956665,0.001855396082762924
65065,130131,130130,260261,2.3736250400543213,0.00184776317951815
65165,130331,130330,260661,2.3768341541290283,0.0018401616772300232
65265,130531,130530,261061,2.3805601596832275,0.001832591446718308
65365,130731,130730,261461,2.383810043334961,0.0018250523593342407
65465,130931,130930,261861,2.3870902061462402,0.0018175442869582783
65566,131133,131132,262265,2.3903801441192627,0.001809992485699441
65666,131333,131332,262665,2.3936309814453125,0.0018025463680507784
65766,131533,131532,263065,2.396876096725464,0.001795130882942572
65866,131733,131732,263465,2.4001190662384033,0.0017877459043557924
65966,131933,131932,263865,2.4033751487731934,0.0017803913067898248
66066,132133,132132,264265,2.406642198562622,0.0017730669652603658
66166,132333,132332,264665,2.410228967666626,0.0017657727552972784
66266,132533,132532,265065,2.41359806060791,0.0017585085529425069
66366,132733,132732,265465,2.4168620109558105,0.0017512742347479118
66466,132933,132932,265865,2.4203851222991943,0.0017440696777732204
66567,133135,133134,266269,2.4237101078033447,0.001736823159664914
66667,133335,133334,266669,2.426983118057251,0.0017296780528846538
66767,133535,133534,267069,2.430253028869629,0.0017225623403179775
66867,133735,133734,267469,2.4336190223693848,0.0017154759010401923
66967,133935,133934,267869,2.437106132507324,0.0017084186146240808
67067,134135,134134,268269,2.4403631687164307,0.0017013903611378695
67167,134335,134334,268669,2.443641185760498,0.001694391021143133
67267,134535,134534,269069,2.446883201599121,0.0016874204756928367
67367,134735,134734,269469,2.450119972229004,0.0016804786063292691
67467,134935,134934,269869,2.453352928161621,0.0016735652950820312
67568,135137,135136,270273,2.4566662311553955,0.001666611718988814
67668,135337,135336,270673,2.4599223136901855,0.0016597554546494539
67768,135537,135536,271073,2.4635610580444336,0.0016529273962564194
67868,135737,135736,271473,2.4674952030181885,0.001646127427773425
67968,135937,135936,271873,2.4711360931396484,0.0016393554336415486
68068,136137,136136,272273,2.4750571250915527,0.001632611298777284
68168,136337,136336,272673,2.4790589809417725,0.0016258949085705442
68268,136537,136536,273073,2.482680082321167,0.001619206148882733
68368,136737,136736,273473,2.4865872859954834,0.001612544906044839
68468,136937,136936,273873,2.4904398918151855,0.0016059110668554268
68569,137139,137138,274277,2.4937491416931152,0.0015992385905348953
68669,137339,137338,274677,2.497007131576538,0.0015926594921201371
68769,137539,137538,275077,2.5004310607910156,0.0015861074594204127
68869,137739,137738,275477,2.503737211227417,0.0015795823810902084
68969,137939,137938,275877,2.5070059299468994,0.0015730841462421178
69069,138139,138138,276277,2.510535955429077,0.0015666126444448963
69169,138339,138338,276677,2.5141451358795166,0.0015601677657215997
69269,138539,138538,277077,2.517402172088623,0.0015537494005477077
69369,138739,138738,277477,2.520659923553467,0.0015473574398492983
69469,138939,138938,277877,2.524022102355957,0.0015409917750011423
69570,139141,139140,278281,2.527338981628418,0.0015345890349359838
69670,139341,139340,278681,2.5305771827697754,0.0015282758979551663
69770,139541,139540,279081,2.5338480472564697,0.001521988732552163
69870,139741,139740,279481,2.537118911743164,0.0015157274318826548
69970,139941,139940,279881,2.5403411388397217,0.0015094918895418635
70070,140141,140140,280281,2.543729305267334,0.0015032819995627511
70170,140341,140340,280681,2.5477402210235596,0.0014970976564141962
70270,140541,140540,281081,2.551131248474121,0.001490938754999273
70370,140741,140740,281481,2.5557761192321777,0.0014848051906533562
70470,140941,140940,281881,2.559143304824829,0.0014786968591424235
70571,141143,141142,282285,2.5625059604644775,0.0014725529511879349
70671,141343,141342,282685,2.5659070014953613,0.0014664950240942938
70771,141543,141542,283085,2.569425106048584,0.0014604620186719783
70871,141743,141742,283485,2.5727570056915283,0.001454453832395876
70971,141943,141942,283885,2.576066017150879,0.00144847036316264
71071,142143,142142,284285,2.5793821811676025,0.0014425115092889865
71171,142343,142342,284685,2.58274507522583,0.0014365771695099103
71271,142543,142542,285085,2.586076259613037,0.0014306672429770244
71371,142743,142742,285485,2.589564323425293,0.0014247816292568235
71471,142943,142942,285885,2.593600034713745,0.0014189202283289575
71572,143145,143144,286289,2.597100019454956,0.0014130246891427183
71672,143345,143344,286689,2.6006901264190674,0.0014072116550229877
71772,143545,143544,287089,2.6042091846466064,0.001401422535110811
71872,143745,143744,287489,2.607793092727661,0.001395657231025652
71972,143945,143944,287889,2.6116490364074707,0.0013899156447917012
72072,144145,144144,288289,2.6156511306762695,0.0013841976788362704
72172,144345,144344,288689,2.6201159954071045,0.0013785032359880003
72272,144545,144544,289089,2.624691963195801,0.001372832219475324
72372,144745,144744,289489,2.629149913787842,0.001367184532924772
72472,144945,144944,289889,2.633350133895874,0.001361560080359351
72573,145147,145146,290293,2.637892246246338,0.0013559028695818089
72673,145347,145346,290693,2.6423659324645996,0.0013503248285861524
72773,145547,145546,291093,2.6466989517211914,0.0013447697350611769
72873,145747,145746,291493,2.651041030883789,0.001339237494603421
72973,145947,145946,291893,2.6552491188049316,0.001333728013197769
73073,146147,146146,292293,2.6596250534057617,0.0013282411972158998
73173,146347,146346,292693,2.6637370586395264,0.0013227769534146663
73273,146547,146546,293093,2.667600154876709,0.0013173351889344982
73373,146747,146746,293493,2.6709721088409424,0.0013119158112978406
73473,146947,146946,293893,2.674309253692627,0.0013065187284075806
73574,147149,147148,294297,2.6776750087738037,0.0013010902115628044
73674,147349,147348,294697,2.6810190677642822,0.0012957376640448696
73774,147549,147548,295097,2.684554100036621,0.0012904071363412947
73874,147749,147748,295497,2.687933921813965,0.0012850985378648904
73974,147949,147948,295897,2.691317081451416,0.0012798117784011552
74074,148149,148148,296297,2.694671154022217,0.0012745467681066836
74174,148349,148348,296697,2.6980249881744385,0.001269303417507698
74274,148549,148548,297097,2.70145320892334,0.0012640816374985138
74374,148749,148748,297497,2.704846143722534,0.0012588813393399842
74474,148949,148948,297897,2.708214044570923,0.0012537024346580565
74575,149151,149150,298301,2.7117602825164795,0.001248493366745823
74675,149351,149350,298701,2.715097188949585,0.0012433571970844517
74775,149551,149550,299101,2.718459129333496,0.0012382421570818233
74875,149751,149750,299501,2.7219130992889404,0.0012331481598127723
74975,149951,149950,299901,2.7253172397613525,0.0012280751187097034
75075,150151,150150,300301,2.7287330627441406,0.0012230229475611747
75175,150351,150350,300701,2.732131004333496,0.0012179915605103951
75275,150551,150550,301101,2.735558271408081,0.001212980872053783
75375,150751,150750,301501,2.7389490604400635,0.0012079907970395229
75475,150951,150950,301901,2.742333173751831,0.0012030212506660963
75576,151153,151152,302305,2.745809316635132,0.0011980227604172593
75676,151353,151352,302705,2.749169111251831,0.0011930942214922022
75776,151553,151552,303105,2.7524731159210205,0.0011881859580550004
75876,151753,151752,303505,2.7559030055999756,0.001183297886694451
75976,151953,151952,303905,2.7592849731445312,0.001178429924342487
76076,152153,152152,304305,2.7629730701446533,0.0011735819882727528
76176,152353,152352,304705,2.7662951946258545,0.0011687539960992717
76276,152553,152552,305105,2.7698750495910645,0.0011639458657749313
76376,152753,152752,305505,2.7739388942718506,0.0011591575155902255
76476,152953,152952,305905,2.777735948562622,0.001154388864171719
76577,153155,153154,306309,2.7817232608795166,0.0011495924389400586
76677,153355,153354,306709,2.7859652042388916,0.001144863137235229
76777,153555,153554,307109,2.7902262210845947,0.001140153291377413
76877,153755,153754,307509,2.794365167617798,0.0011354628213273007
76977,153955,153954,307909,2.798495054244995,0.0011307916473748854
77077,154155,154154,308309,2.802588939666748,0.0011261396901380532
77177,154355,154354,308709,2.8071680068969727,0.0011215068705612604
77277,154555,154554,309109,2.811337947845459,0.0011168931099141952
77377,154755,154754,309509,2.815206289291382,0.0011122983297904595
77477,154955,154954,309909,2.818751096725464,0.0011077224521061743
77578,155157,155156,310313,2.8228821754455566,0.0011031199233709635
77678,155357,155356,310713,2.8266103267669678,0.0010985818046799188
77778,155557,155556,311113,2.829935073852539,0.0010940623553291973
77878,155757,155756,311513,2.833252191543579,0.0010895614985150842
77978,155957,155956,311913,2.836679220199585,0.0010850791577498718
78078,156157,156156,312313,2.84074330329895,0.001080615256860472
78178,156357,156356,312713,2.8440821170806885,0.0010761697199872051
78278,156557,156556,313113,2.847403049468994,0.0010717424715824412
78378,156757,156756,313513,2.850788116455078,0.0010673334364093585
78478,156957,156956,313913,2.8543732166290283,0.0010629425395406503
78579,157159,157158,314317,2.8588011264801025,0.0010585260689953125
78679,157359,157358,314717,2.862999200820923,0.001054171404704609
78779,157559,157558,315117,2.866610288619995,0.0010498346550422174
78879,157759,157758,315517,2.8699920177459717,0.0010455157463092463
78979,157959,157958,315917,2.8745391368865967,0.0010412146051100048
79079,158159,158158,316317,2.8778440952301025,0.0010369311583507488
79179,158359,158358,316717,2.8823111057281494,0.0010326653332384033
79279,158559,158558,317117,2.8857672214508057,0.0010284170572793824
79379,158759,158758,317517,2.890029191970825,0.0010241862582783293
79479,158959,158958,317917,2.893334150314331,0.0010199728643369079
79580,159161,159160,318321,2.8966519832611084,0.0010157349305401128
79680,159361,159360,318721,2.900031089782715,0.0010115563044671315
79780,159561,159560,319121,2.9033701419830322,0.0010073948688198546
79880,159761,159760,319521,2.9081809520721436,0.0010032505528786693
79980,159961,159960,319921,2.9125571250915527,0.000999123286214956
80080,160161,160160,320321,2.9164040088653564,0.0009950129986897663
80180,160361,160360,320721,2.9206771850585938,0.0009909196204527177
80280,160561,160560,321121,2.925488233566284,0.0009868430819407832
80380,160761,160760,321521,2.9293131828308105,0.0009827833138771347
80480,160961,160960,321921,2.9334352016448975,0.0009787402472699015
80581,161163,161162,322325,2.938805103302002,0.0009746736328361112
80681,161363,161362,322725,2.9430739879608154,0.0009706639285989526
80781,161563,161562,323125,2.947453260421753,0.0009666707198609293
80881,161763,161762,323525,2.951794147491455,0.0009626939387612899
80981,161963,161962,323925,2.956806182861328,0.0009587335177184958
81081,162163,162162,324325,2.961050271987915,0.0009547893894289958
81181,162363,162362,324725,2.9654541015625,0.0009508614868661091
81281,162563,162562,325125,2.9696240425109863,0.0009469497432789391
81381,162763,162762,325525,2.973743200302124,0.0009430540921911496
81481,162963,162962,325925,2.977874994277954,0.0009391744673998846
81582,163165,163164,326329,2.9822750091552734,0.000935272246707893
81682,163365,163364,326729,2.986279249191284,0.0009314246356059012
81782,163565,163564,327129,2.9905941486358643,0.0009275928531690238
81882,163765,163764,327529,2.994692087173462,0.0009237768342798167
81982,163965,163964,327929,2.998950242996216,0.0009199765140887116
82082,164165,164164,328329,3.002901077270508,0.0009161918280129229
82182,164365,164364,328729,3.006622076034546,0.0009124227117353531
82282,164565,164564,329129,3.0102710723876953,0.0009086691012035014
82382,164765,164764,329529,3.013606071472168,0.0009049309326283809
82482,164965,164964,329929,3.016956090927124,0.0009012081424833965
82583,165167,165166,330333,3.0203630924224854,0.0008974636698816971
82683,165367,165366,330733,3.0237560272216797,0.0008937715992658582
82783,165567,165566,331133,3.0270471572875977,0.0008900947174380366
82883,165767,165766,331533,3.030333995819092,0.0008864329619131639
82983,165967,165966,331933,3.033628225326538,0.000882786270463232
83083,166167,166166,332333,3.0369069576263428,0.0008791545811162163
83183,166367,166366,332733,3.040318012237549,0.0008755378321550661
83283,166567,166566,333133,3.043642044067383,0.0008719359621165982
83383,166767,166766,333533,3.0469470024108887,0.0008683489097905232
83483,166967,166966,333933,3.0502240657806396,0.0008647766142183077
83584,167169,167168,334337,3.0535261631011963,0.0008611835127072635
83684,167369,167368,334737,3.0568270683288574,0.000857640694820799
83784,167569,167568,335137,3.0600380897521973,0.0008541124517124077
83884,167769,167768,335537,3.063260316848755,0.0008505987234229927
83984,167969,167968,335937,3.066486120223999,0.0008470994502401269
84084,168169,168168,336337,3.069788932800293,0.0008436145726970179
84184,168369,168368,336737,3.0729970932006836,0.0008401440315715475
84284,168569,168568,337137,3.076198101043701,0.0008366877678851835
84384,168769,168768,337537,3.079393148422241,0.0008332457229020795
84484,168969,168968,337937,3.0825998783111572,0.0008298178381279802
84585,169171,169170,338341,3.085824966430664,0.0008263699884994855
84685,169371,169370,338741,3.0890181064605713,0.000822970389769486
84785,169571,169570,339141,3.092302083969116,0.0008195847766291025
84885,169771,169770,339541,3.095506191253662,0.0008162130915430944
84985,169971,169970,339941,3.09871506690979,0.0008128552772129153
85085,170171,170170,340341,3.1019420623779297,0.0008095112765757376
85185,170371,170370,340741,3.1051509380340576,0.0008061810328035038
85285,170571,170570,341141,3.1083619594573975,0.0008028644893019075
85385,170771,170770,341541,3.1115729808807373,0.0007995615897095013
85485,170971,170970,341941,3.114995002746582,0.0007962722778966719
85586,171173,171172,342345,3.1184189319610596,0.0007929638083128772
85686,171373,171372,342745,3.1216881275177,0.000789701639074892
85786,171573,171572,343145,3.125298261642456,0.0007864528900561255
85886,171773,171772,343545,3.128618001937866,0.0007832175060472207
85986,171973,171972,343945,3.131859064102173,0.0007799954320659252
86086,172173,172172,344345,3.1351330280303955,0.0007767866133561951
86186,172373,172372,344745,3.1384010314941406,0.0007735909953872531
86286,172573,172572,345145,3.1417040824890137,0.0007704085238526242
86386,172773,172772,345545,3.1453099250793457,0.0007672391446693147
86486,172973,172972,345945,3.1485209465026855,0.0007640828039767418
86587,173175,173174,346349,3.1524200439453125,0.0007609080799701154
86687,173375,173374,346749,3.155625104904175,0.0007577777846080904
86787,173575,173574,347149,3.1588239669799805,0.000754660366950111
86887,173775,173774,347549,3.1622681617736816,0.0007515557740186439
86987,173975,173974,347949,3.1656482219696045,0.0007484639530541494
87087,174175,174174,348349,3.169098138809204,0.0007453848515140839
87187,174375,174374,348749,3.1723880767822266,0.0007423184170720906
87287,174575,174574,349149,3.1756181716918945,0.0007392645976170561
87387,174775,174774,349549,3.179081916809082,0.0007362233412522726
87487,174975,174974,349949,3.1826329231262207,0.0007331945962945061
87588,175177,175176,350353,3.1859240531921387,0.0007301482111720159
87688,175377,175376,350753,3.189359188079834,0.0007271444586568655
87788,175577,175576,351153,3.192589044570923,0.0007241530632618487
87888,175777,175776,351553,3.1958820819854736,0.0007211739741510998
87988,175977,175976,351953,3.1996560096740723,0.0007182071406978532
88088,176177,176176,352353,3.203274965286255,0.0007152525124836574
88188,176377,176376,352753,3.2070131301879883,0.0007123100392974267
88288,176577,176576,353153,3.210604190826416,0.0007093796711346646
88388,176777,176776,353553,3.214548110961914,0.000706461358196588
88488,176977,176976,353953,3.2185442447662354,0.0007035550508892803
88589,177179,177178,354357,3.222343921661377,0.0007006318165245928
88689,177379,177378,354757,3.2264211177825928,0.0006977494913351491
88789,177579,177578,355157,3.230034112930298,0.0006948790237266729
88889,177779,177778,355557,3.2333950996398926,0.0006920203649183336
88989,177979,177978,355957,3.2384262084960938,0.0006891734663299825
89089,178179,178178,356357,3.2419471740722656,0.0006863382795813204
89189,178379,178378,356757,3.2452139854431152,0.0006835147564910646
89289,178579,178578,357157,3.2485060691833496,0.0006807028490761866
89389,178779,178778,357557,3.2518510818481445,0.0006779025095509966
89489,178979,178978,357957,3.255195140838623,0.0006751136903264208
89590,179181,179180,358361,3.2585642337799072,0.0006723086283243344
89690,179381,179380,358761,3.2619199752807617,0.0006695428217354923
89790,179581,179580,359161,3.265263080596924,0.0006667883933824186
89890,179781,179780,359561,3.268609046936035,0.0006640452964562696
89990,179981,179980,359961,3.2719459533691406,0.000661313484340747
90090,180181,180180,360361,3.2752912044525146,0.0006585929106113304
90190,180381,180380,360761,3.278651237487793,0.0006558835290344818
90290,180581,180580,361161,3.2820122241973877,0.0006531852935668883
90390,180781,180780,361561,3.2857160568237305,0.0006504981583546004
90490,180981,180980,361961,3.2890710830688477,0.0006478220777323728
90591,181183,181182,362365,3.2925779819488525,0.0006451304109503172
90691,181383,181382,362765,3.2959790229797363,0.0006424764126731859
90791,181583,181582,363165,3.2993359565734863,0.0006398333326642635
90891,181783,181782,363565,3.3026959896087646,0.000637201126006946
90991,181983,181982,363965,3.306140899658203,0.0006345797479694101
91091,182183,182182,364365,3.30950927734375,0.0006319691540038736
91191,182383,182382,364765,3.312934160232544,0.0006293692997457922
91291,182583,182582,365165,3.3162741661071777,0.0006267801410131619
91391,182783,182782,365565,3.319714069366455,0.0006242016338056925
91491,182983,182982,365965,3.3230340480804443,0.0006216337343041626
91592,183185,183184,366369,3.3263869285583496,0.0006190508787165712
91692,183385,183384,366769,3.3297040462493896,0.000616504168876702
91792,183585,183584,367169,3.3330130577087402,0.0006139679359317464
91892,183785,183784,367569,3.3363242149353027,0.0006114421367808764
91992,183985,183984,367969,3.3396451473236084,0.0006089267285005744
92092,184185,184184,368369,3.342949151992798,0.0006064216683438989
92192,184385,184384,368769,3.3463191986083984,0.0006039269137397423
92292,184585,184584,369169,3.349705934524536,0.0006014424222921702
92392,184785,184784,369569,3.3530590534210205,0.0005989681517796376
92492,184985,184984,369969,3.356401205062866,0.0005965040601543032
92593,185187,185186,370373,3.3600270748138428,0.0005940256170458203
92693,185387,185386,370773,3.3633511066436768,0.0005915818584856152
92793,185587,185586,371173,3.3673882484436035,0.0005891481532896432
92893,185787,185786,371573,3.3707871437072754,0.0005867244600994535
92993,185987,185986,371973,3.3745882511138916,0.0005843107377267003
93093,186187,186186,372373,3.3780171871185303,0.0005819069451524923
93193,186387,186386,372773,3.3814709186553955,0.0005795130415266957
93293,186587,186586,373173,3.3850691318511963,0.0005771289861672234
93393,186787,186786,373573,3.3884570598602295,0.0005747547385593525
93493,186987,186986,373973,3.3916900157928467,0.0005723902583550136
93594,187189,187188,374377,3.3949670791625977,0.0005700120068292604
93694,187389,187388,374777,3.398426055908203,0.0005676670377216321
93794,187589,187588,375177,3.4016671180725098,0.0005653317155688939
93894,187789,187788,375577,3.404902219772339,0.0005630060006845002
93994,187989,187988,375977,3.408151149749756,0.0005606898535451493
94094,188189,188188,376377,3.4113810062408447,0.0005583832347901581
94194,188389,188388,376777,3.4146649837493896,0.0005560861052207555
94294,188589,188588,377177,3.4179301261901855,0.0005537984257994406
94394,188789,188788,377577,3.4211649894714355,0.0005515201576493039
94494,188989,188988,377977,3.424391984939575,0.000549251262053377
94595,189191,189190,378381,3.4276559352874756,0.0005469691518445876
94695,189391,189390,378781,3.4308888912200928,0.0005447189786051994
94795,189591,189590,379181,3.4341330528259277,0.0005424780623405207
94895,189791,189790,379581,3.4373581409454346,0.0005402463649683385
94995,189991,189990,379981,3.4405839443206787,0.0005380238485631097
95095,190191,190190,380381,3.443808078765869,0.0005358104753552924
95195,190391,190390,380781,3.4470269680023193,0.0005336062077307536
95295,190591,190590,381181,3.45039701461792,0.0005314110082300831
95395,190791,190790,381581,3.453606128692627,0.0005292248395479789
95495,190991,190990,381981,3.456818103790283,0.0005270476645326075
95596,191193,191192,382385,3.4600601196289062,0.0005248578091078595
95696,191393,191392,382785,3.4632701873779297,0.0005226985995938372
95796,191593,191592,383185,3.4666340351104736,0.0005205482728393725
95896,191793,191792,383585,3.4700522422790527,0.0005184067923017403
95996,191993,191992,383985,3.473283052444458,0.0005162741215885456
96096,192193,192192,384385,3.4765000343322754,0.0005141502244571144
96196,192393,192392,384785,3.4797260761260986,0.0005120350648138418
96296,192593,192592,385185,3.4829602241516113,0.0005099286067136191
96396,192793,192792,385585,3.486358165740967,0.0005078308143592323
96496,192993,192992,385985,3.4895901679992676,0.0005057416521007108
96597,193195,193194,386389,3.4928929805755615,0.0005036403220410416
96697,193395,193394,386789,3.496135950088501,0.0005015683990246994
96797,193595,193594,387189,3.499389886856079,0.0004995049996805148
96897,193795,193794,387589,3.5027172565460205,0.0004974500889429897
96997,193995,193994,387989,3.506026029586792,0.0004954036318908944
97097,194195,194194,388389,3.5092689990997314,0.0004933655937466648
97197,194395,194394,388789,3.5125460624694824,0.0004913359398757927
97297,194595,194594,389189,3.515791177749634,0.0004893146357862796
97397,194795,194794,389589,3.519026279449463,0.000487301647128011
97497,194995,194994,389989,3.5223889350891113,0.0004852969396921588
97598,195197,195196,390393,3.525656223297119,0.00048328055634108214
97698,195397,195396,390793,3.528907060623169,0.00048129239124743264
97798,195597,195596,391193,3.532165050506592,0.00047931240525470335
97898,195797,195796,391593,3.5354251861572266,0.00047734056471492676
97998,195997,195996,391993,3.5386621952056885,0.0004753768361185795
98098,196197,196196,392393,3.5419399738311768,0.000473421186093979
98198,196397,196396,392793,3.5452489852905273,0.0004714735814067335
98298,196597,196596,393193,3.548583984375,0.00046953398895918826
98398,196797,196796,393593,3.5519039630889893,0.0004676023757898199
98498,196997,196996,393993,3.5551791191101074,0.00046567870907273816
98599,197199,197198,394397,3.558532238006592,0.0004637438384417335
98699,197399,197398,394797,3.5618250370025635,0.0004618360453391859
98799,197599,197598,395197,3.565160036087036,0.00045993610069567774
98899,197799,197798,395597,3.5684821605682373,0.0004580439722234852
98999,197999,197998,395997,3.5718300342559814,0.0004561596277677057
99099,198199,198198,396397,3.5751349925994873,0.00045428303530572464
99199,198399,198398,396797,3.578705310821533,0.000452414162946645
99299,198599,198598,397197,3.5820579528808594,0.000450552978930778
99399,198799,198798,397597,3.585475206375122,0.0004486994516291035
99499,198999,198998,397997,3.5888519287109375,0.0004468535495427096
99600,199201,199200,398401,3.592280149459839,0.000444996896462976
99700,199401,199400,398801,3.5956621170043945,0.00044316622629691983
99800,199601,199600,399201,3.5991601943969727,0.00044134308731430094
99900,199801,199800,399601,3.6024010181427,0.00043952744853262976
100000,200001,200000,400001,3.606074094772339,0.00043771927909687125


==> plot_data/quadratic_minimax_problem_n20_alpha0/flex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.985664367675781e-05,4.387061074692293
3,11,0,11,0.0006079673767089844,3.4741628962390445
6,24,0,24,0.0011477470397949219,2.033263258797766
8,32,0,32,0.0014929771423339844,1.5522093526709104
11,43,0,43,0.0019519329071044922,0.9650411560238331
14,56,0,56,0.0024890899658203125,0.6482458383208611
17,67,0,67,0.0029799938201904297,0.39693923901169775
20,80,0,80,0.0040760040283203125,0.27680455314284697
23,91,0,91,0.0047149658203125,0.20419425627261448
25,99,0,99,0.0052318572998046875,0.15265852588613407
28,110,0,110,0.006076812744140625,0.0957299899463542
31,124,0,124,0.006824970245361328,0.0894349852981967
34,137,0,137,0.00745081901550293,0.07677925190745234
37,152,0,152,0.0080718994140625,0.0723100619282481
39,161,0,161,0.008491992950439453,0.06988901781410752
42,176,0,176,0.009246826171875,0.06667845344878436
45,191,0,191,0.009894847869873047,0.06472750147395719
48,205,0,205,0.010663747787475586,0.062263640228154726
51,220,0,220,0.011297941207885742,0.06011079359259012
53,230,0,230,0.011838912963867188,0.0591534071850047
56,245,0,245,0.013303995132446289,0.058124715525270716
59,260,0,260,0.014185905456542969,0.05738350575689567
62,274,0,274,0.014801740646362305,0.05606359877987347
65,289,0,289,0.015417814254760742,0.054133236053776436
68,303,0,303,0.01601099967956543,0.052136238317722676
70,312,0,312,0.01639699935913086,0.04865143368456347
73,326,0,326,0.016981840133666992,0.04626360920109495
76,341,0,341,0.017714738845825195,0.044773326928866174
79,356,0,356,0.01866006851196289,0.04379514667363227
82,371,0,371,0.019322872161865234,0.04310283378045328
84,381,0,381,0.019749879837036133,0.04273835653747295
87,396,0,396,0.020467758178710938,0.04228519146178645
90,410,0,410,0.021309852600097656,0.03966934966391387
93,425,0,425,0.022249937057495117,0.038816030745483156
96,439,0,439,0.023055076599121094,0.03599933450388453
99,454,0,454,0.023736953735351562,0.035486005928600885
101,464,0,464,0.024135828018188477,0.035253876471242604
104,478,0,478,0.024715900421142578,0.03426594091783847
107,493,0,493,0.025307893753051758,0.03334683373825475
110,508,0,508,0.025937795639038086,0.03282104627138537
113,523,0,523,0.02652287483215332,0.0324995592738787
115,533,0,533,0.02690601348876953,0.03234898135129565
118,548,0,548,0.02751302719116211,0.03217875120664512
121,563,0,563,0.028342008590698242,0.03204913635210186
124,578,0,578,0.02912306785583496,0.03194368632734536
127,593,0,593,0.02972698211669922,0.03185352886552249
129,602,0,602,0.03012704849243164,0.03135583217504798
132,615,0,615,0.030731916427612305,0.02949416170223632
135,629,0,629,0.03130006790161133,0.028598796880318737
138,644,0,644,0.03194689750671387,0.02769540070249711
141,659,0,659,0.03253293037414551,0.0271178643751746
144,674,0,674,0.03310894966125488,0.02672647502178294
146,684,0,684,0.033490896224975586,0.02652995274857543
149,699,0,699,0.03407406806945801,0.026298164672867236
152,714,0,714,0.034648895263671875,0.026118140915158055
155,729,0,729,0.03522300720214844,0.02597344358746509
158,744,0,744,0.0357968807220459,0.0258540949835161
160,754,0,754,0.03617978096008301,0.02578536994673653
163,769,0,769,0.036766767501831055,0.025695190573519256
166,784,0,784,0.037323951721191406,0.025617604874861144
169,799,0,799,0.037899017333984375,0.025550178350329505
172,814,0,814,0.03871893882751465,0.025491085489001135
175,829,0,829,0.03944277763366699,0.0254389174760374
177,839,0,839,0.0398409366607666,0.02540742712246746
180,854,0,854,0.040428876876831055,0.025364439726939768
183,869,0,869,0.041046857833862305,0.025325870953955235
186,884,0,884,0.04163503646850586,0.02529108241652566
189,899,0,899,0.04220271110534668,0.02525954534023171
191,909,0,909,0.042578935623168945,0.025240105965788188
194,924,0,924,0.043138980865478516,0.025213042563610163
197,939,0,939,0.04374074935913086,0.02518820384732891
200,954,0,954,0.04438185691833496,0.02516530905747868
203,969,0,969,0.04492378234863281,0.02514411911627242
205,979,0,979,0.04527688026428223,0.025130837428951575
208,994,0,994,0.04580092430114746,0.025112049125038345
211,1009,0,1009,0.04630398750305176,0.025094482567631454
214,1024,0,1024,0.04681396484375,0.025078000671437676
217,1039,0,1039,0.04729175567626953,0.02506248470147327
220,1054,0,1054,0.047831058502197266,0.025047831495011625
222,1064,0,1064,0.04819202423095703,0.02503849712182878
225,1079,0,1079,0.04867076873779297,0.02502508773093823
228,1094,0,1094,0.04916977882385254,0.025012325714159102
231,1109,0,1109,0.049626827239990234,0.025000147888817076
234,1124,0,1124,0.05008983612060547,0.024988498615965728
236,1134,0,1134,0.05040097236633301,0.024981001572740483
239,1149,0,1149,0.05086088180541992,0.0249701268596274
242,1164,0,1164,0.05140089988708496,0.024959661833938687
245,1179,0,1179,0.05191969871520996,0.02494957078499455
248,1194,0,1194,0.052391767501831055,0.024939821879930334
251,1209,0,1209,0.052865028381347656,0.02493038667256916
253,1219,0,1219,0.053177833557128906,0.0249242581168589
256,1234,0,1234,0.05364871025085449,0.024915290412866224
259,1249,0,1249,0.05411887168884277,0.024906574083800367
262,1264,0,1264,0.05458879470825195,0.02489808991443535
265,1279,0,1279,0.05506491661071777,0.02488982054909124
267,1289,0,1289,0.05537676811218262,0.024884419154833293
270,1304,0,1304,0.05593085289001465,0.024876473615579844
273,1319,0,1319,0.0563960075378418,0.024868704156350077
276,1334,0,1334,0.056860923767089844,0.02486109861678486
279,1349,0,1349,0.05736494064331055,0.024853645911718306
281,1359,0,1359,0.05793404579162598,0.024848757314232695
284,1374,0,1374,0.05865287780761719,0.024841537267833752
287,1389,0,1389,0.05913686752319336,0.024834444935688718
290,1404,0,1404,0.059593915939331055,0.024827472307222744
293,1419,0,1419,0.0600588321685791,0.024820612024042597
296,1434,0,1434,0.060545921325683594,0.024813857317037228
298,1444,0,1444,0.06086397171020508,0.024809409732708496
301,1459,0,1459,0.06146502494812012,0.024802817369745846
304,1474,0,1474,0.06203794479370117,0.024796315007519106
307,1489,0,1489,0.06258678436279297,0.02478989760439496
310,1504,0,1504,0.06308388710021973,0.024783560494637768
312,1514,0,1514,0.06339788436889648,0.02477937821432344
315,1529,0,1529,0.06386876106262207,0.024773165476567483
318,1544,0,1544,0.0644829273223877,0.024767022187932582
321,1559,0,1559,0.06518077850341797,0.02476094480347465
324,1574,0,1574,0.06585383415222168,0.024754930026306847
327,1589,0,1589,0.0663900375366211,0.02474897478731834
329,1599,0,1599,0.06671404838562012,0.0247450362844543
332,1614,0,1614,0.06735777854919434,0.02473917401667633
335,1629,0,1629,0.06790971755981445,0.024733364081948886
338,1644,0,1644,0.06850886344909668,0.024727604101530513
341,1659,0,1659,0.06901979446411133,0.024721891851965633
343,1669,0,1669,0.06936383247375488,0.02471810917000097
346,1684,0,1684,0.06983184814453125,0.024712471915575854
349,1699,0,1699,0.07029986381530762,0.024706877135234666
352,1714,0,1714,0.07077288627624512,0.024701323081194042
355,1729,0,1729,0.07132887840270996,0.02469580811378722
357,1739,0,1739,0.07188868522644043,0.024692152419549543
360,1754,0,1754,0.07245993614196777,0.02468669922191886
363,1769,0,1769,0.07293200492858887,0.024681281209452247
366,1784,0,1784,0.07346510887145996,0.024675897076540262
369,1799,0,1799,0.07426977157592773,0.024670545594156646
372,1814,0,1814,0.07475090026855469,0.02466522560454406
374,1824,0,1824,0.07506394386291504,0.024661695899235385
377,1839,0,1839,0.07552981376647949,0.02465642600297453
380,1854,0,1854,0.07602572441101074,0.024651184824451968
383,1869,0,1869,0.07649683952331543,0.024645971428046688
386,1884,0,1884,0.07697081565856934,0.024640784929513486
388,1894,0,1894,0.07741999626159668,0.02463734179223725
391,1908,0,1908,0.0779118537902832,0.02425857612550655
394,1921,0,1921,0.07836484909057617,0.021533031711729222
397,1933,0,1933,0.07893586158752441,0.020698134118432476
400,1944,0,1944,0.07949090003967285,0.008007824111302573
403,1956,0,1956,0.07993793487548828,0.004547834043511745
405,1963,0,1963,0.08021688461303711,0.004101530885530421
408,1976,0,1976,0.08076167106628418,0.003702841073098849
411,1989,0,1989,0.08130979537963867,0.0032970324091014433
414,2001,0,2001,0.08182501792907715,0.0025450657237090766
417,2014,0,2014,0.08262276649475098,0.00220973849520187
419,2023,0,2023,0.08308601379394531,0.002073723942848947
422,2037,0,2037,0.0839080810546875,0.0018195650601700558
425,2048,0,2048,0.08455491065979004,0.0015214498210473115
428,2062,0,2062,0.08523893356323242,0.0013508347226733513
431,2077,0,2077,0.08629179000854492,0.001207069572147657
433,2086,0,2086,0.08687472343444824,0.001094651560872261
436,2099,0,2099,0.08754777908325195,0.0009711085179419887
439,2113,0,2113,0.08809804916381836,0.0009015208564362566
442,2126,0,2126,0.08882880210876465,0.0008087831409044648
445,2139,0,2139,0.08974790573120117,0.0007193114120497419
448,2152,0,2152,0.09026288986206055,0.0005630538695601275
450,2162,0,2162,0.09060978889465332,0.0005196780929800157
453,2176,0,2176,0.09106564521789551,0.00044701962085520454
456,2190,0,2190,0.09151792526245117,0.0003921332285953227
459,2205,0,2205,0.09198594093322754,0.0003683139054069744
462,2220,0,2220,0.09244990348815918,0.0003509344481207514
464,2230,0,2230,0.09275698661804199,0.0003417349195812294
467,2244,0,2244,0.09320592880249023,0.0003163611117141438
470,2259,0,2259,0.09367799758911133,0.0003026315136456489
473,2274,0,2274,0.09416604042053223,0.00029285485163113074
476,2288,0,2288,0.09461808204650879,0.00028048113290541363
479,2303,0,2303,0.09508180618286133,0.0002708117098618962
481,2313,0,2313,0.09539294242858887,0.00026580047979549057
484,2327,0,2327,0.09584474563598633,0.00024802594733156624
487,2341,0,2341,0.09629678726196289,0.0002375704954349332
490,2356,0,2356,0.09676575660705566,0.00023003512579139744
493,2370,0,2370,0.09721899032592773,0.00021823060852090652
495,2380,0,2380,0.09753274917602539,0.00021449641183912544
498,2395,0,2395,0.09800076484680176,0.00021048151470706844
501,2408,0,2408,0.09853696823120117,0.0001991828081748395
504,2423,0,2423,0.09923601150512695,0.00019002361184008545
507,2437,0,2437,0.09992194175720215,0.00017853159588839053
509,2447,0,2447,0.10033392906188965,0.00017537599522289416
512,2462,0,2462,0.10082197189331055,0.00017187365361581293
515,2477,0,2477,0.10130882263183594,0.0001692753905596409
518,2492,0,2492,0.10179686546325684,0.00016722076680375774
521,2506,0,2506,0.10230088233947754,0.00015722657261671137
524,2521,0,2521,0.10290098190307617,0.00015364080241469556
526,2531,0,2531,0.10326504707336426,0.00015203404690728063
529,2544,0,2544,0.10389089584350586,0.00014168781018389836
532,2559,0,2559,0.10452699661254883,0.0001351687674395318
535,2574,0,2574,0.10539007186889648,0.0001310270290919476
538,2589,0,2589,0.10609674453735352,0.00012824139523128953
540,2599,0,2599,0.1064918041229248,0.0001268486575808203
543,2614,0,2614,0.10708975791931152,0.00012520604373537895
546,2628,0,2628,0.10760998725891113,0.0001180379145258233
549,2642,0,2642,0.10808396339416504,0.00011115342987551249
552,2657,0,2657,0.10854291915893555,0.00010832397548732163
555,2672,0,2672,0.10901188850402832,0.00010657792598689384
557,2682,0,2682,0.10948705673217773,0.00010576021967873087
560,2696,0,2696,0.11023879051208496,0.00010264351523154555
563,2711,0,2711,0.11073589324951172,0.0001001674594696168
566,2726,0,2726,0.1115577220916748,9.870961917751572e-05
569,2741,0,2741,0.11240601539611816,9.78047198593085e-05
571,2751,0,2751,0.11299300193786621,9.73818264929344e-05
574,2766,0,2766,0.11369085311889648,9.691180391115723e-05
577,2781,0,2781,0.1143949031829834,9.656618028533662e-05
580,2796,0,2796,0.11501789093017578,9.62968596092095e-05
583,2811,0,2811,0.11579680442810059,9.60763743469509e-05
585,2821,0,2821,0.11628174781799316,9.594819392458769e-05
588,2836,0,2836,0.11702394485473633,9.577619943242469e-05
591,2851,0,2851,0.1175689697265625,9.562225972728403e-05
594,2865,0,2865,0.11805987358093262,9.233894708740227e-05
597,2880,0,2880,0.11855292320251465,9.074348250184262e-05
600,2895,0,2895,0.1190330982208252,8.98033451068699e-05
602,2905,0,2905,0.11936402320861816,8.938448390277437e-05
605,2920,0,2920,0.1202390193939209,8.894024604611798e-05
608,2935,0,2935,0.12123274803161621,8.863157896852904e-05
611,2950,0,2950,0.12193775177001953,8.840363147496694e-05
614,2965,0,2965,0.12269902229309082,8.822605488944881e-05
616,2975,0,2975,0.1232140064239502,8.812672739964085e-05
619,2990,0,2990,0.12382102012634277,8.799803275870952e-05
622,3005,0,3005,0.12435603141784668,8.788728924602006e-05
625,3020,0,3020,0.1248319149017334,8.77896732437476e-05
628,3035,0,3035,0.1257648468017578,8.770196816246733e-05
631,3050,0,3050,0.12661385536193848,8.762194495399807e-05
633,3060,0,3060,0.1272268295288086,8.757205531108966e-05
636,3075,0,3075,0.12804484367370605,8.750149341537334e-05
639,3090,0,3090,0.12880587577819824,8.743520810664194e-05
642,3105,0,3105,0.12946391105651855,8.737244436654954e-05
645,3120,0,3120,0.13013696670532227,8.731261013972552e-05
647,3130,0,3130,0.13046598434448242,8.727411138001614e-05
650,3145,0,3145,0.13097596168518066,8.721815835391431e-05
653,3160,0,3160,0.1314549446105957,8.716407070131462e-05
656,3175,0,3175,0.13193798065185547,8.711157767089571e-05
659,3190,0,3190,0.13241887092590332,8.706045611251313e-05
661,3200,0,3200,0.1327347755432129,8.70270443146247e-05
664,3215,0,3215,0.1332089900970459,8.697781298759961e-05
667,3230,0,3230,0.13371801376342773,8.692952567572587e-05
670,3245,0,3245,0.1342940330505371,8.688206778452041e-05
673,3260,0,3260,0.1349937915802002,8.683534295280606e-05
676,3275,0,3275,0.13564682006835938,8.678926992747992e-05
678,3285,0,3285,0.13616466522216797,8.675888232199677e-05
681,3300,0,3300,0.13687586784362793,8.671374826506103e-05
684,3315,0,3315,0.13753390312194824,8.666910531808103e-05
687,3330,0,3330,0.1380629539489746,8.662490913094082e-05
690,3345,0,3345,0.13854289054870605,8.658112192208818e-05
692,3355,0,3355,0.13887476921081543,8.655214153351362e-05
695,3370,0,3370,0.13937783241271973,8.650896662605235e-05
698,3385,0,3385,0.14002585411071777,8.646612470877439e-05
701,3400,0,3400,0.1406557559967041,8.642359443025714e-05
704,3415,0,3415,0.14171481132507324,8.638135742726899e-05
707,3430,0,3430,0.14247488975524902,8.63393978704527e-05
709,3440,0,3440,0.1428358554840088,8.631157213622939e-05
712,3455,0,3455,0.1433117389678955,8.627004550805357e-05
715,3470,0,3470,0.1438288688659668,8.622876377647581e-05
718,3485,0,3485,0.14430785179138184,8.618771755259032e-05
721,3500,0,3500,0.1448078155517578,8.614689863777933e-05
723,3510,0,3510,0.14529204368591309,8.611980872620727e-05
726,3525,0,3525,0.1458759307861328,8.607935313001347e-05
729,3540,0,3540,0.146345853805542,8.603910754978326e-05
732,3555,0,3555,0.14683008193969727,8.599906684234931e-05
735,3570,0,3570,0.14730191230773926,8.595922643557985e-05
737,3580,0,3580,0.14761590957641602,8.593277540835915e-05
740,3595,0,3595,0.14808893203735352,8.589325997278829e-05
743,3610,0,3610,0.14866876602172852,8.585393485315004e-05
746,3625,0,3625,0.14949703216552734,8.581479695827436e-05
749,3640,0,3640,0.15052580833435059,8.577584347731413e-05
752,3655,0,3655,0.15148282051086426,8.573707184096174e-05
754,3665,0,3665,0.15182209014892578,8.571132393462373e-05
757,3680,0,3680,0.15240478515625,8.567285021623055e-05
760,3695,0,3695,0.15304183959960938,8.563455243503083e-05
763,3710,0,3710,0.1535658836364746,8.5596428658544e-05
766,3725,0,3725,0.15405797958374023,8.555847707747548e-05
768,3735,0,3735,0.15438103675842285,8.553327084301889e-05
771,3750,0,3750,0.15485787391662598,8.549560251852483e-05
774,3765,0,3765,0.15547895431518555,8.545810205242587e-05
777,3780,0,3780,0.15604710578918457,8.542076796669812e-05
780,3795,0,3795,0.15656185150146484,8.538359884909064e-05
783,3809,0,3809,0.15703701972961426,8.473435597312562e-05
785,3819,0,3819,0.15735912322998047,8.369876746675917e-05
788,3832,0,3832,0.1578197479248047,8.083098532877663e-05
791,3847,0,3847,0.15830588340759277,7.773591605776785e-05
794,3861,0,3861,0.15877866744995117,7.20388194621843e-05
797,3874,0,3874,0.15922880172729492,6.430678467285645e-05
799,3882,0,3882,0.15961289405822754,5.481306974263296e-05
802,3894,0,3894,0.16024494171142578,4.216985394060329e-05
805,3908,0,3908,0.16080307960510254,3.906693535659981e-05
808,3922,0,3922,0.1612858772277832,3.5846347559104715e-05
811,3936,0,3936,0.1617567539215088,3.314690226320333e-05
813,3946,0,3946,0.16208577156066895,3.144026364469657e-05
816,3961,0,3961,0.16270780563354492,2.9468854605719053e-05
819,3974,0,3974,0.16321873664855957,2.8200070236143918e-05
822,3989,0,3989,0.16393280029296875,2.528968292881505e-05
825,4003,0,4003,0.16464686393737793,2.388522297227764e-05
828,4017,0,4017,0.16559481620788574,2.2163359595651447e-05
830,4027,0,4027,0.16631484031677246,2.0731018463800352e-05
833,4042,0,4042,0.16720890998840332,1.9232854480488476e-05
836,4055,0,4055,0.16805195808410645,1.7702385049621403e-05
839,4070,0,4070,0.1690218448638916,1.6356498608701972e-05
842,4084,0,4084,0.1700117588043213,1.547256757723561e-05
844,4093,0,4093,0.17043089866638184,1.5115075878595152e-05
847,4107,0,4107,0.1709890365600586,1.437964162442583e-05
850,4122,0,4122,0.17157697677612305,1.36901430520209e-05
853,4137,0,4137,0.17234301567077637,1.3227734809238349e-05
856,4152,0,4152,0.17300081253051758,1.289966438856974e-05
859,4167,0,4167,0.17353391647338867,1.2653142796433078e-05
861,4177,0,4177,0.17386174201965332,1.2518633594967207e-05
864,4192,0,4192,0.1743478775024414,1.2347643613453237e-05
867,4207,0,4207,0.17483091354370117,1.2203226882020337e-05
870,4222,0,4222,0.1753098964691162,1.2077982043050281e-05
873,4237,0,4237,0.17593789100646973,1.1967278115135325e-05
875,4247,0,4247,0.17632579803466797,1.1900019058838337e-05
878,4262,0,4262,0.1769850254058838,1.1807336176903783e-05
881,4277,0,4277,0.177825927734375,1.172309189721127e-05
884,4292,0,4292,0.17867588996887207,1.1646083575684098e-05
887,4307,0,4307,0.1791989803314209,1.1575387099841426e-05
889,4317,0,4317,0.1795177459716797,1.1531392716864084e-05
892,4332,0,4332,0.18009591102600098,1.146964319697035e-05
895,4347,0,4347,0.18074989318847656,1.1412510362149718e-05
898,4362,0,4362,0.18126893043518066,1.1359531551012257e-05
901,4377,0,4377,0.1817338466644287,1.1310304875178827e-05
904,4392,0,4392,0.1822209358215332,1.126447720130086e-05
906,4402,0,4402,0.18253087997436523,1.1235657773067644e-05
909,4417,0,4417,0.18299174308776855,1.1194816696832158e-05
912,4432,0,4432,0.18345069885253906,1.115661314084708e-05
915,4447,0,4447,0.18390870094299316,1.1120814464328493e-05
918,4462,0,4462,0.18436694145202637,1.1087211205686159e-05
920,4472,0,4472,0.18467283248901367,1.106593460143653e-05
923,4487,0,4487,0.1851329803466797,1.1035579396534396e-05
926,4502,0,4502,0.18559002876281738,1.1006954933179441e-05
929,4517,0,4517,0.18605375289916992,1.0979916359792147e-05
932,4531,0,4531,0.18650174140930176,1.0780917933850586e-05
935,4546,0,4546,0.18695974349975586,1.0517633952784924e-05
937,4556,0,4556,0.18726587295532227,1.0410789827685753e-05
940,4571,0,4571,0.187727689743042,1.0305912690208607e-05
943,4586,0,4586,0.18827009201049805,1.023795158638631e-05
946,4601,0,4601,0.18883991241455078,1.018956336381165e-05
949,4616,0,4616,0.1893470287322998,1.0152221591257449e-05
951,4626,0,4626,0.18966293334960938,1.0131235249953983e-05
954,4641,0,4641,0.19014286994934082,1.0103771370975127e-05
957,4656,0,4656,0.1906139850616455,1.0079835549198611e-05
960,4671,0,4671,0.19108200073242188,1.005852952156586e-05
963,4686,0,4686,0.19155287742614746,1.003928966140486e-05
965,4696,0,4696,0.1919569969177246,1.0027418684680486e-05
968,4711,0,4711,0.19248199462890625,1.0010834678464665e-05
971,4726,0,4726,0.19297575950622559,9.995523603870158e-06
974,4741,0,4741,0.19345998764038086,9.981311892237406e-06
977,4756,0,4756,0.19404387474060059,9.968060462798886e-06
980,4771,0,4771,0.19477176666259766,9.955655060284528e-06
982,4781,0,4781,0.1952366828918457,9.947806946623828e-06
985,4796,0,4796,0.19585490226745605,9.93660630500167e-06
988,4811,0,4811,0.1963350772857666,9.9260271944874e-06
991,4826,0,4826,0.19681406021118164,9.916006263364884e-06
994,4841,0,4841,0.19728779792785645,9.9064883326067e-06
996,4851,0,4851,0.1976029872894287,9.900398356717726e-06
999,4866,0,4866,0.19815802574157715,9.891614139317713e-06
1002,4881,0,4881,0.19867682456970215,9.883216257540906e-06
1005,4896,0,4896,0.1991569995880127,9.875169831447068e-06
1008,4911,0,4911,0.1996300220489502,9.86744378695498e-06
1011,4926,0,4926,0.20010590553283691,9.860010355060417e-06
1013,4936,0,4936,0.20042181015014648,9.855204900803382e-06
1016,4951,0,4951,0.2009139060974121,9.848205124829809e-06
1019,4966,0,4966,0.2013859748840332,9.841437084196024e-06
1022,4981,0,4981,0.20185494422912598,9.834882001577028e-06
1025,4996,0,4996,0.20232391357421875,9.828522920888324e-06
1027,5006,0,5006,0.20272088050842285,9.824384788681915e-06
1030,5021,0,5021,0.20326495170593262,9.818319014483997e-06
1033,5036,0,5036,0.20375967025756836,9.81241147299784e-06
1036,5051,0,5051,0.20423483848571777,9.806650342677701e-06
1039,5066,0,5066,0.20470976829528809,9.801024875451488e-06
1041,5076,0,5076,0.20502591133117676,9.797345064155639e-06
1044,5091,0,5091,0.20552277565002441,9.791924392360992e-06
1047,5106,0,5106,0.20599699020385742,9.786615178782104e-06
1050,5121,0,5121,0.20650291442871094,9.781409767545147e-06
1053,5136,0,5136,0.20697784423828125,9.77630116236364e-06
1056,5151,0,5151,0.20745396614074707,9.771282963629966e-06
1058,5161,0,5161,0.20776581764221191,9.76798480951047e-06
1061,5176,0,5176,0.20823907852172852,9.763104511693338e-06
1064,5191,0,5191,0.20874905586242676,9.758300062317807e-06
1067,5206,0,5206,0.20944690704345703,9.753566810876437e-06
1070,5221,0,5221,0.21029877662658691,9.748900486351012e-06
1072,5231,0,5231,0.21103405952453613,9.74582483314123e-06
1075,5246,0,5246,0.21199584007263184,9.741261486601564e-06
1078,5261,0,5261,0.2127218246459961,9.73675528439129e-06
1081,5276,0,5276,0.21338272094726562,9.732303079939436e-06
1084,5291,0,5291,0.213972806930542,9.727901973211027e-06
1087,5306,0,5306,0.21451282501220703,9.723549289494574e-06
1089,5316,0,5316,0.21483898162841797,9.720673175003066e-06
1092,5331,0,5331,0.21534204483032227,9.716395804253315e-06
1095,5346,0,5346,0.2158210277557373,9.712160684655322e-06
1098,5361,0,5361,0.21628689765930176,9.707965815924995e-06
1101,5376,0,5376,0.21675586700439453,9.70380934714901e-06
1103,5386,0,5386,0.21706700325012207,9.701058849626607e-06
1106,5401,0,5401,0.2175297737121582,9.696962634738108e-06
1109,5416,0,5416,0.2180027961730957,9.69290052392771e-06
1112,5431,0,5431,0.21846699714660645,9.688871116432851e-06
1115,5446,0,5446,0.2189328670501709,9.684873111873847e-06
1117,5456,0,5456,0.21925592422485352,9.682224621436693e-06
1120,5471,0,5471,0.21972084045410156,9.678276312777542e-06
1123,5486,0,5486,0.2201859951019287,9.674356371026104e-06
1126,5501,0,5501,0.22064781188964844,9.670463800005541e-06
1129,5516,0,5516,0.22110891342163086,9.66659767174215e-06
1132,5531,0,5531,0.2215738296508789,9.662757121196982e-06
1134,5541,0,5541,0.22188186645507812,9.660210563199086e-06
1137,5556,0,5556,0.2223527431488037,9.656410875286065e-06
1140,5571,0,5571,0.22281599044799805,9.652634729784107e-06
1143,5586,0,5586,0.2232809066772461,9.64888145334034e-06
1146,5601,0,5601,0.22374868392944336,9.645150415868398e-06
1148,5610,0,5610,0.2240450382232666,9.54434565710027e-06
1151,5625,0,5625,0.22450566291809082,9.343970830150073e-06
1154,5640,0,5640,0.22521376609802246,9.215348839973716e-06
1157,5655,0,5655,0.2259230613708496,9.130025999475314e-06
1160,5669,0,5669,0.22639203071594238,8.667467459624952e-06
1163,5684,0,5684,0.22686100006103516,8.485604772775578e-06
1165,5693,0,5693,0.2272648811340332,8.271205142103106e-06
1168,5707,0,5707,0.2279069423675537,8.15504650139453e-06
1171,5722,0,5722,0.22850894927978516,7.99493567570226e-06
1174,5737,0,5737,0.22899198532104492,7.881648790359096e-06
1177,5751,0,5751,0.22945189476013184,7.576963851730788e-06
1179,5761,0,5761,0.229766845703125,7.40886370108487e-06
1182,5775,0,5775,0.2302238941192627,7.037796670165057e-06
1185,5789,0,5789,0.23069190979003906,6.794853974180114e-06
1188,5803,0,5803,0.23114895820617676,6.252171919429999e-06
1191,5818,0,5818,0.23161792755126953,6.046848540733421e-06
1193,5828,0,5828,0.23192787170410156,5.948893192085943e-06
1196,5842,0,5842,0.23238396644592285,5.674514613504086e-06
1199,5856,0,5856,0.23284077644348145,5.319581375798123e-06
1202,5871,0,5871,0.2333087921142578,5.162777448579211e-06
1205,5886,0,5886,0.23377680778503418,5.06512378087763e-06
1208,5901,0,5901,0.23424577713012695,4.9997902214123026e-06
1210,5911,0,5911,0.23456478118896484,4.966920232831599e-06
1213,5926,0,5926,0.23503398895263672,4.927582799110493e-06
1216,5941,0,5941,0.23550200462341309,4.8960661352961686e-06
1219,5956,0,5956,0.23597002029418945,4.869633931660045e-06
1222,5971,0,5971,0.23643803596496582,4.846715599320016e-06
1224,5981,0,5981,0.23675107955932617,4.83290759652159e-06
1227,5996,0,5996,0.23721599578857422,4.8139334748251235e-06
1230,6011,0,6011,0.2376880645751953,4.796663021540097e-06
1233,6026,0,6026,0.23815178871154785,4.780791304806196e-06
1236,6041,0,6041,0.23862600326538086,4.766099950877772e-06
1239,6056,0,6056,0.23909783363342285,4.752425696787479e-06
1241,6066,0,6066,0.2394087314605713,4.743810877719791e-06
1244,6081,0,6081,0.23987293243408203,4.73156298012462e-06
1247,6096,0,6096,0.2403428554534912,4.720046669953409e-06
1250,6111,0,6111,0.24080681800842285,4.709187860305923e-06
1253,6126,0,6126,0.24126887321472168,4.698923630233584e-06
1255,6136,0,6136,0.2415788173675537,4.692384052704127e-06
1258,6151,0,6151,0.24204373359680176,4.682993769653421e-06
1261,6166,0,6166,0.24251580238342285,4.674068232531017e-06
1264,6181,0,6181,0.24297690391540527,4.665569024003183e-06
1267,6196,0,6196,0.24344086647033691,4.657461901369535e-06
1269,6206,0,6206,0.24376797676086426,4.6522596895931536e-06
1272,6221,0,6221,0.2442629337310791,4.64473935196866e-06
1275,6236,0,6236,0.24482297897338867,4.637535813993057e-06
1278,6251,0,6251,0.245344877243042,4.630625648117482e-06
1281,6266,0,6266,0.2458176612854004,4.6239875531992655e-06
1284,6281,0,6281,0.24628281593322754,4.6176021103963825e-06
1286,6291,0,6291,0.24659991264343262,4.6134766852006765e-06
1289,6306,0,6306,0.24706506729125977,4.607473646047468e-06
1292,6321,0,6321,0.24753570556640625,4.601679197213094e-06
1295,6336,0,6336,0.2480030059814453,4.5960792622664015e-06
1298,6351,0,6351,0.24846887588500977,4.5906608989084e-06
1300,6361,0,6361,0.24885869026184082,4.587143606496183e-06
1303,6376,0,6376,0.24939274787902832,4.582001849198763e-06
1306,6391,0,6391,0.24988889694213867,4.577011922227536e-06
1309,6406,0,6406,0.2503647804260254,4.572164217359567e-06
1312,6421,0,6421,0.25084686279296875,4.567449855601241e-06
1315,6436,0,6436,0.25132179260253906,4.562860624854962e-06
1317,6446,0,6446,0.25163698196411133,4.559866877636993e-06
1320,6461,0,6461,0.2521090507507324,4.5554695854547025e-06
1323,6476,0,6476,0.2525808811187744,4.5511783762567146e-06
1326,6491,0,6491,0.2530539035797119,4.546987042801007e-06
1329,6506,0,6506,0.2535247802734375,4.542889824956068e-06
1331,6516,0,6516,0.25383973121643066,4.540207975641629e-06
1334,6531,0,6531,0.25431084632873535,4.536255919982673e-06
1337,6545,0,6545,0.2547750473022461,4.4959858113035005e-06
1340,6560,0,6560,0.2552471160888672,4.445723910529185e-06
1343,6575,0,6575,0.2558329105377197,4.4133497244165455e-06
1345,6585,0,6585,0.2564668655395508,4.397710002879452e-06
1348,6600,0,6600,0.25699281692504883,4.379752583817942e-06
1351,6615,0,6615,0.25756001472473145,4.366015613850074e-06
1354,6630,0,6630,0.2581937313079834,4.354900977657653e-06
1357,6645,0,6645,0.2588338851928711,4.345485976457457e-06
1360,6660,0,6660,0.25968289375305176,4.337222988787778e-06
1362,6670,0,6670,0.2601008415222168,4.3321832859222554e-06
1365,6685,0,6685,0.2607448101043701,4.3251599116785e-06
1368,6700,0,6700,0.26142191886901855,4.3186450439425855e-06
1371,6715,0,6715,0.2619650363922119,4.31253346580538e-06
1374,6730,0,6730,0.2624378204345703,4.3067527028001596e-06
1376,6740,0,6740,0.2627599239349365,4.303056532616548e-06
1379,6755,0,6755,0.2633178234100342,4.297719333297836e-06
1382,6770,0,6770,0.2638518810272217,4.2926032735229544e-06
1385,6785,0,6785,0.2643718719482422,4.287683964894399e-06
1388,6800,0,6800,0.2649538516998291,4.282942028669041e-06
1391,6815,0,6815,0.2655611038208008,4.278361700590493e-06
1393,6825,0,6825,0.2658839225769043,4.275391377625988e-06
1396,6840,0,6840,0.2664949893951416,4.271052328459959e-06
1399,6855,0,6855,0.26711177825927734,4.266844250788583e-06
1402,6870,0,6870,0.26772284507751465,4.262758504336945e-06
1405,6885,0,6885,0.26824378967285156,4.258787516531756e-06
1407,6895,0,6895,0.2686300277709961,4.256200603835833e-06
1410,6910,0,6910,0.2692270278930664,4.252406336497507e-06
1413,6925,0,6925,0.2697908878326416,4.248710472838297e-06
1416,6940,0,6940,0.2702939510345459,4.245107960927535e-06
1419,6955,0,6955,0.2707676887512207,4.241594200341387e-06
1421,6965,0,6965,0.2710850238800049,4.239298904769203e-06
1424,6980,0,6980,0.27155590057373047,4.235923868175396e-06
1427,6995,0,6995,0.2720298767089844,4.2326270717306095e-06
1430,7010,0,7010,0.2727029323577881,4.229405105043775e-06
1433,7025,0,7025,0.27324390411376953,4.226254794377718e-06
1436,7040,0,7040,0.2737116813659668,4.223173176270114e-06
1438,7050,0,7050,0.2740299701690674,4.22115554893465e-06
1441,7065,0,7065,0.27449703216552734,4.2181823345391324e-06
1444,7080,0,7080,0.2749598026275635,4.215270778171154e-06
1447,7095,0,7095,0.2754218578338623,4.212418519253865e-06
1450,7110,0,7110,0.27588605880737305,4.209623327220307e-06
1452,7120,0,7120,0.27619194984436035,4.207790522282433e-06
1455,7135,0,7135,0.2767510414123535,4.205085803250886e-06
1458,7149,0,7149,0.277263879776001,4.152078883574742e-06
1461,7164,0,7164,0.277785062789917,4.0642034763299315e-06
1464,7179,0,7179,0.27826786041259766,4.018708847898653e-06
1467,7194,0,7194,0.27874302864074707,3.994508650673759e-06
1469,7204,0,7204,0.27905893325805664,3.984721103310557e-06
1472,7219,0,7219,0.27953290939331055,3.975237666100525e-06
1475,7234,0,7234,0.28000569343566895,3.969247730997641e-06
1478,7249,0,7249,0.28047895431518555,3.96509411358512e-06
1481,7264,0,7264,0.28095197677612305,3.961937723787839e-06
1483,7274,0,7274,0.2812669277191162,3.960164404464964e-06
1486,7289,0,7289,0.2817368507385254,3.957816326937322e-06
1489,7304,0,7304,0.2822120189666748,3.955716883338864e-06
1492,7319,0,7319,0.2826879024505615,3.953783128710263e-06
1495,7334,0,7334,0.2831599712371826,3.951967467207251e-06
1497,7344,0,7344,0.2834749221801758,3.9508080403693986e-06
1500,7359,0,7359,0.28394579887390137,3.949131195046119e-06
1503,7374,0,7374,0.28441905975341797,3.947517480161389e-06
1506,7389,0,7389,0.28488802909851074,3.945957582645496e-06
1509,7404,0,7404,0.28535890579223633,3.944444806867832e-06
1512,7419,0,7419,0.2858269214630127,3.9429741275022745e-06
1514,7429,0,7429,0.28613972663879395,3.94201509400117e-06
1517,7444,0,7444,0.28661608695983887,3.940606265795427e-06
1520,7459,0,7459,0.28708696365356445,3.939230691915703e-06
1523,7474,0,7474,0.28756093978881836,3.937886061411662e-06
1526,7489,0,7489,0.28803086280822754,3.9365704019534984e-06
1528,7499,0,7499,0.2883439064025879,3.93570853691799e-06
1531,7514,0,7514,0.28882670402526855,3.934437464912861e-06
1534,7529,0,7529,0.28929781913757324,3.933191240819024e-06
1537,7544,0,7544,0.28976988792419434,3.931968619927423e-06
1540,7559,0,7559,0.29024481773376465,3.9307684769413155e-06
1543,7574,0,7574,0.29071569442749023,3.929589786353534e-06
1545,7584,0,7584,0.2910289764404297,3.928815442751141e-06
1548,7599,0,7599,0.29149580001831055,3.927670450602858e-06
1551,7613,0,7613,0.29195475578308105,3.8570963186782086e-06
1554,7628,0,7628,0.29244494438171387,3.7583336356450916e-06
1557,7643,0,7643,0.29291582107543945,3.7095491490320506e-06
1559,7653,0,7653,0.2932288646697998,3.6911627234553678e-06
1562,7668,0,7668,0.293712854385376,3.674547697771007e-06
1565,7683,0,7683,0.2941911220550537,3.6649438029970536e-06
1568,7698,0,7698,0.29468202590942383,3.65884552192187e-06
1571,7713,0,7713,0.2951517105102539,3.654585150882366e-06
1573,7723,0,7723,0.29546689987182617,3.652344772103334e-06
1576,7738,0,7738,0.29593801498413086,3.6495485649512218e-06
1579,7753,0,7753,0.29640793800354004,3.6472057072729166e-06
1582,7768,0,7768,0.29687976837158203,3.6451684280419714e-06
1585,7783,0,7783,0.29735279083251953,3.643350070153565e-06
1588,7798,0,7798,0.2978229522705078,3.641696471206535e-06
1590,7808,0,7808,0.29813599586486816,3.6406673632953786e-06
1593,7823,0,7823,0.2986159324645996,3.639214070904899e-06
1596,7838,0,7838,0.2990849018096924,3.637851769097085e-06
1599,7853,0,7853,0.29954981803894043,3.636565410835143e-06
1602,7868,0,7868,0.3000178337097168,3.635343476208962e-06
1604,7878,0,7878,0.30032896995544434,3.634560109944993e-06
1607,7893,0,7893,0.3007967472076416,3.6334264337604504e-06
1610,7908,0,7908,0.30126190185546875,3.6323369687497417e-06
1613,7923,0,7923,0.3017268180847168,3.631286626019028e-06
1616,7938,0,7938,0.30219388008117676,3.6302711989680614e-06
1619,7953,0,7953,0.30266475677490234,3.62928717172017e-06
1621,7963,0,7963,0.3029758930206299,3.628647112920084e-06
1624,7978,0,7978,0.30344295501708984,3.62770904232268e-06
1627,7993,0,7993,0.3039119243621826,3.6267953880390422e-06
1630,8008,0,8008,0.3043808937072754,3.6259041744873273e-06
1633,8023,0,8023,0.30484771728515625,3.6250336804384266e-06
1635,8033,0,8033,0.3051607608795166,3.6244641083410494e-06
1638,8048,0,8048,0.30566978454589844,3.623624877810636e-06
1641,8063,0,8063,0.30614185333251953,3.622802714877514e-06
1644,8078,0,8078,0.30661988258361816,3.621996517988272e-06
1647,8093,0,8093,0.30709075927734375,3.6212052979401776e-06
1649,8103,0,8103,0.3074049949645996,3.6206856938312544e-06
1652,8118,0,8118,0.3078749179840088,3.6199174920375013e-06
1655,8133,0,8133,0.30834388732910156,3.6191620642097487e-06
1658,8148,0,8148,0.3088109493255615,3.6184187145811386e-06
1661,8163,0,8163,0.3092777729034424,3.617686804662481e-06
1664,8178,0,8178,0.30979394912719727,3.6169657463422952e-06
1666,8188,0,8188,0.31010985374450684,3.616490799355358e-06
1669,8203,0,8203,0.310593843460083,3.615786638841968e-06
1672,8218,0,8218,0.31107497215270996,3.61509196626248e-06
1675,8232,0,8232,0.31153297424316406,3.4946140344808295e-06
1678,8246,0,8246,0.31198787689208984,3.24775327766029e-06
1680,8255,0,8255,0.3122878074645996,3.06965095427407e-06
1683,8269,0,8269,0.31278300285339355,2.8366051481229592e-06
1686,8283,0,8283,0.31324195861816406,2.7458737145017493e-06
1689,8298,0,8298,0.31371593475341797,2.653957244783671e-06
1692,8312,0,8312,0.31417393684387207,2.51981753619023e-06
1695,8327,0,8327,0.31475186347961426,2.479516809595056e-06
1697,8336,0,8336,0.3150928020477295,2.4030418020451307e-06
1700,8351,0,8351,0.3155660629272461,2.340838440300571e-06
1703,8366,0,8366,0.3160359859466553,2.3071743892308185e-06
1706,8380,0,8380,0.31649088859558105,2.278288119770602e-06
1709,8394,0,8394,0.31694579124450684,2.140906259896652e-06
1711,8404,0,8404,0.3172588348388672,2.0920558513521657e-06
1714,8419,0,8419,0.3178579807281494,2.045999349270299e-06
1717,8434,0,8434,0.3186607360839844,2.018434869331488e-06
1720,8448,0,8448,0.3192617893218994,1.9725074483073053e-06
1723,8463,0,8463,0.31978392601013184,1.9178156230662533e-06
1725,8473,0,8473,0.32010483741760254,1.8951299737658743e-06
1728,8488,0,8488,0.32062578201293945,1.8725903847944757e-06
1731,8502,0,8502,0.32113099098205566,1.808152236323549e-06
1734,8516,0,8516,0.3217179775238037,1.678003527631557e-06
1737,8530,0,8530,0.3222661018371582,1.5467416838448125e-06
1740,8544,0,8544,0.3228158950805664,1.441546914974886e-06
1742,8553,0,8553,0.3231179714202881,1.3456774512853018e-06
1745,8567,0,8567,0.32358288764953613,1.2646298491235744e-06
1748,8582,0,8582,0.3240549564361572,1.2366322313648642e-06
1751,8597,0,8597,0.3245229721069336,1.2193729002772983e-06
1754,8612,0,8612,0.3249959945678711,1.2079348398224107e-06
1756,8622,0,8622,0.32531285285949707,1.202229486473116e-06
1759,8637,0,8637,0.32578086853027344,1.1954658531649715e-06
1762,8652,0,8652,0.3262519836425781,1.1901174656293516e-06
1765,8667,0,8667,0.3267240524291992,1.1856968534263312e-06
1768,8682,0,8682,0.32719898223876953,1.1819230493116551e-06
1771,8697,0,8697,0.32767677307128906,1.1786260814493233e-06
1773,8707,0,8707,0.3279910087585449,1.1766378796560973e-06
1776,8722,0,8722,0.328463077545166,1.1739132508938875e-06
1779,8737,0,8737,0.3289310932159424,1.1714485389354575e-06
1782,8752,0,8752,0.32939887046813965,1.169202142607201e-06
1785,8767,0,8767,0.33003783226013184,1.1671426014478325e-06
1787,8777,0,8777,0.3304266929626465,1.1658610139859157e-06
1790,8792,0,8792,0.3311159610748291,1.1640606424456483e-06
1793,8807,0,8807,0.33173608779907227,1.1623915253123963e-06
1796,8822,0,8822,0.3323650360107422,1.1608392048561704e-06
1799,8837,0,8837,0.3328697681427002,1.159391438275882e-06
1801,8847,0,8847,0.33318400382995605,1.158479099449652e-06
1804,8862,0,8862,0.3336508274078369,1.1571829547330737e-06
1807,8877,0,8877,0.334122896194458,1.1559663407071445e-06
1810,8892,0,8892,0.33458781242370605,1.1548219533489124e-06
1813,8907,0,8907,0.3350520133972168,1.153743337168737e-06
1816,8922,0,8922,0.3355140686035156,1.1527247574045983e-06
1818,8932,0,8932,0.33582377433776855,1.1520765083774422e-06
1821,8947,0,8947,0.33629274368286133,1.1511468869501839e-06
1824,8962,0,8962,0.33675599098205566,1.1502648133439724e-06
1827,8977,0,8977,0.3372180461883545,1.1494264515305538e-06
1830,8992,0,8992,0.33768486976623535,1.1486283414491954e-06
1832,9002,0,9002,0.3379960060119629,1.1481170730954467e-06
1835,9017,0,9017,0.33846092224121094,1.1473792459196853e-06
1838,9032,0,9032,0.33894801139831543,1.1466739694624335e-06
1841,9047,0,9047,0.3394160270690918,1.1459988330472289e-06
1844,9062,0,9062,0.33987975120544434,1.1453516438292615e-06
1847,9077,0,9077,0.3403468132019043,1.1447304042331746e-06
1849,9087,0,9087,0.34067296981811523,1.1443297544435627e-06
1852,9102,0,9102,0.3411409854888916,1.1437477935212933e-06
1855,9117,0,9117,0.34160470962524414,1.1431872659721497e-06
1858,9132,0,9132,0.3420748710632324,1.142646736595344e-06
1861,9147,0,9147,0.34253787994384766,1.1421248900974248e-06
1863,9157,0,9157,0.3428459167480469,1.1417867716766637e-06
1866,9171,0,9171,0.3432958126068115,1.1233339937626878e-06
1869,9186,0,9186,0.3437938690185547,1.1098288430123701e-06
1872,9201,0,9201,0.3442709445953369,1.102680788014614e-06
1875,9216,0,9216,0.34473586082458496,1.0987636927553564e-06
1877,9226,0,9226,0.3450448513031006,1.0971373012347272e-06
1880,9241,0,9241,0.34551072120666504,1.0955297370913723e-06
1883,9256,0,9256,0.3459758758544922,1.0945014742289326e-06
1886,9271,0,9271,0.3464388847351074,1.093791678331515e-06
1889,9286,0,9286,0.346904993057251,1.0932627041545505e-06
1892,9301,0,9301,0.347369909286499,1.0928402778989915e-06
1894,9311,0,9311,0.3478078842163086,1.0925967236174648e-06
1897,9326,0,9326,0.3483309745788574,1.0922697009202942e-06
1900,9341,0,9341,0.348801851272583,1.0919748743636344e-06
1903,9356,0,9356,0.34926486015319824,1.0917024674060437e-06
1906,9371,0,9371,0.34972286224365234,1.0914464136824493e-06
1908,9381,0,9381,0.35003089904785156,1.0912828084564243e-06
1911,9396,0,9396,0.3504939079284668,1.0910459974202659e-06
1914,9411,0,9411,0.3509528636932373,1.0908177543225284e-06
1917,9426,0,9426,0.3514118194580078,1.0905966350072423e-06
1920,9441,0,9441,0.35187292098999023,1.0903815788629521e-06
1923,9456,0,9456,0.35233569145202637,1.090171782197688e-06
1925,9466,0,9466,0.35264086723327637,1.0900345247123948e-06
1928,9481,0,9481,0.35309886932373047,1.0898321652963394e-06
1931,9496,0,9496,0.353557825088501,1.0896336566882433e-06
1934,9511,0,9511,0.354017972946167,1.089438637167699e-06
1937,9526,0,9526,0.3544750213623047,1.0892468018191574e-06
1939,9536,0,9536,0.354780912399292,1.0891205501690755e-06
1942,9551,0,9551,0.3552398681640625,1.0889334591420538e-06
1945,9566,0,9566,0.35581493377685547,1.0887489296976737e-06
1948,9581,0,9581,0.35634303092956543,1.0885667787803497e-06
1951,9595,0,9595,0.35680484771728516,1.066351139445198e-06
1953,9605,0,9605,0.3571197986602783,1.0506429550223754e-06
1956,9620,0,9620,0.3575899600982666,1.0364346705707832e-06
1959,9635,0,9635,0.35805487632751465,1.0284061917132734e-06
1962,9649,0,9649,0.3585069179534912,9.714040209772587e-07
1965,9663,0,9663,0.35895800590515137,9.30858060445269e-07
1968,9677,0,9677,0.3594088554382324,8.857969771527988e-07
1970,9687,0,9687,0.35971784591674805,8.713906771432708e-07
1973,9700,0,9700,0.36015892028808594,7.720144428553698e-07
1976,9714,0,9714,0.3606538772583008,7.494991372028566e-07
1979,9729,0,9729,0.36112189292907715,7.319502331513122e-07
1982,9743,0,9743,0.3615727424621582,7.165017168656584e-07
1984,9753,0,9753,0.3618810176849365,7.008793278223044e-07
1987,9768,0,9768,0.362346887588501,6.853886205330874e-07
1990,9783,0,9783,0.36281490325927734,6.754277526319672e-07
1993,9797,0,9797,0.3632678985595703,6.503262232067292e-07
1996,9812,0,9812,0.36373400688171387,6.342359041573143e-07
1999,9826,0,9826,0.36418986320495605,6.169253751644511e-07
2001,9834,0,9834,0.3644700050354004,5.507939345656541e-07
2004,9847,0,9847,0.36490583419799805,4.925307247087546e-07
2007,9862,0,9862,0.3653707504272461,4.589143534080287e-07
2010,9877,0,9877,0.3658428192138672,4.362101641560923e-07
2013,9891,0,9891,0.36629700660705566,3.9896957446340153e-07
2015,9900,0,9900,0.3665938377380371,3.818795726761191e-07
2018,9914,0,9914,0.36705994606018066,3.544990152069041e-07
2021,9929,0,9929,0.36752772331237793,3.3779687278303876e-07
2024,9944,0,9944,0.36799001693725586,3.265769754650029e-07
2027,9959,0,9959,0.3684568405151367,3.1843738037908436e-07
2029,9968,0,9968,0.36875391006469727,3.082374271271786e-07
2032,9982,0,9982,0.36920690536499023,2.875113308386601e-07
2035,9996,0,9996,0.369661808013916,2.6006762742524457e-07
2038,10010,0,10010,0.3701167106628418,2.403691803066288e-07
2041,10025,0,10025,0.37059688568115234,2.3362029442830333e-07
2044,10039,0,10039,0.3710489273071289,2.2349396706193594e-07
2046,10049,0,10049,0.371356725692749,2.184961226131644e-07
2049,10064,0,10064,0.37182092666625977,2.1330744786899495e-07
2052,10078,0,10078,0.3722810745239258,2.091664945340977e-07
2055,10093,0,10093,0.37278199195861816,2.0303197368054724e-07
2058,10108,0,10108,0.373248815536499,1.994010150593106e-07
2060,10118,0,10118,0.37355995178222656,1.9776731918073567e-07
2063,10133,0,10133,0.3740239143371582,1.9600184501951104e-07
2066,10148,0,10148,0.37449002265930176,1.9473037789179394e-07
2069,10162,0,10162,0.3749427795410156,1.8681217511754643e-07
2072,10177,0,10177,0.37540507316589355,1.8392067003479502e-07
2075,10192,0,10192,0.3758687973022461,1.8206319304232422e-07
2077,10202,0,10202,0.37617993354797363,1.811671280934889e-07
2080,10217,0,10217,0.37664294242858887,1.8013936205483857e-07
2083,10232,0,10232,0.37711095809936523,1.7935505851935775e-07
2086,10247,0,10247,0.3775777816772461,1.7872383573462034e-07
2089,10262,0,10262,0.3780379295349121,1.7819394007321574e-07
2091,10272,0,10272,0.3783438205718994,1.7788125891019115e-07
2094,10287,0,10287,0.3788027763366699,1.77458057150491e-07
2097,10302,0,10302,0.379260778427124,1.7707782297452296e-07
2100,10317,0,10317,0.37971973419189453,1.7673119356926208e-07
2103,10332,0,10332,0.38018298149108887,1.7641166920251843e-07
2105,10342,0,10342,0.3804898262023926,1.7621133791137764e-07
2108,10356,0,10356,0.3809347152709961,1.7451936073711394e-07
2111,10371,0,10371,0.3813939094543457,1.7340197086981125e-07
2114,10386,0,10386,0.3818528652191162,1.726968974191335e-07
2117,10401,0,10401,0.38231492042541504,1.7220488055015196e-07
2120,10416,0,10416,0.3827848434448242,1.7182862707173617e-07
2122,10426,0,10426,0.38309192657470703,1.7161694575987406e-07
2125,10441,0,10441,0.38354992866516113,1.7133770012044617e-07
2128,10456,0,10456,0.3840138912200928,1.710905043757121e-07
2131,10470,0,10470,0.3844609260559082,1.689688586730036e-07
2134,10485,0,10485,0.3849210739135742,1.6725634458664134e-07
2136,10495,0,10495,0.3852269649505615,1.6652340930993313e-07
2139,10510,0,10510,0.38568902015686035,1.6578742610617398e-07
2142,10525,0,10525,0.38614988327026367,1.6531533381404275e-07
2145,10539,0,10539,0.3865959644317627,1.6191816399705274e-07
2148,10554,0,10554,0.3870539665222168,1.5912226013744034e-07
2151,10569,0,10569,0.38751673698425293,1.5745124988278692e-07
2153,10579,0,10579,0.38782787322998047,1.5670214538014944e-07
2156,10594,0,10594,0.38828587532043457,1.5590787893983557e-07
2159,10609,0,10609,0.3887457847595215,1.5536049686478412e-07
2162,10624,0,10624,0.38921284675598145,1.5496301598682717e-07
2165,10639,0,10639,0.3896749019622803,1.5466090668319326e-07
2167,10649,0,10649,0.3899807929992676,1.5449621491812513e-07
2170,10664,0,10664,0.3904387950897217,1.5428892234774919e-07
2173,10679,0,10679,0.3908977508544922,1.541172974459682e-07
2176,10694,0,10694,0.3913547992706299,1.539721343137459e-07
2179,10709,0,10709,0.3918190002441406,1.5384717809431987e-07
2181,10719,0,10719,0.39212584495544434,1.537728662302743e-07
2184,10734,0,10734,0.39258480072021484,1.5367238887639532e-07
2187,10749,0,10749,0.39307093620300293,1.5358280767989516e-07
2190,10764,0,10764,0.3935418128967285,1.5350210872337497e-07
2193,10779,0,10779,0.39401793479919434,1.5342872973919481e-07
2196,10794,0,10794,0.39449071884155273,1.533614395101836e-07
2198,10804,0,10804,0.3948037624359131,1.5331946824712755e-07
2201,10819,0,10819,0.3952827453613281,1.5326023707016074e-07
2204,10834,0,10834,0.3958888053894043,1.5320487326617983e-07
2207,10849,0,10849,0.3964259624481201,1.531528106127632e-07
2210,10864,0,10864,0.39693689346313477,1.5310358189961073e-07
2212,10874,0,10874,0.3972489833831787,1.5307214275097726e-07
2215,10889,0,10889,0.3977179527282715,1.5302680686605942e-07
2218,10904,0,10904,0.39818477630615234,1.5298340568830895e-07
2221,10919,0,10919,0.3986508846282959,1.529416957939289e-07
2224,10934,0,10934,0.39911484718322754,1.5290147085908608e-07
2227,10949,0,10949,0.3995780944824219,1.5286255519643267e-07
2229,10959,0,10959,0.399965763092041,1.528372636701882e-07
2232,10974,0,10974,0.4005129337310791,1.5280020678522757e-07
2235,10989,0,10989,0.40100693702697754,1.5276410379266562e-07
2238,11004,0,11004,0.40148401260375977,1.527288535989691e-07
2241,11019,0,11019,0.401958703994751,1.526943684632941e-07
2243,11027,0,11027,0.402249813079834,1.4932756880196208e-07
2246,11042,0,11042,0.402724027633667,1.4655871165464555e-07
2249,11057,0,11057,0.4032008647918701,1.4498649208630152e-07
2252,11072,0,11072,0.40368199348449707,1.4404744667811512e-07
2255,11087,0,11087,0.4041929244995117,1.4345176594874085e-07
2257,11097,0,11097,0.40458178520202637,1.4316774586186548e-07
2260,11112,0,11112,0.40530872344970703,1.4284673757794155e-07
2263,11127,0,11127,0.40625977516174316,1.4260743147863405e-07
2266,11142,0,11142,0.40680384635925293,1.424203069266814e-07
2269,11157,0,11157,0.4073038101196289,1.4226822475142808e-07
2272,11172,0,11172,0.4077780246734619,1.4214078499862782e-07
2274,11182,0,11182,0.4080958366394043,1.42066150757525e-07
2277,11197,0,11197,0.40856289863586426,1.419662416450835e-07
2280,11212,0,11212,0.40903687477111816,1.4187785139749322e-07
2283,11227,0,11227,0.40950870513916016,1.417985637288663e-07
2286,11242,0,11242,0.40997767448425293,1.4172661285758624e-07
2288,11252,0,11252,0.41028881072998047,1.4168205355681875e-07
2291,11267,0,11267,0.41075682640075684,1.4161954306963418e-07
2294,11282,0,11282,0.4112229347229004,1.4156147919102157e-07
2297,11297,0,11297,0.4116950035095215,1.415071836261291e-07
2300,11312,0,11312,0.4121589660644531,1.4145611388658148e-07
2303,11327,0,11327,0.4126248359680176,1.414078308416384e-07
2305,11337,0,11337,0.41293787956237793,1.4137701015115599e-07
2308,11352,0,11352,0.413402795791626,1.4133260456027683e-07
2311,11367,0,11367,0.41388678550720215,1.412901596138005e-07
2314,11382,0,11382,0.41435885429382324,1.412494548907215e-07
2317,11397,0,11397,0.41501283645629883,1.4121030395975473e-07
2319,11407,0,11407,0.4154050350189209,1.4118498709474067e-07
2322,11422,0,11422,0.41591978073120117,1.4114808385696967e-07
2325,11437,0,11437,0.41640377044677734,1.4111235837467383e-07
2328,11452,0,11452,0.4168870449066162,1.4107770302189725e-07
2331,11467,0,11467,0.4174199104309082,1.4104402366542377e-07
2333,11477,0,11477,0.4177358150482178,1.410220716728939e-07
2336,11492,0,11492,0.41820693016052246,1.409898397148771e-07
2339,11507,0,11507,0.4186818599700928,1.4095838338736995e-07
2342,11522,0,11522,0.4191579818725586,1.409276422716598e-07
2345,11537,0,11537,0.4196789264678955,1.4089756220254392e-07
2348,11552,0,11552,0.4203648567199707,1.4086809445528708e-07
2350,11562,0,11562,0.4210968017578125,1.4084876756143381e-07
2353,11577,0,11577,0.4217808246612549,1.4082022461214198e-07
2356,11591,0,11591,0.4223368167877197,1.4068028512961337e-07
2359,11606,0,11606,0.42289304733276367,1.3965426845050038e-07
2362,11621,0,11621,0.42360591888427734,1.390537628773132e-07
2364,11631,0,11631,0.4239468574523926,1.387860253922292e-07
2367,11646,0,11646,0.4245269298553467,1.3850003039676964e-07
2370,11661,0,11661,0.42520976066589355,1.3829803674448818e-07
2373,11675,0,11675,0.425872802734375,1.339006857597917e-07
2376,11690,0,11690,0.4264059066772461,1.3067454438403305e-07
2379,11703,0,11703,0.42685484886169434,1.2143827787017815e-07
2381,11713,0,11713,0.42728090286254883,1.1812054094348568e-07
2384,11728,0,11728,0.4278829097747803,1.1483899136847985e-07
2387,11743,0,11743,0.42838382720947266,1.1275939040006616e-07
2390,11758,0,11758,0.42900872230529785,1.1135284077626073e-07
2393,11773,0,11773,0.4294877052307129,1.1033854403570513e-07
2395,11783,0,11783,0.4299278259277344,1.098021052443834e-07
2398,11797,0,11797,0.4306180477142334,1.071862774858893e-07
2401,11812,0,11812,0.4313499927520752,1.0583658269812247e-07
2404,11827,0,11827,0.4321320056915283,1.049765401080674e-07
2407,11841,0,11841,0.43301987648010254,1.0192654559497664e-07
2409,11851,0,11851,0.43355584144592285,9.991520824665187e-08
2412,11866,0,11866,0.434614896774292,9.798213304401845e-08
2415,11881,0,11881,0.4356958866119385,9.67969172653012e-08
2418,11895,0,11895,0.436647891998291,9.297444716257851e-08
2421,11909,0,11909,0.43755173683166504,8.901656291866641e-08
2424,11923,0,11923,0.4384489059448242,8.304853712572549e-08
2426,11932,0,11932,0.43880391120910645,8.120999674631897e-08
2429,11946,0,11946,0.4395129680633545,7.62657671036834e-08
2432,11961,0,11961,0.44026994705200195,7.302065286405779e-08
2435,11975,0,11975,0.4407837390899658,6.827878056263679e-08
2438,11990,0,11990,0.44125795364379883,6.564563391424253e-08
2440,11999,0,11999,0.4415857791900635,6.221922305223164e-08
2443,12014,0,12014,0.44205784797668457,5.9402798195054947e-08
2446,12028,0,12028,0.44251489639282227,5.524175774220139e-08
2449,12043,0,12043,0.44298481941223145,5.279887883075838e-08
2452,12057,0,12057,0.44344091415405273,5.157628517652942e-08
2455,12072,0,12072,0.44391965866088867,4.837058366056095e-08
2457,12081,0,12081,0.44422292709350586,4.454091198634509e-08
2460,12095,0,12095,0.4446897506713867,4.0423351991983995e-08
2463,12109,0,12109,0.445253849029541,3.754075096282243e-08
2466,12122,0,12122,0.4457530975341797,3.3481765340069285e-08
2469,12137,0,12137,0.44623303413391113,3.176816202888542e-08
2471,12147,0,12147,0.4465508460998535,3.1024141113783454e-08
2474,12162,0,12162,0.4470248222351074,3.027480951791328e-08
2477,12177,0,12177,0.4475688934326172,2.9798508423917438e-08
2480,12192,0,12192,0.4481048583984375,2.948270589644058e-08
2483,12207,0,12207,0.448772668838501,2.9263570245401507e-08
2485,12217,0,12217,0.4492669105529785,2.9152384669332276e-08
2488,12232,0,12232,0.4500448703765869,2.902079827615955e-08
2491,12247,0,12247,0.4508237838745117,2.891858264278499e-08
2494,12262,0,12262,0.4513678550720215,2.8836446644299573e-08
2497,12277,0,12277,0.45192384719848633,2.8768527069833554e-08
2500,12292,0,12292,0.4525790214538574,2.871099920425871e-08
2502,12302,0,12302,0.45304083824157715,2.8677110626559696e-08
2505,12317,0,12317,0.4537239074707031,2.863156823815221e-08
2508,12332,0,12332,0.4544041156768799,2.859113539066607e-08
2511,12347,0,12347,0.4550938606262207,2.8554761529048825e-08
2514,12362,0,12362,0.45568394660949707,2.8521659508252908e-08
2516,12372,0,12372,0.4560990333557129,2.8501105894229205e-08
2519,12387,0,12387,0.4568197727203369,2.8472186315956344e-08
2522,12402,0,12402,0.45729780197143555,2.8445211810102548e-08
2525,12417,0,12417,0.45804786682128906,2.8419864229960874e-08
2528,12432,0,12432,0.45860767364501953,2.8395887748479316e-08
2531,12447,0,12447,0.4591097831726074,2.837307488756562e-08
2533,12457,0,12457,0.459453821182251,2.835842778296981e-08
2536,12472,0,12472,0.4600968360900879,2.8337192881757704e-08
2539,12487,0,12487,0.46079301834106445,2.831673374872998e-08
2542,12502,0,12502,0.4613668918609619,2.8296948742421885e-08
2545,12517,0,12517,0.4619467258453369,2.827775318554469e-08
2547,12527,0,12527,0.46227502822875977,2.82652481501863e-08
2550,12542,0,12542,0.46276402473449707,2.824688327953689e-08
2553,12557,0,12557,0.4632587432861328,2.8228943129827823e-08
2556,12571,0,12571,0.4639158248901367,2.7667735500550876e-08
2559,12586,0,12586,0.4644768238067627,2.745758276529151e-08
2561,12595,0,12595,0.46497297286987305,2.6991187442526004e-08
2564,12610,0,12610,0.46581602096557617,2.670885508227408e-08
2567,12625,0,12625,0.4664597511291504,2.6538194314224406e-08
2570,12640,0,12640,0.46697998046875,2.6429145059748153e-08
2573,12655,0,12655,0.46745800971984863,2.6355279272139347e-08
2576,12670,0,12670,0.46793293952941895,2.6302342306556446e-08
2578,12680,0,12680,0.468250036239624,2.627461358122168e-08
2581,12695,0,12695,0.4687318801879883,2.6240725725537048e-08
2584,12710,0,12710,0.4692058563232422,2.621338328037998e-08
2587,12725,0,12725,0.46968984603881836,2.6190635217403035e-08
2590,12740,0,12740,0.47016286849975586,2.6171239839080552e-08
2592,12750,0,12750,0.4704759120941162,2.615975381469525e-08
2595,12765,0,12765,0.4709470272064209,2.614424683034379e-08
2598,12780,0,12780,0.4714198112487793,2.613041588515973e-08
2601,12795,0,12795,0.4718928337097168,2.6117929596678645e-08
2604,12810,0,12810,0.4724619388580322,2.610653824341977e-08
2607,12825,0,12825,0.4730229377746582,2.6096048973238672e-08
2609,12835,0,12835,0.47345685958862305,2.60894809025282e-08
2612,12850,0,12850,0.4739828109741211,2.6080172681809732e-08
2615,12865,0,12865,0.4744608402252197,2.6071424886552254e-08
2618,12880,0,12880,0.47493696212768555,2.6063151169878236e-08
2621,12895,0,12895,0.4754140377044678,2.6055280382627024e-08
2623,12905,0,12905,0.47572875022888184,2.605022746529256e-08
2626,12920,0,12920,0.47620391845703125,2.6042901938024286e-08
2629,12934,0,12934,0.47666287422180176,2.57368836521039e-08
2632,12949,0,12949,0.47719502449035645,2.5307653222783012e-08
2635,12964,0,12964,0.47768187522888184,2.5073464995321157e-08
2637,12974,0,12974,0.47801685333251953,2.4975790031363437e-08
2640,12989,0,12989,0.4786498546600342,2.487826419117487e-08
2643,13004,0,13004,0.4795098304748535,2.4815105296784064e-08
2646,13019,0,13019,0.48058176040649414,2.4771441209478298e-08
2649,13034,0,13034,0.4812448024749756,2.4739502149944557e-08
2652,13049,0,13049,0.48178577423095703,2.471504284340912e-08
2654,13059,0,13059,0.48209691047668457,2.4701639988506566e-08
2657,13074,0,13074,0.4825620651245117,2.4684708639456107e-08
2660,13089,0,13089,0.48302793502807617,2.467064594219388e-08
2663,13104,0,13104,0.4835031032562256,2.4658720550585914e-08
2666,13119,0,13119,0.48396897315979004,2.464842503641043e-08
2668,13129,0,13129,0.48427796363830566,2.464228243734287e-08
2671,13144,0,13144,0.48473691940307617,2.4633941205629575e-08
2674,13159,0,13159,0.485198974609375,2.462645390872799e-08
2677,13174,0,13174,0.48566174507141113,2.4619650280206178e-08
2680,13189,0,13189,0.4861259460449219,2.4613398509079614e-08
2683,13204,0,13204,0.486588716506958,2.4607595431340154e-08
2685,13214,0,13214,0.4868950843811035,2.4603935028769324e-08
2688,13229,0,13229,0.48736095428466797,2.459870713187976e-08
2691,13244,0,13244,0.4878237247467041,2.459374580636285e-08
2694,13259,0,13259,0.48828792572021484,2.4589006146909624e-08
2697,13274,0,13274,0.4887509346008301,2.4584451858072525e-08
2699,13284,0,13284,0.4890599250793457,2.458150384787038e-08
2702,13299,0,13299,0.4895198345184326,2.4577195692006213e-08
2705,13314,0,13314,0.48998188972473145,2.4573005746206148e-08
2708,13329,0,13329,0.49045586585998535,2.4568916657760642e-08
2711,13344,0,13344,0.4909369945526123,2.4564914092412695e-08
2713,13354,0,13354,0.49127793312072754,2.4562287820342205e-08
2716,13369,0,13369,0.49193286895751953,2.4558404005774383e-08
2719,13384,0,13384,0.4924657344818115,2.45545791939352e-08
2722,13399,0,13399,0.4931528568267822,2.4550805993746568e-08
2725,13414,0,13414,0.49381089210510254,2.4547078172882975e-08
2728,13429,0,13429,0.49433088302612305,2.4543390452860132e-08
2730,13438,0,13438,0.49492979049682617,2.397913015427342e-08
2733,13453,0,13453,0.495790958404541,2.3612567587843286e-08
2736,13468,0,13468,0.49648189544677734,2.3401386775532834e-08
2739,13483,0,13483,0.49695777893066406,2.3274276329359807e-08
2742,13498,0,13498,0.4974229335784912,2.3193512906126084e-08
2744,13508,0,13508,0.4977540969848633,2.3155054629603923e-08
2747,13521,0,13521,0.4982168674468994,2.2081451638600125e-08
2750,13535,0,13535,0.49866795539855957,2.0412266315841715e-08
2753,13550,0,13550,0.4991319179534912,1.977551269857693e-08
2756,13565,0,13565,0.49959397315979004,1.9422738986745017e-08
2759,13580,0,13580,0.5000548362731934,1.9215052041393587e-08
2761,13590,0,13590,0.5003697872161865,1.9121128661394468e-08
2764,13605,0,13605,0.5009059906005859,1.9018545680377035e-08
2767,13619,0,13619,0.5013570785522461,1.8502317377245645e-08
2770,13633,0,13633,0.5018069744110107,1.8002281993301368e-08
2773,13648,0,13648,0.5022678375244141,1.7405406396059824e-08
2775,13658,0,13658,0.5025758743286133,1.71521082487451e-08
2778,13673,0,13673,0.5030367374420166,1.6896276125018953e-08
2781,13688,0,13688,0.5034959316253662,1.6728657872771586e-08
2784,13702,0,13702,0.5039448738098145,1.565429137077172e-08
2787,13716,0,13716,0.5043938159942627,1.5382254540500832e-08
2789,13726,0,13726,0.50469970703125,1.4856438323519034e-08
2792,13740,0,13740,0.505155086517334,1.3484472782578e-08
2795,13755,0,13755,0.5056169033050537,1.320970157789651e-08
2798,13770,0,13770,0.506077766418457,1.3048496922056053e-08
2801,13784,0,13784,0.5066177845001221,1.2868992427977004e-08
2804,13799,0,13799,0.5070860385894775,1.2425856805365642e-08
2806,13808,0,13808,0.507408857345581,1.1746813141539921e-08
2809,13821,0,13821,0.5079169273376465,1.0606194629503335e-08
2812,13835,0,13835,0.5083818435668945,9.619894336086575e-09


==> plot_data/quadratic_minimax_problem_n20_alpha0/flex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,8.392333984375e-05,4.387061074692293
1,3,0,3,0.00016164779663085938,3.972820061310639
2,6,0,6,0.0003960132598876953,3.6277138409371137
3,9,0,9,0.0006167888641357422,2.672136101364927
4,12,0,12,0.0008528232574462891,2.4152473972739528
5,15,0,15,0.0010077953338623047,1.5663018362335526
6,18,0,18,0.0012497901916503906,1.4690513148498217
7,21,0,21,0.0014667510986328125,1.1803222473760537
8,24,0,24,0.0017218589782714844,1.1176538879410174
9,27,0,27,0.00185394287109375,0.8371978569777179
10,30,0,30,0.001997709274291992,0.7923042912566547
11,33,0,33,0.0021457672119140625,0.6058665094919226
12,36,0,36,0.0022728443145751953,0.5619155753702526
13,39,0,39,0.002410888671875,0.42304132221998136
14,42,0,42,0.0025877952575683594,0.4063780691579256
15,45,0,45,0.0027539730072021484,0.3530784860644457
16,48,0,48,0.002948760986328125,0.3360230322768205
17,51,0,51,0.0031309127807617188,0.2504581101398312
18,54,0,54,0.003337860107421875,0.243588797432846
19,57,0,57,0.0035886764526367188,0.1848838016190087
20,60,0,60,0.0038819313049316406,0.1816862164365556
21,63,0,63,0.004097938537597656,0.15751868498138488
22,66,0,66,0.004323720932006836,0.1561227700654445
23,69,0,69,0.004530906677246094,0.1545808138595481
24,72,0,72,0.00470280647277832,0.12988551246667496
25,75,0,75,0.004971027374267578,0.12719138145398504
26,78,0,78,0.005266904830932617,0.10732356344913943
27,81,0,81,0.005555868148803711,0.10617061691644449
28,84,0,84,0.005786895751953125,0.08117114256989279
29,87,0,87,0.006093740463256836,0.08036303435426277
30,90,0,90,0.0063707828521728516,0.06214829126500654
31,93,0,93,0.006742954254150391,0.061970560300437724
32,96,0,96,0.0069828033447265625,0.061717184794829856
33,99,0,99,0.0071828365325927734,0.06121124869048925
34,102,0,102,0.007505893707275391,0.06084672549290585
35,105,0,105,0.0076999664306640625,0.05856674623062609
36,108,0,108,0.007946968078613281,0.05787597277782032
37,111,0,111,0.008145809173583984,0.05625417319294632
38,114,0,114,0.008436918258666992,0.056038793600903504
39,117,0,117,0.008713960647583008,0.0552963573363964
40,120,0,120,0.008965730667114258,0.05497342971114778
41,123,0,123,0.009103775024414062,0.05316345066299052
42,126,0,126,0.009258031845092773,0.05283932785082342
43,129,0,129,0.009516716003417969,0.05118715449481558
44,132,0,132,0.009733915328979492,0.05086263778902649
45,135,0,135,0.009911775588989258,0.04993084800057317
46,138,0,138,0.01013493537902832,0.049738277962689266
47,141,0,141,0.010326862335205078,0.04952828116935226
48,144,0,144,0.010498762130737305,0.048005372968441117
49,147,0,147,0.010706901550292969,0.04760555149484625
50,150,0,150,0.01094675064086914,0.043664061901952135
51,153,0,153,0.011182785034179688,0.043286005626506883
52,156,0,156,0.01145792007446289,0.039757614613435924
53,159,0,159,0.011671781539916992,0.03957738430879081
54,162,0,162,0.011902809143066406,0.03937412146945766
55,165,0,165,0.012059926986694336,0.037014885460300836
56,168,0,168,0.012419700622558594,0.036594462984156376
57,171,0,171,0.012756824493408203,0.03431368514505277
58,174,0,174,0.013080835342407227,0.03385857369385655
59,177,0,177,0.013355016708374023,0.03346623467796146
60,180,0,180,0.013510942459106445,0.03307048987133748
61,183,0,183,0.013677835464477539,0.03197270026849882
62,186,0,186,0.013883829116821289,0.031638530647653415
63,189,0,189,0.014087915420532227,0.031443130478376685
64,192,0,192,0.014212846755981445,0.030615578352381635
65,195,0,195,0.014351844787597656,0.030398460189068274
66,198,0,198,0.014587879180908203,0.029841110165628425
67,201,0,201,0.014878988265991211,0.02964165001727839
68,204,0,204,0.015160799026489258,0.02877362039134286
69,207,0,207,0.015398740768432617,0.02863060017451247
70,210,0,210,0.015640735626220703,0.028518665137688314
71,213,0,213,0.015851974487304688,0.02817448293810678
72,216,0,216,0.016092777252197266,0.028082674582857358
73,219,0,219,0.016315937042236328,0.027172113701312513
74,222,0,222,0.01654505729675293,0.026994127218704488
75,225,0,225,0.01676797866821289,0.026553638320037903
76,228,0,228,0.01694488525390625,0.026506401763615454
77,231,0,231,0.01724076271057129,0.02644589410096779
78,234,0,234,0.017491817474365234,0.026170206717207118
79,237,0,237,0.017786741256713867,0.026141887556560862
80,240,0,240,0.018077850341796875,0.026102187193532606
81,243,0,243,0.01824188232421875,0.025990502864028896
82,246,0,246,0.018431901931762695,0.025919918560145867
83,249,0,249,0.018684864044189453,0.025808776728355028
84,252,0,252,0.019008874893188477,0.025728034798173878
85,255,0,255,0.01925182342529297,0.025630582685850768
86,258,0,258,0.019450902938842773,0.025573739310599596
87,261,0,261,0.0196688175201416,0.025517507999333403
88,264,0,264,0.01985788345336914,0.025432156512018418
89,267,0,267,0.020048856735229492,0.025371557097750196
90,270,0,270,0.02028179168701172,0.025318874109738747
91,273,0,273,0.020569801330566406,0.02528553751787723
92,276,0,276,0.020825862884521484,0.025251846574996174
93,279,0,279,0.021077871322631836,0.02523550837025913
94,282,0,282,0.021281719207763672,0.0252208078643251
95,285,0,285,0.021575927734375,0.025197849034583816
96,288,0,288,0.021768808364868164,0.025182614111498046
97,291,0,291,0.022122859954833984,0.02517346942198901
98,294,0,294,0.022476673126220703,0.025143602698253276
99,297,0,297,0.022729873657226562,0.025127560802870735
100,300,0,300,0.02291083335876465,0.025112110720254113
101,303,0,303,0.02319788932800293,0.025095403831304774
102,306,0,306,0.023480653762817383,0.025083159218674395
103,309,0,309,0.02378702163696289,0.02504628132956202
104,312,0,312,0.024096965789794922,0.025021791284194298
105,315,0,315,0.0243227481842041,0.02499549537126386
106,318,0,318,0.024542808532714844,0.024955766978176957
107,321,0,321,0.02478790283203125,0.024927569223363782
108,324,0,324,0.025052785873413086,0.024873251026084023
109,327,0,327,0.02532792091369629,0.02483117438201841
110,330,0,330,0.02557063102722168,0.024802542681656242
111,333,0,333,0.02580881118774414,0.024762008284843512
112,336,0,336,0.025966882705688477,0.02472768088995884
113,339,0,339,0.026113033294677734,0.02467773567790932
114,342,0,342,0.02629566192626953,0.024643813251676697
115,345,0,345,0.026472806930541992,0.02453568678621926
116,348,0,348,0.02664780616760254,0.0244479614223705
117,351,0,351,0.026793956756591797,0.024395302470059776
118,354,0,354,0.02697277069091797,0.02429422758032637
119,357,0,357,0.027107715606689453,0.024232182118100527
120,360,0,360,0.027310848236083984,0.02414935154256594
121,363,0,363,0.027580976486206055,0.02408134217683946
122,366,0,366,0.027811765670776367,0.023792158203970605
123,369,0,369,0.028010845184326172,0.023743524880489458
124,372,0,372,0.02815389633178711,0.023631701057902157
125,375,0,375,0.02832794189453125,0.02354559180556853
126,378,0,378,0.028461694717407227,0.023480298401048993
127,381,0,381,0.02860283851623535,0.02341560714144463
128,384,0,384,0.028872966766357422,0.023360453467267114
129,387,0,387,0.0290377140045166,0.023288550809439906
130,390,0,390,0.029181957244873047,0.023224436198453064
131,393,0,393,0.029318809509277344,0.02314950180124878
132,396,0,396,0.02948784828186035,0.023051303166809204
133,399,0,399,0.02961897850036621,0.022973566894599378
134,402,0,402,0.029748916625976562,0.022878661811576318
135,405,0,405,0.029878854751586914,0.022784563967565605
136,408,0,408,0.030019760131835938,0.02271956133092542
137,411,0,411,0.030150890350341797,0.02264935160935507
138,414,0,414,0.030282974243164062,0.022570257438016234
139,417,0,417,0.0304110050201416,0.022496087349308084
140,420,0,420,0.03056478500366211,0.022419268835885367
141,423,0,423,0.03069281578063965,0.022329503097322047
142,426,0,426,0.030818700790405273,0.022243094016345673
143,429,0,429,0.0309450626373291,0.02216381450101317
144,432,0,432,0.03106999397277832,0.022062268752559674
145,435,0,435,0.03119492530822754,0.022021834885724144
146,438,0,438,0.03131890296936035,0.022002481088871286
147,441,0,441,0.0315248966217041,0.021970995341113762
148,444,0,444,0.03164982795715332,0.02194510553508341
149,447,0,447,0.03177380561828613,0.02191561996988637
150,450,0,450,0.03189682960510254,0.02186870828014489
151,453,0,453,0.03202080726623535,0.021834491719108208
152,456,0,456,0.03214383125305176,0.021801740734786593
153,459,0,459,0.032266855239868164,0.021703556341402124
154,462,0,462,0.03239083290100098,0.021643364325623075
155,465,0,465,0.032514095306396484,0.021529592633798614
156,468,0,468,0.03263688087463379,0.021473785987925927
157,471,0,471,0.0327608585357666,0.021431829106612094
158,474,0,474,0.03288602828979492,0.02131402417332323
159,477,0,477,0.03301501274108887,0.021217851957133695
160,480,0,480,0.033124685287475586,0.02096710207125097
161,483,0,483,0.033247947692871094,0.02089958024088399
162,486,0,486,0.033386945724487305,0.020748329468738103
163,489,0,489,0.033496856689453125,0.02037272088185245
164,492,0,492,0.03377270698547363,0.02028442092042225
165,495,0,495,0.03392195701599121,0.020031660322192776
166,498,0,498,0.03420376777648926,0.019881224350753082
167,501,0,501,0.03450584411621094,0.019689611615161723
168,504,0,504,0.0346529483795166,0.0193546674431722
169,507,0,507,0.03478503227233887,0.019225821673965297
170,510,0,510,0.0349428653717041,0.018668064250054447
171,513,0,513,0.03511381149291992,0.018554241262523204
172,516,0,516,0.035240888595581055,0.018430936036658317
173,519,0,519,0.035388946533203125,0.01807303069025801
174,522,0,522,0.0355687141418457,0.017990033847900284
175,525,0,525,0.03571200370788574,0.01780320114737578
176,528,0,528,0.03583884239196777,0.017727784445290544
177,531,0,531,0.03595280647277832,0.01748739513415375
178,534,0,534,0.036078691482543945,0.017399471685760268
179,537,0,537,0.03619194030761719,0.016997466152534602
180,540,0,540,0.03632473945617676,0.01677723495704939
181,543,0,543,0.03645181655883789,0.016582765830698766
182,546,0,546,0.036563873291015625,0.01597712497027778
183,549,0,549,0.03673291206359863,0.01583628255694669
184,552,0,552,0.03686189651489258,0.015468644680974634
185,555,0,555,0.03713202476501465,0.015344696378623006
186,558,0,558,0.037282705307006836,0.01490479770649758
187,561,0,561,0.03743267059326172,0.014856893665414532
188,564,0,564,0.03757476806640625,0.014803709398303729
189,567,0,567,0.037735939025878906,0.014531536848877369
190,570,0,570,0.03786587715148926,0.014482457077822
191,573,0,573,0.037987709045410156,0.014103984559127276
192,576,0,576,0.03811788558959961,0.013987340283889534
193,579,0,579,0.03825187683105469,0.013628385313621798
194,582,0,582,0.03840994834899902,0.013540634903027664
195,585,0,585,0.03856468200683594,0.013443480008777086
196,588,0,588,0.03870582580566406,0.012864248654926132
197,591,0,591,0.038829803466796875,0.012767007828161632
198,594,0,594,0.03894186019897461,0.01204096748764811
199,597,0,597,0.03906679153442383,0.011913309810325016
200,600,0,600,0.03917694091796875,0.011708014143305315
201,603,0,603,0.039302825927734375,0.011498114632789096
202,606,0,606,0.0394139289855957,0.010147170594668804
203,609,0,609,0.03958296775817871,0.010060162179875206
204,612,0,612,0.03971672058105469,0.009928296622471241
205,615,0,615,0.039830923080444336,0.009289147232938178
206,618,0,618,0.03995680809020996,0.009037974374775498
207,621,0,621,0.040100812911987305,0.007798818856907483
208,624,0,624,0.040230751037597656,0.007439183102129483
209,627,0,627,0.04041767120361328,0.006771607210422805
210,630,0,630,0.040573835372924805,0.0064380246134818275
211,633,0,633,0.04069781303405762,0.005807684565014071
212,636,0,636,0.04083395004272461,0.005608037516448095
213,639,0,639,0.04096674919128418,0.004848426588293971
214,642,0,642,0.04110884666442871,0.004722885208239441
215,645,0,645,0.041237831115722656,0.004563547862102925
216,648,0,648,0.04134988784790039,0.0038164094715552404
217,651,0,651,0.041475772857666016,0.0036820084435547334
218,654,0,654,0.041589975357055664,0.0029610357650605105
219,657,0,657,0.04171586036682129,0.0029405069232614944
220,660,0,660,0.041841745376586914,0.0029126332474896646
221,663,0,663,0.04195380210876465,0.0025121133007097412
222,666,0,666,0.042079925537109375,0.0024786491016706457
223,669,0,669,0.042192935943603516,0.0024060602926836722
224,672,0,672,0.04232287406921387,0.002389661701162551
225,675,0,675,0.04251289367675781,0.0023739151853355805
226,678,0,678,0.04269075393676758,0.002271935821227873
227,681,0,681,0.04290199279785156,0.002259458642279899
228,684,0,684,0.043103933334350586,0.0022353958969186394
229,687,0,687,0.043260812759399414,0.0021989164383788306
230,690,0,690,0.04355883598327637,0.0021793748642264027
231,693,0,693,0.04378986358642578,0.002155194368267689
232,696,0,696,0.04401683807373047,0.0020791240438363732
233,699,0,699,0.04417991638183594,0.0020577628265549797
234,702,0,702,0.044304847717285156,0.0019950365447417152
235,705,0,705,0.0444798469543457,0.0019769965066787514
236,708,0,708,0.044606924057006836,0.0019353349319477457
237,711,0,711,0.04473090171813965,0.0019191826040866303
238,714,0,714,0.04484200477600098,0.001888856817355782
239,717,0,717,0.044966936111450195,0.0018786599253796886
240,720,0,720,0.04507803916931152,0.001795540515409886
241,723,0,723,0.04519987106323242,0.0017725790255446994
242,726,0,726,0.045323848724365234,0.0017492477819463503
243,729,0,729,0.04543781280517578,0.0016875118149609243
244,732,0,732,0.04556083679199219,0.0016713294859251966
245,735,0,735,0.04567074775695801,0.001581409893831218
246,738,0,738,0.045793771743774414,0.0015538296816191928
247,741,0,741,0.04590272903442383,0.0014396185953860167
248,744,0,744,0.046025991439819336,0.0014157581416735492
249,747,0,747,0.04613685607910156,0.0013106844058561682
250,750,0,750,0.046260833740234375,0.001276968698954737
251,753,0,753,0.04636979103088379,0.0011658765079819557
252,756,0,756,0.04649186134338379,0.001138529096308344
253,759,0,759,0.0466008186340332,0.0011121243291445104
254,762,0,762,0.0467226505279541,0.0010907506895613411
255,765,0,765,0.04683279991149902,0.0010030766399126893
256,768,0,768,0.04695606231689453,0.0009777920832235577
257,771,0,771,0.047064781188964844,0.0009263723615043483
258,774,0,774,0.047186851501464844,0.0009053277420171519
259,777,0,777,0.047297000885009766,0.0008138726642452717
260,780,0,780,0.04741978645324707,0.0008031956633546212
261,783,0,783,0.04754376411437988,0.0007883696252152073
262,786,0,786,0.0476527214050293,0.0007570596692707624
263,789,0,789,0.047775983810424805,0.0007450505446718422
264,792,0,792,0.04788470268249512,0.0006877589601576199
265,795,0,795,0.04800677299499512,0.000679919969369227
266,798,0,798,0.04813075065612793,0.0006686907258497329
267,801,0,801,0.048239707946777344,0.0006468129837028057
268,804,0,804,0.04836392402648926,0.0006383698810960447
269,807,0,807,0.04848480224609375,0.0005856127369623604
270,810,0,810,0.048609018325805664,0.0005777780801530086
271,813,0,813,0.04871773719787598,0.0005641514628013675
272,816,0,816,0.04886984825134277,0.0005547513988151061
273,819,0,819,0.04898571968078613,0.0005133030671912891
274,822,0,822,0.049243927001953125,0.0005036948699008166
275,825,0,825,0.04939889907836914,0.00048801940452449167
276,828,0,828,0.04965090751647949,0.00048069579109244373
277,831,0,831,0.04982185363769531,0.0004617756082297141
278,834,0,834,0.04998970031738281,0.00045338818410491587
279,837,0,837,0.050192832946777344,0.00040742875251356165
280,840,0,840,0.050351858139038086,0.00040334471791691426
281,843,0,843,0.05048489570617676,0.0003985425034542327
282,846,0,846,0.05060100555419922,0.00038447726664953886
283,849,0,849,0.05075669288635254,0.00038167215289157554
284,852,0,852,0.050868988037109375,0.0003745399231633024
285,855,0,855,0.050992727279663086,0.0003728373732318537
286,858,0,858,0.051117658615112305,0.00037027010237503517
287,861,0,861,0.05123782157897949,0.0003653886958208418
288,864,0,864,0.051364898681640625,0.0003646619204055766
289,867,0,867,0.05148887634277344,0.0003636720082223627
290,870,0,870,0.05159783363342285,0.0003580193141365563
291,873,0,873,0.051721811294555664,0.00035754488226648763
292,876,0,876,0.05184483528137207,0.00035604326487280935
293,879,0,879,0.05196690559387207,0.0003552820765292755
294,882,0,882,0.05212283134460449,0.0003546402603055537
295,885,0,885,0.05225086212158203,0.00035366510153071105
296,888,0,888,0.052403926849365234,0.00035242628924004053
297,891,0,891,0.05257296562194824,0.000350389167267697
298,894,0,894,0.052754878997802734,0.00034941900474488386
299,897,0,897,0.05293583869934082,0.00034833502583343117
300,900,0,900,0.053117990493774414,0.0003471539689233926
301,903,0,903,0.05327486991882324,0.0003461069996420504
302,906,0,906,0.053540706634521484,0.00034485623981708236
303,909,0,909,0.053740739822387695,0.0003437307546062037
304,912,0,912,0.05393385887145996,0.0003424991684555577
305,915,0,915,0.054086923599243164,0.0003416071686626504
306,918,0,918,0.05424690246582031,0.0003406744408411139
307,921,0,921,0.05437493324279785,0.0003390407860549198
308,924,0,924,0.05450272560119629,0.0003377393203449173
309,927,0,927,0.05463385581970215,0.0003361503734998821
310,930,0,930,0.05477285385131836,0.00033411700995919204
311,933,0,933,0.05489778518676758,0.0003302813477793745
312,936,0,936,0.05502676963806152,0.00032955788805494866
313,939,0,939,0.05515480041503906,0.0003287122109173515
314,942,0,942,0.05526876449584961,0.000321963335618328
315,945,0,945,0.05539584159851074,0.0003205389017663497
316,948,0,948,0.05558300018310547,0.0003169888704945883
317,951,0,951,0.05578494071960449,0.0003147813820029535
318,954,0,954,0.05593395233154297,0.00031126882785723395
319,957,0,957,0.0561368465423584,0.00030782615814854724
320,960,0,960,0.056302785873413086,0.0003053311217874906
321,963,0,963,0.05647587776184082,0.0002873794577962101
322,966,0,966,0.056619882583618164,0.00028383977945179074
323,969,0,969,0.05675387382507324,0.00028045437987531
324,972,0,972,0.05689692497253418,0.00027305566081222413
325,975,0,975,0.057022809982299805,0.0002706400940107079
326,978,0,978,0.05713367462158203,0.0002496205298900962
327,981,0,981,0.05726003646850586,0.00024735247862187087
328,984,0,984,0.05738496780395508,0.0002450661053468627
329,987,0,987,0.0574948787689209,0.00023755024564943073
330,990,0,990,0.05761981010437012,0.0002342997979185247
331,993,0,993,0.05773282051086426,0.0002156680666401115
332,996,0,996,0.05786275863647461,0.0002137792103492424
333,999,0,999,0.05798983573913574,0.00021093303549978308
334,1002,0,1002,0.05810379981994629,0.0002052857359565925
335,1005,0,1005,0.05822896957397461,0.00020297631481599134
336,1008,0,1008,0.05833768844604492,0.00017944174935594876
337,1011,0,1011,0.058461904525756836,0.00017781928547857615
338,1014,0,1014,0.05858588218688965,0.00017527813320914948
339,1017,0,1017,0.05869579315185547,0.00017086867701915695
340,1020,0,1020,0.058818817138671875,0.00016944172474491512
341,1023,0,1023,0.058928728103637695,0.00016538127617032427
342,1026,0,1026,0.0590519905090332,0.00016453811594551246
343,1029,0,1029,0.059160709381103516,0.0001582069992081658
344,1032,0,1032,0.059282779693603516,0.00015749191708308054
345,1035,0,1035,0.059407711029052734,0.0001562786172554505
346,1038,0,1038,0.059517860412597656,0.00014831375879404026
347,1041,0,1041,0.05964064598083496,0.0001473331948686196
348,1044,0,1044,0.059764862060546875,0.00014612661799732804
349,1047,0,1047,0.059874773025512695,0.00013956994382541594
350,1050,0,1050,0.0599977970123291,0.00013816837122184074
351,1053,0,1053,0.06010794639587402,0.00013587130960121733
352,1056,0,1056,0.06023073196411133,0.00013386704570531822
353,1059,0,1059,0.060353994369506836,0.0001323824864778186
354,1062,0,1062,0.06047797203063965,0.000130500867537565
355,1065,0,1065,0.06058788299560547,0.00012687386910669452
356,1068,0,1068,0.06070971488952637,0.00012584653892880307
357,1071,0,1071,0.06081891059875488,0.000122729940198746
358,1074,0,1074,0.060942888259887695,0.00012163709753396291
359,1077,0,1077,0.06105494499206543,0.00011835505913689887
360,1080,0,1080,0.06117892265319824,0.00011709411385093045
361,1083,0,1083,0.061287879943847656,0.00011260346616330967
362,1086,0,1086,0.06141066551208496,0.00011136128961988742
363,1089,0,1089,0.06153392791748047,0.0001102712720820973
364,1092,0,1092,0.061644792556762695,0.00010740350059308273
365,1095,0,1095,0.061769962310791016,0.00010606170858596582
366,1098,0,1098,0.06187796592712402,9.493861115296948e-05
367,1101,0,1101,0.06200075149536133,9.410932119757338e-05
368,1104,0,1104,0.06211090087890625,9.149949919118264e-05
369,1107,0,1107,0.062233686447143555,9.12326808730798e-05
370,1110,0,1110,0.06235790252685547,9.063651554783372e-05
371,1113,0,1113,0.06246685981750488,8.907695777426199e-05
372,1116,0,1116,0.06258893013000488,8.864333679455222e-05
373,1119,0,1119,0.06269693374633789,8.765705687823727e-05
374,1122,0,1122,0.06281876564025879,8.718416483700463e-05
375,1125,0,1125,0.0629277229309082,8.611842616979282e-05
376,1128,0,1128,0.0630500316619873,8.567817365344254e-05
377,1131,0,1131,0.06315898895263672,8.445428282536194e-05
378,1134,0,1134,0.06339383125305176,8.397378451481702e-05
379,1137,0,1137,0.06359505653381348,8.062995061644358e-05
380,1140,0,1140,0.06378698348999023,8.007154488007144e-05
381,1143,0,1143,0.06398797035217285,7.93954451013272e-05
382,1146,0,1146,0.0642387866973877,7.828910878533084e-05
383,1149,0,1149,0.06439661979675293,7.800838947045971e-05
384,1152,0,1152,0.06460785865783691,7.568351300168425e-05
385,1155,0,1155,0.06475377082824707,7.507102019140092e-05
386,1158,0,1158,0.06488776206970215,7.432101358623298e-05
387,1161,0,1161,0.06502199172973633,7.037097153559025e-05
388,1164,0,1164,0.06516098976135254,6.990106247787673e-05
389,1167,0,1167,0.06527185440063477,6.811014655328312e-05
390,1170,0,1170,0.06539797782897949,6.75449911818466e-05
391,1173,0,1173,0.06551289558410645,6.455426542920744e-05
392,1176,0,1176,0.06563782691955566,6.417545401665236e-05
393,1179,0,1179,0.06574892997741699,6.352052560021441e-05
394,1182,0,1182,0.06587386131286621,6.29200219054163e-05
395,1185,0,1185,0.06598401069641113,5.968958503523085e-05
396,1188,0,1188,0.06610774993896484,5.9206987236248936e-05
397,1191,0,1191,0.06621885299682617,5.857258543205062e-05
398,1194,0,1194,0.06634283065795898,5.804224715006852e-05
399,1197,0,1197,0.06645393371582031,5.741872726790468e-05
400,1200,0,1200,0.06657791137695312,5.689511853590122e-05
401,1203,0,1203,0.06669187545776367,5.4351482534800625e-05
402,1206,0,1206,0.06683492660522461,5.413588863501726e-05
403,1209,0,1209,0.06699180603027344,5.3568641499623935e-05
404,1212,0,1212,0.06710195541381836,5.257948720994101e-05
405,1215,0,1215,0.06722688674926758,5.2302809124432265e-05
406,1218,0,1218,0.0673367977142334,4.991825009319234e-05
407,1221,0,1221,0.06746077537536621,4.95479306668863e-05
408,1224,0,1224,0.06758499145507812,4.892937796985905e-05
409,1227,0,1227,0.06769585609436035,4.8251071027781776e-05
410,1230,0,1230,0.06781888008117676,4.780695322159361e-05
411,1233,0,1233,0.06793761253356934,4.704287567673822e-05
412,1236,0,1236,0.06806302070617676,4.662778494282435e-05
413,1239,0,1239,0.06817364692687988,4.487921423160235e-05
414,1242,0,1242,0.0682978630065918,4.445908513141862e-05
415,1245,0,1245,0.06842279434204102,4.396208100942105e-05
416,1248,0,1248,0.06853294372558594,4.14695795170196e-05
417,1251,0,1251,0.0686798095703125,4.0682847919018555e-05
418,1254,0,1254,0.06882786750793457,3.718703757338697e-05
419,1257,0,1257,0.0689847469329834,3.6617745089356084e-05
420,1260,0,1260,0.06909584999084473,3.59427517403704e-05
421,1263,0,1263,0.06921982765197754,3.53202086245103e-05
422,1266,0,1266,0.06932973861694336,3.3826333083432856e-05
423,1269,0,1269,0.06945276260375977,3.357018294960088e-05
424,1272,0,1272,0.06957793235778809,3.313856717836052e-05
425,1275,0,1275,0.06968879699707031,3.2020948124033164e-05
426,1278,0,1278,0.06981396675109863,3.17855805349324e-05
427,1281,0,1281,0.06992387771606445,3.1098323932660256e-05
428,1284,0,1284,0.07004785537719727,3.09160143624036e-05
429,1287,0,1287,0.07017087936401367,3.0594039807190176e-05
430,1290,0,1290,0.07028079032897949,3.002832395478796e-05
431,1293,0,1293,0.0704047679901123,2.9780895166355625e-05
432,1296,0,1296,0.07051491737365723,2.921318786155365e-05
433,1299,0,1299,0.07063889503479004,2.9087334416863025e-05
434,1302,0,1302,0.07074880599975586,2.8116181537577776e-05
435,1305,0,1305,0.07087278366088867,2.802663835033805e-05
436,1308,0,1308,0.07099580764770508,2.7917382575351983e-05
437,1311,0,1311,0.0711207389831543,2.7715544890866593e-05
438,1314,0,1314,0.07124471664428711,2.7559764347458856e-05
439,1317,0,1317,0.07135486602783203,2.7270496280320738e-05
440,1320,0,1320,0.07147908210754395,2.7173801053796204e-05
441,1323,0,1323,0.07158780097961426,2.66805593335359e-05
442,1326,0,1326,0.07171201705932617,2.6613795486854273e-05
443,1329,0,1329,0.07183575630187988,2.6546507164924464e-05
444,1332,0,1332,0.0719449520111084,2.6249015940880735e-05
445,1335,0,1335,0.07206869125366211,2.6179997372188878e-05
446,1338,0,1338,0.07219290733337402,2.6060515186280085e-05
447,1341,0,1341,0.07230281829833984,2.5638393592713574e-05
448,1344,0,1344,0.07242584228515625,2.555999828446608e-05
449,1347,0,1347,0.07253575325012207,2.4902897275752626e-05
450,1350,0,1350,0.07265996932983398,2.483257427602559e-05
451,1353,0,1353,0.07280087471008301,2.4743848009171588e-05
452,1356,0,1356,0.07294487953186035,2.4064204764034042e-05
453,1359,0,1359,0.07307291030883789,2.395108000187263e-05
454,1362,0,1362,0.07320690155029297,2.3666408146311795e-05
455,1365,0,1365,0.07333564758300781,2.3519575642357525e-05
456,1368,0,1368,0.0735468864440918,2.343053161453993e-05
457,1371,0,1371,0.07370591163635254,2.3009714896874774e-05
458,1374,0,1374,0.07384395599365234,2.2834545596203818e-05
459,1377,0,1377,0.07396292686462402,2.212340847368128e-05
460,1380,0,1380,0.07409477233886719,2.2000233868948915e-05
461,1383,0,1383,0.07425379753112793,2.184097062522706e-05
462,1386,0,1386,0.07436800003051758,2.148222970629813e-05
463,1389,0,1389,0.07449483871459961,2.134992482239976e-05
464,1392,0,1392,0.07460689544677734,2.1028098708323825e-05
465,1395,0,1395,0.07473278045654297,2.0904100665737893e-05
466,1398,0,1398,0.0748589038848877,2.0736446399223094e-05
467,1401,0,1401,0.07496881484985352,2.007041198970582e-05
468,1404,0,1404,0.07509398460388184,1.9894851845491257e-05
469,1407,0,1407,0.07520484924316406,1.851205388335129e-05
470,1410,0,1410,0.07533788681030273,1.83781361144113e-05
471,1413,0,1413,0.07546591758728027,1.809277430826064e-05
472,1416,0,1416,0.07557988166809082,1.7000340768903357e-05
473,1419,0,1419,0.07570886611938477,1.6769251433575103e-05
474,1422,0,1422,0.07582378387451172,1.5188824789919228e-05
475,1425,0,1425,0.07594966888427734,1.5006361415023809e-05
476,1428,0,1428,0.07605981826782227,1.4658094661448506e-05
477,1431,0,1431,0.07618379592895508,1.4403163400369987e-05
478,1434,0,1434,0.0762948989868164,1.332126050764602e-05
479,1437,0,1437,0.07641792297363281,1.3138806584213654e-05
480,1440,0,1440,0.07652783393859863,1.2703713675676636e-05
481,1443,0,1443,0.07665085792541504,1.2497762387627942e-05
482,1446,0,1446,0.07675981521606445,1.1877892404848101e-05
483,1449,0,1449,0.07688498497009277,1.178922401118293e-05
484,1452,0,1452,0.07700991630554199,1.168149788583275e-05
485,1455,0,1455,0.0771188735961914,1.1381100495495428e-05
486,1458,0,1458,0.07724189758300781,1.1313739015389735e-05
487,1461,0,1461,0.07735085487365723,1.1070581898952227e-05
488,1464,0,1464,0.07747364044189453,1.1023952356034623e-05
489,1467,0,1467,0.07759690284729004,1.0974874490689117e-05
490,1470,0,1470,0.07770586013793945,1.079422987168599e-05
491,1473,0,1473,0.07782983779907227,1.0768295395106556e-05
492,1476,0,1476,0.07802796363830566,1.0720401065791806e-05
493,1479,0,1479,0.07817769050598145,1.068013626265946e-05
494,1482,0,1482,0.07831382751464844,1.0653518259913007e-05
495,1485,0,1485,0.07853269577026367,1.0612249949750192e-05
496,1488,0,1488,0.07877683639526367,1.0579985903698328e-05
497,1491,0,1491,0.07893180847167969,1.0561478928089496e-05
498,1494,0,1494,0.07916903495788574,1.0540449649208203e-05
499,1497,0,1497,0.07936477661132812,1.0526670491404508e-05
500,1500,0,1500,0.07953476905822754,1.0514244864894189e-05
501,1503,0,1503,0.07973384857177734,1.0480862552111934e-05
502,1506,0,1506,0.07988095283508301,1.0453614453537054e-05
503,1509,0,1509,0.0800168514251709,1.0432094353314266e-05
504,1512,0,1512,0.0801689624786377,1.0383829410311021e-05
505,1515,0,1515,0.08031368255615234,1.0327183654508196e-05
506,1518,0,1518,0.08044290542602539,1.0281450555197764e-05
507,1521,0,1521,0.08055663108825684,1.0139555167374788e-05
508,1524,0,1524,0.08068466186523438,1.0120858405251394e-05
509,1527,0,1527,0.08081269264221191,1.0074976633375055e-05
510,1530,0,1530,0.08094072341918945,1.003919780069679e-05
511,1533,0,1533,0.08106875419616699,1.000959213675731e-05
512,1536,0,1536,0.08118295669555664,9.906697991286027e-06
513,1539,0,1539,0.08131098747253418,9.871768146755468e-06
514,1542,0,1542,0.08143782615661621,9.814237005724638e-06
515,1545,0,1545,0.08156585693359375,9.741568204947319e-06
516,1548,0,1548,0.08169293403625488,9.68293883659254e-06
517,1551,0,1551,0.08180475234985352,9.48344626895615e-06
518,1554,0,1554,0.08193278312683105,9.427120735607736e-06
519,1557,0,1557,0.08206582069396973,9.339078118413334e-06
520,1560,0,1560,0.08217978477478027,9.129446320633113e-06
521,1563,0,1563,0.08231782913208008,9.066193444449166e-06
522,1566,0,1566,0.08243203163146973,8.542784674912371e-06
523,1569,0,1569,0.08256101608276367,8.461794929541228e-06
524,1572,0,1572,0.0826728343963623,8.319123373705684e-06
525,1575,0,1575,0.08279991149902344,8.189966554596326e-06
526,1578,0,1578,0.08291482925415039,7.938378494323898e-06
527,1581,0,1581,0.08304095268249512,7.85270321106863e-06
528,1584,0,1584,0.08315396308898926,7.615761326995724e-06
529,1587,0,1587,0.08328080177307129,7.566115789702946e-06
530,1590,0,1590,0.08340787887573242,7.473898798137073e-06
531,1593,0,1593,0.08351993560791016,7.121663159005809e-06
532,1596,0,1596,0.08364701271057129,7.0350556662566405e-06
533,1599,0,1599,0.08375883102416992,6.634549970611506e-06
534,1602,0,1602,0.08388471603393555,6.5648079513017055e-06
535,1605,0,1605,0.08401203155517578,6.485456089196467e-06
536,1608,0,1608,0.08412384986877441,6.3112865986146096e-06
537,1611,0,1611,0.08424973487854004,6.244419744555582e-06
538,1614,0,1614,0.08436298370361328,6.057939989149085e-06
539,1617,0,1617,0.08448982238769531,5.978519675984361e-06
540,1620,0,1620,0.08460283279418945,5.747701979783532e-06
541,1623,0,1623,0.08472967147827148,5.6899362161785965e-06
542,1626,0,1626,0.08484292030334473,5.447357407802517e-06
543,1629,0,1629,0.08497095108032227,5.390280292139356e-06
544,1632,0,1632,0.0850827693939209,5.33458692688825e-06
545,1635,0,1635,0.08520770072937012,5.247433828914395e-06
546,1638,0,1638,0.08532571792602539,4.963920187182699e-06
547,1641,0,1641,0.08545279502868652,4.935816527436838e-06
548,1644,0,1644,0.08557581901550293,4.877300384720961e-06
549,1647,0,1647,0.08570289611816406,4.856584697727898e-06
550,1650,0,1650,0.08581399917602539,4.787127106934944e-06
551,1653,0,1653,0.08593988418579102,4.754661478384586e-06
552,1656,0,1656,0.08605074882507324,4.7020723478415535e-06
553,1659,0,1659,0.08617591857910156,4.6576016130149145e-06
554,1662,0,1662,0.0862877368927002,4.5255047154382646e-06
555,1665,0,1665,0.08641386032104492,4.50335176413489e-06
556,1668,0,1668,0.08652591705322266,4.377245211545457e-06
557,1671,0,1671,0.08664870262145996,4.353083861001177e-06
558,1674,0,1674,0.0867609977722168,4.267632519066496e-06
559,1677,0,1677,0.08688592910766602,4.257266447888737e-06
560,1680,0,1680,0.08701086044311523,4.24586610392595e-06
561,1683,0,1683,0.08712291717529297,4.1922442982543435e-06
562,1686,0,1686,0.087249755859375,4.164565216933406e-06
563,1689,0,1689,0.08736276626586914,4.0627544224095145e-06
564,1692,0,1692,0.08748793601989746,4.0308017985726785e-06
565,1695,0,1695,0.0876007080078125,3.9051954457590014e-06
566,1698,0,1698,0.08772683143615723,3.88149284454093e-06
567,1701,0,1701,0.08785271644592285,3.842988626282019e-06
568,1704,0,1704,0.08796477317810059,3.67634802694527e-06
569,1707,0,1707,0.08809089660644531,3.6300423117007654e-06
570,1710,0,1710,0.08820199966430664,3.5659625382267923e-06
571,1713,0,1713,0.08832788467407227,3.522275414359392e-06
572,1716,0,1716,0.08844685554504395,3.1142536410305417e-06
573,1719,0,1719,0.08857274055480957,3.0876324259638025e-06
574,1722,0,1722,0.0886998176574707,3.050781075846206e-06
575,1725,0,1725,0.08881187438964844,2.9370048496497498e-06
576,1728,0,1728,0.08893799781799316,2.8956585755234755e-06
577,1731,0,1731,0.0890507698059082,2.5201013446343947e-06
578,1734,0,1734,0.08917784690856934,2.480856765413722e-06
579,1737,0,1737,0.08930373191833496,2.4377146675028232e-06
580,1740,0,1740,0.0894157886505127,2.3487036856845756e-06
581,1743,0,1743,0.08967781066894531,2.304146731329825e-06
582,1746,0,1746,0.08986878395080566,2.141113010898445e-06
583,1749,0,1749,0.09001684188842773,2.104159097598349e-06
584,1752,0,1752,0.09018802642822266,2.078975692016625e-06
585,1755,0,1755,0.0903177261352539,2.0489789969381862e-06
586,1758,0,1758,0.09043097496032715,1.9308915774687576e-06
587,1761,0,1761,0.09055685997009277,1.8888155204441244e-06
588,1764,0,1764,0.0906679630279541,1.8254026365347645e-06
589,1767,0,1767,0.09079194068908691,1.7809128169520266e-06
590,1770,0,1770,0.09090304374694824,1.6903395538873396e-06
591,1773,0,1773,0.09102797508239746,1.6724855426998167e-06
592,1776,0,1776,0.09113883972167969,1.597893584101788e-06
593,1779,0,1779,0.09126591682434082,1.5778952182164914e-06
594,1782,0,1782,0.09139084815979004,1.553795663214016e-06
595,1785,0,1785,0.09150171279907227,1.5077917185201388e-06
596,1788,0,1788,0.09162592887878418,1.486345535819349e-06
597,1791,0,1791,0.09174084663391113,1.4331034339873865e-06
598,1794,0,1794,0.09186577796936035,1.4178831019553621e-06
599,1797,0,1797,0.09197783470153809,1.334931362682562e-06
600,1800,0,1800,0.0921018123626709,1.3196739032290732e-06
601,1803,0,1803,0.09221196174621582,1.2806929660408013e-06
602,1806,0,1806,0.09233474731445312,1.2678075755247928e-06
603,1809,0,1809,0.09244585037231445,1.2187863212887098e-06
604,1812,0,1812,0.09256696701049805,1.2018853948504827e-06
605,1815,0,1815,0.09267783164978027,1.142981630960781e-06
606,1818,0,1818,0.09280085563659668,1.1309435668483667e-06
607,1821,0,1821,0.0929098129272461,1.1075667523477279e-06
608,1824,0,1824,0.0930318832397461,1.091871054534579e-06
609,1827,0,1827,0.09314203262329102,1.0647897201865661e-06
610,1830,0,1830,0.09326577186584473,1.052769509436384e-06
611,1833,0,1833,0.09337592124938965,1.0246695715877961e-06
612,1836,0,1836,0.09349775314331055,1.0065266590498897e-06
613,1839,0,1839,0.09379100799560547,9.451293214132315e-07
614,1842,0,1842,0.09396195411682129,9.369172979022515e-07
615,1845,0,1845,0.09411096572875977,9.177204694151453e-07
616,1848,0,1848,0.09433865547180176,9.05439941730272e-07
617,1851,0,1851,0.09448695182800293,8.956723182228203e-07
618,1854,0,1854,0.09471797943115234,8.757670101724319e-07
619,1857,0,1857,0.09489083290100098,8.686586157276519e-07
620,1860,0,1860,0.09502577781677246,8.105233258376966e-07
621,1863,0,1863,0.09516072273254395,8.060193815809518e-07
622,1866,0,1866,0.09532475471496582,7.985708169669114e-07
623,1869,0,1869,0.09544587135314941,7.803642111780212e-07
624,1872,0,1872,0.09557676315307617,7.741950025859118e-07
625,1875,0,1875,0.0956888198852539,7.509030204247773e-07
626,1878,0,1878,0.09581494331359863,7.469743305182896e-07
627,1881,0,1881,0.09594082832336426,7.407905387481744e-07
628,1884,0,1884,0.0960688591003418,7.288915961145239e-07
629,1887,0,1887,0.0962066650390625,7.238632782735467e-07
630,1890,0,1890,0.09638285636901855,7.017523018753157e-07
631,1893,0,1893,0.09653186798095703,6.93221074415942e-07
632,1896,0,1896,0.09665679931640625,6.726598601977193e-07
633,1899,0,1899,0.09679269790649414,6.631383050016196e-07
634,1902,0,1902,0.09691286087036133,6.488408200292809e-07
635,1905,0,1905,0.09707069396972656,6.391342064434182e-07
636,1908,0,1908,0.0971839427947998,6.044912244945665e-07
637,1911,0,1911,0.09731101989746094,5.963562342177389e-07
638,1914,0,1914,0.09743881225585938,5.869670456715973e-07
639,1917,0,1917,0.09763383865356445,5.337227197567524e-07
640,1920,0,1920,0.09778571128845215,5.235926006610697e-07
641,1923,0,1923,0.09790897369384766,4.4562566527019504e-07
642,1926,0,1926,0.09804892539978027,4.3643161727454984e-07
643,1929,0,1929,0.09816694259643555,4.2754975899982754e-07
644,1932,0,1932,0.09832501411437988,4.195321654358544e-07
645,1935,0,1935,0.09843778610229492,3.972735254550833e-07
646,1938,0,1938,0.09856486320495605,3.889306508671243e-07
647,1941,0,1941,0.0986790657043457,3.757354132471679e-07
648,1944,0,1944,0.09880971908569336,3.6479953319590616e-07
649,1947,0,1947,0.0989229679107666,3.5397751144153776e-07
650,1950,0,1950,0.09904885292053223,3.4574217712243097e-07
651,1953,0,1953,0.09916281700134277,3.0839232424262145e-07
652,1956,0,1956,0.09929704666137695,3.032714598009238e-07
653,1959,0,1959,0.0994119644165039,2.9655806056125473e-07
654,1962,0,1962,0.09953784942626953,2.9187056950664935e-07
655,1965,0,1965,0.09964895248413086,2.8367136581971097e-07
656,1968,0,1968,0.09977483749389648,2.779191356235396e-07
657,1971,0,1971,0.09988784790039062,2.663606803958667e-07
658,1974,0,1974,0.10001373291015625,2.634969774830356e-07
659,1977,0,1977,0.10012578964233398,2.5985649167913903e-07
660,1980,0,1980,0.1002497673034668,2.5673105788409346e-07
661,1983,0,1983,0.10036087036132812,2.284331687738653e-07
662,1986,0,1986,0.10048675537109375,2.25708243709346e-07
663,1989,0,1989,0.1006007194519043,2.2243745164840175e-07
664,1992,0,1992,0.10072588920593262,2.19045679276488e-07
665,1995,0,1995,0.10083675384521484,1.95535731497816e-07
666,1998,0,1998,0.10096263885498047,1.926756422942705e-07
667,2001,0,2001,0.1010737419128418,1.8686589245890332e-07
668,2004,0,2004,0.10124802589416504,1.8353793517517469e-07
669,2007,0,2007,0.1013638973236084,1.799781275796748e-07
670,2010,0,2010,0.10149097442626953,1.758267463744407e-07
671,2013,0,2013,0.10160183906555176,1.7008543249257794e-07
672,2016,0,2016,0.10172796249389648,1.6806176608833155e-07
673,2019,0,2019,0.10184288024902344,1.6409174052122677e-07
674,2022,0,2022,0.10197567939758301,1.6285678540575782e-07
675,2025,0,2025,0.10210299491882324,1.610971591947247e-07
676,2028,0,2028,0.10221576690673828,1.5454722235538694e-07
677,2031,0,2031,0.1023406982421875,1.5393466404292298e-07
678,2034,0,2034,0.10246777534484863,1.529668617689059e-07
679,2037,0,2037,0.10257983207702637,1.514370817304158e-07
680,2040,0,2040,0.1027059555053711,1.5085637353057984e-07
681,2043,0,2043,0.10281705856323242,1.4836731347497793e-07
682,2046,0,2046,0.10294294357299805,1.4773909736791769e-07
683,2049,0,2049,0.10306882858276367,1.4647017712952023e-07
684,2052,0,2052,0.1031947135925293,1.4560774290159201e-07
685,2055,0,2055,0.10332083702087402,1.450942850812771e-07
686,2058,0,2058,0.10344696044921875,1.4446399420517387e-07
687,2061,0,2061,0.10357093811035156,1.4360467118801698e-07
688,2064,0,2064,0.10369682312011719,1.4286908290639438e-07
689,2067,0,2067,0.10382270812988281,1.4233680034158488e-07
690,2070,0,2070,0.10394883155822754,1.413758568760153e-07
691,2073,0,2073,0.10412287712097168,1.4045055245226862e-07
692,2076,0,2076,0.10425281524658203,1.3965998474510557e-07
693,2079,0,2079,0.10437989234924316,1.3911724248433814e-07
694,2082,0,2082,0.1045067310333252,1.3863673105435355e-07
695,2085,0,2085,0.10461997985839844,1.3708035597302682e-07
696,2088,0,2088,0.10474586486816406,1.3650984560687276e-07
697,2091,0,2091,0.1048738956451416,1.3546347429342624e-07
698,2094,0,2094,0.10500097274780273,1.3455462763656953e-07
699,2097,0,2097,0.1051328182220459,1.3373940486023212e-07
700,2100,0,2100,0.10525989532470703,1.3319082166809274e-07
701,2103,0,2103,0.10538697242736816,1.3273009692631637e-07
702,2106,0,2106,0.1055150032043457,1.3181406317403873e-07
703,2109,0,2109,0.10564184188842773,1.3098139913891017e-07
704,2112,0,2112,0.10576987266540527,1.303364849497118e-07
705,2115,0,2115,0.1058969497680664,1.2969984713875086e-07
706,2118,0,2118,0.10601091384887695,1.2823735354902023e-07
707,2121,0,2121,0.10616779327392578,1.2761002987852615e-07
708,2124,0,2124,0.10630679130554199,1.266224218476283e-07
709,2127,0,2127,0.10642194747924805,1.2467941536173984e-07
710,2130,0,2130,0.10657095909118652,1.243552210400254e-07
711,2133,0,2133,0.10669994354248047,1.2367907144872245e-07
712,2136,0,2136,0.10683965682983398,1.228656216816619e-07
713,2139,0,2139,0.10703372955322266,1.2222904975367416e-07
714,2142,0,2142,0.10717988014221191,1.215372383032879e-07
715,2145,0,2145,0.10730695724487305,1.2106399712617807e-07
716,2148,0,2148,0.10743379592895508,1.2073767591690352e-07
717,2151,0,2151,0.10762190818786621,1.2029656506418743e-07
718,2154,0,2154,0.10786676406860352,1.1982427344673527e-07
719,2157,0,2157,0.10804295539855957,1.1925910095525016e-07
720,2160,0,2160,0.10823607444763184,1.1886896385877293e-07
721,2163,0,2163,0.1084449291229248,1.185449581381336e-07
722,2166,0,2166,0.1085970401763916,1.1819838390535132e-07
723,2169,0,2169,0.10876679420471191,1.1783020065426487e-07
724,2172,0,2172,0.10907483100891113,1.1755334965923587e-07
725,2175,0,2175,0.10932302474975586,1.1728741123109292e-07
726,2178,0,2178,0.10954976081848145,1.1707274227819753e-07
727,2181,0,2181,0.10969686508178711,1.1694346508532198e-07
728,2184,0,2184,0.1099557876586914,1.1672783600288433e-07
729,2187,0,2187,0.1102290153503418,1.1653636074722699e-07
730,2190,0,2190,0.11046671867370605,1.1637864293204894e-07
731,2193,0,2193,0.11070799827575684,1.1619280719893698e-07
732,2196,0,2196,0.11096596717834473,1.1595944030926881e-07
733,2199,0,2199,0.11121082305908203,1.1579848593393269e-07
734,2202,0,2202,0.11138081550598145,1.1538311039044871e-07
735,2205,0,2205,0.11153888702392578,1.1516107105618155e-07
736,2208,0,2208,0.11167478561401367,1.1500594288327428e-07
737,2211,0,2211,0.11184096336364746,1.1489162575016877e-07
738,2214,0,2214,0.11197185516357422,1.1470242831595407e-07
739,2217,0,2217,0.11210179328918457,1.1456825075265739e-07
740,2220,0,2220,0.11224985122680664,1.1434112480735817e-07
741,2223,0,2223,0.11246275901794434,1.1405335137863646e-07
742,2226,0,2226,0.11262679100036621,1.1387175132913637e-07
743,2229,0,2229,0.11287403106689453,1.1364326719466676e-07
744,2232,0,2232,0.11311101913452148,1.1339112889563411e-07
745,2235,0,2235,0.11327099800109863,1.13205914184047e-07
746,2238,0,2238,0.11342287063598633,1.1302353205790597e-07
747,2241,0,2241,0.11358785629272461,1.1291199338341836e-07
748,2244,0,2244,0.11374902725219727,1.1275670904819057e-07
749,2247,0,2247,0.1138768196105957,1.1263474190832698e-07
750,2250,0,2250,0.11401081085205078,1.1252264936929204e-07
751,2253,0,2253,0.1141366958618164,1.124120280929509e-07
752,2256,0,2256,0.11426568031311035,1.1228374743602122e-07
753,2259,0,2259,0.11439275741577148,1.1209367400466696e-07
754,2262,0,2262,0.11452388763427734,1.1198604126097159e-07
755,2265,0,2265,0.11466383934020996,1.1188783737150605e-07
756,2268,0,2268,0.11479973793029785,1.116916972812169e-07
757,2271,0,2271,0.11499476432800293,1.1161050901417693e-07
758,2274,0,2274,0.11514496803283691,1.1148406172445418e-07
759,2277,0,2277,0.1153097152709961,1.1135931716567375e-07
760,2280,0,2280,0.11557579040527344,1.1125825070622822e-07
761,2283,0,2283,0.11580371856689453,1.11141822880033e-07
762,2286,0,2286,0.11605501174926758,1.1105679243799846e-07
763,2289,0,2289,0.11623978614807129,1.1089451885037445e-07
764,2292,0,2292,0.11643385887145996,1.108185816103508e-07
765,2295,0,2295,0.11658787727355957,1.1072957991365507e-07
766,2298,0,2298,0.11677694320678711,1.1065151839986839e-07
767,2301,0,2301,0.11692285537719727,1.105644928498888e-07
768,2304,0,2304,0.11708903312683105,1.1043066136253465e-07
769,2307,0,2307,0.1172788143157959,1.1029746446066406e-07
770,2310,0,2310,0.11752486228942871,1.10186558417691e-07
771,2313,0,2313,0.11768770217895508,1.1007908756969911e-07
772,2316,0,2316,0.11789178848266602,1.099972594249422e-07
773,2319,0,2319,0.1180868148803711,1.0985619178013489e-07
774,2322,0,2322,0.11828184127807617,1.0971756967777958e-07
775,2325,0,2325,0.11843299865722656,1.0945146517091961e-07
776,2328,0,2328,0.11857986450195312,1.0927799334738818e-07
777,2331,0,2331,0.11877775192260742,1.0917868232882466e-07
778,2334,0,2334,0.11895394325256348,1.0891937600721172e-07
779,2337,0,2337,0.11911487579345703,1.0880053610643437e-07
780,2340,0,2340,0.11926078796386719,1.0845298001438423e-07
781,2343,0,2343,0.11943292617797852,1.0826814867304146e-07
782,2346,0,2346,0.11960983276367188,1.0812044475227576e-07
783,2349,0,2349,0.11979985237121582,1.0756479503417276e-07
784,2352,0,2352,0.11999678611755371,1.0723603358739097e-07
785,2355,0,2355,0.12019586563110352,1.0671828575717635e-07
786,2358,0,2358,0.12038969993591309,1.0601172318669491e-07
787,2361,0,2361,0.12056493759155273,1.0532716571291144e-07
788,2364,0,2364,0.12070083618164062,1.0436857762732721e-07
789,2367,0,2367,0.12084388732910156,1.0337700709018464e-07
790,2370,0,2370,0.12096381187438965,9.940285275160027e-08
791,2373,0,2373,0.12112784385681152,9.878066655856854e-08
792,2376,0,2376,0.1212468147277832,9.522578256053632e-08
793,2379,0,2379,0.12137770652770996,9.422447908355689e-08
794,2382,0,2382,0.12150192260742188,9.124521873160945e-08
795,2385,0,2385,0.12163472175598145,9.040497333395632e-08
796,2388,0,2388,0.12175679206848145,8.885535799234629e-08
797,2391,0,2391,0.12188887596130371,8.815155744313008e-08
798,2394,0,2394,0.12200593948364258,8.690219088723792e-08
799,2397,0,2397,0.12213778495788574,8.608444280624898e-08
800,2400,0,2400,0.12227368354797363,8.507573678710082e-08
801,2403,0,2403,0.12240099906921387,8.41084836467191e-08
802,2406,0,2406,0.12253475189208984,8.335878017462488e-08
803,2409,0,2409,0.12265491485595703,7.855351121689727e-08
804,2412,0,2412,0.12295198440551758,7.794994259984992e-08
805,2415,0,2415,0.12311601638793945,7.705990041565605e-08
806,2418,0,2418,0.12330389022827148,7.655139511816382e-08
807,2421,0,2421,0.12346982955932617,7.543785063240088e-08
808,2424,0,2424,0.12380790710449219,7.49315988085428e-08
809,2427,0,2427,0.12410283088684082,7.189370683815979e-08
810,2430,0,2430,0.12439393997192383,7.144146114648057e-08
811,2433,0,2433,0.12464094161987305,7.044287848007801e-08
812,2436,0,2436,0.12479376792907715,7.005511198503651e-08
813,2439,0,2439,0.12497591972351074,6.821770231437642e-08
814,2442,0,2442,0.12514305114746094,6.780065611215362e-08
815,2445,0,2445,0.12530303001403809,6.717194970989286e-08
816,2448,0,2448,0.1255018711090088,6.653866445544166e-08
817,2451,0,2451,0.12565302848815918,6.615326138114294e-08
818,2454,0,2454,0.12579083442687988,6.419064640311191e-08
819,2457,0,2457,0.12592482566833496,6.38560524140242e-08
820,2460,0,2460,0.12607264518737793,6.206316929364648e-08
821,2463,0,2463,0.12619900703430176,6.159740079314065e-08
822,2466,0,2466,0.1263117790222168,6.026491465261812e-08
823,2469,0,2469,0.12643980979919434,5.995453349721593e-08
824,2472,0,2472,0.12656593322753906,5.9484489638917944e-08
825,2475,0,2475,0.1266796588897705,5.7784737509302736e-08
826,2478,0,2478,0.12680387496948242,5.735286715060585e-08
827,2481,0,2481,0.12694096565246582,5.682354484599753e-08
828,2484,0,2484,0.12705206871032715,5.503472558695887e-08
829,2487,0,2487,0.12717890739440918,5.454720162122127e-08
830,2490,0,2490,0.127288818359375,5.228085938794279e-08
831,2493,0,2493,0.12741303443908691,5.181036239337535e-08
832,2496,0,2496,0.12752485275268555,5.1034293150658153e-08
833,2499,0,2499,0.12764978408813477,5.054979563383385e-08
834,2502,0,2502,0.12779593467712402,5.017134220788604e-08
835,2505,0,2505,0.12798786163330078,4.9162004612401964e-08
836,2508,0,2508,0.12815284729003906,4.864440668564729e-08
837,2511,0,2511,0.12827491760253906,4.5443366216758414e-08
838,2514,0,2514,0.12840771675109863,4.47997085998742e-08
839,2517,0,2517,0.1285538673400879,4.410474011601823e-08
840,2520,0,2520,0.12868189811706543,4.2978668482575837e-08
841,2523,0,2523,0.12880778312683105,4.2353856180515946e-08
842,2526,0,2526,0.1289217472076416,4.0334400275081584e-08
843,2529,0,2529,0.12904763221740723,3.984142568260527e-08
844,2532,0,2532,0.12915992736816406,3.752276967785586e-08
845,2535,0,2535,0.1292867660522461,3.722293773793764e-08
846,2538,0,2538,0.12941384315490723,3.676590900648622e-08
847,2541,0,2541,0.12952876091003418,3.219652948086933e-08
848,2544,0,2544,0.12967586517333984,3.166536081519135e-08
849,2547,0,2547,0.12984085083007812,2.955183753500885e-08
850,2550,0,2550,0.13002395629882812,2.9110799731823176e-08
851,2553,0,2553,0.13019490242004395,2.8173120385869044e-08
852,2556,0,2556,0.1304159164428711,2.7659721428986954e-08
853,2559,0,2559,0.13054585456848145,2.7340025931978695e-08
854,2562,0,2562,0.1306748390197754,2.6588682974691806e-08
855,2565,0,2565,0.13078784942626953,2.4666315454563727e-08
856,2568,0,2568,0.13091373443603516,2.4328632936178054e-08
857,2571,0,2571,0.1310257911682129,2.3524044057395207e-08
858,2574,0,2574,0.13115191459655762,2.3200949931870967e-08
859,2577,0,2577,0.13126397132873535,2.1148056881821232e-08
860,2580,0,2580,0.13138985633850098,2.0962216202502134e-08
861,2583,0,2583,0.13150596618652344,2.0583031633554178e-08
862,2586,0,2586,0.13162970542907715,2.0437002683221236e-08
863,2589,0,2589,0.13173985481262207,2.0127909279230953e-08
864,2592,0,2592,0.1318666934967041,1.9988931685216725e-08
865,2595,0,2595,0.13197684288024902,1.9534566951970095e-08
866,2598,0,2598,0.13210177421569824,1.9361896296996944e-08
867,2601,0,2601,0.13222765922546387,1.9153485529798993e-08
868,2604,0,2604,0.13234186172485352,1.863047116499935e-08
869,2607,0,2607,0.13247108459472656,1.844715890267007e-08
870,2610,0,2610,0.1325829029083252,1.8120893023219098e-08
871,2613,0,2613,0.1327066421508789,1.7915168420006514e-08
872,2616,0,2616,0.13281679153442383,1.6992482936117585e-08
873,2619,0,2619,0.13295888900756836,1.6803052244734363e-08
874,2622,0,2622,0.13308286666870117,1.656493782050697e-08
875,2625,0,2625,0.13320708274841309,1.5869242621016928e-08
876,2628,0,2628,0.13336181640625,1.577203996808989e-08
877,2631,0,2631,0.13348889350891113,1.560135861421117e-08
878,2634,0,2634,0.13371801376342773,1.550140149277015e-08
879,2637,0,2637,0.1338958740234375,1.535756762283928e-08
880,2640,0,2640,0.13402700424194336,1.4818842547969332e-08
881,2643,0,2643,0.13416600227355957,1.4755857488285754e-08
882,2646,0,2646,0.13433289527893066,1.4604484981306362e-08
883,2649,0,2649,0.13448286056518555,1.4560699210116375e-08
884,2652,0,2652,0.13467168807983398,1.4311855504153442e-08
885,2655,0,2655,0.1348249912261963,1.4284591856792392e-08
886,2658,0,2658,0.1350116729736328,1.4252609505603528e-08
887,2661,0,2661,0.1351480484008789,1.408046998960134e-08
888,2664,0,2664,0.13541197776794434,1.4047114944722992e-08
889,2667,0,2667,0.13569378852844238,1.4000799768501932e-08
890,2670,0,2670,0.13590288162231445,1.3944577341527596e-08
891,2673,0,2673,0.13608598709106445,1.3916037092592749e-08
892,2676,0,2676,0.13622498512268066,1.3884054395437005e-08
893,2679,0,2679,0.13635993003845215,1.3853971959551709e-08
894,2682,0,2682,0.1365036964416504,1.3825808164645481e-08
895,2685,0,2685,0.13664674758911133,1.378483750748058e-08
896,2688,0,2688,0.13679170608520508,1.3730445087105458e-08
897,2691,0,2691,0.13692903518676758,1.3697478536888085e-08
898,2694,0,2694,0.13707971572875977,1.3653487076401481e-08
899,2697,0,2697,0.13727784156799316,1.3621324891501071e-08
900,2700,0,2700,0.13753795623779297,1.3594085452091778e-08
901,2703,0,2703,0.13780784606933594,1.3555276017574436e-08
902,2706,0,2706,0.1380019187927246,1.3511473047058047e-08
903,2709,0,2709,0.13818597793579102,1.3479904076112757e-08
904,2712,0,2712,0.13832783699035645,1.3452456388073237e-08
905,2715,0,2715,0.13848876953125,1.3434972613236804e-08
906,2718,0,2718,0.13884782791137695,1.3408977294985873e-08
907,2721,0,2721,0.13908982276916504,1.3373969686181691e-08
908,2724,0,2724,0.13931703567504883,1.3341914595237028e-08
909,2727,0,2727,0.1395859718322754,1.33151850181086e-08
910,2730,0,2730,0.1397860050201416,1.3304573014448313e-08
911,2733,0,2733,0.1401059627532959,1.3297507289521347e-08
912,2736,0,2736,0.1403210163116455,1.3272549844152144e-08
913,2739,0,2739,0.1405787467956543,1.3259114401926972e-08
914,2742,0,2742,0.1407468318939209,1.3224397146381262e-08
915,2745,0,2745,0.14089083671569824,1.3204780464829279e-08
916,2748,0,2748,0.141068696975708,1.3192623585874733e-08
917,2751,0,2751,0.1413567066192627,1.3173509410583836e-08
918,2754,0,2754,0.14148974418640137,1.3158788827841802e-08
919,2757,0,2757,0.14161992073059082,1.3148588418937786e-08
920,2760,0,2760,0.14174795150756836,1.3132207513557338e-08
921,2763,0,2763,0.1418769359588623,1.3119121959290133e-08
922,2766,0,2766,0.14200687408447266,1.3101551523537522e-08
923,2769,0,2769,0.14214086532592773,1.3086101530854644e-08
924,2772,0,2772,0.14228582382202148,1.307276767472657e-08
925,2775,0,2775,0.14245986938476562,1.3043199289868581e-08
926,2778,0,2778,0.14258980751037598,1.302649088339269e-08
927,2781,0,2781,0.1427309513092041,1.3011712035762512e-08
928,2784,0,2784,0.14286279678344727,1.2977426837128126e-08
929,2787,0,2787,0.14300894737243652,1.2958387673066225e-08
930,2790,0,2790,0.1431417465209961,1.2944925268966009e-08
931,2793,0,2793,0.14327597618103027,1.2921766059364977e-08
932,2796,0,2796,0.14345479011535645,1.289186786727576e-08
933,2799,0,2799,0.14362287521362305,1.2872053956049065e-08
934,2802,0,2802,0.14375591278076172,1.2837593094414986e-08
935,2805,0,2805,0.14388394355773926,1.2812332715086743e-08
936,2808,0,2808,0.1440119743347168,1.2792123980824749e-08
937,2811,0,2811,0.14414167404174805,1.2754699964307134e-08
938,2814,0,2814,0.14428377151489258,1.2734210597031165e-08
939,2817,0,2817,0.14449691772460938,1.2715689352380163e-08
940,2820,0,2820,0.144744873046875,1.2690323800050462e-08
941,2823,0,2823,0.14498305320739746,1.2656117727942453e-08
942,2826,0,2826,0.14516472816467285,1.2617282648665933e-08
943,2829,0,2829,0.14546585083007812,1.2575072317563294e-08
944,2832,0,2832,0.1457526683807373,1.254015212308174e-08
945,2835,0,2835,0.14591479301452637,1.247519940502383e-08
946,2838,0,2838,0.14605474472045898,1.2424050917233253e-08
947,2841,0,2841,0.14620375633239746,1.2374532109987044e-08
948,2844,0,2844,0.14648771286010742,1.2338004691196645e-08
949,2847,0,2847,0.14672470092773438,1.2309127412374472e-08
950,2850,0,2850,0.14688372611999512,1.2259952702722392e-08
951,2853,0,2853,0.1471269130706787,1.2211666928050682e-08
952,2856,0,2856,0.1473388671875,1.2162538971423525e-08
953,2859,0,2859,0.1474769115447998,1.2099667208327316e-08
954,2862,0,2862,0.14761686325073242,1.2056123388007097e-08
955,2865,0,2865,0.1477670669555664,1.1991734142082604e-08
956,2868,0,2868,0.1480410099029541,1.192370238088028e-08
957,2871,0,2871,0.14824700355529785,1.1871889535334694e-08
958,2874,0,2874,0.14838290214538574,1.18238745952083e-08
959,2877,0,2877,0.14853191375732422,1.1767450536834076e-08
960,2880,0,2880,0.14865899085998535,1.1714332088284656e-08
961,2883,0,2883,0.14883875846862793,1.1678209900760734e-08
962,2886,0,2886,0.14900875091552734,1.1635580259957274e-08
963,2889,0,2889,0.1491398811340332,1.1601427855391458e-08
964,2892,0,2892,0.1492769718170166,1.1562398851274897e-08
965,2895,0,2895,0.14940690994262695,1.1513670286932568e-08
966,2898,0,2898,0.14955592155456543,1.1480364039983852e-08
967,2901,0,2901,0.14970803260803223,1.1439004955126458e-08
968,2904,0,2904,0.14983868598937988,1.1366557313774784e-08
969,2907,0,2907,0.14996886253356934,1.1326478052926536e-08
970,2910,0,2910,0.1500988006591797,1.1281368001756043e-08
971,2913,0,2913,0.15021371841430664,1.1162963393720947e-08
972,2916,0,2916,0.1503438949584961,1.1129581043510185e-08
973,2919,0,2919,0.15047979354858398,1.1042180020883108e-08
974,2922,0,2922,0.15059566497802734,1.0903392922648653e-08
975,2925,0,2925,0.1507258415222168,1.0867221208571982e-08
976,2928,0,2928,0.15084075927734375,1.0741386149658869e-08
977,2931,0,2931,0.1509697437286377,1.0714522816791165e-08
978,2934,0,2934,0.15110087394714355,1.0652558661025218e-08
979,2937,0,2937,0.15128397941589355,1.0510700864490138e-08
980,2940,0,2940,0.1515038013458252,1.0447641489313247e-08
981,2943,0,2943,0.15167689323425293,1.026564415591162e-08
982,2946,0,2946,0.15187883377075195,1.016942090736609e-08
983,2949,0,2949,0.15213489532470703,9.959243559104295e-09


==> plot_data/quadratic_minimax_problem_n20_alpha0/flex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.915496826171875e-05,4.387061074692293
1,5,0,5,0.0002422332763671875,4.2514878856800244
2,10,0,10,0.0006430149078369141,3.8546852614608893
3,13,0,13,0.0008800029754638672,3.478351662948141
4,16,0,16,0.00121307373046875,3.416497347893481
5,20,0,20,0.0015110969543457031,3.3058207048491934
6,23,0,23,0.0017261505126953125,3.232429156876266
7,26,0,26,0.0019309520721435547,2.9306400110523825
8,29,0,29,0.0021381378173828125,2.661335825805268
9,32,0,32,0.0023279190063476562,2.3690405162990498
10,35,0,35,0.0025331974029541016,1.574705936211792
11,39,0,39,0.002749204635620117,1.520775780452156
12,43,0,43,0.0030100345611572266,1.4873768897048536
13,46,0,46,0.0032129287719726562,1.4321931702806545
14,49,0,49,0.003434896469116211,1.3612867685608938
15,54,0,54,0.003667116165161133,1.2523733032621758
16,58,0,58,0.003892183303833008,1.1634450518701838
17,61,0,61,0.004083156585693359,1.1304493035466832
18,65,0,65,0.004308938980102539,1.0490884784851864
19,69,0,69,0.004530191421508789,1.0333629673351694
20,72,0,72,0.004723072052001953,0.7504593225166305
21,75,0,75,0.004930973052978516,0.7043616145474156
22,79,0,79,0.005155086517333984,0.6721527858502336
23,83,0,83,0.00537419319152832,0.6275684872258744
24,86,0,86,0.0055789947509765625,0.6067458059024816
25,89,0,89,0.005791902542114258,0.5627057844173515
26,92,0,92,0.005978107452392578,0.3774350180712767
27,95,0,95,0.00617218017578125,0.36624348055570943
28,98,0,98,0.006489992141723633,0.27360860973118356
29,102,0,102,0.006749153137207031,0.2672501843219862
30,105,0,105,0.0069580078125,0.25060346337210215
31,108,0,108,0.0071620941162109375,0.24193320293271187
32,113,0,113,0.0074121952056884766,0.236162747467861
33,118,0,118,0.0076410770416259766,0.23093960191936377
34,123,0,123,0.00797891616821289,0.22618174918983044
35,127,0,127,0.008282184600830078,0.22565862413910037
36,130,0,130,0.008477210998535156,0.21025588936424977
37,133,0,133,0.008669137954711914,0.14630154737886447
38,136,0,136,0.008861064910888672,0.13448460965441264
39,139,0,139,0.009048938751220703,0.1324969318487299
40,143,0,143,0.009274005889892578,0.12422791458147336
41,147,0,147,0.00949716567993164,0.12218109049690261
42,151,0,151,0.009721994400024414,0.11550290277889491
43,154,0,154,0.009911060333251953,0.10169286604791537
44,157,0,157,0.01023721694946289,0.0724491427681876
45,160,0,160,0.010596036911010742,0.07151290218313094
46,164,0,164,0.010996103286743164,0.06922170113813034
47,168,0,168,0.01135706901550293,0.06784237637772056
48,173,0,173,0.01164102554321289,0.06711520764923017
49,178,0,178,0.011980056762695312,0.06645289922371621
50,183,0,183,0.012335062026977539,0.06584585521817748
51,188,0,188,0.012578010559082031,0.06528623187724732
52,193,0,193,0.01282501220703125,0.0647675932860838
53,197,0,197,0.013049125671386719,0.06341646587442311
54,200,0,200,0.013257265090942383,0.06318960685012566
55,203,0,203,0.013543128967285156,0.06065199028853831
56,207,0,207,0.013839006423950195,0.057924669126414266
57,210,0,210,0.014050960540771484,0.05207790987086858
58,213,0,213,0.014243125915527344,0.04573889813603081
59,217,0,217,0.014494180679321289,0.04496774438717166
60,220,0,220,0.014723062515258789,0.04433637795343284
61,225,0,225,0.015008926391601562,0.04387010141612501
62,230,0,230,0.01525115966796875,0.04344863098730567
63,235,0,235,0.015558004379272461,0.04306541052356413
64,240,0,240,0.015796899795532227,0.042715010930761334
65,245,0,245,0.016122102737426758,0.04239292657067039
66,250,0,250,0.016482114791870117,0.042095407976506044
67,255,0,255,0.016820907592773438,0.041819324916231256
68,259,0,259,0.017091989517211914,0.041536830458205665
69,263,0,263,0.017318010330200195,0.0411464513186611
70,266,0,266,0.01754903793334961,0.04064789840843676
71,269,0,269,0.01781916618347168,0.04054330062044691
72,273,0,273,0.01812291145324707,0.04023468805155606
73,276,0,276,0.01843094825744629,0.03992256545827922
74,279,0,279,0.01871514320373535,0.03915876546031952
75,284,0,284,0.019083023071289062,0.038462055687000035
76,289,0,289,0.019479036331176758,0.03782709190521317
77,294,0,294,0.01987600326538086,0.037246108109462585
78,299,0,299,0.020263195037841797,0.036712600895155434
79,304,0,304,0.020615100860595703,0.03622109819500934
80,308,0,308,0.020951032638549805,0.03620578007343768
81,313,0,313,0.021255016326904297,0.035734804219420754
82,318,0,318,0.021531105041503906,0.035303952895963844
83,322,0,322,0.021784067153930664,0.03460571219609875
84,327,0,327,0.022021055221557617,0.03427514444416489
85,332,0,332,0.02225518226623535,0.0339652875569984
86,337,0,337,0.022492170333862305,0.033674521525840856
87,342,0,342,0.022739171981811523,0.03340138689234838
88,346,0,346,0.02295708656311035,0.03218630476712578
89,351,0,351,0.023185014724731445,0.03194041536312966
90,356,0,356,0.02341604232788086,0.03171712993774379
91,361,0,361,0.02364206314086914,0.031513558938983444
92,365,0,365,0.023867130279541016,0.030455154274471524
93,370,0,370,0.02410411834716797,0.03027637616599037
94,375,0,375,0.024335145950317383,0.030118926677209747
95,380,0,380,0.024559974670410156,0.029979441759623048
96,385,0,385,0.024790048599243164,0.02985515471259885
97,390,0,390,0.025141000747680664,0.029743785763353545
98,395,0,395,0.025402069091796875,0.02964345183654465
99,400,0,400,0.025648117065429688,0.029552593062537966
100,405,0,405,0.025925159454345703,0.029469913060360436
101,410,0,410,0.026273012161254883,0.0293943304909836
102,415,0,415,0.026607990264892578,0.029324939791094923
103,420,0,420,0.02696704864501953,0.02926097935995855
104,425,0,425,0.027319908142089844,0.02920180578200157
105,430,0,430,0.027593135833740234,0.029146872928709322
106,435,0,435,0.027857065200805664,0.029095715000416765
107,440,0,440,0.02809000015258789,0.029047932747380708
108,445,0,445,0.02833700180053711,0.02900318225581333
109,450,0,450,0.028574228286743164,0.028961165803604257
110,455,0,455,0.02881002426147461,0.028921624386938023
111,460,0,460,0.029159069061279297,0.028884331596948896
112,465,0,465,0.029488086700439453,0.02884908858836638
113,470,0,470,0.029792070388793945,0.02881571993263034
114,475,0,475,0.030144929885864258,0.028784070188554355
115,480,0,480,0.030532121658325195,0.028754001056202995
116,485,0,485,0.030802249908447266,0.0287253890058
117,490,0,490,0.031054973602294922,0.028698123294460455
118,495,0,495,0.031316280364990234,0.02867210430036916
119,500,0,500,0.03154802322387695,0.028647242117530967
120,505,0,505,0.031858205795288086,0.028623455365061844
121,510,0,510,0.03209519386291504,0.02860067017369859
122,515,0,515,0.032424211502075195,0.028578819319208082
123,520,0,520,0.032675981521606445,0.028557841478013556
124,525,0,525,0.032959938049316406,0.02853768058489521
125,530,0,530,0.033385276794433594,0.02851828527628846
126,535,0,535,0.03384113311767578,0.02849960840566005
127,540,0,540,0.03419685363769531,0.02848160661984041
128,545,0,545,0.03447914123535156,0.028464239987131174
129,550,0,550,0.03480219841003418,0.028447471669584223
130,555,0,555,0.03512310981750488,0.028431267633133216
131,560,0,560,0.03538393974304199,0.028415596390305085
132,565,0,565,0.03562307357788086,0.02840042877109712
133,570,0,570,0.03586292266845703,0.028385737718306304
134,575,0,575,0.036115169525146484,0.02837149810417723
135,580,0,580,0.03638601303100586,0.028357686565709094
136,585,0,585,0.03662705421447754,0.028344281356360457
137,590,0,590,0.03686118125915527,0.028331262212213573
138,595,0,595,0.03710007667541504,0.02831861023093791
139,600,0,600,0.03733491897583008,0.028306307762116036
140,605,0,605,0.037574052810668945,0.02829433830769149
141,610,0,610,0.03780817985534668,0.02828268643145681
142,615,0,615,0.038068294525146484,0.028271337676637365
143,620,0,620,0.038323163986206055,0.02826027849074536
144,625,0,625,0.0385892391204834,0.0282494961569738
145,630,0,630,0.03883099555969238,0.028238978731489214
146,635,0,635,0.03907513618469238,0.028228714986053005
147,640,0,640,0.03932785987854004,0.028218694355465826
148,645,0,645,0.039565086364746094,0.028208906889383354
149,650,0,650,0.03979897499084473,0.028199343208101493
150,655,0,655,0.04005908966064453,0.0281899944619495
151,660,0,660,0.0403590202331543,0.028180852293966524
152,665,0,665,0.040635108947753906,0.028171908805571286
153,670,0,670,0.04092001914978027,0.028163156524960337
154,675,0,675,0.041314125061035156,0.028154588377999383
155,680,0,680,0.04169511795043945,0.02814619766139053
156,685,0,685,0.042086124420166016,0.028137978017923768
157,690,0,690,0.042474985122680664,0.028129923413633427
158,695,0,695,0.042877197265625,0.028122028116701427
159,700,0,700,0.04322409629821777,0.028114286677960187
160,705,0,705,0.04347705841064453,0.028106693912863363
161,710,0,710,0.0437932014465332,0.028099244884803053
162,715,0,715,0.044183969497680664,0.02809193488966376
163,720,0,720,0.04462313652038574,0.02808475944151158
164,725,0,725,0.045037031173706055,0.028077714259328024
165,730,0,730,0.04544711112976074,0.028070795254703813
166,735,0,735,0.0458369255065918,0.02806399852041565
167,740,0,740,0.0461878776550293,0.02805732031981657
168,745,0,745,0.046526193618774414,0.02805075707697485
169,750,0,750,0.04679703712463379,0.0280443053675032
170,755,0,755,0.047181129455566406,0.028037961910023536
171,760,0,760,0.0474390983581543,0.02803172355821921
172,765,0,765,0.047782182693481445,0.02802558729342752
173,770,0,770,0.0481572151184082,0.02801955021773304
174,775,0,775,0.048523902893066406,0.028013609547521367
175,780,0,780,0.04892611503601074,0.028007762607460223
176,785,0,785,0.049363136291503906,0.028002006824874585
177,790,0,790,0.049787044525146484,0.027996339724486233
178,795,0,795,0.05020904541015625,0.027990758923491448
179,800,0,800,0.05064105987548828,0.027985262126950683
180,805,0,805,0.051038265228271484,0.02797984712346799
181,810,0,810,0.051316261291503906,0.027974511781139057
182,815,0,815,0.051651954650878906,0.027969254043747793
183,820,0,820,0.05199098587036133,0.027964071927194245
184,825,0,825,0.05233407020568848,0.027958963516136696
185,830,0,830,0.05269503593444824,0.027953926960833275
186,835,0,835,0.05306601524353027,0.027948960474168616
187,840,0,840,0.05340218544006348,0.027944062328852683
188,845,0,845,0.05364513397216797,0.027939230854780547
189,850,0,850,0.053965091705322266,0.027934464436540567
190,855,0,855,0.05422210693359375,0.027929761511062745
191,860,0,860,0.05448603630065918,0.02792512056539575
192,865,0,865,0.05485105514526367,0.027920540134606098
193,870,0,870,0.05524921417236328,0.027916018799789638
194,875,0,875,0.055541038513183594,0.027911555186188857
195,880,0,880,0.05578112602233887,0.02790714796140937
196,885,0,885,0.0560760498046875,0.027902795833727914
197,890,0,890,0.056539058685302734,0.027898497550487764
198,895,0,895,0.056916236877441406,0.027894251896574705
199,899,0,899,0.05739903450012207,0.02788848071578543
200,904,0,904,0.0578310489654541,0.027870284527089565
201,909,0,909,0.05817914009094238,0.027853739548459454
202,914,0,914,0.05844712257385254,0.027838578817278647
203,919,0,919,0.05882096290588379,0.027824587432018707
204,924,0,924,0.05925798416137695,0.027811591664777216
205,929,0,929,0.059712886810302734,0.027799450426497178
206,933,0,933,0.060012102127075195,0.027784738902869224
207,938,0,938,0.06026315689086914,0.027768475995642774
208,943,0,943,0.06051206588745117,0.02775362071771414
209,948,0,948,0.0608060359954834,0.027739928548222294
210,953,0,953,0.06117510795593262,0.027727206657568757
211,958,0,958,0.06151008605957031,0.027715302377698904
212,962,0,962,0.06182289123535156,0.027700752458607276
213,967,0,967,0.06210803985595703,0.027689600601738192
214,972,0,972,0.062406063079833984,0.02767924231662545
215,977,0,977,0.06265807151794434,0.02766954403823698
216,982,0,982,0.06291818618774414,0.02766039965448348
217,987,0,987,0.06330513954162598,0.027651724543227334
218,992,0,992,0.06370091438293457,0.02764345093545567
219,997,0,997,0.06412506103515625,0.027635524305686006
220,1002,0,1002,0.06457710266113281,0.02762790055856326
221,1007,0,1007,0.06487488746643066,0.027620543833043736
222,1012,0,1012,0.06512928009033203,0.027613424786049667
223,1017,0,1017,0.06540989875793457,0.027606519248736274
224,1022,0,1022,0.06579923629760742,0.027599807172645964
225,1027,0,1027,0.06622314453125,0.02759327180166229
226,1032,0,1032,0.06664490699768066,0.02758689902007315
227,1037,0,1037,0.06699109077453613,0.027580676838181165
228,1042,0,1042,0.06739616394042969,0.027574594985504793
229,1047,0,1047,0.06788015365600586,0.027568644588273378
230,1052,0,1052,0.06827402114868164,0.027562817913077242
231,1057,0,1057,0.06871795654296875,0.027557108162531704
232,1062,0,1062,0.06908607482910156,0.027551509311915964
233,1067,0,1067,0.06951403617858887,0.02754601597815571
234,1072,0,1072,0.06987786293029785,0.027540623314393213
235,1077,0,1077,0.07023501396179199,0.027535326924843666
236,1082,0,1082,0.07050585746765137,0.027530122795775477
237,1087,0,1087,0.0708150863647461,0.027525007239337238
238,1092,0,1092,0.0711359977722168,0.02751997684764709
239,1097,0,1097,0.07142496109008789,0.027515028455103844
240,1102,0,1102,0.07168912887573242,0.027510159107302066
241,1107,0,1107,0.0720219612121582,0.027505366035269988
242,1112,0,1112,0.07234406471252441,0.027500646634008946
243,1117,0,1117,0.07261514663696289,0.027495998444522034
244,1122,0,1122,0.07286810874938965,0.027491419138681455
245,1127,0,1127,0.07312202453613281,0.0274869065064144
246,1132,0,1132,0.07348108291625977,0.027482458444789217
247,1137,0,1137,0.07386994361877441,0.027478072948664677
248,1142,0,1142,0.07423806190490723,0.02747374810263092
249,1147,0,1147,0.07455110549926758,0.027469482074020977
250,1152,0,1152,0.07489824295043945,0.027465273106814243
251,1156,0,1156,0.07522392272949219,0.027460782224937225
252,1161,0,1161,0.07552313804626465,0.02744542235388269
253,1166,0,1166,0.07578206062316895,0.027431721687641054
254,1171,0,1171,0.07616519927978516,0.027419379581339724
255,1176,0,1176,0.07654213905334473,0.027408156198618267
256,1181,0,1181,0.07682919502258301,0.027397859678163123
257,1186,0,1186,0.0772562026977539,0.027388336071538538
258,1191,0,1191,0.0776360034942627,0.027379461445914563
259,1196,0,1196,0.07788515090942383,0.027371135678679104
260,1201,0,1201,0.078125,0.027363277575085936
261,1206,0,1206,0.07838296890258789,0.0273558210213212
262,1211,0,1211,0.07866406440734863,0.02734871194865683
263,1215,0,1215,0.07896900177001953,0.027331414555457435
264,1220,0,1220,0.07921409606933594,0.027312082443708287
265,1225,0,1225,0.07947421073913574,0.027295117430990775
266,1230,0,1230,0.07983517646789551,0.027280084499641245
267,1235,0,1235,0.08020496368408203,0.02726663670021801
268,1240,0,1240,0.08047986030578613,0.027254496539415633
269,1245,0,1245,0.08075404167175293,0.02724344139996646
270,1250,0,1250,0.08110713958740234,0.027233292106982176
271,1255,0,1255,0.08135795593261719,0.027223903950325916
272,1260,0,1260,0.0817101001739502,0.027215159625164236
273,1265,0,1265,0.08203697204589844,0.027206963671831442
274,1269,0,1269,0.08228707313537598,0.027206292491413295
275,1274,0,1274,0.08252620697021484,0.027179575747188853
276,1279,0,1279,0.0827639102935791,0.02715671287976976
277,1284,0,1284,0.08300209045410156,0.02713699692971347
278,1289,0,1289,0.08325695991516113,0.027119858535799606
279,1294,0,1294,0.08349990844726562,0.0271048383057096
280,1299,0,1299,0.0837411880493164,0.02709156483438269
281,1304,0,1304,0.08400201797485352,0.027079737208532476
282,1309,0,1309,0.0842752456665039,0.027069111072521437
283,1314,0,1314,0.08451128005981445,0.027059487520891812
284,1319,0,1319,0.08475613594055176,0.027050704234744677
285,1324,0,1324,0.08512616157531738,0.027042628400088174
286,1329,0,1329,0.0854790210723877,0.027035151042280582
287,1334,0,1334,0.08572006225585938,0.027028182486778202
288,1339,0,1339,0.08597302436828613,0.02702164871661298
289,1344,0,1344,0.08631706237792969,0.027015488444645724
290,1349,0,1349,0.08655929565429688,0.027009650756288524
291,1354,0,1354,0.08680105209350586,0.027004093208151763
292,1359,0,1359,0.08704519271850586,0.026998780291605278
293,1364,0,1364,0.0873720645904541,0.026993682188861536
294,1369,0,1369,0.08774709701538086,0.02698877376392693
295,1374,0,1374,0.08799886703491211,0.02698403374244541
296,1379,0,1379,0.08823490142822266,0.02697944404371822
297,1384,0,1384,0.0884709358215332,0.026974989235537677
298,1389,0,1389,0.08871603012084961,0.026970656088314917
299,1394,0,1394,0.08900809288024902,0.026966433209633583
300,1399,0,1399,0.08925509452819824,0.026962310744067724
301,1404,0,1404,0.08948707580566406,0.026958280126060077
302,1409,0,1409,0.08972001075744629,0.026954333876020784
303,1414,0,1414,0.08995389938354492,0.026950465431699874
304,1419,0,1419,0.09019207954406738,0.02694666900840237
305,1424,0,1424,0.09042596817016602,0.026942939482835614
306,1429,0,1429,0.09065699577331543,0.026939272296355652
307,1434,0,1434,0.09089207649230957,0.026935663374170762
308,1439,0,1439,0.09112310409545898,0.026932109057697058
309,1444,0,1444,0.09137201309204102,0.026928606047775448
310,1449,0,1449,0.09161114692687988,0.026925151356876686
311,1454,0,1454,0.09184408187866211,0.02692174226876079
312,1459,0,1459,0.09208106994628906,0.026918376304329184
313,1464,0,1464,0.0923151969909668,0.02691505119263516
314,1469,0,1469,0.09255003929138184,0.026911764846197932
315,1474,0,1474,0.09278202056884766,0.026908515339916606
316,1479,0,1479,0.0930180549621582,0.026905300893000823
317,1484,0,1484,0.09324908256530762,0.026902119853435796
318,1489,0,1489,0.09348392486572266,0.02689897068458152
319,1494,0,1494,0.09373903274536133,0.0268958519535733
320,1499,0,1499,0.09398007392883301,0.02689276232124498
321,1504,0,1504,0.0942230224609375,0.026889700533345464
322,1509,0,1509,0.09446120262145996,0.026886665412853502
323,1514,0,1514,0.09469318389892578,0.026883655853229504
324,1519,0,1519,0.09493017196655273,0.02688067081246739
325,1524,0,1524,0.09516310691833496,0.026877709307833716
326,1529,0,1529,0.09539914131164551,0.02687477041119564
327,1534,0,1534,0.09562993049621582,0.02687185324485849
328,1539,0,1539,0.09586596488952637,0.02686895697784225
329,1544,0,1544,0.0960991382598877,0.02686608082253995
330,1549,0,1549,0.09633517265319824,0.026863224031707583
331,1554,0,1554,0.09663510322570801,0.02686038589574371
332,1559,0,1559,0.09688019752502441,0.02685756574022263
333,1564,0,1564,0.09715819358825684,0.02685476292365027
334,1569,0,1569,0.09740996360778809,0.026851976835416062
335,1574,0,1574,0.09771895408630371,0.02684920689391904
336,1579,0,1579,0.09795904159545898,0.026846452544847396
337,1584,0,1584,0.09820318222045898,0.026843713259594996
338,1589,0,1589,0.0984339714050293,0.026840988533800954
339,1594,0,1594,0.09866213798522949,0.026838277885998147
340,1599,0,1599,0.09889101982116699,0.026835580856360765
341,1604,0,1604,0.09911704063415527,0.026832897005540715
342,1609,0,1609,0.09935808181762695,0.026830225913584017
343,1614,0,1614,0.09957218170166016,0.026827567178920646
344,1619,0,1619,0.09979104995727539,0.026824920417420288
345,1624,0,1624,0.100006103515625,0.026822285261509
346,1629,0,1629,0.10022401809692383,0.026819661359340857
347,1634,0,1634,0.10054802894592285,0.026817048374020706
348,1639,0,1639,0.10088706016540527,0.026814445982873455
349,1644,0,1644,0.1011502742767334,0.026811853876756404
350,1649,0,1649,0.1013641357421875,0.026809271759411422
351,1654,0,1654,0.10157418251037598,0.026806699346853872
352,1659,0,1659,0.10178804397583008,0.02680413636679557
353,1664,0,1664,0.10200309753417969,0.026801582558099758
354,1669,0,1669,0.1022179126739502,0.026799037670264887
355,1674,0,1674,0.10242819786071777,0.02679650146293735
356,1679,0,1679,0.10264205932617188,0.02679397370544826
357,1684,0,1684,0.10285401344299316,0.026791454176375653
358,1689,0,1689,0.10306715965270996,0.02678894266312795
359,1694,0,1694,0.10327792167663574,0.026786438961550318
360,1699,0,1699,0.10350990295410156,0.026783942875548833
361,1704,0,1704,0.10372614860534668,0.02678145421673507
362,1709,0,1709,0.10394406318664551,0.02677897280408707
363,1714,0,1714,0.10415911674499512,0.02677649846362761
364,1719,0,1719,0.1044001579284668,0.026774031028117547
365,1724,0,1724,0.10463094711303711,0.02677157033676432
366,1729,0,1729,0.10486698150634766,0.026769116234944292
367,1734,0,1734,0.10509896278381348,0.026766668573937624
368,1739,0,1739,0.10535216331481934,0.02676422721067691
369,1744,0,1744,0.10559606552124023,0.026761792007506058
370,1749,0,1749,0.10584497451782227,0.02675936283195166
371,1754,0,1754,0.10609102249145508,0.026756939556503934
372,1759,0,1759,0.10636115074157715,0.02675452205840843
373,1764,0,1764,0.10659909248352051,0.02675211021946683
374,1769,0,1769,0.106842041015625,0.02674970392584693
375,1774,0,1774,0.10707902908325195,0.026747303067901226
376,1779,0,1779,0.10733413696289062,0.026744907539993354
377,1784,0,1784,0.1075592041015625,0.026742517240333195
378,1789,0,1789,0.10786700248718262,0.026740132070817862
379,1794,0,1794,0.10808706283569336,0.026737751936881195
380,1799,0,1799,0.10831403732299805,0.02673537674734911
381,1804,0,1804,0.10854125022888184,0.026733006414301232
382,1809,0,1809,0.10875415802001953,0.026730640852939185
383,1814,0,1814,0.1089639663696289,0.026728279981459893
384,1819,0,1819,0.10931921005249023,0.02672592372093514
385,1824,0,1824,0.10969424247741699,0.02672357199519573
386,1829,0,1829,0.11034798622131348,0.02672122473072098
387,1834,0,1834,0.1106569766998291,0.026718881856532883
388,1839,0,1839,0.11102986335754395,0.026716543304094717
389,1844,0,1844,0.11139130592346191,0.026714209007214246
390,1849,0,1849,0.11175894737243652,0.026711878901950672
391,1854,0,1854,0.1120150089263916,0.026709552926525867
392,1859,0,1859,0.11223220825195312,0.02670723102123923
393,1864,0,1864,0.11245012283325195,0.026704913128386062
394,1869,0,1869,0.11266493797302246,0.026702599192179582
395,1874,0,1874,0.11288213729858398,0.026700289158676005
396,1879,0,1879,0.11309623718261719,0.02669798297570287
397,1884,0,1884,0.11335206031799316,0.026695680592790236
398,1889,0,1889,0.11356616020202637,0.026693381961105076
399,1894,0,1894,0.11378192901611328,0.026691087033387895
400,1899,0,1899,0.1139979362487793,0.026688795763892353
401,1904,0,1904,0.11441802978515625,0.02668650810832727
402,1909,0,1909,0.11478495597839355,0.026684224023801006
403,1914,0,1914,0.11517715454101562,0.02668194346876809
404,1919,0,1919,0.11541295051574707,0.026679666402978048
405,1924,0,1924,0.115631103515625,0.026677392787426386
406,1929,0,1929,0.11584806442260742,0.026675122584307685
407,1934,0,1934,0.11606407165527344,0.026672855756970097
408,1939,0,1939,0.11628198623657227,0.026670592269872298
409,1944,0,1944,0.1165311336517334,0.026668332088542003
410,1949,0,1949,0.11678719520568848,0.026666075179535707
411,1954,0,1954,0.11700296401977539,0.026663821510400875
412,1959,0,1959,0.11722016334533691,0.026661571049638816
413,1964,0,1964,0.11743617057800293,0.02665932376666963
414,1969,0,1969,0.11765217781066895,0.02665707963179823
415,1974,0,1974,0.11786699295043945,0.02665483861618202
416,1979,0,1979,0.11808514595031738,0.026652600691799342
417,1984,0,1984,0.11830019950866699,0.026650365831419904
418,1989,0,1989,0.11851692199707031,0.026648134008575665
419,1994,0,1994,0.11873197555541992,0.02664590519753334
420,1999,0,1999,0.11894917488098145,0.026643679373267795
421,2004,0,2004,0.11916303634643555,0.026641456511436585
422,2009,0,2009,0.11938023567199707,0.02663923658835528
423,2014,0,2014,0.11964011192321777,0.026637019580974083
424,2019,0,2019,0.11986303329467773,0.026634805466855104
425,2024,0,2024,0.12007498741149902,0.026632594224150576
426,2029,0,2029,0.12028622627258301,0.02663038583158201
427,2034,0,2034,0.12055325508117676,0.026628180268420076
428,2039,0,2039,0.12091517448425293,0.026625977514465153
429,2044,0,2044,0.12112617492675781,0.026623777550028996
430,2049,0,2049,0.12137603759765625,0.026621580355916594
431,2054,0,2054,0.12158608436584473,0.026619385913409222
432,2059,0,2059,0.1217961311340332,0.02661719420424772
433,2064,0,2064,0.12200593948364258,0.026615005210616813
434,2069,0,2069,0.12221622467041016,0.026612818915129566
435,2074,0,2074,0.12242412567138672,0.026610635300812976
436,2079,0,2079,0.1226348876953125,0.026608454351093554
437,2084,0,2084,0.12284612655639648,0.02660627604978385
438,2089,0,2089,0.12305617332458496,0.02660410038106931
439,2094,0,2094,0.12326598167419434,0.026601927329495713
440,2099,0,2099,0.12347793579101562,0.02659975687995707
441,2104,0,2104,0.1236882209777832,0.026597589017683727
442,2109,0,2109,0.12389898300170898,0.02659542372823148
443,2114,0,2114,0.12410688400268555,0.02659326099747031
444,2119,0,2119,0.12431812286376953,0.026591100811574415
445,2124,0,2124,0.12452816963195801,0.026588943157011907
446,2129,0,2129,0.12473797798156738,0.02658678802053512
447,2134,0,2134,0.12494707107543945,0.02658463538917145
448,2139,0,2139,0.12515807151794434,0.026582485250214217
449,2144,0,2144,0.1253669261932373,0.026580337591214375
450,2149,0,2149,0.1255779266357422,0.02657819239997161
451,2154,0,2154,0.12578701972961426,0.026576049664526882
452,2159,0,2159,0.12599706649780273,0.02657390937315442
453,2164,0,2164,0.1262061595916748,0.026571771514354237
454,2169,0,2169,0.12641620635986328,0.026569636076845225
455,2174,0,2174,0.12662696838378906,0.026567503049557878
456,2179,0,2179,0.12683796882629395,0.026565372421627848
457,2184,0,2184,0.1270902156829834,0.02656324418238961
458,2189,0,2189,0.12737298011779785,0.0265611183213699
459,2194,0,2194,0.12758326530456543,0.026558994828282036
460,2199,0,2199,0.1277930736541748,0.026556873693020195
461,2204,0,2204,0.12800312042236328,0.026554754905653514
462,2209,0,2209,0.12821292877197266,0.026552638456421154
463,2214,0,2214,0.12842202186584473,0.026550524335726793
464,2219,0,2219,0.1286330223083496,0.026548412534133762
465,2224,0,2224,0.12884116172790527,0.02654630304236031
466,2229,0,2229,0.12905216217041016,0.026544195851274734
467,2234,0,2234,0.12926101684570312,0.026542090951891143
468,2239,0,2239,0.129472017288208,0.02653998833536492
469,2244,0,2244,0.12968111038208008,0.026537887992988653
470,2249,0,2249,0.12989521026611328,0.026535789916188175
471,2254,0,2254,0.13010406494140625,0.02653369409651847
472,2259,0,2259,0.13031601905822754,0.026531600525660035
473,2264,0,2264,0.13052606582641602,0.026529509195415277
474,2269,0,2269,0.1307392120361328,0.02652742009770482
475,2274,0,2274,0.1309490203857422,0.026525333224564355
476,2279,0,2279,0.13116002082824707,0.02652324856814133
477,2284,0,2284,0.13136911392211914,0.02652116612069147
478,2289,0,2289,0.1315779685974121,0.02651908587457624
479,2294,0,2294,0.13178801536560059,0.026517007822259353
480,2299,0,2299,0.13199710845947266,0.026514931956304406
481,2304,0,2304,0.13220596313476562,0.026512858269371824
482,2309,0,2309,0.13242316246032715,0.026510786754216094
483,2314,0,2314,0.13263297080993652,0.026508717403683574
484,2319,0,2319,0.1328439712524414,0.02650665021070974
485,2324,0,2324,0.13305306434631348,0.026504585168316677
486,2329,0,2329,0.13326311111450195,0.026502522269611042
487,2334,0,2334,0.13347291946411133,0.026500461507781556
488,2339,0,2339,0.1336841583251953,0.02649840287609694
489,2344,0,2344,0.1338951587677002,0.026496346367903743
490,2349,0,2349,0.13410496711730957,0.02649429197662449
491,2354,0,2354,0.13431501388549805,0.026492239695755385
492,2359,0,2359,0.13452506065368652,0.026490189518864688
493,2364,0,2364,0.13474011421203613,0.02648814143959058
494,2369,0,2369,0.13508820533752441,0.026486095451639723
495,2374,0,2374,0.1352980136871338,0.026484051548785338
496,2379,0,2379,0.13550829887390137,0.026482009724865363
497,2384,0,2384,0.13571715354919434,0.026479969973781162
498,2389,0,2389,0.1359269618988037,0.026477932289495715
499,2394,0,2394,0.13613605499267578,0.026475896666032155
500,2399,0,2399,0.13634610176086426,0.026473863097472308
501,2404,0,2404,0.13655495643615723,0.026471831577955345
502,2409,0,2409,0.1367661952972412,0.02646980210167613
503,2414,0,2414,0.13697504997253418,0.026467774662884264
504,2419,0,2419,0.13718914985656738,0.026465749255882277
505,2424,0,2424,0.13739895820617676,0.026463725875025025
506,2429,0,2429,0.13760805130004883,0.02646170451471787
507,2434,0,2434,0.13782215118408203,0.02645968516941583
508,2439,0,2439,0.13803315162658691,0.026457667833622224
509,2444,0,2444,0.1382429599761963,0.02645565250188785
510,2449,0,2449,0.13845229148864746,0.026453639168809513
511,2454,0,2454,0.13866114616394043,0.026451627829029378
512,2459,0,2459,0.1388709545135498,0.026449618477233653
513,2464,0,2464,0.13908123970031738,0.02644761110815171
514,2469,0,2469,0.13929104804992676,0.026445605716555215
515,2474,0,2474,0.13949894905090332,0.026443602297257018
516,2479,0,2479,0.1397092342376709,0.02644160084511053
517,2484,0,2484,0.1399211883544922,0.026439601355008457
518,2489,0,2489,0.14013099670410156,0.026437603821882278
519,2494,0,2494,0.14033913612365723,0.026435608240701403
520,2499,0,2499,0.1405501365661621,0.026433614606472065
521,2504,0,2504,0.14076519012451172,0.026431622914236935
522,2509,0,2509,0.1409749984741211,0.02642963315907422
523,2514,0,2514,0.14118504524230957,0.02642764533609687
524,2519,0,2519,0.14146208763122559,0.02642565944045179
525,2524,0,2524,0.14166998863220215,0.02642367546731944
526,2529,0,2529,0.14188098907470703,0.02642169341191292
527,2534,0,2534,0.14208984375,0.02641971326947734
528,2539,0,2539,0.14230108261108398,0.02641773503528938
529,2544,0,2544,0.14251112937927246,0.026415758704656466
530,2549,0,2549,0.14278006553649902,0.02641378427291618
531,2554,0,2554,0.142988920211792,0.02641181173543577
532,2559,0,2559,0.14323186874389648,0.026409841087611637
533,2564,0,2564,0.1434769630432129,0.026407872324868638
534,2569,0,2569,0.1438281536102295,0.02640590544265961
535,2574,0,2574,0.14410686492919922,0.026403940436464896
536,2579,0,2579,0.14433813095092773,0.02640197730179176
537,2584,0,2584,0.14499616622924805,0.026400016034173954
538,2589,0,2589,0.14522004127502441,0.026398056629171322
539,2594,0,2594,0.14544105529785156,0.026396099082368975
540,2599,0,2599,0.14573216438293457,0.02639414338937742
541,2604,0,2604,0.14604806900024414,0.02639218954583162
542,2609,0,2609,0.14635014533996582,0.026390237547390748
543,2614,0,2614,0.14668607711791992,0.02638828738973782
544,2619,0,2619,0.14694809913635254,0.026386339068579217
545,2624,0,2624,0.14716100692749023,0.026384392579644343
546,2629,0,2629,0.1473710536956787,0.026382447918685048
547,2634,0,2634,0.1475849151611328,0.02638050508147566
548,2639,0,2639,0.14790701866149902,0.026378564063812213
549,2644,0,2644,0.14816927909851074,0.026376624861512234
550,2649,0,2649,0.14838123321533203,0.026374687470414444
551,2654,0,2654,0.1486530303955078,0.026372751886378474
552,2659,0,2659,0.1488969326019287,0.02637081810528436
553,2664,0,2664,0.14915800094604492,0.026368886123032228
554,2669,0,2669,0.149367094039917,0.026366955935542207
555,2674,0,2674,0.14957904815673828,0.02636502753875395
556,2679,0,2679,0.14978814125061035,0.026363100928626298
557,2684,0,2684,0.14999794960021973,0.026361176101137133
558,2689,0,2689,0.1502079963684082,0.026359253052283014
559,2694,0,2694,0.15056610107421875,0.026357331778078835
560,2699,0,2699,0.15079307556152344,0.02635541227455777
561,2704,0,2704,0.15104413032531738,0.026353494537770694
562,2708,0,2708,0.15129709243774414,0.026347427380368393
563,2713,0,2713,0.15150904655456543,0.026337636669157373
564,2718,0,2718,0.1518571376800537,0.026328405932720293
565,2723,0,2723,0.1521461009979248,0.02631967028935862
566,2728,0,2728,0.15235614776611328,0.026311375238442895
567,2733,0,2733,0.15256690979003906,0.02630347473640374
568,2737,0,2737,0.15276503562927246,0.026262561192579876
569,2742,0,2742,0.15302300453186035,0.026249214341562258
570,2747,0,2747,0.15336203575134277,0.026236442330971135
571,2751,0,2751,0.1535630226135254,0.026181753165309973
572,2756,0,2756,0.15377306938171387,0.02616338857172021
573,2760,0,2760,0.15397214889526367,0.026138300729742204
574,2765,0,2765,0.15418410301208496,0.02611297914228619
575,2770,0,2770,0.1544349193572998,0.026088991341809357
576,2774,0,2774,0.1546332836151123,0.026080198983602015
577,2779,0,2779,0.1548452377319336,0.026054616293865192
578,2784,0,2784,0.15505504608154297,0.02603034626098535
579,2789,0,2789,0.15526700019836426,0.026007245165615804
580,2794,0,2794,0.15547609329223633,0.02598519274514427
581,2799,0,2799,0.15568804740905762,0.025964087719451082
582,2804,0,2804,0.1558980941772461,0.025943844224824285
583,2809,0,2809,0.15610909461975098,0.02592438896548446
584,2814,0,2814,0.1563282012939453,0.02590565893300093
585,2819,0,2819,0.156541109085083,0.025887599575849757
586,2824,0,2824,0.1567521095275879,0.025870163326405963
587,2829,0,2829,0.15696406364440918,0.025853308412287637
588,2834,0,2834,0.1574702262878418,0.025836997894360825
589,2838,0,2838,0.1578669548034668,0.025796197509325866
590,2843,0,2843,0.1582779884338379,0.025775271507501994
591,2848,0,2848,0.15862011909484863,0.02575529858029857
592,2853,0,2853,0.1588430404663086,0.025736163103450487
593,2858,0,2858,0.15914583206176758,0.02571777041168842
594,2863,0,2863,0.15942811965942383,0.02570004244014853
595,2868,0,2868,0.1596510410308838,0.02568291431871739
596,2872,0,2872,0.15985918045043945,0.025673464970027565
597,2877,0,2877,0.16008210182189941,0.025655112115057003
598,2882,0,2882,0.16031098365783691,0.025637406933913406
599,2887,0,2887,0.16053295135498047,0.02562026370119641
600,2892,0,2892,0.16076207160949707,0.025603613722957552
601,2896,0,2896,0.16097307205200195,0.025568078524267915
602,2901,0,2901,0.16119384765625,0.025552020766732464
603,2906,0,2906,0.16141605377197266,0.025536320746343186
604,2911,0,2911,0.1616370677947998,0.025520935108218495
605,2915,0,2915,0.1618499755859375,0.025485104732586004
606,2920,0,2920,0.16207003593444824,0.02546748315811752
607,2925,0,2925,0.1622922420501709,0.025450279795337184
608,2929,0,2929,0.16250014305114746,0.025382237621583415
609,2933,0,2933,0.16271615028381348,0.025329646522416996
610,2937,0,2937,0.16292405128479004,0.025251680355841633
611,2941,0,2941,0.16313505172729492,0.025122592022094856
612,2945,0,2945,0.1633460521697998,0.02493707039139349
613,2948,0,2948,0.16358208656311035,0.024672065382057393
614,2951,0,2951,0.16397714614868164,0.024176865697497628
615,2954,0,2954,0.16416406631469727,0.02286491895023242
616,2957,0,2957,0.16434407234191895,0.01957540994443955
617,2960,0,2960,0.16457605361938477,0.010493902593661298
618,2963,0,2963,0.16475510597229004,0.008630247063474409
619,2966,0,2966,0.1649341583251953,0.0046034716202297595
620,2969,0,2969,0.16511297225952148,0.004170566791281395
621,2974,0,2974,0.16533708572387695,0.00413735094653529
622,2979,0,2979,0.165557861328125,0.00410727088756372
623,2984,0,2984,0.16578197479248047,0.004079864350285105
624,2989,0,2989,0.16600322723388672,0.004054751823078806
625,2994,0,2994,0.16622519493103027,0.004031620635477792
626,2999,0,2999,0.16644597053527832,0.00401021212945842
627,3004,0,3004,0.16666793823242188,0.003990311340269254
628,3009,0,3009,0.1668870449066162,0.003971738708239337
629,3014,0,3014,0.16710901260375977,0.003954343426915169
630,3019,0,3019,0.16733002662658691,0.003937998105173719
631,3024,0,3024,0.16755294799804688,0.003922594481937824
632,3029,0,3029,0.16777420043945312,0.003908039982746265
633,3034,0,3034,0.16799616813659668,0.003894254948971312
634,3039,0,3039,0.16821599006652832,0.003881170404259485
635,3044,0,3044,0.16844415664672852,0.0038687262500601283
636,3049,0,3049,0.16866493225097656,0.0038568698040348506
637,3054,0,3054,0.1690349578857422,0.0038455546126943715
638,3059,0,3059,0.16945719718933105,0.0038347394836178595
639,3064,0,3064,0.16974210739135742,0.0038243876937665883
640,3068,0,3068,0.17001914978027344,0.003815870456744126
641,3071,0,3071,0.17022204399108887,0.003610483827256078
642,3075,0,3075,0.17043304443359375,0.0035991043083502283
643,3080,0,3080,0.17070317268371582,0.0035693970748949403
644,3085,0,3085,0.17092609405517578,0.0035434669381683667
645,3090,0,3090,0.17114686965942383,0.003520688493879274
646,3095,0,3095,0.17136907577514648,0.0035005486267242016
647,3100,0,3100,0.17158794403076172,0.003482625943715218
648,3105,0,3105,0.17180895805358887,0.0034665738599559295
649,3110,0,3110,0.17203187942504883,0.0034521067582702907
650,3115,0,3115,0.17225003242492676,0.0034389887062372727
651,3120,0,3120,0.172468900680542,0.003427024282257028
652,3125,0,3125,0.17269110679626465,0.0034160511291992436
653,3130,0,3130,0.17290902137756348,0.0034059339160054064
654,3135,0,3135,0.17312908172607422,0.0033965594424679203
655,3140,0,3140,0.17335009574890137,0.0033878326697430504
656,3145,0,3145,0.1735689640045166,0.0033796734991947846
657,3150,0,3150,0.17378926277160645,0.003372014155543419
658,3155,0,3155,0.1740100383758545,0.0033647970578122833
659,3160,0,3160,0.17422723770141602,0.003357973084068216
660,3165,0,3165,0.17444610595703125,0.0033515001542396817
661,3170,0,3170,0.17467212677001953,0.0033453420700885073
662,3175,0,3175,0.17489004135131836,0.003339467563337093
663,3180,0,3180,0.1751091480255127,0.0033338495125428045
664,3185,0,3185,0.17532896995544434,0.003328464297011369
665,3190,0,3190,0.17554616928100586,0.003323291262216842
666,3195,0,3195,0.1757650375366211,0.003318312276146884
667,3200,0,3200,0.1761009693145752,0.0033135113599613623
668,3205,0,3205,0.17648100852966309,0.003308874379535521
669,3210,0,3210,0.17676210403442383,0.0033043887870133474
670,3215,0,3215,0.1769871711730957,0.003300043403548551
671,3220,0,3220,0.17730021476745605,0.0032958282360608993
672,3225,0,3225,0.17752313613891602,0.0032917343221640057
673,3230,0,3230,0.1777498722076416,0.0032877535984927294
674,3235,0,3235,0.17796921730041504,0.0032838787885240707
675,3240,0,3240,0.17818903923034668,0.0032801033066860684
676,3245,0,3245,0.17841100692749023,0.0032764211761178875
677,3250,0,3250,0.17863011360168457,0.0032728269579059797
678,3255,0,3255,0.1788499355316162,0.0032693156899973592
679,3260,0,3260,0.1790759563446045,0.0032658828342983547
680,3265,0,3265,0.17929601669311523,0.003262524230718055
681,3270,0,3270,0.17951607704162598,0.003259236057122147
682,3275,0,3275,0.17973899841308594,0.0032560147943319065
683,3280,0,3280,0.17995691299438477,0.0032528571954429154
684,3285,0,3285,0.18017816543579102,0.0032497602588533107
685,3290,0,3290,0.18040013313293457,0.0032467212044870386
686,3295,0,3295,0.18062400817871094,0.0032437374527769978
687,3300,0,3300,0.1808490753173828,0.003240806606038762
688,3305,0,3305,0.18107104301452637,0.0032379264319211303
689,3310,0,3310,0.1812891960144043,0.003235094848665643
690,3315,0,3315,0.18150901794433594,0.0032323099119460565
691,3320,0,3320,0.1817309856414795,0.003229569803091499
692,3325,0,3325,0.18195390701293945,0.0032268728185243264
693,3330,0,3330,0.1821751594543457,0.0032242173602670798
694,3335,0,3335,0.18239712715148926,0.0032216019273928046
695,3340,0,3340,0.18261504173278809,0.0032190251083095167
696,3345,0,3345,0.18283414840698242,0.003216485573784139
697,3350,0,3350,0.18305611610412598,0.003213982070623282
698,3355,0,3355,0.1832730770111084,0.0032115134159389092
699,3360,0,3360,0.18349313735961914,0.0032090784919357024
700,3365,0,3365,0.1837139129638672,0.003206676241164824
701,3370,0,3370,0.18393206596374512,0.003204305662195529
702,3375,0,3375,0.18415212631225586,0.0032019658056615893
703,3380,0,3380,0.1843729019165039,0.0031996557706448067
704,3385,0,3385,0.18459200859069824,0.0031973747013621036
705,3390,0,3390,0.18481087684631348,0.0031951217841264677
706,3395,0,3395,0.18503212928771973,0.003192896244555388
707,3400,0,3400,0.18525004386901855,0.0031906973450032765
708,3405,0,3405,0.1854701042175293,0.0031885243821969645
709,3410,0,3410,0.18569111824035645,0.003186376685055593
710,3415,0,3415,0.18590903282165527,0.003184253612678013
711,3420,0,3420,0.18621206283569336,0.0031821545524828854
712,3425,0,3425,0.18643593788146973,0.003180078918487911
713,3430,0,3430,0.18665528297424316,0.0031780261497159823
714,3435,0,3435,0.1868760585784912,0.0031759957087175166
715,3440,0,3440,0.18709802627563477,0.0031739870801989795
716,3445,0,3445,0.1873161792755127,0.003171999769748819
717,3450,0,3450,0.18753600120544434,0.0031700333026526526
718,3455,0,3455,0.1877579689025879,0.003168087222790484
719,3460,0,3460,0.18797516822814941,0.003166161091609344
720,3465,0,3465,0.18819403648376465,0.003164254487165317
721,3470,0,3470,0.1884150505065918,0.0031623670032295084
722,3475,0,3475,0.18863296508789062,0.003160498248453018
723,3480,0,3480,0.18885302543640137,0.003158647845586296
724,3485,0,3485,0.18907809257507324,0.003156815430748837
725,3490,0,3490,0.18929600715637207,0.0031550006527454335
726,3495,0,3495,0.18951702117919922,0.0031532031724254513
727,3500,0,3500,0.18973803520202637,0.0031514226620820724
728,3505,0,3505,0.1899559497833252,0.0031496588048885153
729,3510,0,3510,0.19017601013183594,0.003147911294368614
730,3515,0,3515,0.19039607048034668,0.0031461798338993955
731,3520,0,3520,0.1906139850616455,0.0031444641362432307
732,3525,0,3525,0.19083619117736816,0.0031427639231076635
733,3530,0,3530,0.19105911254882812,0.00314107892473096
734,3535,0,3535,0.19127607345581055,0.003139408879491531
735,3540,0,3540,0.1914961338043213,0.003137753533539861
736,3545,0,3545,0.19176316261291504,0.0031361126404511725
737,3550,0,3550,0.191986083984375,0.0031344859608976043
738,3555,0,3555,0.19220495223999023,0.003132873262338608
739,3560,0,3560,0.19242596626281738,0.003131274318728381
740,3565,0,3565,0.19264507293701172,0.003129688910239209
741,3570,0,3570,0.19286608695983887,0.0031281168229997714
742,3575,0,3575,0.19308805465698242,0.003126557848847383
743,3580,0,3580,0.19330596923828125,0.0031250117850933927
744,3585,0,3585,0.19352483749389648,0.0031234784343008738
745,3590,0,3590,0.19379496574401855,0.0031219576040738698
746,3595,0,3595,0.19401311874389648,0.003120449106857496
747,3600,0,3600,0.19423294067382812,0.003118952759748227
748,3605,0,3605,0.19445490837097168,0.003117468384313773
749,3610,0,3610,0.1946730613708496,0.003115995806422024
750,3615,0,3615,0.19489192962646484,0.003114534856078466
751,3620,0,3620,0.1951138973236084,0.0031130853672715485
752,3625,0,3625,0.19533205032348633,0.0031116471778257354
753,3630,0,3630,0.19555187225341797,0.003110220129261513
754,3635,0,3635,0.19577312469482422,0.0031088040666622345
755,3640,0,3640,0.19599008560180664,0.0031073988385472125
756,3645,0,3645,0.19621014595031738,0.003106004296750858
757,3650,0,3650,0.19643115997314453,0.0031046202963074293
758,3655,0,3655,0.19665002822875977,0.0031032466953411384
759,3660,0,3660,0.1968691349029541,0.0031018833549613157
760,3665,0,3665,0.19708991050720215,0.0031005301391623494
761,3670,0,3670,0.1973259449005127,0.003099186914728139
762,3675,0,3675,0.19755101203918457,0.003097853551140859
763,3680,0,3680,0.19790887832641602,0.003096529920493722
764,3685,0,3685,0.19820904731750488,0.003095215897407651
765,3690,0,3690,0.198472261428833,0.0030939113589515586
766,3695,0,3695,0.1987171173095703,0.00309261618456611
767,3700,0,3700,0.19903826713562012,0.0030913302559907006
768,3705,0,3705,0.19926023483276367,0.003090053457193632
769,3710,0,3710,0.19948315620422363,0.0030887856743051587
770,3715,0,3715,0.1997051239013672,0.0030875267955534306
771,3720,0,3720,0.19992709159851074,0.0030862767112030177
772,3725,0,3725,0.2001481056213379,0.003085035313495962
773,3730,0,3730,0.20037126541137695,0.003083802496595363
774,3735,0,3735,0.2005929946899414,0.0030825781565311013
775,3739,0,3739,0.20080304145812988,0.003080686868196376
776,3742,0,3742,0.2010350227355957,0.002993455443975934
777,3745,0,3745,0.20135116577148438,0.0029495920513499933
778,3749,0,3749,0.20156097412109375,0.002928679202933928
779,3752,0,3752,0.2017519474029541,0.002792985018095797
780,3755,0,3755,0.20193004608154297,0.002149576690520089
781,3758,0,3758,0.20210909843444824,0.0014142980567273971
782,3761,0,3761,0.202286958694458,0.0008118826837333725
783,3764,0,3764,0.20246315002441406,0.0006727181052367112
784,3767,0,3767,0.20264005661010742,0.000335780949150917
785,3770,0,3770,0.20283007621765137,0.0003316562315361246
786,3773,0,3773,0.20300889015197754,0.00019560898696204803
787,3776,0,3776,0.2031872272491455,0.00012995723925561043
788,3779,0,3779,0.2033698558807373,8.960494796511472e-05
789,3782,0,3782,0.20355010032653809,5.557787719045879e-05
790,3785,0,3785,0.20372819900512695,3.4676539081345926e-05
791,3788,0,3788,0.20390605926513672,2.5360310410476905e-05
792,3791,0,3791,0.20412421226501465,1.2610300794019908e-05
793,3794,0,3794,0.20430207252502441,6.963790802223473e-06
794,3797,0,3797,0.20447993278503418,2.563222749667823e-06
795,3800,0,3800,0.20465707778930664,1.245310197458052e-06
796,3803,0,3803,0.204833984375,5.483962478958642e-07
797,3806,0,3806,0.20501112937927246,2.7148522811413574e-07
798,3809,0,3809,0.20518803596496582,1.1099044556167601e-07
799,3812,0,3812,0.20543622970581055,6.396594287354097e-08
800,3815,0,3815,0.2056722640991211,3.96006303485275e-08
801,3818,0,3818,0.20592308044433594,2.21694481391203e-08
802,3821,0,3821,0.20612025260925293,1.1487308165073367e-08
803,3824,0,3824,0.2062971591949463,2.924367806202416e-09


==> plot_data/quadratic_minimax_problem_n20_alpha0/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.4849853515625e-05,4.387061074692293
200,201,200,401,0.004639863967895508,0.40381594893679745
400,401,400,801,0.009566068649291992,0.18772146832154463
601,602,601,1203,0.014384984970092773,0.12171316930208559
801,802,801,1603,0.018986940383911133,0.09207570470781463
1001,1002,1001,2003,0.02441692352294922,0.07543468087628187
1201,1202,1201,2403,0.03086090087890625,0.06522583375503957
1401,1402,1401,2803,0.03684592247009277,0.05859653621384203
1602,1603,1602,3205,0.04312491416931152,0.05398535261256449
1802,1803,1802,3605,0.04867196083068848,0.050568720173414815
2002,2003,2002,4005,0.05451202392578125,0.0478422859343471
2202,2203,2202,4405,0.060353994369506836,0.0455476036427356
2402,2403,2402,4805,0.06594514846801758,0.043545396617649314
2603,2604,2603,5207,0.07175898551940918,0.041751034903912645
2803,2804,2803,5607,0.0773019790649414,0.040138971290728194
3003,3004,3003,6007,0.08293914794921875,0.038673603472839595
3203,3204,3203,6407,0.08861207962036133,0.037337563217904775
3403,3404,3403,6807,0.09429693222045898,0.036118120569035975
3604,3605,3604,7209,0.1000511646270752,0.03499974829122583
3804,3805,3804,7609,0.10587000846862793,0.03398476792451849
4004,4005,4004,8009,0.1114962100982666,0.033059488662706915
4204,4205,4204,8409,0.11748409271240234,0.032216669653139886
4404,4405,4404,8809,0.12268805503845215,0.03144956322393217
4605,4606,4605,9211,0.12755298614501953,0.03074852389352344
4805,4806,4805,9611,0.13243889808654785,0.030114575566108637
5005,5006,5005,10011,0.13726305961608887,0.02953851197544041
5205,5206,5205,10411,0.1418750286102295,0.029015147922301927
5405,5406,5405,10811,0.1475832462310791,0.02853965450247292
5606,5607,5606,11213,0.15314912796020508,0.028105491621590647
5806,5807,5806,11613,0.1589951515197754,0.027712818646694996
6006,6007,6006,12013,0.16504597663879395,0.02735555365139795
6206,6207,6206,12413,0.17233920097351074,0.027030191666559268
6406,6407,6406,12813,0.1787738800048828,0.026733525004316607
6607,6608,6607,13215,0.18533611297607422,0.02646133298374186
6807,6808,6807,13615,0.19366908073425293,0.026213651724174072
7007,7008,7007,14015,0.20147013664245605,0.025986651714084007
7207,7208,7207,14415,0.21007704734802246,0.025778149602909813
7407,7408,7407,14815,0.21673107147216797,0.02558617470872729
7608,7609,7608,15217,0.2242898941040039,0.025408100367590745
7808,7809,7808,15617,0.23203015327453613,0.02524409689608381
8008,8009,8008,16017,0.23858404159545898,0.025091812293413254
8208,8209,8208,16417,0.24652314186096191,0.024949965111438623
8408,8409,8408,16817,0.2538609504699707,0.024817409200464654
8609,8610,8609,17219,0.2609739303588867,0.02469251854947162
8809,8810,8809,17619,0.26759910583496094,0.024575618954594473
9009,9010,9009,18019,0.2747502326965332,0.024465255731341735
9209,9210,9209,18419,0.2814829349517822,0.02436070462914114
9409,9410,9409,18819,0.2900969982147217,0.02426132140062413
9610,9611,9610,19221,0.2969820499420166,0.024166070134813377
9810,9811,9810,19621,0.302947998046875,0.024075387996634137
10010,10011,10010,20021,0.30895090103149414,0.023988338824701205
10210,10211,10210,20421,0.3144810199737549,0.023904522278487276
10410,10411,10410,20821,0.3206162452697754,0.023823583347133786
10611,10612,10611,21223,0.3268110752105713,0.023744821428552845
10811,10812,10811,21623,0.3336350917816162,0.023668740318461796
11011,11012,11011,22023,0.33917999267578125,0.02359469518416844
11211,11212,11211,22423,0.34412217140197754,0.02352246746056376
11411,11412,11411,22823,0.34891200065612793,0.023451863654645657
11612,11613,11612,23225,0.3544459342956543,0.023382370138534076
11812,11813,11812,23625,0.35936927795410156,0.023314526250139973
12012,12013,12012,24025,0.3648490905761719,0.023247848743321895
12212,12213,12212,24425,0.3694040775299072,0.023182219061697918
12412,12413,12412,24825,0.3742189407348633,0.02311753233229215
12613,12614,12613,25227,0.37912702560424805,0.023053378605362995
12813,12814,12813,25627,0.3838629722595215,0.02299031386559606
13013,13014,13013,26027,0.38857007026672363,0.022927944371611247
13213,13214,13213,26427,0.39339303970336914,0.022866205989388277
13413,13414,13413,26827,0.3978731632232666,0.02280504199824271
13614,13615,13614,27229,0.4027230739593506,0.022744100274303992
13814,13815,13814,27629,0.4074130058288574,0.022683942661489834
14014,14015,14014,28029,0.4123549461364746,0.02262422547421498
14214,14215,14214,28429,0.41718220710754395,0.022564914016596417
14414,14415,14414,28829,0.421766996383667,0.022505977593175366
14615,14616,14615,29231,0.42669105529785156,0.02244709693370252
14815,14816,14815,29631,0.4316699504852295,0.022388833786727257
15015,15016,15015,30031,0.436845064163208,0.022330873103682564
15215,15216,15215,30431,0.4429008960723877,0.02227319606086596
15415,15416,15415,30831,0.44853806495666504,0.022215785988761734
15616,15617,15616,31233,0.45428013801574707,0.022158342942859316
15816,15817,15816,31633,0.46036195755004883,0.022101425360413096
16016,16017,16016,32033,0.4663050174713135,0.0220447352442792
16216,16217,16216,32433,0.4726550579071045,0.02198826231413797
16416,16417,16416,32833,0.47873806953430176,0.021931997448480497
16617,16618,16617,33235,0.4845390319824219,0.02187565271502125
16817,16818,16817,33635,0.4904959201812744,0.02181978153656305
17017,17018,17017,34035,0.4963371753692627,0.021764096706864775
17217,17218,17217,34435,0.5020089149475098,0.021708592540622386
17417,17418,17417,34835,0.506845235824585,0.0216532639756776
17618,17619,17618,35237,0.5114028453826904,0.021597831135916627
17818,17819,17818,35637,0.5159249305725098,0.021542841550900242
18018,18019,18018,36037,0.5204808712005615,0.021488015417575432
18218,18219,18218,36437,0.5249919891357422,0.021433349521662506
18418,18419,18418,36837,0.5295209884643555,0.021378840984042746
18619,18620,18619,37239,0.5340499877929688,0.021324215837783468
18819,18820,18819,37639,0.5386450290679932,0.021270015286245968
19019,19020,19019,38039,0.5432412624359131,0.02121596508857388
19219,19220,19219,38439,0.5480492115020752,0.02116206335984908
19419,19420,19419,38839,0.5525989532470703,0.021108308395570062
19620,19621,19620,39241,0.5572519302368164,0.02105443096440624
19820,19821,19820,39641,0.5617220401763916,0.021000965750531356
20020,20021,20020,40041,0.5661952495574951,0.02094764306622261
20220,20221,20220,40441,0.5708270072937012,0.020894461742532046
20420,20421,20420,40841,0.5753891468048096,0.020841420707800085
20621,20622,20621,41243,0.580035924911499,0.020788254816175942
20821,20822,20821,41643,0.5844860076904297,0.020735492168325317
21021,21022,21021,42043,0.5889220237731934,0.02068286706790136
21221,21222,21221,42443,0.5933558940887451,0.020630378732431474
21421,21422,21421,42843,0.5977859497070312,0.02057802643208026
21622,21623,21622,43245,0.6025340557098389,0.020525548737833847
21822,21823,21822,43645,0.607025146484375,0.020473467171214583
22022,22023,22022,44045,0.6114659309387207,0.02042151970603057
22222,22223,22222,44445,0.6158959865570068,0.020369705769302023
22422,22423,22422,44845,0.6204588413238525,0.020318024816702637
22623,22624,22623,45247,0.6248950958251953,0.020266218918848774
22823,22824,22823,45647,0.6292939186096191,0.020214803058901585
23023,23024,23023,46047,0.6338410377502441,0.02016351868903903
23223,23224,23223,46447,0.6382660865783691,0.020112365350706877
23423,23424,23423,46847,0.6426711082458496,0.020061342601119834
23624,23625,23624,47249,0.6470749378204346,0.02001019587489068
23824,23825,23824,47649,0.6516032218933105,0.01995943367667865
24024,24025,24024,48049,0.6567468643188477,0.019908800815002316
24224,24225,24224,48449,0.6613161563873291,0.019858296894657453
24424,24425,24424,48849,0.6659281253814697,0.01980792152928542
24625,24626,24625,49251,0.6704521179199219,0.019757423425907274
24825,24826,24825,49651,0.675152063369751,0.019707304680306563
25025,25026,25025,50051,0.6798830032348633,0.01965731337301269
25225,25226,25225,50451,0.6842730045318604,0.01960744914472076
25425,25426,25425,50851,0.6885790824890137,0.019557711641248768
25626,25627,25626,51253,0.6930191516876221,0.01950785277432785
25826,25827,25826,51653,0.6981379985809326,0.019458368305263263
26026,26027,26026,52053,0.702549934387207,0.019409009522747787
26226,26227,26226,52453,0.7074248790740967,0.019359776088611527
26426,26427,26426,52853,0.7119240760803223,0.01931066766780371
26627,26628,26627,53255,0.7167232036590576,0.019261439322129204
26827,26828,26827,53655,0.7210819721221924,0.019212580554907842
27027,27028,27027,54055,0.7253780364990234,0.019163845810381056
27227,27228,27227,54455,0.7297439575195312,0.019115234763562167
27427,27428,27427,54855,0.7341310977935791,0.019066747091503262
27628,27629,27628,55257,0.7389450073242188,0.019018140958691903
27828,27829,27828,55657,0.7444350719451904,0.018969899687618447
28028,28029,28028,56057,0.7496130466461182,0.018921780831721528
28228,28229,28228,56457,0.7545750141143799,0.01887378407490503
28428,28429,28428,56857,0.7593221664428711,0.018825909102526496
28629,28630,28629,57259,0.7643072605133057,0.01877791713848351
28829,28830,28829,57659,0.7695810794830322,0.01873028540149359
29029,29030,29029,58059,0.7746810913085938,0.018682774511433065
29229,29230,29229,58459,0.7791268825531006,0.018635384158768097
29429,29430,29429,58859,0.7836101055145264,0.018588114035100085
29630,29631,29630,59261,0.7880859375,0.01854072838290067
29830,29831,29830,59661,0.7925732135772705,0.018493698393667487
30030,30031,30030,60061,0.7970349788665771,0.018446787713109657
30230,30231,30230,60461,0.8015620708465576,0.018399996036982964
30430,30431,30430,60861,0.8062691688537598,0.018353323062002852
30631,30632,30631,61263,0.8107690811157227,0.018306536009909707
30831,30832,30831,61663,0.8153362274169922,0.018260100120819935
31031,31032,31031,62063,0.819770097732544,0.01821378202705017
31231,31232,31231,62463,0.8242220878601074,0.018167581428940004
31431,31432,31431,62863,0.8288900852203369,0.018121498027690162
31632,31633,31632,63265,0.8334949016571045,0.018075301986046007
31832,31833,31832,63665,0.8379511833190918,0.018029452667758666
32032,32033,32032,64065,0.8423850536346436,0.017983719653487926
32232,32233,32232,64465,0.8468079566955566,0.01793810264775641
32432,32433,32432,64865,0.8512461185455322,0.01789260135589033
32633,32634,32633,65267,0.8557019233703613,0.01784698884415227
32833,32834,32833,65667,0.8601250648498535,0.017801718674069218
33033,33034,33033,66067,0.8645439147949219,0.017756563337113212
33233,33234,33233,66467,0.8689661026000977,0.017711522541752723
33433,33434,33433,66867,0.8733890056610107,0.017666595997224765
33634,33635,33634,67269,0.8780450820922852,0.01762155963645188
33834,33835,33834,67669,0.8824450969696045,0.017576861291980734
34034,34035,34034,68069,0.8868131637573242,0.017532276329172997
34234,34235,34234,68469,0.8911421298980713,0.017487804460294142
34434,34435,34434,68869,0.8954920768737793,0.017443445398355236
34635,34636,34635,69271,0.8998062610626221,0.017398977906631388
34835,34836,34835,69671,0.9048850536346436,0.017354844161028966
35035,35036,35035,70071,0.9092929363250732,0.017310822364414544
35235,35236,35235,70471,0.9136319160461426,0.017266912232749683
35435,35436,35435,70871,0.917992115020752,0.01722311348272494
35636,35637,35636,71273,0.9225950241088867,0.017179207672164687
35836,35837,35836,71673,0.9270989894866943,0.017135631391772068
36036,36037,36036,72073,0.9326870441436768,0.01709216564603267
36236,36237,36236,72473,0.9378170967102051,0.01704881015452894
36436,36437,36436,72873,0.9426250457763672,0.017005564637559117
36637,36638,36637,73275,0.9474530220031738,0.016962213412170267
36837,36838,36837,73675,0.9520621299743652,0.016919187554402863
37037,37038,37037,74075,0.957766056060791,0.01687627083494987
37237,37238,37237,74475,0.9623599052429199,0.016833462976953414
37437,37438,37437,74875,0.9673869609832764,0.01679076370426042
37638,37639,37638,75277,0.9717590808868408,0.016747960058273063
37838,37839,37838,75677,0.9762961864471436,0.01670547767002248
38038,38039,38038,76077,0.981774091720581,0.016663103041455164
38238,38239,38238,76477,0.986260175704956,0.016620835899219973
38438,38439,38438,76877,0.9907019138336182,0.016578675970660334
38639,38640,38639,77279,0.995150089263916,0.016536412987113464
38839,38840,38839,77679,0.9995901584625244,0.016494467203376332
39039,39040,39039,78079,1.0051891803741455,0.016452627818143002
39239,39240,39239,78479,1.0096559524536133,0.016410894561520253
39439,39440,39439,78879,1.0146658420562744,0.016369267164299924
39640,39641,39640,79281,1.019242286682129,0.016327538013772902
39840,39841,39840,79681,1.0237832069396973,0.016286122056409003
40040,40041,40040,80081,1.0286250114440918,0.01624481115358313
40240,40241,40240,80481,1.0332369804382324,0.016203605038813754
40440,40441,40440,80881,1.0390000343322754,0.016162503446295776
40641,40642,40641,81283,1.043808937072754,0.016121301385723173
40841,40842,40841,81683,1.0491528511047363,0.016080408562288893
41041,41042,41041,82083,1.054746150970459,0.01603961946641369
41241,41242,41241,82483,1.0603530406951904,0.01599893383498341
41441,41442,41441,82883,1.06557297706604,0.015958351405551734
41642,41643,41642,83285,1.070216178894043,0.015917669777090578
41842,41843,41842,83685,1.0747220516204834,0.015877293479719213
42042,42043,42042,84085,1.079261064529419,0.015837019599695096
42242,42243,42242,84485,1.083773136138916,0.015796847877228442
42442,42443,42442,84885,1.0882740020751953,0.01575677805318848
42643,42644,42643,85287,1.0928170680999756,0.015716610283118767
42843,42844,42843,85687,1.0973281860351562,0.015676743987432174
43043,43044,43043,86087,1.1019790172576904,0.015636978815433716
43243,43244,43243,86487,1.1065618991851807,0.015597314510615549
43443,43444,43443,86887,1.1110661029815674,0.015557750817120401
43644,43645,43644,87289,1.1156229972839355,0.015518090414770347
43844,43845,43844,87689,1.1202342510223389,0.01547872767881359
44044,44045,44044,88089,1.1258690357208252,0.01543946478922811
44244,44245,44244,88489,1.130647897720337,0.015400301492746243
44444,44445,44444,88889,1.1353390216827393,0.015361237536742746
44645,44646,44645,89291,1.1402668952941895,0.015322078093433228
44845,44846,44845,89691,1.1450350284576416,0.015283212556627904
45045,45046,45045,90091,1.149496078491211,0.015244445605011868
45245,45246,45245,90491,1.1541821956634521,0.015205776988516741
45445,45446,45445,90891,1.1587119102478027,0.015167206457708372
45646,45647,45646,91293,1.1631782054901123,0.015128541645713789
45846,45847,45846,91693,1.167625904083252,0.015090167027826827
46046,46047,46046,92093,1.172051191329956,0.015051889749877964
46246,46247,46246,92493,1.1764910221099854,0.015013709564957529
46446,46447,46446,92893,1.1809141635894775,0.014975626226782036
46647,46648,46647,93295,1.186079978942871,0.014937449798305899
46847,46848,46847,93695,1.1916022300720215,0.01489955989843313
47047,47048,47047,94095,1.196099042892456,0.01486176610897657
47247,47248,47247,94495,1.2005841732025146,0.014824068186145274
47447,47448,47447,94895,1.2050130367279053,0.014786465886766815
47648,47649,47648,95297,1.209428071975708,0.01474877167293099
47848,47849,47848,95697,1.2138121128082275,0.014711360368494216
48048,48049,48048,96097,1.2182419300079346,0.014674043960482231
48248,48249,48248,96497,1.2226450443267822,0.014636822208183553
48448,48449,48448,96897,1.2271180152893066,0.01459969487149727
48649,48650,48649,97299,1.231537103652954,0.014562476781344738
48849,48850,48849,97699,1.235931158065796,0.014525538027101903
49049,49050,49049,98099,1.2403271198272705,0.014488692970626776
49249,49250,49249,98499,1.2447359561920166,0.014451941374248307
49449,49450,49449,98899,1.250218152999878,0.014415283000898296
49650,49651,49650,99301,1.254668951034546,0.014378535020408414
49850,49851,49850,99701,1.259140968322754,0.014342062847476583
50050,50051,50050,100101,1.2635550498962402,0.014305683188795841
50250,50251,50250,100501,1.2679929733276367,0.01426939580969725
50450,50451,50450,100901,1.2724058628082275,0.01423320047610703
50651,50652,50651,101303,1.2768869400024414,0.014196916667223903
50851,50852,50851,101703,1.2813119888305664,0.01416090518211448
51051,51052,51051,102103,1.2857341766357422,0.014124985042688823
51251,51252,51251,102503,1.2903552055358887,0.014089156017242099
51451,51452,51451,102903,1.2948310375213623,0.014053417874657293
51652,51653,51652,103305,1.2993299961090088,0.01401759237432987
51852,51853,51852,103705,1.303814172744751,0.01398203575799627
52052,52053,52052,104105,1.308351993560791,0.013946569333539537
52252,52253,52252,104505,1.3128039836883545,0.01391119287218155
52452,52453,52452,104905,1.317249059677124,0.013875906145724603
52653,52654,52653,105307,1.3217051029205322,0.013840533164959378
52853,52854,52853,105707,1.326153039932251,0.013805425671856716
53053,53054,53053,106107,1.3305730819702148,0.013770407231397955
53253,53254,53253,106507,1.335010051727295,0.013735477617694843
53453,53454,53453,106907,1.3394138813018799,0.013700636605431978
53654,53655,53654,107309,1.3439929485321045,0.013665710428357495
53854,53855,53854,107709,1.348466157913208,0.013631046385514035
54054,54055,54054,108109,1.3529560565948486,0.013596470270471511
54254,54255,54254,108509,1.3574330806732178,0.013561981860194845
54454,54455,54454,108909,1.3619630336761475,0.013527580932214706
54655,54656,54655,109311,1.3664422035217285,0.01349309591515787
54855,54856,54855,109711,1.37089204788208,0.013458869721258501
55055,55056,55055,110111,1.3753490447998047,0.0134247303445252
55255,55256,55255,110511,1.3797919750213623,0.013390677564740074
55455,55456,55455,110911,1.384174108505249,0.013356711162243835
55656,55657,55656,111313,1.3891198635101318,0.013322661732818054
55856,55857,55856,111713,1.393604040145874,0.013288867857299037
56056,56057,56056,112113,1.3978321552276611,0.0132551597023399
56256,56257,56256,112513,1.4021391868591309,0.013221537050504332
56456,56457,56456,112913,1.4064390659332275,0.01318799968490764
56657,56658,56657,113315,1.4106919765472412,0.013154380341112314
56857,56858,56857,113715,1.4149410724639893,0.013121013323267651
57057,57058,57057,114115,1.419166088104248,0.013087730943228121
57257,57258,57257,114515,1.42336106300354,0.013054532986303933
57457,57458,57457,114915,1.427612066268921,0.013021419238349846
57658,57659,57658,115317,1.4318199157714844,0.012988224547681317
57858,57859,57858,115717,1.4360721111297607,0.012955278995780355
58058,58059,58058,116117,1.4402642250061035,0.012922417012606286
58258,58259,58258,116517,1.4444708824157715,0.012889638386181117
58458,58459,58458,116917,1.4486780166625977,0.012856942905064533
58659,58660,58659,117319,1.4530551433563232,0.012824167503638267
58859,58860,58859,117719,1.4593489170074463,0.01279163809405452
59059,59060,59059,118119,1.4650249481201172,0.01275919119762313
59259,59260,59259,118519,1.4694271087646484,0.012726826605043765
59459,59460,59459,118919,1.473663091659546,0.012694544107546796
59660,59661,59660,119321,1.4785881042480469,0.01266218269923065
59860,59861,59860,119721,1.4828600883483887,0.01263006417558137
60060,60061,60060,120121,1.4874699115753174,0.012598027122843218
60260,60261,60260,120521,1.4919159412384033,0.012566071334359498
60460,60461,60460,120921,1.49635910987854,0.012534196603997582
60661,60662,60661,121323,1.500723123550415,0.01250224395955597
60861,60862,60861,121723,1.505167007446289,0.012470531131853028
61061,61062,61061,122123,1.5095462799072266,0.012438898745984694
61261,61262,61261,122523,1.5138940811157227,0.012407346597904542
61461,61462,61461,122923,1.5182502269744873,0.012375874484083775
61662,61663,61662,123325,1.5226280689239502,0.012344325440332713
61862,61863,61862,123725,1.526975154876709,0.012313013184143793
62062,62063,62062,124125,1.5313341617584229,0.012281780353711453
62262,62263,62262,124525,1.5356709957122803,0.012250626747566594
62462,62463,62462,124925,1.5400030612945557,0.012219552164751285
62663,62664,62663,125327,1.545685052871704,0.012188401623724084
62863,62864,62863,125727,1.5500500202178955,0.01215748487934457
63063,63064,63063,126127,1.5544118881225586,0.012126646557477949
63263,63264,63263,126527,1.558772087097168,0.01209588645919991
63463,63464,63463,126927,1.5631248950958252,0.01206520438609078
63664,63665,63664,127329,1.567528247833252,0.012034447314214212
63864,63865,63864,127729,1.5718870162963867,0.012003921085849887
64064,64065,64064,128129,1.5762500762939453,0.011973472289426836
64264,64265,64264,128529,1.580604076385498,0.01194310072853357
64464,64465,64464,128929,1.584834098815918,0.011912806207256604
64665,64666,64665,129331,1.589043140411377,0.011882437634537609
64865,64866,64865,129731,1.5931921005249023,0.011852296989497092
65065,65066,65065,130131,1.5973520278930664,0.011822232798338432
65265,65266,65265,130531,1.6015799045562744,0.011792244867131
65465,65466,65465,130931,1.6061842441558838,0.011762333002436004
65666,65667,65666,131333,1.6103579998016357,0.011732348021658632
65866,65867,65866,131733,1.6144790649414062,0.011702588089556416
66066,66067,66066,132133,1.6186530590057373,0.011672903645630754
66266,66267,66266,132533,1.6227738857269287,0.01164329449840049
66466,66467,66466,132933,1.626889944076538,0.011613760456870287
66667,66668,66667,133335,1.6311299800872803,0.01158415422280255
66867,66868,66867,133735,1.635815143585205,0.011554770194772038
67067,67068,67067,134135,1.6405069828033447,0.011525460701410733
67267,67268,67267,134535,1.6447300910949707,0.011496225553656161
67467,67468,67467,134935,1.648906946182251,0.011467064562925493
67668,67669,67668,135337,1.6538410186767578,0.011437832291536717
67868,67869,67868,135737,1.6589951515197754,0.011408819419453108
68068,68069,68068,136137,1.663304090499878,0.011379880140575388
68268,68269,68268,136537,1.6675770282745361,0.011351014268229114
68468,68469,68468,136937,1.6717760562896729,0.01132222161621349
68669,68670,68669,137339,1.676020860671997,0.011293358583901018
68869,68870,68869,137739,1.6802289485931396,0.011264712179614122
69069,69070,69069,138139,1.6845300197601318,0.011236138438961521
69269,69270,69269,138539,1.6888511180877686,0.011207637177626852
69469,69470,69469,138939,1.6942031383514404,0.011179208211761124
69670,69671,69670,139341,1.698655128479004,0.011150709754587151
69870,69871,69870,139741,1.703038215637207,0.011122425189163782
70070,70071,70070,140141,1.70849609375,0.01109421236954484
70270,70271,70270,140541,1.7140440940856934,0.011066071113742013
70470,70471,70470,140941,1.7197060585021973,0.011038001240228575
70671,70672,70671,141343,1.7246649265289307,0.01100986275316647
70871,70872,70871,141743,1.7292211055755615,0.010981935456142532
71071,71072,71071,142143,1.7337660789489746,0.010954078998686417
71271,71272,71271,142543,1.7386860847473145,0.010926293201108531
71471,71472,71471,142943,1.7439351081848145,0.010898577884175052
71672,71673,71672,143345,1.7487220764160156,0.010870794820365333
71872,71873,71872,143745,1.7543280124664307,0.0108432202790072
72072,72073,72072,144145,1.7614240646362305,0.01081571568242712
72272,72273,72272,144545,1.7672638893127441,0.010788280853205224
72472,72473,72472,144945,1.7727782726287842,0.010760915614371648
72673,72674,72673,145347,1.778320074081421,0.010733483484387142
72873,72874,72873,145747,1.7840921878814697,0.010706257242962484
73073,73074,73073,146147,1.7896850109100342,0.010679100062828434
73273,73274,73273,146547,1.7951562404632568,0.01065201176880613
73473,73474,73473,146947,1.800079107284546,0.010624992186161093
73674,73675,73674,147349,1.8047630786895752,0.010597906557281505
73874,73875,73874,147749,1.8094439506530762,0.01057102421633934
74074,74075,74074,148149,1.8144240379333496,0.010544210064359861
74274,74275,74274,148549,1.8190429210662842,0.010517463928376887
74474,74475,74474,148949,1.8237311840057373,0.010490785635863056
74675,74676,74675,149351,1.8287551403045654,0.010464042131358842
74875,74876,74875,149751,1.8333821296691895,0.010437499347018535
75075,75076,75075,150151,1.837947130203247,0.010411023890331533
75275,75276,75275,150551,1.8426799774169922,0.010384615590516429
75475,75476,75475,150951,1.8472192287445068,0.01035827427722511
75676,75677,75676,151353,1.8517742156982422,0.010331868575649987
75876,75877,75876,151753,1.8564770221710205,0.010305661058899476
76076,76077,76076,152153,1.8613018989562988,0.01027952001937224
76276,76277,76276,152553,1.8660099506378174,0.010253445288444088
76476,76477,76476,152953,1.870615005493164,0.010227436697918604
76677,76678,76677,153355,1.8752970695495605,0.01020136453241153
76877,76878,76877,153755,1.8799800872802734,0.010175488048414078
77077,77078,77077,154155,1.884425163269043,0.010149677201951911
77277,77278,77277,154555,1.8896920680999756,0.010123931826530708
77477,77478,77477,154955,1.8942430019378662,0.01009825175607857
77678,77679,77678,155357,1.8987770080566406,0.010072508913674031
77878,77879,77878,155757,1.9033520221710205,0.010046959281084143
78078,78079,78078,156157,1.9080009460449219,0.010021474456947755
78278,78279,78278,156557,1.9126639366149902,0.00999605427687362
78478,78479,78478,156957,1.9171559810638428,0.009970698576887533
78679,78680,78679,157359,1.9216229915618896,0.009945280897834979
78879,78880,78879,157759,1.9262380599975586,0.00992005398812255
79079,79080,79079,158159,1.9307711124420166,0.009894891068254181
79279,79280,79279,158559,1.9362010955810547,0.009869791975915053
79479,79480,79479,158959,1.9406070709228516,0.009844756549202152
79680,79681,79680,159361,1.945024013519287,0.0098196599262937
79880,79881,79880,159761,1.9494309425354004,0.009794751663076999
80080,80081,80080,160161,1.9538369178771973,0.009769906581434942
80280,80281,80280,160561,1.958456039428711,0.009745124521102926
80480,80481,80480,160961,1.962989091873169,0.009720405322222984
80681,80682,80681,161363,1.9674978256225586,0.009695625700129735
80881,80882,80881,161763,1.9719021320343018,0.009671032058516674
81081,81082,81081,162163,1.9772090911865234,0.009646500800418244
81281,81282,81281,162563,1.9821500778198242,0.009622031767594248
81481,81482,81481,162963,1.9866971969604492,0.00959762480220585
81682,81683,81682,163365,1.9911441802978516,0.009573158176822716
81882,81883,81882,163765,1.995671033859253,0.00954887518276047
82082,82083,82082,164165,2.000185012817383,0.009524653784233334
82282,82283,82282,164565,2.0047049522399902,0.009500493824999873
82482,82483,82482,164965,2.0095322132110596,0.009476395149214984
82683,82684,82683,165367,2.014035224914551,0.009452237567013466
82883,82884,82883,165767,2.0185141563415527,0.00942826129664634
83083,83084,83083,166167,2.0229952335357666,0.009404345843787973
83283,83284,83283,166567,2.027616024017334,0.009380491054170353
83483,83484,83483,166967,2.032104253768921,0.009356696773916966
83684,83685,83684,167369,2.0370590686798096,0.009332844331306532
83884,83885,83884,167769,2.041511058807373,0.009309170910341929
84084,84085,84084,168169,2.0462749004364014,0.009285557538687048
84284,84285,84284,168569,2.0510239601135254,0.00926200406402262
84484,84485,84484,168969,2.055549144744873,0.00923851033441562
84685,84686,84685,169371,2.0600271224975586,0.009214959177112767
84885,84886,84885,169771,2.0646162033081055,0.009191584780195008
85085,85086,85085,170171,2.069549083709717,0.009168269674091326
85285,85286,85285,170571,2.0739681720733643,0.009145013708406362
85485,85486,85485,170971,2.0783820152282715,0.009121816733126262
85686,85687,85686,171373,2.0832738876342773,0.009098563055531797
85886,85887,85886,171773,2.08787202835083,0.009075483905624149
86086,86087,86086,172173,2.092331886291504,0.009052463297615594
86286,86287,86286,172573,2.097454071044922,0.009029501083010509
86486,86487,86486,172973,2.1019480228424072,0.009006597113689825
86687,86688,86687,173375,2.1066689491271973,0.008983637158273886
86887,86888,86887,173775,2.1120030879974365,0.008960849526048196
87087,87088,87087,174175,2.1173322200775146,0.008938119696266369
87287,87288,87287,174575,2.122162103652954,0.008915447522308394
87487,87488,87487,174975,2.1271259784698486,0.008892832857926216
87688,87689,87688,175377,2.1324288845062256,0.008870162914621072
87888,87889,87888,175777,2.1372158527374268,0.008847663117855108
88088,88089,88088,176177,2.142331123352051,0.008825220393417968
88288,88289,88288,176577,2.1470320224761963,0.008802834596541655
88488,88489,88488,176977,2.1516940593719482,0.008780505582825329
88689,88690,88689,177379,2.1576480865478516,0.008758121988425946
88889,88890,88889,177779,2.162445068359375,0.008735906391408432
89089,89090,89089,178179,2.170429229736328,0.00871374714582693
89289,89290,89289,178579,2.1763408184051514,0.008691644108742054
89489,89490,89489,178979,2.181994915008545,0.008669597137576925
89690,89691,89690,179381,2.187751054763794,0.008647496275149014
89890,89891,89890,179781,2.193161964416504,0.008625561288092052
90090,90091,90090,180181,2.1979870796203613,0.008603681940684067
90290,90291,90290,180581,2.202620029449463,0.008581858091791126
90490,90491,90490,180981,2.207059144973755,0.008560089600637352
90691,90692,90691,181383,2.211686134338379,0.00853826789893286
90891,90892,90891,181783,2.2162270545959473,0.008516609977392021
91091,91092,91091,182183,2.220734119415283,0.008495006992703832
91291,91292,91291,182583,2.225343942642212,0.00847345880551707
91491,91492,91491,182983,2.229825019836426,0.008451965276834023
91692,91693,91692,183385,2.2343380451202393,0.008430419209714088
91892,91893,91892,183785,2.2388479709625244,0.008409034854015509
92092,92093,92092,184185,2.243351936340332,0.008387704741250472
92292,92293,92292,184585,2.2479851245880127,0.008366428733827905
92492,92493,92492,184985,2.2525339126586914,0.00834520669450577
92693,92694,92693,185387,2.2571089267730713,0.00832393278037102
92893,92894,92893,185787,2.2617199420928955,0.008302818535046046
93093,93094,93093,186187,2.2664201259613037,0.008281757847500452
93293,93294,93293,186587,2.2709851264953613,0.008260750581881172
93493,93494,93493,186987,2.2755119800567627,0.008239796602679698
93694,93695,93694,187389,2.280048131942749,0.008218791403907525
93894,93895,93894,187789,2.2845520973205566,0.008197943857134187
94094,94095,94094,188189,2.2889561653137207,0.008177149191640472
94294,94295,94294,188589,2.2934298515319824,0.008156407273289274
94494,94495,94494,188989,2.29830002784729,0.008135717968283742
94695,94696,94695,189391,2.3027591705322266,0.008114978090672851
94895,94896,94895,189791,2.3073971271514893,0.008094393873724655
95095,95096,95095,190191,2.311850070953369,0.008073861870101326
95295,95296,95295,190591,2.316822052001953,0.008053381947360104
95495,95496,95495,190991,2.321263074874878,0.008032953973394047
95696,95697,95696,191393,2.325801134109497,0.008012476065616076
95896,95897,95896,191793,2.3302299976348877,0.007992151852317662
96096,96097,96096,192193,2.3348982334136963,0.00797187919282643
96296,96297,96296,192593,2.339334011077881,0.00795165795637253
96496,96497,96496,192993,2.3437511920928955,0.007931488012517734
96697,96698,96697,193395,2.3483200073242188,0.007911268765575635
96897,96898,96897,193795,2.3527660369873047,0.007891201271765257
97097,97098,97097,194195,2.357196092605591,0.00787118468057487
97297,97298,97297,194595,2.3619072437286377,0.007851218862886417
97497,97498,97497,194995,2.36635422706604,0.007831303689909315
97698,97699,97698,195397,2.370897054672241,0.007811339836602728
97898,97899,97898,195797,2.375274181365967,0.007791525819601563
98098,98099,98098,196197,2.3796262741088867,0.007771762062258557
98298,98299,98298,196597,2.384125232696533,0.007752048437086452
98498,98499,98498,196997,2.388500213623047,0.007732384816921514
98699,98700,98699,197399,2.3931009769439697,0.00771267313131878
98899,98900,98899,197799,2.3975861072540283,0.007693109389407008
99099,99100,99099,198199,2.402040958404541,0.007673595272312884
99299,99300,99299,198599,2.4065818786621094,0.007654130654159521
99499,99500,99499,198999,2.410975217819214,0.007634715409389333
99700,99701,99700,199401,2.415682077407837,0.007615252706306204
99900,99901,99900,199801,2.4202122688293457,0.007595936078205624
100100,100101,100100,200201,2.4245541095733643,0.007576668448100985
100300,100301,100300,200601,2.43087100982666,0.007557449691705395
100501,100502,100501,201003,2.4354331493377686,0.007538183957289869
100701,100702,100701,201403,2.4399569034576416,0.007519062819532193
100901,100902,100901,201803,2.4445149898529053,0.007499990183895353
101101,101102,101101,202203,2.448895215988159,0.007480965927350294
101301,101302,101301,202603,2.453577995300293,0.007461989927179993
101502,101503,101502,203005,2.458428144454956,0.007442967542379198
101702,101703,101702,203405,2.4629878997802734,0.007424087927804905
101902,101903,101902,203805,2.467694044113159,0.007405256202710798
102102,102103,102102,204205,2.47290301322937,0.0073864722456217806
102302,102303,102302,204605,2.4774739742279053,0.007367735935370928
102503,102504,102503,205007,2.4820761680603027,0.007348953826383767
102703,102704,102703,205407,2.486721992492676,0.007330312684261829
102903,102904,102903,205807,2.491117000579834,0.007311718826717828
103103,103104,103103,206207,2.4954750537872314,0.00729317213381102
103303,103304,103303,206607,2.5003280639648438,0.0072746724859049225
103504,103505,103504,207009,2.5048270225524902,0.00725612761775619
103704,103705,103704,207409,2.509537935256958,0.007237721935890049
103904,103905,103904,207809,2.514482021331787,0.007219362941340172
104104,104105,104104,208209,2.5191001892089844,0.007201050515680893
104304,104305,104304,208609,2.5236289501190186,0.007182784540786898
104505,104506,104505,209011,2.5281598567962646,0.0071644739168368115
104705,104706,104705,209411,2.532650947570801,0.007146300721077559
104905,104906,104905,209811,2.5370569229125977,0.007128173622917085
105105,105106,105105,210211,2.541674852371216,0.0071100925054255635
105305,105306,105305,210611,2.5462141036987305,0.00709205725196978
105506,105507,105506,211013,2.5506670475006104,0.007073977913429696
105706,105707,105706,211413,2.555239200592041,0.007056034267195547
105906,105907,105906,211813,2.559953212738037,0.00703813613629158
106106,106107,106106,212213,2.568120002746582,0.007020283405264846
106306,106307,106306,212613,2.573618173599243,0.007002475958955426
106507,106508,106507,213015,2.578350067138672,0.006984624984409787
106707,106708,106707,213415,2.583627939224243,0.006966907988211606
106907,106908,106907,213815,2.588456153869629,0.006949235932429703
107107,107108,107107,214215,2.593257188796997,0.006931608703069472
107307,107308,107307,214615,2.598057270050049,0.006914026186425605
107508,107509,107508,215017,2.6026699542999268,0.006896400691360003
107708,107709,107708,215417,2.607964038848877,0.006878907482332652
107908,107909,107908,215817,2.612884998321533,0.006861458646069543
108108,108109,108108,216217,2.6201488971710205,0.006844054070016028
108308,108309,108308,216617,2.6296989917755127,0.006826693641902931
108509,108510,108509,217019,2.635322093963623,0.006809290778237789
108709,108710,108709,217419,2.6412599086761475,0.00679201852967759
108909,108910,108909,217819,2.6479599475860596,0.006774790093399799
109109,109110,109109,218219,2.6549670696258545,0.006757605358271387
109309,109310,109309,218619,2.6624810695648193,0.00674046421344134
109510,109511,109510,219021,2.668572187423706,0.00672328116907173
109710,109711,109710,219421,2.675765037536621,0.006706227089979789
109910,109911,109910,219821,2.6813700199127197,0.006689216269767864
110110,110111,110110,220221,2.6870241165161133,0.006672248598706794
110310,110311,110310,220621,2.6930012702941895,0.006655323967345684
110511,110512,110511,221023,2.6986629962921143,0.0066383579656871085
110711,110712,110711,221423,2.7042269706726074,0.006621519300318119
110911,110912,110911,221823,2.709254026412964,0.00660472334741702
111111,111112,111111,222223,2.7139408588409424,0.0065879699986406
111311,111312,111311,222623,2.718528985977173,0.006571259145920513
111512,111513,111512,223025,2.7232460975646973,0.0065545074454599886
111712,111713,111712,223425,2.728031873703003,0.006537881472877161
111912,111913,111912,223825,2.7329180240631104,0.006521297673251863
112112,112113,112112,224225,2.7375340461730957,0.006504755939609424
112312,112313,112312,224625,2.7422120571136475,0.00648825616524653
112513,112514,112513,225027,2.746751070022583,0.00647171605909978
112713,112714,112713,225427,2.753690004348755,0.006455300092734991
112913,112914,112913,225827,2.7589569091796875,0.006438925766632075
113113,113114,113113,226227,2.764644145965576,0.006422592975167617
113313,113314,113313,226627,2.7728569507598877,0.006406301612986043
113514,113515,113514,227029,2.778931140899658,0.006389970428460015
113714,113715,113714,227429,2.7846460342407227,0.006373761815679773
113914,113915,113914,227829,2.7903661727905273,0.006357594317194347
114114,114115,114114,228229,2.7959132194519043,0.006341467828714488
114314,114315,114314,228629,2.801302909851074,0.006325382246215377
114515,114516,114515,229031,2.8061470985412598,0.006309257344376332
114715,114716,114715,229431,2.8106679916381836,0.006293253466053127
114915,114916,114915,229831,2.8151352405548096,0.0062772901827013025
115115,115116,115115,230231,2.819669008255005,0.006261367391348863
115315,115316,115315,230631,2.8242039680480957,0.006245484989284952
115516,115517,115516,231033,2.828943967819214,0.006229563764532147
115716,115717,115716,231433,2.8334319591522217,0.00621376203462126
115916,115917,115916,231833,2.838203191757202,0.006198000386917952
116116,116117,116116,232233,2.8429200649261475,0.0061822787197509405
116316,116317,116316,232633,2.8475639820098877,0.00616659693170671
116517,116518,116517,233035,2.85209584236145,0.006150876811351268
116717,116718,116717,233435,2.856610059738159,0.006135274676472807
116917,116918,116917,233835,2.86125111579895,0.006119712117515022
117117,117118,117117,234235,2.8657288551330566,0.00610418903409079
117317,117318,117317,234635,2.870225191116333,0.006088705326067621
117518,117519,117518,235037,2.8747270107269287,0.0060731837699168865
117718,117719,117718,235437,2.8796420097351074,0.0060577787089433
117918,117919,117918,235837,2.8842310905456543,0.006042412723998459
118118,118119,118118,236237,2.888791084289551,0.006027085715963259
118318,118319,118318,236637,2.8935799598693848,0.006011797585969998
118519,118520,118519,237039,2.897994041442871,0.005996472085916947
118719,118720,118719,237439,2.902467966079712,0.0059812616095655515
118919,118920,118919,237839,2.907644033432007,0.005966089715665233
119119,119120,119119,238239,2.9121201038360596,0.005950956306348861
119319,119320,119319,238639,2.916670083999634,0.005935861283997545
119520,119521,119520,239041,2.9215641021728516,0.005920729363615683
119720,119721,119720,239441,2.9260220527648926,0.005905711014046461
119920,119921,119920,239841,2.930438995361328,0.005890730759585137
120120,120121,120120,240241,2.9348111152648926,0.005875788503600753
120320,120321,120320,240641,2.9392318725585938,0.005860884149707467
120521,120522,120521,241043,2.9436440467834473,0.005845943363850492
120721,120722,120721,241443,2.9479920864105225,0.0058311147142689635
120921,120922,120921,241843,2.952345132827759,0.005816323678607846
121121,121122,121121,242243,2.9569661617279053,0.0058015701614567644
121321,121322,121321,242643,2.9613301753997803,0.005786854067647373
121522,121523,121522,243045,2.9661879539489746,0.005772102002054286
121722,121723,121722,243445,2.970616102218628,0.005757460656319332
121922,121923,121922,243845,2.975037097930908,0.005742856449395282
122122,122123,122122,244245,2.9794511795043945,0.005728289287076932
122322,122323,122322,244645,2.984351873397827,0.005713759075398043
122523,122524,122523,245047,2.9888739585876465,0.005699193346302701
122723,122724,122723,245447,2.993381977081299,0.005684736938539269
122923,122924,122923,245847,2.998181104660034,0.005670317200478544
123123,123124,123123,246247,3.0026040077209473,0.005655934039105154
123323,123324,123323,246647,3.0071699619293213,0.005641587361639771
123524,123525,123524,247049,3.0119762420654297,0.005627205615386064
123724,123725,123724,247449,3.0163869857788086,0.005612931809603111
123924,123925,123924,247849,3.0208029747009277,0.005598694210339938
124124,124125,124124,248249,3.0262110233306885,0.005584492725756176
124324,124325,124324,248649,3.030644178390503,0.005570327264244377
124525,124526,124525,249051,3.035069227218628,0.005556127176905643
124725,124726,124725,249451,3.0395660400390625,0.00554203366661847
124925,124926,124925,249851,3.0446109771728516,0.005527975905518786
125125,125126,125125,250251,3.049086093902588,0.005513953802926247
125325,125326,125325,250651,3.0535941123962402,0.005499967268390555
125526,125527,125526,251053,3.058664083480835,0.005485946545394132
125726,125727,125726,251453,3.0630991458892822,0.0054720310532517195
125926,125927,125926,251853,3.0675549507141113,0.005458150858741152
126126,126127,126126,252253,3.0722970962524414,0.00544430587232754
126326,126327,126326,252653,3.0767650604248047,0.005430496004702983
126527,126528,126527,253055,3.081233024597168,0.005416652380459474
126727,126728,126727,253455,3.0879158973693848,0.00540291265787657
126927,126928,126927,253855,3.0934791564941406,0.005389207787073566
127127,127128,127127,254255,3.098233938217163,0.005375537679646487
127327,127328,127327,254655,3.103893995285034,0.005361902247415541
127528,127529,127528,255057,3.1098270416259766,0.005348233484952717
127728,127729,127728,255457,3.1144580841064453,0.005334667311746366
127928,127929,127928,255857,3.1198818683624268,0.005321135550099645
128128,128129,128128,256257,3.1251308917999268,0.005307638112725171
128328,128329,128328,256657,3.12985897064209,0.0052941749125570295
128529,128530,128529,257059,3.1359269618988037,0.005280678803158308
128729,128730,128729,257459,3.141576051712036,0.005267283987189191
128929,128930,128929,257859,3.1464109420776367,0.005253923148119931
129129,129130,129129,258259,3.151136875152588,0.005240596199765714
129329,129330,129329,258659,3.1572201251983643,0.005227303056160358
129530,129531,129530,259061,3.162796974182129,0.005213977419007919
129730,129731,129730,259461,3.167579174041748,0.00520075179582609
129930,129931,129930,259861,3.1720900535583496,0.0051875597203746545
130130,130131,130130,260261,3.1775569915771484,0.005174401107557362
130330,130331,130330,260661,3.1819519996643066,0.005161275872493922
130531,130532,130531,261063,3.1864590644836426,0.0051481185543163395
130731,130732,130731,261463,3.190991163253784,0.00513505998681155
130931,130932,130931,261863,3.195528030395508,0.005122034543288542
131131,131132,131131,262263,3.200019121170044,0.005109042139725998
131331,131332,131331,262663,3.20540714263916,0.005096082692315734
131532,131533,131532,263065,3.210055112838745,0.005083091567040063
131732,131733,131732,263465,3.214607000350952,0.005070197945096265
131932,131933,131932,263865,3.219223976135254,0.005057337028738131
132132,132133,132132,264265,3.2241640090942383,0.005044508735005668
132332,132333,132332,264665,3.22868013381958,0.005031712981149237
132533,132534,132533,265067,3.2332651615142822,0.005018885949557319
132733,132734,132733,265467,3.238084077835083,0.0050061551897117975
132933,132934,132933,265867,3.24259614944458,0.004993456722340708
133133,133134,133133,266267,3.247114896774292,0.004980790465531935
133333,133334,133333,266667,3.2516610622406006,0.004968156337581089
133534,133535,133534,267069,3.2561869621276855,0.004955491326970448
133734,133735,133734,267469,3.260715961456299,0.004942921372077208
133934,133935,133934,267869,3.265350103378296,0.004930383301765281
134134,134135,134134,268269,3.2699639797210693,0.004917877035157156
134334,134335,134334,268669,3.274613857269287,0.004905402491580428
134535,134536,134535,269071,3.2791242599487305,0.004892897455429441
134735,134736,134735,269471,3.2837259769439697,0.004880486274326736
134935,134936,134935,269871,3.2880759239196777,0.0048681065750643526
135135,135136,135135,270271,3.2924599647521973,0.004855758277786337
135335,135336,135335,270671,3.2968008518218994,0.004843441302839373
135536,135537,135536,271073,3.3011679649353027,0.004831094220476361
135736,135737,135736,271473,3.3056528568267822,0.004818839807658439
135936,135937,135936,271873,3.3110859394073486,0.004806616479026973
136136,136137,136136,272273,3.3157169818878174,0.004794424155734727
136336,136337,136336,272673,3.320298194885254,0.004782262759134454
136537,136538,136537,273075,3.3253660202026367,0.004770071635411346
136737,136738,136737,273475,3.329951286315918,0.004757972010704472
136937,136938,136937,273875,3.3344669342041016,0.004745903077553035
137137,137138,137137,274275,3.3388898372650146,0.004733864758105729
137337,137338,137337,274675,3.343325138092041,0.004721856974708722
137538,137539,137538,275077,3.3477742671966553,0.0047098198396785425
137738,137739,137738,275477,3.3523099422454834,0.004697873047920935
137938,137939,137938,275877,3.3567872047424316,0.004685956560047129
138138,138139,138138,276277,3.3612220287323,0.004674070299189218
138338,138339,138338,276677,3.365654945373535,0.004662214188674224
138539,138540,138539,277079,3.3701019287109375,0.004650329097272837
138739,138740,138739,277479,3.3745131492614746,0.004638533207998814
138939,138940,138939,277879,3.378941059112549,0.0046267672398337765
139139,139140,139139,278279,3.3838372230529785,0.004615031116880701
139339,139340,139339,278679,3.388705015182495,0.004603324763435134
139540,139541,139540,279081,3.3936879634857178,0.004591589795166921
139740,139741,139740,279481,3.3983170986175537,0.004579942902294908
139940,139941,139940,279881,3.4027931690216064,0.00456832555259194
140140,140141,140140,280281,3.4073169231414795,0.0045567376711197
140340,140341,140340,280681,3.411733865737915,0.004545179183129904
140541,140542,140541,281083,3.416163921356201,0.004533592441757457
140741,140742,140741,281483,3.4205589294433594,0.004522092663282006
140941,140942,140941,281883,3.4249560832977295,0.004510622054809551
141141,141142,141141,282283,3.4293742179870605,0.004499180542348242
141341,141342,141341,282683,3.4338221549987793,0.0044877680520940605
141542,141543,141542,283085,3.438246011734009,0.004476327665331723
141742,141743,141742,283485,3.4426400661468506,0.004464973143019432
141942,141943,141942,283885,3.4470582008361816,0.004453647422257546
142142,142143,142142,284285,3.4514620304107666,0.004442350429988914
142342,142343,142342,284685,3.455867052078247,0.004431082093341641
142543,142544,142543,285087,3.4603209495544434,0.004419786212552994
142743,142744,142743,285487,3.467211961746216,0.004408575111642157
142943,142944,142943,285887,3.4716639518737793,0.0043973924484831915
143143,143144,143143,286287,3.476091146469116,0.004386238150941722
143343,143344,143343,286687,3.4805328845977783,0.004375112147066345
143544,143545,143544,287089,3.4849929809570312,0.00436395894696553
143744,143745,143744,287489,3.489423990249634,0.004352889455869734
143944,143945,143944,287889,3.4938652515411377,0.00434184804332246
144144,144145,144144,288289,3.4983022212982178,0.004330834638100505
144344,144345,144344,288689,3.502737045288086,0.004319849169161288
144545,144546,144545,289091,3.507201910018921,0.00430883684751801
144745,144746,144745,289491,3.511641025543213,0.004297907177533361
144945,144946,144945,289891,3.5161068439483643,0.0042870052314310835
145145,145146,145145,290291,3.520534038543701,0.004276130938887613
145345,145346,145345,290691,3.52496600151062,0.0042652842297577044
145546,145547,145546,291093,3.5294220447540283,0.004254411007105969
145746,145747,145746,291493,3.5338220596313477,0.004243619392122112
145946,145947,145946,291893,3.5382282733917236,0.004232855150834335
146146,146147,146146,292293,3.542628049850464,0.004222118213807327
146346,146347,146346,292693,3.5470340251922607,0.0042114085117819205
146547,146548,146547,293095,3.5515849590301514,0.004200672631132604
146747,146748,146747,293495,3.5560271739959717,0.004190017327347273
146947,146948,146947,293895,3.5606000423431396,0.004179389051495029
147147,147148,147147,294295,3.5650410652160645,0.004168787735017573
147347,147348,147347,294695,3.569599151611328,0.004158213309530556
147548,147549,147548,295097,3.574129104614258,0.004147613036087471
147748,147749,147748,295497,3.5786030292510986,0.004137092321724753
147948,147949,147948,295897,3.5840580463409424,0.004126598293899459
148148,148149,148148,296297,3.5884671211242676,0.00411613088491934
148348,148349,148348,296697,3.5928831100463867,0.004105690027263842
148549,148550,148549,297099,3.598079204559326,0.004095223648143318
148749,148750,148749,297499,3.6027870178222656,0.004084835823175376
148949,148950,148949,297899,3.6076819896698,0.00407447434766153
149149,149150,149149,298299,3.612837076187134,0.004064139154764519
149349,149350,149349,298699,3.6176600456237793,0.004053830177816649
149550,149551,149550,299101,3.622602939605713,0.004043496001770825
149750,149751,149750,299501,3.6272361278533936,0.004033239387643274
149950,149951,149950,299901,3.6314730644226074,0.004023008790144223
150150,150151,150150,300301,3.6357879638671875,0.004012804143280672
150350,150351,150350,300701,3.6404190063476562,0.004002625381226962
150551,150552,150551,301103,3.644974946975708,0.0039924217383705465
150751,150752,150751,301503,3.649306058883667,0.003982294677731186
150951,150952,150951,301903,3.653745174407959,0.003972193305098745
151151,151152,151151,302303,3.6589059829711914,0.003962117555313767
151351,151352,151351,302703,3.6635618209838867,0.003952067363382061
151552,151553,151552,303105,3.66792893409729,0.003941992604922365
151752,151753,151752,303505,3.673567056655884,0.003931993461353369
151952,151953,151952,303905,3.6779088973999023,0.003922019681320576
152152,152153,152152,304305,3.6822640895843506,0.003912071200487557
152352,152353,152352,304705,3.6870720386505127,0.003902147954681117
152553,152554,152553,305107,3.691509962081909,0.003892200452651772
152753,152754,152753,305507,3.6958959102630615,0.0038823276104052538
152953,152954,152953,305907,3.70062518119812,0.0038724798113226686
153153,153154,153153,306307,3.70510196685791,0.0038626569918802553
153353,153354,153353,306707,3.7096481323242188,0.0038528590887154024
153554,153555,153554,307109,3.7141001224517822,0.0038430372357131973
153754,153755,153754,307509,3.7185380458831787,0.003833289099450113
153954,153955,153954,307909,3.722999095916748,0.00382356569002539
154154,154155,154154,308309,3.7283661365509033,0.003813866944717681
154354,154355,154354,308709,3.733494997024536,0.00380419280096468
154555,154556,154555,309111,3.738358974456787,0.0037944950098898144
154755,154756,154755,309511,3.7433021068573,0.003784870004422191
154955,154956,154955,309911,3.747972011566162,0.0037752694134629444
155155,155156,155155,310311,3.7523770332336426,0.0037656931750829664
155355,155356,155355,310711,3.757538080215454,0.0037561412275102057
155556,155557,155556,311113,3.7619640827178955,0.0037465659313099878
155756,155757,155756,311513,3.766451120376587,0.003737062501346391
155956,155957,155956,311913,3.770836114883423,0.0037275831775063118
156156,156157,156156,312313,3.7752392292022705,0.003718127898642853
156356,156357,156356,312713,3.779635190963745,0.0037086966037642288
156557,156558,156557,313115,3.784111976623535,0.003699242255179645
156757,156758,156757,313515,3.788612127304077,0.003689858865073868
156957,156958,156957,313915,3.7932589054107666,0.003680499276602011
157157,157158,157157,314315,3.7978270053863525,0.0036711634293895377
157357,157358,157357,314715,3.8023672103881836,0.0036618512632150438
157558,157559,157558,315117,3.8068931102752686,0.003652516334530871
157758,157759,157758,315517,3.811429977416992,0.0036432514680337824
157958,157959,157958,315917,3.8159191608428955,0.003634010102527092
158158,158159,158158,316317,3.820413112640381,0.0036247921783988278
158358,158359,158358,316717,3.8249130249023438,0.003615597636188298
158559,158560,158559,317119,3.8294520378112793,0.003606380618986234
158759,158760,158759,317519,3.833972930908203,0.0035972327790007672
158959,158960,158959,317919,3.8384859561920166,0.003588108143159671
159159,159160,159159,318319,3.84299898147583,0.00357900665260393
159359,159360,159359,318719,3.8475019931793213,0.003569928248623905
159560,159561,159560,319121,3.8520731925964355,0.003560827653538796
159760,159761,159760,319521,3.8565869331359863,0.0035517953618780505
159960,159961,159960,319921,3.8610970973968506,0.0035427859812651318
160160,160161,160160,320321,3.8657991886138916,0.0035337994535845196
160360,160361,160360,320721,3.870487928390503,0.003524835720868156
160561,160562,160561,321123,3.8782289028167725,0.0035158500773472758
160761,160762,160761,321523,3.882905960083008,0.0035069318744956157
160961,160962,160961,321923,3.887327194213867,0.0034980362932974358
161161,161162,161161,322323,3.8917081356048584,0.003489163276371288
161361,161362,161361,322723,3.8962290287017822,0.003480312766481335
161562,161563,161562,323125,3.900676965713501,0.003471440622546906
161762,161763,161762,323525,3.9051029682159424,0.003462635067424167
161962,161963,161962,323925,3.9096932411193848,0.003453851848215928
162162,162163,162162,324325,3.914144992828369,0.0034450909082656177
162362,162363,162362,324725,3.9185619354248047,0.003436352191060261
162563,162564,162563,325127,3.923245906829834,0.0034275921130747142
162763,162764,162763,325527,3.9278392791748047,0.0034188977828033353
162963,162964,162963,325927,3.932257890701294,0.003410225506316767
163163,163164,163163,326327,3.9366650581359863,0.003401575227674002
163363,163364,163363,326727,3.94154691696167,0.0033929468910759704
163564,163565,163564,327129,3.945966958999634,0.0033842974635103244
163764,163765,163764,327529,3.9503750801086426,0.0033757129531853925
163964,163965,163964,327929,3.954911947250366,0.00336715021807918
164164,164165,164164,328329,3.9594979286193848,0.003358609202957306
164364,164365,164364,328729,3.9638729095458984,0.0033500898527254962
164565,164566,164565,329131,3.9682610034942627,0.003341549677930612
164765,164766,164765,329531,3.97263503074646,0.0033330736003928502
164965,164966,164965,329931,3.977023124694824,0.003324619023026386
165165,165166,165165,330331,3.981421947479248,0.003316185891294523
165365,165366,165365,330731,3.985774040222168,0.003307774150798822
165566,165567,165566,331133,3.9903149604797363,0.0032993418487795648
165766,165767,165766,331533,3.994797945022583,0.0032909728343912706
165966,165967,165966,331933,3.999268054962158,0.003282625048601005
166166,166167,166166,332333,4.006880044937134,0.003274298437560889
166366,166367,166366,332733,4.012535095214844,0.003265992947559694
166567,166568,166567,333135,4.018732070922852,0.0032576671557519505
166767,166768,166767,333535,4.023627042770386,0.0032494038521755724
166967,166968,166967,333935,4.029053211212158,0.003241161509054232
167167,167168,167167,334335,4.036983966827393,0.0032329400732202533
167367,167368,167367,334735,4.046328067779541,0.0032247394916408412
167568,167569,167568,335137,4.052470922470093,0.0032165188646913257
167768,167769,167768,335537,4.058600187301636,0.0032083599366709383
167968,167969,167968,335937,4.065925121307373,0.0032002217043496078
168168,168169,168168,336337,4.072242021560669,0.003192104115231256
168368,168369,168368,336737,4.0799360275268555,0.0031840071169528784
168569,168570,168569,337139,4.087360858917236,0.0031758903265017716
168769,168770,168769,337539,4.096652984619141,0.0031678344556474243
168969,168970,168969,337939,4.102794885635376,0.003159799019080331
169169,169170,169169,338339,4.1094300746917725,0.0031517839649674757
169369,169370,169369,338739,4.115489959716797,0.0031437892416073094
169570,169571,169570,339141,4.1220362186431885,0.0031357749760735796
169770,169771,169770,339541,4.127902269363403,0.0031278208606481373
169970,169971,169970,339941,4.133656024932861,0.0031198869214000883
170170,170171,170170,340341,4.14047908782959,0.0031119731071511014
170370,170371,170370,340741,4.146496057510376,0.0031040793668527487
170571,170572,170571,341143,4.152493953704834,0.0030961663312222025
170771,170772,170771,341543,4.158803224563599,0.003088312685931053
170971,170972,170971,341943,4.165171146392822,0.0030804789619677036
171171,171172,171171,342343,4.170989990234375,0.00307266510880026
171371,171372,171371,342743,4.17682409286499,0.0030648710760250797
171572,171573,171572,343145,4.182631015777588,0.0030570579916411513
171772,171773,171772,343545,4.188448905944824,0.0030493035474245464
171972,171973,171972,343945,4.194558143615723,0.0030415687729051654
172172,172173,172172,344345,4.200323104858398,0.003033853618189424
172372,172373,172372,344745,4.207042932510376,0.0030261580335103197
172573,172574,172573,345147,4.213131904602051,0.0030184436378674433
172773,172774,172773,345547,4.2190210819244385,0.003010787141695362
172973,172974,172973,345947,4.225080966949463,0.0030031500667683534
173173,173174,173173,346347,4.230849981307983,0.0029955323638230598
173373,173374,173373,346747,4.236495018005371,0.002987933983721062
173574,173575,173574,347149,4.242198944091797,0.0029803170302606158
173774,173775,173774,347549,4.247821092605591,0.0029727572449303706
173974,173975,173974,347949,4.253468036651611,0.0029652166355312757
174174,174175,174174,348349,4.260303020477295,0.0029576951534222595
174374,174375,174374,348749,4.266318082809448,0.002950192750085565
174575,174576,174575,349151,4.272324085235596,0.002942672007994456
174775,174776,174775,349551,4.278205156326294,0.002935207711930698
174975,174976,174975,349951,4.283829927444458,0.002927762349582789
175175,175176,175175,350351,4.289273023605347,0.002920335872924058
175375,175376,175375,350751,4.294083118438721,0.002912928234049598
175576,175577,175576,351153,4.298681974411011,0.0029055024880614566
175776,175777,175776,351553,4.303272247314453,0.0028981324751187693
175976,175977,175976,351953,4.307853937149048,0.0028907811567361673
176176,176177,176176,352353,4.3124330043792725,0.0028834484854935324
176376,176377,176376,352753,4.317001104354858,0.0028761344140911024
176577,176578,176577,353155,4.321575164794922,0.00286880246428984
176777,176778,176777,353555,4.326189994812012,0.002861525543557997
176977,176978,176977,353955,4.33063006401062,0.0028542670812512294
177177,177178,177177,354355,4.335105895996094,0.002847027030548416
177377,177378,177377,354755,4.33955717086792,0.00283980534474726
177578,177579,177578,355157,4.344050168991089,0.0028325660063731437
177778,177779,177778,355557,4.348605155944824,0.0028253810019845025
177978,177979,177978,355957,4.35305118560791,0.002818214222868624
178178,178179,178178,356357,4.357568979263306,0.0028110656227957843
178378,178379,178378,356757,4.362022161483765,0.0028039351556535695
178579,178580,178579,357159,4.3665220737457275,0.0027967872589118453
178779,178780,178779,357559,4.3710150718688965,0.0027896930098513886
178979,178980,178979,357959,4.375468015670776,0.0027826167558563718
179179,179180,179179,358359,4.380005121231079,0.0027755584512810113
179379,179380,179379,358759,4.384310960769653,0.0027685180505953692
179580,179581,179580,359161,4.388675928115845,0.0027614604404672034
179780,179781,179780,359561,4.3929221630096436,0.00275445580038499
179980,179981,179980,359961,4.397171258926392,0.0027474689280686704
180180,180181,180180,360361,4.40146017074585,0.002740499778449068
180380,180381,180380,360761,4.405695915222168,0.0027335483065712924
180581,180582,180581,361163,4.413992166519165,0.0027265798426271497
180781,180782,180781,361563,4.418247222900391,0.002719663679652952
180981,180982,180981,361963,4.422490119934082,0.002712765060016202
181181,181182,181181,362363,4.426723957061768,0.0027058839392170007
181381,181382,181381,362763,4.430969953536987,0.0026990202728682925
181582,181583,181582,363165,4.435219049453735,0.0026921398290836373
181782,181783,181782,363565,4.439456939697266,0.0026853110256441957
181982,181983,181982,363965,4.443682909011841,0.002678499543948546
182182,182183,182182,364365,4.447916030883789,0.002671705340058889
182382,182383,182382,364765,4.452163934707642,0.0026649283701488387
182583,182584,182583,365167,4.456423044204712,0.0026581348347221997
182783,182784,182783,365567,4.460663080215454,0.002651392287360521
182983,182984,182983,365967,4.4649200439453125,0.0026446668429479826
183183,183184,183183,366367,4.469156980514526,0.0026379584581017407
183383,183384,183383,366767,4.4734461307525635,0.0026312670895490367
183584,183585,183584,367169,4.47771692276001,0.0026245593647223242
183784,183785,183784,367569,4.48191499710083,0.002617901983919412
183984,183985,183984,367969,4.486170053482056,0.0026112614900346636
184184,184185,184184,368369,4.490373134613037,0.002604637840233177
184384,184385,184384,368769,4.4947121143341064,0.002598030991788761
184585,184586,184585,369171,4.499017238616943,0.002591407993669971
184785,184786,184785,369571,4.503262042999268,0.00258483470366882
184985,184986,184985,369971,4.507582187652588,0.002578278087283528
185185,185186,185185,370371,4.512171983718872,0.002571738102220309
185385,185386,185385,370771,4.516378164291382,0.0025652147062926274
185586,185587,185586,371173,4.520653963088989,0.002558675364680543
185786,185787,185786,371573,4.525377035140991,0.00255218510331225
185986,185987,185986,371973,4.530637979507446,0.0025457113049517865
186186,186187,186186,372373,4.536639213562012,0.002539253927839608
186386,186387,186386,372773,4.5422890186309814,0.00253281293032204
186587,186588,186587,373175,4.546748161315918,0.0025263561885334406
186787,186788,186787,373575,4.551181077957153,0.002519947907045528
186987,186988,186987,373975,4.555535078048706,0.0025135558806177096
187187,187188,187187,374375,4.560405015945435,0.0025071800680178742
187387,187388,187387,374775,4.564992904663086,0.002500820428118482
187588,187589,187588,375177,4.569801092147827,0.002494445242817289
187788,187789,187788,375577,4.574223041534424,0.002488117905704369
187988,187989,187988,375977,4.578836917877197,0.0024818066183304147
188188,188189,188188,376377,4.583453178405762,0.0024755113399840857
188388,188389,188388,376777,4.587907075881958,0.0024692320300573555
188589,188590,188589,377179,4.592449903488159,0.0024629373710861337
188789,188790,188789,377579,4.59685206413269,0.0024566899559225084
188989,188990,188989,377979,4.601490020751953,0.002450458387770133
189189,189190,189189,378379,4.606061935424805,0.002444242626431924
189389,189390,189389,378779,4.610547065734863,0.0024380426318127797
189590,189591,189590,379181,4.614964962005615,0.002431827482026249
189790,189791,189790,379581,4.619652032852173,0.0024256589793006465
189990,189991,189990,379981,4.624585151672363,0.0024195061234192987
190190,190191,190190,380381,4.629069089889526,0.002413368874692881
190390,190391,190390,380781,4.633462905883789,0.002407247193532746
190591,190592,190591,381183,4.638270139694214,0.0024011105486333464
190791,190792,190791,381583,4.642724990844727,0.00239501996158587
190991,190992,190991,381983,4.6473400592803955,0.002388944823744032
191191,191192,191191,382383,4.6520140171051025,0.0023828850959197686
191391,191392,191391,382783,4.656520128250122,0.0023768407390245276
191592,191593,191592,383185,4.66109824180603,0.0023707816074002414
191792,191793,191792,383585,4.665687084197998,0.0023647679518612966
191992,191993,191992,383985,4.670867204666138,0.002358769550385751
192192,192193,192192,384385,4.675429105758667,0.002352786364280576
192392,192393,192392,384785,4.679938077926636,0.00234681835495092
192593,192594,192593,385187,4.685871124267578,0.002340835757514978
192793,192794,192793,385587,4.691040992736816,0.0023348980617462116
192993,192994,192993,385987,4.696424245834351,0.0023289754273635058
193193,193194,193193,386387,4.702118158340454,0.002323067816162557
193393,193394,193393,386787,4.744407892227173,0.002317175190036016
193594,193595,193594,387189,4.759785175323486,0.002311268160068691
193794,193795,193794,387589,4.765887975692749,0.0023054054646059847
193994,193995,193994,387989,4.771918058395386,0.0022995576402857353
194194,194195,194194,388389,4.777663230895996,0.002293724649386227
194394,194395,194394,388789,4.783301115036011,0.002287906454281474
194595,194596,194595,389191,4.788863897323608,0.002282074037273913
194795,194796,194795,389591,4.794321060180664,0.002276285394772344
194995,194996,194995,389991,4.799955129623413,0.0022705114355726507
195195,195196,195195,390391,4.805140256881714,0.0022647521224296095
195395,195396,195395,390791,4.809629201889038,0.0022590074181924507
195596,195597,195596,391193,4.814056158065796,0.0022532486716923756
195796,195797,195796,391593,4.818421840667725,0.0022475331467731283
195996,195997,195996,391993,4.822854042053223,0.0022418321196878443
196196,196197,196196,392393,4.82722020149231,0.002236145553661752
196396,196397,196396,392793,4.831588983535767,0.002230473412013305
196597,196598,196597,393195,4.836055040359497,0.0022247874054727823
196797,196798,196797,393595,4.840457916259766,0.0022191440745720574
196997,196998,196997,393995,4.84543514251709,0.002213515058380037
197197,197198,197197,394395,4.8498921394348145,0.002207900320586445
197397,197398,197397,394795,4.854305982589722,0.0022022998249731293
197598,197599,197598,395197,4.859023094177246,0.0021966856395981573
197798,197799,197798,395597,4.864130020141602,0.0021911135908178176
197998,197999,197998,395997,4.8688600063323975,0.002185555675934069
198198,198199,198198,396397,4.874026298522949,0.0021800118590952437
198398,198399,198398,396797,4.878791093826294,0.0021744821045406922
198599,198600,198599,397199,4.883849143981934,0.0021689388331427354
198799,198800,198799,397599,4.8891191482543945,0.002163437166103118
198999,199000,198999,397999,4.894381046295166,0.002157949454431793
199199,199200,199199,398399,4.900327205657959,0.002152475662729984
199399,199400,199399,398799,4.906171083450317,0.0021470157556886765
199600,199601,199600,399201,4.912016153335571,0.002141542502538169
199800,199801,199800,399601,4.917961120605469,0.002136110328232437
200000,200001,200000,400001,4.924265146255493,0.0021306919330217103


==> plot_data/quadratic_minimax_problem_n20_alpha00001/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.508827209472656e-05,4.387072431292609
200,201,200,401,0.008509159088134766,0.18936632320225483
400,401,400,801,0.01695728302001953,0.09223193431015458
601,602,601,1203,0.02475714683532715,0.0656058045305487
801,802,801,1603,0.03294706344604492,0.058322281162373334
1001,1002,1001,2003,0.04091310501098633,0.0469572063819363
1201,1202,1201,2403,0.04848623275756836,0.04918596952880194
1401,1402,1401,2803,0.05623817443847656,0.03888773044947158
1602,1603,1602,3205,0.06370997428894043,0.03525175629247065
1802,1803,1802,3605,0.07074832916259766,0.034352401565386034
2002,2003,2002,4005,0.07820796966552734,0.031016241446923453
2202,2203,2202,4405,0.0861198902130127,0.035049799478285466
2402,2403,2402,4805,0.09404611587524414,0.028056873132843118
2603,2604,2603,5207,0.1020960807800293,0.030061297549765595
2803,2804,2803,5607,0.10983514785766602,0.025832454724797196
3003,3004,3003,6007,0.11786913871765137,0.024880387381991612
3203,3204,3203,6407,0.12548518180847168,0.024193856608383208
3403,3404,3403,6807,0.13296103477478027,0.024058938603714674
3604,3605,3604,7209,0.13966107368469238,0.022938487728528013
3804,3805,3804,7609,0.1464982032775879,0.022289682909653826
4004,4005,4004,8009,0.15436220169067383,0.02197021947981532
4204,4205,4204,8409,0.1637890338897705,0.02135702103118868
4404,4405,4404,8809,0.17178916931152344,0.02100253807346372
4605,4606,4605,9211,0.17949318885803223,0.02086916290451464
4805,4806,4805,9611,0.1868600845336914,0.020532725704852046
5005,5006,5005,10011,0.1934499740600586,0.021631294533434244
5205,5206,5205,10411,0.20018410682678223,0.023962975766511446
5405,5406,5405,10811,0.20939016342163086,0.02022322378491767
5606,5607,5606,11213,0.21814513206481934,0.019468949583072995
5806,5807,5806,11613,0.22635698318481445,0.019200864140216142
6006,6007,6006,12013,0.23558306694030762,0.01909213074102498
6206,6207,6206,12413,0.24349713325500488,0.018628386500526617
6406,6407,6406,12813,0.2520711421966553,0.018451161085895115
6607,6608,6607,13215,0.2598690986633301,0.0180974497030236
6807,6808,6807,13615,0.2691991329193115,0.018447839173058173
7007,7008,7007,14015,0.2773261070251465,0.017884349215526073
7207,7208,7207,14415,0.2900872230529785,0.017941500555366897
7407,7408,7407,14815,0.3037140369415283,0.01740299098682146
7608,7609,7608,15217,0.3131141662597656,0.018055002919716758
7808,7809,7808,15617,0.3235001564025879,0.016823907178130065
8008,8009,8008,16017,0.3314859867095947,0.016859474518199354
8208,8209,8208,16417,0.3393080234527588,0.016441605892395357
8408,8409,8408,16817,0.34732532501220703,0.019960701559353998
8609,8610,8609,17219,0.3550112247467041,0.016093323168860172
8809,8810,8809,17619,0.3629770278930664,0.015874946252434154
9009,9010,9009,18019,0.37096619606018066,0.015602412735053191
9209,9210,9209,18419,0.37881922721862793,0.015601365957870698
9409,9410,9409,18819,0.38684511184692383,0.0153145626693603
9610,9611,9610,19221,0.39486217498779297,0.015076835135817458
9810,9811,9810,19621,0.4026920795440674,0.015181358822380515
10010,10011,10010,20021,0.40994715690612793,0.01477895305301629
10210,10211,10210,20421,0.4165470600128174,0.014726288203231519
10410,10411,10410,20821,0.42304205894470215,0.016382810727969446
10611,10612,10611,21223,0.42925596237182617,0.014629764591720492
10811,10812,10811,21623,0.43610334396362305,0.01396198876920678
11011,11012,11011,22023,0.4423370361328125,0.013829626942600948
11211,11212,11211,22423,0.44876909255981445,0.013624943905131465
11411,11412,11411,22823,0.45528411865234375,0.015117473715436433
11612,11613,11612,23225,0.46155214309692383,0.013298472572415914
11812,11813,11812,23625,0.46808600425720215,0.01320426748339519
12012,12013,12012,24025,0.47472119331359863,0.012885826262499405
12212,12213,12212,24425,0.48104405403137207,0.012994895968908593
12412,12413,12412,24825,0.4871940612792969,0.012672476183744919
12613,12614,12613,25227,0.4934041500091553,0.012641742579447304
12813,12814,12813,25627,0.4996161460876465,0.01238883748889857
13013,13014,13013,26027,0.5058472156524658,0.012178265993356908
13213,13214,13213,26427,0.5120241641998291,0.015094596451200053
13413,13414,13413,26827,0.5181922912597656,0.012030395735244444
13614,13615,13614,27229,0.5246939659118652,0.012126957956764009
13814,13815,13814,27629,0.5308411121368408,0.012002607330754575
14014,14015,14014,28029,0.5370161533355713,0.011539917288380701
14214,14215,14214,28429,0.5432021617889404,0.011329175291189538
14414,14415,14414,28829,0.5494050979614258,0.011161804582309634
14615,14616,14615,29231,0.5556333065032959,0.011318460044441125
14815,14816,14815,29631,0.5618271827697754,0.011000663185771828
15015,15016,15015,30031,0.5681211948394775,0.010807434981269654
15215,15216,15215,30431,0.5748691558837891,0.010764290775629093
15415,15416,15415,30831,0.5812900066375732,0.010650466539483221
15616,15617,15616,31233,0.5877540111541748,0.010448891170656215
15816,15817,15816,31633,0.5943601131439209,0.010264291978760203
16016,16017,16016,32033,0.602161169052124,0.010240915647861112
16216,16217,16216,32433,0.6088321208953857,0.01215317495361385
16416,16417,16416,32833,0.6155731678009033,0.009895740843234989
16617,16618,16617,33235,0.623751163482666,0.0098090809487204
16817,16818,16817,33635,0.6318521499633789,0.009664723317671082
17017,17018,17017,34035,0.6395430564880371,0.00959986527487779
17217,17218,17217,34435,0.6476039886474609,0.009515207769177341
17417,17418,17417,34835,0.6549220085144043,0.009275128961142574
17618,17619,17618,35237,0.6613750457763672,0.009225325310501744
17818,17819,17818,35637,0.667626142501831,0.008986579994002444
18018,18019,18018,36037,0.6739780902862549,0.010708088533237209
18218,18219,18218,36437,0.6803340911865234,0.008814615837177181
18418,18419,18418,36837,0.6865322589874268,0.00879944874303613
18619,18620,18619,37239,0.6928021907806396,0.008652917092832045
18819,18820,18819,37639,0.6990201473236084,0.008712470530932971
19019,19020,19019,38039,0.7053210735321045,0.008504296575971203
19219,19220,19219,38439,0.7119801044464111,0.008387193883851176
19419,19420,19419,38839,0.7181661128997803,0.008220568209398886
19620,19621,19620,39241,0.7243351936340332,0.008117352777286951
19820,19821,19820,39641,0.7304301261901855,0.008009904006628817
20020,20021,20020,40041,0.7366280555725098,0.007940983569068881
20220,20221,20220,40441,0.7431061267852783,0.007889662933258358
20420,20421,20420,40841,0.749812126159668,0.0077723100979238315
20621,20622,20621,41243,0.7564730644226074,0.007810089276610669
20821,20822,20821,41643,0.7631649971008301,0.0075172092443144154
21021,21022,21021,42043,0.7697570323944092,0.008998716612139681
21221,21222,21221,42443,0.7765100002288818,0.007418951378251925
21421,21422,21421,42843,0.783095121383667,0.00725303773588433
21622,21623,21622,43245,0.7899901866912842,0.007269600127948643
21822,21823,21822,43645,0.7968840599060059,0.007021484866976556
22022,22023,22022,44045,0.8038170337677002,0.006979136237117952
22222,22223,22222,44445,0.8106000423431396,0.006904146298492021
22422,22423,22422,44845,0.8174121379852295,0.007300334625210108
22623,22624,22623,45247,0.8242402076721191,0.006683180186684013
22823,22824,22823,45647,0.8310489654541016,0.006626367437470176
23023,23024,23023,46047,0.8378281593322754,0.006620403077963792
23223,23224,23223,46447,0.8447561264038086,0.007553795138001914
23423,23424,23423,46847,0.8515172004699707,0.00639871498362701
23624,23625,23624,47249,0.8585600852966309,0.006663144832643188
23824,23825,23824,47649,0.865645170211792,0.006194223434858175
24024,24025,24024,48049,0.8725950717926025,0.006645302841427511
24224,24225,24224,48449,0.8795111179351807,0.006135576843184301
24424,24425,24424,48849,0.887714147567749,0.006333564171553187
24625,24626,24625,49251,0.895050048828125,0.005946056495598024
24825,24826,24825,49651,0.902778148651123,0.0058509123411267395
25025,25026,25025,50051,0.9104640483856201,0.0058691425915221905
25225,25226,25225,50451,0.9178721904754639,0.0057862559460983305
25425,25426,25425,50851,0.9243481159210205,0.005663728474846472
25626,25627,25626,51253,0.9305260181427002,0.005552027312139043
25826,25827,25826,51653,0.9367029666900635,0.005579929500003388
26026,26027,26026,52053,0.9429092407226562,0.005437261182126389
26226,26227,26226,52453,0.9491031169891357,0.005394347340894282
26426,26427,26426,52853,0.9553370475769043,0.0052778581011025715
26627,26628,26627,53255,0.9620349407196045,0.005415266220562603
26827,26828,26827,53655,0.9681360721588135,0.00518203603924742
27027,27028,27027,54055,0.9746532440185547,0.0050845789484168505
27227,27228,27227,54455,0.9808392524719238,0.005159841247919578
27427,27428,27427,54855,0.9871721267700195,0.005043737832281305
27628,27629,27628,55257,0.9934902191162109,0.004938746064361496
27828,27829,27828,55657,0.9997291564941406,0.004846336994202827
28028,28029,28028,56057,1.0058810710906982,0.005159935308467211
28228,28229,28228,56457,1.0120329856872559,0.004839691231055434
28428,28429,28428,56857,1.0181410312652588,0.004714567034551519
28629,28630,28629,57259,1.0242841243743896,0.004601631472806232
28829,28830,28829,57659,1.0305161476135254,0.004923546115768655
29029,29030,29029,58059,1.0365381240844727,0.004488375769277907
29229,29230,29229,58459,1.0425710678100586,0.004578261145488517
29429,29430,29429,58859,1.048525094985962,0.00437786755848694
29630,29631,29630,59261,1.0557191371917725,0.0043314455539875665
29830,29831,29830,59661,1.0618741512298584,0.004289557788411757
30030,30031,30030,60061,1.0679171085357666,0.005539839666283146
30230,30231,30230,60461,1.073979139328003,0.0042073426893633635
30430,30431,30430,60861,1.0800011157989502,0.004137473006305593
30631,30632,30631,61263,1.0860931873321533,0.0040915970695461195
30831,30832,30831,61663,1.0923819541931152,0.004002592387646612
31031,31032,31031,62063,1.0983989238739014,0.004197112413802173
31231,31232,31231,62463,1.1048400402069092,0.004114854305821307
31431,31432,31431,62863,1.1112651824951172,0.0038855601763930544
31632,31633,31632,63265,1.11753511428833,0.0038649826746741216
31832,31833,31832,63665,1.1236889362335205,0.0038122965186893577
32032,32033,32032,64065,1.1297039985656738,0.0037627668591842826
32232,32233,32232,64465,1.1357390880584717,0.003858035859669507
32432,32433,32432,64865,1.14182710647583,0.004351484784835877
32633,32634,32633,65267,1.1479182243347168,0.0044259842915955775
32833,32834,32833,65667,1.1540501117706299,0.003572830870195248
33033,33034,33033,66067,1.1601221561431885,0.0035281308133604263
33233,33234,33233,66467,1.1662251949310303,0.0034676550734832534
33433,33434,33433,66867,1.1722922325134277,0.003456781886342454
33634,33635,33634,67269,1.178382158279419,0.0033954657588784166
33834,33835,33834,67669,1.184507131576538,0.0033818201240780376
34034,34035,34034,68069,1.1905710697174072,0.0033702232840683017
34234,34235,34234,68469,1.1966681480407715,0.003318529209116326
34434,34435,34434,68869,1.202775001525879,0.0032244343043375183
34635,34636,34635,69271,1.2090041637420654,0.0038585534259573152
34835,34836,34835,69671,1.2155461311340332,0.003175856125217855
35035,35036,35035,70071,1.2218081951141357,0.0031209457823914155
35235,35236,35235,70471,1.2279181480407715,0.0030992611151014404
35435,35436,35435,70871,1.2340221405029297,0.003047244078095222
35636,35637,35636,71273,1.2401471138000488,0.0030464325878349296
35836,35837,35836,71673,1.246225118637085,0.002964719611763382
36036,36037,36036,72073,1.2523820400238037,0.0029147279175290287
36236,36237,36236,72473,1.2585132122039795,0.0034312153404067315
36436,36437,36436,72873,1.264733076095581,0.003308813677753265
36637,36638,36637,73275,1.2709541320800781,0.0027972694383065736
36837,36838,36837,73675,1.2771499156951904,0.0027573223896803986
37037,37038,37037,74075,1.283318042755127,0.002749260636676773
37237,37238,37237,74475,1.2895112037658691,0.002704614543534682
37437,37438,37437,74875,1.2958650588989258,0.002670902749121971
37638,37639,37638,75277,1.3024020195007324,0.0029432606285557028
37838,37839,37838,75677,1.3088350296020508,0.0025904928060624033
38038,38039,38038,76077,1.3152251243591309,0.0031118128257939196
38238,38239,38238,76477,1.3215880393981934,0.002564314367350419
38438,38439,38438,76877,1.3275032043457031,0.002527417164791063
38639,38640,38639,77279,1.3336162567138672,0.0025171501544321508
38839,38840,38839,77679,1.3397769927978516,0.0024600644260109753
39039,39040,39039,78079,1.3463900089263916,0.0025075659242937386
39239,39240,39239,78479,1.3524999618530273,0.0023913299958036784
39439,39440,39439,78879,1.358557939529419,0.002375559295211246
39640,39641,39640,79281,1.3646202087402344,0.0027013897581320088
39840,39841,39840,79681,1.3706512451171875,0.0023139889145285964
40040,40041,40040,80081,1.3766491413116455,0.00234852905752498
40240,40241,40240,80481,1.38279128074646,0.0022798769941750493
40440,40441,40440,80881,1.388733148574829,0.0022401000885318447
40641,40642,40641,81283,1.394714117050171,0.0022033881697113133
40841,40842,40841,81683,1.401036024093628,0.002213888062684831
41041,41042,41041,82083,1.4071311950683594,0.002137040693037244
41241,41242,41241,82483,1.4132881164550781,0.002147630562696853
41441,41442,41441,82883,1.4193570613861084,0.0020929778249970526
41642,41643,41642,83285,1.4254631996154785,0.0020908003253091727
41842,41843,41842,83685,1.4314391613006592,0.0020563636552439583
42042,42043,42042,84085,1.4372951984405518,0.0023306501074101516
42242,42243,42242,84485,1.443145990371704,0.00199142783074224
42442,42443,42442,84885,1.4491610527038574,0.0019507656611844762
42643,42644,42643,85287,1.4552409648895264,0.0019502284494540497
42843,42844,42843,85687,1.4617242813110352,0.002168060817332156
43043,43044,43043,86087,1.4679701328277588,0.0018967517759683119
43243,43244,43243,86487,1.4741010665893555,0.0019295853546895498
43443,43444,43443,86887,1.4802219867706299,0.0018534573876843319
43644,43645,43644,87289,1.4863512516021729,0.0018212919504890387
43844,43845,43844,87689,1.4924559593200684,0.002042161189273212
44044,44045,44044,88089,1.4993832111358643,0.001794196852668956
44244,44245,44244,88489,1.5081470012664795,0.0017833914042765305
44444,44445,44444,88889,1.5142841339111328,0.0017446666519049857
44645,44646,44645,89291,1.5202751159667969,0.001982087316456891
44845,44846,44845,89691,1.5261411666870117,0.001754287650500231
45045,45046,45045,90091,1.5321271419525146,0.0017783027210222571
45245,45246,45245,90491,1.5380780696868896,0.0016788605181189192
45445,45446,45445,90891,1.5440330505371094,0.0016425052969819233
45646,45647,45646,91293,1.5504071712493896,0.00160881532734715
45846,45847,45846,91693,1.556401252746582,0.0015878052664582108
46046,46047,46046,92093,1.5625312328338623,0.0015844995126847478
46246,46247,46246,92493,1.5684940814971924,0.0015491767718694564
46446,46447,46446,92893,1.5744593143463135,0.001536120923365317
46647,46648,46647,93295,1.5804851055145264,0.0017802034600299737
46847,46848,46847,93695,1.5864770412445068,0.0015108316641576614
47047,47048,47047,94095,1.5924551486968994,0.0014934169793777868
47247,47248,47247,94495,1.598464012145996,0.0014762320963331713
47447,47448,47447,94895,1.6044471263885498,0.0014627195144624881
47648,47649,47648,95297,1.6105320453643799,0.0014758449833815444
47848,47849,47848,95697,1.6165142059326172,0.0017235546750329518
48048,48049,48048,96097,1.6224629878997803,0.00169702435989609
48248,48249,48248,96497,1.628387212753296,0.0016389660027173554
48448,48449,48448,96897,1.6341912746429443,0.0013610546849134224
48649,48650,48649,97299,1.6400620937347412,0.0013329508895245327
48849,48850,48849,97699,1.6461372375488281,0.0013342613164774326
49049,49050,49049,98099,1.6520051956176758,0.001308252165271267
49249,49250,49249,98499,1.6578521728515625,0.001291017864819047
49449,49450,49449,98899,1.6640121936798096,0.0012669938266558207
49650,49651,49650,99301,1.669888973236084,0.001259489771561379
49850,49851,49850,99701,1.6757440567016602,0.001257180356093915
50050,50051,50050,100101,1.6817049980163574,0.0012761061152001517
50250,50251,50250,100501,1.6877210140228271,0.001210896332177958
50450,50451,50450,100901,1.6936731338500977,0.0011958834561842824
50651,50652,50651,101303,1.6996469497680664,0.0011802308236679739
50851,50852,50851,101703,1.7056331634521484,0.0011815262425043948
51051,51052,51051,102103,1.7116711139678955,0.0011511631009639778
51251,51252,51251,102503,1.7175979614257812,0.0011430920456135367
51451,51452,51451,102903,1.7235100269317627,0.0011399293616745616
51652,51653,51652,103305,1.729485034942627,0.0011092160775322967
51852,51853,51852,103705,1.7354261875152588,0.0011480099033130354
52052,52053,52052,104105,1.7414031028747559,0.0010822530136601308
52252,52253,52252,104505,1.7474660873413086,0.0010786503584009493
52452,52453,52452,104905,1.753263235092163,0.001059424522184412
52653,52654,52653,105307,1.7589612007141113,0.0011145389309266038
52853,52854,52853,105707,1.7648100852966309,0.0010418424666027366
53053,53054,53053,106107,1.7708642482757568,0.00105051897296275
53253,53254,53253,106507,1.777036190032959,0.0010196371351831586
53453,53454,53453,106907,1.783271312713623,0.000993383461113229
53654,53655,53654,107309,1.7895371913909912,0.001010762369160719
53854,53855,53854,107709,1.795884132385254,0.000978610576887985
54054,54055,54054,108109,1.8022992610931396,0.001007279354977609
54254,54255,54254,108509,1.8088161945343018,0.0009471167685648379
54454,54455,54454,108909,1.815364122390747,0.0009403220256554005
54655,54656,54655,109311,1.8218750953674316,0.0009333010607565112
54855,54856,54855,109711,1.8283300399780273,0.0009089427186434027
55055,55056,55055,110111,1.834902048110962,0.0009038832135878346
55255,55256,55255,110511,1.8414041996002197,0.0008933525857824101
55455,55456,55455,110911,1.8478331565856934,0.0008886519162789888
55656,55657,55656,111313,1.8546881675720215,0.001066405363168276
55856,55857,55856,111713,1.861295223236084,0.0008620896445564649
56056,56057,56056,112113,1.8678452968597412,0.0008557050380351302
56256,56257,56256,112513,1.8744299411773682,0.0008470371416339308
56456,56457,56456,112913,1.8810372352600098,0.0009403818013693754
56657,56658,56657,113315,1.8876652717590332,0.0008183932863532129
56857,56858,56857,113715,1.8942341804504395,0.0010537181469475701
57057,57058,57057,114115,1.9008400440216064,0.0008009848355961437
57257,57258,57257,114515,1.9073331356048584,0.000791428124913332
57457,57458,57457,114915,1.9139032363891602,0.0009724292912953357
57658,57659,57658,115317,1.9205219745635986,0.0008936225177321889
57858,57859,57858,115717,1.9270520210266113,0.0007594032827857095
58058,58059,58058,116117,1.9334940910339355,0.0007729268571477627
58258,58259,58258,116517,1.9401342868804932,0.000743943561101582
58458,58459,58458,116917,1.9467132091522217,0.000750120000451758
58659,58660,58659,117319,1.9532852172851562,0.0007186203428864305
58859,58860,58859,117719,1.9598701000213623,0.0007182899824800161
59059,59060,59059,118119,1.966454029083252,0.0007089889205573614
59259,59260,59259,118519,1.973114252090454,0.0006941616118195918
59459,59460,59459,118919,1.9790520668029785,0.0006842639126734692
59660,59661,59660,119321,1.9850959777832031,0.0006796811886498607
59860,59861,59860,119721,1.9911561012268066,0.000678502152963456
60060,60061,60060,120121,1.997063159942627,0.0006677944842935721
60260,60261,60260,120521,2.0031590461730957,0.0006541835069575465
60460,60461,60460,120921,2.0094830989837646,0.0007457916555517015
60661,60662,60661,121323,2.0161080360412598,0.0006397622019535159
60861,60862,60861,121723,2.02268123626709,0.0006386283395736357
61061,61062,61061,122123,2.0293021202087402,0.0006238764464738079
61261,61262,61261,122523,2.0359532833099365,0.0006141465441017105
61461,61462,61461,122923,2.042532205581665,0.0006065640587473677
61662,61663,61662,123325,2.0491771697998047,0.0005977095537268667
61862,61863,61862,123725,2.0560362339019775,0.000592998107815703
62062,62063,62062,124125,2.0628769397735596,0.0005833639524103019
62262,62263,62262,124525,2.06980299949646,0.0005749242847428038
62462,62463,62462,124925,2.0766501426696777,0.0005764137800943921
62663,62664,62663,125327,2.083549976348877,0.0005726210672522799
62863,62864,62863,125727,2.090280055999756,0.0005568585558126129
63063,63064,63063,126127,2.097039222717285,0.0005550588498016388
63263,63264,63263,126527,2.103759288787842,0.0005434210513721822
63463,63464,63463,126927,2.1106009483337402,0.0005358084999106396
63664,63665,63664,127329,2.117305040359497,0.0006141556844611439
63864,63865,63864,127729,2.1242172718048096,0.0005234754288909909
64064,64065,64064,128129,2.1311440467834473,0.0005195450188445753
64264,64265,64264,128529,2.1380350589752197,0.0005109078123326022
64464,64465,64464,128929,2.144947052001953,0.0005019191403487335
64665,64666,64665,129331,2.15171217918396,0.0004953302279644816
64865,64866,64865,129731,2.158449172973633,0.0004930574809476508
65065,65066,65065,130131,2.165166139602661,0.0004884452477499748
65265,65266,65265,130531,2.1718993186950684,0.0004912597518909316
65465,65466,65465,130931,2.1786081790924072,0.0005928154665372958
65666,65667,65666,131333,2.1853482723236084,0.0004676712476322441
65866,65867,65866,131733,2.1920571327209473,0.00046334895654448466
66066,66067,66066,132133,2.1987130641937256,0.000479662229086581
66266,66267,66266,132533,2.2054340839385986,0.00045484791674220085
66466,66467,66466,132933,2.212263345718384,0.0004458759191980196
66667,66668,66667,133335,2.2191271781921387,0.000569349976193558
66867,66868,66867,133735,2.2258381843566895,0.00043266922214699356
67067,67068,67067,134135,2.232586145401001,0.00042729314507960466
67267,67268,67267,134535,2.2393059730529785,0.0004264498160471299
67467,67468,67467,134935,2.245936155319214,0.00041423575392115244
67668,67669,67668,135337,2.2526261806488037,0.000417030281584983
67868,67869,67868,135737,2.259369134902954,0.0004757344653838603
68068,68069,68068,136137,2.2662532329559326,0.0004029429726365288
68268,68269,68268,136537,2.273076057434082,0.0004004415233222935
68468,68469,68468,136937,2.2797701358795166,0.0004659878621661099
68669,68670,68669,137339,2.286651134490967,0.00038961160374922254
68869,68870,68869,137739,2.2934420108795166,0.0004004739509990538
69069,69070,69069,138139,2.300537109375,0.0003769642752731677
69269,69270,69269,138539,2.307690143585205,0.00037295116118747494
69469,69470,69469,138939,2.314119338989258,0.00036845300639498516
69670,69671,69670,139341,2.320202112197876,0.0003648788631296523
69870,69871,69870,139741,2.3264191150665283,0.0003723101600442952
70070,70071,70070,140141,2.3324952125549316,0.00035891798740044954
70270,70271,70270,140541,2.3386611938476562,0.00036045059473189015
70470,70471,70470,140941,2.345715045928955,0.00034505583240410244
70671,70672,70671,141343,2.3519370555877686,0.00034901430743082627
70871,70872,70871,141743,2.358417272567749,0.00033664982330264194
71071,71072,71071,142143,2.3645150661468506,0.00034238256451853155
71271,71272,71271,142543,2.3709142208099365,0.0003321969058845939
71471,71472,71471,142943,2.377272129058838,0.0003258016854977912
71672,71673,71672,143345,2.3837382793426514,0.0003528283606996271
71872,71873,71872,143745,2.3902792930603027,0.000316786760886895
72072,72073,72072,144145,2.396698236465454,0.0003124144292271852
72272,72273,72272,144545,2.403118133544922,0.00030911521341396917
72472,72473,72472,144945,2.409658193588257,0.0003057506937818344
72673,72674,72673,145347,2.4162721633911133,0.0003023546905691867
72873,72874,72873,145747,2.423577070236206,0.0003021569283136254
73073,73074,73073,146147,2.43023419380188,0.00030122389268549127
73273,73274,73273,146547,2.4363040924072266,0.0003008908572041375
73473,73474,73473,146947,2.44252610206604,0.00028587018927202787
73674,73675,73674,147349,2.4487321376800537,0.00028090202024747896
73874,73875,73874,147749,2.455151081085205,0.00027967051293527703
74074,74075,74074,148149,2.461663007736206,0.0002799580284167689
74274,74275,74274,148549,2.467957019805908,0.0002733212009032821
74474,74475,74474,148949,2.474274158477783,0.00027076669754557775
74675,74676,74675,149351,2.4807381629943848,0.00027021720573033387
74875,74876,74875,149751,2.487229347229004,0.00026259410635216807
75075,75076,75075,150151,2.4933671951293945,0.00026096778856667574
75275,75276,75275,150551,2.4997990131378174,0.00025496050586454056
75475,75476,75475,150951,2.5070672035217285,0.0002562315654034277
75676,75677,75676,151353,2.514064311981201,0.00024854122035586107
75876,75877,75876,151753,2.5203452110290527,0.00024524485667148184
76076,76077,76076,152153,2.5266170501708984,0.00024391282762353266
76276,76277,76276,152553,2.5329442024230957,0.00024076529931652308
76476,76477,76476,152953,2.539116144180298,0.000243776846986331
76677,76678,76677,153355,2.545271158218384,0.00023555531283554298
76877,76878,76877,153755,2.551464080810547,0.00023285761290924953
77077,77078,77077,154155,2.5576672554016113,0.00023390060270605511
77277,77278,77277,154555,2.5638530254364014,0.00028638126038683427
77477,77478,77477,154955,2.5700459480285645,0.00022436889539241323
77678,77679,77678,155357,2.5762290954589844,0.00022077747087294105
77878,77879,77878,155757,2.5824172496795654,0.0002177276347992638
78078,78079,78078,156157,2.5886871814727783,0.00021413661189858567
78278,78279,78278,156557,2.594870090484619,0.0002145656570745633
78478,78479,78478,156957,2.601081132888794,0.00022014639047870525
78679,78680,78679,157359,2.6072680950164795,0.00024527792614346245
78879,78880,78879,157759,2.6134190559387207,0.00023545947797480523
79079,79080,79079,158159,2.6196091175079346,0.0002047673710091494
79279,79280,79279,158559,2.626967191696167,0.00020928586764659926
79479,79480,79479,158959,2.6332879066467285,0.0001979445048319038
79680,79681,79680,159361,2.639653205871582,0.00020456134958535277
79880,79881,79880,159761,2.645848035812378,0.0002523395527971514
80080,80081,80080,160161,2.6521480083465576,0.000227407815957995
80280,80281,80280,160561,2.6584670543670654,0.00019308668083876194
80480,80481,80480,160961,2.6647801399230957,0.00018689639874739367
80681,80682,80681,161363,2.6709771156311035,0.0001819785439901213
80881,80882,80881,161763,2.677140951156616,0.0001806094474548321
81081,81082,81081,162163,2.683345317840576,0.00017849233474237202
81281,81282,81281,162563,2.689311981201172,0.00017659066354242618
81481,81482,81481,162963,2.695272922515869,0.00017467240529319696
81682,81683,81682,163365,2.7012879848480225,0.0001722781260454133
81882,81883,81882,163765,2.7072713375091553,0.00017651048465356338
82082,82083,82082,164165,2.7132601737976074,0.00017515900581428995
82282,82283,82282,164565,2.7192471027374268,0.00016736783214985662
82482,82483,82482,164965,2.7252471446990967,0.0001644645338704823
82683,82684,82683,165367,2.7312099933624268,0.000162618894098003
82883,82884,82883,165767,2.73711895942688,0.00015997542577295438
83083,83084,83083,166167,2.7429702281951904,0.00015745223230779568
83283,83284,83283,166567,2.749068021774292,0.00015564568164004515
83483,83484,83483,166967,2.7551302909851074,0.00015308416032923394
83684,83685,83684,167369,2.761012077331543,0.0001704053405254614
83884,83885,83884,167769,2.7669100761413574,0.00017467562209046958
84084,84085,84084,168169,2.772775173187256,0.00014825236630237797
84284,84285,84284,168569,2.7786171436309814,0.00014596745582512278
84484,84485,84484,168969,2.7844769954681396,0.00014758683585723594
84685,84686,84685,169371,2.7903659343719482,0.00014236409731893838
84885,84886,84885,169771,2.7964160442352295,0.0001418100602602085
85085,85086,85085,170171,2.802692174911499,0.00014074620383331118
85285,85286,85285,170571,2.8090529441833496,0.00013646176077016282
85485,85486,85485,170971,2.8149361610412598,0.0001366447932558617
85686,85687,85686,171373,2.8208162784576416,0.00013308589987016018
85886,85887,85886,171773,2.8266592025756836,0.00014132619374342066
86086,86087,86086,172173,2.8326022624969482,0.00013034075890192893
86286,86287,86286,172573,2.8400371074676514,0.000128326317736356
86486,86487,86486,172973,2.8462681770324707,0.00012756627924542585
86687,86688,86687,173375,2.8525519371032715,0.00015580749647914802
86887,86888,86887,173775,2.8583340644836426,0.00013192667305912892
87087,87088,87087,174175,2.8643200397491455,0.00012332743389390952
87287,87288,87287,174575,2.8701560497283936,0.00012118098456173516
87487,87488,87487,174975,2.876237154006958,0.00012178805643084498
87688,87689,87688,175377,2.882580041885376,0.00011785917224262932
87888,87889,87888,175777,2.8890221118927,0.00011824858180604125
88088,88089,88088,176177,2.8955280780792236,0.00011418557572960618
88288,88289,88288,176577,2.9021639823913574,0.00012093081173768782
88488,88489,88488,176977,2.9088282585144043,0.00011683565804736673
88689,88690,88689,177379,2.9154093265533447,0.00011153684572822592
88889,88890,88889,177779,2.9214820861816406,0.0001112056541500708
89089,89090,89089,178179,2.9299731254577637,0.00010952328586933862
89289,89290,89289,178579,2.936018943786621,0.00010629033255295073
89489,89490,89489,178979,2.9420223236083984,0.00010485829610616229
89690,89691,89690,179381,2.948078155517578,0.00010557627423730322
89890,89891,89890,179781,2.9545421600341797,0.00010316959027482173
90090,90091,90090,180181,2.961099147796631,0.00012325489755441666
90290,90291,90290,180581,2.968156337738037,0.00010032341656503546
90490,90491,90490,180981,2.974247932434082,9.962978385673239e-05
90691,90692,90691,181383,2.9803152084350586,9.899245481955809e-05
90891,90892,90891,181783,2.986298084259033,0.00011069340406822679
91091,91092,91091,182183,2.9923341274261475,9.551250429228721e-05
91291,91292,91291,182583,2.9983620643615723,9.417254692589146e-05
91491,91492,91491,182983,3.004399061203003,9.344081708993713e-05
91692,91693,91692,183385,3.010498046875,9.116765843064488e-05
91892,91893,91892,183785,3.016498327255249,0.00010681115733310933
92092,92093,92092,184185,3.0224692821502686,8.960218543845837e-05
92292,92293,92292,184585,3.0284390449523926,9.025180454623383e-05
92492,92493,92492,184985,3.0343880653381348,8.782977217522352e-05
92693,92694,92693,185387,3.0403802394866943,8.703177011976952e-05
92893,92894,92893,185787,3.046342134475708,0.0001014868780834589
93093,93094,93093,186187,3.0523180961608887,8.420108282531066e-05
93293,93294,93293,186587,3.058298110961914,8.418813476863588e-05
93493,93494,93493,186987,3.064338207244873,8.987289328429977e-05
93694,93695,93694,187389,3.070350170135498,8.225192504751872e-05
93894,93895,93894,187789,3.0763211250305176,8.317907774141632e-05
94094,94095,94094,188189,3.082393169403076,8.473203710771134e-05
94294,94295,94294,188589,3.088454246520996,7.821065708183481e-05
94494,94495,94494,188989,3.0947062969207764,7.709262644769465e-05
94695,94696,94695,189391,3.1008431911468506,7.707042535309829e-05
94895,94896,94895,189791,3.1071832180023193,7.5419136050492e-05
95095,95096,95095,190191,3.113556146621704,7.437435890532373e-05
95295,95296,95295,190591,3.119739294052124,8.292500816823628e-05
95495,95496,95495,190991,3.125904083251953,8.680202168866334e-05
95696,95697,95696,191393,3.132089138031006,8.60488527819318e-05
95896,95897,95896,191793,3.1382851600646973,7.072734195692914e-05
96096,96097,96096,192193,3.144573926925659,7.00088322942223e-05
96296,96297,96296,192593,3.150930166244507,7.175660495109339e-05
96496,96497,96496,192993,3.1573071479797363,6.969973776882796e-05
96697,96698,96697,193395,3.1637439727783203,7.190156668902314e-05
96897,96898,96897,193795,3.169997215270996,6.647556443484934e-05
97097,97098,97097,194195,3.176302194595337,6.535205237323198e-05
97297,97298,97297,194595,3.18271803855896,6.470286714712475e-05
97497,97498,97497,194995,3.189056158065796,6.394866078499578e-05
97698,97699,97698,195397,3.1955173015594482,6.308510441960049e-05
97898,97899,97898,195797,3.201881170272827,6.225594146552387e-05
98098,98099,98098,196197,3.2081589698791504,6.258031710256728e-05
98298,98299,98298,196597,3.2143962383270264,6.078887219511706e-05
98498,98499,98498,196997,3.2206552028656006,7.219631892191601e-05
98699,98700,98699,197399,3.2269272804260254,5.957118753449854e-05
98899,98900,98899,197799,3.233215093612671,5.818650490089061e-05
99099,99100,99099,198199,3.239474296569824,5.772234705375203e-05
99299,99300,99299,198599,3.2458109855651855,5.733891816689826e-05
99499,99500,99499,198999,3.252230167388916,5.679310143579812e-05
99700,99701,99700,199401,3.2585532665252686,5.589199180689728e-05
99900,99901,99900,199801,3.2648260593414307,5.5096813347387144e-05
100100,100101,100100,200201,3.2710251808166504,5.5105111296008415e-05
100300,100301,100300,200601,3.2795610427856445,5.3775951217307354e-05
100501,100502,100501,201003,3.285814046859741,5.3186995594096465e-05
100701,100702,100701,201403,3.292013168334961,5.2409926041677455e-05
100901,100902,100901,201803,3.2982442378997803,5.211240499657924e-05
101101,101102,101101,202203,3.304561138153076,5.5268578510028415e-05
101301,101302,101301,202603,3.310698986053467,5.137427991622855e-05
101502,101503,101502,203005,3.3168561458587646,5.059432072294306e-05
101702,101703,101702,203405,3.3229622840881348,4.957861833512934e-05
101902,101903,101902,203805,3.3289690017700195,4.8562620513266604e-05
102102,102103,102102,204205,3.3352062702178955,4.854316083345967e-05
102302,102303,102302,204605,3.341177225112915,4.785703916139307e-05
102503,102504,102503,205007,3.347104072570801,4.712196574379781e-05
102703,102704,102703,205407,3.3539161682128906,4.665135155718452e-05
102903,102904,102903,205807,3.359771251678467,4.616656785981134e-05
103103,103104,103103,206207,3.365593194961548,4.52280374975071e-05
103303,103304,103303,206607,3.3714041709899902,4.6073519863402534e-05
103504,103505,103504,207009,3.377275228500366,4.403582340013325e-05
103704,103705,103704,207409,3.383070945739746,4.351158994028342e-05
103904,103905,103904,207809,3.388930082321167,4.309094134786419e-05
104104,104105,104104,208209,3.3949902057647705,4.252588963552499e-05
104304,104305,104304,208609,3.4010801315307617,4.177307915906495e-05
104505,104506,104505,209011,3.406954050064087,4.3668813919207046e-05
104705,104706,104705,209411,3.412877082824707,4.148917433418831e-05
104905,104906,104905,209811,3.418684244155884,4.5928592308759736e-05
105105,105106,105105,210211,3.424499034881592,4.000766264082689e-05
105305,105306,105305,210611,3.430953025817871,4.019060407253873e-05
105506,105507,105506,211013,3.4380931854248047,3.8911708274189055e-05
105706,105707,105706,211413,3.445233106613159,3.872882115816259e-05
105906,105907,105906,211813,3.4512581825256348,3.827069540152509e-05
106106,106107,106106,212213,3.457261085510254,3.770132624007468e-05
106306,106307,106306,212613,3.4631459712982178,3.7578655449777765e-05
106507,106508,106507,213015,3.469052314758301,3.705923062485912e-05
106707,106708,106707,213415,3.4749181270599365,3.636644284606308e-05
106907,106908,106907,213815,3.4808361530303955,3.562177507910643e-05
107107,107108,107107,214215,3.4867401123046875,4.3848943151532606e-05
107307,107308,107307,214615,3.4926531314849854,3.47827342380591e-05
107508,107509,107508,215017,3.498617172241211,3.462390382432192e-05
107708,107709,107708,215417,3.5047261714935303,4.28213473909761e-05
107908,107909,107908,215817,3.510730028152466,3.404959035982612e-05
108108,108109,108108,216217,3.5167901515960693,3.3364485604790165e-05
108308,108309,108308,216617,3.5226380825042725,3.3089848135927206e-05
108509,108510,108509,217019,3.5286121368408203,3.2702920526996506e-05
108709,108710,108709,217419,3.5345962047576904,3.202688358113077e-05
108909,108910,108909,217819,3.540553092956543,3.169108456303799e-05
109109,109110,109109,218219,3.5465259552001953,3.106727202455559e-05
109309,109310,109309,218619,3.552489995956421,3.123434240296276e-05
109510,109511,109510,219021,3.5585060119628906,3.0470769327162635e-05
109710,109711,109710,219421,3.5645172595977783,3.056328971259842e-05
109910,109911,109910,219821,3.5704760551452637,3.474455125580427e-05
110110,110111,110110,220221,3.5764710903167725,2.966146983090472e-05
110310,110311,110310,220621,3.5824172496795654,3.0058354929561093e-05
110511,110512,110511,221023,3.5884170532226562,2.9994930553934403e-05
110711,110712,110711,221423,3.5943901538848877,2.850866773231168e-05
110911,110912,110911,221823,3.6003382205963135,2.8966687695429275e-05
111111,111112,111111,222223,3.6064701080322266,2.7753873113852654e-05
111311,111312,111311,222623,3.612459182739258,2.913819180256128e-05
111512,111513,111512,223025,3.618425130844116,2.720032901244792e-05
111712,111713,111712,223425,3.624303102493286,3.527254635160127e-05
111912,111913,111912,223825,3.6301991939544678,2.6573188955485415e-05
112112,112113,112112,224225,3.636188268661499,2.7386693903152526e-05
112312,112313,112312,224625,3.642252206802368,2.692669458841448e-05
112513,112514,112513,225027,3.648280143737793,2.5468334141809556e-05
112713,112714,112713,225427,3.6575632095336914,2.954828118701907e-05
112913,112914,112913,225827,3.663623332977295,2.498792357288694e-05
113113,113114,113113,226227,3.6696691513061523,2.6825328477614437e-05
113313,113314,113313,226627,3.675751209259033,2.4124509843595786e-05
113514,113515,113514,227029,3.6819651126861572,2.424459651637916e-05
113714,113715,113714,227429,3.6880531311035156,2.3399533516611858e-05
113914,113915,113914,227829,3.6941301822662354,2.330232662361915e-05
114114,114115,114114,228229,3.700179100036621,2.295042193018484e-05
114314,114315,114314,228629,3.7063560485839844,2.6908321163074278e-05
114515,114516,114515,229031,3.7125110626220703,2.241655403630026e-05
114715,114716,114715,229431,3.718635082244873,2.2256491350054897e-05
114915,114916,114915,229831,3.724713087081909,2.5344345066696452e-05
115115,115116,115115,230231,3.7307870388031006,2.1508013675113872e-05
115315,115316,115315,230631,3.736887216567993,2.134952274543923e-05
115516,115517,115516,231033,3.743014097213745,2.228620382910377e-05
115716,115717,115716,231433,3.7491400241851807,2.0814184390845635e-05
115916,115917,115916,231833,3.7552552223205566,2.1309382158407383e-05
116116,116117,116116,232233,3.761404275894165,2.0345587945279152e-05
116316,116317,116316,232633,3.767512083053589,2.002633227705324e-05
116517,116518,116517,233035,3.773587942123413,1.9869182414451293e-05
116717,116718,116717,233435,3.779651165008545,1.9413176083698914e-05
116917,116918,116917,233835,3.7857253551483154,2.0462290925340315e-05
117117,117118,117117,234235,3.791776180267334,1.906969198783235e-05
117317,117318,117317,234635,3.7978382110595703,1.8810826179011795e-05
117518,117519,117518,235037,3.804004192352295,1.8695933900566174e-05
117718,117719,117718,235437,3.8101470470428467,1.836449327587319e-05
117918,117919,117918,235837,3.816202163696289,1.808678135474876e-05
118118,118119,118118,236237,3.8220560550689697,2.1611847643001454e-05
118318,118319,118318,236637,3.827883005142212,2.0897739410018463e-05
118519,118520,118519,237039,3.834151268005371,1.7355096755205724e-05
118719,118720,118719,237439,3.842480182647705,1.7384820138524058e-05
118919,118920,118919,237839,3.8509480953216553,2.1026006823525362e-05
119119,119120,119119,238239,3.859036922454834,1.695395693353354e-05
119319,119320,119319,238639,3.865316152572632,1.6731852206706848e-05
119520,119521,119520,239041,3.8714871406555176,1.637029712752614e-05
119720,119721,119720,239441,3.8772571086883545,1.612001197492694e-05
119920,119921,119920,239841,3.883239269256592,1.6010009661206135e-05
120120,120121,120120,240241,3.8890020847320557,1.58445956919048e-05
120320,120321,120320,240641,3.8947551250457764,1.5612302775042657e-05
120521,120522,120521,241043,3.900759220123291,1.5350187566845035e-05
120721,120722,120721,241443,3.9067063331604004,1.517465190706958e-05
120921,120922,120921,241843,3.912750244140625,1.5024878759271466e-05
121121,121122,121121,242243,3.9186482429504395,1.50480287599429e-05
121321,121322,121321,242643,3.9246132373809814,1.4625559609280584e-05
121522,121523,121522,243045,3.9308102130889893,1.657911933826497e-05
121722,121723,121722,243445,3.936967134475708,1.4433596244964465e-05
121922,121923,121922,243845,3.943143129348755,1.4294441349217588e-05
122122,122123,122122,244245,3.9492852687835693,1.6840266045418116e-05
122322,122323,122322,244645,3.955489158630371,1.386687804613045e-05
122523,122524,122523,245047,3.9617180824279785,1.3594014848095107e-05
122723,122724,122723,245447,3.967834234237671,1.3551728317497118e-05
122923,122924,122923,245847,3.973982095718384,1.3675545394091057e-05
123123,123124,123123,246247,3.980159044265747,1.306384251923826e-05
123323,123324,123323,246647,3.9863080978393555,1.28468745301326e-05
123524,123525,123524,247049,3.9924941062927246,1.290271324902128e-05
123724,123725,123724,247449,3.9986531734466553,1.5562843084246013e-05
123924,123925,123924,247849,4.004827260971069,1.2515793326897772e-05
124124,124125,124124,248249,4.011003255844116,1.2390719373172888e-05
124324,124325,124324,248649,4.0171332359313965,1.247873695493349e-05
124525,124526,124525,249051,4.023289203643799,1.2101885616451989e-05
124725,124726,124725,249451,4.029350280761719,1.3521148209225386e-05
124925,124926,124925,249851,4.035176038742065,1.175331646411607e-05
125125,125126,125125,250251,4.041056156158447,1.1600698601489588e-05
125325,125326,125325,250651,4.047062158584595,1.162323479270221e-05
125526,125527,125526,251053,4.053927898406982,1.119264260569039e-05
125726,125727,125726,251453,4.060307025909424,1.1155715348143569e-05
125926,125927,125926,251853,4.066490173339844,1.1049222949602968e-05
126126,126127,126126,252253,4.072695016860962,1.0944826211755985e-05
126326,126327,126326,252653,4.078886270523071,1.0846348237545397e-05
126527,126528,126527,253055,4.085102081298828,1.054502120633906e-05
126727,126728,126727,253455,4.09502100944519,1.0519849149975148e-05
126927,126928,126927,253855,4.101766109466553,1.1942046871093114e-05
127127,127128,127127,254255,4.107816934585571,1.0335252055105219e-05
127327,127328,127327,254655,4.11392617225647,1.0050350536960756e-05
127528,127529,127528,255057,4.120104074478149,9.923345020746319e-06
127728,127729,127728,255457,4.126197099685669,9.875618081208476e-06
127928,127929,127928,255857,4.132596969604492,9.723419365464508e-06
128128,128129,128128,256257,4.138758182525635,1.096515647646657e-05
128328,128329,128328,256657,4.144896030426025,9.517059715686455e-06
128529,128530,128529,257059,4.1511852741241455,9.31962801075557e-06
128729,128730,128729,257459,4.157404899597168,9.18532761173725e-06
128929,128930,128929,257859,4.1637701988220215,1.146658714643614e-05
129129,129130,129129,258259,4.169922113418579,1.0506673231530585e-05
129329,129330,129329,258659,4.1760241985321045,8.922244494345241e-06
129530,129531,129530,259061,4.182181119918823,8.823926217887748e-06
129730,129731,129730,259461,4.188377141952515,1.0319157005358073e-05
129930,129931,129930,259861,4.194831132888794,8.56661989756683e-06
130130,130131,130130,260261,4.201367139816284,8.488683643402174e-06
130330,130331,130330,260661,4.207776069641113,8.473283295257463e-06
130531,130532,130531,261063,4.214083194732666,8.4617440279455e-06
130731,130732,130731,261463,4.220350027084351,8.360511168548996e-06
130931,130932,130931,261863,4.226482152938843,8.05901117691232e-06
131131,131132,131131,262263,4.232638120651245,7.970971311938229e-06
131331,131332,131331,262663,4.238765239715576,7.891508442731263e-06
131532,131533,131532,263065,4.2449259757995605,7.752015173657623e-06
131732,131733,131732,263465,4.2510740756988525,7.704197414257477e-06
131932,131933,131932,263865,4.257220268249512,7.595000315845007e-06
132132,132133,132132,264265,4.26340913772583,7.490861373962019e-06
132332,132333,132332,264665,4.269548177719116,7.328466186137465e-06
132533,132534,132533,265067,4.275717258453369,7.2899212733774555e-06
132733,132734,132733,265467,4.281890153884888,7.5392497369003365e-06
132933,132934,132933,265867,4.287790060043335,7.4199772692693155e-06
133133,133134,133133,266267,4.293699026107788,7.0261546810501935e-06
133333,133334,133333,266667,4.299812078475952,7.955772806194022e-06
133534,133535,133534,267069,4.3059000968933105,6.8509057737080336e-06
133734,133735,133734,267469,4.311847925186157,6.70854441425976e-06
133934,133935,133934,267869,4.31775426864624,8.365562626696814e-06
134134,134135,134134,268269,4.323650121688843,6.584567144068124e-06
134334,134335,134334,268669,4.329766273498535,6.51884302764629e-06
134535,134536,134535,269071,4.33590030670166,6.4202658255237656e-06
134735,134736,134735,269471,4.342056035995483,6.393396225727438e-06
134935,134936,134935,269871,4.348212957382202,6.271155163365352e-06
135135,135136,135135,270271,4.354537010192871,6.254147814229632e-06
135335,135336,135335,270671,4.360960006713867,6.149579909043258e-06
135536,135537,135536,271073,4.3673601150512695,6.138303393905823e-06
135736,135737,135736,271473,4.373855113983154,6.510428564059207e-06
135936,135937,135936,271873,4.380258083343506,5.884439132029822e-06
136136,136137,136136,272273,4.386660099029541,5.8065031798018565e-06
136336,136337,136336,272673,4.393125295639038,5.739152688081443e-06
136537,136538,136537,273075,4.3995561599731445,5.7346005237905015e-06
136737,136738,136737,273475,4.406141996383667,5.593924919731909e-06
136937,136938,136937,273875,4.412703990936279,6.412481238379042e-06
137137,137138,137137,274275,4.41923713684082,5.423667916281992e-06
137337,137338,137337,274675,4.425746917724609,5.473349183677953e-06
137538,137539,137538,275077,4.432325124740601,5.377551891470863e-06
137738,137739,137738,275477,4.438687086105347,5.2434909023115236e-06
137938,137939,137938,275877,4.445166110992432,6.74214092398881e-06
138138,138139,138138,276277,4.451617002487183,5.173359864058756e-06
138338,138339,138338,276677,4.458080053329468,5.055742365243315e-06
138539,138540,138539,277079,4.464656114578247,4.984002108085313e-06
138739,138740,138739,277479,4.471056222915649,5.019733332321473e-06
138939,138940,138939,277879,4.477553129196167,4.971767170451161e-06
139139,139140,139139,278279,4.483901262283325,4.823178154221928e-06
139339,139340,139339,278679,4.49049711227417,4.7895981547007086e-06
139540,139541,139540,279081,4.4968791007995605,4.715265273764784e-06
139740,139741,139740,279481,4.503442287445068,4.655313321042163e-06
139940,139941,139940,279881,4.509963035583496,4.699516933698947e-06
140140,140141,140140,280281,4.516343116760254,4.58924398000537e-06
140340,140341,140340,280681,4.522862195968628,5.068706332521063e-06
140541,140542,140541,281083,4.529538154602051,5.061311297309117e-06
140741,140742,140741,281483,4.535328149795532,4.388482026364389e-06
140941,140942,140941,281883,4.541093111038208,4.3345970408009775e-06
141141,141142,141141,282283,4.547465085983276,4.440333282547334e-06
141341,141342,141341,282683,4.5533833503723145,4.218827422591186e-06
141542,141543,141542,283085,4.5593390464782715,4.190200862463272e-06
141742,141743,141742,283485,4.565205097198486,4.120620571880089e-06
141942,141943,141942,283885,4.572019100189209,4.073015771920886e-06
142142,142143,142142,284285,4.577911138534546,4.013342770070335e-06
142342,142343,142342,284685,4.583944082260132,4.770913384440841e-06
142543,142544,142543,285087,4.59003210067749,3.9008236184263565e-06
142743,142744,142743,285487,4.598098278045654,3.885084015219158e-06
142943,142944,142943,285887,4.604199171066284,3.8445810031004355e-06
143143,143144,143143,286287,4.610411167144775,3.809993652276734e-06
143343,143344,143343,286687,4.616595983505249,3.7391334834528754e-06
143544,143545,143544,287089,4.62282395362854,3.7000508842302033e-06
143744,143745,143744,287489,4.629065036773682,3.632123497121603e-06
143944,143945,143944,287889,4.635249137878418,3.6120553325909824e-06
144144,144145,144144,288289,4.641423225402832,3.551932092419718e-06
144344,144345,144344,288689,4.647565126419067,3.5110613142969814e-06
144545,144546,144545,289091,4.653842210769653,3.848222867860496e-06
144745,144746,144745,289491,4.66016411781311,3.4053739439048227e-06
144945,144946,144945,289891,4.6663031578063965,3.3793475793066097e-06
145145,145146,145145,290291,4.672421216964722,3.352446436964405e-06
145345,145346,145345,290691,4.678701162338257,3.3402537287269003e-06
145546,145547,145546,291093,4.684972047805786,3.2284317991731692e-06
145746,145747,145746,291493,4.691030025482178,3.17424211479885e-06
145946,145947,145946,291893,4.697184085845947,3.197142763114319e-06
146146,146147,146146,292293,4.70408821105957,3.19394941156465e-06
146346,146347,146346,292693,4.710229158401489,3.097795956795957e-06
146547,146548,146547,293095,4.716462135314941,3.039755019363212e-06
146747,146748,146747,293495,4.7242591381073,3.3030844010869067e-06
146947,146948,146947,293895,4.730990171432495,2.961163347373841e-06
147147,147148,147147,294295,4.737912178039551,2.967744033289512e-06
147347,147348,147347,294695,4.745345115661621,2.8899467973009833e-06
147548,147549,147548,295097,4.753355979919434,2.859079692284836e-06
147748,147749,147748,295497,4.760982036590576,2.8976315906809044e-06
147948,147949,147948,295897,4.7681663036346436,3.3605816146949385e-06
148148,148149,148148,296297,4.774352312088013,3.237954533346689e-06
148348,148349,148348,296697,4.780794143676758,3.2482034431127943e-06
148549,148550,148549,297099,4.786880016326904,2.830747079371265e-06
148749,148750,148749,297499,4.792908191680908,2.673700611277856e-06
148949,148950,148949,297899,4.799045085906982,2.615626146911646e-06
149149,149150,149149,298299,4.805889129638672,2.9829516842277067e-06
149349,149350,149349,298699,4.8126232624053955,2.53642219448654e-06
149550,149551,149550,299101,4.818977117538452,2.998802579479081e-06
149750,149751,149750,299501,4.825067043304443,2.494878586832314e-06
149950,149951,149950,299901,4.831374168395996,2.9105847011236554e-06
150150,150151,150150,300301,4.8377039432525635,2.4277686099235643e-06
150350,150351,150350,300701,4.843707084655762,2.8060586132497682e-06
150551,150552,150551,301103,4.849789142608643,2.363427567667155e-06
150751,150752,150751,301503,4.856857061386108,2.6923195540671134e-06
150951,150952,150951,301903,4.863542079925537,2.3283176914638506e-06
151151,151152,151151,302303,4.870505094528198,2.283739549533846e-06
151351,151352,151351,302703,4.877261161804199,2.2484880411304065e-06
151552,151553,151552,303105,4.885561227798462,2.234059714006241e-06
151752,151753,151752,303505,4.893440008163452,2.2022414402834065e-06
151952,151953,151952,303905,4.9014573097229,2.1741615529572465e-06
152152,152153,152152,304305,4.909405946731567,2.1464236162344803e-06
152352,152353,152352,304705,4.9175660610198975,2.1031574710253403e-06
152553,152554,152553,305107,4.925073146820068,2.551874751533831e-06
152753,152754,152753,305507,4.933286190032959,2.0574818868659264e-06
152953,152954,152953,305907,4.9410319328308105,2.346427881541085e-06
153153,153154,153153,306307,4.949027061462402,2.137233236214591e-06
153353,153354,153353,306707,4.956990003585815,1.994963731213789e-06
153554,153555,153554,307109,4.964978933334351,1.968880771602553e-06
153754,153755,153754,307509,4.973129034042358,1.9324281456758936e-06
153954,153955,153954,307909,4.981215000152588,2.3671340526462756e-06
154154,154155,154154,308309,4.990375280380249,2.2610350557841944e-06
154354,154355,154354,308709,4.998662233352661,1.8784118855223107e-06
154555,154556,154555,309111,5.006860017776489,1.8496738024470624e-06
154755,154756,154755,309511,5.014652252197266,1.8151121406234122e-06
154955,154956,154955,309911,5.023101329803467,1.968086791684213e-06
155155,155156,155155,310311,5.030726194381714,1.7737582537384079e-06
155355,155356,155355,310711,5.038386344909668,1.9835721929413127e-06
155556,155557,155556,311113,5.046025991439819,1.7369805801229169e-06
155756,155757,155756,311513,5.053798198699951,1.7885391550510047e-06
155956,155957,155956,311913,5.061748027801514,1.68347554804395e-06
156156,156157,156156,312313,5.0694310665130615,1.6674199242076368e-06
156356,156357,156356,312713,5.076279163360596,1.6466532173931244e-06
156557,156558,156557,313115,5.082428216934204,1.61536966216874e-06
156757,156758,156757,313515,5.088503122329712,1.6021300591682864e-06
156957,156958,156957,313915,5.0945680141448975,1.6893344748700593e-06
157157,157158,157157,314315,5.100626230239868,1.6191117435629707e-06
157357,157358,157357,314715,5.106697082519531,1.562033313571096e-06
157558,157559,157558,315117,5.112784147262573,1.5328476799195055e-06
157758,157759,157758,315517,5.118851184844971,1.5130510981739198e-06
157958,157959,157958,315917,5.124872922897339,1.7290611386089624e-06
158158,158159,158158,316317,5.1309661865234375,1.46501212005396e-06
158358,158359,158358,316717,5.137024164199829,1.4563921570041354e-06
158559,158560,158559,317119,5.143101930618286,1.4542300765195218e-06
158759,158760,158759,317519,5.150060176849365,1.4213859507896502e-06
158959,158960,158959,317919,5.157613039016724,1.4095916280691822e-06
159159,159160,159159,318319,5.16532826423645,1.3954067021797025e-06
159359,159360,159359,318719,5.173116207122803,1.6772137098729567e-06
159560,159561,159560,319121,5.181244134902954,1.3542034694982418e-06
159760,159761,159760,319521,5.1894001960754395,1.4573683692941357e-06
159960,159961,159960,319921,5.1975202560424805,1.331437208276086e-06
160160,160161,160160,320321,5.20563817024231,1.6428597100288522e-06
160360,160361,160360,320721,5.213794231414795,1.2984642158865822e-06
160561,160562,160561,321123,5.225613117218018,1.2669788269047665e-06
160761,160762,160761,321523,5.233213186264038,1.3132955286524731e-06
160961,160962,160961,321923,5.240850210189819,1.2465015709764924e-06
161161,161162,161161,322323,5.2484331130981445,1.3406194964583646e-06
161361,161362,161361,322723,5.256340980529785,1.2053634081761273e-06
161562,161563,161562,323125,5.264438152313232,1.3571751035262797e-06
161762,161763,161762,323525,5.27230429649353,1.248878487083569e-06
161962,161963,161962,323925,5.279918193817139,1.197208976758363e-06
162162,162163,162162,324325,5.287299156188965,1.1458463393167003e-06
162362,162363,162362,324725,5.293652057647705,1.344090913449894e-06
162563,162564,162563,325127,5.299865245819092,1.119110618503614e-06
162763,162764,162763,325527,5.305885076522827,1.1200603813220862e-06
162963,162964,162963,325927,5.311923980712891,1.1262495678177784e-06
163163,163164,163163,326327,5.317935228347778,1.2548785122388447e-06
163363,163364,163363,326727,5.324733257293701,1.292027461340207e-06
163564,163565,163564,327129,5.331108093261719,1.3931481982201172e-06
163764,163765,163764,327529,5.337768077850342,1.0382828333757645e-06
163964,163965,163964,327929,5.3447980880737305,1.0457599169050823e-06
164164,164165,164164,328329,5.351647138595581,1.0243123953904081e-06
164364,164365,164364,328729,5.357709169387817,1.0620999518342926e-06
164565,164566,164565,329131,5.36378026008606,1.0171395196515647e-06
164765,164766,164765,329531,5.369803190231323,9.78434379225609e-07
164965,164966,164965,329931,5.375805139541626,9.759547907064413e-07
165165,165166,165165,330331,5.381813049316406,9.490796058146061e-07
165365,165366,165365,330731,5.387921333312988,9.45279582051734e-07
165566,165567,165566,331133,5.39406418800354,9.345157961627962e-07
165766,165767,165766,331533,5.400205135345459,9.168052212886356e-07
165966,165967,165966,331933,5.4062793254852295,9.278282129484127e-07
166166,166167,166166,332333,5.4124181270599365,1.0460973403195052e-06
166366,166367,166366,332733,5.418597221374512,8.778413981244975e-07
166567,166568,166567,333135,5.424782037734985,8.778898825139203e-07
166767,166768,166767,333535,5.430952072143555,8.808894429789593e-07
166967,166968,166967,333935,5.437195062637329,8.495609618667069e-07
167167,167168,167167,334335,5.443427085876465,1.0094049328793677e-06
167367,167368,167367,334735,5.4497292041778564,8.316559811955034e-07
167568,167569,167568,335137,5.456059217453003,8.218904686485549e-07
167768,167769,167768,335537,5.46242094039917,8.120137382530798e-07
167968,167969,167968,335937,5.46867299079895,7.970908162706626e-07
168168,168169,168168,336337,5.47487211227417,7.953190319185381e-07
168368,168369,168368,336737,5.481028079986572,9.39905743269962e-07
168569,168570,168569,337139,5.487243175506592,7.718475317865905e-07
168769,168770,168769,337539,5.493648290634155,8.91157684551756e-07
168969,168970,168969,337939,5.500146150588989,7.541180676129317e-07
169169,169170,169169,338339,5.506546974182129,7.500848356316353e-07
169369,169370,169369,338739,5.5129311084747314,7.339631641192981e-07
169570,169571,169570,339141,5.519313335418701,7.308450518671074e-07
169770,169771,169770,339541,5.525588035583496,7.178497791147157e-07
169970,169971,169970,339941,5.532067060470581,7.486589759345663e-07
170170,170171,170170,340341,5.53825831413269,6.960131782114839e-07
170370,170371,170370,340741,5.544412136077881,6.86722926116795e-07
170571,170572,170571,341143,5.550616025924683,6.811976381023194e-07
170771,170772,170771,341543,5.556886196136475,6.805455807747027e-07
170971,170972,170971,341943,5.5633580684661865,6.678455032439412e-07
171171,171172,171171,342343,5.569498062133789,6.530564376657056e-07
171371,171372,171371,342743,5.575593948364258,6.485015371476206e-07
171572,171573,171572,343145,5.581716060638428,6.426672148283572e-07
171772,171773,171772,343545,5.587815999984741,6.347377928410968e-07
171972,171973,171972,343945,5.593919038772583,6.27111119403621e-07
172172,172173,172172,344345,5.6000142097473145,6.204442704316087e-07
172372,172373,172372,344745,5.6060991287231445,6.13033643265527e-07
172573,172574,172573,345147,5.612231969833374,5.980237746988858e-07
172773,172774,172773,345547,5.618337154388428,5.930146587211975e-07
172973,172974,172973,345947,5.62444806098938,5.873739226775485e-07
173173,173174,173173,346347,5.630995035171509,5.826534659390437e-07
173373,173374,173373,346747,5.637484073638916,5.794831750739887e-07
173574,173575,173574,347149,5.644047260284424,6.547062833364874e-07
173774,173775,173774,347549,5.650547027587891,6.881114201570369e-07
173974,173975,173974,347949,5.657111167907715,5.521908981494015e-07
174174,174175,174174,348349,5.663625955581665,5.477814374748971e-07
174374,174375,174374,348749,5.6701672077178955,5.344290551061449e-07
174575,174576,174575,349151,5.676798105239868,5.342960747959366e-07
174775,174776,174775,349551,5.68330717086792,5.298027510612111e-07
174975,174976,174975,349951,5.689774036407471,5.184292629104269e-07
175175,175176,175175,350351,5.696272134780884,6.095993248871051e-07
175375,175376,175375,350751,5.702808141708374,5.166601427492001e-07
175576,175577,175576,351153,5.709398031234741,4.98134045355357e-07
175776,175777,175776,351553,5.715980052947998,5.116180425154327e-07
175976,175977,175976,351953,5.722454071044922,4.886084990056159e-07
176176,176177,176176,352353,5.728446960449219,4.808971776330483e-07
176376,176377,176376,352753,5.734360218048096,4.859343476601997e-07
176577,176578,176577,353155,5.740240097045898,6.414223658683409e-07
176777,176778,176777,353555,5.7461230754852295,5.40137746254862e-07
176977,176978,176977,353955,5.7519659996032715,4.955800923109687e-07
177177,177178,177177,354355,5.757861137390137,5.385386015199274e-07
177377,177378,177377,354755,5.7637622356414795,4.4587948199326497e-07
177578,177579,177578,355157,5.769626140594482,4.434486968134825e-07
177778,177779,177778,355557,5.775459051132202,4.3482492581524586e-07
177978,177979,177978,355957,5.781702280044556,4.319369821179904e-07
178178,178179,178178,356357,5.787539005279541,4.242385340512532e-07
178378,178379,178378,356757,5.793363094329834,4.278421962978861e-07
178579,178580,178579,357159,5.799211025238037,4.162362849203681e-07
178779,178780,178779,357559,5.805069208145142,4.1271525490493114e-07
178979,178980,178979,357959,5.81104302406311,4.0296546973945234e-07
179179,179180,179179,358359,5.8168933391571045,3.9628408734877e-07
179379,179380,179379,358759,5.822747230529785,4.2208390915807247e-07
179580,179581,179580,359161,5.828995227813721,3.8689081680679643e-07
179780,179781,179780,359561,5.836150169372559,3.881880200227472e-07
179980,179981,179980,359961,5.842638254165649,4.4542765894237637e-07
180180,180181,180180,360361,5.850030183792114,3.7380654365853925e-07
180380,180381,180380,360761,5.857254266738892,3.704341157529024e-07
180581,180582,180581,361163,5.8675782680511475,3.730772609061645e-07
180781,180782,180781,361563,5.873530149459839,3.579674960644339e-07
180981,180982,180981,361963,5.879508018493652,4.2248612024190485e-07
181181,181182,181181,362363,5.885439157485962,3.535832058701111e-07
181381,181382,181381,362763,5.891407251358032,3.4396941058582573e-07
181582,181583,181582,363165,5.897385120391846,3.4600245311618503e-07
181782,181783,181782,363565,5.903462171554565,3.380894901256528e-07
181982,181983,181982,363965,5.909440994262695,3.36216238015233e-07
182182,182183,182182,364365,5.915408134460449,3.270776820703556e-07
182382,182383,182382,364765,5.921365022659302,3.2487487109541917e-07
182583,182584,182583,365167,5.927370071411133,3.227232376907563e-07
182783,182784,182783,365567,5.9340691566467285,3.164472051039615e-07
182983,182984,182983,365967,5.940091133117676,3.14998162035889e-07
183183,183184,183183,366367,5.946025133132935,3.1032618997181164e-07
183383,183384,183383,366767,5.9525229930877686,3.34378598861427e-07
183584,183585,183584,367169,5.958611011505127,3.0066649403855614e-07
183784,183785,183784,367569,5.964915990829468,3.386459294131175e-07
183984,183985,183984,367969,5.9712841510772705,3.127985014054831e-07
184184,184185,184184,368369,5.977713108062744,2.903378903689313e-07
184384,184385,184384,368769,5.983988046646118,2.8663279251171254e-07
184585,184586,184585,369171,5.990061044692993,2.813705481461798e-07
184785,184786,184785,369571,5.996148109436035,2.81816944899207e-07
184985,184986,184985,369971,6.002306222915649,2.788483366068662e-07
185185,185186,185185,370371,6.008733034133911,2.7147854038216606e-07
185385,185386,185385,370771,6.015594005584717,2.71399080225899e-07
185586,185587,185586,371173,6.021989107131958,2.663955081024296e-07
185786,185787,185786,371573,6.028144121170044,2.6396369554276765e-07
185986,185987,185986,371973,6.034408092498779,2.612937017011231e-07
186186,186187,186186,372373,6.040472030639648,2.572260469374294e-07
186386,186387,186386,372773,6.0468971729278564,2.536160903215391e-07
186587,186588,186587,373175,6.053547143936157,2.521241032429757e-07
186787,186788,186787,373575,6.060148000717163,2.4707117246757094e-07
186987,186988,186987,373975,6.066766262054443,2.4805714759952017e-07
187187,187188,187187,374375,6.0734169483184814,2.3930966323112394e-07
187387,187388,187387,374775,6.080028295516968,2.401936639844254e-07
187588,187589,187588,375177,6.08669900894165,2.345962781146952e-07
187788,187789,187788,375577,6.0932652950286865,2.3726606208443758e-07
187988,187989,187988,375977,6.099858999252319,2.3050344234547178e-07
188188,188189,188188,376377,6.1064441204071045,2.2582922485090693e-07
188388,188389,188388,376777,6.113084316253662,2.222927340122151e-07
188589,188590,188589,377179,6.119699954986572,2.3106134090567354e-07
188789,188790,188789,377579,6.126265048980713,2.1717638417812283e-07
188989,188990,188989,377979,6.1328771114349365,2.1502886576686213e-07
189189,189190,189189,378379,6.139456033706665,2.1506718352039058e-07
189389,189390,189389,378779,6.146022319793701,2.5062477535138634e-07
189590,189591,189590,379181,6.152720212936401,2.0690793751832288e-07
189790,189791,189790,379581,6.1593310832977295,2.0866425024417212e-07
189990,189991,189990,379981,6.1659791469573975,2.157410786036651e-07
190190,190191,190190,380381,6.17253303527832,2.001656954132337e-07
190390,190391,190390,380781,6.179088115692139,2.0230920898347357e-07
190591,190592,190591,381183,6.185680150985718,1.9641112258544531e-07
190791,190792,190791,381583,6.192276954650879,1.936086054896392e-07
190991,190992,190991,381983,6.198849201202393,2.3792766872551678e-07
191191,191192,191191,382383,6.20542311668396,2.2717787603018825e-07
191391,191392,191391,382783,6.212013006210327,1.847849098733806e-07
191592,191593,191592,383185,6.218583106994629,1.83047528401909e-07
191792,191793,191792,383585,6.225100040435791,1.7996793750428577e-07
191992,191993,191992,383985,6.231601238250732,1.8480635534904752e-07
192192,192193,192192,384385,6.238171100616455,2.0583636510478517e-07
192392,192393,192392,384785,6.2447521686553955,1.7426141188622477e-07
192593,192594,192593,385187,6.251334190368652,1.726980655669138e-07
192793,192794,192793,385587,6.257974147796631,1.9894162122399899e-07
192993,192994,192993,385987,6.264592170715332,1.721460141068036e-07
193193,193194,193193,386387,6.2713470458984375,1.6536183881732199e-07
193393,193394,193393,386787,6.277925252914429,1.6359554968959807e-07
193594,193595,193594,387189,6.284540176391602,1.6198052573489364e-07
193794,193795,193794,387589,6.2910919189453125,1.61210544363033e-07
193994,193995,193994,387989,6.297656059265137,1.5978896186107317e-07
194194,194195,194194,388389,6.304479122161865,1.5803353896488735e-07
194394,194395,194394,388789,6.311105012893677,1.651762119422239e-07
194595,194596,194595,389191,6.317719221115112,1.5204052372855503e-07
194795,194796,194795,389591,6.3243491649627686,1.5230291389973712e-07
194995,194996,194995,389991,6.330897331237793,1.4749212025377241e-07
195195,195196,195195,390391,6.337467193603516,1.4646330285967154e-07
195395,195396,195395,390791,6.3440330028533936,1.4493927597843125e-07
195596,195597,195596,391193,6.350476026535034,1.4611117054541662e-07
195796,195797,195796,391593,6.356771230697632,1.4086911669171404e-07
195996,195997,195996,391993,6.362819194793701,1.4039907603303907e-07
196196,196197,196196,392393,6.369241237640381,1.7611143306998492e-07
196396,196397,196396,392793,6.3754072189331055,1.3591732837203612e-07
196597,196598,196597,393195,6.381468296051025,1.3609154087814068e-07
196797,196798,196797,393595,6.387593984603882,1.5129802630800884e-07
196997,196998,196997,393995,6.393568992614746,1.4386110121848454e-07
197197,197198,197197,394395,6.400371074676514,1.2859402023238371e-07
197397,197398,197397,394795,6.406495094299316,1.3366788903621074e-07
197598,197599,197598,395197,6.412689208984375,1.2688246889409319e-07
197798,197799,197798,395597,6.418874263763428,1.4237206487837949e-07
197998,197999,197998,395997,6.4250853061676025,1.2534540830501232e-07
198198,198199,198198,396397,6.431403160095215,1.218021094035284e-07
198398,198399,198398,396797,6.437704086303711,1.2737020783306333e-07
198599,198600,198599,397199,6.443819999694824,1.197261432476724e-07
198799,198800,198799,397599,6.450104236602783,1.2194609640495158e-07
198999,199000,198999,397999,6.456501007080078,1.1453764526183931e-07
199199,199200,199199,398399,6.462824106216431,1.1477509256293478e-07
199399,199400,199399,398799,6.469006061553955,1.1887058164038474e-07
199600,199601,199600,399201,6.475252151489258,1.1234135752323488e-07
199800,199801,199800,399601,6.481571197509766,1.093100178755101e-07
200000,200001,200000,400001,6.487688064575195,1.0866655368965862e-07


==> plot_data/quadratic_minimax_problem_n20_alpha00001/eag-c.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00020599365234375,4.387072431292609
100,201,0,201,0.006331920623779297,1.0665443360783584
200,401,0,401,0.01179814338684082,0.4043848940096791
300,601,0,601,0.01671910285949707,0.3037256513010002
400,801,0,801,0.02155017852783203,0.21227736203975886
501,1003,0,1003,0.026380062103271484,0.1713519080960906
601,1203,0,1203,0.031150102615356445,0.14928003567712142
701,1403,0,1403,0.03576183319091797,0.12137429974972368
801,1603,0,1603,0.040251970291137695,0.10171803824306211
901,1803,0,1803,0.044178009033203125,0.08906050214503931
1001,2003,0,2003,0.04797005653381348,0.08233857129632127
1101,2203,0,2203,0.05176997184753418,0.08191750433497302
1201,2403,0,2403,0.055808067321777344,0.061593030578000016
1301,2603,0,2603,0.05958890914916992,0.06914220766792943
1401,2803,0,2803,0.06345081329345703,0.0586838214605921
1502,3005,0,3005,0.06720304489135742,0.06233212960539554
1602,3205,0,3205,0.07085704803466797,0.05265842431863991
1702,3405,0,3405,0.07465291023254395,0.046996663053960774
1802,3605,0,3605,0.07829403877258301,0.05056909097153807
1902,3805,0,3805,0.08194208145141602,0.04476072777685633
2002,4005,0,4005,0.08572697639465332,0.041527156932835624
2102,4205,0,4205,0.09007692337036133,0.04040439442284881
2202,4405,0,4405,0.09400296211242676,0.03816373522257505
2302,4605,0,4605,0.09813404083251953,0.03972775316304948
2402,4805,0,4805,0.10270214080810547,0.03598618678174246
2503,5007,0,5007,0.10686302185058594,0.03408181646602452
2603,5207,0,5207,0.11076879501342773,0.03336734604469102
2703,5407,0,5407,0.11461210250854492,0.03269156365903751
2803,5607,0,5607,0.11821389198303223,0.031075952608860105
2903,5807,0,5807,0.12191200256347656,0.026396451665066812
3003,6007,0,6007,0.12561583518981934,0.029108798230438118
3103,6207,0,6207,0.12943315505981445,0.025935621345224893
3203,6407,0,6407,0.13337087631225586,0.027208639669736034
3303,6607,0,6607,0.1373310089111328,0.024079134693056833
3403,6807,0,6807,0.1416001319885254,0.02381717386131816
3504,7009,0,7009,0.14567184448242188,0.02488859104687067
3604,7209,0,7209,0.14948701858520508,0.02239884072798269
3704,7409,0,7409,0.15336203575134277,0.021339136634859323
3804,7609,0,7609,0.15718507766723633,0.020310339504418067
3904,7809,0,7809,0.16113519668579102,0.01975540475030197
4004,8009,0,8009,0.16489195823669434,0.019989282796115032
4104,8209,0,8209,0.16865205764770508,0.01742161430226497
4204,8409,0,8409,0.17271089553833008,0.018091804598004163
4304,8609,0,8609,0.17642712593078613,0.017437357656163884
4404,8809,0,8809,0.1801300048828125,0.018375298536051618
4505,9011,0,9011,0.18388986587524414,0.016121970040532493
4605,9211,0,9211,0.1877450942993164,0.016041963127096742
4705,9411,0,9411,0.19188785552978516,0.01602804982848922
4805,9611,0,9611,0.19617009162902832,0.01532893267477553
4905,9811,0,9811,0.19998788833618164,0.014859385705389836
5005,10011,0,10011,0.20383906364440918,0.013690398322403189
5105,10211,0,10211,0.20784497261047363,0.014041328423962104
5205,10411,0,10411,0.2117629051208496,0.014814579509148792
5305,10611,0,10611,0.21607613563537598,0.013608782861523958
5405,10811,0,10811,0.21987295150756836,0.013792742261871178
5506,11013,0,11013,0.2236170768737793,0.01356600599771525
5606,11213,0,11213,0.227463960647583,0.01391757820023729
5706,11413,0,11413,0.23111701011657715,0.01334828483550954
5806,11613,0,11613,0.2347710132598877,0.012523254102915486
5906,11813,0,11813,0.23870587348937988,0.012638187260244318
6006,12013,0,12013,0.24260306358337402,0.01278900089713829
6106,12213,0,12213,0.24686217308044434,0.012812109991528457
6206,12413,0,12413,0.2506840229034424,0.012145655716269544
6306,12613,0,12613,0.2552671432495117,0.012499084650217753
6406,12813,0,12813,0.25907206535339355,0.012850329986397329
6507,13015,0,13015,0.262829065322876,0.012540191102228926
6607,13215,0,13215,0.26653504371643066,0.012335295680174994
6707,13415,0,13415,0.2706129550933838,0.011776097120117483
6807,13615,0,13615,0.2744021415710449,0.012095884072375579
6907,13815,0,13815,0.27825093269348145,0.01196447816127861
7007,14015,0,14015,0.28200197219848633,0.011295828059595675
7107,14215,0,14215,0.28583407402038574,0.011423637654259524
7207,14415,0,14415,0.2905759811401367,0.01145855019705569
7307,14615,0,14615,0.2946200370788574,0.011680890598844773
7407,14815,0,14815,0.2984440326690674,0.011261977053317994
7508,15017,0,15017,0.30297183990478516,0.011042851984904347
7608,15217,0,15217,0.3069570064544678,0.011027691956134815
7708,15417,0,15417,0.311492919921875,0.010944945605208707
7808,15617,0,15617,0.31609606742858887,0.010500237738669477
7908,15817,0,15817,0.32085514068603516,0.009988836466327282
8008,16017,0,16017,0.32564306259155273,0.01010359663388243
8108,16217,0,16217,0.33031606674194336,0.010084120453508878
8208,16417,0,16417,0.33524203300476074,0.009813928371121798
8308,16617,0,16617,0.3399159908294678,0.009654937242058194
8408,16817,0,16817,0.345304012298584,0.009470216265290928
8509,17019,0,17019,0.3500649929046631,0.009662644185313011
8609,17219,0,17219,0.35465002059936523,0.009253328377386294
8709,17419,0,17419,0.35962796211242676,0.008781181360634363
8809,17619,0,17619,0.36448216438293457,0.00863967708134135
8909,17819,0,17819,0.3693702220916748,0.00855564882190571
9009,18019,0,18019,0.37421202659606934,0.008376388418705475
9109,18219,0,18219,0.3791990280151367,0.008042668608496815
9209,18419,0,18419,0.38396596908569336,0.007988637880765745
9309,18619,0,18619,0.38874292373657227,0.008127833753650802
9409,18819,0,18819,0.3941471576690674,0.00806870102553144
9510,19021,0,19021,0.3992791175842285,0.0077703526949124595
9610,19221,0,19221,0.40404415130615234,0.0075269210373787865
9710,19421,0,19421,0.40952491760253906,0.007612854848940511
9810,19621,0,19621,0.41414594650268555,0.007402934480566772
9910,19821,0,19821,0.4187610149383545,0.007137371588020664
10010,20021,0,20021,0.42337512969970703,0.007002868188865024
10110,20221,0,20221,0.4279799461364746,0.007070565082986567
10210,20421,0,20421,0.4328179359436035,0.007259282933053504
10310,20621,0,20621,0.43740105628967285,0.0070931379165547394
10410,20821,0,20821,0.44208407402038574,0.0070246710372417285
10511,21023,0,21023,0.4466109275817871,0.007135187116885399
10611,21223,0,21223,0.45094990730285645,0.007142362344751027
10711,21423,0,21423,0.4557199478149414,0.006978302090438743
10811,21623,0,21623,0.4602789878845215,0.0067710138596092494
10911,21823,0,21823,0.46456098556518555,0.006804903039138827
11011,22023,0,22023,0.4683840274810791,0.0068949303370660605
11111,22223,0,22223,0.47208094596862793,0.006878272504728402
11211,22423,0,22423,0.47579503059387207,0.006805021875594198
11311,22623,0,22623,0.4797849655151367,0.006898933668830561
11411,22823,0,22823,0.4838850498199463,0.007072103364232585
11512,23025,0,23025,0.4876830577850342,0.006986509657554643
11612,23225,0,23225,0.4915609359741211,0.006867588994009879
11712,23425,0,23425,0.49531102180480957,0.006794629695377734
11812,23625,0,23625,0.49916696548461914,0.006811378879244095
11912,23825,0,23825,0.5029189586639404,0.006775875461716418
12012,24025,0,24025,0.5069580078125,0.006613004642975174
12112,24225,0,24225,0.5107951164245605,0.006614899502687346
12212,24425,0,24425,0.5147030353546143,0.00672756497217622
12312,24625,0,24625,0.5184340476989746,0.006742453412286656
12412,24825,0,24825,0.5221350193023682,0.0066480241698004825
12513,25027,0,25027,0.5260579586029053,0.0065593001805355254
12613,25227,0,25227,0.5297799110412598,0.006554614162620634
12713,25427,0,25427,0.5336110591888428,0.006472341040534518
12813,25627,0,25627,0.5373680591583252,0.0062926941395239884
12913,25827,0,25827,0.5415518283843994,0.0061275500197760895
13013,26027,0,26027,0.54526686668396,0.0061271455076797425
13113,26227,0,26227,0.5489778518676758,0.006134622979855065
13213,26427,0,26427,0.5526840686798096,0.006024894061617505
13313,26627,0,26627,0.5564939975738525,0.005953236452739838
13413,26827,0,26827,0.5602660179138184,0.00593420480897846
13514,27029,0,27029,0.5644569396972656,0.005909614789440949
13614,27229,0,27229,0.5681540966033936,0.005766516899424258
13714,27429,0,27429,0.5718550682067871,0.005553085856832774
13814,27629,0,27629,0.5756030082702637,0.005467213228234064
13914,27829,0,27829,0.5792980194091797,0.005419666878266805
14014,28029,0,28029,0.5831749439239502,0.005312448436598062
14114,28229,0,28229,0.5869150161743164,0.005198705856801084
14214,28429,0,28429,0.5906550884246826,0.005186921295217133
14314,28629,0,28629,0.5943968296051025,0.005230433421113172
14414,28829,0,28829,0.5982930660247803,0.0051866974255970885
14515,29031,0,29031,0.6021051406860352,0.005065163136182162
14615,29231,0,29231,0.6057770252227783,0.004972098121249699
14715,29431,0,29431,0.6096639633178711,0.004952967693699861
14815,29631,0,29631,0.613684892654419,0.004871516834848687
14915,29831,0,29831,0.6180479526519775,0.004739281924386812
15015,30031,0,30031,0.6217830181121826,0.004705354071491604
15115,30231,0,30231,0.6256451606750488,0.004754867436692766
15215,30431,0,30431,0.6297070980072021,0.004803819493196498
15315,30631,0,30631,0.6335539817810059,0.004780552583254227
15415,30831,0,30831,0.6372060775756836,0.004759276388593549
15516,31033,0,31033,0.6412539482116699,0.004804613937714447
15616,31233,0,31233,0.6449310779571533,0.00480160906010214
15716,31433,0,31433,0.6489138603210449,0.004719762963471144
15816,31633,0,31633,0.6525900363922119,0.00464990474195754
15916,31833,0,31833,0.6567990779876709,0.00466732561207649
16016,32033,0,32033,0.660506010055542,0.004708872997249917
16116,32233,0,32233,0.6646349430084229,0.004711773320950185
16216,32433,0,32433,0.6683950424194336,0.004716906262737957
16316,32633,0,32633,0.6725058555603027,0.0047757029273886
16416,32833,0,32833,0.6763269901275635,0.004842870464171625
16517,33035,0,33035,0.6803641319274902,0.004821471405621731
16617,33235,0,33235,0.6844749450683594,0.004759799378513179
16717,33435,0,33435,0.6883730888366699,0.004739996530292616
16817,33635,0,33635,0.6923689842224121,0.004734997678963205
16917,33835,0,33835,0.6964371204376221,0.004705931398490438
17017,34035,0,34035,0.7004668712615967,0.004658571905748072
17117,34235,0,34235,0.7045948505401611,0.004665907532615986
17217,34435,0,34435,0.7085740566253662,0.004719482785742899
17317,34635,0,34635,0.712155818939209,0.00472829744303786
17417,34835,0,34835,0.7161788940429688,0.004686039169487886
17518,35037,0,35037,0.7198519706726074,0.004649545633938963
17618,35237,0,35237,0.7243080139160156,0.004629218708250144
17718,35437,0,35437,0.7279260158538818,0.004571707860271163
17818,35637,0,35637,0.7319061756134033,0.004475630436789604
17918,35837,0,35837,0.7356789112091064,0.004404129163616312
18018,36037,0,36037,0.7396202087402344,0.004389765931005424
18118,36237,0,36237,0.7433888912200928,0.0043828957989951196
18218,36437,0,36437,0.7472879886627197,0.0043365072490303865
18318,36637,0,36637,0.7511820793151855,0.004297993031085548
18418,36837,0,36837,0.7550652027130127,0.004286435521387073
18519,37039,0,37039,0.7589881420135498,0.0042495757352079624
18619,37239,0,37239,0.762714147567749,0.004161544365109822
18719,37439,0,37439,0.7667357921600342,0.004056594586943836
18819,37639,0,37639,0.7704670429229736,0.003993675384305692
18919,37839,0,37839,0.7744059562683105,0.003953887279440949
19019,38039,0,38039,0.7781178951263428,0.003893904654458814
19119,38239,0,38239,0.7820768356323242,0.00384252747039768
19219,38439,0,38439,0.7865641117095947,0.003838514292745753
19319,38639,0,38639,0.791205883026123,0.003849363554465216
19419,38839,0,38839,0.7950100898742676,0.003818720750678488
19520,39041,0,39041,0.7992420196533203,0.00375574023968879
19620,39241,0,39241,0.8034958839416504,0.0037067565424039254
19720,39441,0,39441,0.8078889846801758,0.003675353960046598
19820,39641,0,39641,0.8120582103729248,0.003625559356444488
19920,39841,0,39841,0.8160839080810547,0.00356411894402922
20020,40041,0,40041,0.8201079368591309,0.003550433197617234
20120,40241,0,40241,0.8239810466766357,0.003580706030900932
20220,40441,0,40441,0.8276689052581787,0.0036029431285344595
20320,40641,0,40641,0.8316328525543213,0.0036017159467801717
20420,40841,0,40841,0.8353757858276367,0.003602901079325168
20521,41043,0,41043,0.839155912399292,0.003618723526983722
20621,41243,0,41243,0.8431539535522461,0.0036118279084259887
20721,41443,0,41443,0.8469669818878174,0.0035708964820438034
20821,41643,0,41643,0.8508849143981934,0.0035419596328997295
20921,41843,0,41843,0.854640007019043,0.0035530887763210285
21021,42043,0,42043,0.859065055847168,0.003576275418759701
21121,42243,0,42243,0.8627579212188721,0.0035875671678253364
21221,42443,0,42443,0.8665862083435059,0.0036064166339811734
21321,42643,0,42643,0.8704619407653809,0.003645217858188393
21421,42843,0,42843,0.8743031024932861,0.0036762453972208147
21522,43045,0,43045,0.878087043762207,0.0036681969235645793
21622,43245,0,43245,0.8826601505279541,0.0036396635026805
21722,43445,0,43445,0.886430025100708,0.003626875248367201
21822,43645,0,43645,0.8902640342712402,0.0036206297967762667
21922,43845,0,43845,0.8940348625183105,0.003602588496770977
22022,44045,0,44045,0.8982889652252197,0.0035871845989075015
22122,44245,0,44245,0.9020609855651855,0.0035979149157709766
22222,44445,0,44445,0.9057819843292236,0.0036239238012852884
22322,44645,0,44645,0.9097900390625,0.003628814163858306
22422,44845,0,44845,0.9136099815368652,0.0036082656577017453
22523,45047,0,45047,0.9177210330963135,0.003586287286964641
22623,45247,0,45247,0.9215259552001953,0.003564588707962591
22723,45447,0,45447,0.9253330230712891,0.0035228205211254027
22823,45647,0,45647,0.9297800064086914,0.0034665635222424244
22923,45847,0,45847,0.9338748455047607,0.0034271464125292376
23023,46047,0,46047,0.938452959060669,0.003413500539925737
23123,46247,0,46247,0.9434850215911865,0.00340270640135036
23223,46447,0,46447,0.9483120441436768,0.0033790268191162425
23323,46647,0,46647,0.953139066696167,0.0033568553836871395
23423,46847,0,46847,0.9583349227905273,0.003341985643593583
23524,47049,0,47049,0.9631638526916504,0.0033096143429991844
23624,47249,0,47249,0.9677770137786865,0.003250663893688416
23724,47449,0,47449,0.9723258018493652,0.003187966715326419
23824,47649,0,47649,0.9769868850708008,0.003143567319717368
23924,47849,0,47849,0.9816529750823975,0.003110438239946373
24024,48049,0,48049,0.9862661361694336,0.0030746699901534787
24124,48249,0,48249,0.9907259941101074,0.0030483317510129394
24224,48449,0,48449,0.9947671890258789,0.0030443259184981205
24324,48649,0,48649,0.9992420673370361,0.003043715794161994
24424,48849,0,48849,1.0044159889221191,0.003021665593696061
24525,49051,0,49051,1.0087108612060547,0.002984110524663237
24625,49251,0,49251,1.012557029724121,0.0029519652291317353
24725,49451,0,49451,1.0166740417480469,0.0029245228238957387
24825,49651,0,49651,1.0204448699951172,0.0028910579504520134
24925,49851,0,49851,1.0244548320770264,0.0028604281507752234
25025,50051,0,50051,1.0281810760498047,0.0028554824936915346
25125,50251,0,50251,1.0321941375732422,0.0028730390615702922
25225,50451,0,50451,1.0363969802856445,0.0028874201579118337
25325,50651,0,50651,1.0407838821411133,0.0028916465559343132
25425,50851,0,50851,1.0446348190307617,0.0028967179910624422
25526,51053,0,51053,1.0487518310546875,0.0029026497037709636
25626,51253,0,51253,1.052551031112671,0.0028950544779333697
25726,51453,0,51453,1.056431770324707,0.0028739170734494775
25826,51653,0,51653,1.0602591037750244,0.00286126314355283
25926,51853,0,51853,1.0641610622406006,0.0028690586889458984
26026,52053,0,52053,1.0682439804077148,0.0028846535757463794
26126,52253,0,52253,1.0720329284667969,0.0028981906177031574
26226,52453,0,52453,1.07607102394104,0.0029171326269452603
26326,52653,0,52653,1.0800042152404785,0.0029429582601344204
26426,52853,0,52853,1.0838348865509033,0.0029596675901451854
26527,53055,0,53055,1.087705135345459,0.002955786181355829
26627,53255,0,53255,1.091583013534546,0.0029415910178032215
26727,53455,0,53455,1.0953831672668457,0.0029325020451796357
26827,53655,0,53655,1.0992991924285889,0.002926420148133577
26927,53855,0,53855,1.1031138896942139,0.0029168971936250586
27027,54055,0,54055,1.106816053390503,0.0029124523651783835
27127,54255,0,54255,1.1105079650878906,0.0029219266416132287
27227,54455,0,54455,1.1142170429229736,0.002936016896715295
27327,54655,0,54655,1.1179070472717285,0.0029381679117688234
27427,54855,0,54855,1.1222589015960693,0.002926622083477666
27528,55057,0,55057,1.1259610652923584,0.0029107090599823217
27628,55257,0,55257,1.1296310424804688,0.0028909075809120926
27728,55457,0,55457,1.1332721710205078,0.0028602644694026673
27828,55657,0,55657,1.1368520259857178,0.0028246681067335454
27928,55857,0,55857,1.1405329704284668,0.0027996784645783084
28028,56057,0,56057,1.1441128253936768,0.0027879842904407997
28128,56257,0,56257,1.1476831436157227,0.0027779964454126703
28228,56457,0,56457,1.151353120803833,0.00276338593906699
28328,56657,0,56657,1.1549949645996094,0.002748533266638918
28428,56857,0,56857,1.1586840152740479,0.002733063682126576
28529,57059,0,57059,1.1622898578643799,0.00270580824753568
28629,57259,0,57259,1.1658618450164795,0.002664646793863797
28729,57459,0,57459,1.1694550514221191,0.0026225257646584543
28829,57659,0,57659,1.1730780601501465,0.0025900344335061084
28929,57859,0,57859,1.17665696144104,0.0025642686547482454
29029,58059,0,58059,1.180279016494751,0.0025411764739629076
29129,58259,0,58259,1.1838798522949219,0.0025260126463449283
29229,58459,0,58459,1.1874980926513672,0.002521552844074032
29329,58659,0,58659,1.191161870956421,0.0025168133560171104
29429,58859,0,58859,1.1948249340057373,0.0025003696508405318
29530,59061,0,59061,1.1985769271850586,0.0024754895655524343
29630,59261,0,59261,1.2023448944091797,0.002452126789662086
29730,59461,0,59461,1.2059810161590576,0.0024303504082544046
29830,59661,0,59661,1.2096009254455566,0.0024077379172443444
29930,59861,0,59861,1.2132070064544678,0.0023912094795578765
30030,60061,0,60061,1.2168259620666504,0.002390183037840966
30130,60261,0,60261,1.2204458713531494,0.002401126930704741
30230,60461,0,60461,1.2240850925445557,0.0024114327623809863
30330,60661,0,60661,1.2277429103851318,0.002416895735905329
30430,60861,0,60861,1.2313830852508545,0.002421378641681876
30531,61063,0,61063,1.2349328994750977,0.002423397141596426
30631,61263,0,61263,1.238386869430542,0.0024172137774760745
30731,61463,0,61463,1.2419230937957764,0.0024057795027338474
30831,61663,0,61663,1.2462220191955566,0.00240052422105147
30931,61863,0,61863,1.2498109340667725,0.0024066840016367555
31031,62063,0,62063,1.2533900737762451,0.0024185209563215813
31131,62263,0,62263,1.2570230960845947,0.0024315115949985937
31231,62463,0,62463,1.260603904724121,0.0024476134471870096
31331,62663,0,62663,1.2642099857330322,0.0024650980869235003
31431,62863,0,62863,1.2678091526031494,0.0024750934256310194
31532,63065,0,63065,1.2715198993682861,0.0024730614549414516
31632,63265,0,63265,1.2751259803771973,0.0024651323974305707
31732,63465,0,63465,1.278731107711792,0.002458668857591029
31832,63665,0,63665,1.2824928760528564,0.0024537476565542095
31932,63865,0,63865,1.285999059677124,0.002449042281279254
32032,64065,0,64065,1.2894551753997803,0.002448894993958359
32132,64265,0,64265,1.2928550243377686,0.0024561245034953544
32232,64465,0,64465,1.2962470054626465,0.0024643181630573095
32332,64665,0,64665,1.2996528148651123,0.002464945013251972
32432,64865,0,64865,1.3031129837036133,0.002457127956096754
32533,65067,0,65067,1.3067588806152344,0.002444535642370448
32633,65267,0,65267,1.3102920055389404,0.0024275702256925263
32733,65467,0,65467,1.3138070106506348,0.002404703870977499
32833,65667,0,65667,1.3174920082092285,0.0023806950243071717
32933,65867,0,65867,1.3210608959197998,0.0023634406831830996
33033,66067,0,66067,1.3246448040008545,0.0023536495999074915
33133,66267,0,66267,1.3283560276031494,0.002345257713125191
33233,66467,0,66467,1.3319759368896484,0.002334908157663821
33333,66667,0,66667,1.3356130123138428,0.002323405760873682
33433,66867,0,66867,1.3392541408538818,0.0023089401783089425
33534,67069,0,67069,1.3429489135742188,0.002286328457944004
33634,67269,0,67269,1.3466119766235352,0.0022562635208968965
33734,67469,0,67469,1.3502459526062012,0.0022260872915794306
33834,67669,0,67669,1.3539369106292725,0.002201563040054933
33934,67869,0,67869,1.3575379848480225,0.0021819626540537777
34034,68069,0,68069,1.3612711429595947,0.0021661871089955803
34134,68269,0,68269,1.3649709224700928,0.002156311287251824
34234,68469,0,68469,1.3686180114746094,0.0021517208652154056
34334,68669,0,68669,1.372277021408081,0.002145783233388275
34434,68869,0,68869,1.3759238719940186,0.0021330175346486145
34535,69071,0,69071,1.379612922668457,0.0021152184509339676
34635,69271,0,69271,1.3833260536193848,0.0020974924372559123
34735,69471,0,69471,1.3876399993896484,0.0020807020103184725
34835,69671,0,69671,1.391291856765747,0.002065335905473507
34935,69871,0,69871,1.3949828147888184,0.0020559503899802555
35035,70071,0,70071,1.3985910415649414,0.0020565256415721435
35135,70271,0,70271,1.4023330211639404,0.002064025022165248
35235,70471,0,70471,1.4059689044952393,0.0020716963355108687
35335,70671,0,70671,1.4095239639282227,0.00207678055605356
35435,70871,0,70871,1.4129350185394287,0.002080094927042732
35536,71073,0,71073,1.4167470932006836,0.002080464585469403
35636,71273,0,71273,1.420198917388916,0.00207599345823942
35736,71473,0,71473,1.4236059188842773,0.002069716849181548
35836,71673,0,71673,1.4271581172943115,0.00206799725721463
35936,71873,0,71873,1.4306659698486328,0.0020733152463785925
36036,72073,0,72073,1.434251070022583,0.0020829007135832575
36136,72273,0,72273,1.4378161430358887,0.0020943149921211044
36236,72473,0,72473,1.4414949417114258,0.002107268657553717
36336,72673,0,72673,1.4452481269836426,0.0021193971968109927
36436,72873,0,72873,1.4490430355072021,0.002125781770988691
36537,73075,0,73075,1.4531610012054443,0.002124659594861811
36637,73275,0,73275,1.4580740928649902,0.002119755752606077
36737,73475,0,73475,1.462162971496582,0.002115128541092619
36837,73675,0,73675,1.4662442207336426,0.002111584811220459
36937,73875,0,73875,1.4698669910430908,0.0021094610437798
37037,74075,0,74075,1.473402976989746,0.002110883475118884
37137,74275,0,74275,1.4769349098205566,0.002116171211125743
37237,74475,0,74475,1.480454921722412,0.0021210491780371613
37337,74675,0,74675,1.4842958450317383,0.002120762691538424
37437,74875,0,74875,1.4888169765472412,0.0021146439923422486
37538,75077,0,75077,1.4930140972137451,0.0021042100216869587
37638,75277,0,75277,1.4974830150604248,0.0020900783061744326
37738,75477,0,75477,1.5016989707946777,0.0020727091609449985
37838,75677,0,75677,1.5067059993743896,0.002055645361384762
37938,75877,0,75877,1.5107431411743164,0.0020430379032463923
38038,76077,0,76077,1.5149109363555908,0.0020349092102865634
38138,76277,0,76277,1.518885850906372,0.0020278990536196904
38238,76477,0,76477,1.5228638648986816,0.002019810887831849
38338,76677,0,76677,1.5266098976135254,0.0020101222444848968
38438,76877,0,76877,1.5302300453186035,0.001997153574729158
38539,77079,0,77079,1.5339279174804688,0.0019785087416847695
38639,77279,0,77279,1.5376520156860352,0.0019557132898316266
38739,77479,0,77479,1.5413870811462402,0.0019331855190116388
38839,77679,0,77679,1.5451750755310059,0.0019143493972393645
38939,77879,0,77879,1.5490319728851318,0.0018994130612133495
39039,78079,0,78079,1.5534279346466064,0.0018881300208304225
39139,78279,0,78279,1.5572500228881836,0.0018809923668241363
39239,78479,0,78479,1.5610949993133545,0.001876501623858607
39339,78679,0,78679,1.564866065979004,0.0018705328144519439
39439,78879,0,78879,1.5687291622161865,0.0018603063270764086
39540,79081,0,79081,1.5724811553955078,0.00184687255314482
39640,79281,0,79281,1.576197862625122,0.001833166632657935
39740,79481,0,79481,1.5799198150634766,0.0018203690921582503
39840,79681,0,79681,1.5836291313171387,0.0018098171288269778
39940,79881,0,79881,1.5873548984527588,0.0018043402593742037
40040,80081,0,80081,1.591062068939209,0.0018055225047469248
40140,80281,0,80281,1.594797134399414,0.0018110247329532507
40240,80481,0,80481,1.5985841751098633,0.0018168595580224643
40340,80681,0,80681,1.6023359298706055,0.0018210591784672057
40440,80881,0,80881,1.606208086013794,0.0018233829609901595
40541,81083,0,81083,1.6100749969482422,0.001823130062082156
40641,81283,0,81283,1.6138288974761963,0.0018200793030817444
40741,81483,0,81483,1.6175739765167236,0.0018167217419772046
40841,81683,0,81683,1.6213150024414062,0.0018167740805258745
40941,81883,0,81883,1.6250419616699219,0.001821534420071793
41041,82083,0,82083,1.6287622451782227,0.0018295271038641617
41141,82283,0,82283,1.6324479579925537,0.001839148466390585
41241,82483,0,82483,1.6361069679260254,0.0018493362690764723
41341,82683,0,82683,1.6397271156311035,0.0018579474286627188
41441,82883,0,82883,1.643388032913208,0.0018622031303593422
41542,83085,0,83085,1.6470520496368408,0.0018615204732591404
41642,83285,0,83285,1.650805950164795,0.0018582588216374241
41742,83485,0,83485,1.6545090675354004,0.0018549398807084837
41842,83685,0,83685,1.6583118438720703,0.0018525628838782096
41942,83885,0,83885,1.6624300479888916,0.0018518094174418027
42042,84085,0,84085,1.666903018951416,0.0018536249782104665
42142,84285,0,84285,1.670516014099121,0.001857417631387779
42242,84485,0,84485,1.674138069152832,0.0018602791893855871
42342,84685,0,84685,1.6778030395507812,0.0018593836303518285
42442,84885,0,84885,1.6814148426055908,0.0018541747447988765
42543,85087,0,85087,1.6853599548339844,0.0018453448735626004
42643,85287,0,85287,1.6893692016601562,0.0018336896990333543
42743,85487,0,85487,1.693068027496338,0.0018202718818095891
42843,85687,0,85687,1.697378158569336,0.0018076295460359652
42943,85887,0,85887,1.7010810375213623,0.0017980333556378682
43043,86087,0,86087,1.7048649787902832,0.0017912724582326335
43143,86287,0,86287,1.7085480690002441,0.0017853173791990218
43243,86487,0,86487,1.7121751308441162,0.0017785575963324856
43343,86687,0,86687,1.7157912254333496,0.0017700858944828196
43443,86887,0,86887,1.719451904296875,0.0017586698871172144
43544,87089,0,87089,1.7231171131134033,0.001743284084365561
43644,87289,0,87289,1.7267310619354248,0.0017255228013394412
43744,87489,0,87489,1.730349063873291,0.001708217718870248
43844,87689,0,87689,1.7339608669281006,0.0016935749397162918
43944,87889,0,87889,1.7380809783935547,0.0016820778868647157
44044,88089,0,88089,1.7417058944702148,0.0016736661533953462
44144,88289,0,88289,1.7453489303588867,0.0016681028184714244
44244,88489,0,88489,1.748966932296753,0.001663845973427704
44344,88689,0,88689,1.752612829208374,0.001658273217956796
44444,88889,0,88889,1.7562339305877686,0.0016499013411023916
44545,89091,0,89091,1.75990891456604,0.001639405825868006
44645,89291,0,89291,1.7635350227355957,0.001628703071724025
44745,89491,0,89491,1.767204999923706,0.0016189938981112087
44845,89691,0,89691,1.7707970142364502,0.0016116666330663956
44945,89891,0,89891,1.7744319438934326,0.0016084383630695356
45045,90091,0,90091,1.7780230045318604,0.001609805927195397
45145,90291,0,90291,1.7816319465637207,0.001614009484575527
45245,90491,0,90491,1.7852318286895752,0.0016184936227270224
45345,90691,0,90691,1.7888860702514648,0.001621781044552678
45445,90891,0,90891,1.7926020622253418,0.0016233798161173864
45546,91093,0,91093,1.7962439060211182,0.0016229692793124856
45646,91293,0,91293,1.7999050617218018,0.001620983672444938
45746,91493,0,91493,1.803508996963501,0.0016193408487428724
45846,91693,0,91693,1.8074009418487549,0.0016203044877079538
45946,91893,0,91893,1.8110849857330322,0.0016245977356713723
46046,92093,0,92093,1.8147199153900146,0.0016313259466340423
46146,92293,0,92293,1.818432092666626,0.0016392670384607322
46246,92493,0,92493,1.8220739364624023,0.0016472050724217848
46346,92693,0,92693,1.8256640434265137,0.0016534330982215122
46446,92893,0,92893,1.8294289112091064,0.0016563499101214338
46547,93095,0,93095,1.8331289291381836,0.001655876711064969
46647,93295,0,93295,1.836771011352539,0.0016536002968191067
46747,93495,0,93495,1.8403599262237549,0.0016512305899073992
46847,93695,0,93695,1.843963861465454,0.001649715024426822
46947,93895,0,93895,1.847588062286377,0.0016496630441051622
47047,94095,0,94095,1.851172924041748,0.0016513877697684792
47147,94295,0,94295,1.8547677993774414,0.0016540492440290098
47247,94495,0,94495,1.8584351539611816,0.0016556166026718692
47347,94695,0,94695,1.8622899055480957,0.00165430779202747
47447,94895,0,94895,1.8659851551055908,0.0016496894760770486
47548,95097,0,95097,1.8696818351745605,0.001642149981709537
47648,95297,0,95297,1.8732731342315674,0.0016325481320045713
47748,95497,0,95497,1.8768599033355713,0.0016220147811073506
47848,95697,0,95697,1.8804538249969482,0.0016123385602712548
47948,95897,0,95897,1.884063959121704,0.0016048021624173476
48048,96097,0,96097,1.8877592086791992,0.0015991267195110768
48148,96297,0,96297,1.8914299011230469,0.0015939663768588614
48248,96497,0,96497,1.8950409889221191,0.0015880784558755814
48348,96697,0,96697,1.898643970489502,0.0015805624965131366
48448,96897,0,96897,1.9023020267486572,0.0015706009283711535
48549,97099,0,97099,1.9059898853302002,0.0015578503242424059
48649,97299,0,97299,1.9097537994384766,0.0015437366672655742
48749,97499,0,97499,1.9133620262145996,0.001530171156538347
48849,97699,0,97699,1.9172749519348145,0.0015186649935898988
48949,97899,0,97899,1.9210140705108643,0.0015096976652755351
49049,98099,0,98099,1.9247210025787354,0.0015031924721118752
49149,98299,0,98299,1.928765058517456,0.0014986288856568197
49249,98499,0,98499,1.9324870109558105,0.0014946751725461265
49349,98699,0,98699,1.9361968040466309,0.0014896288646744278
49449,98899,0,98899,1.9405550956726074,0.0014826751168555102
49550,99101,0,99101,1.9442617893218994,0.00147430028866525
49650,99301,0,99301,1.9480319023132324,0.001465891217176323
49750,99501,0,99501,1.9517590999603271,0.0014585307337913198
49850,99701,0,99701,1.955489158630371,0.0014533938427232775
49950,99901,0,99901,1.959195852279663,0.0014515028599327469
50050,100101,0,100101,1.9629628658294678,0.0014528670680083915
50150,100301,0,100301,1.9666879177093506,0.001456150285125152
50250,100501,0,100501,1.9708130359649658,0.0014596079002268572
50350,100701,0,100701,1.9747400283813477,0.0014621158776447682
50450,100901,0,100901,1.9783570766448975,0.0014632152201788688
50551,101103,0,101103,1.982226848602295,0.0014628405287040343
50651,101303,0,101303,1.9864089488983154,0.0014616255954982616
50751,101503,0,101503,1.989988088607788,0.0014610123790097286
50851,101703,0,101703,1.993541955947876,0.0014624311312326991
50951,101903,0,101903,1.9971089363098145,0.0014662870142144843
51051,102103,0,102103,2.0006799697875977,0.0014719538429671893
51151,102303,0,102303,2.0045251846313477,0.0014784335470839857
51251,102503,0,102503,2.0081191062927246,0.0014845988371514464
51351,102703,0,102703,2.011727809906006,0.001489164227415954
51451,102903,0,102903,2.015291929244995,0.0014911970065728732
51552,103105,0,103105,2.0188820362091064,0.0014908280360570322
51652,103305,0,103305,2.0224390029907227,0.0014891893350829622
51752,103505,0,103505,2.0261151790618896,0.0014875093896418632
51852,103705,0,103705,2.0296828746795654,0.0014865858344306206
51952,103905,0,103905,2.0332422256469727,0.0014868593926201496
52052,104105,0,104105,2.036808967590332,0.001488315559944031
52152,104305,0,104305,2.0403671264648438,0.0014901208358318525
52252,104505,0,104505,2.043936014175415,0.0014908245004318528
52352,104705,0,104705,2.047546863555908,0.0014892493313470633
52452,104905,0,104905,2.0511999130249023,0.0014850863629610243
52553,105107,0,105107,2.0548951625823975,0.0014786212784479607
52653,105307,0,105307,2.0584700107574463,0.0014706871814646582
52753,105507,0,105507,2.062150001525879,0.0014622923662275951
52853,105707,0,105707,2.065757989883423,0.0014546915792288848
52953,105907,0,105907,2.069540023803711,0.0014486220644176798
53053,106107,0,106107,2.0731780529022217,0.001443795141312597
53153,106307,0,106307,2.076831102371216,0.0014392459505089114
53253,106507,0,106507,2.080591917037964,0.0014339994067943344
53353,106707,0,106707,2.084401845932007,0.0014272992301729648
53453,106907,0,106907,2.088239908218384,0.0014186429087567197
53554,107109,0,107109,2.092210054397583,0.0014080200608261966
53654,107309,0,107309,2.0962259769439697,0.0013966400472604221
53754,107509,0,107509,2.100896120071411,0.0013858453162019619
53854,107709,0,107709,2.105257987976074,0.0013767083230471695
53954,107909,0,107909,2.1097960472106934,0.001369611351928722
54054,108109,0,108109,2.1140260696411133,0.0013644220144945066
54154,108309,0,108309,2.117974042892456,0.0013605518248431226
54254,108509,0,108509,2.1216540336608887,0.0013569272770124427
54354,108709,0,108709,2.1253299713134766,0.0013524228236435286
54454,108909,0,108909,2.128938913345337,0.0013465921202757826
54555,109111,0,109111,2.1325719356536865,0.001339823827538948
54655,109311,0,109311,2.136169910430908,0.0013331879859197061
54755,109511,0,109511,2.1398420333862305,0.0013275996850738057
54855,109711,0,109711,2.143601894378662,0.0013239710278546326
54955,109911,0,109911,2.1474759578704834,0.0013228925503657272
55055,110111,0,110111,2.151362180709839,0.0013241654495624862
55155,110311,0,110311,2.155147075653076,0.0013267584182937798
55255,110511,0,110511,2.159032106399536,0.0013294249346121913
55355,110711,0,110711,2.162942886352539,0.001331315194888048
55455,110911,0,110911,2.166856050491333,0.0013320819042021775
55556,111113,0,111113,2.1714820861816406,0.001331810683326441
55656,111313,0,111313,2.175353765487671,0.0013311429494452885
55756,111513,0,111513,2.179244041442871,0.0013311527095394358
55856,111713,0,111713,2.1831259727478027,0.0013327683797807125
55956,111913,0,111913,2.1870899200439453,0.001336202565865471
56056,112113,0,112113,2.1909279823303223,0.001340962017779316
56156,112313,0,112313,2.194873809814453,0.0013462140937770635
56256,112513,0,112513,2.198751926422119,0.001350999768418385
56356,112713,0,112713,2.2027242183685303,0.0013543772467118228
56456,112913,0,112913,2.2066359519958496,0.001355805076816239
56557,113115,0,113115,2.210606098175049,0.0013554944060138827
56657,113315,0,113315,2.2145609855651855,0.0013542909778587772
56757,113515,0,113515,2.2184641361236572,0.0013531072170158169
56857,113715,0,113715,2.2223780155181885,0.0013525700991557637
56957,113915,0,113915,2.2262778282165527,0.0013529589692924786
57057,114115,0,114115,2.2301650047302246,0.0013541014050576056
57157,114315,0,114315,2.2340760231018066,0.001355257295520203
57257,114515,0,114515,2.2379400730133057,0.0013553713308112922
57357,114715,0,114715,2.2417900562286377,0.0013536425276679598
57457,114915,0,114915,2.2456588745117188,0.001349871933606939
57558,115117,0,115117,2.2496120929718018,0.0013443127069586425
57658,115317,0,115317,2.2535738945007324,0.001337723609506877
57758,115517,0,115517,2.258148193359375,0.0013309391147085707
57858,115717,0,115717,2.2621262073516846,0.001324839320645578
57958,115917,0,115917,2.2661969661712646,0.0013198468816121155
58058,116117,0,116117,2.270009756088257,0.0013156838413206536
58158,116317,0,116317,2.2740318775177,0.0013116206647561933
58258,116517,0,116517,2.2788639068603516,0.0013068926693654405
58358,116717,0,116717,2.2836270332336426,0.0013009145679796596
58458,116917,0,116917,2.288679838180542,0.0012934050885028562
58559,117119,0,117119,2.2935948371887207,0.0012845084773524169
58659,117319,0,117319,2.2983338832855225,0.0012752290156767337
58759,117519,0,117519,2.3036839962005615,0.001266537052489774
58859,117719,0,117719,2.30873703956604,0.0012592053980336809
58959,117919,0,117919,2.313401937484741,0.001253504096722392
59059,118119,0,118119,2.318265199661255,0.0012492571871808604
59159,118319,0,118319,2.322767972946167,0.0012459047071923292
59259,118519,0,118519,2.3271281719207764,0.0012426097945022773
59359,118719,0,118719,2.3310279846191406,0.0012386192653972975
59459,118919,0,118919,2.3347818851470947,0.001233701050916046
59560,119121,0,119121,2.3389129638671875,0.0012281878695332962
59660,119321,0,119321,2.342956066131592,0.00122293283539052
59760,119521,0,119521,2.346719980239868,0.0012186783697693943
59860,119721,0,119721,2.350497007369995,0.0012160999371078765
59960,119921,0,119921,2.354434013366699,0.0012155199502317728
60060,120121,0,120121,2.3581290245056152,0.0012166623174216734
60160,120321,0,120321,2.3621208667755127,0.0012187194790448054
60260,120521,0,120521,2.365949869155884,0.001220774073314742
60360,120721,0,120721,2.369636058807373,0.0012221922124737875
60460,120921,0,120921,2.373338222503662,0.0012227416255297713
60561,121123,0,121123,2.37713885307312,0.0012225859535593085
60661,121323,0,121323,2.38100004196167,0.0012223006685591498
60761,121523,0,121523,2.3849220275878906,0.0012226827673548582
60861,121723,0,121723,2.3889360427856445,0.0012243436966346238
60961,121923,0,121923,2.3929998874664307,0.0012273735766418648
61061,122123,0,122123,2.3971641063690186,0.001231355625244748
61161,122323,0,122323,2.4013261795043945,0.0012355946766753967
61261,122523,0,122523,2.4057071208953857,0.0012393102536817052
61361,122723,0,122723,2.410037040710449,0.0012418231297598177
61461,122923,0,122923,2.413881778717041,0.0012428266010161833
61562,123125,0,123125,2.4177868366241455,0.0012425542007179964
61662,123325,0,123325,2.421778917312622,0.0012416577061724425
61762,123525,0,123525,2.4264798164367676,0.0012408252971129598
61862,123725,0,123725,2.4306299686431885,0.001240527454760931
61962,123925,0,123925,2.4348080158233643,0.0012409171368314904
62062,124125,0,124125,2.4394960403442383,0.001241756621060979
62162,124325,0,124325,2.4440560340881348,0.001242419831528139
62262,124525,0,124525,2.448763847351074,0.0012421288981733344
62362,124725,0,124725,2.453450918197632,0.0012403312630190884
62462,124925,0,124925,2.45894718170166,0.0012369166854815424
62563,125127,0,125127,2.464885950088501,0.0012321244101146213
62663,125327,0,125327,2.4695229530334473,0.0012266191245696413
62763,125527,0,125527,2.474514961242676,0.0012210652015721226
62863,125727,0,125727,2.4790761470794678,0.0012160797815831434
62963,125927,0,125927,2.4835751056671143,0.0012118976748466703
63063,126127,0,126127,2.4888598918914795,0.0012082599318425065
63163,126327,0,126327,2.493957996368408,0.00120459769003242
63263,126527,0,126527,2.49868106842041,0.0012003163124092928
63363,126727,0,126727,2.503229856491089,0.0011949857968336327
63463,126927,0,126927,2.5081119537353516,0.0011884732611662128
63564,127129,0,127129,2.512755870819092,0.0011809862894665978
63664,127329,0,127329,2.517487049102783,0.0011733513085270203
63764,127529,0,127529,2.5221991539001465,0.001166282644140463
63864,127729,0,127729,2.5268049240112305,0.0011603386315335309
63964,127929,0,127929,2.5310800075531006,0.0011556911564069802
64064,128129,0,128129,2.5350239276885986,0.0011521426419972122
64164,128329,0,128329,2.539297103881836,0.0011491994596888352
64264,128529,0,128529,2.5434019565582275,0.0011462211562759045
64364,128729,0,128729,2.547759771347046,0.001142701648598482
64464,128929,0,128929,2.5522549152374268,0.001138537961479029
64565,129131,0,129131,2.556748151779175,0.0011340239964433986
64665,129331,0,129331,2.5605530738830566,0.0011298491327853466
64765,129531,0,129531,2.564363956451416,0.0011265989399070148
64865,129731,0,129731,2.568125009536743,0.0011247580072782657
64965,129931,0,129931,2.5721118450164795,0.001124482778938924
65065,130131,0,130131,2.5762460231781006,0.001125481170424162
65165,130331,0,130331,2.579946994781494,0.0011271143928382014
65265,130531,0,130531,2.583620071411133,0.0011286957858592074
65365,130731,0,130731,2.587661027908325,0.0011297598731765531
65465,130931,0,130931,2.5914671421051025,0.0011301687237887182
65566,131133,0,131133,2.595366954803467,0.0011301177237282632
65666,131333,0,131333,2.599061965942383,0.0011300947190812367
65766,131533,0,131533,2.6027560234069824,0.0011306897841469575
65866,131733,0,131733,2.6067090034484863,0.0011323060767038677
65966,131933,0,131933,2.610440969467163,0.0011349547693523313
66066,132133,0,132133,2.6142849922180176,0.0011382729635034884
66166,132333,0,132333,2.6180858612060547,0.0011416839897066841
66266,132533,0,132533,2.6217780113220215,0.0011445688993648915
66366,132733,0,132733,2.6255879402160645,0.0011464434170615238
66466,132933,0,132933,2.6293389797210693,0.0011471441637435221
66567,133135,0,133135,2.6331498622894287,0.001146900459096897
66667,133335,0,133335,2.6368980407714844,0.0011462238187286667
66767,133535,0,133535,2.6406540870666504,0.0011456353618359868
66867,133735,0,133735,2.6444170475006104,0.0011454753693114971
66967,133935,0,133935,2.6481668949127197,0.0011458068952820769
67067,134135,0,134135,2.651962995529175,0.0011463761667178858
67167,134335,0,134335,2.655730962753296,0.0011466666459666996
67267,134535,0,134535,2.6594738960266113,0.0011461003474947142
67367,134735,0,134735,2.6632399559020996,0.0011442957842391762
67467,134935,0,134935,2.667125940322876,0.0011412094108021213
67568,135137,0,135137,2.670894145965576,0.001137067405729338
67668,135337,0,135337,2.6746509075164795,0.0011324375541589713
67768,135537,0,135537,2.6783947944641113,0.0011278367412604785
67868,135737,0,135737,2.682138204574585,0.0011236965393762062
67968,135937,0,135937,2.6859030723571777,0.0011201369557607545
68068,136137,0,136137,2.6896369457244873,0.0011169220976706524
68168,136337,0,136337,2.6935129165649414,0.0011136018414512408
68268,136537,0,136537,2.697244882583618,0.001109719167754766
68368,136737,0,136737,2.700972080230713,0.0011049711168708354
68468,136937,0,136937,2.704707145690918,0.0010993207147703295
68569,137139,0,137139,2.708482027053833,0.0010929922937294829
68669,137339,0,137339,2.7122340202331543,0.0010866629247025133
68769,137539,0,137539,2.715970993041992,0.0010808635427060522
68869,137739,0,137739,2.719697952270508,0.0010759954128653647
68969,137939,0,137939,2.72340989112854,0.0010721543000711009
69069,138139,0,138139,2.727112054824829,0.0010691395486156514
69169,138339,0,138339,2.7308249473571777,0.0010665337408767173
69269,138539,0,138539,2.734449863433838,0.0010638525610627803
69369,138739,0,138739,2.7380521297454834,0.0010607576175432302
69469,138939,0,138939,2.7416670322418213,0.0010572247979932106
69570,139141,0,139141,2.7453150749206543,0.0010535154242442976
69670,139341,0,139341,2.7489349842071533,0.0010501882519705393
69770,139541,0,139541,2.752548933029175,0.0010476954289753773
69870,139741,0,139741,2.7561750411987305,0.0010463753921475534
69970,139941,0,139941,2.759812116622925,0.0010462827970036045
70070,140141,0,140141,2.7634592056274414,0.0010471379433144659
70170,140341,0,140341,2.7671260833740234,0.0010484325557060816
70270,140541,0,140541,2.7707340717315674,0.001049648491029378
70370,140741,0,140741,2.7757151126861572,0.00105044966195635
70470,140941,0,140941,2.7793290615081787,0.0010507677261430716
70571,141143,0,141143,2.7829740047454834,0.0010508024443291483
70671,141343,0,141343,2.7866098880767822,0.0010509543518747858
70771,141543,0,141543,2.790226936340332,0.0010516588870526672
70871,141743,0,141743,2.793839931488037,0.001053178419091043
70971,141943,0,141943,2.7974488735198975,0.0010554742041952998
71071,142143,0,142143,2.8010590076446533,0.0010582281038651743
71171,142343,0,142343,2.8047659397125244,0.0010609656934591717
71271,142543,0,142543,2.8083860874176025,0.0010632042048116439
71371,142743,0,142743,2.8125030994415283,0.0010646021469074348
71471,142943,0,142943,2.816215991973877,0.0010650843448377291
71572,143145,0,143145,2.8199729919433594,0.0010648635937145026
71672,143345,0,143345,2.8235881328582764,0.0010643448790118787
71772,143545,0,143545,2.827285051345825,0.0010639216882261714
71872,143745,0,143745,2.830989122390747,0.00106383174166696
71972,143945,0,143945,2.8347620964050293,0.0010640782982930725
72072,144145,0,144145,2.8384902477264404,0.0010644167565945777
72172,144345,0,144345,2.8422200679779053,0.0010644271974064267
72272,144545,0,144545,2.846034049987793,0.0010636787842792672
72372,144745,0,144745,2.849760055541992,0.0010619108678613886
72472,144945,0,144945,2.853476047515869,0.0010591269995805107
72573,145147,0,145147,2.8573708534240723,0.0010555367248304035
72673,145347,0,145347,2.8611772060394287,0.0010516168713079817
72773,145547,0,145547,2.865007162094116,0.0010477632946357175
72873,145747,0,145747,2.8688571453094482,0.0010442758675301403
72973,145947,0,145947,2.8726110458374023,0.001041203816810316
73073,146147,0,146147,2.8764140605926514,0.0010383363154786664
73173,146347,0,146347,2.8803091049194336,0.0010353156549094758
73273,146547,0,146547,2.8842549324035645,0.0010317952156195563
73373,146747,0,146747,2.8878769874572754,0.0010275704218453904
73473,146947,0,146947,2.892030954360962,0.0010226638182729317
73574,147149,0,147149,2.8962459564208984,0.0010172930889581027
73674,147349,0,147349,2.899970054626465,0.0010120114512406852
73774,147549,0,147549,2.9037129878997803,0.0010072146842532584
73874,147749,0,147749,2.9076879024505615,0.001003188086494986
73974,147949,0,147949,2.911350965499878,0.0009999726801396334
74074,148149,0,148149,2.9153800010681152,0.000997377237035575
74174,148349,0,148349,2.9191019535064697,0.00099505777197386
74274,148549,0,148549,2.9230329990386963,0.0009926515478930918
74374,148749,0,148749,2.9266300201416016,0.0009899357360331192
74474,148949,0,148949,2.9303579330444336,0.0009869338253171668
74575,149151,0,149151,2.934303045272827,0.0009838767697040714
74675,149351,0,149351,2.9380741119384766,0.0009812164671481982
74775,149551,0,149551,2.941812038421631,0.00097929595496533
74875,149751,0,149751,2.9455008506774902,0.0009783450193277686
74975,149951,0,149951,2.949453115463257,0.000978357161547767
75075,150151,0,150151,2.953118085861206,0.0009790774893403496
75175,150351,0,150351,2.9567580223083496,0.000980100589609415
75275,150551,0,150551,2.960392951965332,0.000981034602931314
75375,150751,0,150751,2.9654181003570557,0.0009816413244499516
75475,150951,0,150951,2.9697248935699463,0.0009819002227939879
75576,151153,0,151153,2.9742751121520996,0.000982000319323306
75676,151353,0,151353,2.978348970413208,0.0009822636814382027
75776,151553,0,151553,2.982651948928833,0.0009830098496363955
75876,151753,0,151753,2.9872262477874756,0.000984404420740607
75976,151953,0,151953,2.992304801940918,0.0009863787728492824
76076,152153,0,152153,2.996997833251953,0.0009886551260767087
76176,152353,0,152353,3.001579999923706,0.0009908463619869425
76276,152553,0,152553,3.0063071250915527,0.0009925803501111216
76376,152753,0,152753,3.0110011100769043,0.000993619383529523
76476,152953,0,152953,3.015742063522339,0.0009939422958839485
76577,153155,0,153155,3.0206520557403564,0.0009937400033900228
76677,153355,0,153355,3.025573968887329,0.000993333947245347
76777,153555,0,153555,3.0303549766540527,0.0009930191276887174
76877,153755,0,153755,3.035099983215332,0.0009929553249342336
76977,153955,0,153955,3.0396909713745117,0.0009931085575488768
77077,154155,0,154155,3.044239044189453,0.0009932554026247482
77177,154355,0,154355,3.0485680103302,0.0009930579273609704
77277,154555,0,154555,3.052454948425293,0.0009921953177591879
77377,154755,0,154755,3.05656099319458,0.0009904933343706597
77477,154955,0,154955,3.0603787899017334,0.000987986631128149
77578,155157,0,155157,3.064196825027466,0.000984864821685105
77678,155357,0,155357,3.0679821968078613,0.00098152361836514
77778,155557,0,155557,3.0717499256134033,0.000978262400855413
77878,155757,0,155757,3.0755231380462646,0.0009752872288474332
77978,155957,0,155957,3.079241991043091,0.0009726040993864001
78078,156157,0,156157,3.082953929901123,0.0009700278403781985
78178,156357,0,156357,3.086671829223633,0.0009672747355840131
78278,156557,0,156557,3.0905117988586426,0.0009640857132585769
78378,156757,0,156757,3.09452486038208,0.0009603297633460427
78478,156957,0,156957,3.0985729694366455,0.0009560642833016454
78579,157159,0,157159,3.10280704498291,0.0009514891482769838
78679,157359,0,157359,3.106834888458252,0.0009470554020773093
78779,157559,0,157559,3.1105690002441406,0.0009430574321662704
78879,157759,0,157759,3.1143438816070557,0.0009396949600593182
78979,157959,0,157959,3.1186230182647705,0.0009369720116275821
79079,158159,0,158159,3.1224520206451416,0.0009347140098899164
79179,158359,0,158359,3.1272079944610596,0.0009326424888329479
79279,158559,0,158559,3.1313509941101074,0.0009304883439525135
79379,158759,0,158759,3.135787010192871,0.0009281090263503995
79479,158959,0,158959,3.1407811641693115,0.0009255554503174779
79580,159161,0,159161,3.1457059383392334,0.0009230294395768686
79680,159361,0,159361,3.150424003601074,0.0009208947919103661
79780,159561,0,159561,3.1550121307373047,0.0009194075756591737
79880,159761,0,159761,3.159976005554199,0.0009187183951992855
79980,159961,0,159961,3.1646862030029297,0.0009187854986979219
80080,160161,0,160161,3.169408082962036,0.0009193832997417783
80180,160361,0,160361,3.174053907394409,0.0009201884760830486
80280,160561,0,160561,3.1789560317993164,0.0009209051308110858
80380,160761,0,160761,3.1837029457092285,0.0009213680167185524
80480,160961,0,160961,3.188443899154663,0.0009215873917321349
80581,161163,0,161163,3.1931920051574707,0.0009217340119056417
80681,161363,0,161363,3.1979010105133057,0.0009220628390283527
80781,161563,0,161563,3.2024898529052734,0.0009228063409379709
80881,161763,0,161763,3.207273006439209,0.0009240631719373771
80981,161963,0,161963,3.2118918895721436,0.0009257487491280232
81081,162163,0,162163,3.216475009918213,0.000927622517548261
81181,162363,0,162363,3.2210397720336914,0.0009293709788256857
81281,162563,0,162563,3.225713014602661,0.0009307099755542141
81381,162763,0,162763,3.230404853820801,0.0009314768072322573
81481,162963,0,162963,3.2349700927734375,0.0009316826100058701
81582,163165,0,163165,3.239313840866089,0.0009314946914512201
81682,163365,0,163365,3.2431271076202393,0.0009311677916317265
81782,163565,0,163565,3.2470779418945312,0.0009309208069065117
81882,163765,0,163765,3.250877857208252,0.000930855875376851
81982,163965,0,163965,3.254654884338379,0.0009309177892654785
82082,164165,0,164165,3.2588889598846436,0.0009309090794040802
82182,164365,0,164365,3.262892007827759,0.0009305599977330671
82282,164565,0,164565,3.2666139602661133,0.0009296327959692951
82382,164765,0,164765,3.270327091217041,0.0009280151744153849
82482,164965,0,164965,3.274229049682617,0.0009257605978534036
82583,165167,0,165167,3.27828311920166,0.0009230369566347484
82683,165367,0,165367,3.282033920288086,0.0009201698537410303
82783,165567,0,165567,3.2857589721679688,0.0009173830743989654
82883,165767,0,165767,3.2896111011505127,0.0009148158098372631
82983,165967,0,165967,3.293401002883911,0.0009124485342667239
83083,166167,0,166167,3.297312021255493,0.000910121211069249
83183,166367,0,166367,3.3010430335998535,0.0009076100957668707
83283,166567,0,166567,3.3047869205474854,0.0009047247322746157
83383,166767,0,166767,3.308932065963745,0.0009013876631708839
83483,166967,0,166967,3.3128609657287598,0.0008976746998178535
83584,167169,0,167169,3.3166520595550537,0.0008937633025923373
83684,167369,0,167369,3.3203771114349365,0.0008900204562466181
83784,167569,0,167569,3.324122190475464,0.0008866637675201256
83884,167769,0,167769,3.3282151222229004,0.0008838301616397827
83984,167969,0,167969,3.331961154937744,0.0008815002681926106
84084,168169,0,168169,3.335679054260254,0.0008795195447258347
84184,168369,0,168369,3.3392961025238037,0.0008776656237199858
84284,168569,0,168569,3.342897891998291,0.0008757410059643323
84384,168769,0,168769,3.3466949462890625,0.0008736589571555772
84484,168969,0,168969,3.3503639698028564,0.0008714845739135534
84585,169171,0,169171,3.3540899753570557,0.0008693919620829593
84685,169371,0,169371,3.3578319549560547,0.0008676723393720726
84785,169571,0,169571,3.361783027648926,0.0008665136985893719
84885,169771,0,169771,3.3653790950775146,0.0008660098678042812
84985,169971,0,169971,3.368966817855835,0.000866100398655721
85085,170171,0,170171,3.372565984725952,0.0008665895062497029
85185,170371,0,170371,3.3761558532714844,0.0008672198387447541
85285,170571,0,170571,3.3797340393066406,0.0008677688736569731
85385,170771,0,170771,3.383322238922119,0.0008681249606959862
85485,170971,0,170971,3.3869152069091797,0.0008683166737615015
85586,171173,0,171173,3.390558958053589,0.0008684935281884914
85686,171373,0,171373,3.394141912460327,0.0008688546805009033
85786,171573,0,171573,3.397726058959961,0.0008695671429942288
85886,171773,0,171773,3.401348114013672,0.0008706834031409542
85986,171973,0,171973,3.4049739837646484,0.0008721124557149325
86086,172173,0,172173,3.408580780029297,0.0008736479217864585
86186,172373,0,172373,3.41231107711792,0.0008750376661399535
86286,172573,0,172573,3.415919780731201,0.0008760665312859014
86386,172773,0,172773,3.419508934020996,0.0008766256973700005
86486,172973,0,172973,3.423097848892212,0.0008767446218802946
86587,173175,0,173175,3.4267420768737793,0.0008765672592557582
86687,173375,0,173375,3.43033504486084,0.0008762946746439859
86787,173575,0,173575,3.434026002883911,0.0008760871494352047
86887,173775,0,173775,3.437623977661133,0.0008760051932431543
86987,173975,0,173975,3.441316843032837,0.0008759833225121085
87087,174175,0,174175,3.4449169635772705,0.000875850885173712
87187,174375,0,174375,3.448606014251709,0.0008753941671112861
87287,174575,0,174575,3.452207088470459,0.0008744384335426315
87387,174775,0,174775,3.455864191055298,0.0008729155540592252
87487,174975,0,174975,3.459537982940674,0.0008708887952690038
87588,175177,0,175177,3.463247060775757,0.0008685040325875125
87688,175377,0,175377,3.466921091079712,0.0008660275022496727
87788,175577,0,175577,3.4705851078033447,0.0008636244374817609
87888,175777,0,175777,3.474250078201294,0.0008613865064298292
87988,175977,0,175977,3.477914810180664,0.00085928019636098
88088,176177,0,176177,3.481600046157837,0.0008571692576980055
88188,176377,0,176377,3.485274076461792,0.000854878682351542
88288,176577,0,176577,3.4889328479766846,0.000852271182995036
88388,176777,0,176777,3.4925949573516846,0.0008493073375937226
88488,176977,0,176977,3.496264934539795,0.0008460706084560198
88589,177179,0,177179,3.499976873397827,0.0008427149705160478
88689,177379,0,177379,3.5036449432373047,0.0008395384075095698
88789,177579,0,177579,3.5073320865631104,0.00083670018619593
88889,177779,0,177779,3.5110280513763428,0.0008342915682834349
88989,177979,0,177979,3.515974998474121,0.0008322796832178614
89089,178179,0,178179,3.519566059112549,0.0008305308718035362
89189,178379,0,178379,3.5232231616973877,0.000828869610054177
89289,178579,0,178579,3.5269041061401367,0.0008271528407871994
89389,178779,0,178779,3.5306010246276855,0.0008253323885796358
89489,178979,0,178979,3.5343050956726074,0.0008234788525828045
89590,179181,0,179181,3.538043975830078,0.0008217404932841114
89690,179381,0,179381,3.5417490005493164,0.0008203490050212823
89790,179581,0,179581,3.5454530715942383,0.0008194398358134963
89890,179781,0,179781,3.549146890640259,0.0008190667545649459
89990,179981,0,179981,3.552845001220703,0.000819161155235075
90090,180181,0,180181,3.5565550327301025,0.0008195555404714558
90190,180381,0,180381,3.560276985168457,0.0008200457185135016
90290,180581,0,180581,3.5639970302581787,0.0008204653412128683
90390,180781,0,180781,3.5677108764648438,0.0008207415490179744
90490,180981,0,180981,3.5714099407196045,0.0008209124895196915
90591,181183,0,181183,3.575134038925171,0.0008211061019937824
90691,181383,0,181383,3.578839063644409,0.0008214759620807018
90791,181583,0,181583,3.5825448036193848,0.0008221399595659456
90891,181783,0,181783,3.586246967315674,0.0008231191307371879
90991,181983,0,181983,3.589940071105957,0.0008243224039541082
91091,182183,0,182183,3.5936269760131836,0.0008255743427610261
91191,182383,0,182383,3.5973260402679443,0.0008266734507235839
91291,182583,0,182583,3.6010079383850098,0.0008274581678295047
91391,182783,0,182783,3.6046981811523438,0.0008278580779419813
91491,182983,0,182983,3.608398199081421,0.0008279119148059469
91592,183185,0,183185,3.612138032913208,0.0008277416370519857
91692,183385,0,183385,3.6158621311187744,0.0008275050550719453
91792,183585,0,183585,3.619542121887207,0.000827317572768543
91892,183785,0,183785,3.6232330799102783,0.0008272103500172629
91992,183985,0,183985,3.6269309520721436,0.000827114862991511
92092,184185,0,184185,3.630617141723633,0.0008268860851503632
92192,184385,0,184385,3.6343259811401367,0.0008263559706830777
92292,184585,0,184585,3.638104200363159,0.0008253976250002553
92392,184785,0,184785,3.641857147216797,0.0008239740481775639
92492,184985,0,184985,3.6455581188201904,0.0008221519837026714
92593,185187,0,185187,3.6492931842803955,0.0008200561295568657
92693,185387,0,185387,3.6530020236968994,0.0008179031625985509
92793,185587,0,185587,3.656705141067505,0.0008158133732980409
92893,185787,0,185787,3.6604931354522705,0.0008138448883398462
92993,185987,0,185987,3.664271116256714,0.0008119577231530521
93093,186187,0,186187,3.668062925338745,0.0008100375084685403
93193,186387,0,186387,3.6717288494110107,0.0008079487361071991
93293,186587,0,186587,3.675189971923828,0.0008055948568062806
93393,186787,0,186787,3.6786530017852783,0.0008029627484150209
93493,186987,0,186987,3.6821041107177734,0.0008001366470948767
93594,187189,0,187189,3.686462879180908,0.0007972478571888059
93694,187389,0,187389,3.6899120807647705,0.0007945378606313771
93794,187589,0,187589,3.6933839321136475,0.0007921216355275383
93894,187789,0,187789,3.6968750953674316,0.000790057632949688
93994,187989,0,187989,3.7003440856933594,0.0007883063933365945
94094,188189,0,188189,3.7038159370422363,0.0007867544387938208
94194,188389,0,188389,3.7082130908966064,0.0007852647036552051
94294,188589,0,188589,3.711786985397339,0.0007837352734987575
94394,188789,0,188789,3.7152321338653564,0.0007821442378403233
94494,188989,0,188989,3.718729019165039,0.0007805621181205609
94595,189191,0,189191,3.722201108932495,0.0007791136019185556
94695,189391,0,189391,3.7256319522857666,0.000777981860183961
94795,189591,0,189591,3.729098081588745,0.0007772622672379343
94895,189791,0,189791,3.7326409816741943,0.0007769808527342268
94995,189991,0,189991,3.7363200187683105,0.0007770674625305682
95095,190191,0,190191,3.7399749755859375,0.0007773804158384673
95195,190391,0,190391,3.7435781955718994,0.0007777583486906501
95295,190591,0,190591,3.747189998626709,0.0007780778384347758
95395,190791,0,190791,3.750783920288086,0.0007782936444075621
95495,190991,0,190991,3.754379987716675,0.0007784475942381758
95596,191193,0,191193,3.758021831512451,0.0007786471756561169
95696,191393,0,191393,3.7616629600524902,0.000779009221887024
95796,191593,0,191593,3.765273094177246,0.0007796149086672052
95896,191793,0,191793,3.768862009048462,0.0007804643279087903
95996,191993,0,191993,3.772447109222412,0.0007814703907463661
96096,192193,0,192193,3.7760329246520996,0.0007824852398633668
96196,192393,0,192393,3.779616117477417,0.000783348813431286
96296,192593,0,192593,3.7832047939300537,0.0007839408649115961
96396,192793,0,192793,3.7867908477783203,0.0007842180605834987
96496,192993,0,192993,3.7904551029205322,0.0007842226028319198
96597,193195,0,193195,3.7940800189971924,0.0007840563959830368
96697,193395,0,193395,3.797691822052002,0.0007838424795929533
96797,193595,0,193595,3.8013648986816406,0.0007836621620644927
96897,193795,0,193795,3.805060863494873,0.0007835264754578041
96997,193995,0,193995,3.808687210083008,0.0007833684471244575
97097,194195,0,194195,3.8122949600219727,0.0007830664764506844
97197,194395,0,194395,3.8159220218658447,0.0007824894867827737
97297,194595,0,194595,3.819537878036499,0.0007815468176617557
97397,194795,0,194795,3.8231379985809326,0.0007802230093839007
97497,194995,0,194995,3.826741933822632,0.0007785840408823177
97598,195197,0,195197,3.83038592338562,0.0007767349951600943
97698,195397,0,195397,3.8339672088623047,0.0007748516070601287
97798,195597,0,195597,3.8375070095062256,0.0007730199539615395
97898,195797,0,195797,3.841040849685669,0.0007712747588061685
97998,195997,0,195997,3.8446099758148193,0.0007695743899653135
98098,196197,0,196197,3.848155975341797,0.0007678241336359563
98198,196397,0,196397,3.8516759872436523,0.0007659203182002026
98298,196597,0,196597,3.8553810119628906,0.0007637972470008317
98398,196797,0,196797,3.859018087387085,0.0007614593832183158
98498,196997,0,196997,3.8626370429992676,0.0007589875075462111
98599,197199,0,197199,3.8663458824157715,0.0007564920287053173
98699,197399,0,197399,3.870007038116455,0.0007541682908846921
98799,197599,0,197599,3.8735969066619873,0.0007520977847984034
98899,197799,0,197799,3.877207040786743,0.0007503157381845929
98999,197999,0,197999,3.8807990550994873,0.0007487807401688889
99099,198199,0,198199,3.884397029876709,0.0007473979239283026
99199,198399,0,198399,3.887993097305298,0.000746061400009243
99299,198599,0,198599,3.8915960788726807,0.0007447001263067465
99399,198799,0,198799,3.8952109813690186,0.000743309665608991
99499,198999,0,198999,3.8988049030303955,0.0007419570167356046
99600,199201,0,199201,3.902611017227173,0.0007407458020672369
99700,199401,0,199401,3.9062609672546387,0.0007398198908731625
99800,199601,0,199601,3.9097659587860107,0.0007392444402055365
99900,199801,0,199801,3.9133970737457275,0.00073902673139159
100000,200001,0,200001,3.9168179035186768,0.0007390990808655018


==> plot_data/quadratic_minimax_problem_n20_alpha00001/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.009506225585938e-05,4.387072431292609
86,173,172,345,0.003930091857910156,0.2868497587704457
172,345,344,689,0.007955074310302734,0.13032929019998057
258,517,516,1033,0.012627124786376953,0.08632160440198876
344,689,688,1377,0.016607999801635742,0.06653322942944
430,861,860,1721,0.02032184600830078,0.05598508680505433
516,1033,1032,2065,0.024190187454223633,0.049585547253792064
602,1205,1204,2409,0.02833390235900879,0.045146781145719156
688,1377,1376,2753,0.03180098533630371,0.041682144259711534
774,1549,1548,3097,0.035269975662231445,0.03880524720209769
859,1719,1718,3437,0.03900790214538574,0.036345075405360576
945,1891,1890,3781,0.04271984100341797,0.034170284662348845
1031,2063,2062,4125,0.04707002639770508,0.03224283000397655
1117,2235,2234,4469,0.05065417289733887,0.03054296362001096
1203,2407,2406,4813,0.05423617362976074,0.029035296497065512
1289,2579,2578,5157,0.0582270622253418,0.027703106104165674
1375,2751,2750,5501,0.06169891357421875,0.02651442001967155
1461,2923,2922,5845,0.06516909599304199,0.02546101013882364
1547,3095,3094,6189,0.06864094734191895,0.024523010892009242
1633,3267,3266,6533,0.07217097282409668,0.023687346846406998
1719,3439,3438,6877,0.07585000991821289,0.022934052511305033
1805,3611,3610,7221,0.07942390441894531,0.022257869853309322
1891,3783,3782,7565,0.08297204971313477,0.021648462171941926
1977,3955,3954,7909,0.08651900291442871,0.021095497758925386
2063,4127,4126,8253,0.09007906913757324,0.020587438174011014
2149,4299,4298,8597,0.09393811225891113,0.020121465143950207
2235,4471,4470,8941,0.09759306907653809,0.019693562108026922
2321,4643,4642,9285,0.10183215141296387,0.019417368101809336
2407,4815,4814,9629,0.1062021255493164,0.019172183674350887
2492,4985,4984,9969,0.110382080078125,0.018921408268011784
2578,5157,5156,10313,0.11466789245605469,0.018657797857788646
2664,5329,5328,10657,0.11889195442199707,0.018402733495413853
2750,5501,5500,11001,0.12312102317810059,0.01814994244276452
2836,5673,5672,11345,0.12734603881835938,0.017887781919273416
2922,5845,5844,11689,0.1315901279449463,0.01763123858693001
3008,6017,6016,12033,0.1358950138092041,0.017362972320279106
3094,6189,6188,12377,0.14022207260131836,0.017101644176899133
3180,6361,6360,12721,0.14444303512573242,0.016838588007872475
3266,6533,6532,13065,0.14866304397583008,0.016577476525197324
3352,6705,6704,13409,0.15288496017456055,0.016308887663902285
3438,6877,6876,13753,0.15709710121154785,0.016048883260889657
3524,7049,7048,14097,0.16128921508789062,0.01578802292883813
3610,7221,7220,14441,0.16549205780029297,0.015527102971734942
3696,7393,7392,14785,0.1699061393737793,0.01527411001660001
3782,7565,7564,15129,0.17411303520202637,0.015041641676480944
3868,7737,7736,15473,0.17849493026733398,0.01481386172826168
3954,7909,7908,15817,0.18279314041137695,0.014587650653174493
4040,8081,8080,16161,0.18729901313781738,0.014368607038927466
4126,8253,8252,16505,0.19205904006958008,0.0141532462235422
4211,8423,8422,16845,0.19628000259399414,0.01394315930989325
4297,8595,8594,17189,0.20074987411499023,0.013733178164384716
4383,8767,8766,17533,0.20523500442504883,0.013529112474474369
4469,8939,8938,17877,0.20960497856140137,0.013328034900586556
4555,9111,9110,18221,0.21406102180480957,0.013128264427076005
4641,9283,9282,18565,0.21834588050842285,0.012932727260469538
4727,9455,9454,18909,0.22298216819763184,0.012741426784731535
4813,9627,9626,19253,0.22726893424987793,0.012552387467496073
4899,9799,9798,19597,0.23152494430541992,0.012364675018864197
4985,9971,9970,19941,0.23579001426696777,0.01218181838159426
5071,10143,10142,20285,0.24007320404052734,0.01200201492049166
5157,10315,10314,20629,0.24436712265014648,0.011823540354613851
5243,10487,10486,20973,0.24918699264526367,0.011647503178281398
5329,10659,10658,21317,0.2534492015838623,0.01147586158459793
5415,10831,10830,21661,0.2577230930328369,0.011306427707025913
5501,11003,11002,22005,0.26198601722717285,0.011137946778624805
5587,11175,11174,22349,0.266247034072876,0.010972971369030343
5673,11347,11346,22693,0.2705068588256836,0.0108114814781856
5759,11519,11518,23037,0.2746610641479492,0.010651404932836506
5844,11689,11688,23377,0.2787590026855469,0.01049458181460958
5930,11861,11860,23721,0.2832369804382324,0.010339778396450401
6016,12033,12032,24065,0.2873971462249756,0.010187543338711493
6102,12205,12204,24409,0.29154181480407715,0.010036187324563626
6188,12377,12376,24753,0.29570817947387695,0.00988711950530088
6274,12549,12548,25097,0.299854040145874,0.009741653602306147
6360,12721,12720,25441,0.3040039539337158,0.009597882629587688
6446,12893,12892,25785,0.30814290046691895,0.009454996966850584
6532,13065,13064,26129,0.3123340606689453,0.009315129508769995
6618,13237,13236,26473,0.3164830207824707,0.0091781738174004
6704,13409,13408,26817,0.32077503204345703,0.009042217853600898
6790,13581,13580,27161,0.324998140335083,0.008907677551006144
6876,13753,13752,27505,0.3291490077972412,0.00877639749663704
6962,13925,13924,27849,0.33329081535339355,0.008647187287500677
7048,14097,14096,28193,0.3374509811401367,0.008518664510319511
7134,14269,14268,28537,0.34158802032470703,0.008392267355285886
7220,14441,14440,28881,0.3458220958709717,0.008268865659837105
7306,14613,14612,29225,0.3503420352935791,0.008146744005682417
7392,14785,14784,29569,0.3548240661621094,0.008025477935800333
7477,14955,14954,29909,0.35919809341430664,0.00790822083262498
7563,15127,15126,30253,0.3633692264556885,0.007791966187910349
7649,15299,15298,30597,0.3675239086151123,0.007676460165076236
7735,15471,15470,30941,0.3717038631439209,0.007562300686922235
7821,15643,15642,31285,0.3763291835784912,0.007450910158378703
7907,15815,15814,31629,0.3805501461029053,0.007341170771810391
7993,15987,15986,31973,0.3847029209136963,0.007232015278268057
8079,16159,16158,32317,0.3889460563659668,0.00712478263038193
8165,16331,16330,32661,0.39311718940734863,0.007020047977364422
8251,16503,16502,33005,0.39734601974487305,0.006916293890489678
8337,16675,16674,33349,0.40151309967041016,0.006813350702344683
8423,16847,16846,33693,0.4058709144592285,0.006712715350760621
8509,17019,17018,34037,0.41003990173339844,0.006614018642986916
8595,17191,17190,34381,0.4142019748687744,0.0065158954292452425
8681,17363,17362,34725,0.41837310791015625,0.006419046402364501
8767,17535,17534,35069,0.4225449562072754,0.0063245519056610005
8853,17707,17706,35413,0.42670702934265137,0.006231341633729837
8939,17879,17878,35757,0.43085789680480957,0.006138651602685907
9025,18051,18050,36101,0.43498897552490234,0.006047704179447483
9110,18221,18220,36441,0.4390869140625,0.0059598451948832225
9196,18393,18392,36785,0.4432239532470703,0.00587169522507658
9282,18565,18564,37129,0.44746899604797363,0.005784309226104578
9368,18737,18736,37473,0.4517951011657715,0.005698931172562657
9454,18909,18908,37817,0.45615291595458984,0.005615117610524657
9540,19081,19080,38161,0.4603290557861328,0.005531762059042106
9626,19253,19252,38505,0.46448612213134766,0.005449581471700116
9712,19425,19424,38849,0.46864914894104004,0.005369394941756801
9798,19597,19596,39193,0.47278714179992676,0.005290212291516575
9884,19769,19768,39537,0.47684288024902344,0.005211500709606557
9970,19941,19940,39881,0.48090100288391113,0.0051343434991668845
10056,20113,20112,40225,0.4849510192871094,0.005058886888022648
10142,20285,20284,40569,0.4890449047088623,0.004983998328052962
10228,20457,20456,40913,0.493319034576416,0.004909838751653631
10314,20629,20628,41257,0.497377872467041,0.004837424706467703
10400,20801,20800,41601,0.5014450550079346,0.004766250328787064
10486,20973,20972,41945,0.5055241584777832,0.004695449196591222
10572,21145,21144,42289,0.5096738338470459,0.004625737164106255
10658,21317,21316,42633,0.5139648914337158,0.004557703650000855
10743,21487,21486,42973,0.5180630683898926,0.004491220208653245
10829,21659,21658,43317,0.5222170352935791,0.004424384140809679
10915,21831,21830,43661,0.5263779163360596,0.0043589271431272334
11001,22003,22002,44005,0.5305378437042236,0.004294864458747394
11087,22175,22174,44349,0.5346920490264893,0.004231240652507796
11173,22347,22346,44693,0.5388588905334473,0.004168297771068796
11259,22519,22518,45037,0.5429520606994629,0.004106859217038733
11345,22691,22690,45381,0.5471220016479492,0.0040464068625680975
11431,22863,22862,45725,0.5512990951538086,0.0039862692959178
11517,23035,23034,46069,0.5554690361022949,0.003927121796689074
11603,23207,23206,46413,0.5596890449523926,0.0038693811495276336
11689,23379,23378,46757,0.56386399269104,0.0038122349065508373
11775,23551,23550,47101,0.5679349899291992,0.0037554968647981702
11861,23723,23722,47445,0.572105884552002,0.0036999830955663053
11947,23895,23894,47789,0.5763108730316162,0.0036455970370553297
12033,24067,24066,48133,0.5805401802062988,0.003591548137706487
12119,24239,24238,48477,0.58473801612854,0.003538142551957953
12205,24411,24410,48821,0.5889120101928711,0.0034860281025527995
12291,24583,24582,49165,0.5930819511413574,0.003434682977136378
12377,24755,24754,49509,0.5985698699951172,0.0033836111993406732
12462,24925,24924,49849,0.6027770042419434,0.0033340194622823068
12548,25097,25096,50193,0.6071100234985352,0.003285010635203608
12634,25269,25268,50537,0.6110739707946777,0.003236460173267882
12720,25441,25440,50881,0.6150569915771484,0.003188290985784137
12806,25613,25612,51225,0.6189858913421631,0.0031411954242293273
12892,25785,25784,51569,0.6235759258270264,0.0030950131709430242
12978,25957,25956,51913,0.6276509761810303,0.003049097206707865
13064,26129,26128,52257,0.6316251754760742,0.0030037762713220444
13150,26301,26300,52601,0.6355249881744385,0.0029595559159279593
13236,26473,26472,52945,0.6396441459655762,0.002915939996902421
13322,26645,26644,53289,0.6438539028167725,0.002872566688701584
13408,26817,26816,53633,0.6480391025543213,0.002830005108068641
13494,26989,26988,53977,0.6524121761322021,0.002788412107710217
13580,27161,27160,54321,0.6565830707550049,0.002747166018918603
13666,27333,27332,54665,0.6607010364532471,0.002706282787315864
13752,27505,27504,55009,0.6647839546203613,0.002666339906545504
13838,27677,27676,55353,0.6689000129699707,0.0026271254139762505
13924,27849,27848,55697,0.6730148792266846,0.0025881233580337683
14010,28021,28020,56041,0.6771280765533447,0.002549676250010603
14095,28191,28190,56381,0.6812000274658203,0.002512593170729847
14181,28363,28362,56725,0.6854848861694336,0.0024755412385839377
14267,28535,28534,57069,0.6895980834960938,0.0024387087350410193
14353,28707,28706,57413,0.6938128471374512,0.0024026009073280477
14439,28879,28878,57757,0.6979260444641113,0.0023672914784470082
14525,29051,29050,58101,0.7025902271270752,0.002332249370139559
14611,29223,29222,58445,0.7073628902435303,0.002297546765900458
14697,29395,29394,58789,0.7115039825439453,0.002263659340200623
14783,29567,29566,59133,0.7156620025634766,0.0022303545836092013
14869,29739,29738,59477,0.719886064529419,0.0021972246457266204
14955,29911,29910,59821,0.7240941524505615,0.0021646021212277703
15041,30083,30082,60165,0.7284641265869141,0.002132765370108523
15127,30255,30254,60509,0.7327210903167725,0.0021012899536920603
15213,30427,30426,60853,0.7373909950256348,0.002070018894887582
15299,30599,30598,61197,0.7417058944702148,0.00203939585741918
15385,30771,30770,61541,0.7461040019989014,0.0020094229147547757
15471,30943,30942,61885,0.7503242492675781,0.0019796532848930758
15557,31115,31114,62229,0.7545859813690186,0.0019502055952506764
15643,31287,31286,62573,0.7588231563568115,0.0019214624765181093
15728,31457,31456,62913,0.7629599571228027,0.0018935059097175263
15814,31629,31628,63257,0.7671389579772949,0.0018653656037302048
15900,31801,31800,63601,0.7713460922241211,0.0018376866622826565
15986,31973,31972,63945,0.7755370140075684,0.0018106666193886943
16072,32145,32144,64289,0.7797238826751709,0.0017839261736516674
16158,32317,32316,64633,0.7839100360870361,0.0017573754472919039
16244,32489,32488,64977,0.7880969047546387,0.0017313963457822378
16330,32661,32660,65321,0.7922680377960205,0.0017059468597698157
16416,32833,32832,65665,0.7965888977050781,0.0016806559921501232
16502,33005,33004,66009,0.8007850646972656,0.0016556643497731148
16588,33177,33176,66353,0.8050401210784912,0.001631276594265418
16674,33349,33348,66697,0.8092231750488281,0.0016072508079231177
16760,33521,33520,67041,0.8133900165557861,0.0015833528726454885
16846,33693,33692,67385,0.8175849914550781,0.0015598763240507014
16932,33865,33864,67729,0.8218059539794922,0.0015369472329154765
17018,34037,34036,68073,0.8260698318481445,0.0015142301493565745
17104,34209,34208,68417,0.8306601047515869,0.0014916933086761327
17190,34381,34380,68761,0.8348419666290283,0.0014696604614666201
17276,34553,34552,69105,0.8390209674835205,0.0014480527166614644
17361,34723,34722,69445,0.8431930541992188,0.001426817455733807
17447,34895,34894,69789,0.8474001884460449,0.001405609075854444
17533,35067,35066,70133,0.8516309261322021,0.0013849156093619593
17619,35239,35238,70477,0.8558170795440674,0.001364506585931345
17705,35411,35410,70821,0.8599982261657715,0.0013442108651718445
17791,35583,35582,71165,0.8641698360443115,0.0013242936069577402
17877,35755,35754,71509,0.8684360980987549,0.0013048301800883857
17963,35927,35926,71853,0.8726928234100342,0.0012855299642334644
18049,36099,36098,72197,0.876690149307251,0.0012663984539297401
18135,36271,36270,72541,0.8806519508361816,0.0012477063538433985
18221,36443,36442,72885,0.8847651481628418,0.0012293564118769091
18307,36615,36614,73229,0.8887760639190674,0.001211106027501486
18393,36787,36786,73573,0.8928799629211426,0.0011931139439951507
18479,36959,36958,73917,0.8970668315887451,0.0011755583876097867
18565,37131,37130,74261,0.9012079238891602,0.0011582218978856964
18651,37303,37302,74605,0.905203104019165,0.0011409889784705976
18737,37475,37474,74949,0.9092891216278076,0.0011240968055880435
18823,37647,37646,75293,0.9134249687194824,0.0011075767381814765
18909,37819,37818,75637,0.9174399375915527,0.0010911803926775853
18994,37989,37988,75977,0.9213931560516357,0.0010751312942456133
19080,38161,38160,76321,0.9260830879211426,0.0010592729781472806
19166,38333,38332,76665,0.9317290782928467,0.0010436885102697215
19252,38505,38504,77009,0.9368801116943359,0.0010281858720452006
19338,38677,38676,77353,0.9418621063232422,0.0010129195017940175
19424,38849,38848,77697,0.9473249912261963,0.0009980211880464475
19510,39021,39020,78041,0.9518561363220215,0.0009832931482255801
19596,39193,39192,78385,0.9569690227508545,0.0009686602787933046
19682,39365,39364,78729,0.9615190029144287,0.0009543297434186621
19768,39537,39536,79073,0.9657180309295654,0.0009403040886179995
19854,39709,39708,79417,0.969688892364502,0.0009263741508055436
19940,39881,39880,79761,0.9741439819335938,0.0009125940071025121
20026,40053,40052,80105,0.978665828704834,0.0008991432442850173
20112,40225,40224,80449,0.9828178882598877,0.000885907696836284
20198,40397,40396,80793,0.9870529174804688,0.0008727410207703236
20284,40569,40568,81137,0.9913160800933838,0.0008597917363941337
20370,40741,40740,81481,0.9957249164581299,0.0008471503120180681
20456,40913,40912,81825,1.0001890659332275,0.0008346384509959169
20542,41085,41084,82169,1.0047409534454346,0.0008222162697720637
20628,41257,41256,82513,1.0093491077423096,0.0008100625224006755
20713,41427,41426,82853,1.0138778686523438,0.000798293379316805
20799,41599,41598,83197,1.018463134765625,0.0007864591076304904
20885,41771,41770,83541,1.0231311321258545,0.0007747640836662422
20971,41943,41942,83885,1.0278050899505615,0.0007633514896509858
21057,42115,42114,84229,1.0324749946594238,0.0007521090316510449
21143,42287,42286,84573,1.037165880203247,0.000740926172232646
21229,42459,42458,84917,1.0419330596923828,0.0007299397421287687
21315,42631,42630,85261,1.0467791557312012,0.000719209972165391
21401,42803,42802,85605,1.0515649318695068,0.0007085801271039753
21487,42975,42974,85949,1.0564088821411133,0.0006980340554833696
21573,43147,43146,86293,1.061187982559204,0.0006877233459234417
21659,43319,43318,86637,1.0662260055541992,0.0006776122684189515
21745,43491,43490,86981,1.0709989070892334,0.0006675594015334395
21831,43663,43662,87325,1.0756940841674805,0.0006576372690157614
21917,43835,43834,87669,1.0804839134216309,0.0006479560431649065
22003,44007,44006,88013,1.0852241516113281,0.0006384066721074695
22089,44179,44178,88357,1.0899250507354736,0.0006289105777541214
22175,44351,44350,88701,1.0945179462432861,0.000619592603102619
22261,44523,44522,89045,1.0990879535675049,0.0006104863978389804
22346,44693,44692,89385,1.103600025177002,0.0006015604751864536
22432,44865,44864,89729,1.1083040237426758,0.0005926079075377935
22518,45037,45036,90073,1.1129930019378662,0.0005838606023143588
22604,45209,45208,90417,1.11759614944458,0.0005752740165147019
22690,45381,45380,90761,1.1221611499786377,0.0005667342254203769
22776,45553,45552,91105,1.1267340183258057,0.0005583147063076032
22862,45725,45724,91449,1.1314799785614014,0.0005500994341510182
22948,45897,45896,91793,1.136225938796997,0.0005419871706661015
23034,46069,46068,92137,1.140820026397705,0.0005339231138922232
23120,46241,46240,92481,1.145495891571045,0.0005260180410559427
23206,46413,46412,92825,1.1501359939575195,0.000518287500825606
23292,46585,46584,93169,1.1547009944915771,0.0005106151920184472
23378,46757,46756,93513,1.159369945526123,0.000503017485719737
23464,46929,46928,93857,1.1639540195465088,0.0004955984338883548
23550,47101,47100,94201,1.1685240268707275,0.0004883066773896462
23636,47273,47272,94545,1.1731081008911133,0.00048105317247861863
23722,47445,47444,94889,1.1777069568634033,0.0004739110727562024
23808,47617,47616,95233,1.1823348999023438,0.00046694094080637665
23894,47789,47788,95577,1.1869020462036133,0.00046004965388862925
23979,47959,47958,95917,1.191478967666626,0.0004532822610455747
24065,48131,48130,96261,1.196146011352539,0.0004465759450851923
24151,48303,48302,96605,1.2007231712341309,0.000440012699951178
24237,48475,48474,96949,1.205265998840332,0.00043349449923602636
24323,48647,48646,97293,1.2098159790039062,0.00042704592661497857
24409,48819,48818,97637,1.2148499488830566,0.00042075138744751214
24495,48991,48990,97981,1.2194249629974365,0.0004145580837440585
24581,49163,49162,98325,1.2240180969238281,0.00040839704694045696
24667,49335,49334,98669,1.228632926940918,0.00040233728258456036
24753,49507,49506,99013,1.2332251071929932,0.00039642167591287834
24839,49679,49678,99357,1.2377760410308838,0.00039056706307268686
24925,49851,49850,99701,1.242387056350708,0.0003847541849403505
25011,50023,50022,100045,1.2465908527374268,0.0003790666234591592
25097,50195,50194,100389,1.2507619857788086,0.0003734947471600937
25183,50367,50366,100733,1.2549059391021729,0.00036795744836016234
25269,50539,50538,101077,1.2590539455413818,0.0003624859099159946
25355,50711,50710,101421,1.263207197189331,0.0003571466428954446
25441,50883,50882,101765,1.2673461437225342,0.0003518863779935303
25527,51055,51054,102109,1.2714810371398926,0.00034665411227627227
25612,51225,51224,102449,1.2754788398742676,0.00034157339593042415
25698,51397,51396,102793,1.2795171737670898,0.0003365523801120308
25784,51569,51568,103137,1.2835619449615479,0.00033157840176962957
25870,51741,51740,103481,1.2875900268554688,0.00032664339028418886
25956,51913,51912,103825,1.2916340827941895,0.00032181830084266065
26042,52085,52084,104169,1.295665979385376,0.00031708691481147435
26128,52257,52256,104513,1.299712896347046,0.0003123828388058109
26214,52429,52428,104857,1.3037941455841064,0.0003077395903101878
26300,52601,52600,105201,1.3078711032867432,0.000303209107780399
26386,52773,52772,105545,1.3119258880615234,0.0002987407012144213
26472,52945,52944,105889,1.316011905670166,0.00029429713554051626
26558,53117,53116,106233,1.3200480937957764,0.00028993661245456316
26644,53289,53288,106577,1.3242111206054688,0.0002856753684455206
26730,53461,53460,106921,1.3284058570861816,0.00028144974645986687
26816,53633,53632,107265,1.332564115524292,0.00027726122435001724
26902,53805,53804,107609,1.3366801738739014,0.0002731689792783883
26988,53977,53976,107953,1.3407959938049316,0.0002691514445633689
27074,54149,54148,108297,1.345024824142456,0.00026515567382098517
27160,54321,54320,108641,1.349259853363037,0.000261216650180326
27245,54491,54490,108981,1.3533329963684082,0.0002574173877440626
27331,54663,54662,109325,1.3575100898742676,0.0002536214604679812
27417,54835,54834,109669,1.3618800640106201,0.0002498479913891673
27503,55007,55006,110013,1.3661110401153564,0.00024614866956180223
27589,55179,55178,110357,1.370300054550171,0.0002425311892532004
27675,55351,55350,110701,1.3745050430297852,0.00023894115358455144
27761,55523,55522,111045,1.3786919116973877,0.0002353858267478034
27847,55695,55694,111389,1.3828890323638916,0.00023191397602624644
27933,55867,55866,111733,1.3870420455932617,0.000228501899861128
28019,56039,56038,112077,1.3913559913635254,0.00022510772408899013
28105,56211,56210,112421,1.3956210613250732,0.0002217654412464072
28191,56383,56382,112765,1.399975061416626,0.00021850370055519374
28277,56555,56554,113109,1.404306173324585,0.00021527907687030146
28363,56727,56726,113453,1.4086549282073975,0.0002120753435403348
28449,56899,56898,113797,1.4129829406738281,0.00020893792835379238
28535,57071,57070,114141,1.4172930717468262,0.0002058671835755237
28621,57243,57242,114485,1.4216029644012451,0.00020281732871140374
28707,57415,57414,114829,1.4259159564971924,0.00019980039006669165
28793,57587,57586,115173,1.4302220344543457,0.00019685559941080217
28879,57759,57758,115517,1.4345719814300537,0.000193957801084495
28964,57929,57928,115857,1.4388010501861572,0.0001911084462638326
29050,58101,58100,116201,1.4430460929870605,0.00018827264695451453
29136,58273,58272,116545,1.447378158569336,0.00018550439469113933
29222,58445,58444,116889,1.4517788887023926,0.00018276486887027475
29308,58617,58616,117233,1.456169843673706,0.00018004473588478022
29394,58789,58788,117577,1.4605181217193604,0.00017738310929967286
29480,58961,58960,117921,1.4648411273956299,0.00017477580071856478
29566,59133,59132,118265,1.469188928604126,0.0001721847850031262
29652,59305,59304,118609,1.4735260009765625,0.00016962436506255817
29738,59477,59476,118953,1.4779679775238037,0.00016712579142907043
29824,59649,59648,119297,1.4823431968688965,0.0001646643540578786
29910,59821,59820,119641,1.486694097518921,0.0001622159980690703
29996,59993,59992,119985,1.4910991191864014,0.00015981075512621327
30082,60165,60164,120329,1.4956729412078857,0.0001574616350230963
30168,60337,60336,120673,1.500175952911377,0.00015513428416482508
30254,60509,60508,121017,1.5047600269317627,0.00015282534617115558
30340,60681,60680,121361,1.509263038635254,0.0001505680103093439
30426,60853,60852,121705,1.5137948989868164,0.00014835429502618424
30512,61025,61024,122049,1.5182392597198486,0.00014615328113752615
30597,61195,61194,122389,1.522507905960083,0.0001440059673038253
30683,61367,61366,122733,1.5268042087554932,0.0001418858818719644
30769,61539,61538,123077,1.5310490131378174,0.000139794982111015
30855,61711,61710,123421,1.535581111907959,0.00013771566800297645
30941,61883,61882,123765,1.5398361682891846,0.00013567508085086328
31027,62055,62054,124109,1.5444068908691406,0.00013368102734691114
31113,62227,62226,124453,1.5490880012512207,0.0001317037348863373
31199,62399,62398,124797,1.553415060043335,0.00012974367820158203
31285,62571,62570,125141,1.5580651760101318,0.0001278286161480512
31371,62743,62742,125485,1.5637600421905518,0.00012594866772470706
31457,62915,62914,125829,1.5680181980133057,0.00012407894008885568
31543,63087,63086,126173,1.5725128650665283,0.00012223562471463126
31629,63259,63258,126517,1.5768139362335205,0.00012043702768977838
31715,63431,63430,126861,1.5817959308624268,0.00011866091680611881
31801,63603,63602,127205,1.5870380401611328,0.00011689540200436957
31887,63775,63774,127549,1.5926849842071533,0.000115164757577621
31973,63947,63946,127893,1.5985801219940186,0.00011347226024054985
32059,64119,64118,128237,1.604067087173462,0.00011179245862063107
32145,64291,64290,128581,1.6096460819244385,0.00011012906250855806
32230,64461,64460,128921,1.6150829792022705,0.0001085234524122863
32316,64633,64632,129265,1.6205217838287354,0.00010692682983038258
32402,64805,64804,129609,1.6258659362792969,0.00010533860387139698
32488,64977,64976,129953,1.6310780048370361,0.00010377454064005074
32574,65149,65148,130297,1.6361849308013916,0.00010224818513428412
32660,65321,65320,130641,1.6406819820404053,0.00010073930746994355
32746,65493,65492,130985,1.6449670791625977,9.924016194913382e-05
32832,65665,65664,131329,1.6497409343719482,9.777196061038674e-05
32918,65837,65836,131673,1.6545050144195557,9.633502061207089e-05
33004,66009,66008,132017,1.6589438915252686,9.490790118193469e-05
33090,66181,66180,132361,1.6634211540222168,9.349608966011154e-05
33176,66353,66352,132705,1.667593240737915,9.21180197373169e-05
33262,66525,66524,133049,1.6718719005584717,9.076204433342098e-05
33348,66697,66696,133393,1.6761610507965088,8.941312507459291e-05
33434,66869,66868,133737,1.680422067642212,8.808643938394933e-05
33520,67041,67040,134081,1.6846938133239746,8.679130621036814e-05
33606,67213,67212,134425,1.6889400482177734,8.550948251911404e-05
33692,67385,67384,134769,1.6933040618896484,8.423683098066127e-05
33778,67557,67556,135113,1.6978578567504883,8.299165358082923e-05
33863,67727,67726,135453,1.7024359703063965,8.178589019555024e-05
33949,67899,67898,135797,1.7071049213409424,8.057347103075928e-05
34035,68071,68070,136141,1.7117640972137451,7.937528378257008e-05
34121,68243,68242,136485,1.716614007949829,7.820603229035305e-05
34207,68415,68414,136829,1.7210149765014648,7.70542507126082e-05
34293,68587,68586,137173,1.725532054901123,7.590857275817595e-05
34379,68759,68758,137517,1.7304019927978516,7.478298734340383e-05
34465,68931,68930,137861,1.735079050064087,7.36837087504785e-05
34551,69103,69102,138205,1.7403271198272705,7.259469475049524e-05
34637,69275,69274,138549,1.746056079864502,7.151424724146544e-05
34723,69447,69446,138893,1.7517759799957275,7.045789237003418e-05
34809,69619,69618,139237,1.7570960521697998,6.942200848288173e-05
34895,69791,69790,139581,1.7626028060913086,6.839209308285446e-05
34981,69963,69962,139925,1.7677550315856934,6.73755448689287e-05
35067,70135,70134,140269,1.772508144378662,6.638368016748637e-05
35153,70307,70306,140613,1.7768738269805908,6.540535157596749e-05
35239,70479,70478,140957,1.7817890644073486,6.443247004108123e-05
35325,70651,70650,141301,1.7859618663787842,6.347781310836264e-05
35411,70823,70822,141645,1.790315866470337,6.254487174899817e-05
35497,70995,70994,141989,1.7948682308197021,6.161969598850463e-05
35582,71165,71164,142329,1.7998790740966797,6.071323911077984e-05
35668,71337,71336,142673,1.8048980236053467,5.981705787083369e-05
35754,71509,71508,143017,1.8096449375152588,5.8937359798336586e-05
35840,71681,71680,143361,1.8146798610687256,5.8062456854623936e-05
35926,71853,71852,143705,1.8193190097808838,5.719985271334703e-05
36012,72025,72024,144049,1.8236970901489258,5.635817953017027e-05
36098,72197,72196,144393,1.8283019065856934,5.552708358351253e-05
36184,72369,72368,144737,1.8327021598815918,5.470091517882833e-05
36270,72541,72540,145081,1.8368799686431885,5.389101557122807e-05
36356,72713,72712,145425,1.841158151626587,5.309901490973782e-05
36442,72885,72884,145769,1.846200942993164,5.231299886233082e-05
36528,73057,73056,146113,1.850682020187378,5.153460931439487e-05
36614,73229,73228,146457,1.8549840450286865,5.077451161246858e-05
36700,73401,73400,146801,1.8594379425048828,5.002747213092712e-05
36786,73573,73572,147145,1.864603042602539,4.9284354007641924e-05
36872,73745,73744,147489,1.8689000606536865,4.855263077511301e-05
36958,73917,73916,147833,1.8731560707092285,4.783852850501658e-05
37044,74089,74088,148177,1.8774409294128418,4.71325185116135e-05
37130,74261,74260,148521,1.882030963897705,4.643110068238969e-05
37215,74431,74430,148861,1.8862318992614746,4.575210262874361e-05
37301,74603,74602,149205,1.8905272483825684,4.507969415669968e-05
37387,74775,74774,149549,1.8950860500335693,4.441191458506197e-05
37473,74947,74946,149893,1.8996069431304932,4.375125353345036e-05
37559,75119,75118,150237,1.9045448303222656,4.310636520279342e-05
37645,75291,75290,150581,1.9091439247131348,4.2471862515674544e-05
37731,75463,75462,150925,1.9134409427642822,4.184066503592703e-05
37817,75635,75634,151269,1.9180450439453125,4.121982734813917e-05
37903,75807,75806,151613,1.9223690032958984,4.061376370211291e-05
37989,75979,75978,151957,1.9266560077667236,4.001396098963343e-05
38075,76151,76150,152301,1.930945873260498,3.941842168310659e-05
38161,76323,76322,152645,1.9352309703826904,3.8835711686335444e-05
38247,76495,76494,152989,1.939518928527832,3.82648704959913e-05
38333,76667,76666,153333,1.9438130855560303,3.7697580494257353e-05
38419,76839,76838,153677,1.9481329917907715,3.7137012173231695e-05
38505,77011,77010,154021,1.9524450302124023,3.658999222928708e-05
38591,77183,77182,154365,1.956800937652588,3.605108204933596e-05
38677,77355,77354,154709,1.9612131118774414,3.5515040707859434e-05
38763,77527,77526,155053,1.965501070022583,3.498846043069788e-05
38848,77697,77696,155393,1.9697189331054688,3.448009819991181e-05
38934,77869,77868,155737,1.973963975906372,3.397051652556742e-05
39020,78041,78040,156081,1.978896141052246,3.346491542640307e-05
39106,78213,78212,156425,1.9830381870269775,3.297056907412223e-05
39192,78385,78384,156769,1.9871830940246582,3.248583782220024e-05
39278,78557,78556,157113,1.9913971424102783,3.200391088966711e-05
39364,78729,78728,157457,1.9956209659576416,3.1528202432385715e-05
39450,78901,78900,157801,1.9998021125793457,3.106404534277506e-05
39536,79073,79072,158145,2.003955125808716,3.060626079247855e-05
39622,79245,79244,158489,2.008092164993286,3.0151019814877983e-05
39708,79417,79416,158833,2.012255907058716,2.970427531377726e-05
39794,79589,79588,159177,2.016361951828003,2.9267706119114812e-05
39880,79761,79760,159521,2.020500898361206,2.8834792763700906e-05
39966,79933,79932,159865,2.0246810913085938,2.840567072761419e-05
40052,80105,80104,160209,2.028964042663574,2.798640792263026e-05
40138,80277,80276,160553,2.0331790447235107,2.757481092565292e-05
40224,80449,80448,160897,2.0373940467834473,2.716544490000795e-05
40310,80621,80620,161241,2.0416100025177,2.6761880770991175e-05
40396,80793,80792,161585,2.045837879180908,2.6368107487178306e-05
40481,80963,80962,161925,2.050105094909668,2.598375456593364e-05
40567,81135,81134,162269,2.0543370246887207,2.5597163309410875e-05
40653,81307,81306,162613,2.0587282180786133,2.5218159503550513e-05
40739,81479,81478,162957,2.0629348754882812,2.4847545100435236e-05
40825,81651,81650,163301,2.067134141921997,2.447974692544335e-05
40911,81823,81822,163645,2.071337938308716,2.411549571699214e-05
40997,81995,81994,163989,2.0755701065063477,2.3759794228839994e-05
41083,82167,82166,164333,2.0798051357269287,2.3410227394899664e-05
41169,82339,82338,164677,2.0840070247650146,2.306249479144541e-05
41255,82511,82510,165021,2.0882091522216797,2.2720068618989254e-05
41341,82683,82682,165365,2.0924201011657715,2.2385897083742326e-05
41427,82855,82854,165709,2.0966389179229736,2.205553862533701e-05
41513,83027,83026,166053,2.1009440422058105,2.1727317206850885e-05
41599,83199,83198,166397,2.105232000350952,2.1405882316652922e-05
41685,83371,83370,166741,2.1095120906829834,2.109128257499854e-05
41771,83543,83542,167085,2.1137351989746094,2.077882736697973e-05
41857,83715,83714,167429,2.117950201034546,2.0469737473461178e-05
41943,83887,83886,167773,2.122215986251831,2.0168036727199977e-05
42029,84059,84058,168117,2.1264538764953613,1.987115736066685e-05
42114,84229,84228,168457,2.130622148513794,1.9579237063370162e-05
42200,84401,84400,168801,2.134882926940918,1.928870178618181e-05
42286,84573,84572,169145,2.1391031742095947,1.90050898543715e-05
42372,84745,84744,169489,2.143404960632324,1.872442923603327e-05
42458,84917,84916,169833,2.1474931240081787,1.8445752036728972e-05
42544,85089,85088,170177,2.1516408920288086,1.8173062732124407e-05
42630,85261,85260,170521,2.155764102935791,1.790594269184106e-05
42716,85433,85432,170865,2.159848213195801,1.7640494560195586e-05
42802,85605,85604,171209,2.1639490127563477,1.73781746330066e-05
42888,85777,85776,171553,2.168199062347412,1.712218988332349e-05
42974,85949,85948,171897,2.172212839126587,1.6870016056123874e-05
43060,86121,86120,172241,2.176248073577881,1.6619180104599506e-05
43146,86293,86292,172585,2.1806671619415283,1.6372754794858026e-05
43232,86465,86464,172929,2.1852450370788574,1.613208385588255e-05
43318,86637,86636,173273,2.18973708152771,1.5893649736778355e-05
43404,86809,86808,173617,2.1939618587493896,1.565709743635867e-05
43490,86981,86980,173961,2.199265956878662,1.5425827527910273e-05
43576,87153,87152,174305,2.203488826751709,1.5199032187722161e-05
43662,87325,87324,174649,2.2075271606445312,1.497354112181679e-05
43748,87497,87496,174993,2.211498975753784,1.4750986384827463e-05
43833,87667,87666,175333,2.2154128551483154,1.4536337388823615e-05
43919,87839,87838,175677,2.219491958618164,1.4322125419051483e-05
44005,88011,88010,176021,2.223539113998413,1.41090978687209e-05
44091,88183,88182,176365,2.2276298999786377,1.390003279461031e-05
44177,88355,88354,176709,2.231806993484497,1.3695739533211e-05
44263,88527,88526,177053,2.2358651161193848,1.3493168718444876e-05
44349,88699,88698,177397,2.240049123764038,1.3292359543028983e-05
44435,88871,88870,177741,2.2443461418151855,1.3096156820662643e-05
44521,89043,89042,178085,2.249082088470459,1.2903556240787107e-05
44607,89215,89214,178429,2.2533271312713623,1.2712004600631175e-05
44693,89387,89386,178773,2.2574870586395264,1.2523154106154338e-05
44779,89559,89558,179117,2.261539936065674,1.23388846424572e-05
44865,89731,89730,179461,2.2656118869781494,1.2156922636009888e-05
44951,89903,89902,179805,2.2696831226348877,1.1976043740501662e-05
45037,90075,90074,180149,2.273822069168091,1.1798733630411028e-05
45123,90247,90246,180493,2.2779769897460938,1.162533551203661e-05
45209,90419,90418,180837,2.282125949859619,1.1453241007342942e-05
45295,90591,90590,181181,2.2862818241119385,1.1282822730287928e-05
45381,90763,90762,181525,2.290432929992676,1.111641312059396e-05
45466,90933,90932,181865,2.294529914855957,1.0954752298251405e-05
45552,91105,91104,182209,2.2988109588623047,1.0792039753610796e-05
45638,91277,91276,182553,2.303016185760498,1.0631798584918207e-05
45724,91449,91448,182897,2.307237148284912,1.0475420872429507e-05
45810,91621,91620,183241,2.311401844024658,1.0320836850421121e-05
45896,91793,91792,183585,2.315553903579712,1.0167247288089995e-05
45982,91965,91964,183929,2.3196990489959717,1.0016825158744112e-05
46068,92137,92136,184273,2.323889970779419,9.869609514834563e-06
46154,92309,92308,184617,2.3280529975891113,9.723402279054328e-06
46240,92481,92480,184961,2.3321990966796875,9.57875936369615e-06
46326,92653,92652,185305,2.33634090423584,9.437572433829018e-06
46412,92825,92824,185649,2.340553045272827,9.298653611509171e-06
46498,92997,92996,185993,2.3448948860168457,9.160458311247848e-06
46584,93169,93168,186337,2.3490779399871826,9.0245370822514e-06
46670,93341,93340,186681,2.35327410697937,8.891848892719538e-06
46756,93513,93512,187025,2.3574230670928955,8.760527020436626e-06
46842,93685,93684,187369,2.361565113067627,8.630142915123343e-06
46928,93857,93856,187713,2.365694046020508,8.502571203198931e-06
47014,94029,94028,188057,2.3698232173919678,8.377592144176374e-06
47099,94199,94198,188397,2.373812198638916,8.254826579662353e-06
47185,94371,94370,188741,2.377774953842163,8.132069944355527e-06
47271,94543,94542,189085,2.3818578720092773,8.012277312468747e-06
47357,94715,94714,189429,2.3858678340911865,7.894278206045482e-06
47443,94887,94886,189773,2.3899519443511963,7.77690457164301e-06
47529,95059,95058,190117,2.393980026245117,7.661586308115583e-06
47615,95231,95230,190461,2.398106098175049,7.548963859734535e-06
47701,95403,95402,190805,2.402268171310425,7.43739507767848e-06
47787,95575,95574,191149,2.4065210819244385,7.326701946926654e-06
47873,95747,95746,191493,2.410706043243408,7.218475461441527e-06
47959,95919,95918,191837,2.414868116378784,7.112348705324352e-06
48045,96091,96090,192181,2.4190540313720703,7.006833883961287e-06
48131,96263,96262,192525,2.423272132873535,6.902685540359725e-06
48217,96435,96434,192869,2.427597999572754,6.801066504615991e-06
48303,96607,96606,193213,2.431820869445801,6.7008376318654204e-06
48389,96779,96778,193557,2.4361209869384766,6.601166210913315e-06
48475,96951,96950,193901,2.440380096435547,6.503359267493789e-06
48561,97123,97122,194245,2.444650888442993,6.407778460119969e-06
48647,97295,97294,194589,2.448927164077759,6.3129954407065025e-06
48732,97465,97464,194929,2.453130006790161,6.2201282068247805e-06
48818,97637,97636,195273,2.457395076751709,6.128311877854209e-06
48904,97809,97808,195617,2.461643934249878,6.038186609350915e-06
48990,97981,97980,195961,2.4658899307250977,5.948552786946322e-06
49076,98153,98152,196305,2.470128059387207,5.860176411402969e-06
49162,98325,98324,196649,2.4743478298187256,5.773945079570285e-06
49248,98497,98496,196993,2.478616952896118,5.688800227824727e-06
49334,98669,98668,197337,2.4828829765319824,5.6041595139826154e-06
49420,98841,98840,197681,2.487558126449585,5.521183401589622e-06
49506,99013,99012,198025,2.4918088912963867,5.440042288316114e-06
49592,99185,99184,198369,2.4960649013519287,5.359515896675196e-06
49678,99357,99356,198713,2.5004031658172607,5.279769261296706e-06
49764,99529,99528,199057,2.5046679973602295,5.201895573646095e-06
49850,99701,99700,199401,2.508923053741455,5.125361293618182e-06
49936,99873,99872,199745,2.5131611824035645,5.049228600671948e-06
50022,100045,100044,200089,2.517396926879883,4.97426134453938e-06
50108,100217,100216,200433,2.5216450691223145,4.901100126825626e-06
50194,100389,100388,200777,2.525897979736328,4.828769928450503e-06
50280,100561,100560,201121,2.530133008956909,4.756908975385398e-06
50365,100731,100730,201461,2.5343000888824463,4.6873445772367265e-06
50451,100903,100902,201805,2.538512945175171,4.618455908886837e-06
50537,101075,101074,202149,2.542729139328003,4.550042579687513e-06
50623,101247,101246,202493,2.5469720363616943,4.482357069200044e-06
50709,101419,101418,202837,2.5512681007385254,4.4162868200935e-06
50795,101591,101590,203181,2.5555031299591064,4.351282017481602e-06
50881,101763,101762,203525,2.5597710609436035,4.2866154738530175e-06
50967,101935,101934,203869,2.564099073410034,4.223008643016652e-06
51053,102107,102106,204213,2.5681891441345215,4.160916321202825e-06
51139,102279,102278,204557,2.5722410678863525,4.099467090716604e-06
51225,102451,102450,204901,2.576375961303711,4.038453499149208e-06
51311,102623,102622,205245,2.5803639888763428,3.978753116800276e-06
51397,102795,102794,205589,2.5844881534576416,3.9202702474791925e-06
51483,102967,102966,205933,2.5884671211242676,3.8621522443345645e-06
51569,103139,103138,206277,2.5924770832061768,3.8047214734283827e-06
51655,103311,103310,206621,2.596503973007202,3.7486782189012983e-06
51741,103483,103482,206965,2.600576877593994,3.6934670653005266e-06
51827,103655,103654,207309,2.604598045349121,3.6385496080667923e-06
51913,103827,103826,207653,2.6086370944976807,3.5846001225805252e-06
51999,103999,103998,207997,2.612607955932617,3.5319089116620433e-06
52084,104169,104168,208337,2.616734027862549,3.4803106272101887e-06
52170,104341,104340,208681,2.6207010746002197,3.4285113028449526e-06
52256,104513,104512,209025,2.6247169971466064,3.3778641371420924e-06
52342,104685,104684,209369,2.628793954849243,3.328203372336626e-06
52428,104857,104856,209713,2.632766008377075,3.27883063749508e-06
52514,105029,105028,210057,2.6368491649627686,3.230093757012239e-06
52600,105201,105200,210401,2.6409378051757812,3.1825400119746503e-06
52686,105373,105372,210745,2.6450138092041016,3.1356401587593768e-06
52772,105545,105544,211089,2.6491990089416504,3.089000521804642e-06
52858,105717,105716,211433,2.653301954269409,3.0432302942328116e-06
52944,105889,105888,211777,2.657464027404785,2.9985032258083603e-06
53030,106061,106060,212121,2.661518096923828,2.9541514441893848e-06
53116,106233,106232,212465,2.6655662059783936,2.9101869845754885e-06
53202,106405,106404,212809,2.669609785079956,2.8672321704505634e-06
53288,106577,106576,213153,2.673712968826294,2.8250641023212075e-06
53374,106749,106748,213497,2.6778249740600586,2.783124988433654e-06
53460,106921,106920,213841,2.681887149810791,2.7417790906966887e-06
53546,107093,107092,214185,2.6859371662139893,2.701436289403037e-06
53632,107265,107264,214529,2.6899828910827637,2.6615972063793135e-06
53717,107435,107434,214869,2.6940488815307617,2.6224535261267124e-06
53803,107607,107606,215213,2.6981279850006104,2.58362343848867e-06
53889,107779,107778,215557,2.702230930328369,2.5456535939790627e-06
53975,107951,107950,215901,2.7063488960266113,2.5079728587197565e-06
54061,108123,108122,216245,2.7104389667510986,2.4706545193564296e-06
54147,108295,108294,216589,2.7145299911499023,2.4342118269328957e-06
54233,108467,108466,216933,2.7186222076416016,2.398398833906253e-06
54319,108639,108638,217277,2.7227671146392822,2.3627740045185593e-06
54405,108811,108810,217621,2.7269129753112793,2.3276918161992426e-06
54491,108983,108982,217965,2.73095703125,2.2934553991351676e-06
54577,109155,109154,218309,2.735053062438965,2.2596104984447542e-06
54663,109327,109326,218653,2.7391340732574463,2.225984207461046e-06
54749,109499,109498,218997,2.743285894393921,2.1930524687022117e-06
54835,109671,109670,219341,2.7484419345855713,2.1608214791370485e-06
54921,109843,109842,219685,2.7542471885681152,2.1288105029579198e-06
55007,110015,110014,220029,2.7585928440093994,2.0971434882026484e-06
55093,110187,110186,220373,2.762874126434326,2.0662333938999476e-06
55179,110359,110358,220717,2.7670021057128906,2.035818191657563e-06
55265,110531,110530,221061,2.771113157272339,2.005561238477005e-06
55350,110701,110700,221401,2.775238037109375,1.976145207706934e-06
55436,110873,110872,221745,2.7795748710632324,1.9470887612750627e-06
55522,111045,111044,222089,2.7837212085723877,1.9183353401968875e-06
55608,111217,111216,222433,2.788939952850342,1.8897847434834728e-06
55694,111389,111388,222777,2.7930941581726074,1.8618470582435151e-06
55780,111561,111560,223121,2.7979140281677246,1.834480440189711e-06
55866,111733,111732,223465,2.802610158920288,1.8072852947843174e-06
55952,111905,111904,223809,2.807018995285034,1.7804099040601701e-06
56038,112077,112076,224153,2.811241865158081,1.7541835705245169e-06
56124,112249,112248,224497,2.8153979778289795,1.7283484990540143e-06
56210,112421,112420,224841,2.8195600509643555,1.7026503594481936e-06
56296,112593,112592,225185,2.823759078979492,1.6774033914383054e-06
56382,112765,112764,225529,2.8280279636383057,1.6527463255472664e-06
56468,112937,112936,225873,2.832213878631592,1.6283191019548684e-06
56554,113109,113108,226217,2.836367130279541,1.604084299845657e-06
56640,113281,113280,226561,2.8405210971832275,1.580390201992924e-06
56726,113453,113452,226905,2.8453450202941895,1.5571549536249867e-06
56812,113625,113624,227249,2.8498270511627197,1.534053499145587e-06
56898,113797,113796,227593,2.854116916656494,1.5112523027506792e-06
56983,113967,113966,227933,2.8583321571350098,1.4892606233577353e-06
57069,114139,114138,228277,2.8625290393829346,1.4673147747759306e-06
57155,114311,114310,228621,2.8666868209838867,1.4454901121254035e-06
57241,114483,114482,228965,2.8708488941192627,1.4240708319346085e-06
57327,114655,114654,229309,2.875101089477539,1.4031407633709019e-06
57413,114827,114826,229653,2.8792691230773926,1.382387679643485e-06
57499,114999,114998,229997,2.883527994155884,1.3618147172162132e-06
57585,115171,115170,230341,2.8876688480377197,1.341713330992676e-06
57671,115343,115342,230685,2.8918581008911133,1.321981366588748e-06
57757,115515,115514,231029,2.896048069000244,1.3023569332348881e-06
57843,115687,115686,231373,2.9002060890197754,1.2830087358902253e-06
57929,115859,115858,231717,2.9044361114501953,1.2641299405709782e-06
58015,116031,116030,232061,2.908890962600708,1.2454880103384884e-06
58101,116203,116202,232405,2.9130940437316895,1.2269567621183997e-06
58187,116375,116374,232749,2.917257785797119,1.2087907355480076e-06
58273,116547,116546,233093,2.921386957168579,1.1910259335712941e-06
58359,116719,116718,233437,2.9255049228668213,1.1733950939784465e-06
58445,116891,116890,233781,2.929638147354126,1.155935577012221e-06
58531,117063,117062,234125,2.933812141418457,1.1388865215202522e-06
58617,117235,117234,234469,2.937933921813965,1.1221301036185177e-06
58702,117405,117404,234809,2.9420180320739746,1.105654694240285e-06
58788,117577,117576,235153,2.94620418548584,1.0892375396255605e-06
58874,117749,117748,235497,2.9503469467163086,1.0732163319345084e-06
58960,117921,117920,235841,2.954512119293213,1.0573792889264695e-06
59046,118093,118092,236185,2.9587271213531494,1.0416438520249457e-06
59132,118265,118264,236529,2.962862014770508,1.02623260472598e-06
59218,118437,118436,236873,2.9669668674468994,1.0111502647755533e-06
59304,118609,118608,237217,2.9710590839385986,9.961715502333563e-07
59390,118781,118780,237561,2.975148916244507,9.813527402619427e-07
59476,118953,118952,237905,2.9793200492858887,9.668878339297394e-07
59562,119125,119124,238249,2.9834091663360596,9.52655655970987e-07
59648,119297,119296,238593,2.9875340461730957,9.384976340728266e-07
59734,119469,119468,238937,2.991711139678955,9.245722346828855e-07
59820,119641,119640,239281,2.9958410263061523,9.109781283863287e-07
59906,119813,119812,239625,3.000063896179199,8.975242486817724e-07
59992,119985,119984,239969,3.004261016845703,8.841661841904508e-07
60078,120157,120156,240313,3.0086581707000732,8.710960426024825e-07
60164,120329,120328,240657,3.0133919715881348,8.582918717024834e-07
60250,120501,120500,241001,3.017348051071167,8.455672160723083e-07
60335,120671,120670,241341,3.0212562084198,8.331380970426433e-07
60421,120843,120842,241685,3.0253989696502686,8.208651022055911e-07
60507,121015,121014,242029,3.0293610095977783,8.087761479029388e-07
60593,121187,121186,242373,3.033332109451294,7.967512511705442e-07
60679,121359,121358,242717,3.0372769832611084,7.849366331964429e-07
60765,121531,121530,243061,3.0412650108337402,7.733983057192711e-07
60851,121703,121702,243405,3.0453920364379883,7.619681224215152e-07
60937,121875,121874,243749,3.0495150089263916,7.506273985784029e-07
61023,122047,122046,244093,3.0536069869995117,7.395392385002747e-07
61109,122219,122218,244437,3.057873010635376,7.286665245561759e-07
61195,122391,122390,244781,3.0618999004364014,7.178566127175872e-07
61281,122563,122562,245125,3.0660741329193115,7.071863867959877e-07
61367,122735,122734,245469,3.0700619220733643,6.967752898216133e-07
61453,122907,122906,245813,3.07423996925354,6.865069409471636e-07
61539,123079,123078,246157,3.0783369541168213,6.762956787257074e-07
61625,123251,123250,246501,3.082412004470825,6.662751683099156e-07
61711,123423,123422,246845,3.086487054824829,6.564828153798816e-07
61797,123595,123594,247189,3.0907199382781982,6.467723569966794e-07
61883,123767,123766,247533,3.095555067062378,6.371470929144194e-07
61968,123937,123936,247873,3.099945068359375,6.278509776847169e-07
62054,124109,124108,248217,3.104980945587158,6.186176453502346e-07
62140,124281,124280,248561,3.109220027923584,6.094347363001117e-07
62226,124453,124452,248905,3.1144070625305176,6.00380388696284e-07
62312,124625,124624,249249,3.118649959564209,5.915458188819669e-07
62398,124797,124796,249593,3.1231160163879395,5.828228202802797e-07
62484,124969,124968,249937,3.127331018447876,5.741514230209364e-07
62570,125141,125140,250281,3.1325740814208984,5.656503520570673e-07
62656,125313,125312,250625,3.1368610858917236,5.573373718267283e-07
62742,125485,125484,250969,3.1412031650543213,5.490874823680843e-07
62828,125657,125656,251313,3.1456010341644287,5.409172945559627e-07
62914,125829,125828,251657,3.1500420570373535,5.329389216633643e-07
63000,126001,126000,252001,3.154555082321167,5.250979814520983e-07
63086,126173,126172,252345,3.159036159515381,5.172981701231166e-07
63172,126345,126344,252689,3.1635820865631104,5.096175390981975e-07
63258,126517,126516,253033,3.1681339740753174,5.02122024610876e-07
63344,126689,126688,253377,3.1725878715515137,4.947118857930312e-07
63430,126861,126860,253721,3.1771109104156494,4.873497338184561e-07
63516,127033,127032,254065,3.1816020011901855,4.801399240558397e-07
63601,127203,127202,254405,3.1860241889953613,4.731650975202931e-07
63687,127375,127374,254749,3.1904830932617188,4.6615617290114694e-07
63773,127547,127546,255093,3.1949729919433594,4.592216428212069e-07
63859,127719,127718,255437,3.199505090713501,4.524525648672708e-07
63945,127891,127890,255781,3.2040820121765137,4.457928344408863e-07
64031,128063,128062,256125,3.2086880207061768,4.391677309779974e-07
64117,128235,128234,256469,3.2132840156555176,4.3265101248936674e-07
64203,128407,128406,256813,3.217841148376465,4.262895460184727e-07
64289,128579,128578,257157,3.2222039699554443,4.1999415778971956e-07
64375,128751,128750,257501,3.2265989780426025,4.137433146343117e-07
64461,128923,128922,257845,3.230802059173584,4.076268733322464e-07
64547,129095,129094,258189,3.23502516746521,4.016352799802651e-07
64633,129267,129266,258533,3.239230155944824,3.956811482996995e-07
64719,129439,129438,258877,3.2435801029205322,3.8979728645510573e-07
64805,129611,129610,259221,3.248483896255493,3.8405553627259566e-07
64891,129783,129782,259565,3.252769947052002,3.7839916026866765e-07
64977,129955,129954,259909,3.257049083709717,3.7277282380567354e-07
65063,130127,130126,260253,3.2612531185150146,3.672455206814949e-07
65149,130299,130298,260597,3.265449047088623,3.61847224820581e-07
65234,130469,130468,260937,3.2695980072021484,3.565610263395574e-07
65320,130641,130640,261281,3.2737770080566406,3.512541796915096e-07
65406,130813,130812,261625,3.2779722213745117,3.460652659809035e-07
65492,130985,130984,261969,3.282155990600586,3.409775079785002e-07
65578,131157,131156,262313,3.28635311126709,3.359193074437309e-07
65664,131329,131328,262657,3.290541887283325,3.3092612798974264e-07
65750,131501,131500,263001,3.294715166091919,3.260541475370384e-07
65836,131673,131672,263345,3.2989118099212646,3.212492674696828e-07
65922,131845,131844,263689,3.3031139373779297,3.164709891107004e-07
66008,132017,132016,264033,3.307555913925171,3.1178167288877783e-07
66094,132189,132188,264377,3.3117642402648926,3.0719932648522636e-07
66180,132361,132360,264721,3.315988063812256,3.02655535438336e-07
66266,132533,132532,265065,3.3201639652252197,2.9815132156914646e-07
66352,132705,132704,265409,3.3244099617004395,2.9375048332562964e-07
66438,132877,132876,265753,3.328585147857666,2.894303713940966e-07
66524,133049,133048,266097,3.3327488899230957,2.8513376460558833e-07
66610,133221,133220,266441,3.3369429111480713,2.808978215202873e-07
66696,133393,133392,266785,3.341125011444092,2.767646330157876e-07
66782,133565,133564,267129,3.3452961444854736,2.726831381197184e-07
66868,133737,133736,267473,3.3494889736175537,2.686259765371107e-07
66953,133907,133906,267813,3.353640079498291,2.646945235396948e-07
67039,134079,134078,268157,3.357818126678467,2.6080447419024194e-07
67125,134251,134250,268501,3.362013101577759,2.5694412953426907e-07
67211,134423,134422,268845,3.366175889968872,2.5312081968880676e-07
67297,134595,134594,269189,3.3703560829162598,2.493871741595942e-07
67383,134767,134766,269533,3.3744280338287354,2.4571814496690573e-07
67469,134939,134938,269877,3.378453016281128,2.420684214488433e-07
67555,135111,135110,270221,3.3824238777160645,2.384741969378808e-07
67641,135283,135282,270565,3.3864009380340576,2.3496662167502715e-07
67727,135455,135454,270909,3.3904879093170166,2.3149922672541307e-07
67813,135627,135626,271253,3.395163059234619,2.2805417829274326e-07
67899,135799,135798,271597,3.4004011154174805,2.2468022208833382e-07
67985,135971,135970,271941,3.4044671058654785,2.2137813038172684e-07
68071,136143,136142,272285,3.408557891845703,2.1809861907073757e-07
68157,136315,136314,272629,3.4132909774780273,2.1485425593115568e-07
68243,136487,136486,272973,3.41749906539917,2.1168742825761202e-07
68329,136659,136658,273317,3.421588182449341,2.085714092423637e-07
68415,136831,136830,273661,3.4257659912109375,2.054716115408443e-07
68501,137003,137002,274005,3.4302608966827393,2.0242287997676806e-07
68586,137173,137172,274345,3.4344980716705322,1.994810429371442e-07
68672,137345,137344,274689,3.438516139984131,1.965352666088048e-07
68758,137517,137516,275033,3.4425740242004395,1.9361021713799434e-07
68844,137689,137688,275377,3.447005033493042,1.907479132291259e-07
68930,137861,137860,275721,3.451004981994629,1.879441868261561e-07
69016,138033,138032,276065,3.455026149749756,1.8515805677365556e-07
69102,138205,138204,276409,3.459096908569336,1.8240460650698365e-07
69188,138377,138376,276753,3.4631881713867188,1.7971764964595907e-07
69274,138549,138548,277097,3.4672491550445557,1.7707086808549525e-07
69360,138721,138720,277441,3.4713470935821533,1.7443811577633863e-07
69446,138893,138892,277785,3.475512981414795,1.7185151400712543e-07
69532,139065,139064,278129,3.4796760082244873,1.6932536748659634e-07
69618,139237,139236,278473,3.4838387966156006,1.6682282237172872e-07
69704,139409,139408,278817,3.4880192279815674,1.643399517262983e-07
69790,139581,139580,279161,3.492224931716919,1.6191243414305528e-07
69876,139753,139752,279505,3.4964420795440674,1.5953197253299859e-07
69962,139925,139924,279849,3.5006179809570312,1.5716522671071071e-07
70048,140097,140096,280193,3.504791021347046,1.5482917795844218e-07
70134,140269,140268,280537,3.5089399814605713,1.5254985792547496e-07
70219,140439,140438,280877,3.51305890083313,1.503277337479583e-07
70305,140611,140610,281221,3.5184731483459473,1.480918134986167e-07
70391,140783,140782,281565,3.5226449966430664,1.4589736602959086e-07
70477,140955,140954,281909,3.52679705619812,1.4375305872750564e-07
70563,141127,141126,282253,3.530963182449341,1.416269231411525e-07
70649,141299,141298,282597,3.5351221561431885,1.3951920100135785e-07
70735,141471,141470,282941,3.5393152236938477,1.37459763513016e-07
70821,141643,141642,283285,3.5434799194335938,1.3543821781324585e-07
70907,141815,141814,283629,3.547657012939453,1.3342769010037797e-07
70993,141987,141986,283973,3.551846981048584,1.314454075134706e-07
71079,142159,142158,284317,3.556020975112915,1.2951123134862306e-07
71165,142331,142330,284661,3.5601840019226074,1.2760138261223998e-07
71251,142503,142502,285005,3.5645339488983154,1.2570285222835523e-07
71337,142675,142674,285349,3.5687332153320312,1.238416924857981e-07
71423,142847,142846,285693,3.572962999343872,1.2202167380590278e-07
71509,143019,143018,286037,3.5769970417022705,1.2021542058625597e-07
71595,143191,143190,286381,3.58096981048584,1.1842668355062717e-07
71681,143363,143362,286725,3.584951877593994,1.1667997233172219e-07
71767,143535,143534,287069,3.5889101028442383,1.1496327711367511e-07
71852,143705,143704,287409,3.5928730964660645,1.1327535683954595e-07
71938,143877,143876,287753,3.5972259044647217,1.1159336664212353e-07
72024,144049,144048,288097,3.6012048721313477,1.0995196040136061e-07
72110,144221,144220,288441,3.6051838397979736,1.0832947311621003e-07
72196,144393,144392,288785,3.6092231273651123,1.067173744734097e-07
72282,144565,144564,289129,3.613248825073242,1.0513845163394736e-07
72368,144737,144736,289473,3.6174089908599854,1.0359325706979166e-07
72454,144909,144908,289817,3.6214098930358887,1.0205870865171373e-07
72540,145081,145080,290161,3.6254730224609375,1.005405093333378e-07
72626,145253,145252,290505,3.629599094390869,9.905855002591735e-08
72712,145425,145424,290849,3.6336731910705566,9.760046426593418e-08
72798,145597,145596,291193,3.637714147567749,9.614997072037842e-08
72884,145769,145768,291537,3.6418230533599854,9.472327332976307e-08
72970,145941,145940,291881,3.646036148071289,9.333053340411697e-08
73056,146113,146112,292225,3.650163173675537,9.195219155165083e-08
73142,146285,146284,292569,3.6547000408172607,9.058363786087751e-08
73228,146457,146456,292913,3.6588048934936523,8.92445587717115e-08
73314,146629,146628,293257,3.662869930267334,8.793276658724153e-08
73400,146801,146800,293601,3.6669270992279053,8.66291436967578e-08
73485,146971,146970,293941,3.670948028564453,8.535577996270512e-08
73571,147143,147142,294285,3.675062894821167,8.409838669406913e-08
73657,147315,147314,294629,3.6791160106658936,8.285987489309883e-08
73743,147487,147486,294973,3.68322491645813,8.162791663480763e-08
73829,147659,147658,295317,3.68727707862854,8.0417471795338e-08
73915,147831,147830,295661,3.6913340091705322,7.92353523638655e-08
74001,148003,148002,296005,3.69585919380188,7.806433845902442e-08
74087,148175,148174,296349,3.7007510662078857,7.690246409230166e-08
74173,148347,148346,296693,3.704897880554199,7.576644743933038e-08
74259,148519,148518,297037,3.7091591358184814,7.465253688125694e-08
74345,148691,148690,297381,3.713470220565796,7.35450768271276e-08
74431,148863,148862,297725,3.717827081680298,7.245189841041025e-08
74517,149035,149034,298069,3.722278118133545,7.138526191195088e-08
74603,149207,149206,298413,3.7264628410339355,7.033327588955933e-08
74689,149379,149378,298757,3.7307140827178955,6.928713321609036e-08
74775,149551,149550,299101,3.7349119186401367,6.82605085532337e-08
74861,149723,149722,299445,3.739022970199585,6.725727025889046e-08
74947,149895,149894,299789,3.743185043334961,6.626243662732193e-08
75033,150067,150066,300133,3.747375965118408,6.527630752609028e-08
75119,150239,150238,300477,3.7514750957489014,6.431283311667064e-08
75204,150409,150408,300817,3.75553297996521,6.337793382735866e-08
75290,150581,150580,301161,3.759688138961792,6.243715707903415e-08
75376,150753,150752,301505,3.7638039588928223,6.150952706264794e-08
75462,150925,150924,301849,3.767888069152832,6.060441015462716e-08
75548,151097,151096,302193,3.772033929824829,5.971074413048224e-08
75634,151269,151268,302537,3.7761268615722656,5.882235667067096e-08
75720,151441,151440,302881,3.7803738117218018,5.7951400066256276e-08
75806,151613,151612,303225,3.7844619750976562,5.709972644651793e-08
75892,151785,151784,303569,3.788547992706299,5.6254527678756155e-08
75978,151957,151956,303913,3.792628049850464,5.541747253660384e-08
76064,152129,152128,304257,3.796802043914795,5.460006358546363e-08
76150,152301,152300,304601,3.8009250164031982,5.379676107887067e-08
76236,152473,152472,304945,3.8050589561462402,5.2997675615252765e-08
76322,152645,152644,305289,3.8092031478881836,5.2210776967026994e-08
76408,152817,152816,305633,3.813383102416992,5.144284841794538e-08
76494,152989,152988,305977,3.81754207611084,5.068368885858578e-08
76580,153161,153160,306321,3.821693181991577,4.9929438585661096e-08
76666,153333,153332,306665,3.8259780406951904,4.9190778665413243e-08
76752,153505,153504,307009,3.830068826675415,4.846782814268902e-08
76837,153675,153674,307349,3.8342130184173584,4.77581356978799e-08
76923,153847,153846,307693,3.83833909034729,4.704767538771315e-08
77009,154019,154018,308037,3.842519998550415,4.635416358050207e-08
77095,154191,154190,308381,3.846748113632202,4.567187757235517e-08
77181,154363,154362,308725,3.8509860038757324,4.499314052266171e-08
77267,154535,154534,309069,3.855187177658081,4.4325488003848056e-08
77353,154707,154706,309413,3.8594419956207275,4.367374631700277e-08
77439,154879,154878,309757,3.8636980056762695,4.302879124064925e-08
77525,155051,155050,310101,3.8679089546203613,4.2388392465621556e-08
77611,155223,155222,310445,3.872182846069336,4.176174980979716e-08
77697,155395,155394,310789,3.8764078617095947,4.1147907703381816e-08
77783,155567,155566,311133,3.880702018737793,4.053790840194118e-08
77869,155739,155738,311477,3.885004997253418,3.993509240991983e-08
77955,155911,155910,311821,3.889248847961426,3.9346835399714774e-08
78041,156083,156082,312165,3.893562078475952,3.8767341526234933e-08
78127,156255,156254,312509,3.897778034210205,3.8190920699675064e-08
78213,156427,156426,312853,3.9020540714263916,3.7624630528658325e-08
78299,156599,156598,313197,3.9063820838928223,3.707156717241821e-08
78385,156771,156770,313541,3.9107069969177246,3.6523649493361455e-08
78470,156941,156940,313881,3.9149248600006104,3.5986321787912915e-08
78556,157113,157112,314225,3.9191219806671143,3.545470571316525e-08
78642,157285,157284,314569,3.9233250617980957,3.4933462636950824e-08
78728,157457,157456,314913,3.927820920944214,3.4415250255675586e-08
78814,157629,157628,315257,3.932180881500244,3.3903685433969223e-08
78900,157801,157800,315601,3.9365410804748535,3.3404539095146743e-08
78986,157973,157972,315945,3.940778970718384,3.291228166707564e-08
79072,158145,158144,316289,3.945157051086426,3.2422744777370836e-08
79158,158317,158316,316633,3.950389862060547,3.194230946426575e-08
79244,158489,158488,316977,3.9546611309051514,3.147284275201123e-08
79330,158661,158660,317321,3.9589109420776367,3.100733827734708e-08
79416,158833,158832,317665,3.9631850719451904,3.054587993907727e-08
79502,159005,159004,318009,3.9675450325012207,3.009500412702808e-08
79588,159177,159176,318353,3.971860885620117,2.965240872874254e-08
79674,159349,159348,318697,3.976269006729126,2.9212224017473558e-08
79760,159521,159520,319041,3.9806461334228516,2.8778243455480032e-08
79846,159693,159692,319385,3.985038995742798,2.8354790341807537e-08
79932,159865,159864,319729,3.9895389080047607,2.793664238163798e-08
80018,160037,160036,320073,3.994025230407715,2.7520981012359246e-08
80103,160207,160206,320413,3.9984538555145264,2.71181890582594e-08
80189,160379,160378,320757,4.002921104431152,2.6719650233015506e-08
80275,160551,160550,321101,4.007401943206787,2.632416374405349e-08
80361,160723,160722,321445,4.011825084686279,2.593246372177552e-08
80447,160895,160894,321789,4.016248941421509,2.5549943965691178e-08
80533,161067,161066,322133,4.020685911178589,2.517405224901704e-08
80619,161239,161238,322477,4.025193929672241,2.480013909586006e-08
80705,161411,161410,322821,4.029519081115723,2.4431902569201193e-08
80791,161583,161582,323165,4.034151077270508,2.4072545218474064e-08
80877,161755,161754,323509,4.038272857666016,2.371731187670055e-08
80963,161927,161926,323853,4.042313098907471,2.3364361690079283e-08
81049,162099,162098,324197,4.046506881713867,2.3018688248539285e-08
81135,162271,162270,324541,4.050540924072266,2.2680386493930097e-08
81221,162443,162442,324885,4.054560899734497,2.23444044792868e-08
81307,162615,162614,325229,4.058653116226196,2.2012014581943905e-08
81393,162787,162786,325573,4.062763929367065,2.1687565356266404e-08
81479,162959,162958,325917,4.066911220550537,2.136833115017347e-08
81565,163131,163130,326261,4.071042060852051,2.1050759729531756e-08
81651,163303,163302,326605,4.075285911560059,2.073841192555546e-08
81736,163473,163472,326945,4.0794432163238525,2.0437014302397936e-08
81822,163645,163644,327289,4.083652973175049,2.0135221091503995e-08
81908,163817,163816,327633,4.087831974029541,1.9835544977185406e-08
81994,163989,163988,327977,4.092078924179077,1.954229222193997e-08
82080,164161,164160,328321,4.096301078796387,1.925504932524029e-08
82166,164333,164332,328665,4.100451946258545,1.8969613842568104e-08
82252,164505,164504,329009,4.104664087295532,1.868751873297093e-08
82338,164677,164676,329353,4.108897924423218,1.8412234338467856e-08
82424,164849,164848,329697,4.1131391525268555,1.8141072962120723e-08
82510,165021,165020,330041,4.1173670291900635,1.7871349590437002e-08
82596,165193,165192,330385,4.12148904800415,1.7606347301981765e-08
82682,165365,165364,330729,4.1257569789886475,1.7347540181050285e-08
82768,165537,165536,331073,4.1299779415130615,1.7091155550534226e-08
82854,165709,165708,331417,4.134202003479004,1.683678154434382e-08
82940,165881,165880,331761,4.138441801071167,1.6588074746911648e-08
83026,166053,166052,332105,4.142636060714722,1.6344195794721403e-08
83112,166225,166224,332449,4.146772861480713,1.6101723206476462e-08
83198,166397,166396,332793,4.15104603767395,1.5862389020196612e-08
83284,166569,166568,333137,4.155231237411499,1.5628867256799218e-08
83370,166741,166740,333481,4.159489870071411,1.5398542563404687e-08
83455,166911,166910,333821,4.163668870925903,1.5172146521846747e-08
83541,167083,167082,334165,4.1679160594940186,1.4947320956847124e-08
83627,167255,167254,334509,4.1721508502960205,1.472763381542647e-08
83713,167427,167426,334853,4.176382780075073,1.4509812139681856e-08
83799,167599,167598,335197,4.180613994598389,1.4293871833918747e-08
83885,167771,167770,335541,4.184873819351196,1.4082875865071445e-08
83971,167943,167942,335885,4.189079999923706,1.3875768235850092e-08
84057,168115,168114,336229,4.1933770179748535,1.3669790434085243e-08
84143,168287,168286,336573,4.197612047195435,1.3466700576045132e-08
84229,168459,168458,336917,4.201833963394165,1.326853984105131e-08
84315,168631,168630,337261,4.206060886383057,1.3072878239648012e-08
84401,168803,168802,337605,4.210274934768677,1.2878374746091215e-08
84487,168975,168974,337949,4.214541912078857,1.2687694771636195e-08
84573,169147,169146,338293,4.218761205673218,1.2501232807544324e-08
84659,169319,169318,338637,4.222969055175781,1.2316183589663706e-08
84745,169491,169490,338981,4.227115869522095,1.2132925158376114e-08
84831,169663,169662,339325,4.231366157531738,1.1953970188593235e-08
84917,169835,169834,339669,4.235591173171997,1.1778094711041407e-08
85003,170007,170006,340013,4.239814043045044,1.1603141480210885e-08
85088,170177,170176,340353,4.2439820766448975,1.1432840752970768e-08
85174,170349,170348,340697,4.248200178146362,1.1264675659140722e-08
85260,170521,170520,341041,4.252366065979004,1.1098453954634873e-08
85346,170693,170692,341385,4.256622076034546,1.0933294830561487e-08
85432,170865,170864,341729,4.260814905166626,1.0771531035995722e-08
85518,171037,171036,342073,4.265049934387207,1.0613224974630694e-08
85604,171209,171208,342417,4.2692461013793945,1.0456011383738711e-08
85690,171381,171380,342761,4.273447036743164,1.0300469471273685e-08
85776,171553,171552,343105,4.277652978897095,1.0148638901119764e-08
85862,171725,171724,343449,4.281844854354858,9.999258193884267e-09


==> plot_data/quadratic_minimax_problem_n20_alpha00001/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.295608520507812e-05,4.387072431292609
92,185,184,369,0.003635883331298828,0.265498193466344
184,369,368,737,0.006905794143676758,0.12132799283907403
276,553,552,1105,0.009988069534301758,0.08098588184474649
368,737,736,1473,0.013046026229858398,0.06295546836576064
460,921,920,1841,0.017035961151123047,0.0534342328893946
552,1105,1104,2209,0.020149946212768555,0.04755332813973005
644,1289,1288,2577,0.023462772369384766,0.04336819414898068
736,1473,1472,2945,0.026858806610107422,0.040012134760418344
828,1657,1656,3313,0.030059814453125,0.0372103624585227
920,1841,1840,3681,0.034893035888671875,0.03477038957412199
1012,2025,2024,4049,0.03927969932556152,0.03265139713580958
1104,2209,2208,4417,0.042775869369506836,0.03078428506122928
1196,2393,2392,4785,0.04594087600708008,0.029152698139190723
1288,2577,2576,5153,0.049260854721069336,0.027717571667471172
1380,2761,2760,5521,0.05245089530944824,0.026448938785904454
1472,2945,2944,5889,0.05548095703125,0.0253367111154004
1564,3129,3128,6257,0.0586397647857666,0.024347764291400217
1656,3313,3312,6625,0.06255578994750977,0.023480498091803637
1748,3497,3496,6993,0.06614971160888672,0.022695332155553104
1840,3681,3680,7361,0.0693807601928711,0.022005658133093478
1932,3865,3864,7729,0.07249569892883301,0.021375656372689192
2024,4049,4048,8097,0.07589077949523926,0.02081458748885702
2116,4233,4232,8465,0.08002400398254395,0.020293465291431705
2208,4417,4416,8833,0.08359193801879883,0.01982630351650638
2300,4601,4600,9201,0.08737397193908691,0.019389202351310926
2392,4785,4784,9569,0.09133481979370117,0.018986137742038216
2484,4969,4968,9937,0.0944218635559082,0.0186057407100563
2576,5153,5152,10305,0.09764599800109863,0.018253000036295677
2668,5337,5336,10673,0.10088682174682617,0.017918259599596986
2760,5521,5520,11041,0.10417890548706055,0.017597688703256596
2852,5705,5704,11409,0.10752987861633301,0.017293079687255273
2944,5889,5888,11777,0.11089873313903809,0.01700159297397879
3036,6073,6072,12145,0.11423301696777344,0.01672213100002464
3128,6257,6256,12513,0.11756110191345215,0.016447968805384967
3220,6441,6440,12881,0.12093377113342285,0.01618618498607426
3312,6625,6624,13249,0.12436890602111816,0.015930928736841075
3404,6809,6808,13617,0.1278519630432129,0.01568326839769925
3496,6993,6992,13985,0.13132476806640625,0.015438498485822448
3588,7177,7176,14353,0.13480377197265625,0.015203162815280596
3680,7361,7360,14721,0.13841581344604492,0.014972054702171935
3772,7545,7544,15089,0.14188790321350098,0.014745071898047963
3864,7729,7728,15457,0.14533591270446777,0.014521320003355147
3956,7913,7912,15825,0.14876985549926758,0.014304479567288005
4048,8097,8096,16193,0.1521897315979004,0.014091140079077654
4140,8281,8280,16561,0.15564370155334473,0.013879793206978706
4232,8465,8464,16929,0.1589798927307129,0.01367256573915936
4324,8649,8648,17297,0.1623399257659912,0.013470390757701262
4416,8833,8832,17665,0.1657118797302246,0.01327114009934527
4508,9017,9016,18033,0.16915297508239746,0.013073122123599274
4601,9203,9202,18405,0.1725916862487793,0.012877682915089568
4693,9387,9386,18773,0.17622590065002441,0.012688206839978662
4785,9571,9570,19141,0.1796107292175293,0.012500884529289989
4877,9755,9754,19509,0.18302583694458008,0.012315019266588227
4969,9939,9938,19877,0.18642282485961914,0.012133849222633586
5061,10123,10122,20245,0.18982887268066406,0.011955752953232979
5153,10307,10306,20613,0.19339489936828613,0.011779091563424092
5245,10491,10490,20981,0.19673681259155273,0.011604522757011774
5337,10675,10674,21349,0.1998908519744873,0.011434309629244554
5429,10859,10858,21717,0.20307087898254395,0.011266569106741545
5521,11043,11042,22085,0.20621371269226074,0.011099845691387835
5613,11227,11226,22453,0.2092909812927246,0.010935858909671579
5705,11411,11410,22821,0.21239089965820312,0.010775721807310424
5797,11595,11594,23189,0.2154688835144043,0.010617477516402206
5889,11779,11778,23557,0.22146081924438477,0.010460213504775911
5981,11963,11962,23925,0.2245328426361084,0.010306135028158967
6073,12147,12146,24293,0.227586030960083,0.010155337117681955
6165,12331,12330,24661,0.23073506355285645,0.010005895574154346
6257,12515,12514,25029,0.23378872871398926,0.009857696973449577
6349,12699,12698,25397,0.23683786392211914,0.009712878665989464
6441,12883,12882,25765,0.23990583419799805,0.00957074902621629
6533,13067,13066,26133,0.24295377731323242,0.009429574404370878
6625,13251,13250,26501,0.24596691131591797,0.00929005618981176
6717,13435,13434,26869,0.24932193756103516,0.009153875525080868
6809,13619,13618,27237,0.25235986709594727,0.009019791735681399
6901,13803,13802,27605,0.2553868293762207,0.008886468925474024
6993,13987,13986,27973,0.2585878372192383,0.008755226716821038
7085,14171,14170,28341,0.2618579864501953,0.008627086769837568
7177,14355,14354,28709,0.2649190425872803,0.008500489270144644
7269,14539,14538,29077,0.26796388626098633,0.00837467713830362
7361,14723,14722,29445,0.2710988521575928,0.008251280956738483
7453,14907,14906,29813,0.27414798736572266,0.008130610773395611
7545,15091,15090,30181,0.277385950088501,0.008011019211173021
7637,15275,15274,30549,0.2804548740386963,0.007892411026808802
7729,15459,15458,30917,0.2835378646850586,0.007776408916869355
7821,15643,15642,31285,0.28659892082214355,0.007662668823448273
7913,15827,15826,31653,0.28995680809020996,0.007549684538308152
8005,16011,16010,32021,0.2930889129638672,0.007437980592296946
8097,16195,16194,32389,0.2961258888244629,0.007328906930188439
8189,16379,16378,32757,0.29921388626098633,0.007221599435818479
8281,16563,16562,33125,0.3022639751434326,0.007114893454830598
8373,16747,16746,33493,0.3052957057952881,0.007009784309752824
8465,16931,16930,33861,0.3086838722229004,0.006907170505784996
8557,17115,17114,34229,0.31262993812561035,0.006805852309551604
8649,17299,17298,34597,0.3160109519958496,0.006705145554521056
8741,17483,17482,34965,0.3197460174560547,0.006606303590934758
8833,17667,17666,35333,0.32364583015441895,0.00650969024630128
8925,17851,17850,35701,0.32773876190185547,0.0064139795675601475
9017,18035,18034,36069,0.3319737911224365,0.006319021842213154
9109,18219,18218,36437,0.3357207775115967,0.006226099648483291
9201,18403,18402,36805,0.33985304832458496,0.006135049484536082
9293,18587,18586,37173,0.3430447578430176,0.006044625538653565
9385,18771,18770,37541,0.34622883796691895,0.0059551771313401
9477,18955,18954,37909,0.3494267463684082,0.005867811575235608
9569,19139,19138,38277,0.35242581367492676,0.005781921752533535
9661,19323,19322,38645,0.3554098606109619,0.005696516761600805
9753,19507,19506,39013,0.3586287498474121,0.005612334439899687
9845,19691,19690,39381,0.3623940944671631,0.005530155018102414
9937,19875,19874,39749,0.3659708499908447,0.005449066741729208
10029,20059,20058,40117,0.3704869747161865,0.005368453044231705
10121,20243,20242,40485,0.37455296516418457,0.00528928126884425
10213,20427,20426,40853,0.37767696380615234,0.005211921077343562
10305,20611,20610,41221,0.3814530372619629,0.005135324544175749
10397,20795,20794,41589,0.38475894927978516,0.005059299806089426
10489,20979,20978,41957,0.3879818916320801,0.004984867427219348
10581,21163,21162,42325,0.39171886444091797,0.004911974961012428
10673,21347,21346,42693,0.39523768424987793,0.00483960876664503
10765,21531,21530,43061,0.3985006809234619,0.004767981818709862
10857,21715,21714,43429,0.40193772315979004,0.004698003895727218
10949,21899,21898,43797,0.4049100875854492,0.0046292538531218915
11041,22083,22082,44165,0.40804386138916016,0.004560899297492278
11133,22267,22266,44533,0.41120409965515137,0.004493478459971572
11225,22451,22450,44901,0.4143657684326172,0.0044276622138280305
11317,22635,22634,45269,0.41753172874450684,0.004362763648054383
11409,22819,22818,45637,0.42069077491760254,0.004298235352024753
11501,23003,23002,46005,0.423969030380249,0.00423482047838585
11593,23187,23186,46373,0.4274108409881592,0.004172873922160172
11685,23371,23370,46741,0.43082284927368164,0.00411157455832226
11777,23555,23554,47109,0.43450474739074707,0.004050709233969751
11869,23739,23738,47477,0.4378170967102051,0.003991088064324712
11961,23923,23922,47845,0.44106292724609375,0.003932729638024072
12053,24107,24106,48213,0.44449400901794434,0.0038748159003099284
12145,24291,24290,48581,0.44770193099975586,0.0038174611177217363
12237,24475,24474,48949,0.45090675354003906,0.003761409868641858
12329,24659,24658,49317,0.4541287422180176,0.003706377429123302
12421,24843,24842,49685,0.4573369026184082,0.0036516705003094996
12513,25027,25026,50053,0.4606049060821533,0.003597675030105616
12605,25211,25210,50421,0.46386289596557617,0.003544962541065537
12697,25395,25394,50789,0.4671778678894043,0.0034930203102200123
12789,25579,25578,51157,0.47052574157714844,0.0034413691704112204
12881,25763,25762,51525,0.47386693954467773,0.0033905760558328277
12973,25947,25946,51893,0.4771907329559326,0.003340970364213177
13065,26131,26130,52261,0.4804999828338623,0.003291912884447345
13157,26315,26314,52629,0.48380279541015625,0.00324318564432765
13249,26499,26498,52997,0.48708295822143555,0.0031954286291914686
13341,26683,26682,53365,0.4903128147125244,0.003148704613357249
13433,26867,26866,53733,0.4936649799346924,0.00310235732335986
13525,27051,27050,54101,0.4970998764038086,0.0030564322704418776
13617,27235,27234,54469,0.5002810955047607,0.00301153564648463
13709,27419,27418,54837,0.5034918785095215,0.00296748237017715
13802,27605,27604,55209,0.5067148208618164,0.0029232247688510565
13894,27789,27788,55577,0.5099108219146729,0.0028799920729198313
13986,27973,27972,55945,0.5130999088287354,0.002837784026206393
14078,28157,28156,56313,0.5163047313690186,0.002796213973889506
14170,28341,28340,56681,0.5194900035858154,0.0027548750466811545
14262,28525,28524,57049,0.5226709842681885,0.002714202596238064
14354,28709,28708,57417,0.5258688926696777,0.0026744865444963558
14446,28893,28892,57785,0.5290298461914062,0.0026352279723371595
14538,29077,29076,58153,0.5322878360748291,0.0025962244417923573
14630,29261,29260,58521,0.5354406833648682,0.0025579813143309675
14722,29445,29444,58889,0.5385949611663818,0.002520577389079624
14814,29629,29628,59257,0.5417459011077881,0.002483488401584202
14906,29813,29812,59625,0.5448949337005615,0.00244672290927499
14998,29997,29996,59993,0.548027753829956,0.0024107705414662364
15090,30181,30180,60361,0.5511698722839355,0.0023755093897748145
15182,30365,30364,60729,0.5545547008514404,0.0023404709603444887
15274,30549,30548,61097,0.5576808452606201,0.002305848710759603
15366,30733,30732,61465,0.5608177185058594,0.0022720428407652267
15458,30917,30916,61833,0.5639488697052002,0.0022387704994310115
15550,31101,31100,62201,0.5670619010925293,0.002205682619806687
15642,31285,31284,62569,0.5701696872711182,0.002173106409813063
15734,31469,31468,62937,0.5732789039611816,0.0021413008140338066
15826,31653,31652,63305,0.5763928890228271,0.0021098818350858825
15918,31837,31836,63673,0.5795199871063232,0.0020786583248123595
16010,32021,32020,64041,0.5826709270477295,0.0020480255909237784
16102,32205,32204,64409,0.5857930183410645,0.002018076781699672
16194,32389,32388,64777,0.5889127254486084,0.0019883952653954903
16286,32573,32572,65145,0.5920729637145996,0.0019589581143590697
16378,32757,32756,65513,0.5951838493347168,0.0019301601572216638
16470,32941,32940,65881,0.5983107089996338,0.0019019321590398102
16562,33125,33124,66249,0.6014308929443359,0.0018738907105203847
16654,33309,33308,66617,0.6045360565185547,0.0018461648039101739
16746,33493,33492,66985,0.6076228618621826,0.001819088005142344
16838,33677,33676,67353,0.610703706741333,0.0017924564172433744
16930,33861,33860,67721,0.6137478351593018,0.0017659733598326956
17022,34045,34044,68089,0.6167778968811035,0.0017398822854565077
17114,34229,34228,68457,0.6201398372650146,0.0017144108535773336
17206,34413,34412,68825,0.6231777667999268,0.001689265607238832
17298,34597,34596,69193,0.6262528896331787,0.0016642710156157894
17390,34781,34780,69561,0.6293270587921143,0.001639734414830561
17482,34965,34964,69929,0.6324248313903809,0.0016157540197184303
17574,35149,35148,70297,0.6358540058135986,0.0015920005061322458
17666,35333,35332,70665,0.6391270160675049,0.0015684317413351921
17758,35517,35516,71033,0.6423628330230713,0.0015453643826312292
17850,35701,35700,71401,0.6455600261688232,0.001522765977641887
17942,35885,35884,71769,0.6487798690795898,0.0015003245088605383
18034,36069,36068,72137,0.6519737243652344,0.0014781219391614172
18126,36253,36252,72505,0.6552140712738037,0.0014564344150894497
18218,36437,36436,72873,0.6583957672119141,0.0014351175988114616
18310,36621,36620,73241,0.6615910530090332,0.001413921423991352
18402,36805,36804,73609,0.6647248268127441,0.0013930249139625951
18494,36989,36988,73977,0.6678519248962402,0.00137262562945294
18586,37173,37172,74345,0.671180009841919,0.001352501044359688
18678,37357,37356,74713,0.6743838787078857,0.001332493340138499
18770,37541,37540,75081,0.6774709224700928,0.0013128399116096488
18862,37725,37724,75449,0.6805398464202881,0.001293637875208591
18954,37909,37908,75817,0.683708906173706,0.0012746283456325092
19046,38093,38092,76185,0.6867880821228027,0.0012557587104176009
19138,38277,38276,76553,0.6898539066314697,0.001237281558909184
19230,38461,38460,76921,0.6933338642120361,0.0012191894235165886
19322,38645,38644,77289,0.6963949203491211,0.0012012297624199484
19414,38829,38828,77657,0.6994607448577881,0.0011834507626099651
19506,39013,39012,78025,0.7025477886199951,0.001166079589095695
19598,39197,39196,78393,0.7056057453155518,0.0011490164151580393
19690,39381,39380,78761,0.7086760997772217,0.0011320520411398768
19782,39565,39564,79129,0.7119648456573486,0.0011153162905194155
19874,39749,39748,79497,0.7154159545898438,0.0010989787153577704
19966,39933,39932,79865,0.7187540531158447,0.0010828720329040848
20058,40117,40116,80233,0.7228279113769531,0.001066856705379939
20150,40301,40300,80601,0.726942777633667,0.0010511148266447404
20242,40485,40484,80969,0.7307219505310059,0.0010357385162341611
20334,40669,40668,81337,0.734126091003418,0.001020525418182849
20426,40853,40852,81705,0.73726487159729,0.0010054184997175743
20518,41037,41036,82073,0.7403688430786133,0.0009906181465103403
20610,41221,41220,82441,0.7434568405151367,0.0009761332181771718
20702,41405,41404,82809,0.7467210292816162,0.0009617603962747527
20794,41589,41588,83177,0.7497859001159668,0.0009475240788049958
20886,41773,41772,83545,0.7528460025787354,0.0009336100177832578
20978,41957,41956,83913,0.7559018135070801,0.0009199512966263509
21070,42141,42140,84281,0.7590289115905762,0.0009063741034302827
21162,42325,42324,84649,0.7621009349822998,0.0008929709936284395
21254,42509,42508,85017,0.7651770114898682,0.0008798860869909449
21346,42693,42692,85385,0.7682909965515137,0.0008669948604328904
21438,42877,42876,85753,0.7713756561279297,0.0008541756206451709
21530,43061,43060,86121,0.7745959758758545,0.0008415669829172735
21622,43245,43244,86489,0.7780818939208984,0.0008292537945099272
21714,43429,43428,86857,0.7815968990325928,0.0008170788279694626
21806,43613,43612,87225,0.7846786975860596,0.0008049847126842493
21898,43797,43796,87593,0.7877590656280518,0.0007931295369762583
21990,43981,43980,87961,0.790848970413208,0.0007815322228549886
22082,44165,44164,88329,0.7940027713775635,0.0007700299401709775
22174,44349,44348,88697,0.7970578670501709,0.000758630750222288
22266,44533,44532,89065,0.8001337051391602,0.0007474856695962054
22358,44717,44716,89433,0.803210973739624,0.0007365518101358489
22450,44901,44900,89801,0.806290864944458,0.0007256856812763278
22542,45085,45084,90169,0.8094608783721924,0.0007149518624211961
22634,45269,45268,90537,0.8126089572906494,0.0007044718150145092
22726,45453,45452,90905,0.8157439231872559,0.0006941538943671782
22818,45637,45636,91273,0.8188779354095459,0.000683893189650795
22910,45821,45820,91641,0.8220169544219971,0.000673794332587639
23003,46007,46006,92013,0.8251907825469971,0.0006638275156875606
23095,46191,46190,92381,0.8283498287200928,0.0006540843958168244
23187,46375,46374,92749,0.8315038681030273,0.0006444037721387139
23279,46559,46558,93117,0.8346889019012451,0.0006349103317802198
23371,46743,46742,93485,0.8378348350524902,0.0006256262788221503
23463,46927,46926,93853,0.8410019874572754,0.0006164216886807709
23555,47111,47110,94221,0.8443520069122314,0.0006072960816901616
23647,47295,47294,94589,0.8474926948547363,0.0005983712988320675
23739,47479,47478,94957,0.8506288528442383,0.0005896195521110122
23831,47663,47662,95325,0.8537647724151611,0.000580923766582953
23923,47847,47846,95693,0.8568968772888184,0.0005723297201342388
24015,48031,48030,96061,0.8600308895111084,0.0005639379506725266
24107,48215,48214,96429,0.8631877899169922,0.0005556801922258856
24199,48399,48398,96797,0.8663218021392822,0.0005474682509700201
24291,48583,48582,97165,0.8694577217102051,0.000539381765412518
24383,48767,48766,97533,0.8728597164154053,0.000531486824106155
24475,48951,48950,97901,0.8759899139404297,0.0005236892902346711
24567,49135,49134,98269,0.879119873046875,0.0005159397254236186
24659,49319,49318,98637,0.8823227882385254,0.0005083354993011119
24751,49503,49502,99005,0.8854577541351318,0.000500901815490136
24843,49687,49686,99373,0.8885948657989502,0.0004935355795258883
24935,49871,49870,99741,0.891746997833252,0.00048622901670188615
25027,50055,50054,100109,0.894881010055542,0.00047908022736870926
25119,50239,50238,100477,0.8980269432067871,0.0004720740311030119
25211,50423,50422,100845,0.9011528491973877,0.00046511477020851516
25303,50607,50606,101213,0.9042809009552002,0.0004582326134909939
25395,50791,50790,101581,0.9073758125305176,0.0004515111950246925
25487,50975,50974,101949,0.9106910228729248,0.00044490153562262523
25579,51159,51158,102317,0.9137389659881592,0.0004383288604413829
25671,51343,51342,102685,0.916801929473877,0.0004318522378578795
25763,51527,51526,103053,0.919853925704956,0.0004255295446283941
25855,51711,51710,103421,0.9229109287261963,0.00041928899218877106
25947,51895,51894,103789,0.925976037979126,0.00041308547636242454
26039,52079,52078,104157,0.9290728569030762,0.00040699456290012906
26131,52263,52262,104525,0.9321348667144775,0.00040104226183364027
26223,52447,52446,104893,0.9351837635040283,0.00039514720792077434
26315,52631,52630,105261,0.9382328987121582,0.0003892972853707478
26407,52815,52814,105629,0.941321849822998,0.0003835710517549981
26499,52999,52998,105997,0.944591760635376,0.00037796206989134523
26591,53183,53182,106365,0.9477019309997559,0.00037239261455918125
26683,53367,53366,106733,0.9508059024810791,0.0003668815144255489
26775,53551,53550,107101,0.9539029598236084,0.00036149788041558463
26867,53735,53734,107469,0.956995964050293,0.00035620724609618644
26959,53919,53918,107837,0.9602007865905762,0.00035094672325064637
27051,54103,54102,108205,0.9633567333221436,0.0003457595884217484
27143,54287,54286,108573,0.966378927230835,0.0003406959010429492
27235,54471,54470,108941,0.9693927764892578,0.00033570135203015144
27327,54655,54654,109309,0.9724118709564209,0.0003307355947374074
27419,54839,54838,109677,0.97568678855896,0.00032585688648647046
27511,55023,55022,110045,0.9786880016326904,0.0003210906037826207
27603,55207,55206,110413,0.98183274269104,0.00031637288585020226
27695,55391,55390,110781,0.984893798828125,0.00031168936181863
27787,55575,55574,111149,0.9878969192504883,0.0003071025988933133
27879,55759,55758,111517,0.9909067153930664,0.000302612042510919
27971,55943,55942,111885,0.9941260814666748,0.00029815487818055114
28063,56127,56126,112253,0.9982666969299316,0.0002937418313315232
28155,56311,56310,112621,1.001399040222168,0.00028942965630062833
28247,56495,56494,112989,1.0048577785491943,0.00028519470163822154
28339,56679,56678,113357,1.0083980560302734,0.00028098446157715976
28431,56863,56862,113725,1.011920690536499,0.00027683018008864066
28523,57047,57046,114093,1.0149848461151123,0.00027277469741664645
28615,57231,57230,114461,1.018054723739624,0.0002687772948166795
28707,57415,57414,114829,1.0211758613586426,0.00026480244633387884
28799,57599,57598,115197,1.0242419242858887,0.0002608947454917893
28891,57783,57782,115565,1.0275566577911377,0.0002570780412482184
28983,57967,57966,115933,1.0316798686981201,0.00025330249982605387
29075,58151,58150,116301,1.034728765487671,0.0002495529328162509
29167,58335,58334,116669,1.0377569198608398,0.00024587889910674944
29259,58519,58518,117037,1.0410187244415283,0.00024228363517333687
29351,58703,58702,117405,1.044050931930542,0.00023871664504777088
29443,58887,58886,117773,1.0470869541168213,0.00023518298353735343
29535,59071,59070,118141,1.050157070159912,0.00023172898208133612
29627,59255,59254,118509,1.053210735321045,0.00022833895885264214
29719,59439,59438,118877,1.056609869003296,0.00022496937036989891
29811,59623,59622,119245,1.059809923171997,0.0002216423683720039
29903,59807,59806,119613,1.0631158351898193,0.0002183942760326975
29995,59991,59990,119981,1.0663390159606934,0.0002151948747093324
30087,60175,60174,120349,1.0697758197784424,0.00021201328840393769
30179,60359,60358,120717,1.0729749202728271,0.00020888338543868234
30271,60543,60542,121085,1.0761499404907227,0.00020582698227116528
30363,60727,60726,121453,1.079225778579712,0.00020280542651222096
30455,60911,60910,121821,1.0824098587036133,0.00019980367058495432
30547,61095,61094,122189,1.086050033569336,0.00019686075002575942
30639,61279,61278,122557,1.089277744293213,0.00019398218559046177
30731,61463,61462,122925,1.0923848152160645,0.00019112759684743527
30823,61647,61646,123293,1.0957558155059814,0.00018829817775929206
30915,61831,61830,123661,1.099118947982788,0.00018553153597171862
31007,62015,62014,124029,1.103700876235962,0.0001828177853676784
31099,62199,62198,124397,1.1068549156188965,0.0001801210407460635
31191,62383,62382,124765,1.1100668907165527,0.00017745664739668646
31283,62567,62566,125133,1.1142728328704834,0.00017485514910571561
31375,62751,62750,125501,1.117645025253296,0.00017229438503124346
31467,62935,62934,125869,1.1209919452667236,0.00016974781579166378
31559,63119,63118,126237,1.1244587898254395,0.00016724094100036357
31651,63303,63302,126605,1.1279900074005127,0.0001647933111090359
31743,63487,63486,126973,1.1327037811279297,0.000162375139604619
31835,63671,63670,127341,1.1366667747497559,0.00015997212859610518
31927,63855,63854,127709,1.1406466960906982,0.0001576148470484503
32019,64039,64038,128077,1.1447679996490479,0.00015531003427065153
32111,64223,64222,128445,1.148852825164795,0.000153025568670073
32204,64409,64408,128817,1.1528089046478271,0.0001507357196500002
32296,64593,64592,129185,1.156742811203003,0.00014852023872539947
32388,64777,64776,129553,1.160951852798462,0.00014634806719079647
32480,64961,64960,129921,1.164931058883667,0.00014418996234632852
32572,65145,65144,130289,1.168968915939331,0.0001420567253070615
32664,65329,65328,130657,1.172881841659546,0.0001399735989880551
32756,65513,65512,131025,1.176736831665039,0.00013792412750918937
32848,65697,65696,131393,1.1806750297546387,0.00013588604433923462
32940,65881,65880,131761,1.185161828994751,0.00013387871627611108
33032,66065,66064,132129,1.1892828941345215,0.0001319189907571077
33124,66249,66248,132497,1.1932127475738525,0.00012998380352270502
33216,66433,66432,132865,1.1970558166503906,0.00012806039365602517
33308,66617,66616,133233,1.2009477615356445,0.00012617273282482548
33400,66801,66800,133601,1.2047626972198486,0.00012432759097872806
33492,66985,66984,133969,1.2088978290557861,0.00012249946869993122
33584,67169,67168,134337,1.2128639221191406,0.00012068591954823159
33676,67353,67352,134705,1.2169508934020996,0.00011891130740768575
33768,67537,67536,135073,1.2209358215332031,0.00011717236318006302
33860,67721,67720,135441,1.2248330116271973,0.00011544523164664802
33952,67905,67904,135809,1.2286341190338135,0.00011373693881526312
34044,68089,68088,136177,1.2321498394012451,0.00011206844299597608
34136,68273,68272,136545,1.235454797744751,0.00011042799661757901
34228,68457,68456,136913,1.2385609149932861,0.00010879676566996014
34320,68641,68640,137281,1.2416789531707764,0.00010718906780628268
34412,68825,68824,137649,1.2447757720947266,0.00010561960226923476
34504,69009,69008,138017,1.2478649616241455,0.00010407081855074509
34596,69193,69192,138385,1.2509469985961914,0.00010253114478593481
34688,69377,69376,138753,1.2542707920074463,0.00010101915080247275
34780,69561,69560,139121,1.2573628425598145,9.954169475425544e-05
34872,69745,69744,139489,1.2604737281799316,9.807868283564972e-05
34964,69929,69928,139857,1.2636327743530273,9.662669737533456e-05
35056,70113,70112,140225,1.2667288780212402,9.520521883726337e-05
35148,70297,70296,140593,1.2698547840118408,9.381305152733659e-05
35240,70481,70480,140961,1.272958755493164,9.243084201482174e-05
35332,70665,70664,141329,1.2761058807373047,9.106288551765075e-05
35424,70849,70848,141697,1.2793610095977783,8.97264697848083e-05
35516,71033,71032,142065,1.2829928398132324,8.841338087642378e-05
35608,71217,71216,142433,1.286167860031128,8.710781248189942e-05
35700,71401,71400,142801,1.2893388271331787,8.582021395160321e-05
35792,71585,71584,143169,1.2925159931182861,8.45632590282526e-05
35884,71769,71768,143537,1.2956998348236084,8.332370263331216e-05
35976,71953,71952,143905,1.2988557815551758,8.209124294470154e-05
36068,72137,72136,144273,1.3020069599151611,8.088016834109727e-05
36160,72321,72320,144641,1.3051578998565674,7.969709026092745e-05
36252,72505,72504,145009,1.3083267211914062,7.852626302123973e-05
36344,72689,72688,145377,1.3115320205688477,7.736379540152425e-05
36436,72873,72872,145745,1.3147029876708984,7.622517873721227e-05
36528,73057,73056,146113,1.3178627490997314,7.511059773932183e-05
36620,73241,73240,146481,1.321030855178833,7.40044352094628e-05
36712,73425,73424,146849,1.3242318630218506,7.290904551952945e-05
36804,73609,73608,147217,1.327401876449585,7.183860134388646e-05
36896,73793,73792,147585,1.3305718898773193,7.078751416145565e-05
36988,73977,73976,147953,1.3337268829345703,6.974261291654458e-05
37080,74161,74160,148321,1.336869716644287,6.871140616167696e-05
37172,74345,74344,148689,1.3400428295135498,6.770471023668523e-05
37264,74529,74528,149057,1.3432047367095947,6.67126217279365e-05
37356,74713,74712,149425,1.3463380336761475,6.57261051695689e-05
37448,74897,74896,149793,1.3495237827301025,6.475607441240769e-05
37540,75081,75080,150161,1.3526699542999268,6.3808690626651e-05
37632,75265,75264,150529,1.3558619022369385,6.2871687281339e-05
37724,75449,75448,150897,1.3590219020843506,6.19410397507409e-05
37816,75633,75632,151265,1.3621890544891357,6.102899934618879e-05
37908,75817,75816,151633,1.3653669357299805,6.01366264621373e-05
38000,76001,76000,152001,1.3685307502746582,5.9251385215877865e-05
38092,76185,76184,152369,1.371727705001831,5.837428118606883e-05
38184,76369,76368,152737,1.375020980834961,5.751686541022279e-05
38276,76553,76552,153105,1.3782026767730713,5.667547729530797e-05
38368,76737,76736,153473,1.3813939094543457,5.583921373994054e-05
38460,76921,76920,153841,1.3847479820251465,5.5013366726423775e-05
38552,77105,77104,154209,1.388199806213379,5.4207084934912894e-05
38644,77289,77288,154577,1.39158296585083,5.3413041978584466e-05
38736,77473,77472,154945,1.3948557376861572,5.262341088468392e-05
38828,77657,77656,155313,1.3982629776000977,5.1846461084870695e-05
38920,77841,77840,155681,1.401702880859375,5.1087793041045336e-05
39012,78025,78024,156049,1.4054667949676514,5.033790943860535e-05
39104,78209,78208,156417,1.4087069034576416,4.9592876379506964e-05
39196,78393,78392,156785,1.4119117259979248,4.886232816311029e-05
39288,78577,78576,157153,1.4153509140014648,4.814783899776332e-05
39380,78761,78760,157521,1.4186148643493652,4.743939909359214e-05
39472,78945,78944,157889,1.4221539497375488,4.673710432692097e-05
39564,79129,79128,158257,1.4253718852996826,4.6050315993169464e-05
39656,79313,79312,158625,1.4290800094604492,4.537676966340512e-05
39748,79497,79496,158993,1.4325637817382812,4.4707495123863185e-05
39840,79681,79680,159361,1.43611478805542,4.404612978512394e-05
39932,79865,79864,159729,1.439760684967041,4.340034988785914e-05
40024,80049,80048,160097,1.4430017471313477,4.276480268567078e-05
40116,80233,80232,160465,1.4461658000946045,4.2132779607193874e-05
40208,80417,80416,160833,1.449558973312378,4.1510490252938005e-05
40300,80601,80600,161201,1.452678918838501,4.0902928440187974e-05
40392,80785,80784,161569,1.4557888507843018,4.030278928177927e-05
40484,80969,80968,161937,1.4590749740600586,3.970636946595362e-05
40576,81153,81152,162305,1.462212085723877,3.912120100036371e-05
40668,81337,81336,162673,1.4653937816619873,3.8549117494467944e-05
40760,81521,81520,163041,1.4688518047332764,3.798216832895614e-05
40852,81705,81704,163409,1.4721028804779053,3.741986134984287e-05
40944,81889,81888,163777,1.4752418994903564,3.686974150509078e-05
41036,82073,82072,164145,1.478468656539917,3.6330538365849425e-05
41128,82257,82256,164513,1.48164701461792,3.579491490897561e-05
41220,82441,82440,164881,1.48478364944458,3.5265287205416156e-05
41312,82625,82624,165249,1.487973690032959,3.474804915706128e-05
41405,82811,82810,165621,1.491170883178711,3.423383577801234e-05
41497,82995,82994,165989,1.4943747520446777,3.3728014419914725e-05
41589,83179,83178,166357,1.4976539611816406,3.3229731318770864e-05
41681,83363,83362,166725,1.500878095626831,3.274327645723261e-05
41773,83547,83546,167093,1.5040650367736816,3.226300226113365e-05
41865,83731,83730,167461,1.5074667930603027,3.17856210681262e-05
41957,83915,83914,167829,1.510732889175415,3.131703155466878e-05
42049,84099,84098,168197,1.5141229629516602,3.085904094920132e-05
42141,84283,84282,168565,1.5173537731170654,3.0405344941111286e-05
42233,84467,84466,168933,1.5207369327545166,2.995520827208897e-05
42325,84651,84650,169301,1.5240318775177002,2.9514679264135573e-05
42417,84835,84834,169669,1.527297019958496,2.9083070611518622e-05
42509,85019,85018,170037,1.5306627750396729,2.865443588074632e-05
42601,85203,85202,170405,1.5339078903198242,2.8230403498108074e-05
42693,85387,85386,170773,1.5376529693603516,2.7816222792332867e-05
42785,85571,85570,171141,1.540855884552002,2.740908075221723e-05
42877,85755,85754,171509,1.5440268516540527,2.7004236491061818e-05
42969,85939,85938,171877,1.5472629070281982,2.6605156936054884e-05
43061,86123,86122,172245,1.5507798194885254,2.621557181336792e-05
43153,86307,86306,172613,1.553924798965454,2.583119327747372e-05
43245,86491,86490,172981,1.5570869445800781,2.5449056796196093e-05
43337,86675,86674,173349,1.56026291847229,2.5073723340612524e-05
43429,86859,86858,173717,1.5634608268737793,2.4706994244047708e-05
43521,87043,87042,174085,1.5671920776367188,2.434390939003425e-05
43613,87227,87226,174453,1.5703299045562744,2.398351893846167e-05
43705,87411,87410,174821,1.5736486911773682,2.3630651502917647e-05
43797,87595,87594,175189,1.5769257545471191,2.328511019150104e-05
43889,87779,87778,175557,1.581188678741455,2.2942078093906787e-05
43981,87963,87962,175925,1.5851819515228271,2.260252695875759e-05
44073,88147,88146,176293,1.5892317295074463,2.2270779115250287e-05
44165,88331,88330,176661,1.5932908058166504,2.1944881248121035e-05
44257,88515,88514,177029,1.597242832183838,2.1620862855580365e-05
44349,88699,88698,177397,1.602186918258667,2.1301243883609585e-05
44441,88883,88882,177765,1.6062090396881104,2.098923039231683e-05
44533,89067,89066,178133,1.6103878021240234,2.0681594511522806e-05
44625,89251,89250,178501,1.614853858947754,2.0375708953653403e-05
44717,89435,89434,178869,1.6188938617706299,2.0075076092585686e-05
44809,89619,89618,179237,1.6231749057769775,1.9781413850960533e-05
44901,89803,89802,179605,1.6272900104522705,1.949084173697625e-05
44993,89987,89986,179973,1.6314187049865723,1.9202313818962258e-05
45085,90171,90170,180341,1.6354148387908936,1.8919663992451438e-05
45177,90355,90354,180709,1.6394329071044922,1.864301807003898e-05
45269,90539,90538,181077,1.6434028148651123,1.8368494870961034e-05
45361,90723,90722,181445,1.6473829746246338,1.8096602105638193e-05
45453,90907,90906,181813,1.6514108180999756,1.7830877320151142e-05
45545,91091,91090,182181,1.655332088470459,1.757000394751281e-05
45637,91275,91274,182549,1.659390926361084,1.731067976310692e-05
45729,91459,91458,182917,1.6632299423217773,1.7054706462987048e-05
45821,91643,91642,183285,1.6669859886169434,1.6804813018788805e-05
45913,91827,91826,183653,1.6702418327331543,1.6558592806737146e-05
46005,92011,92010,184021,1.6735877990722656,1.631375006165987e-05
46097,92195,92194,184389,1.6768648624420166,1.607295413774309e-05
46189,92379,92378,184757,1.6799979209899902,1.5837793598333784e-05
46281,92563,92562,185125,1.6831169128417969,1.5605250532703724e-05
46373,92747,92746,185493,1.6862719058990479,1.5374263170426554e-05
46465,92931,92930,185861,1.6895079612731934,1.5147858760384209e-05
46557,93115,93114,186229,1.692713975906372,1.4926364176029328e-05
46649,93299,93298,186597,1.6958699226379395,1.4706668621450579e-05
46741,93483,93482,186965,1.6989870071411133,1.4488959743017292e-05
46833,93667,93666,187333,1.7020957469940186,1.4276116071523892e-05
46925,93851,93850,187701,1.7053358554840088,1.4067286909670315e-05
47017,94035,94034,188069,1.7087829113006592,1.385974350602618e-05
47109,94219,94218,188437,1.7122538089752197,1.3654747601262728e-05
47201,94403,94402,188805,1.7162039279937744,1.3454601993220232e-05
47293,94587,94586,189173,1.7198498249053955,1.3257532186414114e-05
47385,94771,94770,189541,1.7237379550933838,1.3061555737262826e-05
47477,94955,94954,189909,1.7276558876037598,1.2868690301076494e-05
47569,95139,95138,190277,1.731994867324829,1.2680371376939848e-05
47661,95323,95322,190645,1.7362878322601318,1.2494266595672808e-05
47753,95507,95506,191013,1.7402429580688477,1.2309350544013742e-05
47845,95691,95690,191381,1.7444558143615723,1.2127999938791617e-05
47937,95875,95874,191749,1.7487258911132812,1.195065594080364e-05
48029,96059,96058,192117,1.7528009414672852,1.177483829486249e-05
48121,96243,96242,192485,1.7567808628082275,1.1600521012361327e-05
48213,96427,96426,192853,1.7611229419708252,1.1430033284620457e-05
48305,96611,96610,193221,1.7654709815979004,1.126286029179358e-05
48397,96795,96794,193589,1.7694189548492432,1.1096760793572647e-05
48489,96979,96978,193957,1.7733068466186523,1.0932594679385211e-05
48581,97163,97162,194325,1.7772448062896729,1.0772290015615763e-05
48673,97347,97346,194693,1.7816798686981201,1.061455543043811e-05
48765,97531,97530,195061,1.7857089042663574,1.0457696391512224e-05
48857,97715,97714,195429,1.7896790504455566,1.0303223814635578e-05
48949,97899,97898,195797,1.79355788230896,1.0152411720682767e-05
49041,98083,98082,196165,1.7975788116455078,1.0003469666979112e-05
49133,98267,98266,196533,1.8013899326324463,9.855440500072648e-06
49225,98451,98450,196901,1.8052637577056885,9.710179152458424e-06
49317,98635,98634,197269,1.808816909790039,9.568180460220801e-06
49409,98819,98818,197637,1.8130989074707031,9.427477355500529e-06
49501,99003,99002,198005,1.816951036453247,9.287907882171835e-06
49593,99187,99186,198373,1.820734977722168,9.151346415409136e-06
49685,99371,99370,198741,1.8282699584960938,9.017515940989037e-06
49777,99555,99554,199109,1.8331959247589111,8.884586209173781e-06
49869,99739,99738,199477,1.8378417491912842,8.75312151133968e-06
49961,99923,99922,199845,1.8426527976989746,8.624724689292646e-06
50053,100107,100106,200213,1.8473179340362549,8.498470752845257e-06
50145,100291,100290,200581,1.8513987064361572,8.37292415815893e-06
50237,100475,100474,200949,1.8557188510894775,8.249204343181273e-06
50329,100659,100658,201317,1.8603029251098633,8.128425599961472e-06
50421,100843,100842,201685,1.864607810974121,8.009223535187804e-06
50513,101027,101026,202053,1.8685507774353027,7.890726736528382e-06
50606,101213,101212,202425,1.8725159168243408,7.7731255090043e-06
50698,101397,101396,202793,1.8772828578948975,7.659445391578745e-06
50790,101581,101580,203161,1.8839709758758545,7.546848914996893e-06
50882,101765,101764,203529,1.8954589366912842,7.4351218706676315e-06
50974,101949,101948,203897,1.905951976776123,7.325765103288293e-06
51066,102133,102132,204265,1.9154908657073975,7.21863888556665e-06
51158,102317,102316,204633,1.9212448596954346,7.112261583235777e-06
51250,102501,102500,205001,1.9258978366851807,7.0070085388562e-06
51342,102685,102684,205369,1.9331018924713135,6.904193856819248e-06
51434,102869,102868,205737,1.938750982284546,6.803145135460273e-06
51526,103053,103052,206105,1.9498028755187988,6.702669723995047e-06
51618,103237,103236,206473,1.9575488567352295,6.603606215051896e-06
51710,103421,103420,206841,1.966156005859375,6.506900122446223e-06
51802,103605,103604,207209,1.9729828834533691,6.4115045720056315e-06
51894,103789,103788,207577,1.9817798137664795,6.316661136491317e-06
51986,103973,103972,207945,1.990710973739624,6.2234894299689755e-06
52078,104157,104156,208313,1.9952607154846191,6.1324609526712e-06
52170,104341,104340,208681,2.000324010848999,6.042351861241501e-06
52262,104525,104524,209049,2.004584789276123,5.952901284826049e-06
52354,104709,104708,209417,2.0095858573913574,5.86530556996465e-06
52446,104893,104892,209785,2.018254041671753,5.779540652275084e-06
52538,105077,105076,210153,2.0238289833068848,5.694408151173242e-06
52630,105261,105260,210521,2.0306448936462402,5.6101257314999054e-06
52722,105445,105444,210889,2.036489963531494,5.527773552954146e-06
52814,105629,105628,211257,2.0410397052764893,5.446888194809428e-06
52906,105813,105812,211625,2.0459299087524414,5.3664728302174834e-06
52998,105997,105996,211993,2.050286054611206,5.287134372217573e-06
53090,106181,106180,212361,2.0543737411499023,5.209683220904636e-06
53182,106365,106364,212729,2.0590689182281494,5.1333333353355e-06
53274,106549,106548,213097,2.06369686126709,5.057415424333019e-06
53366,106733,106732,213465,2.0679500102996826,4.9827874788590494e-06
53458,106917,106916,213833,2.0718798637390137,4.909894802739924e-06
53550,107101,107100,214201,2.076019763946533,4.8377815077350455e-06
53642,107285,107284,214569,2.080256938934326,4.766168207446825e-06
53734,107469,107468,214937,2.0842888355255127,4.696003320080647e-06
53826,107653,107652,215305,2.0888419151306152,4.6273379016286084e-06
53918,107837,107836,215673,2.093397855758667,4.559207806712362e-06
54010,108021,108020,216041,2.098724842071533,4.491719964782375e-06
54102,108205,108204,216409,2.103649854660034,4.425756952066058e-06
54194,108389,108388,216777,2.1081619262695312,4.361009629479392e-06
54286,108573,108572,217145,2.113292932510376,4.2966504940132375e-06
54378,108757,108756,217513,2.1184029579162598,4.233111159542061e-06
54470,108941,108940,217881,2.1229679584503174,4.171079672974764e-06
54562,109125,109124,218249,2.1272568702697754,4.109971717453928e-06
54654,109309,109308,218617,2.132246971130371,4.049204524590929e-06
54746,109493,109492,218985,2.136502981185913,3.989430545541519e-06
54838,109677,109676,219353,2.140605926513672,3.931058622930314e-06
54930,109861,109860,219721,2.144758939743042,3.873346637110213e-06
55022,110045,110044,220089,2.149423837661743,3.81601556079516e-06
55114,110229,110228,220457,2.1534457206726074,3.7598130751159652e-06
55206,110413,110412,220825,2.157482862472534,3.7048360775952642e-06
55298,110597,110596,221193,2.1614677906036377,3.6503129430104537e-06
55390,110781,110780,221561,2.1659319400787354,3.596274846284648e-06
55482,110965,110964,221929,2.1698007583618164,3.5434388003871635e-06
55574,111149,111148,222297,2.1744418144226074,3.49160810924687e-06
55666,111333,111332,222665,2.178309679031372,3.440100169521357e-06
55758,111517,111516,223033,2.1828088760375977,3.389215167415865e-06
55850,111701,111700,223401,2.1867990493774414,3.339532376368276e-06
55942,111885,111884,223769,2.1907238960266113,3.290622449149744e-06
56034,112069,112068,224137,2.194525957107544,3.241983671444466e-06
56126,112253,112252,224505,2.1988730430603027,3.1941079657915138e-06
56218,112437,112436,224873,2.2027478218078613,3.147362752188188e-06
56310,112621,112620,225241,2.2065017223358154,3.101175549887865e-06
56402,112805,112804,225609,2.210233688354492,3.055279787639796e-06
56494,112989,112988,225977,2.2141668796539307,3.01026150853323e-06
56586,113173,113172,226345,2.2179577350616455,2.9662426785263205e-06
56678,113357,113356,226713,2.2217679023742676,2.9226089918872275e-06
56770,113541,113540,227081,2.22541880607605,2.8793416394585464e-06
56862,113725,113724,227449,2.2289090156555176,2.837019896178758e-06
56954,113909,113908,227817,2.233220100402832,2.79552775269708e-06
57046,114093,114092,228185,2.2370927333831787,2.754305483737775e-06
57138,114277,114276,228553,2.24059796333313,2.713555766992273e-06
57230,114461,114460,228921,2.2438528537750244,2.6737626065491253e-06
57322,114645,114644,229289,2.2477848529815674,2.6346148450054686e-06
57414,114829,114828,229657,2.2511448860168457,2.5956847607595452e-06
57506,115013,115012,230025,2.2548367977142334,2.5573396775331364e-06
57598,115197,115196,230393,2.258612871170044,2.51990424654169e-06
57690,115381,115380,230761,2.262126922607422,2.482939882433658e-06
57782,115565,115564,231129,2.266615867614746,2.4461996870959995e-06
57874,115749,115748,231497,2.270495891571045,2.410140253737719e-06
57966,115933,115932,231865,2.2744288444519043,2.374894207759181e-06
58058,116117,116116,232233,2.2782938480377197,2.339975084804948e-06
58150,116301,116300,232601,2.2828190326690674,2.3053328213474158e-06
58242,116485,116484,232969,2.286733865737915,2.2714328631210565e-06
58334,116669,116668,233337,2.2905867099761963,2.2382159894646906e-06
58426,116853,116852,233705,2.294416904449463,2.2052258385120026e-06
58518,117037,117036,234073,2.298923969268799,2.1725936235905645e-06
58610,117221,117220,234441,2.302806854248047,2.1407209385050955e-06
58702,117405,117404,234809,2.3067398071289062,2.1093860462365374e-06
58794,117589,117588,235177,2.310321807861328,2.078227444137373e-06
58886,117773,117772,235545,2.3144898414611816,2.0475163818937188e-06
58978,117957,117956,235913,2.3183627128601074,2.017535770351453e-06
59070,118141,118140,236281,2.3220467567443848,1.987952122668098e-06
59162,118325,118324,236649,2.3257877826690674,1.958541983114862e-06
59254,118509,118508,237017,2.3301098346710205,1.9296588343813625e-06
59346,118693,118692,237385,2.3337740898132324,1.901436263974041e-06
59438,118877,118876,237753,2.337484836578369,1.8734911344299346e-06
59530,119061,119060,238121,2.3413407802581787,1.8457555177207082e-06
59622,119245,119244,238489,2.3452558517456055,1.8186013746163903e-06
59714,119429,119428,238857,2.349745750427246,1.7920084622515903e-06
59807,119615,119614,239229,2.353698968887329,1.765320539497484e-06
59899,119799,119798,239597,2.357844829559326,1.739194761234816e-06
59991,119983,119982,239965,2.361860752105713,1.7136723959477597e-06
60083,120167,120166,240333,2.366259813308716,1.6885930229792115e-06
60175,120351,120350,240701,2.3701658248901367,1.663656787593153e-06
60267,120535,120534,241069,2.3740367889404297,1.6390663021698213e-06
60359,120719,120718,241437,2.3779077529907227,1.6150610548566654e-06
60451,120903,120902,241805,2.3828608989715576,1.59138563090384e-06
60543,121087,121086,242173,2.3868677616119385,1.5678462492134508e-06
60635,121271,121270,242541,2.390944004058838,1.5447175951763247e-06
60727,121455,121454,242909,2.394775867462158,1.522122702060111e-06
60819,121639,121638,243277,2.3993446826934814,1.4997597403039881e-06
60911,121823,121822,243645,2.40321683883667,1.4775577518582697e-06
61003,122007,122006,244013,2.407130718231201,1.4558130166670544e-06
61095,122191,122190,244381,2.41104793548584,1.4345257192476995e-06
61187,122375,122374,244749,2.4156017303466797,1.4133978450722487e-06
61279,122559,122558,245117,2.419583797454834,1.3924775548315298e-06
61371,122743,122742,245485,2.423480987548828,1.3720346545789081e-06
61463,122927,122926,245853,2.4274449348449707,1.3519594801125564e-06
61555,123111,123110,246221,2.4316799640655518,1.3320019053905342e-06
61647,123295,123294,246589,2.435670852661133,1.3123078990941918e-06
61739,123479,123478,246957,2.439525842666626,1.2930821530613655e-06
61831,123663,123662,247325,2.443380832672119,1.2741334051532646e-06
61923,123847,123846,247693,2.447746992111206,1.2552913371918956e-06
62015,124031,124030,248061,2.451687812805176,1.2367660059257572e-06
62107,124215,124214,248429,2.4556047916412354,1.2186725821550857e-06
62199,124399,124398,248797,2.4592947959899902,1.2007757130707108e-06
62291,124583,124582,249165,2.4627137184143066,1.1830011714853004e-06
62383,124767,124766,249533,2.4663538932800293,1.1655834701370917e-06
62475,124951,124950,249901,2.4696288108825684,1.1485401960480685e-06
62567,125135,125134,250269,2.4743947982788086,1.1316319408194742e-06
62659,125319,125318,250637,2.4779508113861084,1.1148804944713148e-06
62751,125503,125502,251005,2.481820821762085,1.0985059489796587e-06
62843,125687,125686,251373,2.4851748943328857,1.0824359838430798e-06
62935,125871,125870,251741,2.4883267879486084,1.0664633399489234e-06
63027,126055,126054,252109,2.4914920330047607,1.0506912328515274e-06
63119,126239,126238,252477,2.4946188926696777,1.0352930216805616e-06
63211,126423,126422,252845,2.4984917640686035,1.0201269677651834e-06
63303,126607,126606,253213,2.501677989959717,1.0050452712568984e-06
63395,126791,126790,253581,2.5048539638519287,9.90207297721576e-07
63487,126975,126974,253949,2.508335828781128,9.757180916840834e-07
63579,127159,127158,254317,2.5117719173431396,9.61395255057095e-07
63671,127343,127342,254685,2.515596866607666,9.471657150159839e-07
63763,127527,127526,255053,2.5187788009643555,9.332140519383784e-07
63855,127711,127710,255421,2.5219650268554688,9.195682180025032e-07
63947,127895,127894,255789,2.5251410007476807,9.06036893652636e-07
64039,128079,128078,256157,2.528373956680298,8.926239897082545e-07
64131,128263,128262,256525,2.5322988033294678,8.795080277572993e-07
64223,128447,128446,256893,2.5354979038238525,8.66643793357391e-07
64315,128631,128630,257261,2.5386757850646973,8.538606127799567e-07
64407,128815,128814,257629,2.5418388843536377,8.412297381316202e-07
64499,128999,128998,257997,2.5450069904327393,8.288967987743431e-07
64591,129183,129182,258365,2.548513889312744,8.16758025732284e-07
64683,129367,129366,258733,2.5515859127044678,8.046865445727458e-07
64775,129551,129550,259101,2.554785966873169,7.928021984072206e-07
64867,129735,129734,259469,2.5578837394714355,7.811989034627063e-07
64959,129919,129918,259837,2.56095290184021,7.697362211598206e-07
65051,130103,130102,260205,2.5644609928131104,7.583450211601594e-07
65143,130287,130286,260573,2.567713975906372,7.471697388873002e-07
65235,130471,130470,260941,2.5709590911865234,7.362437275856207e-07
65327,130655,130654,261309,2.5741429328918457,7.254149014309173e-07
65419,130839,130838,261677,2.5774667263031006,7.146755253210288e-07
65511,131023,131022,262045,2.5807547569274902,7.041696035285491e-07
65603,131207,131206,262413,2.5839180946350098,6.93871275026785e-07
65695,131391,131390,262781,2.5870649814605713,6.836408178423017e-07
65787,131575,131574,263149,2.590197801589966,6.73525846734932e-07
65879,131759,131758,263517,2.5933308601379395,6.636477942983871e-07
65971,131943,131942,263885,2.5965678691864014,6.539317867154504e-07
66063,132127,132126,264253,2.5996909141540527,6.442699357310241e-07
66155,132311,132310,264621,2.6028027534484863,6.347514637935887e-07
66247,132495,132494,264989,2.6059539318084717,6.254590089788171e-07
66339,132679,132678,265357,2.6091368198394775,6.162852000504347e-07
66431,132863,132862,265725,2.6121788024902344,6.071664655509188e-07
66523,133047,133046,266093,2.6152329444885254,5.982151394545897e-07
66615,133231,133230,266461,2.618295907974243,5.894665588426769e-07
66707,133415,133414,266829,2.621387004852295,5.808004710641922e-07
66799,133599,133598,267197,2.6244308948516846,5.722020059150687e-07
66891,133783,133782,267565,2.6274828910827637,5.637866932018878e-07
66983,133967,133966,267933,2.6305787563323975,5.555422063759707e-07
67075,134151,134150,268301,2.6336419582366943,5.473548040285671e-07
67167,134335,134334,268669,2.636704921722412,5.392548435516664e-07
67259,134519,134518,269037,2.6398699283599854,5.31342892797195e-07
67351,134703,134702,269405,2.642974853515625,5.235658866898261e-07
67443,134887,134886,269773,2.646021842956543,5.158328467751338e-07
67535,135071,135070,270141,2.6491448879241943,5.082094309648405e-07
67627,135255,135254,270509,2.6522018909454346,5.007674017519056e-07
67719,135439,135438,270877,2.6552507877349854,4.934253018651696e-07
67811,135623,135622,271245,2.6583499908447266,4.861259124813136e-07
67903,135807,135806,271613,2.661500930786133,4.78956037153505e-07
67995,135991,135990,271981,2.6647279262542725,4.7195072100357624e-07
68087,136175,136174,272349,2.6680078506469727,4.650154016496582e-07
68179,136359,136358,272717,2.6710798740386963,4.5813128136981737e-07
68271,136543,136542,273085,2.67413592338562,4.51390544389617e-07
68363,136727,136726,273453,2.6774237155914307,4.447900747643303e-07
68455,136911,136910,273821,2.680630922317505,4.3823778350699744e-07
68547,137095,137094,274189,2.6836347579956055,4.317516218307784e-07
68639,137279,137278,274557,2.6867129802703857,4.254143489738181e-07
68731,137463,137462,274925,2.689769983291626,4.191892079478661e-07
68823,137647,137646,275293,2.6928207874298096,4.1300005667157706e-07
68915,137831,137830,275661,2.6958320140838623,4.0689455064130484e-07
69008,138017,138016,276033,2.6988778114318848,4.008701770360746e-07
69100,138201,138200,276401,2.701889991760254,3.9499436239904666e-07
69192,138385,138384,276769,2.7049100399017334,3.891520895720616e-07
69284,138569,138568,277137,2.7079317569732666,3.8341071099210205e-07
69376,138753,138752,277505,2.710941791534424,3.778022409984312e-07
69468,138937,138936,277873,2.713993787765503,3.7225227543877414e-07
69560,139121,139120,278241,2.7170989513397217,3.6674166811410643e-07
69652,139305,139304,278609,2.7201168537139893,3.613437617972865e-07
69744,139489,139488,278977,2.723106861114502,3.560601300913546e-07
69836,139673,139672,279345,2.7261109352111816,3.508166936206776e-07
69928,139857,139856,279713,2.7292089462280273,3.456239448463449e-07
70020,140041,140040,280081,2.732200860977173,3.405492452698748e-07
70112,140225,140224,280449,2.7351889610290527,3.355667169420309e-07
70204,140409,140408,280817,2.7383317947387695,3.3061363094411606e-07
70296,140593,140592,281185,2.7413768768310547,3.257250423791776e-07
70388,140777,140776,281553,2.7459449768066406,3.209526150361991e-07
70480,140961,140960,281921,2.7489819526672363,3.1624984883003106e-07
70572,141145,141144,282289,2.752023935317993,3.115734457695158e-07
70664,141329,141328,282657,2.7550859451293945,3.069748003707734e-07
70756,141513,141512,283025,2.7581207752227783,3.0248363877858703e-07
70848,141697,141696,283393,2.7611560821533203,2.980420420999958e-07
70940,141881,141880,283761,2.764188766479492,2.9363038238656585e-07
71032,142065,142064,284129,2.7672338485717773,2.8930662098144237e-07
71124,142249,142248,284497,2.7702760696411133,2.850763406802825e-07
71216,142433,142432,284865,2.773348808288574,2.8088011848112786e-07
71308,142617,142616,285233,2.7765679359436035,2.7672218098428196e-07
71400,142801,142800,285601,2.779857873916626,2.726573887165271e-07
71492,142985,142984,285969,2.782939910888672,2.686688930643806e-07
71584,143169,143168,286337,2.7861807346343994,2.6470480891752743e-07
71676,143353,143352,286705,2.7893028259277344,2.607897723549909e-07
71768,143537,143536,287073,2.7924447059631348,2.569674343286753e-07
71860,143721,143720,287441,2.795522928237915,2.532034462099721e-07
71952,143905,143904,287809,2.798628807067871,2.494603557670797e-07
72044,144089,144088,288177,2.8016769886016846,2.457770617555563e-07
72136,144273,144272,288545,2.8047258853912354,2.4218051088831766e-07
72228,144457,144456,288913,2.8078126907348633,2.3862589666236426e-07
72320,144641,144640,289281,2.810837984085083,2.3509414200655038e-07
72412,144825,144824,289649,2.813823938369751,2.316307932448817e-07
72504,145009,145008,290017,2.8168368339538574,2.2824375343005503e-07
72596,145193,145192,290385,2.820006847381592,2.248856059999347e-07
72688,145377,145376,290753,2.8230838775634766,2.215563710227698e-07
72780,145561,145560,291121,2.8263838291168213,2.1830047719170854e-07
72872,145745,145744,291489,2.8293817043304443,2.1510760165813658e-07
72964,145929,145928,291857,2.832537889480591,2.1193509026390194e-07
73056,146113,146112,292225,2.835510015487671,2.0879981223084403e-07
73148,146297,146296,292593,2.8385887145996094,2.0573835726373788e-07
73240,146481,146480,292961,2.8419268131256104,2.027256743028505e-07
73332,146665,146664,293329,2.845036029815674,1.9972970315623865e-07
73424,146849,146848,293697,2.8480587005615234,1.967796169962621e-07
73516,147033,147032,294065,2.8511528968811035,1.938993914183223e-07
73608,147217,147216,294433,2.854118824005127,1.910545939592078e-07
73700,147401,147400,294801,2.857132911682129,1.8822733695235854e-07
73792,147585,147584,295169,2.8604609966278076,1.8545320047171757e-07
73884,147769,147768,295537,2.8639578819274902,1.8274122384604483e-07
73976,147953,147952,295905,2.8673038482666016,1.8005377067949832e-07
74068,148137,148136,296273,2.870283842086792,1.7738816048590484e-07
74160,148321,148320,296641,2.8733038902282715,1.7478017635370718e-07
74252,148505,148504,297009,2.876476764678955,1.7222412993434655e-07
74344,148689,148688,297377,2.8800058364868164,1.6968515864046426e-07
74436,148873,148872,297745,2.8834497928619385,1.671744075165066e-07
74528,149057,149056,298113,2.886676788330078,1.647223264559211e-07
74620,149241,149240,298481,2.889785051345825,1.6231092412275653e-07
74712,149425,149424,298849,2.8928399085998535,1.599130049490345e-07
74804,149609,149608,299217,2.8962349891662598,1.5755022094741314e-07
74896,149793,149792,299585,2.8993687629699707,1.5524358520297518e-07
74988,149977,149976,299953,2.9030299186706543,1.529668280475569e-07
75080,150161,150160,300321,2.906719923019409,1.5070360877230715e-07
75172,150345,150344,300689,2.9098358154296875,1.484815502718769e-07
75264,150529,150528,301057,2.91290283203125,1.4631001982490972e-07
75356,150713,150712,301425,2.9159939289093018,1.4415930427632923e-07
75448,150897,150896,301793,2.919081926345825,1.4202510746665474e-07
75540,151081,151080,302161,2.922212839126587,1.3993609304816032e-07
75632,151265,151264,302529,2.925407886505127,1.3788979145292274e-07
75724,151449,151448,302897,2.9284868240356445,1.3585786658454815e-07
75816,151633,151632,303265,2.9324939250946045,1.3384730129323495e-07
75908,151817,151816,303633,2.9363648891448975,1.3188326720085005e-07
76000,152001,152000,304001,2.939687728881836,1.2995308794779066e-07
76092,152185,152184,304369,2.943066120147705,1.2803388096782385e-07
76184,152369,152368,304737,2.9464218616485596,1.261415218568605e-07
76276,152553,152552,305105,2.95033597946167,1.242941975609794e-07
76368,152737,152736,305473,2.9537429809570312,1.2247202502767481e-07
76460,152921,152920,305841,2.9569778442382812,1.2066037223085554e-07
76552,153105,153104,306209,2.96042799949646,1.1888054346201887e-07
76644,153289,153288,306577,2.964569091796875,1.171417018683478e-07
76736,153473,153472,306945,2.9681639671325684,1.1542051898111911e-07
76828,153657,153656,307313,2.971881866455078,1.1371185001345835e-07
76920,153841,153840,307681,2.975665807723999,1.1203853133173611e-07
77012,154025,154024,308049,2.979844808578491,1.1040026341583744e-07
77104,154209,154208,308417,2.98393177986145,1.0877413908066418e-07
77196,154393,154392,308785,2.9879610538482666,1.0716416379385071e-07
77288,154577,154576,309153,2.9919819831848145,1.0559101595069752e-07
77380,154761,154760,309521,2.9958860874176025,1.0404598233060232e-07
77472,154945,154944,309889,2.9996910095214844,1.0250995037428603e-07
77564,155129,155128,310257,3.0030970573425293,1.0099439233830102e-07
77656,155313,155312,310625,3.006398916244507,9.951488135418969e-08
77748,155497,155496,310993,3.009777784347534,9.805650168434392e-08
77840,155681,155680,311361,3.0132648944854736,9.660635889522634e-08
77932,155865,155864,311729,3.0165958404541016,9.518076754130286e-08
78024,156049,156048,312097,3.0199568271636963,9.378835495371751e-08
78116,156233,156232,312465,3.0231449604034424,9.241091054569536e-08
78209,156419,156418,312837,3.026371955871582,9.102822078893593e-08
78301,156603,156602,313205,3.0296969413757324,8.968824640006383e-08
78393,156787,156786,313573,3.0330920219421387,8.837681461361381e-08
78485,156971,156970,313941,3.036357879638672,8.7075518782072e-08
78577,157155,157154,314309,3.039508819580078,8.578659925401548e-08
78669,157339,157338,314677,3.042613983154297,8.45268661223366e-08
78761,157523,157522,315045,3.045722007751465,8.32902318842664e-08
78853,157707,157706,315413,3.0489490032196045,8.206097296289424e-08
78945,157891,157890,315781,3.0520570278167725,8.084749474037858e-08
79037,158075,158074,316149,3.0551679134368896,7.9662827894006e-08
79129,158259,158258,316517,3.0598578453063965,7.849567696529446e-08
79221,158443,158442,316885,3.063015937805176,7.733504541147907e-08
79313,158627,158626,317253,3.0661380290985107,7.619349976517837e-08
79405,158811,158810,317621,3.069291830062866,7.507869797408108e-08
79497,158995,158994,317989,3.0724217891693115,7.397639356748442e-08
79589,159179,159178,318357,3.075958013534546,7.28814178485265e-08
79681,159363,159362,318725,3.0791537761688232,7.180808984885597e-08
79773,159547,159546,319093,3.082660675048828,7.075809680968502e-08
79865,159731,159730,319461,3.0867960453033447,6.97166956299279e-08
79957,159915,159914,319829,3.09023380279541,6.868464150055228e-08
80049,160099,160098,320197,3.0939528942108154,6.767560292863167e-08
80141,160283,160282,320565,3.097822904586792,6.668567315486672e-08
80233,160467,160466,320933,3.1018049716949463,6.570186959185193e-08
80325,160651,160650,321301,3.1056768894195557,6.473006049442525e-08
80417,160835,160834,321669,3.1096229553222656,6.378123000626072e-08
80509,161019,161018,322037,3.1134917736053467,6.284706259293495e-08
80601,161203,161202,322405,3.1173598766326904,6.191807575710435e-08
80693,161387,161386,322773,3.121706962585449,6.100375720049496e-08
80785,161571,161570,323141,3.1256470680236816,6.011100928182985e-08
80877,161755,161754,323509,3.129525899887085,5.9228831026124815e-08
80969,161939,161938,323877,3.1334776878356934,5.8352256013700395e-08
81061,162123,162122,324245,3.1373178958892822,5.7492517778530784e-08
81153,162307,162306,324613,3.1410937309265137,5.665181655878648e-08
81245,162491,162490,324981,3.1448328495025635,5.581840560606386e-08
81337,162675,162674,325349,3.1486289501190186,5.499205386857771e-08
81429,162859,162858,325717,3.152477741241455,5.418381347102394e-08
81521,163043,163042,326085,3.156205892562866,5.3391346558311255e-08
81613,163227,163226,326453,3.1601059436798096,5.2603998074571045e-08
81705,163411,163410,326821,3.164320945739746,5.182575064984955e-08
81797,163595,163594,327189,3.1681110858917236,5.106579228017178e-08
81889,163779,163778,327557,3.172074794769287,5.031808269736157e-08
81981,163963,163962,327925,3.175916910171509,4.957452637227752e-08
82073,164147,164146,328293,3.1796798706054688,4.8842219027038e-08
82165,164331,164330,328661,3.1834709644317627,4.8127274008814985e-08
82257,164515,164514,329029,3.187483787536621,4.7421254084634546e-08
82349,164699,164698,329397,3.1913888454437256,4.6719540263283406e-08
82441,164883,164882,329765,3.1952266693115234,4.603089299139288e-08
82533,165067,165066,330133,3.199022054672241,4.5357743713987685e-08
82625,165251,165250,330501,3.202725887298584,4.469078261931747e-08
82717,165435,165434,330869,3.206209897994995,4.402915582651069e-08
82809,165619,165618,331237,3.209707021713257,4.338175109022284e-08
82901,165803,165802,331605,3.2128360271453857,4.2747338414533697e-08
82993,165987,165986,331973,3.2160139083862305,4.2117222905682836e-08
83085,166171,166170,332341,3.219172716140747,4.1494002535057685e-08
83177,166355,166354,332709,3.222532033920288,4.088530871560136e-08
83269,166539,166538,333077,3.225703716278076,4.028682485475968e-08
83361,166723,166722,333445,3.2288808822631836,3.9691700154134313e-08
83453,166907,166906,333813,3.2322537899017334,3.9105183933511736e-08
83545,167091,167090,334181,3.235460042953491,3.85326140420452e-08
83637,167275,167274,334549,3.238755941390991,3.796756736165274e-08
83729,167459,167458,334917,3.241989850997925,3.7405850246068275e-08
83821,167643,167642,335285,3.245210886001587,3.685425158217719e-08
83913,167827,167826,335653,3.24847412109375,3.63152433833782e-08
84005,168011,168010,336021,3.2517077922821045,3.5781487084579576e-08
84097,168195,168194,336389,3.255018949508667,3.525176649878534e-08
84189,168379,168378,336757,3.2581369876861572,3.473319019394859e-08
84281,168563,168562,337125,3.261561870574951,3.422529183462106e-08
84373,168747,168746,337493,3.2647688388824463,3.3721015188852656e-08
84465,168931,168930,337861,3.2680177688598633,3.322195562391213e-08
84557,169115,169114,338229,3.2711007595062256,3.2734410324584665e-08
84649,169299,169298,338597,3.2741658687591553,3.2255357040557166e-08
84741,169483,169482,338965,3.2772939205169678,3.177904378452188e-08
84833,169667,169666,339333,3.280388832092285,3.1309304740099e-08
84925,169851,169850,339701,3.28357195854187,3.085074514799182e-08
85017,170035,170034,340069,3.286655902862549,3.0398515143257757e-08
85109,170219,170218,340437,3.289731025695801,2.994887776823184e-08
85201,170403,170402,340805,3.2928268909454346,2.9507058785678863e-08
85293,170587,170586,341173,3.2959086894989014,2.907544689237405e-08
85385,170771,170770,341541,3.2989916801452637,2.864828961613214e-08
85477,170955,170954,341909,3.3021297454833984,2.8224191560532956e-08
85569,171139,171138,342277,3.3052239418029785,2.7808807422608526e-08
85661,171323,171322,342645,3.308255910873413,2.7402180464040423e-08
85753,171507,171506,343013,3.311262845993042,2.6998614909001605e-08
85845,171691,171690,343381,3.31430983543396,2.6598992767056036e-08
85937,171875,171874,343749,3.317312002182007,2.6208478318966862e-08
86029,172059,172058,344117,3.3203318119049072,2.5825011588691778e-08
86121,172243,172242,344485,3.3233320713043213,2.5443797665178187e-08
86213,172427,172426,344853,3.3263208866119385,2.5067594377167803e-08
86305,172611,172610,345221,3.329556941986084,2.470033424966439e-08
86397,172795,172794,345589,3.332606792449951,2.433838892618536e-08
86489,172979,172978,345957,3.33563494682312,2.397847821664099e-08
86581,173163,173162,346325,3.338660717010498,2.362459548607034e-08
86673,173347,173346,346693,3.3417978286743164,2.3278970477833487e-08
86765,173531,173530,347061,3.344817876815796,2.2937120229033504e-08
86857,173715,173714,347429,3.3478379249572754,2.259759545660908e-08
86949,173899,173898,347797,3.3508448600769043,2.2264869636916508e-08
87041,174083,174082,348165,3.3538668155670166,2.1939310362843644e-08
87133,174267,174266,348533,3.356872797012329,2.1616344298267012e-08
87225,174451,174450,348901,3.3601298332214355,2.1296356941348804e-08
87317,174635,174634,349269,3.363564968109131,2.0983558715423975e-08
87410,174821,174820,349641,3.3667030334472656,2.067327359298059e-08
87502,175005,175004,350009,3.3699567317962646,2.0368196018325836e-08
87594,175189,175188,350377,3.373121976852417,2.006697897043924e-08
87686,175373,175372,350745,3.376343011856079,1.9772906818574094e-08
87778,175557,175556,351113,3.3795077800750732,1.94832382107426e-08
87870,175741,175740,351481,3.38264799118042,1.919518290026481e-08
87962,175925,175924,351849,3.385802984237671,1.8911811478430222e-08
88054,176109,176108,352217,3.388921022415161,1.8635093306291042e-08
88146,176293,176292,352585,3.391995906829834,1.8361525914273146e-08
88238,176477,176476,352953,3.39505672454834,1.8089753202140643e-08
88330,176661,176660,353321,3.3981218338012695,1.7823310998989424e-08
88422,176845,176844,353689,3.4011898040771484,1.756269272887246e-08
88514,177029,177028,354057,3.4042508602142334,1.7304242111875756e-08
88606,177213,177212,354425,3.4073848724365234,1.7048073522185444e-08
88698,177397,177396,354793,3.41054368019104,1.6797590976859782e-08
88790,177581,177580,355161,3.413719892501831,1.655189347781143e-08
88882,177765,177764,355529,3.416958808898926,1.630773409915037e-08
88974,177949,177948,355897,3.420119047164917,1.6066507536576055e-08
89066,178133,178132,356265,3.424514055252075,1.5830976103925172e-08
89158,178317,178316,356633,3.4276950359344482,1.5599128803978717e-08
89250,178501,178500,357001,3.430968999862671,1.53685666815719e-08
89342,178685,178684,357369,3.434175968170166,1.5141602135220025e-08
89434,178869,178868,357737,3.4373559951782227,1.4920000751622412e-08
89526,179053,179052,358105,3.4405078887939453,1.4701062982374358e-08
89618,179237,179236,358473,3.4436628818511963,1.4483499214967246e-08
89710,179421,179420,358841,3.4468178749084473,1.4270078785839407e-08
89802,179605,179604,359209,3.449881076812744,1.4061406768046876e-08
89894,179789,179788,359577,3.4529640674591064,1.3854574333351559e-08
89986,179973,179972,359945,3.4560697078704834,1.3649465536976666e-08
90078,180157,180156,360313,3.4591619968414307,1.3448828523475536e-08
90170,180341,180340,360681,3.4623148441314697,1.325213892815947e-08
90262,180525,180524,361049,3.4653990268707275,1.3056736323083371e-08
90354,180709,180708,361417,3.468564987182617,1.2863558046802787e-08
90446,180893,180892,361785,3.47165584564209,1.2674909983829342e-08
90538,181077,181076,362153,3.47473406791687,1.2489337589024733e-08
90630,181261,181260,362521,3.477832794189453,1.2304798104666865e-08
90722,181445,181444,362889,3.4809088706970215,1.2123015914104993e-08
90814,181629,181628,363257,3.483977794647217,1.1945548036817609e-08
90906,181813,181812,363625,3.4870529174804688,1.1770328267516486e-08
90998,181997,181996,363993,3.4901177883148193,1.1596166154604667e-08
91090,182181,182180,364361,3.493184804916382,1.1425217577417042e-08
91182,182365,182364,364729,3.4962680339813232,1.1258132378580975e-08
91274,182549,182548,365097,3.499325752258301,1.1092608672422978e-08
91366,182733,182732,365465,3.5023837089538574,1.0928387791836457e-08
91458,182917,182916,365833,3.5054588317871094,1.0767676309563755e-08
91550,183101,183100,366201,3.5086047649383545,1.0610214181081646e-08
91642,183285,183284,366569,3.5117719173431396,1.0453833838215315e-08
91734,183469,183468,366937,3.514997959136963,1.0299138019891906e-08
91826,183653,183652,367305,3.5182137489318848,1.014803835416807e-08
91918,183837,183836,367673,3.521383762359619,9.999500834441716e-09


==> plot_data/quadratic_minimax_problem_n20_alpha00001/flex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.200241088867188e-05,4.387072431292609
3,11,0,11,0.0006048679351806641,3.473448194683989
6,24,0,24,0.0010082721710205078,2.032332276860507
8,32,0,32,0.001280069351196289,1.5510168039236454
11,43,0,43,0.0016410350799560547,0.9646848713255388
14,56,0,56,0.002061128616333008,0.6476669392193777
17,67,0,67,0.002443075180053711,0.39656488334482437
19,75,0,75,0.002730131149291992,0.2958255937252611
22,86,0,86,0.003159046173095703,0.21735477306796255
25,99,0,99,0.0036122798919677734,0.15244269907523542
28,110,0,110,0.004024028778076172,0.09558859304145342
30,119,0,119,0.004328012466430664,0.0912229100773483
33,132,0,132,0.004773139953613281,0.07866502189815996
36,147,0,147,0.005275249481201172,0.0733650030902074
39,161,0,161,0.005918979644775391,0.06963621796749558
41,171,0,171,0.006307125091552734,0.06731282773701364
44,186,0,186,0.006953001022338867,0.06502672477720547
47,200,0,200,0.007467985153198242,0.06317514225694952
50,215,0,215,0.007976055145263672,0.06053816577577747
52,225,0,225,0.008409261703491211,0.059386332536707866
55,240,0,240,0.008903980255126953,0.05817356562641064
58,255,0,255,0.009519100189208984,0.057321804640327975
61,269,0,269,0.010187149047851562,0.05596096137084261
63,278,0,278,0.010576248168945312,0.05322957639247789
66,293,0,293,0.011087179183959961,0.05116145604114655
69,307,0,307,0.011588096618652344,0.04726611454488083
72,322,0,322,0.01226496696472168,0.0462312507190202
75,336,0,336,0.012782096862792969,0.04444062553927025
77,345,0,345,0.013100147247314453,0.04206182246313801
80,359,0,359,0.013576030731201172,0.03987436697304369
83,374,0,374,0.014084100723266602,0.038375133617586
86,388,0,388,0.014566898345947266,0.03624269783099602
88,398,0,398,0.01488804817199707,0.03558201456610184
91,413,0,413,0.015382051467895508,0.03492006541815994
94,427,0,427,0.015857219696044922,0.03397514683577285
97,441,0,441,0.01633310317993164,0.03199715988995219
99,451,0,451,0.01665806770324707,0.03149444519387161
102,466,0,466,0.017144203186035156,0.030959248797765144
105,481,0,481,0.017642974853515625,0.030583791077994096
108,496,0,496,0.01822805404663086,0.03030314873520102
110,506,0,506,0.018606185913085938,0.030150480611865493
113,521,0,521,0.01911020278930664,0.029957380970677554
116,536,0,536,0.01960611343383789,0.029795631990181905
119,551,0,551,0.02011704444885254,0.02965659504714112
121,561,0,561,0.02045416831970215,0.029573748370816805
124,576,0,576,0.020965099334716797,0.029461344280374828
127,591,0,591,0.021743059158325195,0.02936061131995728
130,605,0,605,0.022971153259277344,0.02895793316269333
132,615,0,615,0.023478984832763672,0.02838686221647244
135,630,0,630,0.024059295654296875,0.02783363050467214
138,645,0,645,0.024730205535888672,0.027494570768971816
141,660,0,660,0.025501012802124023,0.027274311617796785
144,675,0,675,0.02613091468811035,0.027121746303874254
146,685,0,685,0.026528120040893555,0.027043311258121507
149,700,0,700,0.027096033096313477,0.026948228512619094
152,715,0,715,0.027677059173583984,0.026871415464039736
155,730,0,730,0.02828693389892578,0.02680676810983676
157,740,0,740,0.028621196746826172,0.0267686030492869
160,755,0,755,0.029140949249267578,0.026716923391911406
163,770,0,770,0.029624223709106445,0.026670437956765696
166,785,0,785,0.0301210880279541,0.026627948961460396
168,794,0,794,0.030431032180786133,0.0257439928240897
171,809,0,809,0.030985116958618164,0.025373942231900527
174,824,0,824,0.031638145446777344,0.02515471479929574
177,839,0,839,0.03217315673828125,0.025014722648002457
179,849,0,849,0.0325009822845459,0.024946988421648126
182,864,0,864,0.033000946044921875,0.02486850396251165
185,879,0,879,0.03348708152770996,0.02480801240041188
188,894,0,894,0.0340421199798584,0.024759029374874796
190,904,0,904,0.034371137619018555,0.024730844192112248
193,919,0,919,0.03496813774108887,0.024693539901186435
196,934,0,934,0.03555607795715332,0.024660721242445564
199,949,0,949,0.03611016273498535,0.024631204633016737
201,959,0,959,0.0365140438079834,0.024612962818743575
204,974,0,974,0.037065982818603516,0.024587319882431784
207,989,0,989,0.03758597373962402,0.024563389911519
210,1004,0,1004,0.038099050521850586,0.02454087139499733
213,1019,0,1019,0.03868508338928223,0.0245195253881657
215,1029,0,1029,0.03904008865356445,0.024505847321655227
218,1044,0,1044,0.03951692581176758,0.024486034355315583
221,1059,0,1059,0.04000425338745117,0.024466936393217068
224,1074,0,1074,0.04048609733581543,0.024448429515566503
226,1084,0,1084,0.04080510139465332,0.024436373658271112
229,1099,0,1099,0.04128003120422363,0.024418655642380254
232,1114,0,1114,0.04175615310668945,0.024401323372577194
235,1129,0,1129,0.04224801063537598,0.02438432716462068
237,1139,0,1139,0.04256415367126465,0.02437316138330255
240,1154,0,1154,0.04303789138793945,0.02435663150553974
243,1169,0,1169,0.04350996017456055,0.02434032942777805
246,1184,0,1184,0.043984174728393555,0.02432421844645624
248,1194,0,1194,0.04430222511291504,0.02431356787183183
251,1209,0,1209,0.044775962829589844,0.024297707098148023
254,1224,0,1224,0.04525113105773926,0.024281966322152328
257,1239,0,1239,0.04572319984436035,0.024266329787030562
259,1249,0,1249,0.046038150787353516,0.024255957371899797
262,1264,0,1264,0.04651212692260742,0.024240469957238994
265,1279,0,1279,0.04698491096496582,0.024225062753684922
268,1294,0,1294,0.04745912551879883,0.024209732646130962
270,1304,0,1304,0.047775983810424805,0.02419955450993122
273,1319,0,1319,0.0482633113861084,0.02418434864333217
276,1334,0,1334,0.04874014854431152,0.02416921307156319
279,1349,0,1349,0.04922008514404297,0.024154142460242355
281,1359,0,1359,0.049636125564575195,0.024144128437403028
284,1374,0,1374,0.05016493797302246,0.02412915262155988
287,1389,0,1389,0.05074620246887207,0.024114226716803282
290,1404,0,1404,0.05132412910461426,0.02409934657608907
293,1419,0,1419,0.051870107650756836,0.0240845081816001
295,1429,0,1429,0.052201032638549805,0.02407463698896906
298,1444,0,1444,0.05290508270263672,0.024059858627752156
301,1459,0,1459,0.05413508415222168,0.02404511132248224
304,1474,0,1474,0.05529022216796875,0.0240303932564344
306,1484,0,1484,0.05602407455444336,0.02402059750081836
309,1499,0,1499,0.0569150447845459,0.024005929566763364
312,1514,0,1514,0.057967185974121094,0.02399129480022125
315,1529,0,1529,0.0587460994720459,0.023976695932150512
317,1539,0,1539,0.05912208557128906,0.023966984408981973
320,1554,0,1554,0.059806108474731445,0.023952449785655534
323,1569,0,1569,0.060658931732177734,0.023937954994789658
326,1584,0,1584,0.06183815002441406,0.023923500355032035
328,1594,0,1594,0.06260514259338379,0.02391388637980172
331,1609,0,1609,0.06359720230102539,0.023899499486953107
334,1624,0,1624,0.06468987464904785,0.02388515416260165
337,1639,0,1639,0.06586599349975586,0.023870851209930998
339,1649,0,1649,0.06656002998352051,0.0238613397413695
342,1664,0,1664,0.06781411170959473,0.023847108438385688
345,1679,0,1679,0.0690622329711914,0.023832920015442564
348,1694,0,1694,0.07016110420227051,0.0238187739263808
350,1704,0,1704,0.07091307640075684,0.02380936638293199
353,1719,0,1719,0.07205009460449219,0.023795289420548572
356,1734,0,1734,0.07332921028137207,0.023781253480465375
359,1749,0,1749,0.07424426078796387,0.023767258814967687
362,1764,0,1764,0.07483220100402832,0.023753306189184663
364,1774,0,1774,0.07528185844421387,0.02374402833541098
367,1789,0,1789,0.07596111297607422,0.02373014829784763
370,1804,0,1804,0.0765829086303711,0.023716313354983906
373,1819,0,1819,0.07750415802001953,0.023702524434385964
375,1829,0,1829,0.07807207107543945,0.023693357735822488
378,1844,0,1844,0.07890009880065918,0.02367964693863637
381,1859,0,1859,0.07974720001220703,0.02366598354920625
384,1874,0,1874,0.0807030200958252,0.023652367712436506
386,1884,0,1884,0.08124804496765137,0.023643316824587035
389,1899,0,1899,0.08211421966552734,0.023629779514760828
392,1914,0,1914,0.08274722099304199,0.023616287863794574
395,1929,0,1929,0.08324003219604492,0.02360283981180163
397,1939,0,1939,0.08356499671936035,0.023593897306110015
400,1954,0,1954,0.08405208587646484,0.023580515447624604
403,1969,0,1969,0.08453822135925293,0.02356716887195732
406,1984,0,1984,0.08510017395019531,0.023553854438211477
408,1994,0,1994,0.08546304702758789,0.023544994712877184
411,2009,0,2009,0.08599209785461426,0.023531728558469203
414,2024,0,2024,0.08648395538330078,0.023518489483737588
417,2039,0,2039,0.08697295188903809,0.023505276927906618
419,2048,0,2048,0.08728408813476562,0.023151368023947398
422,2061,0,2061,0.08774209022521973,0.020353620186680906
425,2076,0,2076,0.0882420539855957,0.01963851371864139
428,2089,0,2089,0.08868408203125,0.015932748789237828
431,2100,0,2100,0.08910608291625977,0.005740104870530547
433,2108,0,2108,0.089385986328125,0.003054949672172139
436,2118,0,2118,0.08977890014648438,0.00245713375297892
439,2129,0,2129,0.09020709991455078,0.002218790866146663
442,2143,0,2143,0.0906832218170166,0.0019017410112598919
444,2151,0,2151,0.09097504615783691,0.0016548982805513878
447,2164,0,2164,0.09143495559692383,0.0014642722143068103
450,2179,0,2179,0.09192109107971191,0.0013142740438146004
453,2194,0,2194,0.09240913391113281,0.001207276140700529
455,2202,0,2202,0.09270620346069336,0.0010790085239374481
458,2214,0,2214,0.09315896034240723,0.0009247657554080052
461,2228,0,2228,0.09363102912902832,0.0007226864081897073
464,2242,0,2242,0.09410524368286133,0.0006344769674104682
466,2251,0,2251,0.09441614151000977,0.0005897699074583846
469,2265,0,2265,0.09489202499389648,0.0005269852936455267
472,2280,0,2280,0.0953819751739502,0.000492883106802978
475,2295,0,2295,0.09586811065673828,0.00046966712086979535
477,2304,0,2304,0.0961771011352539,0.00045060004551826825
480,2318,0,2318,0.09664726257324219,0.00042706870879101705
483,2333,0,2333,0.0971379280090332,0.0004021262300165856
486,2348,0,2348,0.0976252555847168,0.00038390963508222334
488,2358,0,2358,0.09794831275939941,0.00037414737763066374
491,2373,0,2373,0.09843826293945312,0.0003619043551609022
494,2387,0,2387,0.09891819953918457,0.000333370184141835
497,2401,0,2401,0.09939718246459961,0.0003086461614974442
500,2415,0,2415,0.0998992919921875,0.000295787330336128
502,2425,0,2425,0.10029911994934082,0.00028516580742615814
505,2440,0,2440,0.10110116004943848,0.00027377807601868795
508,2454,0,2454,0.10187506675720215,0.0002519677795825361
511,2467,0,2467,0.10256791114807129,0.0002366090609854904
513,2477,0,2477,0.10317707061767578,0.0002261319637696321
516,2491,0,2491,0.10394501686096191,0.00020841754409729876
519,2504,0,2504,0.10457921028137207,0.00018429762930736567
522,2518,0,2518,0.10513615608215332,0.00016524781483703992
524,2527,0,2527,0.1055440902709961,0.0001613500977418623
527,2541,0,2541,0.10615301132202148,0.0001445922586235725
530,2556,0,2556,0.1066591739654541,0.00013555968720327738
533,2570,0,2570,0.10715508460998535,0.00012340025129315446
535,2580,0,2580,0.10749006271362305,0.00012023923789030847
538,2595,0,2595,0.10798907279968262,0.00011664568441771645
541,2609,0,2609,0.1084752082824707,0.000108392890713559
544,2624,0,2624,0.10925412178039551,0.00010543365941472121
546,2634,0,2634,0.10971903800964355,0.00010388128417663508
549,2649,0,2649,0.11022520065307617,0.00010194724094062588
552,2663,0,2663,0.11073899269104004,9.508629272769048e-05
555,2678,0,2678,0.11126089096069336,9.306158450757446e-05
557,2687,0,2687,0.11159205436706543,8.622534615216891e-05
560,2702,0,2702,0.11211705207824707,8.422166123462786e-05
563,2716,0,2716,0.11262011528015137,7.815481662875244e-05
566,2731,0,2731,0.11313509941101074,7.631755764665034e-05
569,2746,0,2746,0.11365818977355957,7.511903246828514e-05
571,2756,0,2756,0.11399030685424805,7.451653085816061e-05
574,2771,0,2771,0.11449408531188965,7.378450638376001e-05
577,2785,0,2785,0.11498022079467773,7.024298615536032e-05
580,2800,0,2800,0.11547708511352539,6.878452041157285e-05
582,2809,0,2809,0.11582708358764648,6.762898915642345e-05
585,2824,0,2824,0.1164090633392334,6.487003514776463e-05
588,2838,0,2838,0.11692309379577637,5.953946802080807e-05
591,2852,0,2852,0.11757326126098633,5.6957350923230264e-05
593,2861,0,2861,0.11806321144104004,5.600607184373165e-05
596,2876,0,2876,0.11900496482849121,5.3828971695533674e-05
599,2891,0,2891,0.1197209358215332,5.264584781484228e-05
602,2906,0,2906,0.1204061508178711,5.1964409822150824e-05
604,2916,0,2916,0.12079906463623047,5.1660631158418854e-05
607,2931,0,2931,0.12133622169494629,5.133114509840949e-05
610,2946,0,2946,0.12184309959411621,5.108910669544961e-05
613,2960,0,2960,0.12232804298400879,4.806616619920637e-05
615,2969,0,2969,0.12264513969421387,4.542406572306242e-05
618,2983,0,2983,0.12313127517700195,4.377184665495077e-05
621,2998,0,2998,0.1236269474029541,4.2766192854533955e-05
624,3013,0,3013,0.12412428855895996,4.21500246589246e-05
626,3023,0,3023,0.12445592880249023,4.1865516718071644e-05
629,3038,0,3038,0.12495303153991699,4.155304558876743e-05
632,3053,0,3053,0.12544894218444824,4.132616040619909e-05
635,3068,0,3068,0.12595319747924805,4.115158870586088e-05
638,3083,0,3083,0.1264500617980957,4.101070594540892e-05
640,3092,0,3092,0.12676715850830078,4.016748237121521e-05
643,3107,0,3107,0.12726497650146484,3.937645202850983e-05
646,3122,0,3122,0.12777113914489746,3.890117844804813e-05
649,3137,0,3137,0.12827110290527344,3.86021549133981e-05
651,3147,0,3147,0.12860321998596191,3.8461232045399426e-05
654,3162,0,3162,0.12909793853759766,3.830347618859395e-05
657,3177,0,3177,0.12958908081054688,3.818638218945729e-05
660,3192,0,3192,0.13009214401245117,3.8094277787451636e-05
662,3202,0,3202,0.13042902946472168,3.804214003540849e-05
665,3217,0,3217,0.13092613220214844,3.797362043479353e-05
668,3232,0,3232,0.1314239501953125,3.791346961183545e-05
671,3247,0,3247,0.13191819190979004,3.785934136233678e-05
673,3257,0,3257,0.13225126266479492,3.782582798005282e-05
676,3272,0,3272,0.13274598121643066,3.777862459058906e-05
679,3287,0,3287,0.1332411766052246,3.773442679088611e-05
682,3302,0,3302,0.13373494148254395,3.769268980082534e-05
684,3312,0,3312,0.1340651512145996,3.76660550603469e-05
687,3327,0,3327,0.13457894325256348,3.7627692775729934e-05
690,3342,0,3342,0.13506102561950684,3.759102783506214e-05
693,3357,0,3357,0.1355452537536621,3.7555811219241306e-05
695,3367,0,3367,0.1358661651611328,3.753301648707805e-05
698,3382,0,3382,0.13634419441223145,3.749969507015592e-05
701,3397,0,3397,0.13682198524475098,3.7467271758358166e-05
704,3412,0,3412,0.13730096817016602,3.743562565474461e-05
706,3422,0,3422,0.13763999938964844,3.741491685478529e-05
709,3437,0,3437,0.13813090324401855,3.738438425752245e-05
712,3452,0,3452,0.13863015174865723,3.735442852619704e-05
715,3466,0,3466,0.13911104202270508,3.662166870016281e-05
718,3481,0,3481,0.13960504531860352,3.618294446085004e-05
720,3491,0,3491,0.1399390697479248,3.598821559546591e-05
723,3506,0,3506,0.14043331146240234,3.578102096073539e-05
726,3521,0,3521,0.14093804359436035,3.563523123788376e-05
729,3536,0,3536,0.1414201259613037,3.552536977028174e-05
731,3546,0,3546,0.14174103736877441,3.546508718722154e-05
734,3561,0,3561,0.14222121238708496,3.538796193539509e-05
737,3576,0,3576,0.14272308349609375,3.532234851378486e-05
740,3591,0,3591,0.1432352066040039,3.526507350592354e-05
742,3601,0,3601,0.1436159610748291,3.523048668780329e-05
745,3616,0,3616,0.14410710334777832,3.518292190764519e-05
748,3631,0,3631,0.14458799362182617,3.5139587945004657e-05
751,3646,0,3646,0.14506912231445312,3.509968051667399e-05
753,3656,0,3656,0.14539003372192383,3.507466622496105e-05
756,3671,0,3671,0.14589691162109375,3.503915621462254e-05
759,3686,0,3686,0.1463930606842041,3.500570597199787e-05
762,3701,0,3701,0.14691901206970215,3.497401577489603e-05
764,3711,0,3711,0.14724206924438477,3.495375412851226e-05
767,3726,0,3726,0.14772295951843262,3.492451383047227e-05
770,3741,0,3741,0.14820313453674316,3.489650288899591e-05
773,3756,0,3756,0.14870500564575195,3.486957204039705e-05
775,3766,0,3766,0.1490330696105957,3.485215675358962e-05
778,3781,0,3781,0.14952397346496582,3.482676059004007e-05
781,3796,0,3796,0.15002107620239258,3.480214235107868e-05
784,3811,0,3811,0.1505138874053955,3.477820236769614e-05
787,3826,0,3826,0.15100908279418945,3.475485819151611e-05
789,3836,0,3836,0.15134215354919434,3.473959582995489e-05
792,3851,0,3851,0.15183615684509277,3.4717119025858044e-05
795,3866,0,3866,0.1523280143737793,3.46951083653743e-05
798,3881,0,3881,0.15282320976257324,3.467352776484152e-05
800,3891,0,3891,0.1531531810760498,3.465936151155762e-05
803,3906,0,3906,0.15366101264953613,3.463841423279218e-05
806,3921,0,3921,0.1542370319366455,3.46177915437681e-05
809,3936,0,3936,0.15477514266967773,3.459744939412476e-05
811,3946,0,3946,0.15510201454162598,3.4584023721541536e-05
814,3960,0,3960,0.15558409690856934,3.3630517307195454e-05
817,3975,0,3975,0.15607023239135742,3.291485116783064e-05
820,3990,0,3990,0.15655303001403809,3.2523462229576256e-05
822,4000,0,4000,0.1568770408630371,3.236053825381198e-05
825,4015,0,4015,0.15736126899719238,3.219768303764772e-05
828,4030,0,4030,0.15787124633789062,3.209119135931888e-05
831,4045,0,4045,0.15836596488952637,3.201549727689728e-05
833,4055,0,4055,0.15871214866638184,3.1975332220436726e-05
836,4070,0,4070,0.1591951847076416,3.192494104982753e-05
839,4085,0,4085,0.15968012809753418,3.188252673347464e-05
842,4100,0,4100,0.16016316413879395,3.1845382555096804e-05
844,4110,0,4110,0.16048312187194824,3.182275103458251e-05
847,4125,0,4125,0.16098833084106445,3.179126482316003e-05
850,4140,0,4140,0.1614840030670166,3.176212962378212e-05
853,4155,0,4155,0.16198015213012695,3.173483615403656e-05
856,4170,0,4170,0.1624760627746582,3.1709026154166334e-05
858,4180,0,4180,0.16280698776245117,3.169250602210052e-05
861,4195,0,4195,0.16330814361572266,3.1668585179186475e-05
864,4210,0,4210,0.16382312774658203,3.164555125988876e-05
867,4225,0,4225,0.16432619094848633,3.162327967477323e-05
869,4235,0,4235,0.1646571159362793,3.16088101655293e-05
872,4250,0,4250,0.16515207290649414,3.158761775064959e-05
875,4265,0,4265,0.16566109657287598,3.1566989953774204e-05
878,4280,0,4280,0.16614413261413574,3.1546872876230645e-05
880,4290,0,4290,0.16648197174072266,3.153371630311464e-05
883,4305,0,4305,0.1669631004333496,3.1514316023895383e-05
886,4319,0,4319,0.1674330234527588,3.0491400397619093e-05
889,4333,0,4333,0.16792702674865723,2.9792504724614573e-05
891,4343,0,4343,0.16826319694519043,2.941702355941309e-05
894,4358,0,4358,0.1687612533569336,2.900335940665186e-05
897,4373,0,4373,0.16925811767578125,2.870166777762944e-05
900,4388,0,4388,0.16975903511047363,2.8468959901981102e-05
902,4398,0,4398,0.17009997367858887,2.8339883068689083e-05
905,4413,0,4413,0.17060613632202148,2.8174564784248173e-05
908,4428,0,4428,0.17126822471618652,2.80348559513363e-05
911,4443,0,4443,0.1717970371246338,2.7914337987608337e-05
913,4453,0,4453,0.172133207321167,2.7842515448762227e-05
916,4468,0,4468,0.17264413833618164,2.7745144451809678e-05
919,4483,0,4483,0.17314505577087402,2.765803445970082e-05
922,4498,0,4498,0.17364931106567383,2.757935936169885e-05
925,4513,0,4513,0.1741471290588379,2.7507633850844746e-05
927,4523,0,4523,0.1744840145111084,2.74630593380091e-05
930,4538,0,4538,0.17498397827148438,2.740031525377644e-05
933,4553,0,4553,0.17548418045043945,2.734180480173763e-05
936,4568,0,4568,0.17599010467529297,2.7286929173332113e-05
938,4578,0,4578,0.1763153076171875,2.7252142568166453e-05
941,4593,0,4593,0.1768040657043457,2.7202387899973066e-05
944,4608,0,4608,0.1772899627685547,2.7155267051705107e-05
947,4623,0,4623,0.17777299880981445,2.7110499274351432e-05
949,4633,0,4633,0.17809629440307617,2.7081835491030957e-05
952,4648,0,4648,0.17858409881591797,2.7040442848585814e-05
955,4663,0,4663,0.17906713485717773,2.7000792785199084e-05
958,4678,0,4678,0.1795499324798584,2.696270733156184e-05
960,4688,0,4688,0.1798710823059082,2.6938112717637753e-05
963,4703,0,4703,0.18035626411437988,2.6902324163238344e-05
966,4718,0,4718,0.1808481216430664,2.686776691796304e-05
969,4733,0,4733,0.18133807182312012,2.683434587946491e-05
971,4743,0,4743,0.18166303634643555,2.681265282468206e-05
974,4758,0,4758,0.18215012550354004,2.6780934445928223e-05
977,4773,0,4773,0.1826491355895996,2.675013363214447e-05
980,4788,0,4788,0.18315696716308594,2.6720175178710732e-05
982,4798,0,4798,0.183488130569458,2.6700633697654127e-05
985,4813,0,4813,0.18398523330688477,2.6671914528579638e-05
988,4828,0,4828,0.18448305130004883,2.6643852328028098e-05
991,4843,0,4843,0.18497729301452637,2.661640131142021e-05
994,4858,0,4858,0.18548107147216797,2.658953269751347e-05
996,4868,0,4868,0.1858382225036621,2.65719347814311e-05
999,4883,0,4883,0.18634819984436035,2.654599888517732e-05
1002,4898,0,4898,0.18685698509216309,2.6520602862961714e-05
1005,4913,0,4913,0.1873641014099121,2.6495730299416528e-05
1007,4923,0,4923,0.18771719932556152,2.647943078641533e-05
1010,4938,0,4938,0.18828916549682617,2.6455391408869424e-05
1013,4953,0,4953,0.18880510330200195,2.6431827173218387e-05
1016,4968,0,4968,0.18930625915527344,2.6408718495113254e-05
1018,4977,0,4977,0.18963003158569336,2.6066785276559637e-05
1021,4992,0,4992,0.1901252269744873,2.5486742568781167e-05
1024,5007,0,5007,0.19064021110534668,2.5114446897001688e-05
1027,5022,0,5022,0.19113922119140625,2.4868600370874648e-05
1029,5032,0,5032,0.19147014617919922,2.474994341416943e-05
1032,5047,0,5047,0.19196701049804688,2.4616335070861864e-05
1035,5062,0,5062,0.19246530532836914,2.4518291408977313e-05
1038,5077,0,5077,0.19295907020568848,2.4443199716635536e-05
1040,5087,0,5087,0.19328904151916504,2.4401899986155708e-05
1043,5102,0,5102,0.19378900527954102,2.434915802222618e-05
1046,5117,0,5117,0.19428110122680664,2.43044131191147e-05
1049,5132,0,5132,0.1947951316833496,2.4265321420386894e-05
1051,5142,0,5142,0.1951301097869873,2.4241626468112216e-05
1054,5157,0,5157,0.1956491470336914,2.420881001108642e-05
1057,5172,0,5172,0.19613909721374512,2.4178574442405588e-05
1060,5187,0,5187,0.19662690162658691,2.4150351675500547e-05
1063,5202,0,5202,0.19711709022521973,2.4123736279301175e-05
1065,5212,0,5212,0.19744420051574707,2.410674250596266e-05
1068,5227,0,5227,0.19797706604003906,2.408222920511702e-05
1071,5242,0,5242,0.19849109649658203,2.4058762445613934e-05
1074,5257,0,5257,0.19906401634216309,2.4036231432366847e-05
1076,5267,0,5267,0.19939827919006348,2.4021681075540284e-05
1079,5282,0,5282,0.1998898983001709,2.4000485830639635e-05
1082,5297,0,5297,0.20037412643432617,2.397996045778909e-05
1085,5312,0,5312,0.20087814331054688,2.3960018929018486e-05
1087,5322,0,5322,0.20120716094970703,2.3947012093277185e-05
1090,5337,0,5337,0.20172500610351562,2.3927886504489185e-05
1093,5352,0,5352,0.20223212242126465,2.3909174012531328e-05
1096,5367,0,5367,0.20276093482971191,2.3890830762721643e-05
1098,5377,0,5377,0.20309209823608398,2.387879081100678e-05
1101,5392,0,5392,0.20359301567077637,2.3860996395854664e-05
1104,5407,0,5407,0.20409607887268066,2.384350442358929e-05
1107,5422,0,5422,0.20459389686584473,2.3826298713828807e-05
1109,5432,0,5432,0.20500707626342773,2.381497972869216e-05
1112,5447,0,5447,0.20552611351013184,2.3798217741200522e-05
1115,5462,0,5462,0.20603108406066895,2.378170431234835e-05
1118,5477,0,5477,0.20653533935546875,2.3765429186089707e-05
1120,5487,0,5487,0.20688104629516602,2.3754707382727457e-05
1123,5502,0,5502,0.2073831558227539,2.373881179494123e-05
1126,5517,0,5517,0.20789504051208496,2.3723134394221175e-05
1129,5532,0,5532,0.2083892822265625,2.3707667227836657e-05
1132,5547,0,5547,0.2089090347290039,2.3692400312984834e-05
1134,5557,0,5557,0.2092432975769043,2.3682327367234782e-05
1137,5572,0,5572,0.2097470760345459,2.3667364026544635e-05
1140,5586,0,5586,0.21023321151733398,2.360369239974509e-05
1143,5601,0,5601,0.21075201034545898,2.2950696132183255e-05
1145,5611,0,5611,0.21110200881958008,2.2671775713168907e-05
1148,5626,0,5626,0.21163392066955566,2.239000377233715e-05
1151,5640,0,5640,0.21216106414794922,2.091860634085116e-05
1154,5654,0,5654,0.21265411376953125,1.9454532864490458e-05
1156,5663,0,5663,0.2130732536315918,1.8995920043161296e-05
1159,5677,0,5677,0.2136859893798828,1.8446754406922826e-05
1162,5692,0,5692,0.21422529220581055,1.7937356027810035e-05
1165,5707,0,5707,0.21476316452026367,1.7621636584056884e-05
1167,5716,0,5716,0.21511602401733398,1.730157197880377e-05
1170,5731,0,5731,0.21575403213500977,1.6899213931133806e-05
1173,5746,0,5746,0.21636724472045898,1.6646298437831857e-05
1176,5761,0,5761,0.21713519096374512,1.6478828339235485e-05
1178,5771,0,5771,0.2175900936126709,1.639624715208663e-05
1181,5784,0,5784,0.21814513206481934,1.5540830658492847e-05
1184,5799,0,5799,0.2187483310699463,1.4933822385498646e-05
1187,5813,0,5813,0.2194070816040039,1.3682323059907663e-05
1189,5822,0,5822,0.2198331356048584,1.293718575380223e-05
1192,5837,0,5837,0.22040510177612305,1.2418189810934193e-05
1195,5852,0,5852,0.22095108032226562,1.21062898598503e-05
1198,5867,0,5867,0.22147297859191895,1.1906193827505775e-05
1200,5877,0,5877,0.22183918952941895,1.1809079994781039e-05
1203,5892,0,5892,0.2225341796875,1.1696351232025888e-05
1206,5907,0,5907,0.22340822219848633,1.1608922897635961e-05
1209,5921,0,5921,0.2240140438079834,1.0739177313455844e-05
1212,5933,0,5933,0.22465801239013672,9.367819130110531e-06
1214,5943,0,5943,0.2250208854675293,8.87575982742842e-06
1217,5957,0,5957,0.2255561351776123,8.174348257065711e-06
1220,5972,0,5972,0.22610712051391602,7.804618536566721e-06
1223,5987,0,5987,0.2269299030303955,7.562391177558796e-06
1225,5997,0,5997,0.22732806205749512,7.4423727032102495e-06
1228,6010,0,6010,0.22786521911621094,7.227316402314338e-06
1231,6025,0,6025,0.22841286659240723,6.714926670071287e-06
1234,6040,0,6040,0.22902822494506836,6.403745728914133e-06
1236,6049,0,6049,0.22937917709350586,6.065867706925964e-06
1239,6064,0,6064,0.22991704940795898,5.836689583325869e-06
1242,6078,0,6078,0.23043608665466309,5.369815191970872e-06
1245,6093,0,6093,0.23096823692321777,5.207950537039575e-06
1247,6103,0,6103,0.2313690185546875,5.1332999916009725e-06
1250,6118,0,6118,0.23208904266357422,5.050563351641869e-06
1253,6132,0,6132,0.2326960563659668,4.8786037704937195e-06
1256,6147,0,6147,0.23322510719299316,4.74772457536148e-06
1258,6157,0,6157,0.23357486724853516,4.691382281608048e-06
1261,6172,0,6172,0.23409795761108398,4.632510958881319e-06
1264,6186,0,6186,0.2347550392150879,4.541990350225188e-06
1267,6201,0,6201,0.23535704612731934,4.398096132484898e-06
1269,6211,0,6211,0.23572397232055664,4.3375240288753915e-06
1272,6226,0,6226,0.23624920845031738,4.276833954276136e-06
1275,6240,0,6240,0.23690009117126465,4.0565511998391445e-06
1278,6254,0,6254,0.23738908767700195,3.909044504854309e-06
1281,6269,0,6269,0.23798298835754395,3.7863016728727783e-06
1283,6279,0,6279,0.23842811584472656,3.733747293082147e-06
1286,6293,0,6293,0.23896408081054688,3.55788173519187e-06
1289,6308,0,6308,0.2395031452178955,3.4854026368160607e-06
1292,6322,0,6322,0.24008607864379883,3.332764230497222e-06
1294,6332,0,6332,0.2404332160949707,3.2679878603229918e-06
1297,6347,0,6347,0.24094009399414062,3.200046604697835e-06
1300,6361,0,6361,0.24143695831298828,3.084055513832537e-06
1303,6376,0,6376,0.24197721481323242,2.9762121344656536e-06
1305,6386,0,6386,0.24232029914855957,2.9293472196525147e-06
1308,6401,0,6401,0.24284911155700684,2.8810480380263296e-06
1311,6416,0,6416,0.24348115921020508,2.848650677813087e-06
1314,6431,0,6431,0.24405813217163086,2.825515003819563e-06
1316,6441,0,6441,0.24441814422607422,2.8133566206820866e-06
1319,6456,0,6456,0.24495911598205566,2.7983834964888803e-06
1322,6471,0,6471,0.24558806419372559,2.786149766740908e-06
1325,6486,0,6486,0.24625420570373535,2.775832357995845e-06
1327,6496,0,6496,0.24669408798217773,2.7697557384574726e-06
1330,6511,0,6511,0.2472381591796875,2.7615716638608936e-06
1333,6526,0,6526,0.24777817726135254,2.7542694851530705e-06
1336,6541,0,6541,0.2482900619506836,2.7476600806567245e-06
1338,6551,0,6551,0.24863004684448242,2.7435688675360953e-06
1341,6566,0,6566,0.24922800064086914,2.7378268414341918e-06
1344,6581,0,6581,0.24977993965148926,2.7324872839029086e-06
1347,6596,0,6596,0.25030517578125,2.7274862083249876e-06
1350,6611,0,6611,0.25083208084106445,2.722770326237086e-06
1352,6621,0,6621,0.2511758804321289,2.7197635210725546e-06
1355,6636,0,6636,0.2517051696777344,2.7154345896449282e-06
1358,6651,0,6651,0.25221824645996094,2.711301336472653e-06
1361,6666,0,6666,0.2527310848236084,2.7073452616810315e-06
1363,6676,0,6676,0.25307393074035645,2.704799064619757e-06
1366,6691,0,6691,0.25369811058044434,2.7011068543580946e-06
1369,6706,0,6706,0.25426197052001953,2.697555819575744e-06
1372,6721,0,6721,0.2549459934234619,2.6941335198392325e-06
1374,6731,0,6731,0.25542616844177246,2.6919178248855605e-06
1377,6746,0,6746,0.25597596168518066,2.6886852134865787e-06
1380,6761,0,6761,0.25649404525756836,2.6855530031216895e-06
1383,6776,0,6776,0.25701212882995605,2.6825122813111043e-06
1385,6786,0,6786,0.2573549747467041,2.680532026026334e-06
1388,6801,0,6801,0.257871150970459,2.6776267311060135e-06
1391,6816,0,6816,0.2583901882171631,2.674793964879876e-06
1394,6831,0,6831,0.2589089870452881,2.6720283521045454e-06
1396,6841,0,6841,0.25942206382751465,2.6702197185129234e-06
1399,6856,0,6856,0.26016712188720703,2.667556692117271e-06
1402,6871,0,6871,0.2609071731567383,2.6649507534873763e-06
1405,6886,0,6886,0.2614731788635254,2.662399051781628e-06
1407,6896,0,6896,0.26180505752563477,2.660726763053682e-06
1410,6911,0,6911,0.2623002529144287,2.658259859108976e-06
1413,6926,0,6926,0.2628202438354492,2.6558409451789093e-06
1416,6941,0,6941,0.26333117485046387,2.6534682140728577e-06
1419,6956,0,6956,0.26384687423706055,2.6511401071389585e-06
1421,6966,0,6966,0.2641761302947998,2.6496121401442438e-06
1424,6980,0,6980,0.264660120010376,2.5875773480749696e-06
1427,6995,0,6995,0.2651660442352295,2.5541930994306583e-06
1430,7010,0,7010,0.26566505432128906,2.535035950216586e-06
1432,7020,0,7020,0.26599597930908203,2.5266874549896376e-06
1435,7035,0,7035,0.26657795906066895,2.517992542086424e-06
1438,7050,0,7050,0.26709818840026855,2.51197890441103e-06
1441,7065,0,7065,0.26761913299560547,2.5074567159187727e-06
1443,7075,0,7075,0.2679469585418701,2.5049497090150837e-06
1446,7090,0,7090,0.26843905448913574,2.501680603717086e-06
1449,7105,0,7105,0.26892900466918945,2.4988055693463373e-06
1452,7120,0,7120,0.2694251537322998,2.4961945620156454e-06
1454,7130,0,7130,0.26975107192993164,2.494562713700712e-06
1457,7145,0,7145,0.27024316787719727,2.492242542892562e-06
1460,7160,0,7160,0.27074313163757324,2.4900436769134085e-06
1463,7175,0,7175,0.2712230682373047,2.487943137534847e-06
1465,7185,0,7185,0.27153992652893066,2.486590041500796e-06
1468,7200,0,7200,0.27204203605651855,2.484622160256594e-06
1471,7215,0,7215,0.27253198623657227,2.482717870221401e-06
1474,7230,0,7230,0.2730412483215332,2.480868038594415e-06
1476,7240,0,7240,0.27338290214538574,2.479662012332434e-06
1479,7255,0,7255,0.2738771438598633,2.4778902388718413e-06
1482,7270,0,7270,0.274367094039917,2.4761603814386782e-06
1485,7285,0,7285,0.2748579978942871,2.474469714802195e-06
1488,7300,0,7300,0.27543091773986816,2.472815425290708e-06
1490,7310,0,7310,0.27579498291015625,2.471731143657675e-06
1493,7325,0,7325,0.2763810157775879,2.4701299211508768e-06
1496,7340,0,7340,0.276885986328125,2.4685557546912557e-06
1499,7355,0,7355,0.2773780822753906,2.467005112061121e-06
1501,7365,0,7365,0.2777259349822998,2.465982805701526e-06
1504,7380,0,7380,0.27823686599731445,2.4644645667696225e-06
1507,7395,0,7395,0.278764009475708,2.4629629791726736e-06
1510,7410,0,7410,0.2792961597442627,2.461477033108419e-06
1512,7420,0,7420,0.2796480655670166,2.4604948564909733e-06
1515,7435,0,7435,0.28017616271972656,2.4590340447750368e-06
1518,7450,0,7450,0.28070497512817383,2.4575877623670133e-06
1521,7465,0,7465,0.2812340259552002,2.4561552657092195e-06
1523,7474,0,7474,0.2815732955932617,2.365294737299574e-06
1526,7489,0,7489,0.28209996223449707,2.3370566017095867e-06
1529,7503,0,7503,0.2826361656188965,2.301593800199192e-06
1532,7517,0,7517,0.2831540107727051,2.155350315394666e-06
1534,7526,0,7526,0.28348708152770996,2.0217226014655007e-06
1537,7540,0,7540,0.2840290069580078,1.8856186458565675e-06
1540,7554,0,7554,0.2845580577850342,1.7585380570023783e-06
1543,7567,0,7567,0.28506922721862793,1.6088711448180783e-06
1545,7576,0,7576,0.2854180335998535,1.4506853157722665e-06
1548,7591,0,7591,0.28597307205200195,1.3783156199846519e-06
1551,7604,0,7604,0.28647708892822266,1.2677989582658838e-06
1554,7619,0,7619,0.2870190143585205,1.211423523901795e-06
1557,7634,0,7634,0.2875509262084961,1.1748658080994442e-06
1559,7644,0,7644,0.28791308403015137,1.157184881247898e-06
1562,7659,0,7659,0.28844594955444336,1.136952819519226e-06
1565,7673,0,7673,0.28895998001098633,1.0810180266804684e-06
1568,7687,0,7687,0.2894761562347412,1.0387579905495046e-06
1570,7697,0,7697,0.2898261547088623,1.0071745192261407e-06
1573,7711,0,7711,0.29033923149108887,9.365621526162807e-07
1576,7726,0,7726,0.2908651828765869,9.114518863847938e-07
1579,7739,0,7739,0.29137301445007324,8.817974357476358e-07
1581,7749,0,7749,0.29172420501708984,8.451743249190282e-07
1584,7763,0,7763,0.2922370433807373,7.908873005083428e-07
1587,7778,0,7778,0.2927720546722412,7.643083082059342e-07
1590,7790,0,7790,0.2932569980621338,7.241382598194564e-07
1592,7800,0,7800,0.2936272621154785,6.968844915145934e-07
1595,7814,0,7814,0.2941560745239258,6.406349371428517e-07
1598,7829,0,7829,0.29470014572143555,6.069295930738345e-07
1601,7843,0,7843,0.2952260971069336,5.855593056319066e-07
1603,7853,0,7853,0.2955892086029053,5.635845660583538e-07
1606,7868,0,7868,0.2961452007293701,5.406935608633478e-07
1609,7881,0,7881,0.2966599464416504,4.7570021930097125e-07
1612,7895,0,7895,0.29718923568725586,4.466822404465061e-07
1614,7905,0,7905,0.2975490093231201,4.3200051560295126e-07
1617,7920,0,7920,0.2980940341949463,4.1666486009349335e-07
1620,7934,0,7934,0.29863810539245605,3.862115809222853e-07
1623,7949,0,7949,0.29917311668395996,3.749186875921931e-07
1625,7959,0,7959,0.2995278835296631,3.695942851358647e-07
1628,7973,0,7973,0.30004215240478516,3.445740207570767e-07
1631,7988,0,7988,0.30059218406677246,3.368327921620668e-07
1634,8002,0,8002,0.30112314224243164,3.211379937928808e-07
1637,8016,0,8016,0.3016550540924072,3.00444764427055e-07
1639,8026,0,8026,0.3020191192626953,2.9433450563544893e-07
1642,8041,0,8041,0.3025641441345215,2.8761056925697303e-07
1645,8056,0,8056,0.30311012268066406,2.8264890164228236e-07
1648,8071,0,8071,0.30364012718200684,2.787252317626068e-07
1650,8081,0,8081,0.30399417877197266,2.764897973650421e-07
1653,8094,0,8094,0.30449509620666504,2.589048349747493e-07
1656,8109,0,8109,0.3050539493560791,2.472809025186362e-07
1659,8124,0,8124,0.3056020736694336,2.405587119630202e-07
1661,8134,0,8134,0.3059682846069336,2.375439817306853e-07
1664,8149,0,8149,0.3065159320831299,2.3424132006756656e-07
1667,8163,0,8163,0.3070511817932129,2.2658136697854052e-07
1670,8178,0,8178,0.30759716033935547,2.205810962843325e-07
1672,8188,0,8188,0.30796003341674805,2.178916801516139e-07
1675,8203,0,8203,0.30850815773010254,2.150099873239416e-07
1678,8218,0,8218,0.309053897857666,2.1296900057017473e-07
1681,8233,0,8233,0.3096120357513428,2.1142757288396532e-07
1683,8243,0,8243,0.30997610092163086,2.105824799641614e-07
1686,8258,0,8258,0.31052112579345703,2.095042480815516e-07
1689,8273,0,8273,0.3110690116882324,2.0859291121511745e-07
1692,8288,0,8288,0.3116140365600586,2.0780429391436728e-07
1694,8298,0,8298,0.31197690963745117,2.0733246554998602e-07
1697,8313,0,8313,0.31252098083496094,2.066909523170197e-07
1700,8328,0,8328,0.3130650520324707,2.0611576422667097e-07
1703,8343,0,8343,0.31361889839172363,2.05595880812514e-07
1706,8358,0,8358,0.3141360282897949,2.0512246916714944e-07
1708,8368,0,8368,0.31447815895080566,2.0482920917259011e-07
1711,8383,0,8383,0.3150179386138916,2.0441877401233036e-07
1714,8398,0,8398,0.31554317474365234,2.0403970161921647e-07
1717,8413,0,8413,0.3160691261291504,2.036882454320115e-07
1719,8423,0,8423,0.316425085067749,2.0346773195244446e-07
1722,8438,0,8438,0.31695103645324707,2.0315575312684168e-07
1725,8453,0,8453,0.3174741268157959,2.0286438522402698e-07
1728,8468,0,8468,0.31800007820129395,2.025916069627767e-07
1730,8478,0,8478,0.31834912300109863,2.0241913551981162e-07
1733,8493,0,8493,0.31888628005981445,2.0217313619263958e-07
1736,8508,0,8508,0.319411039352417,2.0194086555091704e-07
1739,8523,0,8523,0.3199450969696045,2.0172069965744723e-07
1741,8533,0,8533,0.320296049118042,2.015798980484293e-07
1744,8548,0,8548,0.3208472728729248,2.013766673059753e-07
1747,8563,0,8563,0.32140493392944336,2.011820399390155e-07
1750,8578,0,8578,0.32195115089416504,2.009952446799885e-07
1752,8588,0,8588,0.3223130702972412,2.0087480841937712e-07
1755,8603,0,8603,0.32285594940185547,2.0069999705599796e-07
1758,8618,0,8618,0.32340192794799805,2.0053183359116154e-07
1761,8633,0,8633,0.3239428997039795,2.0036984044734644e-07
1763,8643,0,8643,0.32430601119995117,2.0026500261758062e-07
1766,8658,0,8658,0.32485008239746094,2.0011204420996341e-07
1769,8673,0,8673,0.3253939151763916,1.9996371269170867e-07
1772,8688,0,8688,0.3259410858154297,1.998194383917363e-07
1775,8703,0,8703,0.32645726203918457,1.9967871472938914e-07
1777,8712,0,8712,0.3268101215362549,1.9618488660504944e-07
1780,8727,0,8727,0.32734203338623047,1.940914046497025e-07
1783,8742,0,8742,0.3278791904449463,1.928820289633566e-07
1786,8757,0,8757,0.3284111022949219,1.9210858946857104e-07
1788,8766,0,8766,0.3287510871887207,1.8264502389573785e-07
1791,8780,0,8780,0.32927632331848145,1.7172140541568078e-07
1794,8793,0,8793,0.32976508140563965,1.6281623685250698e-07
1797,8806,0,8806,0.33025622367858887,1.409479343077729e-07
1799,8815,0,8815,0.3305931091308594,1.2597720854392425e-07
1802,8830,0,8830,0.3311161994934082,1.1590473804700262e-07
1805,8844,0,8844,0.33162498474121094,1.0446801016866022e-07
1808,8857,0,8857,0.33213210105895996,9.655110907394189e-08
1810,8866,0,8866,0.33246707916259766,9.025142100903125e-08
1813,8881,0,8881,0.3330521583557129,8.462339598941031e-08
1816,8895,0,8895,0.33361101150512695,8.035582729783978e-08
1819,8909,0,8909,0.3341529369354248,7.587679362721931e-08
1821,8919,0,8919,0.3345170021057129,7.362580020392493e-08
1824,8933,0,8933,0.33504724502563477,6.808799968232382e-08
1827,8947,0,8947,0.3355591297149658,6.427227856540295e-08
1830,8962,0,8962,0.3360869884490967,6.216457154865567e-08
1832,8972,0,8972,0.3364369869232178,6.115572400885286e-08
1835,8987,0,8987,0.3369762897491455,6.000083496571296e-08
1838,9002,0,9002,0.33750295639038086,5.9116329630256266e-08
1841,9017,0,9017,0.3380601406097412,5.839728255582356e-08
1844,9030,0,9030,0.3385632038116455,5.539048887028729e-08
1846,9040,0,9040,0.33890819549560547,5.319163436277037e-08
1849,9054,0,9054,0.33941006660461426,4.930200825222037e-08
1852,9068,0,9068,0.33991122245788574,4.505976433244823e-08
1855,9082,0,9082,0.34041500091552734,4.2842693542097526e-08
1857,9092,0,9092,0.34077906608581543,4.169370395121293e-08
1860,9107,0,9107,0.34131717681884766,4.055209696675106e-08
1863,9122,0,9122,0.3418450355529785,3.9806160781881566e-08
1866,9135,0,9135,0.3423440456390381,3.714154313862991e-08
1868,9144,0,9144,0.3426802158355713,3.586465989394687e-08
1871,9159,0,9159,0.34320807456970215,3.4308025561017155e-08
1874,9174,0,9174,0.3437371253967285,3.330340345494854e-08
1877,9189,0,9189,0.3442649841308594,3.261870203936447e-08
1879,9198,0,9198,0.34460020065307617,3.099179535356986e-08
1882,9213,0,9213,0.3451261520385742,3.0093552206720244e-08
1885,9228,0,9228,0.34566307067871094,2.948290428774711e-08
1888,9243,0,9243,0.3461933135986328,2.9042807899759837e-08
1890,9252,0,9252,0.3465311527252197,2.7260395878054802e-08
1893,9265,0,9265,0.34702515602111816,2.4800864385637803e-08
1896,9280,0,9280,0.3475489616394043,2.297537955170156e-08
1899,9294,0,9294,0.34806299209594727,2.1609841117307712e-08
1901,9304,0,9304,0.34841299057006836,2.097774165468364e-08
1904,9319,0,9319,0.3489420413970947,2.038640390842626e-08
1907,9334,0,9334,0.34946608543395996,2.003616097280622e-08
1910,9349,0,9349,0.3500070571899414,1.9812302021227525e-08
1913,9364,0,9364,0.35054898262023926,1.9656648569126002e-08
1915,9374,0,9374,0.3509082794189453,1.9575561891699236e-08
1918,9389,0,9389,0.3514530658721924,1.9475392055780312e-08
1921,9404,0,9404,0.35199618339538574,1.9392641393045845e-08
1924,9418,0,9418,0.3525052070617676,1.8838112446948954e-08
1926,9428,0,9428,0.3528561592102051,1.852445203902256e-08
1929,9442,0,9442,0.3533670902252197,1.771375487713998e-08
1932,9457,0,9457,0.3538932800292969,1.742708759207402e-08
1935,9472,0,9472,0.35442304611206055,1.7257891959607907e-08
1937,9482,0,9482,0.3548281192779541,1.7181235408881338e-08
1940,9497,0,9497,0.3553750514984131,1.7097883439139627e-08
1943,9512,0,9512,0.35595011711120605,1.70373873436917e-08
1946,9527,0,9527,0.35648012161254883,1.6990384324263504e-08
1948,9537,0,9537,0.35683512687683105,1.6964032421793135e-08
1951,9552,0,9552,0.35747623443603516,1.69296260791417e-08
1954,9567,0,9567,0.3580300807952881,1.6899657624674903e-08
1957,9582,0,9582,0.35858607292175293,1.6872907545530327e-08
1959,9592,0,9592,0.35893917083740234,1.685644636981152e-08
1962,9607,0,9607,0.35947489738464355,1.683342913872355e-08
1965,9622,0,9622,0.3600001335144043,1.6812064132909067e-08
1968,9637,0,9637,0.3605220317840576,1.6792040758593045e-08
1970,9647,0,9647,0.3608710765838623,1.6779322010352414e-08
1973,9662,0,9662,0.36139488220214844,1.676103946500058e-08
1976,9677,0,9677,0.36191701889038086,1.6743572564045907e-08
1979,9692,0,9692,0.3624420166015625,1.6726792108561862e-08
1982,9707,0,9707,0.3629581928253174,1.6710597410348718e-08
1984,9717,0,9717,0.36329126358032227,1.6700085442855786e-08
1987,9732,0,9732,0.3638150691986084,1.6684694474117155e-08
1990,9747,0,9747,0.3643321990966797,1.6669715972159157e-08
1993,9762,0,9762,0.36484193801879883,1.665511657542947e-08
1995,9772,0,9772,0.36518025398254395,1.6645581484989312e-08
1998,9787,0,9787,0.36568713188171387,1.6631553058445875e-08
2001,9802,0,9802,0.3662281036376953,1.6617819664473662e-08
2004,9817,0,9817,0.36673521995544434,1.660433894975015e-08
2006,9827,0,9827,0.3671150207519531,1.659547191801201e-08
2009,9842,0,9842,0.36762213706970215,1.658232744625533e-08
2012,9857,0,9857,0.3681371212005615,1.656934834192298e-08
2015,9872,0,9872,0.36903810501098633,1.655651623242577e-08
2017,9882,0,9882,0.3695220947265625,1.6548036116226342e-08
2020,9897,0,9897,0.3701629638671875,1.6535419171668465e-08
2023,9912,0,9912,0.3709421157836914,1.6522917769190396e-08
2026,9927,0,9927,0.371751070022583,1.6510523871246643e-08
2028,9937,0,9937,0.3722350597381592,1.6502317367021553e-08
2031,9952,0,9952,0.3730580806732178,1.649008649514873e-08
2034,9967,0,9967,0.37410998344421387,1.6477944135283423e-08
2037,9982,0,9982,0.3749251365661621,1.6465884188087242e-08
2039,9991,0,9991,0.3755199909210205,1.6412587381851952e-08
2042,10006,0,10006,0.3763699531555176,1.6290512459858528e-08
2045,10021,0,10021,0.37724804878234863,1.621935130111196e-08
2048,10036,0,10036,0.37809109687805176,1.6174301230293025e-08
2051,10051,0,10051,0.3791213035583496,1.6143089577953214e-08
2053,10061,0,10061,0.37967610359191895,1.612673435696325e-08
2056,10076,0,10076,0.38027119636535645,1.6106192557470387e-08
2059,10091,0,10091,0.3808262348175049,1.608866371793412e-08
2062,10106,0,10106,0.3813660144805908,1.6072951659548715e-08
2064,10116,0,10116,0.3817911148071289,1.6063156761092564e-08
2067,10131,0,10131,0.38237690925598145,1.6049167256570386e-08
2070,10146,0,10146,0.38292813301086426,1.6035797523954656e-08
2073,10161,0,10161,0.3834550380706787,1.6022888676760145e-08
2075,10171,0,10171,0.38381528854370117,1.6014476364851885e-08
2078,10186,0,10186,0.3843240737915039,1.6002103168210092e-08
2081,10201,0,10201,0.3848581314086914,1.5989973334887265e-08
2084,10216,0,10216,0.3853881359100342,1.597804538143473e-08
2086,10226,0,10226,0.38573527336120605,1.5970195370986e-08
2089,10241,0,10241,0.38626718521118164,1.595854737417193e-08
2092,10256,0,10256,0.38680195808410645,1.5947038253339007e-08
2095,10271,0,10271,0.387404203414917,1.593565244629328e-08
2097,10281,0,10281,0.3877832889556885,1.5928125796556165e-08
2100,10296,0,10296,0.388322114944458,1.5916933667910425e-08
2103,10311,0,10311,0.3888521194458008,1.5905858825808854e-08
2106,10326,0,10326,0.3893849849700928,1.589490445833459e-08
2108,10336,0,10336,0.38976001739501953,1.588766792560338e-08
2111,10351,0,10351,0.3903040885925293,1.587691020327668e-08
2114,10366,0,10366,0.3908541202545166,1.5866263762621322e-08
2117,10381,0,10381,0.39139723777770996,1.5855719919750517e-08
2119,10391,0,10391,0.39178013801574707,1.5848742892762832e-08
2122,10406,0,10406,0.39233899116516113,1.583834661373175e-08
2125,10421,0,10421,0.39290404319763184,1.582802307355258e-08
2128,10436,0,10436,0.3934462070465088,1.5817761407191452e-08
2131,10451,0,10451,0.39403319358825684,1.5807552949593554e-08
2133,10461,0,10461,0.39455509185791016,1.580077399051287e-08
2136,10476,0,10476,0.3954041004180908,1.5790642743901783e-08
2139,10491,0,10491,0.39608311653137207,1.578055433398382e-08
2142,10506,0,10506,0.39675211906433105,1.5770507768145438e-08
2144,10516,0,10516,0.3971900939941406,1.576383321035503e-08
2147,10531,0,10531,0.39788317680358887,1.5753856631369505e-08
2150,10546,0,10546,0.39856410026550293,1.5743923565809794e-08
2153,10561,0,10561,0.3995802402496338,1.5734035833557267e-08
2155,10571,0,10571,0.4000132083892822,1.5727470046486426e-08
2158,10586,0,10586,0.4005711078643799,1.571766106552973e-08
2161,10601,0,10601,0.4011352062225342,1.5707899270273356e-08
2164,10616,0,10616,0.4017021656036377,1.5698182362675736e-08
2166,10626,0,10626,0.4020988941192627,1.5691727404032292e-08
2169,10641,0,10641,0.40269899368286133,1.5682075542886043e-08
2172,10656,0,10656,0.40326929092407227,1.5672455281827832e-08
2175,10671,0,10671,0.4039900302886963,1.5662861258870307e-08
2177,10681,0,10681,0.40442490577697754,1.5656477703418387e-08
2180,10696,0,10696,0.4050130844116211,1.5646919093850514e-08
2183,10711,0,10711,0.40569615364074707,1.5637379759416416e-08
2186,10726,0,10726,0.406278133392334,1.5627860360337763e-08
2188,10736,0,10736,0.40667223930358887,1.5621526014126872e-08
2191,10751,0,10751,0.4072442054748535,1.5612043915048417e-08
2194,10766,0,10766,0.40780115127563477,1.5602586702760675e-08
2197,10781,0,10781,0.4084789752960205,1.5593155449022405e-08
2200,10796,0,10796,0.4092390537261963,1.558375032201824e-08
2202,10806,0,10806,0.40961313247680664,1.557749453011569e-08
2205,10821,0,10821,0.41017603874206543,1.5568131757044223e-08
2208,10836,0,10836,0.4107639789581299,1.5558793599921895e-08
2211,10850,0,10850,0.4113149642944336,1.526535353822427e-08
2213,10860,0,10860,0.41167521476745605,1.5162176132422967e-08
2216,10875,0,10875,0.4122319221496582,1.5072208351013462e-08
2219,10890,0,10890,0.41298723220825195,1.5023078877337182e-08
2222,10905,0,10905,0.4136021137237549,1.499357073461855e-08
2224,10915,0,10915,0.41402125358581543,1.497964906281329e-08
2227,10930,0,10930,0.4145650863647461,1.4963356036743708e-08
2230,10944,0,10944,0.4150850772857666,1.464584982614754e-08
2233,10959,0,10959,0.41562318801879883,1.4549957328876965e-08
2235,10969,0,10969,0.41597604751586914,1.4505429590381275e-08
2238,10984,0,10984,0.41651201248168945,1.4456305659635585e-08
2241,10999,0,10999,0.4170980453491211,1.4420142477128335e-08
2244,11014,0,11014,0.41768908500671387,1.4391793134172084e-08
2246,11024,0,11024,0.4181530475616455,1.4375732172359353e-08
2249,11039,0,11039,0.4187352657318115,1.4354445848311717e-08
2252,11054,0,11054,0.4192819595336914,1.4335524401056583e-08
2255,11069,0,11069,0.4200022220611572,1.4318224212048567e-08
2257,11079,0,11079,0.42058706283569336,1.4307380636677065e-08
2260,11094,0,11094,0.4214811325073242,1.429192238354577e-08
2263,11109,0,11109,0.4223520755767822,1.427726747721741e-08
2266,11124,0,11124,0.4230351448059082,1.4263277468422398e-08
2269,11139,0,11139,0.4236581325531006,1.424982833821754e-08
2271,11149,0,11149,0.4241631031036377,1.4241114051779284e-08
2274,11164,0,11164,0.424868106842041,1.4228349784860817e-08
2277,11179,0,11179,0.425584077835083,1.421589344319854e-08
2280,11194,0,11194,0.4261939525604248,1.4203693802857495e-08
2282,11204,0,11204,0.4266800880432129,1.4195683372628304e-08
2285,11219,0,11219,0.4275178909301758,1.4183838302883063e-08
2288,11234,0,11234,0.4282529354095459,1.4172181868734036e-08
2291,11249,0,11249,0.42909693717956543,1.4160699889767743e-08
2293,11259,0,11259,0.4296700954437256,1.4153134840758209e-08
2296,11274,0,11274,0.43049120903015137,1.4141906092640723e-08
2299,11289,0,11289,0.4311821460723877,1.4130801515450517e-08
2302,11304,0,11304,0.43186306953430176,1.4119799128415522e-08
2304,11314,0,11314,0.43224191665649414,1.4112513083899246e-08
2307,11329,0,11329,0.43285107612609863,1.4101651738110806e-08
2310,11344,0,11344,0.433427095413208,1.4090871368385995e-08
2313,11359,0,11359,0.43396520614624023,1.4080175631611373e-08
2315,11369,0,11369,0.43431711196899414,1.407309331304796e-08
2318,11384,0,11384,0.43485212326049805,1.4062541020944171e-08
2321,11399,0,11399,0.4353799819946289,1.4052067800695415e-08
2324,11413,0,11413,0.4358952045440674,1.3738035157306085e-08
2326,11423,0,11423,0.4362492561340332,1.3703284990979096e-08
2329,11438,0,11438,0.43677592277526855,1.3666969307788606e-08
2332,11453,0,11453,0.4373040199279785,1.3641618931341367e-08
2335,11468,0,11468,0.43785715103149414,1.3622358543574311e-08
2338,11483,0,11483,0.43851494789123535,1.3606635044770476e-08
2340,11493,0,11493,0.43889617919921875,1.3597372155124794e-08
2343,11508,0,11508,0.43944597244262695,1.3584708703093371e-08
2346,11523,0,11523,0.4399881362915039,1.3573048170528368e-08
2349,11538,0,11538,0.44057607650756836,1.3562076911759877e-08
2351,11548,0,11548,0.4409310817718506,1.3555058471514826e-08
2354,11563,0,11563,0.4414541721343994,1.3544867496324308e-08
2357,11578,0,11578,0.44197607040405273,1.3535011910133828e-08
2360,11593,0,11593,0.44249916076660156,1.3525423588900518e-08
2362,11603,0,11603,0.44284796714782715,1.3519150225969387e-08
2365,11618,0,11618,0.44336891174316406,1.350989189621738e-08
2368,11633,0,11633,0.44388818740844727,1.3500781710172063e-08
2371,11648,0,11648,0.4444139003753662,1.3491797199139283e-08
2373,11658,0,11658,0.4447810649871826,1.3485869798635184e-08
2376,11673,0,11673,0.4453110694885254,1.3477064933272303e-08
2379,11688,0,11688,0.44585108757019043,1.3468362014213292e-08
2382,11703,0,11703,0.4463770389556885,1.3459758845291985e-08
2384,11713,0,11713,0.44672203063964844,1.3454077965125577e-08
2387,11728,0,11728,0.4472391605377197,1.3445633990177339e-08
2390,11743,0,11743,0.4477660655975342,1.3437274916713406e-08
2393,11758,0,11758,0.4482691287994385,1.3428989916594936e-08
2395,11768,0,11768,0.44863414764404297,1.3423502084758148e-08
2398,11783,0,11783,0.44973111152648926,1.3415317386322823e-08
2401,11798,0,11798,0.4508180618286133,1.3407183630277758e-08
2404,11813,0,11813,0.451876163482666,1.3399097061475172e-08
2407,11828,0,11828,0.45247626304626465,1.3391054989374389e-08
2409,11838,0,11838,0.45296216011047363,1.3385716734789305e-08
2412,11853,0,11853,0.45381712913513184,1.3377741471402824e-08
2415,11867,0,11867,0.4545552730560303,1.3182110387603094e-08
2418,11882,0,11882,0.45547008514404297,1.308192614929276e-08
2420,11892,0,11892,0.456118106842041,1.3039115605003103e-08
2423,11907,0,11907,0.4569740295410156,1.2995308780502687e-08
2426,11922,0,11922,0.4577779769897461,1.296563869474951e-08
2429,11937,0,11937,0.4586312770843506,1.2943719184953953e-08
2431,11947,0,11947,0.45919108390808105,1.2931707817093523e-08
2434,11962,0,11962,0.460064172744751,1.2916117542729132e-08
2437,11977,0,11977,0.4606201648712158,1.2902411473338783e-08
2440,11992,0,11992,0.4611551761627197,1.288992371709451e-08
2442,12002,0,12002,0.4615061283111572,1.2882080942191163e-08
2445,12017,0,12017,0.46204113960266113,1.2870845270237794e-08
2448,12032,0,12032,0.462583065032959,1.2860092820115589e-08
2451,12047,0,12047,0.46312499046325684,1.2849709407316408e-08
2453,12057,0,12057,0.4634859561920166,1.2842953302795337e-08
2456,12072,0,12072,0.46402406692504883,1.2833033368196003e-08
2459,12087,0,12087,0.4646131992340088,1.2823341608757687e-08
2462,12102,0,12102,0.46520018577575684,1.2813862767788537e-08
2464,12112,0,12112,0.4655799865722656,1.2807655565881246e-08
2467,12127,0,12127,0.46611523628234863,1.2798503948107474e-08
2470,12142,0,12142,0.46665406227111816,1.278953026632331e-08
2473,12157,0,12157,0.4675741195678711,1.2780719018068833e-08
2476,12172,0,12172,0.4685981273651123,1.2772053558780151e-08
2478,12182,0,12182,0.46927690505981445,1.2766348999969079e-08
2481,12197,0,12197,0.47034406661987305,1.2757889118146377e-08
2484,12212,0,12212,0.47144007682800293,1.2749533804985142e-08
2487,12227,0,12227,0.4724850654602051,1.2741273629175323e-08
2489,12237,0,12237,0.47303199768066406,1.2735816795624168e-08
2492,12252,0,12252,0.4740889072418213,1.2727703770918187e-08
2495,12267,0,12267,0.47518205642700195,1.2719674783546974e-08
2498,12282,0,12282,0.4759361743927002,1.2711726086609146e-08
2500,12292,0,12292,0.4763169288635254,1.270646928789056e-08
2503,12307,0,12307,0.4768829345703125,1.2698643883929764e-08
2506,12322,0,12322,0.47742319107055664,1.2690886139468926e-08
2509,12337,0,12337,0.47808098793029785,1.2683192177211242e-08
2511,12347,0,12347,0.47844624519348145,1.2678096703245207e-08
2514,12362,0,12362,0.47898006439208984,1.2670502079047005e-08
2517,12377,0,12377,0.47951626777648926,1.2662963018826459e-08
2520,12392,0,12392,0.4800550937652588,1.2655476155941587e-08
2522,12402,0,12402,0.48041820526123047,1.2650512261661011e-08
2525,12417,0,12417,0.48104310035705566,1.264310540946287e-08
2528,12432,0,12432,0.48186230659484863,1.2635743942017217e-08
2531,12447,0,12447,0.4825270175933838,1.2628427467361792e-08
2533,12457,0,12457,0.48289012908935547,1.262357501071453e-08
2536,12472,0,12472,0.4834320545196533,1.2616334424828416e-08
2539,12487,0,12487,0.4839742183685303,1.2609139324436626e-08
2542,12502,0,12502,0.4845161437988281,1.2601988413015328e-08
2544,12512,0,12512,0.48488306999206543,1.2597244556459097e-08
2547,12526,0,12526,0.4854001998901367,1.190076571131842e-08
2550,12541,0,12541,0.48595404624938965,1.1714081577272082e-08
2553,12556,0,12556,0.486497163772583,1.159445350509966e-08
2556,12571,0,12571,0.48703789710998535,1.1512623494480643e-08
2558,12581,0,12581,0.48738718032836914,1.1471055108371804e-08
2561,12596,0,12596,0.4879722595214844,1.1421419981625326e-08
2564,12611,0,12611,0.48853516578674316,1.1382223615730718e-08
2567,12626,0,12626,0.4890601634979248,1.1350084445534434e-08
2569,12636,0,12636,0.4894070625305176,1.1331487380405223e-08
2572,12651,0,12651,0.48993515968322754,1.1306795244119044e-08
2575,12666,0,12666,0.4904608726501465,1.1285096167202815e-08
2578,12681,0,12681,0.4909839630126953,1.1265702728679248e-08
2580,12691,0,12691,0.4913301467895508,1.1253817251480656e-08
2583,12706,0,12706,0.491879940032959,1.1237272204436978e-08
2586,12721,0,12721,0.4924123287200928,1.1222013015443201e-08
2589,12736,0,12736,0.49294590950012207,1.120779888759389e-08
2591,12746,0,12746,0.4933052062988281,1.119879984252299e-08
2594,12761,0,12761,0.493847131729126,1.1185895969130038e-08
2597,12776,0,12776,0.4943842887878418,1.1173600725299974e-08
2600,12791,0,12791,0.49493408203125,1.1161827083833318e-08
2602,12801,0,12801,0.49530506134033203,1.1154236111589346e-08
2605,12816,0,12816,0.49584412574768066,1.1143198196328444e-08
2608,12831,0,12831,0.4963819980621338,1.1132539067374412e-08
2611,12846,0,12846,0.4969191551208496,1.1122216052374899e-08
2613,12856,0,12856,0.49727511405944824,1.1115501113258914e-08
2616,12871,0,12871,0.4978141784667969,1.1105651997091809e-08
2619,12886,0,12886,0.4983501434326172,1.109604078130264e-08
2622,12901,0,12901,0.4988832473754883,1.1086639669868788e-08
2625,12916,0,12916,0.4994041919708252,1.1077430583401763e-08
2627,12926,0,12926,0.4998021125793457,1.107139323954439e-08
2630,12941,0,12941,0.5003483295440674,1.1062487048713991e-08
2633,12956,0,12956,0.500885009765625,1.105375600794403e-08
2636,12971,0,12971,0.5014200210571289,1.104519087652998e-08
2638,12981,0,12981,0.501777172088623,1.1039565765493986e-08
2641,12996,0,12996,0.5023109912872314,1.1031241952816138e-08
2644,13010,0,13010,0.5028290748596191,1.0999897894240138e-08
2647,13025,0,13025,0.5039370059967041,1.0938282112619736e-08
2649,13035,0,13035,0.5043749809265137,1.0911878084319813e-08
2652,13050,0,13050,0.5049259662628174,1.0884523472348469e-08
2655,13065,0,13065,0.5054771900177002,1.0865527495988633e-08
2658,13080,0,13080,0.5061841011047363,1.0851159943762737e-08
2660,13090,0,13090,0.5067341327667236,1.0843126552889593e-08
2663,13105,0,13105,0.5073580741882324,1.0832526641687128e-08
2666,13120,0,13120,0.5079700946807861,1.0823071696995068e-08
2669,13135,0,13135,0.5086252689361572,1.0814384727931001e-08
2671,13145,0,13145,0.5090723037719727,1.0808911743239023e-08
2674,13160,0,13160,0.5097780227661133,1.0801073579843694e-08
2677,13175,0,13175,0.5104250907897949,1.079359844390247e-08
2680,13190,0,13190,0.5110621452331543,1.078640926771569e-08
2682,13200,0,13200,0.5114302635192871,1.0781739552052102e-08
2685,13215,0,13215,0.5119800567626953,1.0774883633914322e-08
2688,13230,0,13230,0.5125088691711426,1.076816424124393e-08
2691,13245,0,13245,0.5130372047424316,1.076155315569606e-08
2694,13260,0,13260,0.51357102394104,1.0755034594845142e-08
2696,13270,0,13270,0.5139250755310059,1.0750735640946734e-08
2699,13285,0,13285,0.5147171020507812,1.0744357313842805e-08
2702,13300,0,13300,0.5154850482940674,1.0738058252854611e-08
2705,13315,0,13315,0.5161871910095215,1.073183113286705e-08
2707,13325,0,13325,0.5165722370147705,1.0727714579982125e-08
2710,13340,0,13340,0.5171880722045898,1.0721582859815896e-08
2713,13355,0,13355,0.5179860591888428,1.071549495450761e-08
2716,13370,0,13370,0.5188751220703125,1.0709444556906212e-08
2718,13380,0,13380,0.5195791721343994,1.0705430686522191e-08
2721,13395,0,13395,0.5204942226409912,1.069943916137414e-08
2724,13410,0,13410,0.5213272571563721,1.0693482201470206e-08
2727,13425,0,13425,0.5220742225646973,1.068755749947882e-08
2729,13435,0,13435,0.5224592685699463,1.0683623232135962e-08
2732,13450,0,13450,0.523169994354248,1.0677740571494143e-08
2735,13465,0,13465,0.5238831043243408,1.0671874542924163e-08
2738,13480,0,13480,0.5244491100311279,1.0666019753172266e-08
2740,13490,0,13490,0.5249121189117432,1.0662121144859335e-08
2743,13505,0,13505,0.525604248046875,1.0656279180503394e-08
2746,13519,0,13519,0.5261900424957275,1.052949158506634e-08
2749,13534,0,13534,0.5267930030822754,1.0497365971310564e-08
2751,13544,0,13544,0.5271632671356201,1.048266974087325e-08
2754,13559,0,13559,0.5277750492095947,1.0466609091959363e-08
2757,13573,0,13573,0.5283730030059814,9.967380256916036e-09


==> plot_data/quadratic_minimax_problem_n20_alpha00001/flex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,7.295608520507812e-05,4.387072431292609
1,3,0,3,0.00017189979553222656,3.9719937673698036
2,6,0,6,0.0003688335418701172,3.6265995713934247
3,9,0,9,0.0004899501800537109,2.671453375268637
4,12,0,12,0.0006248950958251953,2.4144090921154513
5,15,0,15,0.0007386207580566406,1.5658221694735213
6,18,0,18,0.0008878707885742188,1.4684861444492576
7,21,0,21,0.0010027885437011719,1.1798911647236028
8,24,0,24,0.0011358261108398438,1.117166644632543
9,27,0,27,0.0012538433074951172,0.8368383001013324
10,30,0,30,0.001390695571899414,0.791899118477761
11,33,0,33,0.0015096664428710938,0.6055985084793335
12,36,0,36,0.0016448497772216797,0.5616175798559058
13,39,0,39,0.0017697811126708984,0.4227903890593488
14,42,0,42,0.0019228458404541016,0.4061053285128045
15,45,0,45,0.002045869827270508,0.3528419133996219
16,48,0,48,0.0021889209747314453,0.3357730534047567
17,51,0,51,0.0023186206817626953,0.2502581592012376
18,54,0,54,0.002530813217163086,0.2433781962784082
19,57,0,57,0.002706766128540039,0.18473321536660026
20,60,0,60,0.002873659133911133,0.18152669283485065
21,63,0,63,0.0030210018157958984,0.15738429407532292
22,66,0,66,0.0031769275665283203,0.15596930064324618
23,69,0,69,0.0033278465270996094,0.15441418844404023
24,72,0,72,0.0034618377685546875,0.12974292240134785
25,75,0,75,0.0036127567291259766,0.12704442339728433
26,78,0,78,0.003744840621948242,0.10719610350380714
27,81,0,81,0.003908634185791016,0.10603854634897296
28,84,0,84,0.0040738582611083984,0.08108624863755504
29,87,0,87,0.004220724105834961,0.08027009439315946
30,90,0,90,0.004349946975708008,0.0638939330914072
31,93,0,93,0.004495859146118164,0.06304197476918527
32,96,0,96,0.004624843597412109,0.061981996497830684
33,99,0,99,0.004789829254150391,0.061714185028897445
34,102,0,102,0.00493168830871582,0.06148540189151549
35,105,0,105,0.0050716400146484375,0.060951022819812
36,108,0,108,0.005211830139160156,0.060635107032990326
37,111,0,111,0.005337715148925781,0.0585350634913127
38,114,0,114,0.005478858947753906,0.05799964749239912
39,117,0,117,0.005604743957519531,0.05614581611090632
40,120,0,120,0.0057446956634521484,0.05580850661355847
41,123,0,123,0.005871772766113281,0.05472935751071315
42,126,0,126,0.006081819534301758,0.05448577024452025
43,129,0,129,0.006413698196411133,0.05356067895920529
44,132,0,132,0.0067157745361328125,0.05324735585084745
45,135,0,135,0.007030963897705078,0.05162480880792435
46,138,0,138,0.007487773895263672,0.05140105031967098
47,141,0,141,0.007878780364990234,0.05116693679634146
48,144,0,144,0.00819087028503418,0.049529404058950365
49,147,0,147,0.008530855178833008,0.0493068791924402
50,150,0,150,0.008862972259521484,0.0460716194361311
51,153,0,153,0.009141921997070312,0.04585995135443143
52,156,0,156,0.009457826614379883,0.04565146880844413
53,159,0,159,0.009685993194580078,0.04217592917915784
54,162,0,162,0.009954690933227539,0.04162859787171804
55,165,0,165,0.01012563705444336,0.03907140204258411
56,168,0,168,0.010291814804077148,0.03818517080019767
57,171,0,171,0.01043081283569336,0.03663163635924788
58,174,0,174,0.010680675506591797,0.035901055481322046
59,177,0,177,0.010938882827758789,0.0338782706500878
60,180,0,180,0.011221885681152344,0.03328126152231233
61,183,0,183,0.011490583419799805,0.03294031572574751
62,186,0,186,0.01172780990600586,0.03242192259213498
63,189,0,189,0.011928796768188477,0.03078552357091988
64,192,0,192,0.012151956558227539,0.030335803786928114
65,195,0,195,0.012445926666259766,0.029450995704127094
66,198,0,198,0.012801885604858398,0.029164376272614086
67,201,0,201,0.013107776641845703,0.02881640212142582
68,204,0,204,0.013415813446044922,0.02827588534210063
69,207,0,207,0.013753652572631836,0.02815550424746922
70,210,0,210,0.014047861099243164,0.027713561324896153
71,213,0,213,0.014380931854248047,0.027582182442197966
72,216,0,216,0.01467275619506836,0.027365460541195104
73,219,0,219,0.015024900436401367,0.026999884329266047
74,222,0,222,0.015323877334594727,0.026875269811637733
75,225,0,225,0.015572786331176758,0.02651685309121984
76,228,0,228,0.01587390899658203,0.026470414185559076
77,231,0,231,0.01612377166748047,0.026360742102943854
78,234,0,234,0.016350746154785156,0.026244187492183445
79,237,0,237,0.01658487319946289,0.026121495829515253
80,240,0,240,0.016846656799316406,0.025994641139469706
81,243,0,243,0.01705479621887207,0.025908517075605056
82,246,0,246,0.01729893684387207,0.02576842755569217
83,249,0,249,0.017566919326782227,0.02568897002911488
84,252,0,252,0.017799854278564453,0.025623729099066735
85,255,0,255,0.018080949783325195,0.02552512846908838
86,258,0,258,0.018329858779907227,0.02547191685520478
87,261,0,261,0.01857471466064453,0.02539583515993751
88,264,0,264,0.0188448429107666,0.025350745998375945
89,267,0,267,0.019109725952148438,0.02531401893787343
90,270,0,270,0.0193789005279541,0.02527071651148829
91,273,0,273,0.019634723663330078,0.02524653702302687
92,276,0,276,0.01989603042602539,0.025199319935038805
93,279,0,279,0.020168781280517578,0.025167956914690322
94,282,0,282,0.020352840423583984,0.025142579981223264
95,285,0,285,0.02053976058959961,0.025109724767337395
96,288,0,288,0.0207517147064209,0.02509339592799098
97,291,0,291,0.02097773551940918,0.02506313274605519
98,294,0,294,0.021202802658081055,0.02504550253989337
99,297,0,297,0.021475791931152344,0.02502619918533511
100,300,0,300,0.021773815155029297,0.025008700904128628
101,303,0,303,0.02205681800842285,0.02499743137542306
102,306,0,306,0.022331714630126953,0.024979830689869767
103,309,0,309,0.022522687911987305,0.024969347318028086
104,312,0,312,0.022687911987304688,0.024960112055285425
105,315,0,315,0.02285003662109375,0.02494485709556043
106,318,0,318,0.023027896881103516,0.024933025736361383
107,321,0,321,0.023183822631835938,0.02489592842932073
108,324,0,324,0.023332834243774414,0.024876833025867216
109,327,0,327,0.023544788360595703,0.024862942514154333
110,330,0,330,0.023741722106933594,0.024833628713941337
111,333,0,333,0.023900747299194336,0.02481918117060225
112,336,0,336,0.024052858352661133,0.024800712003671364
113,339,0,339,0.024202823638916016,0.024778211620546255
114,342,0,342,0.024351835250854492,0.024756598904035657
115,345,0,345,0.024600744247436523,0.024722231069264546
116,348,0,348,0.024831771850585938,0.024694408228548608
117,351,0,351,0.025046825408935547,0.02464485777893637
118,354,0,354,0.025275707244873047,0.02462057959579985
119,357,0,357,0.025587797164916992,0.024598353745055444
120,360,0,360,0.0259246826171875,0.02456564580794844
121,363,0,363,0.026190757751464844,0.02454337772448629
122,366,0,366,0.026451826095581055,0.02448364255675555
123,369,0,369,0.026636838912963867,0.024445545047394594
124,372,0,372,0.026788711547851562,0.02441136755208178
125,375,0,375,0.026993751525878906,0.024379208753718462
126,378,0,378,0.027238845825195312,0.02435155746117089
127,381,0,381,0.027431726455688477,0.024269452386885285
128,384,0,384,0.02761983871459961,0.024225779150827846
129,387,0,387,0.027853727340698242,0.024171448071513762
130,390,0,390,0.028070688247680664,0.02412558360837189
131,393,0,393,0.028354883193969727,0.02403859719677517
132,396,0,396,0.02864670753479004,0.023963481215398104
133,399,0,399,0.028973817825317383,0.02390520584736328
134,402,0,402,0.029249906539916992,0.023855284050183445
135,405,0,405,0.029558897018432617,0.023801333458419206
136,408,0,408,0.029803991317749023,0.023721885410648805
137,411,0,411,0.029996871948242188,0.023626620749677776
138,414,0,414,0.030276775360107422,0.023531549734722816
139,417,0,417,0.030566692352294922,0.023434989654914255
140,420,0,420,0.030813932418823242,0.02319479468863174
141,423,0,423,0.031110763549804688,0.02311401381487881
142,426,0,426,0.031357765197753906,0.022772331366697936
143,429,0,429,0.031645774841308594,0.022712343793783427
144,432,0,432,0.03192877769470215,0.02264476412290477
145,435,0,435,0.03216195106506348,0.022509872742809897
146,438,0,438,0.032326698303222656,0.02244423651454695
147,441,0,441,0.03249192237854004,0.02237723158887883
148,444,0,444,0.03263378143310547,0.022087563671959874
149,447,0,447,0.03280186653137207,0.021983527747741344
150,450,0,450,0.03293490409851074,0.02169094413463855
151,453,0,453,0.03308272361755371,0.021609613276818707
152,456,0,456,0.03323078155517578,0.02146679786748275
153,459,0,459,0.03336286544799805,0.021001490377648882
154,462,0,462,0.03354477882385254,0.020908095045159118
155,465,0,465,0.03406476974487305,0.020528279115133156
156,468,0,468,0.03426480293273926,0.020486130849232554
157,471,0,471,0.03447866439819336,0.02042155090350316
158,474,0,474,0.03467082977294922,0.0201608744464448
159,477,0,477,0.03485369682312012,0.020107818604074654
160,480,0,480,0.035042762756347656,0.019734988743270097
161,483,0,483,0.03533172607421875,0.019709618060724594
162,486,0,486,0.03561973571777344,0.01968511498434759
163,489,0,489,0.03590083122253418,0.01957441584645825
164,492,0,492,0.03618192672729492,0.019512764984753517
165,495,0,495,0.03645586967468262,0.01945170709793743
166,498,0,498,0.03673386573791504,0.01932090760125844
167,501,0,501,0.03703761100769043,0.019231223729360012
168,504,0,504,0.03734588623046875,0.019148704962709658
169,507,0,507,0.03764677047729492,0.019064104096234366
170,510,0,510,0.03795289993286133,0.018947355654419067
171,513,0,513,0.03820490837097168,0.018683782126529595
172,516,0,516,0.03849291801452637,0.018633853255029184
173,519,0,519,0.038786888122558594,0.018500292981500934
174,522,0,522,0.03908991813659668,0.01840956108567459
175,525,0,525,0.039381980895996094,0.01831807749253664
176,528,0,528,0.03960871696472168,0.018120711368278378
177,531,0,531,0.039778709411621094,0.017987288192636085
178,534,0,534,0.03991985321044922,0.01724766163208567
179,537,0,537,0.04007387161254883,0.017178592344132645
180,540,0,540,0.040239810943603516,0.017087653069341385
181,543,0,543,0.04038286209106445,0.01658192453500602
182,546,0,546,0.040535926818847656,0.01642643746603651
183,549,0,549,0.04067182540893555,0.016130489687503684
184,552,0,552,0.04082298278808594,0.015871492900802704
185,555,0,555,0.040956735610961914,0.015260409620693116
186,558,0,558,0.041107892990112305,0.014978415942477823
187,561,0,561,0.041240692138671875,0.01285926622354681
188,564,0,564,0.04138970375061035,0.012615529407217888
189,567,0,567,0.041539669036865234,0.012294080654745737
190,570,0,570,0.0416717529296875,0.00980830159442174
191,573,0,573,0.04181981086730957,0.009470333068544053
192,576,0,576,0.04195404052734375,0.008342492936783567
193,579,0,579,0.04210186004638672,0.008111577302213712
194,582,0,582,0.0422358512878418,0.007820397829934165
195,585,0,585,0.04238581657409668,0.007523126185198077
196,588,0,588,0.042517900466918945,0.006522861607147147
197,591,0,591,0.042665958404541016,0.006393684574255771
198,594,0,594,0.0428159236907959,0.006319819591321938
199,597,0,597,0.04296875,0.006175878860235438
200,600,0,600,0.04310488700866699,0.005810035145260915
201,603,0,603,0.04325985908508301,0.0056846156375646
202,606,0,606,0.0433957576751709,0.005314155762290482
203,609,0,609,0.04366278648376465,0.005227953322667981
204,612,0,612,0.04399585723876953,0.00495737030606787
205,615,0,615,0.04418468475341797,0.004880714609683584
206,618,0,618,0.04433083534240723,0.004825520219477261
207,621,0,621,0.04452085494995117,0.004742028457371389
208,624,0,624,0.04477691650390625,0.004281060315970977
209,627,0,627,0.044945716857910156,0.00421815938036587
210,630,0,630,0.045079946517944336,0.004009137687327003
211,633,0,633,0.04522895812988281,0.00393224068662264
212,636,0,636,0.04535984992980957,0.0037817958709922086
213,639,0,639,0.04550766944885254,0.003718051291400541
214,642,0,642,0.0456387996673584,0.0035175276368477047
215,645,0,645,0.045784711837768555,0.0034920211849089663
216,648,0,648,0.04593181610107422,0.0034459467011754463
217,651,0,651,0.046061038970947266,0.0033129918703984165
218,654,0,654,0.046208858489990234,0.0032937703689059974
219,657,0,657,0.046344757080078125,0.003242142200753039
220,660,0,660,0.046489715576171875,0.003191790085506379
221,663,0,663,0.04661989212036133,0.0030819813320071576
222,666,0,666,0.046765804290771484,0.003017237839360968
223,669,0,669,0.04691576957702637,0.0028331694590725326
224,672,0,672,0.04706573486328125,0.0027878431718039156
225,675,0,675,0.047200918197631836,0.0026824037521068446
226,678,0,678,0.04735088348388672,0.0026499719967156385
227,681,0,681,0.0474848747253418,0.002613880657349491
228,684,0,684,0.04763484001159668,0.0025669930096659465
229,687,0,687,0.04776787757873535,0.002300794238216177
230,690,0,690,0.04792976379394531,0.0022657852553129958
231,693,0,693,0.04805779457092285,0.002213156605471406
232,696,0,696,0.0482029914855957,0.0021659428023344538
233,699,0,699,0.04833674430847168,0.0021151149330364467
234,702,0,702,0.048482656478881836,0.0020727449292533176
235,705,0,705,0.04861283302307129,0.0016814590274075107
236,708,0,708,0.0487668514251709,0.0016535384353447452
237,711,0,711,0.04891800880432129,0.0015946222420259626
238,714,0,714,0.04906892776489258,0.001570064889333774
239,717,0,717,0.04920387268066406,0.001539313266893499
240,720,0,720,0.04935765266418457,0.0015150681175784908
241,723,0,723,0.04949378967285156,0.0014198535880699705
242,726,0,726,0.04965400695800781,0.0014051282160094825
243,729,0,729,0.049791812896728516,0.001386285350269362
244,732,0,732,0.04995989799499512,0.0013714491056596465
245,735,0,735,0.05008983612060547,0.0013176168374794334
246,738,0,738,0.050235748291015625,0.0013094627070355995
247,741,0,741,0.050366878509521484,0.0012874609571619908
248,744,0,744,0.05051279067993164,0.0012720728272780934
249,747,0,747,0.05064868927001953,0.0012059537580773707
250,750,0,750,0.05079984664916992,0.00118909085599715
251,753,0,753,0.05094599723815918,0.0011414651456179723
252,756,0,756,0.05108976364135742,0.0011346488821428174
253,759,0,759,0.05123186111450195,0.001124849053485082
254,762,0,762,0.05136990547180176,0.0011069421434018048
255,765,0,765,0.05151486396789551,0.0011017778810861675
256,768,0,768,0.051642656326293945,0.0010767967166861673
257,771,0,771,0.051785945892333984,0.0010676576533637473
258,774,0,774,0.05191183090209961,0.001031416878232423
259,777,0,777,0.05205392837524414,0.001025947388448
260,780,0,780,0.05219459533691406,0.0010177413566925947
261,783,0,783,0.0523226261138916,0.0009863513539062271
262,786,0,786,0.05246472358703613,0.0009791404637128256
263,789,0,789,0.05259275436401367,0.0009448409635365719
264,792,0,792,0.05273580551147461,0.0009354533369074163
265,795,0,795,0.05287981033325195,0.0009217521698288862
266,798,0,798,0.05302882194519043,0.0009144637934911377
267,801,0,801,0.05315876007080078,0.0008949338690277253
268,804,0,804,0.053305625915527344,0.0008881400721893031
269,807,0,807,0.05343985557556152,0.0008729172471181306
270,810,0,810,0.0535888671875,0.0008677979330836488
271,813,0,813,0.053720712661743164,0.0008499564957630037
272,816,0,816,0.053938865661621094,0.0008435297113801884
273,819,0,819,0.05408978462219238,0.0008331392205732868
274,822,0,822,0.05424189567565918,0.0008274421962959793
275,825,0,825,0.05438590049743652,0.0008209591359751657
276,828,0,828,0.054512739181518555,0.0008070259495097694
277,831,0,831,0.05465984344482422,0.0008033616391460187
278,834,0,834,0.05478692054748535,0.0007589962431943003
279,837,0,837,0.054930925369262695,0.0007518021731039839
280,840,0,840,0.055078744888305664,0.0007432753877792076
281,843,0,843,0.0552058219909668,0.0006995545027015209
282,846,0,846,0.055345773696899414,0.0006915972158924699
283,849,0,849,0.05547285079956055,0.000639285381441614
284,852,0,852,0.05561494827270508,0.0006293464430418033
285,855,0,855,0.0557558536529541,0.0006174534798947742
286,858,0,858,0.05588197708129883,0.0005706714966019413
287,861,0,861,0.056024789810180664,0.0005604109870541887
288,864,0,864,0.0561528205871582,0.0005278714466224235
289,867,0,867,0.05629682540893555,0.0005137870832953194
290,870,0,870,0.05642390251159668,0.00048497243692256363
291,873,0,873,0.05656599998474121,0.00047204431095574295
292,876,0,876,0.056691884994506836,0.0004453064868269661
293,879,0,879,0.05689692497253418,0.00043824566400627144
294,882,0,882,0.05707883834838867,0.00042531439248306904
295,885,0,885,0.0572819709777832,0.00041691303118916685
296,888,0,888,0.05746293067932129,0.00039552737023783855
297,891,0,891,0.05766773223876953,0.0003872284250596954
298,894,0,894,0.05785965919494629,0.0003474667961275712
299,897,0,897,0.05805778503417969,0.0003431253165675477
300,900,0,900,0.0582578182220459,0.0003395700213746098
301,903,0,903,0.05842995643615723,0.0003072792491238808
302,906,0,906,0.058573007583618164,0.000300584107224033
303,909,0,909,0.05869793891906738,0.0002575171009324226
304,912,0,912,0.058853864669799805,0.00025081793008133754
305,915,0,915,0.05899691581726074,0.00024403545813014035
306,918,0,918,0.05912375450134277,0.00022506871387435878
307,921,0,921,0.059265851974487305,0.0002196941056966437
308,924,0,924,0.05939292907714844,0.00020609315455761697
309,927,0,927,0.05954790115356445,0.0002010586246740129
310,930,0,930,0.0596768856048584,0.00019566655187200447
311,933,0,933,0.05983996391296387,0.0001913266732059144
312,936,0,936,0.059970855712890625,0.00016404929996082193
313,939,0,939,0.06011795997619629,0.0001604274714068282
314,942,0,942,0.06024980545043945,0.0001566747498462244
315,945,0,945,0.06039595603942871,0.00015447831283416934
316,948,0,948,0.06052684783935547,0.0001497937435299077
317,951,0,951,0.06067490577697754,0.00014855885645727744
318,954,0,954,0.0608220100402832,0.00014709326087815336
319,957,0,957,0.06104874610900879,0.00014286932819367027
320,960,0,960,0.061310768127441406,0.00014165666827397748
321,963,0,963,0.06147193908691406,0.00013456971661870908
322,966,0,966,0.0616297721862793,0.00013383389983709023
323,969,0,969,0.06180286407470703,0.00013280725097085998
324,972,0,972,0.06194281578063965,0.00012770616218214136
325,975,0,975,0.06209874153137207,0.00012669963138275478
326,978,0,978,0.062236785888671875,0.0001234329697282997
327,981,0,981,0.0623927116394043,0.00012272014242462173
328,984,0,984,0.06254792213439941,0.0001220758328618602
329,987,0,987,0.06279778480529785,0.00012038730497875401
330,990,0,990,0.06304669380187988,0.00011968632572121657
331,993,0,993,0.06321573257446289,0.00011569167799041666
332,996,0,996,0.06337666511535645,0.0001147903447260128
333,999,0,999,0.06351685523986816,0.00011278983393982073
334,1002,0,1002,0.06367087364196777,0.00011185659190516713
335,1005,0,1005,0.06382274627685547,0.0001095928875100623
336,1008,0,1008,0.06396985054016113,0.0001086899884084548
337,1011,0,1011,0.0641179084777832,0.00010759139035194271
338,1014,0,1014,0.06424880027770996,0.0001059486896543179
339,1017,0,1017,0.06439590454101562,0.00010547049265231637
340,1020,0,1020,0.06452679634094238,0.00010160053553013474
341,1023,0,1023,0.06467294692993164,0.00010122886390418326
342,1026,0,1026,0.06483983993530273,0.00010077206785352264
343,1029,0,1029,0.06497788429260254,9.843727255104451e-05
344,1032,0,1032,0.06513285636901855,9.807401137858096e-05
345,1035,0,1035,0.06528782844543457,9.728579529997675e-05
346,1038,0,1038,0.06544375419616699,9.667447886302493e-05
347,1041,0,1041,0.06559896469116211,9.621789321905942e-05
348,1044,0,1044,0.06575274467468262,9.547702170145573e-05
349,1047,0,1047,0.06588983535766602,9.42229748603225e-05
350,1050,0,1050,0.06604385375976562,9.373841731654527e-05
351,1053,0,1053,0.06617975234985352,9.160160183868812e-05
352,1056,0,1056,0.06633782386779785,9.104659699008747e-05
353,1059,0,1059,0.06648087501525879,8.992154767496919e-05
354,1062,0,1062,0.06663703918457031,8.956575902807867e-05
355,1065,0,1065,0.06679296493530273,8.869649603895982e-05
356,1068,0,1068,0.06694293022155762,8.661050952286758e-05
357,1071,0,1071,0.0670928955078125,8.589312651636487e-05
358,1074,0,1074,0.06722784042358398,8.216314752533503e-05
359,1077,0,1077,0.06737875938415527,8.189156419341004e-05
360,1080,0,1080,0.06752991676330566,8.160004581014755e-05
361,1083,0,1083,0.06766581535339355,8.067967271488616e-05
362,1086,0,1086,0.06781578063964844,8.030486675593076e-05
363,1089,0,1089,0.06795167922973633,7.827134643823529e-05
364,1092,0,1092,0.06811690330505371,7.758385039114661e-05
365,1095,0,1095,0.06826901435852051,7.673438579112539e-05
366,1098,0,1098,0.06842374801635742,7.610438313542045e-05
367,1101,0,1101,0.0685577392578125,7.471877385554925e-05
368,1104,0,1104,0.06870770454406738,7.440774880249201e-05
369,1107,0,1107,0.06887698173522949,7.391835054583229e-05
370,1110,0,1110,0.06902766227722168,7.336485119259712e-05
371,1113,0,1113,0.06917977333068848,7.290087879774918e-05
372,1116,0,1116,0.06940889358520508,7.250364478938032e-05
373,1119,0,1119,0.06962394714355469,7.223320339018048e-05
374,1122,0,1122,0.06978392601013184,7.192654564753478e-05
375,1125,0,1125,0.06993484497070312,7.162501346947555e-05
376,1128,0,1128,0.07008576393127441,7.137727897445824e-05
377,1131,0,1131,0.07023882865905762,7.10433770633115e-05
378,1134,0,1134,0.0703887939453125,7.084896589551831e-05
379,1137,0,1137,0.07053780555725098,7.068621940877905e-05
380,1140,0,1140,0.07068896293640137,7.041205251232957e-05
381,1143,0,1143,0.07094383239746094,7.025836155554443e-05
382,1146,0,1146,0.07114291191101074,7.014350990242335e-05
383,1149,0,1149,0.0713038444519043,6.997613849136086e-05
384,1152,0,1152,0.07146072387695312,6.98244301949826e-05
385,1155,0,1155,0.07161498069763184,6.96510799049161e-05
386,1158,0,1158,0.07177972793579102,6.952163983453937e-05
387,1161,0,1161,0.07193803787231445,6.917176295247409e-05
388,1164,0,1164,0.07218790054321289,6.89773112571187e-05
389,1167,0,1167,0.07242488861083984,6.8716126596669e-05
390,1170,0,1170,0.07258892059326172,6.853500623823032e-05
391,1173,0,1173,0.07274174690246582,6.831200726283425e-05
392,1176,0,1176,0.07289695739746094,6.791414585734335e-05
393,1179,0,1179,0.07306289672851562,6.756546980803424e-05
394,1182,0,1182,0.07322072982788086,6.720508571579812e-05
395,1185,0,1185,0.07336783409118652,6.670755323333968e-05
396,1188,0,1188,0.07351279258728027,6.639467991110165e-05
397,1191,0,1191,0.07364392280578613,6.564174237516975e-05
398,1194,0,1194,0.07378888130187988,6.525826026858754e-05
399,1197,0,1197,0.0739748477935791,6.403090988206332e-05
400,1200,0,1200,0.0741739273071289,6.369173561889391e-05
401,1203,0,1203,0.0743257999420166,6.15932256519277e-05
402,1206,0,1206,0.07448291778564453,6.128638890107456e-05
403,1209,0,1209,0.07465291023254395,6.0825253976273925e-05
404,1212,0,1212,0.07484889030456543,5.9292237205794206e-05
405,1215,0,1215,0.07506394386291504,5.874953465191718e-05
406,1218,0,1218,0.07520890235900879,5.567365911909027e-05
407,1221,0,1221,0.07538771629333496,5.4815247984436516e-05
408,1224,0,1224,0.07555294036865234,5.4328898348170876e-05
409,1227,0,1227,0.07568669319152832,5.10470630786342e-05
410,1230,0,1230,0.0758368968963623,5.0347006122406135e-05
411,1233,0,1233,0.07596778869628906,4.6519341418492666e-05
412,1236,0,1236,0.07612061500549316,4.576589186951897e-05
413,1239,0,1239,0.07631468772888184,4.515597122556252e-05
414,1242,0,1242,0.07652401924133301,4.4551677907721705e-05
415,1245,0,1245,0.0767066478729248,4.1410732874215455e-05
416,1248,0,1248,0.0768887996673584,4.112089080302465e-05
417,1251,0,1251,0.07707381248474121,4.068481893771839e-05
418,1254,0,1254,0.07723069190979004,3.840102557031192e-05
419,1257,0,1257,0.07739067077636719,3.790528000882402e-05
420,1260,0,1260,0.07761669158935547,3.723560951666276e-05
421,1263,0,1263,0.0778360366821289,3.56948583631248e-05
422,1266,0,1266,0.07800793647766113,3.515453620709023e-05
423,1269,0,1269,0.07814884185791016,3.4165376865936226e-05
424,1272,0,1272,0.07829976081848145,3.351475654382436e-05
425,1275,0,1275,0.0784299373626709,3.207576079615928e-05
426,1278,0,1278,0.07857894897460938,3.177238010971965e-05
427,1281,0,1281,0.07870888710021973,3.0751937690503556e-05
428,1284,0,1284,0.07887101173400879,3.0397990917855048e-05
429,1287,0,1287,0.07900285720825195,3.004883336510241e-05
430,1290,0,1290,0.07914900779724121,2.972539806361043e-05
431,1293,0,1293,0.07929682731628418,2.9282115628188988e-05
432,1296,0,1296,0.07943868637084961,2.7898117388653248e-05
433,1299,0,1299,0.07958769798278809,2.772868673290928e-05
434,1302,0,1302,0.07971882820129395,2.7208767515462438e-05
435,1305,0,1305,0.07988572120666504,2.7026514273442193e-05
436,1308,0,1308,0.08002185821533203,2.6422463206677017e-05
437,1311,0,1311,0.08018088340759277,2.6147816952832093e-05
438,1314,0,1314,0.08031082153320312,2.5187036333982238e-05
439,1317,0,1317,0.08045482635498047,2.4869526748718166e-05
440,1320,0,1320,0.08058285713195801,2.444014433066966e-05
441,1323,0,1323,0.08072590827941895,2.414346162278769e-05
442,1326,0,1326,0.08086180686950684,2.361624824956185e-05
443,1329,0,1329,0.08100676536560059,2.3373200852901532e-05
444,1332,0,1332,0.08113360404968262,2.2111989178653473e-05
445,1335,0,1335,0.08127784729003906,2.194241779041908e-05
446,1338,0,1338,0.08140897750854492,2.1349072038954448e-05
447,1341,0,1341,0.08155989646911621,2.1233023906106364e-05
448,1344,0,1344,0.08170390129089355,2.1114064937281177e-05
449,1347,0,1347,0.08185076713562012,2.045979789151093e-05
450,1350,0,1350,0.08199763298034668,2.033084358936828e-05
451,1353,0,1353,0.08214378356933594,2.0172564111693555e-05
452,1356,0,1356,0.08227396011352539,1.9517874421358366e-05
453,1359,0,1359,0.08242297172546387,1.930282601477055e-05
454,1362,0,1362,0.08255481719970703,1.8996838341730067e-05
455,1365,0,1365,0.08270382881164551,1.8775255898445286e-05
456,1368,0,1368,0.08289480209350586,1.856166702202269e-05
457,1371,0,1371,0.08304381370544434,1.811083404069008e-05
458,1374,0,1374,0.08319473266601562,1.797927537144892e-05
459,1377,0,1377,0.08338284492492676,1.626853128396518e-05
460,1380,0,1380,0.08355188369750977,1.611850464443155e-05
461,1383,0,1383,0.08371496200561523,1.594413568685526e-05
462,1386,0,1386,0.08386397361755371,1.5569219398316693e-05
463,1389,0,1389,0.08400988578796387,1.5451966708043837e-05
464,1392,0,1392,0.08415579795837402,1.5227199102525813e-05
465,1395,0,1395,0.08428478240966797,1.4393317707574952e-05
466,1398,0,1398,0.08451676368713379,1.4242580301315615e-05
467,1401,0,1401,0.08466672897338867,1.342622589917708e-05
468,1404,0,1404,0.08481669425964355,1.3269658300043366e-05
469,1407,0,1407,0.08496379852294922,1.307382173803208e-05
470,1410,0,1410,0.08509182929992676,1.2675022264788921e-05
471,1413,0,1413,0.0852348804473877,1.2522530248024128e-05
472,1416,0,1416,0.0853879451751709,1.1606619265456335e-05
473,1419,0,1419,0.08561182022094727,1.1367976960625284e-05
474,1422,0,1422,0.08577680587768555,1.0712545629665873e-05
475,1425,0,1425,0.08604073524475098,1.0492904322987856e-05
476,1428,0,1428,0.0863039493560791,1.0186816051987526e-05
477,1431,0,1431,0.08661293983459473,9.14561411518982e-06
478,1434,0,1434,0.08687090873718262,8.931363627100013e-06
479,1437,0,1437,0.0870199203491211,7.834929769162489e-06
480,1440,0,1440,0.08717775344848633,7.651453641774849e-06
481,1443,0,1443,0.08738183975219727,7.554698559339343e-06
482,1446,0,1446,0.08761382102966309,7.36770521536352e-06
483,1449,0,1449,0.08782100677490234,6.524403515171131e-06
484,1452,0,1452,0.08804774284362793,6.181383878148966e-06
485,1455,0,1455,0.08822774887084961,5.739086577947242e-06
486,1458,0,1458,0.08848690986633301,5.402262146507937e-06
487,1461,0,1461,0.08873701095581055,4.6947886720868614e-06
488,1464,0,1464,0.0889887809753418,4.5825993433017375e-06
489,1467,0,1467,0.08921480178833008,4.439623008513073e-06
490,1470,0,1470,0.08942794799804688,3.806168433469163e-06
491,1473,0,1473,0.08958578109741211,3.7284819089939114e-06
492,1476,0,1476,0.08972001075744629,3.159689566021068e-06
493,1479,0,1479,0.08986783027648926,3.069908377396534e-06
494,1482,0,1482,0.09000182151794434,2.917586661096243e-06
495,1485,0,1485,0.0901486873626709,2.802853935387038e-06
496,1488,0,1488,0.09027886390686035,2.5657316280525857e-06
497,1491,0,1491,0.09042477607727051,2.4673972535084205e-06
498,1494,0,1494,0.09055471420288086,2.094585416533554e-06
499,1497,0,1497,0.09071779251098633,2.040368148337467e-06
500,1500,0,1500,0.09086275100708008,1.9284614718828594e-06
501,1503,0,1503,0.09101486206054688,1.8794512430434498e-06
502,1506,0,1506,0.09114289283752441,1.6977439710077461e-06
503,1509,0,1509,0.09128379821777344,1.6583927959933698e-06
504,1512,0,1512,0.09141182899475098,1.5457786920622314e-06
505,1515,0,1515,0.09160804748535156,1.5205137735416043e-06
506,1518,0,1518,0.0917518138885498,1.4503958590752955e-06
507,1521,0,1521,0.09190487861633301,1.4151174311461734e-06
508,1524,0,1524,0.09203672409057617,1.37513262040684e-06
509,1527,0,1527,0.09218192100524902,1.3463273878563129e-06
510,1530,0,1530,0.09230995178222656,1.3299766936121285e-06
511,1533,0,1533,0.09246277809143066,1.2975600745590893e-06
512,1536,0,1536,0.09270977973937988,1.1637499006173614e-06
513,1539,0,1539,0.09302496910095215,1.148188862284089e-06
514,1542,0,1542,0.0932307243347168,1.1053471339642678e-06
515,1545,0,1545,0.09339165687561035,1.0772063860096396e-06
516,1548,0,1548,0.09351682662963867,1.0115135269803897e-06
517,1551,0,1551,0.09365487098693848,9.988694818432688e-07
518,1554,0,1554,0.09379291534423828,9.62959616245612e-07
519,1557,0,1557,0.09393477439880371,9.43366138638627e-07
520,1560,0,1560,0.09406089782714844,9.161775885120763e-07
521,1563,0,1563,0.09421777725219727,8.912388964219993e-07
522,1566,0,1566,0.0943758487701416,7.868098217937459e-07
523,1569,0,1569,0.09454774856567383,7.764028601154955e-07
524,1572,0,1572,0.0946817398071289,7.527224272183519e-07
525,1575,0,1575,0.09483790397644043,7.459199704693513e-07
526,1578,0,1578,0.09497380256652832,7.371183647125435e-07
527,1581,0,1581,0.09509396553039551,7.120126241688933e-07
528,1584,0,1584,0.0952298641204834,7.072802317755289e-07
529,1587,0,1587,0.09535098075866699,6.727409395472214e-07
530,1590,0,1590,0.09548592567443848,6.69354465878351e-07
531,1593,0,1593,0.09562063217163086,6.647110593051294e-07
532,1596,0,1596,0.09574174880981445,6.395087707003424e-07
533,1599,0,1599,0.09587788581848145,6.370976233427261e-07
534,1602,0,1602,0.09601378440856934,6.345217897584548e-07
535,1605,0,1605,0.09616875648498535,6.287189751207414e-07
536,1608,0,1608,0.09634995460510254,6.249494527280013e-07
537,1611,0,1611,0.09655594825744629,6.117564929022549e-07
538,1614,0,1614,0.09673595428466797,6.095671525092233e-07
539,1617,0,1617,0.09688973426818848,6.062881176093586e-07
540,1620,0,1620,0.09701871871948242,5.992419141665362e-07
541,1623,0,1623,0.09715986251831055,5.962333840440355e-07
542,1626,0,1626,0.09728479385375977,5.775718897466629e-07
543,1629,0,1629,0.09742379188537598,5.755468615319765e-07
544,1632,0,1632,0.09756278991699219,5.733927999779027e-07
545,1635,0,1635,0.0976870059967041,5.550973068473121e-07
546,1638,0,1638,0.0978248119354248,5.507753083708254e-07
547,1641,0,1641,0.09794878959655762,5.405583209800216e-07
548,1644,0,1644,0.09816288948059082,5.346336065533684e-07
549,1647,0,1647,0.09835386276245117,5.297617177245401e-07
550,1650,0,1650,0.09848284721374512,5.118559539134085e-07
551,1653,0,1653,0.09862494468688965,5.087226614596659e-07
552,1656,0,1656,0.09874773025512695,4.999938482010047e-07
553,1659,0,1659,0.09888672828674316,4.976331547783683e-07
554,1662,0,1662,0.09902477264404297,4.932193807548246e-07
555,1665,0,1665,0.09914684295654297,4.823914814324542e-07
556,1668,0,1668,0.09928488731384277,4.808318074016248e-07
557,1671,0,1671,0.09942173957824707,4.773642281911023e-07
558,1674,0,1674,0.09954285621643066,4.6881240799704113e-07
559,1677,0,1677,0.09967875480651855,4.6596930069034576e-07
560,1680,0,1680,0.09981274604797363,4.5341056606732077e-07
561,1683,0,1683,0.0999448299407959,4.502073290879528e-07
562,1686,0,1686,0.10006284713745117,4.370663724347469e-07
563,1689,0,1689,0.10020089149475098,4.3551440784249196e-07
564,1692,0,1692,0.10033369064331055,4.3288751274983807e-07
565,1695,0,1695,0.10045075416564941,4.2109274562698557e-07
566,1698,0,1698,0.10058188438415527,4.1901605616280465e-07
567,1701,0,1701,0.10069990158081055,4.10878203481897e-07
568,1704,0,1704,0.10083198547363281,4.080551462272771e-07
569,1707,0,1707,0.10094881057739258,3.998122663564874e-07
570,1710,0,1710,0.10107994079589844,3.985732627700979e-07
571,1713,0,1713,0.10121273994445801,3.9648803673841505e-07
572,1716,0,1716,0.10134482383728027,3.936031519605167e-07
573,1719,0,1719,0.10147976875305176,3.911195518548871e-07
574,1722,0,1722,0.10159897804260254,3.8710145389036424e-07
575,1725,0,1725,0.1017305850982666,3.847195617924348e-07
576,1728,0,1728,0.10184788703918457,3.804196061764433e-07
577,1731,0,1731,0.10197973251342773,3.7870333395595645e-07
578,1734,0,1734,0.1021108627319336,3.7566777329707933e-07
579,1737,0,1737,0.10224199295043945,3.7344851780720145e-07
580,1740,0,1740,0.10237383842468262,3.717511672378546e-07
581,1743,0,1743,0.10250473022460938,3.7053038761563366e-07
582,1746,0,1746,0.10263586044311523,3.691277207811244e-07
583,1749,0,1749,0.10276675224304199,3.680545149030595e-07
584,1752,0,1752,0.10289788246154785,3.6710919170153814e-07
585,1755,0,1755,0.10302877426147461,3.6617085019614855e-07
586,1758,0,1758,0.10315990447998047,3.6535345036881556e-07
587,1761,0,1761,0.10329174995422363,3.6458879307874603e-07
588,1764,0,1764,0.10342884063720703,3.639697924109797e-07
589,1767,0,1767,0.10355973243713379,3.6335529749376873e-07
590,1770,0,1770,0.10369181632995605,3.628338707252441e-07
591,1773,0,1773,0.10384082794189453,3.621974147113112e-07
592,1776,0,1776,0.1039738655090332,3.6168051143107475e-07
593,1779,0,1779,0.10411477088928223,3.6106069567939905e-07
594,1782,0,1782,0.1042487621307373,3.604130930384319e-07
595,1785,0,1785,0.10438394546508789,3.599205135479242e-07
596,1788,0,1788,0.10451984405517578,3.5947221778009344e-07
597,1791,0,1791,0.10465574264526367,3.58852511113013e-07
598,1794,0,1794,0.10479187965393066,3.5806398566110384e-07
599,1797,0,1797,0.10492587089538574,3.575051241126019e-07
600,1800,0,1800,0.10506081581115723,3.5722583798548203e-07
601,1803,0,1803,0.1051948070526123,3.5678501813579996e-07
602,1806,0,1806,0.10532975196838379,3.565353028085719e-07
603,1809,0,1809,0.10546469688415527,3.5617076987708195e-07
604,1812,0,1812,0.10559892654418945,3.5591115346380513e-07
605,1815,0,1815,0.10573387145996094,3.5565719934757034e-07
606,1818,0,1818,0.10587382316589355,3.552912953769603e-07
607,1821,0,1821,0.1060798168182373,3.550112437877619e-07
608,1824,0,1824,0.10631179809570312,3.54309201938633e-07
609,1827,0,1827,0.10646581649780273,3.538620407879445e-07
610,1830,0,1830,0.10661768913269043,3.534956566722419e-07
611,1833,0,1833,0.10675978660583496,3.5314464781925733e-07
612,1836,0,1836,0.10689783096313477,3.528386042168315e-07
613,1839,0,1839,0.10703682899475098,3.5249521393397036e-07
614,1842,0,1842,0.10717988014221191,3.520915693931212e-07
615,1845,0,1845,0.10737371444702148,3.5161664306977637e-07
616,1848,0,1848,0.10757184028625488,3.512677710791511e-07
617,1851,0,1851,0.1077268123626709,3.50736487453488e-07
618,1854,0,1854,0.10786986351013184,3.501989341285289e-07
619,1857,0,1857,0.10801482200622559,3.498175503787707e-07
620,1860,0,1860,0.1081547737121582,3.489562444774406e-07
621,1863,0,1863,0.10829782485961914,3.485949202892878e-07
622,1866,0,1866,0.10843491554260254,3.482758561374849e-07
623,1869,0,1869,0.10858273506164551,3.4739339926608607e-07
624,1872,0,1872,0.10872864723205566,3.468054258550146e-07
625,1875,0,1875,0.1089017391204834,3.4594826264300356e-07
626,1878,0,1878,0.10905981063842773,3.453843051849452e-07
627,1881,0,1881,0.10920071601867676,3.4455232662481837e-07
628,1884,0,1884,0.10935068130493164,3.434469228611645e-07
629,1887,0,1887,0.10949087142944336,3.428467798103976e-07
630,1890,0,1890,0.10963296890258789,3.424012587525449e-07
631,1893,0,1893,0.1097719669342041,3.416050120309271e-07
632,1896,0,1896,0.10995292663574219,3.4079249122010236e-07
633,1899,0,1899,0.11013078689575195,3.395860418398772e-07
634,1902,0,1902,0.11032795906066895,3.3808281663508293e-07
635,1905,0,1905,0.11049485206604004,3.363402987495184e-07
636,1908,0,1908,0.11064481735229492,3.346744716195333e-07
637,1911,0,1911,0.11080598831176758,3.3369796675265046e-07
638,1914,0,1914,0.11095380783081055,3.320856895266527e-07
639,1917,0,1917,0.11110591888427734,3.2993971769444884e-07
640,1920,0,1920,0.1112508773803711,3.278659465307237e-07
641,1923,0,1923,0.11139392852783203,3.259772005102182e-07
642,1926,0,1926,0.11152267456054688,3.1852771007451776e-07
643,1929,0,1929,0.1116647720336914,3.170717265116377e-07
644,1932,0,1932,0.11179280281066895,3.1147138793982474e-07
645,1935,0,1935,0.11193490028381348,3.1014188903363787e-07
646,1938,0,1938,0.11207699775695801,3.06858338663146e-07
647,1941,0,1941,0.11220502853393555,2.998671542570708e-07
648,1944,0,1944,0.11234664916992188,2.9744208365489976e-07
649,1947,0,1947,0.11247467994689941,2.822977740769389e-07
650,1950,0,1950,0.11261677742004395,2.7773377380715184e-07
651,1953,0,1953,0.11274886131286621,2.665078220374557e-07
652,1956,0,1956,0.11289167404174805,2.651994417467385e-07
653,1959,0,1959,0.11303496360778809,2.639003743745568e-07
654,1962,0,1962,0.11316490173339844,2.461755344851478e-07
655,1965,0,1965,0.11339378356933594,2.4441199347036585e-07
656,1968,0,1968,0.11359882354736328,2.4215134016445174e-07
657,1971,0,1971,0.11385273933410645,2.2768804353247158e-07
658,1974,0,1974,0.11413764953613281,2.2521770126313465e-07
659,1977,0,1977,0.1143789291381836,2.0581088087293752e-07
660,1980,0,1980,0.11464881896972656,2.035202900868252e-07
661,1983,0,1983,0.11489295959472656,2.0039925091649163e-07
662,1986,0,1986,0.11516284942626953,1.9729333461249382e-07
663,1989,0,1989,0.1154029369354248,1.933111267422245e-07
664,1992,0,1992,0.11567187309265137,1.9039829344158272e-07
665,1995,0,1995,0.11591863632202148,1.8221537926095094e-07
666,1998,0,1998,0.11618399620056152,1.7991522886351323e-07
667,2001,0,2001,0.11642074584960938,1.6605509373021681e-07
668,2004,0,2004,0.11670970916748047,1.6478759257028604e-07
669,2007,0,2007,0.11700582504272461,1.6337143417746603e-07
670,2010,0,2010,0.11716198921203613,1.523640388709641e-07
671,2013,0,2013,0.11730790138244629,1.5026847584813383e-07
672,2016,0,2016,0.11743283271789551,1.428580913671395e-07
673,2019,0,2019,0.11758279800415039,1.4149474663369464e-07
674,2022,0,2022,0.1177067756652832,1.3503614227065848e-07
675,2025,0,2025,0.11786484718322754,1.3358784308633728e-07
676,2028,0,2028,0.11798977851867676,1.3148952239339154e-07
677,2031,0,2031,0.11814761161804199,1.3007140277137118e-07
678,2034,0,2034,0.11832070350646973,1.2345777202456804e-07
679,2037,0,2037,0.11847686767578125,1.220117482543573e-07
680,2040,0,2040,0.11860299110412598,1.1600674692714107e-07
681,2043,0,2043,0.1187446117401123,1.147765996576606e-07
682,2046,0,2046,0.1189570426940918,1.1359713395512595e-07
683,2049,0,2049,0.11908888816833496,1.0731992732446228e-07
684,2052,0,2052,0.11923384666442871,1.0571605656862714e-07
685,2055,0,2055,0.11936187744140625,9.94106618441621e-08
686,2058,0,2058,0.11957287788391113,9.791719497423925e-08
687,2061,0,2061,0.11978960037231445,9.575626903665146e-08
688,2064,0,2064,0.11993694305419922,8.762831647782296e-08
689,2067,0,2067,0.1200859546661377,8.572412804500914e-08
690,2070,0,2070,0.12022280693054199,7.874845806452541e-08
691,2073,0,2073,0.12041282653808594,7.714518460172219e-08
692,2076,0,2076,0.1205596923828125,7.561007770840277e-08
693,2079,0,2079,0.12068986892700195,7.312721181344534e-08
694,2082,0,2082,0.1208498477935791,7.191709356465061e-08
695,2085,0,2085,0.12098288536071777,6.595121038450772e-08
696,2088,0,2088,0.12121796607971191,6.475916071721377e-08
697,2091,0,2091,0.12143373489379883,6.400502639990662e-08
698,2094,0,2094,0.12164974212646484,6.295565314871677e-08
699,2097,0,2097,0.12184381484985352,5.665528466744856e-08
700,2100,0,2100,0.12211489677429199,5.509556593940298e-08
701,2103,0,2103,0.12226986885070801,5.3957487530400283e-08
702,2106,0,2106,0.12242388725280762,5.182691281303634e-08
703,2109,0,2109,0.12255978584289551,4.512467574306617e-08
704,2112,0,2112,0.12270879745483398,4.415711437073289e-08
705,2115,0,2115,0.12284183502197266,3.4182203812323916e-08
706,2118,0,2118,0.12302374839782715,3.367333295056017e-08
707,2121,0,2121,0.12317681312561035,3.28973178872227e-08
708,2124,0,2124,0.12330961227416992,2.954957457385666e-08
709,2127,0,2127,0.12345695495605469,2.9212518986927172e-08
710,2130,0,2130,0.12359762191772461,2.834973882699673e-08
711,2133,0,2133,0.123748779296875,2.773125908791693e-08
712,2136,0,2136,0.12387871742248535,2.6167029745360934e-08
713,2139,0,2139,0.12402582168579102,2.565801174061523e-08
714,2142,0,2142,0.1241767406463623,2.3717443650515254e-08
715,2145,0,2145,0.1243288516998291,2.31764771383782e-08
716,2148,0,2148,0.12446379661560059,2.240562217821725e-08
717,2151,0,2151,0.12461090087890625,2.204242633436258e-08
718,2154,0,2154,0.12475371360778809,1.937924767140861e-08
719,2157,0,2157,0.12489581108093262,1.8675974756390423e-08
720,2160,0,2160,0.12504172325134277,1.5740205735919886e-08
721,2163,0,2163,0.12526178359985352,1.535814224122831e-08
722,2166,0,2166,0.12546181678771973,1.495106959692597e-08
723,2169,0,2169,0.12559890747070312,1.2623855871938907e-08
724,2172,0,2172,0.12574267387390137,1.2170515745117986e-08
725,2175,0,2175,0.1258690357208252,1.0640144202866676e-08
726,2178,0,2178,0.12601065635681152,1.0240679628359536e-08
727,2181,0,2181,0.12613773345947266,9.137954353095484e-09


==> plot_data/quadratic_minimax_problem_n20_alpha00001/flex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.818771362304688e-05,4.387072431292609
1,5,0,5,0.0002732276916503906,4.250665939961823
2,10,0,10,0.0007889270782470703,3.8531382361531192
3,13,0,13,0.0011310577392578125,3.47643061415719
5,20,0,20,0.0019021034240722656,3.303295368639145
6,23,0,23,0.002228975296020508,3.229183586814669
7,26,0,26,0.0025479793548583984,2.927464202635655
8,29,0,29,0.002830982208251953,2.6576504050804624
9,32,0,32,0.003061056137084961,2.364109650726281
10,35,0,35,0.003345966339111328,1.5731827434057166
12,43,0,43,0.004054069519042969,1.4851406117614359
13,46,0,46,0.0043070316314697266,1.428959389206125
14,49,0,49,0.004554033279418945,1.3589248416048003
15,54,0,54,0.004807949066162109,1.2499892853674732
16,58,0,58,0.005051136016845703,1.1607886801500642
17,61,0,61,0.005255937576293945,1.1284557623947926
19,69,0,69,0.005774974822998047,1.0301561099391012
20,72,0,72,0.005992889404296875,0.7487005535647958
21,75,0,75,0.00622105598449707,0.7018803739227168
22,79,0,79,0.006585121154785156,0.6697371491413624
23,83,0,83,0.0069730281829833984,0.6252878423563586
24,86,0,86,0.007313251495361328,0.6040251507432601
25,89,0,89,0.007692098617553711,0.5592892115894429
27,95,0,95,0.008296012878417969,0.365015227053497
28,98,0,98,0.008512020111083984,0.27298158946372514
29,102,0,102,0.008755922317504883,0.26656227211663147
30,105,0,105,0.009026050567626953,0.24993191675182944
31,108,0,108,0.009240150451660156,0.24120720947685145
32,113,0,113,0.009492874145507812,0.23541017893173885
34,123,0,123,0.010002851486206055,0.22537494815742176
35,127,0,127,0.010236263275146484,0.22465340135002562
36,130,0,130,0.010438203811645508,0.2091375961535187
37,133,0,133,0.010641098022460938,0.14542651799264927
38,136,0,136,0.010843038558959961,0.13398403246028887
39,139,0,139,0.011039018630981445,0.13241043565502375
41,147,0,147,0.011505126953125,0.1220773126629361
42,151,0,151,0.01174020767211914,0.11559801522273995
43,154,0,154,0.01193690299987793,0.1019014160647584
44,157,0,157,0.012137889862060547,0.07236278696703202
45,160,0,160,0.01234889030456543,0.07143379541046774
46,164,0,164,0.01258397102355957,0.06941271774350248
47,168,0,168,0.012814044952392578,0.06828718231893252
49,178,0,178,0.01330709457397461,0.06677519825094716
50,183,0,183,0.013651847839355469,0.0661129047530508
51,188,0,188,0.014024019241333008,0.0655016460072836
52,193,0,193,0.014380931854248047,0.06493493450102986
53,197,0,197,0.014760971069335938,0.06349321020457878
54,200,0,200,0.015105962753295898,0.062392854417577526
56,206,0,206,0.015709877014160156,0.0557655321048715
57,209,0,209,0.015924930572509766,0.04937189799031506
58,212,0,212,0.01618194580078125,0.04770875610292767
59,216,0,216,0.016434192657470703,0.04753906751117976
60,221,0,221,0.01669025421142578,0.04695533390285294
61,225,0,225,0.016926050186157227,0.046636016804207904
62,230,0,230,0.017184019088745117,0.046210704014629275
64,240,0,240,0.017701148986816406,0.04542971184825339
65,245,0,245,0.017962932586669922,0.04506946037837129
66,250,0,250,0.018208980560302734,0.04472686424337767
67,254,0,254,0.018438100814819336,0.04470650252601006
68,258,0,258,0.01867222785949707,0.04449460159880891
69,261,0,261,0.01888108253479004,0.04408033772652264
71,267,0,267,0.0193021297454834,0.04117708832178915
72,270,0,270,0.01953411102294922,0.04089658842006494
73,275,0,275,0.01978325843811035,0.040289832328292266
74,280,0,280,0.020035982131958008,0.03972420278007966
75,285,0,285,0.020284175872802734,0.03919518381707911
76,290,0,290,0.020551204681396484,0.03869899501335227
78,300,0,300,0.021052122116088867,0.03779271042148884
79,305,0,305,0.021296024322509766,0.03737754047354443
80,310,0,310,0.021543264389038086,0.03698491596460901
81,315,0,315,0.02178502082824707,0.03661307962263415
82,320,0,320,0.02203202247619629,0.03626045812199019
83,325,0,325,0.022274017333984375,0.03592564810276821
84,329,0,329,0.022526025772094727,0.03365705210890599
86,337,0,337,0.02300119400024414,0.03158284254814927
87,342,0,342,0.023250818252563477,0.03140711289388429
88,347,0,347,0.023519039154052734,0.031249232136625883
89,351,0,351,0.023749113082885742,0.031108563700723096
90,356,0,356,0.023996829986572266,0.03097193934655896
91,361,0,361,0.02427220344543457,0.03084599209867091
93,371,0,371,0.024795055389404297,0.03062011301163786
94,376,0,376,0.025041818618774414,0.030517854336800175
95,381,0,381,0.0252840518951416,0.030421490963022442
96,386,0,386,0.02553105354309082,0.030330333207494384
97,391,0,391,0.025784015655517578,0.03024383228820408
98,396,0,396,0.02603912353515625,0.030161525723068718
100,406,0,406,0.026533126831054688,0.030007957271232896
101,411,0,411,0.02678394317626953,0.029936088229964415
102,416,0,416,0.027035236358642578,0.02986717787041467
103,421,0,421,0.02727818489074707,0.02980102277208913
104,426,0,426,0.027551889419555664,0.029737440851220525
105,431,0,431,0.02780890464782715,0.029676272547063415
106,436,0,436,0.02807021141052246,0.02961737705927143
108,446,0,446,0.028603076934814453,0.029505901587797683
109,451,0,451,0.02886819839477539,0.029453097174865103
110,456,0,456,0.02912306785583496,0.02940211498059582
111,461,0,461,0.029373884201049805,0.029352861810133073
112,466,0,466,0.029626131057739258,0.029305249283010548
113,471,0,471,0.029875993728637695,0.02925919705245527
115,481,0,481,0.030379056930541992,0.02917149639750158
116,486,0,486,0.030651092529296875,0.02912972279345215
117,491,0,491,0.030911922454833984,0.029089253290536455
118,496,0,496,0.03117203712463379,0.029050029809728904
119,501,0,501,0.03144693374633789,0.029011998511224046
120,506,0,506,0.03177905082702637,0.02897511009672682
122,516,0,516,0.03234505653381348,0.028904572532985378
123,521,0,521,0.03259015083312988,0.028870829639290545
124,526,0,526,0.032839059829711914,0.028838046323232135
125,531,0,531,0.0330810546875,0.02880618465322838
126,536,0,536,0.03332805633544922,0.0287752086963322
127,541,0,541,0.0335841178894043,0.028745083381145915
128,546,0,546,0.03382396697998047,0.028715775988208878
130,556,0,556,0.034307003021240234,0.02865950097045366
131,561,0,561,0.03454422950744629,0.028632480394039758
132,566,0,566,0.03477907180786133,0.02860616950840076
133,571,0,571,0.03501415252685547,0.02858054303909503
134,576,0,576,0.0352480411529541,0.02855557660918657
135,581,0,581,0.03548693656921387,0.02853124578637207
137,591,0,591,0.035961151123046875,0.028484391606104525
138,596,0,596,0.036195993423461914,0.02846181981392386
139,601,0,601,0.036431074142456055,0.028439787591688876
140,606,0,606,0.0366671085357666,0.02841827317936027
141,611,0,611,0.03690695762634277,0.028397256052029352
142,616,0,616,0.037145137786865234,0.028376717342738913
143,621,0,621,0.03738117218017578,0.028356639910124177
145,631,0,631,0.03785109519958496,0.028317807029574715
146,636,0,636,0.0380861759185791,0.028299023096484625
147,641,0,641,0.03832387924194336,0.028280643064314083
148,646,0,646,0.038583993911743164,0.028262654145410786
149,651,0,651,0.03882598876953125,0.02824504361895586
150,656,0,656,0.03906702995300293,0.028227798659590984
152,666,0,666,0.03954815864562988,0.028194353834574082
153,671,0,671,0.03979325294494629,0.028178128254798915
154,676,0,676,0.040038108825683594,0.02816221690358547
155,681,0,681,0.040281057357788086,0.028146607319005118
156,686,0,686,0.040521860122680664,0.028131287509833524
157,691,0,691,0.04077410697937012,0.028116246071497653
159,701,0,701,0.04126095771789551,0.028086955513063016
160,706,0,706,0.04150509834289551,0.028072686432879777
161,711,0,711,0.04174685478210449,0.02805865589064311
162,716,0,716,0.04198813438415527,0.028044855391187232
163,721,0,721,0.04222893714904785,0.02803127683849535
164,726,0,726,0.04248404502868652,0.028017912480312934
165,731,0,731,0.04273509979248047,0.028004754925156573
167,741,0,741,0.04322314262390137,0.027979032271140458
168,746,0,746,0.043467044830322266,0.027966453789198355
169,751,0,751,0.04370999336242676,0.02795405532213324
170,756,0,756,0.04401826858520508,0.02794183079958178
171,761,0,761,0.04427695274353027,0.027929774430559804
172,766,0,766,0.04454183578491211,0.027917880672325705
174,776,0,776,0.04503202438354492,0.027894560095486524
175,781,0,781,0.045287132263183594,0.027883123567913195
176,786,0,786,0.0455479621887207,0.027871830250679176
177,791,0,791,0.045790910720825195,0.027860676033852165
178,796,0,796,0.04604005813598633,0.02784965710183529
179,801,0,801,0.046285152435302734,0.027838769950725376
181,811,0,811,0.04677605628967285,0.02781737847894494
182,816,0,816,0.04702305793762207,0.027806868545313845
183,821,0,821,0.04731321334838867,0.02779647909043671
184,826,0,826,0.04758024215698242,0.02778620778089133
185,831,0,831,0.04782509803771973,0.027776052385029854
186,836,0,836,0.04807305335998535,0.02776601070291916
187,841,0,841,0.04831504821777344,0.027756080505161932
189,851,0,851,0.048835039138793945,0.027736545250110933
190,856,0,856,0.04909014701843262,0.027726935239007374
191,861,0,861,0.04933905601501465,0.027717426748781148
192,866,0,866,0.049616098403930664,0.027708016906913813
193,871,0,871,0.049871206283569336,0.027698702691956296
194,876,0,876,0.050132036209106445,0.027689480954807152
196,886,0,886,0.050653934478759766,0.0276713018132495
197,891,0,891,0.050916194915771484,0.027662337695034084
198,896,0,896,0.051177978515625,0.02765345269953784
199,901,0,901,0.051434993743896484,0.027644643465558585
200,906,0,906,0.051696062088012695,0.02763590668297691
201,911,0,911,0.05195426940917969,0.027627239118761734
203,921,0,921,0.05246996879577637,0.027610099256413233
204,926,0,926,0.05274486541748047,0.027601621101309582
205,931,0,931,0.05300092697143555,0.02759320048524791
206,936,0,936,0.05326199531555176,0.02758483489382619
207,941,0,941,0.05351710319519043,0.027576522007604062
208,946,0,946,0.05377793312072754,0.02756825971484573
209,951,0,951,0.05403590202331543,0.027560046119906218
211,961,0,961,0.054553985595703125,0.027543758549757436
212,966,0,966,0.05481386184692383,0.02753568189395366
213,971,0,971,0.05507516860961914,0.027527648562799066
214,976,0,976,0.055336952209472656,0.02751965773408677
215,981,0,981,0.05560803413391113,0.027511708761430127
216,986,0,986,0.05586099624633789,0.027503801150138726
218,996,0,996,0.056365013122558594,0.02748810862075423
219,1001,0,1001,0.05661320686340332,0.027480323207808084
220,1006,0,1006,0.05686593055725098,0.027472578104598577
221,1011,0,1011,0.05711507797241211,0.02746487312828562
222,1016,0,1016,0.05737018585205078,0.027457208073883802
223,1021,0,1021,0.05762195587158203,0.02744958269289922
224,1026,0,1026,0.05788016319274902,0.02744199667690138
226,1036,0,1036,0.058381080627441406,0.02742694114573877
227,1041,0,1041,0.05864119529724121,0.02741947064051377
228,1046,0,1046,0.058895111083984375,0.027412037522515507
229,1051,0,1051,0.05915999412536621,0.027404641116928058
230,1056,0,1056,0.059411048889160156,0.02739728069413539
231,1061,0,1061,0.059676170349121094,0.027389955484018316
233,1071,0,1071,0.06018400192260742,0.027375407515529155
234,1076,0,1076,0.060437917709350586,0.027368183161841874
235,1081,0,1081,0.06068921089172363,0.02736099086305885
236,1086,0,1086,0.060945987701416016,0.02735382989038313
237,1091,0,1091,0.06119489669799805,0.027346699565006273
238,1096,0,1096,0.0614471435546875,0.027339599265920146
240,1106,0,1106,0.06194496154785156,0.027325486574257117
241,1111,0,1111,0.062194108963012695,0.02731847325022875
242,1116,0,1116,0.06244611740112305,0.027311488081295538
243,1121,0,1121,0.06269311904907227,0.027304530733331035
244,1126,0,1126,0.06294608116149902,0.02729760090953389
245,1131,0,1131,0.06319403648376465,0.02729069834003918
246,1136,0,1136,0.063446044921875,0.02728382277130068
248,1146,0,1146,0.06396007537841797,0.027270151643643003
249,1151,0,1151,0.06420087814331055,0.027263355573363214
250,1156,0,1156,0.06444692611694336,0.027256585467150304
251,1161,0,1161,0.06468915939331055,0.02724984102558396
252,1166,0,1166,0.06493902206420898,0.027243121924920788
253,1171,0,1171,0.06518006324768066,0.02723642781583484
255,1181,0,1181,0.06566596031188965,0.02722311304923823
256,1186,0,1186,0.06591010093688965,0.02721649157223756
257,1191,0,1191,0.06615114212036133,0.027209893453345898
258,1196,0,1196,0.06641197204589844,0.027203318238549486
259,1201,0,1201,0.06664800643920898,0.02719676546324824
260,1206,0,1206,0.06688714027404785,0.02719023465672303
262,1216,0,1216,0.06736397743225098,0.027177237064022242
263,1221,0,1221,0.06761693954467773,0.02717076934684195
264,1226,0,1226,0.06786394119262695,0.027164321744930525
265,1231,0,1231,0.06810593605041504,0.02715789382326552
266,1236,0,1236,0.06835103034973145,0.027151485165241015
267,1240,0,1240,0.06857895851135254,0.02713864562911509
268,1245,0,1245,0.06882500648498535,0.027128156901796537
270,1255,0,1255,0.06931304931640625,0.027108368272108795
271,1260,0,1260,0.06955504417419434,0.027098966999433278
272,1265,0,1265,0.06979990005493164,0.027089840307477672
273,1270,0,1270,0.07004117965698242,0.027080958733873898
274,1274,0,1274,0.07027292251586914,0.027066689222577517
275,1279,0,1279,0.07051491737365723,0.0270540258536676
277,1289,0,1289,0.07100892066955566,0.027030435793330615
278,1294,0,1294,0.07125496864318848,0.0270193647276227
279,1299,0,1299,0.07149600982666016,0.027008695049277744
280,1304,0,1304,0.07174086570739746,0.02699838359847791
281,1309,0,1309,0.07198309898376465,0.026988396861171788
282,1313,0,1313,0.07221508026123047,0.026972757951651057
284,1323,0,1323,0.07271122932434082,0.026946865796205578
285,1328,0,1328,0.07294702529907227,0.02693510731723154
286,1333,0,1333,0.07318592071533203,0.026923965527402626
287,1338,0,1338,0.07342100143432617,0.026913342330954222
288,1343,0,1343,0.07366013526916504,0.026903163529566135
289,1348,0,1348,0.07389402389526367,0.02689336888412069
290,1353,0,1353,0.07413196563720703,0.02688390461791578
292,1363,0,1363,0.07460713386535645,0.026865786082740664
293,1368,0,1368,0.07484102249145508,0.0268570659341876
294,1373,0,1373,0.07507920265197754,0.026848540904552447
295,1378,0,1378,0.07531309127807617,0.026840191541409382
296,1383,0,1383,0.0755620002746582,0.026832000057246976
297,1388,0,1388,0.07579803466796875,0.026823951589555677
299,1398,0,1398,0.07627201080322266,0.02680823593290346
300,1403,0,1403,0.07651090621948242,0.026800546537612387
301,1408,0,1408,0.07674598693847656,0.026792956187190933
302,1413,0,1413,0.07698607444763184,0.026785457306720356
303,1418,0,1418,0.07722115516662598,0.026778043220258476
304,1423,0,1423,0.07746291160583496,0.02677070673028807
305,1428,0,1428,0.0776970386505127,0.026763440322234145
307,1438,0,1438,0.07817220687866211,0.026749094015454705
308,1443,0,1443,0.07841110229492188,0.02674200599750481
309,1448,0,1448,0.07865214347839355,0.026734969991858728
310,1453,0,1453,0.07889103889465332,0.02672798240690942
311,1458,0,1458,0.07912802696228027,0.026721040249395093
312,1463,0,1463,0.07936716079711914,0.026714141264426908
314,1473,0,1473,0.07984304428100586,0.026700464568095352
315,1478,0,1478,0.080078125,0.026693682695876016
316,1483,0,1483,0.08031797409057617,0.02668693631725861
317,1488,0,1488,0.08055591583251953,0.02668022436364728
318,1493,0,1493,0.08080196380615234,0.026673545803223665
319,1498,0,1498,0.08103799819946289,0.026666899519265073
321,1508,0,1508,0.08151698112487793,0.02665369988157136
322,1513,0,1513,0.0817568302154541,0.026647144856875245
323,1518,0,1518,0.08199286460876465,0.026640618471932172
324,1523,0,1523,0.08223199844360352,0.02663411979684516
325,1528,0,1528,0.08246493339538574,0.026627648112621534
326,1533,0,1533,0.08270406723022461,0.026621202871329346
327,1538,0,1538,0.08293819427490234,0.02661478346745678
329,1548,0,1548,0.08341193199157715,0.02660201900324444
330,1553,0,1553,0.08365011215209961,0.026595672346341595
331,1558,0,1558,0.08388495445251465,0.02658934840273673
332,1563,0,1563,0.08412408828735352,0.0265830462830499
333,1568,0,1568,0.08435821533203125,0.026576764950534012
334,1573,0,1573,0.08462309837341309,0.02657050337454721
336,1583,0,1583,0.08512401580810547,0.02655803591486202
337,1588,0,1588,0.0853722095489502,0.026551828360433738
338,1593,0,1593,0.08562397956848145,0.02654563718719905
339,1598,0,1598,0.08587217330932617,0.026539461749769053
340,1603,0,1603,0.08612394332885742,0.02653330157827453
341,1608,0,1608,0.08637309074401855,0.026527156312246874
343,1618,0,1618,0.08687686920166016,0.026514909342716084
344,1623,0,1623,0.08712196350097656,0.02650880727781811
345,1628,0,1628,0.08736515045166016,0.026502719403918684
346,1633,0,1633,0.08761382102966309,0.02649664568719961
347,1638,0,1638,0.08785510063171387,0.026490586066813555
348,1643,0,1643,0.08810114860534668,0.026484540461561658
349,1648,0,1648,0.08834314346313477,0.02647850877387098
351,1658,0,1658,0.08882808685302734,0.02646648647626488
352,1663,0,1663,0.08907318115234375,0.026460495302195037
353,1668,0,1668,0.08932089805603027,0.02645451694071303
354,1673,0,1673,0.08956599235534668,0.026448550952367998
355,1678,0,1678,0.08980822563171387,0.026442596851698835
356,1683,0,1683,0.09005403518676758,0.026436654109777635
358,1693,0,1693,0.09054112434387207,0.026424800539655437
359,1698,0,1698,0.0907890796661377,0.026418888699252928
360,1703,0,1703,0.09103512763977051,0.026412986215335582
361,1708,0,1708,0.09127593040466309,0.026407092691210898
362,1713,0,1713,0.09152102470397949,0.026401207795266828
363,1718,0,1718,0.09176206588745117,0.02639533127470486
365,1728,0,1728,0.09224796295166016,0.026383602715835515
366,1733,0,1733,0.09249520301818848,0.0263777505080281
367,1738,0,1738,0.09273600578308105,0.02637190632839646
368,1743,0,1743,0.09298205375671387,0.026366070224511564
369,1748,0,1748,0.09322381019592285,0.026360242275481987
370,1753,0,1753,0.09346890449523926,0.026354422574467806
371,1758,0,1758,0.09371018409729004,0.026348611218396063
373,1768,0,1768,0.09420204162597656,0.026337013903434205
374,1773,0,1773,0.09444808959960938,0.02633122807799438
375,1778,0,1778,0.09468889236450195,0.02632545084027596
376,1783,0,1783,0.09493398666381836,0.026319682163995984
377,1788,0,1788,0.09517598152160645,0.026313921978977226
378,1793,0,1793,0.09542083740234375,0.02630817016663895
380,1803,0,1803,0.09590816497802734,0.0262966909214558
381,1808,0,1808,0.09614896774291992,0.02629096299180711
382,1813,0,1813,0.09639406204223633,0.026285242450986412
383,1818,0,1818,0.09664726257324219,0.02627952894474493
384,1823,0,1823,0.09688496589660645,0.02627382208615892
385,1828,0,1828,0.09711885452270508,0.026268121465189562
386,1833,0,1833,0.09735798835754395,0.026262426660318822
388,1843,0,1843,0.09783196449279785,0.02625105281898063
389,1848,0,1848,0.09806704521179199,0.026245372974390023
390,1853,0,1853,0.09830498695373535,0.02623969734978556
391,1858,0,1858,0.09854006767272949,0.026234025617461895
392,1863,0,1863,0.09877800941467285,0.026228357493993607
393,1868,0,1868,0.09901213645935059,0.026222692743820022
395,1878,0,1878,0.09949684143066406,0.026211372672307987
396,1883,0,1883,0.09972405433654785,0.026205717130923453
397,1888,0,1888,0.09994697570800781,0.026200064516527257
398,1893,0,1893,0.10017991065979004,0.026194414826849893
399,1898,0,1898,0.10040283203125,0.026188768091440013
400,1903,0,1903,0.10064315795898438,0.026183124364486002
402,1913,0,1913,0.1010899543762207,0.026171846227572303
403,1918,0,1918,0.10130810737609863,0.026166211976460938
404,1923,0,1923,0.10154485702514648,0.026160581037380965
405,1928,0,1928,0.10176801681518555,0.02615495347298897
406,1933,0,1933,0.10199403762817383,0.026149329330112443
407,1938,0,1938,0.1022179126739502,0.026143708636273914
408,1943,0,1943,0.10244393348693848,0.02613809139776438
410,1953,0,1953,0.10289406776428223,0.02612686720403735
411,1958,0,1958,0.10311698913574219,0.0261212601559398
412,1963,0,1963,0.10334205627441406,0.026115656380785262
413,1968,0,1968,0.10357499122619629,0.026110055789610127
414,1973,0,1973,0.10379695892333984,0.02610445828198514
415,1978,0,1978,0.10401415824890137,0.02609886374945291
417,1988,0,1988,0.10446786880493164,0.026087683155565315
418,1993,0,1993,0.10469388961791992,0.02608209686662183
419,1998,0,1998,0.10491585731506348,0.0260765131034056
420,2003,0,2003,0.10514307022094727,0.026070931763792767
421,2008,0,2008,0.10536599159240723,0.02606535275375664
422,2013,0,2013,0.10559296607971191,0.026059775988559356
424,2023,0,2023,0.1060478687286377,0.026048628904361413
425,2028,0,2028,0.10627102851867676,0.026043058466931744
426,2033,0,2033,0.10649800300598145,0.0260374900368265
427,2038,0,2038,0.106719970703125,0.026031923578658207
428,2043,0,2043,0.10694694519042969,0.026026359065225924
429,2048,0,2048,0.10717105865478516,0.026020796476511104
430,2053,0,2053,0.10739707946777344,0.02601523579859369
432,2063,0,2063,0.10787105560302734,0.0260041201438572
433,2068,0,2068,0.10809898376464844,0.025998565160939492
434,2073,0,2073,0.10833001136779785,0.025993012075148023
435,2078,0,2078,0.10855817794799805,0.02598746088995531
436,2083,0,2083,0.10879111289978027,0.0259819116107896
437,2088,0,2088,0.10902023315429688,0.02597636424504959
439,2098,0,2098,0.10949301719665527,0.025965275294812767
440,2103,0,2103,0.10971903800964355,0.02595973373790315
441,2108,0,2108,0.10994195938110352,0.025954194150957066
442,2113,0,2113,0.1101691722869873,0.02594865655816679
443,2118,0,2118,0.11039113998413086,0.02594312098945891
444,2123,0,2123,0.11061811447143555,0.025937587481385718
446,2133,0,2133,0.11107301712036133,0.025926526831473447
447,2138,0,2138,0.11129498481750488,0.025920999802971807
448,2143,0,2143,0.1115260124206543,0.02591547506278954
449,2148,0,2148,0.11174917221069336,0.0259099526906835
450,2153,0,2153,0.11197590827941895,0.025904432775826103
451,2158,0,2158,0.11219906806945801,0.025898915416558185
452,2163,0,2163,0.1124410629272461,0.02589340071990961
454,2173,0,2173,0.11290216445922852,0.025882379781684683
455,2178,0,2178,0.11312985420227051,0.025876873790485626
456,2183,0,2183,0.11336183547973633,0.0258713709604969
457,2188,0,2188,0.11360621452331543,0.02586587142864114
458,2193,0,2193,0.11383295059204102,0.02586037533432002
459,2198,0,2198,0.11405587196350098,0.025854882818171596
461,2208,0,2208,0.11450505256652832,0.025843909082053577
462,2213,0,2213,0.1147298812866211,0.025838428139238027
463,2218,0,2218,0.11495304107666016,0.025832951327026645
464,2223,0,2223,0.11517786979675293,0.02582747877634974
465,2228,0,2228,0.11540102958679199,0.025822010613911654
466,2233,0,2233,0.11562705039978027,0.02581654696178628
467,2238,0,2238,0.11584782600402832,0.02581108793716711
469,2248,0,2248,0.11629796028137207,0.02580018421433632
470,2253,0,2253,0.11652493476867676,0.025794739725837082
471,2258,0,2258,0.11674690246582031,0.025789300284655925
472,2263,0,2263,0.1169731616973877,0.025783865984434752
473,2268,0,2268,0.11719298362731934,0.025778436914939425
474,2273,0,2273,0.11742305755615234,0.025773013162464983
476,2283,0,2283,0.11787009239196777,0.025762181938889534
477,2288,0,2288,0.11809301376342773,0.025756774626700646
478,2293,0,2293,0.11832022666931152,0.025751372950071235
479,2298,0,2298,0.11854100227355957,0.02574597698372741
480,2303,0,2303,0.11876821517944336,0.025740586800934603
481,2308,0,2308,0.1189889907836914,0.025735202473612113
483,2318,0,2318,0.11943697929382324,0.025724451666363876
484,2323,0,2323,0.11966419219970703,0.025719085323266947
485,2328,0,2328,0.11988615989685059,0.025713725108861284
486,2333,0,2333,0.12011218070983887,0.02570837108675788
487,2338,0,2338,0.12033295631408691,0.02570302331795688
488,2343,0,2343,0.1205589771270752,0.02569768186036289
489,2348,0,2348,0.12078595161437988,0.025692346768258358
491,2358,0,2358,0.12123489379882812,0.025681695876256423
492,2363,0,2363,0.1214609146118164,0.025676380161917606
493,2368,0,2368,0.12168288230895996,0.025671070983184992
494,2373,0,2373,0.12191009521484375,0.025665768368372963
495,2378,0,2378,0.1221320629119873,0.025660472339332337
496,2383,0,2383,0.12235808372497559,0.025655182911212306
498,2393,0,2393,0.12280607223510742,0.02564462388413116
499,2398,0,2398,0.12302899360656738,0.025639354281309742
500,2403,0,2403,0.1232609748840332,0.025634091271972272
501,2408,0,2408,0.12348484992980957,0.025628834837951878
502,2413,0,2413,0.12371087074279785,0.025623584955193044
503,2418,0,2418,0.1239328384399414,0.02561834159421661
505,2428,0,2428,0.12438082695007324,0.025607874295766962
506,2433,0,2433,0.12460684776306152,0.02560265027712795
507,2438,0,2438,0.12483000755310059,0.025597432619115665
508,2443,0,2443,0.12505698204040527,0.025592221273529545
509,2448,0,2448,0.12527894973754883,0.0255870161901085
510,2453,0,2453,0.1255648136138916,0.025581817317000842
511,2458,0,2458,0.12578821182250977,0.02557662460115893
513,2468,0,2468,0.1262362003326416,0.025566257424846354
514,2473,0,2473,0.12646198272705078,0.025561082854564765
515,2478,0,2478,0.12672901153564453,0.025555914222027402
516,2483,0,2483,0.12695598602294922,0.02555075147077095
517,2488,0,2488,0.12717795372009277,0.02554559454343456
518,2493,0,2493,0.12740612030029297,0.025540443381462264
520,2503,0,2503,0.1278550624847412,0.025530158111098208
521,2508,0,2508,0.1280839443206787,0.025525023875956353
522,2513,0,2513,0.128309965133667,0.02551989515169556
523,2518,0,2518,0.12853288650512695,0.02551477186721207
524,2523,0,2523,0.12875914573669434,0.02550965394741034
525,2528,0,2528,0.12898612022399902,0.025504541312740367
527,2538,0,2538,0.12943792343139648,0.025494331555896105
528,2543,0,2543,0.12966489791870117,0.025489234248935188
529,2548,0,2548,0.12988901138305664,0.02548414185705282
530,2553,0,2553,0.13011598587036133,0.025479054273586127
531,2558,0,2558,0.13033795356750488,0.025473971386032458
532,2563,0,2563,0.13056612014770508,0.02546889307611477
533,2568,0,2568,0.13084006309509277,0.02546381921993312
535,2578,0,2578,0.1313788890838623,0.0254536843465455
536,2583,0,2583,0.1316061019897461,0.025448623055907896
537,2588,0,2588,0.13182902336120605,0.025443565672963835
538,2593,0,2593,0.13205599784851074,0.02543851205062695
539,2598,0,2598,0.1322779655456543,0.025433462038583817
540,2603,0,2603,0.13250517845153809,0.025428415483865575
542,2613,0,2613,0.13295698165893555,0.025418332124855083
543,2618,0,2618,0.1331801414489746,0.025413295006809288
544,2623,0,2623,0.13348817825317383,0.02540826071983647
545,2628,0,2628,0.13371491432189941,0.025403229106904384
546,2633,0,2633,0.1339859962463379,0.025398200012037787
547,2638,0,2638,0.13421106338500977,0.025393173280922384
548,2643,0,2643,0.13451910018920898,0.02538814876149088
550,2653,0,2653,0.13528704643249512,0.02537810576400121
551,2658,0,2658,0.13565421104431152,0.02537308699798415
552,2663,0,2663,0.13596892356872559,0.025368069868718333
553,2668,0,2668,0.13619399070739746,0.025363054243260862
554,2673,0,2673,0.13642120361328125,0.025358039993844117
555,2678,0,2678,0.13664507865905762,0.02535302699823428
557,2688,0,2688,0.13718080520629883,0.0253430043089913
558,2693,0,2693,0.1374530792236328,0.02533799440111367
559,2698,0,2698,0.13772320747375488,0.025332985318913363
560,2703,0,2703,0.13794612884521484,0.025327976971450377
561,2708,0,2708,0.13834905624389648,0.025322969274369993
562,2713,0,2713,0.13860607147216797,0.02531796214986562
564,2723,0,2723,0.13904905319213867,0.025307949339421706
565,2728,0,2728,0.1392660140991211,0.025302943529369255
566,2733,0,2733,0.13948893547058105,0.025297938043149726
567,2738,0,2738,0.13970708847045898,0.025292932832914033
568,2743,0,2743,0.13992905616760254,0.02528792785584598
569,2748,0,2748,0.14014792442321777,0.025282923073736585
570,2753,0,2753,0.14036989212036133,0.025277918452531224
572,2763,0,2763,0.1408381462097168,0.025267909574563076
573,2768,0,2768,0.14106106758117676,0.02526290526622582
574,2772,0,2772,0.14127421379089355,0.02525124562688441
575,2777,0,2777,0.14149713516235352,0.02524199500606629
576,2782,0,2782,0.14173007011413574,0.025233180877829657
577,2787,0,2787,0.1419529914855957,0.025224733758052956
579,2795,0,2795,0.1423799991607666,0.025161895554419018
580,2799,0,2799,0.1425950527191162,0.0251464981535766
581,2804,0,2804,0.14281916618347168,0.025129269769810093
582,2809,0,2809,0.14304614067077637,0.025112890133950825
583,2813,0,2813,0.14325714111328125,0.02510127337215882
584,2818,0,2818,0.14348483085632324,0.02508463536435819
586,2827,0,2827,0.1439211368560791,0.025029716885337915
587,2832,0,2832,0.14414405822753906,0.025014915295573294
588,2837,0,2837,0.14437007904052734,0.02500067423644542
589,2842,0,2842,0.1445939540863037,0.024986934764756615
590,2847,0,2847,0.144819974899292,0.024973635199284624
591,2852,0,2852,0.14504194259643555,0.02496071517786864
592,2857,0,2857,0.14526891708374023,0.024948130678928856
594,2867,0,2867,0.14581298828125,0.0249238557892673
595,2872,0,2872,0.14603686332702637,0.02491210839454105
596,2877,0,2877,0.14626407623291016,0.024900584577251375
597,2882,0,2882,0.14648795127868652,0.024889268308271935
598,2886,0,2886,0.14670419692993164,0.024851273593198515
599,2891,0,2891,0.146928071975708,0.024827150817976797
601,2901,0,2901,0.14746499061584473,0.02478461869376803
602,2906,0,2906,0.14769887924194336,0.02476553729697829
603,2911,0,2911,0.14792180061340332,0.024747567097105357
604,2916,0,2916,0.1481480598449707,0.024730512970314027
605,2921,0,2921,0.14837098121643066,0.024714224796253098
606,2926,0,2926,0.14859890937805176,0.0246985824380741
608,2936,0,2936,0.1490480899810791,0.024668842433005045
609,2941,0,2941,0.14927101135253906,0.02465460100559103
610,2946,0,2946,0.14949703216552734,0.024640718271425163
611,2951,0,2951,0.1497211456298828,0.024627159166943212
612,2956,0,2956,0.1499481201171875,0.024613887220904372
613,2961,0,2961,0.15017104148864746,0.024600869910798004
614,2966,0,2966,0.15039682388305664,0.024588084606551184
616,2976,0,2976,0.15085315704345703,0.024563144526873342
617,2981,0,2981,0.15107512474060059,0.024550952806038598
618,2986,0,2986,0.15130114555358887,0.024538923121899148
619,2991,0,2991,0.15152406692504883,0.024527045140852324
620,2996,0,2996,0.15175104141235352,0.02451531187674653
621,3001,0,3001,0.15197420120239258,0.024503714563703892
623,3011,0,3011,0.15242314338684082,0.024480886949455587
624,3016,0,3016,0.15264892578125,0.024469641901110433
625,3021,0,3021,0.15287303924560547,0.024458502131682144
626,3026,0,3026,0.15309786796569824,0.024447461202687034
627,3031,0,3031,0.15332603454589844,0.02443651282378287
628,3036,0,3036,0.15355324745178223,0.0244256525714055
629,3041,0,3041,0.1537761688232422,0.02441487737699572
631,3051,0,3051,0.15422606468200684,0.024393568446063163
632,3056,0,3056,0.15445184707641602,0.024383027685131363
633,3061,0,3061,0.15471792221069336,0.024372559340102618
634,3066,0,3066,0.15494489669799805,0.024362161301880746
635,3071,0,3071,0.1551680564880371,0.024351830972839855
636,3076,0,3076,0.1553950309753418,0.024341565526790787
638,3086,0,3086,0.15584397315979004,0.024321220313518622
639,3091,0,3091,0.1560659408569336,0.0243111370659839
640,3096,0,3096,0.15629315376281738,0.024301110959117835
641,3101,0,3101,0.15651607513427734,0.02429114012780775
642,3106,0,3106,0.15674304962158203,0.024281223075674287
643,3111,0,3111,0.15696501731872559,0.02427135863383264
645,3121,0,3121,0.15741300582885742,0.024251782540922816
646,3126,0,3126,0.1576392650604248,0.02424206806000556
647,3131,0,3131,0.15786099433898926,0.02423240096058427
648,3136,0,3136,0.15808796882629395,0.02422278021890103
649,3141,0,3141,0.158311128616333,0.02421320480752115
650,3146,0,3146,0.1585369110107422,0.024203673697320294
651,3151,0,3151,0.15876102447509766,0.02419418599117609
653,3161,0,3161,0.15921401977539062,0.024175337870932272
654,3166,0,3166,0.15944123268127441,0.02416597599983756
655,3171,0,3171,0.15966510772705078,0.024156654574113572
656,3176,0,3176,0.15989089012145996,0.02414737288163996
657,3181,0,3181,0.16011404991149902,0.02413813022935322
658,3186,0,3186,0.1603410243988037,0.024128925873503227
660,3196,0,3196,0.1607952117919922,0.024110628822908337
661,3201,0,3201,0.16101908683776855,0.024101534490104753
662,3206,0,3206,0.16124582290649414,0.024092475163250866
663,3211,0,3211,0.1614689826965332,0.02408344994125024
664,3216,0,3216,0.1616959571838379,0.02407445789483538
665,3221,0,3221,0.16191887855529785,0.02406549810526228
667,3231,0,3231,0.162369966506958,0.02404767172994408
668,3235,0,3235,0.1625840663909912,0.023978969461699133
669,3240,0,3240,0.16280698776245117,0.02394970923825519
670,3245,0,3245,0.16303420066833496,0.02392436267942075
671,3250,0,3250,0.16325616836547852,0.023902085376789
672,3255,0,3255,0.1634831428527832,0.02388221433675906
673,3260,0,3260,0.1637129783630371,0.023864239615249812
675,3269,0,3269,0.164154052734375,0.02382989085985306
676,3274,0,3274,0.1643810272216797,0.02375229002733949
677,3279,0,3279,0.16460490226745605,0.02368866075403447
678,3284,0,3284,0.16483712196350098,0.02363596136569743
679,3289,0,3289,0.16506218910217285,0.02359182901776294
680,3294,0,3294,0.16528892517089844,0.02355444073033394
682,3304,0,3304,0.1657390594482422,0.023494502544826087
683,3309,0,3309,0.16596293449401855,0.0234699505414532
684,3314,0,3314,0.16618895530700684,0.023448065546558802
685,3319,0,3319,0.1664109230041504,0.023428348216534757
686,3323,0,3323,0.16672992706298828,0.023399874570025167
687,3328,0,3328,0.16698122024536133,0.02318628216321106
689,3338,0,3338,0.1674330234527588,0.02287712319307391
690,3343,0,3343,0.1676640510559082,0.022765590316713394
691,3348,0,3348,0.16787505149841309,0.022674893392423925
692,3353,0,3353,0.16808795928955078,0.022600777340888004
693,3358,0,3358,0.16829895973205566,0.022539869653770125
694,3363,0,3363,0.16851305961608887,0.022489441958843233
695,3368,0,3368,0.16872406005859375,0.022447306352746506
697,3378,0,3378,0.16921496391296387,0.022381461824366438
698,3383,0,3383,0.16949701309204102,0.022355430498444476
699,3388,0,3388,0.16984915733337402,0.02233283691428922
700,3392,0,3392,0.17008614540100098,0.022111416439716453
701,3397,0,3397,0.17029714584350586,0.021996012679391858
702,3401,0,3401,0.17049908638000488,0.021914107817700167
704,3411,0,3411,0.17093801498413086,0.021784631766488916
705,3416,0,3416,0.17114710807800293,0.021733562725095516
706,3421,0,3421,0.17136096954345703,0.02168948520640234
707,3426,0,3426,0.1715710163116455,0.02165113028929833
708,3431,0,3431,0.1717832088470459,0.021617477016586294
709,3436,0,3436,0.17199301719665527,0.021587730155990005
710,3441,0,3441,0.17220497131347656,0.02156124844100331
712,3451,0,3451,0.17262697219848633,0.021515996757891558
713,3456,0,3456,0.1728370189666748,0.021496438296489395
714,3461,0,3461,0.173051118850708,0.02147853212992469
715,3466,0,3466,0.17325997352600098,0.021462034757915964
716,3471,0,3471,0.17347192764282227,0.021446720756794883
717,3476,0,3476,0.17368102073669434,0.0214324098897975
719,3486,0,3486,0.17410516738891602,0.021406326447155073
720,3491,0,3491,0.1743171215057373,0.021394360341220636
721,3496,0,3496,0.17452502250671387,0.021382979293379865
722,3501,0,3501,0.17473793029785156,0.02137210720469461
723,3506,0,3506,0.17494702339172363,0.021361694563079965
724,3511,0,3511,0.17516016960144043,0.021351700480896067
726,3521,0,3521,0.17562103271484375,0.02133278093808614
727,3526,0,3526,0.17582988739013672,0.02132377519381118
728,3531,0,3531,0.1760420799255371,0.021315041382329033
729,3536,0,3536,0.1762559413909912,0.021306561199154018
730,3541,0,3541,0.1764678955078125,0.021298309566420075
731,3546,0,3546,0.1766810417175293,0.021290260759375075
732,3551,0,3551,0.176893949508667,0.02128239748189811
734,3561,0,3561,0.17731499671936035,0.021267183239203274
735,3566,0,3566,0.17752504348754883,0.02125980305407909
736,3571,0,3571,0.1777358055114746,0.021252554006268437
737,3576,0,3576,0.17794513702392578,0.021245427585615997
738,3581,0,3581,0.17815709114074707,0.02123841733729386
739,3586,0,3586,0.17836594581604004,0.0212315136089906
741,3596,0,3596,0.17878508567810059,0.021217981809505918
742,3601,0,3601,0.17903804779052734,0.02121134043225785
743,3606,0,3606,0.1792459487915039,0.021204776680179505
744,3611,0,3611,0.1794581413269043,0.02119828455134666
745,3616,0,3616,0.17966699600219727,0.021191857609454235
746,3621,0,3621,0.17987918853759766,0.02118549203685979
748,3631,0,3631,0.1802990436553955,0.021172939086887076
749,3636,0,3636,0.18050813674926758,0.021166746457794323
750,3641,0,3641,0.18072223663330078,0.021160605070020686
751,3646,0,3646,0.18093109130859375,0.021154513127344638
752,3651,0,3651,0.18114399909973145,0.021148469815254187
753,3656,0,3656,0.18135285377502441,0.021142473516247717
754,3661,0,3661,0.18156909942626953,0.021136521608739255
756,3671,0,3671,0.18198919296264648,0.021124742966829365
757,3676,0,3676,0.18219804763793945,0.021118914094163756
758,3681,0,3681,0.18241000175476074,0.02111312357434157
759,3686,0,3686,0.1826190948486328,0.021107369344304492
760,3691,0,3691,0.1828310489654541,0.021101649764254434
761,3696,0,3696,0.18306303024291992,0.021095963748486872
763,3706,0,3706,0.18349909782409668,0.021084687233180674
764,3711,0,3711,0.1837301254272461,0.021079093380136568
765,3716,0,3716,0.18395495414733887,0.02107352725424467
766,3721,0,3721,0.18417811393737793,0.02106798785013937
767,3726,0,3726,0.1844010353088379,0.021062474022379204
768,3731,0,3731,0.18463897705078125,0.021056984386149415
770,3741,0,3741,0.18507599830627441,0.021046072780123232
771,3746,0,3746,0.18529415130615234,0.021040648954873516
772,3750,0,3750,0.18550491333007812,0.020999560032069473
773,3755,0,3755,0.18572688102722168,0.02099101401763718
774,3759,0,3759,0.18593311309814453,0.020789843213600345
775,3764,0,3764,0.18615007400512695,0.02077347053965485
776,3769,0,3769,0.1863880157470703,0.020758726026587956
778,3779,0,3779,0.18683695793151855,0.02073299150525714
779,3784,0,3784,0.18705987930297852,0.020721576474893755
780,3789,0,3789,0.18729400634765625,0.02071091872028325
781,3794,0,3794,0.18751788139343262,0.02070089625093696
782,3799,0,3799,0.18774080276489258,0.020691404689700963
783,3804,0,3804,0.18796420097351074,0.02068235655001808
785,3814,0,3814,0.18841910362243652,0.02066533683317147
786,3819,0,3819,0.18864107131958008,0.020657275825201726
787,3824,0,3824,0.18886303901672363,0.020649465002592276
788,3829,0,3829,0.18909215927124023,0.02064187168565404
789,3834,0,3834,0.189316987991333,0.020634469686944188
790,3839,0,3839,0.1895589828491211,0.02062723917969535
791,3844,0,3844,0.18978619575500488,0.020620163309240748
793,3854,0,3854,0.19025206565856934,0.020606415140683704
794,3859,0,3859,0.19048118591308594,0.02059971908888768
795,3864,0,3864,0.19070887565612793,0.020593129732715768
796,3869,0,3869,0.1909470558166504,0.02058663924974401
797,3874,0,3874,0.1911768913269043,0.02058024051930164
798,3879,0,3879,0.1914050579071045,0.020573927366277472
800,3889,0,3889,0.19186806678771973,0.020561534721611926
801,3894,0,3894,0.19209814071655273,0.020555444067656956
802,3899,0,3899,0.19232892990112305,0.020549417996498724
803,3904,0,3904,0.19257593154907227,0.020543453475661444
804,3909,0,3909,0.19281816482543945,0.02053754742507177
805,3914,0,3914,0.19305706024169922,0.020531696204177084
807,3924,0,3924,0.19354605674743652,0.020520145010435076
808,3929,0,3929,0.19378209114074707,0.02051444045735736
809,3934,0,3934,0.19401288032531738,0.020508780551696883
810,3939,0,3939,0.1942429542541504,0.020503162849433428
811,3944,0,3944,0.1944730281829834,0.02049758506289177
812,3949,0,3949,0.19470787048339844,0.020492045459560317
813,3954,0,3954,0.19493913650512695,0.020486542545269375
815,3964,0,3964,0.19541001319885254,0.020475639608132416
816,3969,0,3969,0.19568204879760742,0.02047023592068015
817,3974,0,3974,0.1959090232849121,0.020464862161815353
818,3979,0,3979,0.19613313674926758,0.02045951707505203
819,3984,0,3984,0.19635605812072754,0.020454199300588644
820,3989,0,3989,0.19658899307250977,0.020448907543776727
822,3999,0,3999,0.19703912734985352,0.020438398365707895
823,4004,0,4004,0.19726109504699707,0.020433179478591697
824,4009,0,4009,0.19750714302062988,0.020427983404415824
825,4014,0,4014,0.1977379322052002,0.02042280953680913
826,4019,0,4019,0.1979680061340332,0.020417657494203302
827,4024,0,4024,0.1981959342956543,0.020412526988920873
829,4033,0,4033,0.19867324829101562,0.02040305596836204
830,4038,0,4038,0.1989119052886963,0.020394653670245837
831,4043,0,4043,0.19915103912353516,0.02038695642706138
832,4048,0,4048,0.19939303398132324,0.020379825564414866
833,4053,0,4053,0.1996321678161621,0.02037315560662846
834,4058,0,4058,0.19986820220947266,0.020366869691713
835,4063,0,4063,0.2001030445098877,0.020360903323560064
837,4073,0,4073,0.20060014724731445,0.02034969050958927
838,4078,0,4078,0.20083093643188477,0.02034435625072366
839,4083,0,4083,0.20105910301208496,0.020339170147485246
840,4088,0,4088,0.2012951374053955,0.020334112170524346
841,4093,0,4093,0.20152807235717773,0.020329159395795382
842,4098,0,4098,0.20175695419311523,0.020324292233274383
844,4108,0,4108,0.2022230625152588,0.020314774072358013
845,4113,0,4113,0.2024550437927246,0.020310107984279558
846,4118,0,4118,0.2026841640472412,0.020305491015121916
847,4123,0,4123,0.20291399955749512,0.020300915747931685
848,4128,0,4128,0.20314908027648926,0.020296378913555665
849,4133,0,4133,0.20338106155395508,0.020291877945825206
851,4143,0,4143,0.203840970993042,0.02028296578054838
852,4148,0,4148,0.20407700538635254,0.020278548116466257
853,4153,0,4153,0.20430803298950195,0.02027415521728847
854,4158,0,4158,0.20453810691833496,0.020269786025198473
855,4163,0,4163,0.20476794242858887,0.020265438172315912
856,4168,0,4168,0.20500922203063965,0.02026110980255026
857,4173,0,4173,0.20524096488952637,0.020256800425487605
859,4183,0,4183,0.20570015907287598,0.020248236044645943
860,4188,0,4188,0.20593619346618652,0.02024397786335767
861,4193,0,4193,0.20617914199829102,0.020239734350738687
862,4198,0,4198,0.20642709732055664,0.020235505656218126
863,4203,0,4203,0.20667219161987305,0.020231291667539453
864,4208,0,4208,0.20691990852355957,0.02022709156691616
866,4218,0,4218,0.20741820335388184,0.02021873053998898
867,4223,0,4223,0.20765900611877441,0.020214569596465125
868,4228,0,4228,0.20789718627929688,0.02021042145390919
869,4233,0,4233,0.20813417434692383,0.02020628551120236
870,4238,0,4238,0.2083749771118164,0.020202161461758395
871,4243,0,4243,0.20861196517944336,0.02019804946156375
872,4248,0,4248,0.2088470458984375,0.020193949664472483
874,4258,0,4258,0.20932602882385254,0.020185785778765276
875,4263,0,4263,0.20956110954284668,0.020181721312865292
876,4268,0,4268,0.20980191230773926,0.020177668572025687
877,4273,0,4273,0.2100391387939453,0.020173627448075854
878,4278,0,4278,0.21027398109436035,0.020169597549526505
879,4283,0,4283,0.21051502227783203,0.020165578482561203
881,4293,0,4293,0.21098995208740234,0.020157572013261543
882,4298,0,4298,0.21123504638671875,0.020153584038766638
883,4303,0,4303,0.21147394180297852,0.0201496056123232
884,4308,0,4308,0.21170902252197266,0.02014563633089861
885,4313,0,4313,0.21195101737976074,0.020141675916196835
886,4318,0,4318,0.2121899127960205,0.02013772404644483
888,4328,0,4328,0.21266508102416992,0.02012984412537946
889,4333,0,4333,0.2129039764404297,0.02012591525405827
890,4338,0,4338,0.21313881874084473,0.020121993371021572
891,4343,0,4343,0.2133791446685791,0.020118078154496073
892,4348,0,4348,0.21361708641052246,0.02011416925377376
893,4353,0,4353,0.2138521671295166,0.02011026639036867
894,4358,0,4358,0.21409201622009277,0.02010636939700553
896,4367,0,4367,0.2145531177520752,0.02005080732572487
897,4372,0,4372,0.21479511260986328,0.02001746091219067
898,4377,0,4377,0.21503615379333496,0.019987671668554505
899,4382,0,4382,0.2152712345123291,0.01996085026155687
900,4387,0,4387,0.21551203727722168,0.01993652803374587
901,4392,0,4392,0.21575021743774414,0.01991431203067977
903,4402,0,4402,0.21622610092163086,0.019874961833396633
904,4407,0,4407,0.21648001670837402,0.019857372193107545
905,4412,0,4412,0.21672487258911133,0.019840922410663642
906,4417,0,4417,0.21697211265563965,0.019825443009026604
907,4422,0,4422,0.21721696853637695,0.019810801325420197
908,4427,0,4427,0.21746516227722168,0.019796904533170567
910,4437,0,4437,0.21795916557312012,0.019771033303706578
911,4442,0,4442,0.2182011604309082,0.01975890200724154
912,4447,0,4447,0.2184607982635498,0.01974722973156972
913,4452,0,4452,0.21869897842407227,0.019735981048688348
914,4457,0,4457,0.2189328670501709,0.01972511784532327
915,4462,0,4462,0.21917414665222168,0.019714596721332862
916,4467,0,4467,0.21941184997558594,0.019704383559309122
918,4477,0,4477,0.21988606452941895,0.01968480791534498
919,4481,0,4481,0.22011017799377441,0.019640005567586834
920,4486,0,4486,0.22034502029418945,0.019616728077931418
921,4491,0,4491,0.22058486938476562,0.019595983275758903
922,4496,0,4496,0.2208249568939209,0.01957730362153674
923,4501,0,4501,0.22105908393859863,0.019560306140490577
925,4511,0,4511,0.22155499458312988,0.019530167178482317
926,4516,0,4516,0.22179508209228516,0.019516603985542384
927,4521,0,4521,0.22203993797302246,0.01950384509464084
928,4526,0,4526,0.22228407859802246,0.019491760296982297
929,4531,0,4531,0.2225351333618164,0.01948023239618705
930,4536,0,4536,0.22277402877807617,0.019469174993601592
932,4546,0,4546,0.22324514389038086,0.01944825546913113
933,4551,0,4551,0.22348999977111816,0.019438297726650827
934,4556,0,4556,0.22372698783874512,0.019428611508941995
935,4560,0,4560,0.22394704818725586,0.01925816358105504
936,4564,0,4564,0.22417402267456055,0.019133782124090868
937,4569,0,4569,0.2244129180908203,0.01911111180105541
938,4574,0,4574,0.22464799880981445,0.0190903962157881
940,4584,0,4584,0.2251272201538086,0.019053567010480065
941,4589,0,4589,0.22536110877990723,0.019036985083942783
942,4594,0,4594,0.2256009578704834,0.01902138173415262
943,4599,0,4599,0.22583818435668945,0.019006620582989575
944,4604,0,4604,0.22607207298278809,0.018992595399150276
945,4609,0,4609,0.22631287574768066,0.01897921577495025
947,4619,0,4619,0.22678899765014648,0.01895407321730871
948,4624,0,4624,0.22703003883361816,0.0189421891994676
949,4629,0,4629,0.22726798057556152,0.018930711419596923
950,4634,0,4634,0.22750306129455566,0.018919607397900513
951,4639,0,4639,0.22774410247802734,0.018908842059348802
952,4644,0,4644,0.2279820442199707,0.018898382937593706
953,4649,0,4649,0.22821712493896484,0.018888206034934178
955,4659,0,4659,0.22869491577148438,0.018868630001326072
956,4664,0,4664,0.22892999649047852,0.01885919603247041
957,4669,0,4669,0.2291719913482666,0.018849975379690104
958,4674,0,4674,0.2294158935546875,0.018840955343226953
959,4679,0,4679,0.22965097427368164,0.018832125261485894
960,4684,0,4684,0.22989201545715332,0.01882347333020212
962,4694,0,4694,0.23036479949951172,0.018806655370850363
963,4699,0,4699,0.23060393333435059,0.01879847008989779
964,4704,0,4704,0.23084306716918945,0.018790422627765445
965,4708,0,4708,0.231065034866333,0.018249628900590537
966,4713,0,4713,0.2313070297241211,0.01820837865144621
967,4718,0,4718,0.23154497146606445,0.018173512830991737
969,4728,0,4728,0.23201799392700195,0.018118267851611324
970,4733,0,4733,0.2322549819946289,0.018096086696141437
971,4738,0,4738,0.23250722885131836,0.018076618310384096
972,4743,0,4743,0.23275423049926758,0.01805935877700399
973,4748,0,4748,0.2330000400543213,0.01804392115136201
974,4753,0,4753,0.23324322700500488,0.01802999748228412
975,4758,0,4758,0.23350095748901367,0.018017329062638168
977,4768,0,4768,0.23397397994995117,0.01799491452519822
978,4773,0,4773,0.2342090606689453,0.01798484942588115
979,4778,0,4778,0.23444390296936035,0.01797539327860997
980,4783,0,4783,0.2346789836883545,0.01796645670831567
981,4788,0,4788,0.23491597175598145,0.01795796089658547
982,4793,0,4793,0.23515105247497559,0.01794984043900331
984,4803,0,4803,0.23564910888671875,0.01793454056700574
985,4808,0,4808,0.23589301109313965,0.017927289683847995
986,4813,0,4813,0.23613524436950684,0.01792026143385137
987,4818,0,4818,0.23637914657592773,0.017913428352311158
988,4823,0,4823,0.2366321086883545,0.01790676947142521
989,4828,0,4828,0.23686909675598145,0.017900267930029932
991,4838,0,4838,0.23734021186828613,0.01788767494112359
992,4843,0,4843,0.23757219314575195,0.01788155683017909
993,4848,0,4848,0.2378091812133789,0.017875544763222388
994,4853,0,4853,0.23804306983947754,0.017869631481425792
995,4858,0,4858,0.2382798194885254,0.017863810287617278
996,4863,0,4863,0.23851418495178223,0.01785807541586412
997,4868,0,4868,0.23874998092651367,0.017852422489411466
999,4878,0,4878,0.23921990394592285,0.017841347571612588
1000,4883,0,4883,0.23945403099060059,0.01783591735756803
1001,4888,0,4888,0.23969006538391113,0.017830553541075714
1002,4893,0,4893,0.23992300033569336,0.01782525353968312
1003,4898,0,4898,0.2401599884033203,0.01782001531192571
1004,4903,0,4903,0.24039506912231445,0.017814836611711536
1006,4913,0,4913,0.24089598655700684,0.01780464828672365
1007,4918,0,4918,0.24113988876342773,0.01779963453106848
1008,4923,0,4923,0.2413942813873291,0.017794671552379047
1009,4928,0,4928,0.24163103103637695,0.01778975675730329
1010,4933,0,4933,0.24187111854553223,0.017784887538081898
1011,4937,0,4937,0.2420940399169922,0.017774283220188345
1013,4947,0,4947,0.24256420135498047,0.01775997612065628
1014,4952,0,4952,0.2427990436553955,0.017753614777058085
1015,4957,0,4957,0.24303603172302246,0.017747649855528496
1016,4962,0,4962,0.2432701587677002,0.017742005846540662
1017,4967,0,4967,0.24350619316101074,0.017736624822387147
1018,4972,0,4972,0.24374008178710938,0.017731464690962852
1019,4977,0,4977,0.24397587776184082,0.01772649281841097
1021,4987,0,4987,0.2444469928741455,0.017716998752336482
1022,4992,0,4992,0.24468088150024414,0.01771242957468209
1023,4997,0,4997,0.2449181079864502,0.017707957482230717
1024,5002,0,5002,0.24515295028686523,0.017703569723367757
1025,5007,0,5007,0.2453901767730713,0.017699253093630286
1026,5012,0,5012,0.24562406539916992,0.017694995984969274
1028,5022,0,5022,0.2460951805114746,0.017686636411890454
1029,5027,0,5027,0.24633216857910156,0.017682527780871073
1030,5032,0,5032,0.24658823013305664,0.017678460453373828
1031,5037,0,5037,0.24683213233947754,0.017674428879775925
1032,5042,0,5042,0.24707293510437012,0.017670429331603114
1033,5047,0,5047,0.2473158836364746,0.017666459702840785
1034,5052,0,5052,0.24756717681884766,0.017662517768140807
1036,5062,0,5062,0.2480449676513672,0.01765470591709655
1037,5067,0,5067,0.24828314781188965,0.01765083236071139
1038,5072,0,5072,0.2485182285308838,0.01764697933422644
1039,5077,0,5077,0.24875497817993164,0.01764314578338217
1040,5082,0,5082,0.24898886680603027,0.01763933029983189
1041,5087,0,5087,0.24922490119934082,0.0176355318213337
1043,5097,0,5097,0.2496960163116455,0.017627983603072394
1044,5102,0,5102,0.24992895126342773,0.017624232263936536
1045,5107,0,5107,0.2501659393310547,0.01762049471773211
1046,5112,0,5112,0.2504000663757324,0.01761677031042203
1047,5117,0,5117,0.2506380081176758,0.01761305872110932
1048,5122,0,5122,0.25087523460388184,0.0176093595557785
1050,5132,0,5132,0.2513580322265625,0.017601996199921737
1051,5137,0,5137,0.2516012191772461,0.01759833123107165
1052,5142,0,5142,0.25184106826782227,0.0175946771661108
1053,5147,0,5147,0.25208282470703125,0.017591033708462767
1054,5152,0,5152,0.2523231506347656,0.017587400421702794
1055,5157,0,5157,0.2525649070739746,0.017583776935947967
1056,5162,0,5162,0.2528071403503418,0.01758016304155678
1058,5172,0,5172,0.25328898429870605,0.017572963286037312
1059,5177,0,5177,0.25353217124938965,0.01756937688366663
1060,5182,0,5182,0.25377702713012695,0.017565799111879922
1061,5187,0,5187,0.25401997566223145,0.017562229756796992
1062,5192,0,5192,0.2542600631713867,0.017558668559292577
1063,5197,0,5197,0.2545032501220703,0.01755511518163525
1065,5207,0,5207,0.2549870014190674,0.01754803052442205
1066,5212,0,5212,0.25522804260253906,0.01754449867252747
1067,5217,0,5217,0.25546908378601074,0.017540973437582725
1068,5222,0,5222,0.2557098865509033,0.017537454539933633
1069,5227,0,5227,0.2559521198272705,0.01753394174716728
1070,5232,0,5232,0.2561910152435303,0.017530434891778558
1072,5242,0,5242,0.25667905807495117,0.017523438458092202
1073,5247,0,5247,0.25692200660705566,0.017519948639251767
1074,5252,0,5252,0.25716304779052734,0.01751646431750158
1075,5257,0,5257,0.25742101669311523,0.01751298546701686
1076,5262,0,5262,0.25764918327331543,0.017509512069328582
1077,5267,0,5267,0.25788116455078125,0.017506044096742786
1078,5272,0,5272,0.25810813903808594,0.017502581520813815
1080,5282,0,5282,0.258587121963501,0.017495672454839274
1081,5287,0,5287,0.25882387161254883,0.017492225866416345
1082,5292,0,5292,0.25905704498291016,0.01748878445438945
1083,5297,0,5297,0.2592949867248535,0.017485348096746036
1084,5302,0,5302,0.25952887535095215,0.017481916652219032
1085,5307,0,5307,0.2597649097442627,0.01747848995406619
1087,5317,0,5317,0.2602410316467285,0.017471649998401097
1088,5322,0,5322,0.26047515869140625,0.017468236307756974
1089,5327,0,5327,0.2607128620147705,0.017464826515236138
1090,5332,0,5332,0.26094889640808105,0.017461420399863415
1091,5337,0,5337,0.2611870765686035,0.01745801774455788
1092,5342,0,5342,0.26142001152038574,0.01745461834699164
1094,5352,0,5352,0.26189112663269043,0.017447828635666258
1095,5357,0,5357,0.2621290683746338,0.017444438041458482
1096,5362,0,5362,0.2623631954193115,0.01744105014801821
1097,5367,0,5367,0.2625999450683594,0.0174376648924676
1098,5372,0,5372,0.2628340721130371,0.017434282247955946
1099,5377,0,5377,0.26307201385498047,0.017430902220075466
1100,5382,0,5382,0.2633049488067627,0.017427524843139534
1102,5392,0,5392,0.2637920379638672,0.017420778313504637
1103,5396,0,5396,0.26401782035827637,0.01738734890570715
1104,5401,0,5401,0.2642538547515869,0.017375060283439023
1105,5406,0,5406,0.26449108123779297,0.01736377392212545
1106,5411,0,5411,0.264725923538208,0.01735331964629519
1107,5416,0,5416,0.2649650573730469,0.017343550855916396
1109,5426,0,5426,0.2654390335083008,0.017325633762762332
1110,5431,0,5431,0.265671968460083,0.017317341121019087
1111,5436,0,5436,0.26590991020202637,0.01730941630644797
1112,5440,0,5440,0.26613807678222656,0.01729473896525511
1113,5445,0,5445,0.26637697219848633,0.017284185843520046
1114,5450,0,5450,0.2666161060333252,0.017274410299984763
1115,5455,0,5455,0.26685523986816406,0.017265288169285204
1117,5463,0,5463,0.267301082611084,0.017257086956754125
1118,5468,0,5468,0.2675352096557617,0.017243095535011004
1119,5472,0,5472,0.2677581310272217,0.017205183973887195
1120,5476,0,5476,0.2679789066314697,0.01707439716800974
1121,5480,0,5480,0.2682030200958252,0.01683250351038917
1122,5483,0,5483,0.2684028148651123,0.016258213518308983
1124,5489,0,5489,0.2687962055206299,0.014794557689707164
1125,5492,0,5492,0.2689859867095947,0.011182880253704086
1126,5495,0,5495,0.26917290687561035,0.0076302707377840975
1127,5498,0,5498,0.2693629264831543,0.004868987116940013
1128,5501,0,5501,0.2695648670196533,0.003551850782471617
1129,5504,0,5504,0.2697560787200928,0.0023374942699534934
1131,5510,0,5510,0.27013397216796875,0.0013524024415931585
1132,5513,0,5513,0.27033400535583496,0.0013117130463716877
1133,5516,0,5516,0.2705259323120117,0.000999761815581126
1134,5521,0,5521,0.27076196670532227,0.0009829547704617483
1135,5524,0,5524,0.2709670066833496,0.0009702508566402214
1136,5527,0,5527,0.27116894721984863,0.0008862210109272366
1137,5530,0,5530,0.2713639736175537,0.0006400333606527653
1139,5536,0,5536,0.27173900604248047,0.00021689148695494415
1140,5539,0,5539,0.2719249725341797,0.00012169916241697825
1141,5542,0,5542,0.27211427688598633,6.936422758575171e-05
1142,5545,0,5545,0.27230095863342285,3.856406048344592e-05
1143,5548,0,5548,0.2724909782409668,2.4529313802396054e-05
1144,5551,0,5551,0.2726759910583496,1.9931206686165053e-05
1146,5557,0,5557,0.27305006980895996,7.479902760052434e-06
1147,5560,0,5560,0.2732391357421875,7.023951809827678e-06
1148,5563,0,5563,0.2734251022338867,2.7031879686705585e-06
1149,5566,0,5566,0.27361297607421875,1.2686563336056185e-06
1150,5569,0,5569,0.27379918098449707,9.648555064711824e-07
1151,5572,0,5572,0.2739880084991455,3.354222314142178e-07
1153,5578,0,5578,0.27436304092407227,6.72485448216772e-08
1154,5581,0,5581,0.2745652198791504,3.9051705823188195e-08
1155,5584,0,5584,0.27476000785827637,1.5804890709825776e-08
1156,5587,0,5587,0.2749512195587158,6.862875061217013e-09


==> plot_data/quadratic_minimax_problem_n20_alpha00001/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,6.985664367675781e-05,4.387072431292609
187,188,187,375,0.004339933395385742,0.4268561502630121
374,375,374,749,0.008699893951416016,0.19745276258065977
561,562,561,1123,0.013796091079711914,0.12581339699925403
748,749,748,1497,0.018352031707763672,0.0934848928777029
935,936,935,1871,0.023186922073364258,0.07523137209185625
1123,1124,1123,2247,0.02775287628173828,0.06376853690493829
1310,1311,1310,2621,0.0321657657623291,0.056205750750353285
1497,1498,1497,2995,0.03638601303100586,0.05091764264030393
1684,1685,1684,3369,0.040611982345581055,0.04695280207456066
1871,1872,1871,3743,0.044960975646972656,0.0437972404294198
2058,2059,2058,4117,0.04943990707397461,0.04117031359160079
2245,2246,2245,4491,0.054064035415649414,0.038867931179356635
2432,2433,2432,4865,0.05870199203491211,0.03684030277443672
2619,2620,2619,5239,0.06337785720825195,0.034993125101065906
2806,2807,2806,5613,0.06756973266601562,0.03331461063843964
2994,2995,2994,5989,0.07189393043518066,0.03177870754267203
3181,3182,3181,6363,0.07608294486999512,0.030354916945830392
3368,3369,3368,6737,0.08025288581848145,0.029066080496606667
3555,3556,3555,7111,0.08441376686096191,0.02786500136196921
3742,3743,3742,7485,0.0887138843536377,0.0267577835687742
3929,3930,3929,7859,0.09287381172180176,0.025744063208262037
4116,4117,4116,8233,0.09704399108886719,0.024794878822063784
4303,4304,4303,8607,0.10152792930603027,0.02393050656079627
4490,4491,4490,8981,0.10570597648620605,0.023119442976707722
4677,4678,4677,9355,0.11021089553833008,0.02237284101937738
4864,4865,4864,9729,0.11444973945617676,0.02168486245232052
5052,5053,5052,10105,0.11875605583190918,0.02102912963206462
5239,5240,5239,10479,0.12347006797790527,0.02043606541764476
5426,5427,5426,10853,0.12785601615905762,0.01987485982300528
5613,5614,5613,11227,0.13200783729553223,0.01934990754717838
5800,5801,5800,11601,0.13617300987243652,0.01886341533640373
5987,5988,5987,11975,0.1405189037322998,0.018400255484358547
6174,6175,6174,12349,0.14472603797912598,0.017971270740053537
6361,6362,6361,12723,0.14934301376342773,0.017560142448936594
6548,6549,6548,13097,0.15366697311401367,0.0171756492048547
6735,6736,6735,13471,0.15814971923828125,0.016813272787954178
6923,6924,6923,13847,0.1624150276184082,0.016459547202817882
7110,7111,7110,14221,0.16664695739746094,0.016133178815899436
7297,7298,7297,14595,0.17116999626159668,0.015817381999008492
7484,7485,7484,14969,0.17565202713012695,0.015514264913198478
7671,7672,7671,15343,0.1799170970916748,0.01522677549487873
7858,7859,7858,15717,0.1841588020324707,0.014947917601161646
8045,8046,8045,16091,0.1884000301361084,0.014682193545942156
8232,8233,8232,16465,0.19263982772827148,0.014422275110793912
8419,8420,8419,16839,0.1971268653869629,0.014174385269201931
8606,8607,8606,17213,0.2013390064239502,0.013934918586089796
8794,8795,8794,17589,0.2055809497833252,0.01369703818322894
8981,8982,8981,17963,0.20980191230773926,0.013472596708826617
9168,9169,9168,18337,0.2140038013458252,0.013252271747579555
9355,9356,9355,18711,0.2182457447052002,0.013036502041037724
9542,9543,9542,19085,0.22288990020751953,0.012828176861593373
9729,9730,9729,19459,0.22760796546936035,0.012624249932296478
9916,9917,9916,19833,0.23218083381652832,0.012425715384886363
10103,10104,10103,20207,0.2364640235900879,0.012229720233603896
10290,10291,10290,20581,0.24095797538757324,0.012040529824331786
10477,10478,10477,20955,0.24535799026489258,0.011855113113883795
10664,10665,10664,21329,0.24967694282531738,0.011670728932696805
10852,10853,10852,21705,0.25394773483276367,0.011492422069160376
11039,11040,11039,22079,0.2583191394805908,0.011317526455245284
11226,11227,11226,22453,0.262861967086792,0.01114455606127755
11413,11414,11413,22827,0.2673358917236328,0.010976088678887701
11600,11601,11600,23201,0.2717249393463135,0.010810857488491121
11787,11788,11787,23575,0.2759678363800049,0.010648165195958324
11974,11975,11974,23949,0.2801940441131592,0.01048723525225835
12161,12162,12161,24323,0.28456902503967285,0.010331046987734387
12348,12349,12348,24697,0.28880786895751953,0.010177000422903149
12535,12536,12535,25071,0.29303789138793945,0.010023687607376788
12723,12724,12723,25447,0.2972888946533203,0.009874388351661208
12910,12911,12910,25821,0.301541805267334,0.00972788276227271
13097,13098,13097,26195,0.3057839870452881,0.009582407567945228
13284,13285,13284,26569,0.3100137710571289,0.009440210097111403
13471,13472,13471,26943,0.31427884101867676,0.009300807491451043
13658,13659,13658,27317,0.31868481636047363,0.009162805912689139
13845,13846,13845,27691,0.3229219913482666,0.009026351998973232
14032,14033,14032,28065,0.3271489143371582,0.00889361708138467
14219,14220,14219,28439,0.33136796951293945,0.008762362962220048
14406,14407,14406,28813,0.33560800552368164,0.008631818311148658
14593,14594,14593,29187,0.33982396125793457,0.008504935131714412
14781,14782,14781,29563,0.3440549373626709,0.008379168733483884
14968,14969,14968,29937,0.34828901290893555,0.008254754687540009
15155,15156,15155,30311,0.3530550003051758,0.008132971972377896
15342,15343,15342,30685,0.35790395736694336,0.00801367599825493
15529,15530,15529,31059,0.3624858856201172,0.007895271987635863
15716,15717,15716,31433,0.3673441410064697,0.007778287115184196
15903,15904,15903,31807,0.37218403816223145,0.007664377113772949
16090,16091,16090,32181,0.377392053604126,0.007551615131602499
16277,16278,16277,32555,0.3825337886810303,0.007439546237710235
16464,16465,16464,32929,0.38794398307800293,0.0073304387459651715
16652,16653,16652,33305,0.3921971321105957,0.007222358433041664
16839,16840,16839,33679,0.3975968360900879,0.007115366707040971
17026,17027,17026,34053,0.4030458927154541,0.007010580369468733
17213,17214,17213,34427,0.40810108184814453,0.006907993880371653
17400,17401,17400,34801,0.41236305236816406,0.006806040535705541
17587,17588,17587,35175,0.4165329933166504,0.0067053749515346575
17774,17775,17774,35549,0.4206888675689697,0.006607308327007169
17961,17962,17961,35923,0.4248518943786621,0.0065101815597963944
18148,18149,18148,36297,0.42905688285827637,0.006413705463970871
18335,18336,18335,36671,0.4332888126373291,0.006319698938833546
18523,18524,18523,37047,0.43753480911254883,0.0062266161705918435
18710,18711,18710,37421,0.44176197052001953,0.006134441861422461
18897,18898,18897,37795,0.4460420608520508,0.0060441494603811815
19084,19085,19084,38169,0.45035600662231445,0.005955784028959034
19271,19272,19271,38543,0.45494604110717773,0.0058679024691762754
19458,19459,19458,38917,0.4592769145965576,0.005781171255998769
19645,19646,19645,39291,0.46356797218322754,0.005696657794068482
19832,19833,19832,39665,0.46787405014038086,0.00561293261885974
20019,20020,20019,40039,0.4722170829772949,0.005529799295806987
20206,20207,20206,40413,0.4766080379486084,0.005448758396247348
20393,20394,20393,40787,0.48092198371887207,0.005368958669803844
20581,20582,20581,41163,0.48525381088256836,0.005289077870481344
20768,20769,20768,41537,0.4895598888397217,0.0052112411101270205
20955,20956,20955,41911,0.4939420223236084,0.005135079794354078
21142,21143,21142,42285,0.4982597827911377,0.005059305922840368
21329,21330,21329,42659,0.5025949478149414,0.0049845477762051
21516,21517,21516,43033,0.5069470405578613,0.004911690536079844
21703,21704,21703,43407,0.5115277767181396,0.004839501595318327
21890,21891,21890,43781,0.5158247947692871,0.004767840536468726
22077,22078,22077,44155,0.520150899887085,0.004697967371901102
22264,22265,22264,44529,0.5245480537414551,0.0046291720706896355
22452,22453,22452,44905,0.5288779735565186,0.0045603014920862425
22639,22640,22639,45279,0.5331780910491943,0.004493194112088532
22826,22827,22826,45653,0.5374979972839355,0.004427536615819525
23013,23014,23013,46027,0.5417828559875488,0.004362198228660415
23200,23201,23200,46401,0.5460820198059082,0.004297750083835072
23387,23388,23387,46775,0.5510368347167969,0.004234934945489196
23574,23575,23574,47149,0.555340051651001,0.004172689154264585
23761,23762,23761,47523,0.5595269203186035,0.00411090885270882
23948,23949,23948,47897,0.5637450218200684,0.004050663228690511
24135,24136,24135,48271,0.5680630207061768,0.003991348923488977
24322,24323,24322,48645,0.5722298622131348,0.00393228129136683
24510,24511,24510,49021,0.5765790939331055,0.003874108946001379
24697,24698,24697,49395,0.5808308124542236,0.0038175014797594596
24884,24885,24884,49769,0.5850129127502441,0.003761161252805195
25071,25072,25071,50143,0.589202880859375,0.003705597809745314
25258,25259,25258,50517,0.5933849811553955,0.0036514389321942
25445,25446,25445,50891,0.5976259708404541,0.0035977662035426025
25632,25633,25632,51265,0.6018710136413574,0.0035445013102282335
25819,25820,25819,51639,0.6061060428619385,0.0034925570428766804
26006,26007,26006,52013,0.6103348731994629,0.003441415027124166
26193,26194,26193,52387,0.6146938800811768,0.003390485028179218
26381,26382,26381,52763,0.6190729141235352,0.0033403298414400226
26568,26569,26568,53137,0.6233499050140381,0.003291523035579312
26755,26756,26755,53511,0.6275970935821533,0.0032429422112348854
26942,26943,26942,53885,0.6318190097808838,0.0031950373888009276
27129,27130,27129,54259,0.6361961364746094,0.0031483414658316695
27316,27317,27316,54633,0.6404001712799072,0.0031020610958380555
27503,27504,27503,55007,0.6448569297790527,0.0030561367642648585
27690,27691,27690,55381,0.6492919921875,0.003011350433287845
27877,27878,27877,55755,0.6535708904266357,0.002967253926617867
28064,28065,28064,56129,0.6579461097717285,0.0029233402602818867
28252,28253,28252,56505,0.6623468399047852,0.0028800973980050108
28439,28440,28439,56879,0.6667349338531494,0.002838015510286268
28626,28627,28626,57253,0.6711270809173584,0.002796125791613191
28813,28814,28813,57627,0.6757490634918213,0.0027548234633445285
29000,29001,29000,58001,0.6809210777282715,0.0027145620250565348
29187,29188,29187,58375,0.6866569519042969,0.002674655974004104
29374,29375,29374,58749,0.6919107437133789,0.0026350601225066795
29561,29562,29561,59123,0.6971278190612793,0.002596445648366174
29748,29749,29748,59497,0.702254056930542,0.002558423694653346
29935,29936,29935,59871,0.706618070602417,0.002520559737174191
30122,30123,30122,60245,0.710839033126831,0.002483472184735134
30310,30311,30310,60621,0.7151238918304443,0.0024469927113159313
30497,30498,30497,60995,0.7193319797515869,0.002410872741610936
30684,30685,30684,61369,0.7235229015350342,0.002375262707345216
30871,30872,30871,61743,0.7283368110656738,0.0023405490963662196
31058,31059,31058,62117,0.7325530052185059,0.0023061394876422872
31245,31246,31245,62491,0.736914873123169,0.002271999842067275
31432,31433,31432,62865,0.7411839962005615,0.002238706859569761
31619,31620,31619,63239,0.7454190254211426,0.0022059224976698055
31806,31807,31806,63613,0.7497420310974121,0.0021732748319072044
31993,31994,31993,63987,0.7540299892425537,0.0021412987563475
32181,32182,32181,64363,0.7583498954772949,0.0021098452079797614
32368,32369,32368,64737,0.7626669406890869,0.0020787004024013797
32555,32556,32555,65111,0.7671091556549072,0.0020479980568197816
32742,32743,32742,65485,0.7714197635650635,0.0020180678096168004
32929,32930,32929,65859,0.7757418155670166,0.0019883976344864905
33116,33117,33116,66233,0.7800588607788086,0.0019589622606636424
33303,33304,33303,66607,0.7843718528747559,0.0019302574914298778
33490,33491,33490,66981,0.7888240814208984,0.001901989158075218
33677,33678,33677,67355,0.7932629585266113,0.0018738391836372098
33864,33865,33864,67729,0.7976689338684082,0.0018462701365876725
34051,34052,34051,68103,0.80206298828125,0.0018192937315925127
34239,34240,34239,68479,0.8064699172973633,0.0017922951382207787
34426,34427,34426,68853,0.8108940124511719,0.0017658240745215114
34613,34614,34613,69227,0.8152608871459961,0.0017400180670017755
34800,34801,34800,69601,0.8203020095825195,0.001714434556782584
34987,34988,34987,69975,0.824699878692627,0.001689055195338245
35174,35175,35174,70349,0.8290958404541016,0.0016643063617935718
35361,35362,35361,70723,0.8335018157958984,0.0016399319376308346
35548,35549,35548,71097,0.8378880023956299,0.001615660046207436
35735,35736,35735,71471,0.8422651290893555,0.0015918906517416482
35922,35923,35922,71845,0.8466219902038574,0.0015686307948114557
36110,36111,36110,72221,0.8509061336517334,0.0015453510768855252
36297,36298,36297,72595,0.8553719520568848,0.0015225281380791078
36484,36485,36484,72969,0.8607511520385742,0.0015002780683560184
36671,36672,36671,73343,0.8652548789978027,0.0014782183502988246
36858,36859,36858,73717,0.8696420192718506,0.001456336095182676
37045,37046,37045,74091,0.873938798904419,0.0014349980292786078
37232,37233,37232,74465,0.8781847953796387,0.001413981114709229
37419,37420,37419,74839,0.8825719356536865,0.0013930530528216492
37606,37607,37606,75213,0.8868288993835449,0.00137255963699807
37793,37794,37793,75587,0.8911547660827637,0.0013525042760179707
37981,37982,37981,75963,0.8954248428344727,0.0013324312023538511
38168,38169,38168,76337,0.8997170925140381,0.0013127536132524127
38355,38356,38355,76711,0.9040689468383789,0.0012935694876170215
38542,38543,38542,77085,0.90836501121521,0.0012745482103713932
38729,38730,38729,77459,0.9126479625701904,0.001255681180700022
38916,38917,38916,77833,0.9169809818267822,0.0012372838335572769
39103,39104,39103,78207,0.921889066696167,0.0012191619288234614
39290,39291,39290,78581,0.9261391162872314,0.0012011170404342198
39477,39478,39477,78955,0.9304909706115723,0.0011834480996779726
39664,39665,39664,79329,0.934838056564331,0.001166155739990052
39851,39852,39851,79703,0.9391930103302002,0.0011489393784061142
40039,40040,40039,80079,0.9435498714447021,0.0011318819067622492
40226,40227,40226,80453,0.9478771686553955,0.001115341250087019
40413,40414,40413,80827,0.9521589279174805,0.0010989399098950293
40600,40601,40600,81201,0.956671953201294,0.0010826726292907636
40787,40788,40787,81575,0.9609458446502686,0.0010668107259603123
40974,40975,40974,81949,0.9652400016784668,0.0010511850456671186
41161,41162,41161,82323,0.9696087837219238,0.001035626134311969
41348,41349,41348,82697,0.9739618301391602,0.001020392390872701
41535,41536,41535,83071,0.9783947467803955,0.0010054823686612743
41722,41723,41722,83445,0.9826529026031494,0.0009906374725653308
41910,41911,41910,83821,0.9871499538421631,0.0009759307769135151
42097,42098,42097,84195,0.9916439056396484,0.0009616693294407396
42284,42285,42284,84569,0.9959127902984619,0.0009475270645569473
42471,42472,42471,84943,1.0001840591430664,0.0009335013079019953
42658,42659,42658,85317,1.0044739246368408,0.0009198254240801708
42845,42846,42845,85691,1.008699893951416,0.0009063521177229406
43032,43033,43032,86065,1.0129458904266357,0.0008929367048959243
43219,43220,43219,86439,1.017246961593628,0.0008798025317375594
43406,43407,43406,86813,1.0214660167694092,0.0008669466304561599
43593,43594,43593,87187,1.0257017612457275,0.0008541465471275163
43780,43781,43780,87561,1.0299148559570312,0.0008415331736523942
43968,43969,43968,87937,1.0349397659301758,0.0008291703523994013
44155,44156,44155,88311,1.039167881011963,0.0008169760044934848
44342,44343,44342,88685,1.043375015258789,0.0008048829077523744
44529,44530,44529,89059,1.0475149154663086,0.000793091774372572
44716,44717,44716,89433,1.0516247749328613,0.0007814743576725847
44903,44904,44903,89807,1.0557360649108887,0.0007699071451976803
45090,45091,45090,90181,1.0599470138549805,0.0007585831721729655
45277,45278,45277,90555,1.0640668869018555,0.0007474983954136405
45464,45465,45464,90929,1.0683059692382812,0.0007364614649947085
45651,45652,45651,91303,1.072448968887329,0.0007255864060411758
45839,45840,45839,91679,1.076584815979004,0.0007149271073745293
46026,46027,46026,92053,1.0806918144226074,0.0007044123759109395
46213,46214,46213,92427,1.0848140716552734,0.0006939856339931124
46400,46401,46400,92801,1.088925838470459,0.0006838195014384398
46587,46588,46587,93175,1.0930359363555908,0.0006738023309705584
46774,46775,46774,93549,1.0972118377685547,0.0006638287015945783
46961,46962,46961,93923,1.1013298034667969,0.0006540654403931919
47148,47149,47148,94297,1.1054670810699463,0.0006445077811375885
47335,47336,47335,94671,1.1095941066741943,0.000634991139863052
47522,47523,47522,95045,1.113874912261963,0.0006256148309841272
47710,47711,47710,95421,1.1180698871612549,0.0006164243166301563
47897,47898,47897,95795,1.122565746307373,0.0006073578559281502
48084,48085,48084,96169,1.1266980171203613,0.0005983678582094057
48271,48272,48271,96543,1.1313908100128174,0.0005896027745953714
48458,48459,48458,96917,1.1370689868927002,0.0005809654216387414
48645,48646,48645,97291,1.1412248611450195,0.0005723658348876812
48832,48833,48832,97665,1.145467758178711,0.0005639481824898674
49019,49020,49019,98039,1.1495988368988037,0.0005557072511196488
49206,49207,49206,98413,1.153738021850586,0.00054750148777222
49393,49394,49393,98787,1.158566951751709,0.0005394173797783963
49580,49581,49580,99161,1.1626899242401123,0.0005315351028196626
49768,49769,49768,99537,1.1676008701324463,0.0005236755870301071
49955,49956,49955,99911,1.1718828678131104,0.0005159243611168376
50142,50143,50142,100285,1.1761419773101807,0.0005083672389076913
50329,50330,50329,100659,1.1803350448608398,0.0005009196384750907
50516,50517,50516,101033,1.184433937072754,0.0004935047984842004
50703,50704,50703,101407,1.1885440349578857,0.00048624729810919253
50890,50891,50890,101781,1.1926429271697998,0.00047914169069405115
51077,51078,51077,102155,1.196803092956543,0.00047206623892782895
51264,51265,51264,102529,1.200967788696289,0.0004650962478902133
51451,51452,51451,102903,1.2050628662109375,0.00045830009623682203
51639,51640,51639,103279,1.2091748714447021,0.0004515231296594527
51826,51827,51826,103653,1.2133398056030273,0.0004448399819275751
52013,52014,52013,104027,1.2175049781799316,0.00043832434435669043
52200,52201,52200,104401,1.2216618061065674,0.00043190261253372563
52387,52388,52387,104775,1.225836992263794,0.00042550930152875896
52574,52575,52574,105149,1.229996919631958,0.0004192520567086151
52761,52762,52761,105523,1.234245777130127,0.0004131253615005492
52948,52949,52948,105897,1.2385139465332031,0.0004070245267538294
53135,53136,53135,106271,1.2426879405975342,0.0004010151111022545
53322,53323,53322,106645,1.2468829154968262,0.00039515542186104675
53509,53510,53509,107019,1.251145839691162,0.0003893429463778467
53697,53698,53697,107395,1.25534987449646,0.0003835496539140515
53884,53885,53884,107769,1.2595429420471191,0.00037793196757582764
54071,54072,54071,108143,1.2637391090393066,0.0003723947950661484
54258,54259,54258,108517,1.2679190635681152,0.00036688228080929207
54445,54446,54445,108891,1.2720561027526855,0.00036148743258669944
54632,54633,54632,109265,1.2761988639831543,0.0003562047867527212
54819,54820,54819,109639,1.2805171012878418,0.00035094432038163366
55006,55007,55006,110013,1.284703016281128,0.0003457630986484349
55193,55194,55193,110387,1.288827896118164,0.0003407108320316953
55380,55381,55380,110761,1.2930359840393066,0.0003356989514265951
55568,55569,55568,111137,1.2975449562072754,0.0003307039462884722
55755,55756,55755,111511,1.3016860485076904,0.0003258604591436374
55942,55943,55942,111885,1.305898904800415,0.0003210860016249173
56129,56130,56129,112259,1.31003999710083,0.00031633293976432805
56316,56317,56316,112633,1.3142409324645996,0.0003116816294093094
56503,56504,56503,113007,1.3184947967529297,0.00030712675017526936
56690,56691,56690,113381,1.3226900100708008,0.00030259089545296583
56877,56878,56877,113755,1.3268179893493652,0.0002981237301416173
57064,57065,57064,114129,1.3310589790344238,0.0002937676276306348
57251,57252,57251,114503,1.3352789878845215,0.00028944607016275924
57439,57440,57439,114879,1.3394548892974854,0.0002851393537394223
57626,57627,57626,115253,1.3436839580535889,0.0002809633688917523
57813,57814,57813,115627,1.3479058742523193,0.000276846565735961
58000,58001,58000,116001,1.3521897792816162,0.0002727483288849592
58187,58188,58187,116375,1.3563330173492432,0.00026873807921773657
58374,58375,58374,116749,1.3605430126190186,0.00026481070405130763
58561,58562,58561,117123,1.3648297786712646,0.00026089964904732
58748,58749,58748,117497,1.3690390586853027,0.0002570481323825977
58935,58936,58935,117871,1.3732619285583496,0.00025329226649547766
59122,59123,59122,118245,1.378021001815796,0.0002495659489516071
59309,59310,59309,118619,1.3826570510864258,0.0002458722009310102
59497,59498,59497,118995,1.3869149684906006,0.000242252204687684
59684,59685,59684,119369,1.3911631107330322,0.00023870246703198235
59871,59872,59871,119743,1.395353078842163,0.00023516884179414693
60058,60059,60058,120117,1.3995487689971924,0.0002317112994218359
60245,60246,60245,120491,1.4037489891052246,0.00022832497889522426
60432,60433,60432,120865,1.4079179763793945,0.00022495266019544874
60619,60620,60619,121239,1.4121339321136475,0.00022163194636826454
60806,60807,60806,121613,1.4163179397583008,0.00021839360806899595
60993,60994,60993,121987,1.4205899238586426,0.00021518054373622728
61180,61181,61180,122361,1.4248619079589844,0.00021199577871741196
61368,61369,61368,122737,1.4290738105773926,0.00020887466895676683
61555,61556,61555,123111,1.4332630634307861,0.0002058138862443919
61742,61743,61742,123485,1.4374630451202393,0.00020276708749805613
61929,61930,61929,123859,1.441673994064331,0.0001997860762235303
62116,62117,62116,124233,1.4458868503570557,0.0001968662709630241
62303,62304,62303,124607,1.4503059387207031,0.0001939584799075556
62490,62491,62490,124981,1.455348014831543,0.00019109541606215883
62677,62678,62677,125355,1.4603707790374756,0.00018830329328464444
62864,62865,62864,125729,1.4649288654327393,0.00018553278807336893
63051,63052,63051,126103,1.4702248573303223,0.00018278687126873117
63238,63239,63238,126477,1.4745798110961914,0.00018011005080662335
63426,63427,63426,126853,1.478874921798706,0.00017745671489949457
63613,63614,63613,127227,1.4830987453460693,0.0001748296736363167
63800,63801,63800,127601,1.4871888160705566,0.0001722595161527084
63987,63988,63987,127975,1.4914588928222656,0.0001697419559785232
64174,64175,64174,128349,1.4958388805389404,0.00016723470574940287
64361,64362,64361,128723,1.5002799034118652,0.00016476622054296258
64548,64549,64548,129097,1.504655122756958,0.00016235882771367755
64735,64736,64735,129471,1.509063959121704,0.00015996992474213797
64922,64923,64922,129845,1.5136330127716064,0.0001576023853835781
65109,65110,65109,130219,1.5181629657745361,0.00015529446793741982
65297,65298,65297,130595,1.5227818489074707,0.00015300661261933711
65484,65485,65484,130969,1.5273818969726562,0.00015074149965272035
65671,65672,65671,131343,1.5320518016815186,0.00014852557054781485
65858,65859,65858,131717,1.536651849746704,0.00014635483968029696
66045,66046,66045,132091,1.5413219928741455,0.00014419295730973454
66232,66233,66232,132465,1.5459251403808594,0.00014206467154727874
66419,66420,66419,132839,1.5504088401794434,0.0001399889955190116
66606,66607,66606,133213,1.5550358295440674,0.0001379291339367109
66793,66794,66793,133587,1.5596368312835693,0.00013588783366829993
66980,66981,66980,133961,1.5641188621520996,0.00013389797881273058
67167,67168,67167,134335,1.5686378479003906,0.00013193574579950792
67355,67356,67355,134711,1.5733838081359863,0.0001299722140660792
67542,67543,67542,135085,1.5780677795410156,0.00012806169225653484
67729,67730,67729,135459,1.5828311443328857,0.00012619000944248462
67916,67917,67916,135833,1.5875840187072754,0.00012432592176112224
68103,68104,68103,136207,1.5922138690948486,0.00012249095050165837
68290,68291,68290,136581,1.5968308448791504,0.00012070128307671834
68477,68478,68477,136955,1.6014587879180908,0.00011892514161804504
68664,68665,68664,137329,1.6060898303985596,0.00011716512636873013
68851,68852,68851,137703,1.6106958389282227,0.00011544950032027693
69038,69039,69038,138077,1.6153180599212646,0.0001137575522005755
69226,69227,69226,138453,1.6200129985809326,0.00011206453767014268
69413,69414,69413,138827,1.6248259544372559,0.00011041733077986666
69600,69601,69600,139201,1.6293590068817139,0.0001088034974836542
69787,69788,69787,139575,1.6337499618530273,0.00010719618429535866
69974,69975,69974,139949,1.6380369663238525,0.00010561410404233692
70161,70162,70161,140323,1.6422998905181885,0.00010407103537283537
70348,70349,70348,140697,1.6469669342041016,0.00010253953519663282
70535,70536,70535,141071,1.6512689590454102,0.00010102204525180316
70722,70723,70722,141445,1.655526876449585,9.954285523125846e-05
70909,70910,70909,141819,1.6597659587860107,9.808396173392452e-05
71097,71098,71097,142195,1.6641230583190918,9.662419557322136e-05
71284,71285,71284,142569,1.6684401035308838,9.520401255759551e-05
71471,71472,71471,142943,1.6726980209350586,9.381250606206607e-05
71658,71659,71658,143317,1.6769719123840332,9.2426597511268e-05
71845,71846,71845,143691,1.6813280582427979,9.106255573681657e-05
72032,72033,72032,144065,1.6855731010437012,8.973210643316464e-05
72219,72220,72219,144439,1.6898798942565918,8.841155130848753e-05
72406,72407,72406,144813,1.6941397190093994,8.71031677827014e-05
72593,72594,72593,145187,1.698429822921753,8.582782946020835e-05
72780,72781,72780,145561,1.702692985534668,8.456988862220622e-05
72967,72968,72967,145935,1.7069408893585205,8.331787692839103e-05
73155,73156,73155,146311,1.7112419605255127,8.208678799428864e-05
73342,73343,73342,146685,1.7157728672027588,8.088697944669624e-05
73529,73530,73529,147059,1.7201499938964844,7.969197771693438e-05
73716,73717,73716,147433,1.7244799137115479,7.851592510472913e-05
73903,73904,73903,147807,1.7289578914642334,7.736879793838217e-05
74090,74091,74090,148181,1.7332987785339355,7.623013285887106e-05
74277,74278,74277,148555,1.7377588748931885,7.510204177545216e-05
74464,74465,74464,148929,1.7421259880065918,7.400246145689928e-05
74651,74652,74651,149303,1.7464938163757324,7.291779321502103e-05
74838,74839,74838,149677,1.7508888244628906,7.18382729606123e-05
75026,75027,75026,150053,1.7552800178527832,7.077685691626391e-05
75213,75214,75213,150427,1.759645938873291,6.974233710509548e-05
75400,75401,75400,150801,1.763988971710205,6.871194532311312e-05
75587,75588,75587,151175,1.7681231498718262,6.769797381806686e-05
75774,75775,75774,151549,1.7724449634552002,6.670890853821944e-05
75961,75962,75961,151923,1.7765769958496094,6.572708045283697e-05
76148,76149,76148,152297,1.781285047531128,6.475443822548944e-05
76335,76336,76335,152671,1.7856769561767578,6.380639396660755e-05
76522,76523,76522,153045,1.7900640964508057,6.287113105570844e-05
76709,76710,76709,153419,1.7952229976654053,6.19403381817766e-05
76896,76897,76896,153793,1.8000550270080566,6.1030012126714567e-05
77084,77085,77084,154169,1.8050339221954346,6.0133208114522104e-05
77271,77272,77271,154543,1.8108007907867432,5.924475169351271e-05
77458,77459,77458,154917,1.8152050971984863,5.837052377656789e-05
77645,77646,77645,155291,1.8196039199829102,5.7517740831695094e-05
77832,77833,77832,155665,1.823970079421997,5.66711474266643e-05
78019,78020,78019,156039,1.8283770084381104,5.583253377145629e-05
78206,78207,78206,156413,1.8326399326324463,5.5015141785822924e-05
78393,78394,78393,156787,1.8368780612945557,5.420870453937612e-05
78580,78581,78580,157161,1.8413569927215576,5.3406148904075597e-05
78767,78768,78767,157535,1.8457419872283936,5.2621287127714355e-05
78955,78956,78955,157911,1.8501529693603516,5.1848028848533055e-05
79142,79143,79142,158285,1.8556420803070068,5.1081956537370607e-05
79329,79330,79329,158659,1.8599579334259033,5.032821315381988e-05
79516,79517,79516,159033,1.8643889427185059,4.959293406723678e-05
79703,79704,79703,159407,1.868685007095337,4.88629484713675e-05
79890,79891,79890,159781,1.8729829788208008,4.8139894701805306e-05
80077,80078,80077,160155,1.877267837524414,4.743514930706661e-05
80264,80265,80264,160529,1.8815300464630127,4.673979280293506e-05
80451,80452,80451,160903,1.8858098983764648,4.60478071478506e-05
80638,80639,80638,161277,1.8900859355926514,4.5371117702325076e-05
80826,80827,80826,161653,1.8943758010864258,4.470438499575263e-05
81013,81014,81013,162027,1.89864182472229,4.4043838655355135e-05
81200,81201,81200,162401,1.9028759002685547,4.3393974957106844e-05
81387,81388,81387,162775,1.9071249961853027,4.276000879336506e-05
81574,81575,81574,163149,1.9114348888397217,4.2130569748937e-05
81761,81762,81761,163523,1.915815830230713,4.15071520675612e-05
81948,81949,81948,163897,1.9202649593353271,4.089952903545527e-05
82135,82136,82135,164271,1.9247548580169678,4.029995262096377e-05
82322,82323,82322,164645,1.9292950630187988,3.970330367396945e-05
82509,82510,82509,165019,1.9337809085845947,3.911987785349092e-05
82696,82697,82696,165393,1.9383549690246582,3.8548045155331694e-05
82884,82885,82884,165769,1.9429340362548828,3.7975438997331076e-05
83071,83072,83071,166143,1.947551965713501,3.7415138553727336e-05
83258,83259,83258,166517,1.9521708488464355,3.686852536875304e-05
83445,83446,83445,166891,1.9568419456481934,3.632578385126334e-05
83632,83633,83632,167265,1.9614441394805908,3.578827268195361e-05
83819,83820,83819,167639,1.9660170078277588,3.5264387253500066e-05
84006,84007,84006,168013,1.9706017971038818,3.47473978575505e-05
84193,84194,84193,168387,1.9752271175384521,3.423295101139973e-05
84380,84381,84380,168761,1.9798851013183594,3.3729934884656196e-05
84567,84568,84567,169135,1.9845008850097656,3.323687874229609e-05
84755,84756,84755,169511,1.9891250133514404,3.274314891103856e-05
84942,84943,84942,169885,1.9937548637390137,3.226006833030532e-05
85129,85130,85129,170259,1.9983890056610107,3.178877175301586e-05
85316,85317,85316,170633,2.0029828548431396,3.132078626451701e-05
85503,85504,85503,171007,2.0075879096984863,3.0857343903627296e-05
85690,85691,85690,171381,2.0121960639953613,3.0405655935950376e-05
85877,85878,85877,171755,2.0167810916900635,2.995987775869952e-05
86064,86065,86064,172129,2.0214130878448486,2.9516307945188924e-05
86251,86252,86251,172503,2.026047945022583,2.908261915838893e-05
86438,86439,86438,172877,2.0306930541992188,2.8657487050586945e-05
86625,86626,86625,173251,2.0353541374206543,2.8234023021484022e-05
86813,86814,86813,173627,2.0400187969207764,2.781526547945966e-05
87000,87001,87000,174001,2.0445938110351562,2.7408907654411187e-05
87187,87188,87187,174375,2.049191951751709,2.7005381486189263e-05
87374,87375,87374,174749,2.0537641048431396,2.6605801414724863e-05
87561,87562,87561,175123,2.0583698749542236,2.6216361163541413e-05
87748,87749,87748,175497,2.06292986869812,2.583198535564269e-05
87935,87936,87935,175871,2.0675110816955566,2.5449527751036882e-05
88122,88123,88122,176245,2.072122097015381,2.5075611362282623e-05
88309,88310,88309,176619,2.0767059326171875,2.4709045867219785e-05
88496,88497,88496,176993,2.0813066959381104,2.4343913983341793e-05
88684,88685,88684,177369,2.085984945297241,2.3982869103083224e-05
88871,88872,88871,177743,2.0905709266662598,2.3632502157121766e-05
89058,89059,89058,178117,2.096385955810547,2.3284556841200038e-05
89245,89246,89245,178491,2.101010799407959,2.2940038957551036e-05
89432,89433,89432,178865,2.105602979660034,2.2604267895293994e-05
89619,89620,89619,179239,2.110128879547119,2.2272836717731775e-05
89806,89807,89806,179613,2.1146140098571777,2.1943071792321257e-05
89993,89994,89993,179987,2.1192398071289062,2.162068975784501e-05
90180,90181,90180,180361,2.1239097118377686,2.1304622577706515e-05
90367,90368,90367,180735,2.1287119388580322,2.0989787671283153e-05
90555,90556,90555,181111,2.1334378719329834,2.0678501615143676e-05
90742,90743,90742,181485,2.1381239891052246,2.0376410614917033e-05
90929,90930,90929,181859,2.1428170204162598,2.0076390579461483e-05
91116,91117,91116,182233,2.147420883178711,1.977934740339064e-05
91303,91304,91303,182607,2.152007818222046,1.9489849244247373e-05
91490,91491,91490,182981,2.15659499168396,1.9204069959641847e-05
91677,91678,91677,183355,2.161273956298828,1.8919738139852057e-05
91864,91865,91864,183729,2.165937900543213,1.864178781386721e-05
92051,92052,92051,184103,2.170624017715454,1.8369262176542764e-05
92238,92239,92238,184477,2.1755146980285645,1.8097795901634047e-05
92425,92426,92425,184851,2.18044376373291,1.7830818527634836e-05
92613,92614,92613,185227,2.185357093811035,1.7568944066439988e-05
92800,92801,92800,185601,2.19018292427063,1.731024819765097e-05
92987,92988,92987,185975,2.1949408054351807,1.7054137777743343e-05
93174,93175,93174,186349,2.19973087310791,1.680453554661835e-05
93361,93362,93361,186723,2.204525947570801,1.6558119946092687e-05
93548,93549,93548,187097,2.2093417644500732,1.6312961809951906e-05
93735,93736,93735,187471,2.214207887649536,1.607331945990642e-05
93922,93923,93922,187845,2.2190468311309814,1.583833698793168e-05
94109,94110,94109,188219,2.223914861679077,1.5604265360299654e-05
94296,94297,94296,188593,2.228778839111328,1.537408259337598e-05
94484,94485,94484,188969,2.2337751388549805,1.5148290869013636e-05
94671,94672,94671,189343,2.238529920578003,1.4925227273039049e-05
94858,94859,94858,189717,2.2434568405151367,1.4704409118360275e-05
95045,95046,95045,190091,2.2484798431396484,1.448920467445467e-05
95232,95233,95232,190465,2.2533249855041504,1.427673070911412e-05
95419,95420,95419,190839,2.2581801414489746,1.406534919725595e-05
95606,95607,95606,191213,2.2630269527435303,1.3858735086117635e-05
95793,95794,95793,191587,2.2680089473724365,1.3656123762341962e-05
95980,95981,95980,191961,2.2728869915008545,1.3454295699760046e-05
96167,96168,96167,192335,2.277643918991089,1.3255836568926479e-05
96354,96355,96354,192709,2.2823989391326904,1.30621850642697e-05
96542,96543,96542,193085,2.287161111831665,1.286881656946261e-05
96729,96730,96729,193459,2.2918479442596436,1.2678427432734e-05
96916,96917,96916,193833,2.296588897705078,1.2492880352964783e-05
97103,97104,97103,194207,2.3012988567352295,1.2309672825115145e-05
97290,97291,97290,194581,2.306051015853882,1.212741443448513e-05
97477,97478,97477,194955,2.3106539249420166,1.1949276498073185e-05
97664,97665,97664,195329,2.315268039703369,1.1774576821532299e-05
97851,97852,97851,195703,2.319905996322632,1.1600550792092263e-05
98038,98039,98038,196077,2.3245999813079834,1.1429443194230766e-05
98225,98226,98225,196451,2.3294661045074463,1.1262474152521028e-05
98413,98414,98413,196827,2.3341469764709473,1.1095739892655744e-05
98600,98601,98600,197201,2.338757038116455,1.0931586669747066e-05
98787,98788,98787,197575,2.343461036682129,1.077160982410564e-05
98974,98975,98974,197949,2.3477649688720703,1.0613637512732415e-05
99161,99162,99161,198323,2.3520350456237793,1.0456489857724152e-05
99348,99349,99348,198697,2.356292963027954,1.0302903413991403e-05
99535,99536,99535,199071,2.3606667518615723,1.0152270239699417e-05
99722,99723,99722,199445,2.364922046661377,1.000221652378774e-05
99909,99910,99909,199819,2.3695411682128906,9.854690908197945e-06
100096,100097,100096,200193,2.37441086769104,9.710727807113096e-06
100284,100285,100284,200569,2.3807249069213867,9.566959240369153e-06
100471,100472,100471,200943,2.384960889816284,9.425426627462641e-06
100658,100659,100658,201317,2.3892128467559814,9.287496145729321e-06
100845,100846,100845,201691,2.393415927886963,9.151283102412643e-06
101032,101033,101032,202065,2.397825002670288,9.015786588836505e-06
101219,101220,101219,202439,2.40207576751709,8.883367869682578e-06
101406,101407,101406,202813,2.406338930130005,8.753485771720813e-06
101593,101594,101593,203187,2.410590887069702,8.624102186796792e-06
101780,101781,101780,203561,2.414923906326294,8.49690851360755e-06
101967,101968,101967,203935,2.419221878051758,8.372781418570123e-06
102154,102155,102154,204309,2.423419952392578,8.249473638654357e-06
102342,102343,102342,204685,2.4276390075683594,8.126786173950723e-06
102529,102530,102529,205059,2.4319698810577393,8.007863820417279e-06
102716,102717,102716,205433,2.436149835586548,7.890412883788656e-06
102903,102904,102903,205807,2.4403529167175293,7.77358455114003e-06
103090,103091,103090,206181,2.444559097290039,7.659416151621105e-06
103277,103278,103277,206555,2.448909044265747,7.547426446474483e-06
103464,103465,103464,206929,2.453096866607666,7.43586568047614e-06
103651,103652,103651,207303,2.4572908878326416,7.326201823287667e-06
103838,103839,103838,207677,2.461587905883789,7.219177583850997e-06
104025,104026,104025,208051,2.4658169746398926,7.112854009624092e-06
104213,104214,104213,208427,2.470461845397949,7.0070731382570245e-06
104400,104401,104400,208801,2.474655866622925,6.904539384375117e-06
104587,104588,104587,209175,2.4790759086608887,6.803266230271338e-06
104774,104775,104774,209549,2.4832959175109863,6.702534086080709e-06
104961,104962,104961,209923,2.487504005432129,6.604100688455176e-06
105148,105149,105148,210297,2.491933822631836,6.507538511957495e-06
105335,105336,105335,210671,2.4961321353912354,6.411345466304902e-06
105522,105523,105522,211045,2.5004000663757324,6.316795482318134e-06
105709,105710,105709,211419,2.504795789718628,6.2245175469782834e-06
105896,105897,105896,211793,2.5090909004211426,6.132838809970146e-06
106083,106084,106083,212167,2.5133790969848633,6.04211387141789e-06
106271,106272,106271,212543,2.5179738998413086,5.953231116997114e-06
106458,106459,106458,212917,2.5222740173339844,5.865907392650114e-06
106645,106646,106645,213291,2.526664972305298,5.77905379344793e-06
106832,106833,106832,213665,2.5310728549957275,5.694186749834369e-06
107019,107020,107019,214039,2.5353899002075195,5.610926803063698e-06
107206,107207,107206,214413,2.5396950244903564,5.527984566202865e-06
107393,107394,107393,214787,2.5439929962158203,5.44646547336183e-06
107580,107581,107580,215161,2.548314094543457,5.366901997486145e-06
107767,107768,107767,215535,2.5526130199432373,5.2878509480087e-06
107954,107955,107954,215909,2.556920051574707,5.209628134618074e-06
108142,108143,108142,216285,2.5613629817962646,5.132994213249259e-06
108329,108330,108329,216659,2.565703868865967,5.057698504554659e-06
108516,108517,108516,217033,2.570056915283203,4.982811337183524e-06
108703,108704,108703,217407,2.574458122253418,4.90964089049972e-06
108890,108891,108890,217781,2.578878879547119,4.837850659778172e-06
109077,109078,109077,218155,2.5833189487457275,4.7663339228397066e-06
109264,109265,109264,218529,2.5876519680023193,4.6960498122217484e-06
109451,109452,109451,218903,2.591982126235962,4.627448916350649e-06
109638,109639,109638,219277,2.5963470935821533,4.559286242113124e-06
109825,109826,109825,219651,2.6006689071655273,4.49184275074982e-06
110013,110014,110013,220027,2.6050219535827637,4.425769646000788e-06
110200,110201,110200,220401,2.609369993209839,4.360845198767912e-06
110387,110388,110387,220775,2.6137619018554688,4.296275787205467e-06
110574,110575,110574,221149,2.6182310581207275,4.233189876717868e-06
110761,110762,110761,221523,2.622499942779541,4.1712892984581035e-06
110948,110949,110948,221897,2.6274538040161133,4.109624187575069e-06
111135,111136,111135,222271,2.6316709518432617,4.049026659711502e-06
111322,111323,111322,222645,2.6358609199523926,3.989877853042037e-06
111509,111510,111509,223019,2.640145778656006,3.93110381039468e-06
111696,111697,111696,223393,2.6443488597869873,3.872954238580637e-06
111883,111884,111883,223767,2.6485979557037354,3.816286596150296e-06
112071,112072,112071,224143,2.6529409885406494,3.7600048274759726e-06
112258,112259,112258,224517,2.6572060585021973,3.7043316389209912e-06
112445,112446,112445,224891,2.6614980697631836,3.649940383554433e-06
112632,112633,112632,225265,2.665876865386963,3.596567065886293e-06
112819,112820,112819,225639,2.672712802886963,3.5433965075921052e-06
113006,113007,113006,226013,2.677194833755493,3.4911505612866426e-06
113193,113194,113193,226387,2.68174409866333,3.440151480602137e-06
113380,113381,113380,226761,2.685980796813965,3.3894728971254445e-06
113567,113568,113567,227135,2.69018292427063,3.3393365299366484e-06
113754,113755,113754,227509,2.694535970687866,3.2904781629288617e-06
113942,113943,113942,227885,2.6987509727478027,3.2419486631262925e-06
114129,114130,114129,228259,2.7029848098754883,3.1939460142228856e-06
114316,114317,114316,228633,2.707180976867676,3.147051091054929e-06
114503,114504,114503,229007,2.711411952972412,3.101030326676597e-06
114690,114691,114690,229381,2.7156431674957275,3.0551841840397837e-06
114877,114878,114877,229755,2.719953775405884,3.0101388063667154e-06
115064,115065,115064,230129,2.7245497703552246,2.9661665381162595e-06
115251,115252,115251,230503,2.7288928031921387,2.9224683600527273e-06
115438,115439,115438,230877,2.7331130504608154,2.879240964603016e-06
115625,115626,115625,231251,2.7373178005218506,2.8371156775275918e-06
115812,115813,115812,231625,2.741569995880127,2.795493077687302e-06
116000,116001,116000,232001,2.7457950115203857,2.7538817154258452e-06
116187,116188,116187,232375,2.7501261234283447,2.7134499584416734e-06
116374,116375,116374,232749,2.7543418407440186,2.6737688686372147e-06
116561,116562,116561,233123,2.758549928665161,2.6342381910902593e-06
116748,116749,116748,233497,2.7627508640289307,2.595401000450072e-06
116935,116936,116935,233871,2.766939878463745,2.557487354452493e-06
117122,117123,117122,234245,2.7711710929870605,2.519808112964479e-06
117309,117310,117309,234619,2.7754039764404297,2.4825376196038046e-06
117496,117497,117496,234993,2.77962589263916,2.4462175289935667e-06
117683,117684,117683,235367,2.7838330268859863,2.410328030316202e-06
117871,117872,117871,235743,2.788058042526245,2.3744498149535475e-06
118058,118059,118058,236117,2.792595863342285,2.3395904523992656e-06
118245,118246,118245,236491,2.7968029975891113,2.3053756931419308e-06
118432,118433,118432,236865,2.801146984100342,2.2712905132322475e-06
118619,118620,118619,237239,2.805371046066284,2.23780589717731e-06
118806,118807,118806,237613,2.809678077697754,2.205116087407198e-06
118993,118994,118993,237987,2.813865900039673,2.1726267443665452e-06
119180,119181,119180,238361,2.818150758743286,2.1404922788546726e-06
119367,119368,119367,238735,2.8223800659179688,2.10917737385887e-06
119554,119555,119554,239109,2.826676845550537,2.0782312943984545e-06
119742,119743,119742,239485,2.831016778945923,2.047296333414855e-06
119929,119930,119929,239859,2.835218906402588,2.0172413626205756e-06
120116,120117,120116,240233,2.8394081592559814,1.9877399019095828e-06
120303,120304,120303,240607,2.843596935272217,1.958350090568844e-06
120490,120491,120490,240981,2.84771990776062,1.929480356479852e-06
120677,120678,120677,241355,2.851987838745117,1.901294619387699e-06
120864,120865,120864,241729,2.856260061264038,1.873280326547717e-06
121051,121052,121051,242103,2.8605589866638184,1.8455741315079568e-06
121238,121239,121238,242477,2.8647959232330322,1.8185746515947813e-06
121425,121426,121425,242851,2.8691439628601074,1.79189108145171e-06
121612,121613,121612,243225,2.8733949661254883,1.7653588640214491e-06
121800,121801,121800,243601,2.8776707649230957,1.7393055761729427e-06
121987,121988,121987,243975,2.881967067718506,1.7138681196715793e-06
122174,122175,122174,244349,2.8861899375915527,1.6885268786295739e-06
122361,122362,122361,244723,2.8904287815093994,1.663636002211831e-06
122548,122549,122548,245097,2.894728899002075,1.6393337478974113e-06
122735,122736,122735,245471,2.8989810943603516,1.6151781187238822e-06
122922,122923,122922,245845,2.9031779766082764,1.5912899662961534e-06
123109,123110,123109,246219,2.9073619842529297,1.5680112072536522e-06
123296,123297,123296,246593,2.9115538597106934,1.5450030260410855e-06
123483,123484,123483,246967,2.9158599376678467,1.5221263943804544e-06
123671,123672,123671,247343,2.920197010040283,1.4996638215014759e-06
123858,123859,123858,247717,2.924506902694702,1.4777305214578356e-06
124045,124046,124045,248091,2.9287350177764893,1.455880149434388e-06
124232,124233,124232,248465,2.932987928390503,1.4344197629803027e-06
124419,124420,124419,248839,2.9371750354766846,1.4134659102745938e-06
124606,124607,124606,249213,2.9413628578186035,1.392637458113192e-06
124793,124794,124793,249587,2.9455437660217285,1.3720412105127755e-06
124980,124981,124980,249961,2.9498491287231445,1.3519704245977615e-06
125167,125168,125167,250335,2.95413875579834,1.3321313826633946e-06
125354,125355,125354,250709,2.958393096923828,1.3124066805218723e-06
125541,125542,125541,251083,2.962583065032959,1.2931416288618973e-06
125729,125730,125729,251459,2.9667770862579346,1.2741280741637569e-06
125916,125917,125916,251833,2.971031904220581,1.2552876939649742e-06
126103,126104,126103,252207,2.9753201007843018,1.2367850055225978e-06
126290,126291,126290,252581,2.9795780181884766,1.2187181998561315e-06
126477,126478,126477,252955,2.983773946762085,1.2007586439607143e-06
126664,126665,126664,253329,2.9880030155181885,1.1830006658761244e-06
126851,126852,126851,253703,2.994776964187622,1.1656957672508904e-06
127038,127039,127038,254077,2.99908709526062,1.1485893463400676e-06
127225,127226,127225,254451,3.003325939178467,1.1315823088694163e-06
127412,127413,127412,254825,3.0075669288635254,1.1149724032840394e-06
127600,127601,127600,255201,3.011868953704834,1.098578069764594e-06
127787,127788,127787,255575,3.0161259174346924,1.0823330455517874e-06
127974,127975,127974,255949,3.0204269886016846,1.0663804233047136e-06
128161,128162,128161,256323,3.0247089862823486,1.0508028780979598e-06
128348,128349,128348,256697,3.0290307998657227,1.0353170604498794e-06
128535,128536,128535,257071,3.0333690643310547,1.0200062282335457e-06
128722,128723,128722,257445,3.0375900268554688,1.0050860548689547e-06
128909,128910,128909,257819,3.0418028831481934,9.903358632537747e-07
129096,129097,129096,258193,3.0461349487304688,9.756720566452594e-07
129283,129284,129283,258567,3.050410032272339,9.613513583083727e-07
129470,129471,129470,258941,3.054630756378174,9.47290479189078e-07
129658,129659,129658,259317,3.059141159057617,9.332082424235542e-07
129845,129846,129845,259691,3.063509941101074,9.194542343457325e-07
130032,130033,130032,260065,3.067949056625366,9.06022972105764e-07
130219,130220,130219,260439,3.0723209381103516,8.926701630234539e-07
130406,130407,130406,260813,3.0765650272369385,8.794692506169869e-07
130593,130594,130593,261187,3.080641984939575,8.666051683583116e-07
130780,130781,130780,261561,3.0849769115448,8.538866588057278e-07
130967,130968,130967,261935,3.089171886444092,8.412432371426228e-07
131154,131155,131154,262309,3.0933339595794678,8.288962420503812e-07
131341,131342,131341,262683,3.097531795501709,8.167723206030318e-07
131529,131530,131529,263059,3.1015820503234863,8.046299872612863e-07
131716,131717,131716,263433,3.1079139709472656,7.927715784358725e-07
131903,131904,131903,263807,3.1119189262390137,7.811908787780524e-07
132090,132091,132090,264181,3.1165449619293213,7.69677280117116e-07
132277,132278,132277,264555,3.1206777095794678,7.582955319415095e-07
132464,132465,132464,264929,3.124884843826294,7.47204195567279e-07
132651,132652,132651,265303,3.1290407180786133,7.362375242770884e-07
132838,132839,132838,265677,3.1331467628479004,7.253361221494412e-07
133025,133026,133025,266051,3.1372647285461426,7.146908099303408e-07
133212,133213,133212,266425,3.141300916671753,7.042370171965073e-07
133400,133401,133400,266801,3.145404815673828,6.937673583062973e-07
133587,133588,133587,267175,3.1496188640594482,6.835432953716374e-07
133774,133775,133774,267549,3.153864860534668,6.735581836327191e-07
133961,133962,133961,267923,3.1580867767333984,6.636304644856688e-07
134148,134149,134148,268297,3.162320852279663,6.538171917850861e-07
134335,134336,134335,268671,3.1665499210357666,6.442543036594645e-07
134522,134523,134522,269045,3.170761823654175,6.347981726575333e-07
134709,134710,134709,269419,3.174992084503174,6.253987768253924e-07
134896,134897,134896,269793,3.179297924041748,6.162206177136652e-07
135083,135084,135083,270167,3.183521032333374,6.072068827753552e-07
135270,135271,135270,270541,3.1877219676971436,5.982272346425786e-07
135458,135459,135458,270917,3.191939115524292,5.893645163812807e-07
135645,135646,135645,271291,3.196131944656372,5.807551494252696e-07
135832,135833,135832,271665,3.2003538608551025,5.721948722750327e-07
136019,136020,136019,272039,3.2045629024505615,5.637339318953521e-07
136206,136207,136206,272413,3.2087841033935547,5.554888607671313e-07
136393,136394,136393,272787,3.213050127029419,5.473352086048563e-07
136580,136581,136580,273161,3.217249870300293,5.392308740514155e-07
136767,136768,136767,273535,3.22149395942688,5.313176618707041e-07
136954,136955,136954,273909,3.2257609367370605,5.235456078549778e-07
137141,137142,137141,274283,3.2299749851226807,5.158029592503749e-07
137329,137330,137329,274659,3.234251022338867,5.081617162313897e-07
137516,137517,137516,275033,3.23848295211792,5.007385416909947e-07
137703,137704,137703,275407,3.242722988128662,4.93357356254999e-07
137890,137891,137890,275781,3.2469868659973145,4.86062390195687e-07
138077,138078,138077,276155,3.2510199546813965,4.789535317215973e-07
138264,138265,138264,276529,3.255103826522827,4.7192295543679184e-07
138451,138452,138451,276903,3.259168863296509,4.649352494608263e-07
138638,138639,138638,277277,3.263301134109497,4.581126466015908e-07
138825,138826,138825,277651,3.26743483543396,4.5141122464696227e-07
139012,139013,139012,278025,3.2720067501068115,4.447351736329414e-07
139199,139200,139199,278399,3.2762291431427,4.381816094722867e-07
139387,139388,139387,278775,3.2805349826812744,4.317466434791634e-07
139574,139575,139574,279149,3.284637928009033,4.2538214261452717e-07
139761,139762,139761,279523,3.288749933242798,4.1909247364539517e-07
139948,139949,139948,279897,3.2929489612579346,4.1296325005862696e-07
140135,140136,140135,280271,3.2971549034118652,4.069010577082447e-07
140322,140323,140322,280645,3.3013110160827637,4.008761315761181e-07
140509,140510,140509,281019,3.3054099082946777,3.949938281229224e-07
140696,140697,140696,281393,3.309525966644287,3.892155526202006e-07
140883,140884,140883,281767,3.313713788986206,3.83459170499355e-07
141070,141071,141070,282141,3.3178930282592773,3.778088312002454e-07
141258,141259,141258,282517,3.3231868743896484,3.7226046755732563e-07
141445,141446,141445,282891,3.328665018081665,3.6677261380915337e-07
141632,141633,141632,283265,3.332894802093506,3.61349706537982e-07
141819,141820,141819,283639,3.3370108604431152,3.560651178280321e-07
142006,142007,142006,284013,3.34114408493042,3.5083792472940603e-07
142193,142194,142193,284387,3.3453550338745117,3.4564312666207645e-07
142380,142381,142380,284761,3.3496408462524414,3.4057152876186667e-07
142567,142568,142567,285135,3.3563408851623535,3.355892313149198e-07
142754,142755,142754,285509,3.3606679439544678,3.3062582931825516e-07
142941,142942,142941,285883,3.3651559352874756,3.2575423118729027e-07
143129,143130,143129,286259,3.3695499897003174,3.2097031303285606e-07
143316,143317,143316,286633,3.3747549057006836,3.162383575640425e-07
143503,143504,143503,287007,3.3793249130249023,3.1156276731591115e-07
143690,143691,143690,287381,3.3835787773132324,3.0700641752440606e-07
143877,143878,143877,287755,3.3878419399261475,3.024992114149619e-07
144064,144065,144064,288129,3.392096996307373,2.980201661029779e-07
144251,144252,144251,288503,3.3963420391082764,2.9364754085296806e-07
144438,144439,144438,288877,3.4018709659576416,2.893515713745136e-07
144625,144626,144625,289251,3.4067671298980713,2.850719125142022e-07
144812,144813,144812,289625,3.411733865737915,2.80871728298538e-07
144999,145000,144999,289999,3.4160261154174805,2.7676876323734215e-07
145187,145188,145187,290375,3.420341968536377,2.726667556524391e-07
145374,145375,145374,290749,3.4245359897613525,2.686354977295241e-07
145561,145562,145561,291123,3.4287519454956055,2.6470703124672494e-07
145748,145749,145748,291497,3.4329400062561035,2.608206417130705e-07
145935,145936,145935,291871,3.43715500831604,2.569587322848775e-07
146122,146123,146122,292245,3.4414899349212646,2.5318874611171026e-07
146309,146310,146309,292619,3.4458837509155273,2.494845596386039e-07
146496,146497,146496,292993,3.4503448009490967,2.4579445466600897e-07
146683,146684,146683,293367,3.4548768997192383,2.421731490306202e-07
146870,146871,146870,293741,3.459526777267456,2.38635482836412e-07
147058,147059,147058,294117,3.464223861694336,2.3509848766170576e-07
147245,147246,147245,294491,3.4689650535583496,2.3162276910827044e-07
147432,147433,147432,294865,3.4734349250793457,2.282356600443629e-07
147619,147620,147619,295239,3.4778218269348145,2.248845763107955e-07
147806,147807,147806,295613,3.4821810722351074,2.2155477321519806e-07
147993,147994,147993,295987,3.4865567684173584,2.1830436941342144e-07
148180,148181,148180,296361,3.4909067153930664,2.151104450760749e-07
148367,148368,148367,296735,3.495234966278076,2.1192867965992553e-07
148554,148555,148554,297109,3.499569892883301,2.088064705705582e-07
148741,148742,148741,297483,3.5038809776306152,2.0575621626023136e-07
148928,148929,148928,297857,3.5082128047943115,2.0272259413616273e-07
149116,149117,149116,298233,3.512572765350342,1.9970967272078383e-07
149303,149304,149303,298607,3.516890048980713,1.967893190281721e-07
149490,149491,149490,298981,3.521223783493042,1.9389980855876418e-07
149677,149678,149677,299355,3.5255749225616455,1.910287975334697e-07
149864,149865,149864,299729,3.5299198627471924,1.882263665013078e-07
150051,150052,150051,300103,3.5342750549316406,1.8547241347129842e-07
150238,150239,150238,300477,3.538609743118286,1.8272896092451056e-07
150425,150426,150425,300851,3.542937994003296,1.8003706203624282e-07
150612,150613,150612,301225,3.5471527576446533,1.7740706410564331e-07
150799,150800,150799,301599,3.5512819290161133,1.7479129477704622e-07
150987,150988,150987,301975,3.555433988571167,1.721935786827809e-07
151174,151175,151174,302349,3.5596299171447754,1.6967565909745948e-07
151361,151362,151361,302723,3.5638070106506348,1.671841452918875e-07
151548,151549,151548,303097,3.5685079097747803,1.647087132027681e-07
151735,151736,151735,303471,3.572643995285034,1.6229251472821105e-07
151922,151923,151922,303845,3.5768849849700928,1.5991792516151995e-07
152109,152110,152109,304219,3.58111572265625,1.5755240515411496e-07
152296,152297,152296,304593,3.5852599143981934,1.5523151029432017e-07
152483,152484,152483,304967,3.589366912841797,1.5296386603236943e-07
152670,152671,152670,305341,3.593491792678833,1.5070839451582388e-07
152858,152859,152858,305717,3.5977869033813477,1.4846866568253455e-07
153045,153046,153045,306091,3.6019198894500732,1.462977228006504e-07
153232,153233,153232,306465,3.606074094772339,1.4414938602741438e-07
153419,153420,153419,306839,3.6102120876312256,1.4201502931394068e-07
153606,153607,153606,307213,3.6145458221435547,1.399318323150105e-07
153793,153794,153793,307587,3.618750810623169,1.378843474463667e-07
153980,153981,153980,307961,3.622886896133423,1.3584469746278997e-07
154167,154168,154167,308335,3.6270320415496826,1.3384367416094907e-07
154354,154355,154354,308709,3.6311590671539307,1.3188845879856913e-07
154541,154542,154541,309083,3.6352927684783936,1.2994365769627671e-07
154728,154729,154728,309457,3.6394429206848145,1.2802271924379842e-07
154916,154917,154916,309833,3.6436469554901123,1.2614080178324659e-07
155103,155104,155103,310207,3.64789080619812,1.2428837326937385e-07
155290,155291,155290,310581,3.6520819664001465,1.2244809776594425e-07
155477,155478,155477,310955,3.6562888622283936,1.206520075621557e-07
155664,155665,155664,311329,3.6605348587036133,1.188865675419135e-07
155851,155852,155851,311703,3.664747953414917,1.1712789681402072e-07
156038,156039,156038,312077,3.669055938720703,1.1540265972152531e-07
156225,156226,156225,312451,3.6732118129730225,1.1371682712764783e-07
156412,156413,156412,312825,3.677480936050415,1.1203990470649522e-07
156599,156600,156599,313199,3.6817657947540283,1.103836885341955e-07
156787,156788,156787,313575,3.6860358715057373,1.0876110407652269e-07
156974,156975,156974,313949,3.6902668476104736,1.0716382577077655e-07
157161,157162,157161,314323,3.6946921348571777,1.0557711226218684e-07
157348,157349,157348,314697,3.699476957321167,1.0402855949229468e-07
157535,157536,157535,315071,3.7049999237060547,1.0250631168836324e-07
157722,157723,157722,315445,3.7099671363830566,1.0098991339823764e-07
157909,157910,157909,315819,3.7158660888671875,9.95024530256803e-08
158096,158097,158096,316193,3.720012903213501,9.804888808419536e-08
158283,158284,158283,316567,3.7243950366973877,9.660294669638268e-08
158470,158471,158470,316941,3.728700876235962,9.517497211641233e-08
158657,158658,158657,317315,3.732923746109009,9.378335995732566e-08
158845,158846,158845,317691,3.7372357845306396,9.239871135989565e-08
159032,159033,159032,318065,3.7415030002593994,9.103062334189227e-08
159219,159220,159219,318439,3.745774984359741,8.969549218020015e-08
159406,159407,159406,318813,3.750092029571533,8.838293610725361e-08
159593,159594,159593,319187,3.7543139457702637,8.707543547338188e-08
159780,159781,159780,319561,3.758591890335083,8.579298093650123e-08
159967,159968,159967,319935,3.7627949714660645,8.453968219896845e-08
160154,160155,160154,320309,3.76713490486145,8.329290649778859e-08
160341,160342,160341,320683,3.7713749408721924,8.206172007663993e-08
160528,160529,160528,321057,3.7785818576812744,8.086187514250326e-08
160716,160717,160716,321433,3.7828400135040283,7.966794557522773e-08
160903,160904,160903,321807,3.787095069885254,7.848836014787521e-08
161090,161091,161090,322181,3.7913100719451904,7.733723662582084e-08
161277,161278,161277,322555,3.7955310344696045,7.620548665317318e-08
161464,161465,161464,322929,3.799757957458496,7.507810651337581e-08
161651,161652,161651,323303,3.8039610385894775,7.397240343949954e-08
161838,161839,161838,323677,3.8081939220428467,7.289177867035844e-08
162025,162026,162025,324051,3.812412977218628,7.181673547379847e-08
162212,162213,162212,324425,3.816619873046875,7.075521826307321e-08
162399,162400,162399,324799,3.820905923843384,6.972071427283598e-08
162587,162588,162587,325175,3.825148820877075,6.869123435472955e-08
162774,162775,162774,325549,3.8293590545654297,6.767417895524232e-08
162961,162962,162961,325923,3.833570957183838,6.668170301937797e-08
163148,163149,163148,326297,3.8377788066864014,6.570585263802409e-08
163335,163336,163335,326671,3.842000722885132,6.47337799789688e-08
163522,163523,163522,327045,3.8461339473724365,6.378046804035453e-08
163709,163710,163709,327419,3.85025691986084,6.284872662234328e-08
163896,163897,163896,327793,3.854490041732788,6.1921761421995e-08
164083,164084,164083,328167,3.8587429523468018,6.100653165535744e-08
164270,164271,164270,328541,3.863132953643799,6.011458403097023e-08
164457,164458,164457,328915,3.867577075958252,5.92316210916602e-08
164645,164646,164645,329291,3.872565984725952,5.8349983396150944e-08
164832,164833,164832,329665,3.8772029876708984,5.7494290166987614e-08
165019,165020,165019,330039,3.881387948989868,5.665286383907038e-08
165206,165207,165206,330413,3.88598895072937,5.581470385110371e-08
165393,165394,165393,330787,3.8902530670166016,5.499278014364504e-08
165580,165581,165580,331161,3.8945047855377197,5.4189409360927586e-08
165767,165768,165767,331535,3.8987720012664795,5.3390125798275786e-08
165954,165955,165954,331909,3.903061866760254,5.260102383058928e-08
166141,166142,166141,332283,3.9073410034179688,5.183198780965797e-08
166328,166329,166328,332657,3.9117469787597656,5.107064241780847e-08
166516,166517,166516,333033,3.9161620140075684,5.0310482151614676e-08
166703,166704,166703,333407,3.9210128784179688,4.957272012393854e-08
166890,166891,166890,333781,3.925797700881958,4.8847200666627454e-08
167077,167078,167077,334155,3.9304068088531494,4.8124505769294844e-08
167264,167265,167264,334529,3.9345977306365967,4.7415862018589595e-08
167451,167452,167451,334903,3.9388039112091064,4.672317533712637e-08
167638,167639,167638,335277,3.9429988861083984,4.603398647384917e-08
167825,167826,167825,335651,3.947187900543213,4.5353630821405275e-08
168012,168013,168012,336025,3.951395034790039,4.4690568823628534e-08
168199,168200,168199,336399,3.9555981159210205,4.403408958737512e-08
168386,168387,168386,336773,3.959826946258545,4.33821191228846e-08
168574,168575,168574,337149,3.964092969894409,4.2742584957845226e-08
168761,168762,168761,337523,3.96834397315979,4.211700596310732e-08
168948,168949,168948,337897,3.9726078510284424,4.149386987113811e-08
169135,169136,169135,338271,3.9769768714904785,4.08828935471567e-08
169322,169323,169322,338645,3.9812419414520264,4.02856412882215e-08
169509,169510,169509,339019,3.9854729175567627,3.969138255891882e-08
169696,169697,169696,339393,3.989776134490967,3.910478703350767e-08
169883,169884,169883,339767,3.993980884552002,3.853309552589647e-08
170070,170071,170070,340141,3.9982898235321045,3.7967038360972154e-08
170257,170258,170257,340515,4.002586126327515,3.7404900691561146e-08
170445,170446,170445,340891,4.007117986679077,3.685350663719549e-08
170632,170633,170632,341265,4.011339902877808,3.631410114423049e-08
170819,170820,170819,341639,4.015542030334473,3.577680876241162e-08
171006,171007,171006,342013,4.0197460651397705,3.5250039077813566e-08
171193,171194,171193,342387,4.024014949798584,3.473507265881917e-08
171380,171381,171380,342761,4.028218030929565,3.422266833492817e-08
171567,171568,171567,343135,4.032428979873657,3.371691192635145e-08
171754,171755,171754,343509,4.036618947982788,3.322399979926098e-08
171941,171942,171941,343883,4.040819883346558,3.27359101620612e-08
172128,172129,172128,344257,4.045019865036011,3.225122768154495e-08
172316,172317,172316,344633,4.049232721328735,3.177582627024961e-08
172503,172504,172503,345007,4.053420066833496,3.1310723748089536e-08
172690,172691,172690,345381,4.057626724243164,3.0847449343953033e-08
172877,172878,172877,345755,4.061815977096558,3.039328070909963e-08
173064,173065,173064,346129,4.066055774688721,2.994926311814032e-08
173251,173252,173251,346503,4.070373058319092,2.950743845195563e-08
173438,173439,173438,346877,4.074689865112305,2.9071380796351507e-08
173625,173626,173625,347251,4.079113960266113,2.8646392080266367e-08
173812,173813,173812,347625,4.083492040634155,2.822553080352291e-08
173999,174000,173999,347999,4.087789058685303,2.780763135843333e-08
174186,174187,174186,348373,4.092078924179077,2.739990315000214e-08
174374,174375,174374,348749,4.09627890586853,2.6996714442878874e-08
174561,174562,174561,349123,4.100562810897827,2.6597261327436316e-08
174748,174749,174748,349497,4.104828834533691,2.6205687671125303e-08
174935,174936,174935,349871,4.109675884246826,2.5822843862290246e-08
175122,175123,175122,350245,4.114972829818726,2.5441877126996412e-08
175309,175310,175309,350619,4.120633125305176,2.5065913070254497e-08
175496,175497,175496,350993,4.125016927719116,2.4699487770430386e-08
175683,175684,175683,351367,4.129677057266235,2.4336594972370286e-08
175870,175871,175870,351741,4.1339240074157715,2.3976276842904162e-08
176057,176058,176057,352115,4.138312816619873,2.3624741345245e-08
176245,176246,176245,352491,4.142612934112549,2.3277091667657382e-08
176432,176433,176432,352865,4.146868944168091,2.293266785176763e-08
176619,176620,176619,353239,4.151428937911987,2.2595062110497157e-08
176806,176807,176806,353613,4.155822038650513,2.2264963847638645e-08
176993,176994,176993,353987,4.160130023956299,2.193647239557348e-08
177180,177181,177180,354361,4.164432764053345,2.1612320436636115e-08
177367,177368,177367,354735,4.168722867965698,2.1296388445908573e-08
177554,177555,177554,355109,4.173019886016846,2.09834796874281e-08
177741,177742,177741,355483,4.1772301197052,2.067280901019167e-08
177928,177929,177928,355857,4.1814329624176025,2.0369721713173187e-08
178115,178116,178115,356231,4.185612916946411,2.0071553005666696e-08
178303,178304,178303,356607,4.189847946166992,1.9772985227960805e-08
178490,178491,178490,356981,4.194085121154785,1.9481909446176037e-08
178677,178678,178677,357355,4.198282957077026,1.919728974863388e-08
178864,178865,178864,357729,4.2025768756866455,1.8914045574232594e-08
179051,179052,179051,358103,4.206766128540039,1.8634565521932555e-08
179238,179239,179238,358477,4.210981845855713,1.8362168767574318e-08
179425,179426,179425,358851,4.215178966522217,1.8092359319462724e-08
179612,179613,179612,359225,4.219400882720947,1.782449534564476e-08
179799,179800,179799,359599,4.223622798919678,1.7563179143730434e-08
179986,179987,179986,359973,4.227832078933716,1.730608292129827e-08
180174,180175,180174,360349,4.232095003128052,1.7048646434117338e-08
180361,180362,180361,360723,4.236296892166138,1.6797687684575038e-08
180548,180549,180548,361097,4.24226188659668,1.6552280723680838e-08
180735,180736,180735,361471,4.246525764465332,1.6308051373416883e-08
180922,180923,180922,361845,4.250852108001709,1.6067086955769748e-08
181109,181110,181109,362219,4.255124807357788,1.583222623077113e-08
181296,181297,181296,362593,4.259886980056763,1.55995797012799e-08
181483,181484,181483,362967,4.264092922210693,1.536862429553825e-08
181670,181671,181670,363341,4.268419981002808,1.51433223125604e-08
181857,181858,181857,363715,4.272709846496582,1.49216408435406e-08
182045,182046,182045,364091,4.277017116546631,1.469966940506714e-08
182232,182233,182232,364465,4.281280994415283,1.4483298618388156e-08
182419,182420,182419,364839,4.2855260372161865,1.4271701888326597e-08
182606,182607,182606,365213,4.289830923080444,1.4061113374955824e-08
182793,182794,182793,365587,4.294088840484619,1.3853356754240213e-08
182980,182981,182980,365961,4.298375844955444,1.3650859545166066e-08
183167,183168,183167,366335,4.302585124969482,1.3450257208217989e-08
183354,183355,183354,366709,4.306810140609741,1.325112485841904e-08
183541,183542,183541,367083,4.3110339641571045,1.3056873629458694e-08
183728,183729,183728,367457,4.315233945846558,1.2865728498776868e-08
183915,183916,183915,367831,4.31949782371521,1.267534765172913e-08
184103,184104,184103,368207,4.323732852935791,1.2487786591387566e-08
184290,184291,184290,368581,4.327956914901733,1.2305341906557625e-08
184477,184478,184477,368955,4.3321919441223145,1.2123760498745833e-08
184664,184665,184664,369329,4.336405992507935,1.1944635275202735e-08
184851,184852,184851,369703,4.340651988983154,1.1770041876222476e-08
185038,185039,185038,370077,4.344895839691162,1.1597069976201427e-08
185225,185226,185225,370451,4.34919810295105,1.1425375899939534e-08
185412,185413,185412,370825,4.353798866271973,1.1257896029482623e-08
185599,185600,185599,371199,4.358033895492554,1.1093080874053538e-08
185786,185787,185786,371573,4.3623058795928955,1.0928927415642822e-08
185974,185975,185974,371949,4.366631984710693,1.0767216662943253e-08
186161,186162,186161,372323,4.371365070343018,1.0609907672690896e-08
186348,186349,186348,372697,4.3766467571258545,1.0453337886326874e-08
186535,186536,186535,373071,4.38103175163269,1.0298898344439642e-08
186722,186723,186722,373445,4.385202884674072,1.0148363619096395e-08
186909,186910,186909,373819,4.389369010925293,9.99921645559584e-09


==> plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,4.1961669921875e-05,4.387072431292609
7,25,0,25,0.001046895980834961,1.8599119493748546
14,51,0,51,0.0020608901977539062,0.646060385810488
21,73,0,73,0.0030698776245117188,0.26582040601045587
28,95,0,95,0.004040956497192383,0.1833999765905473
36,121,0,121,0.005692720413208008,0.14479233503308572
43,142,0,142,0.006712913513183594,0.12148628045781244
50,165,0,165,0.00770878791809082,0.10970795608886257
57,186,0,186,0.008830785751342773,0.09676374585392662
64,207,0,207,0.00981593132019043,0.08826038441949174
71,228,0,228,0.010734796524047852,0.08112900746473846
78,249,0,249,0.011662721633911133,0.07580406717955492
85,270,0,270,0.012572765350341797,0.07085971198224368
93,294,0,294,0.013725757598876953,0.06697348496771001
100,315,0,315,0.014948844909667969,0.06333451309322462
107,336,0,336,0.015930652618408203,0.06067674552084343
114,357,0,357,0.016878843307495117,0.05871635172520547
121,378,0,378,0.017834901809692383,0.056659790925287744
128,403,0,403,0.019488811492919922,0.05332127980862829
135,425,0,425,0.020483732223510742,0.05204805447367443
142,450,0,450,0.02148294448852539,0.049579404670590604
150,478,0,478,0.022845745086669922,0.04675689435718442
157,504,0,504,0.023865699768066406,0.045083624619016896
164,527,0,527,0.024821996688842773,0.04301350751104416
171,550,0,550,0.0257718563079834,0.04063370343064385
178,573,0,573,0.02672886848449707,0.03910924173736095
185,600,0,600,0.02775883674621582,0.03822803808081074
192,624,0,624,0.028729677200317383,0.03677797991434598
199,648,0,648,0.02969980239868164,0.03492985198045036
207,677,0,677,0.03085470199584961,0.03391879149751803
214,705,0,705,0.032301902770996094,0.033565670266777495
221,731,0,731,0.0334010124206543,0.033005500441061875
228,758,0,758,0.03451895713806152,0.03231949399972589
235,782,0,782,0.03555488586425781,0.03151048754109619
242,808,0,808,0.03657269477844238,0.030645353634218324
249,833,0,833,0.03755378723144531,0.030081184772192463
256,859,0,859,0.03856396675109863,0.029307968603637585
264,886,0,886,0.03966188430786133,0.02814876150516093
271,910,0,910,0.04063081741333008,0.027039792499845502
278,937,0,937,0.041645050048828125,0.02667730059761686
285,962,0,962,0.0426177978515625,0.02612073706533804
292,991,0,991,0.043673038482666016,0.02582150076757371
299,1019,0,1019,0.04476785659790039,0.025691287272492244
306,1047,0,1047,0.04606986045837402,0.025600828415971277
313,1075,0,1075,0.04742288589477539,0.025523709499047014
320,1100,0,1100,0.04843282699584961,0.025130884984063448
328,1130,0,1130,0.049696922302246094,0.024621272256751328
335,1158,0,1158,0.050752878189086914,0.024450777544715384
342,1187,0,1187,0.0519559383392334,0.024350499141507456
349,1216,0,1216,0.053067922592163086,0.024280694937420518
356,1244,0,1244,0.05420184135437012,0.024214741871332945
363,1271,0,1271,0.055365800857543945,0.024144977691097774
370,1297,0,1297,0.05671286582946777,0.023693693146526727
377,1324,0,1324,0.05797767639160156,0.023468386435305688
385,1352,0,1352,0.05975174903869629,0.0230718920440735
392,1379,0,1379,0.06134295463562012,0.02270568072110944
399,1407,0,1407,0.06255674362182617,0.02256274408688902
406,1434,0,1434,0.0637197494506836,0.022383564707340858
413,1462,0,1462,0.06490492820739746,0.022245878211648428
420,1489,0,1489,0.06615376472473145,0.022061472815687252
427,1517,0,1517,0.06744980812072754,0.021952739670894277
434,1546,0,1546,0.06884074211120605,0.021889230200436587
442,1581,0,1581,0.07019901275634766,0.021838309295896932
449,1609,0,1609,0.07133197784423828,0.02179987744820662
456,1639,0,1639,0.07258176803588867,0.021751620709180335
463,1667,0,1667,0.07374191284179688,0.021707045322382802
470,1695,0,1695,0.07486271858215332,0.021663649470072974
477,1723,0,1723,0.07613205909729004,0.021622498269092405
484,1751,0,1751,0.07725882530212402,0.02158139355226702
491,1779,0,1779,0.07835173606872559,0.021540392700689883
499,1811,0,1811,0.07963061332702637,0.02149427952781886
506,1839,0,1839,0.08072376251220703,0.02145399392835971
513,1867,0,1867,0.08191084861755371,0.02141404610143093
520,1895,0,1895,0.0829918384552002,0.021374292289720615
527,1923,0,1923,0.084075927734375,0.021334715166492976
534,1951,0,1951,0.08514189720153809,0.02129555883622578
541,1979,0,1979,0.08621001243591309,0.021256359756954137
548,2004,0,2004,0.08723282814025879,0.020921216963962697
556,2035,0,2035,0.08844280242919922,0.02055729678707214
563,2061,0,2061,0.08952069282531738,0.020267861625056307
570,2084,0,2084,0.09050989151000977,0.019584040008820063
577,2110,0,2110,0.09155869483947754,0.018973091897810115
584,2131,0,2131,0.0924978256225586,0.018305656258254668
591,2154,0,2154,0.09348082542419434,0.017277265498042312
598,2177,0,2177,0.09446382522583008,0.016598915990918922
605,2202,0,2202,0.09549283981323242,0.016238729235499908
613,2232,0,2232,0.09673190116882324,0.015756773248159
620,2258,0,2258,0.0977938175201416,0.015543776093101907
627,2284,0,2284,0.09886693954467773,0.015066994891946838
634,2311,0,2311,0.09995889663696289,0.014725009626560924
641,2338,0,2338,0.1009976863861084,0.014557724354790743
648,2365,0,2365,0.10205984115600586,0.014297515447903772
655,2391,0,2391,0.10312271118164062,0.014010500853507678
662,2416,0,2416,0.10417890548706055,0.013743857719186509
669,2440,0,2440,0.10532188415527344,0.01326398862732894
677,2471,0,2471,0.1065669059753418,0.01301344918648411
684,2498,0,2498,0.10764575004577637,0.012857413538610266
691,2524,0,2524,0.10905694961547852,0.012667823545067701
698,2553,0,2553,0.1102137565612793,0.012577492348836133
705,2581,0,2581,0.11131787300109863,0.012531026077236728
712,2607,0,2607,0.11236977577209473,0.012322151118212537
719,2635,0,2635,0.11348390579223633,0.012257017369904063
726,2663,0,2663,0.11454892158508301,0.012216447829210407
734,2695,0,2695,0.11574292182922363,0.012180930390465253
741,2723,0,2723,0.1170358657836914,0.012152039184658679
748,2750,0,2750,0.1181337833404541,0.012071384522412111
755,2778,0,2778,0.11960077285766602,0.012017374222100616
762,2805,0,2805,0.1213376522064209,0.011914715395052677
769,2832,0,2832,0.12274503707885742,0.011773116298406956
776,2860,0,2860,0.1239469051361084,0.011721443824168138
783,2885,0,2885,0.12560391426086426,0.011487765543719448
791,2914,0,2914,0.1273508071899414,0.011193753191120821
798,2942,0,2942,0.12911486625671387,0.011074155802639995
805,2970,0,2970,0.13102364540100098,0.011031339378686127
812,2999,0,2999,0.13227272033691406,0.010994569345441348
819,3027,0,3027,0.13341093063354492,0.010954059905350966
826,3055,0,3055,0.13451695442199707,0.010892436456724839
833,3083,0,3083,0.13562893867492676,0.010856460356790219
840,3112,0,3112,0.1367490291595459,0.010830082671694573
848,3145,0,3145,0.13803696632385254,0.010809090497539193
855,3174,0,3174,0.13916778564453125,0.010786129562399546
862,3202,0,3202,0.14028096199035645,0.01076617139498067
869,3230,0,3230,0.14139676094055176,0.010745307346032002
876,3258,0,3258,0.14250802993774414,0.010725306716583508
883,3286,0,3286,0.14371609687805176,0.01070546158461828
890,3314,0,3314,0.14496994018554688,0.010685415774201852
897,3342,0,3342,0.14689874649047852,0.010665656962554934
905,3374,0,3374,0.148298978805542,0.010643393985365762
912,3402,0,3402,0.1501307487487793,0.010624008284960252
919,3430,0,3430,0.15222692489624023,0.01060455927727649
926,3458,0,3458,0.15392374992370605,0.01058519666278113
933,3486,0,3486,0.15535378456115723,0.010565805599911873
940,3514,0,3514,0.15657496452331543,0.0105465054438266
947,3540,0,3540,0.15767598152160645,0.010425788303461638
954,3564,0,3564,0.15900492668151855,0.010149604012924317
961,3590,0,3590,0.1602339744567871,0.009896516371788674
969,3620,0,3620,0.1616077423095703,0.009531479781741344
976,3645,0,3645,0.16321396827697754,0.009287876072602922
983,3671,0,3671,0.16498184204101562,0.009072891497764924
990,3698,0,3698,0.16714882850646973,0.008920205477753405
997,3723,0,3723,0.16893482208251953,0.008724984472195217
1004,3748,0,3748,0.17089462280273438,0.008535198324216247
1011,3776,0,3776,0.1725597381591797,0.008447910433565369
1018,3801,0,3801,0.1739037036895752,0.00823215006695327
1026,3828,0,3828,0.17559480667114258,0.007934355456106141
1033,3851,0,3851,0.17702484130859375,0.00750399194861244
1040,3873,0,3873,0.17857098579406738,0.007045170376187258
1047,3899,0,3899,0.18017888069152832,0.006832579516124469
1054,3926,0,3926,0.18136906623840332,0.0067298775469245824
1061,3952,0,3952,0.18253779411315918,0.006603958983619041
1068,3979,0,3979,0.18372678756713867,0.006485425699952731
1075,4000,0,4000,0.18474388122558594,0.0061917177358785805
1083,4026,0,4026,0.1860957145690918,0.0057632627835811755
1090,4050,0,4050,0.18722772598266602,0.005499813256356118
1097,4072,0,4072,0.1888108253479004,0.0052073244663781194
1104,4098,0,4098,0.19040989875793457,0.0050317779481748245
1111,4123,0,4123,0.1915597915649414,0.004923659896253103
1118,4148,0,4148,0.1929619312286377,0.004790007850628172
1125,4175,0,4175,0.1942768096923828,0.004694884684504137
1132,4200,0,4200,0.19561171531677246,0.004558284467892034
1140,4231,0,4231,0.19837570190429688,0.004447783620024228
1147,4255,0,4255,0.20020675659179688,0.004337150817375206
1154,4282,0,4282,0.2024528980255127,0.004227289301657046
1161,4307,0,4307,0.20400786399841309,0.004114286058133364
1168,4332,0,4332,0.20524287223815918,0.003997462193170067
1175,4358,0,4358,0.20665597915649414,0.003893496984532258
1182,4384,0,4384,0.20812368392944336,0.003833511234926511
1189,4410,0,4410,0.20934391021728516,0.003758958667694934
1197,4440,0,4440,0.21101689338684082,0.0036636716824036113
1204,4466,0,4466,0.2127368450164795,0.003587369974763675
1211,4492,0,4492,0.21468782424926758,0.0034883975647162367
1218,4518,0,4518,0.21705174446105957,0.0034040621504421056
1225,4541,0,4541,0.21844196319580078,0.0032974007765146397
1232,4568,0,4568,0.21974802017211914,0.003234742089075144
1239,4596,0,4596,0.2209939956665039,0.0031957896232695316
1246,4623,0,4623,0.22267985343933105,0.0031410489634962056
1253,4650,0,4650,0.22417974472045898,0.0031027270893140514
1261,4682,0,4682,0.22558879852294922,0.0030609763410219346
1268,4709,0,4709,0.22695088386535645,0.003027626685939332
1275,4737,0,4737,0.22828173637390137,0.0030124081808875053
1282,4764,0,4764,0.23019075393676758,0.0029870357802965486
1289,4790,0,4790,0.23218393325805664,0.0029427594337684566
1296,4817,0,4817,0.23418593406677246,0.002907282658936465
1303,4845,0,4845,0.23625493049621582,0.0028926919923717726
1310,4871,0,4871,0.23790693283081055,0.002844309739643444
1318,4900,0,4900,0.2398838996887207,0.0027739498340588428
1325,4925,0,4925,0.24150705337524414,0.0027086940016188446
1332,4950,0,4950,0.24293184280395508,0.002653446230472659
1339,4977,0,4977,0.24410080909729004,0.0025991854590504317
1346,5002,0,5002,0.2456350326538086,0.002534904913719439
1353,5027,0,5027,0.24679088592529297,0.002432652650888027
1360,5050,0,5050,0.24828267097473145,0.002289230087906931
1367,5077,0,5077,0.25000905990600586,0.0022334445861015577
1375,5106,0,5106,0.2521829605102539,0.0021862977998710863
1382,5131,0,5131,0.25461769104003906,0.002105401575099917
1389,5153,0,5153,0.2567777633666992,0.00197749112587925
1396,5176,0,5176,0.2594449520111084,0.0018785874469849592
1403,5198,0,5198,0.2608938217163086,0.0018037544618197208
1410,5224,0,5224,0.26203274726867676,0.0017486434319929902
1417,5251,0,5251,0.26318883895874023,0.0017220326380171032
1424,5279,0,5279,0.26441478729248047,0.0017047069275176812
1432,5311,0,5311,0.26587581634521484,0.0016941982724202837
1439,5339,0,5339,0.2684779167175293,0.0016869058395555198
1446,5368,0,5368,0.2712829113006592,0.001680824582755222
1453,5396,0,5396,0.27312302589416504,0.0016754288147760802
1460,5426,0,5426,0.27443385124206543,0.001670804374503955
1467,5455,0,5455,0.275925874710083,0.001666318140714204
1474,5483,0,5483,0.27745771408081055,0.0016622105987493172
1481,5512,0,5512,0.2787818908691406,0.0016581169580335243
1489,5545,0,5545,0.28017687797546387,0.0016534828831796093
1496,5577,0,5577,0.2814478874206543,0.0016501593923515852
1503,5605,0,5605,0.2826387882232666,0.0016468676565889037
1510,5634,0,5634,0.28415465354919434,0.0016435453561212375
1517,5663,0,5663,0.28569579124450684,0.0016398868221883568
1524,5691,0,5691,0.28685879707336426,0.0016363873185165567
1531,5719,0,5719,0.28801584243774414,0.0016330509998387008
1538,5747,0,5747,0.28928184509277344,0.0016296619088803758
1546,5779,0,5779,0.29064488410949707,0.001625914193883257
1553,5807,0,5807,0.2918367385864258,0.00162267787999297
1560,5835,0,5835,0.293062686920166,0.0016195354569017272
1567,5863,0,5863,0.2942318916320801,0.0016164029870496038
1574,5891,0,5891,0.2956888675689697,0.0016132506531838316
1581,5919,0,5919,0.29702281951904297,0.001610138448489461
1588,5947,0,5947,0.2982969284057617,0.0016070464838323477
1595,5975,0,5975,0.2996389865875244,0.0016039871300266317
1602,6003,0,6003,0.30170178413391113,0.0016009433343424086
1610,6035,0,6035,0.30335092544555664,0.0015974756394640931
1617,6063,0,6063,0.30495572090148926,0.0015944472316451637
1624,6091,0,6091,0.306182861328125,0.0015914332316285707
1631,6119,0,6119,0.30767297744750977,0.0015884167477150234
1638,6147,0,6147,0.3097968101501465,0.0015854111194303956
1645,6175,0,6175,0.3115408420562744,0.0015824134003774445
1652,6203,0,6203,0.31285691261291504,0.0015794188211790859
1659,6230,0,6230,0.31401491165161133,0.0015737802203411653
1667,6258,0,6258,0.31615471839904785,0.0015357642107741312
1674,6285,0,6285,0.31862497329711914,0.0015115177426354345
1681,6313,0,6313,0.32146406173706055,0.0014998542133134514
1688,6342,0,6342,0.3228909969329834,0.0014946917338918369
1695,6373,0,6373,0.324321985244751,0.0014916019608363902
1702,6402,0,6402,0.3255348205566406,0.0014882508213108297
1709,6430,0,6430,0.32667994499206543,0.0014851037649230051
1716,6459,0,6459,0.3279087543487549,0.001482110004011273
1724,6491,0,6491,0.3293788433074951,0.0014786581568873825
1731,6519,0,6519,0.3307318687438965,0.0014760630929886575
1738,6548,0,6548,0.33199000358581543,0.0014732283116578864
1745,6576,0,6576,0.3331739902496338,0.0014703475014238294
1752,6604,0,6604,0.3343627452850342,0.0014675488744771324
1759,6633,0,6633,0.33633875846862793,0.001464978047325871
1766,6661,0,6661,0.3380467891693115,0.0014622415786642604
1773,6688,0,6688,0.33951568603515625,0.0014592016212316467
1781,6718,0,6718,0.3409006595611572,0.0014339267365587453
1788,6745,0,6745,0.34231090545654297,0.0014171027867715617
1795,6770,0,6770,0.3438568115234375,0.0013767505346596865
1802,6795,0,6795,0.3451356887817383,0.0013363975911142895
1809,6819,0,6819,0.34632396697998047,0.00129496383513475
1816,6845,0,6845,0.3474307060241699,0.0012681858423264668
1823,6867,0,6867,0.34867095947265625,0.0012039796372613747
1830,6893,0,6893,0.34996485710144043,0.0011753729653604839
1838,6927,0,6927,0.3514838218688965,0.0011635930661717986
1845,6955,0,6955,0.3526017665863037,0.0011578487685268526
1852,6982,0,6982,0.3538496494293213,0.0011472259681689155
1859,7009,0,7009,0.35504770278930664,0.0011349101848504833
1866,7037,0,7037,0.3562307357788086,0.0011230393380098473
1873,7064,0,7064,0.3573789596557617,0.0011109830310585172
1880,7090,0,7090,0.3585178852081299,0.0010864882170404555
1887,7118,0,7118,0.35976290702819824,0.0010720939654738637
1894,7147,0,7147,0.36104393005371094,0.001064327566694807
1902,7179,0,7179,0.3628249168395996,0.0010594704047239849
1909,7207,0,7207,0.3645789623260498,0.0010559738768292643
1916,7235,0,7235,0.36592888832092285,0.0010534590023657145
1923,7263,0,7263,0.36733484268188477,0.0010514694688987655
1930,7291,0,7291,0.36862683296203613,0.0010492541026368497
1937,7319,0,7319,0.36981773376464844,0.0010472134231093114
1944,7347,0,7347,0.3711516857147217,0.0010452745401414772
1951,7375,0,7375,0.3729588985443115,0.0010433302710703305
1959,7407,0,7407,0.3747696876525879,0.0010411161152015305
1966,7435,0,7435,0.376018762588501,0.0010391952945919365
1973,7463,0,7463,0.3772158622741699,0.001037314947751924
1980,7491,0,7491,0.3784768581390381,0.0010354265268574967
1987,7519,0,7519,0.3801100254058838,0.0010335230269479685
1994,7547,0,7547,0.3820059299468994,0.0010316408865887548
2001,7575,0,7575,0.3834249973297119,0.0010297556702177572
2008,7603,0,7603,0.384807825088501,0.0010278899612265926
2016,7635,0,7635,0.38619494438171387,0.0010257409655891913
2023,7663,0,7663,0.3873918056488037,0.0010238683032704828
2030,7691,0,7691,0.3885979652404785,0.0010219989933770448
2037,7719,0,7719,0.38979196548461914,0.001020133531236304
2044,7747,0,7747,0.3911867141723633,0.0010182652172315374
2051,7775,0,7775,0.3924729824066162,0.001016406555487199
2058,7803,0,7803,0.3937556743621826,0.0010145482011152784
2065,7827,0,7827,0.3951389789581299,0.0009936259350619597
2073,7855,0,7855,0.3970339298248291,0.0009604254844616037
2080,7878,0,7878,0.39837098121643066,0.000907267473594467
2087,7900,0,7900,0.3997368812561035,0.000856387055155897
2094,7922,0,7922,0.40091586112976074,0.000814006697972245
2101,7944,0,7944,0.4021627902984619,0.0007543719444341699
2108,7972,0,7972,0.4036438465118408,0.0007341672790072191
2115,7999,0,7999,0.4053828716278076,0.0007193713822706727
2122,8026,0,8026,0.40705299377441406,0.0007042062926111283
2130,8055,0,8055,0.4085879325866699,0.0006889698926294775
2137,8080,0,8080,0.40978384017944336,0.0006685491655309611
2144,8106,0,8106,0.41144585609436035,0.0006505178006798233
2151,8136,0,8136,0.41304492950439453,0.0006455137142734156
2158,8163,0,8163,0.4142918586730957,0.0006347913744943423
2165,8189,0,8189,0.4161646366119385,0.000626847833790313
2172,8214,0,8214,0.41735386848449707,0.0006072603681767592
2179,8241,0,8241,0.418820858001709,0.0005999904560247477
2186,8268,0,8268,0.4202139377593994,0.0005881345880837664
2194,8299,0,8299,0.4219329357147217,0.0005794411392145813
2201,8327,0,8327,0.4233419895172119,0.00057637693373513
2208,8352,0,8352,0.4244568347930908,0.0005667785285109741
2215,8378,0,8378,0.42558979988098145,0.0005593958393517749
2222,8405,0,8405,0.4268207550048828,0.0005503516282901374
2229,8433,0,8433,0.42801976203918457,0.0005473488244219273
2236,8463,0,8463,0.42927098274230957,0.0005454501972891038
2243,8492,0,8492,0.4304208755493164,0.0005438675321232291
2251,8524,0,8524,0.4317789077758789,0.0005422821497625454
2258,8553,0,8553,0.43320703506469727,0.0005411079402005408
2265,8581,0,8581,0.43454980850219727,0.0005398248354853959
2272,8609,0,8609,0.4357569217681885,0.0005386738612653564
2279,8638,0,8638,0.4373297691345215,0.0005375956012678048
2286,8666,0,8666,0.4391658306121826,0.0005364996392717083
2293,8694,0,8694,0.44086289405822754,0.0005354114956011809
2300,8722,0,8722,0.44210076332092285,0.0005343824818946956
2308,8754,0,8754,0.44350266456604004,0.0005332140252034864
2315,8782,0,8782,0.4446709156036377,0.000532200847741006
2322,8810,0,8810,0.4459078311920166,0.0005312057679033369
2329,8838,0,8838,0.44725704193115234,0.0005302398453906834
2336,8866,0,8866,0.44911980628967285,0.0005292417129866962
2343,8894,0,8894,0.4513988494873047,0.0005282566064484804
2350,8922,0,8922,0.45304393768310547,0.0005272890953904111
2357,8950,0,8950,0.4547266960144043,0.0005263194424776047
2365,8982,0,8982,0.4566776752471924,0.0005252150082995553
2372,9010,0,9010,0.45799875259399414,0.0005242476441753308
2379,9038,0,9038,0.4595918655395508,0.0005232876750110016
2386,9066,0,9066,0.4610919952392578,0.0005223279494047382
2393,9094,0,9094,0.4625058174133301,0.0005213705776551027
2400,9122,0,9122,0.464277982711792,0.0005204145934960146
2407,9150,0,9150,0.4658827781677246,0.0005194603849088586
2414,9177,0,9177,0.468355655670166,0.0005181644987550393
2422,9206,0,9206,0.4697227478027344,0.0005079842940060036
2429,9233,0,9233,0.4713888168334961,0.0005000755207235917
2436,9259,0,9259,0.47274279594421387,0.0004890949492841227
2443,9281,0,9281,0.4741239547729492,0.0004562870255066304
2450,9304,0,9304,0.4761619567871094,0.0004359118003569785
2457,9328,0,9328,0.47831273078918457,0.00042075064433132105
2464,9355,0,9355,0.48011064529418945,0.0004126764240972104
2471,9381,0,9381,0.4819958209991455,0.0004027773017232554
2478,9404,0,9404,0.48342275619506836,0.00039016986947391707
2486,9435,0,9435,0.4855227470397949,0.00038124010875821774
2493,9461,0,9461,0.4873499870300293,0.0003747119931505209
2500,9485,0,9485,0.4890298843383789,0.00036267960001733023
2507,9507,0,9507,0.490628719329834,0.00033748243198082427
2514,9532,0,9532,0.4926457405090332,0.0003243902013993868
2521,9558,0,9558,0.4941868782043457,0.0003169771201940842
2528,9585,0,9585,0.4963366985321045,0.00031381164970842236
2535,9612,0,9612,0.4988858699798584,0.0003090230823500148
2543,9641,0,9641,0.5015988349914551,0.0003019318740055787
2550,9665,0,9665,0.5036966800689697,0.0002916429930015906
2557,9690,0,9690,0.5056056976318359,0.0002813422660498161
2564,9718,0,9718,0.5079138278961182,0.0002778075713860866
2571,9743,0,9743,0.5104148387908936,0.0002718713513967921
2578,9769,0,9769,0.5129988193511963,0.0002651712574948109
2585,9793,0,9793,0.5154149532318115,0.0002569683760267573
2592,9820,0,9820,0.5185427665710449,0.0002516443025827958
2600,9847,0,9847,0.5210616588592529,0.00024224679464243887
2607,9872,0,9872,0.5233588218688965,0.0002360319376009114
2614,9896,0,9896,0.5258097648620605,0.00022791668273398788
2621,9918,0,9918,0.5284626483917236,0.00021429017936389273
2628,9941,0,9941,0.5304467678070068,0.00020206159163057403
2635,9969,0,9969,0.5323898792266846,0.00019963120690189812
2642,9997,0,9997,0.5343799591064453,0.0001982384945660964
2649,10024,0,10024,0.5365757942199707,0.00019611715591093663
2657,10056,0,10056,0.5386416912078857,0.00019450884112120201
2664,10085,0,10085,0.5402557849884033,0.00019368270235019326
2671,10114,0,10114,0.5424308776855469,0.00019296410401531595
2678,10142,0,10142,0.5441436767578125,0.00019232315922669568
2685,10171,0,10171,0.5464439392089844,0.00019174412703679898
2692,10199,0,10199,0.5490627288818359,0.00019117743781398174
2699,10227,0,10227,0.5514168739318848,0.00019069457996515407
2706,10255,0,10255,0.5531759262084961,0.00019018230602695375
2714,10287,0,10287,0.5557057857513428,0.00018963708692257007
2721,10315,0,10315,0.5582289695739746,0.00018917657138942985
2728,10343,0,10343,0.5609877109527588,0.00018874648405121976
2735,10371,0,10371,0.5636069774627686,0.0001883204169225313
2742,10399,0,10399,0.5663928985595703,0.00018790384364260083
2749,10427,0,10427,0.5690767765045166,0.00018749862943543105
2756,10455,0,10455,0.5714809894561768,0.00018710391692570663
2763,10483,0,10483,0.573793888092041,0.00018671010048460274
2771,10515,0,10515,0.5764298439025879,0.00018627008842162697
2778,10543,0,10543,0.5778517723083496,0.00018588896931889356
2785,10571,0,10571,0.5794088840484619,0.00018551960340144208
2792,10599,0,10599,0.5811009407043457,0.0001851471646208133
2799,10627,0,10627,0.5825338363647461,0.0001847804255051591
2806,10655,0,10655,0.584357738494873,0.00018441643816599875
2813,10683,0,10683,0.5856139659881592,0.00018405896175845705
2820,10711,0,10711,0.5878078937530518,0.00018370188331698207
2827,10739,0,10739,0.5897536277770996,0.0001833502370626352
2835,10771,0,10771,0.5912938117980957,0.00018294927036796162
2842,10799,0,10799,0.5928177833557129,0.000182603005217343
2849,10827,0,10827,0.5941369533538818,0.00018225732836301786
2856,10855,0,10855,0.5957558155059814,0.00018191453819931937
2863,10883,0,10883,0.5973818302154541,0.00018157235299819924
2870,10911,0,10911,0.5989439487457275,0.00018123329641507298
2877,10939,0,10939,0.6013138294219971,0.00018089487845586252
2884,10967,0,10967,0.6039068698883057,0.0001805585209805691
2892,10999,0,10999,0.6054718494415283,0.0001801745660789127
2899,11026,0,11026,0.6067440509796143,0.0001798794964183727
2906,11051,0,11051,0.6081557273864746,0.00017681135976585946
2913,11079,0,11079,0.6094686985015869,0.00017444764702980017
2920,11107,0,11107,0.6106669902801514,0.00017344006829722418
2927,11135,0,11135,0.611818790435791,0.00017264611110601755
2934,11164,0,11164,0.6130077838897705,0.00017171006185993636
2941,11192,0,11192,0.6142950057983398,0.00017125900370942046
2949,11224,0,11224,0.615912914276123,0.0001708199885182744
2956,11252,0,11252,0.6172828674316406,0.00017048535556014573
2963,11280,0,11280,0.6189708709716797,0.00017016742282537805
2970,11308,0,11308,0.6207079887390137,0.0001698530501255912
2977,11336,0,11336,0.6224827766418457,0.0001695442691692197
2984,11364,0,11364,0.6242799758911133,0.0001692355002148899
2991,11392,0,11392,0.6260378360748291,0.00016891689348207323
2998,11420,0,11420,0.6280937194824219,0.00016860654007381243
3006,11452,0,11452,0.6295478343963623,0.00016825445035208717
3013,11480,0,11480,0.6307449340820312,0.00016794814132744645
3020,11508,0,11508,0.6319279670715332,0.0001676411788106067
3027,11536,0,11536,0.6331539154052734,0.00016733545799375545
3034,11564,0,11564,0.6345117092132568,0.00016702964469672584
3041,11592,0,11592,0.6359498500823975,0.00016672424256803089
3048,11620,0,11620,0.6371927261352539,0.0001664188912896719
3055,11648,0,11648,0.6383228302001953,0.00016611436346756288
3063,11679,0,11679,0.6396520137786865,0.00016512972430607657
3070,11701,0,11701,0.6410818099975586,0.00016148936844683948
3077,11729,0,11729,0.6426959037780762,0.00015735661929420607
3084,11752,0,11752,0.6440057754516602,0.00014891119742292225
3091,11774,0,11774,0.6455819606781006,0.00014043130419141422
3098,11798,0,11798,0.6473557949066162,0.00013462065548703754
3105,11821,0,11821,0.6490590572357178,0.0001281664899679807
3112,11845,0,11845,0.6506826877593994,0.00012388876994976676
3119,11869,0,11869,0.6521928310394287,0.0001194498523772209
3127,11895,0,11895,0.6535069942474365,0.0001128104824414329
3134,11916,0,11916,0.6546227931976318,0.00010538029774823286
3141,11938,0,11938,0.6557607650756836,0.00010155949671190874
3148,11961,0,11961,0.6570439338684082,9.594305122677648e-05
3155,11983,0,11983,0.6586878299713135,9.001290807942457e-05
3162,12008,0,12008,0.6601107120513916,8.546601230935816e-05
3169,12036,0,12036,0.6620128154754639,8.409059526767545e-05
3176,12064,0,12064,0.663996696472168,8.354022924940024e-05
3184,12093,0,12093,0.6653728485107422,8.214369999921314e-05
3191,12119,0,12119,0.6665928363800049,7.988921595492196e-05
3198,12145,0,12145,0.6680018901824951,7.814208287175728e-05
3205,12169,0,12169,0.6697437763214111,7.561789164008616e-05
3212,12191,0,12191,0.6713988780975342,7.174396098244739e-05
3219,12219,0,12219,0.6732537746429443,7.013285354721268e-05
3226,12246,0,12246,0.674980640411377,6.904635821260319e-05
3233,12273,0,12273,0.6766757965087891,6.747227845142848e-05
3241,12304,0,12304,0.6787056922912598,6.642013111664749e-05
3248,12331,0,12331,0.6805408000946045,6.545853393914696e-05
3255,12358,0,12358,0.6819667816162109,6.43025179404081e-05
3262,12386,0,12386,0.6831557750701904,6.379206759457226e-05
3269,12413,0,12413,0.6847348213195801,6.303273419782432e-05
3276,12440,0,12440,0.686039924621582,6.241720872930543e-05
3283,12466,0,12466,0.6874668598175049,6.132568535532447e-05
3290,12492,0,12492,0.6886730194091797,6.0002512176449865e-05
3298,12524,0,12524,0.6899466514587402,5.9239892973498944e-05
3305,12551,0,12551,0.6910829544067383,5.863851008505307e-05
3312,12577,0,12577,0.6921839714050293,5.7665457771720396e-05
3319,12604,0,12604,0.6933889389038086,5.722993475914855e-05
3326,12631,0,12631,0.6946158409118652,5.6256133405077205e-05
3333,12656,0,12656,0.6957979202270508,5.473822282871096e-05
3340,12684,0,12684,0.696922779083252,5.422949886726851e-05
3347,12711,0,12711,0.6980068683624268,5.359311377301649e-05
3355,12741,0,12741,0.6992459297180176,5.3105223475638243e-05
3362,12767,0,12767,0.7003109455108643,5.2360721441644076e-05
3369,12795,0,12795,0.7017168998718262,5.140829741546763e-05
3376,12823,0,12823,0.7031219005584717,5.1052971721270924e-05
3383,12853,0,12853,0.7049739360809326,5.0827451216872574e-05
3390,12882,0,12882,0.7065739631652832,5.065000746008877e-05
3397,12910,0,12910,0.7078089714050293,5.0490436777905225e-05
3404,12939,0,12939,0.7091948986053467,5.03777889535372e-05
3411,12968,0,12968,0.7104177474975586,5.0252151843181955e-05
3419,13001,0,13001,0.7117419242858887,5.012898292190632e-05
3426,13030,0,13030,0.7128918170928955,5.0033514114045254e-05
3433,13059,0,13059,0.7140517234802246,4.9922613527473604e-05
3440,13086,0,13086,0.7151987552642822,4.9770106494482394e-05
3447,13116,0,13116,0.7164368629455566,4.9398933279993845e-05
3454,13144,0,13144,0.7177059650421143,4.90117977331486e-05
3461,13172,0,13172,0.7189266681671143,4.8523527410772705e-05
3468,13198,0,13198,0.720038890838623,4.786880092378278e-05
3476,13225,0,13225,0.7214667797088623,4.600446732735145e-05
3483,13253,0,13253,0.7226250171661377,4.543017367675816e-05
3490,13278,0,13278,0.7239139080047607,4.439963505313329e-05
3497,13305,0,13305,0.7252278327941895,4.377459145419221e-05
3504,13332,0,13332,0.7264819145202637,4.297251492329189e-05
3511,13357,0,13357,0.727820873260498,4.200703114925181e-05
3518,13383,0,13383,0.7291817665100098,4.1257249109078846e-05
3525,13410,0,13410,0.7304518222808838,4.066844899102014e-05
3533,13441,0,13441,0.7320399284362793,4.006812095027688e-05
3540,13468,0,13468,0.7333707809448242,3.95932869693593e-05
3547,13495,0,13495,0.734595775604248,3.916637430665686e-05
3554,13523,0,13523,0.7358918190002441,3.890148320549529e-05
3561,13551,0,13551,0.7371077537536621,3.8759733350660105e-05
3568,13581,0,13581,0.7382738590240479,3.8658459533970245e-05
3575,13609,0,13609,0.7393567562103271,3.8578937291494095e-05
3582,13639,0,13639,0.740664005279541,3.849062617252951e-05
3590,13671,0,13671,0.7419860363006592,3.840308548983059e-05
3597,13700,0,13700,0.7431027889251709,3.833111991495522e-05
3604,13728,0,13728,0.7441940307617188,3.824808881080018e-05
3611,13756,0,13756,0.7455449104309082,3.817333233852545e-05
3618,13784,0,13784,0.7467508316040039,3.8097068726295737e-05
3625,13812,0,13812,0.7479598522186279,3.8022662388127024e-05
3632,13840,0,13840,0.7496497631072998,3.795170195228008e-05
3639,13868,0,13868,0.7513647079467773,3.788141553354084e-05
3647,13900,0,13900,0.752835750579834,3.780008356068792e-05
3654,13928,0,13928,0.7543280124664307,3.772971411962875e-05
3661,13956,0,13956,0.7560408115386963,3.766074186818022e-05
3668,13984,0,13984,0.7577018737792969,3.759126361663088e-05
3675,14012,0,14012,0.7597799301147461,3.7522515899295374e-05
3682,14040,0,14040,0.761483907699585,3.745389048585642e-05
3689,14068,0,14068,0.7627058029174805,3.738543114756249e-05
3696,14096,0,14096,0.7638938426971436,3.7316960811443136e-05
3704,14128,0,14128,0.7654218673706055,3.723917606201423e-05
3711,14156,0,14156,0.7667698860168457,3.717115560922603e-05
3718,14184,0,14184,0.7681028842926025,3.710340172721881e-05
3725,14212,0,14212,0.7693097591400146,3.7035616925704946e-05
3732,14240,0,14240,0.7704696655273438,3.696794769155812e-05
3739,14268,0,14268,0.7716178894042969,3.69003243295966e-05
3746,14294,0,14294,0.7727198600769043,3.6645277786614185e-05
3753,14319,0,14319,0.7738139629364014,3.567541611540588e-05
3760,14341,0,14341,0.7749438285827637,3.409919844375527e-05
3768,14368,0,14368,0.7761766910552979,3.2272189488065306e-05
3775,14392,0,14392,0.777228832244873,3.1014605514178164e-05
3782,14413,0,14413,0.7782597541809082,2.8789594328077033e-05
3789,14439,0,14439,0.7794098854064941,2.7578824163837168e-05
3796,14466,0,14466,0.7805118560791016,2.711547056234602e-05
3803,14493,0,14493,0.7816119194030762,2.6768951788799676e-05
3810,14518,0,14518,0.782646894454956,2.6092229734068185e-05
3817,14543,0,14543,0.7836787700653076,2.5329711897819128e-05
3825,14573,0,14573,0.7849059104919434,2.4778708982253764e-05
3832,14599,0,14599,0.7859928607940674,2.419422149748075e-05
3839,14626,0,14626,0.7872068881988525,2.370048295428591e-05
3846,14652,0,14652,0.7884316444396973,2.3180371858751885e-05
3853,14680,0,14680,0.7896528244018555,2.303719398821126e-05
3860,14705,0,14705,0.7906920909881592,2.277872898549078e-05
3867,14732,0,14732,0.791827917098999,2.222400095891307e-05
3874,14759,0,14759,0.7928988933563232,2.191812374837019e-05
3882,14790,0,14790,0.7941339015960693,2.1549330199171835e-05
3889,14818,0,14818,0.795292854309082,2.13290897817859e-05
3896,14845,0,14845,0.7965438365936279,2.098360603221086e-05
3903,14873,0,14873,0.797893762588501,2.0853198442615674e-05
3910,14901,0,14901,0.7990448474884033,2.0783208967586173e-05
3917,14929,0,14929,0.8009688854217529,2.0734951925953185e-05
3924,14958,0,14958,0.8022010326385498,2.06867949723269e-05
3931,14986,0,14986,0.8034050464630127,2.0644156311012498e-05
3939,15018,0,15018,0.8047847747802734,2.0594896541968682e-05
3946,15046,0,15046,0.8060238361358643,2.055359158284702e-05
3953,15074,0,15074,0.8073348999023438,2.0514031834196748e-05
3960,15102,0,15102,0.8085267543792725,2.0475297574596366e-05
3967,15130,0,15130,0.8097789287567139,2.0436224050314375e-05
3974,15158,0,15158,0.8111019134521484,2.0397525506742984e-05
3981,15186,0,15186,0.8122909069061279,2.0360207425939565e-05
3988,15214,0,15214,0.8134667873382568,2.032241749640335e-05
3996,15246,0,15246,0.8147628307342529,2.0279662840635823e-05
4003,15274,0,15274,0.8161377906799316,2.0242088127217777e-05
4010,15302,0,15302,0.8174138069152832,2.020482655791986e-05
4017,15330,0,15330,0.818558931350708,2.0167845245744533e-05
4024,15358,0,15358,0.8198409080505371,2.0130747896323958e-05
4031,15386,0,15386,0.8210239410400391,2.009371815200797e-05
4038,15414,0,15414,0.8227477073669434,2.005666672463187e-05
4045,15442,0,15442,0.8241188526153564,2.0019837134613616e-05
4052,15470,0,15470,0.8261017799377441,1.9982869513783582e-05
4060,15502,0,15502,0.8286440372467041,1.9940817700974506e-05
4067,15528,0,15528,0.829871654510498,1.968883182797778e-05
4074,15554,0,15554,0.8309957981109619,1.937331151049915e-05
4081,15581,0,15581,0.8320879936218262,1.9026948529823784e-05
4088,15605,0,15605,0.8331167697906494,1.8335324989881682e-05
4095,15628,0,15628,0.8341388702392578,1.7732727080401893e-05
4102,15655,0,15655,0.8353090286254883,1.7379632803232314e-05
4109,15681,0,15681,0.8363769054412842,1.703773602480818e-05
4117,15712,0,15712,0.8376197814941406,1.6748437951375675e-05
4124,15739,0,15739,0.8387236595153809,1.6572234422836516e-05
4131,15764,0,15764,0.8398258686065674,1.617956922530982e-05
4138,15788,0,15788,0.8409299850463867,1.5712067890001354e-05
4145,15812,0,15812,0.8422188758850098,1.5107844363421414e-05
4152,15835,0,15835,0.8435108661651611,1.4347063082162085e-05
4159,15857,0,15857,0.8445370197296143,1.3429196931259343e-05
4166,15885,0,15885,0.8458700180053711,1.3226699307018858e-05
4174,15917,0,15917,0.8472256660461426,1.2996129249688421e-05
4181,15947,0,15947,0.8483848571777344,1.2916073864672269e-05
4188,15971,0,15971,0.8494219779968262,1.2555500260257313e-05
4195,15996,0,15996,0.8504917621612549,1.211402215564771e-05
4202,16023,0,16023,0.8515896797180176,1.1919164221954576e-05
4209,16049,0,16049,0.8526918888092041,1.1755063059585746e-05
4216,16074,0,16074,0.8538496494293213,1.143351713243476e-05
4223,16102,0,16102,0.8551087379455566,1.1318219179276868e-05
4231,16129,0,16129,0.8564510345458984,1.0930552342392866e-05
4238,16155,0,16155,0.8576338291168213,1.0627902109930844e-05
4245,16179,0,16179,0.858773946762085,1.0335962740304041e-05
4252,16208,0,16208,0.8599469661712646,1.0109208958543549e-05
4259,16234,0,16234,0.86106276512146,9.920692013910312e-06
4266,16262,0,16262,0.8622777462005615,9.85864847775089e-06
4273,16289,0,16289,0.8634107112884521,9.748441300227755e-06
4280,16313,0,16313,0.8645238876342773,9.5368731122376e-06
4288,16343,0,16343,0.8658490180969238,9.293130897888493e-06
4295,16370,0,16370,0.8671379089355469,9.141468173921254e-06
4302,16397,0,16397,0.8684170246124268,9.088756861554277e-06
4309,16424,0,16424,0.8697116374969482,8.97745176981838e-06
4316,16453,0,16453,0.8711237907409668,8.899700667259383e-06
4323,16481,0,16481,0.8724088668823242,8.826530334549867e-06
4330,16508,0,16508,0.8736827373504639,8.736459307087919e-06
4337,16536,0,16536,0.8750009536743164,8.679606927263661e-06
4344,16565,0,16565,0.8761677742004395,8.647951947563968e-06
4352,16598,0,16598,0.8774948120117188,8.623820759809921e-06
4359,16626,0,16626,0.8786239624023438,8.604455704793656e-06
4366,16654,0,16654,0.8797729015350342,8.585886173544612e-06
4373,16682,0,16682,0.8809168338775635,8.567872339480658e-06
4380,16710,0,16710,0.882009744644165,8.5506666213363e-06
4387,16736,0,16736,0.8830587863922119,8.454646565681268e-06
4394,16765,0,16765,0.8841938972473145,8.403403735870667e-06
4401,16793,0,16793,0.8852987289428711,8.375151568356282e-06
4409,16822,0,16822,0.886483907699585,8.237904935696999e-06
4416,16849,0,16849,0.8875529766082764,8.125384577675353e-06
4423,16877,0,16877,0.8886809349060059,8.066818201069684e-06
4430,16904,0,16904,0.8898088932037354,7.98293583830649e-06
4437,16933,0,16933,0.8909597396850586,7.950697524327242e-06
4444,16962,0,16962,0.8920729160308838,7.930865143676378e-06
4451,16990,0,16990,0.8931708335876465,7.912779983280635e-06
4458,17018,0,17018,0.8942608833312988,7.897194740828278e-06
4466,17052,0,17052,0.89556884765625,7.881135983774613e-06
4473,17079,0,17079,0.8966598510742188,7.833155645469218e-06
4480,17105,0,17105,0.8977179527282715,7.711330001397188e-06
4487,17132,0,17132,0.8987917900085449,7.631491509694346e-06
4494,17158,0,17158,0.899965763092041,7.4812922036708895e-06
4501,17186,0,17186,0.9011218547821045,7.444719897514147e-06
4508,17212,0,17212,0.9022047519683838,7.363263194517682e-06
4515,17238,0,17238,0.903282880783081,7.2109003415544e-06
4523,17268,0,17268,0.9044897556304932,7.00094737421988e-06
4530,17293,0,17293,0.9055328369140625,6.786117364686484e-06
4537,17319,0,17319,0.9065768718719482,6.649227633860014e-06
4544,17345,0,17345,0.9076416492462158,6.52133082443982e-06
4551,17374,0,17374,0.9087507724761963,6.4492834948843345e-06
4558,17403,0,17403,0.909949779510498,6.412369438113758e-06
4565,17431,0,17431,0.9111688137054443,6.360861737096741e-06
4572,17456,0,17456,0.9122307300567627,6.239467866819655e-06
4580,17487,0,17487,0.9135339260101318,6.117432828317573e-06
4587,17514,0,17514,0.9146387577056885,6.052148074979043e-06
4594,17542,0,17542,0.9157419204711914,6.015432017695119e-06
4601,17570,0,17570,0.9173128604888916,5.993270405763718e-06
4608,17598,0,17598,0.918449878692627,5.975906904087513e-06
4615,17627,0,17627,0.9197030067443848,5.962974515879388e-06
4622,17655,0,17655,0.9208476543426514,5.947879491740868e-06
4629,17683,0,17683,0.9219996929168701,5.9347412346461154e-06
4637,17715,0,17715,0.9232947826385498,5.894230359413664e-06
4644,17743,0,17743,0.9244039058685303,5.865563049512942e-06
4651,17771,0,17771,0.9255058765411377,5.850235051276248e-06
4658,17797,0,17797,0.9265639781951904,5.776045004267489e-06
4665,17824,0,17824,0.9277377128601074,5.705417781512533e-06
4672,17850,0,17850,0.9288387298583984,5.6132675329743594e-06
4679,17875,0,17875,0.9298858642578125,5.5133260977171535e-06
4686,17901,0,17901,0.9310269355773926,5.424377785631242e-06
4693,17927,0,17927,0.932110071182251,5.306975639160921e-06
4701,17958,0,17958,0.9333889484405518,5.234186642550911e-06
4708,17982,0,17982,0.9344549179077148,5.1253459750734575e-06
4715,18011,0,18011,0.9356117248535156,5.054762060569852e-06
4722,18039,0,18039,0.9368939399719238,5.024106062638304e-06
4729,18064,0,18064,0.9379758834838867,4.922271450422502e-06
4736,18092,0,18092,0.939140796661377,4.8421595622172034e-06
4743,18120,0,18120,0.9402799606323242,4.817441592308211e-06
4750,18146,0,18146,0.9413816928863525,4.739386745088535e-06
4758,18175,0,18175,0.9426379203796387,4.593591371959052e-06
4765,18202,0,18202,0.943922758102417,4.517480762066167e-06
4772,18227,0,18227,0.945084810256958,4.442501856255591e-06
4779,18251,0,18251,0.9461908340454102,4.269514567863426e-06
4786,18275,0,18275,0.9472978115081787,4.1576425464411565e-06
4793,18301,0,18301,0.9484028816223145,4.0628322724842086e-06
4800,18324,0,18324,0.9494309425354004,3.939598969417445e-06
4807,18350,0,18350,0.950516939163208,3.808400035921573e-06
4815,18379,0,18379,0.9518866539001465,3.6891592650294947e-06
4822,18402,0,18402,0.952908992767334,3.578051014307724e-06
4829,18426,0,18426,0.953941822052002,3.374358125032806e-06
4836,18451,0,18451,0.9550168514251709,3.256210841261218e-06
4843,18475,0,18475,0.956049919128418,3.102618103400824e-06
4850,18500,0,18500,0.9572169780731201,2.9909759011387317e-06
4857,18523,0,18523,0.9582226276397705,2.877700256671949e-06
4864,18547,0,18547,0.9592719078063965,2.7573679028558805e-06
4872,18577,0,18577,0.9605166912078857,2.702885664542084e-06
4879,18602,0,18602,0.9615528583526611,2.5977166501669936e-06
4886,18627,0,18627,0.9626078605651855,2.533794039333388e-06
4893,18656,0,18656,0.9637627601623535,2.5158206038185286e-06
4900,18682,0,18682,0.9648559093475342,2.4876524837491206e-06
4907,18706,0,18706,0.9658827781677246,2.4284676665887886e-06
4914,18733,0,18733,0.9669806957244873,2.375193813609605e-06
4921,18761,0,18761,0.9680817127227783,2.3566086371212654e-06
4929,18793,0,18793,0.9693398475646973,2.3280507025467444e-06
4936,18820,0,18820,0.97039794921875,2.3068536200540477e-06
4943,18847,0,18847,0.9714457988739014,2.2747471580720454e-06
4950,18871,0,18871,0.972491979598999,2.2007284801468767e-06
4957,18895,0,18895,0.9735748767852783,2.1258262799367606e-06
4964,18923,0,18923,0.9746899604797363,2.0973174529891647e-06
4971,18949,0,18949,0.975740909576416,2.0720471403672393e-06
4978,18975,0,18975,0.9767918586730957,2.017185519732861e-06
4985,19003,0,19003,0.9778878688812256,1.992931660899429e-06
4993,19033,0,19033,0.9790949821472168,1.949085936642089e-06
5000,19061,0,19061,0.9801967144012451,1.931064753957067e-06
5007,19086,0,19086,0.9812288284301758,1.8967965802329886e-06
5014,19114,0,19114,0.9823269844055176,1.8742815249590714e-06
5021,19142,0,19142,0.983529806137085,1.8641516630888594e-06
5028,19170,0,19170,0.9846358299255371,1.85776979610943e-06
5035,19198,0,19198,0.9857180118560791,1.8521412721419384e-06
5042,19226,0,19226,0.9868090152740479,1.8475122612015278e-06
5050,19258,0,19258,0.9880478382110596,1.8426418066558836e-06
5057,19286,0,19286,0.9891538619995117,1.8386377287714619e-06
5064,19314,0,19314,0.9902687072753906,1.834642341217786e-06
5071,19342,0,19342,0.9913437366485596,1.830833880908308e-06
5078,19370,0,19370,0.9924228191375732,1.8272093369249092e-06
5085,19398,0,19398,0.9935088157653809,1.8235740311842954e-06
5092,19426,0,19426,0.9946408271789551,1.8199878894167726e-06
5099,19454,0,19454,0.9957537651062012,1.8164538093218398e-06
5107,19486,0,19486,0.996978759765625,1.812463414923315e-06
5114,19514,0,19514,0.9980499744415283,1.80902055924182e-06
5121,19542,0,19542,0.9991178512573242,1.805566248440609e-06
5128,19570,0,19570,1.0003130435943604,1.8021341817349568e-06
5135,19598,0,19598,1.0014269351959229,1.7987337633291773e-06
5142,19626,0,19626,1.0025477409362793,1.7953352929193646e-06
5149,19654,0,19654,1.0037438869476318,1.7919531525910234e-06
5156,19682,0,19682,1.0048549175262451,1.7885861800373124e-06
5164,19714,0,19714,1.0061087608337402,1.7847416523032487e-06
5171,19738,0,19738,1.007124900817871,1.7697578544957163e-06
5178,19763,0,19763,1.0082528591156006,1.7186344097747858e-06
5185,19789,0,19789,1.0093088150024414,1.678481981608128e-06
5192,19812,0,19812,1.01031494140625,1.6204310564030227e-06
5199,19838,0,19838,1.0113739967346191,1.5882653969275065e-06
5206,19864,0,19864,1.0126678943634033,1.559843503814501e-06
5213,19892,0,19892,1.0138769149780273,1.5416640446912937e-06
5221,19923,0,19923,1.0151610374450684,1.5154893566718594e-06
5228,19949,0,19949,1.0162327289581299,1.4982131854180366e-06
5235,19976,0,19976,1.0173308849334717,1.472451237640657e-06
5242,20003,0,20003,1.0184249877929688,1.4537190065257862e-06
5249,20031,0,20031,1.0195319652557373,1.445868069439153e-06
5256,20058,0,20058,1.0206897258758545,1.4321474948515283e-06
5263,20086,0,20086,1.0218768119812012,1.425181924094748e-06
5270,20116,0,20116,1.0230367183685303,1.4209312421952117e-06
5277,20144,0,20144,1.0241899490356445,1.4174080237419364e-06
5285,20176,0,20176,1.025493860244751,1.41365693152687e-06
5292,20205,0,20205,1.0266637802124023,1.4106334563810138e-06
5299,20233,0,20233,1.0278027057647705,1.4074605291056993e-06
5306,20261,0,20261,1.0289368629455566,1.404108560386468e-06
5313,20289,0,20289,1.0300710201263428,1.401059820949211e-06
5320,20317,0,20317,1.0312068462371826,1.3979825797770744e-06
5327,20345,0,20345,1.0323357582092285,1.3950305494655155e-06
5334,20373,0,20373,1.0334959030151367,1.3920911165433214e-06
5342,20405,0,20405,1.0348389148712158,1.3888320501514812e-06
5349,20433,0,20433,1.0360028743743896,1.3859928620006938e-06
5356,20461,0,20461,1.0371577739715576,1.383186538734237e-06
5363,20489,0,20489,1.0383307933807373,1.3804088939823479e-06
5370,20517,0,20517,1.0394937992095947,1.377656396167564e-06
5377,20545,0,20545,1.0406489372253418,1.374931271866723e-06
5384,20573,0,20573,1.0418148040771484,1.3722277134224162e-06
5391,20601,0,20601,1.043001651763916,1.3695419823160564e-06
5399,20632,0,20632,1.0443530082702637,1.3581596616382485e-06
5406,20659,0,20659,1.0455007553100586,1.347166644060398e-06
5413,20688,0,20688,1.0467476844787598,1.3403837987992603e-06
5420,20714,0,20714,1.0479059219360352,1.3164725753443858e-06
5427,20740,0,20740,1.049137830734253,1.2994881547845611e-06
5434,20768,0,20768,1.0504539012908936,1.2925082459933033e-06
5441,20795,0,20795,1.0516548156738281,1.2821995949038718e-06
5448,20820,0,20820,1.0527846813201904,1.264280138896828e-06
5456,20848,0,20848,1.0539987087249756,1.2289612471161277e-06
5463,20873,0,20873,1.0550768375396729,1.1942926991668088e-06
5470,20897,0,20897,1.0561509132385254,1.160192410454563e-06
5477,20920,0,20920,1.0571787357330322,1.0984547704216998e-06
5484,20941,0,20941,1.0581817626953125,1.038086456966703e-06
5491,20967,0,20967,1.0592586994171143,9.954071647475085e-07
5498,20991,0,20991,1.0603058338165283,9.635778445681718e-07
5505,21015,0,21015,1.0613276958465576,9.210107288980169e-07
5513,21042,0,21042,1.062485933303833,8.712513165424523e-07
5520,21067,0,21067,1.0635528564453125,8.410736624959489e-07
5527,21091,0,21091,1.0645737648010254,8.216189031140384e-07
5534,21117,0,21117,1.0656607151031494,7.934125031926161e-07
5541,21141,0,21141,1.066868782043457,7.726452264423939e-07
5548,21168,0,21168,1.068070888519287,7.56750092974531e-07
5555,21195,0,21195,1.0692689418792725,7.448205965692736e-07
5562,21223,0,21223,1.0704870223999023,7.385575874058622e-07
5569,21251,0,21251,1.0716867446899414,7.32544074008361e-07
5577,21281,0,21281,1.0729467868804932,7.188907004369247e-07
5584,21309,0,21309,1.074082851409912,7.125491510814963e-07
5591,21335,0,21335,1.0752618312835693,6.997171312130624e-07
5598,21360,0,21360,1.0762968063354492,6.818423226811764e-07
5605,21385,0,21385,1.077544927597046,6.591813465214124e-07
5612,21411,0,21411,1.0786738395690918,6.432833078043371e-07
5619,21437,0,21437,1.0798640251159668,6.294756707631467e-07
5626,21464,0,21464,1.080948829650879,6.20293505374798e-07
5634,21490,0,21490,1.0821118354797363,5.975964949633523e-07
5641,21518,0,21518,1.0832419395446777,5.896208785010172e-07
5648,21545,0,21545,1.0843279361724854,5.837114681549216e-07
5655,21573,0,21573,1.085420846939087,5.799913861455536e-07
5662,21597,0,21597,1.0864698886871338,5.660091967535813e-07
5669,21623,0,21623,1.087547779083252,5.505441066204511e-07
5676,21647,0,21647,1.0885937213897705,5.349683196561116e-07
5683,21672,0,21672,1.0896167755126953,5.181209410350948e-07
5691,21702,0,21702,1.0908088684082031,5.020943059387169e-07
5698,21727,0,21727,1.0918378829956055,4.84928044850314e-07
5705,21752,0,21752,1.09287691116333,4.684481512555906e-07
5712,21781,0,21781,1.0939807891845703,4.62123671617737e-07
5719,21806,0,21806,1.095181941986084,4.539397198121354e-07
5726,21830,0,21830,1.096275806427002,4.3809130478363e-07
5733,21855,0,21855,1.0975968837738037,4.3095700173913065e-07
5740,21879,0,21879,1.0988409519195557,4.1560943580855173e-07
5748,21906,0,21906,1.1000146865844727,4.017649148212277e-07
5755,21933,0,21933,1.1011450290679932,3.954238876834197e-07
5762,21961,0,21961,1.1022958755493164,3.915168090384025e-07
5769,21988,0,21988,1.1034138202667236,3.868378148356825e-07
5776,22015,0,22015,1.1045448780059814,3.8048225437357324e-07
5783,22042,0,22042,1.105654001235962,3.76254498088536e-07
5790,22068,0,22068,1.1068389415740967,3.7020379777817243e-07
5797,22095,0,22095,1.1087048053741455,3.6700079480461726e-07
5805,22125,0,22125,1.1112098693847656,3.610367766666603e-07
5812,22152,0,22152,1.1135847568511963,3.5826574828440987e-07
5819,22180,0,22180,1.1162469387054443,3.5694138975150476e-07
5826,22207,0,22207,1.1181249618530273,3.552653039880038e-07
5833,22236,0,22236,1.1201977729797363,3.5361237877496177e-07
5840,22264,0,22264,1.1220898628234863,3.5256411104808687e-07
5847,22292,0,22292,1.1239008903503418,3.5028933492130584e-07
5854,22320,0,22320,1.1256937980651855,3.4862630076328547e-07
5862,22350,0,22350,1.1271889209747314,3.446158315205192e-07
5869,22377,0,22377,1.1286067962646484,3.41062901763455e-07
5876,22406,0,22406,1.129856824874878,3.3849990867842644e-07
5883,22433,0,22433,1.1310839653015137,3.353952880523819e-07
5890,22459,0,22459,1.1323556900024414,3.3236791272981936e-07
5897,22483,0,22483,1.1335699558258057,3.167740101663338e-07
5904,22510,0,22510,1.1348137855529785,3.119773807207617e-07
5911,22538,0,22538,1.1360077857971191,3.102611316913229e-07
5918,22566,0,22566,1.1371979713439941,3.079567343660073e-07
5926,22595,0,22595,1.1384468078613281,3.018756932111967e-07
5933,22620,0,22620,1.1395347118377686,2.972486416888085e-07
5940,22644,0,22644,1.140617847442627,2.887701786534975e-07
5947,22670,0,22670,1.1418049335479736,2.8059215847672803e-07
5954,22692,0,22692,1.1428589820861816,2.658580468820237e-07
5961,22714,0,22714,1.1439290046691895,2.5229994344404835e-07
5968,22741,0,22741,1.1452698707580566,2.4718638720619736e-07
5975,22768,0,22768,1.1470329761505127,2.4325543872321186e-07
5983,22800,0,22800,1.148484706878662,2.410557947082424e-07
5990,22826,0,22826,1.1496467590332031,2.3746809699079085e-07
5997,22851,0,22851,1.1507837772369385,2.3204470655020929e-07
6004,22879,0,22879,1.1523559093475342,2.2927561416612984e-07
6011,22905,0,22905,1.1543388366699219,2.2495627854734406e-07
6018,22927,0,22927,1.1556198596954346,2.1119130703411246e-07
6025,22949,0,22949,1.1567168235778809,1.9868545488322546e-07
6032,22976,0,22976,1.157923936843872,1.9403947988662943e-07
6040,23007,0,23007,1.1601216793060303,1.9125009072630712e-07
6047,23033,0,23033,1.1618969440460205,1.8912638099946534e-07
6054,23060,0,23060,1.1636247634887695,1.858711415401725e-07
6061,23087,0,23087,1.1648297309875488,1.8371929847093338e-07
6068,23114,0,23114,1.1664838790893555,1.8190436562136438e-07
6075,23141,0,23141,1.1683666706085205,1.7901500607988515e-07
6082,23167,0,23167,1.1700928211212158,1.7643445480375886e-07
6089,23195,0,23195,1.1722428798675537,1.7532637513568309e-07
6097,23225,0,23225,1.174069881439209,1.7185034800781566e-07
6104,23251,0,23251,1.1755356788635254,1.6791994916984303e-07
6111,23278,0,23278,1.1771557331085205,1.656211946937023e-07
6118,23306,0,23306,1.1791768074035645,1.646637883450899e-07
6125,23334,0,23334,1.180506706237793,1.6404777415764635e-07
6132,23361,0,23361,1.181931972503662,1.622420424182464e-07
6139,23389,0,23389,1.1832859516143799,1.617581200511066e-07
6146,23418,0,23418,1.1846997737884521,1.61353383412383e-07
6154,23450,0,23450,1.1863737106323242,1.6089237234744713e-07
6161,23478,0,23478,1.1876866817474365,1.6055994706685064e-07
6168,23505,0,23505,1.1889078617095947,1.5982263299209343e-07
6175,23532,0,23532,1.190220832824707,1.5783085382845765e-07
6182,23559,0,23559,1.191478967666626,1.549554374708023e-07
6189,23585,0,23585,1.1929118633270264,1.5218023377987237e-07
6196,23610,0,23610,1.194133996963501,1.4871168600776222e-07
6203,23637,0,23637,1.1957628726959229,1.4579365456126706e-07
6210,23664,0,23664,1.1977388858795166,1.4397714559393878e-07
6218,23694,0,23694,1.2001068592071533,1.4078790750154024e-07
6225,23716,0,23716,1.202272891998291,1.3406588622257367e-07
6232,23740,0,23740,1.2037708759307861,1.2840005246811214e-07
6239,23764,0,23764,1.2056238651275635,1.2320995761313044e-07
6246,23790,0,23790,1.2077267169952393,1.1969911058371017e-07
6253,23814,0,23814,1.2094767093658447,1.1631395965821431e-07
6260,23837,0,23837,1.2112739086151123,1.109475402182988e-07
6267,23861,0,23861,1.212683916091919,1.0721919750799521e-07
6275,23890,0,23890,1.2144460678100586,1.0415657986266825e-07
6282,23914,0,23914,1.2162506580352783,1.0066299232493574e-07
6289,23937,0,23937,1.2185766696929932,9.552508020751961e-08
6296,23959,0,23959,1.220780849456787,8.941861058580304e-08
6303,23983,0,23983,1.222890853881836,8.504164520361131e-08
6310,24009,0,24009,1.2251908779144287,8.268043863538359e-08
6317,24035,0,24035,1.2269058227539062,8.07681621624949e-08
6324,24059,0,24059,1.2286148071289062,7.799762074773434e-08
6332,24088,0,24088,1.2301807403564453,7.53602591464044e-08
6339,24114,0,24114,1.2315287590026855,7.329828947892965e-08
6346,24139,0,24139,1.233124017715454,7.158356696221928e-08
6353,24165,0,24165,1.2345006465911865,7.001675324756151e-08
6360,24192,0,24192,1.2357537746429443,6.886564224699489e-08
6367,24220,0,24220,1.237149953842163,6.846784033797885e-08
6374,24248,0,24248,1.2384228706359863,6.821367387740686e-08
6381,24278,0,24278,1.2396719455718994,6.804287535361769e-08
6389,24308,0,24308,1.2410669326782227,6.738594318803002e-08
6396,24333,0,24333,1.2422277927398682,6.629616971300999e-08
6403,24360,0,24360,1.24344801902771,6.530762160225094e-08
6410,24388,0,24388,1.2451567649841309,6.482625312694687e-08
6417,24415,0,24415,1.2473647594451904,6.40090698625337e-08
6424,24443,0,24443,1.2493019104003906,6.368593637519847e-08
6431,24471,0,24471,1.2513427734375,6.349123428929812e-08
6438,24500,0,24500,1.2535128593444824,6.334941290269927e-08
6446,24531,0,24531,1.2556958198547363,6.278816351042726e-08
6453,24559,0,24559,1.2571418285369873,6.255933301255271e-08
6460,24587,0,24587,1.2590408325195312,6.202181382238197e-08
6467,24613,0,24613,1.2603929042816162,6.124092096668293e-08
6474,24637,0,24637,1.261551856994629,5.953473004034816e-08
6481,24660,0,24660,1.26320481300354,5.722141716800324e-08
6488,24686,0,24686,1.2646310329437256,5.603668312077355e-08
6495,24712,0,24712,1.266737699508667,5.481798382645805e-08
6502,24738,0,24738,1.2688438892364502,5.3743544170113136e-08
6510,24767,0,24767,1.2707996368408203,5.235508685808024e-08
6517,24790,0,24790,1.2722139358520508,5.017141156987596e-08
6524,24814,0,24814,1.2733278274536133,4.7974064676849904e-08
6531,24840,0,24840,1.2744958400726318,4.679389140060203e-08
6538,24866,0,24866,1.2760980129241943,4.5665111948413035e-08
6545,24890,0,24890,1.2774949073791504,4.407700828288062e-08
6552,24914,0,24914,1.2790958881378174,4.263934528185718e-08
6559,24941,0,24941,1.280493974685669,4.15800010898813e-08
6567,24972,0,24972,1.2824387550354004,4.088466730703086e-08
6574,24998,0,24998,1.2845370769500732,3.995304547378445e-08
6581,25025,0,25025,1.2864477634429932,3.9302179548649204e-08
6588,25052,0,25052,1.2879819869995117,3.889840989338453e-08
6595,25079,0,25079,1.2891676425933838,3.8239501318146574e-08
6602,25105,0,25105,1.2904508113861084,3.7526969035147006e-08
6609,25132,0,25132,1.2917358875274658,3.719940340058367e-08
6616,25159,0,25159,1.2932348251342773,3.670006599348233e-08
6624,25186,0,25186,1.295137882232666,3.5633068247866875e-08
6631,25210,0,25210,1.297070026397705,3.415980399628645e-08
6638,25236,0,25236,1.2983908653259277,3.340261580171718e-08
6645,25262,0,25262,1.2998828887939453,3.278402444038555e-08
6652,25290,0,25290,1.3018558025360107,3.250116332658021e-08
6659,25316,0,25316,1.3031537532806396,3.195037322548931e-08
6666,25342,0,25342,1.3043358325958252,3.134957353039177e-08
6673,25369,0,25369,1.3055589199066162,3.090872546294765e-08
6681,25396,0,25396,1.3069298267364502,3.012329880449105e-08
6688,25420,0,25420,1.3089609146118164,2.890473792294e-08
6695,25446,0,25446,1.3106427192687988,2.8092278823109895e-08
6702,25473,0,25473,1.3127498626708984,2.7472754744714492e-08
6709,25499,0,25499,1.314894676208496,2.6827691378402163e-08
6716,25526,0,25526,1.3167457580566406,2.646944243258327e-08
6723,25554,0,25554,1.3187358379364014,2.633838195293228e-08
6730,25581,0,25581,1.3209667205810547,2.6061284268189556e-08
6738,25613,0,25613,1.323084831237793,2.595442436204398e-08
6745,25640,0,25640,1.324652910232544,2.5735643549487033e-08
6752,25665,0,25665,1.3264949321746826,2.5271271589189814e-08
6759,25691,0,25691,1.328622817993164,2.477755980797033e-08
6766,25718,0,25718,1.3300299644470215,2.446318627902478e-08
6773,25745,0,25745,1.3313498497009277,2.3932733841027068e-08
6780,25768,0,25768,1.3328838348388672,2.335266245651199e-08
6787,25789,0,25789,1.3343846797943115,2.2210743834025936e-08
6795,25816,0,25816,1.3361327648162842,2.0932202311687303e-08
6802,25842,0,25842,1.3378627300262451,2.040440098157445e-08
6809,25868,0,25868,1.339167833328247,2.0096140819927015e-08
6816,25892,0,25892,1.3404889106750488,1.9177135753395474e-08
6823,25915,0,25915,1.341728925704956,1.813233196163259e-08
6830,25939,0,25939,1.3431217670440674,1.7497994307691187e-08
6837,25961,0,25961,1.3446409702301025,1.6488556132170505e-08
6844,25983,0,25983,1.3460469245910645,1.5541888774750502e-08
6851,26007,0,26007,1.3472037315368652,1.5043871848760217e-08
6859,26039,0,26039,1.3487768173217773,1.4884040122489372e-08
6866,26066,0,26066,1.3504607677459717,1.4721687521431587e-08
6873,26093,0,26093,1.3520028591156006,1.4533439393935259e-08
6880,26122,0,26122,1.3532178401947021,1.4445587289163424e-08
6887,26150,0,26150,1.3543989658355713,1.437543241674673e-08
6894,26179,0,26179,1.3557937145233154,1.4323264105039165e-08
6901,26206,0,26206,1.356935739517212,1.4210069510019986e-08
6908,26234,0,26234,1.3582940101623535,1.4153244119117331e-08
6916,26265,0,26265,1.360172986984253,1.4016677987115124e-08
6923,26292,0,26292,1.3613708019256592,1.3914316263596191e-08
6930,26322,0,26322,1.3628008365631104,1.3827452385260206e-08
6937,26350,0,26350,1.364576816558838,1.3780112982257053e-08
6944,26375,0,26375,1.3661978244781494,1.3503196236270455e-08
6951,26402,0,26402,1.3681137561798096,1.3334135039533535e-08
6958,26431,0,26431,1.3701376914978027,1.3264678173552399e-08
6965,26457,0,26457,1.371931791305542,1.3079852267916881e-08
6973,26489,0,26489,1.3738007545471191,1.2922729100255456e-08
6980,26517,0,26517,1.3750598430633545,1.2850715957532644e-08
6987,26546,0,26546,1.3763267993927002,1.2739923409418842e-08
6994,26574,0,26574,1.3779399394989014,1.2685881710418764e-08
7001,26602,0,26602,1.3802008628845215,1.265182947873991e-08
7008,26631,0,26631,1.3818669319152832,1.2623969365917846e-08
7015,26659,0,26659,1.38307785987854,1.2596657139843705e-08
7022,26687,0,26687,1.3853378295898438,1.2569828558874095e-08
7030,26719,0,26719,1.3882238864898682,1.254199941796893e-08
7037,26748,0,26748,1.3908028602600098,1.2517169470982984e-08
7044,26776,0,26776,1.3927710056304932,1.249231440058803e-08
7051,26803,0,26803,1.3940048217773438,1.2397835135615102e-08
7058,26832,0,26832,1.3954269886016846,1.2352355738618232e-08
7065,26862,0,26862,1.3978769779205322,1.2322687793900526e-08
7072,26888,0,26888,1.3997266292572021,1.2116588802743922e-08
7079,26914,0,26914,1.4013350009918213,1.191157221430938e-08
7087,26942,0,26942,1.4034810066223145,1.1540681023622197e-08
7094,26966,0,26966,1.4055218696594238,1.128305730847928e-08
7101,26990,0,26990,1.4067997932434082,1.0696609958148983e-08
7108,27017,0,27017,1.4079537391662598,1.0444120161463193e-08
7115,27039,0,27039,1.4093990325927734,9.967935277830401e-09


==> plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00011301040649414062,4.387072431292609
1,3,0,3,0.00021696090698242188,3.9719937673698036
2,6,0,6,0.0005321502685546875,3.603279457162108
3,8,0,8,0.0007698535919189453,2.5747483139919263
4,11,0,11,0.0010509490966796875,2.3821779761310036
5,13,0,13,0.001280069351196289,1.5284154711849578
6,16,0,16,0.001558065414428711,1.4544037375349537
7,18,0,18,0.0017781257629394531,1.1578500511436216
8,21,0,21,0.0020439624786376953,1.1078200497689445
9,23,0,23,0.0022389888763427734,0.8205300174792192
10,26,0,26,0.0024662017822265625,0.7828090634793574
11,28,0,28,0.0026688575744628906,0.5904335259461263
12,31,0,31,0.0028810501098632812,0.5604305383001765
13,33,0,33,0.003165006637573242,0.4164400016335764
14,36,0,36,0.0034499168395996094,0.4029047476909755
15,38,0,38,0.0036590099334716797,0.34735376671285706
16,41,0,41,0.003976106643676758,0.33434149110626726
17,43,0,43,0.004236936569213867,0.24756978913335823
18,46,0,46,0.0045719146728515625,0.2409097710242463
19,48,0,48,0.004848957061767578,0.1834515429409959
20,51,0,51,0.0053369998931884766,0.18031175088544588
21,53,0,53,0.005614042282104492,0.15618647131006888
22,56,0,56,0.00586700439453125,0.15307297626153776
23,59,0,59,0.006173133850097656,0.15036750884012243
24,61,0,61,0.0064699649810791016,0.12920014138647526
25,64,0,64,0.006768941879272461,0.12662399358928159
26,66,0,66,0.00706791877746582,0.10695245010079718
27,69,0,69,0.00742793083190918,0.10574280743643055
28,71,0,71,0.007742166519165039,0.0809080860106374
29,74,0,74,0.008087873458862305,0.08004463590673186
30,76,0,76,0.008288145065307617,0.06452922396598361
31,79,0,79,0.008507966995239258,0.0638503852946247
32,81,0,81,0.008692026138305664,0.06168907852433439
33,84,0,84,0.008906126022338867,0.06139635380811543
34,86,0,86,0.009103059768676758,0.06127304660417731
35,89,0,89,0.00933694839477539,0.060974523646598514
36,91,0,91,0.009527206420898438,0.0608998066699066
37,94,0,94,0.009745121002197266,0.06056476298718032
38,96,0,96,0.00994110107421875,0.05917650741552297
39,99,0,99,0.010159969329833984,0.058766825732600024
40,101,0,101,0.010350942611694336,0.05644538238148135
41,104,0,104,0.010689020156860352,0.05612953844198272
42,106,0,106,0.010950088500976562,0.054612055556663756
43,109,0,109,0.01129293441772461,0.054439113489907466
44,111,0,111,0.011613130569458008,0.053131353155977314
45,114,0,114,0.011967182159423828,0.052902817062805835
46,116,0,116,0.012221097946166992,0.0500650836771471
47,119,0,119,0.012521982192993164,0.049764449500167965
48,122,0,122,0.012881040573120117,0.0495074205064623
49,124,0,124,0.013196945190429688,0.048209525062440084
50,127,0,127,0.013548851013183594,0.04795411879639343
51,129,0,129,0.013763904571533203,0.044266066724762305
52,132,0,132,0.014003992080688477,0.04370687090977983
53,134,0,134,0.014201879501342773,0.0436517968686343
54,137,0,137,0.014472007751464844,0.04310351934711104
55,139,0,139,0.014689207077026367,0.04031307861543956
56,142,0,142,0.014918088912963867,0.0397557646513919
57,144,0,144,0.015148162841796875,0.037232088003547444
58,147,0,147,0.015578031539916992,0.03681522592621644
59,149,0,149,0.0159609317779541,0.034221877814705745
60,152,0,152,0.017466068267822266,0.03372964428198596
61,154,0,154,0.017802000045776367,0.03202848740227118
62,157,0,157,0.018130064010620117,0.03150612847922555
63,159,0,159,0.018463134765625,0.031113326965804815
64,162,0,162,0.01881885528564453,0.03067794407746471
65,164,0,164,0.019154071807861328,0.02975234068019789
66,167,0,167,0.01950812339782715,0.02944773800323907
67,169,0,169,0.019789934158325195,0.027440228552082363
68,172,0,172,0.020077943801879883,0.027237737006693286
69,174,0,174,0.020300865173339844,0.026758224983282494
70,177,0,177,0.020622968673706055,0.02664691852573306
71,179,0,179,0.02085113525390625,0.026544883667046645
72,182,0,182,0.02120208740234375,0.0264653465563549
73,184,0,184,0.021479129791259766,0.026154654664001787
74,187,0,187,0.021964073181152344,0.02609952591587975
75,189,0,189,0.02230691909790039,0.025907100093064777
76,192,0,192,0.02264094352722168,0.0258586646290572
77,194,0,194,0.022938966751098633,0.025787682299508275
78,197,0,197,0.023257970809936523,0.025748718874631666
79,199,0,199,0.023553133010864258,0.025626850641597393
80,202,0,202,0.023916244506835938,0.025606022163826802
81,204,0,204,0.024219989776611328,0.02546420714535368
82,207,0,207,0.02455902099609375,0.025444108300930184
83,209,0,209,0.024882078170776367,0.025394788985711323
84,212,0,212,0.0252230167388916,0.025374433914411645
85,214,0,214,0.025504112243652344,0.02534302525643383
86,216,0,216,0.025789976119995117,0.025342498206268483
87,219,0,219,0.02617621421813965,0.025327023702289547
88,221,0,221,0.026445865631103516,0.0252956857088296
89,224,0,224,0.026803016662597656,0.025279498752621515
90,226,0,226,0.027018070220947266,0.025249211758632432
91,229,0,229,0.027247905731201172,0.0252358314099076
92,231,0,231,0.027524948120117188,0.025159974680363743
93,234,0,234,0.027781963348388672,0.025149440649797045
94,236,0,236,0.028051137924194336,0.02509783001752685
95,239,0,239,0.02822399139404297,0.025085649293457565
96,241,0,241,0.028361082077026367,0.025057795223862547
97,244,0,244,0.028522014617919922,0.025046714103002937
98,246,0,246,0.028657913208007812,0.02500596984367437
99,249,0,249,0.028815031051635742,0.02499863335724485
100,251,0,251,0.028950214385986328,0.024993959393221098
101,253,0,253,0.0290830135345459,0.024991382343046018
102,255,0,255,0.029215097427368164,0.024989854426610066
103,257,0,257,0.02935004234313965,0.024987107037376857
104,259,0,259,0.029545068740844727,0.02498364327247985
105,261,0,261,0.029733896255493164,0.024982501370369007
106,263,0,263,0.029927968978881836,0.02498137153239303
107,265,0,265,0.030153989791870117,0.024976051869763812
108,267,0,267,0.030360937118530273,0.024974937796555782
109,269,0,269,0.03060317039489746,0.02497320473077321
110,272,0,272,0.030849933624267578,0.0249615320921041
111,274,0,274,0.031045913696289062,0.024886214233830896
112,277,0,277,0.03127884864807129,0.024872036007287244
113,279,0,279,0.03146982192993164,0.02483130442153756
114,282,0,282,0.03170204162597656,0.024815547033058043
115,284,0,284,0.03189897537231445,0.02479792863186847
116,286,0,286,0.03215909004211426,0.024796866996042288
117,288,0,288,0.032404184341430664,0.024790972642931838
118,290,0,290,0.03266596794128418,0.024788740301041515
119,292,0,292,0.032878875732421875,0.024788001662920677
120,294,0,294,0.03307509422302246,0.024785850734190415
121,296,0,296,0.03326606750488281,0.024784016175308194
122,299,0,299,0.03361916542053223,0.024765925155254078
123,301,0,301,0.03394007682800293,0.024576297414966433
124,304,0,304,0.034214019775390625,0.024552995515626952
125,306,0,306,0.03445792198181152,0.024471271071650445
126,309,0,309,0.03476214408874512,0.02443408979126522
127,311,0,311,0.035127878189086914,0.024141797852023975
128,314,0,314,0.0353701114654541,0.02407880534083864
129,316,0,316,0.03552389144897461,0.02402117201753717
130,319,0,319,0.03568911552429199,0.023958535150324586
131,321,0,321,0.03582501411437988,0.023729016216612855
132,324,0,324,0.035984039306640625,0.023607182107820975
133,326,0,326,0.0361180305480957,0.0230078352557911
134,329,0,329,0.03627514839172363,0.022819945872296455
135,331,0,331,0.0364079475402832,0.022032807339049484
136,334,0,334,0.03656506538391113,0.021846831239892492
137,336,0,336,0.03670001029968262,0.021585636393457817
138,339,0,339,0.03691720962524414,0.021417468165791483
139,341,0,341,0.037079811096191406,0.02100380303764967
140,344,0,344,0.03726387023925781,0.020788884250652732
141,346,0,346,0.03740811347961426,0.0204742098725414
142,349,0,349,0.03756999969482422,0.020236094613916046
143,351,0,351,0.03770804405212402,0.019131646143650677
144,354,0,354,0.037869930267333984,0.018792637564216043
145,356,0,356,0.03800797462463379,0.017343749412532968
146,359,0,359,0.03816986083984375,0.01710527758145567
147,361,0,361,0.03830695152282715,0.01641636972280587
148,364,0,364,0.03851819038391113,0.016253488409619318
149,366,0,366,0.038671016693115234,0.01578188720826893
150,369,0,369,0.0388340950012207,0.01562648798947684
151,371,0,371,0.0390019416809082,0.015430063922102732
152,374,0,374,0.03918600082397461,0.015276090539853413
153,376,0,376,0.0393218994140625,0.01411833878954429
154,379,0,379,0.03948187828063965,0.013934999614757014
155,381,0,381,0.03961801528930664,0.013266927227990449
156,384,0,384,0.03977608680725098,0.01311509975729869
157,386,0,386,0.03992605209350586,0.012824218451721728
158,389,0,389,0.04007887840270996,0.01269524527086348
159,391,0,391,0.040209054946899414,0.012190265791544022
160,394,0,394,0.04036116600036621,0.012089135316601753
161,396,0,396,0.04049110412597656,0.011547975854943042
162,399,0,399,0.04064297676086426,0.011411486012810248
163,401,0,401,0.04077291488647461,0.011270140614958431
164,404,0,404,0.040940046310424805,0.011142639607613029
165,406,0,406,0.04106712341308594,0.010597146338311469
166,409,0,409,0.041216135025024414,0.010466316851957598
167,411,0,411,0.041342973709106445,0.010404531975239772
168,414,0,414,0.041491031646728516,0.010280276859588128
169,416,0,416,0.04161691665649414,0.009869283024349824
170,419,0,419,0.041764020919799805,0.009737523863655406
171,421,0,421,0.04189014434814453,0.008773457507487292
172,424,0,424,0.04204988479614258,0.008619009013584622
173,427,0,427,0.04219818115234375,0.008489056440499717
174,429,0,429,0.042320966720581055,0.007900929406002068
175,432,0,432,0.04246401786804199,0.007802461428474801
176,434,0,434,0.04258584976196289,0.007543900175039028
177,437,0,437,0.04272913932800293,0.007463155358667415
178,439,0,439,0.04287123680114746,0.006520011765501445
179,442,0,442,0.04301714897155762,0.006389877450190307
180,444,0,444,0.0431361198425293,0.0062900238111562225
181,447,0,447,0.04327511787414551,0.006137020680160475
182,449,0,449,0.04339599609375,0.005177381695832927
183,452,0,452,0.04354381561279297,0.0050562270361787474
184,454,0,454,0.04366302490234375,0.004876074961915767
185,457,0,457,0.04380393028259277,0.004730040800397637
186,459,0,459,0.04393815994262695,0.004055893409929831
187,462,0,462,0.04409503936767578,0.003960162362777105
188,464,0,464,0.04425311088562012,0.00370362644891699
189,467,0,467,0.04439210891723633,0.0036143987664560115
190,469,0,469,0.04450702667236328,0.0031656085684533004
191,472,0,472,0.04464292526245117,0.0031056538275489112
192,474,0,474,0.04476594924926758,0.0029918523569502234
193,477,0,477,0.0449831485748291,0.00293982405180531
194,479,0,479,0.04515480995178223,0.00253455428491232
195,482,0,482,0.04536008834838867,0.00249898374513087
196,484,0,484,0.04553103446960449,0.002474336427367068
197,487,0,487,0.04573512077331543,0.002433294677734731
198,489,0,489,0.045905113220214844,0.0022439270961719165
199,492,0,492,0.04612898826599121,0.0022050102106286186
200,494,0,494,0.046305179595947266,0.0021689956442589543
201,497,0,497,0.04651498794555664,0.002137744002808717
202,499,0,499,0.04670286178588867,0.0020116149523409497
203,502,0,502,0.04694104194641113,0.0019877599157594435
204,504,0,504,0.04714703559875488,0.0019095381678440563
205,507,0,507,0.04739999771118164,0.0018873453848715289
206,509,0,509,0.047811031341552734,0.0018091411381228862
207,512,0,512,0.048316001892089844,0.0017885529548749125
208,514,0,514,0.04868602752685547,0.0016826610162362576
209,517,0,517,0.049037933349609375,0.0016640432162830924
210,519,0,519,0.049330949783325195,0.0016483526510358301
211,522,0,522,0.04972410202026367,0.0016279030772106946
212,524,0,524,0.05001497268676758,0.0015044515973380444
213,527,0,527,0.0503849983215332,0.001479620966214013
214,529,0,529,0.05099821090698242,0.0013185673275580795
215,532,0,532,0.051319122314453125,0.0012951043338754495
216,534,0,534,0.051579952239990234,0.0012110029287347147
217,537,0,537,0.05181288719177246,0.001192705723050191
218,539,0,539,0.05206012725830078,0.0011819396165242257
219,542,0,542,0.0523679256439209,0.0011661012018266538
220,544,0,544,0.052642822265625,0.0010467948065573092
221,547,0,547,0.05294489860534668,0.0010279736887212224
222,549,0,549,0.053192138671875,0.0009909863748644178
223,551,0,551,0.05345010757446289,0.0009894920451172186
224,554,0,554,0.05374908447265625,0.000963760608805123
225,556,0,556,0.05401611328125,0.0008766083219467356
226,559,0,559,0.05431699752807617,0.0008548523255813485
227,561,0,561,0.054572105407714844,0.0007620566064714051
228,564,0,564,0.054888010025024414,0.0007534762638939558
229,566,0,566,0.05504298210144043,0.0007260146398137649
230,569,0,569,0.055322885513305664,0.0007178767840691969
231,571,0,571,0.05558300018310547,0.0006954834515069214
232,574,0,574,0.055886030197143555,0.0006910703548144164
233,576,0,576,0.05616283416748047,0.0006887804571151704
234,579,0,579,0.05649709701538086,0.0006839450899692996
235,581,0,581,0.05676698684692383,0.0006432233543448019
236,584,0,584,0.05704307556152344,0.000638511480277454
237,586,0,586,0.057244062423706055,0.00060988795707488
238,589,0,589,0.05746912956237793,0.0006069789037122359
239,591,0,591,0.05765199661254883,0.0006060963331889226
240,594,0,594,0.05786705017089844,0.0006036073978859348
241,596,0,596,0.05806398391723633,0.0005933888838318112
242,599,0,599,0.05828404426574707,0.000591552218993424
243,601,0,601,0.05846691131591797,0.0005847079034844904
244,604,0,604,0.05868196487426758,0.0005829447560491637
245,606,0,606,0.0588529109954834,0.0005802944200858546
246,609,0,609,0.059085845947265625,0.0005791446715277945
247,611,0,611,0.05928301811218262,0.0005767298080078308
248,614,0,614,0.059519052505493164,0.0005754504953198641
249,616,0,616,0.05965399742126465,0.0005657650565495023
250,619,0,619,0.05980801582336426,0.0005644642594745028
251,621,0,621,0.05994892120361328,0.0005637232417403873
252,623,0,623,0.060151100158691406,0.0005636444435034568
253,626,0,626,0.06031012535095215,0.0005622719577539522
254,628,0,628,0.06045198440551758,0.0005536826302070262
255,631,0,631,0.06066012382507324,0.0005522368748636804
256,633,0,633,0.06085991859436035,0.0005498372979590759
257,636,0,636,0.06105208396911621,0.0005484538733158137
258,638,0,638,0.06118416786193848,0.0005452853440957309
259,641,0,641,0.06142020225524902,0.0005436786765546807
260,643,0,643,0.061579227447509766,0.0005382002040336667
261,646,0,646,0.061795949935913086,0.0005364176075670393
262,648,0,648,0.06193804740905762,0.0005314111200103819
263,651,0,651,0.06213998794555664,0.0005296618789994999
264,653,0,653,0.0622859001159668,0.0005264300784876542
265,656,0,656,0.06245112419128418,0.0005249949530219674
266,658,0,658,0.0625920295715332,0.0005212800315797323
267,661,0,661,0.06274914741516113,0.0005199097073329166
268,663,0,663,0.06287908554077148,0.0005153765654150362
269,666,0,666,0.06306910514831543,0.0005140877245702443
270,668,0,668,0.06322813034057617,0.0005122886325368135
271,671,0,671,0.06342887878417969,0.000510974055471679
272,673,0,673,0.06365704536437988,0.0005049583418592644
273,676,0,676,0.0639488697052002,0.0005034300907572648
274,678,0,678,0.06416916847229004,0.0005011762572038463
275,681,0,681,0.06445097923278809,0.0004995448455843385
276,683,0,683,0.06470203399658203,0.000496974642442954
277,686,0,686,0.06499791145324707,0.0004951783280730511
278,688,0,688,0.06528592109680176,0.00047732540741248766
279,691,0,691,0.06552600860595703,0.0004741688845189487
280,693,0,693,0.06573200225830078,0.00047168767473510165
281,696,0,696,0.06596803665161133,0.00046917060715243546
282,698,0,698,0.06613302230834961,0.0004549222033980456
283,701,0,701,0.06646203994750977,0.0004528003038105315
284,703,0,703,0.06673598289489746,0.00044840015785050275
285,706,0,706,0.06704401969909668,0.0004468388757815337
286,708,0,708,0.0673379898071289,0.00044320355727656857
287,711,0,711,0.06763982772827148,0.0004419478595868406
288,713,0,713,0.06788301467895508,0.00043703816062178616
289,716,0,716,0.06819486618041992,0.00043513583534072033
290,718,0,718,0.06843996047973633,0.0004191211657486192
291,721,0,721,0.06874823570251465,0.00041740191628130416
292,723,0,723,0.06891822814941406,0.00041624704000501115
293,726,0,726,0.06907296180725098,0.0004147849113722279
294,728,0,728,0.06922602653503418,0.0004080471465126638
295,731,0,731,0.06937885284423828,0.0004063008094412667
296,733,0,733,0.06950688362121582,0.00039551102154432543
297,736,0,736,0.0696558952331543,0.00039454857697394414
298,738,0,738,0.06978321075439453,0.000391855117426603
299,741,0,741,0.0699310302734375,0.0003911133033861798
300,743,0,743,0.07005715370178223,0.00038890515782799936
301,746,0,746,0.07020401954650879,0.0003882364326896722
302,748,0,748,0.07033109664916992,0.0003868646162171148
303,751,0,751,0.07047796249389648,0.000385850007901088
304,753,0,753,0.0706479549407959,0.00038457347405757014
305,756,0,756,0.07086491584777832,0.00038360819766040786
306,758,0,758,0.07104110717773438,0.0003752177168757174
307,761,0,761,0.0711979866027832,0.0003739627569382523
308,763,0,763,0.07132911682128906,0.00036886391954423403
309,766,0,766,0.0714871883392334,0.00036808819915625033
310,768,0,768,0.07161712646484375,0.00036764825487375176
311,771,0,771,0.07176899909973145,0.0003668135060765918
312,773,0,773,0.07202315330505371,0.0003622745666131673
313,776,0,776,0.07223796844482422,0.00036168238665567216
314,778,0,778,0.07242822647094727,0.00035881562980467056
315,781,0,781,0.0725860595703125,0.0003580674288140866
316,783,0,783,0.07271695137023926,0.0003577176225254508
317,786,0,786,0.07288622856140137,0.00035693274500571854
318,788,0,788,0.07301115989685059,0.0003552139639632777
319,791,0,791,0.07315897941589355,0.000354238381361204
320,793,0,793,0.07328391075134277,0.00034993160396381835
321,796,0,796,0.07343125343322754,0.00034917813283925046
322,798,0,798,0.07361006736755371,0.00034697584763186256
323,801,0,801,0.07391023635864258,0.0003460562395217318
324,803,0,803,0.07420921325683594,0.00034419849008489556
325,806,0,806,0.07454395294189453,0.00034318064013698444
326,808,0,808,0.07482600212097168,0.00034022455386258565
327,811,0,811,0.07516813278198242,0.00033872489797023207
328,813,0,813,0.07545995712280273,0.00032774785413820475
329,816,0,816,0.07575607299804688,0.000326564993184197
330,818,0,818,0.0760490894317627,0.00031825751201886065
331,821,0,821,0.07635116577148438,0.0003162388512086076
332,823,0,823,0.07689309120178223,0.0003140544469543526
333,826,0,826,0.07730793952941895,0.0003122895961240771
334,828,0,828,0.07761287689208984,0.0003003932183434371
335,831,0,831,0.0779259204864502,0.00029848936409578557
336,833,0,833,0.07812213897705078,0.00029547095758248525
337,836,0,836,0.07836294174194336,0.0002934910281422496
338,838,0,838,0.07850313186645508,0.0002853873883397469
339,841,0,841,0.07865619659423828,0.0002827330616546176
340,843,0,843,0.07878804206848145,0.00027266295755995414
341,846,0,846,0.07894301414489746,0.0002702773418232661
342,848,0,848,0.0790719985961914,0.0002644157017310618
343,851,0,851,0.07921910285949707,0.0002618870748126798
344,853,0,853,0.0793449878692627,0.00025742842353550807
345,856,0,856,0.07948994636535645,0.0002552199947426567
346,858,0,858,0.07962703704833984,0.00024501689719540166
347,861,0,861,0.07977414131164551,0.00024378783412825144
348,863,0,863,0.07989692687988281,0.0002383733775789626
349,866,0,866,0.0800788402557373,0.0002369709340086945
350,868,0,868,0.08026885986328125,0.00023462673446606507
351,871,0,871,0.08043503761291504,0.00023338524146235832
352,873,0,873,0.0806119441986084,0.00022964927319791965
353,876,0,876,0.08083105087280273,0.00022884944313829016
354,878,0,878,0.08101201057434082,0.00022642822571360775
355,881,0,881,0.08122611045837402,0.00022552735031151403
356,883,0,883,0.08141088485717773,0.00022444287149530343
357,886,0,886,0.08163905143737793,0.00022372155730665603
358,888,0,888,0.08177804946899414,0.0002203615582223416
359,891,0,891,0.08192801475524902,0.00021956171512195434
360,893,0,893,0.08205389976501465,0.000214797150712168
361,896,0,896,0.08220195770263672,0.00021388747397525177
362,898,0,898,0.08232784271240234,0.00020972574033888296
363,901,0,901,0.08247518539428711,0.00020873954453772803
364,903,0,903,0.08272123336791992,0.00020689152777978443
365,906,0,906,0.0830390453338623,0.0002061567775991051
366,908,0,908,0.08329296112060547,0.0002039854427838234
367,911,0,911,0.08358311653137207,0.00020329976981956394
368,913,0,913,0.08381915092468262,0.00020154719915999714
369,916,0,916,0.08398294448852539,0.00020083750919142193
370,918,0,918,0.08411312103271484,0.00019926852422992255
371,921,0,921,0.08426189422607422,0.0001984406213327379
372,923,0,923,0.08438515663146973,0.00019674587767157367
373,926,0,926,0.08453106880187988,0.00019600508477326552
374,928,0,928,0.08465385437011719,0.0001937212907685551
375,931,0,931,0.08479809761047363,0.00019310243652884279
376,933,0,933,0.08493494987487793,0.00019155544776269502
377,936,0,936,0.08509182929992676,0.00019101194784878564
378,938,0,938,0.0852210521697998,0.0001899501514901634
379,941,0,941,0.08537721633911133,0.0001893441353202228
380,943,0,943,0.08550524711608887,0.00018542267788023518
381,946,0,946,0.08565521240234375,0.0001845137440818155
382,948,0,948,0.08578205108642578,0.00018271696582157336
383,951,0,951,0.08593225479125977,0.00018204047932453851
384,953,0,953,0.08609390258789062,0.00017798255186442257
385,956,0,956,0.08635306358337402,0.00017705262822411918
386,958,0,958,0.0865640640258789,0.00017625021070770828
387,961,0,961,0.08672690391540527,0.00017543503517634086
388,963,0,963,0.08686017990112305,0.0001676633514864088
389,966,0,966,0.08701205253601074,0.00016658191448072501
390,969,0,969,0.08716392517089844,0.00016565113872978697
391,971,0,971,0.08729195594787598,0.0001620685879205377
392,974,0,974,0.08744311332702637,0.00016094839994793426
393,976,0,976,0.08757400512695312,0.00015806781566014583
394,979,0,979,0.08772420883178711,0.00015654591786572989
395,981,0,981,0.08785009384155273,0.0001535684553886544
396,984,0,984,0.08801484107971191,0.00015262576961840905
397,986,0,986,0.08814024925231934,0.00014457023952426499
398,989,0,989,0.08828616142272949,0.00014365029364286412
399,991,0,991,0.0884089469909668,0.0001424809604604232
400,994,0,994,0.08855414390563965,0.00014154734228989972
401,996,0,996,0.08868217468261719,0.00013734079000176578
402,999,0,999,0.08882689476013184,0.00013660293788666245
403,1001,0,1001,0.08896398544311523,0.00013251847722251986
404,1004,0,1004,0.08910489082336426,0.00013121173697745907
405,1006,0,1006,0.08922600746154785,0.0001274625395361197
406,1009,0,1009,0.08936715126037598,0.0001261287465087035
407,1011,0,1011,0.08948683738708496,0.00012433653465412827
408,1014,0,1014,0.08962702751159668,0.00012290837675663072
409,1016,0,1016,0.08974599838256836,0.0001148769434841501
410,1019,0,1019,0.0898890495300293,0.00011339350208295875
411,1021,0,1021,0.09000802040100098,0.00010453702448192062
412,1024,0,1024,0.0901479721069336,0.00010297552415078646
413,1026,0,1026,0.09026694297790527,9.042052313465832e-05
414,1029,0,1029,0.09040713310241699,8.879494750226464e-05
415,1032,0,1032,0.0905461311340332,8.736981415042966e-05
416,1034,0,1034,0.09066414833068848,8.269933951465789e-05
417,1037,0,1037,0.0908050537109375,8.111841789272786e-05
418,1039,0,1039,0.09093999862670898,7.621500314492363e-05
419,1042,0,1042,0.09108495712280273,7.49983198493641e-05
420,1044,0,1044,0.09120607376098633,6.588195282040015e-05
421,1047,0,1047,0.09135007858276367,6.523744276065e-05
422,1049,0,1049,0.09147310256958008,6.387867014976528e-05
423,1052,0,1052,0.09161806106567383,6.326461724445657e-05
424,1054,0,1054,0.09173989295959473,6.12177507910992e-05
425,1057,0,1057,0.09188604354858398,6.0734805784862444e-05
426,1059,0,1059,0.09202790260314941,5.4822123148567635e-05
427,1062,0,1062,0.09217691421508789,5.404710506813866e-05
428,1064,0,1064,0.09230399131774902,5.3577745908468054e-05
429,1067,0,1067,0.0924530029296875,5.270157320775314e-05
430,1069,0,1069,0.09257984161376953,4.95068549538471e-05
431,1072,0,1072,0.0927278995513916,4.857943124786631e-05
432,1074,0,1074,0.09287905693054199,4.5446559188426654e-05
433,1077,0,1077,0.09303617477416992,4.440169568636559e-05
434,1079,0,1079,0.09316420555114746,4.1138378842994205e-05
435,1082,0,1082,0.09331321716308594,4.038369170932972e-05
436,1084,0,1084,0.09344005584716797,3.701231335414682e-05
437,1087,0,1087,0.09358811378479004,3.614516447703074e-05
438,1089,0,1089,0.09371495246887207,3.5092948495037376e-05
439,1092,0,1092,0.09386396408081055,3.446530827810914e-05
440,1094,0,1094,0.09400510787963867,2.9389689929199545e-05
441,1097,0,1097,0.09428215026855469,2.883554220258123e-05
442,1099,0,1099,0.09456801414489746,2.8110294710354895e-05
443,1102,0,1102,0.09488105773925781,2.773161643650222e-05
444,1104,0,1104,0.09515500068664551,2.641212506688725e-05
445,1107,0,1107,0.09545302391052246,2.605084142077559e-05
446,1109,0,1109,0.09575414657592773,2.377743078472058e-05
447,1112,0,1112,0.09612917900085449,2.3446995114178253e-05
448,1114,0,1114,0.09644603729248047,2.2920342346875814e-05
449,1117,0,1117,0.09676408767700195,2.2590318398964677e-05
450,1119,0,1119,0.09703397750854492,2.070021924232252e-05
451,1122,0,1122,0.09734797477722168,2.0428716340895525e-05
452,1124,0,1124,0.09761905670166016,1.9316264121496507e-05
453,1127,0,1127,0.09885025024414062,1.9029111624083498e-05
454,1129,0,1129,0.09943103790283203,1.9018867173368354e-05
455,1132,0,1132,0.09986495971679688,1.8704396366345255e-05
456,1134,0,1134,0.10019993782043457,1.7096168261401418e-05
457,1137,0,1137,0.1005258560180664,1.6759791572329233e-05
458,1139,0,1139,0.10078191757202148,1.5049209183100374e-05
459,1142,0,1142,0.10109305381774902,1.4772200274937666e-05
460,1144,0,1144,0.10136198997497559,1.456655607378357e-05
461,1147,0,1147,0.10166406631469727,1.4320559516835536e-05
462,1149,0,1149,0.1019432544708252,1.4115192759272597e-05
463,1152,0,1152,0.10221290588378906,1.3895370849042113e-05
464,1154,0,1154,0.1024179458618164,1.160799908244687e-05
465,1157,0,1157,0.10264396667480469,1.1496695736729792e-05
466,1159,0,1159,0.10284090042114258,1.1417086832705952e-05
467,1162,0,1162,0.1030721664428711,1.1313605704082058e-05
468,1164,0,1164,0.10326313972473145,1.0963240435929785e-05
469,1167,0,1167,0.10349392890930176,1.0872777266937686e-05
470,1170,0,1170,0.10372495651245117,1.079291627294913e-05
471,1172,0,1172,0.10391783714294434,1.029273284421237e-05
472,1175,0,1175,0.10416293144226074,1.0197901512737987e-05
473,1177,0,1177,0.10442996025085449,9.637221858779567e-06
474,1180,0,1180,0.10466599464416504,9.559990636186515e-06
475,1182,0,1182,0.10482120513916016,9.465201064285316e-06
476,1185,0,1185,0.10499215126037598,9.390973031617546e-06
477,1187,0,1187,0.10513806343078613,9.21562510664092e-06
478,1190,0,1190,0.10537409782409668,9.140117346309221e-06
479,1192,0,1192,0.10560178756713867,8.503614302801095e-06
480,1195,0,1195,0.10583686828613281,8.435232972985004e-06
481,1197,0,1197,0.10598111152648926,8.417681801520858e-06
482,1200,0,1200,0.10614681243896484,8.353050215316486e-06
483,1202,0,1202,0.10628414154052734,8.035298199946566e-06
484,1205,0,1205,0.10644412040710449,7.981391467865321e-06
485,1207,0,1207,0.10658907890319824,7.804991701963421e-06
486,1210,0,1210,0.10683703422546387,7.76132874322662e-06
487,1212,0,1212,0.10706591606140137,7.679766771126224e-06
488,1215,0,1215,0.10734796524047852,7.642421676006113e-06
489,1217,0,1217,0.10755109786987305,7.5296603209471354e-06
490,1220,0,1220,0.10777401924133301,7.480657245427223e-06
491,1222,0,1222,0.10795903205871582,7.429750801504634e-06
492,1225,0,1225,0.10817694664001465,7.372231825980338e-06
493,1227,0,1227,0.10835909843444824,7.183200304721797e-06
494,1230,0,1230,0.10857605934143066,7.124343369316845e-06
495,1232,0,1232,0.10876297950744629,6.828475285953329e-06
496,1235,0,1235,0.10900211334228516,6.786209276682111e-06
497,1237,0,1237,0.10918903350830078,6.508089059784384e-06
498,1240,0,1240,0.10940909385681152,6.470104958209587e-06
499,1242,0,1242,0.10959601402282715,6.459220489141117e-06
500,1245,0,1245,0.10980892181396484,6.415088915301154e-06
501,1247,0,1247,0.10996007919311523,5.767499942250243e-06
502,1250,0,1250,0.11011600494384766,5.681995012666865e-06
503,1252,0,1252,0.11024713516235352,5.635283923824104e-06
504,1255,0,1255,0.11040806770324707,5.555960637609182e-06
505,1257,0,1257,0.11059117317199707,5.206801194649771e-06
506,1260,0,1260,0.11075806617736816,5.140742031582461e-06
507,1262,0,1262,0.11089015007019043,4.824835402991116e-06
508,1265,0,1265,0.11104393005371094,4.781188183116045e-06
509,1267,0,1267,0.1111750602722168,4.67930979866105e-06
510,1270,0,1270,0.1113271713256836,4.610407347000589e-06
511,1272,0,1272,0.11146306991577148,4.413448481895368e-06
512,1275,0,1275,0.11165595054626465,4.363245006110899e-06
513,1277,0,1277,0.11184406280517578,4.287457277833019e-06
514,1280,0,1280,0.11207008361816406,4.2480817631348104e-06
515,1282,0,1282,0.1122739315032959,4.156048970321303e-06
516,1285,0,1285,0.11252689361572266,4.110732154228557e-06
517,1287,0,1287,0.11275601387023926,3.968329041685237e-06
518,1290,0,1290,0.11301112174987793,3.936688471539518e-06
519,1292,0,1292,0.11321091651916504,3.831653968580201e-06
520,1295,0,1295,0.11351418495178223,3.794550412686309e-06
521,1297,0,1297,0.11383605003356934,3.6495593903191764e-06
522,1300,0,1300,0.11415505409240723,3.627477177922878e-06
523,1302,0,1302,0.11445212364196777,3.3807763075003555e-06
524,1305,0,1305,0.11479306221008301,3.354252522571791e-06
525,1307,0,1307,0.1150522232055664,3.3183363526408734e-06
526,1310,0,1310,0.11547493934631348,3.29156462492025e-06
527,1312,0,1312,0.11574196815490723,3.277771222987111e-06
528,1315,0,1315,0.11606788635253906,3.2521717227725894e-06
529,1317,0,1317,0.11647391319274902,3.043226963928818e-06
530,1320,0,1320,0.11796402931213379,3.015860700304135e-06
531,1322,0,1322,0.11834597587585449,2.8991929378810733e-06
532,1325,0,1325,0.11868715286254883,2.8596894418134744e-06
533,1327,0,1327,0.11905598640441895,2.8389204217676324e-06
534,1329,0,1329,0.1193540096282959,2.8375612737680786e-06
535,1332,0,1332,0.11968302726745605,2.799612838986582e-06
536,1334,0,1334,0.11995291709899902,2.538971883339705e-06
537,1337,0,1337,0.12026500701904297,2.4755810613254833e-06
538,1339,0,1339,0.1205589771270752,2.3912625979395218e-06
539,1342,0,1342,0.12089204788208008,2.3294491419911636e-06
540,1344,0,1344,0.1211690902709961,2.0215008336655964e-06
541,1347,0,1347,0.1215050220489502,1.997293412105047e-06
542,1349,0,1349,0.12174797058105469,1.919395253296541e-06
543,1352,0,1352,0.12201714515686035,1.8944443923802444e-06
544,1354,0,1354,0.12224006652832031,1.8485568607462421e-06
545,1357,0,1357,0.12250709533691406,1.818122094654074e-06
546,1359,0,1359,0.1227719783782959,1.5861860129572106e-06
547,1362,0,1362,0.12312507629394531,1.574057604718784e-06
548,1365,0,1365,0.12337017059326172,1.5631790810234462e-06
549,1367,0,1367,0.12356686592102051,1.518779600421288e-06
550,1370,0,1370,0.12379288673400879,1.5064133017711964e-06
551,1372,0,1372,0.12398505210876465,1.4934332861540848e-06
552,1375,0,1375,0.12421798706054688,1.4820238554273696e-06
553,1377,0,1377,0.12450003623962402,1.4054410000757548e-06
554,1380,0,1380,0.12482595443725586,1.3940175648318174e-06
555,1382,0,1382,0.12511301040649414,1.3344403143190267e-06
556,1385,0,1385,0.12549591064453125,1.3239326677329289e-06
557,1387,0,1387,0.1257610321044922,1.3205765499182668e-06
558,1390,0,1390,0.12608599662780762,1.3104033421434842e-06
559,1392,0,1392,0.12635087966918945,1.2261881577905354e-06
560,1395,0,1395,0.12664103507995605,1.2170471925184867e-06
561,1397,0,1397,0.12691116333007812,1.2055198843934083e-06
562,1400,0,1400,0.12721896171569824,1.1968708085093869e-06
563,1402,0,1402,0.1274890899658203,1.1759807307705794e-06
564,1405,0,1405,0.12774896621704102,1.1682296073955922e-06
565,1407,0,1407,0.1279439926147461,1.142968068497633e-06
566,1410,0,1410,0.1281900405883789,1.134084976349064e-06
567,1412,0,1412,0.12833499908447266,1.113814547606519e-06
568,1415,0,1415,0.12849688529968262,1.1079983878346925e-06
569,1417,0,1417,0.12867999076843262,1.079425120811968e-06
570,1420,0,1420,0.12894511222839355,1.0695001854125733e-06
571,1422,0,1422,0.12914204597473145,1.0547633350804992e-06
572,1425,0,1425,0.12936902046203613,1.045630769097356e-06
573,1427,0,1427,0.12955904006958008,1.002162123678714e-06
574,1430,0,1430,0.12977910041809082,9.86994147713235e-07
575,1432,0,1432,0.12996220588684082,9.548009605795478e-07
576,1435,0,1435,0.13019084930419922,9.417723642120751e-07
577,1437,0,1437,0.13032793998718262,7.929523325148092e-07
578,1440,0,1440,0.1305990219116211,7.805102026430853e-07
579,1442,0,1442,0.13085007667541504,7.523986388088494e-07
580,1445,0,1445,0.13114094734191895,7.426206263239531e-07
581,1447,0,1447,0.13138914108276367,7.212471399646794e-07
582,1450,0,1450,0.13168001174926758,7.118033594079328e-07
583,1452,0,1452,0.1319279670715332,6.663906440594595e-07
584,1455,0,1455,0.13217592239379883,6.590556323428829e-07
585,1457,0,1457,0.1323850154876709,5.879794323312678e-07
586,1460,0,1460,0.1326150894165039,5.818111516082263e-07
587,1462,0,1462,0.13286113739013672,5.600508566840352e-07
588,1465,0,1465,0.13313603401184082,5.534660575162157e-07
589,1467,0,1467,0.13338398933410645,5.274412266557018e-07
590,1470,0,1470,0.13365507125854492,5.213578840699602e-07
591,1472,0,1472,0.13388991355895996,5.002927105787785e-07
592,1475,0,1475,0.13413310050964355,4.936327004151889e-07
593,1477,0,1477,0.13434505462646484,4.636050421784175e-07
594,1480,0,1480,0.1345810890197754,4.5615801684290073e-07
595,1482,0,1482,0.1347339153289795,4.060611282187766e-07
596,1485,0,1485,0.13490009307861328,3.997113411615038e-07
597,1487,0,1487,0.1350400447845459,3.921967592975495e-07
598,1490,0,1490,0.13520002365112305,3.8797843786212184e-07
599,1492,0,1492,0.13533306121826172,3.6208188220557375e-07
600,1495,0,1495,0.13548994064331055,3.5583921202712114e-07
601,1497,0,1497,0.13562393188476562,3.4225385869734613e-07
602,1500,0,1500,0.13577985763549805,3.371550080198476e-07
603,1502,0,1502,0.1359109878540039,3.0683429785830947e-07
604,1505,0,1505,0.13608002662658691,3.019894599182677e-07
605,1507,0,1507,0.13620901107788086,2.972006030756682e-07
606,1510,0,1510,0.13635993003845215,2.931295680388044e-07
607,1512,0,1512,0.1364879608154297,2.745286645631176e-07
608,1515,0,1515,0.13663816452026367,2.720456668242411e-07
609,1517,0,1517,0.13676714897155762,2.6632121442757374e-07
610,1520,0,1520,0.1369180679321289,2.640228244465936e-07
611,1522,0,1522,0.13704609870910645,2.5390625064275436e-07
612,1525,0,1525,0.13719797134399414,2.5066521339504135e-07
613,1527,0,1527,0.13733506202697754,2.4418215460096256e-07
614,1530,0,1530,0.1374959945678711,2.417825789985812e-07
615,1532,0,1532,0.13762903213500977,2.3124824298157101e-07
616,1535,0,1535,0.13778209686279297,2.2873201891937197e-07
617,1537,0,1537,0.1379101276397705,2.225303377192742e-07
618,1540,0,1540,0.1380608081817627,2.2034925302485412e-07
619,1542,0,1542,0.13818812370300293,2.1568330879013655e-07
620,1545,0,1545,0.13833880424499512,2.1390081920446974e-07
621,1547,0,1547,0.13846611976623535,2.0888988511702286e-07
622,1550,0,1550,0.13861703872680664,2.074213914356843e-07
623,1552,0,1552,0.13874483108520508,2.0297579736125035e-07
624,1555,0,1555,0.13889503479003906,2.020683122994079e-07
625,1557,0,1557,0.13902711868286133,1.9786989514855383e-07
626,1560,0,1560,0.13917803764343262,1.9695437523368433e-07
627,1562,0,1562,0.13930416107177734,1.9609296658452972e-07
628,1565,0,1565,0.13945412635803223,1.9532811112028172e-07
629,1567,0,1567,0.13958311080932617,1.9245937882262533e-07
630,1570,0,1570,0.13973307609558105,1.9152312278692564e-07
631,1572,0,1572,0.1398611068725586,1.8693708285751703e-07
632,1575,0,1575,0.14001202583312988,1.8609342969893066e-07
633,1577,0,1577,0.14013910293579102,1.8462924022719573e-07
634,1580,0,1580,0.14029192924499512,1.8399502273011834e-07
635,1582,0,1582,0.14042401313781738,1.810051451007273e-07
636,1585,0,1585,0.14057612419128418,1.805551456815927e-07
637,1587,0,1587,0.14070510864257812,1.7848935796068045e-07
638,1590,0,1590,0.14085698127746582,1.7806257385343602e-07
639,1592,0,1592,0.1410069465637207,1.779045805049451e-07
640,1594,0,1594,0.14113211631774902,1.778841498025305e-07
641,1596,0,1596,0.14125609397888184,1.7785738828132427e-07
642,1598,0,1598,0.14137983322143555,1.7778751327187154e-07
643,1601,0,1601,0.1415271759033203,1.7739526092763882e-07
644,1603,0,1603,0.14165210723876953,1.7541512452397732e-07
645,1606,0,1606,0.1417999267578125,1.7494261846388963e-07
646,1608,0,1608,0.14192605018615723,1.7312028831124264e-07
647,1611,0,1611,0.1420738697052002,1.7267829134144452e-07
648,1613,0,1613,0.14219903945922852,1.7071489925737407e-07
649,1616,0,1616,0.14234614372253418,1.7021199473275144e-07
650,1618,0,1618,0.1424710750579834,1.6952905711706792e-07
651,1621,0,1621,0.14261794090270996,1.6898155777049971e-07
652,1623,0,1623,0.14274382591247559,1.6519093571587216e-07
653,1626,0,1626,0.14289212226867676,1.6446711154739032e-07
654,1628,0,1628,0.14302921295166016,1.629168540716764e-07
655,1631,0,1631,0.1431729793548584,1.623476926566118e-07
656,1633,0,1633,0.14330005645751953,1.5860447264358823e-07
657,1636,0,1636,0.14344501495361328,1.5781965691525834e-07
658,1638,0,1638,0.14356684684753418,1.5763528758764685e-07
659,1641,0,1641,0.14371013641357422,1.5686448446192974e-07
660,1643,0,1643,0.14388203620910645,1.5389101052167321e-07
661,1646,0,1646,0.14409613609313965,1.5322857369035548e-07
662,1648,0,1648,0.14441609382629395,1.4917743993167482e-07
663,1651,0,1651,0.1447429656982422,1.480633810221551e-07
664,1653,0,1653,0.1450340747833252,1.450870946687687e-07
665,1656,0,1656,0.14533114433288574,1.438412036264245e-07
666,1658,0,1658,0.14557814598083496,1.371928595968352e-07
667,1661,0,1661,0.1458578109741211,1.3606774701815825e-07
668,1663,0,1663,0.14601898193359375,1.3224089320882868e-07
669,1666,0,1666,0.14618206024169922,1.3083748476638483e-07
670,1668,0,1668,0.14631891250610352,1.2178859103339335e-07
671,1671,0,1671,0.14648008346557617,1.200583185346017e-07
672,1673,0,1673,0.14661407470703125,1.1757269514759812e-07
673,1676,0,1676,0.14695501327514648,1.1611421473344387e-07
674,1678,0,1678,0.1472148895263672,1.0697777275327487e-07
675,1681,0,1681,0.14753389358520508,1.055549108150818e-07
676,1683,0,1683,0.147841215133667,9.895056359911035e-08
677,1686,0,1686,0.1482090950012207,9.78323285715369e-08
678,1688,0,1688,0.14851808547973633,9.070577311702179e-08
679,1691,0,1691,0.14884591102600098,8.956292867969454e-08
680,1694,0,1694,0.1490941047668457,8.855126020824265e-08
681,1696,0,1696,0.14932012557983398,8.13626194785863e-08
682,1699,0,1699,0.1495802402496338,8.036353328612543e-08
683,1701,0,1701,0.1497948169708252,7.842395770549923e-08
684,1704,0,1704,0.15005183219909668,7.766449583476945e-08
685,1706,0,1706,0.15035700798034668,7.343032826068544e-08
686,1709,0,1709,0.1507120132446289,7.223277240791524e-08
687,1711,0,1711,0.15101408958435059,7.024125667207271e-08
688,1714,0,1714,0.1512889862060547,6.92421971308087e-08
689,1716,0,1716,0.15144801139831543,6.612517199948632e-08
690,1719,0,1719,0.1516129970550537,6.555548805643118e-08
691,1721,0,1721,0.15182900428771973,6.458022540726504e-08
692,1724,0,1724,0.15207409858703613,6.391964464789463e-08
693,1726,0,1726,0.15227198600769043,6.195841252749546e-08
694,1729,0,1729,0.15250015258789062,6.161661500721421e-08
695,1731,0,1731,0.15269112586975098,6.065638248755814e-08
696,1734,0,1734,0.15291500091552734,6.01589551757732e-08
697,1736,0,1736,0.15311193466186523,5.931018839631262e-08
698,1739,0,1739,0.15332603454589844,5.879402461795209e-08
699,1741,0,1741,0.1535041332244873,5.581059598223322e-08
700,1744,0,1744,0.15372920036315918,5.531951502336182e-08
701,1746,0,1746,0.15392303466796875,5.1474695410801544e-08
702,1749,0,1749,0.1541600227355957,5.084749207908479e-08
703,1751,0,1751,0.15440797805786133,4.9725961539572927e-08
704,1754,0,1754,0.1546928882598877,4.91538501104908e-08
705,1756,0,1756,0.15493202209472656,4.5730537857160135e-08
706,1759,0,1759,0.15523409843444824,4.478451354884494e-08
707,1761,0,1761,0.1554851531982422,4.0364548181640597e-08
708,1764,0,1764,0.1557750701904297,3.971011499501416e-08
709,1766,0,1766,0.15604424476623535,3.91142748016048e-08
710,1769,0,1769,0.15634894371032715,3.8515271047023955e-08
711,1771,0,1771,0.15660595893859863,3.575165587399895e-08
712,1774,0,1774,0.1569061279296875,3.486318146150352e-08
713,1776,0,1776,0.15716910362243652,2.8201353353049965e-08
714,1779,0,1779,0.15745902061462402,2.7764697212636498e-08
715,1781,0,1781,0.1577160358428955,2.7683493411533322e-08
716,1784,0,1784,0.1580209732055664,2.7296384337593946e-08
717,1786,0,1786,0.15825796127319336,2.53461960306916e-08
718,1789,0,1789,0.15852594375610352,2.4958042474497495e-08
719,1791,0,1791,0.15876317024230957,2.4634747687316124e-08
720,1794,0,1794,0.15904593467712402,2.4216845200243603e-08
721,1796,0,1796,0.15928101539611816,2.1868063987713802e-08
722,1799,0,1799,0.15956592559814453,2.150883400500391e-08
723,1801,0,1801,0.159804105758667,2.1018795514225313e-08
724,1804,0,1804,0.16008520126342773,2.0685178721501665e-08
725,1806,0,1806,0.16032195091247559,1.845804243326748e-08
726,1809,0,1809,0.16060400009155273,1.8213326856711394e-08
727,1811,0,1811,0.16083908081054688,1.8207545737969353e-08
728,1814,0,1814,0.16114211082458496,1.794935438501034e-08
729,1816,0,1816,0.16138410568237305,1.58348521604455e-08
730,1819,0,1819,0.16167783737182617,1.561423707243368e-08
731,1821,0,1821,0.16193294525146484,1.500065560985156e-08
732,1824,0,1824,0.16216206550598145,1.4832965230611533e-08
733,1826,0,1826,0.16234707832336426,1.4265813342510977e-08
734,1829,0,1829,0.16256403923034668,1.4136655785552462e-08
735,1831,0,1831,0.16274499893188477,1.3346625189869403e-08
736,1834,0,1834,0.16297411918640137,1.32124393053341e-08
737,1836,0,1836,0.16315698623657227,1.2310525715577536e-08
738,1839,0,1839,0.16340303421020508,1.2194243693592743e-08
739,1841,0,1841,0.1636519432067871,1.2062657468014853e-08
740,1844,0,1844,0.16384387016296387,1.1958705197512337e-08
741,1846,0,1846,0.16401290893554688,1.1540648693760368e-08
742,1849,0,1849,0.1641700267791748,1.1468842546606532e-08
743,1851,0,1851,0.16430401802062988,1.1342357215424276e-08
744,1854,0,1854,0.16448187828063965,1.127684592619382e-08
745,1856,0,1856,0.16466498374938965,1.1194744293280172e-08
746,1859,0,1859,0.16488409042358398,1.1128406757613543e-08
747,1861,0,1861,0.1650850772857666,1.0618194858139142e-08
748,1864,0,1864,0.1655271053314209,1.0507228460887075e-08
749,1866,0,1866,0.16591501235961914,1.0225933506211761e-08
750,1869,0,1869,0.16630101203918457,1.0094031140986934e-08
751,1871,0,1871,0.1665968894958496,9.513732246910624e-09


==> plot_data/quadratic_minimax_problem_n20_alpha00001/iflex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.00010895729064941406,4.387072431292609
2,7,0,7,0.0008800029754638672,3.8559300609188223
4,13,0,13,0.0018200874328613281,3.1805127365100363
7,21,0,21,0.0031538009643554688,2.615570316233742
9,27,0,27,0.004025936126708984,2.191271192448902
11,33,0,33,0.004875898361206055,1.8826796009926408
13,38,0,38,0.00554203987121582,1.5450747111062477
16,46,0,46,0.006451845169067383,1.2951104535495437
18,52,0,52,0.007108926773071289,1.1158175670995938
20,56,0,56,0.007548093795776367,0.7431866161266337
22,62,0,62,0.008030891418457031,0.6516199660515388
24,67,0,67,0.008543968200683594,0.5649756411926242
27,75,0,75,0.009617805480957031,0.45433073002614544
29,81,0,81,0.010355949401855469,0.3871088390019215
31,86,0,86,0.011082887649536133,0.3208279775251849
33,92,0,92,0.011870861053466797,0.2902653527613473
36,101,0,101,0.013031959533691406,0.2552546357138213
38,107,0,107,0.013736963272094727,0.23687583719133645
40,113,0,113,0.014230012893676758,0.22163539267351257
42,117,0,117,0.014692068099975586,0.1676035625280366
44,122,0,122,0.015157938003540039,0.12665917028755536
47,131,0,131,0.015889883041381836,0.1140913424646257
49,137,0,137,0.016371965408325195,0.10820517019885094
51,143,0,143,0.016859054565429688,0.10340568997867958
53,149,0,149,0.017345905303955078,0.09915460262568171
56,159,0,159,0.018095016479492188,0.09569840037841193
58,165,0,165,0.018581867218017578,0.09264126979900225
60,171,0,171,0.019063949584960938,0.08976631271155329
62,177,0,177,0.019551992416381836,0.08712288757616599
64,183,0,183,0.02004098892211914,0.08495728517642527
67,192,0,192,0.02091193199157715,0.08222009826014123
69,198,0,198,0.02172684669494629,0.08060703893336357
71,204,0,204,0.02266097068786621,0.0791255073512142
73,210,0,210,0.02360701560974121,0.07777358802375395
76,219,0,219,0.024927854537963867,0.07634502043921164
78,226,0,226,0.02585291862487793,0.07567029412637268
80,232,0,232,0.026725053787231445,0.07442393602158026
82,238,0,238,0.02763986587524414,0.07304146057554366
84,246,0,246,0.028828859329223633,0.07224563163750264
87,257,0,257,0.030303955078125,0.07125871305496817
89,264,0,264,0.03130316734313965,0.07068488872528286
91,271,0,271,0.032318830490112305,0.07027851854581647
93,279,0,279,0.033255815505981445,0.06976768901557152
96,291,0,291,0.034750938415527344,0.06907298395998851
98,299,0,299,0.03579902648925781,0.06870886340154092
100,306,0,306,0.03681492805480957,0.06719063569697241
102,314,0,314,0.037834882736206055,0.06673418358244398
104,322,0,322,0.03853106498718262,0.06632372019182742
107,332,0,332,0.039407968521118164,0.06602362973826231
109,338,0,338,0.039987802505493164,0.06587926386504214
111,344,0,344,0.04060697555541992,0.06564447479065666
113,350,0,350,0.04111790657043457,0.06545043502837225
116,361,0,361,0.041944026947021484,0.0651556593911532
118,369,0,369,0.04293704032897949,0.0649114535474169
120,377,0,377,0.04395890235900879,0.06466351143612761
122,383,0,383,0.04490995407104492,0.06447667555488906
125,392,0,392,0.04616498947143555,0.064119065234829
127,398,0,398,0.046946048736572266,0.06388373459021203
129,404,0,404,0.047731876373291016,0.06366001823211934
131,410,0,410,0.04842495918273926,0.06343535829850781
133,416,0,416,0.049054861068725586,0.06319900141816029
136,425,0,425,0.04981493949890137,0.06281322227189919
138,431,0,431,0.05032491683959961,0.06252652230101145
140,437,0,437,0.050827980041503906,0.0622117477412763
142,443,0,443,0.051332950592041016,0.061872962522918185
145,452,0,452,0.05208706855773926,0.061334115737910096
147,458,0,458,0.05258989334106445,0.060969575907031025
149,464,0,464,0.05309295654296875,0.06063775500875791
151,470,0,470,0.05359792709350586,0.060484402688794965
153,477,0,477,0.054121971130371094,0.06006632067189576
156,486,0,486,0.05489778518676758,0.05933078297976143
158,492,0,492,0.05540299415588379,0.058455463354690186
160,498,0,498,0.055906057357788086,0.05723633259420055
162,504,0,504,0.056411027908325195,0.05600515889045329
165,513,0,513,0.0572049617767334,0.054248333482093944
167,519,0,519,0.05772209167480469,0.05327974183274877
169,525,0,525,0.0582277774810791,0.05246333317808791
171,531,0,531,0.058740854263305664,0.05178546447548902
173,537,0,537,0.05929112434387207,0.05116051781473578
176,546,0,546,0.06006598472595215,0.0502934540139301
178,552,0,552,0.060575008392333984,0.04979377036454916
180,558,0,558,0.0611119270324707,0.04933007447800771
182,564,0,564,0.061618804931640625,0.048889860661886615
185,573,0,573,0.062374114990234375,0.04822997522597986
187,579,0,579,0.06287789344787598,0.047777032101011085
189,585,0,585,0.06338000297546387,0.04732043341931912
191,591,0,591,0.06388092041015625,0.046875447842948524
193,597,0,597,0.06439590454101562,0.04645611246292111
196,606,0,606,0.06516289710998535,0.04588416782354392
198,612,0,612,0.06583285331726074,0.04553629448636503
200,618,0,618,0.06645393371582031,0.04521093471569802
202,624,0,624,0.06696581840515137,0.04490519508629148
205,633,0,633,0.06773805618286133,0.044478568459481005
207,639,0,639,0.06824278831481934,0.04421384839306528
209,645,0,645,0.06875801086425781,0.04396429125102419
211,651,0,651,0.06924700736999512,0.04373006657212626
213,657,0,657,0.0697319507598877,0.043511437834275274
216,666,0,666,0.07047295570373535,0.043214382561715864
218,672,0,672,0.07100486755371094,0.043040126001650005
220,678,0,678,0.07157397270202637,0.042894145296285956
222,684,0,684,0.07221078872680664,0.042821094895923714
225,695,0,695,0.07305908203125,0.04263548779463991
227,701,0,701,0.0735468864440918,0.04250966506787771
229,709,0,709,0.07414484024047852,0.042417388649961064
231,716,0,716,0.07468795776367188,0.04230931308675669
233,723,0,723,0.07520890235900879,0.042214563532795624
236,735,0,735,0.07603812217712402,0.04208537280144183
238,743,0,743,0.07663607597351074,0.04200507708870703
240,751,0,751,0.07716917991638184,0.04192859398953693
242,759,0,759,0.07770586013793945,0.041855315718832165
245,771,0,771,0.07851386070251465,0.041749357714559336
247,779,0,779,0.0790860652923584,0.041680931553336645
249,787,0,787,0.07961583137512207,0.041614257694008804
251,795,0,795,0.0801551342010498,0.04154944089222986
253,803,0,803,0.08068609237670898,0.041486481590479386
256,815,0,815,0.08150386810302734,0.04139605421772618
258,823,0,823,0.08217215538024902,0.04133970554499109
260,831,0,831,0.08276486396789551,0.041290420834258185
262,840,0,840,0.08352994918823242,0.04124051361546881
265,850,0,850,0.08431005477905273,0.04005523193423162
267,856,0,856,0.08476781845092773,0.0392868659175843
269,862,0,862,0.08519482612609863,0.03873712666934055
271,868,0,868,0.08568906784057617,0.038341561771442885
273,874,0,874,0.08623099327087402,0.038118543709683914
276,883,0,883,0.08693599700927734,0.03785097598498142
278,889,0,889,0.0873568058013916,0.03773035267330131
280,895,0,895,0.08776593208312988,0.037676444303636834
282,902,0,902,0.08830785751342773,0.037637233072617855
285,914,0,914,0.08927607536315918,0.037534479897880196
287,922,0,922,0.0897378921508789,0.03747041768225319
289,930,0,930,0.09019112586975098,0.03740957120854894
291,938,0,938,0.09065794944763184,0.037352145321999236
293,946,0,946,0.0912008285522461,0.03729832313824962
296,958,0,958,0.09188294410705566,0.03723272042965359
298,967,0,967,0.09244990348815918,0.037200309641917964
300,974,0,974,0.09289693832397461,0.03606330327785142
302,982,0,982,0.09358501434326172,0.03567369325370182
305,991,0,991,0.09434390068054199,0.034407239144140775
307,999,0,999,0.09500408172607422,0.03388038448713157
309,1006,0,1006,0.09564208984375,0.03367496834242815
311,1014,0,1014,0.09609484672546387,0.03344163579665906
313,1020,0,1020,0.09650707244873047,0.033282513842686906
316,1031,0,1031,0.09720015525817871,0.032970843270415336
318,1039,0,1039,0.09767389297485352,0.0328324035975801
320,1047,0,1047,0.09829902648925781,0.0327154231367234
322,1055,0,1055,0.09876608848571777,0.032614148104326855
325,1067,0,1067,0.0994410514831543,0.032485549941864686
327,1075,0,1075,0.09989404678344727,0.03241238584572275
329,1083,0,1083,0.1003408432006836,0.03235023631944958
331,1091,0,1091,0.10079598426818848,0.03228607900296913
333,1097,0,1097,0.10120582580566406,0.03225333327353229
336,1107,0,1107,0.10184097290039062,0.03220861136577456
338,1115,0,1115,0.10231280326843262,0.032148688240387545
340,1123,0,1123,0.10277080535888672,0.03209360293008929
342,1131,0,1131,0.10323286056518555,0.03204203082366148
345,1141,0,1141,0.1038661003112793,0.03201323180801919
347,1147,0,1147,0.1042790412902832,0.032006883730057216
349,1153,0,1153,0.10469293594360352,0.032001761818695455
351,1159,0,1159,0.10510778427124023,0.03199914329875191
353,1165,0,1165,0.10550904273986816,0.03199502012808096
356,1174,0,1174,0.10609102249145508,0.031982426826248134
358,1180,0,1180,0.10647296905517578,0.031973584661430236
360,1186,0,1186,0.1068568229675293,0.03196767008844524
362,1192,0,1192,0.10723876953125,0.031965882145057474
365,1204,0,1204,0.10788083076477051,0.03191711318893563
367,1212,0,1212,0.10830903053283691,0.03188541874953381
369,1220,0,1220,0.10873603820800781,0.03185418362965606
371,1227,0,1227,0.1091470718383789,0.03183639280806016
374,1236,0,1236,0.10973310470581055,0.0318149813802028
376,1242,0,1242,0.1101229190826416,0.03179372803564232
378,1248,0,1248,0.11051487922668457,0.03176881903028347
380,1254,0,1254,0.11092090606689453,0.03174067412206088
382,1260,0,1260,0.11133098602294922,0.03170793953230777
385,1269,0,1269,0.11194801330566406,0.03164741923514511
387,1275,0,1275,0.11236190795898438,0.03159921855737255
389,1281,0,1281,0.11277294158935547,0.03154449030425179
391,1287,0,1287,0.1131889820098877,0.03148159028286644
394,1296,0,1296,0.11379194259643555,0.031366663165563205
396,1302,0,1302,0.11419796943664551,0.03127264216721307
398,1308,0,1308,0.11459803581237793,0.031161893770534806
400,1314,0,1314,0.11499214172363281,0.031032132098980435
402,1320,0,1320,0.115386962890625,0.03088123213721216
405,1329,0,1329,0.11599302291870117,0.03061311297948879
407,1335,0,1335,0.11640501022338867,0.030406961940746307
409,1341,0,1341,0.11680984497070312,0.03018085105034826
411,1347,0,1347,0.11721205711364746,0.02993715706981183
414,1356,0,1356,0.11781597137451172,0.0295443208551814
416,1362,0,1362,0.11821794509887695,0.029267744262235
418,1368,0,1368,0.1186208724975586,0.028982125921187825
420,1374,0,1374,0.11903095245361328,0.02868965954207458
422,1380,0,1380,0.11942291259765625,0.028392471263913806
425,1389,0,1389,0.12002992630004883,0.027942297932590156
427,1395,0,1395,0.12043213844299316,0.02764212316128426
429,1401,0,1401,0.1208338737487793,0.027343945278976888
431,1407,0,1407,0.12123799324035645,0.027049133433693192
434,1416,0,1416,0.12185001373291016,0.02661523284334067
436,1422,0,1422,0.12225198745727539,0.026332342967150195
438,1428,0,1428,0.12265491485595703,0.026055049664319516
440,1434,0,1434,0.12305712699890137,0.025783855709356117
442,1440,0,1440,0.1234591007232666,0.025519500141102713
445,1449,0,1449,0.1240849494934082,0.025138254388256998
447,1455,0,1455,0.12450504302978516,0.024896652162793326
449,1461,0,1461,0.1249380111694336,0.02466778633309911
451,1467,0,1467,0.12536191940307617,0.024455011408625077
454,1476,0,1476,0.12596487998962402,0.024177354537159225
456,1482,0,1482,0.12636685371398926,0.0240313738976892
458,1488,0,1488,0.12679791450500488,0.02392657922458249
460,1494,0,1494,0.12744808197021484,0.023852659644086945
462,1500,0,1500,0.12802886962890625,0.023757837386464573
465,1510,0,1510,0.1287858486175537,0.023633886977671093
467,1518,0,1518,0.12936997413635254,0.023584103293992385
469,1526,0,1526,0.13005304336547852,0.02353791642861742
471,1534,0,1534,0.1307229995727539,0.023494614890544538
474,1546,0,1546,0.13179898262023926,0.023434538955814377
476,1554,0,1554,0.13251495361328125,0.023399210177856452
478,1562,0,1562,0.13332200050354004,0.023374401365987618
480,1570,0,1570,0.13395977020263672,0.023344664839009155
482,1577,0,1577,0.13465380668640137,0.02324951972293133
485,1586,0,1586,0.1356348991394043,0.02305558629967229
487,1592,0,1592,0.13621187210083008,0.022905205861186904
489,1598,0,1598,0.13667893409729004,0.022837997983787536
491,1606,0,1606,0.13720011711120605,0.02278159526662363
494,1618,0,1618,0.13811397552490234,0.022708732005388817
496,1626,0,1626,0.13864398002624512,0.022665624745170487
498,1633,0,1633,0.1390688419342041,0.022645178184221047
500,1639,0,1639,0.13947582244873047,0.02258885675777679
502,1645,0,1645,0.1399059295654297,0.02245811292576543
505,1654,0,1654,0.14048981666564941,0.02220521117861091
507,1660,0,1660,0.14088106155395508,0.021995659248492234
509,1666,0,1666,0.1412978172302246,0.0217461538817221
511,1672,0,1672,0.14181900024414062,0.021510243761398866
514,1681,0,1681,0.14260077476501465,0.021175606196762772
516,1687,0,1687,0.14298486709594727,0.020961028054564634
518,1693,0,1693,0.14347195625305176,0.020755271606469214
520,1699,0,1699,0.14400100708007812,0.020555208556321848
522,1705,0,1705,0.14441204071044922,0.020364423105158458
525,1714,0,1714,0.14500093460083008,0.02009382788247886
527,1720,0,1720,0.14541411399841309,0.019916739544159637
529,1726,0,1726,0.1459031105041504,0.019740430834197274
531,1732,0,1732,0.14641880989074707,0.01956622886545284
534,1741,0,1741,0.14708590507507324,0.01931065332812554
536,1747,0,1747,0.14750099182128906,0.019144840178476372
538,1753,0,1753,0.14791584014892578,0.018983514478777934
540,1759,0,1759,0.14835906028747559,0.018827764889293653
542,1765,0,1765,0.14878582954406738,0.018678470153180797
545,1774,0,1774,0.14945292472839355,0.018467900813938936
547,1780,0,1780,0.1498889923095703,0.018336876550441118
549,1786,0,1786,0.15032482147216797,0.018213501619025033
551,1792,0,1792,0.15076088905334473,0.01809786516614195
554,1801,0,1801,0.15144586563110352,0.017939134943592394
556,1807,0,1807,0.15189385414123535,0.01784336279439049
558,1813,0,1813,0.15234088897705078,0.017755728374905397
560,1819,0,1819,0.1528019905090332,0.0176761539048322
562,1825,0,1825,0.15324783325195312,0.01760437640441547
565,1834,0,1834,0.15392088890075684,0.01751066912365386
567,1840,0,1840,0.15437006950378418,0.01745718432988619
569,1846,0,1846,0.15482211112976074,0.017410732034268357
571,1852,0,1852,0.15526604652404785,0.01737112612173743
574,1861,0,1861,0.15593385696411133,0.01732377757040846
576,1867,0,1867,0.15637803077697754,0.017299481638571
578,1873,0,1873,0.15682387351989746,0.017280312213141236
580,1879,0,1879,0.15727686882019043,0.017265749390223205
582,1885,0,1885,0.15770792961120605,0.01725542459675457
585,1894,0,1894,0.15836215019226074,0.017247493500544216
587,1901,0,1901,0.1588149070739746,0.01724172217308104
589,1907,0,1907,0.1592729091644287,0.017236519188457464
591,1914,0,1914,0.15973806381225586,0.01722724668378157
594,1925,0,1925,0.16045093536376953,0.017212231749048942
596,1931,0,1931,0.16089582443237305,0.01720415646143508
598,1938,0,1938,0.1613600254058838,0.017195091378200644
600,1945,0,1945,0.16182494163513184,0.017183594671473422
602,1952,0,1952,0.1622929573059082,0.017178264795127303
605,1962,0,1962,0.16296100616455078,0.0171634226441996
607,1968,0,1968,0.1633930206298828,0.017141503774710472
609,1974,0,1974,0.16382503509521484,0.017126473338202986
611,1981,0,1981,0.16428494453430176,0.017117949252690258
614,1990,0,1990,0.16493511199951172,0.017071369079167176
616,1996,0,1996,0.16536688804626465,0.017030023747389787
618,2002,0,2002,0.16579985618591309,0.016991444532415495
620,2008,0,2008,0.1662299633026123,0.016954891326185068
623,2017,0,2017,0.16687893867492676,0.016900041297922604
625,2023,0,2023,0.16731476783752441,0.016860840243483895
627,2029,0,2029,0.16774797439575195,0.016817864702147602
629,2035,0,2035,0.16817998886108398,0.016769470279277658
631,2041,0,2041,0.16861295700073242,0.016713941683526832
634,2050,0,2050,0.16929197311401367,0.01661248322073767
636,2056,0,2056,0.16974592208862305,0.01652964499222773
638,2062,0,2062,0.17019200325012207,0.016432867573613005
640,2068,0,2068,0.1706390380859375,0.01632185293327401
643,2077,0,2077,0.1713111400604248,0.01612968602413269
645,2083,0,2083,0.17174506187438965,0.01598476146470863
647,2089,0,2089,0.17220497131347656,0.015824799495502837
649,2095,0,2095,0.17264890670776367,0.01564725276226836
651,2101,0,2101,0.1730940341949463,0.015449724522866155
654,2110,0,2110,0.17375898361206055,0.015113824689857072
656,2116,0,2116,0.17420697212219238,0.014864538181000083
658,2122,0,2122,0.17464184761047363,0.014597456666437254
660,2128,0,2128,0.1750929355621338,0.014315841115717105
663,2137,0,2137,0.17576909065246582,0.01387439307152924
665,2143,0,2143,0.17621493339538574,0.013572560518751123
667,2149,0,2149,0.17664790153503418,0.013268616825823172
669,2155,0,2155,0.17708587646484375,0.012966288350903563
671,2161,0,2161,0.1775190830230713,0.01266948224014334
674,2170,0,2170,0.17818593978881836,0.012241955735661074
676,2176,0,2176,0.17862296104431152,0.011972246846885122
678,2182,0,2182,0.17905402183532715,0.011716345952075281
680,2188,0,2188,0.17948579788208008,0.011474890927861123
683,2197,0,2197,0.18015694618225098,0.011140486184184579
685,2203,0,2203,0.1806011199951172,0.010936676465179731
687,2209,0,2209,0.18105792999267578,0.01074864097845244
689,2215,0,2215,0.1814889907836914,0.010576745619572949
691,2221,0,2221,0.18193697929382324,0.010421106614153424
694,2230,0,2230,0.1826038360595703,0.01021808635705773
696,2236,0,2236,0.18305206298828125,0.010102751992033126
698,2242,0,2242,0.18348312377929688,0.010003106990783044
700,2248,0,2248,0.1839148998260498,0.00991876405097425
703,2257,0,2257,0.18456292152404785,0.009819835106221588
705,2263,0,2263,0.18499493598937988,0.009771012373876934
707,2269,0,2269,0.18542695045471191,0.00973419578487535
709,2275,0,2275,0.18585896492004395,0.009707134232744411
711,2281,0,2281,0.18629097938537598,0.009686926667893456
714,2290,0,2290,0.1869518756866455,0.009661999851172921
716,2296,0,2296,0.18738389015197754,0.009643618635849954
718,2302,0,2302,0.18781590461730957,0.009619552198634824
720,2308,0,2308,0.1882469654083252,0.009586592120419738
723,2317,0,2317,0.18889498710632324,0.009521670352793147
725,2324,0,2324,0.1893470287322998,0.009501444783450885
727,2332,0,2332,0.1898200511932373,0.009494594593009283
729,2340,0,2340,0.1902909278869629,0.00948772513854067
731,2348,0,2348,0.1907639503479004,0.009480791131226903
734,2360,0,2360,0.19147300720214844,0.009470141808048645
736,2366,0,2366,0.19190382957458496,0.009460789692679937
738,2372,0,2372,0.19234490394592285,0.009453824449184878
740,2379,0,2379,0.19279980659484863,0.009449184522688002
743,2389,0,2389,0.19347190856933594,0.009442985376104935
745,2395,0,2395,0.1939067840576172,0.00943723777675974
747,2401,0,2401,0.19434285163879395,0.00943329517962556
749,2407,0,2407,0.19478178024291992,0.009429784799956807
751,2413,0,2413,0.19521594047546387,0.009427517609571676
754,2423,0,2423,0.19588804244995117,0.00938793702009624
756,2429,0,2429,0.19632291793823242,0.009310874072072187
758,2435,0,2435,0.19675803184509277,0.009198125673118094
760,2441,0,2441,0.19719696044921875,0.009056610070875744
763,2450,0,2450,0.1978590488433838,0.008834662418596985
765,2456,0,2456,0.19829392433166504,0.008717484473820886
767,2462,0,2462,0.1987299919128418,0.008624269178182806
769,2468,0,2468,0.19916892051696777,0.008559759955910344
771,2474,0,2474,0.19960594177246094,0.008516469269850089
774,2483,0,2483,0.20026111602783203,0.008474105155700712
776,2489,0,2489,0.20069503784179688,0.008454301374486982
778,2495,0,2495,0.20113205909729004,0.00843963817299671
780,2501,0,2501,0.2015669345855713,0.008429841906389663
783,2510,0,2510,0.20221996307373047,0.008422832740165353
785,2517,0,2517,0.20267701148986816,0.0084153753466445
787,2525,0,2525,0.2031569480895996,0.00840212331430054
789,2533,0,2533,0.20363903045654297,0.008389144913693731
791,2541,0,2541,0.2041158676147461,0.008376394300991408
794,2553,0,2553,0.20483183860778809,0.008357634883532939
796,2561,0,2561,0.2053050994873047,0.008345353954490053
798,2569,0,2569,0.20578289031982422,0.008333236418860756
800,2577,0,2577,0.2062549591064453,0.00832126355556309
803,2589,0,2589,0.2069690227508545,0.008303522131044561
805,2597,0,2597,0.2074439525604248,0.008291776305181705
807,2605,0,2605,0.20791912078857422,0.008280023097035051
809,2612,0,2612,0.2083759307861328,0.0082723953881164
811,2620,0,2620,0.2088479995727539,0.008262182353786368
814,2632,0,2632,0.20956802368164062,0.008247669602334943
816,2640,0,2640,0.21004581451416016,0.008238549715134958
818,2648,0,2648,0.21052002906799316,0.00823004739405143
820,2656,0,2656,0.21099376678466797,0.008222608143552659
823,2668,0,2668,0.21170306205749512,0.008216386599000118
825,2677,0,2677,0.21219396591186523,0.00820348375101317
827,2683,0,2683,0.21262693405151367,0.008129272942245748
829,2689,0,2689,0.2130589485168457,0.00805977459716982
831,2695,0,2695,0.21348977088928223,0.008005362932382992
834,2704,0,2704,0.21413588523864746,0.007953640499151057
836,2710,0,2710,0.2145698070526123,0.007933081695925097
838,2716,0,2716,0.21499991416931152,0.007919789131506897
840,2722,0,2722,0.21543598175048828,0.007911064978325104
843,2731,0,2731,0.21608185768127441,0.007901602668961474
845,2737,0,2737,0.21651387214660645,0.00789491219484538
847,2743,0,2743,0.2169489860534668,0.00788677561665995
849,2749,0,2749,0.21738195419311523,0.007877094939546353
851,2755,0,2755,0.21781301498413086,0.0078660010304196
854,2764,0,2764,0.2184591293334961,0.007847448864439634
856,2770,0,2770,0.21889090538024902,0.007834330987212772
858,2776,0,2776,0.21932196617126465,0.007820957817019709
860,2782,0,2782,0.21975088119506836,0.007807293117446986
863,2791,0,2791,0.22042298316955566,0.00778572237602816
865,2797,0,2797,0.22086191177368164,0.007769819304841385
867,2803,0,2803,0.2212998867034912,0.007751930105202423
869,2809,0,2809,0.22174787521362305,0.007731281558108393
872,2818,0,2818,0.2223968505859375,0.007693765005412085
874,2824,0,2824,0.22283005714416504,0.007663587768429263
876,2830,0,2830,0.22326278686523438,0.007628857663588353
878,2836,0,2836,0.22369718551635742,0.0075893453380081076
880,2842,0,2842,0.22412991523742676,0.007544967158843543
883,2851,0,2851,0.22478199005126953,0.0074692892926611415
885,2857,0,2857,0.22521281242370605,0.007412962186868249
887,2863,0,2863,0.22564697265625,0.007352248541688699
889,2869,0,2869,0.22607994079589844,0.00728756747123147
892,2878,0,2878,0.22674298286437988,0.007184248062826256
894,2884,0,2884,0.22718191146850586,0.007112022332423543
896,2890,0,2890,0.22762393951416016,0.007037812176096466
898,2896,0,2896,0.22806000709533691,0.006962189569717763
900,2902,0,2902,0.22849607467651367,0.006885686416688724
903,2911,0,2911,0.22914814949035645,0.006770340798373578
905,2917,0,2917,0.22958087921142578,0.006693688711597784
907,2923,0,2923,0.2300128936767578,0.006617695054705611
909,2929,0,2929,0.23044490814208984,0.006542718108068289
912,2938,0,2938,0.23111486434936523,0.006432866807640996
914,2944,0,2944,0.23155975341796875,0.00636179857105319
916,2950,0,2950,0.2320239543914795,0.006292762818953005
918,2956,0,2956,0.23246002197265625,0.006225982770911932
920,2962,0,2962,0.23289203643798828,0.006161651613909016
923,2971,0,2971,0.23354005813598633,0.00607009992037009
925,2977,0,2977,0.23397397994995117,0.006012557466045806
927,2983,0,2983,0.23441195487976074,0.005957939205527229
929,2989,0,2989,0.234846830368042,0.0059063403648130655
932,2998,0,2998,0.23549985885620117,0.0058347842469731
934,3004,0,3004,0.2359328269958496,0.005791079178734759
936,3010,0,3010,0.23636794090270996,0.005750643354612887
938,3016,0,3016,0.23680400848388672,0.005713523513983479
940,3022,0,3022,0.23726797103881836,0.005679751944912082
943,3031,0,3031,0.23794889450073242,0.005635399061148743
945,3037,0,3037,0.23839616775512695,0.005610015609783736
947,3043,0,3043,0.23885679244995117,0.005587933460453242
949,3049,0,3049,0.2393169403076172,0.005569082454825697
952,3058,0,3058,0.24001407623291016,0.005546644363127666
954,3064,0,3064,0.24045896530151367,0.005535388699401222
956,3070,0,3070,0.2409038543701172,0.005526912316945203
958,3076,0,3076,0.24135112762451172,0.005521033008279043
960,3082,0,3082,0.24179697036743164,0.005517547744714488
963,3092,0,3092,0.24249005317687988,0.005514855806142043
965,3099,0,3099,0.24295997619628906,0.005513348554444378
967,3107,0,3107,0.24345803260803223,0.005510657645045665
969,3115,0,3115,0.24396491050720215,0.0055080151552424645
972,3127,0,3127,0.24467992782592773,0.005504121063687884
974,3135,0,3135,0.24516797065734863,0.005501570307990202
976,3143,0,3143,0.24564099311828613,0.005499059580649151
978,3151,0,3151,0.24611401557922363,0.0054965883532783425
980,3159,0,3159,0.24658608436584473,0.005494154486918324
983,3171,0,3171,0.24744701385498047,0.005490590529470933
985,3179,0,3179,0.2479548454284668,0.005488301282429976
987,3187,0,3187,0.24845409393310547,0.005486131027691802
989,3195,0,3195,0.24895405769348145,0.00548419482860479
992,3208,0,3208,0.24965500831604004,0.005481679094171321
994,3216,0,3216,0.25013089179992676,0.0054737802917180925
996,3224,0,3224,0.2505769729614258,0.00547042740558922
998,3232,0,3232,0.2510209083557129,0.005467486095622619
1000,3240,0,3240,0.2514638900756836,0.005464789060379803
1003,3252,0,3252,0.2521340847015381,0.0054611528968353095
1005,3260,0,3260,0.25258684158325195,0.005459254897488698
1007,3269,0,3269,0.2530488967895508,0.0054575494688336515
1009,3279,0,3279,0.25353002548217773,0.005455199959987869
1012,3291,0,3291,0.2541959285736084,0.005445283222512154
1014,3299,0,3299,0.2546401023864746,0.005438277990413148
1016,3306,0,3306,0.2550630569458008,0.005410648694121824
1018,3313,0,3313,0.25553083419799805,0.005399029139148863
1020,3321,0,3321,0.25597310066223145,0.005393419558045859
1023,3333,0,3333,0.25663089752197266,0.005387008411046106
1025,3342,0,3342,0.25708699226379395,0.005383719900716452
1027,3350,0,3350,0.2575337886810303,0.0053733675611222975
1029,3356,0,3356,0.257936954498291,0.005289857358004484
1032,3365,0,3365,0.25853991508483887,0.00523612001398744
1034,3371,0,3371,0.2589418888092041,0.0052038818019515464
1036,3377,0,3377,0.25934410095214844,0.005170161195981561
1038,3383,0,3383,0.2597517967224121,0.005133284137207123
1040,3389,0,3389,0.26015615463256836,0.005094247008801212
1043,3398,0,3398,0.26076412200927734,0.005031803752550735
1045,3404,0,3404,0.2611730098724365,0.004987227025423146
1047,3410,0,3410,0.26157689094543457,0.0049415131853581
1049,3416,0,3416,0.2619800567626953,0.004894439763868622
1052,3425,0,3425,0.2625861167907715,0.00482224710019077
1054,3431,0,3431,0.26298999786376953,0.0047736523223939386
1056,3437,0,3437,0.2633998394012451,0.00472505037744895
1058,3443,0,3443,0.26380491256713867,0.004676677513229763
1060,3449,0,3449,0.2642080783843994,0.0046287098125719715
1063,3458,0,3458,0.2648189067840576,0.004558059967931355
1065,3464,0,3464,0.2652249336242676,0.004512119762847943
1067,3470,0,3470,0.2656288146972656,0.004467377840247722
1069,3476,0,3476,0.2660388946533203,0.004423916946586237
1072,3485,0,3485,0.26664185523986816,0.004361292425749065
1074,3491,0,3491,0.2670459747314453,0.004321163593873612
1076,3497,0,3497,0.2674558162689209,0.004282193252437626
1078,3503,0,3503,0.26785993576049805,0.004244181670005731
1080,3509,0,3509,0.2682638168334961,0.004206970294836323
1083,3518,0,3518,0.2688717842102051,0.0041522046535798
1085,3524,0,3524,0.2692739963531494,0.004116101003887295
1087,3530,0,3530,0.26967811584472656,0.004080074402092233
1089,3536,0,3536,0.2700810432434082,0.004043983067927375
1092,3545,0,3545,0.27068305015563965,0.003989511965975219
1094,3551,0,3551,0.2710881233215332,0.003952943366515165
1096,3557,0,3557,0.2714967727661133,0.0039162038768555145
1098,3563,0,3563,0.27190089225769043,0.003879382367298886
1100,3569,0,3569,0.27230405807495117,0.003842593967864856
1103,3578,0,3578,0.27291011810302734,0.003787784414103941
1105,3584,0,3584,0.273313045501709,0.0037517159262971645
1107,3590,0,3590,0.2737147808074951,0.003716207208044626
1109,3596,0,3596,0.27411603927612305,0.003681409787469593
1112,3605,0,3605,0.2747230529785156,0.0036308582746367606
1114,3611,0,3611,0.27512383460998535,0.003598437046254979
1116,3617,0,3617,0.2755250930786133,0.0035671617983390248
1118,3623,0,3623,0.275925874710083,0.0035371113092935074
1121,3632,0,3632,0.2765328884124756,0.003494443648273025
1123,3638,0,3638,0.27693676948547363,0.0034676369264427928
1125,3644,0,3644,0.2773427963256836,0.0034421366918626875
1127,3650,0,3650,0.27774500846862793,0.0034179163141127814
1129,3656,0,3656,0.27814602851867676,0.0033949332114838185
1132,3665,0,3665,0.27875185012817383,0.0033626570890498697
1134,3671,0,3671,0.27915382385253906,0.0033425136979775335
1136,3677,0,3677,0.279555082321167,0.0033233933308235175
1138,3683,0,3683,0.2799558639526367,0.0033052325646051465
1141,3692,0,3692,0.28055596351623535,0.0032796633490160283
1143,3698,0,3698,0.2809567451477051,0.0032636572446550017
1145,3704,0,3704,0.2813589572906494,0.003248432422992421
1147,3710,0,3710,0.2817661762237549,0.0032339525904099514
1149,3716,0,3716,0.2821660041809082,0.0032201867202333295
1152,3725,0,3725,0.2827718257904053,0.003200817696585504
1154,3731,0,3731,0.2831740379333496,0.0031887220347743164
1156,3737,0,3737,0.28357601165771484,0.0031772513808955042
1158,3743,0,3743,0.2839798927307129,0.0031663800495556177
1161,3752,0,3752,0.28458380699157715,0.0031511359340277143
1163,3758,0,3758,0.28498387336730957,0.003141637641924333
1165,3764,0,3764,0.2853848934173584,0.0031326327729136135
1167,3770,0,3770,0.28578805923461914,0.003124086299359342
1169,3776,0,3776,0.2861909866333008,0.0031159608523729353
1172,3785,0,3785,0.286801815032959,0.0031044714843631574
1174,3791,0,3791,0.28720784187316895,0.0030972060720640886
1176,3797,0,3797,0.2876100540161133,0.003090179894383124
1178,3803,0,3803,0.2880120277404785,0.003083292732266651
1181,3812,0,3812,0.28865504264831543,0.0030728041215748263
1183,3818,0,3818,0.28905701637268066,0.0030650690842120728
1185,3824,0,3824,0.2894587516784668,0.003055398898505812
1187,3830,0,3830,0.2898590564727783,0.0030407123283156244
1189,3836,0,3836,0.2903869152069092,0.003015233037622289
1192,3845,0,3845,0.2909989356994629,0.0029498683519832212
1194,3851,0,3851,0.29140281677246094,0.002894917895037683
1196,3855,0,3855,0.2917659282684326,0.001682293255992174
1198,3861,0,3861,0.2923009395599365,0.0016282885634946115
1201,3871,0,3871,0.2929229736328125,0.0015282348810834294
1203,3877,0,3877,0.29332709312438965,0.0014775288853000207
1205,3883,0,3883,0.2937288284301758,0.0014422901441305713
1207,3889,0,3889,0.2941319942474365,0.0014105687742588398
1209,3895,0,3895,0.2945380210876465,0.0013885188945920337
1212,3904,0,3904,0.29514384269714355,0.0013649469442903648
1214,3910,0,3910,0.2955460548400879,0.0013511495914430584
1216,3916,0,3916,0.2959930896759033,0.0013352645797054987
1218,3922,0,3922,0.29639601707458496,0.0013197346869653806
1221,3931,0,3931,0.2970008850097656,0.0012761319369287325
1223,3937,0,3937,0.29741692543029785,0.0012508357987249536
1225,3943,0,3943,0.2978217601776123,0.001230825446763804
1227,3949,0,3949,0.29822516441345215,0.0012129774439988332
1229,3955,0,3955,0.2986280918121338,0.001193101869882779
1232,3964,0,3964,0.2992370128631592,0.0011680316556972857
1234,3971,0,3971,0.29965782165527344,0.001162182840230619
1236,3979,0,3979,0.3000979423522949,0.0011519881247054502
1238,3987,0,3987,0.3005390167236328,0.0011421657905699338
1241,3998,0,3998,0.3011770248413086,0.0011317331519201887
1243,4004,0,4004,0.30157995223999023,0.0011274551040557162
1245,4010,0,4010,0.3019881248474121,0.0011208758807557092
1247,4016,0,4016,0.30239200592041016,0.0011133205250341703
1249,4022,0,4022,0.30280113220214844,0.0011044994294762986
1252,4031,0,4031,0.3034098148345947,0.001084290705356171
1254,4039,0,4039,0.3038499355316162,0.0010679256619129795
1256,4045,0,4045,0.30425381660461426,0.001045381141781954
1258,4051,0,4051,0.3046588897705078,0.001010493756221718
1261,4060,0,4060,0.30525994300842285,0.0009568032881818365
1263,4066,0,4066,0.3056609630584717,0.0009232171947273543
1265,4072,0,4072,0.3060619831085205,0.0008918751985328681
1267,4078,0,4078,0.30646300315856934,0.0008626245803153481
1269,4084,0,4084,0.30686211585998535,0.0008347237234567624
1272,4093,0,4093,0.30747008323669434,0.0007943192154938754
1274,4099,0,4099,0.3078761100769043,0.0007686704478157758
1276,4105,0,4105,0.30827784538269043,0.0007442674505537775
1278,4111,0,4111,0.30867815017700195,0.0007213051508195259
1281,4120,0,4120,0.3092789649963379,0.0006900011184074496
1283,4126,0,4126,0.3096799850463867,0.0006736461610314679
1285,4132,0,4132,0.31008100509643555,0.0006580099207600844
1287,4138,0,4138,0.3104839324951172,0.0006375302673503938
1289,4144,0,4144,0.3108839988708496,0.0006177751835485634
1292,4155,0,4155,0.3115229606628418,0.0006063327191526368
1294,4163,0,4163,0.31195998191833496,0.0006035320569105841
1296,4171,0,4171,0.3123970031738281,0.0006008902379058026
1298,4179,0,4179,0.3128340244293213,0.0005983681480269433
1301,4191,0,4191,0.3134949207305908,0.0005948033281511617
1303,4199,0,4199,0.3139340877532959,0.0005925550572862305
1305,4207,0,4207,0.3143730163574219,0.0005904014888760471
1307,4215,0,4215,0.31481289863586426,0.0005883128707486313
1309,4223,0,4223,0.31525182723999023,0.0005862387828814351
1312,4235,0,4235,0.31591010093688965,0.0005827670227231186
1314,4243,0,4243,0.3163480758666992,0.0005795457699541933
1316,4250,0,4250,0.3167688846588135,0.0005675358633840168
1318,4256,0,4256,0.3171730041503906,0.0005636981460224408
1321,4265,0,4265,0.31777405738830566,0.0005595544915547165
1323,4271,0,4271,0.3181748390197754,0.0005582929220974979
1325,4277,0,4277,0.31858181953430176,0.0005576406703237785
1327,4283,0,4283,0.3189830780029297,0.0005570608688338234
1329,4289,0,4289,0.3193960189819336,0.0005559915416550104
1332,4298,0,4298,0.31998586654663086,0.0005522160517413166
1334,4304,0,4304,0.3203771114349365,0.000548008793876116
1336,4310,0,4310,0.3207688331604004,0.0005423235727615523
1338,4316,0,4316,0.32115912437438965,0.0005354962489513944
1341,4325,0,4325,0.3217451572418213,0.0005245290406199872
1343,4331,0,4331,0.32213497161865234,0.0005177374991628867
1345,4337,0,4337,0.3225247859954834,0.0005120695020076857
1347,4343,0,4343,0.32291603088378906,0.0005077337185852515
1349,4349,0,4349,0.3233070373535156,0.0005053224151782522
1352,4359,0,4359,0.32392096519470215,0.0005042042932937179
1354,4365,0,4365,0.3243098258972168,0.000498507821827991
1356,4371,0,4371,0.3247039318084717,0.0004932352041426618
1358,4377,0,4377,0.32509493827819824,0.0004878617738952511
1361,4386,0,4386,0.32567811012268066,0.00047913729904332155
1363,4392,0,4392,0.3260688781738281,0.00047255498585392007
1365,4398,0,4398,0.3264591693878174,0.00046520498389658805
1367,4404,0,4404,0.32684898376464844,0.0004570963627882384
1370,4413,0,4413,0.32744288444519043,0.0004436744783531016
1372,4419,0,4419,0.3278329372406006,0.0004341711902083563
1374,4425,0,4425,0.32822299003601074,0.00042453241986289156
1376,4431,0,4431,0.32862091064453125,0.00041505304056288326
1378,4437,0,4437,0.3290128707885742,0.0004059723207797176
1381,4446,0,4446,0.32959794998168945,0.00039358151550331224
1383,4452,0,4452,0.3299901485443115,0.00038635451842353565
1385,4458,0,4458,0.3303821086883545,0.0003800767750843431
1387,4464,0,4464,0.33077287673950195,0.0003746888445947284
1390,4473,0,4473,0.3313620090484619,0.0003679109238161607
1392,4479,0,4479,0.33175182342529297,0.0003639342621082517
1394,4485,0,4485,0.33214306831359863,0.0003601466201000277
1396,4491,0,4491,0.3325338363647461,0.00035641841923625953
1398,4497,0,4497,0.33292412757873535,0.0003526625448439112
1401,4506,0,4506,0.3335127830505371,0.0003468735136556136
1403,4512,0,4512,0.3339049816131592,0.00034289137505951877
1405,4518,0,4518,0.3343038558959961,0.00033877468037803074
1407,4524,0,4524,0.3346989154815674,0.00033439883715453587
1410,4533,0,4533,0.33528804779052734,0.0003274573840176903
1412,4539,0,4539,0.3356788158416748,0.00032387180637053316
1414,4546,0,4546,0.3360869884490967,0.000322639062033267
1416,4552,0,4552,0.33647608757019043,0.0003189477630859894
1418,4558,0,4558,0.336867094039917,0.00030997701860275504
1421,4567,0,4567,0.33745503425598145,0.00029550708193436525
1423,4573,0,4573,0.3378469944000244,0.00028744677116758835
1425,4579,0,4579,0.3382377624511719,0.00028318300052574904
1427,4586,0,4586,0.3386538028717041,0.00028214117598365286
1430,4595,0,4595,0.33924293518066406,0.0002700696449331984
1432,4601,0,4601,0.3396339416503906,0.00026237044216896875
1434,4607,0,4607,0.3400249481201172,0.000256213601407221
1436,4613,0,4613,0.34041595458984375,0.00025219144769185106
1438,4620,0,4620,0.34082508087158203,0.0002502675900598488
1441,4630,0,4630,0.3414268493652344,0.00022907514750091415
1443,4636,0,4636,0.34181809425354004,0.00022199626470667977
1445,4642,0,4642,0.3422110080718994,0.00021900281804534591
1447,4649,0,4649,0.342620849609375,0.000217810317298603
1450,4659,0,4659,0.343228816986084,0.00021420369081920715
1452,4665,0,4665,0.3436248302459717,0.00021013432529606762
1454,4671,0,4671,0.34401702880859375,0.00020661342689417222
1456,4677,0,4677,0.3444099426269531,0.0002034289436630768
1458,4683,0,4683,0.3448059558868408,0.00020032419784950245
1461,4692,0,4692,0.34539198875427246,0.00019586054702907857
1463,4698,0,4698,0.34578394889831543,0.00019318672611534057
1465,4704,0,4704,0.3461780548095703,0.00019088874176052546
1467,4710,0,4710,0.3465719223022461,0.00018936779089287682
1470,4721,0,4721,0.3472020626068115,0.00018826460623637506
1472,4729,0,4729,0.34763002395629883,0.00018755862166439094
1474,4737,0,4737,0.3480570316314697,0.00018687384876530953
1476,4744,0,4744,0.3484659194946289,0.00018639059860420853
1478,4750,0,4750,0.348862886428833,0.00018341402546618636
1481,4759,0,4759,0.34944987297058105,0.00017864468191509323
1483,4765,0,4765,0.349841833114624,0.00017468873187716412
1485,4771,0,4771,0.3502340316772461,0.00017004925933493826
1487,4777,0,4777,0.35062599182128906,0.00016465996374788946
1490,4786,0,4786,0.35121774673461914,0.00015464262436347387
1492,4792,0,4792,0.3516120910644531,0.00014610517275362613
1494,4798,0,4798,0.3520030975341797,0.00013984654125410613
1496,4804,0,4804,0.35239601135253906,0.00013363928858105097
1498,4810,0,4810,0.35278797149658203,0.0001289020869387585
1501,4819,0,4819,0.35337209701538086,0.00012338080619706486
1503,4825,0,4825,0.35376787185668945,0.00012055026313802429
1505,4831,0,4831,0.35416102409362793,0.00011863383427344868
1507,4838,0,4838,0.35457301139831543,0.00011727434058868447
1510,4850,0,4850,0.3553457260131836,0.00011609716622165331
1512,4858,0,4858,0.355802059173584,0.00011547334016449303
1514,4866,0,4866,0.3562328815460205,0.0001149143781556153
1516,4874,0,4874,0.3566620349884033,0.00011440702784999671
1518,4882,0,4882,0.3570878505706787,0.00011393153173039176
1521,4894,0,4894,0.3577241897583008,0.00011325645439550503
1523,4902,0,4902,0.3581569194793701,0.0001128266992368323
1525,4908,0,4908,0.3585469722747803,0.00011152156462267781
1527,4914,0,4914,0.3589348793029785,0.00010904937892093302
1530,4923,0,4923,0.3595249652862549,0.00010530147420392743
1532,4929,0,4929,0.3599119186401367,0.00010283870481503879
1534,4935,0,4935,0.36029887199401855,0.00010056243902969934
1536,4941,0,4941,0.3606870174407959,9.84035405632141e-05
1538,4947,0,4947,0.36107373237609863,9.638870306512858e-05
1541,4956,0,4956,0.36165499687194824,9.353702176837043e-05
1543,4962,0,4962,0.3620419502258301,9.173783440473856e-05
1545,4968,0,4968,0.36243391036987305,8.999784560460076e-05
1547,4974,0,4974,0.3628220558166504,8.833222992186812e-05
1550,4983,0,4983,0.3634028434753418,8.596214366419784e-05
1552,4989,0,4989,0.36378908157348633,8.451847791304308e-05
1554,4995,0,4995,0.3641808032989502,8.321555787388493e-05
1556,5001,0,5001,0.36457014083862305,8.221441134214455e-05
1558,5007,0,5007,0.3649568557739258,8.158438402443853e-05
1561,5018,0,5018,0.36557698249816895,8.123423175566536e-05
1563,5027,0,5027,0.36601805686950684,8.105396994715917e-05
1565,5033,0,5033,0.3664071559906006,7.694214361419081e-05
1567,5039,0,5039,0.3667948246002197,7.59305616845876e-05
1570,5048,0,5048,0.367372989654541,7.495539009347608e-05
1572,5054,0,5054,0.36775898933410645,7.455525860053734e-05
1574,5060,0,5060,0.3681468963623047,7.426566256726349e-05
1576,5066,0,5066,0.3685338497161865,7.410723704139354e-05
1578,5072,0,5072,0.36892104148864746,7.401723665517313e-05
1581,5081,0,5081,0.3695058822631836,7.377493354783455e-05
1583,5087,0,5087,0.3698921203613281,7.342448655369731e-05
1585,5093,0,5093,0.3702828884124756,7.283106585806163e-05
1587,5099,0,5099,0.3706700801849365,7.200162400000705e-05
1590,5108,0,5108,0.37137889862060547,7.04146445902893e-05
1592,5114,0,5114,0.37184596061706543,6.917754480101096e-05
1594,5120,0,5120,0.37223196029663086,6.78850832187927e-05
1596,5126,0,5126,0.3726167678833008,6.656291121347176e-05
1598,5132,0,5132,0.3730008602142334,6.527749587905652e-05
1601,5141,0,5141,0.3735799789428711,6.347239008292076e-05
1603,5147,0,5147,0.3739650249481201,6.23477118830472e-05
1605,5153,0,5153,0.37435388565063477,6.126975074565049e-05
1607,5159,0,5159,0.3747420310974121,6.020124307468342e-05
1610,5168,0,5168,0.37543296813964844,5.8599273081769883e-05
1612,5174,0,5174,0.3760650157928467,5.7510480112862386e-05
1614,5180,0,5180,0.376953125,5.6394564843929065e-05
1616,5186,0,5186,0.3776397705078125,5.5234534332187356e-05
1619,5195,0,5195,0.37821483612060547,5.336423341342695e-05
1621,5201,0,5201,0.37871694564819336,5.2020298760549205e-05
1623,5207,0,5207,0.379288911819458,5.061192392927605e-05
1625,5213,0,5213,0.37981200218200684,4.917309921093231e-05
1627,5219,0,5219,0.38028693199157715,4.773732959023608e-05
1630,5228,0,5228,0.3810908794403076,4.562053754385058e-05
1632,5234,0,5234,0.38163304328918457,4.423709270807319e-05
1634,5240,0,5240,0.3820767402648926,4.28786898890405e-05
1636,5246,0,5246,0.3826580047607422,4.155828181284062e-05
1639,5255,0,5255,0.3833730220794678,3.969693039998938e-05
1641,5261,0,5261,0.3838157653808594,3.8559772545746845e-05
1643,5267,0,5267,0.38429689407348633,3.750857172290965e-05
1645,5273,0,5273,0.3847160339355469,3.653067881509502e-05
1647,5279,0,5279,0.38513994216918945,3.5607410985805894e-05
1650,5288,0,5288,0.38587307929992676,3.4294008134025816e-05
1652,5294,0,5294,0.3863189220428467,3.346403863921079e-05
1654,5300,0,5300,0.38678503036499023,3.2682840287297686e-05
1656,5306,0,5306,0.3872489929199219,3.196244691637497e-05
1659,5315,0,5315,0.38788509368896484,3.099655959246561e-05
1661,5321,0,5321,0.3884549140930176,3.0417290817349406e-05
1663,5327,0,5327,0.38891100883483887,2.9881557263745126e-05
1665,5333,0,5333,0.389354944229126,2.9390910657909685e-05
1667,5339,0,5339,0.38974499702453613,2.893748386370718e-05
1670,5348,0,5348,0.3904130458831787,2.8271431493918874e-05
1672,5354,0,5354,0.3909170627593994,2.7801473247666146e-05
1674,5360,0,5360,0.3913099765777588,2.730226090706758e-05
1676,5366,0,5366,0.3918571472167969,2.6779973837111576e-05
1679,5375,0,5375,0.39252710342407227,2.5987234500587162e-05
1681,5381,0,5381,0.3929469585418701,2.5495806076192427e-05
1683,5387,0,5387,0.3933570384979248,2.5078866698824033e-05
1685,5393,0,5393,0.39377880096435547,2.4752195510792075e-05
1687,5399,0,5399,0.39419102668762207,2.449364493805834e-05
1690,5408,0,5408,0.3948557376861572,2.4137044675418963e-05
1692,5414,0,5414,0.39527297019958496,2.3868873891872876e-05
1694,5420,0,5420,0.39568614959716797,2.3560747773715007e-05
1696,5426,0,5426,0.39609599113464355,2.3219062154790987e-05
1699,5435,0,5435,0.3967127799987793,2.2673117573772375e-05
1701,5441,0,5441,0.39713406562805176,2.229306668236678e-05
1703,5447,0,5447,0.3976619243621826,2.1895909766339584e-05
1705,5453,0,5453,0.3980751037597656,2.148047071698765e-05
1707,5459,0,5459,0.39861392974853516,2.1053829159289026e-05
1710,5468,0,5468,0.39934301376342773,2.0439469148333726e-05
1712,5474,0,5474,0.3997988700866699,2.0096054391422358e-05
1714,5480,0,5480,0.40044307708740234,1.9833921028866053e-05
1716,5486,0,5486,0.4009988307952881,1.962261123595421e-05
1719,5495,0,5495,0.40176892280578613,1.930108372999335e-05
1721,5501,0,5501,0.40221190452575684,1.9042896923850195e-05
1723,5507,0,5507,0.4027230739593506,1.874912162400951e-05
1725,5514,0,5514,0.40313005447387695,1.8515402151554002e-05
1727,5520,0,5520,0.40352296829223633,1.8079120917774468e-05
1730,5529,0,5529,0.40410494804382324,1.741825502746379e-05
1732,5535,0,5535,0.4045429229736328,1.698955510205731e-05
1734,5541,0,5541,0.4049341678619385,1.6583739888155938e-05
1736,5547,0,5547,0.40532898902893066,1.6330881662416337e-05
1739,5557,0,5557,0.4059278964996338,1.616016212792727e-05
1741,5563,0,5563,0.40631699562072754,1.5921514365770024e-05
1743,5569,0,5569,0.4067051410675049,1.5713289320304876e-05
1745,5575,0,5575,0.4070918560028076,1.5487734837992152e-05
1747,5581,0,5581,0.4074878692626953,1.521691787094063e-05
1750,5590,0,5590,0.40807008743286133,1.4769056524617066e-05
1752,5596,0,5596,0.4085218906402588,1.4497664861342192e-05
1754,5602,0,5602,0.4089200496673584,1.4245379487636543e-05
1756,5608,0,5608,0.40930891036987305,1.3997842824637247e-05
1759,5617,0,5617,0.4098958969116211,1.3677200081424193e-05
1761,5623,0,5623,0.41028499603271484,1.3472636607561133e-05
1763,5629,0,5629,0.41068100929260254,1.3216978596342795e-05
1765,5635,0,5635,0.41107702255249023,1.295766484641629e-05
1767,5641,0,5641,0.4116699695587158,1.2846020014009613e-05
1770,5650,0,5650,0.4122757911682129,1.2761586994081799e-05
1772,5656,0,5656,0.4126718044281006,1.2700919363519428e-05
1774,5662,0,5662,0.4133429527282715,1.2587752965681648e-05
1776,5668,0,5668,0.4137539863586426,1.2425704583223653e-05
1779,5677,0,5677,0.4143409729003906,1.203921275185801e-05
1781,5683,0,5683,0.4147350788116455,1.1643126924919925e-05
1783,5689,0,5689,0.41513586044311523,1.1125578526104903e-05
1785,5695,0,5695,0.4155261516571045,1.0531981033590863e-05
1787,5701,0,5701,0.41591501235961914,1.004107455968091e-05
1790,5710,0,5710,0.41650891304016113,9.680732243048909e-06
1792,5717,0,5717,0.4169158935546875,9.578844501691676e-06
1794,5724,0,5724,0.41732192039489746,9.517134223987538e-06
1796,5730,0,5730,0.4177100658416748,9.409100814100685e-06
1799,5740,0,5740,0.41831016540527344,9.209762048757914e-06
1801,5746,0,5746,0.41869688034057617,9.018233260832844e-06
1803,5752,0,5752,0.4190850257873535,8.875441621985101e-06
1805,5758,0,5758,0.4194929599761963,8.75846160881895e-06
1807,5764,0,5764,0.419888973236084,8.662995436975649e-06
1810,5773,0,5773,0.4204897880554199,8.560559466334149e-06
1812,5779,0,5779,0.4208860397338867,8.527655812081994e-06
1814,5785,0,5785,0.42129087448120117,8.521617591280786e-06
1816,5791,0,5791,0.42179298400878906,8.490627646973958e-06
1819,5800,0,5800,0.4223799705505371,8.350192370370506e-06
1821,5806,0,5806,0.42276811599731445,8.173966328131916e-06
1823,5812,0,5812,0.4231557846069336,7.955925624686251e-06
1825,5818,0,5818,0.42354297637939453,7.718951564284565e-06
1827,5824,0,5824,0.42392897605895996,7.477979053981631e-06
1830,5833,0,5833,0.42450809478759766,7.138142667306327e-06
1832,5839,0,5839,0.4248948097229004,6.927511065218511e-06
1834,5845,0,5845,0.4252889156341553,6.721855041358632e-06
1836,5851,0,5851,0.425678014755249,6.521863655330292e-06
1839,5860,0,5860,0.4262559413909912,6.244190388892446e-06
1841,5866,0,5866,0.426785945892334,6.101490460858484e-06
1843,5872,0,5872,0.42722201347351074,6.002504902149148e-06
1845,5878,0,5878,0.4276280403137207,5.948389091088092e-06
1847,5884,0,5884,0.4281940460205078,5.925089295977574e-06
1850,5894,0,5894,0.42885279655456543,5.748237750679262e-06
1852,5900,0,5900,0.4292619228363037,5.7043422302176085e-06
1854,5906,0,5906,0.42966604232788086,5.682637315531856e-06
1856,5912,0,5912,0.43007397651672363,5.649566276351529e-06
1859,5921,0,5921,0.4306778907775879,5.5640955448617406e-06
1861,5927,0,5927,0.43108701705932617,5.487684995655611e-06
1863,5933,0,5933,0.4314920902252197,5.41273831356324e-06
1865,5939,0,5939,0.43189096450805664,5.346550280679696e-06
1868,5948,0,5948,0.43249082565307617,5.2558708185729845e-06
1870,5954,0,5954,0.4328939914703369,5.17895700673039e-06
1872,5960,0,5960,0.43329286575317383,5.0937474043927874e-06
1874,5966,0,5966,0.43369102478027344,5.015576699897789e-06
1876,5972,0,5972,0.4340949058532715,4.949038522228099e-06
1879,5981,0,5981,0.43469786643981934,4.8692719010574e-06
1881,5987,0,5987,0.43509793281555176,4.824364530884319e-06
1883,5993,0,5993,0.43549489974975586,4.782891298367901e-06
1885,5999,0,5999,0.43590283393859863,4.744319215840162e-06
1888,6008,0,6008,0.43650293350219727,4.691396960023884e-06
1890,6014,0,6014,0.4369027614593506,4.657859714078091e-06
1892,6020,0,6020,0.4372999668121338,4.622527233215063e-06
1894,6026,0,6026,0.43770313262939453,4.582316324670347e-06
1896,6032,0,6032,0.43810391426086426,4.535013568700559e-06
1899,6041,0,6041,0.4387040138244629,4.459408310185962e-06
1901,6047,0,6047,0.4391000270843506,4.4292942984965235e-06
1903,6054,0,6054,0.43951892852783203,4.4158551519488395e-06
1905,6061,0,6061,0.43993592262268066,4.386750071289866e-06
1908,6070,0,6070,0.4405369758605957,4.288471606420333e-06
1910,6076,0,6076,0.4409348964691162,4.21301580986846e-06
1912,6082,0,6082,0.441342830657959,4.13628491655002e-06
1914,6088,0,6088,0.44174695014953613,4.05522021353777e-06
1916,6094,0,6094,0.4421849250793457,3.968261181833069e-06
1919,6103,0,6103,0.44278907775878906,3.8305371895293474e-06
1921,6109,0,6109,0.4431941509246826,3.7389858090446e-06
1923,6115,0,6115,0.44359898567199707,3.654101688758791e-06
1925,6121,0,6121,0.4439988136291504,3.5745515238017193e-06
1928,6130,0,6130,0.44460296630859375,3.4633911248126237e-06
1930,6136,0,6136,0.4450089931488037,3.3927595922862653e-06
1932,6142,0,6142,0.44541192054748535,3.3236642103792565e-06
1934,6148,0,6148,0.44580984115600586,3.255790125275494e-06
1936,6154,0,6154,0.4462308883666992,3.188753048665506e-06
1939,6163,0,6163,0.4468388557434082,3.0942855988742246e-06
1941,6169,0,6169,0.44723987579345703,3.037652267540049e-06
1943,6175,0,6175,0.44763994216918945,2.9839371077441595e-06
1945,6181,0,6181,0.4480459690093994,2.9306777467746685e-06
1948,6190,0,6190,0.44864988327026367,2.849362419593326e-06
1950,6196,0,6196,0.4490528106689453,2.793264520982154e-06
1952,6202,0,6202,0.44945406913757324,2.7357033646313096e-06
1954,6208,0,6208,0.4498610496520996,2.6754275150212552e-06
1956,6214,0,6214,0.45026183128356934,2.6128258326442256e-06
1959,6223,0,6223,0.4508640766143799,2.522605323830659e-06
1961,6229,0,6229,0.4512639045715332,2.4665344795656467e-06
1963,6235,0,6235,0.4516777992248535,2.411294187796453e-06
1965,6241,0,6241,0.45208001136779785,2.3575256039872623e-06
1968,6250,0,6250,0.4526839256286621,2.281438437999771e-06
1970,6256,0,6256,0.4530830383300781,2.234292040149016e-06
1972,6262,0,6262,0.4534881114959717,2.1891283628042634e-06
1974,6268,0,6268,0.4538888931274414,2.145088517337948e-06
1976,6274,0,6274,0.45428895950317383,2.1049012838142355e-06
1979,6283,0,6283,0.454941987991333,2.0522419854299363e-06
1981,6289,0,6289,0.45534586906433105,2.0183081368319804e-06
1983,6295,0,6295,0.4557459354400635,1.9832804438514418e-06
1985,6301,0,6301,0.4561440944671631,1.9479858041170904e-06
1988,6310,0,6310,0.45674800872802734,1.8963459946000772e-06
1990,6316,0,6316,0.4571499824523926,1.8604135714804818e-06
1992,6322,0,6322,0.4575510025024414,1.8211246664850677e-06
1994,6328,0,6328,0.4579489231109619,1.7805076866726734e-06
1996,6334,0,6334,0.45835304260253906,1.7423223202476073e-06
1999,6343,0,6343,0.458953857421875,1.6902831926970196e-06
2001,6349,0,6349,0.45935606956481934,1.6569814884848666e-06
2003,6355,0,6355,0.45975184440612793,1.6254023749674381e-06
2005,6361,0,6361,0.4601559638977051,1.5964927487773213e-06
2008,6370,0,6370,0.46075987815856934,1.5565234433351884e-06
2010,6376,0,6376,0.46116089820861816,1.5305887810640552e-06
2012,6382,0,6382,0.46158695220947266,1.5043193587196617e-06
2014,6388,0,6388,0.4620089530944824,1.4795586681917858e-06
2016,6394,0,6394,0.46240997314453125,1.4569484858481286e-06
2019,6403,0,6403,0.46303296089172363,1.4247953389929131e-06
2021,6409,0,6409,0.4634389877319336,1.4037394715061155e-06
2023,6415,0,6415,0.46384310722351074,1.383200882515953e-06
2025,6421,0,6421,0.4642488956451416,1.3630435387714828e-06
2028,6430,0,6430,0.4648609161376953,1.3300987966746942e-06
2030,6436,0,6436,0.4652700424194336,1.3044090138463078e-06
2032,6442,0,6442,0.46567392349243164,1.2756931832195159e-06
2034,6448,0,6448,0.4660789966583252,1.2461309343459852e-06
2036,6454,0,6454,0.4664878845214844,1.2178652651607452e-06
2039,6463,0,6463,0.4671039581298828,1.1810590215351881e-06
2041,6469,0,6469,0.46750783920288086,1.160817964198903e-06
2043,6475,0,6475,0.4679138660430908,1.142366376892682e-06
2045,6481,0,6481,0.4683208465576172,1.123853991050659e-06
2048,6490,0,6490,0.4689309597015381,1.0943372624798231e-06
2050,6496,0,6496,0.4693338871002197,1.0730677762364225e-06
2052,6502,0,6502,0.4697420597076416,1.051138599909649e-06
2054,6508,0,6508,0.47014904022216797,1.029146399303692e-06
2056,6514,0,6514,0.4705510139465332,1.0084278412557066e-06
2059,6523,0,6523,0.4711599349975586,9.841325531869042e-07
2061,6529,0,6529,0.47156810760498047,9.715112805133928e-07
2063,6535,0,6535,0.47197484970092773,9.599376948482413e-07
2065,6541,0,6541,0.4723827838897705,9.474792491095004e-07
2068,6550,0,6550,0.4729881286621094,9.234415056089584e-07
2070,6556,0,6556,0.47339296340942383,9.02542329863858e-07
2072,6562,0,6562,0.4737989902496338,8.780335157995937e-07
2074,6568,0,6568,0.4742000102996826,8.5127813255361e-07
2076,6574,0,6574,0.47460508346557617,8.271289897036493e-07
2079,6583,0,6583,0.4752161502838135,8.043360141622986e-07
2081,6589,0,6589,0.47562098503112793,7.944774252971988e-07
2083,6595,0,6595,0.4760251045227051,7.852637020033281e-07
2085,6601,0,6601,0.4764289855957031,7.753368342147057e-07
2088,6610,0,6610,0.4770359992980957,7.568577956673808e-07
2090,6616,0,6616,0.4774470329284668,7.417404232224183e-07
2092,6622,0,6622,0.47784900665283203,7.24866274995817e-07
2094,6628,0,6628,0.4782528877258301,7.066342104972851e-07
2096,6634,0,6634,0.47866010665893555,6.899245312368914e-07
2099,6643,0,6643,0.479266881942749,6.745133255984736e-07
2101,6649,0,6649,0.47967004776000977,6.684811292709167e-07
2103,6655,0,6655,0.4800739288330078,6.629273392297042e-07
2105,6661,0,6661,0.4804809093475342,6.564891308354825e-07
2108,6670,0,6670,0.48108696937561035,6.424264638827556e-07
2110,6676,0,6676,0.4814918041229248,6.287856888299277e-07
2112,6682,0,6682,0.48189592361450195,6.126406646356966e-07
2114,6688,0,6688,0.4823019504547119,5.948985792743869e-07
2117,6697,0,6697,0.4829108715057373,5.692538276314373e-07
2119,6703,0,6703,0.48331212997436523,5.57243674294541e-07
2121,6709,0,6709,0.4837150573730469,5.497807543873073e-07
2123,6715,0,6715,0.48412108421325684,5.444018263839964e-07
2125,6721,0,6721,0.48452281951904297,5.386751308735539e-07
2128,6730,0,6730,0.4851360321044922,5.251632111770311e-07
2130,6736,0,6736,0.48554110527038574,5.135729948036206e-07
2132,6742,0,6742,0.4859480857849121,5.022690404946138e-07
2134,6748,0,6748,0.48635005950927734,4.908702636601856e-07
2137,6757,0,6757,0.4869558811187744,4.717290288789441e-07
2139,6763,0,6763,0.4873619079589844,4.6296373596408433e-07
2141,6769,0,6769,0.4877748489379883,4.595552974928987e-07
2143,6775,0,6775,0.4881770610809326,4.579169912486697e-07
2145,6781,0,6781,0.48858213424682617,4.5654114979161346e-07
2148,6792,0,6792,0.489224910736084,4.5379042778055214e-07
2150,6800,0,6800,0.4896690845489502,4.5146103577810145e-07
2152,6806,0,6806,0.49007201194763184,4.4467386348811894e-07
2154,6812,0,6812,0.4904770851135254,4.3514312120271696e-07
2157,6821,0,6821,0.4910850524902344,4.214231888580186e-07
2159,6827,0,6827,0.49149489402770996,4.099210360843654e-07
2161,6833,0,6833,0.4918971061706543,3.9714466600851936e-07
2163,6839,0,6839,0.4923539161682129,3.8550092923572444e-07
2165,6846,0,6846,0.4927799701690674,3.836021822010396e-07
2168,6855,0,6855,0.4933931827545166,3.8056127134495853e-07
2170,6861,0,6861,0.49379801750183105,3.771949168303902e-07
2172,6867,0,6867,0.4942047595977783,3.730846650311065e-07
2174,6873,0,6873,0.4946119785308838,3.6890055110766584e-07
2177,6882,0,6882,0.4952239990234375,3.6501798563296196e-07
2179,6889,0,6889,0.49564695358276367,3.6439489254979305e-07
2181,6895,0,6895,0.49605298042297363,3.617266437388464e-07
2183,6901,0,6901,0.4964599609375,3.536994912360176e-07
2185,6907,0,6907,0.49686384201049805,3.451812832689304e-07
2188,6916,0,6916,0.49747180938720703,3.3296442285415076e-07
2190,6922,0,6922,0.497877836227417,3.256077488236055e-07
2192,6928,0,6928,0.4982919692993164,3.187117297497461e-07
2194,6934,0,6934,0.49869418144226074,3.1227645664948935e-07
2197,6943,0,6943,0.4993021488189697,3.042769669121999e-07
2199,6949,0,6949,0.4997081756591797,3.0014297709376113e-07
2201,6955,0,6955,0.500114917755127,2.966394122606015e-07
2203,6961,0,6961,0.5005171298980713,2.9362088231916977e-07
2205,6967,0,6967,0.5009210109710693,2.921326576985045e-07
2208,6978,0,6978,0.5015678405761719,2.8707000650015454e-07
2210,6985,0,6985,0.5019938945770264,2.860488136437498e-07
2212,6992,0,6992,0.5024161338806152,2.845360745687516e-07
2214,6998,0,6998,0.5028221607208252,2.8053058930582453e-07
2217,7005,0,7005,0.5033960342407227,1.5120112999847873e-07
2219,7009,0,7009,0.5037648677825928,3.457127791943085e-08
2221,7013,0,7013,0.5041310787200928,9.194847961703968e-09


==> plot_data/quadratic_minimax_problem_n500_alpha0/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.001844167709350586,30.358099469249375
200,201,200,401,0.2851991653442383,1.7006076310549407
400,401,400,801,0.577491044998169,0.9112475403461391
601,602,601,1203,0.8584110736846924,0.6722636706984941
801,802,801,1603,1.160689115524292,0.5549897589038558
1001,1002,1001,2003,1.4554681777954102,0.4774627272054353
1201,1202,1201,2403,1.7318952083587646,0.5020323359805887
1401,1402,1401,2803,2.0084621906280518,0.38067029692333876
1602,1603,1602,3205,2.362065076828003,0.3601892103963759
1802,1803,1802,3605,2.6659011840820312,0.31710086376541813
2002,2003,2002,4005,2.9439010620117188,0.29347919987041415
2202,2203,2202,4405,3.225637197494507,0.27406544712310116
2402,2403,2402,4805,3.5074520111083984,0.2553087833982936
2603,2604,2603,5207,3.7808001041412354,0.28020453691043595
2803,2804,2803,5607,4.054150104522705,0.2712535221053058
3003,3004,3003,6007,4.3579301834106445,0.21318155887917348
3203,3204,3203,6407,4.643322944641113,0.2016132207213287
3403,3404,3403,6807,4.939672231674194,0.19222972981543524
3604,3605,3604,7209,5.267271995544434,0.19720315810070332
3804,3805,3804,7609,5.592290163040161,0.2103584348564755
4004,4005,4004,8009,5.8855061531066895,0.16723134771200343
4204,4205,4204,8409,6.151831150054932,0.16097492421107829
4404,4405,4404,8809,6.322810888290405,0.18559891251431232
4605,4606,4605,9211,6.495526075363159,0.14796662382591377
4805,4806,4805,9611,6.665279150009155,0.14277715729873722
5005,5006,5005,10011,6.83432412147522,0.13693486384378642
5205,5206,5205,10411,7.011662244796753,0.13321751244473776
5405,5406,5405,10811,7.192115068435669,0.12989757235492205
5606,5607,5606,11213,7.396651029586792,0.12372810737229124
5806,5807,5806,11613,7.583511114120483,0.12029605282208732
6006,6007,6006,12013,7.757652044296265,0.11637741263661482
6206,6207,6206,12413,7.934596300125122,0.11304469291731661
6406,6407,6406,12813,8.106170892715454,0.10838983801664176
6607,6608,6607,13215,8.2726469039917,0.10869187317633078
6807,6808,6807,13615,8.456902980804443,0.10290095462612837
7007,7008,7007,14015,8.643841028213501,0.10040248709864004
7207,7208,7207,14415,8.819017171859741,0.09730251506941644
7407,7408,7407,14815,8.987826108932495,0.11108634162819774
7608,7609,7608,15217,9.16200304031372,0.09224893113525348
7808,7809,7808,15617,9.333218097686768,0.08916263693421927
8008,8009,8008,16017,9.512444972991943,0.08742133097297906
8208,8209,8208,16417,9.697824001312256,0.08516906645897578
8408,8409,8408,16817,9.875104188919067,0.0837398182167758
8609,8610,8609,17219,10.070091009140015,0.08038455606222403
8809,8810,8809,17619,10.244209051132202,0.08033410025209158
9009,9010,9009,18019,10.44275712966919,0.07712365252907863
9209,9210,9209,18419,10.710820198059082,0.07546326483973753
9409,9410,9409,18819,10.984771251678467,0.07648345218889664
9610,9611,9610,19221,11.175579071044922,0.07224063238108902
9810,9811,9810,19621,11.43315315246582,0.07113843989150681
10010,10011,10010,20021,11.618467092514038,0.0695586428950319
10210,10211,10210,20421,11.824803113937378,0.08356522464504641
10410,10411,10410,20821,11.981074094772339,0.06712960112109609
10611,10612,10611,21223,12.157926082611084,0.06699359466531633
10811,10812,10811,21623,12.329273223876953,0.06541908874086734
11011,11012,11011,22023,12.506890058517456,0.06382542624128312
11211,11212,11211,22423,12.720428228378296,0.06269648293635686
11411,11412,11411,22823,12.893160104751587,0.0610488090686334
11612,11613,11612,23225,13.046871185302734,0.06338505860176886
11812,11813,11812,23625,13.230136156082153,0.059617103548654356
12012,12013,12012,24025,13.492700099945068,0.05916471716834446
12212,12213,12212,24425,13.692963123321533,0.05832033721416688
12412,12413,12412,24825,13.901644229888916,0.05722802924727787
12613,12614,12613,25227,14.119035959243774,0.05642084573567756
12813,12814,12813,25627,14.306643962860107,0.054970058700584315
13013,13014,13013,26027,14.482401132583618,0.054362710210040736
13213,13214,13213,26427,14.647200107574463,0.0548684809923365
13413,13414,13413,26827,14.816962242126465,0.05329343776503196
13614,13615,13614,27229,14.97458004951477,0.05206264518775205
13814,13815,13814,27629,15.134797096252441,0.053576796645504174
14014,14015,14014,28029,15.307538986206055,0.05143273277248047
14214,14215,14214,28429,15.548218250274658,0.05057808402386697
14414,14415,14414,28829,15.781007289886475,0.05019351604690433
14615,14616,14615,29231,15.967069149017334,0.04907278752747184
14815,14816,14815,29631,16.17525315284729,0.048963949757096954
15015,15016,15015,30031,16.338297128677368,0.048334930520042445
15215,15216,15215,30431,16.545838117599487,0.048956526721502566
15415,15416,15415,30831,16.7501802444458,0.047105109130263494
15616,15617,15616,31233,16.930963039398193,0.04638475401498077
15816,15817,15816,31633,17.100152254104614,0.046620882576732955
16016,16017,16016,32033,17.25538206100464,0.05262818931815664
16216,16217,16216,32433,17.43974995613098,0.04542925345577664
16416,16417,16416,32833,17.680570125579834,0.04522861502190292
16617,16618,16617,33235,17.868226051330566,0.04477520875790979
16817,16818,16817,33635,18.084577083587646,0.04414845185933609
17017,17018,17017,34035,18.289923191070557,0.04366503516601011
17217,17218,17217,34435,18.475831031799316,0.05022539783196252
17417,17418,17417,34835,18.75199604034424,0.04291044853519493
17618,17619,17618,35237,18.93560004234314,0.050873035055087924
17818,17819,17818,35637,19.118653059005737,0.042273969493643954
18018,18019,18018,36037,19.299345016479492,0.05036172028208931
18218,18219,18218,36437,19.47788405418396,0.0415931367633282
18418,18419,18418,36837,19.644554138183594,0.041214840415818035
18619,18620,18619,37239,19.99181318283081,0.04105012665697059
18819,18820,18819,37639,20.18104100227356,0.040860701696957664
19019,19020,19019,38039,20.367293119430542,0.04054281334698695
19219,19220,19219,38439,20.562137126922607,0.039865432952396716
19419,19420,19419,38839,20.87711215019226,0.041147997577064256
19620,19621,19620,39241,21.062576055526733,0.03953747525468505
19820,19821,19820,39641,21.21853494644165,0.03928764681896595
20020,20021,20020,40041,21.394946098327637,0.039082868496820244
20220,20221,20220,40441,21.57203221321106,0.038372768630625304
20420,20421,20420,40841,21.765656232833862,0.037848285778436665
20621,20622,20621,41243,21.937342166900635,0.0417872609059276
20821,20822,20821,41643,22.089575052261353,0.0440074007147347
21021,21022,21021,42043,22.23697805404663,0.03720117020720569
21221,21222,21221,42443,22.4046630859375,0.037688310088188966
21421,21422,21421,42843,22.566400051116943,0.037064899274681075
21622,21623,21622,43245,22.73022699356079,0.037828882228458954
21822,21823,21822,43645,22.931102991104126,0.03677659783669953
22022,22023,22022,44045,23.089967966079712,0.036256182283724556
22222,22223,22222,44445,23.24852204322815,0.03605278245410219
22422,22423,22422,44845,23.404009103775024,0.03598327331237605
22623,22624,22623,45247,23.55874013900757,0.03582717489272665
22823,22824,22823,45647,23.71844792366028,0.043552763093730934
23023,23024,23023,46047,23.880587100982666,0.03500075753036403
23223,23224,23223,46447,24.030436277389526,0.03600642543410127
23423,23424,23423,46847,24.180236101150513,0.03478625972020386
23624,23625,23624,47249,24.332945108413696,0.03488851327720817
23824,23825,23824,47649,24.488089084625244,0.03423711214273072
24024,24025,24024,48049,24.637041091918945,0.03674296420485604
24224,24225,24224,48449,24.799724102020264,0.03412610626459489
24424,24425,24424,48849,24.947165966033936,0.033909140887717654
24625,24626,24625,49251,25.093940019607544,0.03451988308521902
24825,24826,24825,49651,25.251464128494263,0.033948871860907406
25025,25026,25025,50051,25.402979135513306,0.035017848233246836
25225,25226,25225,50451,25.550644159317017,0.03318125025514594
25425,25426,25425,50851,25.69998002052307,0.03308171332205296
25626,25627,25626,51253,25.860636949539185,0.03963620655534278
25826,25827,25826,51653,26.023864269256592,0.03273167493828358
26026,26027,26026,52053,26.183945178985596,0.03273585001029364
26226,26227,26226,52453,26.35003399848938,0.032675332145086236
26426,26427,26426,52853,26.498319149017334,0.032145549115602634
26627,26628,26627,53255,26.651177167892456,0.03203332764990996
26827,26828,26827,53655,26.79727005958557,0.0328141190120363
27027,27028,27027,54055,26.964818954467773,0.03148669957668568
27227,27228,27227,54455,27.11321496963501,0.03821585156448793
27427,27428,27427,54855,27.26255226135254,0.0317038601867372
27628,27629,27628,55257,27.412743091583252,0.03770103610817365
27828,27829,27828,55657,27.558813095092773,0.03107237971700072
28028,28029,28028,56057,27.70581889152527,0.03570891221649926
28228,28229,28228,56457,27.852468013763428,0.031050893488329137
28428,28429,28428,56857,28.00010395050049,0.03099444372477587
28629,28630,28629,57259,28.149030923843384,0.030838816080487313
28829,28830,28829,57659,28.30271005630493,0.03233791651087027
29029,29030,29029,58059,28.467103004455566,0.03542717355646013
29229,29230,29229,58459,28.619551181793213,0.030906676631839124
29429,29430,29429,58859,28.7793390750885,0.030012110790273033
29630,29631,29630,59261,28.95788598060608,0.02983795404344887
29830,29831,29830,59661,29.296247243881226,0.03002670501725421
30030,30031,30030,60061,29.462156057357788,0.029877584039166336
30230,30231,30230,60461,29.63775610923767,0.029568724461103122
30430,30431,30430,60861,29.79379630088806,0.029446427484848898
30631,30632,30631,61263,30.14092707633972,0.02960108497503998
30831,30832,30831,61663,30.308423042297363,0.02905262187562605
31031,31032,31031,62063,30.480440139770508,0.02935833510871864
31231,31232,31231,62463,30.648314952850342,0.0287323953572807
31431,31432,31431,62863,30.822739124298096,0.03100684020902864
31632,31633,31632,63265,30.994270086288452,0.036130863198687704
31832,31833,31832,63665,31.186662912368774,0.03276044561251601
32032,32033,32032,64065,31.36992907524109,0.02941969145489503
32232,32233,32232,64465,31.538377046585083,0.02865252850439644
32432,32433,32432,64865,31.698933124542236,0.02837826018780118
32633,32634,32633,65267,31.86293625831604,0.027867617645529086
32833,32834,32833,65667,32.019264221191406,0.027769006098614483
33033,33034,33033,66067,32.172280073165894,0.027802387375615325
33233,33234,33233,66467,32.33020496368408,0.027692946691787356
33433,33434,33433,66867,32.4995059967041,0.027662822831694623
33634,33635,33634,67269,32.65508413314819,0.029642741706556484
33834,33835,33834,67669,32.813727140426636,0.028898904604688
34034,34035,34034,68069,32.96840190887451,0.0273998198180117
34234,34235,34234,68469,33.16621494293213,0.027348110178125495
34434,34435,34434,68869,33.34608221054077,0.02757111093417047
34635,34636,34635,69271,33.53239297866821,0.02704868541709397
34835,34836,34835,69671,33.710554122924805,0.03455088309289085
35035,35036,35035,70071,33.868221044540405,0.027455113972297614
35235,35236,35235,70471,34.02952718734741,0.02679496865805395
35435,35436,35435,70871,34.20826292037964,0.026701251785294
35636,35637,35636,71273,34.3732750415802,0.026466017926516903
35836,35837,35836,71673,34.53052020072937,0.026475250676945464
36036,36037,36036,72073,34.692973136901855,0.02649334857511161
36236,36237,36236,72473,34.852459192276,0.03260106435085443
36436,36437,36436,72873,35.011834144592285,0.026185302707113816
36637,36638,36637,73275,35.167394161224365,0.03225827264464111
36837,36838,36837,73675,35.335456132888794,0.026713128013641754
37037,37038,37037,74075,35.499940156936646,0.025933681473449245
37237,37238,37237,74475,35.674575328826904,0.026280173564904637
37437,37438,37437,74875,35.834861278533936,0.026168925420021024
37638,37639,37638,75277,35.99336814880371,0.025873610471282373
37838,37839,37838,75677,36.15904712677002,0.025542900344546027
38038,38039,38038,76077,36.31306290626526,0.026901081786780405
38238,38239,38238,76477,36.47179126739502,0.02529367335097412
38438,38439,38438,76877,36.6367130279541,0.027811866616852258
38639,38640,38639,77279,36.79652523994446,0.02527610598335215
38839,38840,38839,77679,36.960472106933594,0.025112990050991022
39039,39040,39039,78079,37.118128061294556,0.025418283680628203
39239,39240,39239,78479,37.28821897506714,0.024842956112366452
39439,39440,39439,78879,37.46559023857117,0.024939275762930098
39640,39641,39640,79281,37.61996817588806,0.024679147976757108
39840,39841,39840,79681,37.78778028488159,0.024681939625606802
40040,40041,40040,80081,37.96039915084839,0.02453795649116443
40240,40241,40240,80481,38.113255977630615,0.024637858555959218
40440,40441,40440,80881,38.26786422729492,0.024564388137275867
40641,40642,40641,81283,38.433757066726685,0.024646483011776986
40841,40842,40841,81683,38.588685274124146,0.024343314299402934
41041,41042,41041,82083,38.74656796455383,0.024251251468409746
41241,41242,41241,82483,38.94645619392395,0.029778130230561847
41441,41442,41441,82883,39.113935232162476,0.02404858714789033
41642,41643,41642,83285,39.27952313423157,0.023936760149282973
41842,41843,41842,83685,39.44606614112854,0.023944416200273703
42042,42043,42042,84085,39.610913038253784,0.023857891869585666
42242,42243,42242,84485,39.76405215263367,0.023874148271617483
42442,42443,42442,84885,39.93184518814087,0.023673734320089707
42643,42644,42643,85287,40.09764623641968,0.023626542539040694
42843,42844,42843,85687,40.252846240997314,0.028651624481657253
43043,43044,43043,86087,40.41276288032532,0.024015123769717952
43243,43244,43243,86487,40.576266050338745,0.02336243383948069
43443,43444,43443,86887,40.73420214653015,0.024508151923644337
43644,43645,43644,87289,40.89054322242737,0.025821325081299265
43844,43845,43844,87689,41.04297614097595,0.023114918596386345
44044,44045,44044,88089,41.20749497413635,0.024528665166417437
44244,44245,44244,88489,41.38906717300415,0.02353646832250001
44444,44445,44444,88889,41.56316113471985,0.02683007715324352
44645,44646,44645,89291,41.72140407562256,0.022905011963139123
44845,44846,44845,89691,41.89132905006409,0.0229479074901674
45045,45046,45045,90091,42.05903506278992,0.022804216155202665
45245,45246,45245,90491,42.23222303390503,0.022675173858634972
45445,45446,45445,90891,42.3913791179657,0.02281835815649117
45646,45647,45646,91293,42.553232192993164,0.02702895904664809
45846,45847,45846,91693,42.70930099487305,0.02256611067697314
46046,46047,46046,92093,42.867419958114624,0.02253197646145024
46246,46247,46246,92493,43.02800798416138,0.0223876499582941
46446,46447,46446,92893,43.19117021560669,0.022171655137270877
46647,46648,46647,93295,43.35110831260681,0.02240833401221567
46847,46848,46847,93695,43.50679111480713,0.022475442667686352
47047,47048,47047,94095,43.6828351020813,0.023773869475390907
47247,47248,47247,94495,43.85932111740112,0.02209162976826666
47447,47448,47447,94895,44.02738308906555,0.022209668720491547
47648,47649,47648,95297,44.20462489128113,0.02250901754905959
47848,47849,47848,95697,44.401094913482666,0.02347167747305269
48048,48049,48048,96097,44.569735050201416,0.021798083184909906
48248,48249,48248,96497,44.73832607269287,0.021860920850733427
48448,48449,48448,96897,44.898242235183716,0.02401069985665101
48649,48650,48649,97299,45.066620111465454,0.02286475559973605
48849,48850,48849,97699,45.26936197280884,0.02233249972215759
49049,49050,49049,98099,45.43558216094971,0.021449405460546286
49249,49250,49249,98499,45.608941078186035,0.022382096814697567
49449,49450,49449,98899,45.76765513420105,0.021516750705197374
49650,49651,49650,99301,45.928842067718506,0.025116030600778924
49850,49851,49850,99701,46.09264016151428,0.021271692750979173
50050,50051,50050,100101,46.26068615913391,0.021209808654068168
50250,50251,50250,100501,46.437785148620605,0.021752525197229484
50450,50451,50450,100901,46.61770009994507,0.02121452811459931
50651,50652,50651,101303,46.80190706253052,0.022474661873852022
50851,50852,50851,101703,46.96491026878357,0.021015955741441588
51051,51052,51051,102103,47.121554136276245,0.023769733002408686
51251,51252,51251,102503,47.286362171173096,0.02291967204938169
51451,51452,51451,102903,47.450494050979614,0.020704511991813297
51652,51653,51652,103305,47.620129108428955,0.02419938209364002
51852,51853,51852,103705,47.789243936538696,0.020749231223402338
52052,52053,52052,104105,47.94547724723816,0.020620607487106726
52252,52253,52252,104505,48.104389905929565,0.020685232419967715
52452,52453,52452,104905,48.262266874313354,0.02036558902563882
52653,52654,52653,105307,48.42462921142578,0.02385088395788482
52853,52854,52853,105707,48.58945417404175,0.020380497047840417
53053,53054,53053,106107,48.756229877471924,0.020337753261422117
53253,53254,53253,106507,48.91973519325256,0.02037664961961324
53453,53454,53453,106907,49.07400703430176,0.020153234964276942
53654,53655,53654,107309,49.25905513763428,0.02647976427329628
53854,53855,53854,107709,49.435271978378296,0.02005722577664801
54054,54055,54054,108109,49.59849190711975,0.020939319830561628
54254,54255,54254,108509,49.78145909309387,0.023854784552125835
54454,54455,54454,108909,49.963935136795044,0.026030499919749883
54655,54656,54655,109311,50.12958121299744,0.020137258994200286
54855,54856,54855,109711,50.39729309082031,0.019906949434133063
55055,55056,55055,110111,50.653836250305176,0.020651124853902584
55255,55256,55255,110511,50.845322132110596,0.019743967917853808
55455,55456,55455,110911,51.005635261535645,0.01962907046913023
55656,55657,55656,111313,51.27200698852539,0.019686220167973903
55856,55857,55856,111713,51.54802417755127,0.019835038598160565
56056,56057,56056,112113,51.72602200508118,0.02232944666929513
56256,56257,56256,112513,51.90032911300659,0.02449304798569066
56456,56457,56456,112913,52.06549906730652,0.019544674350759666
56657,56658,56657,113315,52.2436101436615,0.022574039594402056
56857,56858,56857,113715,52.46863412857056,0.025443530471573023
57057,57058,57057,114115,52.6318621635437,0.019532458163327097
57257,57258,57257,114515,52.79422402381897,0.019342589503502292
57457,57458,57457,114915,52.969149112701416,0.019185174342042918
57658,57659,57658,115317,53.125731229782104,0.019642762255055804
57858,57859,57858,115717,53.342159271240234,0.019079140699214448
58058,58059,58058,116117,53.50138211250305,0.019778510502601005
58258,58259,58258,116517,53.657984018325806,0.01904550931838963
58458,58459,58458,116917,53.81569790840149,0.018888037010169143
58659,58660,58659,117319,53.97003412246704,0.019111321632237926
58859,58860,58859,117719,54.160094022750854,0.018797653314417406
59059,59060,59059,118119,54.31679105758667,0.018843779869422282
59259,59260,59259,118519,54.487590074539185,0.018962402368365158
59459,59460,59459,118919,54.654824018478394,0.01873021573800568
59660,59661,59660,119321,54.82715392112732,0.01871236731439782
59860,59861,59860,119721,55.001466274261475,0.01857267369771664
60060,60061,60060,120121,55.182852268218994,0.01869513943251916
60260,60261,60260,120521,55.34235596656799,0.01865413526086257
60460,60461,60460,120921,55.49633312225342,0.018638327632046432
60661,60662,60661,121323,55.651650190353394,0.02231588678328095
60861,60862,60861,121723,55.804584980010986,0.02104283740568213
61061,61062,61061,122123,55.95757603645325,0.018475950787447168
61261,61262,61261,122523,56.12515211105347,0.018260331725082096
61461,61462,61461,122923,56.29006600379944,0.018424995083053366
61662,61663,61662,123325,56.461634159088135,0.018876204568625387
61862,61863,61862,123725,56.63386607170105,0.01866103394447662
62062,62063,62062,124125,56.80203413963318,0.01833644348252372
62262,62263,62262,124525,56.976911306381226,0.0213161455823791
62462,62463,62462,124925,57.14120602607727,0.02070763618452015
62663,62664,62663,125327,57.3275671005249,0.01801016338788049
62863,62864,62863,125727,57.48940920829773,0.018054005118934183
63063,63064,63063,126127,57.66951513290405,0.01798840849718121
63263,63264,63263,126527,57.84148907661438,0.017820226732605533
63463,63464,63463,126927,58.01320195198059,0.01779550692084509
63664,63665,63664,127329,58.179445028305054,0.017782639732657514
63864,63865,63864,127729,58.350992918014526,0.017795251845324548
64064,64065,64064,128129,58.52941393852234,0.017756334387927248
64264,64265,64264,128529,58.70512795448303,0.017764820182898593
64464,64465,64464,128929,58.91061305999756,0.01767726363769154
64665,64666,64665,129331,59.08381509780884,0.017738505179523894
64865,64866,64865,129731,59.26322913169861,0.01761638975979145
65065,65066,65065,130131,59.45043897628784,0.01797363001266876
65265,65266,65265,130531,59.64099097251892,0.017509799105258204
65465,65466,65465,130931,59.807170152664185,0.017735527388250297
65666,65667,65666,131333,59.98029398918152,0.017379579131193697
65866,65867,65866,131733,60.159669160842896,0.020775241916047654
66066,66067,66066,132133,60.365663051605225,0.021010676567899445
66266,66267,66266,132533,60.55058217048645,0.017334945756246292
66466,66467,66466,132933,60.74827814102173,0.017581446497327086
66667,66668,66667,133335,60.931233167648315,0.02167995598050261
66867,66868,66867,133735,61.166582107543945,0.02122824707557788
67067,67068,67067,134135,61.65830421447754,0.021045458999272938
67267,67268,67267,134535,62.01579189300537,0.017120857847974562
67467,67468,67467,134935,62.27533006668091,0.01688494029381745
67668,67669,67668,135337,62.54130411148071,0.017113718156470465
67868,67869,67868,135737,62.88318920135498,0.016938066044104343
68068,68069,68068,136137,63.16043496131897,0.01708432853341526
68268,68269,68268,136537,63.45049810409546,0.017619598866044493
68468,68469,68468,136937,63.77875995635986,0.017283423762900443
68669,68670,68669,137339,63.97320508956909,0.016643225541608415
68869,68870,68869,137739,64.14732599258423,0.01712715654615588
69069,69070,69069,138139,64.31622409820557,0.01674216501722384
69269,69270,69269,138539,64.54295825958252,0.017426292984704477
69469,69470,69469,138939,64.76776099205017,0.016674579547756394
69670,69671,69670,139341,64.98439311981201,0.019094980375710672
69870,69871,69870,139741,65.23566603660583,0.01658978912873495
70070,70071,70070,140141,65.41444802284241,0.01940435689998246
70270,70271,70270,140541,65.712886095047,0.01665513736190024
70470,70471,70470,140941,65.97577500343323,0.01688376707959082
70671,70672,70671,141343,66.43873620033264,0.016320442559690375
70871,70872,70871,141743,66.68082904815674,0.016399467673715834
71071,71072,71071,142143,66.95831727981567,0.016471362974706832
71271,71272,71271,142543,67.1759901046753,0.016433871311475223
71471,71472,71471,142943,67.43805718421936,0.016304276678523445
71672,71673,71672,143345,67.72649312019348,0.019649387069779405
71872,71873,71872,143745,68.04476714134216,0.016398928867124754
72072,72073,72072,144145,68.36678814888,0.016689615710762603
72272,72273,72272,144545,68.66198921203613,0.01626152835150862
72472,72473,72472,144945,68.9229531288147,0.016314873087065553
72673,72674,72673,145347,69.1053261756897,0.016064256846091165
72873,72874,72873,145747,69.278391122818,0.015983598218756397
73073,73074,73073,146147,69.44797015190125,0.016163364390018354
73273,73274,73273,146547,69.61229801177979,0.01589741843035557
73473,73474,73473,146947,69.77325391769409,0.018704429118366398
73674,73675,73674,147349,69.93091416358948,0.015973272358369855
73874,73875,73874,147749,70.08483004570007,0.015767418260967368
74074,74075,74074,148149,70.23963022232056,0.020060074499005636
74274,74275,74274,148549,70.44899892807007,0.016370083701280475
74474,74475,74474,148949,70.61257100105286,0.015777972849633955
74675,74676,74675,149351,70.76955819129944,0.015673695217123956
74875,74876,74875,149751,70.94456911087036,0.015640090486248235
75075,75076,75075,150151,71.1252920627594,0.015483802438880975
75275,75276,75275,150551,71.29362797737122,0.015875083453601585
75475,75476,75475,150951,71.46879410743713,0.015679891930946724
75676,75677,75676,151353,71.65364098548889,0.015522018411993422
75876,75877,75876,151753,71.88973593711853,0.015515651350156593
76076,76077,76076,152153,72.0450210571289,0.019172175237301647
76276,76277,76276,152553,72.23739814758301,0.01826605117673208
76476,76477,76476,152953,72.41101312637329,0.015489420008557424
76677,76678,76677,153355,72.59922003746033,0.015448653248781079
76877,76878,76877,153755,72.85920214653015,0.015814187188726715
77077,77078,77077,154155,73.02126502990723,0.015253022554040093
77277,77278,77277,154555,73.22256326675415,0.015351540344436334
77477,77478,77477,154955,73.4369249343872,0.0151819946812419
77678,77679,77678,155357,73.60286903381348,0.015317884406705954
77878,77879,77878,155757,73.80817794799805,0.015134925866145022
78078,78079,78078,156157,73.96428513526917,0.017530072381278024
78278,78279,78278,156557,74.1235830783844,0.015477372807974331
78478,78479,78478,156957,74.28442120552063,0.015039927269619837
78679,78680,78679,157359,74.47032809257507,0.015109615762249763
78879,78880,78879,157759,74.64352011680603,0.014961004491263452
79079,79080,79079,158159,74.82810020446777,0.015056746747331054
79279,79280,79279,158559,74.98655009269714,0.014964839789269732
79479,79480,79479,158959,75.14147210121155,0.014861883892788995
79680,79681,79680,159361,75.30649018287659,0.014801881607957345
79880,79881,79880,159761,75.49155521392822,0.014780407867536954
80080,80081,80080,160161,75.65598320960999,0.015277406221414718
80280,80281,80280,160561,75.82381319999695,0.014946267435902291
80480,80481,80480,160961,75.99496507644653,0.014762584548580404
80681,80682,80681,161363,76.16782808303833,0.014737401786930338
80881,80882,80881,161763,76.3424642086029,0.01776307821247424
81081,81082,81081,162163,76.54346299171448,0.014527391654567222
81281,81282,81281,162563,76.71522521972656,0.014727045506573725
81481,81482,81481,162963,76.89745593070984,0.014577351903278255
81682,81683,81682,163365,77.11399817466736,0.014530843011670408
81882,81883,81882,163765,77.28544807434082,0.016861974400582166
82082,82083,82082,164165,77.51314210891724,0.017448226895021526
82282,82283,82282,164565,77.7246081829071,0.014507704448627073
82482,82483,82482,164965,77.88075923919678,0.01451273587397952
82683,82684,82683,165367,78.03357696533203,0.014654598454277627
82883,82884,82883,165767,78.18770003318787,0.0143743086721234
83083,83084,83083,166167,78.34507298469543,0.015190555983361597
83283,83284,83283,166567,78.51148915290833,0.014502384635867269
83483,83484,83483,166967,78.66636800765991,0.014388363138483762
83684,83685,83684,167369,78.82557797431946,0.014360835325272001
83884,83885,83884,167769,79.00286912918091,0.014128426308329552
84084,84085,84084,168169,79.24603605270386,0.014569264888521229
84284,84285,84284,168569,79.42584204673767,0.01616922222725642
84484,84485,84484,168969,79.59760308265686,0.01614332442623157
84685,84686,84685,169371,79.78957390785217,0.014052079513497547
84885,84886,84885,169771,79.95601511001587,0.013962891821019495
85085,85086,85085,170171,80.11181592941284,0.01409555681863181
85285,85286,85285,170571,80.27587795257568,0.013989605992560775
85485,85486,85485,170971,80.46664023399353,0.013975667909497657
85686,85687,85686,171373,80.62461709976196,0.014005264703599885
85886,85887,85886,171773,80.85659408569336,0.01403419892016429
86086,86087,86086,172173,81.05438017845154,0.016684594913685312
86286,86287,86286,172573,81.24004793167114,0.01633826623829239
86486,86487,86486,172973,81.43570303916931,0.016009238985131246
86687,86688,86687,173375,81.61119222640991,0.013898220722144436
86887,86888,86887,173775,81.7781331539154,0.01373810605151921
87087,87088,87087,174175,81.96766400337219,0.013688031395969882
87287,87288,87287,174575,82.19451308250427,0.013800703593006789
87487,87488,87487,174975,82.49215817451477,0.017238578339612683
87688,87689,87688,175377,82.87341809272766,0.013838126249453792
87888,87889,87888,175777,83.19113612174988,0.014610040441163525
88088,88089,88088,176177,83.49578022956848,0.013623594225415748
88288,88289,88288,176577,83.92312407493591,0.013463979960098675
88488,88489,88488,176977,84.36211109161377,0.013666142183179486
88689,88690,88689,177379,84.54315114021301,0.018056632896177982
88889,88890,88889,177779,84.71224093437195,0.013477819521355978
89089,89090,89089,178179,84.89849519729614,0.013565873804621062
89289,89290,89289,178579,85.06662917137146,0.013771769111185793
89489,89490,89489,178979,85.23775601387024,0.01560142996861236
89690,89691,89690,179381,85.5614161491394,0.014902749190971901
89890,89891,89890,179781,85.90626692771912,0.01449821618415836
90090,90091,90090,180181,86.16370797157288,0.013323560697736606
90290,90291,90290,180581,86.34986019134521,0.013287802968408403
90490,90491,90490,180981,86.5174651145935,0.013348869958275358
90691,90692,90691,181383,86.68945121765137,0.013462366228382512
90891,90892,90891,181783,86.8718810081482,0.01317371919729869
91091,91092,91091,182183,87.08196711540222,0.013162862847947645
91291,91292,91291,182583,87.29442310333252,0.013186399768884544
91491,91492,91491,182983,87.58738708496094,0.013356652253427402
91692,91693,91692,183385,87.88721513748169,0.013269390982329522
91892,91893,91892,183785,88.1641161441803,0.01309773135345503
92092,92093,92092,184185,88.34913206100464,0.013040785837659438
92292,92293,92292,184585,88.5307149887085,0.01317509872828938
92492,92493,92492,184985,88.7042281627655,0.012973998902944013
92693,92694,92693,185387,88.87675404548645,0.013066655973427542
92893,92894,92893,185787,89.07757496833801,0.01599176563798967
93093,93094,93093,186187,89.24930810928345,0.01611260530946527
93293,93294,93293,186587,89.444491147995,0.013263634459388551
93493,93494,93493,186987,89.66110610961914,0.012910015218854362
93694,93695,93694,187389,89.88553023338318,0.012892110654134762
93894,93895,93894,187789,90.15001606941223,0.012805016898411934
94094,94095,94094,188189,90.39431500434875,0.01294249037623989
94294,94295,94294,188589,90.60737895965576,0.012853062092041376
94494,94495,94494,188989,90.79513025283813,0.012977144653887284
94695,94696,94695,189391,90.97147011756897,0.013615864220470883
94895,94896,94895,189791,91.14231204986572,0.014648405187975003
95095,95096,95095,190191,91.32156610488892,0.015122422648473263
95295,95296,95295,190591,91.55084919929504,0.012906162741433908
95495,95496,95495,190991,91.74350500106812,0.01253714644483266
95696,95697,95696,191393,91.934396982193,0.012542372764778507
95896,95897,95896,191793,92.11509418487549,0.012746681143910664
96096,96097,96096,192193,92.3457260131836,0.01500593553237307
96296,96297,96296,192593,92.5834641456604,0.015149575036105237
96496,96497,96496,192993,92.75543522834778,0.01253802064752151
96697,96698,96697,193395,92.98802018165588,0.012822815572050164
96897,96898,96897,193795,93.15899014472961,0.012448512944557366
97097,97098,97097,194195,93.45008707046509,0.012404846271103808
97297,97298,97297,194595,93.73636627197266,0.012453320208038618
97497,97498,97497,194995,94.12829399108887,0.012461469044157807
97698,97699,97698,195397,94.48360109329224,0.012464363325068567
97898,97899,97898,195797,94.81160092353821,0.014093359520775573
98098,98099,98098,196197,94.96662926673889,0.01230702634349713
98298,98299,98298,196597,95.13042616844177,0.012269606060666717
98498,98499,98498,196997,95.33817028999329,0.012447858347471684
98699,98700,98699,197399,95.56848120689392,0.012312789878963178
98899,98900,98899,197799,95.72678995132446,0.01484382909505566
99099,99100,99099,198199,95.89674806594849,0.014224649632781425
99299,99300,99299,198599,96.07069802284241,0.012739801233687011
99499,99500,99499,198999,96.23843312263489,0.012134554540379637
99700,99701,99700,199401,96.4112389087677,0.012129207971300047
99900,99901,99900,199801,96.60144114494324,0.012161898810025005
100100,100101,100100,200201,96.79954099655151,0.0121193003684653
100300,100301,100300,200601,96.96107602119446,0.012108584931694666
100501,100502,100501,201003,97.14908719062805,0.01226296230453011
100701,100702,100701,201403,97.31998324394226,0.012026353882558294
100901,100902,100901,201803,97.4936830997467,0.011928954369523594
101101,101102,101101,202203,97.66569805145264,0.012060841542286054
101301,101302,101301,202603,97.83322811126709,0.011942099863048576
101502,101503,101502,203005,98.00671005249023,0.0124207784897671
101702,101703,101702,203405,98.19018602371216,0.011898402978261799
101902,101903,101902,203805,98.3577013015747,0.01217679560229126
102102,102103,102102,204205,98.52115511894226,0.011923691221910093
102302,102303,102302,204605,98.69626712799072,0.011804164298204592
102503,102504,102503,205007,98.88022208213806,0.011864048179084121
102703,102704,102703,205407,99.10545420646667,0.011761085902131778
102903,102904,102903,205807,99.28431010246277,0.011796783610348685
103103,103104,103103,206207,99.44929814338684,0.011872744706361325
103303,103304,103303,206607,99.6044750213623,0.011738274771576523
103504,103505,103504,207009,99.76429390907288,0.011724298227730216
103704,103705,103704,207409,99.93293595314026,0.011783819376983336
103904,103905,103904,207809,100.1128261089325,0.011733144098683129
104104,104105,104104,208209,100.29088997840881,0.01156599305695431
104304,104305,104304,208609,100.44940400123596,0.011605719980288906
104505,104506,104505,209011,100.61313796043396,0.012269477592607674
104705,104706,104705,209411,100.77967429161072,0.011615696522021038
104905,104906,104905,209811,100.96220302581787,0.011553241392740422
105105,105106,105105,210211,101.14305710792542,0.011533835620288787
105305,105306,105305,210611,101.30050611495972,0.01141873101385327
105506,105507,105506,211013,101.45733094215393,0.011544690777160329
105706,105707,105706,211413,101.62643718719482,0.01143594574200608
105906,105907,105906,211813,101.97126412391663,0.011480819638767282
106106,106107,106106,212213,102.16689801216125,0.011534556464425133
106306,106307,106306,212613,102.33386611938477,0.012900737689425424
106507,106508,106507,213015,102.67515707015991,0.011453461218289569
106707,106708,106707,213415,102.94442510604858,0.011410266935850306
106907,106908,106907,213815,103.14092302322388,0.012307663368093405
107107,107108,107107,214215,103.47359418869019,0.011299804614484125
107307,107308,107307,214615,103.67681694030762,0.011241516619958694
107508,107509,107508,215017,103.86155200004578,0.011457745506642247
107708,107709,107708,215417,104.04869818687439,0.012850786765117254
107908,107909,107908,215817,104.31293797492981,0.01318978735044623
108108,108109,108108,216217,104.51949906349182,0.011114226369968885
108308,108309,108308,216617,104.71610307693481,0.011216965687980716
108509,108510,108509,217019,104.88501620292664,0.011136239485539047
108709,108710,108709,217419,105.05681800842285,0.011089214879086234
108909,108910,108909,217819,105.26723408699036,0.0110998353042323
109109,109110,109109,218219,105.44687223434448,0.011202638040689657
109309,109310,109309,218619,105.62309503555298,0.01120224479138858
109510,109511,109510,219021,105.82711625099182,0.014179646918289842
109710,109711,109710,219421,106.09799814224243,0.011059135309609688
109910,109911,109910,219821,106.33467411994934,0.010984270989838773
110110,110111,110110,220221,106.5794460773468,0.01113396497461948
110310,110311,110310,220621,106.84685015678406,0.011301166196161266
110511,110512,110511,221023,107.04477334022522,0.013068348318120359
110711,110712,110711,221423,107.23578190803528,0.0109529549472992
110911,110912,110911,221823,107.46753311157227,0.010954020400936345
111111,111112,111111,222223,107.68378496170044,0.01091904637318369
111311,111312,111311,222623,107.87938117980957,0.011930295123594142
111512,111513,111512,223025,108.07052230834961,0.010991543543120756
111712,111713,111712,223425,108.24532103538513,0.010832119404517261
111912,111913,111912,223825,108.42813229560852,0.010821556301069686
112112,112113,112112,224225,108.61408519744873,0.010733352932146221
112312,112313,112312,224625,108.78882789611816,0.010755916772452233
112513,112514,112513,225027,108.98272609710693,0.01077475462423997
112713,112714,112713,225427,109.18599605560303,0.010726716886486033
112913,112914,112913,225827,109.38346910476685,0.01233583025887605
113113,113114,113113,226227,109.56145906448364,0.012326617809664708
113313,113314,113313,226627,109.77358412742615,0.012900035430581946
113514,113515,113514,227029,110.02549624443054,0.010709826578274056
113714,113715,113714,227429,110.21614694595337,0.010671458032999397
113914,113915,113914,227829,110.53261208534241,0.010859132833548515
114114,114115,114114,228229,110.76699614524841,0.012151001131049659
114314,114315,114314,228629,110.94157814979553,0.010580114384676664
114515,114516,114515,229031,111.1259651184082,0.010613242005584559
114715,114716,114715,229431,111.42464900016785,0.010517361715251293
114915,114916,114915,229831,111.66485714912415,0.010528951674123937
115115,115116,115115,230231,111.86374521255493,0.01051952029493763
115315,115316,115315,230631,112.04085111618042,0.010438443981145344
115516,115517,115516,231033,112.21956729888916,0.010485303445909517
115716,115717,115716,231433,112.40061020851135,0.012250996620992874
115916,115917,115916,231833,112.5551381111145,0.01218725715728835
116116,116117,116116,232233,112.71813106536865,0.010894248462989971
116316,116317,116316,232633,112.8850450515747,0.01044560634174177
116517,116518,116517,233035,113.04864311218262,0.010277112609266937
116717,116718,116717,233435,113.21191310882568,0.010380238942528784
116917,116918,116917,233835,113.37716317176819,0.010343091760791874
117117,117118,117117,234235,113.53854489326477,0.010332286679512087
117317,117318,117317,234635,113.70879316329956,0.010908796523518354
117518,117519,117518,235037,113.88564991950989,0.01027808814539626
117718,117719,117718,235437,114.08132314682007,0.010313122285711475
117918,117919,117918,235837,114.23950815200806,0.010414445175561225
118118,118119,118118,236237,114.40172123908997,0.010142813708327396
118318,118319,118318,236637,114.63504528999329,0.010210946343839369
118519,118520,118519,237039,114.9100329875946,0.010166168063958704
118719,118720,118719,237439,115.16989612579346,0.010158630257559488
118919,118920,118919,237839,115.39216589927673,0.010107553520483875
119119,119120,119119,238239,115.54982113838196,0.010217808098701119
119319,119320,119319,238639,115.70612907409668,0.0100217351108536
119520,119521,119520,239041,115.87060213088989,0.011541666431427686
119720,119721,119720,239441,116.03916597366333,0.010117502632112462
119920,119921,119920,239841,116.20851111412048,0.009997556425028477
120120,120121,120120,240241,116.42821717262268,0.01005956840034649
120320,120321,120320,240641,116.6395161151886,0.010124386396884
120521,120522,120521,241043,116.9223141670227,0.010059213338274
120721,120722,120721,241443,117.1915352344513,0.009928436037329347
120921,120922,120921,241843,117.38760805130005,0.009998451725525236
121121,121122,121121,242243,117.59274125099182,0.009979505084185263
121321,121322,121321,242643,117.8659291267395,0.00996149364456096
121522,121523,121522,243045,118.0432641506195,0.00988967755707389
121722,121723,121722,243445,118.33325505256653,0.010272924040487184
121922,121923,121922,243845,118.5781922340393,0.011234535580851007
122122,122123,122122,244245,118.7420129776001,0.009861471824630735
122322,122323,122322,244645,119.08858823776245,0.009851146241958455
122523,122524,122523,245047,119.26338410377502,0.00995162850168834
122723,122724,122723,245447,119.432687997818,0.009892103426887216
122923,122924,122923,245847,119.62954115867615,0.009949991222945912
123123,123124,123123,246247,119.87240815162659,0.011527609812607423
123323,123324,123323,246647,120.0901460647583,0.009761781264073248
123524,123525,123524,247049,120.291836977005,0.009837274339976672
123724,123725,123724,247449,120.47716307640076,0.010078335224324553
123924,123925,123924,247849,120.65572786331177,0.009725010617936104
124124,124125,124124,248249,120.82745313644409,0.009654695676557136
124324,124325,124324,248649,120.99453210830688,0.009763348826345556
124525,124526,124525,249051,121.16631603240967,0.009630508379325322
124725,124726,124725,249451,121.33256316184998,0.010031573212738662
124925,124926,124925,249851,121.49395728111267,0.010298868374356032
125125,125126,125125,250251,121.66750597953796,0.009559624826556196
125325,125326,125325,250651,121.95039224624634,0.009538026158893853
125526,125527,125526,251053,122.13856220245361,0.009589421010903081
125726,125727,125726,251453,122.31238198280334,0.009678090450041924
125926,125927,125926,251853,122.54311919212341,0.009900632519954693
126126,126127,126126,252253,122.72734212875366,0.009728191795132193
126326,126327,126326,252653,122.93088603019714,0.010108179310892928
126527,126528,126527,253055,123.11342215538025,0.009436023281273288
126727,126728,126727,253455,123.29736089706421,0.009498913462102864
126927,126928,126927,253855,123.49535918235779,0.009452294698635979
127127,127128,127127,254255,123.66302394866943,0.01102878520393662
127327,127328,127327,254655,123.89591932296753,0.009449174077251248
127528,127529,127528,255057,124.15190625190735,0.00947674942285948
127728,127729,127728,255457,124.34173917770386,0.009423879509782651
127928,127929,127928,255857,124.56807208061218,0.009456720156032097
128128,128129,128128,256257,124.82098913192749,0.009417829875795817
128328,128329,128328,256657,125.04939413070679,0.009372796579861977
128529,128530,128529,257059,125.22211623191833,0.00961098785895645
128729,128730,128729,257459,125.39171004295349,0.00925389528871682
128929,128930,128929,257859,125.56152606010437,0.01059893498696668
129129,129130,129129,258259,125.82520508766174,0.0093180754726377
129329,129330,129329,258659,126.02106022834778,0.009304022222332535
129530,129531,129530,259061,126.18066692352295,0.009215106803245483
129730,129731,129730,259461,126.38094115257263,0.009213535628078322
129930,129931,129930,259861,126.55155992507935,0.00931253135001628
130130,130131,130130,260261,126.74574208259583,0.009340083283519086
130330,130331,130330,260661,126.9209291934967,0.009251348471866958
130531,130532,130531,261063,127.14337706565857,0.009242290249366373
130731,130732,130731,261463,127.39124011993408,0.00931353004637865
130931,130932,130931,261863,127.56510400772095,0.009161261458946047
131131,131132,131131,262263,127.76007103919983,0.009335671939552943
131331,131332,131331,262663,127.93418598175049,0.009173141011724669
131532,131533,131532,263065,128.10092902183533,0.009050524137719873
131732,131733,131732,263465,128.28383898735046,0.009113004004221206
131932,131933,131932,263865,128.48217821121216,0.009065373460914836
132132,132133,132132,264265,128.71579813957214,0.009165516539380377
132332,132333,132332,264665,128.92039704322815,0.009063928683591122
132533,132534,132533,265067,129.09946513175964,0.00897545887347874
132733,132734,132733,265467,129.2844259738922,0.010251291997403171
132933,132934,132933,265867,129.45286297798157,0.008971543963634164
133133,133134,133133,266267,129.6189410686493,0.010607985308513881
133333,133334,133333,266667,129.8061592578888,0.009076044816898221
133534,133535,133534,267069,129.9641191959381,0.008943491050210806
133734,133735,133734,267469,130.13363909721375,0.00899229234703203
133934,133935,133934,267869,130.29783987998962,0.009105430727745513
134134,134135,134134,268269,130.48953914642334,0.008854431261487633
134334,134335,134334,268669,130.68420314788818,0.008871215341191386
134535,134536,134535,269071,130.86391401290894,0.008913783722783794
134735,134736,134735,269471,131.04563117027283,0.008869499890056639
134935,134936,134935,269871,131.21175622940063,0.009331767227978722
135135,135136,135135,270271,131.39598608016968,0.008782189408263964
135335,135336,135335,270671,131.5653510093689,0.008758771250236197
135536,135537,135536,271073,131.7448980808258,0.008757699406709911
135736,135737,135736,271473,131.9141390323639,0.008780245605927314
135936,135937,135936,271873,132.07798409461975,0.00878101085470158
136136,136137,136136,272273,132.2607171535492,0.010989781720591155
136336,136337,136336,272673,132.59276604652405,0.008751575469104966
136537,136538,136537,273075,132.77378010749817,0.008772809399974782
136737,136738,136737,273475,132.9396140575409,0.00873624270695012
136937,136938,136937,273875,133.10724902153015,0.00894800842558574
137137,137138,137137,274275,133.47495198249817,0.0087829951074328
137337,137338,137337,274675,133.66870307922363,0.008714111917232979
137538,137539,137538,275077,133.88496017456055,0.01042583758841376
137738,137739,137738,275477,134.08425307273865,0.008774834373895197
137938,137939,137938,275877,134.26160430908203,0.008609071065124744
138138,138139,138138,276277,134.43833923339844,0.008686831116424591
138338,138339,138338,276677,134.61896109580994,0.00924206006899033
138539,138540,138539,277079,134.79979395866394,0.008649698689105083
138739,138740,138739,277479,134.97485494613647,0.00864451472943928
138939,138940,138939,277879,135.14665293693542,0.008525987736081908
139139,139140,139139,278279,135.3116500377655,0.008946204569486263
139339,139340,139339,278679,135.47526502609253,0.008509521011981451
139540,139541,139540,279081,135.63898921012878,0.008588688115487688
139740,139741,139740,279481,135.80885887145996,0.008503458908811757
139940,139941,139940,279881,135.97503900527954,0.009031401962465584
140140,140141,140140,280281,136.14762210845947,0.008465190304366215
140340,140341,140340,280681,136.31745624542236,0.008632334674412882
140541,140542,140541,281083,136.48413610458374,0.008446446126481174
140741,140742,140741,281483,136.64298295974731,0.008436589146717745
140941,140942,140941,281883,136.80612015724182,0.008420219667315633
141141,141142,141141,282283,136.9707682132721,0.008478048542396753
141341,141342,141341,282683,137.14064002037048,0.00839509862325489
141542,141543,141542,283085,137.30417013168335,0.008412266919931646
141742,141743,141742,283485,137.5168342590332,0.008436820500431567
141942,141943,141942,283885,137.6974790096283,0.008353161642363636
142142,142143,142142,284285,137.89439487457275,0.008387687426476878
142342,142343,142342,284685,138.08291101455688,0.00888053140074125
142543,142544,142543,285087,138.28741097450256,0.00835847363634208
142743,142744,142743,285487,138.45022010803223,0.008325230179301363
142943,142944,142943,285887,138.6069691181183,0.008253513999186201
143143,143144,143143,286287,138.76397705078125,0.008269950996072306
143343,143344,143343,286687,138.92216110229492,0.008249171048651084
143544,143545,143544,287089,139.08440399169922,0.0082792658146186
143744,143745,143744,287489,139.24875020980835,0.008275243241087893
143944,143945,143944,287889,139.404314994812,0.008200714539178686
144144,144145,144144,288289,139.55752110481262,0.008121766969706505
144344,144345,144344,288689,139.71018290519714,0.008245778998549632
144545,144546,144545,289091,139.8693652153015,0.008524059794281747
144745,144746,144745,289491,140.04549622535706,0.008177029714609768
144945,144946,144945,289891,140.2011480331421,0.009737302399555033
145145,145146,145145,290291,140.35829830169678,0.008905370623458388
145345,145346,145345,290691,140.51143407821655,0.008124073475947848
145546,145547,145546,291093,140.6761691570282,0.00808116888106706
145746,145747,145746,291493,140.85333728790283,0.008112862918246694
145946,145947,145946,291893,141.02921104431152,0.008095185698134132
146146,146147,146146,292293,141.19852232933044,0.009258644576120287
146346,146347,146346,292693,141.35846996307373,0.00807988420431336
146547,146548,146547,293095,141.5138020515442,0.008096812018507683
146747,146748,146747,293495,141.66849613189697,0.007994822950667587
146947,146948,146947,293895,141.82693815231323,0.007973857188001704
147147,147148,147147,294295,141.98337411880493,0.008031152691236021
147347,147348,147347,294695,142.15061402320862,0.008014149386309366
147548,147549,147548,295097,142.31583499908447,0.00796743333505109
147748,147749,147748,295497,142.46964526176453,0.007914341779779864
147948,147949,147948,295897,142.625018119812,0.007923346518237579
148148,148149,148148,296297,142.78315496444702,0.009454057208496743
148348,148349,148348,296697,142.9380121231079,0.00793589471907791
148549,148550,148549,297099,143.09889221191406,0.00786097599630423
148749,148750,148749,297499,143.25614213943481,0.007881991008647239
148949,148950,148949,297899,143.41129302978516,0.007938148611943627
149149,149150,149149,298299,143.56894898414612,0.007827371511875295
149349,149350,149349,298699,143.72239208221436,0.007906515853022447
149550,149551,149550,299101,143.8817400932312,0.007893637550996343
149750,149751,149750,299501,144.043869972229,0.009155249073513361
149950,149951,149950,299901,144.19972109794617,0.007885306625001124
150150,150151,150150,300301,144.37644720077515,0.007821935693877584
150350,150351,150350,300701,144.53476786613464,0.007800659927461503
150551,150552,150551,301103,144.6893970966339,0.007756089096709396
150751,150752,150751,301503,144.8459711074829,0.007743551452170942
150951,150952,150951,301903,145.00258803367615,0.007805230148917115
151151,151152,151151,302303,145.15796899795532,0.007822679454272697
151351,151352,151351,302703,145.31781315803528,0.007773579658658709
151552,151553,151552,303105,145.47305011749268,0.007786625777609267
151752,151753,151752,303505,145.62621808052063,0.008188088477540606
151952,151953,151952,303905,145.78565621376038,0.007724232013994179
152152,152153,152152,304305,145.939875125885,0.007680748194626401
152352,152353,152352,304705,146.09899926185608,0.007730506354374982
152553,152554,152553,305107,146.25641107559204,0.007706367213526017
152753,152754,152753,305507,146.4165163040161,0.00762715498332955
152953,152954,152953,305907,146.58773612976074,0.00791706489627591
153153,153154,153153,306307,146.74340724945068,0.00763460780652861
153353,153354,153353,306707,146.90388321876526,0.007767040570538845
153554,153555,153554,307109,147.06189513206482,0.007643523845493967
153754,153755,153754,307509,147.21529817581177,0.008772989846751627
153954,153955,153954,307909,147.37680006027222,0.008966614170900118
154154,154155,154154,308309,147.5315752029419,0.007590500179767757
154354,154355,154354,308709,147.68521308898926,0.0076064495755565125
154555,154556,154555,309111,147.84640526771545,0.007501385294664617
154755,154756,154755,309511,148.00435996055603,0.007564479001097998
154955,154956,154955,309911,148.1628930568695,0.007873669962245098
155155,155156,155155,310311,148.32317209243774,0.007565339920360191
155355,155356,155355,310711,148.47743916511536,0.007867875043101585
155556,155557,155556,311113,148.64510011672974,0.007461097036714573
155756,155757,155756,311513,148.8093593120575,0.007500656469029791
155956,155957,155956,311913,148.9647581577301,0.00750294480636719
156156,156157,156156,312313,149.1244831085205,0.007454636396438574
156356,156357,156356,312713,149.28401112556458,0.007391918608558743
156557,156558,156557,313115,149.44246411323547,0.007466534504247478
156757,156758,156757,313515,149.6159701347351,0.008792259862975098
156957,156958,156957,313915,149.77128195762634,0.007352349831027633
157157,157158,157157,314315,149.92721509933472,0.007636624062366665
157357,157358,157357,314715,150.0850031375885,0.007712814862319607
157558,157559,157558,315117,150.2413511276245,0.0073329891806401615
157758,157759,157758,315517,150.40050220489502,0.007322845926917601
157958,157959,157958,315917,150.55524110794067,0.007341118927010941
158158,158159,158158,316317,150.71054434776306,0.008919058511321788
158358,158359,158358,316717,150.8860900402069,0.007704657126456024
158559,158560,158559,317119,151.04381799697876,0.007310468626424947
158759,158760,158759,317519,151.19953608512878,0.007287067545135279
158959,158960,158959,317919,151.35857105255127,0.007347800747026011
159159,159160,159159,318319,151.51284098625183,0.0072693508907606215
159359,159360,159359,318719,151.6679871082306,0.0071948233199174
159560,159561,159560,319121,151.8313500881195,0.00730332955383705
159760,159761,159760,319521,151.9972710609436,0.007222475471885667
159960,159961,159960,319921,152.1707091331482,0.008028507638063906
160160,160161,160160,320321,152.33769702911377,0.0072586390511055
160360,160361,160360,320721,152.50832104682922,0.008699376656412338
160561,160562,160561,321123,152.67820501327515,0.007184173164097839
160761,160762,160761,321523,152.8356339931488,0.007177426609691968
160961,160962,160961,321923,153.06773900985718,0.0072165623601896985
161161,161162,161161,322323,153.25501918792725,0.007279527689931676
161361,161362,161361,322723,153.43290495872498,0.007555670748679247
161562,161563,161562,323125,153.6046290397644,0.007208685451200291
161762,161763,161762,323525,153.75905013084412,0.007109352041474739
161962,161963,161962,323925,154.03298211097717,0.007133319308459207
162162,162163,162162,324325,154.5016052722931,0.007151034511102088
162362,162363,162362,324725,154.91395616531372,0.007415837833856523
162563,162564,162563,325127,155.3045802116394,0.0070354418124986004
162763,162764,162763,325527,155.69009804725647,0.00915390241280144
162963,162964,162963,325927,156.0125172138214,0.0071159804668018386
163163,163164,163163,326327,156.21639823913574,0.00714813505364022
163363,163364,163363,326727,156.40796613693237,0.007147587707735063
163564,163565,163564,327129,156.58833813667297,0.006997457086977219
163764,163765,163764,327529,156.7764801979065,0.007008558036643208
163964,163965,163964,327929,156.9923141002655,0.007004551047061625
164164,164165,164164,328329,157.18797492980957,0.007057053729360782
164364,164365,164364,328729,157.3548390865326,0.006995236933508696
164565,164566,164565,329131,157.53003191947937,0.008715681174227467
164765,164766,164765,329531,157.73478317260742,0.00704238786025648
164965,164966,164965,329931,157.91693019866943,0.007027222218465717
165165,165166,165165,330331,158.08033633232117,0.007273526624039032
165365,165366,165365,330731,158.2382459640503,0.006917692270087891
165566,165567,165566,331133,158.39637517929077,0.0071553487951958395
165766,165767,165766,331533,158.55239605903625,0.0069530513697700965
165966,165967,165966,331933,158.7049241065979,0.006916354580268743
166166,166167,166166,332333,158.86483216285706,0.006890741536764895
166366,166367,166366,332733,159.02222228050232,0.0068774140944735905
166567,166568,166567,333135,159.17742705345154,0.006848700837518759
166767,166768,166767,333535,159.33132028579712,0.0068457376908945605
166967,166968,166967,333935,159.48635029792786,0.00820745202933619
167167,167168,167167,334335,159.6558699607849,0.007101301557516793
167367,167368,167367,334735,159.81241106987,0.006910506932165108
167568,167569,167568,335137,159.96520924568176,0.006844109023073073
167768,167769,167768,335537,160.12548732757568,0.00703566110603919
167968,167969,167968,335937,160.3478500843048,0.006847839856078047
168168,168169,168168,336337,160.52368021011353,0.006902348026370445
168368,168369,168368,336737,160.6905710697174,0.00673786083835732
168569,168570,168569,337139,160.85701894760132,0.007033022338414434
168769,168770,168769,337539,161.03385210037231,0.006783003671104932
168969,168970,168969,337939,161.202054977417,0.0068742895125736905
169169,169170,169169,338339,161.3733992576599,0.006797511961848726
169369,169370,169369,338739,161.53903913497925,0.0067352473323591625
169570,169571,169570,339141,161.70578694343567,0.006735523859930063
169770,169771,169770,339541,161.8975749015808,0.0067261953204085945
169970,169971,169970,339941,162.0712389945984,0.008044465519750906
170170,170171,170170,340341,162.2376091480255,0.0066880302666793645
170370,170371,170370,340741,162.39216208457947,0.007139461514104561
170571,170572,170571,341143,162.54704523086548,0.0066643353769968335
170771,170772,170771,341543,162.70198822021484,0.006692111467564125
170971,170972,170971,341943,162.85624814033508,0.006878438616650221
171171,171172,171171,342343,163.01226019859314,0.006667317994084124
171371,171372,171371,342743,163.16897416114807,0.006713202892431747
171572,171573,171572,343145,163.3215091228485,0.00667475186127107
171772,171773,171772,343545,163.47967219352722,0.0079252238626226
171972,171973,171972,343945,163.76428127288818,0.007032262578603052
172172,172173,172172,344345,164.11213326454163,0.007600198574465188
172372,172373,172372,344745,164.406485080719,0.006602052958166092
172573,172574,172573,345147,164.57944703102112,0.0066336002313243094
172773,172774,172773,345547,164.74891018867493,0.006549669855456327
172973,172974,172973,345947,164.9684660434723,0.006536110604471593
173173,173174,173173,346347,165.16977906227112,0.006509946636779262
173373,173374,173373,346747,165.35704517364502,0.007054299126493971
173574,173575,173574,347149,165.53868913650513,0.006486748411229194
173774,173775,173774,347549,165.69563126564026,0.006500711986352029
173974,173975,173974,347949,165.86422419548035,0.006939852783168362
174174,174175,174174,348349,166.13867902755737,0.006717506179737559
174374,174375,174374,348749,166.3042230606079,0.006481032519986034
174575,174576,174575,349151,166.46356630325317,0.00650337467128419
174775,174776,174775,349551,166.6167721748352,0.006529830275708687
174975,174976,174975,349951,166.77172994613647,0.00766754744698106
175175,175176,175175,350351,166.9896171092987,0.0064405136132717825
175375,175376,175375,350751,167.1790051460266,0.006464089607055333
175576,175577,175576,351153,167.39613819122314,0.006479767604430779
175776,175777,175776,351553,167.56527018547058,0.006431575000341985
175976,175977,175976,351953,167.7673020362854,0.006433068413197165
176176,176177,176176,352353,167.9312620162964,0.0065515364117297555
176376,176377,176376,352753,168.10117506980896,0.006427091946579181
176577,176578,176577,353155,168.2742772102356,0.007583610788692123
176777,176778,176777,353555,168.46595001220703,0.006341176507639105
176977,176978,176977,353955,168.63547015190125,0.006363405897234146
177177,177178,177177,354355,168.8041422367096,0.0063048468935747995
177377,177378,177377,354755,168.97503113746643,0.006357840949663803
177578,177579,177578,355157,169.16733121871948,0.006292928828420557
177778,177779,177778,355557,169.39497208595276,0.006282869209256227
177978,177979,177978,355957,169.5646243095398,0.006310982189794928
178178,178179,178178,356357,169.76467514038086,0.006405452680818838
178378,178379,178378,356757,169.97712588310242,0.007753296757655331
178579,178580,178579,357159,170.2019500732422,0.006329916223735507
178779,178780,178779,357559,170.39128398895264,0.006338468802648996
178979,178980,178979,357959,170.56781697273254,0.006249904512355646
179179,179180,179179,358359,170.73798298835754,0.007480579564437063
179379,179380,179379,358759,170.9151749610901,0.0063122572272611074
179580,179581,179580,359161,171.1033799648285,0.006188527872194101
179780,179781,179780,359561,171.32776618003845,0.006254264602749986
179980,179981,179980,359961,171.5796480178833,0.006215556544600124
180180,180181,180180,360361,171.7715039253235,0.00624531654697829
180380,180381,180380,360761,171.98190116882324,0.00622536509655509
180581,180582,180581,361163,172.1894989013672,0.006209571887635591
180781,180782,180781,361563,172.5296552181244,0.0067603290103265936
180981,180982,180981,361963,172.73101115226746,0.0061479694186351895
181181,181182,181181,362363,173.07157731056213,0.006161536812125701
181381,181382,181381,362763,173.39569211006165,0.006177644940368585
181582,181583,181582,363165,173.6798231601715,0.006113353659113901
181782,181783,181782,363565,173.95360708236694,0.0061682036356954266
181982,181983,181982,363965,174.23387718200684,0.006121840693422839
182182,182183,182182,364365,174.50866222381592,0.006243202242097588
182382,182383,182382,364765,174.88653230667114,0.006134747138029305
182583,182584,182583,365167,175.20333409309387,0.006099577340621476
182783,182784,182783,365567,175.53491616249084,0.006379647022865578
182983,182984,182983,365967,175.7152440547943,0.00639659377947698
183183,183184,183183,366367,175.8970181941986,0.006147094610727292
183383,183384,183383,366767,176.0733151435852,0.00605517422244534
183584,183585,183584,367169,176.24477005004883,0.0061286060185482445
183784,183785,183784,367569,176.40678715705872,0.006002609639392234
183984,183985,183984,367969,176.57780528068542,0.006032450625334812
184184,184185,184184,368369,176.75320601463318,0.006313677937686825
184384,184385,184384,368769,176.92672514915466,0.006043403037192949
184585,184586,184585,369171,177.11764001846313,0.006056962662910708
184785,184786,184785,369571,177.3885042667389,0.006054885261249672
184985,184986,184985,369971,177.59479522705078,0.006058073878730614
185185,185186,185185,370371,177.78032112121582,0.00740973987696174
185385,185386,185385,370771,177.96037101745605,0.006024675498527296
185586,185587,185586,371173,178.1266541481018,0.005984180178193426
185786,185787,185786,371573,178.30271005630493,0.005925951171737144
185986,185987,185986,371973,178.54816317558289,0.005935543058035813
186186,186187,186186,372373,178.768874168396,0.005990615686726449
186386,186387,186386,372773,178.93671107292175,0.006018493547339329
186587,186588,186587,373175,179.1071801185608,0.006012277284874804
186787,186788,186787,373575,179.29962706565857,0.005906337231237099
186987,186988,186987,373975,179.4764120578766,0.005925486164270208
187187,187188,187187,374375,179.6486349105835,0.005903235417230294
187387,187388,187387,374775,179.80592799186707,0.005878703524243212
187588,187589,187588,375177,179.98180627822876,0.005887596127496947
187788,187789,187788,375577,180.14028024673462,0.0059180011340773195
187988,187989,187988,375977,180.2945113182068,0.0059393006735595
188188,188189,188188,376377,180.457417011261,0.006135931182226895
188388,188389,188388,376777,180.61580109596252,0.005853692005958422
188589,188590,188589,377179,180.77295804023743,0.005973391485863774
188789,188790,188789,377579,180.92972707748413,0.0067831598901384816
188989,188990,188989,377979,181.0855040550232,0.006603643895940891
189189,189190,189189,378379,181.24091410636902,0.005799248234351257
189389,189390,189389,378779,181.41825222969055,0.005802333327713945
189590,189591,189590,379181,181.57521605491638,0.0057898230881128976
189790,189791,189790,379581,181.74030423164368,0.005793465360706356
189990,189991,189990,379981,181.90807819366455,0.005789414898781205
190190,190191,190190,380381,182.06684613227844,0.005780591567858376
190390,190391,190390,380781,182.2475781440735,0.005782743635878963
190591,190592,190591,381183,182.4225151538849,0.006977412860854395
190791,190792,190791,381583,182.58565211296082,0.005758826190290514
190991,190992,190991,381983,182.78499722480774,0.005769318108983297
191191,191192,191191,382383,183.02647995948792,0.005790488289332991
191391,191392,191391,382783,183.27716898918152,0.006475180126139326
191592,191593,191592,383185,183.55501914024353,0.005691682214744309
191792,191793,191792,383585,183.86172604560852,0.005949369500595325
191992,191993,191992,383985,184.10692405700684,0.0061715102155348416
192192,192193,192192,384385,184.44330310821533,0.0057347449372095755
192392,192393,192392,384785,184.7663459777832,0.005745203424853079
192593,192594,192593,385187,185.0297770500183,0.005762860027516822
192793,192794,192793,385587,185.3094563484192,0.005682137586648263
192993,192994,192993,385987,185.67203617095947,0.005671018330745232
193193,193194,193193,386387,186.0202922821045,0.0063182659786968935
193393,193394,193393,386787,186.35798621177673,0.006451096022777104
193594,193595,193594,387189,186.69888710975647,0.005676642951078387
193794,193795,193794,387589,186.98595118522644,0.005638826458849299
193994,193995,193994,387989,187.23058795928955,0.006829248203352093
194194,194195,194194,388389,187.4804491996765,0.005662518805251318
194394,194395,194394,388789,187.76417803764343,0.0064715494691431966
194595,194596,194595,389191,188.0267689228058,0.005600368843653895
194795,194796,194795,389591,188.3966453075409,0.00565039732366775
194995,194996,194995,389991,188.68961906433105,0.005597950723103198
195195,195196,195195,390391,189.0507411956787,0.005575669951942582
195395,195396,195395,390791,189.2332649230957,0.006886563409410645
195596,195597,195596,391193,189.41704034805298,0.005584945410830736
195796,195797,195796,391593,189.59671306610107,0.00557124705929816
195996,195997,195996,391993,189.79103112220764,0.005517853055338362
196196,196197,196196,392393,189.97090792655945,0.005618570335416077
196396,196397,196396,392793,190.1597399711609,0.005613990726752969
196597,196598,196597,393195,190.37773489952087,0.005539729397551354
196797,196798,196797,393595,190.58017206192017,0.0055724284858010825
196997,196998,196997,393995,190.7323431968689,0.005502826697989712
197197,197198,197197,394395,190.88750505447388,0.0055304025095857905
197397,197398,197397,394795,191.05578708648682,0.005554831542612902
197598,197599,197598,395197,191.21988201141357,0.005489844418283752
197798,197799,197798,395597,191.38478803634644,0.0066899438090353164
197998,197999,197998,395997,191.55600118637085,0.0058374031437525885
198198,198199,198198,396397,191.8689432144165,0.006416024385678713
198398,198399,198398,396797,192.08561420440674,0.0056518022561128966
198599,198600,198599,397199,192.36643719673157,0.005495770360522918
198799,198800,198799,397599,192.87445306777954,0.005472873238514875
198999,199000,198999,397999,193.45346212387085,0.00546956781320136
199199,199200,199199,398399,193.86799216270447,0.005499488517493203
199399,199400,199399,398799,194.33308601379395,0.005458545254272569
199600,199601,199600,399201,194.82830905914307,0.005437973857626802
199800,199801,199800,399601,195.3700511455536,0.005633167290011079
200000,200001,200000,400001,195.9777889251709,0.005434957686107025


==> plot_data/quadratic_minimax_problem_n500_alpha0/eag-c.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012149810791015625,30.358099469249375
100,201,0,201,0.14583706855773926,6.497570818090755
200,401,0,401,0.2944481372833252,3.18105807646363
300,601,0,601,0.4670841693878174,2.023030291273728
400,801,0,801,0.635936975479126,1.5000642024628064
501,1003,0,1003,0.7899360656738281,1.2103469417860875
601,1203,0,1203,0.949761152267456,0.9917060130889543
701,1403,0,1403,1.13106107711792,0.8254787271305319
801,1603,0,1603,1.2845561504364014,0.7062811064072342
901,1803,0,1803,1.4317481517791748,0.6543601275560126
1001,2003,0,2003,1.5721988677978516,0.5773048961321726
1101,2203,0,2203,1.7155489921569824,0.5144269762928468
1201,2403,0,2403,1.854905128479004,0.45615330695503536
1301,2603,0,2603,2.0115180015563965,0.4404029996357728
1401,2803,0,2803,2.1761410236358643,0.3975980279547153
1502,3005,0,3005,2.345039129257202,0.36949295128494175
1602,3205,0,3205,2.4993951320648193,0.3453935729189495
1702,3405,0,3405,2.660348892211914,0.3224437473756645
1802,3605,0,3605,2.8231329917907715,0.3003083696808211
1902,3805,0,3805,2.9752602577209473,0.2790046640953164
2002,4005,0,4005,3.124285936355591,0.26758608951506263
2102,4205,0,4205,3.2784199714660645,0.2581574044396648
2202,4405,0,4405,3.4347169399261475,0.25392760853436286
2302,4605,0,4605,3.589181900024414,0.24490737158516468
2402,4805,0,4805,3.736598014831543,0.23075280240887205
2503,5007,0,5007,3.885317087173462,0.2222706985986103
2603,5207,0,5207,4.028550863265991,0.21052433242698215
2703,5407,0,5407,4.180194139480591,0.20151474426108304
2803,5607,0,5607,4.326223134994507,0.19525221603049853
2903,5807,0,5807,4.466821193695068,0.18874538823192655
3003,6007,0,6007,4.627024173736572,0.18043529960724145
3103,6207,0,6207,4.79167914390564,0.1724978037257758
3203,6407,0,6407,4.96924901008606,0.16746846548193717
3303,6607,0,6607,5.122457027435303,0.1634600138497955
3403,6807,0,6807,5.288764953613281,0.15782350719656182
3504,7009,0,7009,5.509546995162964,0.15237471620528026
3604,7209,0,7209,5.705277919769287,0.14989467892912553
3704,7409,0,7409,5.883615016937256,0.1451703990021208
3804,7609,0,7609,6.107993125915527,0.14023450784353794
3904,7809,0,7809,6.271381139755249,0.13736999542970416
4004,8009,0,8009,6.436395168304443,0.1351099220664021
4104,8209,0,8209,6.588837146759033,0.1331033881503364
4204,8409,0,8409,6.738521099090576,0.13152319488662384
4304,8609,0,8609,6.8856000900268555,0.1261771953830402
4404,8809,0,8809,7.046363115310669,0.12212300590662446
4505,9011,0,9011,7.207620143890381,0.11881645204132854
4605,9211,0,9211,7.358686923980713,0.11600223873764948
4705,9411,0,9411,7.504754066467285,0.11238929828935541
4805,9611,0,9611,7.663981199264526,0.1107886084508722
4905,9811,0,9811,7.808404922485352,0.10885204316784926
5005,10011,0,10011,7.957789897918701,0.10629086176646911
5105,10211,0,10211,8.105000972747803,0.10292809789710003
5205,10411,0,10411,8.259253025054932,0.10179722659931073
5305,10611,0,10611,8.407384157180786,0.10050868282250508
5405,10811,0,10811,8.548290014266968,0.099685546227355
5506,11013,0,11013,8.689716100692749,0.0964678127262242
5606,11213,0,11213,8.834662199020386,0.09449470383495231
5706,11413,0,11413,8.977593183517456,0.09494493700747744
5806,11613,0,11613,9.130220174789429,0.09259000418131524
5906,11813,0,11813,9.300217151641846,0.09000840286487526
6006,12013,0,12013,9.44390606880188,0.08932099103487805
6106,12213,0,12213,9.589510917663574,0.08768139282884627
6206,12413,0,12413,9.730094194412231,0.08607332518150468
6306,12613,0,12613,9.87195611000061,0.08352982587031096
6406,12813,0,12813,10.024049997329712,0.0814089279433394
6507,13015,0,13015,10.217818260192871,0.07954965480763306
6607,13215,0,13215,10.367501020431519,0.07843490648794667
6707,13415,0,13415,10.51526403427124,0.07684005998000677
6807,13615,0,13615,10.716358184814453,0.0765324674966933
6907,13815,0,13815,10.859550952911377,0.07652741618012764
7007,14015,0,14015,11.004064083099365,0.07518958956214769
7107,14215,0,14215,11.192026138305664,0.07401083218612478
7207,14415,0,14415,11.357577085494995,0.07415698778432939
7307,14615,0,14615,11.50106406211853,0.07370524568149782
7407,14815,0,14815,11.642937183380127,0.07229548772292166
7508,15017,0,15017,11.785389184951782,0.07053739248907821
7608,15217,0,15217,11.929034948348999,0.06961414134153376
7708,15417,0,15417,12.070999145507812,0.06863808673602492
7808,15617,0,15617,12.229730129241943,0.06791716038317355
7908,15817,0,15817,12.37759804725647,0.06696928014533543
8008,16017,0,16017,12.516961097717285,0.06588325042173358
8108,16217,0,16217,12.66623306274414,0.06521640579231851
8208,16417,0,16417,12.807246208190918,0.06353216538231435
8308,16617,0,16617,12.950984954833984,0.0619337233103036
8408,16817,0,16817,13.108495235443115,0.061551238751332026
8509,17019,0,17019,13.28931999206543,0.06112176638605797
8609,17219,0,17219,13.473052978515625,0.060362107536433965
8709,17419,0,17419,13.660864114761353,0.05962927835119283
8809,17619,0,17619,13.81277322769165,0.05927903453218729
8909,17819,0,17819,13.965537071228027,0.05925507795417719
9009,18019,0,18019,14.127811193466187,0.058501062422898764
9109,18219,0,18219,14.307642221450806,0.057743941901409225
9209,18419,0,18419,14.478209018707275,0.057786603017676394
9309,18619,0,18619,14.638758182525635,0.05747442954460791
9409,18819,0,18819,14.912891149520874,0.056414997407415915
9510,19021,0,19021,15.12336015701294,0.05544709063960474
9610,19221,0,19221,15.326128244400024,0.054828760605241174
9710,19421,0,19421,15.48313021659851,0.05442827870017512
9810,19621,0,19621,15.679784059524536,0.05368941434040843
9910,19821,0,19821,15.855808019638062,0.05309150462705312
10010,20021,0,20021,16.005410194396973,0.05259691805190521
10110,20221,0,20221,16.16487717628479,0.05165413161290116
10210,20421,0,20421,16.3333261013031,0.05062121353460223
10310,20621,0,20621,16.47207808494568,0.04998976431105962
10410,20821,0,20821,16.611127138137817,0.05004660945659487
10511,21023,0,21023,16.76579713821411,0.05002121002999302
10611,21223,0,21223,16.91773009300232,0.04950931341763679
10711,21423,0,21423,17.235530138015747,0.049152421689849846
10811,21623,0,21623,17.409735918045044,0.04898914731937789
10911,21823,0,21823,17.577171087265015,0.048625618325843854
11011,22023,0,22023,17.89622712135315,0.04772417739181262
11111,22223,0,22223,18.091238260269165,0.04695438029453348
11211,22423,0,22423,18.306241989135742,0.04676916665120571
11311,22623,0,22623,18.47876214981079,0.04640352444191618
11411,22823,0,22823,18.68700909614563,0.04538483138154528
11512,23025,0,23025,18.88360595703125,0.044632238828966345
11612,23225,0,23225,19.118389129638672,0.04450915944825903
11712,23425,0,23425,19.40050506591797,0.0440873058419543
11812,23625,0,23625,19.659630060195923,0.04340758855526487
11912,23825,0,23825,19.97952890396118,0.0432488719760236
12012,24025,0,24025,20.363765001296997,0.043407749563252246
12112,24225,0,24225,20.760698080062866,0.04335019559836247
12212,24425,0,24425,20.96196985244751,0.042990962082999976
12312,24625,0,24625,21.163926124572754,0.04275388109482999
12412,24825,0,24825,21.42551302909851,0.04243427748617231
12513,25027,0,25027,21.72847318649292,0.041652132862083184
12613,25227,0,25227,21.90793228149414,0.041017066403614355
12713,25427,0,25427,22.06597924232483,0.04106801677464307
12813,25627,0,25627,22.294294118881226,0.041148731544671135
12913,25827,0,25827,22.595750093460083,0.04074551368596436
13013,26027,0,26027,22.805647134780884,0.04019720042014087
13113,26227,0,26227,22.993518114089966,0.039692474672224407
13213,26427,0,26427,23.17101812362671,0.03915314870425332
13313,26627,0,26627,23.359879970550537,0.03877437987814547
13413,26827,0,26827,23.518441915512085,0.03860817952107695
13514,27029,0,27029,23.70565104484558,0.03829721406596253
13614,27229,0,27229,23.879845142364502,0.03789084925919942
13714,27429,0,27429,24.04662823677063,0.037809088516280745
13814,27629,0,27629,24.21387505531311,0.038039240217240436
13914,27829,0,27829,24.399301052093506,0.03836690575386712
14014,28029,0,28029,24.586053133010864,0.038401421007606226
14114,28229,0,28229,24.76908802986145,0.0379733926422984
14214,28429,0,28429,24.926069021224976,0.03743824067400723
14314,28629,0,28629,25.088829040527344,0.036901513051542253
14414,28829,0,28829,25.569329261779785,0.03629662175375142
14515,29031,0,29031,25.920282125473022,0.035756637644634014
14615,29231,0,29231,26.13672113418579,0.03538888317272155
14715,29431,0,29431,26.304471015930176,0.03523456878359604
14815,29631,0,29631,26.476701974868774,0.03515616978529578
14915,29831,0,29831,26.65602993965149,0.034879516177690285
15015,30031,0,30031,26.816050052642822,0.03448536734146079
15115,30231,0,30231,27.101423263549805,0.03424970520560686
15215,30431,0,30431,27.55671715736389,0.03413788977165118
15315,30631,0,30631,27.81310796737671,0.033982143008598475
15415,30831,0,30831,27.971816062927246,0.033750897970925536
15516,31033,0,31033,28.40077495574951,0.03351612176845904
15616,31233,0,31233,28.760765075683594,0.033310987301973405
15716,31433,0,31433,29.149364948272705,0.03323192877731481
15816,31633,0,31633,29.435465097427368,0.03341173197626887
15916,31833,0,31833,29.597187042236328,0.03362120129994118
16016,32033,0,32033,29.750760078430176,0.03345732291929519
16116,32233,0,32233,29.912723064422607,0.03285815081343183
16216,32433,0,32433,30.059065103530884,0.03218086592959834
16316,32633,0,32633,30.212369918823242,0.03172823435553485
16416,32833,0,32833,30.403232097625732,0.031403064531653854
16517,33035,0,33035,30.573549032211304,0.031038743011142587
16617,33235,0,33235,30.739797115325928,0.03077060747667494
16717,33435,0,33435,30.92891216278076,0.03075550190451851
16817,33635,0,33635,31.08741307258606,0.030798908578795723
16917,33835,0,33835,31.23896288871765,0.030671673122604888
17017,34035,0,34035,31.416900157928467,0.030528277136852692
17117,34235,0,34235,31.576598167419434,0.03059192666022504
17217,34435,0,34435,31.737467288970947,0.030676389257550066
17317,34635,0,34635,31.91404700279236,0.03048265770068797
17417,34835,0,34835,32.09281897544861,0.030111193524697766
17518,35037,0,35037,32.27728009223938,0.029762655465028293
17618,35237,0,35237,32.42514896392822,0.029457723322721677
17718,35437,0,35437,32.57607913017273,0.029207667016899887
17818,35637,0,35637,32.770785093307495,0.029069318564550264
17918,35837,0,35837,33.20151710510254,0.028987998646194328
18018,36037,0,36037,33.49682903289795,0.028754622471627602
18118,36237,0,36237,33.71851110458374,0.028352680225392134
18218,36437,0,36437,34.12039089202881,0.028063798048752392
18318,36637,0,36637,34.718510150909424,0.027954735070929704
18418,36837,0,36837,35.31032919883728,0.027846054165244716
18519,37039,0,37039,35.67848801612854,0.027714318313898558
18619,37239,0,37239,36.30276703834534,0.0276464620901262
18719,37439,0,37439,36.58930420875549,0.027595404030343378
18819,37639,0,37639,36.82678198814392,0.02752070848648731
18919,37839,0,37839,37.00404095649719,0.02748038757635805
19019,38039,0,38039,37.1661639213562,0.027443577174033618
19119,38239,0,38239,37.314332246780396,0.02729219931817483
19219,38439,0,38439,37.549986124038696,0.027010347194604205
19319,38639,0,38639,37.85949110984802,0.02668892568665085
19419,38839,0,38839,38.12392020225525,0.026407814489896486
19520,39041,0,39041,38.34471297264099,0.02617565005284747
19620,39241,0,39241,38.58427023887634,0.02600712537624964
19720,39441,0,39441,38.72247815132141,0.02597071652497352
19820,39641,0,39641,38.86555600166321,0.026034849173947057
19920,39841,0,39841,39.025827169418335,0.02599386069255185
20020,40041,0,40041,39.18114900588989,0.025760449013504987
20120,40241,0,40241,39.32174110412598,0.025508959866733277
20220,40441,0,40441,39.46534705162048,0.02542747375051588
20320,40641,0,40641,39.61157417297363,0.025496766064424543
20420,40841,0,40841,39.766937255859375,0.02556557100236526
20521,41043,0,41043,39.9231219291687,0.025535577563808115
20621,41243,0,41243,40.0694260597229,0.02539664856588189
20721,41443,0,41443,40.20889496803284,0.025166565532885876
20821,41643,0,41643,40.349059104919434,0.02492525364309501
20921,41843,0,41843,40.48798418045044,0.024803135239849016
21021,42043,0,42043,40.62782406806946,0.02478630791517705
21121,42243,0,42243,40.76799011230469,0.02468672157348031
21221,42443,0,42443,40.909953117370605,0.02441362752208856
21321,42643,0,42643,41.04973006248474,0.024122766818374605
21421,42843,0,42843,41.189054012298584,0.023996608574734832
21522,43045,0,43045,41.33164691925049,0.024004181569763822
21622,43245,0,43245,41.47215509414673,0.02402138540707371
21722,43445,0,43445,41.61233615875244,0.024009679198209868
21822,43645,0,43645,41.75184416770935,0.023965775830600826
21922,43845,0,43845,41.90221118927002,0.02385117709501578
22022,44045,0,44045,42.05331301689148,0.02363103468017419
22122,44245,0,44245,42.19299006462097,0.023389617318924666
22222,44445,0,44445,42.33120512962341,0.023301785818496224
22322,44645,0,44645,42.47008419036865,0.023387972371325758
22422,44845,0,44845,42.61061906814575,0.023462034108465472
22523,45047,0,45047,42.752732276916504,0.023387684381331424
22623,45247,0,45247,42.89472699165344,0.023207288172031625
22723,45447,0,45447,43.03316402435303,0.022993623405004132
22823,45647,0,45647,43.17344522476196,0.02276272338568233
22923,45847,0,45847,43.31930708885193,0.022547499551862325
23023,46047,0,46047,43.46453809738159,0.022398049185947524
23123,46247,0,46247,43.60546517372131,0.02226787405332401
23223,46447,0,46447,43.744346141815186,0.022070668505965257
23323,46647,0,46647,43.8832950592041,0.021856559123997667
23423,46847,0,46847,44.02893590927124,0.021768471486244098
23524,47049,0,47049,44.18869924545288,0.021842919983068892
23624,47249,0,47249,44.33228898048401,0.021958606858033698
23724,47449,0,47449,44.47100591659546,0.022000080410013646
23824,47649,0,47649,44.609586000442505,0.021944831394345204
23924,47849,0,47849,44.74910116195679,0.021802858151697475
24024,48049,0,48049,44.89036798477173,0.021612095792515745
24124,48249,0,48249,45.029675006866455,0.021460817274071488
24224,48449,0,48449,45.167815923690796,0.02139638466033242
24324,48649,0,48649,45.31343412399292,0.021361147257037003
24424,48849,0,48849,45.453880071640015,0.021286401970289238
24525,49051,0,49051,45.595492124557495,0.021180462801429323
24625,49251,0,49251,45.73885917663574,0.021079262573999932
24725,49451,0,49451,45.880369901657104,0.020985349095730646
24825,49651,0,49651,46.02093505859375,0.020899380883918146
24925,49851,0,49851,46.16615414619446,0.020809470914720605
25025,50051,0,50051,46.32304906845093,0.020661498724937593
25125,50251,0,50251,46.465835094451904,0.02043151742871085
25225,50451,0,50451,46.612611055374146,0.02021435357845601
25325,50651,0,50651,46.75834107398987,0.020147892675608424
25425,50851,0,50851,46.89830303192139,0.020242890401302557
25526,51053,0,51053,47.04146218299866,0.020371346061538193
25626,51253,0,51253,47.17877411842346,0.020412603751708242
25726,51453,0,51453,47.31961011886597,0.02033943832475628
25826,51653,0,51653,47.460347175598145,0.020173734263635626
25926,51853,0,51853,47.60117197036743,0.01996066471172284
26026,52053,0,52053,47.74102807044983,0.0197563625832987
26126,52253,0,52253,47.88426113128662,0.01960803039736928
26226,52453,0,52453,48.03850293159485,0.01953788957476648
26326,52653,0,52653,48.18619227409363,0.01953295733206041
26426,52853,0,52853,48.328680992126465,0.019560820451539
26527,53055,0,53055,48.518759965896606,0.01958528858456055
26627,53255,0,53255,48.71254920959473,0.019557358963775237
26727,53455,0,53455,48.86417317390442,0.019445105239422056
26827,53655,0,53655,49.006033182144165,0.019282746028292032
26927,53855,0,53855,49.14616513252258,0.019142390769744104
27027,54055,0,54055,49.28472399711609,0.019043495418734374
27127,54255,0,54255,49.42277503013611,0.018953928906568628
27227,54455,0,54455,49.56311511993408,0.01888129073058618
27327,54655,0,54655,49.70645093917847,0.01886469059639454
27427,54855,0,54855,49.8493812084198,0.0188782427952823
27528,55057,0,55057,49.99298095703125,0.018839751056161865
27628,55257,0,55257,50.133131980895996,0.018712613694067202
27728,55457,0,55457,50.2748339176178,0.018527342750287033
27828,55657,0,55657,50.41363501548767,0.01832803994536607
27928,55857,0,55857,50.562516927719116,0.018160704485035876
28028,56057,0,56057,50.7113242149353,0.018083941018111865
28128,56257,0,56257,50.85014009475708,0.01811885679441954
28228,56457,0,56457,50.98836398124695,0.018216511192887773
28328,56657,0,56657,51.125893115997314,0.018313769265381974
28428,56857,0,56857,51.263880014419556,0.018376708617969806
28529,57059,0,57059,51.40371108055115,0.01837708615808386
28629,57259,0,57259,51.543421030044556,0.018285559986872788
28729,57459,0,57459,51.683566093444824,0.018111169242099514
28829,57659,0,57659,51.82315492630005,0.01791647271314816
28929,57859,0,57859,51.96472191810608,0.017769560746001847
29029,58059,0,58059,52.10442614555359,0.017686607375438798
29129,58259,0,58259,52.243226051330566,0.017644811695501
29229,58459,0,58459,52.385149002075195,0.017627732777876527
29329,58659,0,58659,52.525336027145386,0.017617898232168125
29429,58859,0,58859,52.6703622341156,0.01756990663997418
29530,59061,0,59061,52.82514524459839,0.017439505064197548
29630,59261,0,59261,52.964022159576416,0.01724628532322213
29730,59461,0,59461,53.10378408432007,0.017057233385210847
29830,59661,0,59661,53.24269223213196,0.016932406354641362
29930,59861,0,59861,53.38509488105774,0.016901776242951534
30030,60061,0,60061,53.52501821517944,0.016968835602166492
30130,60261,0,60261,53.66336107254028,0.017094077208469755
30230,60461,0,60461,53.8031702041626,0.017206794452329508
30330,60661,0,60661,53.94196820259094,0.01726208936669864
30430,60861,0,60861,54.08150601387024,0.017257346955811506
30531,61063,0,61063,54.2209370136261,0.017195906962887628
30631,61263,0,61263,54.36005926132202,0.01708551879920498
30731,61463,0,61463,54.50392699241638,0.016954606640534647
30831,61663,0,61663,54.66234111785889,0.016830574039153768
30931,61863,0,61863,54.80687618255615,0.016704186058886135
31031,62063,0,62063,54.96155023574829,0.016550320581509233
31131,62263,0,62263,55.10046100616455,0.016374896619064844
31231,62463,0,62463,55.23845314979553,0.016220035409053885
31331,62663,0,62663,55.37863302230835,0.0161251296361851
31431,62863,0,62863,55.51714205741882,0.016093542405230095
31532,63065,0,63065,55.657185077667236,0.0160966317919889
31632,63265,0,63265,55.7992582321167,0.016103484325531322
31732,63465,0,63465,55.94099998474121,0.01610923859250133
31832,63665,0,63665,56.08080315589905,0.016130841199404274
31932,63865,0,63865,56.220020055770874,0.016176988298711652
32032,64065,0,64065,56.361868143081665,0.016232251828354742
32132,64265,0,64265,56.50171494483948,0.016266410752709525
32232,64465,0,64465,56.64208507537842,0.01625265375404626
32332,64665,0,64665,56.78187394142151,0.016184515856696263
32432,64865,0,64865,56.92553901672363,0.016077774893097495
32533,65067,0,65067,57.07921004295349,0.01595553044298982
32633,65267,0,65267,57.222116231918335,0.01584379846074374
32733,65467,0,65467,57.35841202735901,0.015761298626634047
32833,65667,0,65667,57.4971079826355,0.01571436719308903
32933,65867,0,65867,57.63566327095032,0.015684113968030808
33033,66067,0,66067,57.77517008781433,0.01563718628207119
33133,66267,0,66267,57.91653108596802,0.015561430080103095
33233,66467,0,66467,58.05879807472229,0.015488253289237384
33333,66667,0,66667,58.198180198669434,0.015462951018103969
33433,66867,0,66867,58.33907413482666,0.015489346495871357
33534,67069,0,67069,58.4794659614563,0.01552245682061283
33634,67269,0,67269,58.620174169540405,0.015517834758103043
33734,67469,0,67469,58.75796723365784,0.015472652186821128
33834,67669,0,67669,58.90006923675537,0.015409418102235955
33934,67869,0,67869,59.042120933532715,0.015344384012833898
34034,68069,0,68069,59.19281196594238,0.01527794784851376
34134,68269,0,68269,59.34297513961792,0.015199265219672048
34234,68469,0,68469,59.48114514350891,0.01508947506158077
34334,68669,0,68669,59.62051606178284,0.014939526306276768
34434,68869,0,68869,59.76243710517883,0.014775825934942855
34535,69071,0,69071,59.90908908843994,0.014647489877268077
34635,69271,0,69271,60.04636001586914,0.014587607965173083
34735,69471,0,69471,60.18569302558899,0.014589804022144593
34835,69671,0,69671,60.3238799571991,0.014632373822527448
34935,69871,0,69871,60.464760065078735,0.014688287391773719
35035,70071,0,70071,60.60201406478882,0.014729599241684948
35135,70271,0,70271,60.74333119392395,0.014740616450661504
35235,70471,0,70471,60.88303899765015,0.014725003569755538
35335,70671,0,70671,61.02042293548584,0.014694288541799551
35435,70871,0,70871,61.157158851623535,0.01465586360281478
35536,71073,0,71073,61.302310943603516,0.014610209900169662
35636,71273,0,71273,61.45533490180969,0.014550017962549452
35736,71473,0,71473,61.59564018249512,0.014463717806083113
35836,71673,0,71673,61.73346519470215,0.014359620897802967
35936,71873,0,71873,61.87047815322876,0.014267943012794502
36036,72073,0,72073,62.01041316986084,0.014202592977174359
36136,72273,0,72273,62.151121854782104,0.014137619246036265
36236,72473,0,72473,62.2890522480011,0.014044284091892898
36336,72673,0,72673,62.42695903778076,0.013935296262172504
36436,72873,0,72873,62.566468238830566,0.013852339077216174
36537,73075,0,73075,62.7069890499115,0.013825530985620362
36637,73275,0,73275,62.84864115715027,0.013859682257077144
36737,73475,0,73475,62.98637413978577,0.013936462377438149
36837,73675,0,73675,63.1252019405365,0.014017397378569496
36937,73875,0,73875,63.26297187805176,0.014062110896130214
37037,74075,0,74075,63.40336513519287,0.014062010591681353
37137,74275,0,74275,63.55707001686096,0.014041075495928992
37237,74475,0,74475,63.700247049331665,0.014016728621862401
37337,74675,0,74675,63.83834505081177,0.013977594335335545
37437,74875,0,74875,63.97820019721985,0.013903071920659935
37538,75077,0,75077,64.11892819404602,0.013783511178033963
37638,75277,0,75277,64.25683903694153,0.013627208042192342
37738,75477,0,75477,64.39514493942261,0.013454974063232074
37838,75677,0,75677,64.53443884849548,0.013307537678005197
37938,75877,0,75877,64.67640614509583,0.013225433458712235
38038,76077,0,76077,64.81557703018188,0.013215142035751413
38138,76277,0,76277,64.95368194580078,0.013244020639857617
38238,76477,0,76477,65.09136509895325,0.01327506530385277
38338,76677,0,76677,65.22844409942627,0.013297328565262034
38438,76877,0,76877,65.36846899986267,0.013319066659406749
38539,77079,0,77079,65.50663089752197,0.013343588920700122
38639,77279,0,77279,65.65363001823425,0.01336029402186117
38739,77479,0,77479,65.80186223983765,0.013358028375924555
38839,77679,0,77679,65.94392609596252,0.013335559627283874
38939,77879,0,77879,66.08235120773315,0.0133027293595509
39039,78079,0,78079,66.22427701950073,0.013273772774273137
39139,78279,0,78279,66.36777710914612,0.013255730213829196
39239,78479,0,78479,66.5070321559906,0.013238501480488848
39339,78679,0,78679,66.64542412757874,0.013200385365776963
39439,78879,0,78879,66.785325050354,0.013127733246447193
39540,79081,0,79081,66.93263912200928,0.013024919177860115
39640,79281,0,79281,67.17652916908264,0.012911563980715109
39740,79481,0,79481,67.4251389503479,0.012806458175856832
39840,79681,0,79681,67.70243716239929,0.012728732496064377
39940,79881,0,79881,67.93281412124634,0.012692754975207858
40040,80081,0,80081,68.11664509773254,0.012700268423175882
40140,80281,0,80281,68.30796003341675,0.012737914631257466
40240,80481,0,80481,68.48801803588867,0.012784080541779309
40340,80681,0,80681,68.65627694129944,0.012818423149746645
40440,80881,0,80881,68.81160187721252,0.012826821499396273
40541,81083,0,81083,68.95763111114502,0.012801435733162211
40641,81283,0,81283,69.10444712638855,0.012742652291862396
40741,81483,0,81483,69.24606585502625,0.012660988437429419
40841,81683,0,81683,69.38697123527527,0.012579907245720553
40941,81883,0,81883,69.5362958908081,0.012526604825476809
41041,82083,0,82083,69.67928910255432,0.012510698329113678
41141,82283,0,82283,69.82203912734985,0.01251063302229887
41241,82483,0,82483,69.97195506095886,0.012487857864645176
41341,82683,0,82683,70.13462805747986,0.012420150434973628
41441,82883,0,82883,70.29066014289856,0.012323207428942624
41542,83085,0,83085,70.43748211860657,0.012239220431054534
41642,83285,0,83285,70.58119010925293,0.012207380477913964
41742,83485,0,83485,70.74080896377563,0.012234490215297893
41842,83685,0,83685,70.89267420768738,0.012300252157371096
41942,83885,0,83885,71.0392918586731,0.012371385369381871
42042,84085,0,84085,71.31161713600159,0.012416809756613483
42142,84285,0,84285,71.59101915359497,0.012418783475341894
42242,84485,0,84485,71.86282396316528,0.012376067277606621
42342,84685,0,84685,72.03845930099487,0.012297601339261218
42442,84885,0,84885,72.20846009254456,0.012194656045983934
42543,85087,0,85087,72.40397596359253,0.012077897272204034
42643,85287,0,85287,72.58356308937073,0.011963407029654996
42743,85487,0,85487,72.75315523147583,0.011864252928732985
42843,85687,0,85687,72.93398714065552,0.01179295357064305
42943,85887,0,85887,73.09883213043213,0.011758091845178325
43043,86087,0,86087,73.25862407684326,0.011757782339821742
43143,86287,0,86287,73.45214915275574,0.011774297477590442
43243,86487,0,86487,73.62145614624023,0.011783651120177454
43343,86687,0,86687,73.81641292572021,0.011776357852712424
43443,86887,0,86887,73.99177408218384,0.011766461342112728
43544,87089,0,87089,74.25992202758789,0.011777174527791477
43644,87289,0,87289,74.43789792060852,0.011816339292235457
43744,87489,0,87489,74.5992739200592,0.01186796113659586
43844,87689,0,87689,74.75884509086609,0.011904220198060422
43944,87889,0,87889,74.95225024223328,0.011902787024105563
44044,88089,0,88089,75.15810203552246,0.011855651617724497
44144,88289,0,88289,75.32253003120422,0.01176967219173793
44244,88489,0,88489,75.48840022087097,0.011662500697635053
44344,88689,0,88689,75.66220903396606,0.01155419492331616
44444,88889,0,88889,75.88904190063477,0.011458434039250462
44545,89091,0,89091,76.07428097724915,0.011380739199294523
44645,89291,0,89291,76.30490708351135,0.011328151393830461
44745,89491,0,89491,76.51421689987183,0.011308211755799847
44845,89691,0,89691,76.75017213821411,0.01132563582406941
44945,89891,0,89891,76.96222591400146,0.011372041161683093
45045,90091,0,90091,77.14995622634888,0.01142555808082766
45145,90291,0,90291,77.33453798294067,0.011461119215912398
45245,90491,0,90491,77.51585507392883,0.011464065199006678
45345,90691,0,90691,77.72482514381409,0.011438328863609314
45445,90891,0,90891,77.97400498390198,0.011402646613409749
45546,91093,0,91093,78.13556718826294,0.011375255963750212
45646,91293,0,91293,78.2939100265503,0.01135984633320136
45746,91493,0,91493,78.45635724067688,0.011342589272360334
45846,91693,0,91693,78.79091000556946,0.011306161416222045
45946,91893,0,91893,78.99419808387756,0.011242877646983236
46046,92093,0,92093,79.22555494308472,0.011157994082515315
46146,92293,0,92293,79.42173409461975,0.011064107853662623
46246,92493,0,92493,79.69337010383606,0.010974201998277262
46346,92693,0,92693,79.86438822746277,0.010897923728098835
46446,92893,0,92893,80.0498309135437,0.010841124492370196
46547,93095,0,93095,80.22939014434814,0.010806369861447986
46647,93295,0,93295,80.49212312698364,0.010794185282570005
46747,93495,0,93495,80.84655427932739,0.010800816793398539
46847,93695,0,93695,81.09682989120483,0.010820798618606456
46947,93895,0,93895,81.41915798187256,0.010847501831649575
47047,94095,0,94095,81.59665727615356,0.010871896080965988
47147,94295,0,94295,81.75271701812744,0.0108819441686309
47247,94495,0,94495,81.90463900566101,0.010868699765496908
47347,94695,0,94695,82.0954749584198,0.010835407193025965
47447,94895,0,94895,82.26882410049438,0.010796416195112847
47548,95097,0,95097,82.4203588962555,0.01076353217104118
47648,95297,0,95297,82.58019304275513,0.010737019324661885
47748,95497,0,95497,82.74245190620422,0.010707345110592546
47848,95697,0,95697,82.89141511917114,0.01066638270101225
47948,95897,0,95897,83.03838324546814,0.010613234755673967
48048,96097,0,96097,83.19222807884216,0.010556517875377341
48148,96297,0,96297,83.37339401245117,0.010512613064664372
48248,96497,0,96497,83.51478815078735,0.010497428713284317
48348,96697,0,96697,83.6601049900055,0.010516058170096446
48448,96897,0,96897,83.80816698074341,0.010559470569999807
48549,97099,0,97099,83.95699214935303,0.01060986397600848
48649,97299,0,97299,84.10341000556946,0.010645589108546268
48749,97499,0,97499,84.24881625175476,0.010651101774952721
48849,97699,0,97699,84.40064692497253,0.010620718499309085
48949,97899,0,97899,84.5804979801178,0.010560435742633007
49049,98099,0,98099,84.73319101333618,0.010482869130013147
49149,98299,0,98299,84.87895202636719,0.010401054788361272
49249,98499,0,98499,85.02480506896973,0.010325869901391437
49349,98699,0,98699,85.17633104324341,0.010265694908262776
49449,98899,0,98899,85.37422513961792,0.010225602614748109
49550,99101,0,99101,85.53511023521423,0.01020620653417577
49650,99301,0,99301,85.68829011917114,0.010204166888293783
49750,99501,0,99501,85.83882808685303,0.010212448385454754
49850,99701,0,99701,85.99549317359924,0.010223767292644901
49950,99901,0,99901,86.14860701560974,0.01023315134381706
50050,100101,0,100101,86.2969400882721,0.01023965838689479
50150,100301,0,100301,86.4434220790863,0.010245897124337582
50250,100501,0,100501,86.59995913505554,0.0102555662351311
50350,100701,0,100701,86.87744402885437,0.010269959048277951
50450,100901,0,100901,87.1458191871643,0.010284999262658146
50551,101103,0,101103,87.48881506919861,0.010291051589591968
50651,101303,0,101303,87.79291605949402,0.01027659087278254
50751,101503,0,101503,88.0866551399231,0.01023480071332151
50851,101703,0,101703,88.23417615890503,0.010167629691904736
50951,101903,0,101903,88.38058114051819,0.0100860867665856
51051,102103,0,102103,88.56365323066711,0.010005760880145822
51151,102303,0,102303,88.98539113998413,0.009940416899247642
51251,102503,0,102503,89.1446590423584,0.009897968346366796
51351,102703,0,102703,89.30694913864136,0.009880784933201063
51451,102903,0,102903,89.44793128967285,0.009887725324315061
51552,103105,0,103105,89.59834694862366,0.00991455167040193
51652,103305,0,103305,89.76583814620972,0.009951024181346326
51752,103505,0,103505,89.92786717414856,0.009983209989003157
51852,103705,0,103705,90.07943916320801,0.00999760941779912
51952,103905,0,103905,90.24006819725037,0.00998848165511447
52052,104105,0,104105,90.39767289161682,0.009961374294335296
52152,104305,0,104305,90.5492250919342,0.009928890571215319
52252,104505,0,104505,90.6996910572052,0.009901124981513002
52352,104705,0,104705,90.85251092910767,0.009879044978898627
52452,104905,0,104905,91.00477695465088,0.009856324318212761
52553,105107,0,105107,91.14627003669739,0.009825568869789384
52653,105307,0,105307,91.29486322402954,0.00978360800731093
52753,105507,0,105507,91.45438313484192,0.009729440421860842
52853,105707,0,105707,91.67771911621094,0.009664478072257468
52953,105907,0,105907,91.83799719810486,0.009592877024314298
53053,106107,0,106107,91.98370718955994,0.009522148907906907
53153,106307,0,106307,92.12481713294983,0.00946278976011986
53253,106507,0,106507,92.26522612571716,0.009426889822560437
53353,106707,0,106707,92.40559005737305,0.009424827446281966
53453,106907,0,106907,92.55488896369934,0.009459845694395718
53554,107109,0,107109,92.70233702659607,0.009524071734436873
53654,107309,0,107309,92.84269690513611,0.009595575912943214
53754,107509,0,107509,92.98202705383301,0.009648773823382207
53854,107709,0,107709,93.12073016166687,0.00966251742752922
53954,107909,0,107909,93.26300501823425,0.009630419090533386
54054,108109,0,108109,93.4037492275238,0.009563693057695272
54154,108309,0,108309,93.54596614837646,0.009483979155647585
54254,108509,0,108509,93.6908118724823,0.009410635282507882
54354,108709,0,108709,93.83538889884949,0.00935210956849279
54454,108909,0,108909,93.99134111404419,0.009306820460860834
54555,109111,0,109111,94.14050507545471,0.009269354349423395
54655,109311,0,109311,94.28131818771362,0.009236959099700737
54755,109511,0,109511,94.42026710510254,0.009208311950714225
54855,109711,0,109711,94.56079316139221,0.009183786808967925
54955,109911,0,109911,94.72638607025146,0.009164227725637315
55055,110111,0,110111,94.86954808235168,0.009151307714527001
55155,110311,0,110311,95.0194091796875,0.009147877192018383
55255,110511,0,110511,95.16169500350952,0.009156784724165366
55355,110711,0,110711,95.30157709121704,0.009178363207267122
55455,110911,0,110911,95.46712398529053,0.009208301629163853
55556,111113,0,111113,95.61296892166138,0.009237516304892487
55656,111313,0,111313,95.75923705101013,0.009252978045276868
55756,111513,0,111513,95.90106225013733,0.009244426210345798
55856,111713,0,111713,96.04289722442627,0.009209236598211837
55956,111913,0,111913,96.20088911056519,0.009155936879803036
56056,112113,0,112113,96.34087824821472,0.00910036276871182
56156,112313,0,112313,96.49300813674927,0.00905627739051067
56256,112513,0,112513,96.63718819618225,0.009027588012698609
56356,112713,0,112713,96.78135299682617,0.009008467868996254
56456,112913,0,112913,96.95831298828125,0.008990939247917419
56557,113115,0,113115,97.1017861366272,0.00897307191494729
56657,113315,0,113315,97.24572706222534,0.008961567255446655
56757,113515,0,113515,97.38780212402344,0.008964087249593874
56857,113715,0,113715,97.53205704689026,0.008981373214387795
56957,113915,0,113915,97.67836809158325,0.009004982587349008
57057,114115,0,114115,97.82190895080566,0.009023596090446203
57157,114315,0,114315,97.96859216690063,0.009030677997272776
57257,114515,0,114515,98.10745120048523,0.00902606081505389
57357,114715,0,114715,98.25449919700623,0.009011678856836569
57457,114915,0,114915,98.40290403366089,0.008987408243565491
57558,115117,0,115117,98.54612517356873,0.008950698567701785
57658,115317,0,115317,98.6900360584259,0.008901513371717367
57758,115517,0,115517,98.8302800655365,0.008843691868708401
57858,115717,0,115717,98.97291016578674,0.008787300874448893
57958,115917,0,115917,99.11548805236816,0.008745068261557316
58058,116117,0,116117,99.25880026817322,0.00872525576680209
58158,116317,0,116317,99.39929819107056,0.008725586194653063
58258,116517,0,116517,99.54189014434814,0.008734363785181786
58358,116717,0,116717,99.68600821495056,0.008738940966493323
58458,116917,0,116917,99.82930421829224,0.008734441587370752
58559,117119,0,117119,99.97381520271301,0.008725393227144565
58659,117319,0,117319,100.11510825157166,0.008720062531385192
58759,117519,0,117519,100.25537514686584,0.00872157286200503
58859,117719,0,117719,100.40582919120789,0.00872491736932361
58959,117919,0,117919,100.57234716415405,0.008720594293963635
59059,118119,0,118119,100.71954298019409,0.008701867785545634
59159,118319,0,118319,100.86195206642151,0.008669512051335006
59259,118519,0,118519,101.00460505485535,0.00863048508896663
59359,118719,0,118719,101.1545820236206,0.008592301584589195
59459,118919,0,118919,101.33240127563477,0.008558521245335883
59560,119121,0,119121,101.47482490539551,0.008528771966214132
59660,119321,0,119321,101.62335705757141,0.008503384429111407
59760,119521,0,119521,101.78289103507996,0.008484025713812909
59860,119721,0,119721,101.94649600982666,0.008474257189050627
59960,119921,0,119921,102.08744812011719,0.008476758026289328
60060,120121,0,120121,102.23201298713684,0.008490815631207767
60160,120321,0,120321,102.3889889717102,0.008511155376715106
60260,120521,0,120521,102.54405999183655,0.008529374172908834
60360,120721,0,120721,102.7081651687622,0.008537724882208097
60460,120921,0,120921,102.8507981300354,0.00853254399020506
60561,121123,0,121123,102.99373507499695,0.00851433021707082
60661,121323,0,121323,103.13467001914978,0.008486065531925444
60761,121523,0,121523,103.28152704238892,0.008449692949333034
60861,121723,0,121723,103.44727396965027,0.008406956450118639
60961,121923,0,121923,103.58982610702515,0.0083614277628768
61061,122123,0,122123,103.7577211856842,0.008319547845256866
61161,122323,0,122323,103.92042398452759,0.008288408962766681
61261,122523,0,122523,104.06824707984924,0.008271527603507639
61361,122723,0,122723,104.23179221153259,0.00826638416412064
61461,122923,0,122923,104.37338399887085,0.008266331753568884
61562,123125,0,123125,104.51748704910278,0.008265511865901546
61662,123325,0,123325,104.66318893432617,0.008262712286568545
61762,123525,0,123525,104.86228609085083,0.008260756087398315
61862,123725,0,123725,105.03070998191833,0.008262294661417733
61962,123925,0,123925,105.18324995040894,0.008266099637052719
62062,124125,0,124125,105.33392906188965,0.008267272638301964
62162,124325,0,124325,105.47421312332153,0.00826089646099475
62262,124525,0,124525,105.61354613304138,0.008245615116643429
62362,124725,0,124725,105.75525498390198,0.008224278966411829
62462,124925,0,124925,105.89363312721252,0.008201624594823608
62563,125127,0,125127,106.04903721809387,0.008180915031660676
62663,125327,0,125327,106.20800518989563,0.008163058711323997
62763,125527,0,125527,106.34765219688416,0.00814623918410569
62863,125727,0,125727,106.48971605300903,0.00812920947165199
62963,125927,0,125927,106.63437223434448,0.008112874939602594
63063,126127,0,126127,106.77502202987671,0.008099760384747095
63163,126327,0,126327,106.92199611663818,0.008091448412741137
63263,126527,0,126527,107.07033801078796,0.008086365394416376
63363,126727,0,126727,107.21544909477234,0.008080307328251025
63463,126927,0,126927,107.3528220653534,0.008069571872648073
63564,127129,0,127129,107.49187994003296,0.008053758640169696
63664,127329,0,127329,107.63630795478821,0.008036623961967478
63764,127529,0,127529,107.77641916275024,0.008022374792557277
63864,127729,0,127729,107.91569519042969,0.008012990310244416
63964,127929,0,127929,108.06306409835815,0.008006587873010325
64064,128129,0,128129,108.2859902381897,0.007998614467900619
64164,128329,0,128329,108.50383114814758,0.007984986689291288
64264,128529,0,128529,108.7120041847229,0.007965083016907822
64364,128729,0,128729,108.94732308387756,0.007942251210508275
64464,128929,0,128929,109.21158504486084,0.007921319846192933
64565,129131,0,129131,109.46561098098755,0.00790517071069707
64665,129331,0,129331,109.60762906074524,0.007893996470141731
64765,129531,0,129531,109.77391219139099,0.0078855679918898
64865,129731,0,129731,109.92638325691223,0.007877940753567424
64965,129931,0,129931,110.06837105751038,0.007870245200442775
65065,130131,0,130131,110.20969009399414,0.007862136263003496
65165,130331,0,130331,110.36030316352844,0.007852399863565363
65265,130531,0,130531,110.54855513572693,0.007838165750774492
65365,130731,0,130731,110.77166223526001,0.00781596014649091
65465,130931,0,130931,111.00593996047974,0.007784159899085373
65566,131133,0,131133,111.16241908073425,0.007744350593429415
65666,131333,0,131333,111.31581902503967,0.007702494869741139
65766,131533,0,131533,111.46036195755005,0.0076642115634012
65866,131733,0,131733,111.59970903396606,0.007634133292263829
65966,131933,0,131933,111.75437211990356,0.00761464881873025
66066,132133,0,132133,111.89346814155579,0.0076061646821752255
66166,132333,0,132333,112.03252100944519,0.0076075837361616536
66266,132533,0,132533,112.17054796218872,0.007616217898863698
66366,132733,0,132733,112.32135605812073,0.007627396335077593
66466,132933,0,132933,112.47076511383057,0.0076350440915828365
66567,133135,0,133135,112.61216425895691,0.007633977765829463
66667,133335,0,133335,112.79449605941772,0.007623128130622374
66767,133535,0,133535,112.95047092437744,0.007606894023666675
66867,133735,0,133735,113.09694600105286,0.007593205965884688
66967,133935,0,133935,113.24551820755005,0.00758907453480992
67067,134135,0,134135,113.40265226364136,0.0075958917001781295
67167,134335,0,134335,113.56182193756104,0.007607483716554586
67267,134535,0,134535,113.73854422569275,0.00761254319284104
67367,134735,0,134735,113.94308924674988,0.007600361443620601
67467,134935,0,134935,114.12176012992859,0.007566652591332655
67568,135137,0,135137,114.27624607086182,0.007515807541995842
67668,135337,0,135337,114.50277805328369,0.007461601028295551
67768,135537,0,135537,114.7565062046051,0.007418814901836168
67868,135737,0,135737,114.96268105506897,0.007398877673403144
67968,135937,0,135937,115.13690710067749,0.00740513455417546
68068,136137,0,136137,115.27897500991821,0.0074325876775086204
68168,136337,0,136337,115.4219741821289,0.007470847309105479
68268,136537,0,136537,115.57301092147827,0.00750778890636362
68368,136737,0,136737,115.72384119033813,0.007532518788231393
68468,136937,0,136937,115.86351799964905,0.007537989774433869
68569,137139,0,137139,116.00249195098877,0.00752313888246152
68669,137339,0,137339,116.1657202243805,0.007494472214611841
68769,137539,0,137539,116.38540601730347,0.0074626970259235245
68869,137739,0,137739,116.74959421157837,0.0074382113425732
68969,137939,0,137939,116.98537921905518,0.007426332099352638
69069,138139,0,138139,117.23238825798035,0.007425476043649583
69169,138339,0,138339,117.4655601978302,0.007428757128498165
69269,138539,0,138539,117.79416298866272,0.007427495777043327
69369,138739,0,138739,118.04842710494995,0.007414904313323584
69469,138939,0,138939,118.24085402488708,0.00738895568792465
69570,139141,0,139141,118.5178382396698,0.007353324134874132
69670,139341,0,139341,118.74239897727966,0.007317827002583507
69770,139541,0,139541,118.95288920402527,0.007292448049569305
69870,139741,0,139741,119.12213826179504,0.00728388975285166
69970,139941,0,139941,119.27743911743164,0.007291894165148003
70070,140141,0,140141,119.44599294662476,0.007309365579618959
70170,140341,0,140341,119.67044925689697,0.007325867165009194
70270,140541,0,140541,119.91828203201294,0.0073324455463139
70370,140741,0,140741,120.14241218566895,0.007325255432384266
70470,140941,0,140941,120.33767104148865,0.007306403915929946
70571,141143,0,141143,120.57073402404785,0.007281757626730526
70671,141343,0,141343,120.76987385749817,0.007258551240901788
70771,141543,0,141543,120.93386387825012,0.007240710587261453
70871,141743,0,141743,121.09307503700256,0.007228516381931737
70971,141943,0,141943,121.29829406738281,0.007219200857401336
71071,142143,0,142143,121.46290302276611,0.007209207853257677
71171,142343,0,142343,121.64872598648071,0.007196392067677429
71271,142543,0,142543,121.81073307991028,0.007180900905418578
71371,142743,0,142743,122.00678396224976,0.00716463625909981
71471,142943,0,142943,122.27190923690796,0.007150167142516548
71572,143145,0,143145,122.45473790168762,0.007139746825675723
71672,143345,0,143345,122.62981104850769,0.007134875475122783
71772,143545,0,143545,122.76861429214478,0.007134671017617759
71872,143745,0,143745,122.91107296943665,0.007135628063166644
71972,143945,0,143945,123.08014106750488,0.007132077045638832
72072,144145,0,144145,123.27140522003174,0.0071184648046096624
72172,144345,0,144345,123.42334413528442,0.007092230226602446
72272,144545,0,144545,123.56926417350769,0.007055402962332105
72372,144745,0,144745,123.70916104316711,0.0070138702045031255
72472,144945,0,144945,123.86496806144714,0.006974888150241082
72573,145147,0,145147,124.08456802368164,0.006944148022073128
72673,145347,0,145347,124.29730725288391,0.006925292778891284
72773,145547,0,145547,124.48046207427979,0.006917875978146587
72873,145747,0,145747,124.75988912582397,0.006919561963211549
72973,145947,0,145947,125.06754112243652,0.006926965599666051
73073,146147,0,146147,125.38351321220398,0.006936733904770021
73173,146347,0,146347,125.76097798347473,0.006946345144078973
73273,146547,0,146547,125.97258019447327,0.006954547425440428
73373,146747,0,146747,126.16247391700745,0.006961255811001066
73473,146947,0,146947,126.31272196769714,0.00696679508052837
73574,147149,0,147149,126.54048418998718,0.00697077657708188
73674,147349,0,147349,126.7157518863678,0.006971004105582384
73774,147549,0,147549,126.93682718276978,0.006963651394628524
73874,147749,0,147749,127.11744999885559,0.0069442068536887955
73974,147949,0,147949,127.29579019546509,0.006909742711247745
74074,148149,0,148149,127.59825420379639,0.0068613430043831265
74174,148349,0,148349,128.00805616378784,0.006805258170282584
74274,148549,0,148549,128.23109102249146,0.00675162599098296
74374,148749,0,148749,128.37661814689636,0.006711022148998466
74474,148949,0,148949,128.5159511566162,0.00669064787234138
74575,149151,0,149151,128.6654450893402,0.006692343965437919
74675,149351,0,149351,128.81358408927917,0.006712614874554916
74775,149551,0,149551,128.95344424247742,0.0067446851634746655
74875,149751,0,149751,129.0954451560974,0.0067806812984054395
74975,149951,0,149951,129.2683892250061,0.006813073022738576
75075,150151,0,150151,129.44060492515564,0.006835877313430314
75175,150351,0,150351,129.59692907333374,0.006845770609036277
75275,150551,0,150551,129.7460720539093,0.006842793501541607
75375,150751,0,150751,129.88874125480652,0.0068299854795553306
75475,150951,0,150951,130.02975797653198,0.006811728305502138
75576,151153,0,151153,130.1709361076355,0.006791315190474841
75676,151353,0,151353,130.32760310173035,0.006770255221856824
75776,151553,0,151553,130.46893119812012,0.00674718501745225
75876,151753,0,151753,130.60745906829834,0.006720412141146164
75976,151953,0,151953,130.75515389442444,0.006690027402633916
76076,152153,0,152153,130.9137840270996,0.006659366259155786
76176,152353,0,152353,131.05522894859314,0.006634464509510205
76276,152553,0,152553,131.19356322288513,0.006621461699591522
76376,152753,0,152753,131.33073902130127,0.006623375903892735
76476,152953,0,152953,131.47144198417664,0.006638321068541665
76577,153155,0,153155,131.61313796043396,0.00666050710470802
76677,153355,0,153355,131.7515001296997,0.006681896805822162
76777,153555,0,153555,131.8924651145935,0.006696350528726327
76877,153755,0,153755,132.0319311618805,0.0067001831171035675
76977,153955,0,153955,132.17081594467163,0.0066924951361885116
77077,154155,0,154155,132.30967092514038,0.006674730594359985
77177,154355,0,154355,132.45038318634033,0.006650244157891902
77277,154555,0,154555,132.59141302108765,0.0066237300386648235
77377,154755,0,154755,132.730544090271,0.006599995913297083
77477,154955,0,154955,132.87072014808655,0.0065821179626207645
77578,155157,0,155157,133.0448341369629,0.006569880636599748
77678,155357,0,155357,133.21061396598816,0.006560369900230933
77778,155557,0,155557,133.37216114997864,0.006549412963816596
77878,155757,0,155757,133.51990604400635,0.006534898622649607
77978,155957,0,155957,133.6829969882965,0.006518202396201701
78078,156157,0,156157,133.84064626693726,0.006503346344703308
78178,156357,0,156357,133.99485111236572,0.006494244861374653
78278,156557,0,156557,134.1360080242157,0.006491961995770056
78378,156757,0,156757,134.27922320365906,0.006493896391631224
78478,156957,0,156957,134.4324071407318,0.006495311502869715
78579,157159,0,157159,134.5813980102539,0.00649189128732712
78679,157359,0,157359,134.7434229850769,0.006481890426976725
78779,157559,0,157559,134.97652006149292,0.00646621042431409
78879,157759,0,157759,135.256902217865,0.0064472093923532625
78979,157959,0,157959,135.4624011516571,0.006427151118644978
79079,158159,0,158159,135.63749194145203,0.0064076356386270905
79179,158359,0,158359,135.82163619995117,0.006390338561238534
79279,158559,0,158559,135.99434614181519,0.006378026697386923
79379,158759,0,158759,136.15573906898499,0.006374354040562347
79479,158959,0,158959,136.31371021270752,0.006381987764305939
79580,159161,0,159161,136.4780011177063,0.006400499533560202
79680,159361,0,159361,136.64591526985168,0.006424634250228352
79780,159561,0,159561,136.81982016563416,0.006447108938133697
79880,159761,0,159761,137.00808310508728,0.0064611995446432055
79980,159961,0,159961,137.14967107772827,0.006463676570429448
80080,160161,0,160161,137.29407405853271,0.006455402007098146
80180,160361,0,160361,137.46699595451355,0.006439537500525273
80280,160561,0,160561,137.61000299453735,0.0064189038214628544
80380,160761,0,160761,137.7492139339447,0.006394550365080233
80480,160961,0,160961,137.89409518241882,0.006366412110291381
80581,161163,0,161163,138.04481720924377,0.00633476790961611
80681,161363,0,161363,138.18306708335876,0.006302652844544775
80781,161563,0,161563,138.32081723213196,0.006273379416846458
80881,161763,0,161763,138.45838809013367,0.006250110339511776
80981,161963,0,161963,138.6232590675354,0.00623428296851125
81081,162163,0,162163,138.78533005714417,0.006225767921737579
81181,162363,0,162363,138.94178318977356,0.0062241374766599305
81281,162563,0,162563,139.09579396247864,0.006229648012739131
81381,162763,0,162763,139.23503994941711,0.006242775916315337
81481,162963,0,162963,139.3761990070343,0.006262545435833627
81582,163165,0,163165,139.54012489318848,0.006285415471730391
81682,163365,0,163365,139.69847297668457,0.006304797167929721
81782,163565,0,163565,139.84699606895447,0.006314784332886062
81882,163765,0,163765,140.04001808166504,0.006311769696584767
81982,163965,0,163965,140.20177006721497,0.006295885385802326
82082,164165,0,164165,140.37134790420532,0.006270414604406458
82182,164365,0,164365,140.52130722999573,0.0062401539050176945
82282,164565,0,164565,140.67409205436707,0.006209843169198895
82382,164765,0,164765,140.8453402519226,0.006183248415187983
82482,164965,0,164965,141.07239198684692,0.006162774478480729
82583,165167,0,165167,141.23631620407104,0.006149160457764209
82683,165367,0,165367,141.38991689682007,0.006141860684657694
82783,165567,0,165567,141.52978515625,0.0061385579843668825
82883,165767,0,165767,141.7024929523468,0.006136649170444279
82983,165967,0,165967,141.8738832473755,0.006134281681145008
83083,166167,0,166167,142.02905011177063,0.006131269071756184
83183,166367,0,166367,142.21356797218323,0.006129075679639593
83283,166567,0,166567,142.3719961643219,0.006129684572197447
83383,166767,0,166767,142.52038097381592,0.0061338914443654
83483,166967,0,166967,142.67695903778076,0.006140086056369522
83584,167169,0,167169,142.88066506385803,0.0061444197967707405
83684,167369,0,167369,143.07481026649475,0.006142181329987699
83784,167569,0,167569,143.23552417755127,0.006130154332257758
83884,167769,0,167769,143.39515495300293,0.0061077195472763225
83984,167969,0,167969,143.55051708221436,0.006076980668892908
84084,168169,0,168169,143.7028350830078,0.006041784508410828
84184,168369,0,168369,143.86478424072266,0.006006468607677769
84284,168569,0,168569,144.02810287475586,0.005974995922252405
84384,168769,0,168769,144.1792929172516,0.005950567818914391
84484,168969,0,168969,144.33288598060608,0.0059353837950796755
84585,169171,0,169171,144.48845100402832,0.005930319703752788
84685,169371,0,169371,144.69210124015808,0.005934749306204196
84785,169571,0,169571,145.14393019676208,0.005946302601364465
84885,169771,0,169771,145.33721804618835,0.005961595824236312
84985,169971,0,169971,145.60494017601013,0.005976809021279678
85085,170171,0,170171,145.81905794143677,0.005988450289491664
85185,170371,0,170371,146.0904290676117,0.005994009929550721
85285,170571,0,170571,146.26588106155396,0.005992288842454574
85385,170771,0,170771,146.40731120109558,0.005983319956613796
85485,170971,0,170971,146.55114912986755,0.005968047788046652
85586,171173,0,171173,146.72802305221558,0.0059478151662689565
85686,171373,0,171373,146.876718044281,0.0059250600803017655
85786,171573,0,171573,147.02845001220703,0.005901958853229086
85886,171773,0,171773,147.1973090171814,0.005880965149342974
85986,171973,0,171973,147.38454818725586,0.00586427969826137
86086,172173,0,172173,147.54360604286194,0.0058535228034056865
86186,172373,0,172373,147.68598914146423,0.005849545555644804
86286,172573,0,172573,147.84255695343018,0.005852347583971968
86386,172773,0,172773,148.01929807662964,0.005860998555274079
86486,172973,0,172973,148.25293707847595,0.005873583691386906
86587,173175,0,173175,148.49322509765625,0.005887486514964398
86687,173375,0,173375,148.6401720046997,0.005899302629644569
86787,173575,0,173575,148.78002524375916,0.005906398532051152
86887,173775,0,173775,148.96458506584167,0.005906905322535014
86987,173975,0,173975,149.1176860332489,0.005900095205211705
87087,174175,0,174175,149.26267313957214,0.005886322665121651
87187,174375,0,174375,149.40297603607178,0.005866832461069674
87287,174575,0,174575,149.5926010608673,0.005843543259147396
87387,174775,0,174775,149.73688292503357,0.005818807354050644
87487,174975,0,174975,149.8978669643402,0.005795134065922443
87588,175177,0,175177,150.12226819992065,0.005774751563722394
87688,175377,0,175377,150.394033908844,0.0057602003714983105
87788,175577,0,175577,150.58864903450012,0.005752966287897469
87888,175777,0,175777,150.73771023750305,0.005754167029551253
87988,175977,0,175977,150.87875819206238,0.0057640217618467925
88088,176177,0,176177,151.01744103431702,0.0057815269173186225
88188,176377,0,176377,151.17997908592224,0.005804336891111161
88288,176577,0,176577,151.35213017463684,0.005828980776768374
88388,176777,0,176777,151.50598406791687,0.005851350362460072
88488,176977,0,176977,151.78775095939636,0.005867315913916857
88589,177179,0,177179,152.01539611816406,0.005873408181646214
88689,177379,0,177379,152.2049651145935,0.00586740827161925
88789,177579,0,177579,152.4389510154724,0.005849364703384342
88889,177779,0,177779,152.59921312332153,0.005821421115083074
88989,177979,0,177979,152.92333507537842,0.005787459836572886
89089,178179,0,178179,153.20737504959106,0.005752011836838357
89189,178379,0,178379,153.48292112350464,0.005718976874847321
89289,178579,0,178579,153.75070595741272,0.0056907436376041716
89389,178779,0,178779,153.97585201263428,0.005668112818975281
89489,178979,0,178979,154.20731019973755,0.005650983102685955
89590,179181,0,179181,154.36929202079773,0.005639235496334816
89690,179381,0,179381,154.53982710838318,0.005633765057962033
89790,179581,0,179581,154.72615098953247,0.0056355897122020255
89890,179781,0,179781,154.9044361114502,0.005645426708772222
89990,179981,0,179981,155.08114624023438,0.00566236652004075
90090,180181,0,180181,155.26510906219482,0.005683207262295265
90190,180381,0,180381,155.43416118621826,0.005702830823730916
90290,180581,0,180581,155.63620615005493,0.005715545795336341
90390,180781,0,180781,155.8432161808014,0.005716761601732068
90490,180981,0,180981,156.04499316215515,0.0057042531501076375
90591,181183,0,181183,156.23493814468384,0.005678325070470195
90691,181383,0,181383,156.44260001182556,0.005642756741327904
90791,181583,0,181583,156.7292160987854,0.005602528721144498
90891,181783,0,181783,156.92201900482178,0.005563790593965239
90991,181983,0,181983,157.10352993011475,0.005532504653793147
91091,182183,0,182183,157.3036549091339,0.0055131895395466824
91191,182383,0,182383,157.6586492061615,0.005507874513499617
91291,182583,0,182583,157.8646101951599,0.0055156575671707645
91391,182783,0,182783,158.12575912475586,0.005533086733695801
91491,182983,0,182983,158.32921504974365,0.00555522504307542
91592,183185,0,183185,158.48205709457397,0.005577163947456304
91692,183385,0,183385,158.62151718139648,0.00559424406777221
91792,183585,0,183585,158.7595419883728,0.00560399156664209
91892,183785,0,183785,158.92972207069397,0.005605229242751816
91992,183985,0,183985,159.08741402626038,0.0055980204747261425
92092,184185,0,184185,159.25258111953735,0.0055833057392780695
92192,184385,0,184385,159.4234402179718,0.0055626118043588775
92292,184585,0,184585,159.5635120868683,0.005537850435101692
92392,184785,0,184785,159.7730791568756,0.005511150727121902
92492,184985,0,184985,159.91712617874146,0.005484685936412427
92593,185187,0,185187,160.05698609352112,0.0054602780189395425
92693,185387,0,185387,160.19417119026184,0.005440197267207892
92793,185587,0,185587,160.3327281475067,0.0054255769176267945
92893,185787,0,185787,160.49437999725342,0.005417333941815742
92993,185987,0,185987,160.78686809539795,0.005415787020576368
93093,186187,0,186187,160.99368906021118,0.005420460680598427
93193,186387,0,186387,161.13362407684326,0.0054298802582267965
93293,186587,0,186587,161.28353714942932,0.005441541401328151
93393,186787,0,186787,161.4314272403717,0.005452245605063026
93493,186987,0,186987,161.57231998443604,0.0054588226864056835
93594,187189,0,187189,161.7124810218811,0.005458984020522355
93694,187389,0,187389,161.85217308998108,0.00545207683244265
93794,187589,0,187589,162.00004601478577,0.005439266584452467
93894,187789,0,187789,162.1392891407013,0.005422988570335444
93994,187989,0,187989,162.27852606773376,0.005406109251133636
94094,188189,0,188189,162.41775798797607,0.005391042041647015
94194,188389,0,188389,162.59652996063232,0.005379224946806167
94294,188589,0,188589,162.90755414962769,0.005371072419949242
94394,188789,0,188789,163.12249493598938,0.005366241645813789
94494,188989,0,188989,163.36865997314453,0.005363978531556854
94595,189191,0,189191,163.62149930000305,0.0053634302585765774
94695,189391,0,189391,163.82281494140625,0.005363942159532877
94795,189591,0,189591,163.9790711402893,0.005365289784470807
94895,189791,0,189791,164.14393496513367,0.0053677573027863705
94995,189991,0,189991,164.30167412757874,0.005371757729534558
95095,190191,0,190191,164.4682490825653,0.005377068704725491
95195,190391,0,190391,164.63850712776184,0.005382109528850887
95295,190591,0,190591,164.8021628856659,0.00538391401878397
95395,190791,0,190791,164.9569342136383,0.005379133902557709
95495,190991,0,190991,165.11231589317322,0.00536569300449913
95596,191193,0,191193,165.25974416732788,0.005343916411313316
95696,191393,0,191393,165.4378261566162,0.005317724918407336
95796,191593,0,191593,165.58636212348938,0.005292123112114019
95896,191793,0,191793,165.77669310569763,0.005272013856169165
95996,191993,0,191993,165.94322729110718,0.005260215581759211
96096,192193,0,192193,166.11901807785034,0.005256712561439429
96196,192393,0,192393,166.33648800849915,0.005259182730322118
96296,192593,0,192593,166.50023102760315,0.005264330145209936
96396,192793,0,192793,166.65622305870056,0.005269261276951765
96496,192993,0,192993,166.82237911224365,0.005272343481352476
96597,193195,0,193195,167.02314019203186,0.005273385547420351
96697,193395,0,193395,167.34566712379456,0.0052732479417374085
96797,193595,0,193595,167.56524395942688,0.005273179784124477
96897,193795,0,193795,167.7676990032196,0.005273944186596878
96997,193995,0,193995,167.9272301197052,0.00527515241631857
97097,194195,0,194195,168.0821681022644,0.005275011084452454
97197,194395,0,194395,168.23834609985352,0.005270773753736013
97297,194595,0,194595,168.39846920967102,0.005259911846164433
97397,194795,0,194795,168.54546904563904,0.0052415800118470295
97497,194995,0,194995,168.7054169178009,0.00521761165427835
97598,195197,0,195197,168.86825299263,0.005192118958281517
97698,195397,0,195397,169.0228090286255,0.005171088175595341
97798,195597,0,195597,169.1705961227417,0.005158694724669456
97898,195797,0,195797,169.31563711166382,0.0051567222851413505
97998,195997,0,195997,169.45689511299133,0.005163904989248781
98098,196197,0,196197,169.59504890441895,0.005176779088487519
98198,196397,0,196397,169.75076913833618,0.005191127951658085
98298,196597,0,196597,169.8930959701538,0.005203257664675528
98398,196797,0,196797,170.1253740787506,0.00521072285287811
98498,196997,0,196997,170.42989492416382,0.005212539288863898
98599,197199,0,197199,170.62508487701416,0.005209005424576518
98699,197399,0,197399,170.77376890182495,0.005201539048528845
98799,197599,0,197599,170.91800713539124,0.00519184917138891
98899,197799,0,197799,171.05900692939758,0.005181312289746743
98999,197999,0,197999,171.19666624069214,0.00517041114718528
99099,198199,0,198199,171.34251308441162,0.005158709458079069
99199,198399,0,198399,171.50559425354004,0.005145468263441513
99299,198599,0,198599,171.66608119010925,0.00513058545292794
99399,198799,0,198799,171.8084740638733,0.0051152403326529565
99499,198999,0,198999,171.94865798950195,0.005101733863730263
99600,199201,0,199201,172.10014605522156,0.005092447789663876
99700,199401,0,199401,172.2924690246582,0.005088920921608587
99800,199601,0,199601,172.4439182281494,0.0050905507120880406
99900,199801,0,199801,172.5864770412445,0.005095285694376357
100000,200001,0,200001,172.79732203483582,0.005100546728053584


==> plot_data/quadratic_minimax_problem_n500_alpha0/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0037419795989990234,30.358099469249375
100,201,200,401,0.6152091026306152,1.725251134601807
200,401,400,801,1.028996229171753,1.0331394156994131
300,601,600,1201,1.2279770374298096,0.7736231354158138
400,801,800,1601,1.394481897354126,0.6349280372139878
501,1003,1002,2005,1.8395888805389404,0.5455617951375803
601,1203,1202,2405,2.2045671939849854,0.482543795209007
701,1403,1402,2805,2.436816930770874,0.43443121283005004
801,1603,1602,3205,2.588085174560547,0.396082748791271
901,1803,1802,3605,2.751868963241577,0.3645989873004372
1001,2003,2002,4005,3.0397660732269287,0.33817775845833975
1101,2203,2202,4405,3.3105008602142334,0.31561971894335344
1201,2403,2402,4805,3.6442410945892334,0.29608763453723413
1301,2603,2602,5205,4.038995981216431,0.2789761387097555
1401,2803,2802,5605,4.247813940048218,0.26383524354104326
1502,3005,3004,6009,4.472510099411011,0.25019483089933037
1602,3205,3204,6409,4.753228187561035,0.23805758726442536
1702,3405,3404,6809,5.428587198257446,0.22707177793944233
1802,3605,3604,7209,6.1581199169158936,0.21706993619439596
1902,3805,3804,7609,6.853977918624878,0.20791616240763086
2002,4005,4004,8009,7.264842987060547,0.19949893614020578
2102,4205,4204,8409,7.922374963760376,0.19172585568559014
2202,4405,4404,8809,8.343006134033203,0.18451971692199934
2302,4605,4604,9209,8.539321184158325,0.17781553946480064
2402,4805,4804,9609,8.701730251312256,0.1715582748285912
2503,5007,5006,10013,8.91798210144043,0.16564432077061936
2603,5207,5206,10413,9.178969860076904,0.16015029105088846
2703,5407,5406,10813,9.39064908027649,0.1549811510589118
2803,5607,5606,11213,9.610925197601318,0.15010700224205265
2903,5807,5806,11613,9.802758932113647,0.14550185344186578
3003,6007,6006,12013,9.96560001373291,0.14114300673996125
3103,6207,6206,12413,10.309340953826904,0.13701055044944
3203,6407,6406,12813,10.62016487121582,0.1330869385687235
3303,6607,6606,13213,11.005867004394531,0.12935664054963755
3403,6807,6806,13613,11.699689149856567,0.12580584861601082
3504,7009,7008,14017,11.944730043411255,0.12238920212160206
3604,7209,7208,14417,12.129282236099243,0.11916321177975675
3704,7409,7408,14817,12.29698896408081,0.11608328196435345
3804,7609,7608,15217,12.449980974197388,0.11314041075772609
3904,7809,7808,15617,12.792578220367432,0.11032642169640298
4004,8009,8008,16017,13.281550884246826,0.10763385857735135
4104,8209,8208,16417,13.531161069869995,0.10505589601363031
4204,8409,8408,16817,13.736955881118774,0.1025862632084499
4304,8609,8608,17217,13.935287237167358,0.10021917884265644
4404,8809,8808,17617,14.59101128578186,0.09794929532145866
4505,9011,9010,18021,15.107478141784668,0.09575032438778178
4605,9211,9210,18421,15.363562107086182,0.09366115602452446
4705,9411,9410,18821,15.621525049209595,0.09165526018334968
4805,9611,9610,19221,15.808576107025146,0.08972860996649396
4905,9811,9810,19621,15.959172248840332,0.08787742990858095
5005,10011,10010,20021,16.144999027252197,0.08609817276901403
5105,10211,10210,20421,16.308143138885498,0.08438749926429683
5205,10411,10410,20821,16.453359127044678,0.0827422603099926
5305,10611,10610,21221,16.64315915107727,0.08115948140902517
5405,10811,10810,21621,16.796471118927002,0.07963634887915819
5506,11013,11012,22025,16.942965030670166,0.07815581524163809
5606,11213,11212,22425,17.1023108959198,0.07674465027683981
5706,11413,11412,22825,17.32118511199951,0.07538551682251976
5806,11613,11612,23225,17.46513795852661,0.07407613635346144
5906,11813,11812,23625,17.635382175445557,0.07281434196761298
6006,12013,12012,24025,17.80742621421814,0.07159807137914267
6106,12213,12212,24425,17.979685068130493,0.07042536057263304
6206,12413,12412,24825,18.182366132736206,0.06929433803403764
6306,12613,12612,25225,18.34694814682007,0.06820321948612608
6406,12813,12812,25625,18.50256109237671,0.06715030306641073
6507,13015,13014,26029,18.724119186401367,0.06612398092841468
6607,13215,13214,26429,18.88314199447632,0.06514301371111987
6707,13415,13414,26829,19.038422107696533,0.06419558041511696
6807,13615,13614,27229,19.20353102684021,0.0632802683993876
6907,13815,13814,27629,19.369935989379883,0.062395728307350413
7007,14015,14014,28029,19.5279700756073,0.06154067100873571
7107,14215,14214,28429,19.70085310935974,0.06071386473424732
7207,14415,14414,28829,20.188430070877075,0.05991413238392325
7307,14615,14614,29229,20.510123014450073,0.059140348992611
7407,14815,14814,29629,20.699604034423828,0.05839143933812523
7508,15017,15016,30033,20.86083197593689,0.05765924210431666
7608,15217,15216,30433,21.08720588684082,0.056957265862180737
7708,15417,15416,30833,21.25450086593628,0.056277204937750555
7808,15617,15616,31233,21.448886156082153,0.055618162011791754
7908,15817,15816,31633,21.624284029006958,0.05497927928204562
8008,16017,16016,32033,21.80279302597046,0.05435973671268472
8108,16217,16216,32433,21.985504150390625,0.05375875036499129
8208,16417,16416,32833,22.23034906387329,0.05317557080411595
8308,16617,16616,33233,22.419522047042847,0.05260948157732764
8408,16817,16816,33633,22.624991178512573,0.05205979775965061
8509,17019,17018,34037,22.838798999786377,0.051520602630384243
8609,17219,17218,34437,23.037046194076538,0.05100194225340503
8709,17419,17418,34837,23.212181091308594,0.05049780221954439
8809,17619,17618,35237,23.375786066055298,0.05000761065391924
8909,17819,17818,35637,23.553126096725464,0.04953082081910589
9009,18019,18018,36037,23.73436188697815,0.0490669099988507
9109,18219,18218,36437,23.980046272277832,0.04861537842924969
9209,18419,18418,36837,24.19733715057373,0.04817574827537324
9309,18619,18618,37237,24.432120084762573,0.04774756265143859
9409,18819,18818,37637,24.64034414291382,0.047330384682744496
9510,19021,19020,38041,24.84428596496582,0.046919782839293905
9610,19221,19220,38441,24.995235204696655,0.04652348509582251
9710,19421,19420,38841,25.165574073791504,0.04613699192550532
9810,19621,19620,39241,25.34954810142517,0.045759938057866614
9910,19821,19820,39641,25.5351402759552,0.04539197410606611
10010,20021,20020,40041,25.735128164291382,0.04503276584703184
10110,20221,20220,40441,25.914966106414795,0.04468199353306405
10210,20421,20420,40841,26.103564023971558,0.044339351233674364
10310,20621,20620,41241,26.24663805961609,0.04400454620646485
10410,20821,20820,41641,26.401906967163086,0.04367729829589823
10511,21023,21022,42045,26.557806253433228,0.043354175700984134
10611,21223,21222,42445,26.75298309326172,0.04304131812212202
10711,21423,21422,42845,26.902826070785522,0.042735244693531745
10811,21623,21622,43245,27.04931902885437,0.042435720216392636
10911,21823,21822,43645,27.215392112731934,0.04214251944861459
11011,22023,22022,44045,27.371469259262085,0.04185542664905385
11111,22223,22222,44445,27.51691198348999,0.04157423514255881
11211,22423,22422,44845,27.661495208740234,0.04129874690496824
11311,22623,22622,45245,27.813106060028076,0.04102877216721476
11411,22823,22822,45645,28.008168935775757,0.04076412903771575
11512,23025,23024,46049,28.279133081436157,0.04050207375577833
11612,23225,23224,46449,28.55593705177307,0.04024762697357275
11712,23425,23424,46849,28.81803607940674,0.03999800830159963
11812,23625,23624,47249,29.09761118888855,0.0397530639846592
11912,23825,23824,47649,29.34407091140747,0.0395126465017495
12012,24025,24024,48049,29.562677145004272,0.039276614282708754
12112,24225,24224,48449,29.81929612159729,0.03904483143818287
12212,24425,24424,48849,30.072418212890625,0.03881716750231484
12312,24625,24624,49249,30.265833139419556,0.038593497187575036
12412,24825,24824,49649,30.415390014648438,0.03837370015117433
12513,25027,25026,50053,30.56013298034668,0.03815551897529549
12613,25227,25226,50453,30.703999996185303,0.037943162063118596
12713,25427,25426,50853,30.847543239593506,0.0377343438492354
12813,25627,25626,51253,31.005712032318115,0.03752896168757155
12913,25827,25826,51653,31.184603929519653,0.03732691686285719
13013,26027,26026,52053,31.44921088218689,0.03712811441614046
13113,26227,26226,52453,31.815949201583862,0.03693246297857628
13213,26427,26426,52853,32.107585191726685,0.03673987461309662
13313,26627,26626,53253,32.28674101829529,0.03655026466358583
13413,26827,26826,53653,32.45838022232056,0.036363551611200175
13514,27029,27028,54057,32.650519132614136,0.036177831965269316
13614,27229,27228,54457,32.82671904563904,0.03599670707644524
13714,27429,27428,54857,32.99233913421631,0.035818251299561545
13814,27629,27628,55257,33.160670042037964,0.035642394384972687
13914,27829,27828,55657,33.32263898849487,0.03546906859650301
14014,28029,28028,56057,33.50303792953491,0.035298208604007716
14114,28229,28228,56457,33.66260313987732,0.03512975138098166
14214,28429,28428,56857,33.80476713180542,0.034963636106970473
14314,28629,28628,57257,33.94815492630005,0.03479980407454928
14414,28829,28828,57657,34.091044902801514,0.034638198600647346
14515,29031,29030,58061,34.342962980270386,0.0344771813926357
14615,29231,29230,58461,34.66441607475281,0.03431988759353739
14715,29431,29430,58861,34.87676501274109,0.034164661121646143
14815,29631,29630,59261,35.043591022491455,0.03401145260098112
14915,29831,29830,59661,35.22201204299927,0.03386021429396292
15015,30031,30030,60061,35.485605001449585,0.03371090003473227
15115,30231,30230,60461,35.73064088821411,0.033563465165527585
15215,30431,30430,60861,35.952505111694336,0.03341786647597316
15315,30631,30630,61261,36.15373492240906,0.033274062145135605
15415,30831,30830,61661,36.43344306945801,0.03313201168621398
15516,31033,31032,62065,36.6370792388916,0.03299028106538275
15616,31233,31232,62465,36.8351628780365,0.032851638543969136
15716,31433,31432,62865,37.080663204193115,0.03271463556051868
15816,31633,31632,63265,37.40368914604187,0.03257923647112261
15916,31833,31832,63665,37.75725221633911,0.032445406724262195
16016,32033,32032,64065,38.15865516662598,0.03231311281884127
16116,32233,32232,64465,38.488017082214355,0.03218232226407853
16216,32433,32432,64865,38.85329794883728,0.032053003541169474
16316,32633,32632,65265,39.061028242111206,0.03192512606663327
16416,32833,32832,65665,39.484559059143066,0.031798660157263375
16517,33035,33034,66069,39.90658903121948,0.03167233305252099
16617,33235,33234,66469,40.254624128341675,0.031548618067915195
16717,33435,33434,66869,40.59261918067932,0.03142623040467131
16817,33635,33634,67269,40.807466983795166,0.031305143667268095
16917,33835,33834,67669,41.002110958099365,0.031185332206444923
17017,34035,34034,68069,41.17033100128174,0.031066771092305608
17117,34235,34234,68469,41.34957695007324,0.030949436088563275
17217,34435,34434,68869,41.519410133361816,0.030833303627871574
17317,34635,34634,69269,41.685863971710205,0.03071835078819308
17417,34835,34834,69669,41.932295083999634,0.030604555270155195
17518,35037,35036,70073,42.11677122116089,0.03049077443936755
17618,35237,35236,70473,42.27711009979248,0.030379240089852988
17718,35437,35436,70873,42.438425064086914,0.030268799484460148
17818,35637,35636,71273,42.68152403831482,0.030159432611547094
17918,35837,35836,71673,43.008729219436646,0.030051119982023665
18018,36037,36036,72073,43.257230281829834,0.029943842611752463
18118,36237,36236,72473,43.41159105300903,0.029837582004660062
18218,36437,36436,72873,43.55804491043091,0.029732320136525433
18318,36637,36636,73273,43.7017879486084,0.029628039439415943
18418,36837,36836,73673,43.85853910446167,0.02952472278674026
18519,37039,37038,74077,44.00399589538574,0.029421334514460707
18619,37239,37238,74477,44.16084408760071,0.029319905494727717
18719,37439,37438,74877,44.32167100906372,0.029219391490043062
18819,37639,37638,75277,44.465888023376465,0.02911977700493755
18919,37839,37838,75677,44.69952321052551,0.0290210469187723
19019,38039,38038,76077,44.908053159713745,0.028923186473965537
19119,38239,38238,76477,45.159136056900024,0.028826181264669258
19219,38439,38438,76877,45.319172859191895,0.028730017225875572
19319,38639,38638,77277,45.68703317642212,0.028634680622934186
19419,38839,38838,77677,45.845000982284546,0.02854015804146322
19520,39041,39040,78081,45.9970281124115,0.028445503162067013
19620,39241,39240,78481,46.141364097595215,0.028352577430754568
19720,39441,39440,78881,46.31768202781677,0.028260427180378078
19820,39641,39640,79281,46.72365212440491,0.028169040186821117
19920,39841,39840,79681,47.10638213157654,0.028078404501042573
20020,40041,40040,80081,47.27374505996704,0.02798850844102124
20120,40241,40240,80481,47.4262490272522,0.027899340583990836
20220,40441,40440,80881,47.5725781917572,0.027810889758952812
20320,40641,40640,81281,47.72615194320679,0.0277231450394556
20420,40841,40840,81681,47.894585847854614,0.027636095736629403
20521,41043,41042,82085,48.04158115386963,0.02754887117325509
20621,41243,41242,82485,48.22660207748413,0.02746318825043482
20721,41443,41442,82885,48.47253894805908,0.027378169938052893
20821,41643,41642,83285,48.65586590766907,0.02729380643475468
20921,41843,41842,83685,48.833433866500854,0.027210088145362795
21021,42043,42042,84085,49.08260798454285,0.027127005675241785
21121,42243,42242,84485,49.2607319355011,0.02704454982485341
21221,42443,42442,84885,49.50607490539551,0.026962711584495463
21321,42643,42642,85285,49.858986139297485,0.02688148212921685
21421,42843,42842,85685,50.1140251159668,0.02680085281390182
21522,43045,43044,86089,50.40891408920288,0.026720017751774044
21622,43245,43244,86489,50.6812949180603,0.026640569269127282
21722,43445,43444,86889,50.86413908004761,0.026561695942841326
21822,43645,43644,87289,51.03327012062073,0.026483389802738927
21922,43845,43844,87689,51.202797174453735,0.026405643036174768
22022,44045,44044,88089,51.3668110370636,0.02632844798400672
22122,44245,44244,88489,51.52278113365173,0.026251797136695613
22222,44445,44444,88889,51.688621044158936,0.0261756831305289
22322,44645,44644,89289,51.860565185546875,0.026100098743962265
22422,44845,44844,89689,52.01291513442993,0.026025036894076908
22523,45047,45046,90093,52.159534215927124,0.025949747751090577
22623,45247,45246,90493,52.30336594581604,0.025875715317000777
22723,45447,45446,90893,52.44973802566528,0.025802184902548382
22823,45647,45646,91293,52.67300510406494,0.025729149947264905
22923,45847,45846,91693,52.82845401763916,0.02565660401313399
23023,46047,46046,92093,53.11584806442261,0.025584540781652128
23123,46247,46246,92493,53.38273215293884,0.02551295405097718
23223,46447,46446,92893,53.53171992301941,0.025441837733162487
23323,46647,46646,93293,53.7332329750061,0.025371185851471904
23423,46847,46846,93693,53.93876791000366,0.025300992537774306
23524,47049,47048,94097,54.08831596374512,0.025230556892376153
23624,47249,47248,94497,54.24022316932678,0.025161267975363354
23724,47449,47448,94897,54.40405988693237,0.025092420593584127
23824,47649,47648,95297,54.57792592048645,0.025024009289734053
23924,47849,47848,95697,54.75172805786133,0.02495602870315468
24024,48049,48048,96097,54.917155265808105,0.024888473567647323
24124,48249,48248,96497,55.09845519065857,0.02482133870934882
24224,48449,48448,96897,55.26069092750549,0.02475461904466623
24324,48649,48648,97297,55.41267013549805,0.024688309578270222
24424,48849,48848,97697,55.56258416175842,0.024622405401142206
24525,49051,49050,98101,55.73962926864624,0.024556248657786196
24625,49251,49250,98501,55.897125005722046,0.024491144601499665
24725,49451,49450,98901,56.04494595527649,0.024426431560359774
24825,49651,49650,99301,56.1893310546875,0.02436210495290391
24925,49851,49850,99701,56.333317041397095,0.024298160274975812
25025,50051,50050,100101,56.48233723640442,0.02423459309807016
25125,50251,50250,100501,56.63387203216553,0.024171399067722248
25225,50451,50450,100901,56.802316188812256,0.024108573901939583
25325,50651,50650,101301,56.94934892654419,0.024046113389674717
25425,50851,50850,101701,57.092865228652954,0.023984013389337876
25526,51053,51052,102105,57.250208139419556,0.02392165417812958
25626,51253,51252,102505,57.431265115737915,0.02386026655180488
25726,51453,51452,102905,57.58782505989075,0.023799227375991334
25826,51653,51652,103305,57.751834869384766,0.023738532773443066
25926,51853,51852,103705,57.90252184867859,0.023678178929477357
26026,52053,52052,104105,58.05001091957092,0.023618162090702013
26126,52253,52252,104505,58.19573211669922,0.023558478563774094
26226,52453,52452,104905,58.33688306808472,0.023499124714190127
26326,52653,52652,105305,58.48480701446533,0.02344009696510563
26426,52853,52852,105705,58.62689805030823,0.023381391796184488
26527,53055,53054,106109,58.77273106575012,0.02332242348188586
26627,53255,53254,106509,58.917301177978516,0.023264356272731823
26727,53455,53454,106909,59.063897132873535,0.023206601377380873
26827,53655,53654,107309,59.20615816116333,0.02314915549108807
26927,53855,53854,107709,59.359869956970215,0.023092015360258213
27027,54055,54054,108109,59.51687407493591,0.023035177781452802
27127,54255,54254,108509,59.658894062042236,0.02297863960041945
27227,54455,54454,108909,59.802566051483154,0.0229223977111454
27327,54655,54654,109309,59.951048135757446,0.02286644905493228
27427,54855,54854,109709,60.10778617858887,0.02281079061949307
27528,55057,55056,110113,60.29968214035034,0.022754867166964565
27628,55257,55256,110513,60.4557671546936,0.02269978314617838
27728,55457,55456,110913,60.59699106216431,0.02264498055048805
27828,55657,55656,111313,60.74193811416626,0.02259045654505676
27928,55857,55856,111713,60.88277792930603,0.02253620833723805
28028,56057,56056,112113,61.02861404418945,0.022482233175790744
28128,56257,56256,112513,61.17051291465759,0.02242852835011063
28228,56457,56456,112913,61.31932711601257,0.022375091189480067
28328,56657,56656,113313,61.46492910385132,0.022321919062333745
28428,56857,56856,113713,61.62556290626526,0.022269009375541767
28529,57059,57058,114117,61.768800020217896,0.022215834379556394
28629,57259,57258,114517,61.969677209854126,0.02216344450540145
28729,57459,57458,114917,62.21535396575928,0.022111309491241765
28829,57659,57658,115317,62.424741983413696,0.022059426891176334
28929,57859,57858,115717,62.682064056396484,0.02200779429437483
29029,58059,58058,116117,62.91287708282471,0.021956409324448933
29129,58259,58258,116517,63.0688898563385,0.021905269638837623
29229,58459,58458,116917,63.27750897407532,0.021854372928205596
29329,58659,58658,117317,63.65252614021301,0.021803716915854494
29429,58859,58858,117717,63.851418018341064,0.021753299357146268
29530,59061,59060,118121,64.0942542552948,0.021702617411362677
29630,59261,59260,118521,64.40037894248962,0.02165267248112565
29730,59461,59460,118921,64.74671006202698,0.021602959436031792
29830,59661,59660,119321,65.03890585899353,0.02155347615445676
29930,59861,59860,119721,65.28599500656128,0.021504220544126505
30030,60061,60060,120121,65.58523917198181,0.021455190541609447
30130,60261,60260,120521,65.9805920124054,0.021406384111819585
30230,60461,60460,120921,66.50212907791138,0.021357799247529348
30330,60661,60660,121321,67.05316615104675,0.02130943396889251
30430,60861,60860,121721,67.57220792770386,0.02126128632297706
30531,61063,61062,122125,68.07628107070923,0.021212876146774994
30631,61263,61262,122525,68.29045009613037,0.02116516014142918
30731,61463,61462,122925,68.5170350074768,0.021117656048338717
30831,61663,61662,123325,68.6888370513916,0.02107036201798955
30931,61863,61862,123725,68.84888505935669,0.021023276225578362
31031,62063,62062,124125,69.01636719703674,0.020976396870598997
31131,62263,62262,124525,69.53290295600891,0.020929722176436568
31231,62463,62462,124925,69.74815392494202,0.02088325038997014
31331,62663,62662,125325,69.90891909599304,0.020836979781182922
31431,62863,62862,125725,70.06239008903503,0.020790908642780062
31532,63065,63064,126129,70.20825004577637,0.020744577549456095
31632,63265,63264,126529,70.38369798660278,0.02069890227185976
31732,63465,63464,126929,70.54967617988586,0.020653421459079477
31832,63665,63664,127329,70.73506999015808,0.020608133491244754
31932,63865,63864,127729,70.91125416755676,0.020563036769401223
32032,64065,64064,128129,71.09860301017761,0.020518129715171387
32132,64265,64264,128529,71.24775719642639,0.02047341077042082
32232,64465,64464,128929,71.41112923622131,0.02042887839693129
32332,64665,64664,129329,71.59334421157837,0.020384531076080074
32432,64865,64864,129729,71.7517409324646,0.020340367308525002
32533,65067,65066,130133,71.91094517707825,0.020295946711456982
32633,65267,65266,130533,72.08745098114014,0.0202521474268461
32733,65467,65466,130933,72.23667907714844,0.020208527295788953
32833,65667,65666,131333,72.45071315765381,0.02016508489321509
32933,65867,65866,131733,72.67786812782288,0.020121818811844584
33033,66067,66066,132133,72.91870903968811,0.020078727661907103
33133,66267,66266,132533,73.06122922897339,0.020035810070866345
33233,66467,66466,132933,73.20446109771729,0.019993064683148747
33333,66667,66666,133333,73.34752917289734,0.019950490159878407
33433,66867,66866,133733,73.50932621955872,0.01990808517861562
33534,67069,67068,134137,73.65241503715515,0.01986542691085773
33634,67269,67268,134537,73.79404616355896,0.019823358773752874
33734,67469,67468,134937,73.9540650844574,0.019781456294749658
33834,67669,67668,135337,74.09579014778137,0.01973971821479264
33934,67869,67868,135737,74.23839116096497,0.01969814329002546
34034,68069,68068,136137,74.40338587760925,0.01965673029155704
34134,68269,68268,136537,74.64577317237854,0.019615478005232466
34234,68469,68468,136937,74.83617305755615,0.01957438523140732
34334,68669,68668,137337,75.01430821418762,0.019533450784726052
34434,68869,68868,137737,75.19437599182129,0.01949267349390492
34535,69071,69070,138141,75.3850929737091,0.019451646772505105
34635,69271,69270,138541,75.57234692573547,0.019411181877591423
34735,69471,69470,138941,75.73530602455139,0.019370870695762887
34835,69671,69670,139341,76.0630931854248,0.019330712110055045
34935,69871,69870,139741,76.54358005523682,0.01929070501654202
35035,70071,70070,140141,77.07055306434631,0.019250848324141225
35135,70271,70270,140541,77.53561615943909,0.019211140954421377
35235,70471,70470,140941,78.10362100601196,0.019171581841413602
35335,70671,70670,141341,78.39099025726318,0.019132169931426305
35435,70871,70870,141741,78.88285303115845,0.019092904182862837
35536,71073,71072,142145,79.32910919189453,0.019053393089335718
35636,71273,71272,142545,79.5004460811615,0.019014418022354724
35736,71473,71472,142945,80.09643411636353,0.018975586052796825
35836,71673,71672,143345,80.63446617126465,0.018936896185798812
35936,71873,71872,143745,81.13734817504883,0.018898347437725855
36036,72073,72072,144145,81.65365409851074,0.018859938836007395
36136,72273,72272,144545,82.12487411499023,0.018821669418975857
36236,72473,72472,144945,82.65082812309265,0.018783538235707962
36336,72673,72672,145345,82.85276818275452,0.018745544345868635
36436,72873,72872,145745,83.01058316230774,0.018707686819558044
36537,73075,73074,146149,83.17037296295166,0.018669588197242667
36637,73275,73274,146549,83.37150406837463,0.018632001990064116
36737,73475,73474,146949,83.59158706665039,0.018594549408885233
36837,73675,73674,147349,83.76536703109741,0.01855722956416187
36937,73875,73874,147749,84.1109709739685,0.01852004157605496
37037,74075,74074,148149,84.52816224098206,0.0184829845742918
37137,74275,74274,148549,84.88972616195679,0.018446057698029945
37237,74475,74474,148949,85.03509306907654,0.01840926009572327
37337,74675,74674,149349,85.1806001663208,0.01837259092499031
37437,74875,74874,149749,85.35110998153687,0.018336049352484656
37538,75077,75076,150153,85.50933623313904,0.01829927104322115
37638,75277,75276,150553,85.87705087661743,0.018262983458128306
37738,75477,75476,150953,86.05156302452087,0.018226821016144038
37838,75677,75676,151353,86.20002794265747,0.018190782918893998
37938,75877,75876,151753,86.36766314506531,0.01815486837642129
38038,76077,76076,152153,86.54233002662659,0.018119076607069226
38138,76277,76276,152553,86.75349521636963,0.018083406837366
38238,76477,76476,152953,86.89756393432617,0.018047858301911218
38338,76677,76676,153353,87.05689001083374,0.018012430243264033
38438,76877,76876,153753,87.20026516914368,0.017977121911833673
38539,77079,77078,154157,87.38330292701721,0.017941581270695787
38639,77279,77278,154557,87.64534401893616,0.017906511354616263
38739,77479,77478,154957,87.89432907104492,0.017871558955778594
38839,77679,77678,155357,88.3599910736084,0.017836723355001523
38939,77879,77878,155757,88.67610311508179,0.017802003840429306
39039,78079,78078,156157,88.99925804138184,0.017767399707431936
39139,78279,78278,156557,89.31689190864563,0.017732910258507373
39239,78479,78478,156957,89.59927725791931,0.01769853480318475
39339,78679,78678,157357,89.76380205154419,0.01766427265792939
39439,78879,78878,157757,89.911141872406,0.017630123146049517
39540,79081,79080,158161,90.08273220062256,0.017595745785285163
39640,79281,79280,158561,90.2271192073822,0.017561820646667444
39740,79481,79480,158961,90.38108491897583,0.017528006144959224
39840,79681,79680,159361,90.53634810447693,0.017494301629998436
39940,79881,79880,159761,90.6774001121521,0.017460706458019143
40040,80081,80080,160161,90.81982803344727,0.017427219991566524
40140,80281,80280,160561,90.97404193878174,0.017393841599413325
40240,80481,80480,160961,91.11889219284058,0.017360570656477215
40340,80681,80680,161361,91.26064491271973,0.017327406543740147
40440,80881,80880,161761,91.40309619903564,0.017294348648168065
40541,81083,81082,162165,91.55879211425781,0.017261067371068674
40641,81283,81282,162565,91.70237803459167,0.017228221141340302
40741,81483,81482,162965,91.86002993583679,0.017195479318873882
40841,81683,81682,163365,92.0263090133667,0.017162841313855037
40941,81883,81882,163765,92.17222309112549,0.017130306542071767
41041,82083,82082,164165,92.3143081665039,0.017097874424841997
41141,82283,82282,164565,92.47436809539795,0.017065544388941797
41241,82483,82482,164965,92.63263487815857,0.01703331586653505
41341,82683,82682,165365,92.84792613983154,0.01700118829510394
41441,82883,82882,165765,93.12865424156189,0.01696916111738057
41542,83085,83084,166169,93.31217789649963,0.016936915010264064
41642,83285,83284,166569,93.47365522384644,0.016905087959018444
41742,83485,83484,166969,93.6231460571289,0.016873359655114786
41842,83685,83684,167369,93.76600813865662,0.016841729561671622
41942,83885,83884,167769,93.90808725357056,0.016810197146730238
42042,84085,84084,168169,94.06002116203308,0.016778761883192207
42142,84285,84284,168569,94.20239400863647,0.016747423248758248
42242,84485,84484,168969,94.34679818153381,0.01671618072586743
42342,84685,84684,169369,94.502934217453,0.016685033801637703
42442,84885,84884,169769,94.65139198303223,0.016653981967807166
42543,85087,85086,170173,94.80828022956848,0.016622715624174927
42643,85287,85286,170573,94.9610800743103,0.016591853402918303
42743,85487,85486,170973,95.10688424110413,0.016561084769496595
42843,85687,85686,171373,95.2484061717987,0.016530409233602147
42943,85887,85886,171773,95.38965511322021,0.01649982630926625
43043,86087,86086,172173,95.54370999336243,0.016469335514805256
43143,86287,86286,172573,95.69015002250671,0.016438936372767995
43243,86487,86486,172973,95.83162713050842,0.016408628409883372
43343,86687,86686,173373,95.98566007614136,0.016378411157009207
43443,86887,86886,173773,96.13035011291504,0.0163482841490817
43544,87089,87088,174177,96.27398204803467,0.016317947004684173
43644,87289,87288,174577,96.41754817962646,0.016287999998496797
43744,87489,87488,174977,96.56966996192932,0.016258141861527946
43844,87689,87688,175377,96.71151494979858,0.01622837214457448
43944,87889,87888,175777,96.8697681427002,0.016198690402268984
44044,88089,88088,176177,97.0287561416626,0.01616909619303347
44144,88289,88288,176577,97.17970705032349,0.016139589079034025
44244,88489,88488,176977,97.34281396865845,0.016110168626135502
44344,88689,88688,177377,97.51295113563538,0.016080834403857398
44444,88889,88888,177777,97.65529298782349,0.016051585985330012
44545,89091,89090,178181,97.8078441619873,0.016022131746618748
44645,89291,89290,178581,97.95734214782715,0.015993054516711416
44745,89491,89490,178981,98.10611009597778,0.015964061827038165
44845,89691,89690,179381,98.24909806251526,0.015935153264782634
44945,89891,89890,179781,98.39956212043762,0.015906328420529737
45045,90091,90090,180181,98.55490803718567,0.015877586888225614
45145,90291,90290,180581,98.701003074646,0.015848928265138035
45245,90491,90490,180981,98.84352898597717,0.015820352151817672
45345,90691,90690,181381,99.0050539970398,0.01579185815205944
45445,90891,90890,181781,99.15490412712097,0.015763445872864972
45546,91093,91092,182185,99.3019630908966,0.01573483202432974
45646,91293,91292,182585,99.45688819885254,0.01570658282740587
45746,91493,91492,182985,99.60717296600342,0.015678414187099022
45846,91693,91692,183385,99.74893498420715,0.015650325722899632
45946,91893,91892,183785,99.89362096786499,0.015622317057323056
46046,92093,92092,184185,100.041983127594,0.015594387815874732
46146,92293,92292,184585,100.18849587440491,0.015566537627016092
46246,92493,92492,184985,100.33146715164185,0.015538766122130529
46346,92693,92692,185385,100.50745606422424,0.01551107293549019
46446,92893,92892,185785,100.65173196792603,0.01548345770422327
46547,93095,93094,186189,100.80931806564331,0.01545564508256718
46647,93295,93294,186589,100.95984601974487,0.015428185455279256
46747,93495,93494,186989,101.10566830635071,0.015400802708031612
46847,93695,93694,187389,101.26279616355896,0.015373496489083502
46947,93895,93894,187789,101.41508793830872,0.015346266449392422
47047,94095,94094,188189,101.56841707229614,0.015319112242583413
47147,94295,94294,188589,101.71161198616028,0.015292033524919778
47247,94495,94494,188989,101.85296702384949,0.015265029955273198
47347,94695,94694,189389,102.00884628295898,0.015238101195095102
47447,94895,94894,189789,102.15328407287598,0.015211246908387922
47548,95097,95096,190193,102.317214012146,0.015184199333494748
47648,95297,95296,190593,102.59435606002808,0.015157493732227002
47748,95497,95496,190993,102.86036419868469,0.015130861608190426
47848,95697,95696,191393,103.0884370803833,0.015104302635337465
47948,95897,95896,191793,103.24170923233032,0.015077816490033957
48048,96097,96096,192193,103.4026050567627,0.015051402851032878
48148,96297,96296,192593,103.55156207084656,0.015025061399448316
48248,96497,96496,192993,103.69479823112488,0.014998791818729911
48348,96697,96696,193393,103.84422516822815,0.014972593794637397
48448,96897,96896,193793,104.00021886825562,0.014946467015215766
48549,97099,97098,194197,104.16743516921997,0.014920150969505643
48649,97299,97298,194597,104.32554721832275,0.014894166457308946
48749,97499,97498,194997,104.46856307983398,0.014868252264343478
48849,97699,97698,195397,104.61175417900085,0.014842408087573906
48949,97899,97898,195797,104.76128220558167,0.014816633626129973
49049,98099,98098,196197,104.92377710342407,0.014790928581283582
49149,98299,98298,196597,105.08374619483948,0.014765292656425929
49249,98499,98498,196997,105.23965287208557,0.014739725557045077
49349,98699,98698,197397,105.39168500900269,0.014714226990703978
49449,98899,98898,197797,105.56291007995605,0.014688796667018477
49550,99101,99100,198201,105.71717715263367,0.014663181016140808
49650,99301,99300,198601,105.89237213134766,0.014637886989959022
49750,99501,99500,199001,106.04707527160645,0.014612660344550686
49850,99701,99700,199401,106.20108199119568,0.014587500797550411
49950,99901,99900,199801,106.38625502586365,0.014562408068540787
50050,100101,100100,200201,106.58542013168335,0.01453738187903176
50150,100301,100300,200601,106.77904915809631,0.014512421952441202
50250,100501,100500,201001,106.95468616485596,0.01448752801407491
50350,100701,100700,201401,107.12670016288757,0.014462699791107488
50450,100901,100900,201801,107.27447199821472,0.014437937012562903
50551,101103,101102,202205,107.42329907417297,0.01441299276149233
50651,101303,101302,202605,107.61627197265625,0.014388360713904908
50751,101503,101502,203005,107.81887602806091,0.014363793306075312
50851,101703,101702,203405,107.99001717567444,0.014339290274256703
50951,101903,101902,203805,108.16236710548401,0.014314851356459529
51051,102103,102102,204205,108.33263897895813,0.0142904762924336
51151,102303,102302,204605,108.51706027984619,0.01426616482365087
51251,102503,102502,205005,108.6861560344696,0.014241916693287952
51351,102703,102702,205405,108.8735408782959,0.014217731646209248
51451,102903,102902,205805,109.022625207901,0.014193609428949962
51552,103105,103104,206209,109.16737103462219,0.014169309508478186
51652,103305,103304,206609,109.32016324996948,0.014145312819084519
51752,103505,103504,207009,109.47689604759216,0.014121378206498671
51852,103705,103704,207409,109.62915420532227,0.014097505423791156
51952,103905,103904,207809,109.81001496315002,0.014073694225622347
52052,104105,104104,208209,109.99552607536316,0.01404994436822647
52152,104305,104304,208609,110.16992712020874,0.014026255609396686
52252,104505,104504,209009,110.3243670463562,0.014002627708469512
52352,104705,104704,209409,110.48928117752075,0.013979060426309933
52452,104905,104904,209809,110.65836906433105,0.013955553525296671
52553,105107,105106,210213,110.82561588287354,0.013931872604684651
52653,105307,105306,210613,110.98361396789551,0.013908486357005244
52753,105507,105506,211013,111.1397168636322,0.013885159784220062
52853,105707,105706,211413,111.29452919960022,0.013861892654632132
52953,105907,105906,211813,111.44832420349121,0.013838684737986525
53053,106107,106106,212213,111.59619402885437,0.013815535805456691
53153,106307,106306,212613,111.77924513816833,0.013792445629630744
53253,106507,106506,213013,111.93545413017273,0.013769413984498097
53353,106707,106706,213413,112.11761689186096,0.013746440645436255
53453,106907,106906,213813,112.2702898979187,0.013723525389197551
53554,107109,107108,214217,112.421875,0.013700439711393808
53654,107309,107308,214617,112.5767571926117,0.01367764053178866
53754,107509,107508,215017,112.73654413223267,0.013654898771199535
53854,107709,107708,215417,112.88861227035522,0.013632214211764027
53954,107909,107908,215817,113.04025101661682,0.01360958663693127
54054,108109,108108,216217,113.18748712539673,0.013587015831450056
54154,108309,108308,216617,113.35040807723999,0.013564501581356529
54254,108509,108508,217017,113.56490206718445,0.01354204367396259
54354,108709,108708,217417,113.76403522491455,0.013519641897843921
54454,108909,108908,217817,113.91616415977478,0.013497296042828549
54555,109111,109110,218221,114.08128428459167,0.013474783279199671
54655,109311,109310,218621,114.27163028717041,0.01345254919482705
54755,109511,109510,219021,114.42909693717957,0.01343037040638306
54855,109711,109710,219421,114.57777214050293,0.013408246708603739
54955,109911,109910,219821,114.72149729728699,0.013386177897421475
55055,110111,110110,220221,114.88675904273987,0.013364163769954158
55155,110311,110310,220621,115.07847309112549,0.013342204124494349
55255,110511,110510,221021,115.24696516990662,0.013320298760499127
55355,110711,110710,221421,115.50527501106262,0.013298447478579412
55455,110911,110910,221821,115.78613519668579,0.013276650080489637
55556,111113,111112,222225,115.99187016487122,0.013254689202457986
55656,111313,111312,222625,116.20966625213623,0.013232999515736827
55756,111513,111512,223025,116.40398597717285,0.013211363122926699
55856,111713,111712,223425,116.58046913146973,0.013189779830267258
55956,111913,111912,223825,116.73071217536926,0.013168249445091837
56056,112113,112112,224225,116.88145589828491,0.01314677177581818
56156,112313,112312,224625,117.03979396820068,0.01312534663193894
56256,112513,112512,225025,117.19827318191528,0.013103973824012185
56356,112713,112712,225425,117.34875512123108,0.013082653163652267
56456,112913,112912,225825,117.4949860572815,0.013061384463520571
56557,113115,113114,226229,117.64878797531128,0.013039955628885188
56657,113315,113314,226629,117.79775309562683,0.013018790806291975
56757,113515,113514,227029,118.00857210159302,0.01299767738626663
56857,113715,113714,227429,118.1763710975647,0.012976615185579705
56957,113915,113914,227829,118.3353979587555,0.012955604022004623
57057,114115,114114,228229,118.50096607208252,0.01293464371430911
57157,114315,114314,228629,118.6631350517273,0.012913734082246801
57257,114515,114514,229029,118.81338405609131,0.012892874946548923
57357,114715,114714,229429,118.96398711204529,0.012872066128916037
57457,114915,114914,229829,119.24495220184326,0.012851307452009776
57558,115117,115116,230233,119.50359416007996,0.012830391904044983
57658,115317,115316,230633,119.7720410823822,0.012809733477388006
57758,115517,115516,231033,119.96573209762573,0.012789124663389556
57858,115717,115716,231433,120.11379218101501,0.012768565288485622
57958,115917,115916,231833,120.31945204734802,0.012748055180034057
58058,116117,116116,232233,120.65886807441711,0.012727594166306812
58158,116317,116316,232633,120.96442914009094,0.012707182076482379
58258,116517,116516,233033,121.26995897293091,0.012686818740638432
58358,116717,116716,233433,121.64639329910278,0.012666503989744518
58458,116917,116916,233833,121.95921587944031,0.012646237655654704
58559,117119,117118,234237,122.21729707717896,0.01262581763335122
58659,117319,117318,234637,122.47918105125427,0.012605648111927934
58759,117519,117518,235037,122.64190697669983,0.01258552650645551
58859,117719,117718,235437,122.80093812942505,0.012565452652263543
58959,117919,117918,235837,122.98144006729126,0.01254542638553089
59059,118119,118118,236237,123.15365314483643,0.012525447543278976
59159,118319,118318,236637,123.43775391578674,0.012505515963364805
59259,118519,118518,237037,123.7783100605011,0.012485631484474713
59359,118719,118718,237437,123.95969796180725,0.012465793946117406
59459,118919,118918,237837,124.11163020133972,0.012446003188617685
59560,119121,119120,238241,124.29236698150635,0.012426061846660291
59660,119321,119320,238641,124.6114718914032,0.01240636463892564
59760,119521,119520,239041,124.85502815246582,0.012386713736286269
59860,119721,119720,239441,125.11234307289124,0.01236710898227509
59960,119921,119920,239841,125.26479911804199,0.012347550221209671
60060,120121,120120,240241,125.4175751209259,0.01232803729818582
60160,120321,120320,240641,125.57542109489441,0.012308570059071607
60260,120521,120520,241041,125.72115993499756,0.012289148350501572
60360,120721,120720,241441,125.86584806442261,0.01226977201987071
60460,120921,120920,241841,126.03351998329163,0.012250440915328632
60561,121123,121122,242245,126.18785309791565,0.012230962252597479
60661,121323,121322,242645,126.48192501068115,0.01221172159616075
60761,121523,121522,243045,126.72979211807251,0.012192525713239316
60861,121723,121722,243445,126.9634461402893,0.012173374454951404
60961,121923,121922,243845,127.12130522727966,0.01215426767314145
61061,122123,122122,244245,127.28732490539551,0.012135205220374895
61161,122323,122322,244645,127.44957113265991,0.012116186949932379
61261,122523,122522,245045,127.60030698776245,0.012097212715804754
61361,122723,122722,245445,127.74444603919983,0.012078282372687483
61461,122923,122922,245845,127.8941900730133,0.01205939577597569
61562,123125,123124,246249,128.0493130683899,0.012040364571523868
61662,123325,123324,246649,128.1929440498352,0.0120215654704518
61762,123525,123524,247049,128.33728313446045,0.012002809684693572
61862,123725,123724,247449,128.48845911026,0.011984097072397587
61962,123925,123924,247849,128.63121509552002,0.011965427492386235
62062,124125,124124,248249,128.776141166687,0.011946800804150993
62162,124325,124324,248649,128.91982126235962,0.011928216867847589
62262,124525,124524,249049,129.0771882534027,0.011909675544291117
62362,124725,124724,249449,129.222088098526,0.011891176694951261
62462,124925,124924,249849,129.3884072303772,0.011872720181947644
62563,125127,125126,250253,129.54953908920288,0.011854121937548822
62663,125327,125326,250653,129.69741296768188,0.011835750106090122
62763,125527,125526,251053,129.8459882736206,0.011817420199822857
62863,125727,125726,251453,130.00257325172424,0.011799132083426103
62963,125927,125926,251853,130.15118408203125,0.011780885622206022
63063,126127,126126,252253,130.29499006271362,0.011762680682091079
63163,126327,126326,252653,130.4551088809967,0.011744517129627865
63263,126527,126526,253053,130.60659098625183,0.011726394831976827
63363,126727,126726,253453,130.7664670944214,0.011708313656907696
63463,126927,126926,253853,130.91522312164307,0.011690273472795353
63564,127129,127128,254257,131.0723741054535,0.011672094361274773
63664,127329,127328,254657,131.218111038208,0.011654136173238737
63764,127529,127528,255057,131.36804008483887,0.011636218583577785
63864,127729,127728,255457,131.5419900417328,0.011618341463051452
63964,127929,127928,255857,131.68955087661743,0.011600504683003719
64064,128129,128128,256257,131.8347852230072,0.011582708115358976
64164,128329,128328,256657,132.01572728157043,0.011564951632618016
64264,128529,128528,257057,132.1861870288849,0.011547235107853984
64364,128729,128728,257457,132.3585970401764,0.011529558414708816
64464,128929,128928,257857,132.52499413490295,0.011511921427388995
64565,129131,129130,258261,132.6794571876526,0.011494148246054431
64665,129331,129330,258661,132.83634901046753,0.011476590689176235
64765,129531,129530,259061,133.00986194610596,0.011459072462854887
64865,129731,129730,259461,133.17453408241272,0.011441593443523404
64965,129931,129930,259861,133.32009601593018,0.011424153508160761
65065,130131,130130,260261,133.47564816474915,0.011406752534288241
65165,130331,130330,260661,133.65278911590576,0.011389390399965822
65265,130531,130530,261061,133.8568992614746,0.011372066983788637
65365,130731,130730,261461,134.02431321144104,0.011354782164883313
65465,130931,130930,261861,134.16691899299622,0.011337535822904688
65566,131133,131132,262265,134.3136022090912,0.011320155951482764
65666,131333,131332,262665,134.49438405036926,0.011302986586194321
65766,131533,131532,263065,134.65001606941223,0.011285855338745761
65866,131733,131732,263465,134.80033493041992,0.011268762090875073
65966,131933,131932,263865,134.96050810813904,0.011251706724831254
66066,132133,132132,264265,135.11840105056763,0.011234689123371028
66166,132333,132332,264665,135.26413226127625,0.011217709169755707
66266,132533,132532,265065,135.41616487503052,0.011200766747747691
66366,132733,132732,265465,135.57280898094177,0.011183861741607555
66466,132933,132932,265865,135.72316193580627,0.011166994036090673
66567,133135,133134,266269,135.88150310516357,0.011149995398649155
66667,133335,133334,266669,136.03799510002136,0.01113320232074906
66767,133535,133534,267069,136.1811981201172,0.011116446199540608
66867,133735,133734,267469,136.3254039287567,0.011099726921732184
66967,133935,133934,267869,136.48156595230103,0.011083044374511446
67067,134135,134134,268269,136.62792825698853,0.011066398445542447
67167,134335,134334,268669,136.7719430923462,0.011049789022962631
67267,134535,134534,269069,136.918062210083,0.011033215995379778
67367,134735,134734,269469,137.07875108718872,0.011016679251869298
67467,134935,134934,269869,137.22458291053772,0.0110001786819711
67568,135137,135136,270273,137.3695409297943,0.010983549712374231
67668,135337,135336,270673,137.5224289894104,0.010967121519153593
67768,135537,135536,271073,137.66208410263062,0.010950729169835593
67868,135737,135736,271473,137.80469727516174,0.010934372555794594
67968,135937,135936,271873,137.97744703292847,0.010918051568855542
68068,136137,136136,272273,138.12958312034607,0.010901766101291118
68168,136337,136336,272673,138.27915906906128,0.01088551604581895
68268,136537,136536,273073,138.42954015731812,0.010869301295599118
68368,136737,136736,273473,138.58255815505981,0.010853121744231246
68468,136937,136936,273873,138.7266550064087,0.010836977285752086
68569,137139,137138,274277,138.8749189376831,0.010820706896251716
68669,137339,137338,274677,139.0323941707611,0.010804632655688488
68769,137539,137538,275077,139.17353296279907,0.010788593191675569
68869,137739,137738,275477,139.31937217712402,0.010772588399976161
68969,137939,137938,275877,139.4695701599121,0.010756618176777446
69069,138139,138138,276277,139.61473202705383,0.01074068241868826
69169,138339,138338,276677,139.75825595855713,0.010724781022736616
69269,138539,138538,277077,139.90133094787598,0.010708913886367213
69369,138739,138738,277477,140.06246614456177,0.010693080907438939
69469,138939,138938,277877,140.2162902355194,0.010677281984222546
69570,139141,139140,278281,140.35920906066895,0.0106613595368379
69670,139341,139340,278681,140.51527905464172,0.010645628759519424
69770,139541,139540,279081,140.65612125396729,0.010629931734169071
69870,139741,139740,279481,140.8010129928589,0.010614268360685181
69970,139941,139940,279881,140.95333099365234,0.01059863853936608
70070,140141,140140,280281,141.10060715675354,0.010583042170907768
70170,140341,140340,280681,141.24358987808228,0.010567479156401759
70270,140541,140540,281081,141.38744807243347,0.010551949397332722
70370,140741,140740,281481,141.53786206245422,0.01053645279557633
70470,140941,140940,281881,141.682391166687,0.01052098925339699
70571,141143,141142,282285,141.83826994895935,0.010505404533777012
70671,141343,141342,282685,141.99474120140076,0.010490007147253242
70771,141543,141542,283085,142.14342713356018,0.010474642528446447
70871,141743,141742,283485,142.4555220603943,0.010459310581157993
70971,141943,141942,283885,142.68545794487,0.010444011209567077
71071,142143,142142,284285,142.9405481815338,0.010428744318228945
71171,142343,142342,284685,143.27153205871582,0.01041350981207237
71271,142543,142542,285085,143.48938822746277,0.010398307596397902
71371,142743,142742,285485,143.64665293693542,0.010383137576875551
71471,142943,142942,285885,143.80594325065613,0.010367999659543051
71572,143145,143144,286289,143.98992323875427,0.010352742853043743
71672,143345,143344,286689,144.1526279449463,0.010337669178347931
71772,143545,143544,287089,144.36156010627747,0.010322627325213274
71872,143745,143744,287489,144.53836798667908,0.010307617201131205
71972,143945,143944,287889,144.70294904708862,0.010292638713950824
72072,144145,144144,288289,144.85395097732544,0.01027769177187676
72172,144345,144344,288689,145.04456210136414,0.010262776283467645
72272,144545,144544,289089,145.33063411712646,0.010247892157633672
72372,144745,144744,289489,145.58928894996643,0.010233039303635262
72472,144945,144944,289889,145.87668704986572,0.01021821763108069
72573,145147,145146,290293,146.0500020980835,0.010203279300820748
72673,145347,145346,290693,146.25933003425598,0.010188520030927118
72773,145547,145546,291093,146.4031891822815,0.010173791672480472
72873,145747,145746,291493,146.59773230552673,0.010159094136466484
72973,145947,145946,291893,146.75331211090088,0.010144427334209621
73073,146147,146146,292293,146.899884223938,0.01012979117737153
73173,146347,146346,292693,147.05008506774902,0.010115185577949172
73273,146547,146546,293093,147.1917760372162,0.01010061044827318
73373,146747,146746,293493,147.36380195617676,0.010086065701005903
73473,146947,146946,293893,147.57088208198547,0.010071551249139847
73574,147149,147148,294297,147.72860193252563,0.01005692231582622
73674,147349,147348,294697,147.87789297103882,0.010042468495840836
73774,147549,147548,295097,148.02761721611023,0.010028044711339279
73874,147749,147748,295497,148.20240712165833,0.010013650876620636
73974,147949,147948,295897,148.39412999153137,0.009999286906305714
74074,148149,148148,296297,148.5553171634674,0.00998495271533535
74174,148349,148348,296697,148.73381519317627,0.009970648218968625
74274,148549,148548,297097,148.91385197639465,0.0099563733327815
74374,148749,148748,297497,149.07170796394348,0.009942127972664876
74474,148949,148948,297897,149.22628712654114,0.00992791205482332
74575,149151,149150,298301,149.37991619110107,0.009913583778163
74675,149351,149350,298701,149.53367614746094,0.009899426787068365
74775,149551,149550,299101,149.68820905685425,0.009885298987900538
74875,149751,149750,299501,149.8557960987091,0.009871200298105322
74975,149951,149950,299901,150.0155210494995,0.009857130635434221
75075,150151,150150,300301,150.17052912712097,0.009843089917942964
75175,150351,150350,300701,150.32769012451172,0.00982907806398986
75275,150551,150550,301101,150.48357105255127,0.00981509499223439
75375,150751,150750,301501,150.6338050365448,0.009801140621635535
75475,150951,150950,301901,150.78635811805725,0.009787214871450541
75576,151153,151152,302305,150.9700312614441,0.009773178832986541
75676,151353,151352,302705,151.1271140575409,0.009759310366780592
75776,151553,151552,303105,151.27773022651672,0.009745470279737227
75876,151753,151752,303505,151.44417691230774,0.009731658492294576
75976,151953,151952,303905,151.6123149394989,0.0097178749251816
76076,152153,152152,304305,151.78411412239075,0.009704119499416724
76176,152353,152352,304705,151.95632791519165,0.009690392136306415
76276,152553,152552,305105,152.14277505874634,0.009676692757443756
76376,152753,152752,305505,152.3011589050293,0.00966302128470716
76476,152953,152952,305905,152.45644187927246,0.009649377640258878
76577,153155,153154,306309,152.63556790351868,0.009635625727486065
76677,153355,153354,306709,152.82549214363098,0.009622037783575196
76777,153555,153554,307109,153.00554299354553,0.009608477435360597
76877,153755,153754,307509,153.26513695716858,0.009594944606129162
76977,153955,153954,307909,153.42644786834717,0.009581439219445069
77077,154155,154154,308309,153.58292508125305,0.009567961199148232
77177,154355,154354,308709,153.74885511398315,0.009554510469353053
77277,154555,154554,309109,153.90931797027588,0.009541086954447145
77377,154755,154754,309509,154.08810091018677,0.00952769057909001
77477,154955,154954,309909,154.25027704238892,0.009514321268211777
77578,155157,155156,310313,154.40946006774902,0.009500845659845384
77678,155357,155356,310713,154.57356023788452,0.00948753052256744
77778,155557,155556,311113,154.7304892539978,0.009474242225428524
77878,155757,155756,311513,154.890310049057,0.009460980694431215
77978,155957,155956,311913,155.05088901519775,0.009447745855842505
78078,156157,156156,312313,155.2399299144745,0.009434537636192349
78178,156357,156356,312713,155.40805411338806,0.009421355962272702
78278,156557,156556,313113,155.581768989563,0.00940820076113614
78378,156757,156756,313513,155.75302815437317,0.00939507196009464
78478,156957,156956,313913,155.92951917648315,0.00938196948671854
78579,157159,157158,314317,156.10309314727783,0.009368762639003063
78679,157359,157358,314717,156.26134204864502,0.009355712866169126
78779,157559,157558,315117,156.41201305389404,0.009342689204533832
78879,157759,157758,315517,156.56671500205994,0.009329691582691197
78979,157959,157958,315917,156.72293901443481,0.00931671992948766
79079,158159,158158,316317,156.87489414215088,0.009303774174020951
79179,158359,158358,316717,157.0335350036621,0.009290854245638795
79279,158559,158558,317117,157.20528507232666,0.009277960073937962
79379,158759,158758,317517,157.42616605758667,0.00926509158876296
79479,158959,158958,317917,157.58858919143677,0.009252248720205199
79580,159161,159160,318321,157.7458300590515,0.009239303354162473
79680,159361,159360,318721,157.90259408950806,0.009226511764519909
79780,159561,159560,319121,158.05861520767212,0.009213745582547072
79880,159761,159760,319521,158.2119472026825,0.009201004739313621
79980,159961,159960,319921,158.36032485961914,0.009188289166130226
80080,160161,160160,320321,158.51122999191284,0.009175598794547902
80180,160361,160360,320721,158.65854907035828,0.009162933556356601
80280,160561,160560,321121,158.80921006202698,0.0091502933835844
80380,160761,160760,321521,158.96527910232544,0.009137678208496288
80480,160961,160960,321921,159.15781712532043,0.009125087963593204
80581,161163,161162,322325,159.3828649520874,0.009112397053121802
80681,161363,161362,322725,159.54592108726501,0.00909985671465115
80781,161563,161562,323125,159.7837221622467,0.009087341104606664
80881,161763,161762,323525,159.95104813575745,0.009074850156424858
80981,161963,161962,323925,160.10062503814697,0.00906238380377307
81081,162163,162162,324325,160.30363011360168,0.009049941980548438
81181,162363,162362,324725,160.49111413955688,0.00903752462087687
81281,162563,162562,325125,160.64197516441345,0.00902513165911197
81381,162763,162762,325525,160.87697410583496,0.009012763029834198
81481,162963,162962,325925,161.030091047287,0.009000418667849718
81582,163165,163164,326329,161.18191504478455,0.008987975428595498
81682,163365,163364,326729,161.36017894744873,0.008975679647564273
81782,163565,163564,327129,161.51563119888306,0.008963407938945957
81882,163765,163764,327529,161.72941207885742,0.008951160238442469
81982,163965,163964,327929,161.90333819389343,0.008938936481976746
82082,164165,164164,328329,162.05979299545288,0.008926736605691652
82182,164365,164364,328729,162.21217894554138,0.00891456054594913
82282,164565,164564,329129,162.36691999435425,0.008902408239329317
82382,164765,164764,329529,162.52047324180603,0.008890279622629579
82482,164965,164964,329929,162.67273092269897,0.008878174632863426
82583,165167,165166,330333,162.82637810707092,0.008865972511791073
82683,165367,165366,330733,162.98238706588745,0.008853914822494502
82783,165567,165566,331133,163.13390016555786,0.00884188057183861
82883,165767,165766,331533,163.2909390926361,0.00882986969769517
82983,165967,165966,331933,163.4484622478485,0.008817882138147685
83083,166167,166166,332333,163.60275793075562,0.008805917831490507
83183,166367,166366,332733,163.75610613822937,0.008793976716227883
83283,166567,166566,333133,163.93417501449585,0.008782058731073293
83383,166767,166766,333533,164.09458899497986,0.008770163814948245
83483,166967,166966,333933,164.24871110916138,0.008758291906981772
83584,167169,167168,334337,164.40531301498413,0.008746324572584651
83684,167369,167368,334737,164.565171957016,0.008734498727712887
83784,167569,167568,335137,164.72057604789734,0.008722695709020326
83884,167769,167768,335537,164.87491416931152,0.008710915456458839
83984,167969,167968,335937,165.03441214561462,0.008699157910183178
84084,168169,168168,336337,165.19156217575073,0.008687423010550298
84184,168369,168368,336737,165.34525799751282,0.008675710698118596
84284,168569,168568,337137,165.50127696990967,0.008664020913647038
84384,168769,168768,337537,165.6563651561737,0.008652353598094296
84484,168969,168968,337937,165.8108720779419,0.008640708692617936
84585,169171,169170,338341,165.9781529903412,0.008628970025709922
84685,169371,169370,338741,166.14727807044983,0.008617369987285886
84785,169571,169570,339141,166.30411291122437,0.008605792183014695
84885,169771,169770,339541,166.4706370830536,0.008594236554843345
84985,169971,169970,339941,166.65434193611145,0.008582703044913742
85085,170171,170170,340341,166.80891609191895,0.008571191595561807
85185,170371,170370,340741,166.96645212173462,0.008559702149316813
85285,170571,170570,341141,167.12177205085754,0.008548234648900484
85385,170771,170770,341541,167.2692370414734,0.008536789037226163
85485,170971,170970,341941,167.41848611831665,0.00852536525739832
85586,171173,171172,342345,167.57306599617004,0.008513849342437672
85686,171373,171372,342745,167.7216169834137,0.008502469273277233
85786,171573,171572,343145,167.88717699050903,0.00849111086585197
85886,171773,171772,343545,168.08141207695007,0.008479774064024255
85986,171973,171972,343945,168.2426450252533,0.008468458811843493
86086,172173,172172,344345,168.39245223999023,0.008457165053545518
86186,172373,172372,344745,168.53993916511536,0.00844589273355175
86286,172573,172572,345145,168.68741011619568,0.008434641796468531
86386,172773,172772,345545,168.83306908607483,0.008423412187086277
86486,172973,172972,345945,168.9887990951538,0.008412203850378878
86587,173175,173174,346349,169.13994097709656,0.008400904967279037
86687,173375,173374,346749,169.29013299942017,0.008389739222929127
86787,173575,173574,347149,169.4428551197052,0.008378594586724877
86887,173775,173774,347549,169.58894300460815,0.008367471004368328
86987,173975,173974,347949,169.7364900112152,0.008356368421741254
87087,174175,174174,348349,169.94163012504578,0.008345286784904541
87187,174375,174374,348749,170.11531925201416,0.008334226040097426
87287,174575,174574,349149,170.26015329360962,0.00832318613373682
87387,174775,174774,349549,170.42459201812744,0.008312167012416565
87487,174975,174974,349949,170.57164025306702,0.008301168622906842
87588,175177,175176,350353,170.71737098693848,0.008290081239294492
87688,175377,175376,350753,170.8599500656128,0.008279124360410202
87788,175577,175576,351153,171.00911712646484,0.008268188054171297
87888,175777,175776,351553,171.1566641330719,0.008257272268047962
87988,175977,175976,351953,171.30464506149292,0.008246376949683042
88088,176177,176176,352353,171.45591521263123,0.008235502046891623
88188,176377,176376,352753,171.59975624084473,0.008224647507660221
88288,176577,176576,353153,171.7439420223236,0.008213813280146202
88388,176777,176776,353553,171.88652920722961,0.00820299931267709
88488,176977,176976,353953,172.03851127624512,0.008192205553749962
88589,177179,177178,354357,172.19757294654846,0.008181324317634046
88689,177379,177378,354757,172.35441994667053,0.008170571022759168
88789,177579,177578,355157,172.51506996154785,0.008159837782418624
88889,177779,177778,355557,172.66641998291016,0.008149124545782496
88989,177979,177978,355957,172.8135540485382,0.008138431262187258
89089,178179,178178,356357,172.96719312667847,0.008127757881134784
89189,178379,178378,356757,173.11011505126953,0.00811710435229215
89289,178579,178578,357157,173.25433707237244,0.008106470625490499
89389,178779,178778,357557,173.3990399837494,0.00809585665072483
89489,178979,178978,357957,173.54697108268738,0.008085262378153189
89590,179181,179180,358361,173.69195914268494,0.008074582110972974
89690,179381,179380,358761,173.8388590812683,0.008064027289693009
89790,179581,179580,359161,173.98827505111694,0.008053492021560556
89890,179781,179780,359561,174.13548398017883,0.008042976257381264
89990,179981,179980,359961,174.2803270816803,0.00803247994812076
90090,180181,180180,360361,174.42828106880188,0.008022003044904101
90190,180381,180380,360761,174.5755331516266,0.008011545499014991
90290,180581,180580,361161,174.7397861480713,0.008001107261895308
90390,180781,180780,361561,174.88754606246948,0.007990688285144496
90490,180981,180980,361961,175.03902316093445,0.007980288520518969
90591,181183,181182,362365,175.18570709228516,0.007969804210541661
90691,181383,181382,362765,175.33200597763062,0.007959442916980157
90791,181583,181582,363165,175.48022890090942,0.00794910069127186
90891,181783,181782,363565,175.62655401229858,0.007938777485796538
90991,181983,181982,363965,175.7720341682434,0.007928473253087964
91091,182183,182182,364365,175.92174005508423,0.007918187945833367
91191,182383,182382,364765,176.06903624534607,0.007907921516872833
91291,182583,182582,365165,176.21473217010498,0.007897673919198569
91391,182783,182782,365565,176.35947012901306,0.007887445105954636
91491,182983,182982,365965,176.51067185401917,0.007877235030436138
91592,183185,183184,366369,176.65729117393494,0.007866941826478525
91692,183385,183384,366769,176.81468510627747,0.0078567692731117
91792,183585,183584,367169,176.97467613220215,0.00784661531779491
91892,183785,183784,367569,177.12155604362488,0.007836479914423562
91992,183985,183984,367969,177.2666199207306,0.007826363017041432
92092,184185,184184,368369,177.4150791168213,0.007816264579839964
92192,184385,184384,368769,177.56440806388855,0.007806184557157917
92292,184585,184584,369169,177.71172904968262,0.0077961229034805455
92392,184785,184784,369569,177.8579671382904,0.007786079573439365
92492,184985,184984,369969,178.01034498214722,0.007776054521811322
92593,185187,185186,370373,178.15927004814148,0.0077659477272617955
92693,185387,185386,370773,178.30659794807434,0.007755959279028298
92793,185587,185586,371173,178.45838904380798,0.00774598897395979
92893,185787,185786,371573,178.6047592163086,0.007736036767411587
92993,185987,185986,371973,178.74888610839844,0.007726102614881864
93093,186187,186186,372373,178.9043369293213,0.00771618647201114
93193,186387,186386,372773,179.0715069770813,0.007706288294581779
93293,186587,186586,373173,179.21204113960266,0.007696408038517362
93393,186787,186786,373573,179.35183310508728,0.007686545659882374
93493,186987,186986,373973,179.4958770275116,0.007676701114881473
93594,187189,187188,374377,179.63777709007263,0.007666776182000901
93694,187389,187388,374777,179.77835202217102,0.007656967350685936
93794,187589,187588,375177,179.91814398765564,0.0076471762220223765
93894,187789,187788,375577,180.06331300735474,0.007637402752772151
93994,187989,187988,375977,180.20455408096313,0.007627646899834897
94094,188189,188188,376377,180.34499406814575,0.007617908620247393
94194,188389,188388,376777,180.49297904968262,0.0076081878711831774
94294,188589,188588,377177,180.63466715812683,0.007598484609951875
94394,188789,188788,377577,180.77437496185303,0.007588798793998877
94494,188989,188988,377977,180.91858792304993,0.007579130380904666
94595,189191,189190,378381,181.0667700767517,0.007569382905387485
94695,189391,189390,378781,181.22139310836792,0.007559749344262658
94795,189591,189590,379181,181.36077904701233,0.007550133059124971
94895,189791,189790,379581,181.50528216362,0.0075405340080920945
94995,189991,189990,379981,181.6448142528534,0.007530952149414454
95095,190191,190190,380381,181.78322529792786,0.007521387441474787
95195,190391,190390,380781,181.92550706863403,0.007511839842787465
95295,190591,190590,381181,182.07065415382385,0.0075023093119982445
95395,190791,190790,381581,182.21088409423828,0.007492795807883659
95495,190991,190990,381981,182.3508701324463,0.007483299289350599
95596,191193,191192,382385,182.4966402053833,0.00747372500512869
95696,191393,191392,382785,182.63633012771606,0.007464262503830366
95796,191593,191592,383185,182.775780916214,0.007454816865205057
95896,191793,191792,383585,182.91661024093628,0.007445388048677621
95996,191993,191992,383985,183.06134724617004,0.007435976013800798
96096,192193,192192,384385,183.2016100883484,0.007426580720254902
96196,192393,192392,384785,183.36102104187012,0.00741720212784732
96296,192593,192592,385185,183.5037431716919,0.00740784019651204
96396,192793,192792,385585,183.6436469554901,0.00739849488630915
96496,192993,192992,385985,183.7841260433197,0.007389166157424452
96597,193195,193194,386389,183.92608904838562,0.007379760931697754
96697,193395,193394,386789,184.06936407089233,0.007370465411328744
96797,193595,193594,387189,184.2090141773224,0.007361186353191253
96897,193795,193794,387589,184.35125517845154,0.0073519237179705925
96997,193995,193994,387989,184.49603700637817,0.007342677466475559
97097,194195,194194,388389,184.63534903526306,0.007333447559637854
97197,194395,194394,388789,184.77447986602783,0.007324233958511813
97297,194595,194594,389189,184.9176368713379,0.0073150366242738735
97397,194795,194794,389589,185.06401419639587,0.007305855518222141
97497,194995,194994,389989,185.20578694343567,0.007296690601775942
97598,195197,195196,390393,185.3487730026245,0.007287450430255907
97698,195397,195396,390793,185.51325392723083,0.0072783179386965826
97798,195597,195596,391193,185.65559101104736,0.007269201521342371
97898,195797,195796,391593,185.79662704467773,0.007260101140094465
97998,195997,195996,391993,185.9428551197052,0.007251016756973199
98098,196197,196196,392393,186.0863392353058,0.007241948334117486
98198,196397,196396,392793,186.2250199317932,0.007232895833784522
98298,196597,196596,393193,186.36408710479736,0.007223859218349286
98398,196797,196796,393593,186.51007509231567,0.007214838450304185
98498,196997,196996,393993,186.65111827850342,0.007205833492258538
98599,197199,197198,394397,186.79327487945557,0.007196754494611566
98699,197399,197398,394797,186.9369239807129,0.007187781202027244
98799,197599,197598,395197,187.0820062160492,0.007178823607598379
98899,197799,197798,395597,187.22448706626892,0.0071698816743992365
98999,197999,197998,395997,187.36818099021912,0.007160955365619003
99099,198199,198198,396397,187.51528000831604,0.007152044644561347
99199,198399,198398,396797,187.67605113983154,0.007143149474644061
99299,198599,198598,397197,187.8164141178131,0.007134269819398599
99399,198799,198798,397597,187.96433115005493,0.0071254056424696855
99499,198999,198998,397997,188.1062831878662,0.007116556907614964
99600,199201,199200,398401,188.24982619285583,0.0071076353230935165
99700,199401,199400,398801,188.39081001281738,0.007098817517627355
99800,199601,199600,399201,188.5376341342926,0.007090015045823082
99900,199801,199800,399601,188.67984914779663,0.007081227871886953
100000,200001,200000,400001,188.82434606552124,0.007072455960136204


==> plot_data/quadratic_minimax_problem_n500_alpha0/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0012407302856445312,30.358099469249375
100,201,200,401,0.18846678733825684,1.725251134601807
200,401,400,801,0.35608386993408203,1.0331394156994131
300,601,600,1201,0.5164837837219238,0.7736231354158138
400,801,800,1601,0.674454927444458,0.6349280372139878
501,1003,1002,2005,0.8346707820892334,0.5455617951375803
601,1203,1202,2405,1.0521190166473389,0.482543795209007
701,1403,1402,2805,1.2395477294921875,0.43443121283005004
801,1603,1602,3205,1.4113609790802002,0.396082748791271
901,1803,1802,3605,1.7056248188018799,0.3645989873004372
1001,2003,2002,4005,1.9532716274261475,0.33817775845833975
1101,2203,2202,4405,2.1195788383483887,0.31561971894335344
1201,2403,2402,4805,2.315887689590454,0.29608763453723413
1301,2603,2602,5205,2.5615928173065186,0.2789761387097555
1401,2803,2802,5605,2.7624619007110596,0.26383524354104326
1502,3005,3004,6009,2.9426259994506836,0.25019483089933037
1602,3205,3204,6409,3.1264870166778564,0.23805758726442536
1702,3405,3404,6809,3.3363149166107178,0.22707177793944233
1802,3605,3604,7209,3.501164674758911,0.21706993619439596
1902,3805,3804,7609,3.646152973175049,0.20791616240763086
2002,4005,4004,8009,3.813706874847412,0.19949893614020578
2102,4205,4204,8409,3.9843246936798096,0.19172585568559014
2202,4405,4404,8809,4.146417856216431,0.18451971692199934
2302,4605,4604,9209,4.311557769775391,0.17781553946480064
2402,4805,4804,9609,4.467228889465332,0.1715582748285912
2503,5007,5006,10013,4.646040678024292,0.16564432077061936
2603,5207,5206,10413,4.8161516189575195,0.16015029105088846
2703,5407,5406,10813,5.031245708465576,0.1549811510589118
2803,5607,5606,11213,5.345148801803589,0.15010700224205265
2903,5807,5806,11613,5.586578845977783,0.14550185344186578
3003,6007,6006,12013,5.804050922393799,0.14114300673996125
3103,6207,6206,12413,5.9886908531188965,0.13701055044944
3203,6407,6406,12813,6.169491767883301,0.1330869385687235
3303,6607,6606,13213,6.327349901199341,0.12935664054963755
3403,6807,6806,13613,6.48043966293335,0.12580584861601082
3504,7009,7008,14017,6.7220728397369385,0.12238920212160206
3604,7209,7208,14417,6.935734033584595,0.11916321177975675
3704,7409,7408,14817,7.086650848388672,0.11608328196435345
3804,7609,7608,15217,7.244872808456421,0.11314041075772609
3904,7809,7808,15617,7.410405874252319,0.11032642169640298
4004,8009,8008,16017,7.567966938018799,0.10763385857735135
4104,8209,8208,16417,7.729620933532715,0.10505589601363031
4204,8409,8408,16817,7.889976739883423,0.1025862632084499
4304,8609,8608,17217,8.035264015197754,0.10021917884265644
4404,8809,8808,17617,8.180601835250854,0.09794929532145866
4505,9011,9010,18021,8.323847770690918,0.09575032438778178
4605,9211,9210,18421,8.462627649307251,0.09366115602452446
4705,9411,9410,18821,8.614176988601685,0.09165526018334968
4805,9611,9610,19221,8.754035949707031,0.08972860996649396
4905,9811,9810,19621,8.93245267868042,0.08787742990858095
5005,10011,10010,20021,9.086054801940918,0.08609817276901403
5105,10211,10210,20421,9.240131855010986,0.08438749926429683
5205,10411,10410,20821,9.383841037750244,0.0827422603099926
5305,10611,10610,21221,9.549936771392822,0.08115948140902517
5405,10811,10810,21621,9.859187841415405,0.07963634887915819
5506,11013,11012,22025,10.050968647003174,0.07815581524163809
5606,11213,11212,22425,10.222308874130249,0.07674465027683981
5706,11413,11412,22825,10.43417477607727,0.07538551682251976
5806,11613,11612,23225,10.581081867218018,0.07407613635346144
5906,11813,11812,23625,10.721892833709717,0.07281434196761298
6006,12013,12012,24025,10.869425773620605,0.07159807137914267
6106,12213,12212,24425,11.020484685897827,0.07042536057263304
6206,12413,12412,24825,11.171380996704102,0.06929433803403764
6306,12613,12612,25225,11.309647798538208,0.06820321948612608
6406,12813,12812,25625,11.453434705734253,0.06715030306641073
6507,13015,13014,26029,11.618983745574951,0.06612398092841468
6607,13215,13214,26429,11.75954294204712,0.06514301371111987
6707,13415,13414,26829,11.903349876403809,0.06419558041511696
6807,13615,13614,27229,12.043097734451294,0.0632802683993876
6907,13815,13814,27629,12.181427955627441,0.062395728307350413
7007,14015,14014,28029,12.321580648422241,0.06154067100873571
7107,14215,14214,28429,12.46141004562378,0.06071386473424732
7207,14415,14414,28829,12.61687183380127,0.05991413238392325
7307,14615,14614,29229,12.777913808822632,0.059140348992611
7407,14815,14814,29629,12.932936906814575,0.05839143933812523
7508,15017,15016,30033,13.098574876785278,0.05765924210431666
7608,15217,15216,30433,13.304144859313965,0.056957265862180737
7708,15417,15416,30833,13.459383726119995,0.056277204937750555
7808,15617,15616,31233,13.607781887054443,0.055618162011791754
7908,15817,15816,31633,13.763822793960571,0.05497927928204562
8008,16017,16016,32033,13.923948764801025,0.05435973671268472
8108,16217,16216,32433,14.070174932479858,0.05375875036499129
8208,16417,16416,32833,14.209722757339478,0.05317557080411595
8308,16617,16616,33233,14.377910852432251,0.05260948157732764
8408,16817,16816,33633,14.527161836624146,0.05205979775965061
8509,17019,17018,34037,14.667198896408081,0.051520602630384243
8609,17219,17218,34437,14.805424928665161,0.05100194225340503
8709,17419,17418,34837,14.946286678314209,0.05049780221954439
8809,17619,17618,35237,15.084581851959229,0.05000761065391924
8909,17819,17818,35637,15.242784023284912,0.04953082081910589
9009,18019,18018,36037,15.460799932479858,0.0490669099988507
9109,18219,18218,36437,15.604127883911133,0.04861537842924969
9209,18419,18418,36837,15.74465274810791,0.04817574827537324
9309,18619,18618,37237,15.882848978042603,0.04774756265143859
9409,18819,18818,37637,16.021324634552002,0.047330384682744496
9510,19021,19020,38041,16.160159826278687,0.046919782839293905
9610,19221,19220,38441,16.299185752868652,0.04652348509582251
9710,19421,19420,38841,16.442853689193726,0.04613699192550532
9810,19621,19620,39241,16.590858936309814,0.045759938057866614
9910,19821,19820,39641,16.797423839569092,0.04539197410606611
10010,20021,20020,40041,16.943206787109375,0.04503276584703184
10110,20221,20220,40441,17.084637880325317,0.04468199353306405
10210,20421,20420,40841,17.285278797149658,0.044339351233674364
10310,20621,20620,41241,17.442389965057373,0.04400454620646485
10410,20821,20820,41641,17.603880882263184,0.04367729829589823
10511,21023,21022,42045,17.750391721725464,0.043354175700984134
10611,21223,21222,42445,17.904260873794556,0.04304131812212202
10711,21423,21422,42845,18.059722900390625,0.042735244693531745
10811,21623,21622,43245,18.2131609916687,0.042435720216392636
10911,21823,21822,43645,18.3535258769989,0.04214251944861459
11011,22023,22022,44045,18.494906902313232,0.04185542664905385
11111,22223,22222,44445,18.647389888763428,0.04157423514255881
11211,22423,22422,44845,18.90201497077942,0.04129874690496824
11311,22623,22622,45245,19.060237646102905,0.04102877216721476
11411,22823,22822,45645,19.20056986808777,0.04076412903771575
11512,23025,23024,46049,19.347285985946655,0.04050207375577833
11612,23225,23224,46449,19.486687898635864,0.04024762697357275
11712,23425,23424,46849,19.659742832183838,0.03999800830159963
11812,23625,23624,47249,19.831783771514893,0.0397530639846592
11912,23825,23824,47649,19.984335899353027,0.0395126465017495
12012,24025,24024,48049,20.134594678878784,0.039276614282708754
12112,24225,24224,48449,20.29679584503174,0.03904483143818287
12212,24425,24424,48849,20.456270694732666,0.03881716750231484
12312,24625,24624,49249,20.713943004608154,0.038593497187575036
12412,24825,24824,49649,21.16642475128174,0.03837370015117433
12513,25027,25026,50053,21.46342396736145,0.03815551897529549
12613,25227,25226,50453,21.814056873321533,0.037943162063118596
12713,25427,25426,50853,22.090587854385376,0.0377343438492354
12813,25627,25626,51253,22.246922969818115,0.03752896168757155
12913,25827,25826,51653,22.467447757720947,0.03732691686285719
13013,26027,26026,52053,22.699781894683838,0.03712811441614046
13113,26227,26226,52453,22.897509813308716,0.03693246297857628
13213,26427,26426,52853,23.052035808563232,0.03673987461309662
13313,26627,26626,53253,23.2518208026886,0.03655026466358583
13413,26827,26826,53653,23.421557903289795,0.036363551611200175
13514,27029,27028,54057,23.578909873962402,0.036177831965269316
13614,27229,27228,54457,23.731831789016724,0.03599670707644524
13714,27429,27428,54857,23.925784826278687,0.035818251299561545
13814,27629,27628,55257,24.077009916305542,0.035642394384972687
13914,27829,27828,55657,24.24483299255371,0.03546906859650301
14014,28029,28028,56057,24.426017999649048,0.035298208604007716
14114,28229,28228,56457,24.570894718170166,0.03512975138098166
14214,28429,28428,56857,24.715914964675903,0.034963636106970473
14314,28629,28628,57257,24.868794679641724,0.03479980407454928
14414,28829,28828,57657,25.055131912231445,0.034638198600647346
14515,29031,29030,58061,25.20734477043152,0.0344771813926357
14615,29231,29230,58461,25.3990159034729,0.03431988759353739
14715,29431,29430,58861,25.536054849624634,0.034164661121646143
14815,29631,29630,59261,25.718302965164185,0.03401145260098112
14915,29831,29830,59661,25.872536659240723,0.03386021429396292
15015,30031,30030,60061,26.03413486480713,0.03371090003473227
15115,30231,30230,60461,26.179157972335815,0.033563465165527585
15215,30431,30430,60861,26.346523761749268,0.03341786647597316
15315,30631,30630,61261,26.487440824508667,0.033274062145135605
15415,30831,30830,61661,26.631536722183228,0.03313201168621398
15516,31033,31032,62065,26.812073945999146,0.03299028106538275
15616,31233,31232,62465,27.001683950424194,0.032851638543969136
15716,31433,31432,62865,27.196424961090088,0.03271463556051868
15816,31633,31632,63265,27.376155853271484,0.03257923647112261
15916,31833,31832,63665,27.599483728408813,0.032445406724262195
16016,32033,32032,64065,27.742371797561646,0.03231311281884127
16116,32233,32232,64465,27.913290977478027,0.03218232226407853
16216,32433,32432,64865,28.211784839630127,0.032053003541169474
16316,32633,32632,65265,28.404131650924683,0.03192512606663327
16416,32833,32832,65665,28.559850931167603,0.031798660157263375
16517,33035,33034,66069,28.70042085647583,0.03167233305252099
16617,33235,33234,66469,28.83767604827881,0.031548618067915195
16717,33435,33434,66869,29.009031772613525,0.03142623040467131
16817,33635,33634,67269,29.212663650512695,0.031305143667268095
16917,33835,33834,67669,29.368215799331665,0.031185332206444923
17017,34035,34034,68069,29.507969617843628,0.031066771092305608
17117,34235,34234,68469,29.678935766220093,0.030949436088563275
17217,34435,34434,68869,29.86170792579651,0.030833303627871574
17317,34635,34634,69269,30.009904861450195,0.03071835078819308
17417,34835,34834,69669,30.15048384666443,0.030604555270155195
17518,35037,35036,70073,30.288200855255127,0.03049077443936755
17618,35237,35236,70473,30.424343824386597,0.030379240089852988
17718,35437,35436,70873,30.57048773765564,0.030268799484460148
17818,35637,35636,71273,30.72139072418213,0.030159432611547094
17918,35837,35836,71673,30.877014875411987,0.030051119982023665
18018,36037,36036,72073,31.012609004974365,0.029943842611752463
18118,36237,36236,72473,31.150194883346558,0.029837582004660062
18218,36437,36436,72873,31.29167103767395,0.029732320136525433
18318,36637,36636,73273,31.433238983154297,0.029628039439415943
18418,36837,36836,73673,31.617568016052246,0.02952472278674026
18519,37039,37038,74077,31.826502799987793,0.029421334514460707
18619,37239,37238,74477,31.96522068977356,0.029319905494727717
18719,37439,37438,74877,32.106199741363525,0.029219391490043062
18819,37639,37638,75277,32.26132297515869,0.02911977700493755
18919,37839,37838,75677,32.455671072006226,0.0290210469187723
19019,38039,38038,76077,32.6348557472229,0.028923186473965537
19119,38239,38238,76477,32.826931953430176,0.028826181264669258
19219,38439,38438,76877,32.99612474441528,0.028730017225875572
19319,38639,38638,77277,33.13695573806763,0.028634680622934186
19419,38839,38838,77677,33.28190588951111,0.02854015804146322
19520,39041,39040,78081,33.42279601097107,0.028445503162067013
19620,39241,39240,78481,33.56275200843811,0.028352577430754568
19720,39441,39440,78881,33.707228899002075,0.028260427180378078
19820,39641,39640,79281,33.848108768463135,0.028169040186821117
19920,39841,39840,79681,34.01906991004944,0.028078404501042573
20020,40041,40040,80081,34.19817876815796,0.02798850844102124
20120,40241,40240,80481,34.5095329284668,0.027899340583990836
20220,40441,40440,80881,34.74326777458191,0.027810889758952812
20320,40641,40640,81281,35.125412702560425,0.0277231450394556
20420,40841,40840,81681,35.37105679512024,0.027636095736629403
20521,41043,41042,82085,35.77547788619995,0.02754887117325509
20621,41243,41242,82485,36.02773976325989,0.02746318825043482
20721,41443,41442,82885,36.212889671325684,0.027378169938052893
20821,41643,41642,83285,36.3827338218689,0.02729380643475468
20921,41843,41842,83685,36.630635023117065,0.027210088145362795
21021,42043,42042,84085,36.823121786117554,0.027127005675241785
21121,42243,42242,84485,36.98919486999512,0.02704454982485341
21221,42443,42442,84885,37.25663375854492,0.026962711584495463
21321,42643,42642,85285,37.4508490562439,0.02688148212921685
21421,42843,42842,85685,37.62565302848816,0.02680085281390182
21522,43045,43044,86089,37.77867078781128,0.026720017751774044
21622,43245,43244,86489,37.93336296081543,0.026640569269127282
21722,43445,43444,86889,38.1052508354187,0.026561695942841326
21822,43645,43644,87289,38.28417205810547,0.026483389802738927
21922,43845,43844,87689,38.454025983810425,0.026405643036174768
22022,44045,44044,88089,38.61916494369507,0.02632844798400672
22122,44245,44244,88489,38.77394986152649,0.026251797136695613
22222,44445,44444,88889,38.96636891365051,0.0261756831305289
22322,44645,44644,89289,39.13918900489807,0.026100098743962265
22422,44845,44844,89689,39.35593295097351,0.026025036894076908
22523,45047,45046,90093,39.55876874923706,0.025949747751090577
22623,45247,45246,90493,39.82313799858093,0.025875715317000777
22723,45447,45446,90893,40.024353981018066,0.025802184902548382
22823,45647,45646,91293,40.24172377586365,0.025729149947264905
22923,45847,45846,91693,40.48831272125244,0.02565660401313399
23023,46047,46046,92093,40.69961500167847,0.025584540781652128
23123,46247,46246,92493,40.96152687072754,0.02551295405097718
23223,46447,46446,92893,41.197232723236084,0.025441837733162487
23323,46647,46646,93293,41.3569598197937,0.025371185851471904
23423,46847,46846,93693,41.52293300628662,0.025300992537774306
23524,47049,47048,94097,41.703112840652466,0.025230556892376153
23624,47249,47248,94497,41.85788893699646,0.025161267975363354
23724,47449,47448,94897,42.01358675956726,0.025092420593584127
23824,47649,47648,95297,42.15718078613281,0.025024009289734053
23924,47849,47848,95697,42.29633688926697,0.02495602870315468
24024,48049,48048,96097,42.48435688018799,0.024888473567647323
24124,48249,48248,96497,42.64991474151611,0.02482133870934882
24224,48449,48448,96897,42.79062294960022,0.02475461904466623
24324,48649,48648,97297,42.92878270149231,0.024688309578270222
24424,48849,48848,97697,43.072160959243774,0.024622405401142206
24525,49051,49050,98101,43.211729764938354,0.024556248657786196
24625,49251,49250,98501,43.3509247303009,0.024491144601499665
24725,49451,49450,98901,43.490561723709106,0.024426431560359774
24825,49651,49650,99301,43.6484317779541,0.02436210495290391
24925,49851,49850,99701,43.84451389312744,0.024298160274975812
25025,50051,50050,100101,43.9916558265686,0.02423459309807016
25125,50251,50250,100501,44.14773082733154,0.024171399067722248
25225,50451,50450,100901,44.31429982185364,0.024108573901939583
25325,50651,50650,101301,44.487979888916016,0.024046113389674717
25425,50851,50850,101701,44.67554569244385,0.023984013389337876
25526,51053,51052,102105,44.89056992530823,0.02392165417812958
25626,51253,51252,102505,45.041064977645874,0.02386026655180488
25726,51453,51452,102905,45.18978786468506,0.023799227375991334
25826,51653,51652,103305,45.3525869846344,0.023738532773443066
25926,51853,51852,103705,45.500067710876465,0.023678178929477357
26026,52053,52052,104105,45.65309691429138,0.023618162090702013
26126,52253,52252,104505,45.79879593849182,0.023558478563774094
26226,52453,52452,104905,45.94884777069092,0.023499124714190127
26326,52653,52652,105305,46.08574390411377,0.02344009696510563
26426,52853,52852,105705,46.22511887550354,0.023381391796184488
26527,53055,53054,106109,46.40944480895996,0.02332242348188586
26627,53255,53254,106509,46.56327176094055,0.023264356272731823
26727,53455,53454,106909,46.74500298500061,0.023206601377380873
26827,53655,53654,107309,46.93255972862244,0.02314915549108807
26927,53855,53854,107709,47.089332818984985,0.023092015360258213
27027,54055,54054,108109,47.256129026412964,0.023035177781452802
27127,54255,54254,108509,47.396286964416504,0.02297863960041945
27227,54455,54454,108909,47.58539271354675,0.0229223977111454
27327,54655,54654,109309,47.741039752960205,0.02286644905493228
27427,54855,54854,109709,47.926652908325195,0.02281079061949307
27528,55057,55056,110113,48.08417987823486,0.022754867166964565
27628,55257,55256,110513,48.230151891708374,0.02269978314617838
27728,55457,55456,110913,48.38407278060913,0.02264498055048805
27828,55657,55656,111313,48.5595908164978,0.02259045654505676
27928,55857,55856,111713,48.707963705062866,0.02253620833723805
28028,56057,56056,112113,48.86145377159119,0.022482233175790744
28128,56257,56256,112513,49.02485489845276,0.02242852835011063
28228,56457,56456,112913,49.20037770271301,0.022375091189480067
28328,56657,56656,113313,49.37436485290527,0.022321919062333745
28428,56857,56856,113713,49.5386528968811,0.022269009375541767
28529,57059,57058,114117,49.697630882263184,0.022215834379556394
28629,57259,57258,114517,49.872092962265015,0.02216344450540145
28729,57459,57458,114917,50.023454904556274,0.022111309491241765
28829,57659,57658,115317,50.20407676696777,0.022059426891176334
28929,57859,57858,115717,50.42264175415039,0.02200779429437483
29029,58059,58058,116117,50.60419678688049,0.021956409324448933
29129,58259,58258,116517,50.77872586250305,0.021905269638837623
29229,58459,58458,116917,50.92407488822937,0.021854372928205596
29329,58659,58658,117317,51.0700306892395,0.021803716915854494
29429,58859,58858,117717,51.20922374725342,0.021753299357146268
29530,59061,59060,118121,51.34666681289673,0.021702617411362677
29630,59261,59260,118521,51.50224184989929,0.02165267248112565
29730,59461,59460,118921,51.65288496017456,0.021602959436031792
29830,59661,59660,119321,51.802671909332275,0.02155347615445676
29930,59861,59860,119721,51.94235897064209,0.021504220544126505
30030,60061,60060,120121,52.08350896835327,0.021455190541609447
30130,60261,60260,120521,52.24099779129028,0.021406384111819585
30230,60461,60460,120921,52.411064863204956,0.021357799247529348
30330,60661,60660,121321,52.55040693283081,0.02130943396889251
30430,60861,60860,121721,52.69883179664612,0.02126128632297706
30531,61063,61062,122125,52.837403774261475,0.021212876146774994
30631,61263,61262,122525,52.97602200508118,0.02116516014142918
30731,61463,61462,122925,53.13238883018494,0.021117656048338717
30831,61663,61662,123325,53.284804821014404,0.02107036201798955
30931,61863,61862,123725,53.431501626968384,0.021023276225578362
31031,62063,62062,124125,53.57593393325806,0.020976396870598997
31131,62263,62262,124525,53.712177753448486,0.020929722176436568
31231,62463,62462,124925,53.871914863586426,0.02088325038997014
31331,62663,62662,125325,54.01842379570007,0.020836979781182922
31431,62863,62862,125725,54.17893886566162,0.020790908642780062
31532,63065,63064,126129,54.3364999294281,0.020744577549456095
31632,63265,63264,126529,54.51204872131348,0.02069890227185976
31732,63465,63464,126929,54.66796278953552,0.020653421459079477
31832,63665,63664,127329,54.806551694869995,0.020608133491244754
31932,63865,63864,127729,54.94544792175293,0.020563036769401223
32032,64065,64064,128129,55.08712697029114,0.020518129715171387
32132,64265,64264,128529,55.2261278629303,0.02047341077042082
32232,64465,64464,128929,55.363783836364746,0.02042887839693129
32332,64665,64664,129329,55.50837302207947,0.020384531076080074
32432,64865,64864,129729,55.64882183074951,0.020340367308525002
32533,65067,65066,130133,55.789103746414185,0.020295946711456982
32633,65267,65266,130533,55.931713819503784,0.0202521474268461
32733,65467,65466,130933,56.07023286819458,0.020208527295788953
32833,65667,65666,131333,56.208141803741455,0.02016508489321509
32933,65867,65866,131733,56.35621666908264,0.020121818811844584
33033,66067,66066,132133,56.50940990447998,0.020078727661907103
33133,66267,66266,132533,56.657301902770996,0.020035810070866345
33233,66467,66466,132933,56.80720782279968,0.019993064683148747
33333,66667,66666,133333,56.944931745529175,0.019950490159878407
33433,66867,66866,133733,57.085874795913696,0.01990808517861562
33534,67069,67068,134137,57.22779393196106,0.01986542691085773
33634,67269,67268,134537,57.365620851516724,0.019823358773752874
33734,67469,67468,134937,57.50315070152283,0.019781456294749658
33834,67669,67668,135337,57.64531683921814,0.01973971821479264
33934,67869,67868,135737,57.80676770210266,0.01969814329002546
34034,68069,68068,136137,57.9539840221405,0.01965673029155704
34134,68269,68268,136537,58.09146285057068,0.019615478005232466
34234,68469,68468,136937,58.22878384590149,0.01957438523140732
34334,68669,68668,137337,58.36618375778198,0.019533450784726052
34434,68869,68868,137737,58.50638484954834,0.01949267349390492
34535,69071,69070,138141,58.65211892127991,0.019451646772505105
34635,69271,69270,138541,58.81844401359558,0.019411181877591423
34735,69471,69470,138941,59.03016185760498,0.019370870695762887
34835,69671,69670,139341,59.18880367279053,0.019330712110055045
34935,69871,69870,139741,59.32988476753235,0.01929070501654202
35035,70071,70070,140141,59.481703758239746,0.019250848324141225
35135,70271,70270,140541,59.65912485122681,0.019211140954421377
35235,70471,70470,140941,59.81502079963684,0.019171581841413602
35335,70671,70670,141341,59.968915939331055,0.019132169931426305
35435,70871,70870,141741,60.1289427280426,0.019092904182862837
35536,71073,71072,142145,60.31520986557007,0.019053393089335718
35636,71273,71272,142545,60.45671081542969,0.019014418022354724
35736,71473,71472,142945,60.597020864486694,0.018975586052796825
35836,71673,71672,143345,60.7391459941864,0.018936896185798812
35936,71873,71872,143745,60.87591290473938,0.018898347437725855
36036,72073,72072,144145,61.0247917175293,0.018859938836007395
36136,72273,72272,144545,61.171191692352295,0.018821669418975857
36236,72473,72472,144945,61.30892276763916,0.018783538235707962
36336,72673,72672,145345,61.44645285606384,0.018745544345868635
36436,72873,72872,145745,61.58362293243408,0.018707686819558044
36537,73075,73074,146149,61.72678875923157,0.018669588197242667
36637,73275,73274,146549,61.86574697494507,0.018632001990064116
36737,73475,73474,146949,62.004087686538696,0.018594549408885233
36837,73675,73674,147349,62.141782999038696,0.01855722956416187
36937,73875,73874,147749,62.282848834991455,0.01852004157605496
37037,74075,74074,148149,62.42117667198181,0.0184829845742918
37137,74275,74274,148549,62.55926489830017,0.018446057698029945
37237,74475,74474,148949,62.700498819351196,0.01840926009572327
37337,74675,74674,149349,62.84014177322388,0.01837259092499031
37437,74875,74874,149749,62.97709584236145,0.018336049352484656
37538,75077,75076,150153,63.12242674827576,0.01829927104322115
37638,75277,75276,150553,63.27608275413513,0.018262983458128306
37738,75477,75476,150953,63.4213228225708,0.018226821016144038
37838,75677,75676,151353,63.58037972450256,0.018190782918893998
37938,75877,75876,151753,63.74756979942322,0.01815486837642129
38038,76077,76076,152153,63.911360025405884,0.018119076607069226
38138,76277,76276,152553,64.06628084182739,0.018083406837366
38238,76477,76476,152953,64.20244574546814,0.018047858301911218
38338,76677,76676,153353,64.33897185325623,0.018012430243264033
38438,76877,76876,153753,64.48206281661987,0.017977121911833673
38539,77079,77078,154157,64.62820076942444,0.017941581270695787
38639,77279,77278,154557,64.76527166366577,0.017906511354616263
38739,77479,77478,154957,64.90788578987122,0.017871558955778594
38839,77679,77678,155357,65.04714179039001,0.017836723355001523
38939,77879,77878,155757,65.23844289779663,0.017802003840429306
39039,78079,78078,156157,65.44151782989502,0.017767399707431936
39139,78279,78278,156557,65.62495374679565,0.017732910258507373
39239,78479,78478,156957,65.76462888717651,0.01769853480318475
39339,78679,78678,157357,65.90310382843018,0.01766427265792939
39439,78879,78878,157757,66.04584693908691,0.017630123146049517
39540,79081,79080,158161,66.18773674964905,0.017595745785285163
39640,79281,79280,158561,66.32471585273743,0.017561820646667444
39740,79481,79480,158961,66.46707773208618,0.017528006144959224
39840,79681,79680,159361,66.65527486801147,0.017494301629998436
39940,79881,79880,159761,66.79989504814148,0.017460706458019143
40040,80081,80080,160161,66.97186374664307,0.017427219991566524
40140,80281,80280,160561,67.12818479537964,0.017393841599413325
40240,80481,80480,160961,67.2722659111023,0.017360570656477215
40340,80681,80680,161361,67.42571687698364,0.017327406543740147
40440,80881,80880,161761,67.58071279525757,0.017294348648168065
40541,81083,81082,162165,67.76575994491577,0.017261067371068674
40641,81283,81282,162565,67.95822381973267,0.017228221141340302
40741,81483,81482,162965,68.10752892494202,0.017195479318873882
40841,81683,81682,163365,68.2504346370697,0.017162841313855037
40941,81883,81882,163765,68.3891327381134,0.017130306542071767
41041,82083,82082,164165,68.53026294708252,0.017097874424841997
41141,82283,82282,164565,68.67226982116699,0.017065544388941797
41241,82483,82482,164965,68.85596990585327,0.01703331586653505
41341,82683,82682,165365,69.0464220046997,0.01700118829510394
41441,82883,82882,165765,69.2004599571228,0.01696916111738057
41542,83085,83084,166169,69.35661697387695,0.016936915010264064
41642,83285,83284,166569,69.51279783248901,0.016905087959018444
41742,83485,83484,166969,69.67628288269043,0.016873359655114786
41842,83685,83684,167369,69.82569694519043,0.016841729561671622
41942,83885,83884,167769,69.97501587867737,0.016810197146730238
42042,84085,84084,168169,70.11370086669922,0.016778761883192207
42142,84285,84284,168569,70.2517638206482,0.016747423248758248
42242,84485,84484,168969,70.41540384292603,0.01671618072586743
42342,84685,84684,169369,70.71274375915527,0.016685033801637703
42442,84885,84884,169769,70.88404989242554,0.016653981967807166
42543,85087,85086,170173,71.04432773590088,0.016622715624174927
42643,85287,85286,170573,71.19496870040894,0.016591853402918303
42743,85487,85486,170973,71.3383858203888,0.016561084769496595
42843,85687,85686,171373,71.47724390029907,0.016530409233602147
42943,85887,85886,171773,71.64236283302307,0.01649982630926625
43043,86087,86086,172173,71.80312776565552,0.016469335514805256
43143,86287,86286,172573,71.95533990859985,0.016438936372767995
43243,86487,86486,172973,72.10585761070251,0.016408628409883372
43343,86687,86686,173373,72.28453183174133,0.016378411157009207
43443,86887,86886,173773,72.44390559196472,0.0163482841490817
43544,87089,87088,174177,72.58720898628235,0.016317947004684173
43644,87289,87288,174577,72.73354983329773,0.016287999998496797
43744,87489,87488,174977,72.874107837677,0.016258141861527946
43844,87689,87688,175377,73.0116229057312,0.01622837214457448
43944,87889,87888,175777,73.15029883384705,0.016198690402268984
44044,88089,88088,176177,73.29105877876282,0.01616909619303347
44144,88289,88288,176577,73.42951083183289,0.016139589079034025
44244,88489,88488,176977,73.56735491752625,0.016110168626135502
44344,88689,88688,177377,73.70588684082031,0.016080834403857398
44444,88889,88888,177777,73.84687161445618,0.016051585985330012
44545,89091,89090,178181,74.00267171859741,0.016022131746618748
44645,89291,89290,178581,74.14775776863098,0.015993054516711416
44745,89491,89490,178981,74.2887806892395,0.015964061827038165
44845,89691,89690,179381,74.42463779449463,0.015935153264782634
44945,89891,89890,179781,74.56226181983948,0.015906328420529737
45045,90091,90090,180181,74.69983100891113,0.015877586888225614
45145,90291,90290,180581,74.83955788612366,0.015848928265138035
45245,90491,90490,180981,74.9762818813324,0.015820352151817672
45345,90691,90690,181381,75.11624884605408,0.01579185815205944
45445,90891,90890,181781,75.25440883636475,0.015763445872864972
45546,91093,91092,182185,75.39442992210388,0.01573483202432974
45646,91293,91292,182585,75.53163599967957,0.01570658282740587
45746,91493,91492,182985,75.6684718132019,0.015678414187099022
45846,91693,91692,183385,75.81126093864441,0.015650325722899632
45946,91893,91892,183785,75.94851303100586,0.015622317057323056
46046,92093,92092,184185,76.09194374084473,0.015594387815874732
46146,92293,92292,184585,76.24334478378296,0.015566537627016092
46246,92493,92492,184985,76.38107895851135,0.015538766122130529
46346,92693,92692,185385,76.51947784423828,0.01551107293549019
46446,92893,92892,185785,76.65733289718628,0.01548345770422327
46547,93095,93094,186189,76.80027890205383,0.01545564508256718
46647,93295,93294,186589,76.94225978851318,0.015428185455279256
46747,93495,93494,186989,77.08212995529175,0.015400802708031612
46847,93695,93694,187389,77.22344398498535,0.015373496489083502
46947,93895,93894,187789,77.36382389068604,0.015346266449392422
47047,94095,94094,188189,77.50110173225403,0.015319112242583413
47147,94295,94294,188589,77.64107489585876,0.015292033524919778
47247,94495,94494,188989,77.78159880638123,0.015265029955273198
47347,94695,94694,189389,77.92050099372864,0.015238101195095102
47447,94895,94894,189789,78.05764675140381,0.015211246908387922
47548,95097,95096,190193,78.19446587562561,0.015184199333494748
47648,95297,95296,190593,78.35085272789001,0.015157493732227002
47748,95497,95496,190993,78.490238904953,0.015130861608190426
47848,95697,95696,191393,78.62536764144897,0.015104302635337465
47948,95897,95896,191793,78.7664098739624,0.015077816490033957
48048,96097,96096,192193,78.90308094024658,0.015051402851032878
48148,96297,96296,192593,79.03997373580933,0.015025061399448316
48248,96497,96496,192993,79.177414894104,0.014998791818729911
48348,96697,96696,193393,79.31887173652649,0.014972593794637397
48448,96897,96896,193793,79.45570302009583,0.014946467015215766
48549,97099,97098,194197,79.59435796737671,0.014920150969505643
48649,97299,97298,194597,79.73344278335571,0.014894166457308946
48749,97499,97498,194997,79.87179493904114,0.014868252264343478
48849,97699,97698,195397,80.01256966590881,0.014842408087573906
48949,97899,97898,195797,80.14983081817627,0.014816633626129973
49049,98099,98098,196197,80.29031181335449,0.014790928581283582
49149,98299,98298,196597,80.4366409778595,0.014765292656425929
49249,98499,98498,196997,80.58321571350098,0.014739725557045077
49349,98699,98698,197397,80.72378873825073,0.014714226990703978
49449,98899,98898,197797,80.86993479728699,0.014688796667018477
49550,99101,99100,198201,81.00838279724121,0.014663181016140808
49650,99301,99300,198601,81.14565563201904,0.014637886989959022
49750,99501,99500,199001,81.28639101982117,0.014612660344550686
49850,99701,99700,199401,81.42433786392212,0.014587500797550411
49950,99901,99900,199801,81.56175589561462,0.014562408068540787
50050,100101,100100,200201,81.70142793655396,0.01453738187903176
50150,100301,100300,200601,81.84194684028625,0.014512421952441202
50250,100501,100500,201001,81.98091387748718,0.01448752801407491
50350,100701,100700,201401,82.11768698692322,0.014462699791107488
50450,100901,100900,201801,82.2574577331543,0.014437937012562903
50551,101103,101102,202205,82.39822173118591,0.01441299276149233
50651,101303,101302,202605,82.54064774513245,0.014388360713904908
50751,101503,101502,203005,82.70129990577698,0.014363793306075312
50851,101703,101702,203405,82.84508085250854,0.014339290274256703
50951,101903,101902,203805,82.98545980453491,0.014314851356459529
51051,102103,102102,204205,83.123783826828,0.0142904762924336
51151,102303,102302,204605,83.26370286941528,0.01426616482365087
51251,102503,102502,205005,83.4079339504242,0.014241916693287952
51351,102703,102702,205405,83.5507378578186,0.014217731646209248
51451,102903,102902,205805,83.6874668598175,0.014193609428949962
51552,103105,103104,206209,83.82985806465149,0.014169309508478186
51652,103305,103304,206609,83.96709871292114,0.014145312819084519
51752,103505,103504,207009,84.10930585861206,0.014121378206498671
51852,103705,103704,207409,84.24886298179626,0.014097505423791156
51952,103905,103904,207809,84.38808965682983,0.014073694225622347
52052,104105,104104,208209,84.52569699287415,0.01404994436822647
52152,104305,104304,208609,84.66377973556519,0.014026255609396686
52252,104505,104504,209009,84.82131481170654,0.014002627708469512
52352,104705,104704,209409,84.96163201332092,0.013979060426309933
52452,104905,104904,209809,85.10119986534119,0.013955553525296671
52553,105107,105106,210213,85.24143981933594,0.013931872604684651
52653,105307,105306,210613,85.38179564476013,0.013908486357005244
52753,105507,105506,211013,85.51813578605652,0.013885159784220062
52853,105707,105706,211413,85.65558195114136,0.013861892654632132
52953,105907,105906,211813,85.79571199417114,0.013838684737986525
53053,106107,106106,212213,85.93458676338196,0.013815535805456691
53153,106307,106306,212613,86.07251977920532,0.013792445629630744
53253,106507,106506,213013,86.21053075790405,0.013769413984498097
53353,106707,106706,213413,86.35120368003845,0.013746440645436255
53453,106907,106906,213813,86.4904727935791,0.013723525389197551
53554,107109,107108,214217,86.64728283882141,0.013700439711393808
53654,107309,107308,214617,86.79507875442505,0.01367764053178866
53754,107509,107508,215017,86.94529485702515,0.013654898771199535
53854,107709,107708,215417,87.09095597267151,0.013632214211764027
53954,107909,107908,215817,87.2293848991394,0.01360958663693127
54054,108109,108108,216217,87.3709008693695,0.013587015831450056
54154,108309,108308,216617,87.51129078865051,0.013564501581356529
54254,108509,108508,217017,87.65002393722534,0.01354204367396259
54354,108709,108708,217417,87.79390382766724,0.013519641897843921
54454,108909,108908,217817,87.93157076835632,0.013497296042828549
54555,109111,109110,218221,88.07498598098755,0.013474783279199671
54655,109311,109310,218621,88.21859669685364,0.01345254919482705
54755,109511,109510,219021,88.35911178588867,0.01343037040638306
54855,109711,109710,219421,88.49843668937683,0.013408246708603739
54955,109911,109910,219821,88.63758182525635,0.013386177897421475
55055,110111,110110,220221,88.77845191955566,0.013364163769954158
55155,110311,110310,220621,88.92056775093079,0.013342204124494349
55255,110511,110510,221021,89.0675618648529,0.013320298760499127
55355,110711,110710,221421,89.21735978126526,0.013298447478579412
55455,110911,110910,221821,89.35700678825378,0.013276650080489637
55556,111113,111112,222225,89.49939584732056,0.013254689202457986
55656,111313,111312,222625,89.6375527381897,0.013232999515736827
55756,111513,111512,223025,89.77822470664978,0.013211363122926699
55856,111713,111712,223425,89.91657185554504,0.013189779830267258
55956,111913,111912,223825,90.05492782592773,0.013168249445091837
56056,112113,112112,224225,90.1920657157898,0.01314677177581818
56156,112313,112312,224625,90.33183002471924,0.01312534663193894
56256,112513,112512,225025,90.470529794693,0.013103973824012185
56356,112713,112712,225425,90.60774278640747,0.013082653163652267
56456,112913,112912,225825,90.75121569633484,0.013061384463520571
56557,113115,113114,226229,90.8914487361908,0.013039955628885188
56657,113315,113314,226629,91.03177690505981,0.013018790806291975
56757,113515,113514,227029,91.1712429523468,0.01299767738626663
56857,113715,113714,227429,91.32769203186035,0.012976615185579705
56957,113915,113914,227829,91.46569275856018,0.012955604022004623
57057,114115,114114,228229,91.63544297218323,0.01293464371430911
57157,114315,114314,228629,91.77768874168396,0.012913734082246801
57257,114515,114514,229029,91.94290471076965,0.012892874946548923
57357,114715,114714,229429,92.08070969581604,0.012872066128916037
57457,114915,114914,229829,92.21828985214233,0.012851307452009776
57558,115117,115116,230233,92.35990786552429,0.012830391904044983
57658,115317,115316,230633,92.49860572814941,0.012809733477388006
57758,115517,115516,231033,92.63767886161804,0.012789124663389556
57858,115717,115716,231433,92.77529883384705,0.012768565288485622
57958,115917,115916,231833,92.91642594337463,0.012748055180034057
58058,116117,116116,232233,93.05344891548157,0.012727594166306812
58158,116317,116316,232633,93.19206285476685,0.012707182076482379
58258,116517,116516,233033,93.33506083488464,0.012686818740638432
58358,116717,116716,233433,93.4882140159607,0.012666503989744518
58458,116917,116916,233833,93.62648701667786,0.012646237655654704
58559,117119,117118,234237,93.76618385314941,0.01262581763335122
58659,117319,117318,234637,93.90521192550659,0.012605648111927934
58759,117519,117518,235037,94.04511570930481,0.01258552650645551
58859,117719,117718,235437,94.18263387680054,0.012565452652263543
58959,117919,117918,235837,94.32349276542664,0.01254542638553089
59059,118119,118118,236237,94.46427965164185,0.012525447543278976
59159,118319,118318,236637,94.60693573951721,0.012505515963364805
59259,118519,118518,237037,94.77573490142822,0.012485631484474713
59359,118719,118718,237437,94.9169328212738,0.012465793946117406
59459,118919,118918,237837,95.07843089103699,0.012446003188617685
59560,119121,119120,238241,95.22105765342712,0.012426061846660291
59660,119321,119320,238641,95.35716462135315,0.01240636463892564
59760,119521,119520,239041,95.50209999084473,0.012386713736286269
59860,119721,119720,239441,95.6588728427887,0.01236710898227509
59960,119921,119920,239841,95.79935574531555,0.012347550221209671
60060,120121,120120,240241,95.93604874610901,0.01232803729818582
60160,120321,120320,240641,96.0763750076294,0.012308570059071607
60260,120521,120520,241041,96.21327090263367,0.012289148350501572
60360,120721,120720,241441,96.3504786491394,0.01226977201987071
60460,120921,120920,241841,96.48836398124695,0.012250440915328632
60561,121123,121122,242245,96.62880682945251,0.012230962252597479
60661,121323,121322,242645,96.77012085914612,0.01221172159616075
60761,121523,121522,243045,96.90875482559204,0.012192525713239316
60861,121723,121722,243445,97.05182886123657,0.012173374454951404
60961,121923,121922,243845,97.19072270393372,0.01215426767314145
61061,122123,122122,244245,97.32937288284302,0.012135205220374895
61161,122323,122322,244645,97.46736097335815,0.012116186949932379
61261,122523,122522,245045,97.61078667640686,0.012097212715804754
61361,122723,122722,245445,97.76535177230835,0.012078282372687483
61461,122923,122922,245845,97.94205284118652,0.01205939577597569
61562,123125,123124,246249,98.08090806007385,0.012040364571523868
61662,123325,123324,246649,98.21970582008362,0.0120215654704518
61762,123525,123524,247049,98.35911178588867,0.012002809684693572
61862,123725,123724,247449,98.49649095535278,0.011984097072397587
61962,123925,123924,247849,98.63636684417725,0.011965427492386235
62062,124125,124124,248249,98.77209973335266,0.011946800804150993
62162,124325,124324,248649,98.9133780002594,0.011928216867847589
62262,124525,124524,249049,99.05206990242004,0.011909675544291117
62362,124725,124724,249449,99.18971586227417,0.011891176694951261
62462,124925,124924,249849,99.32772469520569,0.011872720181947644
62563,125127,125126,250253,99.46958065032959,0.011854121937548822
62663,125327,125326,250653,99.64305186271667,0.011835750106090122
62763,125527,125526,251053,99.78349685668945,0.011817420199822857
62863,125727,125726,251453,99.96423196792603,0.011799132083426103
62963,125927,125926,251853,100.10282492637634,0.011780885622206022
63063,126127,126126,252253,100.2392578125,0.011762680682091079
63163,126327,126326,252653,100.3802878856659,0.011744517129627865
63263,126527,126526,253053,100.51718664169312,0.011726394831976827
63363,126727,126726,253453,100.65838885307312,0.011708313656907696
63463,126927,126926,253853,100.81118583679199,0.011690273472795353
63564,127129,127128,254257,100.95366978645325,0.011672094361274773
63664,127329,127328,254657,101.1182427406311,0.011654136173238737
63764,127529,127528,255057,101.26480793952942,0.011636218583577785
63864,127729,127728,255457,101.40157175064087,0.011618341463051452
63964,127929,127928,255857,101.56029987335205,0.011600504683003719
64064,128129,128128,256257,101.71345090866089,0.011582708115358976
64164,128329,128328,256657,101.86260199546814,0.011564951632618016
64264,128529,128528,257057,102.02452182769775,0.011547235107853984
64364,128729,128728,257457,102.1772358417511,0.011529558414708816
64464,128929,128928,257857,102.31560707092285,0.011511921427388995
64565,129131,129130,258261,102.45570778846741,0.011494148246054431
64665,129331,129330,258661,102.59349083900452,0.011476590689176235
64765,129531,129530,259061,102.77000188827515,0.011459072462854887
64865,129731,129730,259461,102.91005802154541,0.011441593443523404
64965,129931,129930,259861,103.04665398597717,0.011424153508160761
65065,130131,130130,260261,103.18808078765869,0.011406752534288241
65165,130331,130330,260661,103.32536482810974,0.011389390399965822
65265,130531,130530,261061,103.46353101730347,0.011372066983788637
65365,130731,130730,261461,103.5998227596283,0.011354782164883313
65465,130931,130930,261861,103.73961091041565,0.011337535822904688
65566,131133,131132,262265,103.87689280509949,0.011320155951482764
65666,131333,131332,262665,104.01487374305725,0.011302986586194321
65766,131533,131532,263065,104.15892386436462,0.011285855338745761
65866,131733,131732,263465,104.30894684791565,0.011268762090875073
65966,131933,131932,263865,104.44644093513489,0.011251706724831254
66066,132133,132132,264265,104.58685493469238,0.011234689123371028
66166,132333,132332,264665,104.72724199295044,0.011217709169755707
66266,132533,132532,265065,104.86812376976013,0.011200766747747691
66366,132733,132732,265465,105.00647974014282,0.011183861741607555
66466,132933,132932,265865,105.14606285095215,0.011166994036090673
66567,133135,133134,266269,105.28568291664124,0.011149995398649155
66667,133335,133334,266669,105.42239093780518,0.01113320232074906
66767,133535,133534,267069,105.55910181999207,0.011116446199540608
66867,133735,133734,267469,105.70390772819519,0.011099726921732184
66967,133935,133934,267869,105.84437680244446,0.011083044374511446
67067,134135,134134,268269,105.98192262649536,0.011066398445542447
67167,134335,134334,268669,106.12137484550476,0.011049789022962631
67267,134535,134534,269069,106.26188278198242,0.011033215995379778
67367,134735,134734,269469,106.41705393791199,0.011016679251869298
67467,134935,134934,269869,106.55633878707886,0.0110001786819711
67568,135137,135136,270273,106.70031690597534,0.010983549712374231
67668,135337,135336,270673,106.83987474441528,0.010967121519153593
67768,135537,135536,271073,106.97951483726501,0.010950729169835593
67868,135737,135736,271473,107.1165509223938,0.010934372555794594
67968,135937,135936,271873,107.2581148147583,0.010918051568855542
68068,136137,136136,272273,107.39563584327698,0.010901766101291118
68168,136337,136336,272673,107.53469061851501,0.01088551604581895
68268,136537,136536,273073,107.67404699325562,0.010869301295599118
68368,136737,136736,273473,107.81630897521973,0.010853121744231246
68468,136937,136936,273873,107.95468592643738,0.010836977285752086
68569,137139,137138,274277,108.09551477432251,0.010820706896251716
68669,137339,137338,274677,108.23859882354736,0.010804632655688488
68769,137539,137538,275077,108.40253067016602,0.010788593191675569
68869,137739,137738,275477,108.58923292160034,0.010772588399976161
68969,137939,137938,275877,108.7675929069519,0.010756618176777446
69069,138139,138138,276277,108.94416189193726,0.01074068241868826
69169,138339,138338,276677,109.09804391860962,0.010724781022736616
69269,138539,138538,277077,109.2518846988678,0.010708913886367213
69369,138739,138738,277477,109.40329074859619,0.010693080907438939
69469,138939,138938,277877,109.5542049407959,0.010677281984222546
69570,139141,139140,278281,109.75689601898193,0.0106613595368379
69670,139341,139340,278681,109.92366886138916,0.010645628759519424
69770,139541,139540,279081,110.06901097297668,0.010629931734169071
69870,139741,139740,279481,110.21507406234741,0.010614268360685181
69970,139941,139940,279881,110.3663239479065,0.01059863853936608
70070,140141,140140,280281,110.52392983436584,0.010583042170907768
70170,140341,140340,280681,110.69974398612976,0.010567479156401759
70270,140541,140540,281081,110.8492968082428,0.010551949397332722
70370,140741,140740,281481,110.99821996688843,0.01053645279557633
70470,140941,140940,281881,111.15212798118591,0.01052098925339699
70571,141143,141142,282285,111.31580591201782,0.010505404533777012
70671,141343,141342,282685,111.5100679397583,0.010490007147253242
70771,141543,141542,283085,111.66594099998474,0.010474642528446447
70871,141743,141742,283485,111.82035779953003,0.010459310581157993
70971,141943,141942,283885,111.95671772956848,0.010444011209567077
71071,142143,142142,284285,112.09353804588318,0.010428744318228945
71171,142343,142342,284685,112.22856783866882,0.01041350981207237
71271,142543,142542,285085,112.36564302444458,0.010398307596397902
71371,142743,142742,285485,112.50172591209412,0.010383137576875551
71471,142943,142942,285885,112.64160895347595,0.010367999659543051
71572,143145,143144,286289,112.79064989089966,0.010352742853043743
71672,143345,143344,286689,112.94397902488708,0.010337669178347931
71772,143545,143544,287089,113.08701586723328,0.010322627325213274
71872,143745,143744,287489,113.25189185142517,0.010307617201131205
71972,143945,143944,287889,113.40697979927063,0.010292638713950824
72072,144145,144144,288289,113.56158065795898,0.01027769177187676
72172,144345,144344,288689,113.70505595207214,0.010262776283467645
72272,144545,144544,289089,113.84617376327515,0.010247892157633672
72372,144745,144744,289489,113.98944282531738,0.010233039303635262
72472,144945,144944,289889,114.13925766944885,0.01021821763108069
72573,145147,145146,290293,114.28895592689514,0.010203279300820748
72673,145347,145346,290693,114.42805075645447,0.010188520030927118
72773,145547,145546,291093,114.57385683059692,0.010173791672480472
72873,145747,145746,291493,114.71752882003784,0.010159094136466484
72973,145947,145946,291893,114.85452270507812,0.010144427334209621
73073,146147,146146,292293,115.00177001953125,0.01012979117737153
73173,146347,146346,292693,115.15779781341553,0.010115185577949172
73273,146547,146546,293093,115.30930376052856,0.01010061044827318
73373,146747,146746,293493,115.47174382209778,0.010086065701005903
73473,146947,146946,293893,115.66998887062073,0.010071551249139847
73574,147149,147148,294297,115.83818078041077,0.01005692231582622
73674,147349,147348,294697,116.00149297714233,0.010042468495840836
73774,147549,147548,295097,116.17995977401733,0.010028044711339279
73874,147749,147748,295497,116.33520674705505,0.010013650876620636
73974,147949,147948,295897,116.49309802055359,0.009999286906305714
74074,148149,148148,296297,116.65278697013855,0.00998495271533535
74174,148349,148348,296697,116.83286094665527,0.009970648218968625
74274,148549,148548,297097,116.99748873710632,0.0099563733327815
74374,148749,148748,297497,117.14688181877136,0.009942127972664876
74474,148949,148948,297897,117.32297492027283,0.00992791205482332
74575,149151,149150,298301,117.47866797447205,0.009913583778163
74675,149351,149350,298701,117.62337279319763,0.009899426787068365
74775,149551,149550,299101,117.77438068389893,0.009885298987900538
74875,149751,149750,299501,117.93020272254944,0.009871200298105322
74975,149951,149950,299901,118.0708179473877,0.009857130635434221
75075,150151,150150,300301,118.22449684143066,0.009843089917942964
75175,150351,150350,300701,118.37483477592468,0.00982907806398986
75275,150551,150550,301101,118.53635573387146,0.00981509499223439
75375,150751,150750,301501,118.6850597858429,0.009801140621635535
75475,150951,150950,301901,118.83643579483032,0.009787214871450541
75576,151153,151152,302305,118.99709677696228,0.009773178832986541
75676,151353,151352,302705,119.15059566497803,0.009759310366780592
75776,151553,151552,303105,119.29952692985535,0.009745470279737227
75876,151753,151752,303505,119.46893787384033,0.009731658492294576
75976,151953,151952,303905,119.63007998466492,0.0097178749251816
76076,152153,152152,304305,119.78420686721802,0.009704119499416724
76176,152353,152352,304705,119.94194793701172,0.009690392136306415
76276,152553,152552,305105,120.11048769950867,0.009676692757443756
76376,152753,152752,305505,120.26459169387817,0.00966302128470716
76476,152953,152952,305905,120.42042088508606,0.009649377640258878
76577,153155,153154,306309,120.57404685020447,0.009635625727486065
76677,153355,153354,306709,120.72712874412537,0.009622037783575196
76777,153555,153554,307109,120.88072776794434,0.009608477435360597
76877,153755,153754,307509,121.07538890838623,0.009594944606129162
76977,153955,153954,307909,121.2291738986969,0.009581439219445069
77077,154155,154154,308309,121.38247489929199,0.009567961199148232
77177,154355,154354,308709,121.55996894836426,0.009554510469353053
77277,154555,154554,309109,121.71825385093689,0.009541086954447145
77377,154755,154754,309509,121.86335182189941,0.00952769057909001
77477,154955,154954,309909,122.00274300575256,0.009514321268211777
77578,155157,155156,310313,122.14138579368591,0.009500845659845384
77678,155357,155356,310713,122.27969884872437,0.00948753052256744
77778,155557,155556,311113,122.41613984107971,0.009474242225428524
77878,155757,155756,311513,122.55758380889893,0.009460980694431215
77978,155957,155956,311913,122.69669771194458,0.009447745855842505
78078,156157,156156,312313,122.83424162864685,0.009434537636192349
78178,156357,156356,312713,122.97447967529297,0.009421355962272702
78278,156557,156556,313113,123.11390280723572,0.00940820076113614
78378,156757,156756,313513,123.25173497200012,0.00939507196009464
78478,156957,156956,313913,123.38852405548096,0.00938196948671854
78579,157159,157158,314317,123.52968692779541,0.009368762639003063
78679,157359,157358,314717,123.68610095977783,0.009355712866169126
78779,157559,157558,315117,123.83247780799866,0.009342689204533832
78879,157759,157758,315517,123.97322487831116,0.009329691582691197
78979,157959,157958,315917,124.11330199241638,0.00931671992948766
79079,158159,158158,316317,124.25182390213013,0.009303774174020951
79179,158359,158358,316717,124.3929808139801,0.009290854245638795
79279,158559,158558,317117,124.53407263755798,0.009277960073937962
79379,158759,158758,317517,124.6854977607727,0.00926509158876296
79479,158959,158958,317917,124.84223365783691,0.009252248720205199
79580,159161,159160,318321,124.98527693748474,0.009239303354162473
79680,159361,159360,318721,125.1247878074646,0.009226511764519909
79780,159561,159560,319121,125.27179288864136,0.009213745582547072
79880,159761,159760,319521,125.4353289604187,0.009201004739313621
79980,159961,159960,319921,125.58103585243225,0.009188289166130226
80080,160161,160160,320321,125.76985883712769,0.009175598794547902
80180,160361,160360,320721,125.92865085601807,0.009162933556356601
80280,160561,160560,321121,126.06532192230225,0.0091502933835844
80380,160761,160760,321521,126.20504093170166,0.009137678208496288
80480,160961,160960,321921,126.37630796432495,0.009125087963593204
80581,161163,161162,322325,126.54357767105103,0.009112397053121802
80681,161363,161362,322725,126.6927638053894,0.00909985671465115
80781,161563,161562,323125,126.85636782646179,0.009087341104606664
80881,161763,161762,323525,127.00050377845764,0.009074850156424858
80981,161963,161962,323925,127.16283392906189,0.00906238380377307
81081,162163,162162,324325,127.30944776535034,0.009049941980548438
81181,162363,162362,324725,127.47383284568787,0.00903752462087687
81281,162563,162562,325125,127.63724899291992,0.00902513165911197
81381,162763,162762,325525,127.77361989021301,0.009012763029834198
81481,162963,162962,325925,127.9265558719635,0.009000418667849718
81582,163165,163164,326329,128.0838499069214,0.008987975428595498
81682,163365,163364,326729,128.248596906662,0.008975679647564273
81782,163565,163564,327129,128.40805673599243,0.008963407938945957
81882,163765,163764,327529,128.5775318145752,0.008951160238442469
81982,163965,163964,327929,128.71837186813354,0.008938936481976746
82082,164165,164164,328329,128.86724972724915,0.008926736605691652
82182,164365,164364,328729,129.00679683685303,0.00891456054594913
82282,164565,164564,329129,129.1476287841797,0.008902408239329317
82382,164765,164764,329529,129.28996300697327,0.008890279622629579
82482,164965,164964,329929,129.44888281822205,0.008878174632863426
82583,165167,165166,330333,129.60233688354492,0.008865972511791073
82683,165367,165366,330733,129.75061082839966,0.008853914822494502
82783,165567,165566,331133,129.92469787597656,0.00884188057183861
82883,165767,165766,331533,130.08220791816711,0.00882986969769517
82983,165967,165966,331933,130.26175999641418,0.008817882138147685
83083,166167,166166,332333,130.41188097000122,0.008805917831490507
83183,166367,166366,332733,130.56286001205444,0.008793976716227883
83283,166567,166566,333133,130.7161328792572,0.008782058731073293
83383,166767,166766,333533,130.86024284362793,0.008770163814948245
83483,166967,166966,333933,131.00860285758972,0.008758291906981772
83584,167169,167168,334337,131.15351176261902,0.008746324572584651
83684,167369,167368,334737,131.2997727394104,0.008734498727712887
83784,167569,167568,335137,131.45223593711853,0.008722695709020326
83884,167769,167768,335537,131.62589287757874,0.008710915456458839
83984,167969,167968,335937,131.79679107666016,0.008699157910183178
84084,168169,168168,336337,131.96790599822998,0.008687423010550298
84184,168369,168368,336737,132.14559173583984,0.008675710698118596
84284,168569,168568,337137,132.31141781806946,0.008664020913647038
84384,168769,168768,337537,132.4697687625885,0.008652353598094296
84484,168969,168968,337937,132.6296796798706,0.008640708692617936
84585,169171,169170,338341,132.77779984474182,0.008628970025709922
84685,169371,169370,338741,132.92731285095215,0.008617369987285886
84785,169571,169570,339141,133.07367181777954,0.008605792183014695
84885,169771,169770,339541,133.2280478477478,0.008594236554843345
84985,169971,169970,339941,133.3905599117279,0.008582703044913742
85085,170171,170170,340341,133.5473599433899,0.008571191595561807
85185,170371,170370,340741,133.7092628479004,0.008559702149316813
85285,170571,170570,341141,133.85274696350098,0.008548234648900484
85385,170771,170770,341541,133.99913382530212,0.008536789037226163
85485,170971,170970,341941,134.13839983940125,0.00852536525739832
85586,171173,171172,342345,134.27999472618103,0.008513849342437672
85686,171373,171372,342745,134.45551776885986,0.008502469273277233
85786,171573,171572,343145,134.6391658782959,0.00849111086585197
85886,171773,171772,343545,134.783344745636,0.008479774064024255
85986,171973,171972,343945,134.94074082374573,0.008468458811843493
86086,172173,172172,344345,135.116516828537,0.008457165053545518
86186,172373,172372,344745,135.27833771705627,0.00844589273355175
86286,172573,172572,345145,135.43167686462402,0.008434641796468531
86386,172773,172772,345545,135.5699577331543,0.008423412187086277
86486,172973,172972,345945,135.71678471565247,0.008412203850378878
86587,173175,173174,346349,135.85392379760742,0.008400904967279037
86687,173375,173374,346749,135.9954957962036,0.008389739222929127
86787,173575,173574,347149,136.13379788398743,0.008378594586724877
86887,173775,173774,347549,136.28429579734802,0.008367471004368328
86987,173975,173974,347949,136.44430685043335,0.008356368421741254
87087,174175,174174,348349,136.59942078590393,0.008345286784904541
87187,174375,174374,348749,136.7954568862915,0.008334226040097426
87287,174575,174574,349149,136.9629566669464,0.00832318613373682
87387,174775,174774,349549,137.13307070732117,0.008312167012416565
87487,174975,174974,349949,137.2737488746643,0.008301168622906842
87588,175177,175176,350353,137.41599583625793,0.008290081239294492
87688,175377,175376,350753,137.56180477142334,0.008279124360410202
87788,175577,175576,351153,137.71506786346436,0.008268188054171297
87888,175777,175776,351553,137.86152982711792,0.008257272268047962
87988,175977,175976,351953,138.01831483840942,0.008246376949683042
88088,176177,176176,352353,138.17918491363525,0.008235502046891623
88188,176377,176376,352753,138.33376169204712,0.008224647507660221
88288,176577,176576,353153,138.50806975364685,0.008213813280146202
88388,176777,176776,353553,138.65686178207397,0.00820299931267709
88488,176977,176976,353953,138.8043828010559,0.008192205553749962
88589,177179,177178,354357,138.9593858718872,0.008181324317634046
88689,177379,177378,354757,139.1055588722229,0.008170571022759168
88789,177579,177578,355157,139.24058389663696,0.008159837782418624
88889,177779,177778,355557,139.37818479537964,0.008149124545782496
88989,177979,177978,355957,139.5398018360138,0.008138431262187258
89089,178179,178178,356357,139.85568475723267,0.008127757881134784
89189,178379,178378,356757,140.03038692474365,0.00811710435229215
89289,178579,178578,357157,140.19322180747986,0.008106470625490499
89389,178779,178778,357557,140.35840678215027,0.00809585665072483
89489,178979,178978,357957,140.5411388874054,0.008085262378153189
89590,179181,179180,358361,140.74852776527405,0.008074582110972974
89690,179381,179380,358761,140.92117977142334,0.008064027289693009
89790,179581,179580,359161,141.14886665344238,0.008053492021560556
89890,179781,179780,359561,141.31525182724,0.008042976257381264
89990,179981,179980,359961,141.476069688797,0.00803247994812076
90090,180181,180180,360361,141.6473789215088,0.008022003044904101
90190,180381,180380,360761,141.8068187236786,0.008011545499014991
90290,180581,180580,361161,141.97564792633057,0.008001107261895308
90390,180781,180780,361561,142.14224791526794,0.007990688285144496
90490,180981,180980,361961,142.30378985404968,0.007980288520518969
90591,181183,181182,362365,142.46888875961304,0.007969804210541661
90691,181383,181382,362765,142.62367177009583,0.007959442916980157
90791,181583,181582,363165,142.79148173332214,0.00794910069127186
90891,181783,181782,363565,142.98132872581482,0.007938777485796538
90991,181983,181982,363965,143.16447162628174,0.007928473253087964
91091,182183,182182,364365,143.34598183631897,0.007918187945833367
91191,182383,182382,364765,143.52281379699707,0.007907921516872833
91291,182583,182582,365165,143.68189001083374,0.007897673919198569
91391,182783,182782,365565,143.85624885559082,0.007887445105954636
91491,182983,182982,365965,144.01464176177979,0.007877235030436138
91592,183185,183184,366369,144.170649766922,0.007866941826478525
91692,183385,183384,366769,144.32359886169434,0.0078567692731117
91792,183585,183584,367169,144.50121188163757,0.00784661531779491
91892,183785,183784,367569,144.67777585983276,0.007836479914423562
91992,183985,183984,367969,144.8327558040619,0.007826363017041432
92092,184185,184184,368369,145.00227880477905,0.007816264579839964
92192,184385,184384,368769,145.18119978904724,0.007806184557157917
92292,184585,184584,369169,145.3630018234253,0.0077961229034805455
92392,184785,184784,369569,145.52877593040466,0.007786079573439365
92492,184985,184984,369969,145.93147373199463,0.007776054521811322
92593,185187,185186,370373,146.18923687934875,0.0077659477272617955
92693,185387,185386,370773,146.42428994178772,0.007755959279028298
92793,185587,185586,371173,146.88805294036865,0.00774598897395979
92893,185787,185786,371573,147.36049103736877,0.007736036767411587
92993,185987,185986,371973,147.71583676338196,0.007726102614881864
93093,186187,186186,372373,147.96683478355408,0.00771618647201114
93193,186387,186386,372773,148.20012068748474,0.007706288294581779
93293,186587,186586,373173,148.3766577243805,0.007696408038517362
93393,186787,186786,373573,148.6666738986969,0.007686545659882374
93493,186987,186986,373973,148.8832356929779,0.007676701114881473
93594,187189,187188,374377,149.0786018371582,0.007666776182000901
93694,187389,187388,374777,149.2723948955536,0.007656967350685936
93794,187589,187588,375177,149.469340801239,0.0076471762220223765
93894,187789,187788,375577,149.66383171081543,0.007637402752772151
93994,187989,187988,375977,149.84480786323547,0.007627646899834897
94094,188189,188188,376377,149.99498963356018,0.007617908620247393
94194,188389,188388,376777,150.15068697929382,0.0076081878711831774
94294,188589,188588,377177,150.30525588989258,0.007598484609951875
94394,188789,188788,377577,150.44918990135193,0.007588798793998877
94494,188989,188988,377977,150.60815000534058,0.007579130380904666
94595,189191,189190,378381,150.7547047138214,0.007569382905387485
94695,189391,189390,378781,150.89684581756592,0.007559749344262658
94795,189591,189590,379181,151.08981776237488,0.007550133059124971
94895,189791,189790,379581,151.2778959274292,0.0075405340080920945
94995,189991,189990,379981,151.46065998077393,0.007530952149414454
95095,190191,190190,380381,151.66411805152893,0.007521387441474787
95195,190391,190390,380781,151.8393428325653,0.007511839842787465
95295,190591,190590,381181,152.03225684165955,0.0075023093119982445
95395,190791,190790,381581,152.18784165382385,0.007492795807883659
95495,190991,190990,381981,152.338223695755,0.007483299289350599
95596,191193,191192,382385,152.50071501731873,0.00747372500512869
95696,191393,191392,382785,152.6608738899231,0.007464262503830366
95796,191593,191592,383185,152.8243477344513,0.007454816865205057
95896,191793,191792,383585,152.98349380493164,0.007445388048677621
95996,191993,191992,383985,153.1467640399933,0.007435976013800798
96096,192193,192192,384385,153.3053708076477,0.007426580720254902
96196,192393,192392,384785,153.4774248600006,0.00741720212784732
96296,192593,192592,385185,153.63528776168823,0.00740784019651204
96396,192793,192792,385585,153.78881001472473,0.00739849488630915
96496,192993,192992,385985,154.19797086715698,0.007389166157424452
96597,193195,193194,386389,154.39213490486145,0.007379760931697754
96697,193395,193394,386789,154.53018188476562,0.007370465411328744
96797,193595,193594,387189,154.67356896400452,0.007361186353191253
96897,193795,193794,387589,154.81192874908447,0.0073519237179705925
96997,193995,193994,387989,155.01846885681152,0.007342677466475559
97097,194195,194194,388389,155.2080478668213,0.007333447559637854
97197,194395,194394,388789,155.36803770065308,0.007324233958511813
97297,194595,194594,389189,155.5416009426117,0.0073150366242738735
97397,194795,194794,389589,155.6977777481079,0.007305855518222141
97497,194995,194994,389989,155.83943486213684,0.007296690601775942
97598,195197,195196,390393,155.97863602638245,0.007287450430255907
97698,195397,195396,390793,156.1172788143158,0.0072783179386965826
97798,195597,195596,391193,156.2650008201599,0.007269201521342371
97898,195797,195796,391593,156.41580963134766,0.007260101140094465
97998,195997,195996,391993,156.55590987205505,0.007251016756973199
98098,196197,196196,392393,156.70049571990967,0.007241948334117486
98198,196397,196396,392793,156.84124064445496,0.007232895833784522
98298,196597,196596,393193,156.9839518070221,0.007223859218349286
98398,196797,196796,393593,157.12638902664185,0.007214838450304185
98498,196997,196996,393993,157.26476073265076,0.007205833492258538
98599,197199,197198,394397,157.40242886543274,0.007196754494611566
98699,197399,197398,394797,157.5398347377777,0.007187781202027244
98799,197599,197598,395197,157.6781439781189,0.007178823607598379
98899,197799,197798,395597,157.81642293930054,0.0071698816743992365
98999,197999,197998,395997,157.9548478126526,0.007160955365619003
99099,198199,198198,396397,158.09150981903076,0.007152044644561347
99199,198399,198398,396797,158.2294316291809,0.007143149474644061
99299,198599,198598,397197,158.36894369125366,0.007134269819398599
99399,198799,198798,397597,158.52389287948608,0.0071254056424696855
99499,198999,198998,397997,158.66252779960632,0.007116556907614964
99600,199201,199200,398401,158.8016209602356,0.0071076353230935165
99700,199401,199400,398801,158.93969583511353,0.007098817517627355
99800,199601,199600,399201,159.07932376861572,0.007090015045823082
99900,199801,199800,399601,159.21761679649353,0.007081227871886953
100000,200001,200000,400001,159.35746574401855,0.007072455960136204


==> plot_data/quadratic_minimax_problem_n500_alpha0/flex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007658004760742188,30.358099469249375
100,459,0,459,0.7737970352172852,0.4215230331922254
200,946,0,946,1.682675838470459,0.14415849683191745
300,1439,0,1439,2.456393003463745,0.08296605369719261
400,1934,0,1934,3.3106391429901123,0.062152216402440015
501,2439,0,2439,4.015656232833862,0.05516804045776081
601,2936,0,2936,4.708676099777222,0.04367911425214777
701,3436,0,3436,5.647229194641113,0.04257054126154854
801,3934,0,3934,7.0424559116363525,0.03609704005457046
901,4433,0,4433,8.301010847091675,0.03464549120420115
1001,4931,0,4931,9.518473863601685,0.027923755909865604
1101,5431,0,5431,10.941987991333008,0.027367716864216383
1201,5930,0,5930,12.25145697593689,0.02563948412180267
1301,6430,0,6430,13.408919095993042,0.024929295322853623
1401,6925,0,6925,14.608083009719849,0.018852531343604755
1502,7430,0,7430,15.793203115463257,0.017711548583424178
1602,7930,0,7930,16.942715167999268,0.01744872389806109
1702,8430,0,8430,18.04382300376892,0.017277335657916865
1802,8929,0,8929,19.158313035964966,0.01624345545841913
1902,9429,0,9429,20.258270978927612,0.015892218609013832
2002,9925,0,9925,21.372305154800415,0.01252232208241908
2102,10422,0,10422,22.47426700592041,0.009447387251569574
2202,10922,0,10922,23.612605810165405,0.009215036792858521
2302,11422,0,11422,24.72783613204956,0.009092578858768892
2402,11921,0,11921,25.832401037216187,0.008625108105700349
2503,12426,0,12426,26.942195892333984,0.008411289735192114
2603,12926,0,12926,28.046991109848022,0.008330120159723786
2703,13425,0,13425,29.304179906845093,0.007820011044585375
2803,13925,0,13925,30.534913063049316,0.007692774522163792
2903,14425,0,14425,31.59478497505188,0.007636663845164925
3003,14925,0,14925,32.55903100967407,0.007602754988352579
3103,15425,0,15425,33.513426065444946,0.007578790450769863
3203,15919,0,15919,34.520222902297974,0.005293676943958086
3303,16414,0,16414,35.61281204223633,0.0036085656182544283
3403,16914,0,16914,36.73590016365051,0.0034271129373004165
3504,17419,0,17419,37.98022389411926,0.0033262958100213733
3604,17919,0,17919,39.141324043273926,0.0032643605357133565
3704,18419,0,18419,40.24874806404114,0.003222736346880356
3804,18919,0,18919,41.34216809272766,0.003192812212130553
3904,19419,0,19419,42.46130609512329,0.003169946832750147
4004,19917,0,19917,43.614588022232056,0.0029371126523334494
4104,20417,0,20417,44.86804008483887,0.0028292052830992233
4204,20917,0,20917,45.99265718460083,0.002779301627360435
4304,21417,0,21417,47.11980104446411,0.0027491676300833543
4404,21917,0,21917,48.33974504470825,0.0027278821444051094
4505,22422,0,22422,49.453787088394165,0.0027114179130843267
4605,22922,0,22922,50.66906809806824,0.0026983545362234246
4705,23421,0,23421,51.77903890609741,0.0026161719723428495
4805,23921,0,23921,52.90787696838379,0.002541686084152088
4905,24421,0,24421,54.31958508491516,0.0025047428276595615
5005,24921,0,24921,55.53780007362366,0.0024828284896996696
5105,25421,0,25421,56.971012115478516,0.002468301939107873
5205,25921,0,25921,58.198824882507324,0.0024579266179626264
5305,26420,0,26420,59.46351194381714,0.0023760284154975995
5405,26920,0,26920,60.80050992965698,0.002314845987550788
5506,27425,0,27425,61.91122817993164,0.0022859141051942175
5606,27925,0,27925,63.02983808517456,0.0022687141955904625
5706,28425,0,28425,64.13093590736389,0.002257211602285903
5806,28925,0,28925,65.24243307113647,0.002249077473075496
5906,29425,0,29425,66.34016990661621,0.0022430796868371378
6006,29925,0,29925,67.43895101547241,0.00223848457250731
6106,30425,0,30425,68.53821897506714,0.002234830042701346
6206,30924,0,30924,69.63856887817383,0.002132951801704158
6306,31424,0,31424,70.73419904708862,0.0020811789782760872
6406,31924,0,31924,71.8436279296875,0.0020632462997641167
6507,32429,0,32429,73.02259612083435,0.0020544806331060064
6607,32929,0,32929,74.1492190361023,0.002049188344675788
6707,33429,0,33429,75.30297708511353,0.0020454918546595176
6807,33928,0,33928,76.47895693778992,0.001990149044989715
6907,34428,0,34428,77.63214683532715,0.0019476073657675428
7007,34928,0,34928,78.76351714134216,0.0019292345755647455
7107,35428,0,35428,79.86471796035767,0.0019183620866525238
7207,35928,0,35928,80.96234488487244,0.001910902595981127
7307,36428,0,36428,82.0872790813446,0.0019053630377742002
7407,36928,0,36928,83.1859838962555,0.0019010240235913544
7508,37433,0,37433,84.3192241191864,0.0018974510214569372
7608,37933,0,37933,85.45661902427673,0.0018944690699334874
7708,38433,0,38433,86.595468044281,0.0018918839274351677
7808,38933,0,38933,87.70897507667542,0.0018895926298098194
7908,39433,0,39433,88.81377100944519,0.0018875250451852474
8008,39933,0,39933,89.94094109535217,0.001885632277754813
8108,40433,0,40433,91.04318499565125,0.0018838794991216097
8208,40932,0,40932,92.19147205352783,0.001818760712723228
8308,41432,0,41432,93.30373811721802,0.001789968389969063
8408,41932,0,41932,94.39993214607239,0.0017736841118643847
8509,42437,0,42437,95.54891109466553,0.0017630636554577294
8609,42937,0,42937,96.69876503944397,0.0017555361023137363
8709,43437,0,43437,97.79296612739563,0.001749753337854293
8809,43937,0,43937,98.89291596412659,0.001745112907184908
8909,44437,0,44437,100.13803505897522,0.0017412824566138965
9009,44937,0,44937,101.3314118385315,0.0017380585900383778
9109,45437,0,45437,102.56417989730835,0.001735305801026813
9209,45937,0,45937,103.84314012527466,0.00173292789076306
9309,46437,0,46437,105.08283114433289,0.0017308533956030628
9409,46937,0,46937,106.65674686431885,0.0017290274990321652
9510,47442,0,47442,108.02126097679138,0.001727391894159333
9610,47942,0,47942,109.24916100502014,0.0017259443884881584
9710,48442,0,48442,110.58175110816956,0.0017246401418321206
9810,48941,0,48941,111.8296492099762,0.0016566217528740093
9910,49441,0,49441,113.13871502876282,0.0016355190794475785
10010,49941,0,49941,114.36730003356934,0.001623278665956409
10110,50441,0,50441,115.5941870212555,0.0016155208792982
10210,50941,0,50941,116.83213686943054,0.0016102240815659657
10310,51441,0,51441,117.95291590690613,0.001606383580265625
10410,51941,0,51941,119.18492102622986,0.001603461815794071
10511,52446,0,52446,120.35008811950684,0.001601130676987706
10611,52946,0,52946,121.52515602111816,0.0015992491856991766
10711,53446,0,53446,122.84983110427856,0.001597674155605504
10811,53946,0,53946,124.03976202011108,0.0015963280313644876
10911,54446,0,54446,125.2580578327179,0.0015951577712940757
11011,54946,0,54946,126.43523716926575,0.001594125935720596
11111,55446,0,55446,127.77248001098633,0.0015932053251746364
11211,55946,0,55946,128.9714539051056,0.0015923756535023295
11311,56446,0,56446,130.06284999847412,0.001591621427864598
11411,56946,0,56946,131.07624220848083,0.0015909305645563751
11512,57451,0,57451,132.1764190196991,0.0015902873370042285
11612,57951,0,57951,133.4612112045288,0.0015896966775691592
11712,58451,0,58451,134.80274391174316,0.0015891456375254516
11812,58951,0,58951,136.0407190322876,0.0015886289817222728
11912,59451,0,59451,137.31993913650513,0.0015881423354250222
12012,59951,0,59951,138.8134000301361,0.0015876820125445648
12112,60451,0,60451,140.33017897605896,0.0015872448850688084
12212,60951,0,60951,141.69598603248596,0.001586828282093145
12312,61451,0,61451,143.0696530342102,0.001586429910538285
12412,61951,0,61951,144.56727814674377,0.0015860477920604298
12513,62456,0,62456,145.91614890098572,0.0015856766046706992
12613,62956,0,62956,147.10823106765747,0.0015853221954172773
12713,63456,0,63456,148.44882988929749,0.0015849795179945934
12813,63955,0,63955,149.81937408447266,0.0015701138571453039
12913,64455,0,64455,151.1908860206604,0.0015401165917221908
13013,64955,0,64955,152.42096519470215,0.0015256935044077274
13113,65455,0,65455,153.9053831100464,0.0015152047311114206
13213,65955,0,65955,155.0322539806366,0.0015074338869126118
13313,66455,0,66455,156.21609115600586,0.0015015640917532417
13413,66955,0,66955,157.51556086540222,0.0014970422161749725
13514,67460,0,67460,158.77929210662842,0.0014934591259298169
13614,67960,0,67960,160.20272397994995,0.0014906237674928216
13714,68460,0,68460,161.88144302368164,0.0014883154713495991
13814,68960,0,68960,163.5579960346222,0.0014864064375659173
13914,69460,0,69460,165.82221508026123,0.001484805072472107
14014,69960,0,69960,167.52975296974182,0.0014834447352621882
14114,70460,0,70460,169.26739597320557,0.0014822761774845338
14214,70960,0,70960,170.77102994918823,0.001481262423698918
14314,71460,0,71460,172.07248902320862,0.001480375273999726
14414,71960,0,71960,173.35135412216187,0.0014795928907542146
14515,72465,0,72465,174.89433789253235,0.00147889156131945
14615,72965,0,72965,176.10711908340454,0.0014782714062944252
14715,73465,0,73465,177.51745510101318,0.0014777140680310014
14815,73965,0,73965,178.78357815742493,0.0014772105686330535
14915,74465,0,74465,180.2507529258728,0.0014767535052233086
15015,74965,0,74965,182.02218413352966,0.0014763367165983934
15115,75465,0,75465,183.29220604896545,0.001475955032258607
15215,75965,0,75965,184.50288820266724,0.0014756040809814964
15315,76465,0,76465,185.9276750087738,0.001475280142958771
15415,76965,0,76965,187.3540861606598,0.0014749800341990994
15516,77470,0,77470,188.5548870563507,0.0014746983231414155
15616,77970,0,77970,189.78364419937134,0.0014744382018808887
15716,78470,0,78470,190.9731891155243,0.001474194727116462
15816,78970,0,78970,192.25431895256042,0.0014739661098606962
15916,79470,0,79470,193.65815496444702,0.0014737507857434508
16016,79970,0,79970,195.18037700653076,0.0014735473824631503
16116,80470,0,80470,196.6473560333252,0.001473354692677223
16216,80970,0,80970,197.8795518875122,0.0014731716512845997
16316,81470,0,81470,199.42486810684204,0.0014729973162833812
16416,81970,0,81970,200.9453740119934,0.0014728308525596907
16517,82475,0,82475,202.60086917877197,0.0014726699584566392
16617,82975,0,82975,204.0821590423584,0.001472517154151235
16717,83475,0,83475,205.6740870475769,0.001472370223352663
16817,83975,0,83975,206.92817616462708,0.001472228639679986
16917,84475,0,84475,208.15181803703308,0.0014720919316991159
17017,84975,0,84975,209.3706841468811,0.0014719596764349169
17117,85475,0,85475,210.62831711769104,0.0014718314937380694
17217,85975,0,85975,212.07923913002014,0.001471707041381574
17317,86475,0,86475,213.35312509536743,0.001471586010782027
17417,86975,0,86975,214.7158510684967,0.0014714681232576364
17518,87480,0,87480,216.07056403160095,0.0014713519905920223
17618,87980,0,87980,218.05108308792114,0.001471239682327715
17718,88479,0,88479,220.1360239982605,0.001453726355615352
17818,88979,0,88979,221.94627499580383,0.0014398274654221306
17918,89479,0,89479,223.36386919021606,0.001428443320114839
18018,89979,0,89979,224.68647289276123,0.0014190832050994422
18118,90479,0,90479,226.40856909751892,0.0014113554373204476
18218,90979,0,90979,227.89763712882996,0.0014049471186303526
18318,91479,0,91479,229.2643210887909,0.0013996080137561534
18418,91979,0,91979,231.05897116661072,0.001395137718930886
18519,92484,0,92484,232.8597390651703,0.0013913409649710562
18619,92984,0,92984,234.7061550617218,0.0013881627893074368
18719,93484,0,93484,236.57717299461365,0.0013854584796166465
18819,93984,0,93984,237.89364290237427,0.0013831442424122957
18919,94484,0,94484,239.4499580860138,0.0013811522955727328
19019,94984,0,94984,240.78904604911804,0.0013794276768312346
19119,95484,0,95484,242.19161891937256,0.0013779257064189723
19219,95984,0,95984,243.46078515052795,0.001376609966952614
19319,96484,0,96484,244.75834584236145,0.0013754506926929812
19419,96984,0,96984,246.24877405166626,0.0013744234831896884
19520,97489,0,97489,247.79069900512695,0.0013734996292509543
19620,97989,0,97989,248.92548084259033,0.0013726807498526863
19720,98489,0,98489,250.03408312797546,0.0013719434925000403
19820,98989,0,98989,251.22583103179932,0.0013712764946652363
19920,99489,0,99489,252.4295711517334,0.001370670280247951
20020,99989,0,99989,253.58058905601501,0.0013701169149399786
20120,100489,0,100489,254.7513861656189,0.0013696097277896505
20220,100989,0,100989,255.98862886428833,0.0013691430858591969
20320,101489,0,101489,257.20357394218445,0.0013687122115252184
20420,101989,0,101989,258.7736849784851,0.0013683130340783618
20521,102494,0,102494,260.22864985466003,0.0013679384912659868
20621,102994,0,102994,261.43095302581787,0.0013675929799974653
20721,103494,0,103494,262.54585099220276,0.0013672700703054746
20821,103994,0,103994,263.6580410003662,0.0013669675167993843
20921,104494,0,104494,264.87980580329895,0.0013666833607098906
21021,104994,0,104994,266.0875520706177,0.0013664158854195408
21121,105494,0,105494,267.21782183647156,0.0013661635797571222
21221,105994,0,105994,268.5346260070801,0.0013659251076128494
21321,106494,0,106494,269.8905441761017,0.00136569928270858
21421,106994,0,106994,271.1915910243988,0.001365485047580314
21522,107499,0,107499,272.61920714378357,0.0013652794708947091
21622,107999,0,107999,273.84390020370483,0.0013650857671117862
21722,108499,0,108499,275.00320506095886,0.0013649010842918306
21822,108999,0,108999,276.1452510356903,0.001364724731112728
21922,109499,0,109499,277.34990096092224,0.0013645560808691443
22022,109999,0,109999,278.4691791534424,0.001364394563893769
22122,110499,0,110499,279.6695899963379,0.00136423966107005
22222,110999,0,110999,280.85793805122375,0.0013640908982552843
22322,111499,0,111499,282.04875802993774,0.0013639478414652275
22422,111999,0,111999,283.2534370422363,0.0013638100926986756
22523,112504,0,112504,284.4695611000061,0.0013636759820346493
22623,113004,0,113004,285.7271420955658,0.0013635478259691111
22723,113504,0,113504,286.96196699142456,0.0013634239626941452
22823,114004,0,114004,288.0769820213318,0.0013633041062352154
22923,114504,0,114504,289.32564187049866,0.0013631879923299258
23023,115004,0,115004,290.4861249923706,0.0013630753764940782
23123,115504,0,115504,291.59612703323364,0.001362966032298095
23223,116004,0,116004,292.7869770526886,0.0013628597498247291
23323,116504,0,116504,294.072722196579,0.0013627563342855226
23423,117004,0,117004,295.21978425979614,0.0013626556047754011
23524,117509,0,117509,296.32627606391907,0.0013625564232096173
23624,118009,0,118009,297.48679208755493,0.0013624605959271082
23724,118509,0,118509,298.69608902931213,0.0013623669831404747
23824,119009,0,119009,299.8309419155121,0.001362275449346738
23924,119509,0,119509,301.0782949924469,0.0013621858682550186
24024,120009,0,120009,302.3685739040375,0.001362098122090599
24124,120508,0,120508,303.54374384880066,0.0013496038612603265
24224,121008,0,121008,304.76537799835205,0.0013353275625803697
24324,121508,0,121508,306.0356469154358,0.0013234724561885377
24424,122008,0,122008,307.1708950996399,0.0013136215587083737
24525,122513,0,122513,308.3975601196289,0.0013053524753233582
24625,123013,0,123013,309.57282996177673,0.001298537863261558
24725,123513,0,123513,310.75980401039124,0.001292849323433793
24825,124013,0,124013,311.86107110977173,0.0012880896791945952
24925,124513,0,124513,312.9664990901947,0.0012840964428289625
25025,125013,0,125013,314.059739112854,0.0012807359139930705
25125,125513,0,125513,315.16960620880127,0.0012778981926325167
25225,126013,0,126013,316.2655260562897,0.0012754929973965582
25325,126513,0,126513,317.45694303512573,0.0012734461813433053
25425,127013,0,127013,318.5698800086975,0.0012716968431868603
25526,127518,0,127518,319.68397307395935,0.0012701810265898668
25626,128018,0,128018,320.77422404289246,0.0012688872985362634
25726,128518,0,128518,321.874489068985,0.001267765695935465
25826,129018,0,129018,322.97775506973267,0.0012667883749106455
25926,129518,0,129518,324.07425713539124,0.0012659323629714654
26026,130018,0,130018,325.177796125412,0.0012651786765798898
26126,130518,0,130518,326.2821969985962,0.00126451160021098
26226,131018,0,131018,327.3811800479889,0.001263918097595848
26326,131518,0,131518,328.4706599712372,0.0012633873309912703
26426,132018,0,132018,329.57163095474243,0.0012629102686370205
26527,132523,0,132523,330.68808913230896,0.0012624752658956023
26627,133023,0,133023,331.7960319519043,0.0012620845662822129
26727,133523,0,133523,332.9800088405609,0.0012617283391550204
26827,134023,0,134023,334.12314009666443,0.0012614021123656476
26927,134523,0,134523,335.22499203681946,0.0012611021030160413
27027,135023,0,135023,336.33029198646545,0.0012608251000913767
27127,135523,0,135523,337.4251592159271,0.001260568368150225
27227,136023,0,136023,338.5307819843292,0.001260329568193407
27327,136523,0,136523,339.6239960193634,0.0012601066925568751
27427,137023,0,137023,340.73203921318054,0.0012598980112602284
27528,137528,0,137528,341.8365080356598,0.001259700127463341
27628,138028,0,138028,342.94312810897827,0.001259515649879399
27728,138528,0,138528,344.0347559452057,0.001259341426297973
27828,139028,0,139028,345.24867701530457,0.0012591764658930254
27928,139528,0,139528,346.4206681251526,0.0012590198979254626
28028,140028,0,140028,347.6017599105835,0.0012588709542865667
28128,140528,0,140528,348.8383231163025,0.0012587289548988655
28228,141028,0,141028,350.0099160671234,0.0012585932954738512
28328,141528,0,141528,351.1330101490021,0.001258463437216876
28428,142028,0,142028,352.23163414001465,0.0012583388981442822
28529,142533,0,142533,353.3437659740448,0.0012582180725397663
28629,143033,0,143033,354.4567680358887,0.0012581029606474792
28729,143533,0,143533,355.56677508354187,0.001257991991421701
28829,144033,0,144033,356.7377362251282,0.0012578848471878202
28929,144533,0,144533,357.996386051178,0.0012577812397275194
29029,145033,0,145033,359.1471028327942,0.0012576809069366106
29129,145533,0,145533,360.2776219844818,0.0012575836099384269
29229,146033,0,146033,361.38605523109436,0.0012574891305823807
29329,146533,0,146533,362.5019519329071,0.0012573972692680893
29429,147033,0,147033,363.60836601257324,0.0012573078430463108
29530,147538,0,147538,364.7943789958954,0.0012572198232800509
29630,148038,0,148038,365.8967430591583,0.0012571347972722107
29730,148538,0,148538,367.0342161655426,0.0012570517403927865
29830,149038,0,149038,368.1408030986786,0.0012569705216402926
29930,149538,0,149538,369.2565040588379,0.001256891020084921
30030,150038,0,150038,370.37522411346436,0.001256813123967454
30130,150538,0,150538,371.52588415145874,0.0012567367298946196
30230,151038,0,151038,372.72015404701233,0.0012566617421183837
30330,151538,0,151538,373.97816801071167,0.001256588071888809
30430,152038,0,152038,375.16714215278625,0.0012565156368715327
30531,152543,0,152543,376.2782099246979,0.0012564436534663736
30631,153043,0,153043,377.382817029953,0.0012563734754893212
30731,153543,0,153543,378.4848449230194,0.0012563043185648414
30831,154043,0,154043,379.588103055954,0.0012562361212808668
30931,154543,0,154543,380.6855900287628,0.001256168826457197
31031,155043,0,155043,381.781555891037,0.001256102380820952
31131,155543,0,155543,382.883327960968,0.001256036734710361
31231,156043,0,156043,383.9871621131897,0.0012559718418038853
31331,156543,0,156543,385.08619809150696,0.0012559076588721208
31431,157043,0,157043,386.19041991233826,0.0012558441455502534
31532,157548,0,157548,387.29684615135193,0.0012557806383849642
31632,158048,0,158048,388.39893198013306,0.0012557183594161508
31732,158548,0,158548,389.48647594451904,0.0012556566438264164
31832,159048,0,159048,390.59896898269653,0.0012555954608026334
31932,159547,0,159547,391.6956989765167,0.0012464530625578571
32032,160047,0,160047,392.7939021587372,0.0012364923687016626
32132,160547,0,160547,393.96175718307495,0.0012279957206674822
32232,161047,0,161047,395.2146830558777,0.0012207364269669618
32332,161547,0,161547,396.3714668750763,0.0012145258183443894
32432,162047,0,162047,397.61739802360535,0.0012092041617442217
32533,162552,0,162552,398.82832193374634,0.001204593992948788
32633,163052,0,163052,399.93348717689514,0.0012006714165854397
32733,163552,0,163552,401.25598096847534,0.00119729076863617
32833,164052,0,164052,402.4299781322479,0.0011943705502557632
32933,164552,0,164552,403.60028314590454,0.0011918419077725556
33033,165052,0,165052,404.7598559856415,0.001189646660731773
33133,165552,0,165552,405.9167149066925,0.0011877356290642173
33233,166052,0,166052,407.0704171657562,0.0011860672179252261
33333,166552,0,166552,408.2175660133362,0.001184606223108426
33433,167052,0,167052,409.50787806510925,0.0011833228243183223
33534,167557,0,167557,410.70369601249695,0.0011821811206033511
33634,168057,0,168057,411.9112219810486,0.0011811820979201195
33734,168557,0,168557,413.0944170951843,0.001180295524597782
33834,169057,0,169057,414.3856518268585,0.0011795059117805568
33934,169557,0,169557,415.48475098609924,0.0011788000649648007
34034,170057,0,170057,416.5913870334625,0.0011781667289730412
34134,170557,0,170557,417.6896290779114,0.0011775962894242206
34234,171057,0,171057,418.7869381904602,0.0011770805215820601
34334,171557,0,171557,419.90468287467957,0.0011766123789291325
34434,172057,0,172057,421.197252035141,0.0011761858150522101
34535,172562,0,172562,422.3963270187378,0.0011757918996976738
34635,173062,0,173062,423.5483319759369,0.0011754339257815135
34735,173562,0,173562,424.6639370918274,0.001175103967945771
34835,174062,0,174062,425.93229699134827,0.0011747986995168226
34935,174562,0,174562,427.1183490753174,0.0011745152421165279
35035,175062,0,175062,428.16879200935364,0.0011742511008375081
35135,175562,0,175562,429.36598110198975,0.0011740041092469572
35235,176062,0,176062,430.51185512542725,0.0011737723826739416
35335,176562,0,176562,431.63199615478516,0.001173554278485417
35435,177062,0,177062,432.7447819709778,0.0011733483622642549
35536,177567,0,177567,433.8657920360565,0.0011731514805143294
35636,178067,0,178067,434.96127104759216,0.0011729664231411787
35736,178567,0,178567,436.16198801994324,0.0011727902228744255
35836,179067,0,179067,437.30660700798035,0.0011726220300208744
35936,179567,0,179567,438.43443393707275,0.0011724610950725298
36036,180067,0,180067,439.53066420555115,0.0011723067554987347
36136,180567,0,180567,440.6698069572449,0.0011721584244003245
36236,181067,0,181067,441.77562403678894,0.001172015580750487
36336,181567,0,181567,442.88837909698486,0.0011718777609893193
36436,182067,0,182067,444.00212025642395,0.0011717445517747563
36537,182572,0,182572,445.13153886795044,0.0011716143143106316
36637,183072,0,183072,446.2217240333557,0.0011714892941312102
36737,183572,0,183572,447.32184314727783,0.0011713678844774132
36837,184072,0,184072,448.454421043396,0.0011712498184368728
36937,184572,0,184572,449.5621428489685,0.0011711348553267835
37037,185072,0,185072,450.6744728088379,0.00117102277762916
37137,185572,0,185572,451.94183802604675,0.001170913388322258
37237,186072,0,186072,453.1692600250244,0.0011708065085534616
37337,186572,0,186572,454.2804260253906,0.0011707019756068918
37437,187072,0,187072,455.479376077652,0.001170599641126218
37538,187577,0,187577,456.69460797309875,0.001170498376831037
37638,188077,0,188077,457.80696392059326,0.0011704000628555754
37738,188577,0,188577,458.9056921005249,0.001170303572706706
37838,189077,0,189077,460.0026590824127,0.001170208801774726
37938,189577,0,189577,461.1578071117401,0.0011701156536928674
38038,190077,0,190077,462.49005103111267,0.0011700240395172432
38138,190577,0,190577,463.82910990715027,0.001169933877001791
38238,191077,0,191077,465.3217740058899,0.0011698450899560117
38338,191577,0,191577,466.4388451576233,0.0011697576076754176
38438,192077,0,192077,467.6019570827484,0.0011696713644353503
38539,192582,0,192582,469.1100389957428,0.0011695854541382798
38639,193082,0,193082,470.42359495162964,0.0011695015204534608
38739,193582,0,193582,472.0490322113037,0.001169418653732017
38839,194082,0,194082,473.3986930847168,0.0011693368041558246
38939,194582,0,194582,474.62152004241943,0.0011692559250638945
39039,195082,0,195082,475.80223298072815,0.0011691759726944646
39139,195582,0,195582,477.02212023735046,0.0011690969059527294
39239,196082,0,196082,478.3972358703613,0.001169018686201509
39339,196582,0,196582,479.5561351776123,0.0011689412770723535
39439,197082,0,197082,480.9054801464081,0.0011688646442946401
39540,197587,0,197587,482.2337498664856,0.0011687880003058068
39640,198087,0,198087,483.43563413619995,0.0011687128320370323
39740,198587,0,198587,484.8579728603363,0.0011686383481356376
39840,199087,0,199087,486.0132761001587,0.0011685645213240364
39940,199587,0,199587,487.6300220489502,0.0011684913257754208
40040,200087,0,200087,488.95951104164124,0.0011684187370166563
40140,200587,0,200587,490.2770240306854,0.0011683467318394283
40240,201087,0,201087,491.7254910469055,0.0011682752882186305
40340,201587,0,201587,492.84861516952515,0.0011682043852374738
40440,202087,0,202087,494.18026900291443,0.001168134003018333
40541,202592,0,202592,495.5617241859436,0.001168063426328588
40641,203092,0,203092,496.6706430912018,0.0011679940345957784
40741,203592,0,203592,497.7821092605591,0.0011679251094489072
40841,204092,0,204092,498.8820400238037,0.0011678566345860162
40941,204592,0,204592,500.081326007843,0.0011677885944702904
41041,205092,0,205092,501.31694889068604,0.0011677209742869824
41141,205592,0,205592,502.4361729621887,0.0011676537599030407
41241,206092,0,206092,503.5850410461426,0.0011675869378295913
41341,206592,0,206592,504.6983449459076,0.0011675204951870123
41441,207092,0,207092,505.8300368785858,0.0011674544196722853
41542,207597,0,207597,507.17655897140503,0.0011673880440832356
41642,208097,0,208097,508.426322221756,0.0011673226714572036
41742,208597,0,208597,509.66099095344543,0.001167257632109
41842,209097,0,209097,511.1403748989105,0.0011671929157601835
41942,209597,0,209597,512.369117975235,0.0011671285125742393
42042,210097,0,210097,513.5285110473633,0.0011670644131344678
42142,210597,0,210597,514.886293888092,0.0011670006084231151
42242,211097,0,211097,516.1898999214172,0.00116693708980181
42342,211597,0,211597,517.8492851257324,0.0011668738489931654
42442,212097,0,212097,519.2863590717316,0.0011668108780632752
42543,212602,0,212602,520.4765071868896,0.0011667475436183627
42643,213102,0,213102,521.7834041118622,0.0011666850924512927
42743,213602,0,213602,523.0830330848694,0.0011666228891943073
42843,214102,0,214102,524.5062720775604,0.001166560927135047
42943,214602,0,214602,525.9150400161743,0.0011664991998310234
43043,215102,0,215102,527.0491859912872,0.0011664377010970745
43143,215602,0,215602,528.3537662029266,0.0011663764249937763
43243,216102,0,216102,529.8757100105286,0.0011663153658161604
43343,216602,0,216602,531.2435839176178,0.0011662545180831927
43443,217102,0,217102,532.4977991580963,0.001166193876527728
43544,217607,0,217607,533.8453891277313,0.0011661328326815457
43644,218107,0,218107,534.8974871635437,0.001166072590426508
43744,218607,0,218607,535.9173521995544,0.0011660125396919393
43844,219107,0,219107,537.0365629196167,0.0011659526759772415
43944,219607,0,219607,538.3577561378479,0.0011658929949525047
44044,220107,0,220107,539.7520911693573,0.0011658334924510207
44144,220607,0,220607,541.2168428897858,0.0011657741644622817
44244,221107,0,221107,542.5073919296265,0.001165715007125243
44344,221607,0,221607,543.695953130722,0.0011656560167219727
44444,222107,0,222107,545.0843288898468,0.0011655971896715315
44545,222612,0,222612,546.481987953186,0.0011655379366488428
44645,223112,0,223112,547.701208114624,0.0011654794276298422
44745,223612,0,223612,549.0969462394714,0.0011654210719545745
44845,224112,0,224112,550.4801268577576,0.001165362866535833
44945,224612,0,224612,551.9189438819885,0.0011653048083968096
45045,225112,0,225112,553.1148941516876,0.0011652468946665839
45145,225612,0,225612,554.3427498340607,0.001165189122575819
45245,226112,0,226112,555.7498700618744,0.001165131489452384
45345,226612,0,226612,556.9607129096985,0.0011650739927176388
45445,227112,0,227112,558.3731780052185,0.0011650166298823768
45546,227617,0,227617,559.6745629310608,0.0011649588268859367
45646,228117,0,228117,561.0565748214722,0.0011649017260022525
45746,228617,0,228617,562.293879032135,0.001164844752029862
45846,229117,0,229117,563.6021611690521,0.0011647879028034236
45946,229617,0,229617,564.8245379924774,0.0011647311762305128
46046,230117,0,230117,566.1079480648041,0.0011646745702884299
46146,230617,0,230617,567.4345571994781,0.0011646180830216606
46246,231117,0,231117,568.6075391769409,0.0011645617125391023
46346,231617,0,231617,570.0551290512085,0.001164505457011427
46446,232117,0,232117,571.5342650413513,0.0011644493146688146
46547,232622,0,232622,573.1243650913239,0.0011643927240470393
46647,233122,0,233122,574.9363398551941,0.0011643368040809617
46747,233622,0,233622,576.5000722408295,0.0011642809923081553
46847,234122,0,234122,577.7596299648285,0.0011642252871744783
46947,234622,0,234622,579.1096520423889,0.0011641696871744617
47047,235122,0,235122,580.4869010448456,0.001164114190849333
47147,235622,0,235622,581.707267999649,0.0011640587967853687
47247,236122,0,236122,583.2367050647736,0.0011640035036119857
47347,236622,0,236622,584.5325360298157,0.0011639483100002058
47447,237122,0,237122,585.8523499965668,0.0011638932146609718
47548,237627,0,237627,587.5313560962677,0.0011638376668464227
47648,238127,0,238127,589.1273920536041,0.0011637827652896868
47748,238627,0,238627,590.9089782238007,0.0011637279583517344
47848,239127,0,239127,592.3150510787964,0.0011636732448891862
47948,239627,0,239627,593.730663061142,0.0011636186237914715
48048,240127,0,240127,595.2894699573517,0.0011635640939798545
48148,240627,0,240627,596.7445681095123,0.0011635096544060025
48248,241127,0,241127,597.9692499637604,0.0011634553040510772
48348,241627,0,241627,599.2758052349091,0.0011634010419244196
48448,242127,0,242127,600.774934053421,0.0011633468670626756
48549,242632,0,242632,602.2666170597076,0.001163292238076192
48649,243132,0,243132,603.4865279197693,0.001163238235807756
48749,243632,0,243632,604.9298942089081,0.0011631843180589213
48849,244132,0,244132,606.3763098716736,0.0011631304839658364
48949,244632,0,244632,607.9852139949799,0.001163076732687278
49049,245132,0,245132,609.4518389701843,0.0011630230634037248
49149,245632,0,245632,610.9615862369537,0.001162969475316747
49249,246132,0,246132,612.1285791397095,0.0011629159676480045
49349,246632,0,246632,613.29669713974,0.0011628625396387867
49449,247132,0,247132,614.4800050258636,0.0011628091905491556
49550,247637,0,247637,615.8414509296417,0.0011627553873408388
49650,248137,0,248137,616.9054980278015,0.001162702194713821
49750,248637,0,248637,617.9491939544678,0.0011626490788860366
49850,249137,0,249137,619.1326420307159,0.0011625960391864589
49950,249637,0,249637,620.2742509841919,0.0011625430749598506
50050,250137,0,250137,621.4626648426056,0.0011624901855660581
50150,250637,0,250637,622.6167411804199,0.0011624373703795947
50250,251137,0,251137,623.82248711586,0.0011623846287891326
50350,251637,0,251637,625.00364112854,0.0011623319601969618
50450,252137,0,252137,626.3378400802612,0.001162279364018462
50551,252642,0,252642,627.6597239971161,0.0011622263147994475
50651,253142,0,253142,628.855740070343,0.001162173862455327
50751,253642,0,253642,630.0507500171661,0.001162121480840517
50851,254142,0,254142,631.2655851840973,0.001162069169418962
50951,254642,0,254642,632.7342059612274,0.0011620169276656865
51051,255142,0,255142,634.1528401374817,0.0011619647550664839
51151,255642,0,255642,635.4534261226654,0.001161912651117372
51251,256142,0,256142,636.9761221408844,0.0011618606153245474
51351,256642,0,256642,638.2013831138611,0.0011618086472037963
51451,257142,0,257142,639.542845249176,0.0011617567462803248
51552,257647,0,257647,640.8315620422363,0.001161704394081913
51652,258147,0,258147,642.0221679210663,0.001161652626825034
51752,258647,0,258647,643.3485460281372,0.0011616009253898158
51852,259147,0,259147,644.7727379798889,0.001161549289336086
51952,259647,0,259647,645.9163391590118,0.001161497718231684
52052,260147,0,260147,647.143196105957,0.001161446211652078
52152,260647,0,260647,648.3185641765594,0.0011613947691802313
52252,261147,0,261147,649.4882090091705,0.001161343390406321
52352,261647,0,261647,650.6765470504761,0.001161292074927608
52452,262147,0,262147,651.9382410049438,0.0011612408223480304
52553,262652,0,262652,653.3714978694916,0.0011611891206918545
52653,263152,0,263152,654.5300850868225,0.001161137993368067
52753,263652,0,263652,655.8925080299377,0.0011610869277903328
52853,264152,0,264152,657.1314148902893,0.0011610359235879224
52953,264652,0,264652,658.36523604393,0.0011609849803957972
53053,265152,0,265152,659.6284132003784,0.0011609340978546898
53153,265652,0,265652,660.9873280525208,0.0011608832756107002
53253,266152,0,266152,662.1964020729065,0.0011608325133153274
53353,266652,0,266652,663.363254070282,0.0011607818106252087
53453,267152,0,267152,664.6139280796051,0.0011607311672019633
53554,267657,0,267657,665.8527390956879,0.0011606800771637538
53654,268157,0,268157,667.0894808769226,0.0011606295518630794
53754,268657,0,268657,668.6622641086578,0.0011605790848396957
53854,269157,0,269157,669.7262508869171,0.0011605286757739954
53954,269657,0,269657,670.8940751552582,0.0011604783243507378
54054,270157,0,270157,672.1740441322327,0.0011604280302588595
54154,270657,0,270657,673.3631780147552,0.0011603777931914108
54254,271157,0,271157,674.7428379058838,0.0011603276128454554
54354,271657,0,271657,675.9990210533142,0.0011602774889219291
54454,272157,0,272157,677.0983700752258,0.00116022742112559
54555,272662,0,272662,678.2162930965424,0.001160176909326209
54655,273161,0,273161,679.378583908081,0.0011124430619838003
54755,273661,0,273661,680.5047149658203,0.001111420554645428
54855,274161,0,274161,681.6806139945984,0.0011106558237035785
54955,274661,0,274661,682.8106820583344,0.0011099260088512299
55055,275161,0,275161,683.9800939559937,0.0011092203675606813
55155,275661,0,275661,685.1784749031067,0.0011085362346735413
55255,276161,0,276161,686.395092010498,0.0011078722935100324
55355,276661,0,276661,687.5458040237427,0.0011072276147345583
55455,277161,0,277161,688.7286529541016,0.0011066014251988761
55556,277666,0,277666,689.943284034729,0.0011059870364096614
55656,278166,0,278166,691.0634212493896,0.0011053959680213785
55756,278666,0,278666,692.198930978775,0.0011048214452034676
55856,279166,0,279166,693.3259189128876,0.001104262893798323
55956,279666,0,279666,694.6064400672913,0.0011037197652057505
56056,280166,0,280166,695.7239999771118,0.0011031915336896685
56156,280666,0,280666,696.9815149307251,0.001102677694495342
56256,281166,0,281166,698.4169130325317,0.0011021777624309684
56356,281666,0,281666,699.7756369113922,0.0011016912707308571
56456,282166,0,282166,701.0069401264191,0.0011012177700990826
56557,282671,0,282671,702.3950130939484,0.0011007522804499456
56657,283171,0,283171,703.8846929073334,0.0011003035992256409
56757,283671,0,283671,705.4887170791626,0.0010998666541294918
56857,284171,0,284171,707.1264810562134,0.0010994410583110425
56957,284671,0,284671,708.5008821487427,0.0010990264388967403
57057,285171,0,285171,709.8408100605011,0.001098622436433862
57157,285671,0,285671,711.0992512702942,0.0010982287043639976
57257,286171,0,286171,712.4395759105682,0.0010978449085231922
57357,286671,0,286671,713.7068030834198,0.0010974707266652175
57457,287171,0,287171,714.9929032325745,0.0010971058480069118
57558,287676,0,287676,716.2283928394318,0.0010967464585212039
57658,288176,0,288176,717.5901610851288,0.001096399383325513
57758,288676,0,288676,718.8046219348907,0.0010960607407596839
57858,289176,0,289176,720.0929610729218,0.001095730261817897
57958,289676,0,289676,721.263836145401,0.0010954076869527584
58058,290176,0,290176,722.5014090538025,0.0010950927657226717
58158,290676,0,290676,723.8284530639648,0.0010947852564530398
58258,291176,0,291176,725.1628441810608,0.001094484925911081
58358,291676,0,291676,726.4260430335999,0.001094191548992963
58458,292176,0,292176,727.7283198833466,0.0010939049084233616
58559,292681,0,292681,728.9754469394684,0.0010936220255952428
58659,293181,0,293181,730.2781019210815,0.0010933482980195434
58759,293681,0,293681,731.5844888687134,0.0010930806971822973
58859,294181,0,294181,733.1550829410553,0.0010928190344074344
58959,294681,0,294681,734.5173070430756,0.001092563127507021
59059,295181,0,295181,735.9786942005157,0.0010923128005434028
59159,295681,0,295681,737.1589648723602,0.0010920678836008337
59259,296181,0,296181,738.3723628520966,0.001091828212565474
59359,296681,0,296681,739.6891760826111,0.0010915936289139037
59459,297181,0,297181,741.0707249641418,0.0010913639795095773
59560,297686,0,297686,742.3812530040741,0.001091136891459056
59660,298186,0,298186,743.5159091949463,0.0010909167174435513
59760,298686,0,298686,744.6194200515747,0.0010907010473079433
59860,299186,0,299186,745.773766040802,0.0010904897476231674
59960,299686,0,299686,746.8848180770874,0.0010902826894374673
60060,300186,0,300186,747.9872438907623,0.0010900797481148744
60160,300686,0,300686,749.0782001018524,0.0010898808031797969
60260,301186,0,301186,750.222305059433,0.0010896857381674277
60360,301686,0,301686,751.347009897232,0.001089494440479704
60460,302186,0,302186,752.4497120380402,0.0010893068012467612
60561,302691,0,302691,753.5590581893921,0.0010891208919292035
60661,303191,0,303191,754.6740698814392,0.0010889402912578996
60761,303691,0,303691,755.7678399085999,0.001088763042523427
60861,304191,0,304191,756.8666999340057,0.0010885890505153142
60961,304691,0,304691,757.9734709262848,0.001088418223131134
61061,305191,0,305191,759.1388530731201,0.001088250471266347
61161,305691,0,305691,760.3171420097351,0.0010880857087081296
61261,306191,0,306191,761.4961981773376,0.0010879238520331805
61361,306691,0,306691,762.7288310527802,0.0010877648205093189
61461,307191,0,307191,763.9235241413116,0.0010876085360007586
61562,307696,0,307696,765.5158960819244,0.0010874533999864478
61662,308196,0,308196,766.6863548755646,0.0010873024106538276
61762,308696,0,308696,767.869145154953,0.0010871539479145648
61862,309196,0,309196,768.9537761211395,0.0010870079431612935
61962,309696,0,309696,770.1763031482697,0.0010868643299586204
62062,310196,0,310196,771.375864982605,0.0010867230439675197
62162,310696,0,310696,772.6298179626465,0.0010865840228725821
62262,311196,0,311196,773.8038010597229,0.0010864472063119215
62362,311696,0,311696,775.0005149841309,0.001086312535809675
62462,312196,0,312196,776.27002120018,0.0010861799547108187
62563,312701,0,312701,777.318118095398,0.0010860481127456152
62663,313201,0,313201,778.4633920192719,0.0010859195670113364
62763,313701,0,313701,780.0143179893494,0.001085792950518287
62863,314201,0,314201,781.2461738586426,0.0010856682133064861
62963,314701,0,314701,782.599335193634,0.0010855453069451518
63063,315201,0,315201,783.9562270641327,0.0010854241844805335
63163,315701,0,315701,785.0928821563721,0.0010853048003857883
63263,316201,0,316201,786.3158462047577,0.0010851871105127175
63363,316701,0,316701,787.594850063324,0.00108507107204515
63463,317201,0,317201,788.7828369140625,0.001084956643454075
63564,317706,0,317706,789.974053144455,0.0010848426636575243
63664,318206,0,318206,791.3065011501312,0.0010847313502778083
63764,318706,0,318706,792.6789319515228,0.0010846215291119676
63864,319206,0,319206,793.9429621696472,0.0010845131633732536
63964,319706,0,319706,795.3696339130402,0.0010844062173603081
64064,320206,0,320206,796.8654720783234,0.0010843006564212828
64164,320706,0,320706,798.4370110034943,0.001084196446918974
64264,321206,0,321206,799.8587260246277,0.001084093556197409
64364,321706,0,321706,801.0384528636932,0.0010839919525494931
64464,322206,0,322206,802.1421627998352,0.0010838916051859198
64565,322711,0,322711,803.2787570953369,0.0010837914990895032
64665,323211,0,323211,804.5780870914459,0.001083693587277994
64765,323711,0,323711,805.7975289821625,0.0010835968443161416
64865,324211,0,324211,807.2249920368195,0.0010835012428035003
64965,324711,0,324711,808.5293831825256,0.0010834067561171432
65065,325211,0,325211,809.6474649906158,0.0010833133583866112
65165,325711,0,325711,810.7474229335785,0.0010832210244696185
65265,326211,0,326211,811.8418979644775,0.001083129729928735
65365,326711,0,326711,812.9461140632629,0.0010830394510088495
65465,327211,0,327211,814.0306348800659,0.0010829501646153904
65566,327716,0,327716,815.2729640007019,0.0010828609699545725
65666,328216,0,328216,816.5046410560608,0.0010827736112422855
65766,328716,0,328716,817.7767150402069,0.0010826871793201767
65866,329216,0,329216,819.0686681270599,0.0010826016535386946
65966,329716,0,329716,820.5352170467377,0.0010825170138107087
66066,330216,0,330216,822.0522830486298,0.0010824332405938947
66166,330716,0,330716,823.3899819850922,0.0010823503148736462
66266,331216,0,331216,824.5937190055847,0.0010822682181468601
66366,331716,0,331716,825.8589119911194,0.0010821869324057888
66466,332216,0,332216,827.0712850093842,0.0010821064401230767
66567,332721,0,332721,828.3284640312195,0.0010820259309420686
66667,333221,0,333221,829.4628810882568,0.0010819469823566336
66767,333721,0,333721,830.8752839565277,0.0010818687772235827
66867,334221,0,334221,832.1106350421906,0.001081791299797576
66967,334721,0,334721,833.2254371643066,0.0010817145347443464
67067,335221,0,335221,834.6979749202728,0.0010816384671280862
67167,335721,0,335721,835.999941110611,0.0010815630823995512
67267,336221,0,336221,837.2846279144287,0.001081488366384507
67367,336721,0,336721,838.7410538196564,0.001081414305272191
67467,337221,0,337221,839.9496080875397,0.0010813408856048758
67568,337726,0,337726,841.1749789714813,0.0010812673694832024
67668,338226,0,338226,842.8015122413635,0.0010811951997835305
67768,338726,0,338726,844.1938889026642,0.001081123633046015
67868,339226,0,339226,845.5955600738525,0.0010810526571256808
67968,339726,0,339726,847.2136659622192,0.0010809822601811
68068,340226,0,340226,848.5073299407959,0.0010809124306656287
68168,340726,0,340726,849.868588924408,0.0010808431573187283
68268,341226,0,341226,851.1542918682098,0.0010807744291577751
68368,341726,0,341726,852.6634769439697,0.0010807062354699004
68468,342226,0,342226,853.878543138504,0.0010806385658043254
68569,342731,0,342731,855.0401570796967,0.001080570740967388
68669,343231,0,343231,856.4148321151733,0.0010805040939942869
68769,343731,0,343731,857.7037711143494,0.0010804379410936248
68869,344231,0,344231,858.9196960926056,0.0010803722727923228
68969,344731,0,344731,860.2008838653564,0.0010803070798440768
69069,345231,0,345231,861.3555178642273,0.0010802423532229625
69169,345731,0,345731,862.6368548870087,0.0010801780841171742
69269,346230,0,346230,863.8128571510315,0.0010627107461176914
69369,346730,0,346730,865.2313649654388,0.0010611792955333272
69469,347230,0,347230,866.426323890686,0.0010597084212616023
69570,347735,0,347735,867.5721299648285,0.0010582691890635954
69670,348235,0,348235,868.678624868393,0.0010568872370447552
69770,348735,0,348735,869.7909739017487,0.0010555462897183776
69870,349235,0,349235,870.941890001297,0.0010542448072450412
69970,349735,0,349735,872.2951741218567,0.0010529813711810804
70070,350235,0,350235,873.4948351383209,0.001051754641783036
70170,350735,0,350735,874.6322510242462,0.0010505633413833346
70270,351235,0,351235,875.8295950889587,0.001049406246399014
70370,351735,0,351735,877.0185990333557,0.0010482821826549834
70470,352231,0,352231,878.1255860328674,0.0010131479128127807
70571,352736,0,352736,879.2975850105286,0.001012661652461844
70671,353236,0,353236,880.5043818950653,0.0010122015481232353
70771,353736,0,353736,881.7016229629517,0.0010117613286002383
70871,354236,0,354236,883.0782370567322,0.0010113398072038192
70971,354736,0,354736,884.3170599937439,0.001010935915369123
71071,355236,0,355236,885.7851660251617,0.001010548677340959
71171,355736,0,355736,886.9821691513062,0.0010101771934913864
71271,356236,0,356236,888.186222076416,0.0010098206287417165
71371,356736,0,356736,889.6418302059174,0.001009478204150353
71471,357236,0,357236,890.9554190635681,0.0010091491905485804
71572,357741,0,357741,892.5585720539093,0.00100882980273829
71672,358241,0,358241,893.7858741283417,0.001008525716403308
71772,358741,0,358741,894.9171929359436,0.001008233100875547
71872,359241,0,359241,896.271646976471,0.0010079513847400673
71972,359741,0,359741,897.7609939575195,0.0010076800285911116
72072,360241,0,360241,899.13046002388,0.001007418522840397
72172,360741,0,360741,900.3764719963074,0.0010071663857564677
72272,361241,0,361241,901.5416660308838,0.001006923161692335
72372,361741,0,361741,902.7317202091217,0.0010066884194693934
72472,362241,0,362241,903.8736801147461,0.0010064617508943605
72573,362746,0,362746,905.0201561450958,0.001006240617139747
72673,363246,0,363246,906.1762249469757,0.0010060290279042745
72773,363746,0,363746,907.4072208404541,0.0010058244090765443
72873,364246,0,364246,908.5959658622742,0.0010056264318449248
72973,364746,0,364746,909.9544689655304,0.0010054347844323784
73073,365246,0,365246,911.4532120227814,0.0010052491711369422
73173,365746,0,365746,912.7636389732361,0.0010050693114324579
73273,366246,0,366246,914.0386390686035,0.0010048949391251519
73373,366746,0,366746,915.3876130580902,0.0010047258015617613
73473,367246,0,367246,916.522901058197,0.001004561658885512
73574,367751,0,367751,918.3723051548004,0.0010044007129138487
73674,368251,0,368251,920.3712339401245,0.0010042459326238434
73774,368751,0,368751,922.1428751945496,0.0010040954956360413
73874,369251,0,369251,923.975643157959,0.0010039492067845173
73974,369751,0,369751,925.7767460346222,0.0010038068805847096
74074,370251,0,370251,927.6883220672607,0.0010036683407161312
74174,370751,0,370751,929.3277292251587,0.0010035334195345282
74274,371251,0,371251,930.9470808506012,0.0010034019576121102
74374,371751,0,371751,932.7575540542603,0.001003273803303748
74474,372251,0,372251,934.2589612007141,0.0010031488123378033
74575,372756,0,372756,936.1769549846649,0.0010030256426150157
74675,373256,0,373256,937.6854319572449,0.0010029066014194594
74775,373756,0,373756,939.1427550315857,0.001002790330024593
74875,374256,0,374256,940.4350068569183,0.0010026767100593788
74975,374756,0,374756,941.8152539730072,0.0010025656287966152
75075,375256,0,375256,943.2046551704407,0.0010024569788631037
75175,375756,0,375756,944.6051139831543,0.0010023506579657283
75275,376256,0,376256,946.233964920044,0.0010022465686325111
75375,376756,0,376756,947.7768850326538,0.0010021446179680055
75475,377256,0,377256,949.5988550186157,0.0010020447174217998
75576,377761,0,377761,951.5289168357849,0.0010019458128721185
75676,378261,0,378261,953.0126020908356,0.001001849781666429
75776,378761,0,378761,954.6362869739532,0.0010017555581173748
75876,379261,0,379261,955.9703028202057,0.001001663069014874
75976,379761,0,379761,957.3673050403595,0.0010015722445091495
76076,380261,0,380261,958.8503510951996,0.0010014830179447456
76176,380761,0,380761,960.2130448818207,0.0010013953257031669
76276,381261,0,381261,961.5185990333557,0.0010013091070537967
76376,381761,0,381761,962.8100941181183,0.0010012243040128498
76476,382261,0,382261,964.0743000507355,0.0010011408612094893
76577,382766,0,382766,965.3661630153656,0.0010010579108338349
76677,383266,0,383266,966.632285118103,0.00100097704453864
76777,383766,0,383766,967.9122211933136,0.001000897386339385
76877,384266,0,384266,969.1722228527069,0.00100081889013423
76977,384766,0,384766,970.4475922584534,0.0010007415118617024
77077,385266,0,385266,971.7449510097504,0.001000665209403484
77177,385766,0,385766,973.3208739757538,0.0010005899424920359
77277,386266,0,386266,974.9285480976105,0.0010005156726232258
77377,386766,0,386766,976.3028740882874,0.0010004423629729315
77477,387266,0,387266,977.7434411048889,0.0010003699783182796
77578,387771,0,387771,979.2737641334534,0.0010002977744198063
77678,388271,0,388271,980.6194379329681,0.001000227148553861
77778,388771,0,388771,982.4782059192657,0.0010001573505889897
77878,389271,0,389271,983.936402797699,0.0010000883510067086
77978,389771,0,389771,985.7973418235779,0.00100002012154977
78078,390271,0,390271,987.4387891292572,0.0009999526351641653
78178,390771,0,390771,989.5420920848846,0.0009998858659438607
78278,391271,0,391271,991.7075419425964,0.0009998197890782887
78378,391771,0,391771,993.5766279697418,0.0009997543808024057
78478,392271,0,392271,995.0680739879608,0.0009996896183491117
78579,392776,0,392776,996.6663122177124,0.0009996248415994845
78679,393276,0,393276,998.3626420497894,0.0009995613121867822
78779,393776,0,393776,1000.1034018993378,0.0009994983656459924
78879,394276,0,394276,1002.069384098053,0.0009994359827792925
78979,394776,0,394776,1003.6162359714508,0.000999374145181073
79079,395276,0,395276,1005.2721991539001,0.0009993128352026985
79179,395776,0,395776,1007.192461013794,0.0009992520359187996
79279,396276,0,396276,1008.8200640678406,0.0009991917310951985
79379,396776,0,396776,1010.4745950698853,0.000999131905158334
79479,397276,0,397276,1012.4346139431,0.000999072543166189
79580,397781,0,397781,1013.9567821025848,0.0009990130438800252
79680,398281,0,398281,1015.4120831489563,0.000998954571630389
79780,398781,0,398781,1016.8065431118011,0.0009988965218876624
79880,399281,0,399281,1018.2217981815338,0.0009988388819759566
79980,399781,0,399781,1019.6307120323181,0.0009987816397241205
80080,400281,0,400281,1021.0587708950043,0.0009987247834439663
80180,400781,0,400781,1022.4780530929565,0.0009986683019092754
80280,401281,0,401281,1023.8864040374756,0.0009986121843359953
80380,401781,0,401781,1025.4508130550385,0.000998556420363063
80480,402281,0,402281,1027.4131281375885,0.0009985010000344143
80581,402786,0,402786,1029.198026895523,0.000998445364574735
80681,403286,0,403286,1031.0756459236145,0.0009983906064038892
80781,403786,0,403786,1033.6144859790802,0.0009983361641826766
80881,404286,0,404286,1035.4325439929962,0.0009982820294124968
80981,404786,0,404786,1037.1614508628845,0.0009982281939204438
81081,405286,0,405286,1038.769049167633,0.000998174649845404
81181,405786,0,405786,1040.3544821739197,0.0009981213896251234
81281,406286,0,406286,1041.9363749027252,0.0009980684059834892
81381,406786,0,406786,1043.7816832065582,0.000998015691918577
81481,407286,0,407286,1045.4394800662994,0.0009979632406912253
81582,407791,0,407791,1047.0990130901337,0.0009979105251384831
81682,408291,0,408291,1048.7543559074402,0.0009978585828355796
81782,408791,0,408791,1050.567514181137,0.000997806884562805
81882,409291,0,409291,1052.163892030716,0.0009977554245291882
81982,409791,0,409791,1053.7594389915466,0.0009977041971561457
82082,410291,0,410291,1055.3463559150696,0.000997653197068746
82182,410791,0,410791,1056.9474210739136,0.0009976024190874867
82282,411291,0,411291,1058.5352098941803,0.000997551858219994
82382,411791,0,411791,1060.1158549785614,0.0009975015096536078
82482,412291,0,412291,1061.703506231308,0.0009974513687479164
82583,412796,0,412796,1063.3077201843262,0.0009974009326619482
82683,413296,0,413296,1064.906681060791,0.0009973511957781934
82783,413796,0,413796,1066.5089378356934,0.000997301653558031
82883,414296,0,414296,1068.0960409641266,0.0009972523019843645
82983,414796,0,414796,1069.6789209842682,0.0009972031371801025
83083,415296,0,415296,1071.2564420700073,0.0009971541554025208
83183,415796,0,415796,1072.8470141887665,0.0009971053530379143
83283,416296,0,416296,1074.4309208393097,0.0009970567265963207
83383,416796,0,416796,1076.008682012558,0.0009970082727066203
83483,417296,0,417296,1077.5977680683136,0.0009969599881118553
83584,417801,0,417801,1079.2038760185242,0.000996911389308784
83684,418301,0,418301,1080.802225112915,0.0009968634355828642
83784,418801,0,418801,1082.375051021576,0.0009968156419921724
83884,419301,0,419301,1083.9636731147766,0.0009967680056935557
83984,419801,0,419801,1085.566085100174,0.000996720523937052
84084,420301,0,420301,1087.1492249965668,0.0009966731940622016
84184,420801,0,420801,1088.7457950115204,0.0009966260134945905
84284,421301,0,421301,1090.3263640403748,0.000996578979742471
84384,421801,0,421801,1091.9163620471954,0.0009965320903934224
84484,422301,0,422301,1093.4880681037903,0.0009964853431114308
84585,422806,0,422806,1095.0956881046295,0.000996438270257591
84685,423306,0,423306,1096.6889200210571,0.0009963918017575242
84785,423806,0,423806,1098.2736990451813,0.0009963454687244308
84885,424306,0,424306,1099.8768801689148,0.0009962992690997685
84985,424806,0,424806,1101.4876132011414,0.0009962532008876647
85085,425306,0,425306,1103.1068170070648,0.000996207262152484
85185,425806,0,425806,1104.712984085083,0.00099616145101656
85285,426306,0,426306,1106.295737028122,0.000996115765657918
85385,426806,0,426806,1107.8875901699066,0.0009960702043082512
85485,427306,0,427306,1109.5461649894714,0.0009960247652508309
85586,427811,0,427811,1111.2565190792084,0.0009959789942378435
85686,428311,0,428311,1112.9975290298462,0.000995933795993393
85786,428811,0,428811,1114.6998660564423,0.0009958887151658453
85886,429311,0,429311,1116.4390230178833,0.000995843750226554
85986,429811,0,429811,1118.0907709598541,0.0009957988996893911
86086,430311,0,430311,1119.663358926773,0.0009957541621092698
86186,430811,0,430811,1121.2480170726776,0.0009957095360805357
86286,431311,0,431311,1122.833534002304,0.0009956650202355803
86386,431811,0,431811,1124.4476840496063,0.000995620613243358
86486,432311,0,432311,1126.0233631134033,0.0009955763138081643
86587,432816,0,432816,1127.6587150096893,0.0009955316792693825
86687,433316,0,433316,1129.3200340270996,0.0009954875922401562
86787,433816,0,433816,1130.9650650024414,0.000995443609067789
86887,434316,0,434316,1132.6098899841309,0.0009953997285854907
86987,434816,0,434816,1134.2075021266937,0.0009953559496557365
87087,435316,0,435316,1135.826672077179,0.0009953122711692688
87187,435816,0,435816,1137.4092309474945,0.0009952686920440183
87287,436316,0,436316,1139.0059251785278,0.0009952252112241974
87387,436816,0,436816,1140.606411933899,0.0009951818276793163
87487,437316,0,437316,1142.1952650547028,0.0009951385404033456
87588,437821,0,437821,1143.7724730968475,0.000995094916971815
87688,438321,0,438321,1145.3682868480682,0.000995051820247372
87788,438821,0,438821,1146.9478161334991,0.0009950088169025
87888,439321,0,439321,1148.5341639518738,0.0009949659060207326
87988,439821,0,439821,1150.108328819275,0.0009949230867060841
88088,440321,0,440321,1151.6977670192719,0.0009948803580822423
88188,440821,0,440821,1153.29576587677,0.000994837719292042
88288,441321,0,441321,1154.8734331130981,0.0009947951694966159
88388,441821,0,441821,1156.459079027176,0.0009947527078749286
88488,442321,0,442321,1158.056936264038,0.0009947103336231035
88589,442826,0,442826,1159.6635210514069,0.0009946676235117772
88689,443326,0,443326,1161.2265961170197,0.000994625422508149
88789,443826,0,443826,1162.8103229999542,0.000994583306552595
88889,444326,0,444326,1164.4012501239777,0.0009945412749045469
88989,444826,0,444826,1166.0013980865479,0.0009944993268379096
89089,445326,0,445326,1167.5668740272522,0.000994457461640552
89189,445826,0,445826,1169.144688129425,0.0009944156786139049
89289,446326,0,446326,1170.7467260360718,0.0009943739770726142
89389,446826,0,446826,1172.3354361057281,0.000994332356343912
89489,447326,0,447326,1173.8989639282227,0.0009942908157673576
89590,447831,0,447831,1175.538892030716,0.0009942489404830119
89690,448331,0,448331,1177.4305021762848,0.0009942075590621798
89790,448831,0,448831,1179.0191190242767,0.000994166255875874
89890,449331,0,449331,1180.589921951294,0.0009941250303091783
89990,449831,0,449831,1182.1696200370789,0.000994083881757629
90090,450331,0,450331,1183.7645418643951,0.000994042809626897
90190,450831,0,450831,1185.3461220264435,0.0009940018133325133
90290,451331,0,451331,1186.9639730453491,0.0009939608922995354
90390,451831,0,451831,1188.5574970245361,0.0009939200459623087
90490,452331,0,452331,1190.1407470703125,0.000993879273764106
90591,452836,0,452836,1191.730280160904,0.0009938381685406584
90691,453336,0,453336,1193.3202149868011,0.0009937975437127912
90791,453836,0,453836,1194.9115450382233,0.0009937569913997996
90891,454336,0,454336,1196.5064270496368,0.0009937165110784183
90991,454836,0,454836,1198.077075958252,0.000993676102233045
91091,455336,0,455336,1199.6597301959991,0.000993635764355674
91191,455836,0,455836,1201.2489340305328,0.0009935954969455517
91291,456336,0,456336,1202.8347170352936,0.0009935552995090496
91391,456836,0,456836,1204.4133307933807,0.000993515171559389
91491,457336,0,457336,1206.019623041153,0.0009934751126165601
91592,457841,0,457841,1207.6071631908417,0.0009934347226474678
91692,458341,0,458341,1209.1568920612335,0.0009933948009824003
91792,458841,0,458841,1210.7410390377045,0.000993354946917942
91892,459341,0,459341,1212.3323020935059,0.0009933151599991288
91992,459841,0,459841,1213.9237711429596,0.000993275439776908
92092,460341,0,460341,1215.5041861534119,0.0009932357858079288
92192,460841,0,460841,1217.0896360874176,0.0009931961976543408
92292,461341,0,461341,1218.6614079475403,0.0009931566748838056
92392,461841,0,461841,1220.2254619598389,0.0009931172170691345
92492,462341,0,462341,1221.8074889183044,0.0009930778237883576
92593,462846,0,462846,1223.407921075821,0.0009930381016552312
92693,463346,0,463346,1224.994973897934,0.0009929988368311536
92793,463846,0,463846,1226.5622498989105,0.0009929596353005392
92893,464346,0,464346,1228.14391207695,0.000992920496660714
92993,464846,0,464846,1229.7245230674744,0.0009928814205136622
93093,465346,0,465346,1231.3247270584106,0.0009928424064656858
93193,465846,0,465846,1232.8923690319061,0.0009928034541275075
93293,466346,0,466346,1234.4782240390778,0.0009927645631140148
93393,466845,0,466845,1236.0621621608734,0.0009566144773827764
93493,467345,0,467345,1237.6367909908295,0.0009552999840845761
93594,467850,0,467850,1239.2466940879822,0.0009540324558370261
93694,468350,0,468350,1240.836660861969,0.0009528220217901115
93794,468850,0,468850,1242.4292831420898,0.0009516529242226994
93894,469350,0,469350,1243.997458934784,0.0009505233527251142
93994,469850,0,469850,1245.5787391662598,0.0009494317804610445
94094,470350,0,470350,1247.1631710529327,0.000948376798156342
94194,470850,0,470850,1248.7456822395325,0.0009473570696901612
94294,471350,0,471350,1250.3074889183044,0.0009463713164634329
94394,471850,0,471850,1251.8975939750671,0.0009454183103379334
94494,472350,0,472350,1253.4902279376984,0.000944496869651086
94595,472855,0,472855,1255.0683801174164,0.0009435970963039847
94695,473355,0,473355,1256.650209903717,0.0009427357024540015
94795,473855,0,473855,1258.22598195076,0.000941902573360107
94895,474355,0,474355,1259.8383479118347,0.0009410966915345943
94995,474855,0,474855,1261.4190969467163,0.0009403170764220693
95095,475355,0,475355,1263.0051591396332,0.0009395627830543342
95195,475855,0,475855,1264.5943059921265,0.0009388329007734867
95295,476355,0,476355,1266.1753520965576,0.0009381265520108231
95395,476855,0,476855,1267.7434520721436,0.0009374428911137835
95495,477355,0,477355,1269.329400062561,0.0009367811032163659
95596,477860,0,477860,1270.9336659908295,0.0009361341000585821
95696,478360,0,478360,1272.688217163086,0.0009355139308819656
95796,478860,0,478860,1274.3659601211548,0.0009349133569568505
95896,479360,0,479360,1275.966245174408,0.0009343316762882444
95996,479860,0,479860,1277.5606231689453,0.0009337682125641215
96096,480360,0,480360,1279.14186501503,0.0009332223142367763
96196,480860,0,480860,1280.709811925888,0.0009326933536346096
96296,481360,0,481360,1282.2860178947449,0.0009321807261036787
96396,481860,0,481860,1283.8849141597748,0.0009316838491780523
96496,482360,0,482360,1285.4470751285553,0.0009312021617781276
96597,482865,0,482865,1287.0535850524902,0.0009307305252525971
96697,483365,0,483365,1288.6421279907227,0.0009302777540848755
96797,483865,0,483865,1290.2385551929474,0.0009298386049870601
96897,484365,0,484365,1291.802892923355,0.0009294125951201126
96997,484865,0,484865,1293.4338691234589,0.0009289992594080521
97097,485365,0,485365,1295.0364301204681,0.0009285981498877851
97197,485865,0,485865,1296.7013280391693,0.0009282088350819412
97297,486365,0,486365,1298.2774670124054,0.0009278308993933276
97397,486865,0,486865,1299.8802328109741,0.0009274639425209293
97497,487365,0,487365,1301.4888491630554,0.0009271075788963207
97598,487870,0,487870,1303.075101852417,0.0009267580261217038
97698,488370,0,488370,1304.6612470149994,0.0009264218454001378
97798,488870,0,488870,1306.2399332523346,0.0009260951808975818
97898,489370,0,489370,1307.8212690353394,0.0009257777008559627
97998,489870,0,489870,1309.4007630348206,0.0009254690857149768
98098,490370,0,490370,1310.9844698905945,0.0009251690276595051
98198,490870,0,490870,1312.5741090774536,0.0009248772301831271
98298,491370,0,491370,1314.1562111377716,0.0009245934076677388
98398,491870,0,491870,1315.7232098579407,0.0009243172849783144
98498,492370,0,492370,1317.3153629302979,0.0009240485970724168
98599,492875,0,492875,1318.9260499477386,0.0009237845089559853
98699,493375,0,493375,1320.514552116394,0.0009235300021168621
98799,493875,0,493875,1322.1019690036774,0.0009232821894713222
98899,494375,0,494375,1323.684697151184,0.0009230408428063386
98999,494875,0,494875,1325.2765119075775,0.0009228057422507594
99099,495375,0,495375,1326.8513040542603,0.0009225766759633897
99199,495875,0,495875,1328.4406859874725,0.0009223534398329786
99299,496375,0,496375,1330.0236120224,0.000922135837188981
99399,496875,0,496875,1331.612864971161,0.0009219236785233151
99499,497375,0,497375,1333.1818130016327,0.000921716781222369
99600,497880,0,497880,1334.7830669879913,0.0009215129762920005
99700,498380,0,498380,1336.369507074356,0.0009213161284996661
99800,498880,0,498880,1337.9339179992676,0.0009211240314615933
99900,499380,0,499380,1339.5383558273315,0.00092093652771461
100000,499880,0,499880,1341.131443977356,0.0009207534654906799


==> plot_data/quadratic_minimax_problem_n500_alpha0/flex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0015969276428222656,30.358099469249375
100,300,0,300,1.5694160461425781,0.2558362703474601
200,600,0,600,2.9680771827697754,0.08934174715128616
300,900,0,900,4.286312103271484,0.049966668660965975
400,1200,0,1200,5.708057165145874,0.0398780202880175
501,1503,0,1503,7.092475175857544,0.031023146174764506
601,1803,0,1803,8.427781105041504,0.02740508280333077
701,2103,0,2103,10.170363187789917,0.024792823540412883
801,2403,0,2403,11.865816116333008,0.022930474266950565
901,2703,0,2703,13.542758226394653,0.02066662381302666
1001,3003,0,3003,15.095815896987915,0.019409901675894764
1101,3303,0,3303,16.74511694908142,0.018346287894342544
1201,3603,0,3603,18.314565181732178,0.017428700280383937
1301,3903,0,3903,19.77242612838745,0.01688683574575832
1401,4203,0,4203,21.255264043807983,0.01580968769943279
1502,4506,0,4506,22.689154148101807,0.014860562367812719
1602,4806,0,4806,24.108537197113037,0.014170136818821281
1702,5106,0,5106,25.54394006729126,0.013542236609947626
1802,5406,0,5406,26.951202154159546,0.012716719834548059
1902,5706,0,5706,28.359397172927856,0.012120752412907982
2002,6006,0,6006,29.75666618347168,0.01106241751364803
2102,6306,0,6306,31.185136079788208,0.010520432173213728
2202,6606,0,6606,32.65068221092224,0.010198448836670001
2302,6906,0,6906,34.07006311416626,0.009612793657862223
2402,7206,0,7206,35.42251396179199,0.00894129650469258
2503,7509,0,7509,36.78331398963928,0.008526140473015769
2603,7809,0,7809,38.16009497642517,0.008155833364238745
2703,8109,0,8109,39.52156710624695,0.007773304942162857
2803,8409,0,8409,40.88197708129883,0.0075149241134036164
2903,8709,0,8709,42.25773215293884,0.007148950227893117
3003,9009,0,9009,43.656453132629395,0.006681389289289457
3103,9309,0,9309,45.031299114227295,0.006478944627865752
3203,9609,0,9609,46.399781227111816,0.006326875119112185
3303,9909,0,9909,47.76416015625,0.006028816379464502
3403,10209,0,10209,49.18382215499878,0.0054719963395598575
3504,10512,0,10512,50.629339933395386,0.005227779175794816
3604,10812,0,10812,52.0320930480957,0.0047220832941419835
3704,11112,0,11112,53.40615105628967,0.0044675117660608115
3804,11412,0,11412,54.766002893447876,0.004345113970815105
3904,11712,0,11712,56.148781061172485,0.004235563763521706
4004,12012,0,12012,57.544105052948,0.004142363327059376
4104,12312,0,12312,59.009462118148804,0.00396323733230897
4204,12612,0,12612,60.46846413612366,0.003711737119918045
4304,12912,0,12912,61.87884497642517,0.003607266074338986
4404,13212,0,13212,63.249160051345825,0.0034960592919285093
4505,13515,0,13515,64.68282914161682,0.0033088980902778917
4605,13815,0,13815,66.07096815109253,0.0032198439028488287
4705,14115,0,14115,67.47292590141296,0.003114687304005925
4805,14415,0,14415,68.88489818572998,0.0028966919178996012
4905,14715,0,14715,70.26894211769104,0.0028122775230047395
5005,15015,0,15015,71.68890595436096,0.0027295703794356025
5105,15315,0,15315,73.0758171081543,0.0025972937540775873
5205,15615,0,15615,74.51222610473633,0.0024631905500353984
5305,15915,0,15915,75.92449522018433,0.0024212514694853943
5405,16215,0,16215,77.31047201156616,0.002371449467810702
5506,16518,0,16518,78.70583200454712,0.0023261257472835836
5606,16818,0,16818,80.08439707756042,0.0022749912533666116
5706,17118,0,17118,81.49479293823242,0.0022429914236220655
5806,17418,0,17418,82.88986611366272,0.0022137995710937385
5906,17718,0,17718,84.28218913078308,0.002183990393921515
6006,18018,0,18018,85.65504097938538,0.0021310959063658556
6106,18318,0,18318,87.10112404823303,0.002096316275208014
6206,18618,0,18618,88.5438141822815,0.002053213593059352
6306,18918,0,18918,90.36730599403381,0.0020068434135671
6406,19218,0,19218,91.82156610488892,0.0019819352881957474
6507,19521,0,19521,93.22777915000916,0.0019492732078105854
6607,19821,0,19821,94.6450879573822,0.001923921533106785
6707,20121,0,20121,95.96497106552124,0.0018979154427699056
6807,20421,0,20421,97.31627798080444,0.0018741497301274957
6907,20721,0,20721,98.62140393257141,0.0018335562128723223
7007,21021,0,21021,100.05377316474915,0.0017489235812159728
7107,21321,0,21321,101.36753511428833,0.0017345246459863064
7207,21621,0,21621,102.63075709342957,0.0017128237066868625
7307,21921,0,21921,103.8886251449585,0.0016886356793179888
7407,22221,0,22221,105.13262224197388,0.001675870049511331
7508,22524,0,22524,106.49311304092407,0.0016634591742988047
7608,22824,0,22824,107.80947613716125,0.0016531797803861776
7708,23124,0,23124,109.16131210327148,0.00163707663617967
7808,23424,0,23424,110.4352970123291,0.0016288359103853955
7908,23724,0,23724,111.94999718666077,0.0016177937496011001
8008,24024,0,24024,113.36350202560425,0.0016046359767386395
8108,24324,0,24324,114.68658995628357,0.001583557087554361
8208,24624,0,24624,115.99757814407349,0.001573486183530159
8308,24924,0,24924,117.34181213378906,0.0015682218204635125
8408,25224,0,25224,118.72475290298462,0.0015624137298700408
8509,25527,0,25527,120.08925223350525,0.0015497819417693538
8609,25827,0,25827,121.38509607315063,0.0015282786511432722
8709,26127,0,26127,122.69814610481262,0.0015220383718983147
8809,26427,0,26427,124.07480716705322,0.001512859579084859
8909,26727,0,26727,125.55700516700745,0.0015006782333938451
9009,27027,0,27027,126.9446542263031,0.0014962553365997443
9109,27327,0,27327,128.33493399620056,0.0014911645579553977
9209,27627,0,27627,129.72102308273315,0.0014864907957856022
9309,27927,0,27927,131.09399700164795,0.0014783035177133763
9409,28227,0,28227,132.50326204299927,0.0014606623735140688
9510,28530,0,28530,133.8767511844635,0.0014501532326496656
9610,28830,0,28830,135.31188201904297,0.001446006011782139
9710,29130,0,29130,136.74404406547546,0.0014406175584614836
9810,29430,0,29430,138.16079115867615,0.001434236196280784
9910,29730,0,29730,139.5326521396637,0.0014319336103881216
10010,30030,0,30030,140.79992699623108,0.0014290112593095304
10110,30330,0,30330,142.09016132354736,0.0014250441319356144
10210,30630,0,30630,143.38939595222473,0.0014228873511461758
10310,30930,0,30930,144.67839097976685,0.0014204135096037756
10410,31230,0,31230,145.97482800483704,0.001417568299210541
10511,31533,0,31533,147.2867341041565,0.001414572959186711
10611,31833,0,31833,148.58600497245789,0.0014112818923716383
10711,32133,0,32133,149.8955042362213,0.001405574446687046
10811,32433,0,32433,151.16408514976501,0.0014008713172486422
10911,32733,0,32733,152.45430827140808,0.0013988167794346151
11011,33033,0,33033,153.74529790878296,0.0013976274601485415
11111,33333,0,33333,155.01189613342285,0.0013944267714944508
11211,33633,0,33633,156.284921169281,0.0013817367089062624
11311,33933,0,33933,157.55410504341125,0.0013758678224940223
11411,34233,0,34233,158.83529806137085,0.0013727133104956125
11512,34536,0,34536,160.14355516433716,0.0013705249464476656
11612,34836,0,34836,161.4009358882904,0.0013682075070303975
11712,35136,0,35136,162.6720061302185,0.0013631955166533399
11812,35436,0,35436,163.92781019210815,0.001360984485595176
11912,35736,0,35736,165.1882860660553,0.001358832794136238
12012,36036,0,36036,166.46630907058716,0.0013576474996599922
12112,36336,0,36336,167.72675728797913,0.0013542963012866496
12212,36636,0,36636,168.980486869812,0.0013509068043028795
12312,36936,0,36936,170.24967408180237,0.0013473320656411149
12412,37236,0,37236,171.54247093200684,0.001344224837772137
12513,37539,0,37539,172.83207297325134,0.0013433558619534497
12613,37839,0,37839,174.13171005249023,0.0013411752125357978
12713,38139,0,38139,175.43692111968994,0.0013393772505745861
12813,38439,0,38439,176.70044898986816,0.0013370498173664001
12913,38739,0,38739,178.1264271736145,0.0013342270627008281
13013,39039,0,39039,179.4231722354889,0.001333120817809904
13113,39339,0,39339,180.7413730621338,0.001332049551729179
13213,39639,0,39639,182.05028200149536,0.0013306183461351316
13313,39939,0,39939,183.7640299797058,0.0013291970498147427
13413,40239,0,40239,185.6734049320221,0.0013273655877062795
13514,40542,0,40542,187.06827592849731,0.001326042818516791
13614,40842,0,40842,188.3376920223236,0.0013223803814937153
13714,41142,0,41142,189.60523796081543,0.0013207989779952184
13814,41442,0,41442,190.84255695343018,0.0013192049404253485
13914,41742,0,41742,192.09608912467957,0.0013173567517233255
14014,42042,0,42042,193.3544099330902,0.0013134377299470516
14114,42342,0,42342,194.6783411502838,0.001310072728884646
14214,42642,0,42642,196.05291223526,0.0013082768899863543
14314,42942,0,42942,197.48633408546448,0.001306923211637527
14414,43242,0,43242,198.78944516181946,0.0013053866128682064
14515,43545,0,43545,200.1372790336609,0.0013037819168319998
14615,43845,0,43845,201.47660493850708,0.0013010462448687123
14715,44145,0,44145,202.74161505699158,0.00129825757002798
14815,44445,0,44445,204.00518918037415,0.0012958474844030298
14915,44745,0,44745,205.23338222503662,0.0012947299907995627
15015,45045,0,45045,206.49479818344116,0.0012921293217062419
15115,45345,0,45345,207.7180049419403,0.0012903560298100775
15215,45645,0,45645,208.9744701385498,0.0012882961400547499
15315,45945,0,45945,210.21420907974243,0.0012855284155758198
15415,46245,0,46245,211.45613598823547,0.0012829062707881034
15516,46548,0,46548,212.7536702156067,0.0012756397016340279
15616,46848,0,46848,214.0136260986328,0.0012645033221337267
15716,47148,0,47148,215.26300692558289,0.0012555683953441909
15816,47448,0,47448,216.52209305763245,0.0012501938211999305
15916,47748,0,47748,217.7616400718689,0.0012489939513468913
16016,48048,0,48048,219.08295512199402,0.001247226973879457
16116,48348,0,48348,220.3043611049652,0.0012445684350924308
16216,48648,0,48648,221.5479290485382,0.0012429850380510459
16316,48948,0,48948,222.76180624961853,0.001241099755936911
16416,49248,0,49248,223.99760794639587,0.0012393126369919165
16517,49551,0,49551,225.23018288612366,0.001237581221266661
16617,49851,0,49851,226.48560619354248,0.0012354001604315433
16717,50151,0,50151,227.7475130558014,0.0012338322866639476
16817,50451,0,50451,229.02727818489075,0.0012324222031389281
16917,50751,0,50751,230.31390523910522,0.0012310173003230664
17017,51051,0,51051,231.5667369365692,0.0012285346644902687
17117,51351,0,51351,232.79679894447327,0.0012274328710083565
17217,51651,0,51651,234.04590320587158,0.0012263145218749053
17317,51951,0,51951,235.27164506912231,0.0012238342024227069
17417,52251,0,52251,236.53643703460693,0.0012216112577641746
17518,52554,0,52554,237.76628828048706,0.001220241082545021
17618,52854,0,52854,239.0133090019226,0.0012183853347775071
17718,53154,0,53154,240.23838305473328,0.0012169969823719036
17818,53454,0,53454,241.49704718589783,0.0012149643647868633
17918,53754,0,53754,242.7138650417328,0.0012141074109121128
18018,54054,0,54054,243.92589712142944,0.0012121871220570981
18118,54354,0,54354,245.17532110214233,0.0012108359369192177
18218,54654,0,54654,246.40770411491394,0.0012091431277658615
18318,54954,0,54954,247.67426300048828,0.0012082790090564275
18418,55254,0,55254,248.92826390266418,0.0012071700638810277
18519,55557,0,55557,250.18697309494019,0.001205665404832755
18619,55857,0,55857,251.4319360256195,0.00120419756257901
18719,56157,0,56157,252.66520309448242,0.0012013663299247804
18819,56457,0,56457,253.92733502388,0.001197721873697065
18919,56757,0,56757,255.154314994812,0.0011967313717130622
19019,57057,0,57057,256.3873369693756,0.001194491952860044
19119,57357,0,57357,257.63742423057556,0.0011913341766767826
19219,57657,0,57657,258.8881149291992,0.001189105529927936
19319,57957,0,57957,260.14413499832153,0.0011878832368097184
19419,58257,0,58257,261.34748125076294,0.0011869613654411967
19520,58560,0,58560,262.60861325263977,0.0011861219081959592
19620,58860,0,58860,263.8351800441742,0.0011840736328174784
19720,59160,0,59160,265.0949990749359,0.0011809701342142633
19820,59460,0,59460,266.3303849697113,0.0011795762681907599
19920,59760,0,59760,267.58639001846313,0.0011781804675730374
20020,60060,0,60060,268.8307681083679,0.001175191660263676
20120,60360,0,60360,270.08409309387207,0.0011735573855025186
20220,60660,0,60660,271.35529804229736,0.0011721708347211144
20320,60960,0,60960,272.58766317367554,0.0011709727622967888
20420,61260,0,61260,273.83371901512146,0.0011696954333838745
20521,61563,0,61563,275.0834450721741,0.0011687254715802803
20621,61863,0,61863,276.32500195503235,0.0011675281919757243
20721,62163,0,62163,277.5738801956177,0.0011651024941697309
20821,62463,0,62463,278.818852186203,0.0011627230942854781
20921,62763,0,62763,280.06044006347656,0.0011607014210462878
21021,63063,0,63063,281.26293206214905,0.0011588680697333766
21121,63363,0,63363,282.495726108551,0.0011570776426560504
21221,63663,0,63663,283.7233350276947,0.0011542018562777276
21321,63963,0,63963,284.9812271595001,0.0011519860081981074
21421,64263,0,64263,286.2240540981293,0.0011500335881051854
21522,64566,0,64566,287.4732129573822,0.0011475045841565384
21622,64866,0,64866,288.72698497772217,0.0011418899922247385
21722,65166,0,65166,289.9748511314392,0.0011402733751764316
21822,65466,0,65466,291.2055311203003,0.0011392082999825087
21922,65766,0,65766,292.4308979511261,0.001137221906467666
22022,66066,0,66066,293.6828920841217,0.001133317702732984
22122,66366,0,66366,294.92602014541626,0.0011311187942485736
22222,66666,0,66666,296.14018416404724,0.0011290886661458898
22322,66966,0,66966,297.3732180595398,0.001126332697710338
22422,67266,0,67266,298.6148102283478,0.0011236954582241982
22523,67569,0,67569,299.87996006011963,0.0011224338066998273
22623,67869,0,67869,301.11781096458435,0.0011210565512563826
22723,68169,0,68169,302.3471989631653,0.0011199772450964807
22823,68469,0,68469,303.59064412117004,0.0011165611626388731
22923,68769,0,68769,304.80954122543335,0.0011137227140037868
23023,69069,0,69069,306.06455397605896,0.0011126272174653165
23123,69369,0,69369,307.2867810726166,0.0011109850978361204
23223,69669,0,69669,308.5380861759186,0.0011075967627041832
23323,69969,0,69969,309.7471261024475,0.0011029654586524676
23423,70269,0,70269,310.9844410419464,0.00110198720281138
23524,70572,0,70572,312.2997760772705,0.0011010999679867694
23624,70872,0,70872,313.89983105659485,0.0010988681551477267
23724,71172,0,71172,315.31279706954956,0.0010963683956424098
23824,71472,0,71472,316.5659761428833,0.0010947487012730732
23924,71772,0,71772,317.8002200126648,0.0010934433982869524
24024,72072,0,72072,319.13704919815063,0.0010916564024955949
24124,72372,0,72372,320.7117991447449,0.0010909954158764956
24224,72672,0,72672,322.2054352760315,0.0010898106470108835
24324,72972,0,72972,323.72267508506775,0.001088992810956058
24424,73272,0,73272,325.04703307151794,0.001087229150851696
24525,73575,0,73575,326.4398150444031,0.0010844650877890793
24625,73875,0,73875,327.8295261859894,0.0010785449139202074
24725,74175,0,74175,329.1407370567322,0.0010772225576503962
24825,74475,0,74475,330.39199209213257,0.0010758334475003317
24925,74775,0,74775,331.6338601112366,0.00107476291446671
25025,75075,0,75075,332.8800461292267,0.001073821502103086
25125,75375,0,75375,334.12925601005554,0.0010729084401243517
25225,75675,0,75675,335.36172318458557,0.0010716638054432505
25325,75975,0,75975,336.60751700401306,0.001069648078673986
25425,76275,0,76275,337.8526039123535,0.0010687599149591643
25526,76578,0,76578,339.08982706069946,0.001067665265103101
25626,76878,0,76878,340.64274311065674,0.0010659502585364097
25726,77178,0,77178,342.0128939151764,0.001055176792738626
25826,77478,0,77478,343.43451595306396,0.0010500520417326311
25926,77778,0,77778,344.95423316955566,0.0010488120193617163
26026,78078,0,78078,346.21037220954895,0.0010479146966527306
26126,78378,0,78378,347.5883960723877,0.0010471850642398517
26226,78678,0,78678,348.9197361469269,0.00104624198879052
26326,78978,0,78978,350.229807138443,0.0010455014447005642
26426,79278,0,79278,351.58213210105896,0.0010443354575868336
26527,79581,0,79581,352.8150689601898,0.0010425088718980277
26627,79881,0,79881,354.0677399635315,0.0010400259361896486
26727,80181,0,80181,355.2736802101135,0.00103756220906455
26827,80481,0,80481,356.6804051399231,0.0010367439331607916
26927,80781,0,80781,357.92480206489563,0.0010357784032456532
27027,81081,0,81081,359.2541608810425,0.001034996647003929
27127,81381,0,81381,360.5507252216339,0.0010337245962706355
27227,81681,0,81681,361.9320650100708,0.0010317018359446884
27327,81981,0,81981,363.2376801967621,0.001026612199637923
27427,82281,0,82281,364.50400614738464,0.0010240708877735328
27528,82584,0,82584,365.76367592811584,0.0010229652606323475
27628,82884,0,82884,367.1836030483246,0.001020932625230162
27728,83184,0,83184,368.5045120716095,0.0010189074511659432
27828,83484,0,83484,369.7486379146576,0.0010179436005081231
27928,83784,0,83784,370.9839632511139,0.0010164304809585324
28028,84084,0,84084,372.2045199871063,0.0010149426125149084
28128,84384,0,84384,373.43443298339844,0.0010141109076974787
28228,84684,0,84684,374.6699929237366,0.0010127375122014563
28328,84984,0,84984,375.8980002403259,0.001010998801106065
28428,85284,0,85284,377.1416709423065,0.001007927966664411
28529,85587,0,85587,378.3781991004944,0.0010067351260886494
28629,85887,0,85887,379.66813707351685,0.0010059473082282278
28729,86187,0,86187,380.8970482349396,0.0010051039512799325
28829,86487,0,86487,382.1628460884094,0.0010044338159953623
28929,86787,0,86787,383.40486311912537,0.0010038318649663218
29029,87087,0,87087,384.7445991039276,0.001002838655349658
29129,87387,0,87387,386.08296513557434,0.0010018314839037503
29229,87687,0,87687,387.45009207725525,0.0010006644287503955
29329,87987,0,87987,388.83616518974304,0.0009996994568165303
29429,88287,0,88287,390.0820801258087,0.0009989170483502966
29530,88590,0,88590,391.49170899391174,0.0009979989470967961
29630,88890,0,88890,392.8507490158081,0.0009969161349651443
29730,89190,0,89190,394.12720799446106,0.000996024895611673
29830,89490,0,89490,395.3598699569702,0.0009929890572871823
29930,89790,0,89790,396.5858380794525,0.000990840489829741
30030,90090,0,90090,397.92262291908264,0.000990237948234242
30130,90390,0,90390,399.1714780330658,0.0009895731447058561
30230,90690,0,90690,400.4008300304413,0.0009889563903741434
30330,90990,0,90990,401.6436140537262,0.0009880760514876137
30430,91290,0,91290,402.8750801086426,0.0009860076920814233
30531,91593,0,91593,404.12044405937195,0.0009829239010519229
30631,91893,0,91893,405.30564403533936,0.0009820160466940484
30731,92193,0,92193,406.5220990180969,0.000981219598050536
30831,92493,0,92493,407.7319700717926,0.0009802290086488182
30931,92793,0,92793,408.96454405784607,0.0009776153304173084
31031,93093,0,93093,410.181174993515,0.0009702062725641716
31131,93393,0,93393,411.39081501960754,0.0009660700498601589
31231,93693,0,93693,412.62924218177795,0.0009653853495388265
31331,93993,0,93993,413.8395709991455,0.0009642610571845044
31431,94293,0,94293,415.0666460990906,0.0009608375399531007
31532,94596,0,94596,416.2826511859894,0.0009595135649580971
31632,94896,0,94896,417.5091631412506,0.0009583537017346258
31732,95196,0,95196,418.7291660308838,0.0009564247213903133
31832,95496,0,95496,419.94564723968506,0.0009558543193272055
31932,95796,0,95796,421.17721700668335,0.0009549605630046007
32032,96096,0,96096,422.38077425956726,0.000954379228112735
32132,96396,0,96396,423.6159989833832,0.0009533922144121178
32232,96696,0,96696,424.82818508148193,0.0009515847300693806
32332,96996,0,96996,426.06440806388855,0.0009502919741958354
32432,97296,0,97296,427.27361607551575,0.0009483752513997578
32533,97599,0,97599,428.5167360305786,0.0009472043966983365
32633,97899,0,97899,429.748987197876,0.0009460277097995238
32733,98199,0,98199,430.9790871143341,0.0009437044879418617
32833,98499,0,98499,432.2127842903137,0.000939923060989245
32933,98799,0,98799,433.4258270263672,0.0009368303632945965
33033,99099,0,99099,434.65540409088135,0.0009351119005235398
33133,99399,0,99399,435.865198135376,0.0009336357123907699
33233,99699,0,99699,437.088191986084,0.0009324027768001497
33333,99999,0,99999,438.30022621154785,0.0009306255485093633
33433,100299,0,100299,439.53014612197876,0.0009292189548498899
33534,100602,0,100602,440.757755279541,0.0009278480201448256
33634,100902,0,100902,441.9720530509949,0.0009267720281092097
33734,101202,0,101202,443.20889496803284,0.000926040137566008
33834,101502,0,101502,444.42588114738464,0.0009251699542349449
33934,101802,0,101802,445.6523151397705,0.0009245582660759196
34034,102102,0,102102,446.856733083725,0.000923417847127761
34134,102402,0,102402,448.08529710769653,0.0009228602668796006
34234,102702,0,102702,449.29829716682434,0.0009219950058296013
34334,103002,0,103002,450.50719594955444,0.0009203500519986921
34434,103302,0,103302,451.7210760116577,0.0009193816228026097
34535,103605,0,103605,452.9386579990387,0.0009179665410526352
34635,103905,0,103905,454.178857088089,0.0009164231101394209
34735,104205,0,104205,455.379182100296,0.0009155325139882658
34835,104505,0,104505,456.6069450378418,0.0009138366044695793
34935,104805,0,104805,457.827702999115,0.0009119637904842533
35035,105105,0,105105,459.0925509929657,0.0009098010984321253
35135,105405,0,105405,460.35284304618835,0.0009071015102123827
35235,105705,0,105705,461.6326730251312,0.0009050247993081462
35335,106005,0,106005,462.96211099624634,0.0009041540394820126
35435,106305,0,106305,464.2832701206207,0.0009030773128404266
35536,106608,0,106608,465.68634128570557,0.0009015991287620287
35636,106908,0,106908,467.1455910205841,0.0008994103870773476
35736,107208,0,107208,468.5390999317169,0.0008960840022690119
35836,107508,0,107508,469.78106212615967,0.000894633647849851
35936,107808,0,107808,471.11541724205017,0.0008906145956874567
36036,108108,0,108108,472.4869439601898,0.0008895003752354714
36136,108408,0,108408,473.84032011032104,0.0008886173120793334
36236,108708,0,108708,475.1144902706146,0.0008879448005233853
36336,109008,0,109008,476.4608702659607,0.0008872894996239657
36436,109308,0,109308,477.96062111854553,0.0008866367554571187
36537,109611,0,109611,479.3088541030884,0.0008861426498784016
36637,109911,0,109911,480.5995891094208,0.0008853913358486045
36737,110211,0,110211,481.8702480792999,0.0008847359523240251
36837,110511,0,110511,483.3176620006561,0.0008842243757289713
36937,110811,0,110811,484.55541706085205,0.0008832651437926074
37037,111111,0,111111,485.76682305336,0.0008820021613373829
37137,111411,0,111411,486.9919822216034,0.0008801733384268476
37237,111711,0,111711,488.21957302093506,0.0008777143833189377
37337,112011,0,112011,489.44221901893616,0.0008767292930296168
37437,112311,0,112311,490.6730260848999,0.0008761448296295143
37538,112614,0,112614,491.9037609100342,0.0008748193212632686
37638,112914,0,112914,493.1417751312256,0.0008727923735337776
37738,113214,0,113214,494.36538004875183,0.0008719879738567836
37838,113514,0,113514,495.5904881954193,0.0008711837190499763
37938,113814,0,113814,496.81163024902344,0.0008695644063248293
38038,114114,0,114114,498.0359799861908,0.0008687438241928864
38138,114414,0,114414,499.2672700881958,0.0008648899299744492
38238,114714,0,114714,500.489706993103,0.00085969240292651
38338,115014,0,115014,501.7139639854431,0.0008577549013736174
38438,115314,0,115314,502.9428701400757,0.0008572831017019176
38539,115617,0,115617,504.1942400932312,0.0008563726502165314
38639,115917,0,115917,505.5049510002136,0.0008555725479002678
38739,116217,0,116217,506.91988706588745,0.0008544889979270137
38839,116517,0,116517,508.31813502311707,0.0008533311217068639
38939,116817,0,116817,509.5243682861328,0.0008524786138481396
39039,117117,0,117117,510.73708319664,0.0008517692982830438
39139,117417,0,117417,512.0229871273041,0.0008504550413735417
39239,117717,0,117717,513.4491541385651,0.0008497756585359997
39339,118017,0,118017,514.7585589885712,0.0008489372530253166
39439,118317,0,118317,516.0033342838287,0.0008482525047326497
39540,118620,0,118620,517.2516810894012,0.0008474655744270842
39640,118920,0,118920,518.4912271499634,0.0008468124336527605
39740,119220,0,119220,519.7162082195282,0.0008449799560189141
39840,119520,0,119520,520.9409620761871,0.0008440275514948031
39940,119820,0,119820,522.1587331295013,0.0008429611068873121
40040,120120,0,120120,523.3891499042511,0.000841536496613625
40140,120420,0,120420,524.610758304596,0.0008401715507470532
40240,120720,0,120720,525.8275480270386,0.0008386097913270066
40340,121020,0,121020,527.0438079833984,0.0008373759551088232
40440,121320,0,121320,528.2632701396942,0.0008367487827636548
40541,121623,0,121623,529.4910368919373,0.000835949485029184
40641,121923,0,121923,530.7242529392242,0.0008350252319187682
40741,122223,0,122223,531.9498281478882,0.0008333132101913377
40841,122523,0,122523,533.1663889884949,0.0008303043126705423
40941,122823,0,122823,534.3838069438934,0.0008119140811226807
41041,123123,0,123123,535.6061260700226,0.0007590166832365952
41141,123423,0,123423,536.8244531154633,0.0007487985111082222
41241,123723,0,123723,538.0472500324249,0.0007470430947968511
41341,124023,0,124023,539.2710690498352,0.000745548757977841
41441,124323,0,124323,540.4919991493225,0.0007439000025036214
41542,124626,0,124626,541.7217390537262,0.0007411874641129794
41642,124926,0,124926,542.9377040863037,0.000740311961204941
41742,125226,0,125226,544.1587951183319,0.0007397537447510106
41842,125526,0,125526,545.3816199302673,0.0007383930003967323
41942,125826,0,125826,546.5928530693054,0.0007378595320380245
42042,126126,0,126126,547.8210439682007,0.0007372264300234999
42142,126426,0,126426,549.0428080558777,0.0007367461977622037
42242,126726,0,126726,550.2661399841309,0.000735785826992971
42342,127026,0,127026,551.5043683052063,0.0007343167893560696
42442,127326,0,127326,552.7151770591736,0.0007336047388088667
42543,127629,0,127629,553.9680099487305,0.0007328752686529141
42643,127929,0,127929,555.1962969303131,0.0007323955315045733
42743,128229,0,128229,556.4223830699921,0.000731901421297615
42843,128529,0,128529,557.6452550888062,0.0007312553701311701
42943,128829,0,128829,558.8852250576019,0.0007306142411620908
43043,129129,0,129129,560.1170451641083,0.000729638534647603
43143,129429,0,129429,561.330983877182,0.0007287879947397675
43243,129729,0,129729,562.5588660240173,0.00072828228959458
43343,130029,0,130029,563.7703051567078,0.000727701221827724
43443,130329,0,130329,564.9930801391602,0.0007266882989497586
43544,130632,0,130632,566.2096331119537,0.0007261962582747437
43644,130932,0,130932,567.4349009990692,0.0007256099450452921
43744,131232,0,131232,568.6552813053131,0.0007250928529656784
43844,131532,0,131532,569.883632183075,0.000724507093826673
43944,131832,0,131832,571.1084380149841,0.0007241269439781214
44044,132132,0,132132,572.3270552158356,0.0007234663905146113
44144,132432,0,132432,573.5825481414795,0.0007220397082833272
44244,132732,0,132732,574.8638331890106,0.0007209867072720764
44344,133032,0,133032,576.1847450733185,0.000720436017096445
44444,133332,0,133332,577.5400750637054,0.0007195726834625768
44545,133635,0,133635,578.8453681468964,0.0007177771251470691
44645,133935,0,133935,580.2542111873627,0.000717235544023042
44745,134235,0,134235,581.6388449668884,0.0007167867639739866
44845,134535,0,134535,582.9369232654572,0.0007157385050023212
44945,134835,0,134835,584.169379234314,0.0007152487454922015
45045,135135,0,135135,585.3787660598755,0.0007145734588752367
45145,135435,0,135435,586.6105711460114,0.0007137823424339932
45245,135735,0,135735,587.8287010192871,0.0007123261506942164
45345,136035,0,136035,589.0607490539551,0.0007108672708572434
45445,136335,0,136335,590.2803020477295,0.0007102244750550476
45546,136638,0,136638,591.497955083847,0.0007095909275271812
45646,136938,0,136938,592.702320098877,0.0007081567756591645
45746,137238,0,137238,593.9122622013092,0.0007074597539630707
45846,137538,0,137538,595.226998090744,0.0007068721203844337
45946,137838,0,137838,596.657552242279,0.0007060976121716529
46046,138138,0,138138,597.9949040412903,0.0007054518994480115
46146,138438,0,138438,599.3453462123871,0.0007047942565629794
46246,138738,0,138738,600.6528551578522,0.0007039881164621114
46346,139038,0,139038,601.9522559642792,0.0007032546790122766
46446,139338,0,139338,603.1853060722351,0.0007025878884524528
46547,139641,0,139641,604.464714050293,0.0007016723357656403
46647,139941,0,139941,605.6923110485077,0.0007012425206700386
46747,140241,0,140241,606.9221441745758,0.0007007239349467312
46847,140541,0,140541,608.1836092472076,0.0007000515230333616
46947,140841,0,140841,609.4050571918488,0.0006994433612603057
47047,141141,0,141141,610.6421670913696,0.0006982772927788506
47147,141441,0,141441,611.8637609481812,0.0006973727375403176
47247,141741,0,141741,613.0858361721039,0.000696917017147061
47347,142041,0,142041,614.3551690578461,0.0006959844877530698
47447,142341,0,142341,615.575777053833,0.0006948342166578055
47548,142644,0,142644,616.8963141441345,0.0006864544057144053
47648,142944,0,142944,618.2634408473969,0.0006852113229276288
47748,143244,0,143244,619.6108741760254,0.0006844070407610722
47848,143544,0,143544,620.8368740081787,0.0006827593859874263
47948,143844,0,143844,622.0683121681213,0.0006815144199454441
48048,144144,0,144144,623.3129489421844,0.0006804808975328117
48148,144444,0,144444,624.5993421077728,0.000678942987145915
48248,144744,0,144744,625.8469409942627,0.0006776952543140685
48348,145044,0,145044,627.0991492271423,0.0006770043692948831
48448,145344,0,145344,628.3401942253113,0.00067638028477074
48549,145647,0,145647,629.5828862190247,0.0006758065599945088
48649,145947,0,145947,630.7894999980927,0.0006751556961370021
48749,146247,0,146247,632.0311989784241,0.0006744109781835276
48849,146547,0,146547,633.2358210086823,0.0006738992708169269
48949,146847,0,146847,634.4911119937897,0.0006732451528439657
49049,147147,0,147147,635.6897668838501,0.0006727189795708835
49149,147447,0,147447,636.9060659408569,0.0006700191944843335
49249,147747,0,147747,638.1447460651398,0.0006686761599754407
49349,148047,0,148047,639.3697581291199,0.000667317842151808
49449,148347,0,148347,640.6028780937195,0.0006662611993357956
49550,148650,0,148650,641.8321652412415,0.0006655523811570574
49650,148950,0,148950,643.0769250392914,0.0006647984177003939
49750,149250,0,149250,644.2973189353943,0.0006640611085803307
49850,149550,0,149550,645.5276951789856,0.0006635406523901869
49950,149850,0,149850,646.7368819713593,0.0006628078044517721
50050,150150,0,150150,647.9690170288086,0.0006608911734069305
50150,150450,0,150450,649.1909019947052,0.0006562164335811679
50250,150750,0,150750,650.4004333019257,0.0006544368205241681
50350,151050,0,151050,651.638833284378,0.0006536878375239248
50450,151350,0,151350,652.8553750514984,0.0006530443907935748
50551,151653,0,151653,654.0985569953918,0.0006520902862785296
50651,151953,0,151953,655.3026621341705,0.0006509325063735403
50751,152253,0,152253,656.5384089946747,0.0006503200436920259
50851,152553,0,152553,657.7635791301727,0.000649641206773616
50951,152853,0,152853,659.0028111934662,0.0006491383619415057
51051,153153,0,153153,660.2401180267334,0.0006486193543861046
51151,153453,0,153453,661.4646921157837,0.0006480233225472775
51251,153753,0,153753,662.6930310726166,0.0006474110254226607
51351,154053,0,154053,663.9042510986328,0.0006466904427954644
51451,154353,0,154353,665.1404581069946,0.000645088345250674
51552,154656,0,154656,666.3624069690704,0.0006445218147952175
51652,154956,0,154956,667.5855560302734,0.0006436004279815873
51752,155256,0,155256,668.820405960083,0.0006430177708872788
51852,155556,0,155556,670.0479681491852,0.000642633360288959
51952,155856,0,155856,671.2761981487274,0.0006417063740433708
52052,156156,0,156156,672.5000672340393,0.0006402564242491376
52152,156456,0,156456,673.7222490310669,0.00063807349326587
52252,156756,0,156756,674.9371101856232,0.000637572344085148
52352,157056,0,157056,676.1612710952759,0.0006371480234957903
52452,157356,0,157356,677.3805260658264,0.0006363309096176427
52553,157659,0,157659,678.6029100418091,0.0006331733252719376
52653,157959,0,157959,679.8477811813354,0.0006315959426697869
52753,158259,0,158259,681.1299710273743,0.0006307803525219773
52853,158559,0,158559,682.4489049911499,0.0006301313291565285
52953,158859,0,158859,683.7920892238617,0.0006296154308539065
53053,159159,0,159159,685.0764091014862,0.0006292316352709571
53153,159459,0,159459,686.4276280403137,0.0006288605389822458
53253,159759,0,159759,687.8275241851807,0.0006282301234460855
53353,160059,0,160059,689.0614039897919,0.0006278347307699257
53453,160359,0,160359,690.2691051959991,0.0006274087294359957
53554,160662,0,160662,691.5061190128326,0.0006264337806461785
53654,160962,0,160962,692.7293939590454,0.0006248610367358952
53754,161262,0,161262,693.9509391784668,0.0006244146688379872
53854,161562,0,161562,695.1856400966644,0.0006238257039013878
53954,161862,0,161862,696.3962481021881,0.0006230003201073192
54054,162162,0,162162,697.6152052879333,0.0006220912279851379
54154,162462,0,162462,698.9199471473694,0.0006214936301118038
54254,162762,0,162762,700.1833872795105,0.0006209047999644951
54354,163062,0,163062,701.9442460536957,0.000620255403023788
54454,163362,0,163362,703.2725040912628,0.0006196711802078532
54555,163665,0,163665,705.2190940380096,0.000619036750498362
54655,163965,0,163965,706.5347471237183,0.0006184952308997191
54755,164265,0,164265,708.0725839138031,0.0006176874404313761
54855,164565,0,164565,709.7319722175598,0.0006169454939926869
54955,164865,0,164865,711.2085099220276,0.000616000770849363
55055,165165,0,165165,712.5812659263611,0.0006154948635263304
55155,165465,0,165465,714.1699810028076,0.0006143347267016441
55255,165765,0,165765,715.5163321495056,0.0006133731859060464
55355,166065,0,166065,716.7922630310059,0.000612888596729997
55455,166365,0,166365,718.0101759433746,0.0006124731132866772
55556,166668,0,166668,719.7303411960602,0.0006117183645350648
55656,166968,0,166968,721.9904389381409,0.000610487206527667
55756,167268,0,167268,723.7813980579376,0.0006093784033561696
55856,167568,0,167568,725.0034160614014,0.0006089685738227394
55956,167868,0,167868,726.20942902565,0.0006086798626941223
56056,168168,0,168168,727.4254789352417,0.0006081931171287217
56156,168468,0,168468,728.6548140048981,0.0006075243906265929
56256,168768,0,168768,729.874715089798,0.000606458571810622
56356,169068,0,169068,731.1044390201569,0.0006051050847458595
56456,169368,0,169368,732.3384199142456,0.0006047528964456979
56557,169671,0,169671,733.5940201282501,0.0006040568613076421
56657,169971,0,169971,734.8227939605713,0.0006034897393757673
56757,170271,0,170271,736.0212481021881,0.0006026961113316634
56857,170571,0,170571,737.258373260498,0.0006020155026849796
56957,170871,0,170871,738.4874041080475,0.0006013615186289335
57057,171171,0,171171,739.7215840816498,0.0005996902355359091
57157,171471,0,171471,740.9552371501923,0.0005971181389293232
57257,171771,0,171771,742.2011280059814,0.0005965495577200221
57357,172071,0,172071,743.4441123008728,0.0005961369616345668
57457,172371,0,172371,744.6636111736298,0.0005955298448284727
57558,172674,0,172674,745.93119597435,0.0005948726395337213
57658,172974,0,172974,747.0970942974091,0.0005943580401264034
57758,173274,0,173274,748.3021581172943,0.0005938729367378186
57858,173574,0,173574,749.4788701534271,0.000593239563667743
57958,173874,0,173874,750.6790752410889,0.0005926033466683658
58058,174174,0,174174,752.0660212039948,0.0005922181890898773
58158,174474,0,174474,753.3775329589844,0.0005912305538758527
58258,174774,0,174774,754.6557152271271,0.000590572800410807
58358,175074,0,175074,755.8211042881012,0.0005894691578600356
58458,175374,0,175374,757.1501250267029,0.0005890257071211079
58559,175677,0,175677,758.4196510314941,0.0005881614742855243
58659,175977,0,175977,760.0574991703033,0.0005868217406184607
58759,176277,0,176277,761.3517181873322,0.0005859421863997383
58859,176577,0,176577,762.5510110855103,0.0005844577717837775
58959,176877,0,176877,763.8500111103058,0.0005815446862197296
59059,177177,0,177177,765.124537229538,0.0005801208622523852
59159,177477,0,177477,766.3319702148438,0.0005789864121289067
59259,177777,0,177777,767.6357560157776,0.0005771138648279465
59359,178077,0,178077,768.9127922058105,0.0005766174464682126
59459,178377,0,178377,770.1498839855194,0.000575442152788154
59560,178680,0,178680,771.3668642044067,0.0005747741090570921
59660,178980,0,178980,772.54421210289,0.0005743993091414956
59760,179280,0,179280,773.7525990009308,0.000573806528693677
59860,179580,0,179580,774.9620401859283,0.00057303628080431
59960,179880,0,179880,776.2717771530151,0.000572565903642297
60060,180180,0,180180,777.7211589813232,0.0005721312707595731
60160,180480,0,180480,778.9830729961395,0.0005717689179896899
60260,180780,0,180780,780.2867901325226,0.0005711682167462691
60360,181080,0,181080,781.5978391170502,0.0005707173037757159
60460,181380,0,181380,782.88818526268,0.0005701610254948574
60561,181683,0,181683,784.1372489929199,0.0005694624940560586
60661,181983,0,181983,785.3476741313934,0.0005690612857129664
60761,182283,0,182283,786.591982126236,0.0005685445470392144
60861,182583,0,182583,787.9121179580688,0.0005676979321994044
60961,182883,0,182883,789.521595954895,0.000566956291887927
61061,183183,0,183183,790.7123122215271,0.0005662545416269846
61161,183483,0,183483,791.8912279605865,0.0005657423723739387
61261,183783,0,183783,793.152596950531,0.0005648299753100237
61361,184083,0,184083,794.7179141044617,0.0005639695573972716
61461,184383,0,184383,795.908215045929,0.0005634476386195715
61562,184686,0,184686,797.1836321353912,0.000562754587035744
61662,184986,0,184986,798.3014781475067,0.0005621684732616463
61762,185286,0,185286,799.4205319881439,0.0005617752140069521
61862,185586,0,185586,800.5364952087402,0.000560669579413228
61962,185886,0,185886,801.6321301460266,0.0005581142092160341
62062,186186,0,186186,802.7453792095184,0.0005571935883617886
62162,186486,0,186486,803.8506519794464,0.0005567609041974142
62262,186786,0,186786,804.9670789241791,0.0005562738739972281
62362,187086,0,187086,806.0639569759369,0.0005558627348703859
62462,187386,0,187386,807.173798084259,0.0005552435353033494
62563,187689,0,187689,808.2784271240234,0.0005544952578693931
62663,187989,0,187989,809.3904950618744,0.0005533856606164424
62763,188289,0,188289,810.4954700469971,0.0005528438286388633
62863,188589,0,188589,811.6175980567932,0.0005522224555336209
62963,188889,0,188889,812.7290229797363,0.0005515992960435067
63063,189189,0,189189,813.8234710693359,0.0005511368743598585
63163,189489,0,189489,814.9228720664978,0.0005507479393848278
63263,189789,0,189789,816.0236940383911,0.0005501372745601703
63363,190089,0,190089,817.1325371265411,0.0005498106158902674
63463,190389,0,190389,818.2435519695282,0.0005490574970581004
63564,190692,0,190692,819.3747310638428,0.0005476270428156373
63664,190992,0,190992,820.4751009941101,0.0005446095395582427
63764,191292,0,191292,821.5910320281982,0.0005424007889692499
63864,191592,0,191592,822.6962890625,0.0005416379453507622
63964,191892,0,191892,823.8030490875244,0.0005410688831858528
64064,192192,0,192192,824.903923034668,0.0005407070440719842
64164,192492,0,192492,826.0154249668121,0.0005402984385255615
64264,192792,0,192792,827.1120011806488,0.0005397376379087241
64364,193092,0,193092,828.2192461490631,0.0005391212681581047
64464,193392,0,193392,829.3088021278381,0.0005385712357714674
64565,193695,0,193695,830.4218621253967,0.0005382630198933264
64665,193995,0,193995,831.5202391147614,0.0005378466686390083
64765,194295,0,194295,832.6273851394653,0.0005372771413147472
64865,194595,0,194595,833.7251441478729,0.0005363422865862864
64965,194895,0,194895,834.8265030384064,0.0005353884923918622
65065,195195,0,195195,835.9229040145874,0.0005349399879971648
65165,195495,0,195495,837.0370519161224,0.0005342669435196994
65265,195795,0,195795,838.1325681209564,0.0005338235945966457
65365,196095,0,196095,839.2406551837921,0.0005331810176995092
65465,196395,0,196395,840.3286850452423,0.0005321898075030306
65566,196698,0,196698,841.4483089447021,0.0005316526940853353
65666,196998,0,196998,842.5590310096741,0.0005309665590372361
65766,197298,0,197298,843.6643152236938,0.0005303400198899217
65866,197598,0,197598,844.7610702514648,0.000529961910624051
65966,197898,0,197898,845.8759210109711,0.0005294674951389832
66066,198198,0,198198,846.976674079895,0.0005287847874388455
66166,198498,0,198498,848.103226184845,0.0005273148480771423
66266,198798,0,198798,849.1967470645905,0.0005262471453920353
66366,199098,0,199098,850.2999889850616,0.0005257304375208429
66466,199398,0,199398,851.3972091674805,0.0005244198620124955
66567,199701,0,199701,852.5274062156677,0.000522557094275223
66667,200001,0,200001,853.632404088974,0.0005220566534213724
66767,200301,0,200301,854.7500381469727,0.0005216571240952762
66867,200601,0,200601,855.8574631214142,0.0005209613749127301
66967,200901,0,200901,856.9698979854584,0.0005204568355129876
67067,201201,0,201201,858.132826089859,0.0005196463079730917
67167,201501,0,201501,859.2898831367493,0.0005188437269134972
67267,201801,0,201801,860.4568800926208,0.0005178540722818069
67367,202101,0,202101,861.7431440353394,0.0005170933852292802
67467,202401,0,202401,862.9984781742096,0.0005167490186967363
67568,202704,0,202704,864.3050670623779,0.0005162916875287171
67668,203004,0,203004,865.5311779975891,0.000515580869003265
67768,203304,0,203304,866.654443025589,0.0005148390084276197
67868,203604,0,203604,867.7677590847015,0.0005141907162216273
67968,203904,0,203904,868.8719229698181,0.0005111375859949342
68068,204204,0,204204,869.9903008937836,0.0005101981853689954
68168,204504,0,204504,871.1027159690857,0.0005096760066557091
68268,204804,0,204804,872.2146060466766,0.0005089732938106612
68368,205104,0,205104,873.3406701087952,0.0005082718874911528
68468,205404,0,205404,874.4439611434937,0.0005074038920096846
68569,205707,0,205707,875.5730969905853,0.0005070267492171268
68669,206007,0,206007,876.7158210277557,0.0005060023844627907
68769,206307,0,206307,877.8630900382996,0.000505156616016454
68869,206607,0,206607,879.0017399787903,0.0005048327815682712
68969,206907,0,206907,880.123594045639,0.0005045461938443676
69069,207207,0,207207,881.267664194107,0.0005040347843203674
69169,207507,0,207507,882.3741393089294,0.0005033624915792105
69269,207807,0,207807,883.4902031421661,0.0005028559477344767
69369,208107,0,208107,884.5989890098572,0.0005021103184002664
69469,208407,0,208407,885.6982390880585,0.0005007512522101072
69570,208710,0,208710,886.9205601215363,0.0004984075197913206
69670,209010,0,209010,888.2502992153168,0.0004980172082220609
69770,209310,0,209310,889.4995341300964,0.000497225198149776
69870,209610,0,209610,890.6811480522156,0.0004966792240987585
69970,209910,0,209910,891.7849841117859,0.0004961352959364887
70070,210210,0,210210,892.8879020214081,0.0004956020176086365
70170,210510,0,210510,893.9965372085571,0.0004951255932356604
70270,210810,0,210810,895.1012370586395,0.0004946015961860883
70370,211110,0,211110,896.2047622203827,0.0004940031093638795
70470,211410,0,211410,897.3107631206512,0.0004934403103136281
70571,211713,0,211713,898.4202382564545,0.0004930900225894213
70671,212013,0,212013,899.5374143123627,0.0004927059980740222
70771,212313,0,212313,900.6369531154633,0.0004922583925407336
70871,212613,0,212613,901.7416388988495,0.000491876656397582
70971,212913,0,212913,902.8826420307159,0.0004912457047843515
71071,213213,0,213213,904.1405341625214,0.0004905299596944029
71171,213513,0,213513,905.3562109470367,0.0004899796415272428
71271,213813,0,213813,906.5932130813599,0.0004893326696859011
71371,214113,0,214113,907.6965661048889,0.0004888460948290847
71471,214413,0,214413,908.8113920688629,0.0004883770514314606
71572,214716,0,214716,910.0099079608917,0.00048794652300085785
71672,215016,0,215016,911.2348790168762,0.0004872604887556261
71772,215316,0,215316,912.4262480735779,0.0004865268251114978
71872,215616,0,215616,913.6701571941376,0.0004856029875293046
71972,215916,0,215916,914.9214148521423,0.0004852205427598473
72072,216216,0,216216,916.0292711257935,0.0004847765633196455
72172,216516,0,216516,917.1385090351105,0.0004844751133646553
72272,216816,0,216816,918.2415151596069,0.00048403786932774086
72372,217116,0,217116,919.3458518981934,0.0004836741201958151
72472,217416,0,217416,920.4308910369873,0.0004832313424054268
72573,217719,0,217719,921.5535428524017,0.0004829235948065574
72673,218019,0,218019,922.6551780700684,0.00048257172199848785
72773,218319,0,218319,923.762552022934,0.00048224529176755534
72873,218619,0,218619,924.9161880016327,0.0004810976487404138
72973,218919,0,218919,926.0275819301605,0.00047857269123685673
73073,219219,0,219219,927.1237711906433,0.00047755417577535834
73173,219519,0,219519,928.2290949821472,0.0004769788614952369
73273,219819,0,219819,929.3295521736145,0.00047655249940224584
73373,220119,0,220119,930.4425389766693,0.00047630947929024753
73473,220419,0,220419,931.5495979785919,0.00047577930024776324
73574,220722,0,220722,932.6716091632843,0.0004754492590724056
73674,221022,0,221022,933.7717161178589,0.0004751546654916138
73774,221322,0,221322,934.8876402378082,0.00047490139345277406
73874,221622,0,221622,935.9947619438171,0.0004740945513420383
73974,221922,0,221922,937.1118421554565,0.0004730054114912867
74074,222222,0,222222,938.2265350818634,0.0004726719668715093
74174,222522,0,222522,939.3722941875458,0.00047220275315679953
74274,222822,0,222822,940.6456918716431,0.00047178508421315924
74374,223122,0,223122,941.8419210910797,0.0004709733174584925
74474,223422,0,223422,943.0998950004578,0.0004702665197045311
74575,223725,0,223725,944.3025450706482,0.00046980776820888597
74675,224025,0,224025,945.5947918891907,0.000469355822981002
74775,224325,0,224325,946.6924750804901,0.00046868316978229175
74875,224625,0,224625,947.8044202327728,0.00046661929283167247
74975,224925,0,224925,948.8978481292725,0.00046494847420212187
75075,225225,0,225225,950.0104231834412,0.00046455883550238056
75175,225525,0,225525,951.0993139743805,0.00046382970658304817
75275,225825,0,225825,952.2007710933685,0.00046302207194441673
75375,226125,0,226125,953.2941410541534,0.000461919997087925
75475,226425,0,226425,954.4032802581787,0.0004613342667836558
75576,226728,0,226728,955.5208201408386,0.00046060544834356214
75676,227028,0,227028,956.6273670196533,0.00045995855246999163
75776,227328,0,227328,957.7228710651398,0.00045860626122338366
75876,227628,0,227628,958.829118013382,0.00045798575185682685
75976,227928,0,227928,959.9265310764313,0.0004565894504983974
76076,228228,0,228228,961.0369470119476,0.0004561786465257795
76176,228528,0,228528,962.1314740180969,0.00045576023938751094
76276,228828,0,228828,963.2422270774841,0.00045546406449586296
76376,229128,0,229128,964.3516800403595,0.00045514925515126244
76476,229428,0,229428,965.4620831012726,0.0004548621381002862
76577,229731,0,229731,966.584529876709,0.00045384593283627505
76677,230031,0,230031,967.7962622642517,0.0004491853475986565
76777,230331,0,230331,969.0749661922455,0.00043900999345650074
76877,230631,0,230631,970.2259521484375,0.00042973297367062134
76977,230931,0,230931,971.4221200942993,0.0004196769048801795
77077,231231,0,231231,972.5619411468506,0.00040054739661930745
77177,231531,0,231531,973.7222049236298,0.0003773720401448776
77277,231831,0,231831,974.8984639644623,0.00036790630655279117
77377,232131,0,232131,976.0893449783325,0.00036069038050100884
77477,232431,0,232431,977.3107709884644,0.00035851744035582405
77578,232734,0,232734,978.8712818622589,0.00035796356380773844
77678,233034,0,233034,980.0742740631104,0.0003576692811063946
77778,233334,0,233334,981.1946649551392,0.0003573019715404646
77878,233634,0,233634,982.3800251483917,0.0003566204661239445
77978,233934,0,233934,983.6968531608582,0.00035623092503510675
78078,234234,0,234234,984.8589670658112,0.0003559144610051128
78178,234534,0,234534,985.9630982875824,0.00035536736980298526
78278,234834,0,234834,987.0973470211029,0.0003547461956996096
78378,235134,0,235134,988.2020878791809,0.00035427261262623396
78478,235434,0,235434,989.3539352416992,0.0003539875991934468
78579,235737,0,235737,990.5014090538025,0.0003537871456752606
78679,236037,0,236037,991.6150379180908,0.0003535167452448984
78779,236337,0,236337,992.7444059848785,0.000353127408251749
78879,236637,0,236637,993.8709151744843,0.0003529153703106347
78979,236937,0,236937,995.1454889774323,0.00035209057451026596
79079,237237,0,237237,996.3894562721252,0.00035092392453489943
79179,237537,0,237537,997.6438360214233,0.00035062734370245387
79279,237837,0,237837,998.8848309516907,0.0003503322890290421
79379,238137,0,238137,1000.243411064148,0.0003497658626550906
79479,238437,0,238437,1001.6137919425964,0.0003481132297727646
79580,238740,0,238740,1002.9704160690308,0.0003471649216615669
79680,239040,0,239040,1004.4318861961365,0.00034686187678573165
79780,239340,0,239340,1005.6606621742249,0.0003463829263741389
79880,239640,0,239640,1006.9738161563873,0.0003459257909723785
79980,239940,0,239940,1008.1406750679016,0.0003455695394248755
80080,240240,0,240240,1009.4456970691681,0.0003450417939904828
80180,240540,0,240540,1010.9087340831757,0.00034408495257489324
80280,240840,0,240840,1012.1685791015625,0.00034300936719330286
80380,241140,0,241140,1013.3647191524506,0.0003427004899014929
80480,241440,0,241440,1014.6269490718842,0.0003419820672641981
80581,241743,0,241743,1015.8515660762787,0.0003409098086309755
80681,242043,0,242043,1017.7725791931152,0.00034062183892319344
80781,242343,0,242343,1019.4999680519104,0.0003404302248377472
80881,242643,0,242643,1020.9882230758667,0.0003401514856662899
80981,242943,0,242943,1022.465891122818,0.000339648174753989
81081,243243,0,243243,1023.7569489479065,0.00033941996153949585
81181,243543,0,243543,1025.1506659984589,0.000339086814402488
81281,243843,0,243843,1026.5533361434937,0.0003385779763570661
81381,244143,0,244143,1027.7833001613617,0.00033818281055672024
81481,244443,0,244443,1029.2949771881104,0.00033788533484052684
81582,244746,0,244746,1030.795704126358,0.0003375512395270128
81682,245046,0,245046,1032.1314401626587,0.00033622288819832604
81782,245346,0,245346,1033.3574678897858,0.00033465014652021965
81882,245646,0,245646,1034.591698884964,0.0003343743150409968
81982,245946,0,245946,1035.8603670597076,0.000334176831529614
82082,246246,0,246246,1037.5018792152405,0.00033387562209004926
82182,246546,0,246546,1038.8140170574188,0.00033327583281270965
82282,246846,0,246846,1040.0820128917694,0.0003329978561527485
82382,247146,0,247146,1041.446468114853,0.00033264140550767426
82482,247446,0,247446,1042.646409034729,0.0003322519306883843
82583,247749,0,247749,1044.0785138607025,0.0003318492786837376
82683,248049,0,248049,1045.7478892803192,0.0003315398743705227
82783,248349,0,248349,1046.9688420295715,0.00033128985119582386
82883,248649,0,248649,1048.2204420566559,0.0003307530008846778
82983,248949,0,248949,1049.7379751205444,0.00033037896102199835
83083,249249,0,249249,1051.143478155136,0.0003300735012342284
83183,249549,0,249549,1052.5967061519623,0.0003297931293158224
83283,249849,0,249849,1054.649274110794,0.00032951010493831686
83383,250149,0,250149,1056.098562002182,0.00032917624764774436
83483,250449,0,250449,1057.9252791404724,0.000328755104240709
83584,250752,0,250752,1059.3249552249908,0.00032777607618080906
83684,251052,0,251052,1060.706838130951,0.0003257761047070793
83784,251352,0,251352,1062.1765570640564,0.0003254817811371501
83884,251652,0,251652,1063.4085550308228,0.0003252100780699897
83984,251952,0,251952,1064.5531070232391,0.00032428678026692525
84084,252252,0,252252,1065.7218761444092,0.0003231416831751566
84184,252552,0,252552,1066.927011013031,0.00032290182466849756
84284,252852,0,252852,1068.1650612354279,0.0003226672705189777
84384,253152,0,253152,1069.4361250400543,0.0003223299611254034
84484,253452,0,253452,1070.7192521095276,0.0003219120071608304
84585,253755,0,253755,1072.0217349529266,0.00032115089266205265
84685,254055,0,254055,1074.1585030555725,0.0003209594861430343
84785,254355,0,254355,1076.3663301467896,0.00032053608728901793
84885,254655,0,254655,1077.564227104187,0.00032013940335683545
84985,254955,0,254955,1079.002515077591,0.00031987495238093664
85085,255255,0,255255,1080.3505091667175,0.00031961409605120884
85185,255555,0,255555,1081.5965740680695,0.00031933051400407205
85285,255855,0,255855,1082.8659720420837,0.00031903021371731504
85385,256155,0,256155,1084.0959060192108,0.00031865441431358586
85485,256455,0,256455,1085.278789281845,0.0003184161149761428
85586,256758,0,256758,1086.6199769973755,0.000318139387502692
85686,257058,0,257058,1087.9776740074158,0.00031781585155334476
85786,257358,0,257358,1089.777107000351,0.00031764210284560365
85886,257658,0,257658,1091.0829739570618,0.00031736625287325806
85986,257958,0,257958,1092.4066429138184,0.0003168893110947384
86086,258258,0,258258,1093.601511001587,0.0003158955909572499
86186,258558,0,258558,1094.9216890335083,0.0003153252185612974
86286,258858,0,258858,1096.205999135971,0.00031512773352363897
86386,259158,0,259158,1097.4252190589905,0.0003145567595576184
86486,259458,0,259458,1098.652713060379,0.0003143039295924938
86587,259761,0,259761,1099.8588271141052,0.0003139634192786742
86687,260061,0,260061,1100.9959480762482,0.0003136309144466823
86787,260361,0,260361,1102.2470149993896,0.00031335223246709693
86887,260661,0,260661,1103.5317871570587,0.0003130949545698649
86987,260961,0,260961,1104.7988941669464,0.0003124129102637962
87087,261261,0,261261,1106.015291929245,0.00031109813805775126
87187,261561,0,261561,1107.1420328617096,0.000310438876853793
87287,261861,0,261861,1108.3311650753021,0.0003099699768670068
87387,262161,0,262161,1109.5704340934753,0.00030932894413669736
87487,262461,0,262461,1110.7208971977234,0.0003080360524963414
87588,262764,0,262764,1111.901223897934,0.00030737947078492893
87688,263064,0,263064,1113.1059908866882,0.0003070945209911111
87788,263364,0,263364,1114.2854762077332,0.0003067121576765181
87888,263664,0,263664,1115.4725770950317,0.0003065073967358242
87988,263964,0,263964,1116.64719414711,0.00030601772852751247
88088,264264,0,264264,1117.8803040981293,0.0003056097866603009
88188,264564,0,264564,1119.057433128357,0.000305429562510674
88288,264864,0,264864,1120.205574274063,0.0003052109275263911
88388,265164,0,265164,1121.4052522182465,0.00030476419938246395
88488,265464,0,265464,1122.5595829486847,0.0003043758391850442
88589,265767,0,265767,1123.6852259635925,0.0003040685796488399
88689,266067,0,266067,1125.0057830810547,0.0003032809253853687
88789,266367,0,266367,1126.1730592250824,0.0003024063662564672
88889,266667,0,266667,1127.3286180496216,0.0003021589210895428
88989,266967,0,266967,1128.5882921218872,0.00030193237179398366
89089,267267,0,267267,1129.8247590065002,0.0003010347194880094
89189,267567,0,267567,1130.9648230075836,0.0003000329067674452
89289,267867,0,267867,1132.1738109588623,0.0002988639503051206
89389,268167,0,268167,1133.4813890457153,0.00029757641775162976
89489,268467,0,268467,1134.7474880218506,0.000295975582174794
89590,268770,0,268770,1135.9519202709198,0.00029436548990082454
89690,269070,0,269070,1137.2049720287323,0.0002930954106884687
89790,269370,0,269370,1138.3595910072327,0.0002926109418470654
89890,269670,0,269670,1139.7142641544342,0.0002920593090839834
89990,269970,0,269970,1141.076267004013,0.0002912975205495239
90090,270270,0,270270,1142.5016651153564,0.00029027091426612794
90190,270570,0,270570,1143.8823680877686,0.00028999724976842096
90290,270870,0,270870,1145.1891751289368,0.0002897192139375945
90390,271170,0,271170,1146.5089061260223,0.00028924203424352706
90490,271470,0,271470,1147.8621079921722,0.0002887272827438098
90591,271773,0,271773,1149.6140999794006,0.0002879498023615841
90691,272073,0,272073,1150.9418320655823,0.0002877023018439956
90791,272373,0,272373,1152.178601026535,0.0002873502840199174
90891,272673,0,272673,1153.351718902588,0.00028704411721687615
90991,272973,0,272973,1154.5859310626984,0.00028669915885673274
91091,273273,0,273273,1155.907613992691,0.0002864295782507335
91191,273573,0,273573,1157.053169965744,0.00028598930416887054
91291,273873,0,273873,1159.025318145752,0.000285472817865217
91391,274173,0,274173,1160.443144083023,0.0002851813251819474
91491,274473,0,274473,1161.772931098938,0.0002847282457293065
91592,274776,0,274776,1163.3703980445862,0.0002841431834195013
91692,275076,0,275076,1165.2892701625824,0.0002839330260436813
91792,275376,0,275376,1166.5507571697235,0.0002836994683356116
91892,275676,0,275676,1168.2139892578125,0.00028284003184951757
91992,275976,0,275976,1169.7034690380096,0.0002806318146225018
92092,276276,0,276276,1171.1308181285858,0.00027868171348989707
92192,276576,0,276576,1172.4443361759186,0.00027749845402537317
92292,276876,0,276876,1173.6920709609985,0.00027727501380593383
92392,277176,0,277176,1174.9630160331726,0.0002770610367514565
92492,277476,0,277476,1176.335398197174,0.0002767320739882955
92593,277779,0,277779,1177.7397520542145,0.0002762493917165333
92693,278079,0,278079,1179.031524181366,0.00027605688550258917
92793,278379,0,278379,1180.7677791118622,0.00027580122766529964
92893,278679,0,278679,1182.1475920677185,0.0002754753057292166
92993,278979,0,278979,1183.582150220871,0.00027512587540812677
93093,279279,0,279279,1185.0189189910889,0.0002747577732311563
93193,279579,0,279579,1186.2829520702362,0.0002745551932469773
93293,279879,0,279879,1187.8594481945038,0.00027436173964850134
93393,280179,0,280179,1189.9859981536865,0.0002740084018411443
93493,280479,0,280479,1191.5062851905823,0.0002736865871095069
93594,280782,0,280782,1192.7286050319672,0.0002734861407039395
93694,281082,0,281082,1194.0296819210052,0.00027331886059816005
93794,281382,0,281382,1195.2562580108643,0.0002731502502574717
93894,281682,0,281682,1196.578292131424,0.00027297649734718776
93994,281982,0,281982,1197.9180850982666,0.00027272476268723635
94094,282282,0,282282,1199.059730052948,0.0002722863238900686
94194,282582,0,282582,1200.2792329788208,0.00027175944170888214
94294,282882,0,282882,1201.5448861122131,0.0002714175709044705
94394,283182,0,283182,1202.7905631065369,0.00027119884568146783
94494,283482,0,283482,1203.9337768554688,0.0002709288677969388
94595,283785,0,283785,1205.145478963852,0.0002702022943620325
94695,284085,0,284085,1206.3169662952423,0.0002697030036424473
94795,284385,0,284385,1207.4901161193848,0.00026942285726331595
94895,284685,0,284685,1208.6915700435638,0.0002688729615798026
94995,284985,0,284985,1209.8869190216064,0.0002685451036907283
95095,285285,0,285285,1211.1463060379028,0.0002682681617024928
95195,285585,0,285585,1212.5168042182922,0.00026764917343044515
95295,285885,0,285885,1214.0104739665985,0.0002665456600956138
95395,286185,0,286185,1215.4577569961548,0.00026604631491745575
95495,286485,0,286485,1216.9031450748444,0.0002658289168207139
95596,286788,0,286788,1218.2902002334595,0.0002654188568500362
95696,287088,0,287088,1220.1334400177002,0.00026492891551649
95796,287388,0,287388,1221.5608069896698,0.00026471723321008767
95896,287688,0,287688,1222.8038671016693,0.00026180091970937536
95996,287988,0,287988,1224.09969997406,0.0002597445789562826
96096,288288,0,288288,1225.356994152069,0.0002589341259698407
96196,288588,0,288588,1226.7739081382751,0.00025852640023053114
96296,288888,0,288888,1228.0384030342102,0.0002580564155410985
96396,289188,0,289188,1229.3532531261444,0.0002571232037598842
96496,289488,0,289488,1230.5567581653595,0.00025681164011832306
96597,289791,0,289791,1231.8940780162811,0.0002565629772039285
96697,290091,0,290091,1233.0879430770874,0.0002560155173701239
96797,290391,0,290391,1234.3976180553436,0.0002557180388991759
96897,290691,0,290691,1235.6935200691223,0.00025546044552454455
96997,290991,0,290991,1236.924576997757,0.0002549577395916713
97097,291291,0,291291,1238.1293630599976,0.00025452498914714977
97197,291591,0,291591,1239.2784280776978,0.0002540331767307239
97297,291891,0,291891,1240.432224035263,0.00025379537206609036
97397,292191,0,292191,1241.6381719112396,0.0002535970259417424
97497,292491,0,292491,1243.0206871032715,0.00025296453534016944
97598,292794,0,292794,1244.2035970687866,0.00025272949399594895
97698,293094,0,293094,1245.3505311012268,0.0002525087845061461
97798,293394,0,293394,1246.5448100566864,0.00025237331172359417
97898,293694,0,293694,1247.8006720542908,0.00025220590594731524
97998,293994,0,293994,1249.0164322853088,0.0002518619483135389
98098,294294,0,294294,1250.3026020526886,0.0002515931964728533
98198,294594,0,294594,1251.5402262210846,0.00025139503313426477
98298,294894,0,294894,1252.7948710918427,0.00025123107640206646
98398,295194,0,295194,1254.0257320404053,0.0002506370224762924
98498,295494,0,295494,1255.1903822422028,0.000249491526346033
98599,295797,0,295797,1256.3606390953064,0.0002477186644189012
98699,296097,0,296097,1257.6960220336914,0.0002454797293666816
98799,296397,0,296397,1258.8365659713745,0.00024497832447304687
98899,296697,0,296697,1260.047520160675,0.0002447613227597163
98999,296997,0,296997,1261.2104818820953,0.0002445616949539183
99099,297297,0,297297,1262.4763650894165,0.0002442181961478204
99199,297597,0,297597,1263.5758032798767,0.00024378004627149299
99299,297897,0,297897,1264.7617771625519,0.00024359529896258767
99399,298197,0,298197,1265.9567830562592,0.00024330113640774314
99499,298497,0,298497,1267.1086032390594,0.00024294206740279475
99600,298800,0,298800,1268.443638086319,0.00024264776968781952
99700,299100,0,299100,1269.739690065384,0.00024229777104748664
99800,299400,0,299400,1270.9619920253754,0.00024202806828230674
99900,299700,0,299700,1272.230621099472,0.0002415872942918838
100000,300000,0,300000,1273.4924311637878,0.00024120510503400068


==> plot_data/quadratic_minimax_problem_n500_alpha0/flex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0020329952239990234,30.358099469249375
100,424,0,424,11.530822992324829,0.7211239886005693
200,904,0,904,22.382174968719482,0.40714633829939134
300,1404,0,1404,34.79979491233826,0.3624245498130248
400,1902,0,1902,48.25783395767212,0.3234305807147064
501,2407,0,2407,61.11792182922363,0.29927923547289564
601,2907,0,2907,85.75802087783813,0.2798141171444672
701,3407,0,3407,98.99608302116394,0.2632947441677823
801,3907,0,3907,112.55429983139038,0.24894925517918357
901,4407,0,4407,126.18071508407593,0.23628795092033392
1001,4907,0,4907,139.6558690071106,0.22497484237422974
1101,5407,0,5407,152.25598907470703,0.21476752442670155
1201,5907,0,5907,165.7279508113861,0.2054846363539787
1301,6407,0,6407,184.41180896759033,0.19698661111494115
1401,6907,0,6907,201.8121268749237,0.18916356405203077
1502,7412,0,7412,221.29149985313416,0.18185766975309853
1602,7912,0,7912,241.743145942688,0.17514117836096976
1702,8412,0,8412,254.947429895401,0.16887965154176085
1802,8912,0,8912,267.55008482933044,0.16302350106398145
1902,9412,0,9412,280.15908002853394,0.1575308461743764
2002,9906,0,9906,292.8066408634186,0.1498909696800842
2102,10406,0,10406,305.7974798679352,0.14511979342703413
2202,10906,0,10906,319.88458704948425,0.1406365536270806
2302,11406,0,11406,334.51855397224426,0.1363983502206184
2402,11906,0,11906,348.7635259628296,0.13238114794475966
2503,12411,0,12411,363.64821791648865,0.12852939777278136
2603,12911,0,12911,379.149533033371,0.12490383158500992
2703,13407,0,13407,392.99544882774353,0.11553399137809793
2803,13907,0,13907,406.1307227611542,0.11231346686490083
2903,14407,0,14407,419.2718060016632,0.10933628292944855
3003,14907,0,14907,434.93468499183655,0.10651303192284882
3103,15407,0,15407,448.0619008541107,0.10382200685747961
3203,15907,0,15907,461.18357396125793,0.10125140448760439
3303,16407,0,16407,479.00568985939026,0.09879265478836109
3403,16907,0,16907,492.33714485168457,0.09643871785544907
3504,17412,0,17412,509.0118637084961,0.09416140847986092
3604,17912,0,17912,521.8378748893738,0.09200032233161215
3704,18412,0,18412,535.0510878562927,0.08992748237389693
3804,18912,0,18912,552.0745508670807,0.08793835459711602
3904,19412,0,19412,568.6648321151733,0.08602875165783933
4004,19912,0,19912,585.7096610069275,0.08419478483088971
4104,20412,0,20412,598.5380339622498,0.0824328268805458
4204,20912,0,20912,613.5069599151611,0.08073948242407632
4304,21412,0,21412,626.9345738887787,0.07911156369042999
4404,21912,0,21912,641.1888289451599,0.07754607031317048
4505,22407,0,22407,659.2055780887604,0.07412162093332915
4605,22907,0,22907,672.944258928299,0.07266764686185315
4705,23407,0,23407,686.1172778606415,0.07129191334254018
4805,23907,0,23907,699.1751177310944,0.06997352237985814
4905,24407,0,24407,712.2094647884369,0.06870656535722068
5005,24907,0,24907,725.0786509513855,0.06748769686123084
5105,25407,0,25407,738.0261557102203,0.06631436994781609
5205,25907,0,25907,750.802943944931,0.06518438528819169
5305,26407,0,26407,763.7665297985077,0.0640957425747773
5405,26907,0,26907,777.0606007575989,0.06304658122831297
5506,27412,0,27412,793.9410650730133,0.06202522276507799
5606,27912,0,27912,810.2395877838135,0.06105022534018896
5706,28412,0,28412,826.6118190288544,0.06010972354705247
5806,28912,0,28912,842.4531509876251,0.05920222813705618
5906,29412,0,29412,859.3099689483643,0.05832632196249025
6006,29912,0,29912,873.7724928855896,0.0574806551447777
6106,30412,0,30412,887.4118149280548,0.056663940917151684
6206,30912,0,30912,901.9954099655151,0.05587495195963205
6306,31412,0,31412,914.8183000087738,0.0551125171130183
6406,31912,0,31912,928.5312740802765,0.05437551839647884
6507,32417,0,32417,942.1256458759308,0.05365588154699887
6607,32917,0,32917,954.4354367256165,0.05296682890984573
6707,33417,0,33417,966.618992805481,0.05230014171908473
6807,33917,0,33917,978.741593837738,0.051654889779197126
6907,34417,0,34417,990.6945848464966,0.05103018423515985
7007,34917,0,34917,1002.7270920276642,0.05042517565306127
7107,35417,0,35417,1015.2092890739441,0.04983905221077293
7207,35917,0,35917,1028.6408529281616,0.04927103798794479
7307,36417,0,36417,1045.7464368343353,0.04872039134625246
7407,36917,0,36917,1060.7387809753418,0.04818640339217861
7508,37422,0,37422,1076.133887052536,0.04766329493547635
7608,37922,0,37922,1093.0635027885437,0.0471607715793348
7708,38422,0,38422,1114.8128159046173,0.04667295638047154
7808,38922,0,38922,1135.1672189235687,0.04619925775612519
7908,39422,0,39422,1149.1382939815521,0.04573911020535582
8008,39922,0,39922,1162.4239869117737,0.04529197315535938
8108,40422,0,40422,1176.490732908249,0.04485732985844246
8208,40922,0,40922,1189.6200489997864,0.044434686336964735
8308,41422,0,41422,1202.6657400131226,0.044023570373814894
8408,41922,0,41922,1215.597286939621,0.04362353054621258
8509,42427,0,42427,1229.867672920227,0.04323029369210993
8609,42927,0,42927,1243.8667237758636,0.042851230758281296
8709,43427,0,43427,1257.5102939605713,0.04248200154872427
8809,43927,0,43927,1271.3605818748474,0.042122229124322834
8909,44427,0,44427,1284.8668088912964,0.04177155308608374
9009,44927,0,44927,1299.300086736679,0.04142962883171067
9109,45427,0,45427,1313.060154914856,0.04109612684404679
9209,45927,0,45927,1326.3377480506897,0.040770732010117626
9309,46427,0,46427,1338.2295548915863,0.04045314296956796
9409,46927,0,46927,1352.7918779850006,0.040143071491339014
9510,47432,0,47432,1367.3644816875458,0.03983724925067063
9610,47932,0,47932,1379.565703868866,0.03954146625473345
9710,48432,0,48432,1391.9209508895874,0.03925240660388256
9810,48932,0,48932,1403.9370110034943,0.03896982898442213
9910,49432,0,49432,1416.0391960144043,0.03869350247681848
10010,49932,0,49932,1428.6557099819183,0.03842320608021646
10110,50432,0,50432,1441.0178439617157,0.0381587282582497
10210,50932,0,50932,1453.5225479602814,0.03789986650528598
10310,51432,0,51432,1465.6704320907593,0.0376464269322772
10410,51932,0,51932,1477.6191189289093,0.03739822387140901
10511,52437,0,52437,1489.7092170715332,0.03715267301898622
10611,52937,0,52937,1501.7192778587341,0.0369144650422313
10711,53437,0,53437,1514.0669329166412,0.036680980616877995
10811,53937,0,53937,1526.2341759204865,0.036452063422408636
10911,54437,0,54437,1538.2167429924011,0.03622756363542651
11011,54937,0,54937,1550.234736919403,0.036007337631807586
11111,55437,0,55437,1562.2655770778656,0.03579124770272562
11211,55937,0,55937,1574.1058077812195,0.03557916178394309
11311,56437,0,56437,1586.0512640476227,0.03537095319778201
11411,56937,0,56937,1597.9737689495087,0.03516650040720988
11512,57442,0,57442,1615.3587369918823,0.03496369664043619
11612,57942,0,57942,1629.4004759788513,0.03476644495400363
11712,58442,0,58442,1642.5760068893433,0.034572611954376276
11812,58942,0,58942,1655.720473766327,0.034382094473384965
11912,59442,0,59442,1670.0420188903809,0.03419479341549434
12012,59942,0,59942,1682.9648687839508,0.034010613573976216
12112,60442,0,60442,1695.883455991745,0.03382946345581324
12212,60942,0,60942,1708.6967058181763,0.033651255114921674
12312,61442,0,61442,1721.6466648578644,0.03347590399330601
12412,61942,0,61942,1734.8478050231934,0.03330332876976875
12513,62447,0,62447,1748.1637229919434,0.03313176580641659
12613,62947,0,62947,1761.2309248447418,0.032964536502534676
12713,63447,0,63447,1777.8363211154938,0.03279985643632003
12813,63947,0,63947,1793.2251427173615,0.032637655886183815
12913,64447,0,64447,1806.698473930359,0.03247786771108069
13013,64947,0,64947,1819.7779068946838,0.03232042723762245
13113,65447,0,65447,1832.9393289089203,0.03216527215255024
13213,65947,0,65947,1846.071567773819,0.03201234240030491
13313,66447,0,66447,1860.9739437103271,0.03186158008544811
13413,66947,0,66947,1877.415676832199,0.031712929379698634
13514,67452,0,67452,1890.791702747345,0.03156488071824445
13614,67952,0,67952,1903.9150910377502,0.031420313377671524
13714,68452,0,68452,1926.4961490631104,0.031277701206731325
13814,68952,0,68952,1942.3393449783325,0.031136995817789413
13914,69452,0,69452,1959.0758409500122,0.030998150486561515
14014,69952,0,69952,1974.363665819168,0.030861120082511715
14114,70452,0,70452,1988.509057044983,0.030725861002498165
14214,70952,0,70952,2001.7513778209686,0.030592331107508468
14314,71452,0,71452,2016.0631008148193,0.030460489662333293
14414,71952,0,71952,2033.0121738910675,0.03033029727803295
14515,72457,0,72457,2051.217803001404,0.03020043805249401
14615,72957,0,72957,2068.4985258579254,0.030073446295327814
14715,73457,0,73457,2081.939071893692,0.029947992622735602
14815,73957,0,73957,2095.5886929035187,0.02982404251793523
14915,74457,0,74457,2109.1607768535614,0.029701562559652565
15015,74957,0,74957,2123.9330780506134,0.029580520378722924
15115,75457,0,75457,2141.0875968933105,0.029460884616658703
15215,75957,0,75957,2158.284019947052,0.02934262488608667
15315,76457,0,76457,2172.0095648765564,0.029225711732965277
15415,76957,0,76957,2186.205173969269,0.02911011660049324
15516,77462,0,77462,2199.3033339977264,0.028994675171147264
15616,77962,0,77962,2215.05273604393,0.028881646329353566
15716,78462,0,78462,2227.8991067409515,0.028769854627310715
15816,78962,0,78962,2240.834687948227,0.028659274774876783
15916,79462,0,79462,2253.863869905472,0.02854988222107437
16016,79962,0,79962,2267.1133980751038,0.028441653126581905
16116,80462,0,80462,2280.759913921356,0.028334564337422295
16216,80962,0,80962,2296.527907848358,0.02822859335979148
16316,81462,0,81462,2313.0370268821716,0.02812371833597236
16416,81962,0,81962,2327.2373938560486,0.02801991802128283
16517,82467,0,82467,2342.548015832901,0.027916149553975544
16617,82967,0,82967,2358.561978816986,0.02781444750641096
16717,83467,0,83467,2374.3455760478973,0.02771375970348491
16817,83967,0,83967,2392.520315885544,0.027614067146357803
16917,84467,0,84467,2407.9821660518646,0.027515351347660956
17017,84967,0,84967,2421.888589859009,0.02741759431370801
17117,85467,0,85467,2435.336438894272,0.02732077852744474
17217,85967,0,85967,2448.6152000427246,0.027224886932101754
17317,86467,0,86467,2463.8463571071625,0.027129902915518755
17417,86967,0,86967,2480.4564638137817,0.027035810295108976
17518,87472,0,87472,2498.2942447662354,0.026941665503121628
17618,87972,0,87972,2515.1728279590607,0.026849317300399776
17718,88472,0,88472,2529.5761048793793,0.026757814234302894
17818,88972,0,88972,2543.8529908657074,0.02666714170567395
17918,89472,0,89472,2559.0662229061127,0.026577285478252936
18018,89972,0,89972,2575.4600887298584,0.02648823166691711
18118,90472,0,90472,2591.9184987545013,0.02639996672638456
18218,90972,0,90972,2608.3714809417725,0.026312477440357824
18318,91472,0,91472,2622.5750579833984,0.026225750911090542
18418,91972,0,91972,2636.3040828704834,0.026139774549356072
18519,92477,0,92477,2649.4175939559937,0.026053687365394207
18619,92977,0,92977,2664.025887966156,0.025969181956384153
18719,93477,0,93477,2678.234997987747,0.025885390587905288
18819,93977,0,93977,2697.1511340141296,0.025802301814638235
18919,94477,0,94477,2715.4963080883026,0.025719904455001306
19019,94977,0,94977,2729.0815908908844,0.02563818758319546
19119,95477,0,95477,2742.195200920105,0.025557140521545334
19219,95977,0,95977,2755.179090976715,0.025476752833121646
19319,96477,0,96477,2768.1082389354706,0.02539701431463412
19419,96977,0,96977,2781.5839698314667,0.025317914989583464
19520,97482,0,97482,2794.8082020282745,0.025238663548976383
19620,97982,0,97982,2808.130770921707,0.025160819707165254
19720,98482,0,98482,2823.2386009693146,0.025083586332892437
19820,98982,0,98982,2838.657737016678,0.025006954295131875
19920,99482,0,99482,2852.1092739105225,0.02493091465886757
20020,99982,0,99982,2865.699343919754,0.02485545867958763
20120,100482,0,100482,2881.40762591362,0.02478057779796985
20220,100982,0,100982,2895.5104768276215,0.024706263634751913
20320,101482,0,101482,2909.3388438224792,0.024632507985778672
20420,101982,0,101982,2923.0371339321136,0.024559302817217885
20521,102487,0,102487,2937.539256811142,0.024485916349359912
20621,102987,0,102987,2951.006284713745,0.024413794009141166
20721,103487,0,103487,2964.9109346866608,0.024342198949622917
20821,103987,0,103987,2979.3916108608246,0.024271123775095913
20921,104487,0,104487,2994.557282924652,0.024200561238531683
21021,104987,0,104987,3009.3928248882294,0.024130504237684668
21121,105487,0,105487,3022.657185792923,0.02406094581132183
21221,105987,0,105987,3035.9876239299774,0.023991879135575656
21321,106487,0,106487,3049.6288447380066,0.023923297520414007
21421,106987,0,106987,3062.98609995842,0.023855194406224477
21522,107492,0,107492,3077.362186908722,0.023786889412548983
21622,107992,0,107992,3091.7328329086304,0.023719728752867975
21722,108492,0,108492,3105.5426609516144,0.023653027604014453
21822,108992,0,108992,3119.379554748535,0.02358677989717937
21922,109492,0,109492,3133.3999869823456,0.023520979678421098
22022,109992,0,109992,3147.999525785446,0.023455621105846466
22122,110492,0,110492,3161.8533248901367,0.023390698446878175
22222,110992,0,110992,3175.673744916916,0.023326206075605784
22322,111492,0,111492,3188.8049507141113,0.02326213847021747
22422,111992,0,111992,3203.571299791336,0.023198490210508734
22523,112497,0,112497,3217.2878918647766,0.02313462570618456
22623,112997,0,112997,3231.0257470607758,0.02307180433358704
22723,113497,0,113497,3244.6159019470215,0.02300938658106969
22823,113997,0,113997,3258.044862985611,0.022947367412315362
22923,114497,0,114497,3271.4005880355835,0.022885741881207046
23023,114997,0,114997,3285.445354938507,0.02282450512974702
23123,115497,0,115497,3298.755598783493,0.022763652386037187
23223,115997,0,115997,3312.2299988269806,0.022703178962316377
23323,116497,0,116497,3325.908143758774,0.022643080253054206
23423,116997,0,116997,3339.0548827648163,0.02258335173309895
23524,117502,0,117502,3352.250956773758,0.02252339716025753
23624,118002,0,118002,3365.502891778946,0.0224643993479438
23724,118502,0,118502,3378.5407979488373,0.022405758571431213
23824,119002,0,119002,3393.227765083313,0.02234747061030448
23924,119502,0,119502,3406.7748880386353,0.022289531315998343
24024,120002,0,120002,3420.1193149089813,0.022231936610233788
24124,120502,0,120502,3433.1112859249115,0.02217468248349646
24224,121002,0,121002,3446.3205959796906,0.022117764993556097
24324,121502,0,121502,3460.9685950279236,0.022061180264026363
24424,122002,0,122002,3480.8348059654236,0.022004924482962318
24525,122507,0,122507,3498.894775867462,0.021948436225412243
24625,123007,0,123007,3514.59432888031,0.021892830353131793
24725,123507,0,123507,3530.4318029880524,0.021837542330694057
24825,124007,0,124007,3547.2124388217926,0.021782568591209733
24925,124507,0,124507,3563.7903077602386,0.02172790562574264
25025,125007,0,125007,3580.576714038849,0.02167354998211346
25125,125507,0,125507,3596.5768909454346,0.02161949826373493
25225,126007,0,126007,3612.113711833954,0.021565747128475997
25325,126507,0,126507,3641.0656049251556,0.021512293287554933
25425,127007,0,127007,3657.1694588661194,0.02145913350446069
25526,127512,0,127512,3672.471748828888,0.021405737363052093
25626,128012,0,128012,3686.926495075226,0.021353159051635536
25726,128512,0,128512,3701.5981509685516,0.02130086536113156
25826,129012,0,129012,3715.98739695549,0.021248853254326214
25926,129512,0,129512,3731.783205986023,0.02119711974126094
26026,130012,0,130012,3763.9249007701874,0.02114566187830369
26126,130512,0,130512,3777.7061519622803,0.021094476767243103
26226,131012,0,131012,3791.025691986084,0.021043561554404063
26326,131512,0,131512,3804.8346440792084,0.020992913429784776
26426,132012,0,132012,3824.6084909439087,0.020942529626214106
26527,132517,0,132517,3844.4832859039307,0.02089190750839625
26627,133017,0,133017,3863.2962958812714,0.020842046788341756
26727,133517,0,133517,3877.8396260738373,0.020792442310443675
26827,134017,0,134017,3891.7798190116882,0.020743091471211724
26927,134517,0,134517,3912.4444386959076,0.020693991706054377
27027,135017,0,135017,3928.9311068058014,0.020645140488547858
27127,135517,0,135517,3942.8960959911346,0.020596535329722145
27227,136017,0,136017,3955.988848924637,0.020548173777362965
27327,136517,0,136517,3969.3295669555664,0.0205000534153299
27427,137017,0,137017,3982.509911775589,0.02045217186288995
27528,137522,0,137522,4002.5028450489044,0.020404051509468234
27628,138022,0,138022,4019.693542957306,0.02035664290235741
27728,138522,0,138522,4035.799248933792,0.02030946614602425
27828,139022,0,139022,4049.135593891144,0.020262518995318703
27928,139522,0,139522,4062.397782802582,0.020215799237376042
28028,140022,0,140022,4076.047504901886,0.020169304691034666
28128,140522,0,140522,4090.8753077983856,0.020123033206266266
28228,141022,0,141022,4105.253634929657,0.02007698266361863
28328,141522,0,141522,4118.593531847,0.02003115097367041
28428,142022,0,142022,4132.012501955032,0.01998553607649742
28529,142527,0,142527,4146.797644853592,0.01993968301754575
28629,143027,0,143027,4159.864371061325,0.019894497759117436
28729,143527,0,143527,4173.096580982208,0.019849523265905597
28829,144027,0,144027,4192.606646060944,0.01980475759113729
28929,144527,0,144527,4208.911221981049,0.01976019881503058
29029,145027,0,145027,4223.244927883148,0.019715845044325317
29129,145527,0,145527,4237.85560297966,0.019671694411823874
29229,146027,0,146027,4252.322020769119,0.019627745075941727
29329,146527,0,146527,4267.300783872604,0.019583995220266548
29429,147027,0,147027,4281.34526181221,0.019540443053127403
29530,147532,0,147532,4295.324011802673,0.019496654228195475
29630,148032,0,148032,4311.269765853882,0.019453494093028642
29730,148532,0,148532,4326.035781860352,0.019410526398567277
29830,149032,0,149032,4339.166349887848,0.01936774944819416
29930,149532,0,149532,4355.426744937897,0.019325161568001153
30030,150032,0,150032,4368.682328939438,0.0192827611064077
30130,150532,0,150532,4383.8657059669495,0.019240546433787326
30230,151032,0,151032,4397.069748878479,0.019198515942101216
30330,151532,0,151532,4410.050049781799,0.01915666804453937
30430,152032,0,152032,4423.111400842667,0.01911500117516862
30531,152537,0,152537,4436.278606891632,0.01907309981593275
30631,153037,0,153037,4456.402772903442,0.019031792158875335
30731,153537,0,153537,4471.444902896881,0.01899066093910085
30831,154037,0,154037,4488.370275735855,0.01894970467099488
30931,154537,0,154537,4504.540289878845,0.01890892188815806
31031,155037,0,155037,4519.899147987366,0.018868311143093695
31131,155537,0,155537,4535.248259782791,0.01882787100690095
31231,156037,0,156037,4550.9323189258575,0.018787600068974442
31331,156537,0,156537,4569.61999797821,0.018747496936709015
31431,157037,0,157037,4584.237385034561,0.018707560235210693
31532,157542,0,157542,4599.297220945358,0.018667391719801824
31632,158042,0,158042,4613.85847401619,0.018627785455204972
31732,158542,0,158542,4628.2091019153595,0.01858834158699828
31832,159042,0,159042,4646.012814760208,0.018549058808511803
31932,159542,0,159542,4662.45658493042,0.0185099358294176
32032,160042,0,160042,4679.039926767349,0.0184709713754715
32132,160542,0,160542,4692.881323099136,0.018432164188259957
32232,161042,0,161042,4706.196378946304,0.01839351302495138
32332,161542,0,161542,4719.370559930801,0.018355016658052243
32432,162042,0,162042,4732.771465063095,0.018316673875167538
32533,162547,0,162547,4746.5471959114075,0.018278102340338775
32633,163047,0,163047,4759.842113018036,0.01824006465363167
32733,163547,0,163547,4777.969171047211,0.018202176990402413
32833,164047,0,164047,4795.4258460998535,0.01816443819648226
32933,164547,0,164547,4814.262102842331,0.018126847131665447
33033,165047,0,165047,4832.705144882202,0.018089402669494978
33133,165547,0,165547,4847.444257736206,0.018052103697051465
33233,166047,0,166047,4860.538408994675,0.018014949114746843
33333,166547,0,166547,4873.884225130081,0.017977937836121154
33433,167047,0,167047,4887.096767902374,0.01794106878764295
33534,167552,0,167552,4900.351341724396,0.017903974339070337
33634,168052,0,168052,4913.354231834412,0.017867387976990452
33734,168552,0,168552,4926.283223867416,0.017830940689796432
33834,169052,0,169052,4940.268539905548,0.017794631453867293
33934,169552,0,169552,4953.855808019638,0.017758459257563333
34034,170052,0,170052,4967.848495960236,0.01772242310104717
34134,170552,0,170552,4982.223167896271,0.017686521996107273
34234,171052,0,171052,4995.872387886047,0.017650754965985373
34334,171552,0,171552,5009.0225076675415,0.017615121045206236
34434,172052,0,172052,5022.987432956696,0.01757961927941072
34535,172557,0,172557,5036.348809957504,0.01754389567910357
34635,173057,0,173057,5051.768779039383,0.01750865670196066
34735,173557,0,173557,5065.557888031006,0.01747354707262698
34835,174057,0,174057,5079.538151025772,0.017438565879698543
34935,174557,0,174557,5092.561466932297,0.017403712222093276
35035,175057,0,175057,5106.118617773056,0.017368985208900296
35135,175557,0,175557,5119.45906996727,0.01733438395923207
35235,176057,0,176057,5132.653561830521,0.01729990760207896
35335,176557,0,176557,5148.04207277298,0.017265555276166467
35435,177057,0,177057,5162.374044895172,0.01723132612981449
35536,177562,0,177562,5177.928067922592,0.017196878867686657
35636,178062,0,178062,5194.768429756165,0.017162894773974095
35736,178562,0,178562,5209.9944977760315,0.01712903135278741
35836,179062,0,179062,5225.215190887451,0.017095287789555744
35936,179562,0,179562,5238.336013793945,0.017061663278633687
36036,180062,0,180062,5251.6657338142395,0.01702815702317388
36136,180562,0,180562,5265.9399428367615,0.016994768235002625
36236,181062,0,181062,5284.2644629478455,0.016961496134496833
36336,181562,0,181562,5299.245818853378,0.016928339950463292
36436,182062,0,182062,5312.542953014374,0.016895298920020185
36537,182567,0,182567,5326.563638687134,0.016862043597346197
36637,183067,0,183067,5339.495131969452,0.016829231750880573
36737,183567,0,183567,5352.5287029743195,0.01679653281072208
36837,184067,0,184067,5366.93318104744,0.016763946046162676
36937,184567,0,184567,5381.473133802414,0.016731470734239515
37037,185067,0,185067,5394.607323884964,0.01669910615962714
37137,185567,0,185567,5407.707150936127,0.016666851614531842
37237,186067,0,186067,5421.348628997803,0.01663470639858739
37337,186567,0,186567,5434.490186929703,0.016602669818753087
37437,187067,0,187067,5447.700494766235,0.016570741189212392
37538,187572,0,187572,5460.95339179039,0.01653860215713823
37638,188072,0,188072,5473.7521867752075,0.016506888461770806
37738,188572,0,188572,5487.338315963745,0.01647528069499903
37838,189072,0,189072,5501.364946842194,0.016443778198997023
37938,189572,0,189572,5514.500148057938,0.016412380322682447
38038,190072,0,190072,5527.543098926544,0.016381086421625245
38138,190572,0,190572,5541.824126005173,0.01634989585795756
38238,191072,0,191072,5555.6445298194885,0.016318808000285154
38338,191572,0,191572,5570.4866898059845,0.016287822223600232
38438,192072,0,192072,5585.365421772003,0.016256937909195864
38539,192577,0,192577,5598.920983791351,0.016225847117169866
38639,193077,0,193077,5613.690835952759,0.01619516489538033
38739,193577,0,193577,5629.315346956253,0.016164582310744288
38839,194077,0,194077,5644.550004959106,0.01613409876898572
38939,194577,0,194577,5660.0046479702,0.01610371368171962
39039,195077,0,195077,5674.547621965408,0.016073426466373834
39139,195577,0,195577,5688.5592448711395,0.01604323654611205
39239,196077,0,196077,5703.5236558914185,0.01601314334975852
39339,196577,0,196577,5717.834055900574,0.015983146311723512
39439,197077,0,197077,5731.921963691711,0.015953244871929933
39540,197582,0,197582,5750.148716688156,0.015923140889886618
39640,198082,0,198082,5770.076623916626,0.01589342993022341
39740,198582,0,198582,5782.537007808685,0.015863812915517462
39840,199082,0,199082,5798.9937908649445,0.015834289307083964
39940,199582,0,199582,5814.733668804169,0.015804858571400248
40040,200082,0,200082,5826.63295006752,0.015775520180039016
40140,200582,0,200582,5837.680618047714,0.015746273609602627
40240,201082,0,201082,5848.406774044037,0.015717118341658398
40340,201582,0,201582,5860.883694887161,0.01568805386267456
40440,202082,0,202082,5871.830550670624,0.015659079663957663
40541,202587,0,202587,5980.4942400455475,0.015629906849044677
40641,203087,0,203087,6015.667729854584,0.015601112594092522
40741,203587,0,203587,6114.309729814529,0.01557240711682054
40841,204087,0,204087,8462.870710134506,0.015543789927324686
40941,204587,0,204587,8478.548333883286,0.015515260540238501
41041,205087,0,205087,8490.662370920181,0.015486818474675602
41141,205587,0,205587,8503.30750989914,0.015458463254173419
41241,206087,0,206087,8514.521641016006,0.015430194406637503
41341,206587,0,206587,8523.777676820755,0.015402011464286505
41441,207087,0,207087,8536.65109205246,0.015373913963598523
41542,207592,0,207592,8547.320729970932,0.015345621747691426
41642,208092,0,208092,8556.726190805435,0.015317694599522324
41742,208592,0,208592,8566.654465675354,0.01528985152298752
41842,209092,0,209092,8576.300031900406,0.01526209207111819
41942,209592,0,209592,8589.799907922745,0.015234415800945773
42042,210092,0,210092,8600.66377401352,0.015206822273453048
42142,210592,0,210592,8611.90098786354,0.01517931105352502
42242,211092,0,211092,8621.686147928238,0.015151881709901453
42342,211592,0,211592,8632.926278829575,0.015124533815129113
42442,212092,0,212092,8643.166986942291,0.015097266945515624
42543,212597,0,212597,8653.303467035294,0.015069809224083524
42643,213097,0,213097,8663.546886920929,0.015042703948323055
42743,213597,0,213597,8673.581441879272,0.015015678444644109
42843,214097,0,214097,8684.581675052643,0.014988732303980259
42943,214597,0,214597,8695.264791727066,0.014961865120802649
43043,215097,0,215097,8706.205473899841,0.014935076493077156
43143,215597,0,215597,8716.964755058289,0.014908366022222253
43243,216097,0,216097,8727.35228395462,0.014881733313067844
43343,216597,0,216597,8737.118810892105,0.014855177973814119
43443,217097,0,217097,8748.437743902206,0.014828699615991578
43544,217602,0,217602,8758.989706993103,0.014802034222321552
43644,218102,0,218102,8768.638134002686,0.014775709435300896
43744,218602,0,218602,8778.854786872864,0.014749460480118768
43844,219102,0,219102,8790.55037689209,0.0147232869812667
43944,219602,0,219602,8802.799507856369,0.014697188566373151
44044,220102,0,220102,8812.342067956924,0.014671164866166667
44144,220602,0,220602,8821.702325105667,0.014645215514439392
44244,221102,0,221102,8831.326150894165,0.014619340148011173
44344,221602,0,221602,8840.806788921356,0.01459353840669427
44444,222102,0,222102,8850.518721103668,0.014567809933258246
44545,222607,0,222607,8860.03893995285,0.014541898184819248
44645,223107,0,223107,8869.607310771942,0.01451631591096859
44745,223607,0,223607,8879.940785884857,0.014490805847239295
44845,224107,0,224107,8890.661899089813,0.01446536764791936
44945,224607,0,224607,8900.345633745193,0.014440000970086792
45045,225107,0,225107,8910.384489059448,0.014414705473577092
45145,225607,0,225607,8920.296431779861,0.014389480820952032
45245,226107,0,226107,8930.53647685051,0.014364326677468316
45345,226607,0,226607,8940.612289905548,0.014339242711046633
45445,227107,0,227107,8951.079374790192,0.014314228592241771
45546,227612,0,227612,8961.427661895752,0.014289034898212531
45646,228112,0,228112,8971.977705001831,0.01426416018702744
45746,228612,0,228612,8982.57979297638,0.014239354347424453
45846,229112,0,229112,8991.973784923553,0.014214617060223608
45946,229612,0,229612,9001.40749502182,0.014189948008732791
46046,230112,0,230112,9010.779054880142,0.014165346878720174
46146,230612,0,230612,9020.4052298069,0.014140813358386344
46246,231112,0,231112,9029.789062976837,0.014116347138337447
46346,231612,0,231612,9038.98078083992,0.014091947911558225
46446,232112,0,232112,9049.335260868073,0.014067615373385564
46547,232617,0,232617,9063.075752973557,0.01404310689419705
46647,233117,0,233117,9076.069846868515,0.014018907487881985
46747,233617,0,233617,9085.790934801102,0.013994773867072288
46847,234117,0,234117,9096.873322963715,0.013970705736278823
46947,234617,0,234617,9107.707082986832,0.013946702802237558
47047,235117,0,235117,9118.63350391388,0.013922764773885177
47147,235617,0,235617,9128.700438022614,0.013898891362334923
47247,236117,0,236117,9139.862745761871,0.013875082280853107
47347,236617,0,236617,9150.109851837158,0.013851337244835636
47447,237117,0,237117,9159.630943059921,0.013827655971784755
47548,237622,0,237622,9169.623924970627,0.013803802323024887
47648,238122,0,238122,9179.314591884613,0.013780248367369756
47748,238622,0,238622,9189.516897678375,0.013756757336847912
47848,239122,0,239122,9199.453819990158,0.01373332895718288
47948,239622,0,239622,9209.531202793121,0.013709962956093497
48048,240122,0,240122,9219.181861877441,0.013686659063272712
48148,240622,0,240622,9228.894155979156,0.013663417010366425
48248,241122,0,241122,9238.673070907593,0.01364023653095287
48348,241622,0,241622,9248.462516069412,0.013617117360522103
48448,242122,0,242122,9259.434008836746,0.013594059236455555
48549,242627,0,242627,9270.479694843292,0.013570832230711864
48649,243127,0,243127,9281.913579702377,0.013547896022951412
48749,243627,0,243627,9293.315866947174,0.013525020082289785
48849,244127,0,244127,9305.835292816162,0.01350220415349594
48949,244627,0,244627,9315.83553481102,0.013479447983133096
49049,245127,0,245127,9327.18855881691,0.013456751319540033
49149,245627,0,245627,9340.198323965073,0.013434113912812476
49249,246127,0,246127,9351.889665842056,0.013411535514785296
49349,246627,0,246627,9363.710286855698,0.013389015879013984
49449,247127,0,247127,9375.097569704056,0.013366554760757455
49550,247632,0,247632,9386.244505882263,0.013343928181989996
49650,248132,0,248132,9397.081467866898,0.013321583950381998
49750,248632,0,248632,9409.173973083496,0.013299297509721149
49850,249132,0,249132,9419.769766807556,0.013277068621922374
49950,249632,0,249632,9430.282648801804,0.013254897050518232
50050,250132,0,250132,9441.471932888031,0.013232782560642654
50150,250632,0,250632,9452.255786895752,0.013210724919014412
50250,251132,0,251132,9463.111022949219,0.013188723893921499
50350,251632,0,251632,9473.654136896133,0.013166779255205102
50450,252132,0,252132,9484.40483379364,0.013144890774244073
50551,252637,0,252637,9495.40102982521,0.013122840180121564
50651,253137,0,253137,9506.44905090332,0.013101063890797796
50751,253637,0,253637,9517.493181943893,0.013079343080205072
50851,254137,0,254137,9527.247332811356,0.013057677525735313
50951,254637,0,254637,9536.703794956207,0.01303606700624295
51051,255137,0,255137,9546.241921901703,0.013014511302030145
51151,255637,0,255637,9555.758731126785,0.0129930101948329
51251,256137,0,256137,9565.529066085815,0.012971563467806608
51351,256637,0,256637,9574.995750904083,0.012950170905512329
51451,257137,0,257137,9584.98644208908,0.012928832293903073
51552,257642,0,257642,9594.834426879883,0.012907334842234943
51652,258142,0,258142,9604.41866183281,0.012886104029558693
51752,258642,0,258642,9614.154953956604,0.012864926531549642
51852,259142,0,259142,9623.658471822739,0.012843802139607324
51952,259642,0,259642,9633.586021900177,0.012822730646456703
52052,260142,0,260142,9645.739177942276,0.012801711846135494
52152,260642,0,260642,9656.986498832703,0.012780745533981574
52252,261142,0,261142,9667.616150856018,0.01275983150662033
52352,261642,0,261642,9678.139098882675,0.012738969561952617
52452,262142,0,262142,9688.14860701561,0.012718159499142416
52553,262647,0,262647,9698.389791965485,0.012697193795122888
52653,263147,0,263147,9708.687941789627,0.012676487412354482
52753,263647,0,263647,9718.845253944397,0.012655832314430389
52853,264147,0,264147,9728.714332818985,0.012635228305461002
52953,264647,0,264647,9740.06717801094,0.012614675190761109
53053,265147,0,265147,9749.807730913162,0.012594172776838702
53153,265647,0,265647,9759.459573030472,0.012573720871383866
53253,266147,0,266147,9769.20603299141,0.012553319283257768
53353,266647,0,266647,9778.770887851715,0.012532967822481577
53453,267147,0,267147,9788.293083906174,0.012512666300225964
53554,267652,0,267652,9798.461561918259,0.0124922122616956
53654,268152,0,268152,9809.273385047913,0.012472010549241996
53754,268652,0,268652,9819.720811128616,0.012451858213762679
53854,269152,0,269152,9829.896369934082,0.012431755070931843
53954,269652,0,269652,9841.372262954712,0.012411700937521041
54054,270152,0,270152,9851.040782928467,0.012391695631389314
54154,270652,0,270652,9861.472233057022,0.012371738971472954
54254,271152,0,271152,9871.528511047363,0.012351830777776155
54354,271652,0,271652,9881.639705896378,0.012331970871361097
54454,272152,0,272152,9891.533362865448,0.012312159074338453
54555,272657,0,272657,9902.298974990845,0.012292197812676754
54655,273157,0,273157,9912.802681922913,0.012272482181600725
54755,273657,0,273657,9922.16532588005,0.012252814130703515
54855,274157,0,274157,9931.523387908936,0.012233193486206616
54955,274657,0,274657,9941.04154586792,0.01221362007533396
55055,275157,0,275157,9950.810774087906,0.012194093726302781
55155,275657,0,275657,9961.264544963837,0.012174614268315105
55255,276157,0,276157,9971.24548983574,0.012155181531548763
55355,276657,0,276657,9981.108448028564,0.012135795347149092
55455,277157,0,277157,9990.698747873306,0.012116455547220285
55556,277662,0,277662,10000.510905742645,0.012096969261828967
55656,278162,0,278162,10010.250191926956,0.012077722190628097
55756,278662,0,278662,10020.198305130005,0.012058521004234522
55856,279162,0,279162,10029.852886676788,0.012039365538514214
55956,279662,0,279662,10040.266149997711,0.012020255630250977
56056,280162,0,280162,10049.796983718872,0.012001191117138554
56156,280662,0,280662,10059.662708997726,0.011982171837772702
56256,281162,0,281162,10069.092726707458,0.011963197631643505
56356,281662,0,281662,10078.742745876312,0.011944268339127729
56456,282162,0,282162,10088.130006790161,0.011925383801481315
56557,282667,0,282667,10097.623077869415,0.011906355686108048
56657,283167,0,283167,10106.969592809677,0.011887560629056925
56757,283667,0,283667,10117.104251861572,0.011868809854285914
56857,284167,0,284167,10128.098474025726,0.011850103206501834
56957,284667,0,284667,10138.67577290535,0.011831440531254036
57057,285167,0,285167,10151.567501783371,0.011812821674927346
57157,285667,0,285667,10162.390696048737,0.011794246484734911
57257,286167,0,286167,10173.01578593254,0.011775714808711491
57357,286667,0,286667,10184.410044908524,0.011757226495706576
57457,287167,0,287167,10194.92893910408,0.011738781395377575
57558,287672,0,287672,10205.336720943451,0.011720195554776075
57658,288172,0,288172,10216.433094978333,0.011701836860364911
57758,288672,0,288672,10226.771605968475,0.011683520930907548
57858,289172,0,289172,10237.523194789886,0.011665247619234901
57958,289672,0,289672,10248.265272855759,0.011647016778953086
58058,290172,0,290172,10257.995198965073,0.011628828264437282
58158,290672,0,290672,10267.64555978775,0.011610681930825262
58258,291172,0,291172,10277.806315660477,0.011592577634011208
58358,291672,0,291672,10289.835191726685,0.011574515230639765
58458,292172,0,292172,10300.367659807205,0.011556494578099982
58559,292677,0,292677,10311.139449834824,0.011538335953730394
58659,293177,0,293177,10320.948433876038,0.011520398791936125
58759,293677,0,293677,10330.873176813126,0.011502502956146488
58859,294177,0,294177,10341.18550491333,0.011484648306675909
58959,294677,0,294677,10351.21304678917,0.011466834704553803
59059,295177,0,295177,10361.330662965775,0.011449062011518962
59159,295677,0,295677,10371.81419301033,0.011431330090014059
59259,296177,0,296177,10382.624109745026,0.011413638803179929
59359,296677,0,296677,10393.03354382515,0.011395988014850231
59459,297177,0,297177,10403.236515760422,0.011378377589545999
59560,297682,0,297682,10414.537937879562,0.011360631893197696
59660,298182,0,298182,10424.552181959152,0.011343102190496137
59760,298682,0,298682,10434.73710489273,0.011325612447122808
59860,299182,0,299182,10444.900592803955,0.01130816253030177
59960,299682,0,299682,10456.019409894943,0.011290752307918168
60060,300182,0,300182,10465.937663078308,0.011273381648513173
60160,300682,0,300682,10475.393593788147,0.011256050421278814
60260,301182,0,301182,10485.239919900894,0.011238758496053363
60360,301682,0,301682,10495.174738883972,0.011221505743315869
60460,302182,0,302182,10505.711631774902,0.011204292034181855
60561,302687,0,302687,10515.210540771484,0.011186945688550458
60661,303187,0,303187,10524.639120817184,0.011169810069725263
60761,303687,0,303687,10534.51963186264,0.011152713110352302
60861,304187,0,304187,10544.810466766357,0.011135654684050271
60961,304687,0,304687,10554.497265815735,0.0111186346650506
61061,305187,0,305187,10564.095353841782,0.011101652928192663
61161,305687,0,305687,10573.61340379715,0.011084709348919355
61261,306187,0,306187,10583.305442810059,0.011067803803272592
61361,306687,0,306687,10593.345868825912,0.011050936167888823
61461,307187,0,307187,10603.586822986603,0.011034106319994894
61562,307692,0,307692,10613.463243961334,0.011017146405375251
61662,308192,0,308192,10623.480993032455,0.011000392141305071
61762,308692,0,308692,10633.266429901123,0.010983675298695589
61862,309192,0,309192,10643.514310836792,0.01096699575709726
61962,309692,0,309692,10657.100888729095,0.01095035339662931
62062,310192,0,310192,10669.566437959671,0.010933748097975846
62162,310692,0,310692,10681.027782917023,0.01091717974238177
62262,311192,0,311192,10691.426622867584,0.010900648211648588
62362,311692,0,311692,10701.616724014282,0.010884153388130622
62462,312192,0,312192,10711.930752038956,0.010867695154730812
62563,312697,0,312697,10722.40866279602,0.010851109361097273
62663,313197,0,313197,10733.002998113632,0.010834724321809909
62763,313697,0,313697,10743.46959900856,0.010818375523451294
62863,314197,0,314197,10753.475327014923,0.010802062851086045
62963,314697,0,314697,10763.40349984169,0.010785786190308306
63063,315197,0,315197,10773.309302091599,0.010769545427238037
63163,315697,0,315697,10783.368887901306,0.010753340448517331
63263,316197,0,316197,10794.259662866592,0.010737171141306746
63363,316697,0,316697,10804.783824920654,0.010721037393281787
63463,317197,0,317197,10816.469074010849,0.010704939092629151
63564,317702,0,317702,10826.451053857803,0.010688715676469408
63664,318202,0,318202,10837.714394807816,0.010672688288844195
63764,318702,0,318702,10848.224430799484,0.010656696015083776
63864,319202,0,319202,10859.21707701683,0.010640738745390092
63964,319702,0,319702,10869.950998783112,0.010624816370458944
64064,320202,0,320202,10880.611844778061,0.010608928781476753
64164,320702,0,320702,10891.909802913666,0.010593075870117026
64264,321202,0,321202,10902.584411859512,0.010577257528537401
64364,321702,0,321702,10912.320845842361,0.010561473649376006
64464,322202,0,322202,10923.036822795868,0.010545724125748446
64565,322707,0,322707,10934.3197119236,0.010529851871098747
64665,323207,0,323207,10945.217736005783,0.010514171080677709
64765,323707,0,323707,10956.440607070923,0.010498524326917459
64865,324207,0,324207,10967.028987884521,0.010482911504816192
64965,324707,0,324707,10976.864063978195,0.01046733250983362
65065,325207,0,325207,10986.665052890778,0.010451787237888107
65165,325707,0,325707,10996.565737009048,0.010436275585353615
65265,326207,0,326207,11006.542742013931,0.010420797449056666
65365,326707,0,326707,11017.005421876907,0.010405352726273402
65465,327207,0,327207,11026.658280849457,0.010389941314726632
65566,327712,0,327712,11036.28273177147,0.010374409497925577
65666,328212,0,328212,11045.669867753983,0.010359064734361963
65766,328712,0,328712,11055.943378925323,0.010343752976846966
65866,329212,0,329212,11066.218785762787,0.010328474124865645
65966,329712,0,329712,11075.997896909714,0.01031322807833529
66066,330212,0,330212,11086.437386989594,0.010298014737602838
66166,330712,0,330712,11096.32517194748,0.010282834003442078
66266,331212,0,331212,11106.033344984055,0.010267685777050832
66366,331712,0,331712,11116.07791185379,0.01025256996004845
66466,332212,0,332212,11126.196492910385,0.010237486454472896
66567,332717,0,332717,11137.560546875,0.010222284812212408
66667,333217,0,333217,11151.138458967209,0.010207265957944597
66767,333717,0,333717,11162.646119832993,0.010192279122738455
66867,334217,0,334217,11172.585657835007,0.010177324210284857
66967,334717,0,334717,11182.68602180481,0.010162401124680144
67067,335217,0,335217,11193.12596487999,0.01014750977042398
67167,335717,0,335717,11205.460018873215,0.010132650052416637
67267,336217,0,336217,11217.020622968674,0.01011782187595667
67367,336717,0,336717,11226.686923980713,0.01010302514673816
67467,337217,0,337217,11237.22343492508,0.010088259770848646
67568,337722,0,337722,11248.542474985123,0.01007337847115224
67668,338222,0,338222,11258.748418807983,0.010058675832941918
67768,338722,0,338722,11269.115036010742,0.010044004267733175
67868,339222,0,339222,11279.634219884872,0.010029363683166441
67968,339722,0,339722,11290.17475104332,0.010014753987263647
68068,340222,0,340222,11301.393749952316,0.010000175088425746
68168,340722,0,340722,11312.228873968124,0.009985626895430482
68268,341222,0,341222,11322.344904899597,0.00997110931743021
68368,341722,0,341722,11332.638699054718,0.009956622263949484
68468,342222,0,342222,11343.332186937332,0.009942165644882985
68569,342727,0,342727,11353.892427921295,0.009927595260687146
68669,343227,0,343227,11364.123274087906,0.009913199543705072
68769,343727,0,343727,11374.355710029602,0.009898833992131227
68869,344227,0,344227,11384.912506818771,0.009884498517322133
68969,344727,0,344727,11396.370728969574,0.009870193030993572
69069,345227,0,345227,11406.558943033218,0.009855917445218387
69169,345727,0,345727,11416.597603797913,0.009841671672424392
69269,346227,0,346227,11426.747312784195,0.009827455625392278
69369,346727,0,346727,11437.085006952286,0.009813269217253612
69469,347227,0,347227,11448.138040781021,0.009799112361488766
69570,347732,0,347732,11458.04262304306,0.00978484384654294
69670,348232,0,348232,11467.934571027756,0.00977074613072348
69770,348732,0,348732,11478.979167938232,0.009756677708938531
69870,349232,0,349232,11488.632525920868,0.009742638496047024
69970,349732,0,349732,11498.18231511116,0.009728628407246753
70070,350232,0,350232,11508.97919178009,0.009714647358072485
70170,350732,0,350732,11520.734184980392,0.009700695264393818
70270,351232,0,351232,11532.754180908203,0.009686772042413642
70370,351732,0,351732,11543.24861907959,0.009672877608665807
70470,352232,0,352232,11555.67118191719,0.009659011880013748
70571,352737,0,352737,11566.945377111435,0.00964503654684775
70671,353237,0,353237,11577.863404750824,0.009631228265267692
70771,353737,0,353737,11587.745622873306,0.009617448440510861
70871,354237,0,354237,11597.881050825119,0.009603696990742629
70971,354737,0,354737,11607.897282838821,0.00958997383444859
71071,355237,0,355237,11618.466060876846,0.009576278890432836
71171,355737,0,355737,11630.501217126846,0.009562612077815969
71271,356237,0,356237,11641.333519935608,0.009548973316033592
71371,356737,0,356737,11652.32924079895,0.00953536252483438
71471,357237,0,357237,11663.648709774017,0.009521779624278486
71572,357742,0,357742,11674.483215808868,0.009508089124017292
71672,358242,0,358242,11683.940743923187,0.009494562043083053
71772,358742,0,358742,11694.419682741165,0.009481062614035508
71872,359242,0,359242,11704.739424943924,0.009467590758166729
71972,359742,0,359742,11858.060126066208,0.009454146397071614
72072,360242,0,360242,11870.410477876663,0.00944072945264662
72172,360742,0,360742,11880.718903779984,0.009427339847087882
72272,361242,0,361242,11890.213956832886,0.009413977502889696
72372,361742,0,361742,11900.395734786987,0.009400642342842902
72472,362242,0,362242,11912.137720823288,0.009387334290033298
72573,362747,0,362747,11922.545905828476,0.009373920593864169
72673,363247,0,363247,11933.32832288742,0.009360666795116655
72773,363747,0,363747,11946.424739837646,0.00934743987385884
72873,364247,0,364247,11959.48798084259,0.009334239754343675
72973,364747,0,364747,11970.289983034134,0.009321066361111194
73073,365247,0,365247,11980.020337820053,0.00930791961898726
73173,365747,0,365747,11989.362310886383,0.009294799453081844
73273,366247,0,366247,11999.604336977005,0.00928170578878762
73373,366747,0,366747,12009.886146783829,0.009268638551778471
73473,367247,0,367247,12020.363102912903,0.009255597668008087
73574,367752,0,367752,12032.291608810425,0.0092424530501279
73674,368252,0,368252,12044.373602867126,0.0092294649134975
73774,368752,0,368752,12054.628666877747,0.009216502908900139
73874,369252,0,369252,12064.524953842163,0.009203566963396942
73974,369752,0,369752,12074.676825761795,0.009190657004321437
74074,370252,0,370252,12084.651273965836,0.009177772959278449
74174,370752,0,370752,12094.500089883804,0.009164914756142605
74274,371252,0,371252,12104.051033973694,0.009152082323056926
74374,371752,0,371752,12113.583316087723,0.009139275588431556
74474,372252,0,372252,12123.17876291275,0.009126494480942193
74575,372757,0,372757,12133.364844799042,0.009113611502833364
74675,373257,0,373257,12143.433889865875,0.009100881691195857
74775,373757,0,373757,12153.24691581726,0.00908817729359864
74875,374257,0,374257,12162.93075799942,0.009075498239769579
74975,374757,0,374757,12172.653393983841,0.009062844459695595
75075,375257,0,375257,12182.241153001785,0.009050215883621465
75175,375757,0,375757,12192.114384889603,0.009037612442048298
75275,376257,0,376257,12201.910492897034,0.009025034065732537
75375,376757,0,376757,12211.556963920593,0.009012480685684554
75475,377257,0,377257,12223.015185832977,0.008999952233167345
75576,377762,0,377762,12233.967998981476,0.00898732372906778
75676,378262,0,378262,12244.232633829117,0.008974845173970078
75776,378762,0,378762,12253.928231954575,0.00896239134101734
75876,379262,0,379262,12263.73308801651,0.008949962162473353
75976,379762,0,379762,12273.298439979553,0.008937557570848572
76076,380262,0,380262,12282.897511005402,0.008925177498898616
76176,380762,0,380762,12292.453680992126,0.008912821879623369
76276,381262,0,381262,12303.155387878418,0.008900490646265528
76376,381762,0,381762,12312.657185792923,0.008888183732309636
76476,382262,0,382262,12322.564269781113,0.008875901071480823
76577,382767,0,382767,12334.046644926071,0.008863520134928261
76677,383267,0,383267,12344.250470876694,0.00885128602336697
76777,383767,0,383767,12354.353832960129,0.00883907596688567
76877,384267,0,384267,12365.246877908707,0.008826889900162714
76977,384767,0,384767,12375.282857894897,0.00881472775811127
77077,385267,0,385267,12385.18101477623,0.008802589475878288
77177,385767,0,385767,12395.753201007843,0.008790474988843324
77277,386267,0,386267,12406.077651977539,0.008778384232617462
77377,386767,0,386767,12415.72970199585,0.008766317143042213
77477,387267,0,387267,12426.66630411148,0.008754273656188475
77578,387772,0,387772,12437.256542921066,0.008742133627534144
77678,388272,0,388272,12447.806750059128,0.008730137389683685
77778,388772,0,388772,12458.746620893478,0.008718164563501302
77878,389272,0,389272,12469.348270893097,0.008706215085966727
77978,389772,0,389772,12479.718670845032,0.008694288894283768
78078,390272,0,390272,12489.988988876343,0.00868238592587914
78178,390772,0,390772,12500.18431186676,0.008670506118401441
78278,391272,0,391272,12510.168486833572,0.008658649409720299
78378,391772,0,391772,12521.988092899323,0.00864681573792507
78478,392272,0,392272,12532.61269569397,0.008635005041324043
78579,392777,0,392777,12542.731447696686,0.008623099496121365
78679,393277,0,393277,12552.61932182312,0.008611334793919933
78779,393777,0,393777,12561.961922883987,0.008599592882531265
78879,394277,0,394277,12574.220978021622,0.008587873701131213
78979,394777,0,394777,12591.14508485794,0.008576177189109406
79079,395277,0,395277,12602.095505952835,0.00856450328606849
79179,395777,0,395777,12612.612853050232,0.00855285193182291
79279,396277,0,396277,12625.271368980408,0.00854122306639819
79379,396777,0,396777,12637.811251878738,0.008529616630029812
79479,397277,0,397277,12648.869386911392,0.00851803256316229
79580,397782,0,397782,12660.23443889618,0.008506355301347166
79680,398282,0,398282,12671.577410936356,0.008494816017858713
79780,398782,0,398782,12681.931404829025,0.008483298925861395
79880,399282,0,399282,12694.247112989426,0.008471803966628642
79980,399782,0,399782,12703.817835092545,0.008460331081638335
80080,400282,0,400282,12713.264189958572,0.008448880212571787
80180,400782,0,400782,12723.853051900864,0.0084374513013129
80280,401282,0,401282,12733.579011917114,0.008426044289947223
80380,401782,0,401782,12743.502896785736,0.00841465912076111
80480,402282,0,402282,12753.524314880371,0.008403295736240804
80581,402787,0,402787,12763.415397882462,0.008391840772029537
80681,403287,0,403287,12773.16028380394,0.008380521001509248
80781,403787,0,403787,12783.206682920456,0.008369222843735764
80881,404287,0,404287,12794.610837936401,0.008357946241988035
80981,404787,0,404787,12806.897563934326,0.008346691139740556
81081,405287,0,405287,12818.268851041794,0.008335457480662466
81181,405787,0,405787,12829.871589899063,0.008324245208616701
81281,406287,0,406287,12841.061709880829,0.008313054267659136
81381,406787,0,406787,12851.428687810898,0.008301884602037818
81481,407287,0,407287,12861.72916483879,0.008290736156192073
81582,407792,0,407792,12872.992948055267,0.00827949770863063
81682,408292,0,408292,12883.369881868362,0.00826839174722913
81782,408792,0,408792,12895.631880044937,0.008257306839511638
81882,409292,0,409292,12906.072833061218,0.008246242930676172
81982,409792,0,409792,12917.561244010925,0.008235199966108064
82082,410292,0,410292,12928.737320899963,0.008224177891378928
82182,410792,0,410792,12940.106654882431,0.008213176652245989
82282,411292,0,411292,12951.685611009598,0.008202196194651235
82382,411792,0,411792,12961.962002038956,0.00819123646472067
82482,412292,0,412292,12972.195574045181,0.008180297408763517
82583,412797,0,412797,12982.069355010986,0.008169269892869238
82683,413297,0,413297,12992.01236486435,0.008158372229918127
82783,413797,0,413797,13001.890798807144,0.008147495080428932
82883,414297,0,414297,13012.753487825394,0.008136638391437702
82983,414797,0,414797,13023.096176862717,0.008125802110159891
83083,415297,0,415297,13034.685487985611,0.008114986183989498
83183,415797,0,415797,13045.602393865585,0.008104190560498365
83283,416297,0,416297,13056.647297143936,0.00809341518743536
83383,416797,0,416797,13067.446592092514,0.008082660012725782
83483,417297,0,417297,13077.734493970871,0.008071924984470532
83584,417802,0,417802,13087.33752989769,0.008061103002913819
83684,418302,0,418302,13098.572657823563,0.008050408312740509
83784,418802,0,418802,13109.415833950043,0.008039733613857488
83884,419302,0,419302,13120.74457192421,0.00802907885506238
83984,419802,0,419802,13131.119787693024,0.008018443985324891
84084,420302,0,420302,13141.35398197174,0.00800782895378588
84184,420802,0,420802,13152.292392969131,0.00799723370975684
84284,421302,0,421302,13165.624024868011,0.007986658202718997
84384,421802,0,421802,13176.336890935898,0.007976102382322723
84484,422302,0,422302,13188.248998880386,0.00796556619838685
84585,422807,0,422807,13198.215997934341,0.007954944533665867
84685,423307,0,423307,13207.83170390129,0.007944447667892422
84785,423807,0,423807,13217.324961900711,0.007933970288543597
84885,424307,0,424307,13227.471884727478,0.007923512346106694
84985,424807,0,424807,13239.36557173729,0.007913073791234043
85085,425307,0,425307,13250.704677820206,0.00790265457474222
85185,425807,0,425807,13260.59997177124,0.007892254647611542
85285,426307,0,426307,13270.823391914368,0.007881873960985272
85385,426807,0,426807,13282.479831695557,0.007871512466168936
85485,427307,0,427307,13292.75188589096,0.007861170114629865
85586,427812,0,427812,13304.172152757645,0.007850743721695924
85686,428312,0,428312,13314.584637880325,0.007840439701980386
85786,428812,0,428812,13324.330173969269,0.007830154680427536
85886,429312,0,429312,15087.304672002792,0.007819888609146272
85986,429812,0,429812,15095.892345905304,0.007809641440404051
86086,430312,0,430312,15104.568359851837,0.0077994131266259144
86186,430812,0,430812,15113.906498908997,0.0077892036203942
86286,431312,0,431312,15122.520075082779,0.007779012874447677
86386,431812,0,431812,15131.858960866928,0.007768840841681057
86486,432312,0,432312,15142.028854846954,0.007758687475144215
86587,432817,0,432817,15155.241741895676,0.007748451474440908
86687,433317,0,433317,15461.041640043259,0.00773833548562429
86787,433817,0,433817,15472.429379940033,0.007728238022648513
86887,434317,0,434317,15481.12131690979,0.0077181590391798074
86987,434817,0,434817,15490.189616918564,0.007708098489036773
87087,435317,0,435317,15499.855998039246,0.007698056326189408
87187,435817,0,435817,15509.65214395523,0.007688032504758776
87287,436317,0,436317,15518.601984977722,0.007678026979016267
87387,436817,0,436817,15531.033084869385,0.007668039703383057
87487,437317,0,437317,15542.000818014145,0.00765807063242958
87588,437822,0,437822,15553.572204828262,0.0076480203033114065
87688,438322,0,438322,15563.030554771423,0.007638087686937562
87788,438822,0,438822,15572.761148929596,0.007628173139394758
87888,439322,0,439322,15582.102011919022,0.007618276615845734
87988,439822,0,439822,15591.982543945312,0.007608398071599532
88088,440322,0,440322,15601.266079902649,0.007598537462110887
88188,440822,0,440822,16824.69021987915,0.007588694742979678
88288,441322,0,441322,16833.946037054062,0.007578869869950294
88388,441822,0,441822,16842.3015229702,0.007569062798911131
88488,442322,0,442322,16850.672110795975,0.007559273485894136
88589,442827,0,442827,16860.1533100605,0.007549404260394502
88689,443327,0,443327,16869.99819803238,0.007539650508573227
88789,443827,0,443827,16880.72551393509,0.007529914383289964
88889,444327,0,444327,16890.48481988907,0.0075201958411461635
88989,444827,0,444827,16899.928216934204,0.007510494838883947
89089,445327,0,445327,17370.99649000168,0.007500811333385456
89189,445827,0,445827,17380.454955101013,0.007491145281672662
89289,446327,0,446327,17388.93695998192,0.007481496640906325
89389,446827,0,446827,17397.431469917297,0.007471865368385775
89489,447327,0,447327,17406.18833589554,0.0074622514215483765
89590,447832,0,447832,17415.450124025345,0.007452558878470288
89690,448332,0,448332,17424.941165924072,0.007442979628056925
89790,448832,0,448832,17435.632968902588,0.007433417576040308
89890,449332,0,449332,17445.69460296631,0.0074238726804056925
89990,449832,0,449832,17455.73383307457,0.007414344899273755
90090,450332,0,450332,17466.071660757065,0.00740483419089985
90190,450832,0,450832,17476.645174741745,0.007395340513673718
90290,451332,0,451332,17486.81414294243,0.007385863826118839
90390,451832,0,451832,17495.84269595146,0.00737640408689199
90490,452332,0,452332,17505.84803891182,0.007366961254782764
90591,452837,0,452837,17515.66375684738,0.0073574411140870585
90691,453337,0,453337,17525.394073963165,0.007348032141154787
90791,453837,0,453837,17535.555070877075,0.007338639952092819
90891,454337,0,454337,17545.49502801895,0.007329264506218072
90991,454837,0,454837,17554.885261774063,0.0073199057629777225
91091,455337,0,455337,17564.64334177971,0.007310563681948621
91191,455837,0,455837,17574.296652793884,0.007301238222837031
91291,456337,0,456337,17583.75923895836,0.007291929345477963
91391,456837,0,456837,17593.51507472992,0.007282637009834631
91491,457337,0,457337,17603.02508497238,0.007273361175998208
91592,457842,0,457842,17612.72210097313,0.0072640092934679315
91692,458342,0,458342,17622.229910850525,0.007254766508051344
91792,458842,0,458842,17631.57049393654,0.007245540105082393
91892,459342,0,459342,17641.12450194359,0.007236330045159958
91992,459842,0,459842,17650.448009967804,0.0072271362890082265
92092,460342,0,460342,17660.037187814713,0.007217958797476529
92192,460842,0,460842,17669.44623374939,0.0072087975315385
92292,461342,0,461342,17678.822188854218,0.007199652452291912
92392,461842,0,461842,17688.17142391205,0.007190523520958018
92492,462342,0,462342,17697.514234781265,0.0071814106988812455
92593,462847,0,462847,17707.074559926987,0.007172223061042053
92693,463347,0,463347,17716.44420981407,0.007163142502132242
92793,463847,0,463847,17726.087445020676,0.007154077936864347
92893,464347,0,464347,17735.72278571129,0.0071450293270718425
92993,464847,0,464847,17747.433388710022,0.007135996634708912
93093,465347,0,465347,17757.99951696396,0.0071269798218501655
93193,465847,0,465847,17768.26766705513,0.00711797885069003
93293,466347,0,466347,17778.4398458004,0.007108993683542557
93393,466847,0,466847,17790.06019592285,0.007100024282840741
93493,467347,0,467347,17801.919726848602,0.007091070611136209
93594,467852,0,467852,17813.336525917053,0.007082043330415176
93694,468352,0,468352,17825.16347503662,0.007073121161189108
93794,468852,0,468852,17834.8581738472,0.007064214608951908
93894,469352,0,469352,17844.179510831833,0.007055323636726295
93994,469852,0,469852,17853.6309838295,0.007046448207651482
94094,470352,0,470352,17863.161146879196,0.007037588284982597
94194,470852,0,470852,17874.401653051376,0.007028743832090383
94294,471352,0,471352,17884.576715946198,0.0070199148124606295
94394,471852,0,471852,17894.132405996323,0.007011101189693909
94494,472352,0,472352,17905.13010287285,0.007002302927505031
94595,472857,0,472857,17915.84119772911,0.006993432237611076
94695,473357,0,473357,17926.112967014313,0.00698466474087926
94795,473857,0,473857,17936.278655052185,0.00697591249619243
94895,474357,0,474357,17945.845795869827,0.006967175467719562
94995,474857,0,474857,17955.441718816757,0.006958453619741743
95095,475357,0,475357,17965.01329112053,0.006949746916651864
95195,475857,0,475857,17974.588701963425,0.006941055322954289
95295,476357,0,476357,17984.068623781204,0.006932378803264259
95395,476857,0,476857,17993.701808929443,0.006923717322307627
95495,477357,0,477357,18003.255145072937,0.006915070844920406
95596,477862,0,477862,18012.97402191162,0.006906353096432363
95696,478362,0,478362,18022.504853963852,0.006897736670290314
95796,478862,0,478862,18032.14077591896,0.006889135142534957
95896,479362,0,479362,18041.745065927505,0.006880548478440099
95996,479862,0,479862,18051.30794596672,0.006871976643387665
96096,480362,0,480362,18060.829210996628,0.006863419602867391
96196,480862,0,480862,18070.32433271408,0.0068548773224764385
96296,481362,0,481362,18079.94973707199,0.006846349767918926
96396,481862,0,481862,18089.555818080902,0.006837836905005648
96496,482362,0,482362,18099.007297754288,0.006829338699653576
96597,482867,0,482867,18109.5432677269,0.006820770355802233
96697,483367,0,483367,18119.607299804688,0.006812301509472928
96797,483867,0,483867,18129.147530078888,0.006803847218752175
96897,484367,0,484367,18138.62798690796,0.006795407449979118
96997,484867,0,484867,18148.823266744614,0.0067869821695972134
97097,485367,0,485367,18158.723965883255,0.0067785713441538
97197,485867,0,485867,18168.208043813705,0.006770174940299822
97297,486367,0,486367,18178.21631169319,0.006761792924789532
97397,486867,0,486867,18188.72185778618,0.006753425264479824
97497,487367,0,487367,18199.72372198105,0.006745071926330205
97598,487872,0,487872,18210.52154994011,0.00673664955896222
97698,488372,0,488372,18221.143618822098,0.0067283249088173165
97798,488872,0,488872,18231.155718803406,0.006720014481995018
97898,489372,0,489372,18241.412020921707,0.006711718245861882
97998,489872,0,489872,18251.454318761826,0.006703436167885163
98098,490372,0,490372,18261.516823768616,0.00669516821563234
98198,490872,0,490872,18272.45702981949,0.006686914356770828
98298,491372,0,491372,18284.328454971313,0.006678674559067552
98398,491872,0,491872,18295.765505075455,0.006670448790388656
98498,492372,0,492372,18306.535614967346,0.006662237018699133
98599,492877,0,492877,18316.013466835022,0.006653957304411834
98699,493377,0,493377,18325.755074739456,0.006645773570161275
98799,493877,0,493877,18335.480105876923,0.006637603737067666
98899,494377,0,494377,18345.098648786545,0.006629447773488743
98999,494877,0,494877,18355.9884288311,0.006621305647879393
99099,495377,0,495377,18365.758004903793,0.006613177328791244
99199,495877,0,495877,18375.88257598877,0.006605062784872306
99299,496377,0,496377,18387.318913698196,0.0065969619848665765
99399,496877,0,496877,18397.86950492859,0.006588874897613887
99499,497377,0,497377,18408.301431894302,0.0065808014920493456
99600,497882,0,497882,18418.195657014847,0.00657266120848623
99700,498382,0,498382,18427.903971910477,0.006564615209526012
99800,498882,0,498882,18439.140279769897,0.006556582799320839
99900,499382,0,499382,18451.404489040375,0.006548563947184871
100000,499882,0,499882,18461.5774269104,0.006540558622526011


==> plot_data/quadratic_minimax_problem_n500_alpha0/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0014910697937011719,30.358099469249375
200,201,200,401,0.1721489429473877,2.443647106553536
400,401,400,801,0.34951090812683105,1.4623020054181544
601,602,601,1203,0.5220968723297119,1.0864359863509294
801,802,801,1603,0.6736180782318115,0.884172469333225
1001,1002,1001,2003,1.1403388977050781,0.756423386206226
1201,1202,1201,2403,1.335745096206665,0.6677556741322215
1401,1402,1401,2803,1.4906928539276123,0.6018803012446704
1602,1603,1602,3205,1.6921212673187256,0.5501556568527358
1802,1803,1802,3605,1.9836199283599854,0.5083939523309472
2002,2003,2002,4005,2.1715409755706787,0.4735281727112222
2202,2203,2202,4405,2.31919002532959,0.44380632430760936
2402,2403,2402,4805,2.564152240753174,0.41806194377676287
2603,2604,2603,5207,2.7299749851226807,0.3953741725141351
2803,2804,2803,5607,2.8932979106903076,0.37537408529409977
3003,3004,3003,6007,3.1782779693603516,0.3574967775454968
3203,3204,3203,6407,3.357166051864624,0.34139925351073
3403,3404,3403,6807,3.551548957824707,0.32681143125199247
3604,3605,3604,7209,3.7118289470672607,0.31345351992341636
3804,3805,3804,7609,3.8677680492401123,0.3012822006287603
4004,4005,4004,8009,4.030489921569824,0.29008382263827337
4204,4205,4204,8409,4.224907159805298,0.279738735984933
4404,4405,4404,8809,4.38552713394165,0.2701466855862572
4605,4606,4605,9211,4.5640881061553955,0.26117989625642984
4805,4806,4805,9611,4.792270183563232,0.25285519172052956
5005,5006,5005,10011,4.97637414932251,0.24506456097986604
5205,5206,5205,10411,5.165646076202393,0.2377546752075857
5405,5406,5405,10811,5.488664150238037,0.23087923832463025
5606,5607,5606,11213,5.897052049636841,0.22436636221942408
5806,5807,5806,11613,6.258732080459595,0.21824526706125563
6006,6007,6006,12013,6.574193954467773,0.21245137964008523
6206,6207,6206,12413,6.776195049285889,0.20695707567728125
6406,6407,6406,12813,6.952604055404663,0.2017378176032389
6607,6608,6607,13215,7.166656970977783,0.19674750585888232
6807,6808,6807,13615,7.338606119155884,0.19201616179110503
7007,7008,7007,14015,7.5286102294921875,0.18750081290361562
7207,7208,7207,14415,7.729483127593994,0.18318569600874168
7407,7408,7407,14815,7.881656169891357,0.17905660071913546
7608,7609,7608,15217,8.065749168395996,0.17508132201764354
7808,7809,7808,15617,8.232303857803345,0.17128774083740186
8008,8009,8008,16017,8.402020931243896,0.1676451094270218
8208,8209,8208,16417,8.578912019729614,0.1641438367768636
8408,8409,8408,16817,8.735471963882446,0.16077518492537093
8609,8610,8609,17219,8.901782989501953,0.15751525889048315
8809,8810,8809,17619,9.06904411315918,0.1543891739329465
9009,9010,9009,18019,9.23555302619934,0.15137372855239975
9209,9210,9209,18419,9.37932801246643,0.14846279486717895
9409,9410,9409,18819,9.580969095230103,0.14565073983046334
9610,9611,9610,19221,9.86003589630127,0.14291901173762436
9810,9811,9810,19621,10.053208112716675,0.1402899883101414
10010,10011,10010,20021,10.23738408088684,0.13774542960476252
10210,10211,10210,20421,10.430102109909058,0.13528124533194744
10410,10411,10410,20821,10.600186824798584,0.13289364321357225
10611,10612,10611,21223,10.757214069366455,0.13056770656886155
10811,10812,10811,21623,10.958417892456055,0.12832328956712113
11011,11012,11011,22023,11.114824056625366,0.1261455885687076
11211,11212,11211,22423,11.28009295463562,0.12403175478829191
11411,11412,11411,22823,11.430287837982178,0.12197912473265268
11612,11613,11612,23225,11.577897071838379,0.11997537797070633
11812,11813,11812,23625,11.732659101486206,0.11803810315282258
12012,12013,12012,24025,11.89461612701416,0.11615498909882122
12212,12213,12212,24425,12.042931079864502,0.11432396789326375
12412,12413,12412,24825,12.187634944915771,0.11254309058936256
12613,12614,12613,25227,12.340112924575806,0.110801973111828
12813,12814,12813,25627,12.48270297050476,0.1091161940007785
13013,13014,13013,26027,12.627492904663086,0.10747532590128248
13213,13214,13213,26427,12.77098798751831,0.10587780854087535
13413,13414,13413,26827,12.917166233062744,0.10432216072143556
13614,13615,13614,27229,13.062029123306274,0.1027994978932257
13814,13815,13814,27629,13.206346988677979,0.10132362536127505
14014,14015,14014,28029,13.367260932922363,0.09988559085904321
14214,14215,14214,28429,13.528511047363281,0.09848417612377038
14414,14415,14414,28829,13.671755075454712,0.09711821743955897
14615,14616,14615,29231,13.819056034088135,0.0957800283723399
14815,14816,14815,29631,14.055022239685059,0.09448185460311487
15015,15016,15015,30031,14.202134132385254,0.09321593291789647
15215,15216,15215,30431,14.392217874526978,0.09198128436427426
15415,15416,15415,30831,14.539200067520142,0.09077696909114973
15616,15617,15616,31233,14.685840845108032,0.08959628204623568
15816,15817,15816,31633,14.890947818756104,0.08845009932042187
16016,16017,16016,32033,15.037644147872925,0.08733163829440838
16216,16217,16216,32433,15.185374021530151,0.08624009403053348
16416,16417,16416,32833,15.332825899124146,0.08517469069943166
16617,16618,16617,33235,15.512036085128784,0.08412954255472277
16817,16818,16817,33635,15.662084817886353,0.08311432399365244
17017,17018,17017,34035,15.816444873809814,0.0821230752025654
17217,17218,17217,34435,15.965311050415039,0.08115512255151293
17417,17418,17417,34835,16.122087001800537,0.0802098148541593
17618,17619,17618,35237,16.277503967285156,0.07928196013273325
17818,17819,17818,35637,16.43550395965576,0.078380178893659
18018,18019,18018,36037,16.590744018554688,0.07749921063335644
18218,18219,18218,36437,16.734294176101685,0.07663848419961432
18418,18419,18418,36837,16.8800048828125,0.07579744628785841
18619,18620,18619,37239,17.031764030456543,0.07497149851088454
18819,18820,18819,37639,17.17979907989502,0.0741683373353586
19019,19020,19019,38039,17.324185848236084,0.07338330217372391
19219,19220,19219,38439,17.491147994995117,0.0726159042077601
19419,19420,19419,38839,17.63406491279602,0.07186566918245992
19620,19621,19620,39241,17.77882409095764,0.07112851041108008
19820,19821,19820,39641,17.93207812309265,0.07041131424899968
20020,20021,20020,40041,18.074905157089233,0.06970993822399434
20220,20221,20220,40441,18.223223209381104,0.06902396125842604
20420,20421,20420,40841,18.38381600379944,0.06835297440345825
20621,20622,20621,41243,18.528983116149902,0.06769333446935327
20821,20822,20821,41643,18.673547983169556,0.06705121754971857
21021,21022,21021,42043,18.829493045806885,0.06642293080248314
21221,21222,21221,42443,18.98547101020813,0.06580810992625838
21421,21422,21421,42843,19.160052061080933,0.0652064008787552
21622,21623,21622,43245,19.315546989440918,0.0646145463605294
21822,21823,21822,43645,19.46136713027954,0.064038099621106
22022,22023,22022,44045,19.60757303237915,0.06347375937579187
22222,22223,22222,44445,19.761258125305176,0.06292120957063496
22422,22423,22422,44845,19.95094394683838,0.06238014292701027
22623,22624,22623,45247,20.095844984054565,0.06184763887898292
22823,22824,22823,45647,20.240041971206665,0.06132870428205937
23023,23024,23023,46047,20.403598070144653,0.060820379709791594
23223,23224,23223,46447,20.609939098358154,0.06032239051084022
23423,23424,23423,46847,20.763883113861084,0.05983446959782742
23624,23625,23624,47249,20.948374032974243,0.05935399088605918
23824,23825,23824,47649,21.101516008377075,0.05888548162126789
24024,24025,24024,48049,21.29066801071167,0.05842628142641032
24224,24225,24224,48449,21.436206817626953,0.05797615141237147
24424,24425,24424,48849,21.586517095565796,0.05753485924196196
24625,24626,24625,49251,21.731067895889282,0.05710003681135416
24825,24826,24825,49651,21.91562008857727,0.05667579003434358
25025,25026,25025,50051,22.062901973724365,0.05625972054690382
25225,25226,25225,50451,22.207606077194214,0.0558516204757849
25425,25426,25425,50851,22.352801084518433,0.05545128763916859
25626,25627,25626,51253,22.500121116638184,0.055056580276372336
25826,25827,25826,51653,22.657701015472412,0.05467123377464037
26026,26027,26026,52053,22.810935020446777,0.054293079648154545
26226,26227,26226,52453,22.965838193893433,0.053921936982787105
26426,26427,26426,52853,23.112565994262695,0.05355762981499894
26627,26628,26627,53255,23.25819492340088,0.05319821524473985
26827,26828,26827,53655,23.405689239501953,0.052847102387807154
27027,27028,27027,54055,23.55393099784851,0.05250232470432488
27227,27228,27227,54455,23.6998770236969,0.05216372473443906
27427,27428,27427,54855,23.847538948059082,0.05183114932581228
27628,27629,27628,55257,23.99309015274048,0.05150283053382608
27828,27829,27828,55657,24.13757610321045,0.05118188972906709
28028,28029,28028,56057,24.289198875427246,0.05086653801236315
28228,28229,28228,56457,24.441261053085327,0.05055663832946747
28428,28429,28428,56857,24.590600967407227,0.05025205737277767
28629,28630,28629,57259,24.74024510383606,0.0499511813428624
28829,28830,28829,57659,24.896986961364746,0.049656877392330066
29029,29030,29029,58059,25.041050910949707,0.0493675131009554
29229,29230,29229,58459,25.185364961624146,0.049082969158376004
29429,29430,29429,58859,25.326876878738403,0.048803129510607654
29630,29631,29630,59261,25.477782011032104,0.048526516378772415
29830,29831,29830,59661,25.623910903930664,0.04825577187211327
30030,30031,30030,60061,25.76947593688965,0.04798940161853438
30230,30231,30230,60461,25.91222882270813,0.04772730172426648
30430,30431,30430,60861,26.059629201889038,0.04746937112319351
30631,30632,30631,61263,26.207449913024902,0.04721425226639098
30831,30832,30831,61663,26.35277485847473,0.046964387612019744
31031,31032,31031,62063,26.498263120651245,0.04671840478045996
31231,31232,31231,62463,26.64272427558899,0.04647621325984695
31431,31432,31431,62863,26.78769302368164,0.04623772499135371
31632,31633,31632,63265,26.947783946990967,0.046001688895038945
31832,31833,31832,63665,27.112432956695557,0.04577036988910864
32032,32033,32032,64065,27.258835077285767,0.04554250359696158
32232,32233,32232,64465,27.410036087036133,0.04531801111171686
32432,32433,32432,64865,27.561098098754883,0.04509681565269014
32633,32634,32633,65267,27.716853141784668,0.0448777606127259
32833,32834,32833,65667,27.864712953567505,0.0446629526387775
33033,33034,33033,66067,28.01070213317871,0.04445122316461319
33233,33234,33233,66467,28.166537046432495,0.04424250333914123
33433,33434,33433,66867,28.311180114746094,0.044036726152848336
33634,33635,33634,67269,28.457129955291748,0.04383281900891723
33834,33835,33834,67669,28.60214900970459,0.04363274709200168
34034,34035,34034,68069,28.745763063430786,0.0434354270151071
34234,34235,34234,68469,28.88890504837036,0.04324079863493503
34434,34435,34434,68869,29.041901111602783,0.043048803402420996
34635,34636,34635,69271,29.2080020904541,0.04285844360072434
34835,34836,34835,69671,29.358524084091187,0.04267155763409157
35035,35036,35035,70071,29.503119945526123,0.04248713801960008
35235,35236,35235,70471,29.657550811767578,0.04230513215120475
35435,35436,35435,70871,29.800734043121338,0.042125488802573635
35636,35637,35636,71273,29.950026035308838,0.041947277162603804
35836,35837,35836,71673,30.105008840560913,0.04177222169836566
36036,36037,36036,72073,30.249951124191284,0.04159938273239527
36236,36237,36236,72473,30.393401861190796,0.04142871418144415
36436,36437,36436,72873,30.53843903541565,0.04126017115626857
36637,36638,36637,73275,30.683300256729126,0.04109288278002668
36837,36838,36837,73675,30.826402187347412,0.04092847083658302
37037,37038,37037,74075,30.99558401107788,0.04076605637549582
37237,37238,37237,74475,31.18208909034729,0.04060559895868889
37437,37438,37437,74875,31.34405207633972,0.04044705918159016
37638,37639,37638,75277,31.49356698989868,0.040289619999451236
37838,37839,37838,75677,31.657145977020264,0.040134810392883795
38038,38039,38038,76077,31.81377410888672,0.039981805944153945
38238,38239,38238,76477,31.96026611328125,0.03983057110228058
38438,38439,38438,76877,32.10705804824829,0.03968107121126238
38639,38640,38639,77279,32.25269889831543,0.039532537709657874
38839,38840,38839,77679,32.399226903915405,0.039386415466236425
39039,39040,39039,78079,32.54489207267761,0.039241929167629405
39239,39240,39239,78479,32.69813513755798,0.039099047495965364
39439,39440,39439,78879,32.88307523727417,0.03895773990892605
39640,39641,39640,79281,33.03171110153198,0.038817281632442746
39840,39841,39840,79681,33.17893314361572,0.038679041085945186
40040,40041,40040,80081,33.32568311691284,0.03854228729564062
40240,40241,40240,80481,33.49166011810303,0.038406992613132955
40440,40441,40440,80881,33.63779401779175,0.038273130062700625
40641,40642,40641,81283,33.78247880935669,0.03814001452752626
40841,40842,40841,81683,33.93452501296997,0.03800894474858745
41041,41042,41041,82083,34.07732892036438,0.03787922990179488
41241,41242,41241,82483,34.22087812423706,0.037750845522796
41441,41442,41441,82883,34.3671932220459,0.03762376773133308
41642,41643,41642,83285,34.51578497886658,0.03749734742828437
41842,41843,41842,83685,34.68741989135742,0.03737281967346745
42042,42043,42042,84085,34.86278510093689,0.037249530100944415
42242,42243,42242,84485,35.02073907852173,0.03712745701249274
42442,42443,42442,84885,35.17447805404663,0.03700657921773478
42643,42644,42643,85287,35.3259642124176,0.03688628042127037
42843,42844,42843,85687,35.47142720222473,0.03676773732690133
43043,43044,43043,86087,35.633002042770386,0.03665032876749169
43243,43244,43243,86487,35.788504123687744,0.03653403545120651
43443,43444,43443,86887,35.93386697769165,0.03641883852841708
43644,43645,43644,87289,36.078866958618164,0.03630415166299038
43844,43845,43844,87689,36.223310232162476,0.036191097942920594
44044,44045,44044,88089,36.37023901939392,0.03607908651570536
44244,44245,44244,88489,36.51558208465576,0.035968100186186944
44444,44445,44444,88889,36.66073703765869,0.03585812214489164
44645,44646,44645,89291,36.80644989013672,0.03574859349167758
44845,44846,44845,89691,36.95969891548157,0.0356405879290156
45045,45046,45045,90091,37.12867212295532,0.035533542360903794
45245,45246,45245,90491,37.30207586288452,0.035427441422120065
45445,45446,45445,90891,37.446547985076904,0.035322270084430264
45646,45647,45646,91293,37.59386205673218,0.03521749463992091
45846,45847,45846,91693,37.780027866363525,0.03511414319045893
46046,46047,46046,92093,37.92984986305237,0.035011678122097524
46246,46247,46246,92493,38.075993061065674,0.034910085669676794
46446,46447,46446,92893,38.221956968307495,0.034809352363038934
46647,46648,46647,93295,38.36754107475281,0.034708967686338764
46847,46848,46847,93695,38.51212501525879,0.03460991753600919
47047,47048,47047,94095,38.655054807662964,0.03451168775291461
47247,47248,47247,94495,38.80659198760986,0.03441426597369256
47447,47448,47447,94895,38.9509482383728,0.03431764009374857
47648,47649,47648,95297,39.09393095970154,0.03422132100179268
47848,47849,47848,95697,39.26690602302551,0.03412625544220422
48048,48049,48048,96097,39.423166036605835,0.03403195089917383
48248,48249,48248,96497,39.570794105529785,0.033938396239960346
48448,48449,48448,96897,39.715779066085815,0.03384558055928565
48649,48650,48649,97299,39.872374057769775,0.033753034548853804
48849,48850,48849,97699,40.03850197792053,0.03366166855399277
49049,49050,49049,98099,40.185940980911255,0.03357101007938353
49249,49250,49249,98499,40.338980197906494,0.03348104907494266
49449,49450,49449,98899,40.486855030059814,0.03339177569096829
49650,49651,49650,99301,40.63190293312073,0.03330273898351182
49850,49851,49850,99701,40.777180910110474,0.0332148153872823
50050,50051,50050,100101,40.92346000671387,0.033127550969873985
50250,50251,50250,100501,41.0677809715271,0.03304093663579046
50450,50451,50450,100901,41.21245503425598,0.0329549634664552
50651,50652,50651,101303,41.35889911651611,0.03286919758663817
50851,50852,50851,101703,41.503172874450684,0.032784483775300924
51051,51052,51051,102103,41.64769005775452,0.03270038535043529
51251,51252,51251,102503,41.8093581199646,0.032616894060114525
51451,51452,51451,102903,41.957218170166016,0.03253400180897552
51652,51653,51652,103305,42.11891794204712,0.03245129062069263
51852,51853,51852,103705,42.26580786705017,0.03236957566668825
52052,52053,52052,104105,42.45754098892212,0.03228843633043651
52252,52253,52252,104505,42.61540603637695,0.03220786510719228
52452,52453,52452,104905,42.761038064956665,0.03212785463108102
52653,52654,52653,105307,42.908485889434814,0.03204800176579049
52853,52854,52853,105707,43.053614139556885,0.03196909394012309
53053,53054,53053,106107,43.20104002952576,0.03189072553060704
53253,53254,53253,106507,43.34565711021423,0.03181288969584784
53453,53454,53453,106907,43.50075602531433,0.03173557971791675
53654,53655,53654,107309,43.645997047424316,0.0316584063396373
53854,53855,53854,107709,43.793062925338745,0.03158213094916858
54054,54055,54054,108109,43.93716096878052,0.03150636194305282
54254,54255,54254,108509,44.08216309547424,0.03143109307020482
54454,54455,54454,108909,44.236693143844604,0.031356318189567724
54655,54656,54655,109311,44.390405893325806,0.031281661049028214
54855,54856,54855,109711,44.53461503982544,0.03120785855288486
55055,55056,55055,110111,44.67984199523926,0.031134532232669453
55255,55256,55255,110511,44.825031995773315,0.03106167636384517
55455,55456,55455,110911,44.96980309486389,0.03098928532016012
55656,55657,55656,111313,45.116421937942505,0.030916995057551307
55856,55857,55856,111713,45.270655155181885,0.030845519423554735
56056,56057,56056,112113,45.41688513755798,0.030774492277794035
56256,56257,56256,112513,45.56502413749695,0.030703908366513225
56456,56457,56456,112913,45.71100187301636,0.030633762523957244
56657,56658,56657,113315,45.85827422142029,0.030563702185668725
56857,56858,56857,113715,46.0038640499115,0.03049441945341709
57057,57058,57057,114115,46.148810148239136,0.030425559777533903
57257,57258,57257,114515,46.31422209739685,0.030357118326168723
57457,57458,57457,114915,46.47625494003296,0.03028909034644813
57658,57659,57658,115317,46.64840817451477,0.030221134086234405
57858,57859,57858,115717,46.83412194252014,0.03015392110834263
58058,58059,58058,116117,46.98229789733887,0.030087107778424313
58258,58259,58258,116517,47.14052104949951,0.030020689643612493
58458,58459,58458,116917,47.285582065582275,0.029954662322081667
58659,58660,58659,117319,47.45509195327759,0.029888694261406282
58859,58860,58859,117719,47.6107861995697,0.02982343759855683
59059,59060,59059,118119,47.75490403175354,0.02975855899453978
59259,59260,59259,118519,47.901166915893555,0.029694054337697912
59459,59460,59459,118919,48.047029972076416,0.029629919580423218
59660,59661,59660,119321,48.20169496536255,0.02956583280639606
59860,59861,59860,119721,48.389853954315186,0.029502427755384367
60060,60061,60060,120121,48.54690909385681,0.029439380813448743
60260,60261,60260,120521,48.7493371963501,0.029376688176829046
60460,60461,60460,120921,48.91277813911438,0.02931434609963969
60661,60662,60661,121323,49.06389617919922,0.029252041782077156
60861,60862,60861,121723,49.210273027420044,0.029190391519037764
61061,61062,61061,122123,49.37461709976196,0.02912908089594321
61261,61262,61261,122523,49.520103931427,0.029068106387489193
61461,61462,61461,122923,49.665579080581665,0.029007464520781623
61662,61663,61662,123325,49.867257833480835,0.028946851132574117
61862,61863,61862,123725,50.023386001586914,0.028886865956128206
62062,62063,62062,124125,50.1683509349823,0.028827203290694058
62262,62263,62262,124525,50.31146717071533,0.028767859863347005
62462,62463,62462,124925,50.495718002319336,0.028708832448727063
62663,62664,62663,125327,50.65342116355896,0.02864982507595059
62863,62864,62863,125727,50.81220507621765,0.02859142173718802
63063,63064,63063,126127,50.960427045822144,0.028533324996223377
63263,63264,63263,126527,51.10419297218323,0.028475531809367304
63463,63464,63463,126927,51.27660393714905,0.028418039176188254
63664,63665,63664,127329,51.420865058898926,0.028360558906318195
63864,63865,63864,127729,51.56771802902222,0.028303660014377258
64064,64065,64064,128129,51.71280097961426,0.028247052912161407
64264,64265,64264,128529,51.858356952667236,0.028190734764629403
64464,64465,64464,128929,52.00304317474365,0.02813470277616253
64665,64666,64665,129331,52.14745807647705,0.028078676154383548
64865,64866,64865,129731,52.29981017112732,0.028023209647965723
65065,65066,65065,130131,52.44391894340515,0.027968021129900187
65265,65266,65265,130531,52.613439083099365,0.02791310795544317
65465,65466,65465,130931,52.76088809967041,0.02785846751584931
65666,65667,65666,131333,52.92721486091614,0.027803826060845374
65866,65867,65866,131733,53.098570108413696,0.027749724737346673
66066,66067,66066,132133,53.24498510360718,0.02769588851970521
66266,66267,66266,132533,53.389366149902344,0.02764231493708164
66466,66467,66466,132933,53.5340838432312,0.027589001551572824
66667,66668,66667,133335,53.68196415901184,0.02753568132337202
66867,66868,66867,133735,53.82524609565735,0.027482882418456027
67067,67068,67067,134135,53.97227907180786,0.0274303365772643
67267,67268,67267,134535,54.12544393539429,0.027378041488187697
67467,67468,67467,134935,54.2680242061615,0.027325994869808547
67668,67669,67668,135337,54.42033100128174,0.02727393608327075
67868,67869,67868,135737,54.56872606277466,0.027222380894687342
68068,68069,68068,136137,54.724679946899414,0.02717106749771543
68268,68269,68268,136537,54.87518811225891,0.027119993726812338
68468,68469,68468,136937,55.030369997024536,0.02706915744416197
68669,68670,68669,137339,55.233251094818115,0.027018304122564073
68869,68870,68869,137739,55.40829801559448,0.026967937672853978
69069,69070,69069,138139,55.55328011512756,0.026917802449511842
69269,69270,69269,138539,55.69691705703735,0.026867896421229432
69469,69470,69469,138939,55.879064083099365,0.026818217582206205
69670,69671,69670,139341,56.02959585189819,0.02676851724612232
69870,69871,69870,139741,56.17482900619507,0.026719287979562044
70070,70071,70070,140141,56.31904482841492,0.026670280024185245
70270,70271,70270,140541,56.46415400505066,0.026621491472260554
70470,70471,70470,140941,56.6119749546051,0.026572920439563243
70671,70672,70671,141343,56.75709390640259,0.026524323826871515
70871,70872,70871,141743,56.909610986709595,0.026476183336627983
71071,71072,71071,142143,57.053694009780884,0.026428254841232568
71271,71272,71271,142543,57.22221493721008,0.026380536546912005
71471,71472,71471,142943,57.370487213134766,0.026333026681591643
71672,71673,71672,143345,57.516215085983276,0.026285487494986652
71872,71873,71872,143745,57.660582065582275,0.026238390276976633
72072,72073,72072,144145,57.80519104003906,0.02619149629007485
72272,72273,72272,144545,57.94912910461426,0.026144803845767835
72472,72473,72472,144945,58.09306287765503,0.02609831127560433
72673,72674,72673,145347,58.23859405517578,0.026051785954460557
72873,72874,72873,145747,58.38152098655701,0.02600568918486195
73073,73074,73073,146147,58.527925968170166,0.025959787393368128
73273,73274,73273,146547,58.67115497589111,0.025914078988845155
73473,73474,73473,146947,58.81699514389038,0.02586856239873594
73674,73675,73674,147349,58.961143016815186,0.02582300991257253
73874,73875,73874,147749,59.105080127716064,0.025777873246323864
74074,74075,74074,148149,59.296574115753174,0.025732923777959413
74274,74275,74274,148549,59.463916063308716,0.025688160006570537
74474,74475,74474,148949,59.60796284675598,0.025643580448476134
74675,74676,74675,149351,59.753445863723755,0.02559896210961971
74875,74876,74875,149751,59.899775981903076,0.025554747497581246
75075,75076,75075,150151,60.04368996620178,0.025510712741510854
75275,75276,75275,150551,60.18608117103577,0.025466856424219003
75475,75476,75475,150951,60.33824396133423,0.02542317714451537
75676,75677,75676,151353,60.48305416107178,0.025379456437858338
75876,75877,75876,151753,60.62781119346619,0.025336127960596044
76076,76077,76076,152153,60.770721197128296,0.025292972404311383
76276,76277,76276,152553,60.93907594680786,0.025249988429606376
76476,76477,76476,152953,61.08324098587036,0.025207174711961728
76677,76678,76677,153355,61.23025107383728,0.025164317139971276
76877,76878,76877,153755,61.37714600563049,0.02512184085637671
77077,77078,77077,154155,61.536519050598145,0.02507953093708606
77277,77278,77277,154555,61.68795394897461,0.025037386115082563
77477,77478,77477,154955,61.83451294898987,0.024995405137204354
77678,77679,77678,155357,62.00006723403931,0.02495337807856421
77878,77879,77878,155757,62.14507603645325,0.024911721887739973
78078,78079,78078,156157,62.28817319869995,0.02487022585673279
78278,78279,78278,156557,62.4317991733551,0.02482888878596061
78478,78479,78478,156957,62.57485914230347,0.024787709488759215
78679,78680,78679,157359,62.72279095649719,0.024746482069218284
78879,78880,78879,157759,62.86543607711792,0.02470561558424707
79079,79080,79079,158159,63.00995111465454,0.0246649033828868
79279,79280,79279,158559,63.156569957733154,0.02462434432845971
79479,79480,79479,158959,63.30122089385986,0.024583937296346954
79680,79681,79680,159361,63.44505715370178,0.024543480270519773
79880,79881,79880,159761,63.58997416496277,0.024503374702898924
80080,80081,80080,160161,63.75097393989563,0.024463417849054953
80280,80281,80280,160561,63.89435911178589,0.024423608631058615
80480,80481,80480,160961,64.05810403823853,0.024383945982250764
80681,80682,80681,161363,64.2038049697876,0.024344231625261305
80881,80882,80881,161763,64.3485472202301,0.024304859678926337
81081,81082,81081,162163,64.49523997306824,0.02426563116279573
81281,81282,81281,162563,64.68703103065491,0.02422654505387042
81481,81482,81481,162963,64.86237001419067,0.024187600339695938
81682,81683,81682,163365,65.0089659690857,0.024148602347684355
81882,81883,81882,163765,65.15400505065918,0.024109938121669453
82082,82083,82082,164165,65.32472395896912,0.024071412310059215
82282,82283,82282,164565,65.47256398200989,0.024033023941270815
82482,82483,82482,164965,65.618155002594,0.02399477205359773
82683,82684,82683,165367,65.77394104003906,0.023956465452220882
82883,82884,82883,165767,65.95595407485962,0.02391848435111394
83083,83084,83083,166167,66.09992599487305,0.023880636899360104
83283,83284,83283,166567,66.24738788604736,0.023842922173554222
83483,83484,83483,166967,66.39188885688782,0.023805339259551344
83684,83685,83684,167369,66.5388810634613,0.02376770031970814
83884,83885,83884,167769,66.6840169429779,0.023730378971149334
84084,84085,84084,168169,66.83482503890991,0.02369318674194137
84284,84285,84284,168569,66.97942209243774,0.023656122753867637
84484,84485,84484,168969,67.12439393997192,0.02361918613740254
84685,84686,84685,169371,67.27791118621826,0.023582192297496748
84885,84886,84885,169771,67.48792600631714,0.02354550847605718
85085,85086,85085,170171,67.64093494415283,0.023508949464517127
85285,85286,85285,170571,67.79163002967834,0.02347251442708628
85485,85486,85485,170971,67.94395303726196,0.023436202536138387
85686,85687,85686,171373,68.1066780090332,0.023399832330270882
85886,85887,85886,171773,68.25006794929504,0.023363764887116164
86086,86087,86086,172173,68.39575505256653,0.023327818151553645
86286,86287,86286,172573,68.57274389266968,0.023291991327662267
86486,86487,86486,172973,68.71927881240845,0.023256283627197154
86687,86688,86687,173375,68.86592316627502,0.023220516618742672
86887,86888,86887,173775,69.0448808670044,0.02318504541655343
87087,87088,87087,174175,69.19160413742065,0.023149691014377808
87287,87288,87287,174575,69.3385169506073,0.02311445265379425
87487,87488,87487,174975,69.48255324363708,0.023079329583604948
87688,87689,87688,175377,69.63171696662903,0.023044146303687254
87888,87889,87888,175777,69.81081509590149,0.023009252156363423
88088,88089,88088,176177,69.9568829536438,0.02297447108469143
88288,88289,88288,176577,70.10617399215698,0.022939802365550592
88488,88489,88488,176977,70.28427815437317,0.02290524528262353
88689,88690,88689,177379,70.46723508834839,0.022870627173054606
88889,88890,88889,177779,70.61145496368408,0.022836291789779976
89089,89090,89089,178179,70.7601969242096,0.022802065930324977
89289,89290,89289,178579,70.94643521308899,0.022767948904826824
89489,89490,89489,178979,71.09942507743835,0.022733940029835305
89690,89691,89690,179381,71.24540495872498,0.022699869390128184
89890,89891,89890,179781,71.38959908485413,0.022666075323415778
90090,90091,90090,180181,71.53361701965332,0.02263238739128656
90290,90291,90290,180581,71.68002510070801,0.022598804935235167
90490,90491,90490,180981,71.8209958076477,0.02256532730280536
90691,90692,90691,181383,71.97346997261047,0.02253178724091115
90891,90892,90891,181783,72.11741709709167,0.02249851783828896
91091,91092,91091,182183,72.33427786827087,0.022465351334364565
91291,91292,91291,182583,72.48896384239197,0.022432287100220567
91491,91492,91491,182983,72.63413906097412,0.022399324512650004
91692,91693,91692,183385,72.77975821495056,0.022366298899103878
91892,91893,91892,183785,72.94000697135925,0.022333538258133594
92092,92093,92092,184185,73.08689403533936,0.022300877424714302
92292,92293,92292,184585,73.26979613304138,0.022268315797867092
92492,92493,92492,184985,73.41590404510498,0.02223585278200714
92693,92694,92693,185387,73.56088304519653,0.022203326207200454
92893,92894,92893,185787,73.70901799201965,0.02217105913355348
93093,93094,93093,186187,73.8532440662384,0.022138888913017123
93293,93294,93293,186587,73.9967110157013,0.02210681497101136
93493,93494,93493,186987,74.14053416252136,0.022074836738055006
93694,93695,93694,187389,74.33741021156311,0.022042794472377135
93894,93895,93894,187789,74.63045310974121,0.02201100644071868
94094,94095,94094,188189,74.9087188243866,0.021979312436937914
94294,94295,94294,188589,75.20732021331787,0.021947711911415337
94494,94495,94494,188989,75.44865012168884,0.021916204319354645
94695,94696,94695,189391,75.66354990005493,0.02188463227597407
94895,94896,94895,189791,75.85635805130005,0.021853309393429936
95095,95096,95095,190191,76.00604605674744,0.021822077835729637
95295,95296,95295,190591,76.15144920349121,0.021790937076869497
95495,95496,95495,190991,76.32559490203857,0.021759886595411046
95696,95697,95696,191393,76.549880027771,0.02172877129548686
95896,95897,95896,191793,76.73746705055237,0.021697900267488288
96096,96097,96096,192193,77.00180196762085,0.02166711797694334
96296,96297,96296,192593,77.23951387405396,0.021636423920205743
96496,96497,96496,192993,77.43079805374146,0.021605817597952125
96697,96698,96697,193395,77.66598606109619,0.021575146138085165
96897,96898,96897,193795,77.93670701980591,0.021544714236408004
97097,97098,97097,194195,78.19677805900574,0.021514368594300223
97297,97298,97297,194595,78.36417317390442,0.02148410872929325
97497,97498,97497,194995,78.54626417160034,0.02145393416301556
97698,97699,97698,195397,78.7552490234375,0.021423694184768718
97898,97899,97898,195797,78.98840498924255,0.021393689217598464
98098,98099,98098,196197,79.13775396347046,0.021363768135867073
98298,98299,98298,196597,79.30823516845703,0.021333930477178447
98498,98499,98498,196997,79.48175382614136,0.021304175783020872
98699,98700,98699,197399,79.658362865448,0.02127435544435141
98899,98900,98899,197799,80.01540303230286,0.021244765728221073
99099,99100,99099,198199,80.32066202163696,0.021215257621758108
99299,99300,99299,198599,80.61465406417847,0.02118583068160165
99499,99500,99499,198999,81.12660098075867,0.0211564844680754
99700,99701,99700,199401,81.3901309967041,0.021127072416536986
99900,99901,99900,199801,81.81817698478699,0.021097886749999017
100100,100101,100100,200201,82.06132197380066,0.021068780510652408
100300,100301,100300,200601,82.37980103492737,0.021039753273197036
100501,100502,100501,201003,82.71208190917969,0.021010660069271752
100701,100702,100701,201403,82.8975019454956,0.02098178996341439
100901,100902,100901,201803,83.06662893295288,0.020952997602320545
101101,101102,101101,202203,83.23614120483398,0.02092428257448031
101301,101302,101301,202603,83.42758798599243,0.02089564447173891
101502,101503,101502,203005,83.66565895080566,0.020866940272931584
101702,101703,101702,203405,84.14139914512634,0.020838455188762917
101902,101903,101902,203805,84.50460815429688,0.020810045823034595
102102,102103,102102,204205,84.81919598579407,0.020781711780688713
102302,102303,102302,204605,85.1617579460144,0.02075345266985473
102503,102504,102503,205007,85.47239303588867,0.020725127365616724
102703,102704,102703,205407,85.7914400100708,0.02069701732460451
102903,102904,102903,205807,86.01125192642212,0.020668981056389424
103103,103104,103103,206207,86.30404615402222,0.02064101818154518
103303,103304,103303,206607,86.49008417129517,0.020613128323674873
103504,103505,103504,207009,86.6409637928009,0.02058517220520253
103704,103705,103704,207409,86.79329705238342,0.020557427624493984
103904,103905,103904,207809,87.09816002845764,0.02052975494761059
104104,104105,104104,208209,87.56422090530396,0.020502153809985553
104304,104305,104304,208609,87.85783004760742,0.020474623849932278
104505,104506,104505,209011,88.19082903862,0.020447027590242448
104705,104706,104705,209411,88.50776100158691,0.02041963926307493
104905,104906,104905,209811,88.82140398025513,0.020392321043656736
105105,105106,105105,210211,89.19775009155273,0.020365072581552512
105305,105306,105305,210611,89.75777697563171,0.020337893529066852
105506,105507,105506,211013,90.24157404899597,0.020310648164226914
105706,105707,105706,211413,90.62009716033936,0.02028360724147293
105906,105907,105906,211813,90.87632703781128,0.020256634699730023
106106,106107,106106,212213,91.10560393333435,0.020229730202008103
106306,106307,106306,212613,91.5157859325409,0.020202893413924592
106507,106508,106507,213015,91.95376420021057,0.02017599032536053
106707,106708,106707,213415,92.47454595565796,0.020149288298128884
106907,106908,106907,213815,92.7461051940918,0.020122652991151957
107107,107108,107107,214215,93.06649708747864,0.020096084080237445
107307,107308,107307,214615,93.25553894042969,0.02006958124367558
107508,107509,107508,215017,93.4267930984497,0.020043012141484632
107708,107709,107708,215417,93.6297459602356,0.02001664082470869
107908,107909,107908,215817,93.81002807617188,0.019990334630246288
108108,108109,108108,216217,94.0137369632721,0.019964093246091698
108308,108309,108308,216617,94.2135272026062,0.01993791636260392
108509,108510,108509,217019,94.41410422325134,0.019911673269805932
108709,108710,108709,217419,94.60288381576538,0.01988562478675329
108909,108910,108909,217819,94.78238701820374,0.019859639887898215
109109,109110,109109,218219,94.95816802978516,0.019833718272844497
109309,109310,109309,218619,95.13093209266663,0.019807859643449135
109510,109511,109510,219021,95.31779217720032,0.019781934881116445
109710,109711,109710,219421,95.50830912590027,0.019756201648760182
109910,109911,109910,219821,95.6895260810852,0.019730530519486488
110110,110111,110110,220221,95.87189197540283,0.019704921203963034
110310,110311,110310,220621,96.06289482116699,0.01967937341500557
110511,110512,110511,221023,96.25576090812683,0.01965375958821328
110711,110712,110711,221423,96.43538212776184,0.019628334303410103
110911,110912,110911,221823,96.65899014472961,0.01960296969490564
111111,111112,111111,222223,96.82693409919739,0.019577665483915933
111311,111312,111311,222623,97.01247906684875,0.019552421393705496
111512,111513,111512,223025,97.19070792198181,0.01952711137825143
111712,111713,111712,223425,97.37936210632324,0.019501987004674468
111912,111913,111912,223825,97.56143403053284,0.019476921932419247
112112,112113,112112,224225,97.76227903366089,0.019451915892762284
112312,112313,112312,224625,97.95990204811096,0.019426968618934372
112513,112514,112513,225027,98.13153791427612,0.019401955548779173
112713,112714,112713,225427,98.30627799034119,0.01937712530455918
112913,112914,112913,225827,98.47410416603088,0.019352353036102266
113113,113114,113113,226227,98.65419101715088,0.019327638484284045
113313,113314,113313,226627,98.8318841457367,0.019302981391844724
113514,113515,113514,227029,99.01250004768372,0.019278258647228156
113714,113715,113714,227429,99.18897199630737,0.01925371599325822
113914,113915,113914,227829,99.37077903747559,0.019229230036650467
114114,114115,114114,228229,99.61290717124939,0.01920480052744221
114314,114315,114314,228629,99.87265491485596,0.019180427217451
114515,114516,114515,229031,100.23680210113525,0.019155988413642223
114715,114716,114715,229431,100.47864818572998,0.01913172704250599
114915,114916,114915,229831,100.67521595954895,0.01910752113534766
115115,115116,115115,230231,100.88848114013672,0.01908337045095245
115315,115316,115315,230631,101.095134973526,0.019059274749805576
115516,115517,115516,231033,101.2664909362793,0.019035113726448963
115716,115717,115716,231433,101.43588900566101,0.019011127551933474
115916,115917,115916,231833,101.61319208145142,0.0189871956510003
116116,116117,116116,232233,101.79511094093323,0.01896331779078996
116316,116317,116316,232633,101.96328806877136,0.018939493740067266
116517,116518,116517,233035,102.1286768913269,0.01891560455108807
116717,116718,116717,233435,102.31941604614258,0.018891887698247435
116917,116918,116917,233835,102.49638414382935,0.01886822396965953
117117,117118,117117,234235,102.67105317115784,0.01884461314044846
117317,117318,117317,234635,102.90744400024414,0.018821054987290517
117518,117519,117518,235037,103.16175603866577,0.018797431891326603
117718,117719,117718,235437,103.37848401069641,0.018773978687062175
117918,117919,117918,235837,103.60213088989258,0.018750577496964436
118118,118119,118118,236237,103.77558207511902,0.018727228103788053
118318,118319,118318,236637,103.97674798965454,0.018703930291771757
118519,118520,118519,237039,104.17846989631653,0.018680567743100486
118719,118720,118719,237439,104.34484004974365,0.0186573727072281
118919,118920,118919,237839,104.54178786277771,0.01863422861295066
119119,119120,119119,238239,104.70593309402466,0.01861113525031887
119319,119320,119319,238639,104.85725283622742,0.018588092410802587
119520,119521,119520,239041,105.02472615242004,0.018564985050733673
119720,119721,119720,239441,105.19577193260193,0.01854204288750886
119920,119921,119920,239841,105.36012196540833,0.01851915062918099
120120,120121,120120,240241,105.51761102676392,0.01849630807277906
120320,120321,120320,240641,105.66812491416931,0.018473515016689774
120521,120522,120521,241043,105.81609296798706,0.018450657665397007
120721,120722,120721,241443,105.9718668460846,0.018427963255472003
120921,120922,120921,241843,106.12227988243103,0.018405317748062047
121121,121122,121121,242243,106.27423906326294,0.018382720946873002
121321,121322,121321,242643,106.4192111492157,0.01836017265690967
121522,121523,121522,243045,106.58080220222473,0.018337560305676757
121722,121723,121722,243445,106.73410320281982,0.01831510869846413
121922,121923,121922,243845,106.88154911994934,0.01829270502422189
122122,122123,122122,244245,107.03662896156311,0.018270349093046007
122322,122323,122322,244645,107.18932604789734,0.01824804071627606
122523,122524,122523,245047,107.34285593032837,0.018225668520131973
122723,122724,122723,245447,107.50798010826111,0.018203454926551815
122923,122924,122923,245847,107.65634894371033,0.018181288327829507
123123,123124,123123,246247,107.80871510505676,0.018159168540178933
123323,123324,123323,246647,107.95928907394409,0.01813709538100483
123524,123525,123524,247049,108.1122510433197,0.018114958651727256
123724,123725,123724,247449,108.26519203186035,0.018092978437316373
123924,123925,123924,247849,108.41017293930054,0.018071044309747725
124124,124125,124124,248249,108.56620121002197,0.01804915609109422
124324,124325,124324,248649,108.71780800819397,0.018027313604569765
124525,124526,124525,249051,108.86403894424438,0.018005407804036002
124725,124726,124725,249451,109.01729416847229,0.017983656482398552
124925,124926,124925,249851,109.17241716384888,0.017961950368415185
125125,125126,125125,250251,109.3513731956482,0.017940289289771996
125325,125326,125325,250651,109.54384016990662,0.0179186730752483
125526,125527,125526,251053,109.73314094543457,0.017896993809113654
125726,125727,125726,251453,109.89602518081665,0.017875467035694384
125926,125927,125926,251853,110.05623507499695,0.01785398461836148
126126,126127,126126,252253,110.21472811698914,0.017832546390180205
126326,126327,126326,252653,110.36692786216736,0.01781115218526362
126527,126528,126527,253055,110.52819681167603,0.017789695196949878
126727,126728,126727,253455,110.69402289390564,0.017768388763111733
126927,126928,126927,253855,110.85124516487122,0.01774712586026452
127127,127128,127127,254255,111.01627016067505,0.017725906326630136
127327,127328,127327,254655,111.17286515235901,0.017704730001434802
127528,127529,127528,255057,111.32887983322144,0.01768349116641106
127728,127729,127728,255457,111.48809599876404,0.017662400993801224
127928,127929,127928,255857,111.67101216316223,0.017641353552466602
128128,128129,128128,256257,111.84167003631592,0.017620348685573644
128328,128329,128328,256657,111.99901223182678,0.017599386237252088
128529,128530,128529,257059,112.15100121498108,0.017578361557592338
128729,128730,128729,257459,112.2999210357666,0.017557483692780127
128929,128930,128929,257859,112.45570993423462,0.017536647783867064
129129,129130,129129,258259,112.62201714515686,0.017515853678762478
129329,129330,129329,258659,112.78935194015503,0.017495101226299718
129530,129531,129530,259061,112.9758632183075,0.01747428682550234
129730,129731,129730,259461,113.1497311592102,0.017453617434874686
129930,129931,129930,259861,113.31706309318542,0.017432989248119635
130130,130131,130130,260261,113.50125503540039,0.017412402117697078
130330,130331,130330,260661,113.65484285354614,0.017391855896953967
130531,130532,130531,261063,113.81499695777893,0.01737124801500831
130731,130732,130731,261463,113.99158191680908,0.017350783379909175
130931,130932,130931,261863,114.1657350063324,0.017330359219062202
131131,131132,131131,262263,114.71819496154785,0.017309975389295077
131331,131332,131331,262663,115.2302758693695,0.01728963174828689
131532,131533,131532,263065,115.5592520236969,0.017269226736975007
131732,131733,131732,263465,115.87081098556519,0.01724896324907479
131932,131933,131932,263865,116.1800148487091,0.017228739527314234
132132,132133,132132,264265,116.39066815376282,0.017208555432714115
132332,132333,132332,264665,116.65201306343079,0.01718841082711301
132533,132534,132533,265067,116.8627541065216,0.01716820514553219
132733,132734,132733,265467,117.05178189277649,0.017148139302416307
132933,132934,132933,265867,117.24356889724731,0.017128112537978787
133133,133134,133133,266267,117.4433491230011,0.017108124717267505
133333,133334,133333,266667,117.61293196678162,0.017088175706115843
133534,133535,133534,267069,117.79211807250977,0.017068165916412272
133734,133735,133734,267469,118.02055311203003,0.017048294317375944
133934,133935,133934,267869,118.30064010620117,0.01702846112939173
134134,134135,134134,268269,118.610524892807,0.01700866622137614
134334,134335,134334,268669,118.8448588848114,0.016988909463000308
134535,134536,134535,269071,119.13627195358276,0.01696909222630119
134735,134736,134735,269471,119.58361411094666,0.016949411568340487
134935,134936,134935,269871,119.84097599983215,0.016929768672862312
135135,135136,135135,270271,120.04284024238586,0.01691016341250063
135335,135336,135335,270671,120.25642013549805,0.01689059566061461
135536,135537,135536,271073,120.43568897247314,0.01687096773314944
135736,135737,135736,271473,120.62568807601929,0.016851474807138087
135936,135937,135936,271873,120.77935004234314,0.016832019013353957
136136,136137,136136,272273,120.96827101707458,0.01681260022800411
136336,136337,136336,272673,121.12147521972656,0.01679321832799294
136537,136538,136537,273075,121.28461003303528,0.01677377655739345
136737,136738,136737,273475,121.48669505119324,0.01675446824443602
136937,136938,136937,273875,121.70843505859375,0.01673519645105615
137137,137138,137137,274275,121.86726999282837,0.016715961056896576
137337,137338,137337,274675,122.07329487800598,0.01669676194227066
137538,137539,137538,275077,122.34273600578308,0.016677503264040557
137738,137739,137738,275477,122.72558689117432,0.016658376531992113
137938,137939,137938,275877,123.1265161037445,0.016639285723801425
138138,138139,138138,276277,123.38740611076355,0.016620230722415596
138338,138339,138338,276677,123.83141803741455,0.016601211411426512
138539,138540,138539,277079,124.49972200393677,0.016582132845572133
138739,138740,138739,277479,124.88034200668335,0.016563184745717146
138939,138940,138939,277879,125.22710514068604,0.016544271990284538
139139,139140,139139,278279,125.71898698806763,0.016525394465400304
139339,139340,139339,278679,126.23578000068665,0.01650655205781082
139540,139541,139540,279081,126.5786828994751,0.016487650705624704
139740,139741,139740,279481,126.86967992782593,0.01646887836950588
139940,139941,139940,279881,127.22705316543579,0.016450140814042353
140140,140141,140140,280281,127.53091502189636,0.01643143792841908
140340,140341,140340,280681,127.75574827194214,0.016412769602418446
140541,140542,140541,281083,127.92901611328125,0.016394042643407807
140741,140742,140741,281483,128.1114649772644,0.016375443279798008
140941,140942,140941,281883,128.27822494506836,0.01635687814815601
141141,141142,141141,282283,128.4381959438324,0.016338347140611515
141341,141342,141341,282683,128.61757111549377,0.016319850149869385
141542,141543,141542,283085,128.80689311027527,0.016301294838822408
141742,141743,141742,283485,128.98598790168762,0.016282865730831965
141942,141943,141942,283885,129.1663420200348,0.01626447032063926
142142,142143,142142,284285,129.49136114120483,0.016246108503209424
142342,142343,142342,284685,129.82109117507935,0.01622778017406136
142543,142544,142543,285087,130.1201310157776,0.01620939383824413
142743,142744,142743,285487,130.4587049484253,0.016191132340557263
142943,142944,142943,285887,130.70747184753418,0.016172904020478093
143143,143144,143143,286287,130.9761140346527,0.016154708775702725
143343,143344,143343,286687,131.17097806930542,0.0161365465044607
143544,143545,143544,287089,131.365327835083,0.01611832654093865
143744,143745,143744,287489,131.65677189826965,0.01610023007717204
143944,143945,143944,287889,131.90359711647034,0.016082166284289594
144144,144145,144144,288289,132.22609305381775,0.016064135062618397
144344,144345,144344,288689,132.51507306098938,0.016046136312999705
144545,144546,144545,289091,132.7636160850525,0.016028080186077015
144745,144746,144745,289491,133.0052990913391,0.016010146246254867
144945,144946,144945,289891,133.1956820487976,0.015992244483568716
145145,145146,145145,290291,133.35949110984802,0.015974374800881243
145345,145346,145345,290691,133.54571390151978,0.015956537101550528
145546,145547,145546,291093,133.7086570262909,0.01593864234032183
145746,145747,145746,291493,133.86085510253906,0.015920868478461383
145946,145947,145946,291893,134.02755522727966,0.015903126312494586
146146,146147,146146,292293,134.19387102127075,0.01588541574772831
146346,146347,146346,292693,134.34757781028748,0.01586773668994704
146547,146548,146547,293095,134.51984906196594,0.015850000885955833
146747,146748,146747,293495,134.76410508155823,0.015832384717758295
146947,146948,146947,293895,134.9617109298706,0.015814799776268592
147147,147148,147147,294295,135.14457297325134,0.015797245969150258
147347,147348,147347,294695,135.31169414520264,0.015779723204527703
147548,147549,147548,295097,135.46246099472046,0.015762144009526545
147748,147749,147748,295497,135.6378300189972,0.015744683210167636
147948,147949,147948,295897,135.81058597564697,0.015727253179957493
148148,148149,148148,296297,136.14891815185547,0.015709853828832755
148348,148349,148348,296697,136.29900813102722,0.015692485067174616
148549,148550,148549,297099,136.50564312934875,0.01567506019098154
148749,148750,148749,297499,136.72690796852112,0.01565775249299771
148949,148950,148949,297899,136.88738799095154,0.01564047511781886
149149,149150,149149,298299,137.04393100738525,0.015623227977574705
149349,149350,149349,298699,137.21404504776,0.015606010984823967
149550,149551,149550,299101,137.5362000465393,0.015588738193271088
149750,149751,149750,299501,137.88937187194824,0.01557158138453604
149950,149951,149950,299901,138.20247888565063,0.015554454463083543
150150,150151,150150,300301,138.47727394104004,0.01553735734315997
150350,150351,150350,300701,138.68938183784485,0.015520289939425365
150551,150552,150551,301103,138.84492015838623,0.015503167052395052
150751,150752,150751,301503,138.99984407424927,0.01548615897418229
150951,150952,150951,301903,139.15181708335876,0.015469180358174218
151151,151152,151151,302303,139.46476006507874,0.015452231120660161
151351,151352,151351,302703,139.6172649860382,0.01543531117832888
151552,151553,151552,303105,139.78192496299744,0.015418336067872964
151752,151753,151752,303505,139.93382096290588,0.015401474613000838
151952,151953,151952,303905,140.17891907691956,0.01538464220533878
152152,152153,152152,304305,140.40819215774536,0.015367838763148707
152352,152353,152352,304705,140.58041501045227,0.015351064205078464
152553,152554,152553,305107,140.74355006217957,0.015334234793617153
152753,152754,152753,305507,140.9064269065857,0.015317517904671849
152953,152954,152953,305907,141.06758999824524,0.015300829657679208
153153,153154,153153,306307,141.22729206085205,0.01528416997280646
153353,153354,153353,306707,141.43145203590393,0.015267538770593631
153554,153555,153554,307109,141.68973183631897,0.01525085302918961
153754,153755,153754,307509,141.8783519268036,0.015234278696822683
153954,153955,153954,307909,142.04777002334595,0.015217732610556657
154154,154155,154154,308309,142.21890211105347,0.015201214692399627
154354,154355,154354,308709,142.38844108581543,0.015184724864719704
154555,154556,154555,309111,142.54863381385803,0.015168180811424514
154755,154756,154755,309511,142.70023608207703,0.01515174707272128
154955,154956,154955,309911,142.91387009620667,0.015135341193355243
155155,155156,155155,310311,143.12122297286987,0.015118963097113238
155355,155356,155355,310711,143.2969090938568,0.015102612708130257
155556,155557,155556,311113,143.4691789150238,0.015086208406399376
155756,155757,155756,311513,143.6172239780426,0.015069913343315196
155956,155957,155956,311913,143.7619960308075,0.015053645761587743
156156,156157,156156,312313,143.90876126289368,0.015037405586723394
156356,156357,156356,312713,144.0804841518402,0.015021192744564978
156557,156558,156557,313115,144.28727102279663,0.015004926301738056
156757,156758,156757,313515,144.4692840576172,0.01498876803959884
156957,156958,156957,313915,144.61916399002075,0.014972636889327111
157157,157158,157157,314315,144.76444697380066,0.014956532778091695
157357,157358,157357,314715,144.91650319099426,0.01494045563338711
157558,157559,157558,315117,145.08203196525574,0.014924325199230664
157758,157759,157758,315517,145.23880410194397,0.014908301905294985
157958,157959,157958,315917,145.4051170349121,0.014892305361948495
158158,158159,158158,316317,145.5800530910492,0.014876335497968062
158358,158359,158358,316717,145.74273419380188,0.01486039224244552
158559,158560,158559,317119,145.9043550491333,0.014844396007755426
158759,158760,158759,317519,146.25039911270142,0.014828505889835244
158959,158960,158959,317919,146.4655740261078,0.014812642169168208
159159,159160,159159,318319,146.66415214538574,0.014796804776086773
159359,159360,159359,318719,146.8201081752777,0.014780993641228092
159560,159561,159560,319121,146.9780809879303,0.014765129836488408
159760,159761,159760,319521,147.15531706809998,0.014749371141625759
159960,159961,159960,319921,147.41854691505432,0.014733638498364414
160160,160161,160160,320321,147.58690404891968,0.014717931838542293
160360,160361,160360,320721,147.8507149219513,0.014702251094292056
160561,160562,160561,321123,148.14994096755981,0.014686517988388263
160761,160762,160761,321523,148.53721499443054,0.014670889001585228
160961,160962,160961,321923,148.79797315597534,0.01465528572816858
161161,161162,161161,322323,149.01392221450806,0.014639708101433143
161361,161362,161361,322723,149.1786229610443,0.014624156054959366
161562,161563,161562,323125,149.34968090057373,0.014608551953943116
161762,161763,161762,323525,149.68451523780823,0.014593050996943122
161962,161963,161962,323925,149.84952998161316,0.014577575422313457
162162,162163,162162,324325,150.012864112854,0.014562125164759954
162362,162363,162362,324725,150.16230511665344,0.01454670015926456
162563,162564,162563,325127,150.38920903205872,0.014531223405168
162763,162764,162763,325527,150.62011694908142,0.014515848835284985
162963,162964,162963,325927,150.8484091758728,0.014500499323727394
163163,163164,163163,326327,151.03194904327393,0.014485174806567074
163363,163364,163363,326727,151.23158407211304,0.014469875220143699
163564,163565,163564,327129,151.4066240787506,0.014454524189840648
163764,163765,163764,327529,151.66316199302673,0.01443927439883565
163964,163965,163964,327929,151.8793239593506,0.01442404934886278
164164,164165,164164,328329,152.04515314102173,0.014408848977317415
164364,164365,164364,328729,152.2441601753235,0.014393673221854256
164565,164566,164565,329131,152.43265104293823,0.014378446325966611
164765,164766,164765,329531,152.64070105552673,0.014363319738968011
164965,164966,164965,329931,152.79958200454712,0.014348217582249327
165165,165166,165165,330331,152.95859909057617,0.014333139794488374
165365,165366,165365,330731,153.11702704429626,0.01431808631461438
165566,165567,165566,331133,153.36847496032715,0.014302981996461298
165766,165767,165766,331533,153.7010498046875,0.01428797707092742
165966,165967,165966,331933,154.18773007392883,0.014272996271260266
166166,166167,166166,332333,154.35868906974792,0.014258039537380442
166366,166367,166366,332733,154.69493889808655,0.01424310680945244
166567,166568,166567,333135,154.96888303756714,0.01422812354404065
166767,166768,166767,333535,155.18236017227173,0.014213238768763469
166967,166968,166967,333935,155.56017112731934,0.014198377821084076
167167,167168,167167,334335,155.75552701950073,0.014183540642128204
167367,167368,167367,334735,155.92896604537964,0.014168727173257845
167568,167569,167568,335137,156.20543384552002,0.014153863466311117
167768,167769,167768,335537,156.46810293197632,0.014139097360458012
167968,167969,167968,335937,156.62174105644226,0.014124354789891257
168168,168169,168168,336337,156.86052203178406,0.014109635696905064
168368,168369,168368,336737,157.14733123779297,0.014094940024022957
168569,168570,168569,337139,157.42311310768127,0.014080194411049447
168769,168770,168769,337539,157.84897994995117,0.014065545523242238
168969,168970,168969,337939,158.2048032283783,0.014050919884187666
169169,169170,169169,338339,158.6185359954834,0.01403631743731344
169369,169370,169369,338739,158.9317979812622,0.014021738126269712
169570,169571,169570,339141,159.16430020332336,0.014007109171664653
169770,169771,169770,339541,159.3924059867859,0.01399257607909387
169970,169971,169970,339941,159.56525111198425,0.013978065954346936
170170,170171,170170,340341,159.71751403808594,0.01396357874195131
170370,170371,170370,340741,160.04846906661987,0.013949114386650249
170571,170572,170571,341143,160.39174509048462,0.013934600682833198
170771,170772,170771,341543,160.8002769947052,0.013920181990406436
170971,170972,170971,341943,161.1066062450409,0.013905785990313307
171171,171172,171171,342343,161.28786301612854,0.013891412628148622
171371,171372,171371,342743,161.44521713256836,0.013877061849716453
171572,171573,171572,343145,161.81622314453125,0.013862662016301429
171772,171773,171772,343545,161.9832468032837,0.013848356355823693
171972,171973,171972,343945,162.15621709823608,0.013834073117468116
172172,172173,172172,344345,162.3104109764099,0.013819812247865385
172372,172373,172372,344745,162.45834302902222,0.013805573693849686
172573,172574,172573,345147,162.60726499557495,0.013791286376846467
172773,172774,172773,345547,162.79657912254333,0.013777092406231706
172973,172974,172973,345947,163.13076210021973,0.013762920592652243
173173,173174,173173,346347,163.48642587661743,0.013748770883744857
173373,173374,173373,346747,163.6594569683075,0.013734643227343675
173574,173575,173574,347149,163.83354306221008,0.013720467098389266
173774,173775,173774,347549,164.02900004386902,0.013706383500901462
173974,173975,173974,347949,164.19817185401917,0.013692321800338587
174174,174175,174174,348349,164.37744808197021,0.01367828194531447
174374,174375,174374,348749,164.54338693618774,0.013664263884634634
174575,174576,174575,349151,164.7053210735321,0.013650197640253452
174775,174776,174775,349551,164.86615085601807,0.013636223123776088
174975,174976,174975,349951,165.03352189064026,0.01362227024894711
175175,175176,175175,350351,165.18846917152405,0.013608338965329427
175375,175376,175375,350751,165.35198283195496,0.013594429222672419
175576,175577,175576,351153,165.50966095924377,0.013580471583563876
175776,175777,175776,351553,165.65728998184204,0.013566604879896318
175976,175977,175976,351953,165.85201692581177,0.013552759567297087
176176,176177,176176,352353,166.03105998039246,0.013538935596251295
176376,176377,176376,352753,166.17734503746033,0.01352513291742541
176577,176578,176577,353155,166.32454895973206,0.01351128262777808
176777,176778,176777,353555,166.5005021095276,0.01349752249195837
176977,176978,176977,353955,166.65226912498474,0.013483783501190873
177177,177178,177177,354355,166.99047899246216,0.013470065606857288
177377,177378,177377,354755,167.26576805114746,0.01345636876051547
177578,177579,177578,355157,167.43769192695618,0.013442624587346162
177778,177779,177778,355557,167.6031711101532,0.01342896979699826
177978,177979,177978,355957,167.76939392089844,0.013415335910123028
178178,178179,178178,356357,167.95436692237854,0.01340172287897384
178378,178379,178378,356757,168.11885809898376,0.013388130655975128
178579,178580,178579,357159,168.28612804412842,0.013374491388492452
178779,178780,178779,357559,168.4530692100525,0.013360940743197557
178979,178980,178979,357959,168.63531303405762,0.013347410764109634
179179,179180,179179,358359,168.85060000419617,0.01333390140432948
179379,179380,179379,358759,169.2741892337799,0.01332041261712447
179580,179581,179580,359161,169.63185787200928,0.01330687706611521
179780,179781,179780,359561,169.94374108314514,0.013293429386805838
179980,179981,179980,359961,170.2794508934021,0.01328000214063301
180180,180181,180180,360361,170.44016098976135,0.013266595281521893
180380,180381,180380,360761,170.65238094329834,0.01325320876355983
180581,180582,180581,361163,170.9646019935608,0.01323977576079786
180781,180782,180781,361563,171.24908804893494,0.013226429889173861
180981,180982,180981,361963,171.53779196739197,0.013213104221697108
181181,181182,181181,362363,171.8571000099182,0.01319979871309497
181381,181382,181381,362763,172.1307249069214,0.01318651331825238
181582,181583,181582,363165,172.40933108329773,0.013173181715928505
181782,181783,181782,363565,172.6954231262207,0.013159936513894015
181982,181983,181982,363965,172.99497199058533,0.013146711290988617
182182,182183,182182,364365,173.2867729663849,0.013133506002720226
182382,182383,182382,364765,173.56283497810364,0.013120320604750199
182583,182584,182583,365167,173.86382222175598,0.013107089274922568
182783,182784,182783,365567,174.12664914131165,0.01309394362404301
182983,182984,182983,365967,174.4371621608734,0.013080817731139309
183183,183184,183183,366367,174.70014691352844,0.013067711552479296
183383,183384,183383,366767,174.95543313026428,0.013054625044480014
183584,183585,183584,367169,175.24494695663452,0.013041492878544045
183784,183785,183784,367569,175.51670718193054,0.0130284456795225
183984,183985,183984,367969,175.81583380699158,0.013015418021086265
184184,184185,184184,368369,176.07255101203918,0.013002409860242843
184384,184385,184384,368769,176.32972502708435,0.012989421154145319
184585,184586,184585,369171,176.59699892997742,0.012976387062322368
184785,184786,184785,369571,176.8660809993744,0.012963437234494451
184985,184986,184985,369971,177.13706493377686,0.012950506733525043
185185,185186,185185,370371,177.4492380619049,0.012937595517142115
185385,185386,185385,370771,177.73463821411133,0.012924703543215408
185586,185587,185586,371173,177.98808598518372,0.012911766454059235
185786,185787,185786,371573,178.251060962677,0.012898912934905625
185986,185987,185986,371973,178.51727318763733,0.012886078532452105
186186,186187,186186,372373,178.78109908103943,0.012873263205128554
186386,186387,186386,372773,179.08431696891785,0.012860466911502982
186587,186588,186587,373175,179.34046387672424,0.012847625771423796
186787,186788,186787,373575,179.61219310760498,0.012834867516099666
186987,186988,186987,373975,179.871906042099,0.012822128170793754
187187,187188,187187,374375,180.14872908592224,0.012809407694619851
187387,187388,187387,374775,180.40133714675903,0.012796706046826107
187588,187589,187588,375177,180.65937900543213,0.012783959819630803
187788,187789,187788,375577,180.9085350036621,0.012771295800512016
187988,187989,187988,375977,181.16794800758362,0.012758650488117097
188188,188189,188188,376377,181.41744303703308,0.012746023842226367
188388,188389,188388,376777,181.6872899532318,0.012733415822751162
188589,188590,188589,377179,181.9435751438141,0.012720763489199705
188789,188790,188789,377579,182.2555022239685,0.01270819269544401
188989,188990,188989,377979,182.59690594673157,0.01269564040841988
189189,189190,189189,378379,182.8854100704193,0.012683106588557138
189389,189390,189389,378779,183.15725111961365,0.012670591196413564
189590,189591,189590,379181,183.49442791938782,0.012658031753790431
189790,189791,189790,379581,183.78661799430847,0.01264555319091445
189990,189991,189990,379981,184.0613009929657,0.012633092937996618
190190,190191,190190,380381,184.33464908599854,0.012620650956100207
190390,190391,190390,380781,184.60978603363037,0.012608227206413303
190591,190592,190591,381183,184.88445401191711,0.012595759668113684
190791,190792,190791,381583,185.1632890701294,0.01258337235758367
190991,190992,190991,381983,185.4648699760437,0.012571003163377328
191191,191192,191191,382383,185.75304293632507,0.012558652047175819
191391,191392,191391,382783,186.02570009231567,0.012546318970781947
191592,191593,191592,383185,186.27959203720093,0.012533942365911765
191792,191793,191792,383585,186.54488921165466,0.01252164534474869
191992,191993,191992,383985,186.80352997779846,0.012509366249336453
192192,192193,192192,384385,187.0598659515381,0.012497105041958905
192392,192393,192392,384785,187.3183000087738,0.012484861685018573
192593,192594,192593,385187,187.5782721042633,0.012472575058008382
192793,192794,192793,385587,187.8343629837036,0.01246036737840599
192993,192994,192993,385987,188.11197113990784,0.012448177436968485
193193,193194,193193,386387,188.39670515060425,0.01243600519656792
193393,193394,193393,386787,188.71788001060486,0.012423850620191823
193594,193595,193594,387189,189.029855966568,0.0124116530304233
193794,193795,193794,387589,189.2832431793213,0.012399533759379243
193994,193995,193994,387989,189.56267714500427,0.01238743204182887
194194,194195,194194,388389,189.82626008987427,0.012375347841218022
194394,194395,194394,388789,190.09212017059326,0.012363281121105529
194595,194596,194595,389191,190.3741340637207,0.012351171642550602
194795,194796,194795,389591,190.6549220085144,0.012339139861509708
194995,194996,194995,389991,190.90519094467163,0.012327125452136108
195195,195196,195195,390391,191.16355109214783,0.012315128378435855
195395,195396,195395,390791,191.4142370223999,0.01230314860452532
195596,195597,195596,391193,191.78357315063477,0.012291126325397235
195796,195797,195796,391593,192.1901478767395,0.012279181129906532
195996,195997,195996,391993,192.5356171131134,0.012267253127034037
196196,196197,196196,392393,192.85761404037476,0.012255342281332869
196396,196397,196396,392793,193.13268613815308,0.012243448557463772
196597,196598,196597,393195,193.41151213645935,0.012231512579879523
196797,196798,196797,393595,193.67630290985107,0.012219653079254817
196997,196998,196997,393995,193.94125699996948,0.012207810594911227
197197,197198,197197,394395,194.21065711975098,0.012195985091936068
197397,197398,197397,394795,194.50506401062012,0.01218417653552182
197598,197599,197598,395197,194.85397791862488,0.012172325975175915
197798,197799,197798,395597,195.1694757938385,0.012160551292179151
197998,197999,197998,395997,195.46474027633667,0.012148793451775195
198198,198199,198198,396397,195.77117800712585,0.012137052419573156
198398,198399,198398,396797,196.05830192565918,0.01212532816128502
198599,198600,198599,397199,196.35362887382507,0.012113562147133486
198799,198800,198799,397599,196.60926222801208,0.012101871417660505
198999,199000,198999,397999,196.90903496742249,0.012090197359679635
199199,199200,199199,398399,197.18434596061707,0.012078539939309909
199399,199400,199399,398799,197.4826738834381,0.012066899122770751
199600,199601,199600,399201,197.9259111881256,0.012055216796725702
199800,199801,199800,399601,198.25263381004333,0.01204360916950424
200000,200001,200000,400001,198.56298303604126,0.012032018045202673


==> plot_data/quadratic_minimax_problem_n500_alpha00001/agraal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007648468017578125,30.358106049564984
200,201,200,401,0.07058382034301758,1.5266697976090917
400,401,400,801,0.14265894889831543,0.9949572917608964
601,602,601,1203,0.21718192100524902,0.654469703896404
801,802,801,1603,0.28324294090270996,0.5449375577615801
1001,1002,1001,2003,0.3540990352630615,0.466558339137924
1201,1202,1201,2403,0.41872286796569824,0.40790445856812785
1401,1402,1401,2803,0.49037909507751465,0.36324839772486234
1602,1603,1602,3205,0.5683107376098633,0.332410758519307
1802,1803,1802,3605,0.6348049640655518,0.2959221037316122
2002,2003,2002,4005,0.7040529251098633,0.3178597359959202
2202,2203,2202,4405,0.7678680419921875,0.25472097014152784
2402,2403,2402,4805,0.8338320255279541,0.29365243117227025
2603,2604,2603,5207,0.8970508575439453,0.22189710215379213
2803,2804,2803,5607,0.9613039493560791,0.2068581685238522
3003,3004,3003,6007,1.0259227752685547,0.20204829271238317
3203,3204,3203,6407,1.0907468795776367,0.1826780936969815
3403,3404,3403,6807,1.172070026397705,0.17350693079852542
3604,3605,3604,7209,1.2582969665527344,0.16618529329681433
3804,3805,3804,7609,1.3289129734039307,0.1559774946123097
4004,4005,4004,8009,1.3955929279327393,0.1479860340576209
4204,4205,4204,8409,1.477985143661499,0.1420812036193549
4404,4405,4404,8809,1.5451500415802002,0.1354867762288171
4605,4606,4605,9211,1.6106619834899902,0.12804190617601624
4805,4806,4805,9611,1.683297872543335,0.14492790348498927
5005,5006,5005,10011,1.7669079303741455,0.11843714281990657
5205,5206,5205,10411,1.8366169929504395,0.1355149934683695
5405,5406,5405,10811,1.9066479206085205,0.10967509053331728
5606,5607,5606,11213,1.9756591320037842,0.1047390441099821
5806,5807,5806,11613,2.045254945755005,0.11116670419397351
6006,6007,6006,12013,2.1133010387420654,0.1104731554284347
6206,6207,6206,12413,2.188856840133667,0.11339589037345801
6406,6407,6406,12813,2.261047840118408,0.08959043022299047
6607,6608,6607,13215,2.329741954803467,0.08790212998533639
6807,6808,6807,13615,2.398026943206787,0.09725045222241159
7007,7008,7007,14015,2.4656009674072266,0.08069814582142183
7207,7208,7207,14415,2.5341639518737793,0.0779170467991856
7407,7408,7407,14815,2.605954885482788,0.07497417734907265
7608,7609,7608,15217,2.6990559101104736,0.07228850125978122
7808,7809,7808,15617,2.7877659797668457,0.0705158943683833
8008,8009,8008,16017,2.8560547828674316,0.0679033528756303
8208,8209,8208,16417,2.925092935562134,0.06556943872126361
8408,8409,8408,16817,2.9941329956054688,0.06338593380502335
8609,8610,8609,17219,3.062572717666626,0.06190721473282491
8809,8810,8809,17619,3.132429838180542,0.05959173999795306
9009,9010,9009,18019,3.2028727531433105,0.060609997754527266
9209,9210,9209,18419,3.270448923110962,0.05630214481997626
9409,9410,9409,18819,3.3394088745117188,0.055273169854554924
9610,9611,9610,19221,3.4086318016052246,0.060694624115735125
9810,9811,9810,19621,3.47737193107605,0.06022217748508646
10010,10011,10010,20021,3.5437488555908203,0.05237237177653837
10210,10211,10210,20421,3.60870099067688,0.04917242783563536
10410,10411,10410,20821,3.677323818206787,0.04802124407245041
10611,10612,10611,21223,3.751830816268921,0.04673826584019885
10811,10812,10811,21623,3.8200840950012207,0.046157854104341846
11011,11012,11011,22023,3.8845887184143066,0.04441507929785954
11211,11212,11211,22423,3.9493319988250732,0.05715923333272001
11411,11412,11411,22823,4.015138864517212,0.04361524161548882
11612,11613,11612,23225,4.083329916000366,0.04145315231159302
11812,11813,11812,23625,4.174379110336304,0.04103833274219849
12012,12013,12012,24025,4.269699811935425,0.04152388108257078
12212,12213,12212,24425,4.353366136550903,0.039097157612056385
12412,12413,12412,24825,4.431055784225464,0.037917942679045025
12613,12614,12613,25227,4.51396107673645,0.037175633239289456
12813,12814,12813,25627,4.590471029281616,0.03648102445539223
13013,13014,13013,26027,4.667370080947876,0.035984507698872216
13213,13214,13213,26427,4.766811847686768,0.0352288901109299
13413,13414,13413,26827,4.851867914199829,0.034248478249940977
13614,13615,13614,27229,4.929779052734375,0.03353697604508712
13814,13815,13814,27629,5.002672910690308,0.03819334980340488
14014,14015,14014,28029,5.079078912734985,0.0325092445410024
14214,14215,14214,28429,5.159695863723755,0.03167357404618877
14414,14415,14414,28829,5.246571063995361,0.03132145035056967
14615,14616,14615,29231,5.326661825180054,0.03841943100962133
14815,14816,14815,29631,5.393293857574463,0.03149950765100605
15015,15016,15015,30031,5.464583873748779,0.029597435605700283
15215,15216,15215,30431,5.53377103805542,0.029165739782345785
15415,15416,15415,30831,5.601186752319336,0.028491164325146364
15616,15617,15616,31233,5.671533823013306,0.02851613638181219
15816,15817,15816,31633,5.7581799030303955,0.027993301187548506
16016,16017,16016,32033,5.83270788192749,0.02703679477218751
16216,16217,16216,32433,5.9094390869140625,0.026840158619861415
16416,16417,16416,32833,5.991601943969727,0.027075123915141455
16617,16618,16617,33235,6.076669931411743,0.025867205065584178
16817,16818,16817,33635,6.153759956359863,0.02565841084456606
17017,17018,17017,34035,6.237292766571045,0.02510285720067962
17217,17218,17217,34435,6.306429862976074,0.024945733381901144
17417,17418,17417,34835,6.388155937194824,0.02460658271122539
17618,17619,17618,35237,6.45967173576355,0.024043042391285803
17818,17819,17818,35637,6.532362937927246,0.024140354635167706
18018,18019,18018,36037,6.6014978885650635,0.023224035515757097
18218,18219,18218,36437,6.674348831176758,0.02837802755604619
18418,18419,18418,36837,6.763919830322266,0.022630684792705146
18619,18620,18619,37239,6.842882871627808,0.028489056280565198
18819,18820,18819,37639,6.941777944564819,0.022012179950758437
19019,19020,19019,38039,7.02716588973999,0.021879992934182038
19219,19220,19219,38439,7.098832845687866,0.021379257636480943
19419,19420,19419,38839,7.1653358936309814,0.0211590445178449
19620,19621,19620,39241,7.248676776885986,0.02101117273983544
19820,19821,19820,39641,7.316822052001953,0.02060057744243322
20020,20021,20020,40041,7.38716197013855,0.021566496480300155
20220,20221,20220,40441,7.457338809967041,0.02329234709472489
20420,20421,20420,40841,7.5306408405303955,0.01966194102571158
20621,20622,20621,41243,7.6009838581085205,0.01939121445690968
20821,20822,20821,41643,7.686722755432129,0.021866674330809285
21021,21022,21021,42043,7.76284384727478,0.021319881520695454
21221,21222,21221,42443,7.832942962646484,0.018911686871858128
21421,21422,21421,42843,7.905105829238892,0.018525947804047094
21622,21623,21622,43245,7.989865064620972,0.018143955833611978
21822,21823,21822,43645,8.065656900405884,0.018002548560382317
22022,22023,22022,44045,8.140564918518066,0.017729104951395253
22222,22223,22222,44445,8.231756925582886,0.02169050636890875
22422,22423,22422,44845,8.305401802062988,0.017236578274391543
22623,22624,22623,45247,8.378979921340942,0.017171275398090772
22823,22824,22823,45647,8.443895816802979,0.01723805741314565
23023,23024,23023,46047,8.50954794883728,0.016654232836777864
23223,23224,23223,46447,8.603161811828613,0.01637114345988508
23423,23424,23423,46847,8.726433753967285,0.016227383642620392
23624,23625,23624,47249,8.870965003967285,0.016374949911371936
23824,23825,23824,47649,8.973904848098755,0.015916322428547805
24024,24025,24024,48049,9.084212064743042,0.015611470770124466
24224,24225,24224,48449,9.200434923171997,0.01555084344791199
24424,24425,24424,48849,9.312075138092041,0.015342097353781697
24625,24626,24625,49251,9.386159896850586,0.015391270753840378
24825,24826,24825,49651,9.456448078155518,0.015486797363564774
25025,25026,25025,50051,9.526516914367676,0.014677686574071513
25225,25226,25225,50451,9.606059074401855,0.01534233015075886
25425,25426,25425,50851,9.678344011306763,0.01556508241279493
25626,25627,25626,51253,9.752928018569946,0.014207276405747475
25826,25827,25826,51653,9.820349931716919,0.014142692041634954
26026,26027,26026,52053,9.892266988754272,0.014088435968873334
26226,26227,26226,52453,9.959378004074097,0.016665082548559758
26426,26427,26426,52853,10.028705835342407,0.013678763379293758
26627,26628,26627,53255,10.094225883483887,0.01369319682065927
26827,26828,26827,53655,10.159865856170654,0.01328961165000624
27027,27028,27027,54055,10.23310899734497,0.013220549972175111
27227,27228,27227,54455,10.29791808128357,0.013591861749911147
27427,27428,27427,54855,10.364189863204956,0.013831233353945824
27628,27629,27628,55257,10.43020486831665,0.014749725228936158
27828,27829,27828,55657,10.494779825210571,0.01256930069071054
28028,28029,28028,56057,10.556712865829468,0.012629597210061889
28228,28229,28228,56457,10.61829400062561,0.012300447149308504
28428,28429,28428,56857,10.689611911773682,0.01231187615166595
28629,28630,28629,57259,10.759116888046265,0.012458374687134907
28829,28830,28829,57659,10.823574781417847,0.014645047653422776
29029,29030,29029,58059,10.889255046844482,0.011795066129494085
29229,29230,29229,58459,10.95370078086853,0.011668990359557234
29429,29430,29429,58859,11.018799781799316,0.011615872707566222
29630,29631,29630,59261,11.08354902267456,0.011457230857455845
29830,29831,29830,59661,11.148549795150757,0.011421642485357902
30030,30031,30030,60061,11.243512868881226,0.011334904959888356
30230,30231,30230,60461,11.31685996055603,0.011225895298390203
30430,30431,30430,60861,11.38327693939209,0.010993701864656555
30631,30632,30631,61263,11.448609828948975,0.010913376892857702
30831,30832,30831,61663,11.512871026992798,0.010747762786247785
31031,31032,31031,62063,11.575301885604858,0.01073682524299021
31231,31232,31231,62463,11.63721489906311,0.010730464815948637
31431,31432,31431,62863,11.706426858901978,0.010854346578810811
31632,31633,31632,63265,11.772215843200684,0.010411782149919039
31832,31833,31832,63665,11.834995031356812,0.010152821733948561
32032,32033,32032,64065,11.899375915527344,0.010511679414757436
32232,32233,32232,64465,11.963735818862915,0.010064149640755443
32432,32433,32432,64865,12.027154922485352,0.009914715275102915
32633,32634,32633,65267,12.09280276298523,0.00977876819260044
32833,32834,32833,65667,12.155019760131836,0.011954528918934865
33033,33034,33033,66067,12.224967956542969,0.009664945259027457
33233,33234,33233,66467,12.289203882217407,0.009554960255956228
33433,33434,33433,66867,12.352880954742432,0.009444683517121213
33634,33635,33634,67269,12.416938066482544,0.009212533363045217
33834,33835,33834,67669,12.481770038604736,0.009180858805514457
34034,34035,34034,68069,12.545536994934082,0.009070482856211867
34234,34235,34234,68469,12.609080791473389,0.009000496104865696
34434,34435,34434,68869,12.677753925323486,0.010391459253913101
34635,34636,34635,69271,12.747344970703125,0.009174443415102351
34835,34836,34835,69671,12.811465978622437,0.008735193068431655
35035,35036,35035,70071,12.874258041381836,0.00928060929193001
35235,35236,35235,70471,12.93698787689209,0.008593752526951411
35435,35436,35435,70871,13.001312017440796,0.009870002714740315
35636,35637,35636,71273,13.064252853393555,0.009788365239237392
35836,35837,35836,71673,13.127983808517456,0.008403676416654269
36036,36037,36036,72073,13.199471950531006,0.008436883971701758
36236,36237,36236,72473,13.26845383644104,0.008169385430545057
36436,36437,36436,72873,13.346472978591919,0.008023441650148011
36637,36638,36637,73275,13.425243854522705,0.007995745222023636
36837,36838,36837,73675,13.488154888153076,0.007959178876352183
37037,37038,37037,74075,13.554846048355103,0.0078077471474318665
37237,37238,37237,74475,13.621104001998901,0.007775713071278348
37437,37438,37437,74875,13.690204858779907,0.007821110627525184
37638,37639,37638,75277,13.759541988372803,0.007615333998271852
37838,37839,37838,75677,13.82467007637024,0.0075492781256574475
38038,38039,38038,76077,13.891592025756836,0.00922783902817441
38238,38239,38238,76477,13.959971904754639,0.0073557743007614555
38438,38439,38438,76877,14.025761127471924,0.008778804720289588
38639,38640,38639,77279,14.090030908584595,0.007238039933108067
38839,38840,38839,77679,14.154340982437134,0.007204657438835355
39039,39040,39039,78079,14.231267929077148,0.0073630940174610705
39239,39240,39239,78479,14.297241926193237,0.007026960416637018
39439,39440,39439,78879,14.362963914871216,0.007017946115219119
39640,39641,39640,79281,14.42605972290039,0.006883763708289022
39840,39841,39840,79681,14.490798950195312,0.007184939890910387
40040,40041,40040,80081,14.555286884307861,0.006723037949343745
40240,40241,40240,80481,14.620985984802246,0.006882357757456093
40440,40441,40440,80881,14.696257829666138,0.0066258467979763555
40641,40642,40641,81283,14.789479970932007,0.006564814215815098
40841,40842,40841,81683,14.89287781715393,0.008178163031538722
41041,41042,41041,82083,14.986050844192505,0.006528907249864797
41241,41242,41241,82483,15.068204164505005,0.0063335389213702645
41441,41442,41441,82883,15.140449047088623,0.006314806052776884
41642,41643,41642,83285,15.222745895385742,0.006223445179829302
41842,41843,41842,83685,15.304805994033813,0.006199636624925208
42042,42043,42042,84085,15.392822742462158,0.0064046066167128355
42242,42243,42242,84485,15.504727840423584,0.00610804918979095
42442,42443,42442,84885,15.59882402420044,0.006041011956911219
42643,42644,42643,85287,15.683449983596802,0.0075950802945418385
42843,42844,42843,85687,15.766734838485718,0.007055789738607428
43043,43044,43043,86087,15.83751392364502,0.005834122826214432
43243,43244,43243,86487,15.912606000900269,0.00694474369668056
43443,43444,43443,86887,15.99439787864685,0.005736101214718079
43644,43645,43644,87289,16.072885036468506,0.0056928854547508186
43844,43845,43844,87689,16.148908853530884,0.005672448661857534
44044,44045,44044,88089,16.258142948150635,0.005627258336581377
44244,44245,44244,88489,16.34809184074402,0.005509747309315578
44444,44445,44444,88889,16.440847873687744,0.005473784102890646
44645,44646,44645,89291,16.529570817947388,0.0054048743362980975
44845,44846,44845,89691,16.62104892730713,0.005324414430335031
45045,45046,45045,90091,16.721986770629883,0.0052861248235699055
45245,45246,45245,90491,16.810781955718994,0.00637676824949535
45445,45446,45445,90891,16.90523076057434,0.005469393148718725
45646,45647,45646,91293,16.995255947113037,0.005210261815777803
45846,45847,45846,91693,17.075894117355347,0.005184262453052653
46046,46047,46046,92093,17.154412746429443,0.005037390976195141
46246,46247,46246,92493,17.241500854492188,0.005045379447369975
46446,46447,46446,92893,17.325258016586304,0.005448903738972202
46647,46648,46647,93295,17.408763885498047,0.004882146582864415
46847,46848,46847,93695,17.48288583755493,0.004853254380033408
47047,47048,47047,94095,17.55060887336731,0.004817968873446524
47247,47248,47247,94495,17.640344858169556,0.004796794497335832
47447,47448,47447,94895,17.732635974884033,0.004784359936242819
47648,47649,47648,95297,17.825819969177246,0.0047058598691657955
47848,47849,47848,95697,17.919836044311523,0.0047183983197354685
48048,48049,48048,96097,17.995261907577515,0.004660405774696224
48248,48249,48248,96497,18.081974744796753,0.004574980937427125
48448,48449,48448,96897,18.15975785255432,0.005159583751182835
48649,48650,48649,97299,18.236470699310303,0.004494401066177711
48849,48850,48849,97699,18.305125951766968,0.004421364876352003
49049,49050,49049,98099,18.372591972351074,0.0044448900327837635
49249,49250,49249,98499,18.4457049369812,0.004359621142493204
49449,49450,49449,98899,18.519243717193604,0.004307696151307247
49650,49651,49650,99301,18.61645197868347,0.005022210110713118
49850,49851,49850,99701,18.785408973693848,0.004242293444367986
50050,50051,50050,100101,18.859556913375854,0.004314994502392726
50250,50251,50250,100501,18.930732011795044,0.004176033581827324
50450,50451,50450,100901,18.998551845550537,0.004128143289650036
50651,50652,50651,101303,19.20180583000183,0.0041339792521615185
50851,50852,50851,101703,19.30881690979004,0.004090779154477809
51051,51052,51051,102103,19.401330947875977,0.004540151194279124
51251,51252,51251,102503,19.467595100402832,0.003997643491167043
51451,51452,51451,102903,19.540467023849487,0.004016891260842929
51652,51653,51652,103305,19.612465858459473,0.003923721621086954
51852,51853,51852,103705,19.683265924453735,0.004033590827142122
52052,52053,52052,104105,19.77008581161499,0.003854374146784114
52252,52253,52252,104505,19.849427938461304,0.00382778701247259
52452,52453,52452,104905,19.919520139694214,0.0038141899436616206
52653,52654,52653,105307,19.985893964767456,0.003747986112886527
52853,52854,52853,105707,20.05150604248047,0.004460738481297694
53053,53054,53053,106107,20.116740942001343,0.0036757285816074185
53253,53254,53253,106507,20.188909769058228,0.003637104726922998
53453,53454,53453,106907,20.256837844848633,0.003995768159929085
53654,53655,53654,107309,20.322123050689697,0.0035756642346731204
53854,53855,53854,107709,20.386443853378296,0.003573966665545678
54054,54055,54054,108109,20.453223943710327,0.0035404520710186098
54254,54255,54254,108509,20.516972064971924,0.0034997189135236814
54454,54455,54454,108909,20.60979700088501,0.0034448207345215824
54655,54656,54655,109311,20.687989950180054,0.003426571604658671
54855,54856,54855,109711,20.75858211517334,0.004015792697265188
55055,55056,55055,110111,20.825946807861328,0.003410811756743703
55255,55256,55255,110511,20.895997047424316,0.0033149110083684195
55455,55456,55455,110911,20.967813968658447,0.0038234971026624765
55656,55657,55656,111313,21.048868894577026,0.0032725110883480963
55856,55857,55856,111713,21.11504888534546,0.003225975893467207
56056,56057,56056,112113,21.1821928024292,0.0032021457962409035
56256,56257,56256,112513,21.265304803848267,0.0032830659578713508
56456,56457,56456,112913,21.336288928985596,0.00313358158283242
56657,56658,56657,113315,21.40790295600891,0.0031038112335010836
56857,56858,56857,113715,21.475820064544678,0.003068666183747005
57057,57058,57057,114115,21.54113483428955,0.0030822686207365277
57257,57258,57257,114515,21.61165690422058,0.003164432014817304
57457,57458,57457,114915,21.68510890007019,0.003050757363447427
57658,57659,57658,115317,21.761884927749634,0.0029547128947588278
57858,57859,57858,115717,21.831382036209106,0.0029595848542652054
58058,58059,58058,116117,21.917004823684692,0.002948310317680173
58258,58259,58258,116517,21.997490882873535,0.0028914202693623367
58458,58459,58458,116917,22.06484580039978,0.0028542302821310877
58659,58660,58659,117319,22.1301908493042,0.0028519728113630865
58859,58860,58859,117719,22.195585012435913,0.0028124123956395175
59059,59060,59059,118119,22.263853788375854,0.003193031212689097
59259,59260,59259,118519,22.327585697174072,0.00278173229810129
59459,59460,59459,118919,22.390971899032593,0.0027773343329458217
59660,59661,59660,119321,22.454447984695435,0.0026988259601007573
59860,59861,59860,119721,22.51838707923889,0.0027471317469777118
60060,60061,60060,120121,22.582087993621826,0.003181692819311271
60260,60261,60260,120521,22.64557385444641,0.002669606356282548
60460,60461,60460,120921,22.7260160446167,0.002624876205875502
60661,60662,60661,121323,22.816571950912476,0.0025962358122678915
60861,60862,60861,121723,22.89116096496582,0.0028076605843462324
61061,61062,61061,122123,22.95526695251465,0.0028074716422748073
61261,61262,61261,122523,23.019766092300415,0.00254828190463533
61461,61462,61461,122923,23.084678888320923,0.00318563405813102
61662,61663,61662,123325,23.150120973587036,0.0024778961399352724
61862,61863,61862,123725,23.223878860473633,0.0029140708423549704
62062,62063,62062,124125,23.299428939819336,0.002452993365505163
62262,62263,62262,124525,23.36921191215515,0.0024264842511566515
62462,62463,62462,124925,23.434172868728638,0.0023942474532321536
62663,62664,62663,125327,23.507672786712646,0.002441924424476341
62863,62864,62863,125727,23.5724880695343,0.0023417762048479358
63063,63064,63063,126127,23.64223599433899,0.002833884411476546
63263,63264,63263,126527,23.711061000823975,0.002357950099527221
63463,63464,63463,126927,23.783836841583252,0.0023047279434673796
63664,63665,63664,127329,23.852894067764282,0.0022688397453119328
63864,63865,63864,127729,23.917147874832153,0.002308256475268803
64064,64065,64064,128129,24.010740041732788,0.002582592843548127
64264,64265,64264,128529,24.151176929473877,0.002226765580596944
64464,64465,64464,128929,24.251598834991455,0.0021978579451071172
64665,64666,64665,129331,24.33493399620056,0.0021853380456726035
64865,64866,64865,129731,24.404742002487183,0.002604607519962246
65065,65066,65065,130131,24.474050760269165,0.0021531408089884613
65265,65266,65265,130531,24.54742980003357,0.0021206520081071887
65465,65466,65465,130931,24.613870859146118,0.002086560712841971
65666,65667,65666,131333,24.68449091911316,0.002165790937774461
65866,65867,65866,131733,24.75597381591797,0.0023925285189972524
66066,66067,66066,132133,24.823237895965576,0.0023525402657535114
66266,66267,66266,132533,24.893287897109985,0.0023846004288762546
66466,66467,66466,132933,24.960285902023315,0.001992598457079472
66667,66668,66667,133335,25.02826189994812,0.002337947473440871
66867,66868,66867,133735,25.09685492515564,0.0021039676693394155
67067,67068,67067,134135,25.164212942123413,0.0019623741433012825
67267,67268,67267,134535,25.236160039901733,0.0019258740897910005
67467,67468,67467,134935,25.302230834960938,0.0019376569302019043
67668,67669,67668,135337,25.372169971466064,0.001911136566718753
67868,67869,67868,135737,25.438562870025635,0.001891672979873212
68068,68069,68068,136137,25.504350900650024,0.0018745668576293179
68268,68269,68268,136537,25.570355892181396,0.0018530288909395798
68468,68469,68468,136937,25.63900089263916,0.001837330898563454
68669,68670,68669,137339,25.749825716018677,0.0018137680102064703
68869,68870,68869,137739,25.867790937423706,0.0017969900262357198
69069,69070,69069,138139,25.967891931533813,0.0018039159747469103
69269,69270,69269,138539,26.042635917663574,0.001770846421773793
69469,69470,69469,138939,26.119290828704834,0.00207024027663629
69670,69671,69670,139341,26.207242012023926,0.0018858783838663878
69870,69871,69870,139741,26.293115854263306,0.0017299934099322858
70070,70071,70070,140141,26.36950993537903,0.0017123410169292488
70270,70271,70270,140541,26.449445962905884,0.0017040543167285227
70470,70471,70470,140941,26.525012016296387,0.0016892286019085452
70671,70672,70671,141343,26.597505807876587,0.0016711880487108768
70871,70872,70871,141743,26.666029930114746,0.0016556449301216329
71071,71072,71071,142143,26.82124900817871,0.0016554248251239646
71271,71272,71271,142543,26.927687883377075,0.0016215431188463794
71471,71472,71471,142943,27.0234477519989,0.0016102418672560433
71672,71673,71672,143345,27.096342086791992,0.0015974073694012484
71872,71873,71872,143745,27.164005994796753,0.001578047951775619
72072,72073,72072,144145,27.247804880142212,0.001648645113678236
72272,72273,72272,144545,27.317007780075073,0.0015686714573804894
72472,72473,72472,144945,27.388449907302856,0.0016259957829209304
72673,72674,72673,145347,27.454643964767456,0.0015339215429024933
72873,72874,72873,145747,27.520258903503418,0.0017087978179110028
73073,73074,73073,146147,27.587308883666992,0.0014991866267269245
73273,73274,73273,146547,27.654689073562622,0.0014865607022882153
73473,73474,73473,146947,27.729750871658325,0.0014810440750317052
73674,73675,73674,147349,27.796249866485596,0.0014696465353717996
73874,73875,73874,147749,27.863275051116943,0.0014498492895373702
74074,74075,74074,148149,27.929237127304077,0.0014344159097007775
74274,74275,74274,148549,27.99513602256775,0.0014283313859918445
74474,74475,74474,148949,28.062901973724365,0.001491166883556748
74675,74676,74675,149351,28.12894296646118,0.0014157961336949336
74875,74876,74875,149751,28.211358070373535,0.0013898441223984133
75075,75076,75075,150151,28.285249710083008,0.0013650476288958441
75275,75276,75275,150551,28.36661195755005,0.0013784488199792759
75475,75476,75475,150951,28.45638394355774,0.0015164276592423446
75676,75677,75676,151353,28.534773111343384,0.0013289431458864361
75876,75877,75876,151753,28.599914073944092,0.0013325628600834502
76076,76077,76076,152153,28.668128967285156,0.0013213682093171186
76276,76277,76276,152553,28.74641990661621,0.0015468465679421067
76476,76477,76476,152953,28.813735961914062,0.0013148445430109102
76677,76678,76677,153355,28.880621910095215,0.0012853842079396524
76877,76878,76877,153755,28.947283029556274,0.001320721497792898
77077,77078,77077,154155,29.020328044891357,0.0012861340208206746
77277,77278,77277,154555,29.090600967407227,0.0014294178260157717
77477,77478,77477,154955,29.252268075942993,0.0012499461922213144
77678,77679,77678,155357,29.37106680870056,0.0012171055006695505
77878,77879,77878,155757,29.46290373802185,0.0012131845461831254
78078,78079,78078,156157,29.5429368019104,0.001203724167682169
78278,78279,78278,156557,29.609725952148438,0.0012029701152497963
78478,78479,78478,156957,29.68287992477417,0.0013968161589793567
78679,78680,78679,157359,29.76009202003479,0.0011711489114842977
78879,78880,78879,157759,29.82782793045044,0.0011666695324699192
79079,79080,79079,158159,29.89389705657959,0.0011939322695306825
79279,79280,79279,158559,29.96120285987854,0.0011572430973980875
79479,79480,79479,158959,30.025644779205322,0.0011822069778385919
79680,79681,79680,159361,30.092138051986694,0.0011191015910363014
79880,79881,79880,159761,30.158751010894775,0.0011296573052424674
80080,80081,80080,160161,30.23062777519226,0.0011143579502772409
80280,80281,80280,160561,30.296111822128296,0.0011636204332137114
80480,80481,80480,160961,30.362751007080078,0.0012157709469575808
80681,80682,80681,161363,30.43578290939331,0.0010721082027020353
80881,80882,80881,161763,30.51568102836609,0.0010744123509593773
81081,81082,81081,162163,30.586927890777588,0.0011354488638184678
81281,81282,81281,162563,30.65473175048828,0.0010638817804371173
81481,81482,81481,162963,30.738807916641235,0.0010450378790161315
81682,81683,81682,163365,30.804508924484253,0.0010270518758330998
81882,81883,81882,163765,30.872061014175415,0.0010161208792489568
82082,82083,82082,164165,30.942807912826538,0.0011430844999268841
82282,82283,82282,164565,31.011684894561768,0.0010077093732481514
82482,82483,82482,164965,31.07704997062683,0.001010810569371863
82683,82684,82683,165367,31.143462896347046,0.0011804711262358462
82883,82884,82883,165767,31.213510990142822,0.0011773922194710325
83083,83084,83083,166167,31.28351378440857,0.0009733440183544112
83283,83284,83283,166567,31.352479934692383,0.0009605642811630366
83483,83484,83483,166967,31.421129941940308,0.0009664882428141598
83684,83685,83684,167369,31.491182804107666,0.0009448851639991226
83884,83885,83884,167769,31.59106683731079,0.0011003214330268336
84084,84085,84084,168169,31.66012692451477,0.0009265574902956548
84284,84285,84284,168569,31.737135887145996,0.0009652703345799466
84484,84485,84484,168969,31.82335090637207,0.00091640678821691
84685,84686,84685,169371,31.901907920837402,0.0009285919016374308
84885,84886,84885,169771,31.968256950378418,0.0009248315463882673
85085,85086,85085,170171,32.03635597229004,0.001059902085054254
85285,85286,85285,170571,32.10348296165466,0.0008905256652327223
85485,85486,85485,170971,32.17238402366638,0.0009701047042841164
85686,85687,85686,171373,32.24503779411316,0.0008651777349804145
85886,85887,85886,171773,32.310100078582764,0.0008680604197107588
86086,86087,86086,172173,32.37353301048279,0.0008565030322585804
86286,86287,86286,172573,32.43905186653137,0.0008448046842769668
86486,86487,86486,172973,32.50310683250427,0.0008387022794562168
86687,86688,86687,173375,32.57859492301941,0.000875066704367894
86887,86888,86887,173775,32.659955978393555,0.0010023588171795435
87087,87088,87087,174175,32.73519587516785,0.0008295156535442173
87287,87288,87287,174575,32.80304193496704,0.0008175970618709544
87487,87488,87487,174975,32.86812973022461,0.0008052802023323822
87688,87689,87688,175377,32.935343980789185,0.0008000983363289993
87888,87889,87888,175777,33.00088882446289,0.0008014624912253244
88088,88089,88088,176177,33.06593680381775,0.0007866351780767682
88288,88289,88288,176577,33.13161611557007,0.0007794580165739173
88488,88489,88488,176977,33.211360931396484,0.0007788527266861594
88689,88690,88689,177379,33.27821493148804,0.0007671347477646322
88889,88890,88889,177779,33.34786891937256,0.0007561657409285105
89089,89090,89089,178179,33.438294887542725,0.0007483303111641605
89289,89290,89289,178579,33.50483798980713,0.0007490567879696018
89489,89490,89489,178979,33.56978893280029,0.0007829541762407832
89690,89691,89690,179381,33.63518810272217,0.0007363015416707622
89890,89891,89890,179781,33.70776295661926,0.0007231589573518299
90090,90091,90090,180181,33.77466893196106,0.000730531819713983
90290,90291,90290,180581,33.83894991874695,0.0007225465148316321
90490,90491,90490,180981,33.90539503097534,0.0007143109795995234
90691,90692,90691,181383,33.97271394729614,0.0008081588432625499
90891,90892,90891,181783,34.03639197349548,0.0007453443755951767
91091,91092,91091,182183,34.10164475440979,0.0009470296869915553
91291,91292,91291,182583,34.16637086868286,0.0006863479038542696
91491,91492,91491,182983,34.24159383773804,0.0006805103096089165
91692,91693,91692,183385,34.30829191207886,0.0006748041521433704
91892,91893,91892,183785,34.37256193161011,0.0006659536155933086
92092,92093,92092,184185,34.43748092651367,0.0006825730077668522
92292,92293,92292,184585,34.51169395446777,0.0008026629843615761
92492,92493,92492,184985,34.64661002159119,0.0006553079695202399
92693,92694,92693,185387,34.75331687927246,0.0006503418122260605
92893,92894,92893,185787,34.84022498130798,0.0006413345148204258
93093,93094,93093,186187,34.915302991867065,0.0006336012382768772
93293,93294,93293,186587,34.991076946258545,0.000706838769011653
93493,93494,93493,186987,35.08476972579956,0.0006283195705348358
93694,93695,93694,187389,35.157965898513794,0.0006209445123949274
93894,93895,93894,187789,35.23479890823364,0.0006128555084708953
94094,94095,94094,188189,35.313117027282715,0.0006117315879973153
94294,94295,94294,188589,35.389585971832275,0.0006033332826324221
94494,94495,94494,188989,35.45924687385559,0.0006224920253842942
94695,94696,94695,189391,35.526110887527466,0.0005938602037109243
94895,94896,94895,189791,35.591460943222046,0.0005987093636249723
95095,95096,95095,190191,35.662808895111084,0.0005900435391081641
95295,95296,95295,190591,35.76694989204407,0.0005872105580052622
95495,95496,95495,190991,35.84499788284302,0.0005798798529917621
95696,95697,95696,191393,35.91755700111389,0.00057690175363858
95896,95897,95896,191793,35.994006872177124,0.0005641953689872038
96096,96097,96096,192193,36.06928896903992,0.0005812790334422416
96296,96297,96296,192593,36.1491117477417,0.0005584327763594603
96496,96497,96496,192993,36.231634855270386,0.0005564439260513722
96697,96698,96697,193395,36.308435916900635,0.0005504497653999888
96897,96898,96897,193795,36.385339975357056,0.0005360268359049048
97097,97098,97097,194195,36.45727586746216,0.0006468484726535112
97297,97298,97297,194595,36.52602791786194,0.0005375701727467738
97497,97498,97497,194995,36.59143781661987,0.0005262813840142763
97698,97699,97698,195397,36.65985703468323,0.0005258084264976563
97898,97899,97898,195797,36.73699998855591,0.0005711344108401231
98098,98099,98098,196197,36.80221486091614,0.0005999564651891176
98298,98299,98298,196597,36.882944107055664,0.0005174432666217847
98498,98499,98498,196997,36.9634907245636,0.0005149795138194943
98699,98700,98699,197399,37.03633379936218,0.0005031968920002441
98899,98900,98899,197799,37.103511810302734,0.0005266223574202575
99099,99100,99099,198199,37.169431924819946,0.0004909474612806615
99299,99300,99299,198599,37.244560956954956,0.0005768510059589779
99499,99500,99499,198999,37.31195592880249,0.0004838628707059759
99700,99701,99700,199401,37.38048791885376,0.00048621886713974403
99900,99901,99900,199801,37.4457049369812,0.00047859867076574563
100100,100101,100100,200201,37.51304507255554,0.0005093230922730786
100300,100301,100300,200601,37.580482721328735,0.0005452480449979306
100501,100502,100501,201003,37.64610695838928,0.00046411700233118993
100701,100702,100701,201403,37.72410988807678,0.0005273829662152502
100901,100902,100901,201803,37.790788888931274,0.00045771420397045756
101101,101102,101101,202203,37.85646295547485,0.00045371688074914376
101301,101302,101301,202603,37.920788049697876,0.00045324498048581157
101502,101503,101502,203005,37.99383997917175,0.00044891638162703265
101702,101703,101702,203405,38.057262897491455,0.00044276882321106096
101902,101903,101902,203805,38.119335889816284,0.00043991763267018475
102102,102103,102102,204205,38.18784284591675,0.0004341588763127202
102302,102303,102302,204605,38.25527286529541,0.0004995534290153268
102503,102504,102503,205007,38.31994605064392,0.0004280087043108906
102703,102704,102703,205407,38.395545959472656,0.00042676931478402054
102903,102904,102903,205807,38.459924936294556,0.0004200103882236883
103103,103104,103103,206207,38.52315282821655,0.00042058750693246453
103303,103304,103303,206607,38.58637595176697,0.0004730756125101285
103504,103505,103504,207009,38.648892879486084,0.00040884644695077737
103704,103705,103704,207409,38.71822500228882,0.00041280217148092195
103904,103905,103904,207809,38.78163003921509,0.000485063812090237
104104,104105,104104,208209,38.84443187713623,0.0003993037801619884
104304,104305,104304,208609,38.90769290924072,0.00039658590979544365
104505,104506,104505,209011,38.979599952697754,0.00041561692300329424
104705,104706,104705,209411,39.059484004974365,0.00040630497048711365
104905,104906,104905,209811,39.12865114212036,0.0003925000042432693
105105,105106,105105,210211,39.2020218372345,0.0004656458797485168
105305,105306,105305,210611,39.26526498794556,0.00038922669148773806
105506,105507,105506,211013,39.327977895736694,0.0003776014906903302
105706,105707,105706,211413,39.39116811752319,0.0003729140047258833
105906,105907,105906,211813,39.453896045684814,0.0003744338502468438
106106,106107,106106,212213,39.51564693450928,0.0003721521331152258
106306,106307,106306,212613,39.57726287841797,0.00036792596837777793
106507,106508,106507,213015,39.640625,0.0003618501557837311
106707,106708,106707,213415,39.71079993247986,0.0003574074158582934
106907,106908,106907,213815,39.77424192428589,0.00036173967681687086
107107,107108,107107,214215,39.83814883232117,0.0003692788365756077
107307,107308,107307,214615,39.90148401260376,0.00035124457813046555
107508,107509,107508,215017,39.96787691116333,0.0003806432753762807
107708,107709,107708,215417,40.03036284446716,0.0003468769586082119
107908,107909,107908,215817,40.09519386291504,0.00034768591092550276
108108,108109,108108,216217,40.15775799751282,0.0003894305694058081
108308,108309,108308,216617,40.22933292388916,0.0003376787571690502
108509,108510,108509,217019,40.29369306564331,0.00033419879609328555
108709,108710,108709,217419,40.35649394989014,0.000340119642561156
108909,108910,108909,217819,40.41839599609375,0.0003495444154893001
109109,109110,109109,218219,40.48121976852417,0.00032450634771038816
109309,109310,109309,218619,40.54380393028259,0.00037054407615513243
109510,109511,109510,219021,40.6086699962616,0.0003199344625380786
109710,109711,109710,219421,40.674763917922974,0.00032797617539243756
109910,109911,109910,219821,40.74669790267944,0.00031848523012838935
110110,110111,110110,220221,40.80939197540283,0.00036160632052969447
110310,110311,110310,220621,40.8718957901001,0.00032356089159483027
110511,110512,110511,221023,40.93637299537659,0.0003045955283471815
110711,110712,110711,221423,40.9999098777771,0.0003057225511695573
110911,110912,110911,221823,41.065775871276855,0.00040580979723856995
111111,111112,111111,222223,41.147236824035645,0.00029872505376238366
111311,111312,111311,222623,41.227372884750366,0.0002983452908101658
111512,111513,111512,223025,41.293051958084106,0.0002921991658618583
111712,111713,111712,223425,41.35870289802551,0.0002920190499410021
111912,111913,111912,223825,41.42456674575806,0.0002988139353219697
112112,112113,112112,224225,41.49069690704346,0.00029122983914017363
112312,112313,112312,224625,41.55626392364502,0.00028547472690218387
112513,112514,112513,225027,41.62075185775757,0.00029322007910188847
112713,112714,112713,225427,41.695317029953,0.00028415621452410327
112913,112914,112913,225827,41.76138091087341,0.00028034909040907914
113113,113114,113113,226227,41.82507300376892,0.0002862537698865424
113313,113314,113313,226627,41.889673948287964,0.00027207281238986376
113514,113515,113514,227029,41.95430779457092,0.000271094254250346
113714,113715,113714,227429,42.019113063812256,0.0003186256043844505
113914,113915,113914,227829,42.084091901779175,0.0002940680931066336
114114,114115,114114,228229,42.14868783950806,0.00026589660364078287
114314,114315,114314,228629,42.21989393234253,0.0003112575460793506
114515,114516,114515,229031,42.28494071960449,0.0002622830677987649
114715,114716,114715,229431,42.35090494155884,0.00026069893989963785
114915,114916,114915,229831,42.41645073890686,0.00025561258378783763
115115,115116,115115,230231,42.48042893409729,0.0002650900876431717
115315,115316,115315,230631,42.544599771499634,0.000251187410798559
115516,115517,115516,231033,42.60983681678772,0.0002589538945950648
115716,115717,115716,231433,42.67655086517334,0.00025833014521034454
115916,115917,115916,231833,42.74566102027893,0.00028810770226381097
116116,116117,116116,232233,42.80987811088562,0.00025000880134558453
116316,116317,116316,232633,42.875152826309204,0.00024181192021742608
116517,116518,116517,233035,42.93953490257263,0.00024206343260350897
116717,116718,116717,233435,43.00589394569397,0.00023664808074604134
116917,116918,116917,233835,43.06930994987488,0.00023643825461349655
117117,117118,117117,234235,43.13277292251587,0.0002347528403456462
117317,117318,117317,234635,43.20738482475281,0.0002316841126644065
117518,117519,117518,235037,43.30873203277588,0.00022917684722461584
117718,117719,117718,235437,43.384952783584595,0.00023571330638898834
117918,117919,117918,235837,43.47274875640869,0.00023293782471396992
118118,118119,118118,236237,43.55723977088928,0.00023206164036119505
118318,118319,118318,236637,43.6293568611145,0.00023228138934603245
118519,118520,118519,237039,43.6984589099884,0.0002727569651125273
118719,118720,118719,237439,43.77105689048767,0.00021787300175039707
118919,118920,118919,237839,43.84252691268921,0.0002595203062734971
119119,119120,119119,238239,43.91203308105469,0.00024078617837036817
119319,119320,119319,238639,43.9750919342041,0.00021417634608272707
119520,119521,119520,239041,44.044665813446045,0.00024361903579351283
119720,119721,119720,239441,44.12766480445862,0.00020939717310639164
119920,119921,119920,239841,44.22193384170532,0.00021076439761725846
120120,120121,120120,240241,44.315502882003784,0.00020444864485875212
120320,120321,120320,240641,44.41967010498047,0.0002037651599473274
120521,120522,120521,241043,44.505435943603516,0.00020219273679139798
120721,120722,120721,241443,44.585729122161865,0.00020061219543260895
120921,120922,120921,241843,44.66915988922119,0.00020408220176145676
121121,121122,121121,242243,44.7483549118042,0.00020778093101333895
121321,121322,121321,242643,44.82202506065369,0.00019472973647033083
121522,121523,121522,243045,44.899247884750366,0.0001938774921903541
121722,121723,121722,243445,44.970491886138916,0.000192182138278952
121922,121923,121922,243845,45.036351919174194,0.00019126463450956665
122122,122123,122122,244245,45.103529930114746,0.0001888029252405674
122322,122323,122322,244645,45.17131590843201,0.0001923083039550761
122523,122524,122523,245047,45.247586727142334,0.00018670612531901428
122723,122724,122723,245447,45.32976484298706,0.00018473246330555834
122923,122924,122923,245847,45.489752769470215,0.00018204205253217188
123123,123124,123123,246247,45.582329988479614,0.00022656400138616766
123323,123324,123323,246647,45.67662501335144,0.00018368106136972635
123524,123525,123524,247049,45.74907088279724,0.00017869721073357302
123724,123725,123724,247449,45.86841702461243,0.00017872187989690147
123924,123925,123924,247849,45.942789793014526,0.0001769575066423175
124124,124125,124124,248249,46.02781701087952,0.0001739732840351933
124324,124325,124324,248649,46.09930992126465,0.00017260085259708987
124525,124526,124525,249051,46.163562059402466,0.00017445859572388155
124725,124726,124725,249451,46.232691049575806,0.00018882061041088186
124925,124926,124925,249851,46.2977659702301,0.0001673700468897207
125125,125126,125125,250251,46.363986015319824,0.0001672240356612481
125325,125326,125325,250651,46.42899203300476,0.00018962410112142368
125526,125527,125526,251053,46.49412417411804,0.00016421675173464224
125726,125727,125726,251453,46.56040406227112,0.00019649398922978032
125926,125927,125926,251853,46.625303745269775,0.0001654520561215418
126126,126127,126126,252253,46.70616388320923,0.0001626108975080058
126326,126327,126326,252653,46.7737820148468,0.00018690661512672956
126527,126528,126527,253055,46.83810591697693,0.00016468691847333758
126727,126728,126727,253455,46.90501880645752,0.0001564688083674855
126927,126928,126927,253855,46.97080612182617,0.0001840954686455205
127127,127128,127127,254255,47.036515951156616,0.00017376515485707198
127327,127328,127327,254655,47.102067947387695,0.00015146344895175268
127528,127529,127528,255057,47.168529987335205,0.00015935304609455208
127728,127729,127728,255457,47.24303698539734,0.0001497470880243413
127928,127929,127928,255857,47.31846499443054,0.00014809913545038429
128128,128129,128128,256257,47.4066059589386,0.000149256290112432
128328,128329,128328,256657,47.475172996520996,0.0001471485472175194
128529,128530,128529,257059,47.54940605163574,0.00014502711338056816
128729,128730,128729,257459,47.63383984565735,0.00014457830352967364
128929,128930,128929,257859,47.71554493904114,0.00016347542788958572
129129,129130,129129,258259,47.785337924957275,0.00016660390842092158
129329,129330,129329,258659,47.8507719039917,0.00014167591996885868
129530,129531,129530,259061,47.918423891067505,0.00013921868339999437
129730,129731,129730,259461,47.994534969329834,0.00013952844089690482
129930,129931,129930,259861,48.10513210296631,0.00013691912705496995
130130,130131,130130,260261,48.23697209358215,0.00013567999040744826
130330,130331,130330,260661,48.325045108795166,0.00016897389028923767
130531,130532,130531,261063,48.411322832107544,0.0001323561823563359
130731,130732,130731,261463,48.47838377952576,0.00013312171444892666
130931,130932,130931,261863,48.54245209693909,0.0001387492538816508
131131,131132,131131,262263,48.61523103713989,0.00012959465072680596
131331,131332,131331,262663,48.68899583816528,0.00012987401090343534
131532,131533,131532,263065,48.75428581237793,0.0001311729586442298
131732,131733,131732,263465,48.82112693786621,0.00015364622017195276
131932,131933,131932,263865,48.885615825653076,0.00013999881335071294
132132,132133,132132,264265,48.95142197608948,0.00013518138362311353
132332,132333,132332,264665,49.02133297920227,0.00012336901765903064
132533,132534,132533,265067,49.10306906700134,0.00012375024302195965
132733,132734,132733,265467,49.17459988594055,0.00012196954970905207
132933,132934,132933,265867,49.25077676773071,0.00012043612322105873
133133,133134,133133,266267,49.31604194641113,0.00011981585083038713
133333,133334,133333,266667,49.3808319568634,0.0001198250690442835
133534,133535,133534,267069,49.44689702987671,0.00011961563522740877
133734,133735,133734,267469,49.51091694831848,0.00011752697316186241
133934,133935,133934,267869,49.57864785194397,0.0001166181711923264
134134,134135,134134,268269,49.64753580093384,0.0001160422312848565
134334,134335,134334,268669,49.74508190155029,0.00011392885901520261
134535,134536,134535,269071,49.89667987823486,0.00011373807145986395
134735,134736,134735,269471,49.986222982406616,0.00012856258416784401
134935,134936,134935,269871,50.07552170753479,0.00011339916194495924
135135,135136,135135,270271,50.14086890220642,0.00011379903715873143
135335,135336,135335,270671,50.212599754333496,0.00011001481322224674
135536,135537,135536,271073,50.28650879859924,0.00011679720869627482
135736,135737,135736,271473,50.35615277290344,0.00010763387762289136
135936,135937,135936,271873,50.4236319065094,0.00013187356045771343
136136,136137,136136,272273,50.49057579040527,0.00010654864477437506
136336,136337,136336,272673,50.55665683746338,0.00013258091895106274
136537,136538,136537,273075,50.62621593475342,0.00010646439757504464
136737,136738,136737,273475,50.698668003082275,0.00010389703825020822
136937,136938,136937,273875,50.768314838409424,0.00010299086095545126
137137,137138,137137,274275,50.83277177810669,0.0001021330450886693
137337,137338,137337,274675,50.89908576011658,0.00010217630618454856
137538,137539,137538,275077,50.963984966278076,0.00010166933861882493
137738,137739,137738,275477,51.031566858291626,9.897784705146196e-05
137938,137939,137938,275877,51.09869194030762,9.853501545935032e-05
138138,138139,138138,276277,51.16286897659302,9.874414059854649e-05
138338,138339,138338,276677,51.23936891555786,0.00010291121056961455
138539,138540,138539,277079,51.304250955581665,9.582742988463976e-05
138739,138740,138739,277479,51.37292504310608,9.653339325814909e-05
138939,138940,138939,277879,51.44041991233826,0.00010312680411150754
139139,139140,139139,278279,51.505654096603394,9.37560019873352e-05
139339,139340,139339,278679,51.57122588157654,9.371176399321355e-05
139540,139541,139540,279081,51.63642978668213,9.174452155919e-05
139740,139741,139740,279481,51.71177697181702,9.194929497338977e-05
139940,139941,139940,279881,51.775707960128784,9.092507693284067e-05
140140,140141,140140,280281,51.85531187057495,9.002930812843955e-05
140340,140341,140340,280681,51.93307089805603,9.949210621541076e-05
140541,140542,140541,281083,51.998334884643555,8.783333304017521e-05
140741,140742,140741,281483,52.066540002822876,8.824524089881631e-05
140941,140942,140941,281883,52.13166809082031,0.00010429493791617036
141141,141142,141141,282283,52.20343613624573,8.875151496493305e-05
141341,141342,141341,282683,52.26841711997986,8.586632713388242e-05
141542,141543,141542,283085,52.335808992385864,8.500046136241476e-05
141742,141743,141742,283485,52.40011286735535,8.537487712826522e-05
141942,141943,141942,283885,52.46521186828613,9.783945090103757e-05
142142,142143,142142,284285,52.52998900413513,8.382210024623598e-05
142342,142343,142342,284685,52.59608292579651,8.255641495883449e-05
142543,142544,142543,285087,52.660836935043335,9.484831784373542e-05
142743,142744,142743,285487,52.73432397842407,8.624334365519478e-05
142943,142944,142943,285887,52.80699396133423,8.050110647744244e-05
143143,143144,143143,286287,52.87541198730469,7.962263428846227e-05
143343,143344,143343,286687,52.93836808204651,9.523532753013052e-05
143544,143545,143544,287089,53.00574994087219,7.894442558028543e-05
143744,143745,143744,287489,53.0689480304718,7.854699685926919e-05
143944,143945,143944,287889,53.13272976875305,7.797565308734925e-05
144144,144145,144144,288289,53.199896812438965,8.956701960178264e-05
144344,144345,144344,288689,53.26440405845642,7.60104307585942e-05
144545,144546,144545,289091,53.32704997062683,7.612520764377942e-05
144745,144746,144745,289491,53.3878059387207,7.476055761411095e-05
144945,144946,144945,289891,53.451897859573364,7.365727497367591e-05
145145,145146,145145,290291,53.51666784286499,7.357659630272369e-05
145345,145346,145345,290691,53.57898497581482,7.292173248920831e-05
145546,145547,145546,291093,53.64110493659973,7.244695901604426e-05
145746,145747,145746,291493,53.70946002006531,7.150598810829629e-05
145946,145947,145946,291893,53.77152991294861,7.190262367510043e-05
146146,146147,146146,292293,53.83381414413452,7.091588383066895e-05
146346,146347,146346,292693,53.89574980735779,7.070186259317419e-05
146547,146548,146547,293095,53.96789574623108,6.980497573878492e-05
146747,146748,146747,293495,54.04617786407471,6.865439936298941e-05
146947,146948,146947,293895,54.1124370098114,7.029299049303743e-05
147147,147148,147147,294295,54.175220012664795,6.813462482619054e-05
147347,147348,147347,294695,54.24706792831421,6.761817277109127e-05
147548,147549,147548,295097,54.31199598312378,7.229710238902535e-05
147748,147749,147748,295497,54.37777805328369,6.618031424898521e-05
147948,147949,147948,295897,54.44094896316528,7.590045673125923e-05
148148,148149,148148,296297,54.504169940948486,6.563465571551925e-05
148348,148349,148348,296697,54.56735706329346,6.42599719903498e-05
148549,148550,148549,297099,54.63081693649292,6.593522288403782e-05
148749,148750,148749,297499,54.70032286643982,6.325158291457148e-05
148949,148950,148949,297899,54.76271080970764,6.357234306901179e-05
149149,149150,149149,298299,54.82577109336853,6.247986568539039e-05
149349,149350,149349,298699,54.88940501213074,7.559154613027303e-05
149550,149551,149550,299101,54.95313382148743,6.155013848095213e-05
149750,149751,149750,299501,55.016305923461914,6.121710661037563e-05
149950,149951,149950,299901,55.07974410057068,6.0689623661091054e-05
150150,150151,150150,300301,55.14231204986572,6.043805943900582e-05
150350,150351,150350,300701,55.21337080001831,6.389810328122044e-05
150551,150552,150551,301103,55.277997732162476,5.9505227477730134e-05
150751,150752,150751,301503,55.34183192253113,5.8558413861974257e-05
150951,150952,150951,301903,55.405694007873535,5.7695682747601486e-05
151151,151152,151151,302303,55.46881175041199,5.821052533332896e-05
151351,151352,151351,302703,55.532275915145874,7.055893709483815e-05
151552,151553,151552,303105,55.59876894950867,5.663685507499758e-05
151752,151753,151752,303505,55.66244101524353,6.46073997313166e-05
151952,151953,151952,303905,55.733946800231934,5.5498772173815967e-05
152152,152153,152152,304305,55.7957718372345,5.685822681347772e-05
152352,152353,152352,304705,55.861167907714844,6.335323923990663e-05
152553,152554,152553,305107,55.92494177818298,5.4643817163495384e-05
152753,152754,152753,305507,55.988762855529785,5.3472253407157616e-05
152953,152954,152953,305907,56.050609827041626,6.576487144240396e-05
153153,153154,153153,306307,56.12912106513977,5.344167851059788e-05
153353,153354,153353,306707,56.20781898498535,5.296115449199122e-05
153554,153555,153554,307109,56.272642850875854,5.247286026512555e-05
153754,153755,153754,307509,56.33785891532898,5.401221460655201e-05
153954,153955,153954,307909,56.40167307853699,5.208557055054735e-05
154154,154155,154154,308309,56.466338872909546,6.0809321170391063e-05
154354,154355,154354,308709,56.53033185005188,5.123187742822885e-05
154555,154556,154555,309111,56.59428882598877,5.064422381215114e-05
154755,154756,154755,309511,56.65813899040222,4.96468975112124e-05
154955,154956,154955,309911,56.73147487640381,4.9450662490294586e-05
155155,155156,155155,310311,56.79628801345825,4.952027156469974e-05
155355,155356,155355,310711,56.86235594749451,4.8499185328768754e-05
155556,155557,155556,311113,56.92832589149475,4.820176692408304e-05
155756,155757,155756,311513,56.9948890209198,4.8707388151135155e-05
155956,155957,155956,311913,57.05992603302002,4.718544870468868e-05
156156,156157,156156,312313,57.127805948257446,4.736685199020415e-05
156356,156357,156356,312713,57.1995689868927,4.903274832668688e-05
156557,156558,156557,313115,57.26588296890259,4.598288153326294e-05
156757,156758,156757,313515,57.331905126571655,5.488755141257684e-05
156957,156958,156957,313915,57.397989988327026,4.54819404849507e-05
157157,157158,157157,314315,57.4629020690918,4.530840716274448e-05
157357,157358,157357,314715,57.527161836624146,4.457333206695802e-05
157558,157559,157558,315117,57.59168291091919,4.4149445541578824e-05
157758,157759,157758,315517,57.65585494041443,4.4886397726325016e-05
157958,157959,157958,315917,57.73095512390137,4.377038644154132e-05
158158,158159,158158,316317,57.79482984542847,4.340185998662825e-05
158358,158359,158358,316717,57.85910892486572,4.295343654740348e-05
158559,158560,158559,317119,57.92373299598694,4.334195481395645e-05
158759,158760,158759,317519,57.98809790611267,4.236399749430526e-05
158959,158960,158959,317919,58.05095887184143,4.219640791919178e-05
159159,159160,159159,318319,58.11596083641052,4.211685264975678e-05
159359,159360,159359,318719,58.187220096588135,4.1497683069042795e-05
159560,159561,159560,319121,58.27242994308472,4.1228167840209144e-05
159760,159761,159760,319521,58.34707999229431,4.10776669055825e-05
159960,159961,159960,319921,58.4101357460022,4.050731097462188e-05
160160,160161,160160,320321,58.47441792488098,4.7889674645347517e-05
160360,160361,160360,320721,58.53868293762207,4.16235000580039e-05
160561,160562,160561,321123,58.60433888435364,3.942638949358079e-05
160761,160762,160761,321523,58.67130398750305,3.957494080266781e-05
160961,160962,160961,321923,58.74077892303467,3.89679406236358e-05
161161,161162,161161,322323,58.80508804321289,3.8759420575968616e-05
161361,161362,161361,322723,58.8703179359436,4.775163004515131e-05
161562,161563,161562,323125,58.93441104888916,3.781668470206771e-05
161762,161763,161762,323525,59.00938296318054,3.774555158683405e-05
161962,161963,161962,323925,59.11662793159485,3.739959460676e-05
162162,162163,162162,324325,59.21823000907898,3.6878560468410325e-05
162362,162363,162362,324725,59.29449200630188,3.8942412863417256e-05
162563,162564,162563,325127,59.37088108062744,4.029531178497658e-05
162763,162764,162763,325527,59.44822883605957,3.6046697066374674e-05
162963,162964,162963,325927,59.52490496635437,4.7983650867463446e-05
163163,163164,163163,326327,59.60086512565613,3.61455247369907e-05
163363,163364,163363,326727,59.67850089073181,3.542471727001728e-05
163564,163565,163564,327129,59.754008769989014,3.8572733388331275e-05
163764,163765,163764,327529,59.8246009349823,3.485210946053706e-05
163964,163965,163964,327929,59.89461302757263,4.287172400246614e-05
164164,164165,164164,328329,59.96113681793213,3.8762512938776434e-05
164364,164365,164364,328729,60.02522301673889,3.479940562906852e-05
164565,164566,164565,329131,60.08925914764404,3.3740316865595474e-05
164765,164766,164765,329531,60.15424394607544,3.685925617577931e-05
164965,164966,164965,329931,60.22800397872925,3.3036973596040614e-05
165165,165166,165165,330331,60.29315900802612,3.316160679008095e-05
165365,165366,165365,330731,60.368370056152344,3.25970272668575e-05
165566,165567,165566,331133,60.44872498512268,3.224205119466628e-05
165766,165767,165766,331533,60.51491594314575,3.207661430411782e-05
165966,165967,165966,331933,60.580278158187866,3.793423523419757e-05
166166,166167,166166,332333,60.645028829574585,3.384054230804874e-05
166366,166367,166366,332733,60.71939301490784,3.135095878803887e-05
166567,166568,166567,333135,60.78639483451843,3.073874549646531e-05
166767,166768,166767,333535,60.851516008377075,3.0889570161048815e-05
166967,166968,166967,333935,60.91677808761597,3.019311715120866e-05
167167,167168,167167,334335,60.983717918395996,3.0501004857513827e-05
167367,167368,167367,334735,61.04768180847168,2.9898613313477533e-05
167568,167569,167568,335137,61.114166021347046,2.9994861530625792e-05
167768,167769,167768,335537,61.178767919540405,2.9485648890471344e-05
167968,167969,167968,335937,61.255982875823975,2.9270166525021802e-05
168168,168169,168168,336337,61.321362018585205,2.921109351677763e-05
168368,168369,168368,336737,61.38575077056885,2.90116860066858e-05
168569,168570,168569,337139,61.44992685317993,2.8699747176317407e-05
168769,168770,168769,337539,61.51311683654785,2.8539617010191023e-05
168969,168970,168969,337939,61.578359842300415,2.8251129845524487e-05
169169,169170,169169,338339,61.64324998855591,2.7867727534734185e-05
169369,169370,169369,338739,61.71668791770935,2.7733557361142062e-05
169570,169571,169570,339141,61.78283190727234,2.750858122068453e-05
169770,169771,169770,339541,61.849544048309326,2.7137618176971612e-05
169970,169971,169970,339941,61.91417098045349,2.6794160439180114e-05
170170,170171,170170,340341,61.97864890098572,2.6811890973119676e-05
170370,170371,170370,340741,62.043203830718994,2.6555661475857818e-05
170571,170572,170571,341143,62.107940912246704,2.9500873688809605e-05
170771,170772,170771,341543,62.173826932907104,2.5924761213001017e-05
170971,170972,170971,341943,62.24441409111023,2.624943519500069e-05
171171,171172,171171,342343,62.310006856918335,2.9446236434885365e-05
171371,171372,171371,342743,62.37576389312744,2.560293982990846e-05
171572,171573,171572,343145,62.44026589393616,2.513015187492961e-05
171772,171773,171772,343545,62.51561498641968,2.4978042069918828e-05
171972,171973,171972,343945,62.594982862472534,2.5045130636507086e-05
172172,172173,172172,344345,62.66012907028198,2.474149762171939e-05
172372,172373,172372,344745,62.730653047561646,2.5613411048983442e-05
172573,172574,172573,345147,62.797780990600586,2.4236135827244624e-05
172773,172774,172773,345547,62.86223006248474,2.4169759976764823e-05
172973,172974,172973,345947,62.92622900009155,2.4051798011853342e-05
173173,173174,173173,346347,62.99005079269409,2.3741525919557993e-05
173373,173374,173373,346747,63.05427575111389,2.3533094468429617e-05
173574,173575,173574,347149,63.119022846221924,2.3333359789382096e-05
173774,173775,173774,347549,63.18737292289734,2.3569148767226634e-05
173974,173975,173974,347949,63.25644493103027,2.2880205090162753e-05
174174,174175,174174,348349,63.32080101966858,2.3120261769558065e-05
174374,174375,174374,348749,63.38904094696045,2.2905250313062878e-05
174575,174576,174575,349151,63.45304298400879,2.2577638718334215e-05
174775,174776,174775,349551,63.518380880355835,2.2471148524402526e-05
174975,174976,174975,349951,63.5821897983551,2.2309096282710858e-05
175175,175176,175175,350351,63.64787697792053,2.912658334063008e-05
175375,175376,175375,350751,63.72519493103027,2.1911951693096282e-05
175576,175577,175576,351153,63.79039001464844,2.256764661607228e-05
175776,175777,175776,351553,63.855058908462524,2.138114943855892e-05
175976,175977,175976,351953,63.91907787322998,2.4373396124255646e-05
176176,176177,176176,352353,63.985265016555786,2.161799147950915e-05
176376,176377,176376,352753,64.05079293251038,2.089273971244562e-05
176577,176578,176577,353155,64.11640501022339,2.0806740788502674e-05
176777,176778,176777,353555,64.18282508850098,2.07193010267432e-05
176977,176978,176977,353955,64.2518539428711,2.048667615696006e-05
177177,177178,177177,354355,64.31975507736206,2.0511692739726507e-05
177377,177378,177377,354755,64.38561272621155,2.0141987445730457e-05
177578,177579,177578,355157,64.45244288444519,1.989507723900504e-05
177778,177779,177778,355557,64.51903295516968,1.9928621446447497e-05
177978,177979,177978,355957,64.58805394172668,1.9508542716461334e-05
178178,178179,178178,356357,64.67279291152954,2.0310836983707785e-05
178378,178379,178378,356757,64.75750780105591,1.9352746862370587e-05
178579,178580,178579,357159,64.8254930973053,1.911042073546386e-05
178779,178780,178779,357559,64.89472484588623,1.91750904262206e-05
178979,178980,178979,357959,64.96158003807068,2.1901674461263277e-05
179179,179180,179179,358359,65.02745389938354,1.8621537103763344e-05
179379,179380,179379,358759,65.09559988975525,2.037920447658315e-05
179580,179581,179580,359161,65.16385889053345,1.8353550081400794e-05
179780,179781,179780,359561,65.23386287689209,2.2428986924702833e-05
179980,179981,179980,359961,65.30101108551025,2.0689661561384377e-05
180180,180181,180180,360361,65.36806893348694,1.8767157968672402e-05
180380,180381,180380,360761,65.43474888801575,2.0330757195062246e-05
180581,180582,180581,361163,65.50270175933838,1.7810137691829764e-05
180781,180782,180781,361563,65.56873393058777,1.8084036402242967e-05
180981,180982,180981,361963,65.63504600524902,1.7376074792103355e-05
181181,181182,181181,362363,65.71305394172668,1.7204857063559666e-05
181381,181382,181381,362763,65.78161478042603,1.7208030494893437e-05
181582,181583,181582,363165,65.8492329120636,1.6788371424648805e-05
181782,181783,181782,363565,65.91516184806824,2.0364829746733358e-05
181982,181983,181982,363965,65.981684923172,1.6613792954431888e-05
182182,182183,182182,364365,66.05102181434631,2.0048395887529046e-05
182382,182383,182382,364765,66.12112188339233,1.656824197009149e-05
182583,182584,182583,365167,66.19386506080627,1.6306846581755764e-05
182783,182784,182783,365567,66.26604390144348,1.78045986804804e-05
182983,182984,182983,365967,66.33778214454651,1.6052021123486903e-05
183183,183184,183183,366367,66.40486788749695,1.577891809696849e-05
183383,183384,183383,366767,66.47479605674744,1.8559509973725917e-05
183584,183585,183584,367169,66.5418770313263,1.5682180395720893e-05
183784,183785,183784,367569,66.60933208465576,1.8699574711081203e-05
183984,183985,183984,367969,66.68280100822449,1.5886148912080177e-05
184184,184185,184184,368369,66.75842380523682,1.5351065367949774e-05
184384,184385,184384,368769,66.83759593963623,1.5053285110781263e-05
184585,184586,184585,369171,66.91258597373962,1.5333486812535775e-05
184785,184786,184785,369571,66.97915697097778,1.4918711384618207e-05
184985,184986,184985,369971,67.04396176338196,1.4821562690640722e-05
185185,185186,185185,370371,67.1088080406189,1.4990328260285264e-05
185385,185386,185385,370771,67.1764030456543,1.4639564064734033e-05
185586,185587,185586,371173,67.25073289871216,1.4434035462804549e-05
185786,185787,185786,371573,67.31569600105286,1.4941743980228804e-05
185986,185987,185986,371973,67.38059878349304,1.4365393082150865e-05
186186,186187,186186,372373,67.44461584091187,1.7308601515036298e-05
186386,186387,186386,372773,67.50939869880676,1.71825674589924e-05
186587,186588,186587,373175,67.57413482666016,1.3913155568583969e-05
186787,186788,186787,373575,67.63936686515808,1.368197728838774e-05
186987,186988,186987,373975,67.71131610870361,1.3752062352254422e-05
187187,187188,187187,374375,67.77591609954834,1.3631643372238521e-05
187387,187388,187387,374775,67.84269189834595,1.3453417608744274e-05
187588,187589,187588,375177,67.908038854599,1.3320052046459817e-05
187788,187789,187788,375577,67.97315192222595,1.323098971307281e-05
187988,187989,187988,375977,68.03631806373596,1.3100265765192315e-05
188188,188189,188188,376377,68.10023188591003,1.3183846584495748e-05
188388,188389,188388,376777,68.16347885131836,1.3319921349469084e-05
188589,188590,188589,377179,68.23658990859985,1.4336921071725118e-05
188789,188790,188789,377579,68.30802202224731,1.2705460722879558e-05
188989,188990,188989,377979,68.37816405296326,1.264104266709439e-05
189189,189190,189189,378379,68.4495370388031,1.3926855003709742e-05
189389,189390,189389,378779,68.52197980880737,1.2383667320245366e-05
189590,189591,189590,379181,68.5885419845581,1.2706340624772496e-05
189790,189791,189790,379581,68.65622186660767,1.266978576459434e-05
189990,189991,189990,379981,68.73620676994324,1.2127715141789028e-05
190190,190191,190190,380381,68.80706000328064,1.2445643558535981e-05
190390,190391,190390,380781,68.87924790382385,1.1960891804182084e-05
190591,190592,190591,381183,68.96231198310852,1.4877585302126947e-05
190791,190792,190791,381583,69.0361099243164,1.1743689272225778e-05
190991,190992,190991,381983,69.10325789451599,1.1649748350356186e-05
191191,191192,191191,382383,69.16712999343872,1.164688106998137e-05
191391,191392,191391,382783,69.23829793930054,1.145533809433758e-05
191592,191593,191592,383185,69.30279088020325,1.1338258257270108e-05
191792,191793,191792,383585,69.36959075927734,1.1319544318632654e-05
191992,191993,191992,383985,69.43322777748108,1.1457282133390425e-05
192192,192193,192192,384385,69.49620580673218,1.1100461992951215e-05
192392,192393,192392,384785,69.55876302719116,1.1086976985472297e-05
192593,192594,192593,385187,69.6212067604065,1.0957293136732626e-05
192793,192794,192793,385587,69.69252896308899,1.07879278532948e-05
192993,192994,192993,385987,69.75531888008118,1.0715072531270601e-05
193193,193194,193193,386387,69.81832098960876,1.2122374718399783e-05
193393,193394,193393,386787,69.88072896003723,1.0578543209430875e-05
193594,193595,193594,387189,69.94338989257812,1.054329478714354e-05
193794,193795,193794,387589,70.00741696357727,1.053031180390229e-05
193994,193995,193994,387989,70.06862378120422,1.032134338534349e-05
194194,194195,194194,388389,70.13046097755432,1.030193891597823e-05
194394,194395,194394,388789,70.20085883140564,1.0129029535373847e-05
194595,194596,194595,389191,70.2649998664856,1.1552154485315494e-05
194795,194796,194795,389591,70.32689595222473,1.1472556047323885e-05
194995,194996,194995,389991,70.38975501060486,1.0098606268895488e-05
195195,195196,195195,390391,70.4525740146637,9.999383471381214e-06
195395,195396,195395,390791,70.51463794708252,9.827421135950824e-06
195596,195597,195596,391193,70.57807183265686,9.718608837140094e-06
195796,195797,195796,391593,70.63890480995178,9.585797405985884e-06
195996,195997,195996,391993,70.70722579956055,9.574691747991579e-06
196196,196197,196196,392393,70.77061486244202,9.503125260895581e-06
196396,196397,196396,392793,70.83236575126648,9.346109612510969e-06
196597,196598,196597,393195,70.89644384384155,9.361326313287235e-06
196797,196798,196797,393595,70.95899200439453,9.342742635101381e-06
196997,196998,196997,393995,71.0295958518982,9.243965484742884e-06
197197,197198,197197,394395,71.11311602592468,1.1076624156361041e-05
197397,197398,197397,394795,71.19796991348267,9.05124975085931e-06
197598,197599,197598,395197,71.26477980613708,9.072644958385547e-06
197798,197799,197798,395597,71.3312668800354,8.985084254281026e-06
197998,197999,197998,395997,71.39227890968323,8.808044456682028e-06
198198,198199,198198,396397,71.45394492149353,8.782904120895869e-06
198398,198399,198398,396797,71.51484894752502,8.958245860313968e-06
198599,198600,198599,397199,71.57707595825195,1.0813126203080966e-05
198799,198800,198799,397599,71.63833713531494,8.695899320432537e-06
198999,199000,198999,397999,71.71731781959534,8.507299181512479e-06
199199,199200,199199,398399,71.79246807098389,9.596035632475866e-06
199399,199400,199399,398799,71.85807704925537,8.337505548866718e-06
199600,199601,199600,399201,71.92366909980774,8.367295817649188e-06
199800,199801,199800,399601,71.98608899116516,8.258122890338423e-06
200000,200001,200000,400001,72.0513129234314,8.177125483508661e-06


==> plot_data/quadratic_minimax_problem_n500_alpha00001/eag-c.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007338523864746094,30.358106049564984
100,201,0,201,0.1048591136932373,6.493450136861272
200,401,0,401,0.18327093124389648,3.177507289781097
300,601,0,601,0.2569589614868164,2.0200540878033326
400,801,0,801,0.32503795623779297,1.4973870829094331
501,1003,0,1003,0.3924698829650879,1.2077208389856788
601,1203,0,1203,0.467242956161499,0.989316830878674
701,1403,0,1403,0.5347979068756104,0.8233653449454962
801,1603,0,1603,0.6016550064086914,0.7043998342234868
901,1803,0,1803,0.6758987903594971,0.6522505355825833
1001,2003,0,2003,0.7689969539642334,0.5753800609690223
1101,2203,0,2203,0.841871976852417,0.5126912067869833
1201,2403,0,2403,0.9125769138336182,0.45466603800015104
1301,2603,0,2603,0.9789519309997559,0.43864535988365744
1401,2803,0,2803,1.0438988208770752,0.3960641705985294
1502,3005,0,3005,1.106048822402954,0.36800860768665794
1602,3205,0,3205,1.17116379737854,0.3439575007189226
1702,3405,0,3405,1.2306506633758545,0.3210982972833532
1802,3605,0,3605,1.2873649597167969,0.29907689517926345
1902,3805,0,3805,1.3432068824768066,0.27792100029923855
2002,4005,0,4005,1.3986527919769287,0.2664558386879063
2102,4205,0,4205,1.45784592628479,0.2569607227315315
2202,4405,0,4405,1.5139529705047607,0.2525404359365554
2302,4605,0,4605,1.5709469318389893,0.24348000315202725
2402,4805,0,4805,1.6382169723510742,0.2294540764756248
2503,5007,0,5007,1.7050459384918213,0.22096504244071943
2603,5207,0,5207,1.773900032043457,0.20933355408296336
2703,5407,0,5407,1.8667550086975098,0.2003706010584758
2803,5607,0,5607,1.9311738014221191,0.19409314830020635
2903,5807,0,5807,1.9882957935333252,0.18758713015755707
3003,6007,0,6007,2.0513458251953125,0.17936651120038055
3103,6207,0,6207,2.127657890319824,0.17151651282570124
3203,6407,0,6407,2.1956210136413574,0.16648509708971368
3303,6607,0,6607,2.2529866695404053,0.16243960781487446
3403,6807,0,6807,2.3101680278778076,0.15685359329638138
3504,7009,0,7009,2.3786909580230713,0.15145019004331028
3604,7209,0,7209,2.443467855453491,0.1489031461598561
3704,7409,0,7409,2.5167369842529297,0.14421961397682728
3804,7609,0,7609,2.580432891845703,0.13933800424958753
3904,7809,0,7809,2.6425321102142334,0.13643824780422475
4004,8009,0,8009,2.700342893600464,0.13412666254906758
4104,8209,0,8209,2.766908884048462,0.13205883724844866
4204,8409,0,8409,2.832261800765991,0.13040429550311303
4304,8609,0,8609,2.893021821975708,0.12518696134067447
4404,8809,0,8809,2.9549429416656494,0.12120779775877681
4505,9011,0,9011,3.015314817428589,0.11793867947372813
4605,9211,0,9211,3.078489065170288,0.11514283592056614
4705,9411,0,9411,3.1398088932037354,0.11160654494049432
4805,9611,0,9611,3.200960874557495,0.10996968850546354
4905,9811,0,9811,3.2702958583831787,0.10801958387209429
5005,10011,0,10011,3.331705093383789,0.10548909035279165
5105,10211,0,10211,3.3897409439086914,0.10221391810925645
5205,10411,0,10411,3.4467618465423584,0.1010294983374759
5305,10611,0,10611,3.51163387298584,0.09970007478805022
5405,10811,0,10811,3.585360050201416,0.09881179743007851
5506,11013,0,11013,3.649481773376465,0.09570070788914996
5606,11213,0,11213,3.7157979011535645,0.09374846854657858
5706,11413,0,11413,3.792156934738159,0.0940464827703189
5806,11613,0,11613,3.869720935821533,0.09174830703767393
5906,11813,0,11813,3.9345688819885254,0.08924541998206977
6006,12013,0,12013,3.9989490509033203,0.08850053343835623
6106,12213,0,12213,4.063514947891235,0.08687853786897974
6206,12413,0,12413,4.132277011871338,0.0852908463906032
6306,12613,0,12613,4.197494029998779,0.08284840439442
6406,12813,0,12813,4.289319753646851,0.08079935314962451
6507,13015,0,13015,4.394905090332031,0.07899258511759796
6607,13215,0,13215,4.495901823043823,0.07787498942184042
6707,13415,0,13415,4.592221736907959,0.07632367495431167
6807,13615,0,13615,4.670635938644409,0.0759460752235735
6907,13815,0,13815,4.756820917129517,0.07584697075460098
7007,14015,0,14015,4.8478288650512695,0.07453511218689807
7107,14215,0,14215,4.9284327030181885,0.07336599203349224
7207,14415,0,14415,4.988650798797607,0.07340253199369183
7307,14615,0,14615,5.050331115722656,0.07290157202157466
7407,14815,0,14815,5.11274790763855,0.07153615631743382
7508,15017,0,15017,5.1749889850616455,0.06985831748037355
7608,15217,0,15217,5.237165927886963,0.06893807749832585
7708,15417,0,15417,5.302053689956665,0.06797271403369433
7808,15617,0,15617,5.364564895629883,0.06723807472828548
7908,15817,0,15817,5.446307897567749,0.06630195961927388
8008,16017,0,16017,5.50873589515686,0.06524329737100265
8108,16217,0,16217,5.570310831069946,0.06456382281314012
8208,16417,0,16417,5.634135007858276,0.0629767120173992
8308,16617,0,16617,5.695662021636963,0.06146963170293714
8408,16817,0,16817,5.757710933685303,0.06105128835195123
8509,17019,0,17019,5.819674968719482,0.06059338471273952
8609,17219,0,17219,5.881176948547363,0.0598431014110998
8709,17419,0,17419,5.951133966445923,0.05911898717921063
8809,17619,0,17619,6.0178139209747314,0.05873404789957919
8909,17819,0,17819,6.078969955444336,0.05863766599263057
9009,18019,0,18019,6.1383748054504395,0.057894940882902264
9109,18219,0,18219,6.197645902633667,0.057150907916840105
9209,18419,0,18419,6.257231950759888,0.05711564635271991
9309,18619,0,18619,6.3178510665893555,0.05677012916598475
9409,18819,0,18819,6.393862724304199,0.055767262439525386
9510,19021,0,19021,6.470256090164185,0.05484772960673859
9610,19221,0,19221,6.5312769412994385,0.05423758049087429
9710,19421,0,19421,6.59601092338562,0.05381902319484677
9810,19621,0,19621,6.664269924163818,0.05310568959428667
9910,19821,0,19821,6.724441051483154,0.05251756126365489
10010,20021,0,20021,6.785211801528931,0.05202112985688373
10110,20221,0,20221,6.842751979827881,0.05113442285242482
10210,20421,0,20421,6.903863906860352,0.050170814328476504
10310,20621,0,20621,6.963104009628296,0.049559061615367966
10410,20821,0,20821,7.022135019302368,0.04954515670001858
10511,21023,0,21023,7.080155849456787,0.04946131894130097
10611,21223,0,21223,7.138887882232666,0.04895753711135221
10711,21423,0,21423,7.197191953659058,0.04858863825436371
10811,21623,0,21623,7.255569934844971,0.048386863253826226
10911,21823,0,21823,7.313831806182861,0.04801247066539187
11011,22023,0,22023,7.374481916427612,0.04717683486265263
11111,22223,0,22223,7.440400123596191,0.04645725156277679
11211,22423,0,22423,7.507816791534424,0.046240757861431524
11311,22623,0,22623,7.573101997375488,0.04587148810738096
11411,22823,0,22823,7.632601976394653,0.044945876521436924
11512,23025,0,23025,7.691704034805298,0.04424786232894383
11612,23225,0,23225,7.754400968551636,0.044086267051293995
11712,23425,0,23425,7.815758943557739,0.04367249224835261
11812,23625,0,23625,7.875954866409302,0.04304100055155869
11912,23825,0,23825,7.938638925552368,0.04285121358920512
12012,24025,0,24025,7.997853755950928,0.04293031836131672
12112,24225,0,24225,8.057036876678467,0.042827151959074335
12212,24425,0,24425,8.11679482460022,0.04247002207493495
12312,24625,0,24625,8.17540192604065,0.04221675633652936
12412,24825,0,24825,8.233855962753296,0.041896213469312986
12513,25027,0,25027,8.293205976486206,0.04118777502728249
12613,25227,0,25227,8.351789951324463,0.04060350594824031
12713,25427,0,25427,8.409115076065063,0.04059383070041453
12813,25627,0,25627,8.468544006347656,0.0406103244830042
12913,25827,0,25827,8.54479694366455,0.040222491379367314
13013,26027,0,26027,8.61377501487732,0.039714453252492746
13113,26227,0,26227,8.67233681678772,0.03924484088077877
13213,26427,0,26427,8.729663848876953,0.03874781288387245
13313,26627,0,26627,8.78616189956665,0.03838444957203775
13413,26827,0,26827,8.843533039093018,0.03819813983779849
13514,27029,0,27029,8.901780843734741,0.03789297249811301
13614,27229,0,27229,8.962234735488892,0.037510380513344974
13714,27429,0,27429,9.02123212814331,0.03739576969169575
13814,27629,0,27629,9.077712774276733,0.03753807996642545
13914,27829,0,27829,9.136817932128906,0.037761064009475924
14014,28029,0,28029,9.200476884841919,0.03774299003687111
14114,28229,0,28229,9.257323980331421,0.03734377079737995
14214,28429,0,28429,9.314065933227539,0.03685797290551392
14314,28629,0,28629,9.373105764389038,0.03637333766629744
14414,28829,0,28829,9.43221402168274,0.035834183972586406
14515,29031,0,29031,9.491670846939087,0.03534846475132066
14615,29231,0,29231,9.549797773361206,0.03500427217938494
14715,29431,0,29431,9.608212947845459,0.034833754704270595
14815,29631,0,29631,9.668735980987549,0.03472558058408438
14915,29831,0,29831,9.728851795196533,0.0344579493769088
15015,30031,0,30031,9.787823915481567,0.03409658761431861
15115,30231,0,30231,9.848418951034546,0.033864512486068934
15215,30431,0,30431,9.90700387954712,0.03373298390191974
15315,30631,0,30631,9.966417789459229,0.033565919555018066
15415,30831,0,30831,10.026336908340454,0.03333822902925942
15516,31033,0,31033,10.086672067642212,0.03310810334141374
15616,31233,0,31233,10.14652681350708,0.03290241684355466
15716,31433,0,31433,10.207526922225952,0.03279683987739169
15816,31633,0,31633,10.270567893981934,0.03289865625135315
15916,31833,0,31833,10.329388856887817,0.033026082338673164
16016,32033,0,32033,10.38875699043274,0.03285544629813413
16116,32233,0,32233,10.450913906097412,0.03233679960845518
16216,32433,0,32433,10.512165784835815,0.03175743640624014
16316,32633,0,32633,10.57535195350647,0.0313589115493064
16416,32833,0,32833,10.644627809524536,0.03106260820852627
16517,33035,0,33035,10.71979284286499,0.03073466043598325
16617,33235,0,33235,10.790297985076904,0.03048290037772186
16717,33435,0,33435,10.849900007247925,0.03043170726562068
16817,33635,0,33635,10.909243822097778,0.030428124358431837
16917,33835,0,33835,10.969339847564697,0.030290627457881737
17017,34035,0,34035,11.028676986694336,0.030140520317679664
17117,34235,0,34235,11.090879917144775,0.030153790900751137
17217,34435,0,34435,11.15061092376709,0.030184430609046603
17317,34635,0,34635,11.20901870727539,0.02999649717802615
17417,34835,0,34835,11.267674922943115,0.02966875149034884
17518,35037,0,35037,11.326984882354736,0.029358972453177232
17618,35237,0,35237,11.391083002090454,0.029084109708836348
17718,35437,0,35437,11.451097965240479,0.028852334473472123
17818,35637,0,35637,11.509781837463379,0.028708187377669923
17918,35837,0,35837,11.569560050964355,0.028609977284311902
18018,36037,0,36037,11.629380941390991,0.02839569974855992
18118,36237,0,36237,11.686888933181763,0.028051743783738453
18218,36437,0,36437,11.746120929718018,0.027794924366970925
18318,36637,0,36637,11.804812908172607,0.02767626478551603
18418,36837,0,36837,11.866729974746704,0.027557560636513892
18519,37039,0,37039,11.9271080493927,0.027420607830366865
18619,37239,0,37239,11.98679804801941,0.027333681249766553
18719,37439,0,37439,12.04630970954895,0.027260816004700896
18819,37639,0,37639,12.10727071762085,0.027170525439944963
18919,37839,0,37839,12.171175956726074,0.02710689243810413
19019,38039,0,38039,12.236690759658813,0.027046412034836546
19119,38239,0,38239,12.31233286857605,0.026898664181944625
19219,38439,0,38439,12.396403789520264,0.02665161118030196
19319,38639,0,38639,12.47156286239624,0.0263749707542372
19419,38839,0,38839,12.532453060150146,0.026129407395588417
19520,39041,0,39041,12.593605041503906,0.025920630669609878
19620,39241,0,39241,12.65378189086914,0.02576008635326071
19720,39441,0,39441,12.711575031280518,0.025699577917577262
19820,39641,0,39641,12.778547763824463,0.025716225642238483
19920,39841,0,39841,12.854021787643433,0.0256549453913596
20020,40041,0,40041,12.924274921417236,0.02544924349488219
20120,40241,0,40241,12.98586893081665,0.02523030938098149
20220,40441,0,40441,13.043525695800781,0.025138858919045336
20320,40641,0,40641,13.101611852645874,0.025159752558046682
20420,40841,0,40841,13.169097900390625,0.025179805492266012
20521,41043,0,41043,13.23695683479309,0.025125779467433156
20621,41243,0,41243,13.294464826583862,0.02499131737954627
20721,41443,0,41443,13.35439682006836,0.02478939281786251
20821,41643,0,41643,13.413368940353394,0.02457934912691372
20921,41843,0,41843,13.47173810005188,0.02445842505472295
21021,42043,0,42043,13.52979588508606,0.024416880307477993
21121,42243,0,42243,13.588018894195557,0.024314961087311328
21221,42443,0,42443,13.645341873168945,0.024084617053506983
21321,42643,0,42643,13.703597068786621,0.023840979818897906
21421,42843,0,42843,13.76629090309143,0.023718554677641834
21522,43045,0,43045,13.82770299911499,0.02369414846280551
21622,43245,0,43245,13.88621473312378,0.023677310346186517
21722,43445,0,43445,13.944880723953247,0.023639853778932216
21822,43645,0,43645,14.001960754394531,0.0235796095178903
21922,43845,0,43845,14.06073784828186,0.023468162526206347
22022,44045,0,44045,14.122384071350098,0.02327975972881778
22122,44245,0,44245,14.202729940414429,0.02307577106376024
22222,44445,0,44445,14.271947860717773,0.022983367189758165
22322,44645,0,44645,14.335178852081299,0.023017729620847555
22422,44845,0,44845,14.392729043960571,0.023043878449885407
22523,45047,0,45047,14.45179009437561,0.0229619275014972
22623,45247,0,45247,14.515070915222168,0.02280308834227863
22723,45447,0,45447,14.576184034347534,0.02262047460606344
22823,45647,0,45647,14.636901140213013,0.0224262429231567
22923,45847,0,45847,14.69775390625,0.02224427244348681
23023,46047,0,46047,14.75629997253418,0.02211054437688033
23123,46247,0,46247,14.81484580039978,0.02199153129407551
23223,46447,0,46447,14.889219045639038,0.021824858028409087
23323,46647,0,46647,14.987433910369873,0.02164568683903626
23423,46847,0,46847,15.05506181716919,0.021555633631657745
23524,47049,0,47049,15.114195823669434,0.021580969113077778
23624,47249,0,47249,15.171954870223999,0.021636693489933006
23724,47449,0,47449,15.230187892913818,0.02164022553079419
23824,47649,0,47649,15.288805723190308,0.021575359795960713
23924,47849,0,47849,15.348649978637695,0.02144930247069973
24024,48049,0,48049,15.409942865371704,0.021288811201526803
24124,48249,0,48249,15.47545599937439,0.021156154408774882
24224,48449,0,48449,15.544080018997192,0.0210849817338012
24324,48649,0,48649,15.605079889297485,0.021034993926427017
24424,48849,0,48849,15.66410493850708,0.020957618113806267
24525,49051,0,49051,15.722323894500732,0.020858089013003407
24625,49251,0,49251,15.783370971679688,0.020762111311030666
24725,49451,0,49451,15.841320753097534,0.02067131968520767
24825,49651,0,49651,15.899703025817871,0.02058622266616884
24925,49851,0,49851,15.954837799072266,0.020498677311905744
25025,50051,0,50051,16.011334896087646,0.020371107425787387
25125,50251,0,50251,16.067996740341187,0.020186823664900336
25225,50451,0,50451,16.12308979034424,0.02001152416491854
25325,50651,0,50651,16.17862296104431,0.019940533820777578
25425,50851,0,50851,16.234494924545288,0.019981704092350745
25526,51053,0,51053,16.289469957351685,0.02004673463452749
25626,51253,0,51253,16.344926834106445,0.020052145884274925
25726,51453,0,51453,16.39993190765381,0.019978373039478668
25826,51653,0,51653,16.456936836242676,0.01984050088941162
25926,51853,0,51853,16.5141818523407,0.019669868507508348
26026,52053,0,52053,16.572908878326416,0.01950550006373346
26126,52253,0,52253,16.628321886062622,0.019380214861140273
26226,52453,0,52453,16.686492919921875,0.019309285231855437
26326,52653,0,52653,16.74790072441101,0.019283459901069413
26426,52853,0,52853,16.808418035507202,0.019280157726637968
26527,53055,0,53055,16.86550807952881,0.01927425484247622
26627,53255,0,53255,16.922626972198486,0.019232670284111807
26727,53455,0,53455,16.980002880096436,0.01913339643183112
26827,53655,0,53655,17.03870987892151,0.019000087467065527
26927,53855,0,53855,17.10796284675598,0.018882153540277495
27027,54055,0,54055,17.173404932022095,0.01879275596720773
27127,54255,0,54255,17.228379726409912,0.018709809952036083
27227,54455,0,54455,17.285077810287476,0.018638289412378627
27327,54655,0,54655,17.341936826705933,0.01860480387168761
27427,54855,0,54855,17.398530960083008,0.01859216781350349
27528,55057,0,55057,17.45945906639099,0.018544704494266734
27628,55257,0,55257,17.522567749023438,0.018438044904286018
27728,55457,0,55457,17.582704067230225,0.018292609915055567
27828,55657,0,55657,17.63833785057068,0.018138041955773496
27928,55857,0,55857,17.695989847183228,0.018004912078191555
28028,56057,0,56057,17.751610040664673,0.017932120121679825
28128,56257,0,56257,17.80669093132019,0.017933853916027087
28228,56457,0,56457,17.861888885498047,0.017977756925577393
28328,56657,0,56657,17.918412923812866,0.018021628087101546
28428,56857,0,56857,17.97753071784973,0.018042635866574928
28529,57059,0,57059,18.03495502471924,0.018021752807430024
28629,57259,0,57259,18.091931104660034,0.017939971020218468
28729,57459,0,57459,18.14798593521118,0.017803406729614103
28829,57659,0,57659,18.205467700958252,0.017653927696853842
28929,57859,0,57859,18.26340079307556,0.017536491299037758
29029,58059,0,58059,18.319134950637817,0.01746137680867546
29129,58259,0,58259,18.375683069229126,0.017413363779105004
29229,58459,0,58459,18.43251609802246,0.0173816952989395
29329,58659,0,58659,18.48864984512329,0.017355041399424412
29429,58859,0,58859,18.547055959701538,0.01730370652956164
29530,59061,0,59061,18.603786945343018,0.017198577432622486
29630,59261,0,59261,18.663089752197266,0.01705303841661969
29730,59461,0,59461,18.719273805618286,0.01691061120626897
29830,59661,0,59661,18.775563955307007,0.0168100581368708
29930,59861,0,59861,18.834040880203247,0.0167704820639451
30030,60061,0,60061,18.898255109786987,0.016794060014096338
30130,60261,0,60261,18.96183180809021,0.016855402988974474
30230,60461,0,60461,19.020549774169922,0.016908765293439203
30330,60661,0,60661,19.07852005958557,0.01692488790054963
30430,60861,0,60861,19.134845972061157,0.016902160314933117
30531,61063,0,61063,19.205026865005493,0.016842887715150606
30631,61263,0,61263,19.27654480934143,0.016752720399801812
30731,61463,0,61463,19.337794065475464,0.01664984792970389
30831,61663,0,61663,19.39590072631836,0.01655171899535322
30931,61863,0,61863,19.455347776412964,0.016452096738699826
31031,62063,0,62063,19.513372898101807,0.01633476712879096
31131,62263,0,62263,19.57232403755188,0.016203729221512798
31231,62463,0,62463,19.630377769470215,0.01608608011933965
31331,62663,0,62663,19.68768286705017,0.016006817105991705
31431,62863,0,62863,19.74578881263733,0.015967907789441387
31532,63065,0,63065,19.807383060455322,0.015951001587740734
31632,63265,0,63265,19.87288999557495,0.015936944993008243
31732,63465,0,63465,19.934342861175537,0.01592240456960927
31832,63665,0,63665,19.994480848312378,0.015917961362566277
31932,63865,0,63865,20.054110765457153,0.01592903947671259
32032,64065,0,64065,20.11510396003723,0.015945864179848168
32132,64265,0,64265,20.17277193069458,0.015949275982233252
32232,64465,0,64465,20.232053995132446,0.01592228614983197
32332,64665,0,64665,20.290992736816406,0.015860958861401375
32432,64865,0,64865,20.357630968093872,0.01577562495562067
32533,65067,0,65067,20.419798851013184,0.015680988263899107
32633,65267,0,65267,20.482417821884155,0.015593713082745228
32733,65467,0,65467,20.546449899673462,0.015524975110512186
32833,65667,0,65667,20.63054394721985,0.015478368034192422
32933,65867,0,65867,20.695467948913574,0.015442003371100488
33033,66067,0,66067,20.755472898483276,0.015395178244318611
33133,66267,0,66267,20.81645894050598,0.01533041885680635
33233,66467,0,66467,20.87836194038391,0.015267287065115298
33333,66667,0,66667,20.94036889076233,0.015233899131623783
33433,66867,0,66867,21.002001762390137,0.015232736474147414
33534,67069,0,67069,21.061830759048462,0.015235903757457899
33634,67269,0,67269,21.121252059936523,0.015216193310743625
33734,67469,0,67469,21.180259943008423,0.015171602821131185
33834,67669,0,67669,21.24015498161316,0.015115967626649116
33934,67869,0,67869,21.301931858062744,0.01505916076807911
34034,68069,0,68069,21.378523111343384,0.015001289992075584
34134,68269,0,68269,21.462382078170776,0.01493578930057414
34234,68469,0,68469,21.527481079101562,0.014851476926887448
34334,68669,0,68669,21.597272872924805,0.014743263628310686
34434,68869,0,68869,21.658897876739502,0.01462745667545257
34535,69071,0,69071,21.72029685974121,0.014533519250429795
34635,69271,0,69271,21.782367944717407,0.014481322506551092
34735,69471,0,69471,21.84491276741028,0.014466455654823735
34835,69671,0,69671,21.90491795539856,0.014475680813181
34935,69871,0,69871,21.96626305580139,0.014492784929933637
35035,70071,0,70071,22.02590298652649,0.014501068085698577
35135,70271,0,70271,22.087218761444092,0.014491143625437143
35235,70471,0,70471,22.147265911102295,0.01446526130181465
35335,70671,0,70671,22.207313776016235,0.014430427786110204
35435,70871,0,70871,22.26609492301941,0.014391163902417622
35536,71073,0,71073,22.43672800064087,0.014347688051080488
35636,71273,0,71273,22.50159001350403,0.014296018525278677
35736,71473,0,71473,22.561421871185303,0.014229045522591962
35836,71673,0,71673,22.62057375907898,0.014151555839997615
35936,71873,0,71873,22.68016791343689,0.014081308678462075
36036,72073,0,72073,22.743097066879272,0.014026467939148628
36136,72273,0,72273,22.807029008865356,0.013971811722765227
36236,72473,0,72473,22.86996293067932,0.013900654975927679
36336,72673,0,72673,22.930275917053223,0.013820804877356693
36436,72873,0,72873,22.991225957870483,0.013756838310642528
36537,73075,0,73075,23.052356004714966,0.01372597870996677
36637,73275,0,73275,23.11270809173584,0.01373097745024174
36737,73475,0,73475,23.174161911010742,0.013760824776911656
36837,73675,0,73675,23.233861684799194,0.013793008327880838
36937,73875,0,73875,23.303188800811768,0.013803767400256056
37037,74075,0,74075,23.38690495491028,0.013787993250131325
37137,74275,0,74275,23.45000386238098,0.0137599538493293
37237,74475,0,74475,23.525381088256836,0.013730172714679363
37337,74675,0,74675,23.59705376625061,0.01369213003246609
37437,74875,0,74875,23.65492606163025,0.013633781415766289
37538,75077,0,75077,23.71427869796753,0.013549438974218946
37638,75277,0,75277,23.773251056671143,0.013444374719117696
37738,75477,0,75477,23.85354495048523,0.013330483862197822
37838,75677,0,75677,23.929778814315796,0.013230981252340838
37938,75877,0,75877,23.99554991722107,0.013168810857294952
38038,76077,0,76077,24.054109811782837,0.01314764661795424
38138,76277,0,76277,24.112834930419922,0.013149057885518796
38238,76477,0,76477,24.17127275466919,0.013152027446406141
38338,76677,0,76677,24.22957682609558,0.013150257780348246
38438,76877,0,76877,24.291014909744263,0.01314838097384909
38539,77079,0,77079,24.349254846572876,0.013148047316145675
38639,77279,0,77279,24.407803773880005,0.01314337960076272
38739,77479,0,77479,24.466187953948975,0.01312779409481676
38839,77679,0,77679,24.523308038711548,0.013100575190709325
38939,77879,0,77879,24.585474967956543,0.013067362754982794
39039,78079,0,78079,24.644478797912598,0.013036315478978202
39139,78279,0,78279,24.702456951141357,0.01301153583082338
39239,78479,0,78479,24.760849714279175,0.012987422746797107
39339,78679,0,78679,24.822677850723267,0.012951757300121236
39439,78879,0,78879,24.882494926452637,0.012896824579535322
39540,79081,0,79081,24.94611096382141,0.012824944589761824
39640,79281,0,79281,25.021371841430664,0.01274740713587557
39740,79481,0,79481,25.093785047531128,0.01267454698349436
39840,79681,0,79681,25.153040885925293,0.012616986999912665
39940,79881,0,79881,25.210163831710815,0.012582711255122262
40040,80081,0,80081,25.267971992492676,0.01257275859448868
40140,80281,0,80281,25.326634883880615,0.012579811327479462
40240,80481,0,80481,25.38430404663086,0.012591853533341099
40340,80681,0,80681,25.442384004592896,0.01259742017533472
40440,80881,0,80881,25.50052809715271,0.01258849190341614
40541,81083,0,81083,25.571687936782837,0.012560541913467603
40641,81283,0,81283,25.658350944519043,0.012514174766199287
40741,81483,0,81483,25.729399919509888,0.012455248374482742
40841,81683,0,81683,25.789623022079468,0.012396846616790623
40941,81883,0,81883,25.848505973815918,0.01235398096053491
41041,82083,0,82083,25.90678906440735,0.012331918929629492
41141,82283,0,82283,25.963871955871582,0.012318793236578474
41241,82483,0,82483,26.0235378742218,0.01229335439518043
41341,82683,0,82683,26.10819697380066,0.012243316292336999
41441,82883,0,82883,26.173155069351196,0.012177252007486651
41542,83085,0,83085,26.233048915863037,0.012118010425831119
41642,83285,0,83285,26.292101860046387,0.012087090460390948
41742,83485,0,83485,26.34912896156311,0.012088127312532573
41842,83685,0,83685,26.40723490715027,0.012110371833813933
41942,83885,0,83885,26.46609878540039,0.012135932239867675
42042,84085,0,84085,26.523667812347412,0.012147828630524984
42142,84285,0,84285,26.58194088935852,0.012136180513043398
42242,84485,0,84485,26.64787983894348,0.0121001820674274
42342,84685,0,84685,26.72251009941101,0.012044754084458532
42442,84885,0,84885,26.78745174407959,0.011976185315968956
42543,85087,0,85087,26.845487117767334,0.011900281583547345
42643,85287,0,85287,26.90305995941162,0.011826030360169054
42743,85487,0,85487,26.960463047027588,0.011760251744006477
42843,85687,0,85687,27.018021821975708,0.011709484257061179
42943,85887,0,85887,27.07562804222107,0.011678161181881907
43043,86087,0,86087,27.1333589553833,0.011665284912635208
43143,86287,0,86287,27.19233202934265,0.011661557046158623
43243,86487,0,86487,27.25080895423889,0.011654251647284975
43343,86687,0,86687,27.31066393852234,0.011638139887697936
43443,86887,0,86887,27.369441032409668,0.011620426126678702
43544,87089,0,87089,27.43018889427185,0.011613182061582477
43644,87289,0,87289,27.49273180961609,0.011620954996574983
43744,87489,0,87489,27.56327486038208,0.011635423697052902
43844,87689,0,87689,27.626671075820923,0.011642043944076405
43944,87889,0,87889,27.685884714126587,0.011629010495441568
44044,88089,0,88089,27.748373985290527,0.011592024496400686
44144,88289,0,88289,27.820713996887207,0.011534680568930086
44244,88489,0,88489,27.891062021255493,0.011466320788135588
44344,88689,0,88689,27.95071291923523,0.011397536868197866
44444,88889,0,88889,28.012284755706787,0.011335486160834109
44545,89091,0,89091,28.078927040100098,0.01128284361526051
44645,89291,0,89291,28.14059591293335,0.011243375601964594
44745,89491,0,89491,28.20009994506836,0.011220761802009007
44845,89691,0,89691,28.25770902633667,0.01121746067995878
44945,89891,0,89891,28.314608812332153,0.011229293587269767
45045,90091,0,90091,28.37148380279541,0.011245097228247812
45145,90291,0,90291,28.428205966949463,0.011251871740763758
45245,90491,0,90491,28.486281871795654,0.011241843654263232
45345,90691,0,90691,28.549630880355835,0.01121686892123499
45445,90891,0,90891,28.60671591758728,0.01118656187702132
45546,91093,0,91093,28.663472890853882,0.011160249748534945
45646,91293,0,91293,28.719721794128418,0.011140194340159842
45746,91493,0,91493,28.776439905166626,0.01111930314035044
45846,91693,0,91693,28.83249592781067,0.011088771340286978
45946,91893,0,91893,28.887523889541626,0.011044707465559092
46046,92093,0,92093,28.943612813949585,0.01098984467688487
46146,92293,0,92293,29.001101970672607,0.010930643704773547
46246,92493,0,92493,29.061012983322144,0.010873694523576862
46346,92693,0,92693,29.119663953781128,0.01082380548721227
46446,92893,0,92893,29.17910599708557,0.010783799089033042
46547,93095,0,93095,29.237950801849365,0.010754718881999654
46647,93295,0,93295,29.29659390449524,0.010736986488226635
46747,93495,0,93495,29.35502791404724,0.010728629818643321
46847,93695,0,93695,29.411854028701782,0.010727019924492298
46947,93895,0,93895,29.467697858810425,0.010728965033804052
47047,94095,0,94095,29.523905038833618,0.010730000831684327
47147,94295,0,94295,29.581729888916016,0.0107240351026295
47247,94495,0,94495,29.63773488998413,0.010706450883217408
47347,94695,0,94695,29.692798852920532,0.010678777959679388
47447,94895,0,94895,29.74857783317566,0.01064818883866156
47548,95097,0,95097,29.804638862609863,0.010620516735535754
47648,95297,0,95297,29.86134910583496,0.010596177674995228
47748,95497,0,95497,29.937216997146606,0.010570355682742946
47848,95697,0,95697,30.006205797195435,0.010539022967456207
47948,95897,0,95897,30.06705594062805,0.010501730332484763
48048,96097,0,96097,30.12835693359375,0.010462734800943467
48148,96297,0,96297,30.187551975250244,0.01043010513085045
48248,96497,0,96497,30.247389793395996,0.0104116521722781
48348,96697,0,96697,30.307400941848755,0.010409880958250434
48448,96897,0,96897,30.36747694015503,0.01042037546379682
48549,97099,0,97099,30.426774978637695,0.010434267562523369
48649,97299,0,97299,30.485368013381958,0.010441058806138433
48749,97499,0,97499,30.545423984527588,0.010432928440863113
48849,97699,0,97699,30.605193853378296,0.010407114079506216
48949,97899,0,97899,30.664292097091675,0.010366716716095693
49049,98099,0,98099,30.72211503982544,0.010318096482632004
49149,98299,0,98299,30.77842402458191,0.01026769768614067
49249,98499,0,98499,30.836700916290283,0.010220756251457273
49349,98699,0,98699,30.897849082946777,0.010181201622673683
49449,98899,0,98899,30.956984996795654,0.010151357804525554
49550,99101,0,99101,31.019827842712402,0.010131345942205258
49650,99301,0,99301,31.081645965576172,0.010119764719979418
49750,99501,0,99501,31.141824960708618,0.010113155924813612
49850,99701,0,99701,31.207668781280518,0.010108054805557778
49950,99901,0,99901,31.266979932785034,0.010102099529774842
50050,100101,0,100101,31.3242449760437,0.010094850227981282
50150,100301,0,100301,31.3831889629364,0.010087549177962243
50250,100501,0,100501,31.44161081314087,0.010081936442045393
50350,100701,0,100701,31.498867988586426,0.010078588344514266
50450,100901,0,100901,31.556868076324463,0.010075515692014154
50551,101103,0,101103,31.617185831069946,0.010067978668233897
50651,101303,0,101303,31.675770044326782,0.010050676222643046
50751,101503,0,101503,31.73632001876831,0.010020317179777671
50851,101703,0,101703,31.7973690032959,0.00997796358476609
50951,101903,0,101903,31.859923839569092,0.00992897930183474
51051,102103,0,102103,31.918441772460938,0.009880793242002436
51151,102303,0,102303,31.983218908309937,0.009839848554861003
51251,102503,0,102503,32.05856204032898,0.009809776476626992
51351,102703,0,102703,32.139697790145874,0.009791614168874984
51451,102903,0,102903,32.20601010322571,0.009784783451054603
51552,103105,0,103105,32.27678298950195,0.009787186820364233
51652,103305,0,103305,32.34217596054077,0.009794241275637485
51752,103505,0,103505,32.404431104660034,0.009799329806767938
51852,103705,0,103705,32.465680837631226,0.009796122861830327
51952,103905,0,103905,32.52687883377075,0.00978193423058491
52052,104105,0,104105,32.587557792663574,0.009759385620641454
52152,104305,0,104305,32.64889693260193,0.00973437959087421
52252,104505,0,104505,32.708656787872314,0.009711593241208185
52352,104705,0,104705,32.780293703079224,0.009691426212141223
52452,104905,0,104905,32.8442018032074,0.009670917717797904
52553,105107,0,105107,32.90506386756897,0.009646576410917958
52653,105307,0,105307,32.967296838760376,0.00961722411200527
52753,105507,0,105507,33.02649283409119,0.009582394451196366
52853,105707,0,105707,33.08771085739136,0.009542799487996762
52953,105907,0,105907,33.16471076011658,0.009500359302009185
53053,106107,0,106107,33.239099740982056,0.009458474681742261
53153,106307,0,106307,33.30424690246582,0.009421856755248283
53253,106507,0,106507,33.36993193626404,0.009395915501364949
53353,106707,0,106707,33.43184995651245,0.009385310563629866
53453,106907,0,106907,33.495574951171875,0.009391548110275202
53554,107109,0,107109,33.55557584762573,0.009411072457460702
53654,107309,0,107309,33.61705493927002,0.00943419536432631
53754,107509,0,107509,33.67711877822876,0.00944912820161948
53854,107709,0,107709,33.74218797683716,0.009446093078997672
53954,107909,0,107909,33.81305909156799,0.009422107841772777
54054,108109,0,108109,33.897191762924194,0.009382360344359863
54154,108309,0,108309,33.957801818847656,0.009336810375311424
54254,108509,0,108509,34.01818108558655,0.00929427135758262
54354,108709,0,108709,34.0782949924469,0.009258522867911774
54454,108909,0,108909,34.13970398902893,0.009228811124972792
54555,109111,0,109111,34.21723008155823,0.009202596807682553
54655,109311,0,109311,34.290260791778564,0.009178828227337144
54755,109511,0,109511,34.351677894592285,0.009156802884742335
54855,109711,0,109711,34.42925477027893,0.009136660725316645
54955,109911,0,109911,34.51308989524841,0.00911875986228487
55055,110111,0,110111,34.57393407821655,0.009103842066035372
55155,110311,0,110311,34.63504099845886,0.00909317139789591
55255,110511,0,110511,34.695016860961914,0.009087997126030018
55355,110711,0,110711,34.75754475593567,0.00908844933787792
55455,110911,0,110911,34.8187198638916,0.009092617388602002
55556,111113,0,111113,34.88218092918396,0.009096407742470185
55656,111313,0,111313,34.94228792190552,0.00909425669420223
55756,111513,0,111513,35.0039598941803,0.009081550495760288
55856,111713,0,111713,35.06560683250427,0.009057153480114162
55956,111913,0,111913,35.12426781654358,0.009024857757038924
56056,112113,0,112113,35.184958934783936,0.008991625747655088
56156,112313,0,112313,35.24343395233154,0.008963439897264922
56256,112513,0,112513,35.30313181877136,0.008941959049597503
56356,112713,0,112713,35.36354303359985,0.008924641593044305
56456,112913,0,112913,35.42447304725647,0.008908045328560928
56557,113115,0,113115,35.4864559173584,0.008891264505246181
56657,113315,0,113315,35.55115103721619,0.008877386429474528
56757,113515,0,113515,35.61001491546631,0.008869639102887246
56857,113715,0,113715,35.67106509208679,0.008868356751634032
56957,113915,0,113915,35.73099207878113,0.008869889185627759
57057,114115,0,114115,35.79543900489807,0.008869293833110402
57157,114315,0,114315,35.85559701919556,0.008863673051179213
57257,114515,0,114515,35.91524076461792,0.008852915396300908
57357,114715,0,114715,35.97946381568909,0.00883787178734264
57457,114915,0,114915,36.036499977111816,0.008818550505109582
57558,115117,0,115117,36.09719395637512,0.00879385957034237
57658,115317,0,115317,36.15493297576904,0.008764060965915617
57758,115517,0,115517,36.22045373916626,0.00873077453460896
57858,115717,0,115717,36.278778076171875,0.008698285125955298
57958,115917,0,115917,36.35150408744812,0.008671913545105497
58058,116117,0,116117,36.421327114105225,0.00865504459304375
58158,116317,0,116317,36.48056888580322,0.008646641211054728
58258,116517,0,116517,36.539146900177,0.008641745002057164
58358,116717,0,116717,36.59872889518738,0.008635029316991108
58458,116917,0,116917,36.656533002853394,0.008624477304093159
58559,117119,0,117119,36.71570086479187,0.008611980946762743
58659,117319,0,117319,36.77411603927612,0.008601260689291576
58759,117519,0,117519,36.8334219455719,0.008593572397725983
58859,117719,0,117719,36.892021894454956,0.008586778771436394
58959,117919,0,117919,36.955410957336426,0.008576794606098668
59059,118119,0,118119,37.013378858566284,0.00856068599414247
59159,118319,0,118319,37.070536851882935,0.008538731500761284
59259,118519,0,118519,37.13079380989075,0.008513888543393513
59359,118719,0,118719,37.1904239654541,0.008489404000839883
59459,118919,0,118919,37.24812197685242,0.008466879924593705
59560,119121,0,119121,37.30629301071167,0.008446156616738426
59660,119321,0,119321,37.364428997039795,0.008427536476468628
59760,119521,0,119521,37.42911887168884,0.008411546756467375
59860,119721,0,119721,37.511812925338745,0.008399538163253178
59960,119921,0,119921,37.57483100891113,0.008392508542412209
60060,120121,0,120121,37.63401007652283,0.008390118272212626
60160,120321,0,120321,37.69202494621277,0.008390217268757667
60260,120521,0,120521,37.75257682800293,0.008389399843624358
60360,120721,0,120721,37.81327509880066,0.008384529028844144
60460,120921,0,120921,37.87101483345032,0.008374148006962285
60561,121123,0,121123,37.930497884750366,0.008358437768991745
60661,121323,0,121323,37.98843193054199,0.008338831265213073
60761,121523,0,121523,38.051620960235596,0.008316050103701327
60861,121723,0,121723,38.113778829574585,0.008290772274662472
60961,121923,0,121923,38.17318797111511,0.008264392935395931
61061,122123,0,122123,38.23195195198059,0.008239464058084029
61161,122323,0,122323,38.28912091255188,0.008218811913607873
61261,122523,0,122523,38.347200870513916,0.008203856759050901
61361,122723,0,122723,38.40511393547058,0.008193636846330265
61461,122923,0,122923,38.47827386856079,0.008185550279572806
61562,123125,0,123125,38.55898094177246,0.008177208211007935
61662,123325,0,123325,38.61817288398743,0.008168280889727262
61762,123525,0,123525,38.67889595031738,0.008159784506111377
61862,123725,0,123725,38.73768496513367,0.0081527302888562
61962,123925,0,123925,38.8012809753418,0.008146574457245271
62062,124125,0,124125,38.86097979545593,0.008139313373725462
62162,124325,0,124325,38.920379877090454,0.008128958687563971
62262,124525,0,124525,38.98643183708191,0.008114985073655382
62362,124725,0,124725,39.0489399433136,0.008098585694314937
62462,124925,0,124925,39.11163091659546,0.008081718980543
62563,125127,0,125127,39.18022298812866,0.00806566026323462
62663,125327,0,125327,39.23856568336487,0.008050938447781866
62763,125527,0,125527,39.29608082771301,0.008036718809978216
62863,125727,0,125727,39.35888886451721,0.008022436566841503
62963,125927,0,125927,39.41777992248535,0.008008376872473362
63063,126127,0,126127,39.475050926208496,0.007995498217915745
63163,126327,0,126327,39.532957792282104,0.00798443917076437
63263,126527,0,126527,39.59140872955322,0.00797463550190673
63363,126727,0,126727,39.6503427028656,0.007964494618723894
63463,126927,0,126927,39.70822191238403,0.00795259788605402
63564,127129,0,127129,39.76776695251465,0.007938716998042907
63664,127329,0,127329,39.82600498199463,0.007924458292761012
63764,127529,0,127529,39.882359981536865,0.007911366017282132
63864,127729,0,127729,39.94049596786499,0.007900195708787371
63964,127929,0,127929,40.00132608413696,0.007890208253394872
64064,128129,0,128129,40.06131196022034,0.0078796292244711
64164,128329,0,128329,40.12240409851074,0.007866866990561395
64264,128529,0,128529,40.18260598182678,0.007851684943009597
64364,128729,0,128729,40.24278283119202,0.007835404840250538
64464,128929,0,128929,40.303375005722046,0.007819928313755078
64565,129131,0,129131,40.371562004089355,0.0078063123957002375
64665,129331,0,129331,40.43684196472168,0.007794756342410101
64765,129531,0,129531,40.50225591659546,0.007784270154336194
64865,129731,0,129731,40.56979703903198,0.0077740387715886546
64965,129931,0,129931,40.64959788322449,0.007763691083291243
65065,130131,0,130131,40.721349000930786,0.007753114028405276
65165,130331,0,130331,40.787142753601074,0.007741911868765912
65265,130531,0,130531,40.85050702095032,0.007729068728458717
65365,130731,0,130731,40.91455888748169,0.007713310803468315
65465,130931,0,130931,40.97849178314209,0.007694026173873848
65566,131133,0,131133,41.03638792037964,0.007671718853971496
65666,131333,0,131333,41.10054397583008,0.007648748658338769
65766,131533,0,131533,41.16223978996277,0.007627125665096509
65866,131733,0,131733,41.23462986946106,0.007608570456612985
65966,131933,0,131933,41.30830693244934,0.007593980306732783
66066,132133,0,132133,41.37694478034973,0.007583528865600308
66166,132333,0,132333,41.43973183631897,0.007576836481283961
66266,132533,0,132533,41.50126886367798,0.007572924457868866
66366,132733,0,132733,41.56327295303345,0.007570054165316188
66466,132933,0,132933,41.62948298454285,0.007565931664868809
66567,133135,0,133135,41.69281983375549,0.00755849912675663
66667,133335,0,133335,41.75550293922424,0.007547440245384631
66767,133535,0,133535,41.821499824523926,0.007534294067707244
66867,133735,0,133735,41.88503289222717,0.007522022028853063
66967,133935,0,133935,41.94787383079529,0.007513283269721713
67067,134135,0,134135,42.0118887424469,0.007508679212265767
67167,134335,0,134335,42.07460808753967,0.0075059912699163844
67267,134535,0,134535,42.13754391670227,0.0075010316262593595
67367,134735,0,134735,42.196656703948975,0.007489770051496491
67467,134935,0,134935,42.25996494293213,0.007470557468473313
67568,135137,0,135137,42.32095289230347,0.007444938243277958
67668,135337,0,135337,42.3879017829895,0.007418143938868498
67768,135537,0,135537,42.44826889038086,0.007395531627407984
67868,135737,0,135737,42.51859784126282,0.007381259739505908
67968,135937,0,135937,42.58176589012146,0.007376550128270628
68068,136137,0,136137,42.64091992378235,0.007379625699092857
68168,136337,0,136337,42.70161509513855,0.00738675278434639
68268,136537,0,136537,42.77451682090759,0.007393523733379229
68368,136737,0,136737,42.84514284133911,0.00739592150847186
68468,136937,0,136937,42.90839600563049,0.007391300476336427
68569,137139,0,137139,42.97109603881836,0.007379146992632278
68669,137339,0,137339,43.03500199317932,0.007361951396987905
68769,137539,0,137539,43.09627103805542,0.00734356504381411
68869,137739,0,137739,43.16517972946167,0.007327800931907256
68969,137939,0,137939,43.227736949920654,0.007316631763900394
69069,138139,0,138139,43.28911995887756,0.007309529614787006
69169,138339,0,138339,43.35026979446411,0.007304022636236255
69269,138539,0,138539,43.41263389587402,0.0072969470711801545
69369,138739,0,138739,43.47513484954834,0.007285798279211084
69469,138939,0,138939,43.549519062042236,0.007269808260700402
69570,139141,0,139141,43.628785848617554,0.007250236639896668
69670,139341,0,139341,43.690653800964355,0.007230770528532205
69770,139541,0,139541,43.75343680381775,0.007214938155404445
69870,139741,0,139741,43.812532901763916,0.007205144090509089
69970,139941,0,139941,43.870720863342285,0.007201314247952143
70070,140141,0,140141,43.92833685874939,0.007200943119254834
70170,140341,0,140341,43.98700475692749,0.007200314375620685
70270,140541,0,140541,44.075368881225586,0.007196209665670404
70370,140741,0,140741,44.1864218711853,0.0071872218522481025
70470,140941,0,140941,44.300132036209106,0.00717407704365403
70571,141143,0,141143,44.41515803337097,0.007158786495265605
70671,141343,0,141343,44.500794887542725,0.007144044763525589
70771,141543,0,141543,44.64507269859314,0.00713118422212801
70871,141743,0,141743,44.7812979221344,0.007120324195044202
70971,141943,0,141943,44.922796964645386,0.007110513928758536
71071,142143,0,142143,45.00236797332764,0.007100518047407643
71171,142343,0,142343,45.0625159740448,0.007089584315541332
71271,142543,0,142543,45.123570919036865,0.0070777548822075894
71371,142743,0,142743,45.18486499786377,0.007065679810021526
71471,142943,0,142943,45.246872901916504,0.007054237575246948
71572,143145,0,143145,45.309454917907715,0.007044131004119543
71672,143345,0,143345,45.3707058429718,0.007035998909686463
71772,143545,0,143545,45.43130278587341,0.00702947289088109
71872,143745,0,143745,45.493982791900635,0.007023353311468679
71972,143945,0,143945,45.55838394165039,0.007015700281112519
72072,144145,0,144145,45.620276927948,0.007004619222931381
72172,144345,0,144345,45.680861949920654,0.006989253281603668
72272,144545,0,144545,45.74539494514465,0.006970323959531712
72372,144745,0,144745,45.83016276359558,0.006949854181600146
72472,144945,0,144945,46.028889894485474,0.006930297860325547
72573,145147,0,145147,46.15583086013794,0.006913487436533727
72673,145347,0,145347,46.221725940704346,0.006900753721687424
72773,145547,0,145547,46.28430414199829,0.006891879031289255
72873,145747,0,145747,46.34586000442505,0.0068860953682525535
72973,145947,0,145947,46.407212018966675,0.00688228880743852
73073,146147,0,146147,46.46871995925903,0.0068793486117229175
73173,146347,0,146347,46.52868700027466,0.006876429026804945
73273,146547,0,146547,46.590110778808594,0.0068730977688470085
73373,146747,0,146747,46.65826392173767,0.006869306088026997
73473,146947,0,146947,46.718008041381836,0.006865138305280393
73574,147149,0,147149,46.78008580207825,0.006860376845665334
73674,147349,0,147349,46.84416580200195,0.006854380787444337
73774,147549,0,147549,46.96904683113098,0.006845791731786861
73874,147749,0,147749,47.10303473472595,0.006833104297550502
73974,147949,0,147949,47.18367671966553,0.006815379017061515
74074,148149,0,148149,47.25083589553833,0.006793051817513773
74174,148349,0,148349,47.31292200088501,0.006768281771649881
74274,148549,0,148549,47.380316734313965,0.006744464128574958
74374,148749,0,148749,47.44466185569763,0.006725054177901147
74474,148949,0,148949,47.50959897041321,0.006712342451137187
74575,149151,0,149151,47.573077917099,0.006706809677988415
74675,149351,0,149351,47.65765595436096,0.006707415662442803
74775,149551,0,149551,47.72567296028137,0.006711900739219873
74875,149751,0,149751,47.7928409576416,0.006717709306782018
74975,149951,0,149951,47.85724592208862,0.006722380954435715
75075,150151,0,150151,47.92622995376587,0.006723944499778406
75175,150351,0,150351,47.99016284942627,0.006721295573593966
75275,150551,0,150551,48.05873775482178,0.006714440080525755
75375,150751,0,150751,48.14179491996765,0.0067043739097575735
75475,150951,0,150951,48.215879917144775,0.006692528711834919
75576,151153,0,151153,48.289658069610596,0.0066799108345765865
75676,151353,0,151353,48.34842801094055,0.006667117829434347
75776,151553,0,151553,48.406288146972656,0.0066536456949247355
75876,151753,0,151753,48.471709966659546,0.0066389633321500535
75976,151953,0,151953,48.60356283187866,0.006623135417455093
76076,152153,0,152153,48.79920983314514,0.006607276601182124
76176,152353,0,152353,48.91937184333801,0.0065933515810765505
76276,152553,0,152553,49.00571894645691,0.006583330443035823
76376,152753,0,152753,49.107178926467896,0.006578167301260679
76476,152953,0,152953,49.20204281806946,0.006577243849496588
76577,153155,0,153155,49.28557085990906,0.006578627385069742
76677,153355,0,153355,49.35515284538269,0.006579815926972762
76777,153555,0,153555,49.4372398853302,0.006578736850265117
76877,153755,0,153755,49.504010915756226,0.006574181476056478
76977,153955,0,153955,49.5633749961853,0.006565875733439574
77077,154155,0,154155,49.6264328956604,0.006554333835824532
77177,154355,0,154355,49.6840717792511,0.006540691750363322
77277,154555,0,154555,49.740955114364624,0.006526489431994804
77377,154755,0,154755,49.79803276062012,0.006513258191939193
77477,154955,0,154955,49.856268882751465,0.006501939956851516
77578,155157,0,155157,49.91542196273804,0.006492363508745275
77678,155357,0,155357,49.97348499298096,0.006483685405936677
77778,155557,0,155557,50.03473496437073,0.006474519071467548
77878,155757,0,155757,50.10678696632385,0.0064642082835428775
77978,155957,0,155957,50.168789863586426,0.006453209584259463
78078,156157,0,156157,50.23889493942261,0.006442810793705656
78178,156357,0,156357,50.30047583580017,0.006434253029869735
78278,156557,0,156557,50.365375995635986,0.006427870533849245
78378,156757,0,156757,50.43112897872925,0.006422841146226097
78478,156957,0,156957,50.49474787712097,0.006417669582351367
78579,157159,0,157159,50.56021189689636,0.006410937843777352
78679,157359,0,157359,50.62605309486389,0.006402211862557696
78779,157559,0,157559,50.691579818725586,0.0063917322546618175
78879,157759,0,157759,50.772785902023315,0.006380258567283409
78979,157959,0,157959,50.83979272842407,0.006368515630427897
79079,158159,0,158159,50.910902976989746,0.006357004488378025
79179,158359,0,158359,50.97817587852478,0.006346226200388647
79279,158559,0,158559,51.04487705230713,0.006336999685115724
79379,158759,0,158759,51.13918209075928,0.006330413577212286
79479,158959,0,158959,51.23459601402283,0.006327271775837482
79580,159161,0,159161,51.31260371208191,0.00632740443821423
79680,159361,0,159361,51.401349782943726,0.006329342729805803
79780,159561,0,159561,51.463939905166626,0.006330813851845528
79880,159761,0,159761,51.523271799087524,0.006329738140063581
79980,159961,0,159961,51.594330072402954,0.006325092835385952
80080,160161,0,160161,51.65858197212219,0.006317122940496106
80180,160361,0,160361,51.724153995513916,0.006306800561403505
80280,160561,0,160561,51.79211211204529,0.006295007089784566
80380,160761,0,160761,51.85697674751282,0.0062820854308129155
80480,160961,0,160961,51.91534686088562,0.006268037078644111
80581,161163,0,161163,51.972330808639526,0.00625291267142599
80681,161363,0,161363,52.05174493789673,0.006237760268742908
80781,161563,0,161563,52.13692593574524,0.006223538031024847
80881,161763,0,161763,52.20077085494995,0.006211200134098993
80981,161963,0,161963,52.2591028213501,0.006201164968657516
81081,162163,0,162163,52.315762758255005,0.006193363718402701
81181,162363,0,162363,52.37102484703064,0.006187625782028468
81281,162563,0,162563,52.42745900154114,0.006183987463252627
81381,162763,0,162763,52.489274740219116,0.006182574323561393
81481,162963,0,162963,52.55641579627991,0.0061831137879147235
81582,163165,0,163165,52.634567737579346,0.006184537046620509
81682,163365,0,163365,52.695019006729126,0.006185017612347482
81782,163565,0,163565,52.76571583747864,0.006182742342665173
81882,163765,0,163765,52.841062784194946,0.0061766169792434825
81982,163965,0,163965,52.90946984291077,0.006166664472020179
82082,164165,0,164165,53.019059896469116,0.006153859411214947
82182,164365,0,164365,53.10757279396057,0.006139633799702057
82282,164565,0,164565,53.20490288734436,0.0061254006253893024
82382,164765,0,164765,53.33006572723389,0.006112278575012047
82482,164965,0,164965,53.38868188858032,0.006100980846818899
82583,165167,0,165167,53.45101189613342,0.006091678814200914
82683,165367,0,165367,53.52882194519043,0.006084326190826553
82783,165567,0,165567,53.61269807815552,0.006078196839987096
82883,165767,0,165767,53.733647108078,0.0060725231814704956
82983,165967,0,165967,53.79172873497009,0.0060667427637404675
83083,166167,0,166167,53.849623918533325,0.006060770691237532
83183,166367,0,166367,53.908535957336426,0.006055006466621789
83283,166567,0,166567,53.968082904815674,0.00605001569575465
83383,166767,0,166767,54.02493381500244,0.006046039570402898
83483,166967,0,166967,54.08955001831055,0.006042636499109429
83584,167169,0,167169,54.15880012512207,0.006038666314505754
83684,167369,0,167369,54.322656869888306,0.00603288532128104
83784,167569,0,167569,54.50905084609985,0.006024319511563222
83884,167769,0,167769,54.67722487449646,0.006012797186594294
83984,167969,0,167969,54.73674273490906,0.005998931857247583
84084,168169,0,168169,54.79460096359253,0.0059838283176214145
84184,168369,0,168369,54.861488819122314,0.005968713208247137
84284,168569,0,168569,54.936309814453125,0.0059546905452422015
84384,168769,0,168769,55.07400393486023,0.0059426467692178615
84484,168969,0,168969,55.15817904472351,0.0059332001706545005
84585,169171,0,169171,55.238380908966064,0.005926567043396884
84685,169371,0,169371,55.34575891494751,0.005922710538937718
84785,169571,0,169571,55.41110181808472,0.005920943028175706
84885,169771,0,169771,55.47823882102966,0.005920317878003945
84985,169971,0,169971,55.53898000717163,0.005919732673488156
85085,170171,0,170171,55.61734175682068,0.005918155798456033
85185,170371,0,170371,55.690253019332886,0.005914834954634404
85285,170571,0,170571,55.7512948513031,0.005909411892869939
85385,170771,0,170771,55.80970287322998,0.005901907530898961
85485,170971,0,170971,55.86982583999634,0.0058926221881736825
85586,171173,0,171173,55.97798490524292,0.005881923811601864
85686,171373,0,171373,56.077223777770996,0.00587062522168571
85786,171573,0,171573,56.188347816467285,0.005859294641033896
85886,171773,0,171773,56.3428111076355,0.005848604498415193
85986,171973,0,171973,56.45743680000305,0.00583913806808359
86086,172173,0,172173,56.52031683921814,0.005831308960912624
86186,172373,0,172373,56.581559896469116,0.005825322830233905
86286,172573,0,172573,56.64234375953674,0.005821168032310239
86386,172773,0,172773,56.71188282966614,0.005818601001814395
86486,172973,0,172973,56.771047830581665,0.005817126994080715
86587,173175,0,173175,56.83198094367981,0.005816014046640073
86687,173375,0,173375,56.89234685897827,0.005814445508239555
86787,173575,0,173575,56.95396590232849,0.0058116438428099096
86887,173775,0,173775,57.01354789733887,0.005807067710837212
86987,173975,0,173975,57.07573390007019,0.005800480224528795
87087,174175,0,174175,57.13900375366211,0.005791950234930695
87187,174375,0,174375,57.19788885116577,0.005781811875236365
87287,174575,0,174575,57.35693097114563,0.005770606630741553
87387,174775,0,174775,57.535736083984375,0.005759008093047142
87487,174975,0,174975,57.617923974990845,0.0057477316857425294
87588,175177,0,175177,57.68238592147827,0.005737355473919624
87688,175377,0,175377,57.75417995452881,0.005728667339739714
87788,175577,0,175577,57.831946849823,0.005722008654751628
87888,175777,0,175777,57.891886949539185,0.005717660494168233
87988,175977,0,175977,57.94994592666626,0.005715660451452239
88088,176177,0,176177,58.00777888298035,0.005715722673143242
88188,176377,0,176377,58.065287828445435,0.0057172097050312435
88288,176577,0,176577,58.125372886657715,0.0057191899739203085
88388,176777,0,176777,58.185404777526855,0.005720563860147484
88488,176977,0,176977,58.24121904373169,0.005720222478877015
88589,177179,0,177179,58.29753375053406,0.00571718083201398
88689,177379,0,177379,58.35325789451599,0.005710924526099272
88789,177579,0,177579,58.40887689590454,0.005701413356890998
88889,177779,0,177779,58.466187953948975,0.005689226055388126
88989,177979,0,177979,58.52672982215881,0.005675416373485961
89089,178179,0,178179,58.59200096130371,0.0056612132705200265
89189,178379,0,178379,58.65049481391907,0.005647672322363392
89289,178579,0,178579,58.710103034973145,0.005635439724838899
89389,178779,0,178779,58.76986384391785,0.005624733518825825
89489,178979,0,178979,58.826204776763916,0.005615527377784496
89590,179181,0,179181,58.885822772979736,0.005607739954246668
89690,179381,0,179381,58.94602108001709,0.005601693943797764
89790,179581,0,179581,59.00799894332886,0.005597604118614028
89890,179781,0,179781,59.08019709587097,0.005595653441929693
89990,179981,0,179981,59.14371991157532,0.005595597276718549
90090,180181,0,180181,59.20821285247803,0.005596584856012616
90190,180381,0,180381,59.26894783973694,0.005597253885880519
90290,180581,0,180581,59.327499866485596,0.0055960866036244205
90390,180781,0,180781,59.387425899505615,0.005591863564624203
90490,180981,0,180981,59.443504095077515,0.005584010503220677
90591,181183,0,181183,59.50449776649475,0.00557259645155361
90691,181383,0,181383,59.56158685684204,0.005558746212822594
90791,181583,0,181583,59.62523102760315,0.005543743258983847
90891,181783,0,181783,59.68232274055481,0.0055291874545232225
90991,181983,0,181983,59.73874092102051,0.005516596925405587
91091,182183,0,182183,59.79445195198059,0.0055071025103751526
91191,182383,0,182383,59.85331392288208,0.005501204347254055
91291,182583,0,182583,59.92333388328552,0.005498673297552836
91391,182783,0,182783,59.990679025650024,0.005498643484430579
91491,182983,0,182983,60.0522198677063,0.005499867238591489
91592,183185,0,183185,60.11906695365906,0.005501044618695045
91692,183385,0,183385,60.178921937942505,0.005501054058664265
91792,183585,0,183585,60.2383987903595,0.0054991938166189845
91892,183785,0,183785,60.29708480834961,0.0054951414124938085
91992,183985,0,183985,60.354623794555664,0.005488902161121889
92092,184185,0,184185,60.41201400756836,0.0054807186733045925
92192,184385,0,184385,60.46904802322388,0.005470995085045587
92292,184585,0,184585,60.526187896728516,0.005460240397625913
92392,184785,0,184785,60.58510684967041,0.005449017392084609
92492,184985,0,184985,60.64248085021973,0.005437890116056643
92593,185187,0,185187,60.69886898994446,0.005427275518267758
92693,185387,0,185387,60.75572395324707,0.0054178233125894565
92793,185587,0,185587,60.81301403045654,0.005409758919085763
92893,185787,0,185787,60.869855880737305,0.005403301163180252
92993,185987,0,185987,60.92565989494324,0.00539852713865669
93093,186187,0,186187,60.98336577415466,0.005395323499740656
93193,186387,0,186387,61.04075884819031,0.005393331017795206
93293,186587,0,186587,61.11120676994324,0.005391930482023636
93393,186787,0,186787,61.171475887298584,0.005390321149126888
93493,186987,0,186987,61.22734785079956,0.005387700515157615
93594,187189,0,187189,61.283955812454224,0.0053834398714257305
93694,187389,0,187389,61.33971405029297,0.0053774504937556195
93794,187589,0,187589,61.39638686180115,0.005369978520308289
93894,187789,0,187789,61.453266859054565,0.005361637684975971
93994,187989,0,187989,61.510132789611816,0.005353153887437914
94094,188189,0,188189,61.566473960876465,0.005345141080713081
94194,188389,0,188389,61.62502384185791,0.005337967722451684
94294,188589,0,188589,61.68226599693298,0.005331740623447432
94394,188789,0,188789,61.74195384979248,0.005326367464065984
94494,188989,0,188989,61.803133964538574,0.0053216428161738
94595,189191,0,189191,61.86123204231262,0.005317289439703156
94695,189391,0,189391,61.91892385482788,0.005313208184613084
94795,189591,0,189591,61.97979378700256,0.005309293393753237
94895,189791,0,189791,62.05171084403992,0.0053056223589581335
94995,189991,0,189991,62.12613487243652,0.005302317679326149
95095,190191,0,190191,62.18473696708679,0.005299352112559907
95195,190391,0,190391,62.2432599067688,0.00529636113764621
95295,190591,0,190591,62.301405906677246,0.005292627508405846
95395,190791,0,190791,62.35898804664612,0.005287325316621155
95495,190991,0,190991,62.421345949172974,0.00527993261485608
95596,191193,0,191193,62.4806969165802,0.0052704765342773815
95696,191393,0,191393,62.538455963134766,0.005259989968454442
95796,191593,0,191593,62.598809003829956,0.005249646040618858
95896,191793,0,191793,62.657179832458496,0.005240631331917189
95996,191993,0,191993,62.71567392349243,0.005233629392546392
96096,192193,0,192193,62.77440571784973,0.005228645098702569
96196,192393,0,192393,62.83569288253784,0.0052251286552501665
96296,192593,0,192593,62.89667081832886,0.0052222879537750025
96396,192793,0,192793,62.95800185203552,0.0052194160286189615
96496,192993,0,192993,63.01988077163696,0.005216102206355348
96597,193195,0,193195,63.08355402946472,0.005212243055105286
96697,193395,0,193395,63.14274501800537,0.0052081177949299205
96797,193595,0,193595,63.20288395881653,0.00520398702169877
96897,193795,0,193795,63.26231074333191,0.00520004424728759
96997,193995,0,193995,63.31996989250183,0.0051962131578217816
97097,194195,0,194195,63.37672686576843,0.005192083295763352
97197,194395,0,194395,63.43492293357849,0.005187013862526274
97297,194595,0,194595,63.493138790130615,0.0051804108162943905
97397,194795,0,194795,63.552156925201416,0.005172075470399447
97497,194995,0,194995,63.61806583404541,0.005162438383244741
97598,195197,0,195197,63.67643213272095,0.0051524183020271635
97698,195397,0,195397,63.736480951309204,0.005143481166171602
97798,195597,0,195597,63.79411506652832,0.005136543719886977
97898,195797,0,195797,63.85253190994263,0.0051320146477682165
97998,195997,0,195997,63.90936803817749,0.005129609302065471
98098,196197,0,196197,63.966535806655884,0.005128541084653189
98198,196397,0,196397,64.02423787117004,0.0051278443046347
98298,196597,0,196597,64.08372712135315,0.005126663800300864
98398,196797,0,196797,64.15274691581726,0.005124425809643827
98498,196997,0,196997,64.22431683540344,0.005120893229623032
98599,197199,0,197199,64.29015684127808,0.005116088785268417
98699,197399,0,197399,64.35843300819397,0.005110415494816555
98799,197599,0,197599,64.42149710655212,0.005104227058415538
98899,197799,0,197799,64.48144507408142,0.005097841201350138
98999,197999,0,197999,64.53929686546326,0.005091371797212367
99099,198199,0,198199,64.61247205734253,0.005084724362292203
99199,198399,0,198399,64.70184183120728,0.005077737566869527
99299,198599,0,198599,64.78288674354553,0.00507039631052385
99399,198799,0,198799,64.8698480129242,0.00506297460937025
99499,198999,0,198999,64.97063398361206,0.00505599421150402
99600,199201,0,199201,65.08398413658142,0.0050499475735867085
99700,199401,0,199401,65.23796391487122,0.0050452487255632636
99800,199601,0,199601,65.32781982421875,0.005041712194349829
99900,199801,0,199801,65.40050387382507,0.005038869882085438
100000,200001,0,200001,65.46437382698059,0.005036140328868398


==> plot_data/quadratic_minimax_problem_n500_alpha00001/eg-aa.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007221698760986328,30.358106049564984
100,201,200,401,0.07111811637878418,1.7063375198016169
200,401,400,801,0.15479707717895508,1.0108894113540814
300,601,600,1201,0.22110509872436523,0.7489939892258344
400,801,800,1601,0.28597021102905273,0.6081938727196392
501,1003,1002,2005,0.3430659770965576,0.5168895867181229
601,1203,1202,2405,0.399658203125,0.452278382327617
701,1403,1402,2805,0.45823097229003906,0.40291992726905773
801,1603,1602,3205,0.5149731636047363,0.3634630940471491
901,1803,1802,3605,0.5751190185546875,0.33097564129661755
1001,2003,2002,4005,0.6394898891448975,0.3037093528611154
1101,2203,2202,4405,0.6969859600067139,0.2803953971483973
1201,2403,2402,4805,0.7553591728210449,0.26019451460291226
1301,2603,2602,5205,0.8123140335083008,0.24250818197445992
1401,2803,2802,5605,0.8706750869750977,0.22685332490806293
1502,3005,3004,6009,0.9271430969238281,0.2127929708960007
1602,3205,3204,6409,0.9837710857391357,0.20030755961093588
1702,3405,3404,6809,1.0433928966522217,0.18902363243190226
1802,3605,3604,7209,1.1205999851226807,0.17874588608055825
1902,3805,3804,7609,1.190566062927246,0.16936686708805634
2002,4005,4004,8009,1.253993034362793,0.16078928006504323
2102,4205,4204,8409,1.315399169921875,0.15289388141740703
2202,4405,4404,8809,1.377676010131836,0.1455894973020299
2302,4605,4604,9209,1.4560480117797852,0.13880996643974702
2402,4805,4804,9609,1.5163989067077637,0.13250544845542997
2503,5007,5006,10013,1.5813071727752686,0.12658272496808612
2603,5207,5206,10413,1.6557328701019287,0.12107898410631822
2703,5407,5406,10813,1.7226440906524658,0.11592039425419869
2803,5607,5606,11213,1.7872650623321533,0.11108349163202878
2903,5807,5806,11613,1.8494648933410645,0.10652119458942605
3003,6007,6006,12013,1.909250020980835,0.10222880204007911
3103,6207,6206,12413,1.9699392318725586,0.09818713706730445
3203,6407,6406,12813,2.0313398838043213,0.09436920147170691
3303,6607,6606,13213,2.096950054168701,0.09073320222110537
3403,6807,6806,13613,2.1620609760284424,0.08729857820057606
3504,7009,7008,14017,2.2354400157928467,0.08401838454826126
3604,7209,7208,14417,2.312311887741089,0.08093927928962326
3704,7409,7408,14817,2.374199867248535,0.07800912151469362
3804,7609,7608,15217,2.4395711421966553,0.0752232971485176
3904,7809,7808,15617,2.500128984451294,0.07257609242688355
4004,8009,8008,16017,2.5602238178253174,0.07005957569801338
4104,8209,8208,16417,2.632909059524536,0.06766082262576223
4204,8409,8408,16817,2.6967039108276367,0.0653627511027669
4304,8609,8608,17217,2.7577710151672363,0.06318097775381688
4404,8809,8808,17617,2.8185360431671143,0.06110300953777403
4505,9011,9010,18021,2.8820929527282715,0.0590937428271714
4605,9211,9210,18421,2.944782018661499,0.05717733161162599
4705,9411,9410,18821,3.007866144180298,0.05535773017085458
4805,9611,9610,19221,3.0684731006622314,0.05361798797459647
4905,9811,9810,19621,3.1422371864318848,0.05194900886724691
5005,10011,10010,20021,3.2039499282836914,0.05035243765185992
5105,10211,10210,20421,3.2653040885925293,0.04882063373100812
5205,10411,10410,20821,3.3260772228240967,0.047359071023488915
5305,10611,10610,21221,3.3886728286743164,0.045955467781552156
5405,10811,10810,21621,3.4485411643981934,0.04461009631068081
5506,11013,11012,22025,3.515192985534668,0.043314099629270165
5606,11213,11212,22425,3.5777299404144287,0.04207838125332836
5706,11413,11412,22825,3.6468799114227295,0.040893441689385045
5806,11613,11612,23225,3.7094480991363525,0.039758063729968526
5906,11813,11812,23625,3.770732879638672,0.03866727459590865
6006,12013,12012,24025,3.8318021297454834,0.03762274291255587
6106,12213,12212,24425,3.894062042236328,0.036611040471708
6206,12413,12412,24825,3.9540770053863525,0.03562856314436133
6306,12613,12612,25225,4.015941143035889,0.03469692269248736
6406,12813,12812,25625,4.07974910736084,0.033799683286082904
6507,13015,13014,26029,4.142674207687378,0.032929696359171264
6607,13215,13214,26429,4.2083611488342285,0.03210090886963369
6707,13415,13414,26829,4.292970895767212,0.03129562467976816
6807,13615,13614,27229,4.390583038330078,0.030518070810675323
6907,13815,13814,27629,4.473135948181152,0.02976476100537671
7007,14015,14014,28029,4.543805122375488,0.029042946413349643
7107,14215,14214,28429,4.625964879989624,0.028345043787213003
7207,14415,14414,28829,4.70111608505249,0.0276787893149401
7307,14615,14614,29229,4.772382020950317,0.027025990891256242
7407,14815,14814,29629,4.85260796546936,0.02639680752696954
7508,15017,15016,30033,4.928344011306763,0.025790202933365928
7608,15217,15216,30433,5.000643968582153,0.025208342940185372
7708,15417,15416,30833,5.073904037475586,0.024644675806295535
7808,15617,15616,31233,5.149876832962036,0.024097814611134232
7908,15817,15816,31633,5.22419810295105,0.023566249852129673
8008,16017,16016,32033,5.298389911651611,0.02305376193088568
8108,16217,16216,32433,5.364605188369751,0.022559992497924237
8208,16417,16416,32833,5.4363110065460205,0.022127591431272717
8308,16617,16616,33233,5.499424934387207,0.02183072302642047
8408,16817,16816,33633,5.56223201751709,0.021543699371941685
8509,17019,17018,34037,5.635188817977905,0.021261309515999933
8609,17219,17218,34437,5.6984312534332275,0.02098255850015554
8709,17419,17418,34837,5.761754035949707,0.020702356282380815
8809,17619,17618,35237,5.82614803314209,0.020420375359117754
8909,17819,17818,35637,5.891563892364502,0.020138484850655773
9009,18019,18018,36037,5.968167066574097,0.019856479540637278
9109,18219,18218,36437,6.0351080894470215,0.019579994634302125
9209,18419,18418,36837,6.106342077255249,0.019317725373640755
9309,18619,18618,37237,6.17547607421875,0.01905872209024548
9409,18819,18818,37637,6.247542858123779,0.01879995540818351
9510,19021,19020,38041,6.312247037887573,0.01854074106529157
9610,19221,19220,38441,6.376391172409058,0.018285940160676868
9710,19421,19420,38841,6.442178964614868,0.018033973880335365
9810,19621,19620,39241,6.522934913635254,0.017784346530271056
9910,19821,19820,39641,6.61003303527832,0.01754157169669738
10010,20021,20020,40041,6.683986186981201,0.017298410407666644
10110,20221,20220,40441,6.761784076690674,0.017056909972164882
10210,20421,20420,40841,6.838958024978638,0.016821123610325783
10310,20621,20620,41241,6.9127678871154785,0.016589128045374983
10410,20821,20820,41641,6.979252815246582,0.016354305165659166
10511,21023,21022,42045,7.045183897018433,0.016116668275785968
10611,21223,21222,42445,7.123002052307129,0.015890884021779093
10711,21423,21422,42845,7.190722942352295,0.015665347331383236
10811,21623,21622,43245,7.256376028060913,0.015434709267468974
10911,21823,21822,43645,7.320688962936401,0.015212370568155185
11011,22023,22022,44045,7.389062166213989,0.014993947575038701
11111,22223,22222,44445,7.460387945175171,0.014771376883042104
11211,22423,22422,44845,7.537173271179199,0.014550765644058933
11311,22623,22622,45245,7.622260808944702,0.014334080098261178
11411,22823,22822,45645,7.703177213668823,0.014116158028222484
11512,23025,23024,46049,7.7780539989471436,0.013902809895313464
11612,23225,23224,46449,7.840038061141968,0.013695643382817462
11712,23425,23424,46849,7.9021852016448975,0.013484527177849842
11812,23625,23624,47249,7.9816858768463135,0.01328034081915178
11912,23825,23824,47649,8.047395944595337,0.013080685802734427
12012,24025,24024,48049,8.113860130310059,0.012879287348580218
12112,24225,24224,48449,8.175557136535645,0.012688001335773287
12212,24425,24424,48849,8.241299152374268,0.012500327290257563
12312,24625,24624,49249,8.310078144073486,0.012310316549936438
12412,24825,24824,49649,8.38286304473877,0.012127368917885458
12513,25027,25026,50053,8.45032000541687,0.011942693247676607
12613,25227,25226,50453,8.513161182403564,0.011759630765673523
12713,25427,25426,50853,8.577107191085815,0.011577998632949813
12813,25627,25626,51253,8.665873050689697,0.011398773287604
12913,25827,25826,51653,8.751668214797974,0.011225178439008686
13013,26027,26026,52053,8.829296112060547,0.011052352318824609
13113,26227,26226,52453,8.898505210876465,0.010881101841824966
13213,26427,26426,52853,8.976408958435059,0.010711517925130679
13313,26627,26626,53253,9.050190925598145,0.01053970825186124
13413,26827,26826,53653,9.129212141036987,0.010373069909673675
13514,27029,27028,54057,9.199381828308105,0.010208010736618077
13614,27229,27228,54457,9.267427921295166,0.010047203235739155
13714,27429,27428,54857,9.33531904220581,0.009886819102132356
13814,27629,27628,55257,9.420829057693481,0.009727176920220567
13914,27829,27828,55657,9.537475109100342,0.009571825961645079
14014,28029,28028,56057,9.689951181411743,0.009420559812505053
14114,28229,28228,56457,9.78522515296936,0.009264481496922659
14214,28429,28428,56857,9.88527512550354,0.009111795150308254
14314,28629,28628,57257,9.986868858337402,0.008960426757708433
14414,28829,28828,57657,10.092884063720703,0.008811356820738444
14515,29031,29030,58061,10.16550588607788,0.008661971411963471
14615,29231,29230,58461,10.231786251068115,0.0085147352050275
14715,29431,29430,58861,10.297982215881348,0.008371399791506053
14815,29631,29630,59261,10.361873149871826,0.008230277060289374
14915,29831,29830,59661,10.435137033462524,0.008088785214119236
15015,30031,30030,60061,10.5000638961792,0.007957725611132869
15115,30231,30230,60461,10.563796043395996,0.007828766165637954
15215,30431,30430,60861,10.637076139450073,0.007702214071622525
15315,30631,30630,61261,10.709483861923218,0.007579056214627207
15415,30831,30830,61661,10.788156032562256,0.007458542171695687
15516,31033,31032,62065,10.865755081176758,0.007338314326559178
15616,31233,31232,62465,10.929435968399048,0.007220560957340546
15716,31433,31432,62865,10.995519161224365,0.007104786479107159
15816,31633,31632,63265,11.059489965438843,0.006993305890992013
15916,31833,31832,63665,11.12909197807312,0.006883644391807818
16016,32033,32032,64065,11.193243026733398,0.006775302164585744
16116,32233,32232,64465,11.256379127502441,0.006668338416285847
16216,32433,32432,64865,11.319308042526245,0.006564102840771003
16316,32633,32632,65265,11.38358211517334,0.00646168482265777
16416,32833,32832,65665,11.443063974380493,0.00636063742741675
16517,33035,33034,66069,11.504501819610596,0.006261352045845996
16617,33235,33234,66469,11.56729793548584,0.00616446061075423
16717,33435,33434,66869,11.638481140136719,0.006068326088936202
16817,33635,33634,67269,11.697715044021606,0.00597415591209079
16917,33835,33834,67669,11.760159254074097,0.005881769753432209
17017,34035,34034,68069,11.822763919830322,0.00579088832402879
17117,34235,34234,68469,11.88634991645813,0.005700441037070479
17217,34435,34434,68869,11.948215007781982,0.00561125633315622
17317,34635,34634,69269,12.009923934936523,0.005523652669130749
17417,34835,34834,69669,12.069901943206787,0.005438853698557275
17518,35037,35036,70073,12.145321130752563,0.00535317600669035
17618,35237,35236,70473,12.203764200210571,0.005268893774460433
17718,35437,35436,70873,12.266256093978882,0.005187057729373812
17818,35637,35636,71273,12.326190948486328,0.005106914522064102
17918,35837,35836,71673,12.386100053787231,0.005027095355570396
18018,36037,36036,72073,12.44614315032959,0.004950044526937833
18118,36237,36236,72473,12.507622003555298,0.004873844016375647
18218,36437,36436,72873,12.571474075317383,0.004799462694000384
18318,36637,36636,73273,12.645108938217163,0.004727414678885444
18418,36837,36836,73673,12.707042932510376,0.004655481375666323
18519,37039,37038,74077,12.767330884933472,0.0045841911071727815
18619,37239,37238,74477,12.828294038772583,0.004514961509392858
18719,37439,37438,74877,12.896565914154053,0.004446586256726498
18819,37639,37638,75277,12.971626043319702,0.004380327440970527
18919,37839,37838,75677,13.036288022994995,0.0043153148028974115
19019,38039,38038,76077,13.098992109298706,0.00425092402749638
19119,38239,38238,76477,13.165167093276978,0.004187519836059987
19219,38439,38438,76877,13.235447883605957,0.0041249477063166114
19319,38639,38638,77277,13.30347990989685,0.004063816790596845
19419,38839,38838,77677,13.37231993675232,0.004003700540499531
19520,39041,39040,78081,13.439068078994751,0.003943925277498849
19620,39241,39240,78481,13.505311965942383,0.003884819167590979
19720,39441,39440,78881,13.57625412940979,0.0038269317385694777
19820,39641,39640,79281,13.652884244918823,0.0037708737474745195
19920,39841,39840,79681,13.723875045776367,0.0037145532579593273
20020,40041,40040,80081,13.798302173614502,0.0036584291949138853
20120,40241,40240,80481,13.858078241348267,0.003603366768594275
20220,40441,40440,80881,13.919543981552124,0.0035489978910629868
20320,40641,40640,81281,13.983485221862793,0.003495686226694369
20420,40841,40840,81681,14.048204898834229,0.0034434990275128852
20521,41043,41042,82085,14.118958950042725,0.0033915132480723444
20621,41243,41242,82485,14.183348178863525,0.00334116452748544
20721,41443,41442,82885,14.248977184295654,0.0032915124515810216
20821,41643,41642,83285,14.309129238128662,0.0032425950542720214
20921,41843,41842,83685,14.370642185211182,0.0031948643660281817
21021,42043,42042,84085,14.43604588508606,0.0031476492059488745
21121,42243,42242,84485,14.501023054122925,0.00310126261251773
21221,42443,42442,84885,14.562581062316895,0.003056129359842945
21321,42643,42642,85285,14.636733055114746,0.0030119612035079987
21421,42843,42842,85685,14.699596881866455,0.002968074746125493
21522,43045,43044,86089,14.76484489440918,0.002924371116217384
21622,43245,43244,86489,14.8334219455719,0.002881569865576798
21722,43445,43444,86889,14.898208856582642,0.002839747643428888
21822,43645,43644,87289,14.967154026031494,0.0027993270866922136
21922,43845,43844,87689,15.048724174499512,0.0027593892451250423
22022,44045,44044,88089,15.132683992385864,0.0027192847850162744
22122,44245,44244,88489,15.204129934310913,0.002679927023142476
22222,44445,44444,88889,15.268203020095825,0.0026419890819075124
22322,44645,44644,89289,15.332620859146118,0.002604373986547768
22422,44845,44844,89689,15.396627187728882,0.002566633685588737
22523,45047,45046,90093,15.461143970489502,0.002528809218388413
22623,45247,45246,90493,15.525268077850342,0.002492101292504614
22723,45447,45446,90893,15.597223043441772,0.002456077738520633
22823,45647,45646,91293,15.662830114364624,0.0024203499482636833
22923,45847,45846,91693,15.72950792312622,0.00238499805154855
23023,46047,46046,92093,15.792171001434326,0.00235038580587238
23123,46247,46246,92493,15.853379964828491,0.0023159784172378144
23223,46447,46446,92893,15.915328025817871,0.0022817855748038618
23323,46647,46646,93293,15.978865146636963,0.002248907300292022
23423,46847,46846,93693,16.042865991592407,0.0022164926452908577
23524,47049,47048,94097,16.111135244369507,0.002183712668552709
23624,47249,47248,94497,16.173521995544434,0.002151878226282065
23724,47449,47448,94897,16.236832857131958,0.002120901752936091
23824,47649,47648,95297,16.302364110946655,0.002090389310674898
23924,47849,47848,95697,16.36510992050171,0.0020602076568302114
24024,48049,48048,96097,16.426560878753662,0.0020300358244441674
24124,48249,48248,96497,16.490967988967896,0.0020007501763382183
24224,48449,48448,96897,16.552967071533203,0.0019725999537984077
24324,48649,48648,97297,16.62134599685669,0.0019446288771185157
24424,48849,48848,97697,16.685590028762817,0.0019167010082839434
24525,49051,49050,98101,16.748387098312378,0.001889088983518954
24625,49251,49250,98501,16.81114625930786,0.0018623959407974152
24725,49451,49450,98901,16.872386932373047,0.0018362003689114308
24825,49651,49650,99301,16.933897256851196,0.0018102601128650523
24925,49851,49850,99701,16.99528408050537,0.0017846602201538415
25025,50051,50050,100101,17.057823181152344,0.0017593600818294342
25125,50251,50250,100501,17.12725305557251,0.001734419535061171
25225,50451,50450,100901,17.204463005065918,0.0017098739985286888
25325,50651,50650,101301,17.28036403656006,0.0016857110768930476
25425,50851,50850,101701,17.341629028320312,0.0016620538342593714
25526,51053,51052,102105,17.40421485900879,0.0016380740395514435
25626,51253,51252,102505,17.466536045074463,0.0016144983521808722
25726,51453,51452,102905,17.526948928833008,0.0015918118810752276
25826,51653,51652,103305,17.594922065734863,0.0015693254066215358
25926,51853,51852,103705,17.659789085388184,0.0015467781832337205
26026,52053,52052,104105,17.722559928894043,0.0015244602389677497
26126,52253,52252,104505,17.784492015838623,0.0015026502572782145
26226,52453,52452,104905,17.84726905822754,0.001481330595269735
26326,52653,52652,105305,17.914132118225098,0.001460079165254246
26426,52853,52852,105705,17.97667694091797,0.0014389821807388493
26527,53055,53054,106109,18.04431700706482,0.0014182443538461934
26627,53255,53254,106509,18.111519813537598,0.0013982646585259067
26727,53455,53454,106909,18.176138877868652,0.0013783474126149002
26827,53655,53654,107309,18.239681005477905,0.0013585571513145516
26927,53855,53854,107709,18.300904035568237,0.0013393216720983194
27027,54055,54054,108109,18.361008167266846,0.0013204230171340332
27127,54255,54254,108509,18.42322087287903,0.0013017306960680928
27227,54455,54454,108909,18.486028909683228,0.0012834669603326036
27327,54655,54654,109309,18.548516988754272,0.0012655251522662237
27427,54855,54854,109709,18.6266610622406,0.0012478452688603019
27528,55057,55056,110113,18.69686484336853,0.0012302125465743373
27628,55257,55256,110513,18.760345935821533,0.0012132053247634216
27728,55457,55456,110913,18.820992946624756,0.0011966904873274232
27828,55657,55656,111313,18.882877111434937,0.0011802019934684825
27928,55857,55856,111713,18.945513248443604,0.0011637458216228502
28028,56057,56056,112113,19.007467031478882,0.0011476477124180966
28128,56257,56256,112513,19.071022987365723,0.0011320792744783767
28228,56457,56456,112913,19.139606952667236,0.0011165924841270373
28328,56657,56656,113313,19.202129125595093,0.0011009499922181403
28428,56857,56856,113713,19.2660551071167,0.0010854847205532423
28529,57059,57058,114117,19.342783212661743,0.0010701102187086783
28629,57259,57258,114517,19.41591215133667,0.0010551348959841258
28729,57459,57458,114917,19.47808599472046,0.0010403849838116121
28829,57659,57658,115317,19.541871070861816,0.0010256658519945917
28929,57859,57858,115717,19.612452030181885,0.0010111866354786103
29029,58059,58058,116117,19.67368793487549,0.0009969480513930067
29129,58259,58258,116517,19.734447956085205,0.0009829123913166627
29229,58459,58458,116917,19.79522204399109,0.0009690605140732158
29329,58659,58658,117317,19.856840133666992,0.0009553096585697534
29429,58859,58858,117717,19.920674085617065,0.0009418003635743267
29530,59061,59060,118121,19.98335099220276,0.0009284304652033482
29630,59261,59260,118521,20.047746896743774,0.0009154142986187284
29730,59461,59460,118921,20.11328101158142,0.0009026317855767636
29830,59661,59660,119321,20.1770441532135,0.0008899873045686885
29930,59861,59860,119721,20.243183135986328,0.0008775041211860132
30030,60061,60060,120121,20.30452013015747,0.0008653225516324965
30130,60261,60260,120521,20.366421937942505,0.0008535461698688634
30230,60461,60460,120921,20.427445888519287,0.0008419674667357488
30330,60661,60660,121321,20.488420009613037,0.0008303386774036522
30430,60861,60860,121721,20.55075693130493,0.0008188580681519754
30531,61063,61062,122125,20.621551036834717,0.0008076775110276781
30631,61263,61262,122525,20.682762145996094,0.0007968731855088166
30731,61463,61462,122925,20.74382996559143,0.0007860349944779897
30831,61663,61662,123325,20.804694890975952,0.0007751927084849044
30931,61863,61862,123725,20.86746907234192,0.0007645015410756932
31031,62063,62062,124125,20.940480947494507,0.0007540276429651918
31131,62263,62262,124525,21.005068063735962,0.0007437460770822886
31231,62463,62462,124925,21.06995391845703,0.0007335321327945892
31331,62663,62662,125325,21.142383098602295,0.0007233619219762391
31431,62863,62862,125725,21.205503940582275,0.0007132575624108962
31532,63065,63064,126129,21.271016120910645,0.0007031791518934151
31632,63265,63264,126529,21.33330202102661,0.000693407276131615
31732,63465,63464,126929,21.396509170532227,0.0006837682224038886
31832,63665,63664,127329,21.474234104156494,0.0006742308091293568
31932,63865,63864,127729,21.548655033111572,0.0006647500198807649
32032,64065,64064,128129,21.622551918029785,0.000655433217201054
32132,64265,64264,128529,21.703758001327515,0.0006463353889688796
32232,64465,64464,128929,21.86014723777771,0.000637319651456879
32332,64665,64664,129329,21.934923887252808,0.0006283514193170035
32432,64865,64864,129729,21.997992038726807,0.0006194827952186915
32533,65067,65066,130133,22.061700105667114,0.0006108092191794662
32633,65267,65266,130533,22.141151189804077,0.0006024799485118703
32733,65467,65466,130933,22.208763122558594,0.0005941212182405992
32833,65667,65666,131333,22.27108120918274,0.0005857944968891536
32933,65867,65866,131733,22.333060026168823,0.0005777440995846808
33033,66067,66066,132133,22.39333701133728,0.0005699266972724137
33133,66267,66266,132533,22.458478927612305,0.0005621643248891333
33233,66467,66466,132933,22.52424907684326,0.0005544437387228325
33333,66667,66666,133333,22.59811019897461,0.0005468635377227691
33433,66867,66866,133733,22.664429903030396,0.0005394013065281456
33534,67069,67068,134137,22.730762243270874,0.00053198819381291
33634,67269,67268,134537,22.797364950180054,0.0005247955643287588
33734,67469,67468,134937,22.8648841381073,0.0005177029627606521
33834,67669,67668,135337,22.945531129837036,0.0005106466347315166
33934,67869,67868,135737,23.018501043319702,0.0005035834270797113
34034,68069,68068,136137,23.09039807319641,0.0004966855250277016
34134,68269,68268,136537,23.16755509376526,0.0004900003000226095
34234,68469,68468,136937,23.24531126022339,0.00048332097387309884
34334,68669,68668,137337,23.31636905670166,0.00047661937030205715
34434,68869,68868,137737,23.38484287261963,0.0004700321654022045
34535,69071,69070,138141,23.46036696434021,0.0004635443572416771
34635,69271,69270,138541,23.529834270477295,0.0004571787334096308
34735,69471,69470,138941,23.6158230304718,0.0004508047311539187
34835,69671,69670,139341,23.694399118423462,0.00044452928748924935
34935,69871,69870,139741,23.792896032333374,0.000438393552017286
35035,70071,70070,140141,23.933488130569458,0.00043236688364006173
35135,70271,70270,140541,24.024163961410522,0.00042636610962974963
35235,70471,70470,140941,24.117117166519165,0.00042040513674547903
35335,70671,70670,141341,24.180429935455322,0.00041459402541517236
35435,70871,70870,141741,24.24325704574585,0.000408864711072116
35536,71073,71072,142145,24.312637090682983,0.000403132403442468
35636,71273,71272,142545,24.37627410888672,0.0003975786292588106
35736,71473,71472,142945,24.439263105392456,0.0003921131712407527
35836,71673,71672,143345,24.49909806251526,0.00038673475432789335
35936,71873,71872,143745,24.563776969909668,0.0003814759245695828
36036,72073,72072,144145,24.631532907485962,0.0003763491886690569
36136,72273,72272,144545,24.69352698326111,0.0003712963254442391
36236,72473,72472,144945,24.75804090499878,0.00036626315303797457
36336,72673,72672,145345,24.81902503967285,0.0003613073808415068
36436,72873,72872,145745,24.886712074279785,0.0003564998014459769
36537,73075,73074,146149,24.960304975509644,0.0003517684228451117
36637,73275,73274,146549,25.045418977737427,0.0003470859518399967
36737,73475,73474,146949,25.154603004455566,0.00034238542432181635
36837,73675,73674,147349,25.23512315750122,0.0003377721888417434
36937,73875,73874,147749,25.311609983444214,0.00033324931614373926
37037,74075,74074,148149,25.387518167495728,0.00032877466863530646
37137,74275,74274,148549,25.46184206008911,0.00032432875466882036
37237,74475,74474,148949,25.529502153396606,0.0003199121004637346
37337,74675,74674,149349,25.607481956481934,0.00031556178091294234
37437,74875,74874,149749,25.67674422264099,0.00031127821212167646
37538,75077,75076,150153,25.760698080062866,0.0003069851531376528
37638,75277,75276,150553,25.841336965560913,0.00030276286615262644
37738,75477,75476,150953,25.905210971832275,0.0002985986174564337
37838,75677,75676,151353,25.96740698814392,0.0002944822463885652
37938,75877,75876,151753,26.03170609474182,0.0002904160362283441
38038,76077,76076,152153,26.10307812690735,0.0002864124403290968
38138,76277,76276,152553,26.17518401145935,0.00028244167543167503
38238,76477,76476,152953,26.23824191093445,0.00027852478478472456
38338,76677,76676,153353,26.300260066986084,0.0002747069173555146
38438,76877,76876,153753,26.36370015144348,0.0002709858114772953
38539,77079,77078,154157,26.429996967315674,0.0002672924926913349
38639,77279,77278,154557,26.49428915977478,0.00026366082676329935
38739,77479,77478,154957,26.55736207962036,0.000260081088605521
38839,77679,77678,155357,26.628175020217896,0.00025660497097583425
38939,77879,77878,155757,26.69702911376953,0.0002532170740752753
39039,78079,78078,156157,26.762163162231445,0.000249862105894635
39139,78279,78278,156557,26.82266902923584,0.0002465091480622687
39239,78479,78478,156957,26.8856520652771,0.00024319187606019246
39339,78679,78678,157357,26.949084043502808,0.00023995092088109765
39439,78879,78878,157757,27.01382327079773,0.00023679246371633084
39540,79081,79080,158161,27.07866406440735,0.00023363741432170235
39640,79281,79280,158561,27.156179189682007,0.0002304928539276233
39740,79481,79480,158961,27.221257209777832,0.00022736031600356234
39840,79681,79680,159361,27.28466010093689,0.00022429472809569855
39940,79881,79880,159761,27.348665952682495,0.0002212867186009496
40040,80081,80080,160161,27.410118103027344,0.00021831011598046925
40140,80281,80280,160561,27.473133087158203,0.00021535368556492132
40240,80481,80480,160961,27.53454613685608,0.00021241060690121028
40340,80681,80680,161361,27.60273027420044,0.00020949154846723123
40440,80881,80880,161761,27.665507078170776,0.00020661824863053065
40541,81083,81082,162165,27.727718114852905,0.00020375826404380435
40641,81283,81282,162565,27.794356107711792,0.0002009538471022078
40741,81483,81482,162965,27.866849899291992,0.00019817875758919694
40841,81683,81682,163365,27.942869186401367,0.00019544804153826215
40941,81883,81882,163765,28.00429892539978,0.00019278533445070357
41041,82083,82082,164165,28.066054105758667,0.00019015671141277296
41141,82283,82282,164565,28.138342142105103,0.00018753012692844666
41241,82483,82482,164965,28.198880910873413,0.00018495469044205076
41341,82683,82682,165365,28.261354207992554,0.0001824572218249232
41441,82883,82882,165765,28.326224088668823,0.00018000883348511461
41542,83085,83084,166169,28.39138913154602,0.00017754663065170265
41642,83285,83284,166569,28.453316926956177,0.00017511878633630218
41742,83485,83484,166969,28.514064073562622,0.0001727470353796481
41842,83685,83684,167369,28.57817006111145,0.00017044773814906474
41942,83885,83884,167769,28.645754098892212,0.000168192474392055
42042,84085,84084,168169,28.706175804138184,0.00016594484112919473
42142,84285,84284,168569,28.768144130706787,0.0001637009127920054
42242,84485,84484,168969,28.828400135040283,0.00016148554606379298
42342,84685,84684,169369,28.88987112045288,0.00015931595937799484
42442,84885,84884,169769,28.951460123062134,0.00015720535074066857
42543,85087,85086,170173,29.01414203643799,0.00015510712129106604
42643,85287,85286,170573,29.07933497428894,0.00015301902981589138
42743,85487,85486,170973,29.150655269622803,0.0001509367516719879
42843,85687,85686,171373,29.213417053222656,0.00014889851699325993
42943,85887,85886,171773,29.27625584602356,0.0001469105714322364
43043,86087,86086,172173,29.342037200927734,0.0001449367195781464
43143,86287,86286,172573,29.40394616127014,0.00014295863287460748
43243,86487,86486,172973,29.465830087661743,0.00014100991283424506
43343,86687,86686,173373,29.52681303024292,0.00013910681993530323
43443,86887,86886,173773,29.594522953033447,0.00013722626148631592
43544,87089,87088,174177,29.660703897476196,0.000135330376518051
43644,87289,87288,174577,29.719914197921753,0.0001334722217873584
43744,87489,87488,174977,29.779982089996338,0.00013165091614106763
43844,87689,87688,175377,29.84107995033264,0.00012985707738058373
43944,87889,87888,175777,29.90396213531494,0.00012808233222352916
44044,88089,88088,176177,29.968348026275635,0.00012632859787115798
44144,88289,88288,176577,30.041334867477417,0.00012460328112476625
44244,88489,88488,176977,30.11862802505493,0.00012291591583379693
44344,88689,88688,177377,30.17786693572998,0.00012126476652245682
44444,88889,88888,177777,30.23773193359375,0.00011963918984645939
44545,89091,89090,178181,30.29670810699463,0.0001180115232430339
44645,89291,89290,178581,30.35511589050293,0.00011642165919494814
44745,89491,89490,178981,30.415800094604492,0.00011487050360592513
44845,89691,89690,179381,30.47470498085022,0.0001133586478329886
44945,89891,89890,179781,30.536998987197876,0.00011187049871040026
45045,90091,90090,180181,30.60517120361328,0.00011038597274011977
45145,90291,90290,180581,30.665380001068115,0.00010891380767797004
45245,90491,90490,180981,30.72723913192749,0.00010747689955334446
45345,90691,90690,181381,30.78827404975891,0.00010607221084003018
45445,90891,90890,181781,30.853456020355225,0.00010468177171523861
45546,91093,91092,182185,30.9131019115448,0.00010328126335128754
45646,91293,91292,182585,30.972707986831665,0.00010190659295263786
45746,91493,91492,182985,31.031719207763672,0.00010055628125608383
45846,91693,91692,183385,31.101589918136597,9.92241229077307e-05
45946,91893,91892,183785,31.16430926322937,9.790250789804027e-05
46046,92093,92092,184185,31.222779035568237,9.659153629019783e-05
46146,92293,92292,184585,31.282708168029785,9.529140614959256e-05
46246,92493,92492,184985,31.354470014572144,9.400391902551128e-05
46346,92693,92692,185385,31.456881999969482,9.27287251912711e-05
46446,92893,92892,185785,31.531164169311523,9.146443006662153e-05
46547,93095,93094,186189,31.605782985687256,9.020271076744699e-05
46647,93295,93294,186589,31.674801111221313,8.897630178099456e-05
46747,93495,93494,186989,31.742414951324463,8.777381094506822e-05
46847,93695,93694,187389,31.813075065612793,8.658846118821059e-05
46947,93895,93894,187789,31.88187313079834,8.541711280645088e-05
47047,94095,94094,188189,31.95291805267334,8.426705601910498e-05
47147,94295,94294,188589,32.02509903907776,8.3142579848123e-05
47247,94495,94494,188989,32.09729290008545,8.20371103771542e-05
47347,94695,94694,189389,32.18608617782593,8.09461441831052e-05
47447,94895,94894,189789,32.25328707695007,7.986790705155107e-05
47548,95097,95096,190193,32.31927704811096,7.87933300547785e-05
47648,95297,95296,190593,32.38481593132019,7.775255755500025e-05
47748,95497,95496,190993,32.4462571144104,7.673850706710915e-05
47848,95697,95696,191393,32.50702404975891,7.574244841671685e-05
47948,95897,95896,191793,32.56598711013794,7.474644786992331e-05
48048,96097,96096,192193,32.63795304298401,7.37476297947579e-05
48148,96297,96296,192593,32.70254397392273,7.276879183600468e-05
48248,96497,96496,192993,32.764564037323,7.18187705444913e-05
48348,96697,96696,193393,32.82630896568298,7.088018018560328e-05
48448,96897,96896,193793,32.88952898979187,6.993998250413446e-05
48549,97099,97098,194197,32.95270109176636,6.899415075101884e-05
48649,97299,97298,194597,33.01601696014404,6.807162562031932e-05
48749,97499,97498,194997,33.07984924316406,6.716226835834011e-05
48849,97699,97698,195397,33.148359060287476,6.626242939790226e-05
48949,97899,97898,195797,33.2096049785614,6.537060257053136e-05
49049,98099,98098,196197,33.27069091796875,6.448441349648132e-05
49149,98299,98298,196597,33.34979009628296,6.360437385327254e-05
49249,98499,98498,196997,33.41513109207153,6.27370202351133e-05
49349,98699,98698,197397,33.47600293159485,6.188935257025183e-05
49449,98899,98898,197797,33.53846216201782,6.105386954099493e-05
49550,99101,99100,198201,33.606016874313354,6.021347451309473e-05
49650,99301,99300,198601,33.66944098472595,5.939477914033675e-05
49750,99501,99500,199001,33.73003101348877,5.8596880940775086e-05
49850,99701,99700,199401,33.79337406158447,5.78095514535441e-05
49950,99901,99900,199801,33.855968952178955,5.702430316514268e-05
50050,100101,100100,200201,33.91671419143677,5.625085952137154e-05
50150,100301,100300,200601,33.98117280006409,5.550218145903701e-05
50250,100501,100500,201001,34.05390405654907,5.47715840925131e-05
50350,100701,100700,201401,34.12641406059265,5.404165415300788e-05
50450,100901,100900,201801,34.1874520778656,5.330900168319847e-05
50551,101103,101102,202205,34.25862693786621,5.258362986721415e-05
50651,101303,101302,202605,34.33473300933838,5.1891280024244815e-05
50751,101503,101502,203005,34.40293002128601,5.121517489468884e-05
50851,101703,101702,203405,34.465912103652954,5.054302430131499e-05
50951,101903,101902,203805,34.52834701538086,4.9869805247115786e-05
51051,102103,102102,204205,34.5994610786438,4.919962326813747e-05
51151,102303,102302,204605,34.6715190410614,4.8542907552255166e-05
51251,102503,102502,205005,34.7339301109314,4.7903805839046464e-05
51351,102703,102702,205405,34.79580783843994,4.7275188382929695e-05
51451,102903,102902,205805,34.863425970077515,4.6645444226357086e-05
51552,103105,103104,206209,34.93513011932373,4.600790896694399e-05
51652,103305,103304,206609,34.99431800842285,4.538790974174408e-05
51752,103505,103504,207009,35.055480003356934,4.478528964614289e-05
51852,103705,103704,207409,35.125855922698975,4.419048837744402e-05
51952,103905,103904,207809,35.18850111961365,4.3593100219979635e-05
52052,104105,104104,208209,35.25419306755066,4.3000121795820345e-05
52152,104305,104304,208609,35.31726312637329,4.242106793022669e-05
52252,104505,104504,209009,35.38417911529541,4.1849358053769155e-05
52352,104705,104704,209409,35.44851112365723,4.127925059440351e-05
52452,104905,104904,209809,35.51094388961792,4.071679436286542e-05
52553,105107,105106,210213,35.57446813583374,4.0162450637070424e-05
52653,105307,105306,210613,35.64508605003357,3.962534499645836e-05
52753,105507,105506,211013,35.71227788925171,3.909372862896381e-05
52853,105707,105706,211413,35.775182008743286,3.856626123627558e-05
52953,105907,105906,211813,35.84217596054077,3.8047723509301315e-05
53053,106107,106106,212213,35.90400290489197,3.7540968902855066e-05
53153,106307,106306,212613,35.96542191505432,3.7045041913201895e-05
53253,106507,106506,213013,36.02898406982422,3.655809932056742e-05
53353,106707,106706,213413,36.0948269367218,3.6075458184646713e-05
53453,106907,106906,213813,36.15817594528198,3.559490123886709e-05
53554,107109,107108,214217,36.22224402427673,3.5118493460720987e-05
53654,107309,107308,214617,36.287328004837036,3.4660711534279084e-05
53754,107509,107508,215017,36.350005865097046,3.421245636981651e-05
53854,107709,107708,215417,36.4267361164093,3.376704634216113e-05
53954,107909,107908,215817,36.50159811973572,3.332276737184541e-05
54054,108109,108108,216217,36.56227898597717,3.2884403631103596e-05
54154,108309,108308,216617,36.63444209098816,3.245579737633296e-05
54254,108509,108508,217017,36.69692397117615,3.2033869085343e-05
54354,108709,108708,217417,36.75911211967468,3.1613480934277026e-05
54454,108909,108908,217817,36.82325601577759,3.1194518887740196e-05
54555,109111,109110,218221,36.88676595687866,3.0776372601044885e-05
54655,109311,109310,218621,36.94714093208313,3.036802552294471e-05
54755,109511,109510,219021,37.01154398918152,2.9963686866388003e-05
54855,109711,109710,219421,37.07317113876343,2.956257478028908e-05
54955,109911,109910,219821,37.145703077316284,2.9165464605280825e-05
55055,110111,110110,220221,37.208394050598145,2.8773619442781398e-05
55155,110311,110310,220621,37.27583980560303,2.8386589314722217e-05
55255,110511,110510,221021,37.34181809425354,2.800494489162376e-05
55355,110711,110710,221421,37.408133029937744,2.7631059997973393e-05
55455,110911,110910,221821,37.47089409828186,2.726392266646076e-05
55556,111113,111112,222225,37.533912897109985,2.6897065123078456e-05
55656,111313,111312,222625,37.59982395172119,2.653832313575744e-05
55756,111513,111512,223025,37.66287708282471,2.6185534068532448e-05
55856,111713,111712,223425,37.72564911842346,2.5837702618988175e-05
55956,111913,111912,223825,37.78809404373169,2.5494838960718564e-05
56056,112113,112112,224225,37.85161900520325,2.5159354731689546e-05
56156,112313,112312,224625,37.91311812400818,2.4831966216797645e-05
56256,112513,112512,225025,37.978302240371704,2.4509057222825604e-05
56356,112713,112712,225425,38.03989791870117,2.418681248729199e-05
56456,112913,112912,225825,38.110198974609375,2.3868444022129383e-05
56557,113115,113114,226229,38.17477798461914,2.3556191364100272e-05
56657,113315,113314,226629,38.23762607574463,2.32534513938797e-05
56757,113515,113514,227029,38.30114698410034,2.2951018693094992e-05
56857,113715,113714,227429,38.36210918426514,2.2648708787882594e-05
56957,113915,113914,227829,38.4267361164093,2.2350633422186926e-05
57057,114115,114114,228229,38.4897198677063,2.205838726543763e-05
57157,114315,114314,228629,38.565540075302124,2.1769862680747687e-05
57257,114515,114514,229029,38.64131283760071,2.148277781867182e-05
57357,114715,114714,229429,38.70189881324768,2.1196788944415933e-05
57457,114915,114914,229829,38.76415705680847,2.0913232059006286e-05
57558,115117,115116,230233,38.825916051864624,2.0630572754566984e-05
57658,115317,115316,230633,38.88910984992981,2.0355435530547253e-05
57758,115517,115516,231033,38.95036602020264,2.0084670740451143e-05
57858,115717,115716,231433,39.01076292991638,1.9815118005125117e-05
57958,115917,115916,231833,39.073758125305176,1.9546345144101378e-05
58058,116117,116116,232233,39.14449715614319,1.9282543162836305e-05
58158,116317,116316,232633,39.20508003234863,1.9025150872184732e-05
58258,116517,116516,233033,39.26600694656372,1.877090736336764e-05
58358,116717,116716,233433,39.3273069858551,1.8517925372826664e-05
58458,116917,116916,233833,39.389875173568726,1.8269186960708648e-05
58559,117119,117118,234237,39.45094108581543,1.8024862487983653e-05
58659,117319,117318,234637,39.511905908584595,1.7786248144470147e-05
58759,117519,117518,235037,39.57428812980652,1.754725716304952e-05
58859,117719,117718,235437,39.64064908027649,1.731171578395909e-05
58959,117919,117918,235837,39.708184003829956,1.708469970895182e-05
59059,118119,118118,236237,39.76994299888611,1.6863221199562754e-05
59159,118319,118318,236637,39.83060598373413,1.6641336201894356e-05
59259,118519,118518,237037,39.895217180252075,1.641927382851309e-05
59359,118719,118718,237437,39.95704793930054,1.6201047542240282e-05
59459,118919,118918,237837,40.01704692840576,1.598856763751764e-05
59560,119121,119120,238241,40.08372116088867,1.5779008401789754e-05
59660,119321,119320,238641,40.15004205703735,1.557431044986517e-05
59760,119521,119520,239041,40.2139630317688,1.536968477946451e-05
59860,119721,119720,239441,40.27495312690735,1.5164558149519381e-05
59960,119921,119920,239841,40.33594298362732,1.4962404983243916e-05
60060,120121,120120,240241,40.398828983306885,1.4766685971927884e-05
60160,120321,120320,240641,40.46017408370972,1.457505770578934e-05
60260,120521,120520,241041,40.5226411819458,1.4382059827067614e-05
60360,120721,120720,241441,40.58719086647034,1.4187539157506675e-05
60460,120921,120920,241841,40.66245698928833,1.3996562486301185e-05
60561,121123,121122,242245,40.73913311958313,1.3808914828650358e-05
60661,121323,121322,242645,40.80331110954285,1.3625179787876983e-05
60761,121523,121522,243045,40.86395311355591,1.344206446166368e-05
60861,121723,121722,243445,40.92599105834961,1.326128379466981e-05
60961,121923,121922,243845,40.98927712440491,1.308392771305674e-05
61061,122123,122122,244245,41.05084705352783,1.2908697534080166e-05
61161,122323,122322,244645,41.11640000343323,1.273450965751624e-05
61261,122523,122522,245045,41.18063926696777,1.2562947305821196e-05
61361,122723,122722,245445,41.24595499038696,1.2395661101612578e-05
61461,122923,122922,245845,41.30947399139404,1.2231749394925177e-05
61562,123125,123124,246249,41.37196397781372,1.2068110216465646e-05
61662,123325,123324,246649,41.43293499946594,1.190761661267762e-05
61762,123525,123524,247049,41.49506115913391,1.1748879106988308e-05
61862,123725,123724,247449,41.55664610862732,1.1592878919587142e-05
61962,123925,123924,247849,41.62825322151184,1.1441064976767601e-05
62062,124125,124124,248249,41.68939208984375,1.129329834429313e-05
62162,124325,124324,248649,41.75192999839783,1.1147214705800233e-05
62262,124525,124524,249049,41.81422805786133,1.1001034686926076e-05
62362,124725,124724,249449,41.87589120864868,1.0856280824629917e-05
62462,124925,124924,249849,41.937427043914795,1.0715669831420112e-05
62563,125127,125126,250253,42.00268602371216,1.0577419157284645e-05
62663,125327,125326,250653,42.06531023979187,1.0441099034850115e-05
62763,125527,125526,251053,42.13240098953247,1.0304129621921061e-05
62863,125727,125726,251453,42.19511604309082,1.016850405473781e-05
62963,125927,125926,251853,42.255818128585815,1.003590734087636e-05
63063,126127,126126,252253,42.31610417366028,9.905663515528842e-06
63163,126327,126326,252653,42.37799406051636,9.776231674630495e-06
63263,126527,126526,253053,42.439424991607666,9.646969993890194e-06
63363,126727,126726,253453,42.50305199623108,9.518397385894576e-06
63463,126927,126926,253853,42.563010931015015,9.391345600739486e-06
63564,127129,127128,254257,42.63484311103821,9.265171867246204e-06
63664,127329,127328,254657,42.69580101966858,9.142481799285115e-06
63764,127529,127528,255057,42.76039791107178,9.021334224134595e-06
63864,127729,127728,255457,42.83613109588623,8.901121562321754e-06
63964,127929,127928,255857,42.908565282821655,8.782294051120254e-06
64064,128129,128128,256257,42.97164988517761,8.665488081012583e-06
64164,128329,128328,256657,43.03434991836548,8.550460750440408e-06
64264,128529,128528,257057,43.09929895401001,8.43674364180119e-06
64364,128729,128728,257457,43.16047501564026,8.324758719936274e-06
64464,128929,128928,257857,43.22327995300293,8.215242654047104e-06
64565,129131,129130,258261,43.28415393829346,8.106802506795829e-06
64665,129331,129330,258661,43.344380140304565,8.000536206253941e-06
64765,129531,129530,259061,43.40612602233887,7.895380604105163e-06
64865,129731,129730,259461,43.47316384315491,7.792696216688844e-06
64965,129931,129930,259861,43.53782391548157,7.692953330640033e-06
65065,130131,130130,260261,43.60539412498474,7.594610385406215e-06
65165,130331,130330,260661,43.66908311843872,7.496273077682297e-06
65265,130531,130530,261061,43.73137903213501,7.398593347159155e-06
65365,130731,130730,261461,43.792842864990234,7.302999744868574e-06
65465,130931,130930,261861,43.856045961380005,7.209465408994336e-06
65566,131133,131132,262265,43.920734167099,7.115722701213056e-06
65666,131333,131332,262665,43.98829197883606,7.0229707376554675e-06
65766,131533,131532,263065,44.049681186676025,6.930881685774421e-06
65866,131733,131732,263465,44.11652398109436,6.8400844726079e-06
65966,131933,131932,263865,44.17905807495117,6.750581686664404e-06
66066,132133,132132,264265,44.242534160614014,6.66209894777586e-06
66166,132333,132332,264665,44.3046350479126,6.5741509130985995e-06
66266,132533,132532,265065,44.36621809005737,6.48645199468879e-06
66366,132733,132732,265465,44.42738199234009,6.399695302363347e-06
66466,132933,132932,265865,44.487658977508545,6.314753666567243e-06
66567,133135,133134,266269,44.551188230514526,6.230391419451172e-06
66667,133335,133334,266669,44.62120699882507,6.147231091210102e-06
66767,133535,133534,267069,44.68229699134827,6.064590273535045e-06
66867,133735,133734,267469,44.743597984313965,5.983633197660427e-06
66967,133935,133934,267869,44.805083990097046,5.904500097168502e-06
67067,134135,134134,268269,44.86585307121277,5.8261195620669355e-06
67167,134335,134334,268669,44.934552907943726,5.7483127715344485e-06
67267,134535,134534,269069,45.011234998703,5.6722020976153525e-06
67367,134735,134734,269469,45.07902002334595,5.59811751231062e-06
67467,134935,134934,269869,45.14584684371948,5.524869320789642e-06
67568,135137,135136,270273,45.210299015045166,5.451012558301816e-06
67668,135337,135336,270673,45.271103858947754,5.378938124540822e-06
67768,135537,135536,271073,45.33196210861206,5.3088875837808785e-06
67868,135737,135736,271473,45.40041422843933,5.240498582477052e-06
67968,135937,135936,271873,45.47211313247681,5.172779183017556e-06
68068,136137,136136,272273,45.54034614562988,5.1052908066521035e-06
68168,136337,136336,272673,45.60788917541504,5.038372022308147e-06
68268,136537,136536,273073,45.67269587516785,4.972691850730634e-06
68368,136737,136736,273473,45.73454809188843,4.908635577391338e-06
68468,136937,136936,273873,45.79585289955139,4.845681559774986e-06
68569,137139,137138,274277,45.85769200325012,4.781987861208881e-06
68669,137339,137338,274677,45.9191529750824,4.718427398654161e-06
68769,137539,137538,275077,45.988105058670044,4.655627763733472e-06
68869,137739,137738,275477,46.052348136901855,4.5947647018922884e-06
68969,137939,137938,275877,46.13656687736511,4.5351459607733985e-06
69069,138139,138138,276277,46.24317717552185,4.475362057572486e-06
69169,138339,138338,276677,46.3341338634491,4.415412801732109e-06
69269,138539,138538,277077,46.42189884185791,4.356381009844091e-06
69369,138739,138738,277477,46.50967597961426,4.2986476065856275e-06
69469,138939,138938,277877,46.60119700431824,4.241636799821523e-06
69570,139141,139140,278281,46.713606119155884,4.184458058229318e-06
69670,139341,139340,278681,46.833035945892334,4.128573691093181e-06
69770,139541,139540,279081,47.00057792663574,4.073628937244107e-06
69870,139741,139740,279481,47.163334131240845,4.019384169356878e-06
69970,139941,139940,279881,47.26028895378113,3.9656849566078106e-06
70070,140141,140140,280281,47.35255408287048,3.912716865861502e-06
70170,140341,140340,280681,47.52888107299805,3.860739730706228e-06
70270,140541,140540,281081,47.682695150375366,3.8099352109141677e-06
70370,140741,140740,281481,47.79028105735779,3.7602608635376523e-06
70470,140941,140940,281881,47.89018988609314,3.711283297876071e-06
70571,141143,141142,282285,48.01051902770996,3.6621119616174e-06
70671,141343,141342,282685,48.13720202445984,3.6140261599831843e-06
70771,141543,141542,283085,48.28184103965759,3.5672574638238214e-06
70871,141743,141742,283485,48.451282024383545,3.5218198378121066e-06
70971,141943,141942,283885,48.55519199371338,3.4767756128437345e-06
71071,142143,142142,284285,48.64660286903381,3.4314777890495462e-06
71171,142343,142342,284685,48.73191499710083,3.3865220333733076e-06
71271,142543,142542,285085,48.851682901382446,3.342875262033436e-06
71371,142743,142742,285485,48.950061082839966,3.300474337122758e-06
71471,142943,142942,285885,49.062719106674194,3.258373914769819e-06
71572,143145,143144,286289,49.14175605773926,3.2155494402842386e-06
71672,143345,143344,286689,49.20627808570862,3.173140221056529e-06
71772,143545,143544,287089,49.277894020080566,3.131373868268516e-06
71872,143745,143744,287489,49.34457993507385,3.0905167018022717e-06
71972,143945,143944,287889,49.404491901397705,3.0502612173691828e-06
72072,144145,144144,288289,49.46297526359558,3.0101730893575022e-06
72172,144345,144344,288689,49.52546405792236,2.9702133934267824e-06
72272,144545,144544,289089,49.59100008010864,2.930729137943508e-06
72372,144745,144744,289489,49.6502890586853,2.891960787883277e-06
72472,144945,144944,289889,49.709312915802,2.853758575963227e-06
72573,145147,145146,290293,49.76775789260864,2.8154894636607945e-06
72673,145347,145346,290693,49.826874017715454,2.7779771944394187e-06
72773,145547,145546,291093,49.885855197906494,2.7411133582366744e-06
72873,145747,145746,291493,49.94642901420593,2.704941901160451e-06
72973,145947,145946,291893,50.0100839138031,2.669262329436456e-06
73073,146147,146146,292293,50.06869697570801,2.6340008269975367e-06
73173,146347,146346,292693,50.13275098800659,2.5993981340683537e-06
73273,146547,146546,293093,50.19088411331177,2.5657203667815465e-06
73373,146747,146746,293493,50.24940609931946,2.532789066555339e-06
73473,146947,146946,293893,50.30942106246948,2.50011134279012e-06
73574,147149,147148,294297,50.369611978530884,2.467259826246608e-06
73674,147349,147348,294697,50.42786192893982,2.4353362963411973e-06
73774,147549,147548,295097,50.48671293258667,2.4043138531598285e-06
73874,147749,147748,295497,50.547229051589966,2.37386541896849e-06
73974,147949,147948,295897,50.61403799057007,2.3434816861004225e-06
74074,148149,148148,296297,50.674803018569946,2.3131430997051076e-06
74174,148349,148348,296697,50.74156618118286,2.283247669469385e-06
74274,148549,148548,297097,50.806737184524536,2.253975807006888e-06
74374,148749,148748,297497,50.87626004219055,2.2250664127367224e-06
74474,148949,148948,297897,50.943613052368164,2.196226531684181e-06
74575,149151,149150,298301,51.01614189147949,2.1671703462334003e-06
74675,149351,149350,298701,51.08936524391174,2.1386841571338265e-06
74775,149551,149550,299101,51.16186785697937,2.1106847409432683e-06
74875,149751,149750,299501,51.22897696495056,2.083160119411901e-06
74975,149951,149950,299901,51.29247808456421,2.055870114067057e-06
75075,150151,150150,300301,51.37346601486206,2.0286581622842124e-06
75175,150351,150350,300701,51.46055793762207,2.001678594610852e-06
75275,150551,150550,301101,51.52391004562378,1.9751612161495315e-06
75375,150751,150750,301501,51.58907103538513,1.9490634140730767e-06
75475,150951,150950,301901,51.65888595581055,1.9231725683858647e-06
75576,151153,151152,302305,51.73671317100525,1.897276205675667e-06
75676,151353,151352,302705,51.82238817214966,1.8721762234944973e-06
75776,151553,151552,303105,51.91272211074829,1.8476386645876327e-06
75876,151753,151752,303505,51.99655795097351,1.8233658248114926e-06
75976,151953,151952,303905,52.083575963974,1.7992795376471934e-06
76076,152153,152152,304305,52.174535036087036,1.7756602025019653e-06
76176,152353,152352,304705,52.25943207740784,1.7526567163773291e-06
76276,152553,152552,305105,52.343437910079956,1.730046675658995e-06
76376,152753,152752,305505,52.4360671043396,1.7075830281189038e-06
76476,152953,152952,305905,52.51924705505371,1.6853197299998661e-06
76577,153155,153154,306309,52.60535407066345,1.6632740162371466e-06
76677,153355,153354,306709,52.7059428691864,1.641958314212697e-06
76777,153555,153554,307109,52.807437896728516,1.6209768166841254e-06
76877,153755,153754,307509,52.89422607421875,1.6001114613554674e-06
76977,153955,153954,307909,52.966979026794434,1.5793171581909331e-06
77077,154155,154154,308309,53.04375910758972,1.5587758224610203e-06
77177,154355,154354,308709,53.11430311203003,1.5387101828945736e-06
77277,154555,154554,309109,53.18322491645813,1.5190614429729995e-06
77377,154755,154754,309509,53.249943017959595,1.499491205619686e-06
77477,154955,154954,309909,53.32708406448364,1.479828142619619e-06
77578,155157,155156,310313,53.40073585510254,1.4601140259797666e-06
77678,155357,155356,310713,53.469146966934204,1.4410305389634888e-06
77778,155557,155556,311113,53.55173707008362,1.4223108037130692e-06
77878,155757,155756,311513,53.63024401664734,1.4036687264117373e-06
77978,155957,155956,311913,53.698304891586304,1.3850540833661777e-06
78078,156157,156156,312313,53.76786017417908,1.3667010044589633e-06
78178,156357,156356,312713,53.840993881225586,1.3487264235601684e-06
78278,156557,156556,313113,53.911596059799194,1.3309778004710473e-06
78378,156757,156756,313513,53.9773850440979,1.3133286935518504e-06
78478,156957,156956,313913,54.04286813735962,1.2958550399914074e-06
78579,157159,157158,314317,54.112529039382935,1.2785058880452096e-06
78679,157359,157358,314717,54.21315598487854,1.2616366022587691e-06
78779,157559,157558,315117,54.3035409450531,1.2450022667915494e-06
78879,157759,157758,315517,54.407307863235474,1.228564228909038e-06
78979,157959,157958,315917,54.550549268722534,1.2123972180442847e-06
79079,158159,158158,316317,54.69971203804016,1.1966345570892125e-06
79179,158359,158358,316717,54.81678605079651,1.1812765634458496e-06
79279,158559,158558,317117,54.9197359085083,1.1661133984540584e-06
79379,158759,158758,317517,55.053932905197144,1.1509604386044877e-06
79479,158959,158958,317917,55.3762149810791,1.1359297236404193e-06
79580,159161,159160,318321,55.515713930130005,1.1211606615215198e-06
79680,159361,159360,318721,55.788756132125854,1.106994003751121e-06
79780,159561,159560,319121,55.90830707550049,1.0930002808288197e-06
79880,159761,159760,319521,56.0097599029541,1.0789334353930932e-06
79980,159961,159960,319921,56.10833501815796,1.0648759325701037e-06
80080,160161,160160,320321,56.21704697608948,1.0511011777225084e-06
80180,160361,160360,320721,56.333479166030884,1.037718651993088e-06
80280,160561,160560,321121,56.413639068603516,1.02453581122427e-06
80380,160761,160760,321521,56.48496913909912,1.0113074792462165e-06
80480,160961,160960,321921,56.55391502380371,9.980409102504748e-07
80581,161163,161162,322325,56.62382984161377,9.84812725307809e-07
80681,161363,161362,322725,56.687779903411865,9.71989968978785e-07
80781,161563,161562,323125,56.75088405609131,9.59338485035773e-07
80881,161763,161762,323525,56.81665015220642,9.467388385549771e-07
80981,161963,161962,323925,56.881009101867676,9.342113440382171e-07
81081,162163,162162,324325,56.94509315490723,9.218428893081178e-07
81181,162363,162362,324725,57.011871099472046,9.096524955728146e-07
81281,162563,162562,325125,57.079885959625244,8.975950408413405e-07
81381,162763,162762,325525,57.14629101753235,8.856597116835539e-07
81481,162963,162962,325925,57.212536096572876,8.739086048007357e-07
81582,163165,163164,326329,57.28051018714905,8.623056274364478e-07
81682,163365,163364,326729,57.34314298629761,8.510728628959714e-07
81782,163565,163564,327129,57.404136180877686,8.399859576997568e-07
81882,163765,163764,327529,57.46626019477844,8.28973399623453e-07
81982,163965,163964,327929,57.528002977371216,8.18121036949982e-07
82082,164165,164164,328329,57.5944390296936,8.07562756459861e-07
82182,164365,164364,328729,57.672703981399536,7.972682338575978e-07
82282,164565,164564,329129,57.80600118637085,7.870567860262749e-07
82382,164765,164764,329529,57.9662880897522,7.76845055511189e-07
82482,164965,164964,329929,58.10435509681702,7.667710316043862e-07
82583,165167,165166,330333,58.20024108886719,7.56899448496898e-07
82683,165367,165366,330733,58.339402198791504,7.473681430137038e-07
82783,165567,165566,331133,58.41625690460205,7.378826751550724e-07
82883,165767,165766,331533,58.48291492462158,7.283698627410048e-07
82983,165967,165966,331933,58.555341958999634,7.189291587429368e-07
83083,166167,166166,332333,58.62894606590271,7.096616351320971e-07
83183,166367,166366,332733,58.69477295875549,7.005564449327429e-07
83283,166567,166566,333133,58.76033806800842,6.915363164143912e-07
83383,166767,166766,333533,58.82162809371948,6.825485567282871e-07
83483,166967,166966,333933,58.88571619987488,6.736054163060824e-07
83584,167169,167168,334337,58.948275089263916,6.64675622170777e-07
83684,167369,167368,334737,59.00863003730774,6.559731621402759e-07
83784,167569,167568,335137,59.07350206375122,6.473728992648623e-07
83884,167769,167768,335537,59.14472699165344,6.388193986135177e-07
83984,167969,167968,335937,59.20524621009827,6.303404185190975e-07
84084,168169,168168,336337,59.26683211326599,6.220153400005334e-07
84184,168369,168368,336737,59.32881307601929,6.138386465811043e-07
84284,168569,168568,337137,59.3892240524292,6.057323681299346e-07
84384,168769,168768,337537,59.44555401802063,5.976997003102e-07
84484,168969,168968,337937,59.50339126586914,5.898358063044231e-07
84585,169171,169170,338341,59.56257605552673,5.820911172253894e-07
84685,169371,169370,338741,59.640340089797974,5.745292798689279e-07
84785,169571,169570,339141,59.697405099868774,5.670188052183681e-07
84885,169771,169770,339541,59.75347399711609,5.596269024825933e-07
84985,169971,169970,339941,59.812660932540894,5.524269980773158e-07
85085,170171,170170,340341,59.870933055877686,5.453812953359679e-07
85185,170371,170370,340741,59.92925190925598,5.384007097581502e-07
85285,170571,170570,341141,59.98823308944702,5.314629742103067e-07
85385,170771,170770,341541,60.057323932647705,5.246125249619598e-07
85485,170971,170970,341941,60.138755083084106,5.178940241492014e-07
85586,171173,171172,342345,60.19812226295471,5.112461401192589e-07
85686,171373,171372,342745,60.25745511054993,5.047510456620906e-07
85786,171573,171572,343145,60.3152060508728,4.98279971848266e-07
85886,171773,171772,343545,60.37279200553894,4.918378873496897e-07
85986,171973,171972,343945,60.430197954177856,4.855003412850737e-07
86086,172173,172172,344345,60.488065004348755,4.793014542702111e-07
86186,172373,172372,344745,60.54468107223511,4.731707162234944e-07
86286,172573,172572,345145,60.61127591133118,4.6703370544062936e-07
86386,172773,172772,345545,60.66874313354492,4.6092387943038116e-07
86486,172973,172972,345945,60.72702097892761,4.549208125067141e-07
86587,173175,173174,346349,60.79018211364746,4.489617986992717e-07
86687,173375,173374,346749,60.84961915016174,4.4309639238041163e-07
86787,173575,173574,347149,60.90852117538452,4.372536356281754e-07
86887,173775,173774,347549,60.96709609031677,4.3148845364379756e-07
86987,173975,173974,347949,61.02718806266785,4.2582792364123674e-07
87087,174175,174174,348349,61.09632921218872,4.202407683102412e-07
87187,174375,174374,348749,61.16103219985962,4.1470201511649623e-07
87287,174575,174574,349149,61.221421003341675,4.0923929625836375e-07
87387,174775,174774,349549,61.28217792510986,4.038954064719308e-07
87487,174975,174974,349949,61.34342002868652,3.9866535927738726e-07
87588,175177,175176,350353,61.40755915641785,3.934479138385259e-07
87688,175377,175376,350753,61.46937298774719,3.8831585236473277e-07
87788,175577,175576,351153,61.53162622451782,3.8324783431102253e-07
87888,175777,175776,351553,61.59987282752991,3.783014300808727e-07
87988,175977,175976,351953,61.66361403465271,3.7349043189766426e-07
88088,176177,176176,352353,61.728219985961914,3.687543516557307e-07
88188,176377,176376,352753,61.793983936309814,3.6402077382938554e-07
88288,176577,176576,353153,61.85445499420166,3.592973850894314e-07
88388,176777,176776,353553,61.913514137268066,3.5466825079840123e-07
88488,176977,176976,353953,61.97700500488281,3.501833935038594e-07
88589,177179,177178,354357,62.03881001472473,3.457401211960559e-07
88689,177379,177378,354757,62.10493302345276,3.413307633637492e-07
88789,177579,177578,355157,62.17434000968933,3.3690559595217554e-07
88889,177779,177778,355557,62.2491180896759,3.325447541066129e-07
88989,177979,177978,355957,62.31930208206177,3.2829432744079283e-07
89089,178179,178178,356357,62.38290095329285,3.241100511424351e-07
89189,178379,178378,356757,62.445334911346436,3.1992958901349495e-07
89289,178579,178578,357157,62.50740385055542,3.157490857419479e-07
89389,178779,178778,357557,62.57143998146057,3.1160703902677945e-07
89489,178979,178978,357957,62.639281034469604,3.075258219620171e-07
89590,179181,179180,358361,62.70172095298767,3.034554244735506e-07
89690,179381,179380,358761,62.763108015060425,2.994642989567752e-07
89790,179581,179580,359161,62.82370710372925,2.955189481870578e-07
89890,179781,179780,359561,62.88573718070984,2.916317893811425e-07
89990,179981,179980,359961,62.94618320465088,2.878017806375548e-07
90090,180181,180180,360361,63.008506059646606,2.840178070243734e-07
90190,180381,180380,360761,63.06947708129883,2.802761809596499e-07
90290,180581,180580,361161,63.13551092147827,2.7659266984286624e-07
90390,180781,180780,361561,63.199581146240234,2.729884454726329e-07
90490,180981,180980,361961,63.260847091674805,2.694570228341854e-07
90591,181183,181182,362365,63.32175087928772,2.659236718974791e-07
90691,181383,181382,362765,63.38357400894165,2.6243452007327257e-07
90791,181583,181582,363165,63.44469404220581,2.58993114677176e-07
90891,181783,181782,363565,63.505364179611206,2.5566217880270534e-07
90991,181983,181982,363965,63.56713104248047,2.5243783962857854e-07
91091,182183,182182,364365,63.638176918029785,2.4924061306646697e-07
91191,182383,182382,364765,63.70151996612549,2.4601781448732245e-07
91291,182583,182582,365165,63.76726007461548,2.428088448939167e-07
91391,182783,182782,365565,63.829344034194946,2.3968076488781484e-07
91491,182983,182982,365965,63.890239238739014,2.3664058088134135e-07
91592,183185,183184,366369,63.95210099220276,2.3361125845763882e-07
91692,183385,183384,366769,64.01482892036438,2.306154779676401e-07
91792,183585,183584,367169,64.08338809013367,2.2762646922499224e-07
91892,183785,183784,367569,64.15010404586792,2.2467076897077982e-07
91992,183985,183984,367969,64.21209907531738,2.2176874456018583e-07
92092,184185,184184,368369,64.27449011802673,2.1891465319048568e-07
92192,184385,184384,368769,64.35121083259583,2.160808283472879e-07
92292,184585,184584,369169,64.42587995529175,2.132515083416634e-07
92392,184785,184784,369569,64.4876389503479,2.1044556050318778e-07
92492,184985,184984,369969,64.54858899116516,2.0768665827082568e-07
92593,185187,185186,370373,64.61726188659668,2.049393320298659e-07
92693,185387,185386,370773,64.67952394485474,2.0223895870476415e-07
92793,185587,185586,371173,64.73956108093262,1.9956986565865546e-07
92893,185787,185786,371573,64.80754017829895,1.9695624011774926e-07
92993,185987,185986,371973,64.87872195243835,1.9439022761319223e-07
93093,186187,186186,372373,64.93885827064514,1.9184348751990393e-07
93193,186387,186386,372773,65.00127601623535,1.8931807932418783e-07
93293,186587,186586,373173,65.06279993057251,1.8684723828702833e-07
93393,186787,186786,373573,65.13407516479492,1.8444155622733132e-07
93493,186987,186986,373973,65.19764590263367,1.8207093099068698e-07
93594,187189,187188,374377,65.26067900657654,1.7968696706717006e-07
93694,187389,187388,374777,65.32538414001465,1.773497535135692e-07
93794,187589,187588,375177,65.39113807678223,1.750610675730683e-07
93894,187789,187788,375577,65.4549069404602,1.7282639514493302e-07
93994,187989,187988,375977,65.51540112495422,1.7063077085102618e-07
94094,188189,188188,376377,65.57798600196838,1.6845547286051536e-07
94194,188389,188388,376777,65.64220094680786,1.662951619960348e-07
94294,188589,188588,377177,65.70305395126343,1.6416455155661717e-07
94394,188789,188788,377577,65.76529288291931,1.620813442127127e-07
94494,188989,188988,377977,65.8293149471283,1.6003768625909009e-07
94595,189191,189190,378381,65.89374089241028,1.5798376968129012e-07
94695,189391,189390,378781,65.95532894134521,1.5594927282129926e-07
94795,189591,189590,379181,66.0213840007782,1.5393724878015208e-07
94895,189791,189790,379581,66.09096693992615,1.5196762477585909e-07
94995,189991,189990,379981,66.15965104103088,1.500259445314524e-07
95095,190191,190190,380381,66.22487902641296,1.4808877558474724e-07
95195,190391,190390,380781,66.28939414024353,1.461591711799253e-07
95295,190591,190590,381181,66.35283493995667,1.4425512259684798e-07
95395,190791,190790,381581,66.41977000236511,1.4237927665839035e-07
95495,190991,190990,381981,66.49664902687073,1.4052204863592887e-07
95596,191193,191192,382385,66.57035994529724,1.3866669116723945e-07
95696,191393,191392,382785,66.64188313484192,1.36861693201495e-07
95796,191593,191592,383185,66.70394110679626,1.3508902453702186e-07
95896,191793,191792,383585,66.76589703559875,1.3333551394461236e-07
95996,191993,191992,383985,66.82851600646973,1.3159468565300743e-07
96096,192193,192192,384385,66.88961505889893,1.298758445492291e-07
96196,192393,192392,384785,66.95433688163757,1.2819087595875126e-07
96296,192593,192592,385185,67.01899695396423,1.2654030129500964e-07
96396,192793,192792,385585,67.09030389785767,1.2491296775374385e-07
96496,192993,192992,385985,67.15491914749146,1.232975807588221e-07
96597,193195,193194,386389,67.21621489524841,1.21681086645127e-07
96697,193395,193394,386789,67.27611207962036,1.2011397492136512e-07
96797,193595,193594,387189,67.33674001693726,1.1859255832053948e-07
96897,193795,193794,387589,67.39828491210938,1.1710314294690344e-07
96997,193995,193994,387989,67.46118593215942,1.1561863928819943e-07
97097,194195,194194,388389,67.52262115478516,1.1413259145640853e-07
97197,194395,194394,388789,67.58765411376953,1.1266647268651179e-07
97297,194595,194594,389189,67.65419793128967,1.1123815389220658e-07
97397,194795,194794,389589,67.71676707267761,1.0983707308542618e-07
97497,194995,194994,389989,67.77789402008057,1.0844044261370887e-07
97598,195197,195196,390393,67.84028601646423,1.0702971110083916e-07
97698,195397,195396,390793,67.9024760723114,1.0564846004107998e-07
97798,195597,195596,391193,67.96525812149048,1.0429443531656666e-07
97898,195797,195796,391593,68.02767515182495,1.0296136319101379e-07
97998,195997,195996,391993,68.09445810317993,1.0163519263577301e-07
98098,196197,196196,392393,68.15877223014832,1.0031055309750041e-07
98198,196397,196396,392793,68.220046043396,9.899313081771302e-08
98298,196597,196596,393193,68.28225922584534,9.769131601394468e-08
98398,196797,196796,393593,68.34306192398071,9.641004054117868e-08
98498,196997,196996,393993,68.40409517288208,9.514998789068313e-08
98599,197199,197198,394397,68.46648097038269,9.389684417067932e-08
98699,197399,197398,394797,68.52869296073914,9.267288763188241e-08
98799,197599,197598,395197,68.60963296890259,9.146341848563611e-08
98899,197799,197798,395597,68.68404603004456,9.026603997886941e-08
98999,197999,197998,395997,68.74426889419556,8.908089308017963e-08
99099,198199,198198,396397,68.80768084526062,8.791512840493742e-08
99199,198399,198398,396797,68.87003302574158,8.677837459261317e-08
99299,198599,198598,397197,68.93086504936218,8.566834892541664e-08
99399,198799,198798,397597,68.99082899093628,8.456765038740797e-08
99499,198999,198998,397997,69.05367422103882,8.346420550597914e-08
99600,199201,199200,398401,69.12402701377869,8.235951600078817e-08
99700,199401,199400,398801,69.1858160495758,8.129874259265131e-08
99800,199601,199600,399201,69.24980020523071,8.027370658637301e-08
99900,199801,199800,399601,69.31107902526855,7.926245077442256e-08
100000,200001,200000,400001,69.37177109718323,7.824581526884113e-08


==> plot_data/quadratic_minimax_problem_n500_alpha00001/eg.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0006909370422363281,30.358106049564984
100,201,200,401,0.06297898292541504,1.7063375198016169
200,401,400,801,0.12068986892700195,1.0108894113540814
300,601,600,1201,0.1797010898590088,0.7489939892258344
400,801,800,1601,0.2371671199798584,0.6081938727196392
501,1003,1002,2005,0.29901909828186035,0.5168895867181229
601,1203,1202,2405,0.3597109317779541,0.452278382327617
701,1403,1402,2805,0.4363288879394531,0.40291992726905773
801,1603,1602,3205,0.5007870197296143,0.3634630940471491
901,1803,1802,3605,0.5554502010345459,0.33097564129661755
1001,2003,2002,4005,0.612037181854248,0.3037093528611154
1101,2203,2202,4405,0.6704959869384766,0.2803953971483973
1201,2403,2402,4805,0.731205940246582,0.26019451460291226
1301,2603,2602,5205,0.7891478538513184,0.24250818197445992
1401,2803,2802,5605,0.8446431159973145,0.22685332490806293
1502,3005,3004,6009,0.8997559547424316,0.2127929708960007
1602,3205,3204,6409,0.9590818881988525,0.20030755961093588
1702,3405,3404,6809,1.0188090801239014,0.18902363243190226
1802,3605,3604,7209,1.1354889869689941,0.17874588608055825
1902,3805,3804,7609,1.1929447650909424,0.16936686708805634
2002,4005,4004,8009,1.2480969429016113,0.16078928006504323
2102,4205,4204,8409,1.3040919303894043,0.15289388141740703
2202,4405,4404,8809,1.3596839904785156,0.1455894973020299
2302,4605,4604,9209,1.4141571521759033,0.13880996643974702
2402,4805,4804,9609,1.471203088760376,0.13250544845542997
2503,5007,5006,10013,1.527184009552002,0.12658272496808612
2603,5207,5206,10413,1.5825860500335693,0.12107898410631822
2703,5407,5406,10813,1.639333963394165,0.11592039425419869
2803,5607,5606,11213,1.6979539394378662,0.11108349163202878
2903,5807,5806,11613,1.770596981048584,0.10652119458942605
3003,6007,6006,12013,1.842939853668213,0.10222880204007911
3103,6207,6206,12413,1.9022667407989502,0.09818713706730445
3203,6407,6406,12813,1.964468002319336,0.09436920147170691
3303,6607,6606,13213,2.0247550010681152,0.09073320222110537
3403,6807,6806,13613,2.0829389095306396,0.08729857820057606
3504,7009,7008,14017,2.1414718627929688,0.08401838454826126
3604,7209,7208,14417,2.202371120452881,0.08093927928962326
3704,7409,7408,14817,2.260944128036499,0.07800912151469362
3804,7609,7608,15217,2.3210020065307617,0.0752232971485176
3904,7809,7808,15617,2.3794310092926025,0.07257609242688355
4004,8009,8008,16017,2.437541961669922,0.07005957569801338
4104,8209,8208,16417,2.5040807723999023,0.06766082262576223
4204,8409,8408,16817,2.5689220428466797,0.0653627511027669
4304,8609,8608,17217,2.628204107284546,0.06318097775381688
4404,8809,8808,17617,2.686371088027954,0.06110300953777403
4505,9011,9010,18021,2.7455148696899414,0.0590937428271714
4605,9211,9210,18421,2.809199094772339,0.05717733161162599
4705,9411,9410,18821,2.868955135345459,0.05535773017085458
4805,9611,9610,19221,2.930063009262085,0.05361798797459647
4905,9811,9810,19621,2.9879109859466553,0.05194900886724691
5005,10011,10010,20021,3.047333002090454,0.05035243765185992
5105,10211,10210,20421,3.1072051525115967,0.04882063373100812
5205,10411,10410,20821,3.167013168334961,0.047359071023488915
5305,10611,10610,21221,3.2246079444885254,0.045955467781552156
5405,10811,10810,21621,3.281989812850952,0.04461009631068081
5506,11013,11012,22025,3.3391427993774414,0.043314099629270165
5606,11213,11212,22425,3.396791934967041,0.04207838125332836
5706,11413,11412,22825,3.453721046447754,0.040893441689385045
5806,11613,11612,23225,3.5102310180664062,0.039758063729968526
5906,11813,11812,23625,3.5669801235198975,0.03866727459590865
6006,12013,12012,24025,3.623012065887451,0.03762274291255587
6106,12213,12212,24425,3.6800589561462402,0.036611040471708
6206,12413,12412,24825,3.73641300201416,0.03562856314436133
6306,12613,12612,25225,3.7920429706573486,0.03469692269248736
6406,12813,12812,25625,3.847104072570801,0.033799683286082904
6507,13015,13014,26029,3.916735887527466,0.032929696359171264
6607,13215,13214,26429,3.986114978790283,0.03210090886963369
6707,13415,13414,26829,4.0440239906311035,0.03129562467976816
6807,13615,13614,27229,4.101706027984619,0.030518070810675323
6907,13815,13814,27629,4.159929990768433,0.02976476100537671
7007,14015,14014,28029,4.215943813323975,0.029042946413349643
7107,14215,14214,28429,4.273210763931274,0.028345043787213003
7207,14415,14414,28829,4.332073926925659,0.0276787893149401
7307,14615,14614,29229,4.389107942581177,0.027025990891256242
7407,14815,14814,29629,4.444912910461426,0.02639680752696954
7508,15017,15016,30033,4.501189947128296,0.025790202933365928
7608,15217,15216,30433,4.556909084320068,0.025208342940185372
7708,15417,15416,30833,4.618888854980469,0.024644675806295535
7808,15617,15616,31233,4.677147150039673,0.024097814611134232
7908,15817,15816,31633,4.733443021774292,0.023566249852129673
8008,16017,16016,32033,4.789669036865234,0.02305376193088568
8108,16217,16216,32433,4.846141815185547,0.022559992497924237
8208,16417,16416,32833,4.908447027206421,0.02207759737706084
8308,16617,16616,33233,4.984722852706909,0.02161238570044299
8408,16817,16816,33633,5.062398910522461,0.021164310044291958
8509,17019,17018,34037,5.142366886138916,0.020719969130055856
8609,17219,17218,34437,5.212211847305298,0.020289142488751587
8709,17419,17418,34837,5.279783010482788,0.019873623405900084
8809,17619,17618,35237,5.348188877105713,0.019475522501521056
8909,17819,17818,35637,5.415401935577393,0.019087241660711515
9009,18019,18018,36037,5.503641128540039,0.018709462863585432
9109,18219,18218,36437,5.573260068893433,0.01834242177141693
9209,18419,18418,36837,5.632857084274292,0.017986694060080653
9309,18619,18618,37237,5.694960832595825,0.017639570923587207
9409,18819,18818,37637,5.756062030792236,0.017304090160352722
9510,19021,19020,38041,5.8246400356292725,0.01697037256681031
9610,19221,19220,38441,5.888021945953369,0.016650869536836047
9710,19421,19420,38841,5.954566955566406,0.016338428904114157
9810,19621,19620,39241,6.032789945602417,0.016032065561002222
9910,19821,19820,39641,6.127771854400635,0.015736215804187048
10010,20021,20020,40041,6.189207077026367,0.015443306257313391
10110,20221,20220,40441,6.24676513671875,0.015159276298873113
10210,20421,20420,40841,6.303054094314575,0.014880353086775216
10310,20621,20620,41241,6.359117031097412,0.014610834315845698
10410,20821,20820,41641,6.417567014694214,0.01434706491684801
10511,21023,21022,42045,6.476357936859131,0.014085199618959468
10611,21223,21222,42445,6.544482946395874,0.013835652154810913
10711,21423,21422,42845,6.605547904968262,0.013589342281853576
10811,21623,21622,43245,6.6685590744018555,0.013354002367906608
10911,21823,21822,43645,6.734792947769165,0.013122741296041598
11011,22023,22022,44045,6.803910970687866,0.012897126910157219
11111,22223,22222,44445,6.863466024398804,0.01267746338992712
11211,22423,22422,44845,6.920316934585571,0.012460920442064519
11311,22623,22622,45245,6.983184099197388,0.012248712357741501
11411,22823,22822,45645,7.046810150146484,0.0120408501101333
11512,23025,23024,46049,7.1042139530181885,0.01183763020113523
11612,23225,23224,46449,7.1639931201934814,0.01164006612654538
11712,23425,23424,46849,7.2256200313568115,0.0114466669419765
11812,23625,23624,47249,7.294600963592529,0.011256805141840357
11912,23825,23824,47649,7.368479013442993,0.011068964054448644
12012,24025,24024,48049,7.446143865585327,0.010886822962676155
12112,24225,24224,48449,7.520823955535889,0.010708973654508593
12212,24425,24424,48849,7.58391809463501,0.010535118108427515
12312,24625,24624,49249,7.648624897003174,0.01036397438479419
12412,24825,24824,49649,7.719846963882446,0.010195631666659726
12513,25027,25026,50053,7.783802032470703,0.010030569936909036
12613,25227,25226,50453,7.8466479778289795,0.009871252990260712
12713,25427,25426,50853,7.9123311042785645,0.009711746042621023
12813,25627,25626,51253,7.975193977355957,0.009556048647357459
12913,25827,25826,51653,8.044059991836548,0.009403642583312196
13013,26027,26026,52053,8.1022047996521,0.00925358377989855
13113,26227,26226,52453,8.180286884307861,0.009106999391905887
13213,26427,26426,52853,8.257080078125,0.008961927882435695
13313,26627,26626,53253,8.322768926620483,0.008819693970361838
13413,26827,26826,53653,8.385426998138428,0.008681359896065092
13514,27029,27028,54057,8.449901103973389,0.008543950765493025
13614,27229,27228,54457,8.524857997894287,0.008409233988912568
13714,27429,27428,54857,8.595554113388062,0.008279902665875727
13814,27629,27628,55257,8.669323921203613,0.008152617209461761
13914,27829,27828,55657,8.750864028930664,0.008026512120131583
14014,28029,28028,56057,8.840687990188599,0.007903728658445882
14114,28229,28228,56457,8.916973114013672,0.007783622588777366
14214,28429,28428,56857,8.985424041748047,0.007665939539988106
14314,28629,28628,57257,9.051099061965942,0.0075494264729885005
14414,28829,28828,57657,9.114238977432251,0.00743439393415637
14515,29031,29030,58061,9.174548864364624,0.007320070375111831
14615,29231,29230,58461,9.250110864639282,0.007210816307447554
14715,29431,29430,58861,9.338696956634521,0.0071037168090751475
14815,29631,29630,59261,9.445648193359375,0.0069978140175911705
14915,29831,29830,59661,9.544960021972656,0.006893302443676335
15015,30031,30030,60061,9.64279294013977,0.006790653764443709
15115,30231,30230,60461,9.73103404045105,0.006690559735818359
15215,30431,30430,60861,9.828573942184448,0.0065917079510694355
15315,30631,30630,61261,9.921413898468018,0.006494426826239039
15415,30831,30830,61661,9.998661041259766,0.0063998511647646306
15516,31033,31032,62065,10.06583285331726,0.006305414231237228
15616,31233,31232,62465,10.129904985427856,0.006212675033630323
15716,31433,31432,62865,10.193603038787842,0.006121818345902143
15816,31633,31632,63265,10.257379055023193,0.006032477348766477
15916,31833,31832,63665,10.338679075241089,0.005944909152241164
16016,32033,32032,64065,10.41720199584961,0.005857863671652319
16116,32233,32232,64465,10.484701871871948,0.005771793092418668
16216,32433,32432,64865,10.547355890274048,0.005686836282398767
16316,32633,32632,65265,10.610591888427734,0.005603883184672335
16416,32833,32832,65665,10.674334049224854,0.005523094010000106
16517,33035,33034,66069,10.736692905426025,0.005441233723712932
16617,33235,33234,66469,10.80310606956482,0.005360929256303944
16717,33435,33434,66869,10.866544008255005,0.005282785119962842
16817,33635,33634,67269,10.933731079101562,0.005206396925919889
16917,33835,33834,67669,10.993803024291992,0.0051302409911087345
17017,34035,34034,68069,11.054204940795898,0.005055965898887682
17117,34235,34234,68469,11.114509105682373,0.004983635292561712
17217,34435,34434,68869,11.174429893493652,0.004911618144718041
17317,34635,34634,69269,11.23395299911499,0.0048421856219658796
17417,34835,34834,69669,11.292272090911865,0.004773995674033953
17518,35037,35036,70073,11.352333068847656,0.004705333144626182
17618,35237,35236,70473,11.41235613822937,0.004638693046376321
17718,35437,35436,70873,11.4688880443573,0.004573244929095878
17818,35637,35636,71273,11.525978088378906,0.004508469981765339
17918,35837,35836,71673,11.583799123764038,0.004445483827106951
18018,36037,36036,72073,11.640419960021973,0.00438394267520254
18118,36237,36236,72473,11.697082757949829,0.004322926095325923
18218,36437,36436,72873,11.753015041351318,0.0042627725542947305
18318,36637,36636,73273,11.809151887893677,0.004203371011086959
18418,36837,36836,73673,11.865689992904663,0.004144912239114603
18519,37039,37038,74077,11.923050880432129,0.0040871017415159425
18619,37239,37238,74477,11.980955123901367,0.004030763356925354
18719,37439,37438,74877,12.03951096534729,0.003975243272120712
18819,37639,37638,75277,12.096816778182983,0.00391979960089009
18919,37839,37838,75677,12.153985977172852,0.003865249257327049
19019,38039,38038,76077,12.209196090698242,0.003812422175678236
19119,38239,38238,76477,12.266581058502197,0.003759977232970467
19219,38439,38438,76877,12.330405950546265,0.0037071795738251047
19319,38639,38638,77277,12.39159083366394,0.003655243445506932
19419,38839,38838,77677,12.457733154296875,0.0036040650125742524
19520,39041,39040,78081,12.529053926467896,0.0035530551680510373
19620,39241,39240,78481,12.590693950653076,0.003503527828498237
19720,39441,39440,78881,12.646501779556274,0.003454955033293234
19820,39641,39640,79281,12.706362962722778,0.0034069870116554025
19920,39841,39840,79681,12.7659010887146,0.0033599647905396923
20020,40041,40040,80081,12.822373867034912,0.0033136982134211444
20120,40241,40240,80481,12.876863956451416,0.0032678620157086794
20220,40441,40440,80881,12.930071115493774,0.003223120084991087
20320,40641,40640,81281,12.989405870437622,0.0031790344510985186
20420,40841,40840,81681,13.04877495765686,0.0031354275182303225
20521,41043,41042,82085,13.11289095878601,0.0030922796795635156
20621,41243,41242,82485,13.177001953125,0.003050653756733758
20721,41443,41442,82885,13.24402403831482,0.0030097410406953982
20821,41643,41642,83285,13.30899715423584,0.0029690653918482655
20921,41843,41842,83685,13.372453212738037,0.002928941552300115
21021,42043,42042,84085,13.436490058898926,0.0028892309435148283
21121,42243,42242,84485,13.4984130859375,0.0028502035305651967
21221,42443,42442,84885,13.55840802192688,0.002812368444327073
21321,42643,42642,85285,13.617565870285034,0.0027753887202941023
21421,42843,42842,85685,13.677345037460327,0.0027383639017034803
21522,43045,43044,86089,13.737701892852783,0.002701066335187053
21622,43245,43244,86489,13.796871900558472,0.00266506837031242
21722,43445,43444,86889,13.852432012557983,0.002630204759457289
21822,43645,43644,87289,13.908066987991333,0.002595477065467895
21922,43845,43844,87689,13.96227502822876,0.0025606755089754452
22022,44045,44044,88089,14.017725944519043,0.0025261160067499896
22122,44245,44244,88489,14.072899103164673,0.0024921225384463733
22222,44445,44444,88889,14.126906871795654,0.0024588130892679687
22322,44645,44644,89289,14.182556867599487,0.002425832369400067
22422,44845,44844,89689,14.239289999008179,0.002393106439487853
22523,45047,45046,90093,14.294556856155396,0.0023605301690849414
22623,45247,45246,90493,14.35108995437622,0.0023288843176608766
22723,45447,45446,90893,14.413082122802734,0.0022972369973633788
22823,45647,45646,91293,14.480237007141113,0.002265961526679049
22923,45847,45846,91693,14.545683860778809,0.002235816087229212
23023,46047,46046,92093,14.616159915924072,0.0022060734692023747
23123,46247,46246,92493,14.684607982635498,0.0021762834304517465
23223,46447,46446,92893,14.740747928619385,0.0021468772759382663
23323,46647,46646,93293,14.800012111663818,0.0021182539411345163
23423,46847,46846,93693,14.857270002365112,0.0020901150321934697
23524,47049,47048,94097,14.915755987167358,0.00206207789073199
23624,47249,47248,94497,14.971490144729614,0.0020344391567394537
23724,47449,47448,94897,15.026384115219116,0.002006940904425779
23824,47649,47648,95297,15.08187484741211,0.0019803639994873975
23924,47849,47848,95697,15.137509822845459,0.0019546652026762577
24024,48049,48048,96097,15.194405794143677,0.0019290901174034071
24124,48249,48248,96497,15.251051902770996,0.001903528857177315
24224,48449,48448,96897,15.30784296989441,0.0018784219515933262
24324,48649,48648,97297,15.369674921035767,0.0018538691308578855
24424,48849,48848,97697,15.431391954421997,0.0018297957217538296
24525,49051,49050,98101,15.492722988128662,0.0018057761889676575
24625,49251,49250,98501,15.552910089492798,0.0017822167607118604
24725,49451,49450,98901,15.609447956085205,0.001758972691668677
24825,49651,49650,99301,15.663542032241821,0.0017359592620280221
24925,49851,49850,99701,15.719966888427734,0.0017132828288529494
25025,50051,50050,100101,15.774657964706421,0.0016909282912083354
25125,50251,50250,100501,15.829487085342407,0.0016688915753794746
25225,50451,50450,100901,15.883656024932861,0.001647304466976178
25325,50651,50650,101301,15.945784091949463,0.00162574981053356
25425,50851,50850,101701,16.009171962738037,0.0016041325357932313
25526,51053,51052,102105,16.06874108314514,0.0015829334740507929
25626,51253,51252,102505,16.12596607208252,0.001562492810147561
25726,51453,51452,102905,16.184367179870605,0.0015420038491380406
25826,51653,51652,103305,16.245408058166504,0.0015215474186297943
25926,51853,51852,103705,16.307536125183105,0.0015013343540489692
26026,52053,52052,104105,16.368361949920654,0.0014815744346237615
26126,52253,52252,104505,16.428653955459595,0.0014622147309564825
26226,52453,52452,104905,16.495178937911987,0.0014429248404153458
26326,52653,52652,105305,16.563716173171997,0.0014237214420007012
26426,52853,52852,105705,16.62933921813965,0.0014049123676458826
26527,53055,53054,106109,16.694168090820312,0.0013864561895997449
26627,53255,53254,106509,16.770139932632446,0.0013684126049319189
26727,53455,53454,106909,16.842320919036865,0.0013503584389416101
26827,53655,53654,107309,16.900689840316772,0.0013325648333129781
26927,53855,53854,107709,16.959105014801025,0.001315245020235094
27027,54055,54054,108109,17.016618013381958,0.0012981464405400504
27127,54255,54254,108509,17.07396411895752,0.0012812362433527523
27227,54455,54454,108909,17.131526947021484,0.0012646847846415278
27327,54655,54654,109309,17.191128969192505,0.001248413516773543
27427,54855,54854,109709,17.24991798400879,0.001232365332832007
27528,55057,55056,110113,17.31125807762146,0.0012163422628432249
27628,55257,55256,110513,17.37301206588745,0.0012007487414121831
27728,55457,55456,110913,17.434780836105347,0.0011856211157098915
27828,55657,55656,111313,17.49788999557495,0.0011707441759108525
27928,55857,55856,111713,17.566428899765015,0.001155830152379695
28028,56057,56056,112113,17.62775707244873,0.001140997998677747
28128,56257,56256,112513,17.689734935760498,0.0011264985706258485
28228,56457,56456,112913,17.75053381919861,0.0011124366296351694
28328,56657,56656,113313,17.836575031280518,0.0010984739176887336
28428,56857,56856,113713,17.899847984313965,0.0010843713433919646
28529,57059,57058,114117,17.959800004959106,0.001070209207251639
28629,57259,57258,114517,18.0197970867157,0.0010564074790777433
28729,57459,57458,114917,18.078557014465332,0.0010427852142414643
28829,57659,57658,115317,18.185598850250244,0.001029395984928758
28929,57859,57858,115717,18.259788036346436,0.0010161170668409893
29029,58059,58058,116117,18.317878007888794,0.0010028852735070662
29129,58259,58258,116517,18.375805854797363,0.0009898803582890777
29229,58459,58458,116917,18.43610119819641,0.0009770654043842024
29329,58659,58658,117317,18.49589991569519,0.0009644180681854901
29429,58859,58858,117717,18.553328037261963,0.0009519341434160016
29530,59061,59060,118121,18.61894392967224,0.0009394078877329043
29630,59261,59260,118521,18.679674863815308,0.0009271719139192254
29730,59461,59460,118921,18.757979154586792,0.0009151672911712378
29830,59661,59660,119321,18.82108497619629,0.0009033591387170011
29930,59861,59860,119721,18.90194606781006,0.0008917409664697023
30030,60061,60060,120121,18.973127841949463,0.0008802988455081966
30130,60261,60260,120521,19.031333923339844,0.0008689573566629654
30230,60461,60460,120921,19.089675903320312,0.0008577630739799271
30330,60661,60660,121321,19.147475957870483,0.0008468217024087507
30430,60861,60860,121721,19.204583883285522,0.000836213587043217
30531,61063,61062,122125,19.263252019882202,0.0008257063914645861
30631,61263,61262,122525,19.32655906677246,0.0008152790889900327
30731,61463,61462,122925,19.38561201095581,0.0008048872648082177
30831,61663,61662,123325,19.444437980651855,0.0007947666008145213
30931,61863,61862,123725,19.50159215927124,0.0007849734815241334
31031,62063,62062,124125,19.55939507484436,0.0007752914069039619
31131,62263,62262,124525,19.624118089675903,0.0007655604481768055
31231,62463,62462,124925,19.689514875411987,0.0007558522460640074
31331,62663,62662,125325,19.755456924438477,0.0007462777872553389
31431,62863,62862,125725,19.82245182991028,0.0007368841449350017
31532,63065,63064,126129,19.882932901382446,0.0007275646600866449
31632,63265,63264,126529,19.94701600074768,0.000718412068472922
31732,63465,63464,126929,20.005971908569336,0.0007092889757316277
31832,63665,63664,127329,20.06532597541809,0.0007002188384096632
31932,63865,63864,127729,20.123368978500366,0.0006912156096667298
32032,64065,64064,128129,20.182201147079468,0.0006823576365028392
32132,64265,64264,128529,20.25461983680725,0.000673656100169962
32232,64465,64464,128929,20.31817603111267,0.000665055300941808
32332,64665,64664,129329,20.377231121063232,0.0006565317276488504
32432,64865,64864,129729,20.43596601486206,0.0006480549560862117
32533,65067,65066,130133,20.496307849884033,0.0006396228151107925
32633,65267,65266,130533,20.55435585975647,0.0006314627450635855
32733,65467,65466,130933,20.613343954086304,0.0006233959751778609
32833,65667,65666,131333,20.67063593864441,0.0006153678410492319
32933,65867,65866,131733,20.73310112953186,0.0006073919539786686
33033,66067,66066,132133,20.793298959732056,0.0005995633916072135
33133,66267,66266,132533,20.85431694984436,0.000591997289100956
33233,66467,66466,132933,20.912963151931763,0.000584575855427674
33333,66667,66666,133333,20.98826789855957,0.0005771084756582733
33433,66867,66866,133733,21.058488130569458,0.0005696863929570546
33534,67069,67068,134137,21.124410152435303,0.0005624184792915367
33634,67269,67268,134537,21.182942867279053,0.0005554280076784693
33734,67469,67468,134937,21.242225885391235,0.0005485061715251781
33834,67669,67668,135337,21.30128502845764,0.0005416028141252545
33934,67869,67868,135737,21.35988187789917,0.0005347875483740765
34034,68069,68068,136137,21.41763997077942,0.0005280879963183113
34134,68269,68268,136537,21.480144023895264,0.0005214761486977644
34234,68469,68468,136937,21.540777921676636,0.0005149780357951228
34334,68669,68668,137337,21.599519968032837,0.0005085924872539106
34434,68869,68868,137737,21.673937797546387,0.000502283302734517
34535,69071,69070,138141,21.750813961029053,0.0004959370176206457
34635,69271,69270,138541,21.829829216003418,0.0004896480072764031
34735,69471,69470,138941,21.897983074188232,0.0004834708223313215
34835,69671,69670,139341,21.95793104171753,0.0004774844483334934
34935,69871,69870,139741,22.02361297607422,0.00047155902265240136
35035,70071,70070,140141,22.084518909454346,0.0004655961549946899
35135,70271,70270,140541,22.15023112297058,0.0004596667679794084
35235,70471,70470,140941,22.215925931930542,0.0004538614263627269
35335,70671,70670,141341,22.279546976089478,0.0004481761276762892
35435,70871,70870,141741,22.351382970809937,0.0004425184464727837
35536,71073,71072,142145,22.42578101158142,0.00043680176754632056
35636,71273,71272,142545,22.491870880126953,0.0004312203765765617
35736,71473,71472,142945,22.55123996734619,0.00042575428452023656
35836,71673,71672,143345,22.611583948135376,0.00042038476598061774
35936,71873,71872,143745,22.672756910324097,0.00041505590545173237
36036,72073,72072,144145,22.73304009437561,0.00040973613464931807
36136,72273,72272,144545,22.792383909225464,0.0004045053016307405
36236,72473,72472,144945,22.851099967956543,0.00039938870744720605
36336,72673,72672,145345,22.913501977920532,0.0003943161478983263
36436,72873,72872,145745,22.974884033203125,0.00038930292427483316
36537,73075,73074,146149,23.033108949661255,0.0003843384904795294
36637,73275,73274,146549,23.093466997146606,0.00037949383715535454
36737,73475,73474,146949,23.167191982269287,0.00037471805399694864
36837,73675,73674,147349,23.240005016326904,0.00037003549227508593
36937,73875,73874,147749,23.298479080200195,0.00036546155835562636
37037,74075,74074,148149,23.357487201690674,0.00036096921619585884
37137,74275,74274,148549,23.414644956588745,0.0003565014206840077
37237,74475,74474,148949,23.476386070251465,0.000352062057915611
37337,74675,74674,149349,23.53265690803528,0.0003477120342057831
37437,74875,74874,149749,23.589515924453735,0.00034348744847546874
37538,75077,75076,150153,23.653085947036743,0.0003393050059050072
37638,75277,75276,150553,23.714929819107056,0.0003351577637960295
37738,75477,75476,150953,23.7754909992218,0.0003309970271766664
37838,75677,75676,151353,23.8392550945282,0.000326900350872223
37938,75877,75876,151753,23.900689840316772,0.0003228846532448041
38038,76077,76076,152153,23.962080001831055,0.0003189160308931518
38138,76277,76276,152553,24.02362895011902,0.0003149758244353602
38238,76477,76476,152953,24.084390878677368,0.00031105373060227745
38338,76677,76676,153353,24.14223313331604,0.00030716800811117354
38438,76877,76876,153753,24.1994891166687,0.000303341062980693
38539,77079,77078,154157,24.262148141860962,0.00029952467808556975
38639,77279,77278,154557,24.32418394088745,0.000295770123073343
38739,77479,77478,154957,24.385011911392212,0.0002920403117529768
38839,77679,77678,155357,24.44435715675354,0.0002883565324695118
38939,77879,77878,155757,24.50125789642334,0.0002847147761708351
39039,78079,78078,156157,24.55760884284973,0.00028111084788081915
39139,78279,78278,156557,24.616069078445435,0.0002775582991780617
39239,78479,78478,156957,24.67562484741211,0.00027404218510427046
39339,78679,78678,157357,24.73312211036682,0.0002705538266859334
39439,78879,78878,157757,24.79091787338257,0.00026712591648868713
39540,79081,79080,158161,24.848469972610474,0.0002637482063303302
39640,79281,79280,158561,24.90454387664795,0.0002604784557069851
39740,79481,79480,158961,24.9617760181427,0.00025725518783974654
39840,79681,79680,159361,25.0186870098114,0.0002540514538603606
39940,79881,79880,159761,25.075504779815674,0.0002508852192821218
40040,80081,80080,160161,25.132127046585083,0.00024779788249145465
40140,80281,80280,160561,25.18770408630371,0.0002447909742628181
40240,80481,80480,160961,25.248164176940918,0.00024182806361832822
40340,80681,80680,161361,25.32140588760376,0.00023887223116086424
40440,80881,80880,161761,25.393603086471558,0.00023592433769801732
40541,81083,81082,162165,25.45724320411682,0.00023299001283526215
40641,81283,81282,162565,25.516025066375732,0.00023015205982570444
40741,81483,81482,162965,25.575045824050903,0.00022737815731754086
40841,81683,81682,163365,25.635541915893555,0.00022462806821962373
40941,81883,81882,163765,25.698019981384277,0.00022186189036798443
41041,82083,82082,164165,25.757588863372803,0.00021909822002065988
41141,82283,82282,164565,25.819732904434204,0.0002163819483350431
41241,82483,82482,164965,25.884191036224365,0.00021371975005363353
41341,82683,82682,165365,25.949743032455444,0.00021109100878277169
41441,82883,82882,165765,26.009356021881104,0.00020848231493860272
41542,83085,83084,166169,26.069872856140137,0.00020586057062015395
41642,83285,83284,166569,26.164395093917847,0.000203276428634973
41742,83485,83484,166969,26.243167877197266,0.00020071608930321316
41842,83685,83684,167369,26.301923990249634,0.00019819393778978066
41942,83885,83884,167769,26.360217094421387,0.00019570568988827228
42042,84085,84084,168169,26.42016887664795,0.00019323998709289668
42142,84285,84284,168569,26.47700309753418,0.0001907964104118274
42242,84485,84484,168969,26.537559032440186,0.00018838356809352383
42342,84685,84684,169369,26.597509145736694,0.00018602079675367187
42442,84885,84884,169769,26.655256032943726,0.0001837037199078083
42543,85087,85086,170173,26.713130950927734,0.0001813725643109436
42643,85287,85286,170573,26.77079486846924,0.0001790752341245966
42743,85487,85486,170973,26.83228898048401,0.0001768292416121034
42843,85687,85686,171373,26.893616914749146,0.00017464499844021015
42943,85887,85886,171773,26.95403790473938,0.0001724984090081392
43043,86087,86086,172173,27.021099090576172,0.00017036015715322754
43143,86287,86286,172573,27.081203937530518,0.0001682264437269874
43243,86487,86486,172973,27.143790006637573,0.00016612877051334118
43343,86687,86686,173373,27.20639419555664,0.0001640901907504747
43443,86887,86886,173773,27.2626690864563,0.00016209982549336856
43544,87089,87088,174177,27.327502965927124,0.00016010996865951747
43644,87289,87288,174577,27.39045286178589,0.00015814021033291694
43744,87489,87488,174977,27.46026110649109,0.00015617824455206657
43844,87689,87688,175377,27.526331901550293,0.00015424229798519386
43944,87889,87888,175777,27.583168983459473,0.00015234525595818335
44044,88089,88088,176177,27.639450073242188,0.00015049565825211848
44144,88289,88288,176577,27.697808980941772,0.00014867539777357647
44244,88489,88488,176977,27.754178047180176,0.00014685057794439226
44344,88689,88688,177377,27.81309199333191,0.0001450222279675677
44444,88889,88888,177777,27.882429838180542,0.0001432193365019815
44545,89091,89090,178181,27.957441091537476,0.00014144207418414795
44645,89291,89290,178581,28.016216039657593,0.00013971263705615558
44745,89491,89490,178981,28.07327103614807,0.00013798442866319154
44845,89691,89690,179381,28.13095712661743,0.00013625729341167262
44945,89891,89890,179781,28.187152862548828,0.0001345574945113164
45045,90091,90090,180181,28.244781970977783,0.00013289356624013315
45145,90291,90290,180581,28.30297017097473,0.00013124863589701358
45245,90491,90490,180981,28.362141847610474,0.00012960722090503565
45345,90691,90690,181381,28.4181911945343,0.0001279765553778598
45445,90891,90890,181781,28.475268125534058,0.00012637317921053898
45546,91093,91092,182185,28.53309202194214,0.00012478124938241402
45646,91293,91292,182585,28.58947515487671,0.0001232226103641434
45746,91493,91492,182985,28.645385026931763,0.0001216789573696633
45846,91693,91692,183385,28.701069116592407,0.00012015315637023151
45946,91893,91892,183785,28.757527112960815,0.00011865199055657371
46046,92093,92092,184185,28.81669592857361,0.00011718150186085775
46146,92293,92292,184585,28.87310791015625,0.00011573985523195458
46246,92493,92492,184985,28.930819988250732,0.00011431914546291289
46346,92693,92692,185385,28.991714000701904,0.00011291029269743087
46446,92893,92892,185785,29.045536041259766,0.00011151509618881839
46547,93095,93094,186189,29.10007095336914,0.00011013293195193942
46647,93295,93294,186589,29.155529022216797,0.00010879776392846443
46747,93495,93494,186989,29.211116075515747,0.00010748995831141965
46847,93695,93694,187389,29.267162084579468,0.00010619429652382873
46947,93895,93894,187789,29.3270001411438,0.00010490064689802641
47047,94095,94094,188189,29.383702993392944,0.0001036202161873568
47147,94295,94294,188589,29.441559076309204,0.00010236838243776943
47247,94495,94494,188989,29.499955892562866,0.00010114275966565546
47347,94695,94694,189389,29.573400020599365,9.993016057126198e-05
47447,94895,94894,189789,29.641712188720703,9.872110501904615e-05
47548,95097,95096,190193,29.70058012008667,9.75059895762616e-05
47648,95297,95296,190593,29.755668878555298,9.631948607871723e-05
47748,95497,95496,190993,29.813584089279175,9.515161555636806e-05
47848,95697,95696,191393,29.87356686592102,9.399530073302256e-05
47948,95897,95896,191793,29.931760787963867,9.28471926355752e-05
48048,96097,96096,192193,29.985819816589355,9.170756160305401e-05
48148,96297,96296,192593,30.039971113204956,9.057703727985186e-05
48248,96497,96496,192993,30.096269130706787,8.945683711013203e-05
48348,96697,96696,193393,30.150660037994385,8.834664826830426e-05
48448,96897,96896,193793,30.20555281639099,8.724529971294314e-05
48549,97099,97098,194197,30.26754403114319,8.614377724831555e-05
48649,97299,97298,194597,30.324755907058716,8.506922825433246e-05
48749,97499,97498,194997,30.381598949432373,8.401407780519597e-05
48849,97699,97698,195397,30.438168048858643,8.297560476609393e-05
48949,97899,97898,195797,30.494565963745117,8.194880047050278e-05
49049,98099,98098,196197,30.55080795288086,8.093404397391337e-05
49149,98299,98298,196597,30.60677695274353,7.993719206597883e-05
49249,98499,98498,196997,30.665284156799316,7.896040056880056e-05
49349,98699,98698,197397,30.72007393836975,7.799917656674808e-05
49449,98899,98898,197797,30.777384996414185,7.704973967353492e-05
49550,99101,99100,198201,30.831660985946655,7.610103818764431e-05
49650,99301,99300,198601,30.88604497909546,7.517184384615252e-05
49750,99501,99500,199001,30.941736936569214,7.425796140602551e-05
49850,99701,99700,199401,30.997534036636353,7.336513538575964e-05
49950,99901,99900,199801,31.051828861236572,7.249215031877041e-05
50050,100101,100100,200201,31.10466194152832,7.162912904509873e-05
50150,100301,100300,200601,31.16011118888855,7.076374828155986e-05
50250,100501,100500,201001,31.21823215484619,6.989779254409602e-05
50350,100701,100700,201401,31.279018878936768,6.904789460229943e-05
50450,100901,100900,201801,31.341397047042847,6.822109192835934e-05
50551,101103,101102,202205,31.404046058654785,6.739825052923212e-05
50651,101303,101302,202605,31.460876941680908,6.658374608708562e-05
50751,101503,101502,203005,31.518566846847534,6.5769342162764e-05
50851,101703,101702,203405,31.583723068237305,6.496287089872317e-05
50951,101903,101902,203805,31.648922204971313,6.416833091828788e-05
51051,102103,102102,204205,31.726086854934692,6.338345579829246e-05
51151,102303,102302,204605,31.7989718914032,6.260605350774292e-05
51251,102503,102502,205005,31.861091136932373,6.183457044517785e-05
51351,102703,102702,205405,31.92189311981201,6.106720440061781e-05
51451,102903,102902,205805,31.977428913116455,6.03044512704491e-05
51552,103105,103104,206209,32.0339560508728,5.9543515796248956e-05
51652,103305,103304,206609,32.0915892124176,5.88052090248075e-05
51752,103505,103504,207009,32.14947986602783,5.807945163953757e-05
51852,103705,103704,207409,32.20608305931091,5.735804563044207e-05
51952,103905,103904,207809,32.26321887969971,5.6642141078523705e-05
52052,104105,104104,208209,32.318832874298096,5.594056268989919e-05
52152,104305,104304,208609,32.37707281112671,5.5253799854957306e-05
52252,104505,104504,209009,32.4332070350647,5.4573053162603945e-05
52352,104705,104704,209409,32.489898920059204,5.38941665184917e-05
52452,104905,104904,209809,32.54667806625366,5.322499244773153e-05
52553,105107,105106,210213,32.60425806045532,5.256861249834601e-05
52653,105307,105306,210613,32.65957713127136,5.1935010621913895e-05
52753,105507,105506,211013,32.71627497673035,5.130504389247485e-05
52853,105707,105706,211413,32.77573299407959,5.067170372996229e-05
52953,105907,105906,211813,32.83437395095825,5.004264910824949e-05
53053,106107,106106,212213,32.889896869659424,4.943097693078666e-05
53153,106307,106306,212613,32.9466450214386,4.8838420422606406e-05
53253,106507,106506,213013,33.004218101501465,4.825600154277218e-05
53353,106707,106706,213413,33.063244104385376,4.7675519375717334e-05
53453,106907,106906,213813,33.120627880096436,4.709396250384261e-05
53554,107109,107108,214217,33.176679849624634,4.65088751547906e-05
53654,107309,107308,214617,33.23550009727478,4.593947365555237e-05
53754,107509,107508,215017,33.29430079460144,4.538427313598944e-05
53854,107709,107708,215417,33.35377097129822,4.4839924568434876e-05
53954,107909,107908,215817,33.41346096992493,4.429786408307091e-05
54054,108109,108108,216217,33.47206711769104,4.3752986327879746e-05
54154,108309,108308,216617,33.52920389175415,4.3210486002077905e-05
54254,108509,108508,217017,33.58775496482849,4.267955958200301e-05
54354,108709,108708,217417,33.645511865615845,4.2161652558707596e-05
54454,108909,108908,217817,33.70328092575073,4.164867775421944e-05
54555,109111,109110,218221,33.76313495635986,4.112885835827202e-05
54655,109311,109310,218621,33.832813024520874,4.0617115059512164e-05
54755,109511,109510,219021,33.90419888496399,4.011556600117012e-05
54855,109711,109710,219421,33.96665382385254,3.962175682848879e-05
54955,109911,109910,219821,34.028241872787476,3.912986292665664e-05
55055,110111,110110,220221,34.08597183227539,3.8641230415958725e-05
55155,110311,110310,220621,34.14530611038208,3.8161329532574645e-05
55255,110511,110510,221021,34.20331907272339,3.7692351736237234e-05
55355,110711,110710,221421,34.260704040527344,3.7231349641486495e-05
55455,110911,110910,221821,34.32121181488037,3.6774056160339804e-05
55556,111113,111112,222225,34.383376121520996,3.631561794124037e-05
55656,111313,111312,222625,34.44138288497925,3.586853618338635e-05
55756,111513,111512,223025,34.5012788772583,3.543063896381011e-05
55856,111713,111712,223425,34.55884385108948,3.5001678275984944e-05
55956,111913,111912,223825,34.622671127319336,3.458036953387617e-05
56056,112113,112112,224225,34.68872022628784,3.4163923529434016e-05
56156,112313,112312,224625,34.75506615638733,3.3749151866548185e-05
56256,112513,112512,225025,34.820693016052246,3.333767616873116e-05
56356,112713,112712,225425,34.88981819152832,3.2935047409620035e-05
56456,112913,112912,225825,34.94925498962402,3.254313896618875e-05
56557,113115,113114,226229,35.00871801376343,3.2154292626006215e-05
56657,113315,113314,226629,35.067848920822144,3.177133310919726e-05
56757,113515,113514,227029,35.128411054611206,3.138908123423236e-05
56857,113715,113714,227429,35.19170618057251,3.101070281404708e-05
56957,113915,113914,227829,35.25103688240051,3.063970639219593e-05
57057,114115,114114,228229,35.31182098388672,3.0275373577068552e-05
57157,114315,114314,228629,35.38250803947449,2.991388537029835e-05
57257,114515,114514,229029,35.44860601425171,2.955302671387017e-05
57357,114715,114714,229429,35.5103440284729,2.9194265670138282e-05
57457,114915,114914,229829,35.56964612007141,2.883980869161243e-05
57558,115117,115116,230233,35.63014602661133,2.8486187328171287e-05
57658,115317,115316,230633,35.689621925354004,2.813926683908595e-05
57758,115517,115516,231033,35.748201847076416,2.779495508601753e-05
57858,115717,115716,231433,35.80846905708313,2.745369249468967e-05
57958,115917,115916,231833,35.873023986816406,2.7116351653188816e-05
58058,116117,116116,232233,35.94576096534729,2.678291896668392e-05
58158,116317,116316,232633,36.029350996017456,2.645333939183334e-05
58258,116517,116516,233033,36.09479904174805,2.612901913459722e-05
58358,116717,116716,233433,36.157835960388184,2.58107745199425e-05
58458,116917,116916,233833,36.21775197982788,2.5497007013748194e-05
58559,117119,117118,234237,36.27802491188049,2.5183129971058986e-05
58659,117319,117318,234637,36.336517095565796,2.4876044596642697e-05
58759,117519,117518,235037,36.4106879234314,2.457347765599679e-05
58859,117719,117718,235437,36.47808790206909,2.4274853671780186e-05
58959,117919,117918,235837,36.55821108818054,2.398003763226692e-05
59059,118119,118118,236237,36.62785291671753,2.369053102535686e-05
59159,118319,118318,236637,36.68765687942505,2.3407479214200692e-05
59259,118519,118518,237037,36.746947050094604,2.3129425461007423e-05
59359,118719,118718,237437,36.808470010757446,2.2853056793730952e-05
59459,118919,118918,237837,36.86618113517761,2.257753619579934e-05
59560,119121,119120,238241,36.923264026641846,2.230378247370312e-05
59660,119321,119320,238641,36.9802188873291,2.203996402099865e-05
59760,119521,119520,239041,37.04773497581482,2.1780738696627824e-05
59860,119721,119720,239441,37.12630081176758,2.1521899919741736e-05
59960,119921,119920,239841,37.1899049282074,2.1262925510155518e-05
60060,120121,120120,240241,37.24769902229309,2.100657189920181e-05
60160,120321,120320,240641,37.30599904060364,2.0754818000468815e-05
60260,120521,120520,241041,37.36414694786072,2.0506905544200124e-05
60360,120721,120720,241441,37.42199492454529,2.0260907500736043e-05
60460,120921,120920,241841,37.47836494445801,2.0015703200571263e-05
60561,121123,121122,242245,37.535022020339966,1.9769142415078984e-05
60661,121323,121322,242645,37.59245014190674,1.95271560438472e-05
60761,121523,121522,243045,37.64995980262756,1.9288216974140812e-05
60861,121723,121722,243445,37.70765686035156,1.9053059032174804e-05
60961,121923,121922,243845,37.76319098472595,1.8821337750601712e-05
61061,122123,122122,244245,37.82112002372742,1.859094706708093e-05
61161,122323,122322,244645,37.87753176689148,1.8360908210656085e-05
61261,122523,122522,245045,37.936439037323,1.813353036416554e-05
61361,122723,122722,245445,37.993499994277954,1.7911140701155434e-05
61461,122923,122922,245845,38.048762798309326,1.7692781977111633e-05
61562,123125,123124,246249,38.11831712722778,1.747383818606132e-05
61662,123325,123324,246649,38.194157123565674,1.7258481408639023e-05
61762,123525,123524,247049,38.2535080909729,1.704703743092231e-05
61862,123725,123724,247449,38.314889907836914,1.684069277206451e-05
61962,123925,123924,247849,38.37279796600342,1.6636866760599375e-05
62062,124125,124124,248249,38.42946791648865,1.6432933169106245e-05
62162,124325,124324,248649,38.486958026885986,1.6230787858329705e-05
62262,124525,124524,249049,38.5439190864563,1.6034483921626006e-05
62362,124725,124724,249449,38.60022592544556,1.5844054850809136e-05
62462,124925,124924,249849,38.65756797790527,1.5655322456021593e-05
62563,125127,125126,250253,38.7193877696991,1.5463800228088604e-05
62663,125327,125326,250653,38.77476716041565,1.527490295176856e-05
62763,125527,125526,251053,38.83280301094055,1.5089518052572588e-05
62863,125727,125726,251453,38.88856387138367,1.490874251698392e-05
62963,125927,125926,251853,38.944035053253174,1.4731912971443898e-05
63063,126127,126126,252253,39.00144100189209,1.4557331629105517e-05
63163,126327,126326,252653,39.05631685256958,1.4382971086898616e-05
63263,126527,126526,253053,39.11260008811951,1.4207992781036855e-05
63363,126727,126726,253453,39.16908001899719,1.4034193211534196e-05
63463,126927,126926,253853,39.22593092918396,1.3864633190085699e-05
63564,127129,127128,254257,39.28409504890442,1.3698226329689802e-05
63664,127329,127328,254657,39.34245991706848,1.3535004997494248e-05
63764,127529,127528,255057,39.401139974594116,1.337016634326633e-05
63864,127729,127728,255457,39.46233081817627,1.3204777443682471e-05
63964,127929,127928,255857,39.519351959228516,1.3042338690329268e-05
64064,128129,128128,256257,39.57603311538696,1.2883874802985627e-05
64164,128329,128328,256657,39.63296580314636,1.2727393250809385e-05
64264,128529,128528,257057,39.69308590888977,1.2571467360142818e-05
64364,128729,128728,257457,39.74922490119934,1.2416855998330114e-05
64464,128929,128928,257857,39.805294036865234,1.226474162350922e-05
64565,129131,129130,258261,39.86303091049194,1.2113403151036171e-05
64665,129331,129330,258661,39.91895604133606,1.196468836691997e-05
64765,129531,129530,259061,39.97746992111206,1.181703522784001e-05
64865,129731,129730,259461,40.03536510467529,1.1671817670465344e-05
64965,129931,129930,259861,40.09169793128967,1.1529884131356623e-05
65065,130131,130130,260261,40.145890951156616,1.1390525546333348e-05
65165,130331,130330,260661,40.200434923172,1.1252672981294376e-05
65265,130531,130530,261061,40.27051281929016,1.1115931871594509e-05
65365,130731,130730,261461,40.339536905288696,1.0980426805545521e-05
65465,130931,130930,261861,40.39665985107422,1.084674026435279e-05
65566,131133,131132,262265,40.4542510509491,1.0714629587763982e-05
65666,131333,131332,262665,40.51187515258789,1.0587298622667517e-05
65766,131533,131532,263065,40.56867980957031,1.0462491711023173e-05
65866,131733,131732,263465,40.62665390968323,1.0338359466017731e-05
65966,131933,131932,263865,40.68463683128357,1.0214164794199344e-05
66066,132133,132132,264265,40.742563009262085,1.0091304726756888e-05
66166,132333,132332,264665,40.81301188468933,9.971637656672554e-06
66266,132533,132532,265065,40.891687870025635,9.855010388847102e-06
66366,132733,132732,265465,40.97929000854492,9.739335207116926e-06
66466,132933,132932,265865,41.0387818813324,9.62316683784727e-06
66567,133135,133134,266269,41.09726309776306,9.50610647254751e-06
66667,133335,133334,266669,41.15543508529663,9.392095066044943e-06
66767,133535,133534,267069,41.21656918525696,9.280424253491105e-06
66867,133735,133734,267469,41.275416135787964,9.170239306057968e-06
66967,133935,133934,267869,41.338168144226074,9.060523613700948e-06
67067,134135,134134,268269,41.40409183502197,8.950957972531323e-06
67167,134335,134334,268669,41.47491717338562,8.841936371605017e-06
67267,134535,134534,269069,41.53999590873718,8.734071405446393e-06
67367,134735,134734,269469,41.595649003982544,8.627825823699079e-06
67467,134935,134934,269869,41.65282893180847,8.523341225358271e-06
67568,135137,135136,270273,41.7100830078125,8.419241955921861e-06
67668,135337,135336,270673,41.767356872558594,8.317036260076293e-06
67768,135537,135536,271073,41.82347011566162,8.215638493292519e-06
67868,135737,135736,271473,41.878671169281006,8.115523509994341e-06
67968,135937,135936,271873,41.93357491493225,8.016963483756674e-06
68068,136137,136136,272273,41.990293979644775,7.919697759081764e-06
68168,136337,136336,272673,42.04576897621155,7.823480169844544e-06
68268,136537,136536,273073,42.101075887680054,7.728619256198935e-06
68368,136737,136736,273473,42.1570041179657,7.635601207358444e-06
68468,136937,136936,273873,42.21132278442383,7.54430973431086e-06
68569,137139,137138,274277,42.26684808731079,7.453148381780344e-06
68669,137339,137338,274677,42.32094597816467,7.3635964668142864e-06
68769,137539,137538,275077,42.389569997787476,7.27542146253942e-06
68869,137739,137738,275477,42.45802593231201,7.189484388474654e-06
68969,137939,137938,275877,42.517159938812256,7.1055288487371216e-06
69069,138139,138138,276277,42.57176399230957,7.022312705499155e-06
69169,138339,138338,276677,42.62604117393494,6.939098886723639e-06
69269,138539,138538,277077,42.67967200279236,6.856455544096988e-06
69369,138739,138738,277477,42.735495805740356,6.775378889890081e-06
69469,138939,138938,277877,42.79190993309021,6.695987965602475e-06
69570,139141,139140,278281,42.84895205497742,6.616655930332594e-06
69670,139341,139340,278681,42.90510702133179,6.538226471548594e-06
69770,139541,139540,279081,42.959882974624634,6.460030861001193e-06
69870,139741,139740,279481,43.01756691932678,6.382613441749748e-06
69970,139941,139940,279881,43.07386493682861,6.306259823450284e-06
70070,140141,140140,280281,43.13016486167908,6.230892851423573e-06
70170,140341,140340,280681,43.18636393547058,6.156249624909426e-06
70270,140541,140540,281081,43.24262499809265,6.081959454547285e-06
70370,140741,140740,281481,43.30242609977722,6.007875543194663e-06
70470,140941,140940,281881,43.35768008232117,5.934462161537935e-06
70571,141143,141142,282285,43.41320180892944,5.861652838489431e-06
70671,141343,141342,282685,43.47144913673401,5.790838125308727e-06
70771,141543,141542,283085,43.52771306037903,5.720581615096783e-06
70871,141743,141742,283485,43.58302593231201,5.650543197181403e-06
70971,141943,141942,283885,43.640198945999146,5.581282776119708e-06
71071,142143,142142,284285,43.69596481323242,5.513459814412596e-06
71171,142343,142342,284685,43.75305104255676,5.44685617676832e-06
71271,142543,142542,285085,43.808547019958496,5.380767811599903e-06
71371,142743,142742,285485,43.86606216430664,5.3151780693665394e-06
71471,142943,142942,285885,43.924400091171265,5.250825918860528e-06
71572,143145,143144,286289,43.98071908950806,5.1874131901174406e-06
71672,143345,143344,286689,44.03733205795288,5.125518230870441e-06
71772,143545,143544,287089,44.09349799156189,5.0637814364658e-06
71872,143745,143744,287489,44.1505331993103,5.0024513766612885e-06
71972,143945,143944,287889,44.20655417442322,4.94236750504133e-06
72072,144145,144144,288289,44.26260185241699,4.883853912679247e-06
72172,144345,144344,288689,44.31959080696106,4.826416012203579e-06
72272,144545,144544,289089,44.376242876052856,4.769375478264605e-06
72372,144745,144744,289489,44.4318368434906,4.712488852995498e-06
72472,144945,144944,289889,44.49554896354675,4.656024305780815e-06
72573,145147,145146,290293,44.5655779838562,4.599931985925764e-06
72673,145347,145346,290693,44.62777805328369,4.545656886890169e-06
72773,145547,145546,291093,44.68605589866638,4.492411346688132e-06
72873,145747,145746,291493,44.74427890777588,4.439407275639548e-06
72973,145947,145946,291893,44.803394079208374,4.386006831905729e-06
73073,146147,146146,292293,44.85916805267334,4.332545884219682e-06
73173,146347,146346,292693,44.915178060531616,4.280074221116293e-06
73273,146547,146546,293093,44.97339606285095,4.229084003681615e-06
73373,146747,146746,293493,45.030192136764526,4.17890006971674e-06
73473,146947,146946,293893,45.08670496940613,4.1286033338218005e-06
73574,147149,147148,294297,45.1425199508667,4.077661664965336e-06
73674,147349,147348,294697,45.19752502441406,4.02779468290231e-06
73774,147549,147548,295097,45.25349712371826,3.978923750967165e-06
73874,147749,147748,295497,45.310160875320435,3.930799654075014e-06
73974,147949,147948,295897,45.36684584617615,3.88304790887971e-06
74074,148149,148148,296297,45.4257447719574,3.835693206481368e-06
74174,148349,148348,296697,45.481691122055054,3.788979237704592e-06
74274,148549,148548,297097,45.53824305534363,3.7429383792721963e-06
74374,148749,148748,297497,45.59435701370239,3.6973933638966984e-06
74474,148949,148948,297897,45.6505970954895,3.6522737645715735e-06
74575,149151,149150,298301,45.70987606048584,3.607274416361103e-06
74675,149351,149350,298701,45.76693081855774,3.563482168429292e-06
74775,149551,149550,299101,45.82470917701721,3.5205864102551228e-06
74875,149751,149750,299501,45.88205695152283,3.4785840333324177e-06
74975,149951,149950,299901,45.940165758132935,3.437232033917708e-06
75075,150151,150150,300301,45.99926996231079,3.396183273743073e-06
75175,150351,150350,300701,46.0587899684906,3.3553860780812256e-06
75275,150551,150550,301101,46.11621809005737,3.3152474957659398e-06
75375,150751,150750,301501,46.1750111579895,3.27619188733722e-06
75475,150951,150950,301901,46.232362031936646,3.2380646459740446e-06
75576,151153,151152,302305,46.292336225509644,3.199811534489327e-06
75676,151353,151352,302705,46.35120987892151,3.1617547769410877e-06
75776,151553,151552,303105,46.41008901596069,3.123862331596677e-06
75876,151753,151752,303505,46.474480867385864,3.0868381291892873e-06
75976,151953,151952,303905,46.535008907318115,3.050891933502293e-06
76076,152153,152152,304305,46.595513105392456,3.015519454078934e-06
76176,152353,152352,304705,46.66762018203735,2.980087313997555e-06
76276,152553,152552,305105,46.739147901535034,2.9444371836527494e-06
76376,152753,152752,305505,46.796468019485474,2.9089164427503043e-06
76476,152953,152952,305905,46.853739976882935,2.873964365160425e-06
76577,153155,153154,306309,46.91430187225342,2.839374636206642e-06
76677,153355,153354,306709,46.972999811172485,2.8056021503826897e-06
76777,153555,153554,307109,47.03123879432678,2.7719913898512007e-06
76877,153755,153754,307509,47.08911204338074,2.7384654014684527e-06
76977,153955,153954,307909,47.14860486984253,2.7052216726317153e-06
77077,154155,154154,308309,47.20912504196167,2.6724856093026847e-06
77177,154355,154354,308709,47.26658892631531,2.640266871948551e-06
77277,154555,154554,309109,47.326213121414185,2.6083904100481276e-06
77377,154755,154754,309509,47.38679099082947,2.5767476251300735e-06
77477,154955,154954,309909,47.44647288322449,2.5454416752342155e-06
77578,155157,155156,310313,47.50515294075012,2.514332615142905e-06
77678,155357,155356,310713,47.56483292579651,2.484043679463038e-06
77778,155557,155556,311113,47.62333583831787,2.454131113219411e-06
77878,155757,155756,311513,47.680959939956665,2.424531709374477e-06
77978,155957,155956,311913,47.741377115249634,2.39538126672463e-06
78078,156157,156156,312313,47.80099105834961,2.3668899806164365e-06
78178,156357,156356,312713,47.859477043151855,2.3390592183608774e-06
78278,156557,156556,313113,47.917937994003296,2.311600961737528e-06
78378,156757,156756,313513,47.977883100509644,2.284248279986976e-06
78478,156957,156956,313913,48.03696298599243,2.257089860950576e-06
78579,157159,157158,314317,48.09598207473755,2.2301987948627292e-06
78679,157359,157358,314717,48.15446591377258,2.204255759855994e-06
78779,157559,157558,315117,48.2147159576416,2.1787470364288214e-06
78879,157759,157758,315517,48.27278804779053,2.1533181734215166e-06
78979,157959,157958,315917,48.33109188079834,2.1278972232336987e-06
79079,158159,158158,316317,48.38876795768738,2.1027236570610617e-06
79179,158359,158358,316717,48.449328899383545,2.0780145237559054e-06
79279,158559,158558,317117,48.50731587409973,2.0537082068619643e-06
79379,158759,158758,317517,48.565123081207275,2.029572080373028e-06
79479,158959,158958,317917,48.622811794281006,2.005466593302359e-06
79580,159161,159160,318321,48.682340145111084,1.9812061757979417e-06
79680,159361,159360,318721,48.74190306663513,1.957436420804103e-06
79780,159561,159560,319121,48.81387495994568,1.9340506022440755e-06
79880,159761,159760,319521,48.88178205490112,1.9110343604610897e-06
79980,159961,159960,319921,48.93891000747681,1.8882278700788334e-06
80080,160161,160160,320321,48.99518799781799,1.8654956029839672e-06
80180,160361,160360,320721,49.055476903915405,1.84288459661759e-06
80280,160561,160560,321121,49.114808082580566,1.8205615113476113e-06
80380,160761,160760,321521,49.171207904815674,1.7985967443388238e-06
80480,160961,160960,321921,49.22890901565552,1.7768822480899738e-06
80581,161163,161162,322325,49.286808013916016,1.7550968820435613e-06
80681,161363,161362,322725,49.34321308135986,1.7337630722222715e-06
80781,161563,161562,323125,49.40301012992859,1.7128444775480456e-06
80881,161763,161762,323525,49.467808961868286,1.69233877985594e-06
80981,161963,161962,323925,49.52469205856323,1.6720580518476242e-06
81081,162163,162162,324325,49.58422088623047,1.6519175810706472e-06
81181,162363,162362,324725,49.64551591873169,1.6320669099062695e-06
81281,162563,162562,325125,49.70415210723877,1.6126683350884614e-06
81381,162763,162762,325525,49.77119588851929,1.5936662567809742e-06
81481,162963,162962,325925,49.83410692214966,1.5748616763579407e-06
81582,163165,163164,326329,49.897356033325195,1.5559683386047738e-06
81682,163365,163364,326729,49.95923089981079,1.5374564417569558e-06
81782,163565,163564,327129,50.02065110206604,1.519293092644214e-06
81882,163765,163764,327529,50.08230710029602,1.50151075505598e-06
81982,163965,163964,327929,50.14322304725647,1.4839881080529522e-06
82082,164165,164164,328329,50.20658302307129,1.4665680444731932e-06
82182,164365,164364,328729,50.267874002456665,1.4491922368872726e-06
82282,164565,164564,329129,50.32859802246094,1.4319541090504765e-06
82382,164765,164764,329529,50.385550022125244,1.4150245506421163e-06
82482,164965,164964,329929,50.44566202163696,1.398469566077759e-06
82583,165167,165166,330333,50.50911211967468,1.3819754764775833e-06
82683,165367,165366,330733,50.56925392150879,1.3656398166042768e-06
82783,165567,165566,331133,50.63046193122864,1.3492558431596208e-06
82883,165767,165766,331533,50.68891215324402,1.333012304645386e-06
82983,165967,165966,331933,50.74998998641968,1.3170952876362194e-06
83083,166167,166166,332333,50.808692932128906,1.3014693974912791e-06
83183,166367,166366,332733,50.86673617362976,1.285946154819672e-06
83283,166567,166566,333133,50.94594407081604,1.2704370756107218e-06
83383,166767,166766,333533,51.03136897087097,1.2550541174487275e-06
83483,166967,166966,333933,51.08991098403931,1.2399378091000795e-06
83584,167169,167168,334337,51.14828014373779,1.2249248579436813e-06
83684,167369,167368,334737,51.20559906959534,1.210193380828141e-06
83784,167569,167568,335137,51.26391100883484,1.1955466545686345e-06
83884,167769,167768,335537,51.32126498222351,1.1810477825428527e-06
83984,167969,167968,335937,51.38298487663269,1.1667702203684663e-06
84084,168169,168168,336337,51.4657940864563,1.1527200880534965e-06
84184,168369,168368,336737,51.53338289260864,1.1388506085924966e-06
84284,168569,168568,337137,51.59806680679321,1.125128099406927e-06
84384,168769,168768,337537,51.65502214431763,1.1115867961346459e-06
84484,168969,168968,337937,51.713643074035645,1.0983170826698765e-06
84585,169171,169170,338341,51.77281618118286,1.0852439558232223e-06
84685,169371,169370,338741,51.83971881866455,1.072548792244412e-06
84785,169571,169570,339141,51.899137020111084,1.059936933322973e-06
84885,169771,169770,339541,51.95536994934082,1.047330660994618e-06
84985,169971,169970,339941,52.01953601837158,1.0348436064616e-06
85085,170171,170170,340341,52.07485103607178,1.0226645380021594e-06
85185,170371,170370,340741,52.13043403625488,1.010832983269347e-06
85285,170571,170570,341141,52.20146989822388,9.99178229461375e-07
85385,170771,170770,341541,52.26221585273743,9.875010076943707e-07
85485,170971,170970,341941,52.31873416900635,9.757801452259015e-07
85586,171173,171172,342345,52.376686096191406,9.640626074038956e-07
85686,171373,171372,342745,52.43189811706543,9.527427857566978e-07
85786,171573,171572,343145,52.48674702644348,9.416911920594927e-07
85886,171773,171772,343545,52.54271411895752,9.307391423669506e-07
85986,171973,171972,343945,52.59853792190552,9.197445803809259e-07
86086,172173,172172,344345,52.65353298187256,9.087329804441159e-07
86186,172373,172372,344745,52.708779096603394,8.978422577979304e-07
86286,172573,172572,345145,52.763787031173706,8.871564333162901e-07
86386,172773,172772,345545,52.82499980926514,8.766308807481549e-07
86486,172973,172972,345945,52.88568711280823,8.661736296787638e-07
86587,173175,173174,346349,52.94337511062622,8.556525158306274e-07
86687,173375,173374,346749,52.999096155166626,8.45321449677144e-07
86787,173575,173574,347149,53.06352400779724,8.351200297068377e-07
86887,173775,173774,347549,53.15099501609802,8.250424542315373e-07
86987,173975,173974,347949,53.223780155181885,8.150602593278484e-07
87087,174175,174174,348349,53.28210210800171,8.051750218774361e-07
87187,174375,174374,348749,53.33717608451843,7.954323645021531e-07
87287,174575,174574,349149,53.394065856933594,7.858838602241302e-07
87387,174775,174774,349549,53.450072050094604,7.765301579008759e-07
87487,174975,174974,349949,53.50781321525574,7.673062606232353e-07
87588,175177,175176,350353,53.56339502334595,7.580544056193875e-07
87688,175377,175376,350753,53.619112968444824,7.489751482107979e-07
87788,175577,175576,351153,53.673758029937744,7.400693693352457e-07
87888,175777,175776,351553,53.73484206199646,7.31391980703694e-07
87988,175977,175976,351953,53.804786920547485,7.228777660174844e-07
88088,176177,176176,352353,53.85926699638367,7.144046670104168e-07
88188,176377,176376,352753,53.91450381278992,7.059364633497453e-07
88288,176577,176576,353153,53.96984505653381,6.975692796330037e-07
88388,176777,176776,353553,54.024659872055054,6.89416427342105e-07
88488,176977,176976,353953,54.080551862716675,6.814691083508181e-07
88589,177179,177178,354357,54.13791584968567,6.735275193521018e-07
88689,177379,177378,354757,54.19391417503357,6.656533138892045e-07
88789,177579,177578,355157,54.24929618835449,6.577873098848816e-07
88889,177779,177778,355557,54.30608105659485,6.500120907498784e-07
88989,177979,177978,355957,54.36630082130432,6.423747085292166e-07
89089,178179,178178,356357,54.422404050827026,6.348526156295191e-07
89189,178379,178378,356757,54.47751593589783,6.273913774085267e-07
89289,178579,178578,357157,54.53214693069458,6.199554915866075e-07
89389,178779,178778,357557,54.58626103401184,6.125515655286833e-07
89489,178979,178978,357957,54.640592098236084,6.052174083098207e-07
89590,179181,179180,358361,54.695703983306885,5.979130086102331e-07
89690,179381,179380,358761,54.75102996826172,5.907730523524126e-07
89790,179581,179580,359161,54.810559034347534,5.836845864861313e-07
89890,179781,179780,359561,54.86387085914612,5.766346507718779e-07
89990,179981,179980,359961,54.91804480552673,5.696635572283088e-07
90090,180181,180180,360361,54.973772048950195,5.628111482474999e-07
90190,180381,180380,360761,55.02847695350647,5.56058189399204e-07
90290,180581,180580,361161,55.08458995819092,5.493586766951103e-07
90390,180781,180780,361561,55.140880823135376,5.42718415155775e-07
90490,180981,180980,361961,55.20684599876404,5.361959827254872e-07
90591,181183,181182,362365,55.27693009376526,5.297568661274034e-07
90691,181383,181382,362765,55.337804079055786,5.234841580130019e-07
90791,181583,181582,363165,55.40873384475708,5.172588115196956e-07
90891,181783,181782,363565,55.484740018844604,5.110912350881152e-07
90991,181983,181982,363965,55.55750489234924,5.050398418078285e-07
91091,182183,182182,364365,55.61807990074158,4.991300116461012e-07
91191,182383,182382,364765,55.676182985305786,4.933209744936856e-07
91291,182583,182582,365165,55.733349084854126,4.875567713044838e-07
91391,182783,182782,365565,55.790714740753174,4.818242773626119e-07
91491,182983,182982,365965,55.847482204437256,4.761525891898084e-07
91592,183185,183184,366369,55.90445590019226,4.705210408575822e-07
91692,183385,183384,366769,55.96260404586792,4.6505153643708156e-07
91792,183585,183584,367169,56.021775007247925,4.596626586778346e-07
91892,183785,183784,367569,56.07817602157593,4.543090846393008e-07
91992,183985,183984,367969,56.13455295562744,4.489680542075586e-07
92092,184185,184184,368369,56.19244909286499,4.436687872582898e-07
92192,184385,184384,368769,56.25176811218262,4.3846155321911535e-07
92292,184585,184584,369169,56.308927059173584,4.33352780368806e-07
92392,184785,184784,369569,56.378578901290894,4.282909121109862e-07
92492,184985,184984,369969,56.43732190132141,4.2322909376327765e-07
92593,185187,185186,370373,56.49701404571533,4.181329603788996e-07
92693,185387,185386,370773,56.55479192733765,4.131559665817443e-07
92793,185587,185586,371173,56.6130428314209,4.082632033682309e-07
92893,185787,185786,371573,56.66951084136963,4.034187034706379e-07
92993,185987,185986,371973,56.728158950805664,3.985916245233719e-07
93093,186187,186186,372373,56.78599715232849,3.937975922901961e-07
93193,186387,186386,372773,56.8431670665741,3.8907122174639353e-07
93293,186587,186586,373173,56.90111994743347,3.8441927296461854e-07
93393,186787,186786,373573,56.9732449054718,3.7981954445602524e-07
93493,186987,186986,373973,57.03116488456726,3.7525845597535504e-07
93594,187189,187188,374377,57.08942890167236,3.7070867586690696e-07
93694,187389,187388,374777,57.14697599411011,3.662888906221662e-07
93794,187589,187588,375177,57.203441858291626,3.619575877507921e-07
93894,187789,187788,375577,57.25941491127014,3.5768672225747386e-07
93994,187989,187988,375977,57.32280492782593,3.5344565669422275e-07
94094,188189,188188,376377,57.39587616920471,3.492347546739041e-07
94194,188389,188388,376777,57.462379932403564,3.4508773212149264e-07
94294,188589,188588,377177,57.518900871276855,3.4103909026113684e-07
94394,188789,188788,377577,57.574923038482666,3.37085531076439e-07
94494,188989,188988,377977,57.630714893341064,3.3318082584499075e-07
94595,189191,189190,378381,57.68688106536865,3.2923862170050655e-07
94695,189391,189390,378781,57.747523069381714,3.2533952460003263e-07
94795,189591,189590,379181,57.80948805809021,3.214977312434846e-07
94895,189791,189790,379581,57.87031388282776,3.1775956604912793e-07
94995,189991,189990,379981,57.92848515510559,3.14110023343391e-07
95095,190191,190190,380381,57.99215316772461,3.1048573131058114e-07
95195,190391,190390,380781,58.050256967544556,3.068440555883996e-07
95295,190591,190590,381181,58.108142137527466,3.032072396505976e-07
95395,190791,190790,381581,58.1653528213501,2.996300069060547e-07
95495,190991,190990,381981,58.2395179271698,2.9613407849212896e-07
95596,191193,191192,382385,58.31120681762695,2.9265440062324074e-07
95696,191393,191392,382785,58.377326011657715,2.8921730647704145e-07
95796,191593,191592,383185,58.43732500076294,2.857782416067841e-07
95896,191793,191792,383585,58.49573612213135,2.823587629851113e-07
95996,191993,191992,383985,58.556060791015625,2.7898097333163993e-07
96096,192193,192192,384385,58.61667084693909,2.756476156238138e-07
96196,192393,192392,384785,58.675390005111694,2.72349630487867e-07
96296,192593,192592,385185,58.73500108718872,2.69083354886126e-07
96396,192793,192792,385585,58.79481911659241,2.6585464550193153e-07
96496,192993,192992,385985,58.85456681251526,2.6266918325117704e-07
96597,193195,193194,386389,58.91514015197754,2.594933049732299e-07
96697,193395,193394,386789,58.97560501098633,2.563825507026551e-07
96797,193595,193594,387189,59.03331780433655,2.5330324488576193e-07
96897,193795,193794,387589,59.09281516075134,2.5026511118370755e-07
96997,193995,193994,387989,59.15105104446411,2.472831493770019e-07
97097,194195,194194,388389,59.21201205253601,2.443597490981179e-07
97197,194395,194394,388789,59.28445887565613,2.4147455799511677e-07
97297,194595,194594,389189,59.35992503166199,2.386011384964809e-07
97397,194795,194794,389589,59.42307186126709,2.3573956436651094e-07
97497,194995,194994,389989,59.49651789665222,2.3292593978037373e-07
97598,195197,195196,390393,59.57461094856262,2.3017015707292656e-07
97698,195397,195396,390793,59.63399386405945,2.2751776349706035e-07
97798,195597,195596,391193,59.69600510597229,2.2488909301872662e-07
97898,195797,195796,391593,59.75695204734802,2.22244563497206e-07
97998,195997,195996,391993,59.81830596923828,2.195981575788809e-07
98098,196197,196196,392393,59.87866401672363,2.1699600910404e-07
98198,196397,196396,392793,59.937726974487305,2.1446359062865682e-07
98298,196597,196596,393193,59.99684000015259,2.119844681379751e-07
98398,196797,196796,393593,60.05543303489685,2.095247981742123e-07
98498,196997,196996,393993,60.117424964904785,2.0706618745094666e-07
98599,197199,197198,394397,60.182496070861816,2.0459068060364503e-07
98699,197399,197398,394797,60.267776012420654,2.0216660642634568e-07
98799,197599,197598,395197,60.3420889377594,1.9978337868365573e-07
98899,197799,197798,395597,60.410048961639404,1.974380034542728e-07
98999,197999,197998,395997,60.468979835510254,1.9511284662155972e-07
99099,198199,198198,396397,60.52646803855896,1.9279331230797625e-07
99199,198399,198398,396797,60.58385396003723,1.9048403478150112e-07
99299,198599,198598,397197,60.64099884033203,1.8820207742954967e-07
99399,198799,198798,397597,60.70054602622986,1.859541448470476e-07
99499,198999,198998,397997,60.77490997314453,1.8373022571709705e-07
99600,199201,199200,398401,60.85618615150452,1.8150118851289065e-07
99700,199401,199400,398801,60.91706299781799,1.79321443504642e-07
99800,199601,199600,399201,60.975502014160156,1.771818899670854e-07
99900,199801,199800,399601,61.03328895568848,1.7507729766674394e-07
100000,200001,200000,400001,61.0918710231781,1.7299025675631476e-07


==> plot_data/quadratic_minimax_problem_n500_alpha00001/flex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.001444101333618164,30.358106049564984
100,459,0,459,1.3437139987945557,0.4177783180862636
200,946,0,946,2.6486191749572754,0.14175932992192242
300,1438,0,1438,3.8425540924072266,0.07601728769773797
400,1938,0,1938,5.278935194015503,0.0725310775598768
501,2437,0,2437,6.596522092819214,0.04538065490306894
601,2937,0,2937,7.757116317749023,0.044068625079784526
701,3433,0,3433,8.949284076690674,0.03533688712286274
801,3932,0,3932,10.12729811668396,0.02924057673082615
901,4432,0,4432,11.279781103134155,0.028390523873332518
1001,4932,0,4932,12.379555225372314,0.027765611371221067
1101,5430,0,5430,13.49347996711731,0.025054014706036555
1201,5930,0,5930,14.596665143966675,0.023414283276782594
1301,6430,0,6430,15.710084199905396,0.022681373934310387
1401,6928,0,6928,16.8121120929718,0.01990069636099634
1502,7433,0,7433,17.952710151672363,0.019121594206419255
1602,7933,0,7933,19.07693910598755,0.01858096791255499
1702,8433,0,8433,20.180617094039917,0.018144552419579744
1802,8929,0,8929,21.27962899208069,0.015316418393985001
1902,9429,0,9429,22.385278940200806,0.013597420394604117
2002,9929,0,9929,23.636065006256104,0.01315521950758562
2102,10429,0,10429,24.871247053146362,0.012806038390595714
2202,10928,0,10928,25.925913095474243,0.011881428256675928
2302,11428,0,11428,26.899526119232178,0.011480478014737422
2402,11928,0,11928,27.853302001953125,0.011214057586319317
2503,12432,0,12432,28.869408130645752,0.010327181404105597
2603,12932,0,12932,29.957327127456665,0.010045841745684337
2703,13431,0,13431,31.071592092514038,0.009314577543619739
2803,13931,0,13931,32.31199526786804,0.008984460058306986
2903,14431,0,14431,33.474244117736816,0.008797737119575492
3003,14929,0,14929,34.5835599899292,0.007795128751181283
3103,15429,0,15429,35.681008100509644,0.007402164356026432
3203,15929,0,15929,36.79555296897888,0.007164753451444441
3303,16429,0,16429,37.94761109352112,0.006977696664473585
3403,16929,0,16929,39.20013999938965,0.006822265438383189
3504,17432,0,17432,40.3418550491333,0.006299274488423881
3604,17932,0,17932,41.46460318565369,0.00594520532488727
3704,18432,0,18432,42.68791198730469,0.0057305625896245
3804,18932,0,18932,43.79246807098389,0.0055721034066578716
3904,19432,0,19432,45.004515171051025,0.005445026156827749
4004,19931,0,19931,46.117182970047,0.005114177517521077
4104,20431,0,20431,47.24500513076782,0.00495361539262455
4204,20931,0,20931,48.64005923271179,0.0048415489454242755
4304,21431,0,21431,49.85076093673706,0.004751275876701585
4404,21930,0,21930,51.281538009643555,0.004404655749844648
4505,22435,0,22435,52.51587104797363,0.004291968948930966
4605,22934,0,22934,53.79017496109009,0.004042927019732852
4705,23434,0,23434,55.138615131378174,0.0039104690294445976
4805,23934,0,23934,56.236714124679565,0.003831582489277955
4905,24434,0,24434,57.356343030929565,0.0037687916076420106
5005,24934,0,24934,58.45380520820618,0.0037140079593162567
5105,25434,0,25434,59.57071304321289,0.0036637177711404166
5205,25933,0,25933,60.664454221725464,0.0034308828938173887
5305,26433,0,26433,61.76676607131958,0.0033183566038330276
5405,26933,0,26933,62.86151719093323,0.0032534607671240515
5506,27434,0,27434,63.97145128250122,0.002601333708075385
5606,27934,0,27934,65.06941103935242,0.002461351895938841
5706,28434,0,28434,66.18212413787842,0.0023769331894139428
5806,28934,0,28934,67.34075117111206,0.0023126743631039413
5906,29434,0,29434,68.47047710418701,0.002260107506134496
6006,29934,0,29934,69.6246280670166,0.002214863776737378
6106,30434,0,30434,70.80647921562195,0.0021747861671821147
6206,30934,0,30934,71.95562601089478,0.002138376884605648
6306,31434,0,31434,73.09168219566345,0.0021045387067470957
6406,31931,0,31931,74.19195508956909,0.001768305579215513
6507,32436,0,32436,75.29798197746277,0.0016444399345383839
6607,32936,0,32936,76.42410230636597,0.00158055689094123
6707,33436,0,33436,77.52315211296082,0.0015376571350073102
6807,33936,0,33936,78.64048218727112,0.0015042413216694644
6907,34436,0,34436,79.77792692184448,0.0014757756509199908
7007,34936,0,34936,80.92021918296814,0.001450372558477935
7107,35436,0,35436,82.03440809249878,0.0014271372478449598
7207,35936,0,35936,83.14057302474976,0.0014054709197256073
7307,36436,0,36436,84.2688980102539,0.0013852217253169
7407,36935,0,36935,85.36927223205566,0.0013174525609556354
7508,37440,0,37440,86.52415800094604,0.001271514913751273
7608,37940,0,37940,87.6423671245575,0.001241946102043871
7708,38440,0,38440,88.73730206489563,0.00121903349112773
7808,38940,0,38940,89.87076997756958,0.0011995365763850234
7908,39438,0,39438,91.02064418792725,0.0010934910665205695
8008,39938,0,39938,92.12119197845459,0.0010382455800063799
8108,40438,0,40438,93.21584796905518,0.0010079355365055036
8208,40938,0,40938,94.46010613441467,0.0009860915212939875
8308,41438,0,41438,95.6563949584961,0.0009681037842690677
8408,41938,0,41938,96.89652991294861,0.0009523147156473299
8509,42443,0,42443,98.17666101455688,0.0009377770408143001
8609,42943,0,42943,99.4133551120758,0.000924456937117362
8709,43443,0,43443,100.9830310344696,0.0009119188525692536
8809,43943,0,43943,102.34749794006348,0.0009000652893896586
8909,44443,0,44443,103.57060194015503,0.0008886739611242621
9009,44942,0,44942,104.90580916404724,0.0008443116261274162
9109,45442,0,45442,106.14191794395447,0.0008210645325951795
9209,45942,0,45942,107.44775819778442,0.0008036742749053365
9309,46442,0,46442,108.69150018692017,0.0007892526970755217
9409,46942,0,46942,109.91604709625244,0.0007766510134182753
9510,47447,0,47447,111.1652340888977,0.0007651295061535939
9610,47947,0,47947,112.29032492637634,0.0007545677099223517
9710,48446,0,48446,113.52125906944275,0.0007324156725780625
9810,48946,0,48946,114.67651510238647,0.0007014458974664369
9910,49446,0,49446,115.83966898918152,0.0006852987940345988
10010,49946,0,49946,117.16943216323853,0.0006733674818009415
10110,50446,0,50446,118.36485004425049,0.0006631582277245041
10210,50946,0,50946,119.5842182636261,0.0006538674943510608
10310,51446,0,51446,120.76018905639648,0.0006451683380868496
10410,51946,0,51946,122.0774872303009,0.0006368829577454346
10511,52451,0,52451,123.30457806587219,0.0006288208138258747
10611,52951,0,52951,124.40029501914978,0.0006211169030631502
10711,53451,0,53451,125.4135811328888,0.0006136395843641378
10811,53951,0,53951,126.49870014190674,0.0006063908319252937
10911,54451,0,54451,127.75040626525879,0.0005992932638615387
11011,54950,0,54950,129.09409308433533,0.0005620960651881439
11111,55450,0,55450,130.3426811695099,0.0005473522747839182
11211,55950,0,55950,131.60787892341614,0.0005374317940319283
11311,56450,0,56450,132.99244594573975,0.0005293268932826646
11411,56950,0,56950,134.60720205307007,0.0005221184689501902
11512,57455,0,57455,135.9972381591797,0.0005153643422958937
11612,57955,0,57955,137.35430717468262,0.0005090204624176557
11712,58455,0,58455,138.8443431854248,0.0005029207592326038
11812,58955,0,58955,140.2047061920166,0.0004970207468232001
11912,59455,0,59455,141.39050388336182,0.000491300283093536
12012,59955,0,59955,142.71889424324036,0.00048573766154281497
12112,60455,0,60455,144.04824805259705,0.0004803182608662925
12212,60954,0,60954,145.46413111686707,0.0004563348145047628
12312,61454,0,61454,146.68298387527466,0.00044436700353847494
12412,61954,0,61954,148.17941212654114,0.00043649320553683217
12513,62459,0,62459,149.3172469139099,0.0004300656099434651
12613,62959,0,62959,150.4829502105713,0.00042438606294749933
12713,63459,0,63459,151.7871081829071,0.0004190957602749606
12813,63959,0,63959,153.04019403457642,0.0004140468736639998
12913,64459,0,64459,154.41687393188477,0.0004091800198050311
13013,64959,0,64959,156.07093000411987,0.0004044434858118401
13113,65459,0,65459,157.75449919700623,0.00039980169698236893
13213,65959,0,65959,160.0249059200287,0.00039525038160553
13313,66459,0,66459,161.69914603233337,0.00039076420679845525
13413,66959,0,66959,163.48623895645142,0.00038635133171211817
13514,67464,0,67464,165.0318672657013,0.0003819460308852868
13614,67964,0,67964,166.36785411834717,0.0003776505137463102
13714,68464,0,68464,167.63716506958008,0.00037340694758298117
13814,68964,0,68964,169.11024808883667,0.0003692209066811099
13914,69464,0,69464,170.3735601902008,0.00036510333860995635
14014,69964,0,69964,171.77043509483337,0.00036103490449362414
14114,70464,0,70464,173.04830312728882,0.00035703451515604174
14214,70964,0,70964,174.4976770877838,0.0003530803603711334
14314,71464,0,71464,176.26417422294617,0.0003491786256077799
14414,71964,0,71964,177.54377698898315,0.0003453250709973222
14515,72468,0,72468,178.73351192474365,0.00033438566170958576
14615,72968,0,72968,180.18937397003174,0.0003256733222885569
14715,73468,0,73468,181.6072871685028,0.00031889909115047983
14815,73968,0,73968,182.8272180557251,0.000313323314360583
14915,74468,0,74468,184.04116916656494,0.0003085027848760246
15015,74968,0,74968,185.24681496620178,0.00030417286917158037
15115,75468,0,75468,186.50020623207092,0.00030018353704620247
15215,75968,0,75968,187.90470814704895,0.00029642753700423284
15315,76468,0,76468,189.4217710494995,0.00029283841574578395
15415,76968,0,76968,190.89225697517395,0.0002893826395526868
15516,77473,0,77473,192.13032007217407,0.00028598247437223615
15616,77973,0,77973,193.6739902496338,0.0002826946981087163
15716,78473,0,78473,195.1978461742401,0.0002794712137918587
15816,78973,0,78973,196.79899406433105,0.00027629751150990453
15916,79473,0,79473,198.27394723892212,0.0002731705321914717
16016,79973,0,79973,199.80794215202332,0.00027008693640050125
16116,80473,0,80473,201.13425207138062,0.0002670446304588568
16216,80973,0,80973,202.38352012634277,0.00026404001567025963
16316,81473,0,81473,203.59275603294373,0.00026107951000241465
16416,81973,0,81973,204.84079003334045,0.0002581564813065858
16517,82478,0,82478,206.31258010864258,0.0002552462808488027
16617,82978,0,82978,207.58086705207825,0.0002524050521029749
16717,83478,0,83478,208.93677496910095,0.00024960119026006526
16817,83978,0,83978,210.2335660457611,0.00024683866603185525
16917,84478,0,84478,212.07190918922424,0.00024411248382455884
17017,84978,0,84978,214.2612280845642,0.00024142666906205965
17117,85478,0,85478,216.1512451171875,0.00023878212756152758
17217,85978,0,85978,217.5940990447998,0.0002361746668935683
17317,86478,0,86478,218.87350511550903,0.00023361317058781127
17417,86978,0,86978,220.64686012268066,0.00023108962894049834
17518,87483,0,87483,222.1141140460968,0.00022858497820521425
17618,87983,0,87983,223.50740313529968,0.0002261444358158042
17718,88483,0,88483,225.2631549835205,0.00022374153408966625
17818,88983,0,88983,227.03921008110046,0.00022137357621910511
17918,89482,0,89482,228.8451452255249,0.0002155168875996505
18018,89982,0,89982,230.73800706863403,0.00021083043928781856
18118,90482,0,90482,232.11134099960327,0.00020684969946099986
18218,90982,0,90982,233.66431427001953,0.00020336187707748732
18318,91482,0,91482,234.99761509895325,0.00020024622982228057
18418,91982,0,91982,236.40107321739197,0.00019739572932560512
18519,92487,0,92487,237.69369220733643,0.0001947157209637144
18619,92987,0,92987,238.94412422180176,0.00019221221107425495
18719,93487,0,93487,240.4250612258911,0.0001898185981769276
18819,93987,0,93987,241.9810061454773,0.00018751631835416916
18919,94487,0,94487,243.17607927322388,0.00018529069359485832
19019,94987,0,94987,244.25333499908447,0.00018312069041499755
19119,95487,0,95487,245.42418217658997,0.0001810091211522038
19219,95987,0,95987,246.6499960422516,0.00017893778333190536
19319,96487,0,96487,247.79554319381714,0.00017691253864272224
19419,96987,0,96987,248.94996404647827,0.0001749222375333678
19520,97492,0,97492,250.24643301963806,0.00017295354273458966
19620,97992,0,97992,251.44610214233398,0.00017103491865520966
19720,98492,0,98492,252.99484014511108,0.00016915081471442455
19820,98992,0,98992,254.39477610588074,0.000167300366168136
19920,99492,0,99492,255.65587401390076,0.00016547689978376978
20020,99992,0,99992,256.7851951122284,0.00016368722019534468
20120,100492,0,100492,257.88951301574707,0.00016192382266078174
20220,100992,0,100992,259.09400820732117,0.0001601862650150349
20320,101492,0,101492,260.32452416419983,0.00015847404154761398
20420,101992,0,101992,261.4506139755249,0.00015678359310343867
20521,102497,0,102497,262.6436128616333,0.00015510021801141535
20621,102997,0,102997,264.1100420951843,0.00015345134606217754
20721,103497,0,103497,265.4151191711426,0.00015182013742909097
20821,103997,0,103997,266.8133592605591,0.00015020498991846754
20921,104497,0,104497,268.05882024765015,0.00014860336021587476
21021,104997,0,104997,269.2431321144104,0.0001470157093916856
21121,105497,0,105497,270.36021995544434,0.00014544042156765767
21221,105997,0,105997,271.58097219467163,0.00014387567760265006
21321,106497,0,106497,272.7089989185333,0.00014232258250607304
21421,106997,0,106997,273.89279413223267,0.00014078150182636855
21522,107502,0,107502,275.1102452278137,0.00013923581265492196
21622,108002,0,108002,276.29761719703674,0.00013771666997906994
21722,108502,0,108502,277.49145007133484,0.00013621260987070301
21822,109002,0,109002,278.6788651943207,0.00013472124940212642
21922,109502,0,109502,279.95566415786743,0.0001332453210948506
22022,110002,0,110002,281.20237493515015,0.00013178703065396482
22122,110502,0,110502,282.27047085762024,0.0001303441077582096
22222,111002,0,111002,283.5417721271515,0.00012891935454397417
22322,111502,0,111502,284.70920610427856,0.00012751316206831967
22422,112002,0,112002,285.8222200870514,0.00012612426406327691
22523,112507,0,112507,287.01996326446533,0.0001247398451410863
22623,113006,0,113006,288.302855014801,0.0001219657756015339
22723,113506,0,113506,289.4547052383423,0.0001192346332761072
22823,114006,0,114006,290.5561349391937,0.00011687087247224473
22923,114506,0,114506,291.71707010269165,0.00011478003341600703
23023,115006,0,115006,292.92033314704895,0.00011289891523710435
23123,115506,0,115506,294.05291223526,0.00011118691534247451
23223,116006,0,116006,295.2617530822754,0.00010960693505900789
23323,116506,0,116506,296.5679852962494,0.00010812648506114296
23423,117006,0,117006,297.76085805892944,0.0001067246270977538
23524,117511,0,117511,298.93977308273315,0.00010537409894352683
23624,118011,0,118011,300.2640380859375,0.00010408742653686867
23724,118511,0,118511,301.40400218963623,0.00010284182505709286
23824,119011,0,119011,302.6144971847534,0.00010163698539779948
23924,119511,0,119511,303.80491399765015,0.00010046050819300394
24024,120011,0,120011,304.98391103744507,9.930408893726373e-05
24124,120511,0,120511,306.0897569656372,9.817126151220233e-05
24224,121011,0,121011,307.19545006752014,9.705915282310924e-05
24324,121511,0,121511,308.28785514831543,9.596430722778784e-05
24424,122011,0,122011,309.39580488204956,9.488622230077426e-05
24525,122516,0,122516,310.5050871372223,9.381386532289594e-05
24625,123016,0,123016,311.6967911720276,9.276572470910681e-05
24725,123516,0,123516,312.80940222740173,9.173063275885457e-05
24825,124016,0,124016,313.90950202941895,9.071297074896527e-05
24925,124516,0,124516,315.00067615509033,8.970884883966132e-05
25025,125016,0,125016,316.10490918159485,8.871666237168206e-05
25125,125516,0,125516,317.2046048641205,8.774064529236145e-05
25225,126016,0,126016,318.3036811351776,8.677980866962623e-05
25325,126516,0,126516,319.39744424819946,8.582937053546485e-05
25425,127016,0,127016,320.50361800193787,8.48955757202122e-05
25526,127521,0,127521,321.6128010749817,8.39687798843142e-05
25626,128021,0,128021,322.7121069431305,8.306106069174072e-05
25726,128521,0,128521,323.80378818511963,8.216805926327842e-05
25826,129021,0,129021,324.9125680923462,8.128919739224383e-05
25926,129521,0,129521,326.01856803894043,8.042003796319915e-05
26026,130021,0,130021,327.20936822891235,7.956288142042239e-05
26126,130521,0,130521,328.34621596336365,7.87171528088483e-05
26226,131021,0,131021,329.44941306114197,7.78789414092479e-05
26326,131521,0,131521,330.5596580505371,7.705167112803877e-05
26426,132021,0,132021,331.6555550098419,7.623337710794204e-05
26527,132526,0,132526,332.7722361087799,7.541157643651911e-05
26627,133026,0,133026,333.8605649471283,7.460622772078033e-05
26727,133526,0,133526,334.9705421924591,7.380995793479146e-05
26827,134026,0,134026,336.067675113678,7.30190492240955e-05
26927,134526,0,134526,337.1739110946655,7.223385281532876e-05
27027,135026,0,135026,338.26326608657837,7.14554312265782e-05
27127,135526,0,135526,339.477441072464,7.068458652004796e-05
27227,136026,0,136026,340.62790513038635,6.991971092065215e-05
27327,136526,0,136526,341.8284249305725,6.916301012470776e-05
27427,137026,0,137026,343.0550148487091,6.841555453601123e-05
27528,137531,0,137531,344.2509171962738,6.766803018466e-05
27628,138031,0,138031,345.36024618148804,6.693574791512647e-05
27728,138531,0,138531,346.46640515327454,6.621359794780738e-05
27828,139031,0,139031,347.5654022693634,6.550048252689829e-05
27928,139531,0,139531,348.6863172054291,6.47964029500481e-05
28028,140031,0,140031,349.78642320632935,6.41021997713222e-05
28128,140531,0,140531,350.9590232372284,6.341535689360674e-05
28228,141031,0,141031,352.2096121311188,6.27362524787659e-05
28328,141531,0,141531,353.37068223953247,6.206724113449434e-05
28428,142031,0,142031,354.50374603271484,6.140669338183834e-05
28529,142536,0,142536,355.6264362335205,6.074685561704041e-05
28629,143036,0,143036,356.7418580055237,6.010014450474079e-05
28729,143536,0,143536,357.8444890975952,5.946024030645318e-05
28829,144036,0,144036,359.020467042923,5.8827617649597955e-05
28929,144536,0,144536,360.1247491836548,5.8200998472433624e-05
29029,145036,0,145036,361.262971162796,5.7580150303739074e-05
29129,145536,0,145536,362.36615085601807,5.696491601605392e-05
29229,146036,0,146036,363.48220205307007,5.635382166322748e-05
29329,146536,0,146536,364.6006200313568,5.574845768244752e-05
29429,147036,0,147036,365.75716829299927,5.5148876508038447e-05
29530,147541,0,147541,366.8916952610016,5.454668860012277e-05
29630,148041,0,148041,368.1958529949188,5.395511398766742e-05
29730,148541,0,148541,369.394602060318,5.3369513084395924e-05
29830,149041,0,149041,370.50001096725464,5.278793963577943e-05
29930,149541,0,149541,371.60943698883057,5.221111654658672e-05
30030,150041,0,150041,372.7125220298767,5.164013549641547e-05
30130,150541,0,150541,373.81547713279724,5.107447867883836e-05
30230,151041,0,151041,374.90629601478577,5.051551635517621e-05
30330,151541,0,151541,376.00977897644043,4.996345977756957e-05
30430,152041,0,152041,377.1147041320801,4.9417322109135715e-05
30531,152546,0,152546,378.22979521751404,4.8873001649191144e-05
30631,153046,0,153046,379.3265149593353,4.834182106417658e-05
30731,153546,0,153546,380.42329597473145,4.781706619897961e-05
30831,154046,0,154046,381.52603006362915,4.7299173016522024e-05
30931,154546,0,154546,382.6278142929077,4.678882397764038e-05
31031,155046,0,155046,383.71620512008667,4.6285255072989336e-05
31131,155546,0,155546,384.8272111415863,4.5787709052220686e-05
31231,156046,0,156046,385.91948413848877,4.5296705020198724e-05
31331,156546,0,156546,387.02377820014954,4.481258660975853e-05
31431,157046,0,157046,388.18974709510803,4.4334317480227565e-05
31532,157551,0,157551,389.43935799598694,4.3856803884512845e-05
31632,158051,0,158051,390.6116752624512,4.3389859810586404e-05
31732,158551,0,158551,391.7695748806,4.292810598805867e-05
31832,159051,0,159051,393.0380349159241,4.247120840025504e-05
31932,159551,0,159551,394.16399788856506,4.201923426372581e-05
32032,160051,0,160051,395.45793318748474,4.157134146272643e-05
32132,160551,0,160551,396.6441011428833,4.1127112315303414e-05
32232,161051,0,161051,397.82328701019287,4.0687236378794365e-05
32332,161551,0,161551,398.98485708236694,4.0251435204314086e-05
32432,162051,0,162051,400.14693808555603,3.981927041455882e-05
32533,162556,0,162556,401.3103759288788,3.938671245407388e-05
32633,163056,0,163056,402.4476249217987,3.8962296806084434e-05
32733,163556,0,163556,403.70908403396606,3.8541840517381724e-05
32833,164056,0,164056,404.925833940506,3.8125571125778e-05
32933,164556,0,164556,406.1161060333252,3.77137137044239e-05
33033,165056,0,165056,407.3067798614502,3.730651175474961e-05
33133,165556,0,165556,408.6058192253113,3.690387241427071e-05
33233,166056,0,166056,409.7139341831207,3.6506091315853715e-05
33333,166556,0,166556,410.819699048996,3.611349689655464e-05
33433,167056,0,167056,411.9143600463867,3.572614335949348e-05
33534,167561,0,167561,413.02788519859314,3.534042359211925e-05
33634,168061,0,168061,414.140593290329,3.496377120346445e-05
33734,168561,0,168561,415.40378308296204,3.459184043731972e-05
33834,169061,0,169061,416.6263520717621,3.422499397078352e-05
33934,169561,0,169561,417.7780559062958,3.3863431683571225e-05
34034,170061,0,170061,418.88633608818054,3.350619492469981e-05
34134,170561,0,170561,420.140114068985,3.3152904294663406e-05
34234,171061,0,171061,421.3447461128235,3.280382950337981e-05
34334,171561,0,171561,422.40831422805786,3.2458523992637095e-05
34434,172061,0,172061,423.59988713264465,3.211653296004344e-05
34535,172566,0,172566,424.7572650909424,3.1774177407125385e-05
34635,173066,0,173066,425.8721332550049,3.1437892288382413e-05
34735,173566,0,173566,426.9955220222473,3.1104364938236076e-05
34835,174066,0,174066,428.1071779727936,3.0773635760124096e-05
34935,174566,0,174566,429.20178627967834,3.044529487963321e-05
35035,175066,0,175066,430.3812119960785,3.0119233678843722e-05
35135,175566,0,175566,431.53869915008545,2.9795992019045267e-05
35235,176066,0,176066,432.6748080253601,2.947575054294454e-05
35335,176566,0,176566,433.771931886673,2.915824954069372e-05
35435,177066,0,177066,434.906023979187,2.8843605479757906e-05
35536,177571,0,177571,436.02695202827454,2.852901007438208e-05
35636,178071,0,178071,437.13678216934204,2.8220720793562377e-05
35736,178571,0,178571,438.24673199653625,2.7915647927604747e-05
35836,179071,0,179071,439.36513209342957,2.7614011920278146e-05
35936,179571,0,179571,440.453910112381,2.7315891781905105e-05
36036,180071,0,180071,441.56283712387085,2.7021301315368236e-05
36136,180571,0,180571,442.6819839477539,2.6730381151970066e-05
36236,181071,0,181071,443.80851006507874,2.64431347746308e-05
36336,181567,0,181567,444.9054489135742,2.4758139166353404e-05
36436,182067,0,182067,446.13187193870544,2.4469446948454398e-05
36537,182572,0,182572,447.40120911598206,2.4184550018347918e-05
36637,183072,0,183072,448.5311322212219,2.3904667681089315e-05
36737,183572,0,183572,449.66693210601807,2.3630675006035834e-05
36837,184072,0,184072,450.9198820590973,2.336107354573459e-05
36937,184572,0,184572,452.0492310523987,2.3093597436580734e-05
37037,185072,0,185072,453.14620327949524,2.2830130498251928e-05
37137,185572,0,185572,454.2426931858063,2.2571112477224215e-05
37237,186072,0,186072,455.39273715019226,2.2315598689357874e-05
37337,186572,0,186572,456.7113561630249,2.2062388797824966e-05
37437,187072,0,187072,458.0724730491638,2.1811888098543773e-05
37538,187577,0,187577,459.56900215148926,2.1563625478502556e-05
37638,188077,0,188077,460.6954290866852,2.1320250500516268e-05
37738,188577,0,188577,461.84151816368103,2.107872049068823e-05
37838,189077,0,189077,463.3122401237488,2.084160383876619e-05
37938,189577,0,189577,464.6571829319,2.060663066464926e-05
38038,190077,0,190077,466.1898310184479,2.0372314453985773e-05
38138,190577,0,190577,467.66381907463074,2.014342031196946e-05
38238,191077,0,191077,468.868243932724,1.9916955741012533e-05
38338,191577,0,191577,470.0531499385834,1.9691330357419506e-05
38438,192077,0,192077,471.22212505340576,1.947050083882645e-05
38539,192582,0,192582,472.67108607292175,1.924966067524094e-05
38639,193082,0,193082,473.829430103302,1.903288005243698e-05
38739,193582,0,193582,475.1398551464081,1.8821127446457076e-05
38839,194082,0,194082,476.49254298210144,1.861171809428198e-05
38939,194582,0,194582,477.6452660560608,1.8404191265212173e-05
39039,195082,0,195082,479.0962071418762,1.8200850302727075e-05
39139,195582,0,195582,480.26216411590576,1.800075789666051e-05
39239,196082,0,196082,481.73844504356384,1.7802422524324302e-05
39339,196582,0,196582,483.19166707992554,1.7607417973754064e-05
39439,197082,0,197082,484.4575791358948,1.74156142538411e-05
39540,197587,0,197587,485.99728202819824,1.7224118202948158e-05
39640,198087,0,198087,487.11669993400574,1.7037157341547638e-05
39740,198587,0,198587,488.4004611968994,1.6852511050901508e-05
39840,199087,0,199087,489.82164192199707,1.6670016156615018e-05
39940,199587,0,199587,490.928111076355,1.6489118675185517e-05
40040,200087,0,200087,492.0403730869293,1.631086879528157e-05
40140,200587,0,200587,493.1430780887604,1.61352835984699e-05
40240,201087,0,201087,494.33528304100037,1.596035824198345e-05
40340,201587,0,201587,495.5726180076599,1.578714394595393e-05
40440,202087,0,202087,496.6937780380249,1.561610088306341e-05
40541,202592,0,202592,497.8550579547882,1.5444942817258926e-05
40641,203092,0,203092,498.96627616882324,1.5277682043544248e-05
40741,203592,0,203592,500.0883550643921,1.511214688382398e-05
40841,204092,0,204092,501.42877221107483,1.4947787394190242e-05
40941,204592,0,204592,502.6802680492401,1.4784939211747223e-05
41041,205092,0,205092,503.86689710617065,1.4624214532359079e-05
41141,205592,0,205592,505.3698959350586,1.446558141684178e-05
41241,206092,0,206092,506.62630915641785,1.430869176679836e-05
41341,206592,0,206592,507.78914618492126,1.4153384217204847e-05
41441,207092,0,207092,509.14081621170044,1.400006063232184e-05
41542,207597,0,207597,510.4381241798401,1.3847053831841963e-05
41642,208097,0,208097,512.0749409198761,1.369756240558973e-05
41742,208597,0,208597,513.5662100315094,1.35506180790394e-05
41842,209097,0,209097,514.7336041927338,1.3405192571801446e-05
41942,209597,0,209597,516.0427210330963,1.32609326834922e-05
42042,210097,0,210097,517.3415009975433,1.3119066120366419e-05
42142,210597,0,210597,518.7288720607758,1.297907002693116e-05
42242,211097,0,211097,520.1692962646484,1.2840392779078467e-05
42342,211597,0,211597,521.3566892147064,1.2703684297929615e-05
42442,212097,0,212097,522.5749711990356,1.2568365212262749e-05
42543,212602,0,212602,524.1707429885864,1.2432700312574631e-05
42643,213102,0,213102,525.5208430290222,1.2300135104970066e-05
42743,213602,0,213602,526.7800760269165,1.2168930976972997e-05
42843,214102,0,214102,528.101722240448,1.2038432346894075e-05
42943,214602,0,214602,529.1917371749878,1.190922197178555e-05
43043,215102,0,215102,530.2155709266663,1.1781110989271377e-05
43143,215602,0,215602,531.330225944519,1.165367766608862e-05
43243,216102,0,216102,532.607565164566,1.1527504201565588e-05
43343,216602,0,216602,534.0210120677948,1.1402599783942539e-05
43443,217102,0,217102,535.4736812114716,1.1278615848864776e-05
43544,217607,0,217607,536.7904171943665,1.1154699707662718e-05
43644,218107,0,218107,537.9828369617462,1.1033741065935602e-05
43744,218607,0,218607,539.3387341499329,1.0913911730099933e-05
43844,219107,0,219107,540.7572391033173,1.079504229435253e-05
43944,219607,0,219607,541.9644842147827,1.0677788708144172e-05
44044,220107,0,220107,543.3072640895844,1.056202118274933e-05
44144,220607,0,220607,544.7767701148987,1.0447523140499555e-05
44244,221107,0,221107,546.2127890586853,1.033445795302614e-05
44344,221607,0,221607,547.4186842441559,1.0222578304510024e-05
44444,222107,0,222107,548.6016340255737,1.0111783868246907e-05
44545,222612,0,222612,550.0508270263672,1.0001498870790633e-05
44645,223112,0,223112,551.2722780704498,9.893952869875802e-06
44745,223612,0,223612,552.6659409999847,9.787657129104306e-06
44845,224112,0,224112,553.9673020839691,9.68257563538978e-06
44945,224612,0,224612,555.337159872055,9.578706777845712e-06
45045,225112,0,225112,556.5738251209259,9.476125578111888e-06
45145,225612,0,225612,557.8944320678711,9.374897006080215e-06
45245,226112,0,226112,559.1110031604767,9.274821855774882e-06
45345,226612,0,226612,560.355978012085,9.175674678850745e-06
45445,227112,0,227112,561.7197189331055,9.077296727833068e-06
45546,227617,0,227617,562.9068269729614,8.978814620662631e-06
45646,228117,0,228117,564.3138749599457,8.882527169408377e-06
45746,228617,0,228617,565.7685790061951,8.787227697704095e-06
45846,229117,0,229117,567.3318920135498,8.692570000329447e-06
45946,229617,0,229617,569.1224598884583,8.598733243853218e-06
46046,230117,0,230117,570.732990026474,8.505680711096603e-06
46146,230617,0,230617,571.9922111034393,8.413416227556367e-06
46246,231117,0,231117,573.3036210536957,8.322285798499552e-06
46346,231617,0,231617,574.7364768981934,8.232094221539659e-06
46446,232117,0,232117,575.9339289665222,8.142510877800837e-06
46547,232622,0,232622,577.4758882522583,8.053018364660047e-06
46647,233122,0,233122,578.7865509986877,7.965549155284193e-06
46747,233622,0,233622,580.0548889636993,7.879072191243845e-06
46847,234122,0,234122,581.7701930999756,7.793759723184333e-06
46947,234622,0,234622,583.3120901584625,7.709576091986175e-06
47047,235122,0,235122,585.1055092811584,7.626335744686339e-06
47147,235622,0,235622,586.4364020824432,7.544207552546298e-06
47247,236122,0,236122,587.9403269290924,7.463289250335407e-06
47347,236622,0,236622,589.436517238617,7.383386638930977e-06
47447,237122,0,237122,590.895565032959,7.304460610108644e-06
47548,237627,0,237627,592.200010061264,7.225792707767383e-06
47648,238127,0,238127,593.4756910800934,7.14884092621591e-06
47748,238627,0,238627,594.9542169570923,7.072793744541637e-06
47848,239127,0,239127,596.4605782032013,6.9976511787271436e-06
47948,239627,0,239627,597.6695930957794,6.923314425945499e-06
48048,240127,0,240127,599.1140029430389,6.849790007182898e-06
48148,240627,0,240627,600.551351070404,6.777201605451543e-06
48248,241127,0,241127,602.184112071991,6.705407334108922e-06
48348,241627,0,241627,603.6099870204926,6.634146783057482e-06
48448,242127,0,242127,605.1305811405182,6.563493932586385e-06
48549,242632,0,242632,606.3585002422333,6.492886823556212e-06
48649,243132,0,243132,607.4993751049042,6.423674063546567e-06
48749,243632,0,243632,608.6822011470795,6.355112350079974e-06
48849,244132,0,244132,609.9928300380707,6.28709163586412e-06
48949,244632,0,244632,611.1296110153198,6.219529692078332e-06
49049,245132,0,245132,612.1762969493866,6.152609529540781e-06
49149,245632,0,245632,613.2930839061737,6.086510876243468e-06
49249,246132,0,246132,614.4515080451965,6.0211948925853215e-06
49349,246632,0,246632,615.6385731697083,5.956518357559711e-06
49449,247132,0,247132,616.8118500709534,5.89244063486401e-06
49550,247637,0,247637,618.0155708789825,5.828433434927389e-06
49650,248137,0,248137,619.2043631076813,5.765914393117245e-06
49750,248637,0,248637,620.4580931663513,5.704284944771898e-06
49850,249137,0,249137,621.8597140312195,5.643427604310878e-06
49950,249637,0,249637,623.030601978302,5.583230683097488e-06
50050,250137,0,250137,624.2044270038605,5.523685846079038e-06
50150,250637,0,250637,625.4220752716064,5.4649257358620515e-06
50250,251137,0,251137,626.8180379867554,5.406970412073335e-06
50350,251637,0,251637,628.2238001823425,5.349641367533867e-06
50450,252137,0,252137,629.602462053299,5.292879735346801e-06
50551,252642,0,252642,631.085942029953,5.236121298926422e-06
50651,253142,0,253142,632.3479082584381,5.180442810130622e-06
50751,253642,0,253642,633.7183170318604,5.125309556299008e-06
50851,254142,0,254142,634.9585840702057,5.070704491540264e-06
50951,254642,0,254642,636.180006980896,5.016512455800144e-06
51051,255142,0,255142,637.3791260719299,4.962734851058347e-06
51151,255642,0,255642,638.9390542507172,4.909446702543266e-06
51251,256142,0,256142,640.076336145401,4.856630884357071e-06
51351,256642,0,256642,641.2633411884308,4.804292390243072e-06
51451,257142,0,257142,642.4672420024872,4.752458312717086e-06
51552,257647,0,257647,643.6414220333099,4.700579900590139e-06
51652,258147,0,258147,644.8333592414856,4.649687520125507e-06
51752,258647,0,258647,646.0264592170715,4.5993004555764e-06
51852,259147,0,259147,647.5063440799713,4.54938739374054e-06
51952,259647,0,259647,648.6776130199432,4.499935824229093e-06
52052,260147,0,260147,649.997040271759,4.451000921406495e-06
52152,260647,0,260647,651.2552120685577,4.402613685668961e-06
52252,261147,0,261147,652.4635081291199,4.354763297578256e-06
52352,261647,0,261647,653.7326469421387,4.307472928879753e-06
52452,262147,0,262147,655.094722032547,4.260760688189293e-06
52553,262652,0,262652,656.2899420261383,4.214178224397701e-06
52653,263152,0,263152,657.4762830734253,4.168719244035852e-06
52753,263652,0,263652,658.7085950374603,4.123926758411941e-06
52853,264152,0,264152,659.9352209568024,4.07968454676253e-06
52953,264652,0,264652,661.1873750686646,4.035936273349656e-06
53053,265152,0,265152,662.6879460811615,3.992730931437731e-06
53153,265652,0,265652,663.8382489681244,3.950083229128714e-06
53253,266152,0,266152,664.9742422103882,3.907970731733579e-06
53353,266652,0,266652,666.2713451385498,3.866339973221415e-06
53453,267152,0,267152,667.4203140735626,3.825107616081232e-06
53554,267657,0,267657,668.8276031017303,3.783854811990382e-06
53654,268157,0,268157,670.1129860877991,3.7434435340904455e-06
53754,268657,0,268657,671.2189040184021,3.70348029452732e-06
53854,269157,0,269157,672.3195662498474,3.6639227884685946e-06
53954,269657,0,269657,673.485405921936,3.624702255017439e-06
54054,270157,0,270157,674.6021802425385,3.585800921864586e-06
54154,270657,0,270657,675.7524642944336,3.547256348220438e-06
54254,271157,0,271157,676.9088032245636,3.5091020479121405e-06
54354,271657,0,271657,678.0899262428284,3.4713340217678622e-06
54454,272157,0,272157,679.2746822834015,3.43392024959705e-06
54555,272662,0,272662,680.4837760925293,3.3964697104966667e-06
54655,273162,0,273162,681.6685838699341,3.3597691136665096e-06
54755,273662,0,273662,682.8344540596008,3.3235108893186466e-06
54855,274162,0,274162,684.0618412494659,3.2876922516835745e-06
54955,274662,0,274662,685.1641721725464,3.252291008176687e-06
55055,275162,0,275162,686.2957921028137,3.217302299311481e-06
55155,275662,0,275662,687.4388899803162,3.1827223493908774e-06
55255,276162,0,276162,688.6692910194397,3.1485724731475995e-06
55355,276662,0,276662,689.8090550899506,3.11486951630993e-06
55455,277162,0,277162,691.0313301086426,3.0815865990125865e-06
55556,277667,0,277667,692.4643530845642,3.048375143167118e-06
55656,278167,0,278167,693.8435909748077,3.015903328397608e-06
55756,278667,0,278667,695.0714020729065,2.983845248792869e-06
55856,279167,0,279167,696.3174510002136,2.9521879575373566e-06
55956,279667,0,279667,697.7693231105804,2.9209188025561865e-06
56056,280167,0,280167,699.5180361270905,2.8900172442733567e-06
56156,280667,0,280667,701.106761932373,2.8594576786021798e-06
56256,281167,0,281167,702.3628122806549,2.829224517237732e-06
56356,281667,0,281667,703.8369920253754,2.7992897396153717e-06
56456,282167,0,282167,705.1463899612427,2.769612752245971e-06
56557,282672,0,282672,706.500214099884,2.739887156767084e-06
56657,283172,0,283172,707.7341680526733,2.710712553700366e-06
56757,283672,0,283672,709.0301020145416,2.6817900837441286e-06
56857,284172,0,284172,710.2775540351868,2.6531072069180945e-06
56957,284672,0,284672,711.5293231010437,2.624659963102356e-06
57057,285172,0,285172,712.8238871097565,2.596455687108258e-06
57157,285672,0,285672,714.1425909996033,2.5685278529025478e-06
57257,286172,0,286172,715.3020920753479,2.5409120285667194e-06
57357,286672,0,286672,716.5518610477448,2.513597678007661e-06
57457,287172,0,287172,717.8724591732025,2.4865542317522048e-06
57558,287677,0,287677,719.2196769714355,2.4595210038146708e-06
57658,288177,0,288177,720.484857082367,2.4330650476121033e-06
57758,288677,0,288677,721.776330947876,2.4069395385034546e-06
57858,289177,0,289177,722.9995710849762,2.3811411544842593e-06
57958,289677,0,289677,724.2573821544647,2.355642481194301e-06
58058,290177,0,290177,725.607017993927,2.3304266351697466e-06
58158,290677,0,290677,727.0561451911926,2.305507406843027e-06
58258,291177,0,291177,728.4293241500854,2.2809041912074893e-06
58358,291677,0,291677,730.0410740375519,2.2566101276976258e-06
58458,292177,0,292177,731.1794831752777,2.232591363131543e-06
58559,292682,0,292682,732.4047412872314,2.2085802823311447e-06
58659,293182,0,293182,733.711837053299,2.18504535220302e-06
58759,293682,0,293682,735.0189161300659,2.1617560171912653e-06
58859,294182,0,294182,736.4402911663055,2.138715567453138e-06
58959,294682,0,294682,737.5500569343567,2.115910359983238e-06
59059,295182,0,295182,738.672749042511,2.0933188463638463e-06
59159,295682,0,295682,739.8101010322571,2.070932134942229e-06
59259,296182,0,296182,740.9286830425262,2.0487537693900075e-06
59359,296682,0,296682,742.0417320728302,2.0267769814991227e-06
59459,297182,0,297182,743.1364369392395,2.0049843102786204e-06
59560,297687,0,297687,744.275778055191,1.983154072163781e-06
59660,298187,0,298187,745.4090020656586,1.9617197432343142e-06
59760,298687,0,298687,746.5111691951752,1.940465844698492e-06
59860,299187,0,299187,747.613970041275,1.919398664091869e-06
59960,299687,0,299687,748.7269592285156,1.8985245914405751e-06
60060,300187,0,300187,749.8192069530487,1.8778517757200504e-06
60160,300687,0,300687,750.9204621315002,1.8573968346508762e-06
60260,301187,0,301187,752.0272481441498,1.8371758450952007e-06
60360,301687,0,301687,753.1747372150421,1.8171957321028884e-06
60460,302187,0,302187,754.3466281890869,1.7974622734397234e-06
60561,302692,0,302692,755.5574929714203,1.7777878963175178e-06
60661,303192,0,303192,756.7267861366272,1.7585629416855465e-06
60761,303692,0,303692,757.9780879020691,1.7395915348907301e-06
60861,304192,0,304192,759.5097260475159,1.7208696471669597e-06
60961,304692,0,304692,760.6648828983307,1.7023852443145815e-06
61061,305192,0,305192,761.8683881759644,1.6841310014724146e-06
61161,305692,0,305692,762.9726221561432,1.666107461913062e-06
61261,306192,0,306192,764.1426281929016,1.648312293064047e-06
61361,306692,0,306692,765.3440041542053,1.6307369013636357e-06
61461,307192,0,307192,766.6034359931946,1.6133699854806846e-06
61562,307697,0,307697,767.8217039108276,1.596030097821916e-06
61662,308197,0,308197,768.9660580158234,1.5790546241561168e-06
61762,308697,0,308697,770.2983989715576,1.56226855175351e-06
61862,309197,0,309197,771.380392074585,1.5456617706098238e-06
61962,309697,0,309697,772.3771729469299,1.5292151046108995e-06
62062,310197,0,310197,773.9125680923462,1.5129155286745008e-06
62162,310697,0,310697,775.2344450950623,1.4967636708336828e-06
62262,311197,0,311197,776.4098889827728,1.4807653824030726e-06
62362,311697,0,311697,777.9692978858948,1.4649224020491598e-06
62462,312197,0,312197,779.035001039505,1.4492310340943158e-06
62563,312702,0,312702,780.2772641181946,1.4335322534561939e-06
62663,313202,0,313202,781.4909110069275,1.4181384309461403e-06
62763,313702,0,313702,782.7617359161377,1.4029015400270456e-06
62863,314202,0,314202,783.9474971294403,1.3878284588765156e-06
62963,314702,0,314702,785.1676530838013,1.372917683004314e-06
63063,315202,0,315202,786.522607088089,1.3581651685270229e-06
63163,315702,0,315702,787.9034571647644,1.343574266252901e-06
63263,316202,0,316202,789.2312331199646,1.3291535375019734e-06
63363,316702,0,316702,790.6810302734375,1.3149102227338883e-06
63463,317202,0,317202,792.4052650928497,1.300847728933644e-06
63564,317707,0,317707,793.6700432300568,1.2868271288751973e-06
63664,318207,0,318207,795.028017282486,1.273124112667211e-06
63764,318707,0,318707,796.1452040672302,1.2595983232861884e-06
63864,319207,0,319207,797.2306351661682,1.246245674252732e-06
63964,319707,0,319707,798.5016980171204,1.2330560630652104e-06
64064,320207,0,320207,799.7373292446136,1.220017727777629e-06
64164,320707,0,320707,801.1655292510986,1.2071203141340176e-06
64264,321207,0,321207,802.4481720924377,1.1943543120133008e-06
64364,321707,0,321707,803.6061880588531,1.1817107691135147e-06
64464,322207,0,322207,804.7187671661377,1.1691810338006463e-06
64565,322712,0,322712,805.8359370231628,1.1566347794900402e-06
64665,323212,0,323212,806.9315211772919,1.1443183832653459e-06
64765,323712,0,323712,808.0164921283722,1.1321079286975326e-06
64865,324212,0,324212,809.1929879188538,1.1200035742706644e-06
64965,324712,0,324712,810.4263648986816,1.1080049605588141e-06
65065,325212,0,325212,811.6726689338684,1.096113182685053e-06
65165,325712,0,325712,812.971687078476,1.0843296767510358e-06
65265,326212,0,326212,814.269366979599,1.0726561183002456e-06
65365,326712,0,326712,815.7760078907013,1.061095014062317e-06
65465,327212,0,327212,817.1639502048492,1.0496470246169862e-06
65566,327717,0,327717,818.5193231105804,1.0381999563225477e-06
65666,328217,0,328217,819.728935956955,1.0269847576143703e-06
65766,328717,0,328717,820.9627850055695,1.0158925689194452e-06
65866,329217,0,329217,822.1954131126404,1.0049259481510315e-06
65966,329717,0,329717,823.3959438800812,9.940855267346418e-07
66066,330217,0,330217,824.8061690330505,9.833719876582508e-07
66166,330717,0,330717,826.0516889095306,9.727880520583622e-07
66266,331217,0,331217,827.1310141086578,9.623374351265779e-07
66366,331717,0,331717,828.5359020233154,9.520207180885351e-07
66466,332217,0,332217,829.8170540332794,9.418336128162383e-07
66567,332722,0,332722,831.1911280155182,9.316700240749915e-07
66667,333222,0,333222,832.4936230182648,9.217271623936702e-07
66767,333722,0,333722,833.8469939231873,9.11900973918843e-07
66867,334222,0,334222,835.01664686203,9.021860095887457e-07
66967,334722,0,334722,836.3188381195068,8.925742305820325e-07
67067,335222,0,335222,837.9499042034149,8.830583492669215e-07
67167,335722,0,335722,839.3354511260986,8.736334425874546e-07
67267,336222,0,336222,840.7900710105896,8.642967840073961e-07
67367,336722,0,336722,842.2618980407715,8.550463039981891e-07
67467,337222,0,337222,843.6369421482086,8.458785940951659e-07
67568,337727,0,337727,844.939572095871,8.366993440625389e-07
67668,338227,0,338227,846.3133561611176,8.27688677308282e-07
67768,338727,0,338727,847.7448298931122,8.18755980318171e-07
67868,339227,0,339227,848.8757572174072,8.099026085895654e-07
67968,339727,0,339727,850.1825132369995,8.011302377917576e-07
68068,340227,0,340227,851.5032961368561,7.924414715768279e-07
68168,340727,0,340727,852.7664840221405,7.838404281018891e-07
68268,341227,0,341227,853.9650990962982,7.753324173023301e-07
68368,341727,0,341727,855.1945641040802,7.669213846430057e-07
68468,342227,0,342227,856.3974311351776,7.586078537484956e-07
68569,342732,0,342732,857.7091052532196,7.503095311112588e-07
68669,343232,0,343232,859.1275510787964,7.421920083133684e-07
68769,343732,0,343732,860.2548019886017,7.34174652470198e-07
68869,344232,0,344232,861.4629671573639,7.262580664381888e-07
68969,344732,0,344732,862.5710980892181,7.184413830674902e-07
69069,345232,0,345232,863.6713888645172,7.107234815614449e-07
69169,345732,0,345732,864.7739901542664,7.031041351747459e-07
69269,346232,0,346232,866.1137421131134,6.955832124596854e-07
69369,346732,0,346732,867.3621790409088,6.881590632382932e-07
69469,347232,0,347232,868.5072388648987,6.80828915953804e-07
69570,347737,0,347737,869.6841771602631,6.735181579151269e-07
69670,348237,0,348237,870.8883509635925,6.663685179595736e-07
69770,348737,0,348737,872.0507090091705,6.593027248894223e-07
69870,349237,0,349237,873.1298530101776,6.523151435487793e-07
69970,349737,0,349737,874.348197221756,6.454002002365713e-07
70070,350237,0,350237,875.5348181724548,6.385538337749787e-07
70170,350737,0,350737,876.8410220146179,6.317739874753919e-07
70270,351237,0,351237,878.1292741298676,6.250590924957788e-07
70370,351737,0,351737,879.5745780467987,6.18406469376686e-07
70470,352237,0,352237,880.8100821971893,6.118130803177087e-07
70571,352742,0,352742,881.9977641105652,6.052126087688966e-07
70671,353242,0,353242,883.3625910282135,5.987371272322172e-07
70771,353742,0,353742,884.7426512241364,5.923232533738532e-07
70871,354242,0,354242,886.0685188770294,5.859719379929252e-07
70971,354742,0,354742,887.6396610736847,5.79682969630108e-07
71071,355242,0,355242,888.7544991970062,5.734572256210388e-07
71171,355742,0,355742,889.9984481334686,5.672980778254223e-07
71271,356242,0,356242,891.528430223465,5.612100452919797e-07
71371,356742,0,356742,892.8338010311127,5.551961002915604e-07
71471,357242,0,357242,894.2078430652618,5.492566417481415e-07
71572,357747,0,357747,895.3448770046234,5.433325783386095e-07
71672,358247,0,358247,896.5125141143799,5.375405726517072e-07
71772,358747,0,358747,897.6940412521362,5.31820978206146e-07
71872,359247,0,359247,898.8109750747681,5.261721461709098e-07
71972,359747,0,359747,899.946475982666,5.205905248497584e-07
72072,360247,0,360247,901.1907262802124,5.150714020625476e-07
72172,360747,0,360747,902.3855590820312,5.096110004691253e-07
72272,361247,0,361247,903.6012489795685,5.042072646492409e-07
72372,361747,0,361747,904.9967851638794,4.988586021967168e-07
72472,362247,0,362247,906.4272162914276,4.935628346604749e-07
72573,362752,0,362752,907.6680572032928,4.882654528657139e-07
72673,363252,0,363252,909.1285061836243,4.830696874710901e-07
72773,363752,0,363752,910.2853510379791,4.779217151643314e-07
72873,364252,0,364252,911.7562811374664,4.7282023909427746e-07
72973,364752,0,364752,913.8338840007782,4.677634359780377e-07
73073,365252,0,365252,915.5222232341766,4.6274950986825224e-07
73173,365752,0,365752,917.3557231426239,4.5777760280808976e-07
73273,366252,0,366252,919.2206149101257,4.5284780451463425e-07
73373,366752,0,366752,920.8000400066376,4.4796048281614885e-07
73473,367252,0,367252,922.6352829933167,4.431161211775417e-07
73574,367757,0,367757,924.2834870815277,4.382679443680102e-07
73674,368257,0,368257,925.9735641479492,4.335138917638465e-07
73774,368757,0,368757,927.7830860614777,4.28808411545749e-07
73874,369257,0,369257,929.2755930423737,4.241540818848665e-07
73974,369757,0,369757,931.1942729949951,4.1955297033080294e-07
74074,370257,0,370257,932.6176381111145,4.1500699046842446e-07
74174,370757,0,370757,933.995364189148,4.1051775539140377e-07
74274,371257,0,371257,935.3330659866333,4.0608577355642756e-07
74374,371757,0,371757,936.7164940834045,4.0171017541439516e-07
74474,372257,0,372257,938.1453161239624,3.97389361630678e-07
74575,372762,0,372762,939.5851151943207,3.930795785906087e-07
74675,373262,0,373262,941.2376089096069,3.8886555044741166e-07
74775,373762,0,373762,942.7373330593109,3.847038269104982e-07
74875,374262,0,374262,944.8398399353027,3.805928897538682e-07
74975,374762,0,374762,946.4137001037598,3.765300579367665e-07
75075,375262,0,375262,947.932361125946,3.7251254896109623e-07
75175,375762,0,375762,949.5506980419159,3.6853859679069454e-07
75275,376262,0,376262,950.8452560901642,3.6460725536611033e-07
75375,376762,0,376762,952.3972039222717,3.607170845970729e-07
75475,377262,0,377262,953.7450549602509,3.568654882258914e-07
75576,377767,0,377767,955.127965927124,3.5301169792769407e-07
75676,378267,0,378267,956.3969552516937,3.492306163246594e-07
75776,378767,0,378767,957.6851599216461,3.454842474717345e-07
75876,379267,0,379267,958.9495980739594,3.417733468821678e-07
75976,379767,0,379767,960.2265720367432,3.380977784564849e-07
76076,380267,0,380267,961.5105290412903,3.3445678396509216e-07
76176,380767,0,380767,962.7736341953278,3.308502241693137e-07
76276,381267,0,381267,964.0410890579224,3.2727904260973124e-07
76376,381767,0,381767,965.3070380687714,3.237445262706469e-07
76476,382267,0,382267,966.6593432426453,3.202473806887258e-07
76577,382772,0,382772,968.4219992160797,3.1675322385484505e-07
76677,383272,0,383272,969.8314712047577,3.1333142841406253e-07
76777,383772,0,383772,971.2163372039795,3.0994822648801524e-07
76877,384272,0,384272,972.6924481391907,3.066050600212221e-07
76977,384772,0,384772,974.1578528881073,3.0330295431052714e-07
77077,385272,0,385272,975.8345630168915,3.0004234658145314e-07
77177,385772,0,385772,977.39923620224,2.9682355758550837e-07
77277,386272,0,386272,979.0857059955597,2.936470343978693e-07
77377,386772,0,386772,980.7823450565338,2.90512900577482e-07
77477,387272,0,387272,982.5395820140839,2.874203035996396e-07
77578,387777,0,387777,984.6919181346893,2.8433710807050587e-07
77678,388277,0,388277,986.7006452083588,2.813223085813156e-07
77778,388777,0,388777,988.5044801235199,2.7834334007996905e-07
77878,389277,0,389277,989.9508941173553,2.753983415705869e-07
77978,389777,0,389777,991.5994391441345,2.724851945866657e-07
78078,390277,0,390277,993.3086750507355,2.69601786143182e-07
78178,390777,0,390777,994.9976019859314,2.667464765234163e-07
78278,391277,0,391277,996.9593873023987,2.6391813193734857e-07
78378,391777,0,391777,998.520268201828,2.6111566473942905e-07
78478,392277,0,392277,1000.2901840209961,2.58337802164423e-07
78579,392782,0,392782,1002.0880541801453,2.555561782408286e-07
78679,393282,0,393282,1003.7121760845184,2.528259361608583e-07
78779,393782,0,393782,1005.6193599700928,2.501203306519358e-07
78879,394282,0,394282,1007.3233091831207,2.474402599637395e-07
78979,394782,0,394782,1008.8062300682068,2.44786097395252e-07
79079,395282,0,395282,1010.2384760379791,2.4215808811323914e-07
79179,395782,0,395782,1011.660177230835,2.3955704003237335e-07
79279,396282,0,396282,1013.0586822032928,2.369843150730864e-07
79379,396782,0,396782,1014.4697642326355,2.3444098451284756e-07
79479,397282,0,397282,1015.9024691581726,2.319271164825373e-07
79580,397787,0,397787,1017.3222389221191,2.2941737371723322e-07
79680,398287,0,398287,1018.7383649349213,2.2696109624584757e-07
79780,398787,0,398787,1020.3676810264587,2.2453366048435663e-07
79880,399287,0,399287,1022.3726091384888,2.2213554443704942e-07
79980,399787,0,399787,1024.2603340148926,2.1976650649725233e-07
80080,400287,0,400287,1026.0705962181091,2.1742556138219275e-07
80180,400787,0,400787,1028.650446176529,2.151116692584531e-07
80280,401287,0,401287,1030.3638241291046,2.1282422158841604e-07
80380,401787,0,401787,1032.063333272934,2.105627699539956e-07
80480,402287,0,402287,1033.6501660346985,2.0832641849530947e-07
80581,402792,0,402792,1035.22500705719,2.0609165413513596e-07
80681,403292,0,403292,1036.8531498908997,2.0390105832040527e-07
80781,403792,0,403792,1038.736699104309,2.017310596775534e-07
80881,404292,0,404292,1040.3302111625671,1.9958071061103183e-07
80981,404792,0,404792,1041.9483880996704,1.974491858869539e-07
81081,405292,0,405292,1043.6014242172241,1.9533560406603796e-07
81181,405792,0,405792,1045.4311010837555,1.932391696408168e-07
81281,406292,0,406292,1047.0285680294037,1.9115949736179776e-07
81381,406792,0,406792,1048.5969669818878,1.8909673978364401e-07
81481,407292,0,407292,1050.1837491989136,1.8705140147130446e-07
81582,407797,0,407797,1051.805017232895,1.8500395611322046e-07
81682,408297,0,408297,1053.4021861553192,1.829957422257774e-07
81782,408797,0,408797,1054.9698412418365,1.8100733966442422e-07
81882,409297,0,409297,1056.5558788776398,1.7903970858366988e-07
81982,409797,0,409797,1058.1505391597748,1.7709361365501961e-07
82082,410297,0,410297,1059.7654480934143,1.7516956844360552e-07
82182,410797,0,410797,1061.3488171100616,1.732679994081638e-07
82282,411297,0,411297,1062.9395849704742,1.7138936428328358e-07
82382,411797,0,411797,1064.5247910022736,1.6953401577948357e-07
82482,412297,0,412297,1066.1033971309662,1.6770200626748427e-07
82583,412802,0,412802,1067.6997339725494,1.658751496211222e-07
82683,413302,0,413302,1069.290580034256,1.640893765127288e-07
82783,413802,0,413802,1070.8786671161652,1.6232634020806648e-07
82883,414302,0,414302,1072.4616770744324,1.605858293473245e-07
82983,414802,0,414802,1074.0512311458588,1.5886733224531213e-07
83083,415302,0,415302,1075.639983177185,1.571700695377117e-07
83183,415802,0,415802,1077.2212760448456,1.5549325045732196e-07
83283,416302,0,416302,1078.8043360710144,1.538361977149693e-07
83383,416802,0,416802,1080.4100461006165,1.5219817603018555e-07
83483,417302,0,417302,1082.0035572052002,1.5057818932078878e-07
83584,417807,0,417807,1083.5997860431671,1.489591377779871e-07
83684,418307,0,418307,1085.1817240715027,1.4737214785214525e-07
83784,418807,0,418807,1086.7700581550598,1.4580066753788848e-07
83884,419307,0,419307,1088.3592519760132,1.4424458891379322e-07
83984,419807,0,419807,1089.9345531463623,1.4270371127421584e-07
84084,420307,0,420307,1091.5313630104065,1.4117751928112094e-07
84184,420807,0,420807,1093.1178810596466,1.3966542322879032e-07
84284,421307,0,421307,1094.7311081886292,1.3816717373656054e-07
84384,421807,0,421807,1096.3240802288055,1.3668295928903521e-07
84484,422307,0,422307,1097.945808172226,1.352131078965057e-07
84585,422812,0,422812,1099.5643410682678,1.3374333530404756e-07
84685,423312,0,423312,1101.1429080963135,1.3230290905467397e-07
84785,423812,0,423812,1102.736577987671,1.3087764695245663e-07
84885,424312,0,424312,1104.4204270839691,1.2946836026184611e-07
84985,424812,0,424812,1106.1351101398468,1.280759217099276e-07
85085,425312,0,425312,1107.8310191631317,1.2670087325426363e-07
85185,425812,0,425812,1109.5269072055817,1.2534333765623355e-07
85285,426312,0,426312,1111.3066291809082,1.2400321172538125e-07
85385,426812,0,426812,1112.9040920734406,1.2268032333935662e-07
85485,427312,0,427312,1114.4855270385742,1.2137439402136777e-07
85586,427817,0,427817,1116.0740151405334,1.2007212121651653e-07
85686,428317,0,428317,1117.6682181358337,1.1879860492874518e-07
85786,428817,0,428817,1119.2727680206299,1.1754014370768598e-07
85886,429317,0,429317,1120.8516192436218,1.1629606350237402e-07
85986,429817,0,429817,1122.5073821544647,1.1506568257806039e-07
86086,430317,0,430317,1124.1513350009918,1.1384822756141683e-07
86186,430817,0,430817,1125.7959260940552,1.1264289975567055e-07
86286,431317,0,431317,1127.414796113968,1.1144904631032075e-07
86386,431817,0,431817,1128.9994912147522,1.1026622766645966e-07
86486,432317,0,432317,1130.621407032013,1.0909411811604476e-07
86587,432822,0,432822,1132.2306640148163,1.0792084519753453e-07
86687,433322,0,433322,1133.8134751319885,1.0676940440432179e-07
86787,433822,0,433822,1135.4172701835632,1.0562807228160408e-07
86887,434322,0,434322,1136.9975781440735,1.0449695369204678e-07
86987,434822,0,434822,1138.5855731964111,1.0337616993505784e-07
87087,435322,0,435322,1140.1556041240692,1.0226577602820133e-07
87187,435822,0,435822,1141.7396240234375,1.0116583872930589e-07
87287,436322,0,436322,1143.3182721138,1.0007656176555969e-07
87387,436822,0,436822,1144.9098958969116,9.899828792728952e-08
87487,437322,0,437322,1146.494590997696,9.79313684574609e-08
87588,437827,0,437827,1148.1045010089874,9.686557205223534e-08
87688,438327,0,438327,1149.68931722641,9.582223633488851e-08
87788,438827,0,438827,1151.2641341686249,9.479106385389852e-08
87888,439327,0,439327,1152.8641331195831,9.37724231224351e-08
87988,439827,0,439827,1154.457337141037,9.276654578127547e-08
88088,440327,0,440327,1156.0410749912262,9.177336598869574e-08
88188,440827,0,440827,1157.6006231307983,9.079255908547777e-08
88288,441327,0,441327,1159.1943318843842,8.982371127793521e-08
88388,441827,0,441827,1160.7793788909912,8.886641747962162e-08
88488,442327,0,442327,1162.3613948822021,8.792022357791811e-08
88589,442832,0,442832,1163.951495885849,8.697523106061668e-08
88689,443332,0,443332,1165.5525150299072,8.604946233965795e-08
88789,443832,0,443832,1167.132344007492,8.513290304670765e-08
88889,444332,0,444332,1168.6859872341156,8.422513737655318e-08
88989,444832,0,444832,1170.306384086609,8.33258908517979e-08
89089,445332,0,445332,1172.1851279735565,8.243490841931046e-08
89189,445832,0,445832,1173.7761180400848,8.155190875416452e-08
89289,446332,0,446332,1175.3497650623322,8.067664487432395e-08
89389,446832,0,446832,1176.9403901100159,7.980898052170264e-08
89489,447332,0,447332,1178.527932882309,7.89489005210313e-08
89590,447837,0,447837,1180.1413979530334,7.808798205228035e-08
89690,448337,0,448337,1181.742887020111,7.724338356573574e-08
89790,448837,0,448837,1183.330794095993,7.640670443715367e-08
89890,449337,0,449337,1184.9271869659424,7.557815897630344e-08
89990,449837,0,449837,1186.5108571052551,7.475798541877854e-08
90090,450337,0,450337,1188.0815312862396,7.394641513045673e-08
90190,450837,0,450837,1189.667550086975,7.314366529759329e-08
90290,451337,0,451337,1191.261766910553,7.234994511926245e-08
90390,451837,0,451837,1192.8410739898682,7.156545233708477e-08
90490,452337,0,452337,1194.432615995407,7.07903512866788e-08
90591,452842,0,452842,1196.0304062366486,7.001714492380071e-08
90691,453342,0,453342,1197.6096460819244,6.926120834847599e-08
90791,453842,0,453842,1199.1888101100922,6.851487782755482e-08
90891,454342,0,454342,1200.784882068634,6.777816971003707e-08
90991,454842,0,454842,1202.3526380062103,6.705103970488444e-08
91091,455342,0,455342,1203.914447069168,6.633334226418673e-08
91191,455842,0,455842,1205.4939231872559,6.562483866422212e-08
91291,456342,0,456342,1207.077977180481,6.49252524811353e-08
91391,456842,0,456842,1208.666519165039,6.42343104866385e-08
91491,457342,0,457342,1210.2492291927338,6.355172145956567e-08
91592,457847,0,457847,1211.8372721672058,6.287041737365335e-08
91692,458347,0,458347,1213.4085400104523,6.220344669719794e-08
91792,458847,0,458847,1214.989984035492,6.154356253289933e-08
91892,459347,0,459347,1216.551996231079,6.089033949338582e-08
91992,459847,0,459847,1218.1395750045776,6.024340524160767e-08
92092,460347,0,460347,1219.718641281128,5.9602437652332105e-08
92192,460847,0,460847,1221.3043801784515,5.8967191993712113e-08
92292,461347,0,461347,1222.8735330104828,5.833755447657805e-08
92392,461847,0,461847,1224.4757282733917,5.771356289967479e-08
92492,462347,0,462347,1226.057590007782,5.709535845468965e-08
92593,462852,0,462852,1227.6372311115265,5.6477015936762434e-08
92693,463352,0,463352,1229.2176880836487,5.5870934565764556e-08
92793,463852,0,463852,1230.8034081459045,5.5271121619224754e-08
92893,464352,0,464352,1232.4111471176147,5.467776851502992e-08
92993,464852,0,464852,1233.9784710407257,5.409107684263335e-08
93093,465352,0,465352,1235.5743391513824,5.3511198524894656e-08
93193,465852,0,465852,1237.1547572612762,5.2938198200698075e-08
93293,466352,0,466352,1238.7348201274872,5.237207621662884e-08
93393,466852,0,466852,1240.3060281276703,5.181281910158578e-08
93493,467352,0,467352,1241.8969662189484,5.126041202478091e-08
93594,467857,0,467857,1243.493881225586,5.070937672949822e-08
93694,468357,0,468357,1245.0592849254608,5.01704836030814e-08
93794,468857,0,468857,1246.6399500370026,4.9638021400772925e-08
93894,469357,0,469357,1248.2302031517029,4.9111728970494083e-08
93994,469857,0,469857,1249.8091831207275,4.85913450270099e-08
94094,470357,0,470357,1251.3814179897308,4.807661898807941e-08
94194,470857,0,470857,1252.9555351734161,4.756730471856346e-08
94294,471357,0,471357,1254.5765330791473,4.7063158869899435e-08
94394,471857,0,471857,1256.1558530330658,4.6563946765815976e-08
94494,472357,0,472357,1257.7291841506958,4.606944630958849e-08
94595,472862,0,472862,1259.3346712589264,4.557457024401372e-08
94695,473362,0,473362,1260.9222321510315,4.508892520046027e-08
94795,473862,0,473862,1262.4950630664825,4.4607430812461174e-08
94895,474362,0,474362,1264.0768041610718,4.412997718660471e-08
94995,474862,0,474862,1265.6605050563812,4.365650664513423e-08
95095,475362,0,475362,1267.470115184784,4.318700574747207e-08
95195,475862,0,475862,1269.1050810813904,4.272150611444266e-08
95295,476362,0,476362,1270.6918790340424,4.226010616267049e-08
95395,476862,0,476862,1272.2772579193115,4.1802989731364147e-08
95495,477362,0,477362,1273.8635420799255,4.135040698391273e-08
95596,477867,0,477867,1275.4421200752258,4.089816700860786e-08
95696,478367,0,478367,1277.0229880809784,4.0455448953385145e-08
95796,478867,0,478867,1278.6083211898804,4.001791203536293e-08
95896,479367,0,479367,1280.1899890899658,3.958565578190874e-08
95996,479867,0,479867,1281.7630190849304,3.9158716211616864e-08
96096,480367,0,480367,1283.3571269512177,3.87370660156384e-08
96196,480867,0,480867,1284.9581551551819,3.83206289114138e-08
96296,481367,0,481367,1286.5195109844208,3.790930486674825e-08
96396,481867,0,481867,1288.145518064499,3.750298885396706e-08
96496,482367,0,482367,1289.7459170818329,3.7101572269938415e-08
96597,482872,0,482872,1291.430762052536,3.670099122870077e-08
96697,483372,0,483372,1293.0140390396118,3.6309036831582725e-08
96797,483872,0,483872,1294.6020259857178,3.5921561709229526e-08
96897,484372,0,484372,1296.1947910785675,3.553839422848413e-08
96997,484872,0,484872,1297.7837541103363,3.5159347923588836e-08
97097,485372,0,485372,1299.3578329086304,3.4784222109441415e-08
97197,485872,0,485872,1300.9443500041962,3.441281657496174e-08
97297,486372,0,486372,1302.52738904953,3.4044959312246065e-08
97397,486872,0,486872,1304.0981419086456,3.368052747784616e-08
97497,487372,0,487372,1305.6792619228363,3.331944530141719e-08
97598,487877,0,487877,1307.2851340770721,3.295810436247961e-08
97698,488377,0,488377,1308.8756980895996,3.2603627596715596e-08
97798,488877,0,488877,1310.4458711147308,3.2252406392916555e-08
97898,489377,0,489377,1312.035521030426,3.1904452685634734e-08
97998,489877,0,489877,1313.6236779689789,3.1559805654004965e-08
98098,490377,0,490377,1315.2228360176086,3.121852230611505e-08
98198,490877,0,490877,1316.797294139862,3.0880668825624187e-08
98298,491377,0,491377,1318.3908851146698,3.054631967917101e-08
98398,491877,0,491877,1319.9855270385742,3.021555948709407e-08
98498,492377,0,492377,1321.5605518817902,2.9888480738356374e-08
98599,492882,0,492882,1323.153531074524,2.9561964792174407e-08
98699,493382,0,493382,1324.730191230774,2.9242572997470586e-08
98799,493882,0,493882,1326.3234610557556,2.892714749025802e-08
98899,494382,0,494382,1327.8999559879303,2.8615771893396364e-08
98999,494882,0,494882,1329.4905610084534,2.83084972401931e-08
99099,495382,0,495382,1331.0588071346283,2.8005320775437747e-08
99199,495882,0,495882,1332.6506271362305,2.770618214474585e-08
99299,496382,0,496382,1334.2306282520294,2.7410975683418705e-08
99399,496882,0,496882,1335.7188980579376,2.7119562772877072e-08
99499,497382,0,497382,1337.20174908638,2.683177513919919e-08
99600,497887,0,497887,1338.9910521507263,2.654458979816938e-08
99700,498387,0,498387,1340.5689561367035,2.6263480033161935e-08
99800,498887,0,498887,1342.2582149505615,2.598538006390332e-08
99900,499387,0,499387,1343.8986320495605,2.5710111389207502e-08
100000,499887,0,499887,1345.763931274414,2.543753277181282e-08


==> plot_data/quadratic_minimax_problem_n500_alpha00001/flex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.002183198928833008,30.358106049564984
81,243,0,243,1.5511021614074707,0.3480833949950039
161,483,0,483,2.8602840900421143,0.1404995373723559
242,726,0,726,4.128584146499634,0.0657505266695044
323,969,0,969,5.4588141441345215,0.047872603732171684
404,1212,0,1212,6.717121124267578,0.040075349061280297
484,1452,0,1452,7.978608131408691,0.0349076173897176
565,1695,0,1695,9.15440320968628,0.027651117536782024
646,1938,0,1938,10.332130193710327,0.025409925734020556
726,2178,0,2178,11.478452205657959,0.0231275888349837
807,2421,0,2421,12.613002300262451,0.020163481540391753
888,2664,0,2664,13.759902238845825,0.0175729995196827
969,2907,0,2907,14.921958208084106,0.016525311952617056
1049,3147,0,3147,16.04424023628235,0.015535577115170254
1130,3390,0,3390,17.195394039154053,0.014592647167650692
1211,3633,0,3633,18.31826615333557,0.013980455794172727
1291,3873,0,3873,19.430898189544678,0.013197949521073149
1372,4116,0,4116,20.578806161880493,0.01176124001048875
1453,4359,0,4359,21.75723624229431,0.009922311591465031
1534,4602,0,4602,22.946632146835327,0.008414422846928291
1614,4842,0,4842,24.036660194396973,0.007605961060768524
1695,5085,0,5085,25.139055252075195,0.006937635577089381
1776,5328,0,5328,26.222589254379272,0.006305743416037854
1856,5568,0,5568,27.313225269317627,0.0058652162185436904
1937,5811,0,5811,28.428125143051147,0.0054911984702519295
2018,6054,0,6054,29.530946016311646,0.005194270247685958
2099,6297,0,6297,30.631890296936035,0.0049487176596587
2179,6537,0,6537,31.722941160202026,0.00475622538625983
2260,6780,0,6780,32.82115316390991,0.00430966740160458
2341,7023,0,7023,33.96980619430542,0.0037520236708764127
2421,7263,0,7263,35.05737614631653,0.0034737644520284163
2502,7506,0,7506,36.16252899169922,0.0033426259493403603
2583,7749,0,7749,37.258249282836914,0.0032097501407459526
2664,7992,0,7992,38.362269163131714,0.0030874382573407373
2744,8232,0,8232,39.528802156448364,0.0029493325518515677
2825,8475,0,8475,40.66103219985962,0.0028080108482399554
2906,8718,0,8718,41.77852511405945,0.0027087765236887096
2986,8958,0,8958,42.87853527069092,0.0026184777362827836
3067,9201,0,9201,43.98224925994873,0.002551425503315686
3148,9444,0,9444,45.102431297302246,0.0024903413663226
3229,9687,0,9687,46.20412635803223,0.0024307605944403916
3309,9927,0,9927,47.307706117630005,0.002340125866489356
3390,10170,0,10170,48.506089210510254,0.0022070913495341364
3471,10413,0,10413,49.713144063949585,0.0021438371877831697
3551,10653,0,10653,50.81929922103882,0.0020936678965963827
3632,10896,0,10896,51.95348310470581,0.002042137449285472
3713,11139,0,11139,53.07148814201355,0.0019933598396542664
3794,11382,0,11382,54.21267032623291,0.0019348643384052891
3874,11622,0,11622,55.31523609161377,0.0018941166766654426
3955,11865,0,11865,56.447652101516724,0.0018347022448073828
4036,12108,0,12108,57.58098316192627,0.0017933055308741582
4117,12351,0,12351,58.70805907249451,0.0017525719468298665
4197,12591,0,12591,59.803715229034424,0.001692363084264814
4278,12834,0,12834,60.954116106033325,0.0016194349172522523
4359,13077,0,13077,62.0742461681366,0.0015844956675461694
4439,13317,0,13317,63.18284225463867,0.0015493031402927574
4520,13560,0,13560,64.3548800945282,0.0015067512068902128
4601,13803,0,13803,65.49377822875977,0.001479513069900397
4682,14046,0,14046,66.62090802192688,0.0014514051485658693
4762,14286,0,14286,67.71512699127197,0.0014172538953305632
4843,14529,0,14529,68.82560110092163,0.0013888605372912133
4924,14772,0,14772,69.927894115448,0.0013649907855192208
5004,15012,0,15012,71.07868218421936,0.0013329083575399142
5085,15255,0,15255,72.19899916648865,0.001287879628891363
5166,15498,0,15498,73.31371426582336,0.0012620309310185413
5247,15741,0,15741,74.43545126914978,0.0012406644968982114
5327,15981,0,15981,75.54670214653015,0.0012154280546489821
5408,16224,0,16224,76.70524525642395,0.0011939858625329626
5489,16467,0,16467,77.85846495628357,0.0011791180555029237
5569,16707,0,16707,79.17857813835144,0.0011646149078970568
5650,16950,0,16950,80.61054825782776,0.0011475629474139754
5731,17193,0,17193,81.73575806617737,0.0011244273343234315
5812,17436,0,17436,82.85056710243225,0.0011050408593391368
5892,17676,0,17676,83.98881506919861,0.0010909641582438373
5973,17919,0,17919,85.07292795181274,0.0010764608033646654
6054,18162,0,18162,86.10837602615356,0.0010593142855032129
6134,18402,0,18402,87.19927906990051,0.001046074730011907
6215,18645,0,18645,88.2378671169281,0.0010319213713828154
6296,18888,0,18888,89.40985321998596,0.001016436659764876
6377,19131,0,19131,90.4904272556305,0.0010024952711078503
6457,19371,0,19371,91.51207327842712,0.0009902603524803153
6538,19614,0,19614,92.5363540649414,0.000978603307830104
6619,19857,0,19857,93.5622010231018,0.0009653271236132528
6699,20097,0,20097,94.55389428138733,0.0009542165888680154
6780,20340,0,20340,95.64333629608154,0.0009418272319643379
6861,20583,0,20583,96.693115234375,0.0009283668819297392
6942,20826,0,20826,97.79451632499695,0.0009179293019847279
7022,21066,0,21066,98.83344316482544,0.0009062454956422808
7103,21309,0,21309,99.86559319496155,0.0008933913286452246
7184,21552,0,21552,101.05973720550537,0.0008831299576373038
7264,21792,0,21792,102.25181913375854,0.0008732393841611175
7345,22035,0,22035,103.34003520011902,0.0008630413507915407
7426,22278,0,22278,104.39491128921509,0.000852657788352591
7507,22521,0,22521,105.4545750617981,0.000842431876865029
7587,22761,0,22761,106.51916217803955,0.0008324927626706043
7668,23004,0,23004,107.63288521766663,0.0008205478420038041
7749,23247,0,23247,108.7430510520935,0.0008107502036878812
7829,23487,0,23487,109.81752228736877,0.0008014040290956084
7910,23730,0,23730,110.85525417327881,0.0007923219829443787
7991,23973,0,23973,111.92157816886902,0.0007819872876492861
8072,24216,0,24216,113.03729104995728,0.0007715269636013926
8152,24456,0,24456,114.12199330329895,0.0007629054157914433
8233,24699,0,24699,115.30718612670898,0.000753605057822457
8314,24942,0,24942,116.43123316764832,0.0007434144871642799
8394,25182,0,25182,117.53237724304199,0.0007341388558184425
8475,25425,0,25425,118.63340210914612,0.0007255801754850654
8556,25668,0,25668,119.76549124717712,0.0007169783373218987
8637,25911,0,25911,120.86697006225586,0.0007076856209678048
8717,26151,0,26151,122.00175523757935,0.0006967875219464598
8798,26394,0,26394,123.0933129787445,0.0006864184852366698
8879,26637,0,26637,124.25888299942017,0.0006774085551221286
8959,26877,0,26877,125.35234093666077,0.0006691258840228312
9040,27120,0,27120,126.51745915412903,0.0006563078502706747
9121,27363,0,27363,127.66072916984558,0.0006360079096048793
9202,27606,0,27606,128.7800953388214,0.0006236128457970461
9282,27846,0,27846,129.799574136734,0.0006156028827488595
9363,28089,0,28089,130.83956813812256,0.0006086584416160589
9444,28332,0,28332,131.88965511322021,0.0006019502883541746
9524,28572,0,28572,132.93441820144653,0.000595437722671563
9605,28815,0,28815,133.97568321228027,0.0005880241250489464
9686,29058,0,29058,135.04152011871338,0.0005789848691005312
9767,29301,0,29301,136.0813512802124,0.0005699611163116421
9847,29541,0,29541,137.12313604354858,0.000563476868005442
9928,29784,0,29784,138.169753074646,0.0005566992028133563
10009,30027,0,30027,139.2357861995697,0.000549361208313688
10089,30267,0,30267,140.2457892894745,0.0005389991292516782
10170,30510,0,30510,141.28163027763367,0.0005311179557140108
10251,30753,0,30753,142.32065200805664,0.0005246627503710169
10332,30996,0,30996,143.35987210273743,0.0005187066290061334
10412,31236,0,31236,144.3734781742096,0.0005129441058615777
10493,31479,0,31479,145.4150640964508,0.0005069189540784983
10574,31722,0,31722,146.44230604171753,0.000500557188628404
10654,31962,0,31962,147.4693250656128,0.000494321487813889
10735,32205,0,32205,148.49873614311218,0.0004871345955917951
10816,32448,0,32448,149.54499912261963,0.0004809525501577373
10897,32691,0,32691,150.57236409187317,0.0004724174831837188
10977,32931,0,32931,151.57052206993103,0.0004650943285123979
11058,33174,0,33174,152.60595726966858,0.0004596190610330869
11139,33417,0,33417,153.62273812294006,0.0004538377614646511
11219,33657,0,33657,154.63517832756042,0.0004480610509165946
11300,33900,0,33900,155.66501235961914,0.00044262094766303145
11381,34143,0,34143,156.70185232162476,0.00043738163372860245
11462,34386,0,34386,157.70102906227112,0.0004322526714794509
11542,34626,0,34626,158.71261310577393,0.0004270684125982953
11623,34869,0,34869,159.7472870349884,0.00042198749392822257
11704,35112,0,35112,160.7873411178589,0.0004170153266451099
11784,35352,0,35352,161.80606508255005,0.0004121512550797726
11865,35595,0,35595,162.867445230484,0.00040459431522320353
11946,35838,0,35838,163.90884518623352,0.00039483475750917246
12027,36081,0,36081,164.9715051651001,0.0003898953417790388
12107,36321,0,36321,165.98597121238708,0.0003852391753859573
12188,36564,0,36564,166.9994490146637,0.0003808049197300928
12269,36807,0,36807,168.19934821128845,0.00037618283544764474
12350,37050,0,37050,169.23240613937378,0.0003711538071010317
12430,37290,0,37290,170.2794930934906,0.00036634773908470765
12511,37533,0,37533,171.32184720039368,0.0003613622473801487
12592,37776,0,37776,172.5373091697693,0.00035581963717513937
12672,38016,0,38016,174.19309425354004,0.00035152571980898335
12753,38259,0,38259,175.5674023628235,0.0003473956500269698
12834,38502,0,38502,176.6374740600586,0.00034325282691448366
12915,38745,0,38745,177.659850358963,0.0003391186427016064
12995,38985,0,38985,178.6923942565918,0.0003352556959642115
13076,39228,0,39228,179.69052124023438,0.000331361757590497
13157,39471,0,39471,180.6965880393982,0.0003273418136440311
13237,39711,0,39711,181.7023961544037,0.0003236567029578451
13318,39954,0,39954,182.71415495872498,0.00031991290125473897
13399,40197,0,40197,183.73569202423096,0.0003162992426817924
13480,40440,0,40440,184.85821723937988,0.00031258998694652743
13560,40680,0,40680,185.94151496887207,0.0003089953941341313
13641,40923,0,40923,187.13082909584045,0.00030505235181169706
13722,41166,0,41166,188.18464732170105,0.0003009121339056543
13802,41406,0,41406,189.19853115081787,0.0002970371314844219
13883,41649,0,41649,190.31761026382446,0.00029351706635609415
13964,41892,0,41892,191.35679006576538,0.0002901038402527842
14045,42135,0,42135,192.38454604148865,0.000286316192439031
14125,42375,0,42375,193.3949031829834,0.0002812103707274026
14206,42618,0,42618,194.39420533180237,0.00027438895396675013
14287,42861,0,42861,195.4131100177765,0.0002698194946365138
14367,43101,0,43101,196.40215921401978,0.0002645065976453638
14448,43344,0,43344,197.40798616409302,0.0002565766411141783
14529,43587,0,43587,198.41477513313293,0.0002523658368973472
14610,43830,0,43830,199.41171026229858,0.0002492435430270792
14690,44070,0,44070,200.41243529319763,0.00024616974378079246
14771,44313,0,44313,201.41702127456665,0.0002433569783411979
14852,44556,0,44556,202.46815609931946,0.00024064972695210404
14932,44796,0,44796,203.46481728553772,0.0002378600725601445
15013,45039,0,45039,204.47644329071045,0.00023495222214183845
15094,45282,0,45282,205.4812400341034,0.0002318830676390698
15175,45525,0,45525,206.49949622154236,0.00022853534919956196
15255,45765,0,45765,207.51059412956238,0.00022572032577562238
15336,46008,0,46008,208.57741832733154,0.00022325248879972445
15417,46251,0,46251,209.5733962059021,0.00022081785397212616
15497,46491,0,46491,210.562509059906,0.0002184259510267074
15578,46734,0,46734,211.55107712745667,0.0002159613382976906
15659,46977,0,46977,212.54403519630432,0.0002133262531584226
15740,47220,0,47220,213.53955912590027,0.00021083353443803428
15820,47460,0,47460,214.51433801651,0.00020853210428045096
15901,47703,0,47703,215.53128910064697,0.00020587175692144647
15982,47946,0,47946,216.5468032360077,0.00020294551722523085
16062,48186,0,48186,217.5576560497284,0.00020066383758018952
16143,48429,0,48429,218.58622312545776,0.00019820749834460912
16224,48672,0,48672,219.63318514823914,0.00019519955053906438
16305,48915,0,48915,220.63932418823242,0.00019276478795614418
16385,49155,0,49155,221.63673210144043,0.00019033882298879974
16466,49398,0,49398,222.63009214401245,0.0001881164406934317
16547,49641,0,49641,223.6370050907135,0.0001859763901271092
16627,49881,0,49881,224.62501502037048,0.00018388594167621057
16708,50124,0,50124,225.6299183368683,0.00018165638644415357
16789,50367,0,50367,226.63575720787048,0.00017885793680569236
16870,50610,0,50610,227.64129114151,0.00017556143848836855
16950,50850,0,50850,228.62742400169373,0.00017331529282015853
17031,51093,0,51093,229.62489128112793,0.00017117557187565526
17112,51336,0,51336,230.6423442363739,0.00016906705749047786
17192,51576,0,51576,231.61991715431213,0.00016693615311487708
17273,51819,0,51819,232.6099100112915,0.00016494175197668702
17354,52062,0,52062,233.59377312660217,0.0001630802083147647
17435,52305,0,52305,234.61081910133362,0.00016106438893092944
17515,52545,0,52545,235.59733605384827,0.00015920823715108703
17596,52788,0,52788,236.621502161026,0.0001573198240797075
17677,53031,0,53031,237.64499020576477,0.0001553698787248588
17757,53271,0,53271,238.63878393173218,0.00015348496679289152
17838,53514,0,53514,239.6476480960846,0.00015130682657987297
17919,53757,0,53757,240.64684534072876,0.00014769479201195968
18000,54000,0,54000,241.65408301353455,0.0001440894166964002
18080,54240,0,54240,242.65068221092224,0.00014204715164550937
18161,54483,0,54483,243.67315196990967,0.00014015644186687447
18242,54726,0,54726,244.6621961593628,0.00013843070752574994
18322,54966,0,54966,245.65150833129883,0.0001368689682768621
18403,55209,0,55209,246.6627161502838,0.0001352858688683965
18484,55452,0,55452,247.67483806610107,0.00013376239237667474
18565,55695,0,55695,248.6858789920807,0.00013222428960784325
18645,55935,0,55935,249.6871359348297,0.00013058945285524508
18726,56178,0,56178,250.66064715385437,0.00012900180809092665
18807,56421,0,56421,251.6620500087738,0.000127487221399713
18887,56661,0,56661,252.6582682132721,0.00012582842172339603
18968,56904,0,56904,253.65658521652222,0.00012429743170148822
19049,57147,0,57147,254.6764793395996,0.00012276416402801405
19130,57390,0,57390,255.6793510913849,0.00012059262508771417
19210,57630,0,57630,256.6831040382385,0.00011873127393593348
19291,57873,0,57873,257.69016909599304,0.00011715380222171674
19372,58116,0,58116,258.70229291915894,0.00011562619806928655
19452,58356,0,58356,259.7204101085663,0.00011427699908216215
19533,58599,0,58599,260.7401351928711,0.00011290318341274583
19614,58842,0,58842,261.7422614097595,0.00011157694985924556
19695,59085,0,59085,262.7472622394562,0.00011019848183511988
19775,59325,0,59325,263.738801240921,0.00010893736381904522
19856,59568,0,59568,264.738893032074,0.00010769228280468276
19937,59811,0,59811,265.7466821670532,0.00010643963068289392
20017,60051,0,60051,266.73356008529663,0.0001052417436760213
20098,60294,0,60294,267.7583432197571,0.00010400426853815942
20179,60537,0,60537,268.7591972351074,0.00010270571771308619
20260,60780,0,60780,269.7559931278229,0.000101453774232364
20340,61020,0,61020,270.72467017173767,0.00010013113492921062
20421,61263,0,61263,271.7163722515106,9.884687866337915e-05
20502,61506,0,61506,272.7210052013397,9.765142930127606e-05
20583,61749,0,61749,273.72799921035767,9.652200986396901e-05
20663,61989,0,61989,274.71843123435974,9.543741294682565e-05
20744,62232,0,62232,275.73053908348083,9.436679898310941e-05
20825,62475,0,62475,276.7325723171234,9.326272625436728e-05
20905,62715,0,62715,277.7238802909851,9.221343484757358e-05
20986,62958,0,62958,278.7429041862488,9.115338343630033e-05
21067,63201,0,63201,279.7533302307129,9.010513041497147e-05
21148,63444,0,63444,280.7482521533966,8.896593034037422e-05
21228,63684,0,63684,281.73161005973816,8.794131308085983e-05
21309,63927,0,63927,282.74293303489685,8.690321942002466e-05
21390,64170,0,64170,283.7485980987549,8.584858676211071e-05
21470,64410,0,64410,284.72904419898987,8.486354484163871e-05
21551,64653,0,64653,285.7178521156311,8.384445923772092e-05
21632,64896,0,64896,286.7209703922272,8.286669231782388e-05
21713,65139,0,65139,287.72909212112427,8.175152566669745e-05
21793,65379,0,65379,288.7223081588745,8.08099343620428e-05
21874,65622,0,65622,289.7378532886505,7.983613033651663e-05
21955,65865,0,65865,290.73622703552246,7.882327023134608e-05
22035,66105,0,66105,291.7217471599579,7.79210800748475e-05
22116,66348,0,66348,292.7185592651367,7.688894236694817e-05
22197,66591,0,66591,293.7129020690918,7.580312029928105e-05
22278,66834,0,66834,294.7150902748108,7.474882939542122e-05
22358,67074,0,67074,295.71956610679626,7.368447894603685e-05
22439,67317,0,67317,296.70524525642395,7.273540722686048e-05
22520,67560,0,67560,297.72329211235046,7.19117932111266e-05
22600,67800,0,67800,298.69623708724976,7.109332093593545e-05
22681,68043,0,68043,299.69451427459717,7.02210764796654e-05
22762,68286,0,68286,300.6804132461548,6.935403462450602e-05
22843,68529,0,68529,301.73746514320374,6.855452752846548e-05
22923,68769,0,68769,303.03819012641907,6.764574250161276e-05
23004,69012,0,69012,304.28361535072327,6.684309292097991e-05
23085,69255,0,69255,305.29205226898193,6.60367468970667e-05
23165,69495,0,69495,306.294575214386,6.528072078011078e-05
23246,69738,0,69738,307.29644322395325,6.450033463594196e-05
23327,69981,0,69981,308.3106791973114,6.366513487286744e-05
23408,70224,0,70224,309.67106914520264,6.28909739021375e-05
23488,70464,0,70464,310.87833428382874,6.217787765426251e-05
23569,70707,0,70707,312.07445216178894,6.131778474558084e-05
23650,70950,0,70950,313.25587129592896,6.052421693301976e-05
23730,71190,0,71190,314.3217062950134,5.9836603184543235e-05
23811,71433,0,71433,315.3923850059509,5.913060171143436e-05
23892,71676,0,71676,316.5373842716217,5.804925160000002e-05
23973,71919,0,71919,317.6277141571045,5.6626734482117294e-05
24053,72159,0,72159,318.6751160621643,5.577750301902754e-05
24134,72402,0,72402,319.6919243335724,5.483569275140096e-05
24215,72645,0,72645,320.6942801475525,5.393351487467421e-05
24295,72885,0,72885,321.69396018981934,5.326755589713977e-05
24376,73128,0,73128,322.7020699977875,5.261703233331714e-05
24457,73371,0,73371,323.7109181880951,5.195767573246348e-05
24538,73614,0,73614,324.7109582424164,5.1350832589576785e-05
24618,73854,0,73854,325.70325922966003,5.0761260851757245e-05
24699,74097,0,74097,326.70745611190796,5.0182901442732845e-05
24780,74340,0,74340,327.7100751399994,4.959823385494271e-05
24860,74580,0,74580,328.6913080215454,4.89249340572144e-05
24941,74823,0,74823,329.92508721351624,4.8288367492714105e-05
25022,75066,0,75066,331.0930211544037,4.773165700396556e-05
25103,75309,0,75309,332.1798713207245,4.718080259267982e-05
25183,75549,0,75549,333.3665962219238,4.6625177760142904e-05
25264,75792,0,75792,334.57836532592773,4.6067887889297795e-05
25345,76035,0,76035,335.58521604537964,4.545699846186177e-05
25425,76275,0,76275,336.6897542476654,4.490278357197959e-05
25506,76518,0,76518,337.75656509399414,4.435942823501054e-05
25587,76761,0,76761,338.80293226242065,4.384423437992647e-05
25668,77004,0,77004,339.87396121025085,4.3339895540573765e-05
25748,77244,0,77244,340.96864008903503,4.282730115696036e-05
25829,77487,0,77487,341.946475982666,4.2246794214487655e-05
25910,77730,0,77730,342.9587562084198,4.1745227028838506e-05
25990,77970,0,77970,343.9479591846466,4.126926077580295e-05
26071,78213,0,78213,344.92587208747864,4.077754377003677e-05
26152,78456,0,78456,346.0445611476898,4.026007059936987e-05
26233,78699,0,78699,347.12242126464844,3.9786469556692846e-05
26313,78939,0,78939,348.1221241950989,3.9341221188743484e-05
26394,79182,0,79182,349.2408859729767,3.888561477938234e-05
26475,79425,0,79425,350.2558183670044,3.842212777506334e-05
26555,79665,0,79665,351.3674931526184,3.798493575878026e-05
26636,79908,0,79908,352.44785714149475,3.750993664911282e-05
26717,80151,0,80151,353.46881914138794,3.706697913017369e-05
26798,80394,0,80394,354.4790372848511,3.662937575078214e-05
26878,80634,0,80634,355.5020351409912,3.617319235938368e-05
26959,80877,0,80877,356.6347529888153,3.5491025947757096e-05
27040,81120,0,81120,357.73149514198303,3.4951747630693016e-05
27120,81360,0,81360,358.7254741191864,3.452896759032316e-05
27201,81603,0,81603,359.72897720336914,3.4126156664960286e-05
27282,81846,0,81846,360.72215127944946,3.373644690337386e-05
27363,82089,0,82089,361.71445417404175,3.3309375571912514e-05
27443,82329,0,82329,362.70174622535706,3.289868780931361e-05
27524,82572,0,82572,363.7013213634491,3.2514000228160875e-05
27605,82815,0,82815,364.6896231174469,3.214111021901643e-05
27685,83055,0,83055,365.6794981956482,3.1788719351803576e-05
27766,83298,0,83298,366.68666315078735,3.1435471623784446e-05
27847,83541,0,83541,367.68260502815247,3.107662438464155e-05
27928,83784,0,83784,368.69050312042236,3.072865552686948e-05
28008,84024,0,84024,369.70672512054443,3.0371425966312114e-05
28089,84267,0,84267,370.70838022232056,3.0028480063761294e-05
28170,84510,0,84510,371.73922204971313,2.9680389177130735e-05
28251,84753,0,84753,372.74231910705566,2.9310600512236267e-05
28331,84993,0,84993,373.7961163520813,2.892946494695495e-05
28412,85236,0,85236,374.88393807411194,2.8600159630833536e-05
28493,85479,0,85479,376.0805969238281,2.8269741843215465e-05
28573,85719,0,85719,377.0465130805969,2.7905800327059594e-05
28654,85962,0,85962,378.19972825050354,2.7516827776140224e-05
28735,86205,0,86205,379.19451427459717,2.7147068279837557e-05
28816,86448,0,86448,380.319402217865,2.6724471411860252e-05
28896,86688,0,86688,381.405225276947,2.6364157950300775e-05
28977,86931,0,86931,382.47104716300964,2.6054803774373826e-05
29058,87174,0,87174,383.50255823135376,2.5713447092804537e-05
29138,87414,0,87414,384.49383330345154,2.539230328724914e-05
29219,87657,0,87657,385.4778561592102,2.507752513783104e-05
29300,87900,0,87900,386.4810471534729,2.4759487937193936e-05
29381,88143,0,88143,387.58067297935486,2.4382195385001114e-05
29461,88383,0,88383,388.58602023124695,2.4083819736067054e-05
29542,88626,0,88626,389.5854630470276,2.3783331904976318e-05
29623,88869,0,88869,390.5810480117798,2.3507866765853092e-05
29703,89109,0,89109,391.5706133842468,2.323306413788995e-05
29784,89352,0,89352,392.5705201625824,2.2962806365873374e-05
29865,89595,0,89595,393.5686902999878,2.268699826851181e-05
29946,89838,0,89838,394.53045296669006,2.2413484733804996e-05
30026,90078,0,90078,395.49812602996826,2.2152304709010987e-05
30107,90321,0,90321,396.4732060432434,2.184974996862894e-05
30188,90564,0,90564,397.46104526519775,2.1588154818590982e-05
30268,90804,0,90804,398.44334411621094,2.1313923877411837e-05
30349,91047,0,91047,399.4220151901245,2.1064409238123383e-05
30430,91290,0,91290,400.4154040813446,2.0820607422987357e-05
30511,91533,0,91533,401.40441608428955,2.056537502090521e-05
30591,91773,0,91773,402.3901810646057,2.0331487325499936e-05
30672,92016,0,92016,403.37318325042725,2.00896469477783e-05
30753,92259,0,92259,404.3657112121582,1.9830321492929204e-05
30833,92499,0,92499,405.332288980484,1.960268171194981e-05
30914,92742,0,92742,406.3223023414612,1.9358013675140125e-05
30995,92985,0,92985,407.3064031600952,1.9129679309168815e-05
31076,93228,0,93228,408.2994501590729,1.8864469590073645e-05
31156,93468,0,93468,409.27315306663513,1.8633055719927125e-05
31237,93711,0,93711,410.26085233688354,1.8397792556940768e-05
31318,93954,0,93954,411.25450325012207,1.8136441459436326e-05
31398,94194,0,94194,412.22276306152344,1.7922468355413082e-05
31479,94437,0,94437,413.22021412849426,1.7719455839225505e-05
31560,94680,0,94680,414.2051491737366,1.7497808917485034e-05
31641,94923,0,94923,415.20734310150146,1.729721390360899e-05
31721,95163,0,95163,416.17994117736816,1.7099901888310084e-05
31802,95406,0,95406,417.169291973114,1.6903944065220988e-05
31883,95649,0,95649,418.1574110984802,1.67055150923507e-05
31963,95889,0,95889,419.1426901817322,1.6509435010491178e-05
32044,96132,0,96132,420.1482172012329,1.6313702584413172e-05
32125,96375,0,96375,421.1392431259155,1.6108442439274954e-05
32206,96618,0,96618,422.1378049850464,1.5917947440241218e-05
32286,96858,0,96858,423.1086571216583,1.5718280786315898e-05
32367,97101,0,97101,424.106014251709,1.553754029472218e-05
32448,97344,0,97344,425.08945417404175,1.5358210560541707e-05
32528,97584,0,97584,426.0707960128784,1.5179370710831978e-05
32609,97827,0,97827,427.04850912094116,1.4996856546583724e-05
32690,98070,0,98070,428.04015827178955,1.4804636692068353e-05
32771,98313,0,98313,429.02504229545593,1.4632695414654816e-05
32851,98553,0,98553,429.9937391281128,1.4466080321907063e-05
32932,98796,0,98796,430.98203706741333,1.4297971562023328e-05
33013,99039,0,99039,431.96419501304626,1.4128421881986545e-05
33093,99279,0,99279,432.96157002449036,1.396300861817067e-05
33174,99522,0,99522,433.9469401836395,1.3803580728999722e-05
33255,99765,0,99765,434.9406931400299,1.3641305382086006e-05
33336,100008,0,100008,435.91919922828674,1.3486643919244949e-05
33416,100248,0,100248,436.90220618247986,1.333596704555e-05
33497,100491,0,100491,437.881019115448,1.3181252095529816e-05
33578,100734,0,100734,438.86767411231995,1.3034848709717255e-05
33658,100974,0,100974,439.8311142921448,1.2888583599515774e-05
33739,101217,0,101217,440.8067891597748,1.2741068092395331e-05
33820,101460,0,101460,441.79656434059143,1.25962045420259e-05
33901,101703,0,101703,442.77802634239197,1.2448407627698665e-05
33981,101943,0,101943,443.7732231616974,1.2297794034184826e-05
34062,102186,0,102186,444.7457482814789,1.214995088574474e-05
34143,102429,0,102429,445.738144159317,1.2012858770584548e-05
34223,102669,0,102669,446.70521116256714,1.1875434581513134e-05
34304,102912,0,102912,447.7086272239685,1.1721679148438922e-05
34385,103155,0,103155,448.73030614852905,1.1578691461957041e-05
34466,103398,0,103398,449.7541871070862,1.1444507159184726e-05
34546,103638,0,103638,450.7795560359955,1.1316756803044628e-05
34627,103881,0,103881,451.86549496650696,1.1187126772036785e-05
34708,104124,0,104124,452.916561126709,1.1060564422469409e-05
34788,104364,0,104364,453.96685004234314,1.0935796478948367e-05
34869,104607,0,104607,455.08161520957947,1.0810435346712288e-05
34950,104850,0,104850,456.3198971748352,1.066277604550648e-05
35031,105093,0,105093,457.3217830657959,1.0543031327776853e-05
35111,105333,0,105333,458.47629618644714,1.0426358078966089e-05
35192,105576,0,105576,459.47779512405396,1.030232311509309e-05
35273,105819,0,105819,460.57184624671936,1.017216764530965e-05
35353,106059,0,106059,461.6829752922058,1.003106833671925e-05
35434,106302,0,106302,462.7608313560486,9.912552580902047e-06
35515,106545,0,106545,463.8195900917053,9.789141025901564e-06
35596,106788,0,106788,464.90858125686646,9.659530913826953e-06
35676,107028,0,107028,465.9392640590668,9.546824278436659e-06
35757,107271,0,107271,467.15995812416077,9.42949094142981e-06
35838,107514,0,107514,468.28589820861816,9.30452537614298e-06
35918,107754,0,107754,469.32843017578125,9.198173784576179e-06
35999,107997,0,107997,470.3499183654785,9.089694468147069e-06
36080,108240,0,108240,471.3821151256561,8.982271140477139e-06
36161,108483,0,108483,472.59742307662964,8.877927029527435e-06
36241,108723,0,108723,473.57861328125,8.778312658028272e-06
36322,108966,0,108966,474.57728719711304,8.674768186915056e-06
36403,109209,0,109209,475.5578501224518,8.572784522253109e-06
36484,109452,0,109452,476.5504550933838,8.469096228245093e-06
36564,109692,0,109692,477.53798508644104,8.372800779324935e-06
36645,109935,0,109935,478.52973103523254,8.276328858712707e-06
36726,110178,0,110178,479.5154240131378,8.164936115686671e-06
36806,110418,0,110418,480.5014691352844,8.068857401124506e-06
36887,110661,0,110661,481.490825176239,7.971394181075959e-06
36968,110904,0,110904,482.49268221855164,7.878781279266806e-06
37049,111147,0,111147,483.4776861667633,7.790963084969156e-06
37129,111387,0,111387,484.46276807785034,7.69814058079229e-06
37210,111630,0,111630,485.44458413124084,7.603767493297982e-06
37291,111873,0,111873,486.4378023147583,7.516190630504553e-06
37371,112113,0,112113,487.4167082309723,7.4291088701261104e-06
37452,112356,0,112356,488.414626121521,7.330639606357164e-06
37533,112599,0,112599,489.4115061759949,7.243702494262601e-06
37614,112842,0,112842,490.39718413352966,7.16090653030799e-06
37694,113082,0,113082,491.3780152797699,7.0775820284440175e-06
37775,113325,0,113325,492.37753534317017,6.974460879413449e-06
37856,113568,0,113568,493.38250637054443,6.861737413431167e-06
37936,113808,0,113808,494.3638062477112,6.777370080906541e-06
38017,114051,0,114051,495.5393841266632,6.6925485694316516e-06
38098,114294,0,114294,496.62904596328735,6.604054151819736e-06
38179,114537,0,114537,497.76621317863464,6.525508454115682e-06
38259,114777,0,114777,498.72698616981506,6.451327240845057e-06
38340,115020,0,115020,499.7084562778473,6.374536659661261e-06
38421,115263,0,115263,500.6922962665558,6.294882705913517e-06
38501,115503,0,115503,501.76667308807373,6.2209958371075235e-06
38582,115746,0,115746,502.909704208374,6.146003618881788e-06
38663,115989,0,115989,504.0024423599243,6.0725467140564985e-06
38744,116232,0,116232,505.01033210754395,5.994846427250902e-06
38824,116472,0,116472,505.98405027389526,5.917935471827616e-06
38905,116715,0,116715,506.996707201004,5.84449623092824e-06
38986,116958,0,116958,507.99892711639404,5.778183855286883e-06
39066,117198,0,117198,508.98318219184875,5.712463532768936e-06
39147,117441,0,117441,509.96777415275574,5.643177639870138e-06
39228,117684,0,117684,510.9651691913605,5.576572574632584e-06
39309,117927,0,117927,511.94584608078003,5.513004071254282e-06
39389,118167,0,118167,512.9355492591858,5.449859997806579e-06
39470,118410,0,118410,513.9207742214203,5.386782543632739e-06
39551,118653,0,118653,514.9121601581573,5.305184200563142e-06
39631,118893,0,118893,515.882336139679,5.1952171040937725e-06
39712,119136,0,119136,516.8657021522522,5.107011361411317e-06
39793,119379,0,119379,517.8577802181244,5.043105291727307e-06
39874,119622,0,119622,518.839380979538,4.981029334425426e-06
39954,119862,0,119862,519.8264021873474,4.9259275455891106e-06
40035,120105,0,120105,520.8181781768799,4.868950731890643e-06
40116,120348,0,120348,521.8135211467743,4.812105380814399e-06
40196,120588,0,120588,522.7836112976074,4.7556688805809696e-06
40277,120831,0,120831,523.7744960784912,4.7002915497162505e-06
40358,121074,0,121074,524.7611091136932,4.646630556745637e-06
40439,121317,0,121317,525.7504560947418,4.592639138226357e-06
40519,121557,0,121557,526.7286560535431,4.536541303425066e-06
40600,121800,0,121800,527.7126572132111,4.483285029957933e-06
40681,122043,0,122043,528.7088482379913,4.430665616845248e-06
40761,122283,0,122283,529.6794052124023,4.3806830164190065e-06
40842,122526,0,122526,530.674149274826,4.325944878371009e-06
40923,122769,0,122769,531.6569261550903,4.269307961701926e-06
41004,123012,0,123012,532.6445531845093,4.2203116210449425e-06
41084,123252,0,123252,533.6206901073456,4.173335790237046e-06
41165,123495,0,123495,534.6176760196686,4.125790922507842e-06
41246,123738,0,123738,535.6002812385559,4.07462278373258e-06
41326,123978,0,123978,536.572859287262,4.004806163674379e-06
41407,124221,0,124221,537.5674123764038,3.949785081762136e-06
41488,124464,0,124464,538.5529420375824,3.898757514934125e-06
41569,124707,0,124707,539.550065279007,3.85105043482576e-06
41649,124947,0,124947,540.5191342830658,3.8080679536999403e-06
41730,125190,0,125190,541.5175712108612,3.7650065270523733e-06
41811,125433,0,125433,542.5084342956543,3.7221101954751793e-06
41891,125673,0,125673,543.5013191699982,3.6773692759432235e-06
41972,125916,0,125916,544.4991521835327,3.6333210448344737e-06
42053,126159,0,126159,545.4977152347565,3.5915500720841957e-06
42134,126402,0,126402,546.4851629734039,3.547497774184947e-06
42214,126642,0,126642,547.4647271633148,3.505810601549735e-06
42295,126885,0,126885,548.4699392318726,3.464202339101528e-06
42376,127128,0,127128,549.4580552577972,3.4254670274310923e-06
42456,127368,0,127368,550.445127248764,3.383381073977785e-06
42537,127611,0,127611,551.4251942634583,3.339953752526385e-06
42618,127854,0,127854,552.4174520969391,3.296653397812262e-06
42699,128097,0,128097,553.4000582695007,3.2569650575195574e-06
42779,128337,0,128337,554.3733742237091,3.218130408205287e-06
42860,128580,0,128580,555.3446731567383,3.1817309949065857e-06
42941,128823,0,128823,556.3499729633331,3.145859852311753e-06
43021,129063,0,129063,557.3203711509705,3.1039335142812648e-06
43102,129306,0,129306,558.3154852390289,3.0638299570646425e-06
43183,129549,0,129549,559.3081841468811,3.0276636767022087e-06
43264,129792,0,129792,560.2915840148926,2.9912533637749195e-06
43344,130032,0,130032,561.2793362140656,2.9550753583892913e-06
43425,130275,0,130275,562.2681651115417,2.9155053966169555e-06
43506,130518,0,130518,563.290999174118,2.8797132322106536e-06
43586,130758,0,130758,564.313826084137,2.8467581667527964e-06
43667,131001,0,131001,565.3783621788025,2.814351060176646e-06
43748,131244,0,131244,566.4447801113129,2.7812684763341036e-06
43829,131487,0,131487,567.5328731536865,2.7483534505353716e-06
43909,131727,0,131727,568.5715272426605,2.717339117434181e-06
43990,131970,0,131970,569.7272822856903,2.687341087273499e-06
44071,132213,0,132213,570.8267493247986,2.6580473330266395e-06
44151,132453,0,132453,571.9362041950226,2.6292051877188426e-06
44232,132696,0,132696,572.9201972484589,2.5990160801490853e-06
44313,132939,0,132939,573.9195981025696,2.5696768386558515e-06
44394,133182,0,133182,574.9004023075104,2.540535613556355e-06
44474,133422,0,133422,575.8868641853333,2.511425752217734e-06
44555,133665,0,133665,576.8737301826477,2.476963256858052e-06
44636,133908,0,133908,577.8673651218414,2.4439046094495586e-06
44717,134151,0,134151,578.8606061935425,2.4159597871380704e-06
44797,134391,0,134391,579.8386559486389,2.3870209544701467e-06
44878,134634,0,134634,580.8108870983124,2.3582179198052154e-06
44959,134877,0,134877,581.7723062038422,2.3310056519484826e-06
45039,135117,0,135117,582.7570853233337,2.3054905022667085e-06
45120,135360,0,135360,583.788378238678,2.2760985210683383e-06
45201,135603,0,135603,584.8166661262512,2.246838849922501e-06
45282,135846,0,135846,585.9969210624695,2.218583817647409e-06
45362,136086,0,136086,587.0682570934296,2.1929160267368603e-06
45443,136329,0,136329,588.1360101699829,2.165039811039391e-06
45524,136572,0,136572,589.2299160957336,2.1390512170092195e-06
45604,136812,0,136812,590.2660903930664,2.1122002977007046e-06
45685,137055,0,137055,591.3235011100769,2.08389359839177e-06
45766,137298,0,137298,592.3143889904022,2.054277239796439e-06
45847,137541,0,137541,593.3570771217346,2.0254278804145765e-06
45927,137781,0,137781,594.3408010005951,2.0003122069640575e-06
46008,138024,0,138024,595.3371713161469,1.9747356389313396e-06
46089,138267,0,138267,596.3343861103058,1.9508156059295617e-06
46169,138507,0,138507,597.3399653434753,1.9289966372014855e-06
46250,138750,0,138750,598.3445491790771,1.9065026415173665e-06
46331,138993,0,138993,599.3334031105042,1.8817989852913878e-06
46412,139236,0,139236,600.3358392715454,1.8551198445229599e-06
46492,139476,0,139476,601.3123240470886,1.8286276625046594e-06
46573,139719,0,139719,602.3024210929871,1.800172997757878e-06
46654,139962,0,139962,603.2855112552643,1.775507334919584e-06
46734,140202,0,140202,604.318695306778,1.754338216040686e-06
46815,140445,0,140445,605.3022420406342,1.7339778612371382e-06
46896,140688,0,140688,606.3725731372833,1.713938328697328e-06
46977,140931,0,140931,607.4828369617462,1.6937291474414172e-06
47057,141171,0,141171,608.6061222553253,1.672929663751161e-06
47138,141414,0,141414,609.6034822463989,1.6532248181551918e-06
47219,141657,0,141657,610.6025810241699,1.6337047302845793e-06
47299,141897,0,141897,611.5785751342773,1.6143008751226381e-06
47380,142140,0,142140,612.5867691040039,1.5941931027234638e-06
47461,142383,0,142383,613.6422362327576,1.5756029149938633e-06
47542,142626,0,142626,614.6401782035828,1.5574277344647955e-06
47622,142866,0,142866,615.6435701847076,1.5391043407276238e-06
47703,143109,0,143109,616.6570081710815,1.5207355853545207e-06
47784,143352,0,143352,617.6696441173553,1.5018424914184847e-06
47864,143592,0,143592,618.6462602615356,1.4822890677003447e-06
47945,143835,0,143835,619.6406271457672,1.4644707237319372e-06
48026,144078,0,144078,620.6160712242126,1.4482137657948267e-06
48107,144321,0,144321,621.6256561279297,1.4318634882901794e-06
48187,144561,0,144561,622.591203212738,1.416209444295558e-06
48268,144804,0,144804,623.6069769859314,1.400075257412946e-06
48349,145047,0,145047,624.5913331508636,1.384170384821825e-06
48429,145287,0,145287,625.5534262657166,1.3678126615761397e-06
48510,145530,0,145530,626.5401482582092,1.352119663080252e-06
48591,145773,0,145773,627.5456502437592,1.336588058555002e-06
48672,146016,0,146016,628.5441591739655,1.3206623307852659e-06
48752,146256,0,146256,629.5175621509552,1.3046334958130003e-06
48833,146499,0,146499,630.5151772499084,1.2897106748200752e-06
48914,146742,0,146742,631.5027372837067,1.2724126683406458e-06
48994,146982,0,146982,632.4979650974274,1.25588510396962e-06
49075,147225,0,147225,633.4896550178528,1.2415535494651558e-06
49156,147468,0,147468,634.4882972240448,1.227265020945802e-06
49237,147711,0,147711,635.4705860614777,1.2127183240405117e-06
49317,147951,0,147951,636.4399790763855,1.1974930573805572e-06
49398,148194,0,148194,637.4367311000824,1.1830632709300124e-06
49479,148437,0,148437,638.4227902889252,1.1689268673827813e-06
49559,148677,0,148677,639.3977062702179,1.154674940153797e-06
49640,148920,0,148920,640.3873162269592,1.141339254140654e-06
49721,149163,0,149163,641.385968208313,1.1283144951290247e-06
49802,149406,0,149406,642.3781070709229,1.1149751705220813e-06
49882,149646,0,149646,643.3621480464935,1.1020176451849843e-06
49963,149889,0,149889,644.3429291248322,1.0884635170054324e-06
50044,150132,0,150132,645.338002204895,1.0760069870229254e-06
50124,150372,0,150372,646.312420129776,1.063832572394624e-06
50205,150615,0,150615,647.3113222122192,1.0500598086842157e-06
50286,150858,0,150858,648.3101880550385,1.0361464339956899e-06
50367,151101,0,151101,649.3039462566376,1.0242813514072417e-06
50447,151341,0,151341,650.3052232265472,1.012282270209607e-06
50528,151584,0,151584,651.2864303588867,1.0000825344819094e-06
50609,151827,0,151827,652.2849702835083,9.857774770479197e-07
50689,152067,0,152067,653.258807182312,9.747615128821186e-07
50770,152310,0,152310,654.2617189884186,9.633936066798772e-07
50851,152553,0,152553,655.2449593544006,9.525369999142846e-07
50932,152796,0,152796,656.2333052158356,9.409997820904622e-07
51012,153036,0,153036,657.2026791572571,9.28685368563375e-07
51093,153279,0,153279,658.2032833099365,9.176568051338674e-07
51174,153522,0,153522,659.2006442546844,9.071292450392671e-07
51254,153762,0,153762,660.1787431240082,8.967201197550455e-07
51335,154005,0,154005,661.1769931316376,8.856038895295746e-07
51416,154248,0,154248,662.1669580936432,8.754610493591227e-07
51497,154491,0,154491,663.1600000858307,8.653501536959438e-07
51577,154731,0,154731,664.1340799331665,8.551723924579907e-07
51658,154974,0,154974,665.126894235611,8.444906243868554e-07
51739,155217,0,155217,666.1021921634674,8.345873657928628e-07
51819,155457,0,155457,667.0892651081085,8.251075196219255e-07
51900,155700,0,155700,668.0657069683075,8.150025131154973e-07
51981,155943,0,155943,669.0547392368317,8.038387820371657e-07
52062,156186,0,156186,670.0783972740173,7.927025977729405e-07
52142,156426,0,156426,671.1294510364532,7.824188154935469e-07
52223,156669,0,156669,672.1847763061523,7.720247504876115e-07
52304,156912,0,156912,673.2872252464294,7.62777208210536e-07
52384,157152,0,157152,674.3247621059418,7.542963802853742e-07
52465,157395,0,157395,675.3729913234711,7.451683453291219e-07
52546,157638,0,157638,676.4834370613098,7.358871316996487e-07
52627,157881,0,157881,677.6013412475586,7.273296953220709e-07
52707,158121,0,158121,678.5831651687622,7.183285353846352e-07
52788,158364,0,158364,679.5665531158447,7.102297492426302e-07
52869,158607,0,158607,680.5524532794952,7.015345280907807e-07
52950,158850,0,158850,681.5393903255463,6.931859385008576e-07
53030,159090,0,159090,682.5205721855164,6.848536703035208e-07
53111,159333,0,159333,683.5106720924377,6.76592780164335e-07
53192,159576,0,159576,684.5133621692657,6.685322377283015e-07
53272,159816,0,159816,685.4830090999603,6.609721557212757e-07
53353,160059,0,160059,686.4684300422668,6.53190783038286e-07
53434,160302,0,160302,687.4643051624298,6.444101469713111e-07
53515,160545,0,160545,688.5540981292725,6.345573731878413e-07
53595,160785,0,160785,689.5366570949554,6.268683482987676e-07
53676,161028,0,161028,690.9589900970459,6.195282978816697e-07
53757,161271,0,161271,692.0919380187988,6.108528238908876e-07
53837,161511,0,161511,693.366800069809,6.036398058803796e-07
53918,161754,0,161754,694.8188591003418,5.967888560723387e-07
53999,161997,0,161997,695.8806340694427,5.8986865712815e-07
54080,162240,0,162240,697.0360932350159,5.829917207635249e-07
54160,162480,0,162480,698.394314289093,5.761449852414903e-07
54241,162723,0,162723,699.7002260684967,5.696900897846539e-07
54322,162966,0,162966,700.8361411094666,5.631720237044722e-07
54402,163206,0,163206,701.9322690963745,5.562354508349563e-07
54483,163449,0,163449,703.178697347641,5.491779533172514e-07
54564,163692,0,163692,704.4039573669434,5.417849802516875e-07
54645,163935,0,163935,705.4299902915955,5.355417340665507e-07
54725,164175,0,164175,706.4324793815613,5.294077620656792e-07
54806,164418,0,164418,707.4213533401489,5.232025362290644e-07
54887,164661,0,164661,708.8366861343384,5.170973240367281e-07
54967,164901,0,164901,710.0430183410645,5.103656287696002e-07
55048,165144,0,165144,712.2740621566772,5.040910389981217e-07
55129,165387,0,165387,713.440838098526,4.981761704679595e-07
55210,165630,0,165630,714.4303641319275,4.920856159495648e-07
55290,165870,0,165870,715.3984682559967,4.842862677465382e-07
55371,166113,0,166113,716.3865621089935,4.780132558572223e-07
55452,166356,0,166356,717.3941791057587,4.7261891219334875e-07
55532,166596,0,166596,718.3516461849213,4.6723049545346854e-07
55613,166839,0,166839,719.3443331718445,4.6118734036549435e-07
55694,167082,0,167082,720.3341870307922,4.5543679123839807e-07
55775,167325,0,167325,721.3388242721558,4.4966458826716333e-07
55855,167565,0,167565,722.3323471546173,4.443960187642256e-07
55936,167808,0,167808,723.3315541744232,4.3917499300391026e-07
56017,168051,0,168051,724.3307361602783,4.331567288297316e-07
56097,168291,0,168291,725.2836892604828,4.2811466370458605e-07
56178,168534,0,168534,726.2833631038666,4.229555106405524e-07
56259,168777,0,168777,727.2821941375732,4.178855383136236e-07
56340,169020,0,169020,728.290271282196,4.123678156457122e-07
56420,169260,0,169260,729.2672202587128,4.0701891790617744e-07
56501,169503,0,169503,730.2565021514893,4.021092981070933e-07
56582,169746,0,169746,731.2749791145325,3.97482757197119e-07
56662,169986,0,169986,732.2651121616364,3.929093839380588e-07
56743,170229,0,170229,733.2722842693329,3.8810059825777276e-07
56824,170472,0,170472,734.258542060852,3.8329029460917905e-07
56905,170715,0,170715,735.2864460945129,3.789196274504232e-07
56985,170955,0,170955,736.2234652042389,3.7474946102372676e-07
57066,171198,0,171198,737.1540122032166,3.705765794104164e-07
57147,171441,0,171441,738.1473162174225,3.6581798770025556e-07
57227,171681,0,171681,739.0753161907196,3.616727307468893e-07
57308,171924,0,171924,740.0186631679535,3.574073761167997e-07
57389,172167,0,172167,741.130410194397,3.532930132143596e-07
57470,172410,0,172410,742.1465473175049,3.4896743849081536e-07
57550,172650,0,172650,743.2979121208191,3.4457472537339574e-07
57631,172893,0,172893,744.275003194809,3.406646881496375e-07
57712,173136,0,173136,745.2067880630493,3.365410368443703e-07
57792,173376,0,173376,746.2421622276306,3.3260120562625696e-07
57873,173619,0,173619,747.2854731082916,3.288316115146902e-07
57954,173862,0,173862,748.4614503383636,3.24385676914022e-07
58035,174105,0,174105,749.6896362304688,3.2029700987513944e-07
58115,174345,0,174345,750.7308542728424,3.16353530268085e-07
58196,174588,0,174588,751.640691280365,3.121084637219063e-07
58277,174831,0,174831,752.7389991283417,3.0752353394147807e-07
58357,175071,0,175071,753.7435622215271,3.034655134822391e-07
58438,175314,0,175314,754.7611210346222,2.998011910276632e-07
58519,175557,0,175557,755.7262289524078,2.9640670334813917e-07
58600,175800,0,175800,756.7333121299744,2.930425502738339e-07
58680,176040,0,176040,757.8145883083344,2.8974465218015807e-07
58761,176283,0,176283,758.8414142131805,2.8646740713654845e-07
58842,176526,0,176526,759.8256561756134,2.8315112751013534e-07
58922,176766,0,176766,760.7830011844635,2.799841843470536e-07
59003,177009,0,177009,761.7333731651306,2.7672873102074534e-07
59084,177252,0,177252,762.7039411067963,2.73366498304352e-07
59165,177495,0,177495,763.7061471939087,2.6980408090337326e-07
59245,177735,0,177735,764.6685853004456,2.666589701422103e-07
59326,177978,0,177978,765.7294273376465,2.6329456249310113e-07
59407,178221,0,178221,766.9089632034302,2.599373571320903e-07
59487,178461,0,178461,767.9071569442749,2.568658456677521e-07
59568,178704,0,178704,768.9965691566467,2.5391655088783036e-07
59649,178947,0,178947,770.0086901187897,2.5087813238071466e-07
59730,179190,0,179190,771.0857400894165,2.480398514840979e-07
59810,179430,0,179430,772.1357712745667,2.4515864562589214e-07
59891,179673,0,179673,773.1282851696014,2.4204524705923046e-07
59972,179916,0,179916,774.1434643268585,2.384537584082937e-07
60052,180156,0,180156,775.110062122345,2.3569305239509883e-07
60133,180399,0,180399,776.100554227829,2.3288328204405646e-07
60214,180642,0,180642,777.1297471523285,2.301220472936791e-07
60295,180885,0,180885,778.4257509708405,2.2761838423037262e-07
60375,181125,0,181125,779.537750005722,2.2510447860266348e-07
60456,181368,0,181368,780.4747681617737,2.226485676463608e-07
60537,181611,0,181611,781.425555229187,2.2005455878438145e-07
60618,181854,0,181854,782.3729200363159,2.1711498985962484e-07
60698,182094,0,182094,783.7717821598053,2.1428840214563683e-07
60779,182337,0,182337,784.71679520607,2.1182461985121644e-07
60860,182580,0,182580,785.7127270698547,2.0932082245471687e-07
60940,182820,0,182820,786.7180693149567,2.0655531793868869e-07
61021,183063,0,183063,787.6297290325165,2.03687350396514e-07
61102,183306,0,183306,788.5424020290375,2.0083105964705568e-07
61183,183549,0,183549,789.4383971691132,1.9837069570249646e-07
61263,183789,0,183789,790.3205230236053,1.960681682502312e-07
61344,184032,0,184032,791.2082500457764,1.9380221026041903e-07
61425,184275,0,184275,792.1162922382355,1.914213906781907e-07
61505,184515,0,184515,792.999231338501,1.889490526219643e-07
61586,184758,0,184758,793.904886007309,1.8647909472855743e-07
61667,185001,0,185001,794.7955513000488,1.8414100213942238e-07
61748,185244,0,185244,795.6897232532501,1.8168531677891274e-07
61828,185484,0,185484,796.5779991149902,1.7918745356072573e-07
61909,185727,0,185727,797.4542970657349,1.7699874569812475e-07
61990,185970,0,185970,798.3603000640869,1.7493854717802205e-07
62070,186210,0,186210,799.2428662776947,1.7283693764233066e-07
62151,186453,0,186453,800.1415662765503,1.707475390426392e-07
62232,186696,0,186696,801.0521941184998,1.6822070454473353e-07
62313,186939,0,186939,801.9395792484283,1.659116614122422e-07
62393,187179,0,187179,802.8329961299896,1.640803637433141e-07
62474,187422,0,187422,803.7210080623627,1.622409383036632e-07
62555,187665,0,187665,804.6258392333984,1.603377094925803e-07
62635,187905,0,187905,805.5011200904846,1.5847400954422034e-07
62716,188148,0,188148,806.3941969871521,1.5661166876264622e-07
62797,188391,0,188391,807.3030190467834,1.54784682078637e-07
62878,188634,0,188634,808.2108919620514,1.530140584012006e-07
62958,188874,0,188874,809.0977461338043,1.5125703032099004e-07
63039,189117,0,189117,809.9855341911316,1.493858275202795e-07
63120,189360,0,189360,810.885231256485,1.4766132196910677e-07
63200,189600,0,189600,811.7747230529785,1.4591003063699802e-07
63281,189843,0,189843,812.6731812953949,1.4371290268303773e-07
63362,190086,0,190086,813.5707061290741,1.411730368744625e-07
63443,190329,0,190329,814.4591763019562,1.3937780931911772e-07
63523,190569,0,190569,815.3492243289948,1.3775291896540768e-07
63604,190812,0,190812,816.2356312274933,1.361053015458188e-07
63685,191055,0,191055,817.1282112598419,1.3452566065759986e-07
63765,191295,0,191295,818.01629114151,1.3282280450028082e-07
63846,191538,0,191538,818.896154165268,1.3103260508998937e-07
63927,191781,0,191781,819.7943332195282,1.2913198554346628e-07
64008,192024,0,192024,820.6799993515015,1.275551484503531e-07
64088,192264,0,192264,821.5602931976318,1.261288538125974e-07
64169,192507,0,192507,822.4531493186951,1.245466841942326e-07
64250,192750,0,192750,823.346363067627,1.2307443963351046e-07
64330,192990,0,192990,824.2311992645264,1.216691135622767e-07
64411,193233,0,193233,825.1230940818787,1.2026082913519838e-07
64492,193476,0,193476,826.0184302330017,1.1879253609512997e-07
64573,193719,0,193719,826.9060142040253,1.1731350665115544e-07
64653,193959,0,193959,827.7846562862396,1.1597610811712089e-07
64734,194202,0,194202,828.6886100769043,1.1439343738628103e-07
64815,194445,0,194445,829.5693881511688,1.1277220252803983e-07
64895,194685,0,194685,830.4513840675354,1.1146708940159478e-07
64976,194928,0,194928,831.3469862937927,1.0999367326196501e-07
65057,195171,0,195171,832.2451839447021,1.0864063410145678e-07
65138,195414,0,195414,833.1444611549377,1.0741466265813645e-07
65218,195654,0,195654,834.0250751972198,1.0616228978460562e-07
65299,195897,0,195897,834.9196982383728,1.048043789172652e-07
65380,196140,0,196140,835.8142120838165,1.0331376381481127e-07
65460,196380,0,196380,836.6991271972656,1.0203899318043924e-07
65541,196623,0,196623,837.6158950328827,1.0087713134729978e-07
65622,196866,0,196866,838.5025551319122,9.967445721723814e-08
65703,197109,0,197109,839.3966012001038,9.842182255896307e-08
65783,197349,0,197349,840.2716221809387,9.722999298187672e-08
65864,197592,0,197592,841.1786532402039,9.594968141429208e-08
65945,197835,0,197835,842.0728101730347,9.485143009494407e-08
66025,198075,0,198075,842.9539232254028,9.378736138119117e-08
66106,198318,0,198318,843.8665761947632,9.275113164200344e-08
66187,198561,0,198561,844.755383014679,9.170653319626913e-08
66268,198804,0,198804,845.6631932258606,9.047328194170179e-08
66348,199044,0,199044,846.5485641956329,8.934296367465562e-08
66429,199287,0,199287,847.4766161441803,8.825656572199044e-08
66510,199530,0,199530,848.4170973300934,8.726374681672423e-08
66590,199770,0,199770,849.3428809642792,8.627005840726135e-08
66671,200013,0,200013,850.2901382446289,8.523167595327812e-08
66752,200256,0,200256,851.3643431663513,8.413217722554494e-08
66833,200499,0,200499,852.3970251083374,8.314343353263649e-08
66913,200739,0,200739,853.4421119689941,8.220968025891248e-08
66994,200982,0,200982,854.4272701740265,8.127675103929872e-08
67075,201225,0,201225,855.401015996933,8.034020024903309e-08
67155,201465,0,201465,856.2893822193146,7.939087165154297e-08
67236,201708,0,201708,857.1936461925507,7.840776762828963e-08
67317,201951,0,201951,858.0894801616669,7.747101934239955e-08
67398,202194,0,202194,858.9889500141144,7.651144741368084e-08
67478,202434,0,202434,859.8760361671448,7.561744499674314e-08
67559,202677,0,202677,860.7791132926941,7.461839420123173e-08
67640,202920,0,202920,861.6829171180725,7.372503051204359e-08
67720,203160,0,203160,862.5788090229034,7.27740197945749e-08
67801,203403,0,203403,863.4820141792297,7.184414798084608e-08
67882,203646,0,203646,864.3759431838989,7.100047326043176e-08
67963,203889,0,203889,865.2836573123932,7.015618172931456e-08
68043,204129,0,204129,866.1980781555176,6.9275620240548e-08
68124,204372,0,204372,867.1347062587738,6.844582915182549e-08
68205,204615,0,204615,868.0553162097931,6.762369820951593e-08
68285,204855,0,204855,868.9522061347961,6.680619879652525e-08
68366,205098,0,205098,869.8875381946564,6.598579765181763e-08
68447,205341,0,205341,870.8010311126709,6.50970854179892e-08
68528,205584,0,205584,871.6998870372772,6.417230550111293e-08
68608,205824,0,205824,872.5895352363586,6.322064581419618e-08
68689,206067,0,206067,873.4815862178802,6.246798015815812e-08
68770,206310,0,206310,874.3842780590057,6.173915548540316e-08
68851,206553,0,206553,875.2757661342621,6.103128208768966e-08
68931,206793,0,206793,876.2571151256561,6.021681120988601e-08
69012,207036,0,207036,877.2488460540771,5.9462287544064524e-08
69093,207279,0,207279,878.2985022068024,5.872782723079215e-08
69173,207519,0,207519,879.3276510238647,5.8071082840882155e-08
69254,207762,0,207762,880.2783091068268,5.7425757764555105e-08
69335,208005,0,208005,881.1787111759186,5.669042997340267e-08
69416,208248,0,208248,882.0666670799255,5.602749842638723e-08
69496,208488,0,208488,882.9534740447998,5.5334386428442945e-08
69577,208731,0,208731,883.8438541889191,5.460730286144479e-08
69658,208974,0,208974,884.7442831993103,5.3958838117421334e-08
69738,209214,0,209214,885.6200833320618,5.3350382333485885e-08
69819,209457,0,209457,886.5098810195923,5.272420893086978e-08
69900,209700,0,209700,887.4059519767761,5.213624955905513e-08
69981,209943,0,209943,888.2991251945496,5.1541687998789754e-08
70061,210183,0,210183,889.1910603046417,5.096549524639667e-08
70142,210426,0,210426,890.0832660198212,5.036282007678217e-08
70223,210669,0,210669,890.9808020591736,4.975114074513109e-08
70303,210909,0,210909,891.8596971035004,4.920730415449812e-08
70384,211152,0,211152,892.8581602573395,4.8599692927177735e-08
70465,211395,0,211395,893.8521473407745,4.8016123802964405e-08
70546,211638,0,211638,894.843120098114,4.744508631807766e-08
70626,211878,0,211878,895.852833032608,4.6817385237339666e-08
70707,212121,0,212121,896.7379519939423,4.622697879538841e-08
70788,212364,0,212364,897.6573832035065,4.565483132322711e-08
70868,212604,0,212604,898.536609172821,4.4982464995962364e-08
70949,212847,0,212847,899.4941880702972,4.442499848653815e-08
71030,213090,0,213090,900.5119481086731,4.3906829197186e-08
71111,213333,0,213333,901.4683382511139,4.340852776790437e-08
71191,213573,0,213573,902.4826669692993,4.28563804677737e-08
71272,213816,0,213816,903.4250411987305,4.229989661372699e-08
71353,214059,0,214059,904.4631900787354,4.1783894499687114e-08
71433,214299,0,214299,905.3453192710876,4.131211693243385e-08
71514,214542,0,214542,906.2552759647369,4.079849018701583e-08
71595,214785,0,214785,907.145524263382,4.029268576313134e-08
71676,215028,0,215028,908.0431361198425,3.980364424154585e-08
71756,215268,0,215268,908.9218831062317,3.932720844991519e-08
71837,215511,0,215511,909.8020341396332,3.8869000321816135e-08
71918,215754,0,215754,910.7006492614746,3.842876770361828e-08
71998,215994,0,215994,911.5829241275787,3.7980681929652913e-08
72079,216237,0,216237,912.4732391834259,3.7546482522007253e-08
72160,216480,0,216480,913.3706691265106,3.711347581153508e-08
72241,216723,0,216723,914.3204343318939,3.667461660360431e-08
72321,216963,0,216963,915.2077231407166,3.617939454079023e-08
72402,217206,0,217206,916.0965051651001,3.555883715436353e-08
72483,217449,0,217449,916.9889063835144,3.4947607798421336e-08
72563,217689,0,217689,917.8731231689453,3.44778624947751e-08
72644,217932,0,217932,918.7665781974792,3.394426893242253e-08
72725,218175,0,218175,919.6686503887177,3.3283202926847035e-08
72806,218418,0,218418,920.5633180141449,3.273628802023906e-08
72886,218658,0,218658,921.4538552761078,3.2286211000274716e-08
72967,218901,0,218901,922.346931219101,3.179364417376546e-08
73048,219144,0,219144,923.2418763637543,3.143405094321134e-08
73128,219384,0,219384,924.1402730941772,3.108439357310815e-08
73209,219627,0,219627,925.0333223342896,3.073047098253282e-08
73290,219870,0,219870,925.930474281311,3.032583525922226e-08
73371,220113,0,220113,926.8320572376251,2.9869238065072715e-08
73451,220353,0,220353,927.7272613048553,2.948117226163062e-08
73532,220596,0,220596,928.6513311862946,2.912865853022082e-08
73613,220839,0,220839,929.634124994278,2.8798981517619408e-08
73693,221079,0,221079,930.6359171867371,2.846592926320367e-08
73774,221322,0,221322,931.6143500804901,2.8120889992762496e-08
73855,221565,0,221565,932.6448712348938,2.7781170829488354e-08
73936,221808,0,221808,933.631637096405,2.7460182085864134e-08
74016,222048,0,222048,934.6681971549988,2.7113386665776168e-08
74097,222291,0,222291,935.5930511951447,2.6795461852781946e-08
74178,222534,0,222534,936.4768922328949,2.648749729408174e-08
74258,222774,0,222774,937.3712959289551,2.6188639833127655e-08
74339,223017,0,223017,938.257847070694,2.588775224888217e-08
74420,223260,0,223260,939.1635823249817,2.5581937493622185e-08
74501,223503,0,223503,940.0458722114563,2.5286001196021694e-08
74581,223743,0,223743,940.9175040721893,2.4996339525114803e-08
74662,223986,0,223986,941.8085989952087,2.4708454261052366e-08
74743,224229,0,224229,942.698046207428,2.438224805882196e-08
74823,224469,0,224469,943.5903143882751,2.4101975945417076e-08
74904,224712,0,224712,944.4715812206268,2.382593011658333e-08
74985,224955,0,224955,945.3793902397156,2.3531850532307275e-08
75066,225198,0,225198,946.2704360485077,2.32473371104662e-08
75146,225438,0,225438,947.147613286972,2.2993404570718276e-08
75227,225681,0,225681,948.0486409664154,2.2730758060572946e-08
75308,225924,0,225924,948.933895111084,2.2456378706610354e-08
75388,226164,0,226164,949.8181862831116,2.2202634766342186e-08
75469,226407,0,226407,950.7102739810944,2.1945767546257168e-08
75550,226650,0,226650,951.6000211238861,2.1687041993568232e-08
75631,226893,0,226893,952.5021879673004,2.1423387085598933e-08
75711,227133,0,227133,953.3836002349854,2.1165586559640587e-08
75792,227376,0,227376,954.2918100357056,2.090796533456048e-08
75873,227619,0,227619,955.1829102039337,2.0636906427955986e-08
75953,227859,0,227859,956.071857213974,2.039474474267415e-08
76034,228102,0,228102,957.0384492874146,2.013865225231108e-08
76115,228345,0,228345,958.0832431316376,1.9882123355551508e-08
76196,228588,0,228588,959.0511300563812,1.9650182963491314e-08
76276,228828,0,228828,959.9987812042236,1.9352941227185247e-08
76357,229071,0,229071,960.9558181762695,1.905149810137536e-08
76438,229314,0,229314,961.880232334137,1.8810116085819577e-08
76518,229554,0,229554,962.7731292247772,1.857031161521524e-08
76599,229797,0,229797,963.75923204422,1.835286446940648e-08
76680,230040,0,230040,964.7330982685089,1.8116928411561804e-08
76761,230283,0,230283,965.6753401756287,1.790102374793967e-08
76841,230523,0,230523,966.6430780887604,1.769605136685407e-08
76922,230766,0,230766,967.8439872264862,1.750086847176048e-08
77003,231009,0,231009,968.938285112381,1.7293304750605303e-08
77084,231252,0,231252,969.9148080348969,1.707323564593434e-08
77164,231492,0,231492,970.7939450740814,1.6860575943072575e-08
77245,231735,0,231735,971.772824048996,1.666694147247108e-08
77326,231978,0,231978,972.7700700759888,1.6473731370733043e-08
77406,232218,0,232218,973.7786569595337,1.6288383180934982e-08
77487,232461,0,232461,974.7079651355743,1.6079929009122865e-08
77568,232704,0,232704,975.6153931617737,1.5884814519790404e-08
77649,232947,0,232947,976.531387090683,1.5687028394155958e-08
77729,233187,0,233187,977.4122381210327,1.550140947647424e-08
77810,233430,0,233430,978.3476121425629,1.5322697615034088e-08
77891,233673,0,233673,979.2634701728821,1.5137867583922058e-08
77971,233913,0,233913,980.1705992221832,1.4949784230970968e-08
78052,234156,0,234156,981.0737912654877,1.4764333878209806e-08
78133,234399,0,234399,981.9776341915131,1.4595799188839316e-08
78214,234642,0,234642,982.8995640277863,1.44227494772913e-08
78294,234882,0,234882,983.8446581363678,1.4203783118124382e-08
78375,235125,0,235125,984.8703191280365,1.4026971509176022e-08
78456,235368,0,235368,985.8847050666809,1.3864044978239717e-08
78536,235608,0,235608,986.8831751346588,1.3710428744989397e-08
78617,235851,0,235851,987.8936071395874,1.3538694675089312e-08
78698,236094,0,236094,988.9774310588837,1.3384367107067192e-08
78779,236337,0,236337,989.9961311817169,1.3231282214232228e-08
78859,236577,0,236577,991.118643283844,1.3082167738669648e-08
78940,236820,0,236820,992.2337710857391,1.2930103243473856e-08
79021,237063,0,237063,993.4094982147217,1.2780094255332154e-08
79101,237303,0,237303,994.445652961731,1.2630310375081759e-08
79182,237546,0,237546,995.439070224762,1.248200718940627e-08
79263,237789,0,237789,996.5035660266876,1.2329955482837858e-08
79344,238032,0,238032,997.4391143321991,1.2184661761036052e-08
79424,238272,0,238272,998.3659310340881,1.2043795017026338e-08
79505,238515,0,238515,999.5904240608215,1.1884258677019082e-08
79586,238758,0,238758,1000.7630572319031,1.1724532862008892e-08
79666,238998,0,238998,1001.7329850196838,1.1589404179443818e-08
79747,239241,0,239241,1002.6943731307983,1.1448631747648767e-08
79828,239484,0,239484,1003.6987042427063,1.1293209519242333e-08
79909,239727,0,239727,1004.7500221729279,1.11517584708479e-08
79989,239967,0,239967,1005.6809930801392,1.1012320240755549e-08
80070,240210,0,240210,1007.3818881511688,1.0888540684155097e-08
80151,240453,0,240453,1008.7387020587921,1.076349191687153e-08
80231,240693,0,240693,1010.0119452476501,1.064183705219615e-08
80312,240936,0,240936,1011.1586651802063,1.0498198560384532e-08
80393,241179,0,241179,1012.2761881351471,1.0358514538174821e-08
80474,241422,0,241422,1013.341117143631,1.0236379903292454e-08
80554,241662,0,241662,1014.4755623340607,1.0114850702076874e-08
80635,241905,0,241905,1015.5418121814728,9.999789548452178e-09


==> plot_data/quadratic_minimax_problem_n500_alpha00001/flex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0006730556488037109,30.358106049564984
100,423,0,423,9.699470043182373,0.6740708090137648
200,904,0,904,19.293302059173584,0.36479367437778243
300,1398,0,1398,30.14501118659973,0.3011071376998588
400,1898,0,1898,41.2958869934082,0.27284904918698316
501,2403,0,2403,51.33675408363342,0.2513713270154871
601,2903,0,2903,62.01597213745117,0.234106610900458
701,3403,0,3403,72.63560199737549,0.21948271100161407
801,3903,0,3903,83.10749697685242,0.20671330437256502
901,4403,0,4403,93.06895780563354,0.19533775315508978
1001,4903,0,4903,102.56371402740479,0.18508769923021168
1101,5403,0,5403,112.03076696395874,0.17574157451435118
1201,5903,0,5903,121.87506914138794,0.16718224618280828
1301,6403,0,6403,132.27479004859924,0.1592768985844412
1401,6903,0,6903,144.16654109954834,0.1519401173686006
1502,7408,0,7408,154.95235800743103,0.14506500219313892
1602,7908,0,7908,167.59047603607178,0.1387179106376333
1702,8408,0,8408,180.78743600845337,0.13278191151715082
1802,8908,0,8908,191.2439830303192,0.12719265855275141
1902,9408,0,9408,201.48468589782715,0.1219400560136374
2002,9908,0,9908,211.64182591438293,0.11701191228993676
2102,10408,0,10408,223.53338313102722,0.11236629569478193
2202,10908,0,10908,234.19905924797058,0.1079741884630845
2302,11408,0,11408,244.99614310264587,0.10381508154336361
2402,11908,0,11908,255.05940914154053,0.09987308583851982
2503,12413,0,12413,265.158056974411,0.09610822382464428
2603,12913,0,12913,276.82814717292786,0.09255337945643131
2703,13413,0,13413,288.7055678367615,0.08917858033816427
2803,13913,0,13913,298.69650411605835,0.08597224804076486
2903,14413,0,14413,309.3056402206421,0.08291247365497094
3003,14913,0,14913,319.35656118392944,0.08000772731563129
3103,15413,0,15413,329.2388961315155,0.07724586090048079
3203,15913,0,15913,339.0263350009918,0.07461367196444577
3303,16413,0,16413,348.7440061569214,0.07208114636080319
3403,16913,0,16913,358.83766198158264,0.06967606694973875
3504,17418,0,17418,368.7782881259918,0.06735533287282698
3604,17918,0,17918,380.54287099838257,0.0651705839756705
3704,18418,0,18418,391.6623890399933,0.06307331943822765
3804,18918,0,18918,401.6895110607147,0.061069200263926635
3904,19418,0,19418,412.3128261566162,0.059158459188021435
4004,19918,0,19918,422.791640996933,0.05732596943137648
4104,20418,0,20418,433.3351631164551,0.05557071732301238
4204,20918,0,20918,443.52463603019714,0.05388292866896858
4304,21418,0,21418,453.3360779285431,0.05226988215909881
4404,21918,0,21918,463.94493794441223,0.05073371062024936
4505,22423,0,22423,473.92792320251465,0.049239908680385955
4605,22923,0,22923,484.96298480033875,0.047811337373014344
4705,23423,0,23423,495.05528497695923,0.04644612916767309
4805,23923,0,23923,505.56760907173157,0.045138535468762855
4905,24423,0,24423,516.5812230110168,0.043876713568457695
5005,24923,0,24923,527.3454110622406,0.042667078190062255
5105,25423,0,25423,538.0618500709534,0.04150156967641493
5205,25923,0,25923,548.302276134491,0.040382780754147994
5305,26423,0,26423,558.2923929691315,0.03930801613506081
5405,26923,0,26923,569.6716032028198,0.038272359434075295
5506,27428,0,27428,580.1642160415649,0.03727117225157682
5606,27928,0,27928,591.4966111183167,0.036313514972909265
5706,28428,0,28428,603.2202050685883,0.03539102472124249
5806,28928,0,28928,615.5168859958649,0.03450565883793069
5906,29428,0,29428,626.8991320133209,0.03365118833915721
6006,29928,0,29928,638.1180880069733,0.03282710655393964
6106,30428,0,30428,649.4500699043274,0.032030826600110085
6206,30928,0,30928,660.9912848472595,0.031251986584151854
6306,31428,0,31428,671.9112968444824,0.030508918236367304
6406,31928,0,31928,681.8826060295105,0.029793637817455157
6507,32433,0,32433,692.0171658992767,0.029095611888973298
6607,32933,0,32933,701.9363031387329,0.02843036289544006
6707,33433,0,33433,711.8595790863037,0.027781592628328324
6807,33933,0,33933,721.8995070457458,0.027152829857074155
6907,34433,0,34433,731.6549100875854,0.026538935137007263
7007,34933,0,34933,741.6377792358398,0.02595172271031554
7107,35433,0,35433,751.6755850315094,0.02538157140054715
7207,35933,0,35933,761.9250719547272,0.024834885215656122
7307,36433,0,36433,772.5627608299255,0.024298489003464614
7407,36933,0,36933,783.2905461788177,0.02377729330308051
7508,37438,0,37438,794.0686919689178,0.023275230739235382
7608,37938,0,37938,805.6115131378174,0.02279203498650222
7708,38438,0,38438,817.3950800895691,0.022322806772084865
7808,38938,0,38938,829.3922560214996,0.021865528571221024
7908,39438,0,39438,840.5269300937653,0.021419479492325068
8008,39938,0,39938,850.5700421333313,0.02098867118647162
8108,40438,0,40438,860.5083179473877,0.020572205964901655
8208,40938,0,40938,870.4831459522247,0.02016582322980434
8308,41438,0,41438,880.3280801773071,0.01977047541984274
8408,41938,0,41938,890.2508971691132,0.019389799980957342
8509,42443,0,42443,901.1762101650238,0.019011432923092448
8609,42943,0,42943,911.14927983284,0.018643052388337335
8709,43443,0,43443,921.5642149448395,0.018285644353247893
8809,43943,0,43943,931.7266509532928,0.01794423210894945
8909,44443,0,44443,944.0602648258209,0.017609809355168732
9009,44943,0,44943,955.7249300479889,0.017283162120705936
9109,45443,0,45443,968.0701911449432,0.016964699513328976
9209,45943,0,45943,979.5202269554138,0.016655877057779756
9309,46443,0,46443,990.6654980182648,0.016353440897675802
9409,46943,0,46943,1000.8383059501648,0.016060743806844174
9510,47448,0,47448,1012.6331398487091,0.015769300195604255
9610,47948,0,47948,1024.1976990699768,0.015487873408863198
9710,48448,0,48448,1037.8917889595032,0.01521403141112706
9810,48948,0,48948,1049.1274650096893,0.014943237769159498
9910,49448,0,49448,1060.8081979751587,0.014682259050626364
10010,49948,0,49948,1071.976175069809,0.014423437798893483
10110,50448,0,50448,1084.1940269470215,0.014171277133404974
10210,50948,0,50948,1095.340166091919,0.01392333594599989
10310,51448,0,51448,1106.6179921627045,0.013682338157944274
10410,51948,0,51948,1118.0536391735077,0.013447507339058948
10511,52453,0,52453,1128.1963860988617,0.01321293134250753
10611,52953,0,52953,1138.5358068943024,0.012989574657526023
10711,53453,0,53453,1149.5386338233948,0.012768769040499405
10811,53953,0,53953,1159.6291601657867,0.012556441467346625
10911,54453,0,54453,1169.4987869262695,0.012349143740692738
11011,54953,0,54953,1179.5461390018463,0.01214524355860213
11111,55453,0,55453,1189.547888994217,0.011947266766893203
11211,55953,0,55953,1199.7248990535736,0.011751695137031887
11311,56453,0,56453,1210.1026470661163,0.011559599614786942
11411,56953,0,56953,1221.7343001365662,0.011371096600628265
11512,57458,0,57458,1234.2979729175568,0.011186639526794611
11612,57958,0,57958,1245.2664771080017,0.0110072713543146
11712,58458,0,58458,1256.0167319774628,0.010831155361876243
11812,58958,0,58958,1268.3479030132294,0.010658408334752617
11912,59458,0,59458,1279.9490900039673,0.010486890162832036
12012,59958,0,59958,1290.2467019557953,0.010320351943382359
12112,60458,0,60458,1300.134365081787,0.010157743210582122
12212,60958,0,60958,1310.082113981247,0.009998570256356795
12312,61458,0,61458,1319.9124610424042,0.00984163501184768
12412,61958,0,61958,1329.6916460990906,0.009687127901705582
12513,62463,0,62463,1340.343815088272,0.009534941649700859
12613,62963,0,62963,1350.4492959976196,0.00938868992799043
12713,63463,0,63463,1360.2311689853668,0.009241979730494933
12813,63963,0,63963,1369.8919689655304,0.009097986425696137
12913,64463,0,64463,1379.7811110019684,0.008957248416518902
13013,64963,0,64963,1389.614872932434,0.008818201482802683
13113,65463,0,65463,1399.2509980201721,0.00868249810425601
13213,65963,0,65963,1409.0612919330597,0.008548064509870506
13313,66463,0,66463,1418.9324080944061,0.008416005396848438
13413,66963,0,66963,1428.7228798866272,0.008287377199784856
13514,67468,0,67468,1438.553619146347,0.008159888099818451
13614,67968,0,67968,1448.5758690834045,0.008034419436160416
13714,68468,0,68468,1459.4919679164886,0.007913611752316004
13814,68968,0,68968,1469.9276340007782,0.007795390316821144
13914,69468,0,69468,1480.1929891109467,0.007677743815105847
14014,69968,0,69968,1490.2318949699402,0.007562860481353119
14114,70468,0,70468,1500.4205849170685,0.007450605242903559
14214,70968,0,70968,1512.4886538982391,0.007340636657919483
14314,71468,0,71468,1523.2430560588837,0.007231841509013097
14414,71968,0,71968,1534.38387799263,0.00712416435095943
14515,72473,0,72473,1545.5344948768616,0.007017012543646849
14615,72973,0,72973,1557.550113916397,0.006914271553971753
14715,73473,0,73473,1571.8863739967346,0.006814068949784387
14815,73973,0,73973,1585.2750871181488,0.006714731852956441
14915,74473,0,74473,1596.212457895279,0.006616603931633526
15015,74973,0,74973,1606.6555409431458,0.006520031544543469
15115,75473,0,75473,1616.9285678863525,0.006425897019206822
15215,75973,0,75973,1627.102919101715,0.006332988037277899
15315,76473,0,76473,1637.5276579856873,0.0062413727734129
15415,76973,0,76973,1648.013345003128,0.006152090206288771
15516,77478,0,77478,1659.0314919948578,0.006063241357561435
15616,77978,0,77978,1669.8793561458588,0.0059757368861365805
15716,78478,0,78478,1679.9648249149323,0.005889920085292591
15816,78978,0,78978,1690.3627171516418,0.0058055010224595084
15916,79478,0,79478,1700.636183977127,0.005722752804225829
16016,79978,0,79978,1710.8188710212708,0.005640623693481606
16116,80478,0,80478,1723.4660189151764,0.005559186804897125
16216,80978,0,80978,1735.31405210495,0.005478765407526689
16316,81478,0,81478,1746.2166528701782,0.005399980840299835
16416,81978,0,81978,1757.2159872055054,0.0053234970975538495
16517,82483,0,82483,1767.9029412269592,0.005246187465325018
16617,82983,0,82983,1777.981750011444,0.005169919168812627
16717,83483,0,83483,1788.2994439601898,0.005095591710316658
16817,83983,0,83983,1798.3705258369446,0.005023072144022762
16917,84483,0,84483,1808.396311044693,0.004950929151437472
17017,84983,0,84983,1818.3841049671173,0.004880086256069801
17117,85483,0,85483,1828.5262398719788,0.004811328271177826
17217,85983,0,85983,1839.1046750545502,0.004742862582062508
17317,86483,0,86483,1849.5185267925262,0.004676545072588412
17417,86983,0,86983,1859.5849928855896,0.004611783740845919
17518,87488,0,87488,1869.7007129192352,0.0045464589241467615
17618,87988,0,87988,1879.7228882312775,0.004482863327512462
17718,88488,0,88488,1889.8140211105347,0.004420565297487159
17818,88988,0,88988,1900.3921859264374,0.004358859020481772
17918,89488,0,89488,1911.3747289180756,0.004298649030839239
18018,89988,0,89988,1922.3947660923004,0.004239974742757932
18118,90488,0,90488,1934.451828956604,0.004181856626744563
18218,90988,0,90988,1946.0246698856354,0.0041244299516009445
18318,91488,0,91488,1957.5522480010986,0.004067760539698059
18418,91988,0,91988,1968.596971988678,0.0040118943588045184
18519,92493,0,92493,1979.6483471393585,0.003956686811520169
18619,92993,0,92993,1989.5692410469055,0.0039028743511904385
18719,93493,0,93493,2000.7066910266876,0.0038498559976971668
18819,93993,0,93993,2011.4981219768524,0.00379690826235795
18919,94493,0,94493,2023.023059129715,0.0037446131980354196
19019,94993,0,94993,2033.502333164215,0.003693937852466599
19119,95493,0,95493,2044.1939160823822,0.003643936854438327
19219,95993,0,95993,2054.6254019737244,0.0035934791019181455
19319,96493,0,96493,2065.5397329330444,0.0035436462446997857
19419,96993,0,96993,2076.525779247284,0.0034946011434185665
19520,97498,0,97498,2088.421856880188,0.0034456566818429034
19620,97998,0,97998,2099.9350969791412,0.0033980930796209544
19720,98498,0,98498,2111.536989927292,0.00335146003228404
19820,98998,0,98998,2122.7096660137177,0.00330542664071531
19920,99498,0,99498,2134.9520611763,0.0032601993139334583
20020,99998,0,99998,2146.1293098926544,0.003215795253064266
20120,100498,0,100498,2156.7036378383636,0.0031717673149927856
20220,100998,0,100998,2167.7782320976257,0.0031287050460743733
20320,101498,0,101498,2178.990291118622,0.003086363301907172
20420,101998,0,101998,2189.954290151596,0.003044445551693037
20521,102503,0,102503,2201.237939119339,0.003002888075763937
20621,103003,0,103003,2212.2980678081512,0.0029627838629593117
20721,103503,0,103503,2223.615624189377,0.002923467941498095
20821,104003,0,104003,2234.6899812221527,0.0028843921347016734
20921,104503,0,104503,2246.304037094116,0.002845777648144417
21021,105003,0,105003,2257.4469170570374,0.002807604420269065
21121,105503,0,105503,2267.7689850330353,0.002769985193498142
21221,106003,0,106003,2278.3883991241455,0.002733459822412864
21321,106503,0,106503,2289.9377069473267,0.0026978773884618443
21421,107003,0,107003,2300.036851167679,0.0026623464651141624
21522,107508,0,107508,2311.3211500644684,0.0026264289794471363
21622,108008,0,108008,2323.0846149921417,0.0025916193404392565
21722,108508,0,108508,2334.5994980335236,0.0025579546784296786
21822,109008,0,109008,2344.7696890830994,0.002524605794318878
21922,109508,0,109508,2355.329129934311,0.002491127632570393
22022,110008,0,110008,2366.1014540195465,0.0024578116424554754
22122,110508,0,110508,2376.3520691394806,0.002424961584814794
22222,111008,0,111008,2387.1287038326263,0.0023927861578514503
22322,111508,0,111508,2398.808699131012,0.0023609871178997513
22422,112008,0,112008,2409.445496082306,0.0023294175969082037
22523,112513,0,112513,2420.378399848938,0.002297924573733798
22623,113013,0,113013,2431.156378030777,0.0022673511708853006
22723,113513,0,113513,2441.5369188785553,0.0022368688187186956
22823,114013,0,114013,2452.4181020259857,0.0022065841664088244
22923,114513,0,114513,2463.393405199051,0.0021773461430529164
23023,115013,0,115013,2474.069747209549,0.002148654163350126
23123,115513,0,115513,2484.856570959091,0.0021199231946575975
23223,116013,0,116013,2496.0955300331116,0.0020914531135217424
23323,116513,0,116513,2507.2227470874786,0.002063706162551783
23423,117013,0,117013,2518.055771112442,0.002036499504599918
23524,117518,0,117518,2529.393872976303,0.0020093881755093514
23624,118018,0,118018,2540.6054809093475,0.001982709735082616
23724,118518,0,118518,2551.240509033203,0.0019561014206939077
23824,119018,0,119018,2562.076261997223,0.0019302603745496515
23924,119518,0,119518,2573.6392302513123,0.0019053454353859243
24024,120018,0,120018,2584.430788040161,0.0018806693008264134
24124,120518,0,120518,2595.309977054596,0.0018559450999957043
24224,121018,0,121018,2606.504457950592,0.0018315873716478475
24324,121518,0,121518,2617.153336048126,0.0018077804981858035
24424,122018,0,122018,2627.7042989730835,0.001784454642912226
24525,122523,0,122523,2638.1886451244354,0.001761209015094746
24625,123023,0,123023,2652.4952681064606,0.001738391988894958
24725,123523,0,123523,2664.1773421764374,0.00171586423485638
24825,124023,0,124023,2675.329486131668,0.0016935761857893345
24925,124523,0,124523,2685.6356739997864,0.0016715839296080578
25025,125023,0,125023,2695.5852320194244,0.0016499198063745875
25125,125523,0,125523,2705.47967004776,0.0016285428820247592
25225,126023,0,126023,2715.3987679481506,0.0016075924236171844
25325,126523,0,126523,2725.428989171982,0.0015867531763290267
25425,127023,0,127023,2735.258108139038,0.0015658059260057534
25526,127528,0,127528,2746.1808359622955,0.0015451444418893383
25626,128028,0,128028,2757.429119825363,0.0015253098082737766
25726,128528,0,128528,2769.2243649959564,0.0015054972300539602
25826,129028,0,129028,2779.19335603714,0.001485658988449537
25926,129528,0,129528,2789.3767268657684,0.0014660199308520123
26026,130028,0,130028,2799.4655232429504,0.0014467936258351932
26126,130528,0,130528,2810.6020560264587,0.001427990732161791
26226,131028,0,131028,2822.444680929184,0.0014092965002787707
26326,131528,0,131528,2833.286127090454,0.0013906476526894666
26426,132028,0,132028,2844.106440782547,0.001372328535017738
26527,132533,0,132533,2854.1336619853973,0.0013543540128066133
26627,133033,0,133033,2865.0407269001007,0.0013368473809247214
26727,133533,0,133533,2875.7185368537903,0.0013193386765255664
26827,134033,0,134033,2886.70029091835,0.0013020111015608902
26927,134533,0,134533,2897.2351191043854,0.0012851365408325561
27027,135033,0,135033,2909.5016429424286,0.0012685326536822016
27127,135533,0,135533,2920.6220610141754,0.0012520846679355017
27227,136033,0,136033,2932.4789202213287,0.0012359650670930196
27327,136533,0,136533,2944.3751668930054,0.0012201408011003109
27427,137033,0,137033,2956.187180042267,0.0012045337051295054
27528,137538,0,137538,2967.347860813141,0.0011889538197235156
27628,138038,0,138038,2978.3903341293335,0.0011737633960006634
27728,138538,0,138538,2988.4745378494263,0.001159006846744811
27828,139038,0,139038,2998.5308899879456,0.0011445533289527732
27928,139538,0,139538,3008.649559020996,0.0011300831995496015
28028,140038,0,140038,3019.242676973343,0.0011156508556234065
28128,140538,0,140538,3029.5465109348297,0.0011014996204924891
28228,141038,0,141038,3039.560481071472,0.0010877816852691465
28328,141538,0,141538,3049.548295021057,0.0010742364195470795
28428,142038,0,142038,3059.584760904312,0.001060561563204573
28529,142543,0,142543,3069.873728990555,0.0010467721196679356
28629,143043,0,143043,3082.125308036804,0.0010333276400003775
28729,143543,0,143543,3094.005252122879,0.001020061240369355
28829,144043,0,144043,3104.0048570632935,0.0010070101018600408
28929,144543,0,144543,3113.9865849018097,0.0009940971974781159
29029,145043,0,145043,3123.9651350975037,0.000981219744957462
29129,145543,0,145543,3134.2727541923523,0.0009685331546077873
29229,146043,0,146043,3145.138696193695,0.0009560472782302953
29329,146543,0,146543,3155.305980205536,0.0009437195548886938
29429,147043,0,147043,3165.5753259658813,0.0009315581817663742
29530,147548,0,147548,3175.7362768650055,0.0009193600921322451
29630,148048,0,148048,3186.603451013565,0.0009074241261998246
29730,148548,0,148548,3197.3450758457184,0.0008957086455786554
29830,149048,0,149048,3208.7932970523834,0.0008841907846550142
29930,149548,0,149548,3220.082731962204,0.0008728574992763401
30030,150048,0,150048,3231.5073561668396,0.0008617020424861686
30130,150548,0,150548,3242.758847951889,0.0008506497334819705
30230,151048,0,151048,3253.341505050659,0.0008397281367189477
30330,151548,0,151548,3263.9292089939117,0.0008290370498930587
30430,152048,0,152048,3275.066766023636,0.0008186622279307561
30531,152553,0,152553,3286.536719083786,0.0008084208423240097
30631,153053,0,153053,3297.751591205597,0.000798282359315857
30731,153553,0,153553,3307.9708340168,0.000788147202886754
30831,154053,0,154053,3319.026332139969,0.0007782398130713101
30931,154553,0,154553,3329.44251704216,0.0007686620024254315
31031,155053,0,155053,3340.012946128845,0.0007592367536939216
31131,155553,0,155553,3350.8919909000397,0.0007497737075312852
31231,156053,0,156053,3361.204619884491,0.0007403085738802685
31331,156553,0,156553,3372.3822388648987,0.0007309587843850111
31431,157053,0,157053,3384.4223189353943,0.0007217810233619198
31532,157558,0,157558,3396.237493991852,0.000712683668522996
31632,158058,0,158058,3406.8846728801727,0.0007037663169281105
31732,158558,0,158558,3419.962462902069,0.0006948741795556393
31832,159058,0,159058,3431.159548997879,0.0006860266726231893
31932,159558,0,159558,3441.3197770118713,0.0006772414696078435
32032,160058,0,160058,3451.2048139572144,0.0006685827834672235
32132,160558,0,160558,3461.5287709236145,0.000660081657837168
32232,161058,0,161058,3472.9723591804504,0.0006516862415802117
32332,161558,0,161558,3484.501163959503,0.0006433685659208209
32432,162058,0,162058,3495.945027112961,0.0006350972787162443
32533,162563,0,162563,3507.18661403656,0.0006268495826922653
32633,163063,0,163063,3519.25572180748,0.0006188660737521514
32733,163563,0,163563,3531.4071238040924,0.0006109919566066389
32833,164063,0,164063,3541.318706035614,0.0006031590939862547
32933,164563,0,164563,3551.117156982422,0.0005953726448863385
33033,165063,0,165063,3561.048539161682,0.0005877081411343943
33133,165563,0,165563,3570.868008852005,0.0005802879828078687
33233,166063,0,166063,3581.6455929279327,0.0005730434328837904
33333,166563,0,166563,3592.8631222248077,0.0005657733459171801
33433,167063,0,167063,3604.600296020508,0.0005585136075059691
33534,167568,0,167568,3616.593600988388,0.0005513825762683625
33634,168068,0,168068,3627.925632953644,0.0005445406263639869
33734,168568,0,168568,3641.015226125717,0.0005377888213738135
33834,169068,0,169068,3655.4783000946045,0.0005310529670369452
33934,169568,0,169568,3669.0734169483185,0.0005243854838288612
34034,170068,0,170068,3682.604264974594,0.000517831328721706
34134,170568,0,170568,3696.2952330112457,0.0005113676747452104
34234,171068,0,171068,3707.7795989513397,0.0005050098629617553
34334,171568,0,171568,3719.447010040283,0.00049876465823154
34434,172068,0,172068,3731.1519269943237,0.00049259800225575
34535,172573,0,172573,3742.3255751132965,0.00048640436343996184
34635,173073,0,173073,3752.4785430431366,0.0004802655788187519
34735,173573,0,173573,3762.590150117874,0.0004742093471004622
34835,174073,0,174073,3773.7791390419006,0.00046833814235534523
34935,174573,0,174573,3784.5149841308594,0.00046255593506026025
35035,175073,0,175073,3794.9408628940582,0.0004567417559355909
35135,175573,0,175573,3806.5286231040955,0.0004509403254617686
35235,176073,0,176073,3818.0886929035187,0.0004452489705895118
35335,176573,0,176573,3829.545721054077,0.00043968320882483726
35435,177073,0,177073,3840.4341008663177,0.0004341618047082116
35536,177578,0,177578,3850.8316111564636,0.0004285787620269132
35636,178078,0,178078,3861.076411008835,0.0004231109704062924
35736,178578,0,178578,3871.5602831840515,0.000417754151896793
35836,179078,0,179078,3881.842430114746,0.0004124976682262871
35936,179578,0,179578,3892.650361061096,0.0004072915540156594
36036,180078,0,180078,3902.9509768486023,0.00040209175212119734
36136,180578,0,180578,3913.0800700187683,0.0003969624072696761
36236,181078,0,181078,3923.2705760002136,0.00039194998090848215
36336,181578,0,181578,3933.602425098419,0.0003869921380551484
36436,182078,0,182078,3944.1750168800354,0.0003820833837071302
36537,182583,0,182583,3954.5932910442352,0.00037721896684675903
36637,183083,0,183083,3964.9579350948334,0.00037247645990617516
36737,183583,0,183583,3975.144170999527,0.0003677983537082144
36837,184083,0,184083,3985.300096988678,0.0003632073892757746
36937,184583,0,184583,3995.521896123886,0.00035872169287079296
37037,185083,0,185083,4005.375247001648,0.0003543231172937472
37137,185583,0,185583,4015.2529859542847,0.0003499555631106733
37237,186083,0,186083,4025.297404050827,0.0003456091543287095
37337,186583,0,186583,4035.3080911636353,0.00034133904036296543
37437,187083,0,187083,4047.33403301239,0.0003371897041997399
37538,187588,0,187588,4061.1254189014435,0.0003330940770030127
37638,188088,0,188088,4074.0332090854645,0.00032904613341672536
37738,188588,0,188588,4086.394381046295,0.0003249776189030221
37838,189088,0,189088,4102.193630933762,0.00032095873374849646
37938,189588,0,189588,4119.534715175629,0.00031702222306425227
38038,190088,0,190088,4135.752055883408,0.00031313764609344373
38138,190588,0,190588,4151.646120786667,0.00030928319204809014
38238,191088,0,191088,4167.047230243683,0.0003054462282524585
38338,191588,0,191588,4182.352931022644,0.0003016392954409308
38438,192088,0,192088,4197.769783973694,0.0002978876644134703
38539,192593,0,192593,4213.78545498848,0.00029414997270711386
38639,193093,0,193093,4230.038600921631,0.0002904760483259826
38739,193593,0,193593,4246.434118032455,0.0002868238988232153
38839,194093,0,194093,4262.640264034271,0.0002832135956908058
38939,194593,0,194593,4279.589560031891,0.0002796467182235892
39039,195093,0,195093,4296.195240974426,0.0002761159716255151
39139,195593,0,195593,4312.778830051422,0.00027263345480684793
39239,196093,0,196093,4328.883623123169,0.00026919021860002734
39339,196593,0,196593,4346.072429895401,0.0002657728031629332
39439,197093,0,197093,4361.5704691410065,0.00026240807660154433
39540,197598,0,197598,4377.396242141724,0.0002590910973433425
39640,198098,0,198098,4393.116788864136,0.00025588265341784086
39740,198598,0,198598,4409.757657051086,0.0002527241050797486
39840,199098,0,199098,4425.880966186523,0.0002495867002298357
39940,199598,0,199598,4441.948101043701,0.0002464799047741714
40040,200098,0,200098,4458.030071973801,0.00024344507406500032
40140,200598,0,200598,4474.289134979248,0.00024049217401295308
40240,201098,0,201098,4490.09783911705,0.00023758925035202111
40340,201598,0,201598,4505.819542884827,0.0002346974720580825
40440,202098,0,202098,4522.433734178543,0.00023181002222996108
40541,202603,0,202603,4538.322981119156,0.00022892956364527054
40641,203103,0,203103,4554.054399967194,0.00022614114331804207
40741,203603,0,203603,4570.510680913925,0.00022341837448286615
40841,204103,0,204103,4586.327925920486,0.00022072753023352708
40941,204603,0,204603,4601.550536155701,0.00021802439763574777
41041,205103,0,205103,4616.743934869766,0.0002153160438144532
41141,205603,0,205603,4632.020478248596,0.00021264765748837884
41241,206103,0,206103,4647.64825797081,0.0002100345412956692
41341,206603,0,206603,4663.386606931686,0.00020745813187193632
41441,207103,0,207103,4679.035411834717,0.00020490261520566503
41542,207608,0,207608,4694.72914814949,0.00020233465972032793
41642,208108,0,208108,4710.382244110107,0.000199802884274177
41742,208608,0,208608,4727.360029935837,0.00019729182682935609
41842,209108,0,209108,4744.93544793129,0.00019481621710768968
41942,209608,0,209608,4761.359313011169,0.0001923755958623994
42042,210108,0,210108,4777.545238018036,0.0001899588719947242
42142,210608,0,210608,4793.727998256683,0.00018756344101920325
42242,211108,0,211108,4809.673326015472,0.0001851956797072706
42342,211608,0,211608,4825.901910066605,0.0001828731912447905
42442,212108,0,212108,4842.284168243408,0.00018059845025777968
42543,212613,0,212613,4858.905063152313,0.00017831601776185699
42643,213113,0,213113,4875.176419019699,0.00017606275381638659
42743,213613,0,213613,4891.423650979996,0.00017385303972389696
42843,214113,0,214113,4907.281273126602,0.00017170521327511962
42943,214613,0,214613,4923.398113965988,0.00016959968472830621
43043,215113,0,215113,4938.465106010437,0.00016750607326702926
43143,215613,0,215613,4953.645373106003,0.00016541434271077386
43243,216113,0,216113,4968.637050151825,0.00016335144342275186
43343,216613,0,216613,4984.335066080093,0.00016134497849539813
43443,217113,0,217113,5000.016824007034,0.0001593898471032139
43544,217618,0,217618,5016.038820981979,0.0001574400345603422
43644,218118,0,218118,5031.447181940079,0.00015551106209193895
43744,218618,0,218618,5046.764511823654,0.0001535865154520082
43844,219118,0,219118,5060.537490129471,0.00015168479499473708
43944,219618,0,219618,5071.468253850937,0.00014981951633575002
44044,220118,0,220118,5084.250503063202,0.00014800011208480985
44144,220618,0,220618,5095.068859100342,0.00014621436322828963
44244,221118,0,221118,5105.955325126648,0.00014442878139451362
44344,221618,0,221618,5116.180061101913,0.00014263665106754294
44444,222118,0,222118,5126.776809930801,0.00014086422000602705
44545,222623,0,222623,5136.680850028992,0.00013911567700658194
44645,223123,0,223123,5149.801614046097,0.0001374183201096502
44745,223623,0,223623,5160.80236697197,0.00013572641144805178
44845,224123,0,224123,5171.212321996689,0.0001340328188139223
44945,224623,0,224623,5182.8889808654785,0.00013236112328072992
45045,225123,0,225123,5193.261703014374,0.00013072490474152403
45145,225623,0,225623,5204.158057928085,0.00012911114446064365
45245,226123,0,226123,5214.659335136414,0.0001275024555124265
45345,226623,0,226623,5225.636590957642,0.00012590161085567313
45445,227123,0,227123,5235.858992099762,0.0001243253689193958
45546,227628,0,227628,5246.176659107208,0.00012276184114542522
45646,228128,0,228128,5256.821223020554,0.00012123236403793853
45746,228628,0,228628,5268.682576179504,0.00011971705681063681
45846,229128,0,229128,5279.8755848407745,0.00011821828297044659
45946,229628,0,229628,5290.658276081085,0.00011674246354088736
46046,230128,0,230128,5302.027095079422,0.00011529636776283101
46146,230628,0,230628,5312.606182098389,0.00011387938281053799
46246,231128,0,231128,5323.567645072937,0.00011248413550743903
46346,231628,0,231628,5333.8440721035,0.00011110133225261212
46446,232128,0,232128,5345.98227596283,0.00010973060229597501
46547,232633,0,232633,5357.968587875366,0.00010837044060160703
46647,233133,0,233133,5369.910881996155,0.00010705609787735993
46747,233633,0,233633,5380.724584102631,0.00010577023960898871
46847,234133,0,234133,5391.075186014175,0.00010449901468025544
46947,234633,0,234633,5402.657609939575,0.00010323012198943327
47047,235133,0,235133,5414.355530977249,0.0001019711063233136
47147,235633,0,235633,5425.338212013245,0.00010073847118361565
47247,236133,0,236133,5436.322461843491,9.95332678283808e-05
47347,236633,0,236633,5447.608019113541,9.834313200863676e-05
47447,237133,0,237133,5459.032230138779,9.715722569053257e-05
47548,237638,0,237638,5468.938488006592,9.596396705510397e-05
47648,238138,0,238138,5480.643612146378,9.479710229733944e-05
47748,238638,0,238638,5491.835803985596,9.364910772111053e-05
47848,239138,0,239138,5502.464318037033,9.251380757307025e-05
47948,239638,0,239638,5513.385139226913,9.13867477461328e-05
48048,240138,0,240138,5524.085081100464,9.026786264199883e-05
48148,240638,0,240638,5534.6294901371,8.915781353468074e-05
48248,241138,0,241138,5545.310627937317,8.805773416627259e-05
48348,241638,0,241638,5556.044322013855,8.69675689652116e-05
48448,242138,0,242138,5566.0253229141235,8.588622089057175e-05
48549,242643,0,242643,5576.991172075272,8.480414492731312e-05
48649,243143,0,243143,5586.782181978226,8.374749475827166e-05
48749,243643,0,243643,5596.789686918259,8.270959085165348e-05
48849,244143,0,244143,5608.708170890808,8.168875746491998e-05
48949,244643,0,244643,5619.888361930847,8.06798311353179e-05
49049,245143,0,245143,5630.383345127106,7.968206226361594e-05
49149,245643,0,245643,5640.4056968688965,7.870088224222207e-05
49249,246143,0,246143,5650.5806131362915,7.773961196312214e-05
49349,246643,0,246643,5664.6444981098175,7.679457098557647e-05
49449,247143,0,247143,5675.3483710289,7.586140452421898e-05
49550,247648,0,247648,5686.687590122223,7.492898581986418e-05
49650,248148,0,248148,5697.687673091888,7.401539953566568e-05
49750,248648,0,248648,5709.435055017471,7.311576962833046e-05
49850,249148,0,249148,5720.492058038712,7.223622243787864e-05
49950,249648,0,249648,5731.650343179703,7.137692837144109e-05
50050,250148,0,250148,5742.451267004013,7.052945389542406e-05
50150,250648,0,250648,5754.456598997116,6.96812230872659e-05
50250,251148,0,251148,5766.383048057556,6.883077822095232e-05
50350,251648,0,251648,5776.532115936279,6.799313079537122e-05
50450,252148,0,252148,5788.189209938049,6.717832156914836e-05
50551,252653,0,252653,5799.261986017227,6.63699769841229e-05
50651,253153,0,253153,5811.425168991089,6.557122498319466e-05
50751,253653,0,253653,5822.612858057022,6.477172120144465e-05
50851,254153,0,254153,5833.877405166626,6.39785325928235e-05
50951,254653,0,254653,5845.606907129288,6.3196892000334e-05
51051,255153,0,255153,5856.48584318161,6.242540291110463e-05
51151,255653,0,255653,5866.708245038986,6.166159549818611e-05
51251,256153,0,256153,5876.728462934494,6.090383717036853e-05
51351,256653,0,256653,5887.35281920433,6.015023768958237e-05
51451,257153,0,257153,5898.7205810546875,5.940073889040863e-05
51552,257658,0,257658,5911.1345472335815,5.8651865665582604e-05
51652,258158,0,258158,5925.064723968506,5.792444861161008e-05
51752,258658,0,258658,5939.021440029144,5.721048972807709e-05
51852,259158,0,259158,5950.682116031647,5.6502167509600485e-05
51952,259658,0,259658,5961.630486965179,5.5798308658219694e-05
52052,260158,0,260158,5972.797118902206,5.510701241845707e-05
52152,260658,0,260658,5984.750582933426,5.443082609636523e-05
52252,261158,0,261158,5996.236657142639,5.376211681440372e-05
52352,261658,0,261658,6006.32682800293,5.309523238551592e-05
52452,262158,0,262158,6016.70072221756,5.243602968171447e-05
52553,262663,0,262663,6029.032459020615,5.178827310196105e-05
52653,263163,0,263163,6041.968382835388,5.116432646511327e-05
52753,263663,0,263663,6052.81179690361,5.0546094355125655e-05
52853,264163,0,264163,6064.334852933884,4.992475474952824e-05
52953,264663,0,264663,6076.129531145096,4.9305458189211e-05
53053,265163,0,265163,6086.65403008461,4.870146174345732e-05
53153,265663,0,265663,6097.275139093399,4.811701072913669e-05
53253,266163,0,266163,6109.2286829948425,4.754425147170306e-05
53353,266663,0,266663,6119.959048986435,4.6974322415576416e-05
53453,267163,0,267163,6133.7770228385925,4.6403347753107346e-05
53554,267668,0,267668,6146.680429935455,4.582793347846726e-05
53654,268168,0,268168,6158.142493009567,4.52666957593962e-05
53754,268668,0,268668,6170.289953947067,4.4719194940977955e-05
53854,269168,0,269168,6181.105171918869,4.4183427521040305e-05
53954,269668,0,269668,6192.268524885178,4.365136830142839e-05
54054,270168,0,270168,6204.213971853256,4.31167376149825e-05
54154,270668,0,270668,6215.025235176086,4.258290992679035e-05
54254,271168,0,271168,6225.477875947952,4.205908285827396e-05
54354,271668,0,271668,6236.485089063644,4.1548568653170534e-05
54454,272168,0,272168,6246.922183036804,4.104464310971055e-05
54555,272673,0,272673,6257.59080696106,4.053456050487089e-05
54655,273173,0,273173,6268.075711011887,4.003101014439587e-05
54755,273673,0,273673,6279.13339805603,3.9536609048265145e-05
54855,274173,0,274173,6290.79912686348,3.905074868028278e-05
54955,274673,0,274673,6302.76767206192,3.856746088754561e-05
55055,275173,0,275173,6313.452828168869,3.808667433350143e-05
55155,275673,0,275673,6324.294550895691,3.761361509352135e-05
55255,276173,0,276173,6336.340926170349,3.715133146176335e-05
55355,276673,0,276673,6346.533806085587,3.669761805121421e-05
55455,277173,0,277173,6357.025889873505,3.624803255944671e-05
55556,277678,0,277678,6367.056698083878,3.579695148717814e-05
55656,278178,0,278178,6379.1499218940735,3.535638456565927e-05
55756,278678,0,278678,6391.788635015488,3.492468851005458e-05
55856,279178,0,279178,6402.51203083992,3.4501966117265636e-05
55956,279678,0,279678,6412.714081048965,3.408698164918513e-05
56056,280178,0,280178,6424.369830131531,3.367725370251476e-05
56156,280678,0,280678,6436.093647956848,3.3269482232394996e-05
56256,281178,0,281178,6447.307321071625,3.286428965720167e-05
56356,281678,0,281678,6459.3706040382385,3.24669249857232e-05
56456,282178,0,282178,6471.490961074829,3.208024682398501e-05
56557,282683,0,282683,6482.914742946625,3.169744112148325e-05
56657,283183,0,283183,6494.129553079605,3.1321034590272914e-05
56757,283683,0,283683,6505.204050064087,3.094515801096704e-05
56857,284183,0,284183,6515.903891086578,3.057238034810527e-05
56957,284683,0,284683,6526.247464895248,3.020649591614506e-05
57057,285183,0,285183,6536.924968957901,2.9847595156331716e-05
57157,285683,0,285683,6546.851748943329,2.9492154503065965e-05
57257,286183,0,286183,6556.6168801784515,2.913746429593703e-05
57357,286683,0,286683,6566.864846944809,2.8784420646033977e-05
57457,287183,0,287183,6577.05441904068,2.843532848160415e-05
57558,287688,0,287688,6587.2089920043945,2.8087189030733185e-05
57658,288188,0,288188,6597.35404419899,2.7745860106050404e-05
57758,288688,0,288688,6607.326265096664,2.7407162839921218e-05
57858,289188,0,289188,6617.126899957657,2.7071326266381847e-05
57958,289688,0,289688,6627.1219618320465,2.6739190178275027e-05
58058,290188,0,290188,6637.546228885651,2.6410925229716104e-05
58158,290688,0,290688,6648.207372903824,2.6086367958370422e-05
58258,291188,0,291188,6659.602993011475,2.5766683252885666e-05
58358,291688,0,291688,6670.1374168396,2.5452975440638598e-05
58458,292188,0,292188,6681.113091945648,2.514404787451879e-05
58559,292693,0,292693,6692.361999034882,2.4835147731110157e-05
58659,293193,0,293193,6703.0110239982605,2.453267844457917e-05
58759,293693,0,293693,6713.4556839466095,2.423452607592489e-05
58859,294193,0,294193,6723.779681921005,2.3940369527728506e-05
58959,294693,0,294693,6733.762773990631,2.3649905073596144e-05
59059,295193,0,295193,6744.086612939835,2.3364383810442608e-05
59159,295693,0,295693,6753.886604070663,2.3085114829939177e-05
59259,296193,0,296193,6763.924510002136,2.2811124086163103e-05
59359,296693,0,296693,6774.61822104454,2.2539297566656647e-05
59459,297193,0,297193,6784.747424840927,2.2268166985798894e-05
59560,297698,0,297698,6795.346617937088,2.1998025226468197e-05
59660,298198,0,298198,6805.752916812897,2.1737482353724425e-05
59760,298698,0,298698,6816.246340036392,2.1482166447829375e-05
59860,299198,0,299198,6826.596555948257,2.122781924720474e-05
59960,299698,0,299698,6837.983086109161,2.0973127821090152e-05
60060,300198,0,300198,6849.00009894371,2.072045241848122e-05
60160,300698,0,300698,6859.638548851013,2.0472132603119684e-05
60260,301198,0,301198,6870.9410190582275,2.0227903076502737e-05
60360,301698,0,301698,6881.027704954147,1.99859004894402e-05
60460,302198,0,302198,6893.978182077408,1.9744752980151056e-05
60561,302703,0,302703,6905.232540130615,1.9502097143049546e-05
60661,303203,0,303203,6916.065119981766,1.9263740048814972e-05
60761,303703,0,303703,6926.609055995941,1.9028254320624857e-05
60861,304203,0,304203,6936.42778801918,1.879640352376301e-05
60961,304703,0,304703,6949.411941051483,1.856810872955397e-05
61061,305203,0,305203,6959.861864089966,1.834152653927029e-05
61161,305703,0,305703,6969.767720937729,1.8115267056308347e-05
61261,306203,0,306203,6979.71617102623,1.7891078537923152e-05
61361,306703,0,306703,6992.218241930008,1.7671529500087545e-05
61461,307203,0,307203,7002.830684185028,1.7456300651615e-05
61562,307708,0,307708,7014.223702907562,1.724088864167901e-05
61662,308208,0,308208,7025.016810894012,1.702883657183779e-05
61762,308708,0,308708,7035.705771923065,1.6820139487432884e-05
61862,309208,0,309208,7046.708790063858,1.6616437198468514e-05
61962,309708,0,309708,7057.425010204315,1.6415781455011375e-05
62062,310208,0,310208,7068.179789066315,1.6215269491729208e-05
62162,310708,0,310708,7079.070896148682,1.6015926923471743e-05
62262,311208,0,311208,7089.849462985992,1.5821743945411168e-05
62362,311708,0,311708,7100.450437068939,1.5633682532013225e-05
62462,312208,0,312208,7110.686372041702,1.5448057925095894e-05
62563,312713,0,312713,7120.846509933472,1.5259823138989655e-05
62663,313213,0,313213,7131.936958789825,1.5073660432910923e-05
62763,313713,0,313713,7143.246261835098,1.4890539453984543e-05
62863,314213,0,314213,7153.255699872971,1.471194688591665e-05
62963,314713,0,314713,7164.991657972336,1.4537473343843078e-05
63063,315213,0,315213,7175.849265098572,1.4365525927233611e-05
63163,315713,0,315713,7186.353193998337,1.419406376977266e-05
63263,316213,0,316213,7197.1034190654755,1.4021966492575e-05
63363,316713,0,316713,7207.352340936661,1.3850582501577993e-05
63463,317213,0,317213,7217.210174798965,1.3682926077482154e-05
63564,317718,0,317718,7227.301638126373,1.351854427035557e-05
63664,318218,0,318218,7237.692618846893,1.3358002802942096e-05
63764,318718,0,318718,7248.437001943588,1.3196208161531564e-05
63864,319218,0,319218,7259.534518957138,1.3033401960233011e-05
63964,319718,0,319718,7269.617192029953,1.2872915895864413e-05
64064,320218,0,320218,7280.072406053543,1.2716411538794653e-05
64164,320718,0,320718,7290.092262983322,1.256229329689525e-05
64264,321218,0,321218,7300.259962081909,1.240884540457742e-05
64364,321718,0,321718,7311.23024892807,1.2256464403812075e-05
64464,322218,0,322218,7322.2292058467865,1.2106384198338822e-05
64565,322723,0,322723,7333.1550278663635,1.1957185940358784e-05
64665,323223,0,323223,7345.096871137619,1.1810736102235363e-05
64765,323723,0,323723,7357.874403953552,1.1665225775315255e-05
64865,324223,0,324223,7369.435894012451,1.1521857854975412e-05
64965,324723,0,324723,7380.838091850281,1.1381684996550782e-05
65065,325223,0,325223,7391.244906902313,1.1244233793864254e-05
65165,325723,0,325723,7402.2139530181885,1.110839091237824e-05
65265,326223,0,326223,7415.348847150803,1.0973628399049542e-05
65365,326723,0,326723,7426.652863025665,1.084002190681997e-05
65465,327223,0,327223,7437.020606994629,1.070808932479147e-05
65566,327728,0,327728,7447.504498004913,1.0577548709982288e-05
65666,328228,0,328228,7457.638253927231,1.0451705231888057e-05
65766,328728,0,328728,7467.821354866028,1.032857305839718e-05
65866,329228,0,329228,7480.227919101715,1.0206369491877351e-05
65966,329728,0,329728,7491.062546014786,1.0084085694189604e-05
66066,330228,0,330228,7502.000921964645,9.962796521261307e-06
66166,330728,0,330728,7512.096980810165,9.844425337186806e-06
66266,331228,0,331228,7522.149739027023,9.729233141456767e-06
66366,331728,0,331728,7532.883182048798,9.615360798668503e-06
66466,332228,0,332228,7544.056796073914,9.501110706701497e-06
66567,332733,0,332733,7555.87803196907,9.385727062177156e-06
66667,333233,0,333233,7566.945299863815,9.273100846351122e-06
66767,333733,0,333733,7579.952338218689,9.162812309478779e-06
66867,334233,0,334233,7591.248291969299,9.05419126298213e-06
66967,334733,0,334733,7601.962802171707,8.946185400333436e-06
67067,335233,0,335233,7612.834730863571,8.838327949177462e-06
67167,335733,0,335733,7622.906352043152,8.7309013665276e-06
67267,336233,0,336233,7632.966763019562,8.624506803984673e-06
67367,336733,0,336733,7644.047981023788,8.519646962427412e-06
67467,337233,0,337233,7654.224003076553,8.416529560453575e-06
67568,337738,0,337738,7664.681875944138,8.313879931990155e-06
67668,338238,0,338238,7674.693104982376,8.213176903991008e-06
67768,338738,0,338738,7685.22611284256,8.113231147006209e-06
67868,339238,0,339238,7696.519285917282,8.014448500882732e-06
67968,339738,0,339738,7707.783769130707,7.917174008170553e-06
68068,340238,0,340238,7718.804968833923,7.821235962083843e-06
68168,340738,0,340738,7731.059731245041,7.726353490189221e-06
68268,341238,0,341238,7743.393457174301,7.632733335193862e-06
68368,341738,0,341738,7754.452805042267,7.540857793780057e-06
68468,342238,0,342238,7765.899022102356,7.450726400350624e-06
68569,342743,0,342743,7777.555006027222,7.360829704940503e-06
68669,343243,0,343243,7788.8782551288605,7.272520826994498e-06
68769,343743,0,343743,7799.497274160385,7.185416877213837e-06
68869,344243,0,344243,7809.913864850998,7.10041092511972e-06
68969,344743,0,344743,7820.662106990814,7.017476141930946e-06
69069,345243,0,345243,7831.939733982086,6.935487419753565e-06
69169,345743,0,345743,7843.548296928406,6.853546824655216e-06
69269,346243,0,346243,7854.345700979233,6.772003892192333e-06
69369,346743,0,346743,7865.363977909088,6.6918603396319896e-06
69469,347243,0,347243,7876.952253103256,6.613439390162124e-06
69570,347748,0,347748,7888.399921178818,6.535255410034448e-06
69670,348248,0,348248,7898.362425088882,6.4580355621939035e-06
69770,348748,0,348748,7908.906986951828,6.380964256554013e-06
69870,349248,0,349248,7919.775504112244,6.304562553291221e-06
69970,349748,0,349748,7931.08017706871,6.229197731588296e-06
70070,350248,0,350248,7942.179601192474,6.154844301725254e-06
70170,350748,0,350748,7953.288635015488,6.0812530919903525e-06
70270,351248,0,351248,7963.603061914444,6.008062867164837e-06
70370,351748,0,351748,7973.745256900787,5.9350679201890356e-06
70470,352248,0,352248,7983.8870260715485,5.862624598788322e-06
70571,352753,0,352753,7994.222963094711,5.790686639940149e-06
70671,353253,0,353253,8004.237703084946,5.720781203751951e-06
70771,353753,0,353753,8014.349300861359,5.6515601315417865e-06
70871,354253,0,354253,8025.310355901718,5.58256227896653e-06
70971,354753,0,354753,8036.551556110382,5.514191688115782e-06
71071,355253,0,355253,8046.803771018982,5.4471488303813e-06
71171,355753,0,355753,8056.950939178467,5.381394753226443e-06
71271,356253,0,356253,8067.050184965134,5.3162605959038245e-06
71371,356753,0,356753,8077.116829872131,5.25156318847827e-06
71471,357253,0,357253,8087.104264974594,5.187943077863158e-06
71572,357758,0,357758,8097.886803150177,5.1252439720202605e-06
71672,358258,0,358258,8107.884136199951,5.064192259549665e-06
71772,358758,0,358758,8117.938899040222,5.003372443879174e-06
71872,359258,0,359258,8127.939598083496,4.942844028802305e-06
71972,359758,0,359758,8138.028110980988,4.883403931652314e-06
72072,360258,0,360258,8148.109980106354,4.825517142315816e-06
72172,360758,0,360758,8159.7845339775085,4.768811951364597e-06
72272,361258,0,361258,8170.136236906052,4.712590234626802e-06
72372,361758,0,361758,8180.233290910721,4.656510941771423e-06
72472,362258,0,362258,8190.700958967209,4.600771635839923e-06
72573,362763,0,362763,8200.763972997665,4.545319161800006e-06
72673,363263,0,363263,8211.475556135178,4.49163768046558e-06
72773,363763,0,363763,8222.078131198883,4.4390485475585575e-06
72873,364263,0,364263,8232.09399485588,4.386838637899525e-06
72973,364763,0,364763,8242.248409032822,4.3342982188364444e-06
73073,365263,0,365263,8252.175286054611,4.281576131095425e-06
73173,365763,0,365763,8262.2346200943,4.2296501639935e-06
73273,366263,0,366263,8272.853219985962,4.179175764370202e-06
73373,366763,0,366763,8282.893640041351,4.129668929193826e-06
73473,367263,0,367263,8293.163993120193,4.080178785002099e-06
73574,367768,0,367768,8303.254494905472,4.029990904521975e-06
73674,368268,0,368268,8313.2496240139,3.980724361220513e-06
73774,368768,0,368768,8323.32605791092,3.9324068003479145e-06
73874,369268,0,369268,8333.296340942383,3.884900283850381e-06
73974,369768,0,369768,8343.209218978882,3.8378132522559294e-06
74074,370268,0,370268,8353.231389045715,3.7910883191817865e-06
74174,370768,0,370768,8363.285363912582,3.74495270750956e-06
74274,371268,0,371268,8373.239120006561,3.6994887306868326e-06
74374,371768,0,371768,8383.127228021622,3.6545402768982055e-06
74474,372268,0,372268,8394.748512983322,3.610004437295071e-06
74575,372773,0,372773,8404.862775087357,3.5655550728876476e-06
74675,373273,0,373273,8415.010241985321,3.522271888103921e-06
74775,373773,0,373773,8425.035134792328,3.479859715581925e-06
74875,374273,0,374273,8434.977724075317,3.438335872023861e-06
74975,374773,0,374773,8444.935008049011,3.3974942134196173e-06
75075,375273,0,375273,8455.660915136337,3.3569935744140695e-06
75175,375773,0,375773,8465.624948978424,3.3167215376770292e-06
75275,376273,0,376273,8475.508156061172,3.2770191808049407e-06
75375,376773,0,376773,8485.63809299469,3.238339314663213e-06
75475,377273,0,377273,8495.793001890182,3.200639849545891e-06
75576,377778,0,377778,8505.812535047531,3.162932581585882e-06
75676,378278,0,378278,8515.849556922913,3.1254453042316184e-06
75776,378778,0,378778,8525.805340051651,3.088018220483115e-06
75876,379278,0,379278,8535.830066204071,3.0513405285614642e-06
75976,379778,0,379778,8546.097909927368,3.0157423691184174e-06
76076,380278,0,380278,8556.045169115067,2.98082563734777e-06
76176,380778,0,380778,8565.912060022354,2.945938597627906e-06
76276,381278,0,381278,8576.694001197815,2.910823892473102e-06
76376,381778,0,381778,8586.789266109467,2.8757570416664807e-06
76476,382278,0,382278,8596.813979148865,2.841188117774775e-06
76577,382783,0,382783,8607.062808036804,2.806981833913361e-06
76677,383283,0,383283,8618.327803134918,2.773639887322699e-06
76777,383783,0,383783,8629.469297170639,2.7405040231281728e-06
76877,384283,0,384283,8640.240701198578,2.7074447669029232e-06
76977,384783,0,384783,8651.925164937973,2.6746186950540377e-06
77077,385283,0,385283,8663.439660072327,2.6422625148284447e-06
77177,385783,0,385783,8674.401023864746,2.610430148248178e-06
77277,386283,0,386283,8684.361283063889,2.5789694714312174e-06
77377,386783,0,386783,8694.284075021744,2.5477477899275487e-06
77477,387283,0,387283,8704.403366088867,2.516831377958988e-06
77578,387788,0,387788,8714.516211986542,2.486082510242937e-06
77678,388288,0,388288,8724.568189144135,2.4561477478741123e-06
77778,388788,0,388788,8735.094249010086,2.4266042053456264e-06
77878,389288,0,389288,8745.520187139511,2.397370447835066e-06
77978,389788,0,389788,8755.776276826859,2.368549404643999e-06
78078,390288,0,390288,8765.844856977463,2.340348034409946e-06
78178,390788,0,390788,8776.663370847702,2.312812525989693e-06
78278,391288,0,391288,8786.695687055588,2.285697881548084e-06
78378,391788,0,391788,8796.759368896484,2.2587148143703633e-06
78478,392288,0,392288,8807.548408985138,2.231885488289706e-06
78579,392793,0,392793,8817.613168001175,2.205262114083957e-06
78679,393293,0,393293,8827.852659225464,2.179574121104268e-06
78779,393793,0,393793,8838.93760895729,2.1543737990090806e-06
78879,394293,0,394293,8849.883383989334,2.1293016375157224e-06
78979,394793,0,394793,8862.190739870071,2.104223237199212e-06
79079,395293,0,395293,8872.50890994072,2.0793378899130188e-06
79179,395793,0,395793,8883.631740093231,2.0548897962925964e-06
79279,396293,0,396293,8895.347617864609,2.0308694285468953e-06
79379,396793,0,396793,8907.007479906082,2.0070570583497095e-06
79479,397293,0,397293,8918.976606845856,1.983284126090729e-06
79580,397798,0,397798,8929.980680942535,1.959337509116158e-06
79680,398298,0,398298,8940.948719024658,1.9358471423802834e-06
79780,398798,0,398798,8951.548768997192,1.9127221340013505e-06
79880,399298,0,399298,8963.385838985443,1.8899760287855021e-06
79980,399798,0,399798,8976.452963113785,1.8674683572181417e-06
80080,400298,0,400298,8986.675666093826,1.84504911630453e-06
80180,400798,0,400798,8997.288135051727,1.822730084517522e-06
80280,401298,0,401298,9008.043860912323,1.8006650704767812e-06
80380,401798,0,401798,9019.685525894165,1.7789510774956006e-06
80480,402298,0,402298,9031.002485990524,1.7575092766457708e-06
80581,402803,0,402803,9041.957247018814,1.736008377650817e-06
80681,403303,0,403303,9053.494703054428,1.7149256615739081e-06
80781,403803,0,403803,9064.679111003876,1.694224009211713e-06
80881,404303,0,404303,9076.675405979156,1.6739433017325245e-06
80981,404803,0,404803,9088.728958129883,1.653918615837566e-06
81081,405303,0,405303,9100.076959848404,1.6340323035835647e-06
81181,405803,0,405803,9110.291207075119,1.614396647301692e-06
81281,406303,0,406303,9120.585021018982,1.595188215227578e-06
81381,406803,0,406803,9130.671277046204,1.576394034450736e-06
81481,407303,0,407303,9141.113435029984,1.5578271858809005e-06
81582,407808,0,407808,9153.397113084793,1.539174287682051e-06
81682,408308,0,408308,9164.156883239746,1.5208703338087525e-06
81782,408808,0,408808,9174.789902925491,1.5028880935384535e-06
81882,409308,0,409308,9184.785419940948,1.4852880986081142e-06
81982,409808,0,409808,9194.869901895523,1.467969979540936e-06
82082,410308,0,410308,9205.201012849808,1.4507735754026616e-06
82182,410808,0,410808,9216.057704210281,1.4336198508094424e-06
82282,411308,0,411308,9226.316649913788,1.4165787062829164e-06
82382,411808,0,411808,9237.442347049713,1.3998155182539427e-06
82482,412308,0,412308,9248.875534057617,1.3834235588149686e-06
82583,412813,0,412813,9260.516491889954,1.367128533762217e-06
82683,413313,0,413313,9273.894635915756,1.3510243339280215e-06
82783,413813,0,413813,9288.989939212799,1.3348636529034483e-06
82883,414313,0,414313,9307.07862997055,1.3188013965027595e-06
82983,414813,0,414813,9321.508517026901,1.3030399118081953e-06
83083,415313,0,415313,9335.148608922958,1.2875877165294154e-06
83183,415813,0,415813,9347.1849629879,1.272271387542137e-06
83283,416313,0,416313,9359.586441993713,1.2569718792905136e-06
83383,416813,0,416813,9370.791877985,1.241768459846931e-06
83483,417313,0,417313,9385.862338066101,1.226809561698296e-06
83584,417818,0,417818,9401.746915102005,1.2119654003170777e-06
83684,418318,0,418318,9417.44703412056,1.1974202555366888e-06
83784,418818,0,418818,9434.063554048538,1.1829598561404605e-06
83884,419318,0,419318,9451.605717897415,1.1686310679546217e-06
83984,419818,0,419818,9466.542996883392,1.1545103355095708e-06
84084,420318,0,420318,9479.290688037872,1.1406150658179736e-06
84184,420818,0,420818,9492.005101919174,1.126904111113114e-06
84284,421318,0,421318,9504.622109889984,1.1133391927262904e-06
84384,421818,0,421818,9520.028578996658,1.0999434662189247e-06
84484,422318,0,422318,9533.47388792038,1.08680125591519e-06
84585,422823,0,422823,9547.546399831772,1.0738497766797403e-06
84685,423323,0,423323,9561.360790967941,1.0612907740686426e-06
84785,423823,0,423823,9574.861290931702,1.0488388533110951e-06
84885,424323,0,424323,9588.487112045288,1.0363937218026013e-06
84985,424823,0,424823,9601.15775513649,1.0240374727506334e-06
85085,425323,0,425323,9615.091645002365,1.0119574546266437e-06
85185,425823,0,425823,9627.830102920532,1.0002279036832895e-06
85285,426323,0,426323,9642.542552947998,9.88709477066939e-07
85385,426823,0,426823,9655.59915304184,9.771949083304086e-07
85485,427323,0,427323,9669.32161617279,9.656266706509858e-07
85586,427828,0,427828,9682.696079015732,9.540283847683607e-07
85686,428328,0,428328,9695.490464925766,9.428041318476358e-07
85786,428828,0,428828,9708.276285171509,9.318601359038285e-07
85886,429328,0,429328,9722.775444984436,9.21047590502841e-07
85986,429828,0,429828,9736.677142858505,9.102091743055808e-07
86086,430328,0,430328,9751.191452026367,8.993390385924364e-07
86186,430828,0,430828,9764.710792064667,8.885633598470528e-07
86286,431328,0,431328,9778.272904872894,8.779833926057646e-07
86386,431828,0,431828,9791.593980073929,8.675763132781875e-07
86486,432328,0,432328,9804.823837041855,8.572519797554856e-07
86587,432833,0,432833,9818.734462022781,8.468645578197761e-07
86687,433333,0,433333,9832.866523981094,8.366543974243173e-07
86787,433833,0,433833,9846.515981912613,8.265660551735608e-07
86887,434333,0,434333,9860.538617134094,8.166024854378622e-07
86987,434833,0,434833,9874.071400880814,8.067367722541181e-07
87087,435333,0,435333,9887.07683300972,7.969640997202253e-07
87187,435833,0,435833,9900.298805952072,7.873236356098735e-07
87287,436333,0,436333,9913.12799501419,7.778678890753506e-07
87387,436833,0,436833,9925.999376058578,7.686071819970119e-07
87487,437333,0,437333,9939.52075791359,7.594861394654874e-07
87588,437838,0,437838,9952.78317785263,7.503447309879999e-07
87688,438338,0,438338,9965.406202077866,7.413655187322485e-07
87788,438838,0,438838,9978.333084106445,7.325415044509022e-07
87888,439338,0,439338,9991.488641023636,7.239395544253552e-07
87988,439838,0,439838,10004.347578048706,7.155149277502511e-07
88088,440338,0,440338,10017.165160179138,7.071486520630352e-07
88188,440838,0,440838,10030.396478176117,6.987842483304137e-07
88288,441338,0,441338,10043.297369003296,6.904980867258026e-07
88388,441838,0,441838,10056.026651144028,6.824094175438729e-07
88488,442338,0,442338,10069.02336883545,6.745346444418822e-07
88589,442843,0,442843,10082.082602977753,6.666886989286523e-07
88689,443343,0,443343,10095.540673017502,6.589189160145157e-07
88789,443843,0,443843,10108.25803399086,6.511470289268204e-07
88889,444343,0,444343,10121.039928913116,6.434507722597442e-07
88989,444843,0,444843,10134.374951124191,6.358876324817013e-07
89089,445343,0,445343,10148.264940977097,6.284461048901472e-07
89189,445843,0,445843,10161.012730121613,6.21073984934571e-07
89289,446343,0,446343,10173.661363124847,6.137305530707677e-07
89389,446843,0,446843,10186.471033096313,6.064151666382232e-07
89489,447343,0,447343,10199.385757923126,5.991615201109122e-07
89590,447848,0,447848,10212.901964902878,5.919333547295761e-07
89690,448348,0,448348,10225.714333057404,5.848721390347853e-07
89790,448848,0,448848,10238.403115034103,5.778690989340779e-07
89890,449348,0,449348,10251.078357934952,5.709035383388992e-07
89990,449848,0,449848,10263.78957104683,5.640067020564769e-07
90090,450348,0,450348,10276.35076713562,5.572220934647574e-07
90190,450848,0,450848,10289.064678192139,5.505419988977327e-07
90290,451348,0,451348,10301.83118891716,5.439215470794279e-07
90390,451848,0,451848,10314.52474784851,5.373548007262276e-07
90490,452348,0,452348,10327.07319688797,5.30893855805643e-07
90591,452853,0,452853,10340.449472904205,5.245140751246722e-07
90691,453353,0,453353,10353.376642942429,5.183089174233402e-07
90791,453853,0,453853,10367.045224189758,5.121567061821848e-07
90891,454353,0,454353,10379.859923124313,5.060548737970674e-07
90991,454853,0,454853,10392.486715078354,5.000575152824616e-07
91091,455353,0,455353,10405.314053058624,4.94199881362548e-07
91191,455853,0,455853,10417.923154115677,4.884514677237207e-07
91291,456353,0,456353,10430.571514129639,4.827546020805439e-07
91391,456853,0,456853,10444.262926101685,4.77087146026773e-07
91491,457353,0,457353,10456.925355911255,4.7147303006827536e-07
91592,457858,0,457858,10469.738337039948,4.658935648248148e-07
91692,458358,0,458358,10482.222696065903,4.6047473921125185e-07
91792,458858,0,458858,10494.986747980118,4.5514144822299656e-07
91892,459358,0,459358,10508.133114099503,4.498502128584671e-07
91992,459858,0,459858,10521.504952907562,4.445722638312317e-07
92092,460358,0,460358,10534.521472930908,4.393279957765096e-07
92192,460858,0,460858,10547.328594207764,4.341673887932187e-07
92292,461358,0,461358,10560.223947048187,4.291073454532109e-07
92392,461858,0,461858,10573.135232925415,4.241047301347092e-07
92492,462358,0,462358,10586.174937009811,4.1910748674936426e-07
92593,462863,0,462863,10599.007339000702,4.140695833550609e-07
92693,463363,0,463363,10612.064541816711,4.091405825935459e-07
92793,463863,0,463863,10624.618805885315,4.042958343224479e-07
92893,464363,0,464363,10637.746643066406,3.9950695492971593e-07
92993,464863,0,464863,10654.493494987488,3.9473872726521834e-07
93093,465363,0,465363,10669.731975078583,3.8999822328826155e-07
93193,465863,0,465863,10685.405428886414,3.853191905985674e-07
93293,466363,0,466363,10700.866775989532,3.8071448934806765e-07
93393,466863,0,466863,10714.122199058533,3.761654550541832e-07
93493,467363,0,467363,10728.293938159943,3.7165515673551745e-07
93594,467868,0,467868,10741.697640895844,3.6715155353449804e-07
93694,468368,0,468368,10754.912420034409,3.627723516319842e-07
93794,468868,0,468868,10768.439208984375,3.584817718186077e-07
93894,469368,0,469368,10781.25291800499,3.5425617427110855e-07
93994,469868,0,469868,10793.950731992722,3.5006336378189063e-07
94094,470368,0,470368,10806.909447193146,3.4589761576338323e-07
94194,470868,0,470868,10820.22015094757,3.41788180926873e-07
94294,471368,0,471368,10833.476355075836,3.377716317616492e-07
94394,471868,0,471868,10846.660092115402,3.338523163528971e-07
94494,472368,0,472368,10859.99115896225,3.299900266084305e-07
94595,472873,0,472873,10874.136531114578,3.2609612514685875e-07
94695,473373,0,473373,10887.7418050766,3.222403130137195e-07
94795,473873,0,473873,10901.060275793076,3.184308192479056e-07
94895,474373,0,474373,10914.09284901619,3.147189226859762e-07
94995,474873,0,474873,10926.993079900742,3.1110138488153563e-07
95095,475373,0,475373,10941.072956085205,3.0752029780828136e-07
95195,475873,0,475873,10954.160082101822,3.039257673050809e-07
95295,476373,0,476373,10967.299841880798,3.0032870180524155e-07
95395,476873,0,476873,10981.056184053421,2.967816506133494e-07
95495,477373,0,477373,10994.007575035095,2.93314823603615e-07
95596,477878,0,477878,11007.013916015625,2.898717945610179e-07
95696,478378,0,478378,11020.664552927017,2.864773027479392e-07
95796,478878,0,478878,11034.746318101883,2.830801499500689e-07
95896,479378,0,479378,11047.868606805801,2.79697442317601e-07
95996,479878,0,479878,11060.411998987198,2.763528094948653e-07
96096,480378,0,480378,11073.8444378376,2.7305283433312867e-07
96196,480878,0,480878,11086.450933933258,2.6978984696796766e-07
96296,481378,0,481378,11099.651950120926,2.665586193558936e-07
96396,481878,0,481878,11112.449972867966,2.6336339553895497e-07
96496,482378,0,482378,11125.6771838665,2.60210085782993e-07
96597,482883,0,482883,11138.553885936737,2.5706654168937546e-07
96697,483383,0,483383,11152.460648059845,2.5398810678479437e-07
96797,483883,0,483883,11165.196208000183,2.5094041796416254e-07
96897,484383,0,484383,11177.777813911438,2.479315489293004e-07
96997,484883,0,484883,11190.917102098465,2.4497626599950387e-07
97097,485383,0,485383,11204.116236925125,2.420795392259713e-07
97197,485883,0,485883,11217.065440893173,2.3922438097890714e-07
97297,486383,0,486383,11229.770483970642,2.3638398417627645e-07
97397,486883,0,486883,11242.722643852234,2.3355292838287652e-07
97497,487383,0,487383,11255.535018920898,2.307621329794332e-07
97598,487888,0,487888,11268.552514076233,2.2802403602709497e-07
97698,488388,0,488388,11281.13172698021,2.253929128398195e-07
97798,488888,0,488888,11293.737134933472,2.2279463636503166e-07
97898,489388,0,489388,11306.471274852753,2.2018443844183878e-07
97998,489888,0,489888,11319.118954896927,2.1756671343567745e-07
98098,490388,0,490388,11332.065693855286,2.1498479523494467e-07
98198,490888,0,490888,11344.99044919014,2.1247019592222995e-07
98298,491388,0,491388,11357.652485132217,2.100133635687261e-07
98398,491888,0,491888,11370.233179092407,2.0758136485339637e-07
98498,492388,0,492388,11382.912325143814,2.0515183591758173e-07
98599,492893,0,492893,11395.797316074371,2.0270312197099453e-07
98699,493393,0,493393,11410.707262992859,2.0030192815790147e-07
98799,493893,0,493893,11424.639863014221,1.9793972521497838e-07
98899,494393,0,494393,11439.30077791214,1.9561670399271592e-07
98999,494893,0,494893,11455.605652809143,1.9331718154504723e-07
99099,495393,0,495393,11469.480743169785,1.9102492818857112e-07
99199,495893,0,495893,11483.159214019775,1.8874075588192863e-07
99299,496393,0,496393,11495.787558078766,1.8648043337005755e-07
99399,496893,0,496893,11508.550247192383,1.8425358087527368e-07
99499,497393,0,497393,11524.668349027634,1.820528808003072e-07
99600,497898,0,497898,11538.51731300354,1.798478277600863e-07
99700,498398,0,498398,11551.692916870117,1.7768914180874953e-07
99800,498898,0,498898,11565.631859064102,1.7556845899534468e-07
99900,499398,0,499398,11579.3521630764,1.734841473779228e-07
100000,499898,0,499898,11592.777736902237,1.7141988818164217e-07


==> plot_data/quadratic_minimax_problem_n500_alpha00001/graal.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007808208465576172,30.358106049564984
200,201,200,401,0.0998227596282959,2.414250482001093
400,401,400,801,0.22975373268127441,1.4275908626167872
601,602,601,1203,0.3741638660430908,1.0481327108822946
801,802,801,1603,0.4691016674041748,0.8429375202786947
1001,1002,1001,2003,0.5529468059539795,0.712546757650721
1201,1202,1201,2403,0.6229298114776611,0.6216049129860671
1401,1402,1401,2803,0.6938376426696777,0.5537429058139829
1602,1603,1602,3205,0.7582828998565674,0.5000986009063654
1802,1803,1802,3605,0.826683759689331,0.45667916724582736
2002,2003,2002,4005,0.8925986289978027,0.4202781269214063
2202,2203,2202,4405,0.9591360092163086,0.3891795414674984
2402,2403,2402,4805,1.0277667045593262,0.3622391831349261
2603,2604,2603,5207,1.0952939987182617,0.3384582011656795
2803,2804,2803,5607,1.1621119976043701,0.31752317710822264
3003,3004,3003,6007,1.2292418479919434,0.29883215313746203
3203,3204,3203,6407,1.2940788269042969,0.2819775426177739
3403,3404,3403,6807,1.3601548671722412,0.26670561631211803
3604,3605,3604,7209,1.4431788921356201,0.25276560852787017
3804,3805,3804,7609,1.5205450057983398,0.2401055723226409
4004,4005,4004,8009,1.585622787475586,0.22846023614234734
4204,4205,4204,8409,1.655843734741211,0.21770086095284105
4404,4405,4404,8809,1.7517130374908447,0.20775800709081435
4605,4606,4605,9211,1.8446357250213623,0.1985038770076265
4805,4806,4805,9611,1.9472477436065674,0.18990251157422125
5005,5006,5005,10011,2.0685219764709473,0.1818747411628254
5205,5206,5205,10411,2.2111048698425293,0.17434340626448766
5405,5406,5405,10811,2.3722238540649414,0.16728300153126816
5606,5607,5606,11213,2.5538408756256104,0.160633268379683
5806,5807,5806,11613,2.6838557720184326,0.15441655428221882
6006,6007,6006,12013,2.795325994491577,0.14851457510308494
6206,6207,6206,12413,2.8963546752929688,0.14294923202773954
6406,6407,6406,12813,3.02213191986084,0.13771396492213575
6607,6608,6607,13215,3.1218698024749756,0.1327078081501456
6807,6808,6807,13615,3.197584867477417,0.1279733204842423
7007,7008,7007,14015,3.270822763442993,0.1234929697394868
7207,7208,7207,14415,3.33375883102417,0.11924831821808715
7407,7408,7407,14815,3.3939709663391113,0.11520151401373714
7608,7609,7608,15217,3.4551918506622314,0.11130828412606891
7808,7809,7808,15617,3.5261318683624268,0.10763225790397134
8008,8009,8008,16017,3.587575674057007,0.10410544232711587
8208,8209,8208,16417,3.6487040519714355,0.1007179744877205
8408,8409,8408,16817,3.711887836456299,0.09746696840937676
8609,8610,8609,17219,3.772451877593994,0.09434882795438675
8809,8810,8809,17619,3.8359789848327637,0.09137534470607764
9009,9010,9009,18019,3.8959407806396484,0.0885193771554489
9209,9210,9209,18419,3.9575066566467285,0.08578457445722024
9409,9410,9409,18819,4.021582841873169,0.08316491320092234
9610,9611,9610,19221,4.085938930511475,0.08062202500580945
9810,9811,9810,19621,4.148967981338501,0.0781987404264939
10010,10011,10010,20021,4.216129779815674,0.07587040387611937
10210,10211,10210,20421,4.282110929489136,0.07362716634542461
10410,10411,10410,20821,4.3428590297698975,0.07146898013709031
10611,10612,10611,21223,4.4074718952178955,0.06939222244711075
10811,10812,10811,21623,4.470516920089722,0.06740602586817149
11011,11012,11011,22023,4.540755987167358,0.06547371912052025
11211,11212,11211,22423,4.616089820861816,0.06359931972978485
11411,11412,11411,22823,4.691934823989868,0.0618161493160939
11612,11613,11612,23225,4.77783989906311,0.06008443835215906
11812,11813,11812,23625,4.863937616348267,0.05842555290063512
12012,12013,12012,24025,4.940488815307617,0.05681918985701662
12212,12213,12212,24425,5.0184009075164795,0.05526606485487973
12412,12413,12412,24825,5.091875791549683,0.05375274885738671
12613,12614,12613,25227,5.164814710617065,0.05228513371423172
12813,12814,12813,25627,5.241544961929321,0.05087511391319227
13013,13014,13013,26027,5.328923940658569,0.049522783486822604
13213,13214,13213,26427,5.402685880661011,0.04820197361145632
13413,13414,13413,26827,5.47279691696167,0.04693521698349971
13614,13615,13614,27229,5.550067901611328,0.045706745813395094
13814,13815,13814,27629,5.628948926925659,0.04452360855372407
14014,14015,14014,28029,5.703023910522461,0.0433763721780153
14214,14215,14214,28429,5.770842790603638,0.04226061105568543
14414,14415,14414,28829,5.833544969558716,0.04118127656962729
14615,14616,14615,29231,5.907144784927368,0.0401316692196825
14815,14816,14815,29631,5.976404905319214,0.03911041866917804
15015,15016,15015,30031,6.049389839172363,0.03813405903053661
15215,15216,15215,30431,6.112715005874634,0.03719165623735689
15415,15416,15415,30831,6.176487922668457,0.03626697015308906
15616,15617,15616,31233,6.251130819320679,0.03535864291108896
15816,15817,15816,31633,6.320572853088379,0.034494222993455295
16016,16017,16016,32033,6.394276857376099,0.03365678154923456
16216,16217,16216,32433,6.469841957092285,0.032845838033466045
16416,16417,16416,32833,6.5453996658325195,0.032061208749318754
16617,16618,16617,33235,6.612817764282227,0.03129721841714124
16817,16818,16817,33635,6.7028748989105225,0.030556098940941044
17017,17018,17017,34035,6.790320873260498,0.02984051176722835
17217,17218,17217,34435,6.862180709838867,0.029142401033406744
17417,17418,17417,34835,6.929933786392212,0.028470800358547748
17618,17619,17618,35237,7.0103278160095215,0.027805739275565008
17818,17819,17818,35637,7.085132837295532,0.027168587461877294
18018,18019,18018,36037,7.172886610031128,0.026542462800522252
18218,18219,18218,36437,7.241873741149902,0.025937138597594767
18418,18419,18418,36837,7.304742813110352,0.025348137806732438
18619,18620,18619,37239,7.36555290222168,0.024778349241448845
18819,18820,18819,37639,7.432898759841919,0.024220654667310187
19019,19020,19019,38039,7.508040904998779,0.023678878924503273
19219,19220,19219,38439,7.588047742843628,0.02315031703978796
19419,19420,19419,38839,7.655030727386475,0.02264257839251141
19620,19621,19620,39241,7.72562575340271,0.022151147579476792
19820,19821,19820,39641,7.7916176319122314,0.021672090117837047
20020,20021,20020,40041,7.858196973800659,0.02120921831064929
20220,20221,20220,40441,7.925842761993408,0.02075570698828225
20420,20421,20420,40841,8.008630752563477,0.02031370878660496
20621,20622,20621,41243,8.07701563835144,0.019879977638748533
20821,20822,20821,41643,8.145489931106567,0.019461332292364485
21021,21022,21021,42043,8.210661888122559,0.01905270173018761
21221,21222,21221,42443,8.284356832504272,0.018655438567671153
21421,21422,21421,42843,8.36153769493103,0.01826461329502448
21622,21623,21622,43245,8.431259870529175,0.017883178399155375
21822,21823,21822,43645,8.51243281364441,0.017513143034382662
22022,22023,22022,44045,8.596333742141724,0.01715455890696065
22222,22223,22222,44445,8.66556978225708,0.016803639978213655
22422,22423,22422,44845,8.735138654708862,0.016460030699083934
22623,22624,22623,45247,8.817302703857422,0.016127447412081736
22823,22824,22823,45647,8.91060996055603,0.015801860181463883
23023,23024,23023,46047,9.005409002304077,0.015485163393882322
23223,23224,23223,46447,9.101175785064697,0.015178813136378878
23423,23424,23423,46847,9.214393854141235,0.014878525182719083
23624,23625,23624,47249,9.30024766921997,0.014585243934590297
23824,23825,23824,47649,9.389579057693481,0.014297362178958349
24024,24025,24024,48049,9.479281902313232,0.01401645597216914
24224,24225,24224,48449,9.575916767120361,0.013744226255763914
24424,24425,24424,48849,9.639563798904419,0.013477770026210168
24625,24626,24625,49251,9.702123880386353,0.01321594361264385
24825,24826,24825,49651,9.763345956802368,0.01296429246837232
25025,25026,25025,50051,9.831681728363037,0.012717620000985775
25225,25226,25225,50451,9.897501945495605,0.012478225383583879
25425,25426,25425,50851,9.965598821640015,0.012244582484215888
25626,25627,25626,51253,10.038213729858398,0.012015557704819681
25826,25827,25826,51653,10.103692770004272,0.01179130703147413
26026,26027,26026,52053,10.171680927276611,0.011571882118872726
26226,26227,26226,52453,10.236456871032715,0.011355654830260733
26426,26427,26426,52853,10.299535751342773,0.011148219667720513
26627,26628,26627,53255,10.36247181892395,0.010943676907023008
26827,26828,26827,53655,10.42749285697937,0.01074522513160762
27027,27028,27027,54055,10.489075899124146,0.010548775920777511
27227,27228,27227,54455,10.556520938873291,0.010358722082939848
27427,27428,27427,54855,10.620369911193848,0.010172159658524638
27628,27629,27628,55257,10.68336796760559,0.009988764060444055
27828,27829,27828,55657,10.745329856872559,0.009813163371585729
28028,28029,28028,56057,10.803769826889038,0.009638983575030355
28228,28229,28228,56457,10.866344928741455,0.009467965790070835
28428,28429,28428,56857,10.93319582939148,0.009300625776855543
28629,28630,28629,57259,11.009480953216553,0.009136602769963467
28829,28830,28829,57659,11.078519821166992,0.008975902937212192
29029,29030,29029,58059,11.13966679573059,0.008818024394642158
29229,29230,29229,58459,11.197703838348389,0.00866292883888886
29429,29430,29429,58859,11.257059812545776,0.008511678026513717
29630,29631,29630,59261,11.31827998161316,0.008363218844996047
29830,29831,29830,59661,11.378100872039795,0.008216051498970374
30030,30031,30030,60061,11.437477827072144,0.008073663848700455
30230,30231,30230,60461,11.497763872146606,0.007934750631176627
30430,30431,30430,60861,11.563050985336304,0.007798140666873259
30631,30632,30631,61263,11.625550746917725,0.007662623076051517
30831,30832,30831,61663,11.689152956008911,0.007533805220532293
31031,31032,31031,62063,11.749683856964111,0.007404610967447344
31231,31232,31231,62463,11.808461666107178,0.00728022952838245
31431,31432,31431,62863,11.86711072921753,0.007158144334321176
31632,31633,31632,63265,11.92573595046997,0.007037952484911452
31832,31833,31832,63665,11.988050937652588,0.006920325767066486
32032,32033,32032,64065,12.052917957305908,0.0068042998434466595
32232,32233,32232,64465,12.116415023803711,0.0066914444469923905
32432,32433,32432,64865,12.217423915863037,0.006581723560901589
32633,32634,32633,65267,12.290897846221924,0.006472507824112722
32833,32834,32833,65667,12.361841917037964,0.006366363710213357
33033,33034,33033,66067,12.437455892562866,0.006262015618217894
33233,33234,33233,66467,12.52313494682312,0.006159532537137357
33433,33434,33433,66867,12.603120803833008,0.006058832312036503
33634,33635,33634,67269,12.680173873901367,0.0059606195867872
33834,33835,33834,67669,12.752911806106567,0.005864351565763597
34034,34035,34034,68069,12.827451944351196,0.005768973366694284
34234,34235,34234,68469,12.890244722366333,0.005675764774787819
34434,34435,34434,68869,12.951738834381104,0.005584832012078923
34635,34636,34635,69271,13.018412828445435,0.005493306709717078
34835,34836,34835,69671,13.12154769897461,0.00540449770885505
35035,35036,35035,70071,13.20741081237793,0.005317348312845285
35235,35236,35235,70471,13.277415752410889,0.005231947250737163
35435,35436,35435,70871,13.345885992050171,0.00514782201418232
35636,35637,35636,71273,13.421756744384766,0.005065554524006182
35836,35837,35836,71673,13.503736734390259,0.00498479457631076
36036,36037,36036,72073,13.583715677261353,0.004906358614123558
36236,36237,36236,72473,13.660415887832642,0.004827827470599538
36436,36437,36436,72873,13.754400968551636,0.004752128129901982
36637,36638,36637,73275,13.822187900543213,0.004676998180425202
36837,36838,36837,73675,13.892031908035278,0.004603554237245189
37037,37038,37037,74075,13.959884643554688,0.004531881341661738
37237,37238,37237,74475,14.033780813217163,0.004462223226885377
37437,37438,37437,74875,14.132718801498413,0.004393187752783643
37638,37639,37638,75277,14.233873844146729,0.00432441711561532
37838,37839,37838,75677,14.371985912322998,0.004256883467388916
38038,38039,38038,76077,14.462279796600342,0.004190689686153657
38238,38239,38238,76477,14.563907861709595,0.004126787870819854
38438,38439,38438,76877,14.656815767288208,0.00406433357007835
38639,38640,38639,77279,14.748534679412842,0.004001716479706899
38839,38840,38839,77679,14.809635877609253,0.003940384703575844
39039,39040,39039,78079,14.880784749984741,0.003880924798548449
39239,39240,39239,78479,14.945762634277344,0.0038228121366734066
39439,39440,39439,78879,15.009676694869995,0.003764360096574885
39640,39641,39640,79281,15.076802730560303,0.0037067996330946997
39840,39841,39840,79681,15.14657998085022,0.003650440390922143
40040,40041,40040,80081,15.220487833023071,0.0035954524551109544
40240,40241,40240,80481,15.304881811141968,0.003540610701209632
40440,40441,40440,80881,15.374084711074829,0.0034867425605838265
40641,40642,40641,81283,15.438676834106445,0.0034334999285360987
40841,40842,40841,81683,15.511445045471191,0.003381513462800075
41041,41042,41041,82083,15.584027767181396,0.0033291338453381785
41241,41242,41241,82483,15.647459745407104,0.0032788073218907184
41441,41442,41441,82883,15.718439817428589,0.0032295807210981444
41642,41643,41642,83285,15.786356925964355,0.0031803058117023703
41842,41843,41842,83685,15.851436853408813,0.003131895555236221
42042,42043,42042,84085,15.920766830444336,0.003085091861613188
42242,42243,42242,84485,15.986969709396362,0.0030386227745741803
42442,42443,42442,84885,16.05426788330078,0.0029931437585829397
42643,42644,42643,85287,16.123273849487305,0.002947558377769868
42843,42844,42843,85687,16.189010858535767,0.0029029578458183844
43043,43044,43043,86087,16.25371789932251,0.0028602814351204155
43243,43244,43243,86487,16.3186297416687,0.0028183875158611428
43443,43444,43443,86887,16.392581939697266,0.0027765025285384957
43644,43645,43644,87289,16.459617614746094,0.0027351757125747317
43844,43845,43844,87689,16.530570030212402,0.0026948025095869
44044,44045,44044,88089,16.59780478477478,0.0026554861101548404
44244,44245,44244,88489,16.667418718338013,0.0026166536366824178
44444,44445,44444,88889,16.73674964904785,0.0025781487494501874
44645,44646,44645,89291,16.804128885269165,0.0025401004267223575
44845,44846,44845,89691,16.868340969085693,0.002502670875081852
45045,45046,45045,90091,16.942838668823242,0.0024660908620435257
45245,45246,45245,90491,17.01849389076233,0.0024297484740241023
45445,45446,45445,90891,17.092187881469727,0.0023945898657533634
45646,45647,45646,91293,17.17642879486084,0.002359495924673806
45846,45847,45846,91693,17.25420379638672,0.002324312954622752
46046,46047,46046,92093,17.325815677642822,0.0022905734822706177
46246,46247,46246,92493,17.416401863098145,0.0022572288759543264
46446,46447,46446,92893,17.493868827819824,0.0022240926990488748
46647,46648,46647,93295,17.56468892097473,0.0021912751721729594
46847,46848,46847,93695,17.639939785003662,0.002159044420522511
47047,47048,47047,94095,17.706451892852783,0.0021277474055163763
47247,47248,47247,94495,17.776371955871582,0.0020967624176808928
47447,47448,47447,94895,17.853158950805664,0.0020660158741620228
47648,47649,47648,95297,17.922785758972168,0.0020357121738329887
47848,47849,47848,95697,17.98897385597229,0.0020065025203099933
48048,48049,48048,96097,18.06256103515625,0.0019774418100411977
48248,48249,48248,96497,18.125463724136353,0.0019484401490789073
48448,48449,48448,96897,18.193220853805542,0.001920249382427428
48649,48650,48649,97299,18.25882601737976,0.0018925841498516108
48849,48850,48849,97699,18.358308792114258,0.0018651858688157736
49049,49050,49049,98099,18.448017835617065,0.00183845475060204
49249,49250,49249,98499,18.546611785888672,0.0018120057084521023
49449,49450,49449,98899,18.660993814468384,0.0017861424962992067
49650,49651,49650,99301,18.77947187423706,0.0017604834723886778
49850,49851,49850,99701,18.95735502243042,0.001735423415429767
50050,50051,50050,100101,19.12859082221985,0.0017113103824172341
50250,50251,50250,100501,19.23507571220398,0.0016872408695702877
50450,50451,50450,100901,19.334600925445557,0.0016633012642137846
50651,50652,50651,101303,19.427254676818848,0.0016396682472135512
50851,50852,50851,101703,19.556941747665405,0.0016169950820499877
51051,51052,51051,102103,19.700292825698853,0.0015944675560115307
51251,51252,51251,102503,19.783323764801025,0.0015716622090984887
51451,51452,51451,102903,19.857956886291504,0.0015492553900764248
51652,51653,51652,103305,19.921722888946533,0.001527176303403981
51852,51853,51852,103705,19.98626685142517,0.001505445349073074
52052,52053,52052,104105,20.058103799819946,0.001484245856792927
52252,52253,52252,104505,20.118204832077026,0.0014629445411834046
52452,52453,52452,104905,20.180480003356934,0.0014421049889295926
52653,52654,52653,105307,20.24366593360901,0.0014214444338141385
52853,52854,52853,105707,20.344700813293457,0.0014011662784877354
53053,53054,53053,106107,20.460314750671387,0.0013813471286380874
53253,53254,53253,106507,20.64758563041687,0.001361516242499634
53453,53454,53453,106907,20.795440912246704,0.0013420694852652086
53654,53655,53654,107309,20.950684785842896,0.0013229857804086388
53854,53855,53854,107709,21.072896003723145,0.0013041680220790717
54054,54055,54054,108109,21.162375926971436,0.001285681193302624
54254,54255,54254,108509,21.254411697387695,0.0012674397307182532
54454,54455,54454,108909,21.340853929519653,0.0012494631133587516
54655,54656,54655,109311,21.430083751678467,0.0012317951624588018
54855,54856,54855,109711,21.56891703605652,0.001214740451435602
55055,55056,55055,110111,21.681241750717163,0.001198068908133733
55255,55256,55255,110511,21.870383739471436,0.0011813586308002065
55455,55456,55455,110911,22.005879640579224,0.001164898014376947
55656,55657,55656,111313,22.10655164718628,0.0011489008558959466
55856,55857,55856,111713,22.19888472557068,0.001133360041498177
56056,56057,56056,112113,22.285945892333984,0.0011177788184968504
56256,56257,56256,112513,22.34503984451294,0.0011022341200223466
56456,56457,56456,112913,22.420657873153687,0.0010869053952228757
56657,56658,56657,113315,22.573540687561035,0.0010717393145513415
56857,56858,56857,113715,22.677367687225342,0.001056993589320401
57057,57058,57057,114115,22.77505373954773,0.0010423515497593968
57257,57258,57257,114515,22.86415982246399,0.0010278089335622775
57457,57458,57457,114915,22.97651982307434,0.0010133800167104817
57658,57659,57658,115317,23.078893661499023,0.0009990405303262366
57858,57859,57858,115717,23.18005394935608,0.000985171225215665
58058,58059,58058,116117,23.34823489189148,0.0009713478109232805
58258,58259,58258,116517,23.484036684036255,0.0009578258157588103
58458,58459,58458,116917,23.582965850830078,0.000944344056779163
58659,58660,58659,117319,23.686124086380005,0.0009310880523488776
58859,58860,58859,117719,23.769497871398926,0.0009181986036367689
59059,59060,59059,118119,23.84630298614502,0.0009053506535363928
59259,59260,59259,118519,23.92694401741028,0.0008926713870727155
59459,59460,59459,118919,23.986445665359497,0.0008800631211703855
59660,59661,59660,119321,24.05625081062317,0.000867757824119764
59860,59861,59860,119721,24.115604877471924,0.0008559232080171846
60060,60061,60060,120121,24.175585746765137,0.0008439675461950424
60260,60261,60260,120521,24.236061811447144,0.0008321523330809723
60460,60461,60460,120921,24.297268867492676,0.0008207510878751708
60661,60662,60661,121323,24.358999729156494,0.000809543933693382
60861,60862,60861,121723,24.422651767730713,0.0007984087943771305
61061,61062,61061,122123,24.4853777885437,0.000787401761296789
61261,61262,61261,122523,24.550297737121582,0.0007766897090699121
61461,61462,61461,122923,24.617421865463257,0.0007660440878736943
61662,61663,61662,123325,24.68082571029663,0.0007555310694615147
61862,61863,61862,123725,24.74148988723755,0.0007453060022503595
62062,62063,62062,124125,24.7999107837677,0.0007352070737036983
62262,62263,62262,124525,24.855523824691772,0.0007252083327034155
62462,62463,62462,124925,24.91512179374695,0.0007151117086181869
62663,62664,62663,125327,24.976260900497437,0.0007052874783128918
62863,62864,62863,125727,25.04423499107361,0.000695812412316171
63063,63064,63063,126127,25.10442280769348,0.0006862675044512559
63263,63264,63263,126527,25.162450790405273,0.0006767757209854186
63463,63464,63463,126927,25.224589824676514,0.0006674786788505068
63664,63665,63664,127329,25.285412788391113,0.0006583418685454106
63864,63865,63864,127729,25.344217777252197,0.000649294656981525
64064,64065,64064,128129,25.406036853790283,0.0006402167772949971
64264,64265,64264,128529,25.466083765029907,0.0006314111760917227
64464,64465,64464,128929,25.531226873397827,0.0006227022062097387
64665,64666,64665,129331,25.59368872642517,0.0006141548347277872
64865,64866,64865,129731,25.653435945510864,0.0006056621845365376
65065,65066,65065,130131,25.716009855270386,0.0005972326087198623
65265,65266,65265,130531,25.778077840805054,0.0005890812087043755
65465,65466,65465,130931,25.840853929519653,0.0005809251161722342
65666,65667,65666,131333,25.901893854141235,0.0005728011393250753
65866,65867,65866,131733,25.978290796279907,0.0005649453908827207
66066,66067,66066,132133,26.05366086959839,0.0005571700505206695
66266,66267,66266,132533,26.11438274383545,0.0005495749505089508
66466,66467,66466,132933,26.17395782470703,0.0005421377525967819
66667,66668,66667,133335,26.23481774330139,0.0005348393249119986
66867,66868,66867,133735,26.295796871185303,0.0005276507513632958
67067,67068,67067,134135,26.354442834854126,0.0005205129190188357
67267,67268,67267,134535,26.41383385658264,0.0005135457681473184
67467,67468,67467,134935,26.470966815948486,0.000506764725224965
67668,67669,67668,135337,26.535094738006592,0.0005000928247213803
67868,67869,67868,135737,26.602425813674927,0.0004934188469972313
68068,68069,68068,136137,26.669710874557495,0.0004867385232472511
68268,68269,68268,136537,26.744807958602905,0.00048024995466902827
68468,68469,68468,136937,26.81201481819153,0.0004738044266190112
68669,68670,68669,137339,26.87824273109436,0.00046742372070168254
68869,68870,68869,137739,26.943737745285034,0.000461124091922516
69069,69070,69069,138139,27.012919664382935,0.0004548786777582282
69269,69270,69269,138539,27.083574056625366,0.0004487518784170736
69469,69470,69469,138939,27.145458936691284,0.0004427236243523446
69670,69671,69670,139341,27.229451656341553,0.00043669511516001094
69870,69871,69870,139741,27.350368976593018,0.0004307362373976232
70070,70071,70070,140141,27.446368932724,0.00042489590050800763
70270,70271,70270,140541,27.520296812057495,0.00041907546041301775
70470,70471,70470,140941,27.59122896194458,0.00041333937381831564
70671,70672,70671,141343,27.65649676322937,0.0004076815185040909
70871,70872,70871,141743,27.72305679321289,0.0004020654503486046
71071,71072,71071,142143,27.78665590286255,0.000396556742976547
71271,71272,71271,142543,27.853256940841675,0.00039117311645054276
71471,71472,71471,142943,27.91619372367859,0.000385911953870524
71672,71673,71672,143345,27.981177806854248,0.00038072737128825175
71872,71873,71872,143745,28.063323736190796,0.00037559004326054394
72072,72073,72072,144145,28.147477865219116,0.000370561797002656
72272,72273,72272,144545,28.22171688079834,0.0003656758113238041
72472,72473,72472,144945,28.29997682571411,0.0003608795112190771
72673,72674,72673,145347,28.367281913757324,0.00035609170149239586
72873,72874,72873,145747,28.433165788650513,0.0003513430128400182
73073,73074,73073,146147,28.50076174736023,0.00034668513637330886
73273,73274,73273,146547,28.576075792312622,0.0003421025586494241
73473,73474,73473,146947,28.64472484588623,0.0003376295253542471
73674,73675,73674,147349,28.714691877365112,0.00033315939733987587
73874,73875,73874,147749,28.78032374382019,0.00032868956875648213
74074,74075,74074,148149,28.84452986717224,0.0003242839217397435
74274,74275,74274,148549,28.91039800643921,0.0003199796305699049
74474,74475,74474,148949,28.97793984413147,0.00031571054543250577
74675,74676,74675,149351,29.048738718032837,0.00031147335008010563
74875,74876,74875,149751,29.113420724868774,0.0003073010484012992
75075,75076,75075,150151,29.179404735565186,0.0003031494030948048
75275,75276,75275,150551,29.249295711517334,0.00029903002348332286
75475,75476,75475,150951,29.331641674041748,0.0002949852636513685
75676,75677,75676,151353,29.3995578289032,0.00029094578013623374
75876,75877,75876,151753,29.46917462348938,0.000286982384500676
76076,76077,76076,152153,29.538426876068115,0.00028306905396511915
76276,76277,76276,152553,29.61085271835327,0.0002792104289754811
76476,76477,76476,152953,29.677942752838135,0.00027548101433197907
76677,76678,76677,153355,29.74287486076355,0.0002717304334394931
76877,76878,76877,153755,29.806745767593384,0.0002680250278693373
77077,77078,77077,154155,29.874717950820923,0.0002644374612590234
77277,77278,77277,154555,29.938817024230957,0.00026090501907984683
77477,77478,77477,154955,30.00443983078003,0.00025743017560501323
77678,77679,77678,155357,30.07512879371643,0.0002539505537003658
77878,77879,77878,155757,30.142282009124756,0.00025053510697876073
78078,78079,78078,156157,30.224236726760864,0.0002472262217203472
78278,78279,78278,156557,30.320952653884888,0.0002439843296962419
78478,78479,78478,156957,30.393688678741455,0.00024077804228057434
78679,78680,78679,157359,30.461734771728516,0.0002375478298160555
78879,78880,78879,157759,30.530012845993042,0.000234376033896664
79079,79080,79079,158159,30.597282648086548,0.0002312653422273322
79279,79280,79279,158559,30.660669803619385,0.00022820904506292496
79479,79480,79479,158959,30.726417779922485,0.0002252427294164842
79680,79681,79680,159361,30.792545795440674,0.00022225844585727962
79880,79881,79880,159761,30.860062837600708,0.00021927946587457943
80080,80081,80080,160161,30.92627787590027,0.00021634930238812963
80280,80281,80280,160561,30.991522789001465,0.0002134732091149855
80480,80481,80480,160961,31.06964683532715,0.00021066211710877295
80681,80682,80681,161363,31.135995864868164,0.00020782078990606146
80881,80882,80881,161763,31.198004007339478,0.00020501839368127547
81081,81082,81081,162163,31.421247005462646,0.00020229213450807402
81281,81282,81281,162563,31.563532829284668,0.00019961007869545965
81481,81482,81481,162963,31.641480922698975,0.00019694117448136215
81682,81683,81682,163365,31.70418882369995,0.00019426424598944543
81882,81883,81882,163765,31.772944927215576,0.0001916476235991479
82082,82083,82082,164165,31.841065883636475,0.00018907448604913964
82282,82283,82282,164565,31.90999484062195,0.00018652478862011307
82482,82483,82482,164965,31.970524787902832,0.0001840166903292946
82683,82684,82683,165367,32.05263376235962,0.000181522524462458
82883,82884,82883,165767,32.114866971969604,0.00017909325462996182
83083,83084,83083,166167,32.178645849227905,0.00017671236929102637
83283,83284,83283,166567,32.24138379096985,0.0001743766204616717
83483,83484,83483,166967,32.3161838054657,0.00017207254045355536
83684,83685,83684,167369,32.39297103881836,0.00016977180754932516
83884,83885,83884,167769,32.4690728187561,0.00016753791629444398
84084,84085,84084,168169,32.53374886512756,0.00016535367966499911
84284,84285,84284,168569,32.600828886032104,0.0001632140529359304
84484,84485,84484,168969,32.67393159866333,0.00016109142354260478
84685,84686,84685,169371,32.73785972595215,0.0001589549689838746
84885,84886,84885,169771,32.802926778793335,0.00015687626017223092
85085,85086,85085,170171,32.863478660583496,0.00015484737734202268
85285,85286,85285,170571,33.06275200843811,0.00015284588505977358
85485,85486,85485,170971,33.14992380142212,0.00015086235588029624
85686,85687,85686,171373,33.23125195503235,0.0001488766919747069
85886,85887,85886,171773,33.29426097869873,0.00014693657661973524
86086,86087,86086,172173,33.35585284233093,0.00014502658759247948
86286,86287,86286,172573,33.42884564399719,0.00014312233106591744
86486,86487,86486,172973,33.4903678894043,0.00014124532704896616
86687,86688,86687,173375,33.56534194946289,0.00013936944657912147
86887,86888,86887,173775,33.627206802368164,0.0001375151858629905
87087,87088,87087,174175,33.68797588348389,0.0001356800052169127
87287,87288,87287,174575,33.74841380119324,0.00013385863911910908
87487,87488,87487,174975,33.81177091598511,0.00013205408250652198
87688,87689,87688,175377,33.871909856796265,0.00013027215991237207
87888,87889,87888,175777,33.93316888809204,0.00012853502017459755
88088,88089,88088,176177,33.994038820266724,0.00012683158912569036
88288,88289,88288,176577,34.06755304336548,0.0001251491384305391
88488,88489,88488,176977,34.129692792892456,0.00012349052317589667
88689,88690,88689,177379,34.19181180000305,0.00012186584028103135
88889,88890,88889,177779,34.251808881759644,0.00012027287603101767
89089,89090,89089,178179,34.31524085998535,0.00011869415000336098
89289,89290,89289,178579,34.375372648239136,0.00011714361051289847
89489,89490,89489,178979,34.43821477890015,0.00011560991291645352
89690,89691,89690,179381,34.50911998748779,0.00011409823814248318
89890,89891,89890,179781,34.59699892997742,0.00011262817240842538
90090,90091,90090,180181,34.660789012908936,0.00011118492744508618
90290,90291,90290,180581,34.724445819854736,0.00010975617891016497
90490,90491,90490,180981,34.783981800079346,0.00010831303405022587
90691,90692,90691,181383,34.845011949539185,0.00010688529218467811
90891,90892,90891,181783,34.90629291534424,0.00010551489052971607
91091,91092,91091,182183,34.96820282936096,0.00010416108704950234
91291,91292,91291,182583,35.038023948669434,0.00010280807289617169
91491,91492,91491,182983,35.097503900527954,0.00010145655695681298
91692,91693,91692,183385,35.157978773117065,0.00010012076502267505
91892,91893,91892,183785,35.21774482727051,9.880718901499401e-05
92092,92093,92092,184185,35.28087091445923,9.75004821291043e-05
92292,92293,92292,184585,35.342928886413574,9.620895449813824e-05
92492,92493,92492,184985,35.405704975128174,9.492811418366405e-05
92693,92694,92693,185387,35.470035791397095,9.365556703365862e-05
92893,92894,92893,185787,35.53815674781799,9.240260564614021e-05
93093,93094,93093,186187,35.60113000869751,9.117756638754565e-05
93293,93294,93293,186587,35.665966749191284,8.997766313029656e-05
93493,93494,93493,186987,35.727733850479126,8.8771635618125e-05
93694,93695,93694,187389,35.78912091255188,8.757612997979614e-05
93894,93895,93894,187789,35.850502729415894,8.642151207130415e-05
94094,94095,94094,188189,35.91406273841858,8.528485519510682e-05
94294,94295,94294,188589,35.976048946380615,8.415286765755978e-05
94494,94495,94494,188989,36.04261088371277,8.30299689787259e-05
94695,94696,94695,189391,36.10566568374634,8.193880178712148e-05
94895,94896,94895,189791,36.16950988769531,8.087893491730921e-05
95095,95096,95095,190191,36.231773853302,7.982364297143526e-05
95295,95296,95295,190591,36.2920618057251,7.87624228514586e-05
95495,95496,95495,190991,36.366238832473755,7.771620909848523e-05
95696,95697,95696,191393,36.4291877746582,7.670667108932885e-05
95896,95897,95896,191793,36.495656967163086,7.572251973128162e-05
96096,96097,96096,192193,36.563193798065186,7.474684782147175e-05
96296,96297,96296,192593,36.630066871643066,7.377343752456229e-05
96496,96497,96496,192993,36.71545076370239,7.280039418638807e-05
96697,96698,96697,193395,36.78489685058594,7.184202468711155e-05
96897,96898,96897,193795,36.8485209941864,7.091048919782164e-05
97097,97098,97097,194195,36.90989685058594,6.99970260363001e-05
97297,97298,97297,194595,36.981276750564575,6.908558276468211e-05
97497,97498,97497,194995,37.05090570449829,6.816907100040238e-05
97698,97699,97698,195397,37.11262798309326,6.726533398147265e-05
97898,97899,97898,195797,37.17632794380188,6.638904664777338e-05
98098,98099,98098,196197,37.236143827438354,6.552769550097537e-05
98298,98299,98298,196597,37.29703092575073,6.465832545740876e-05
98498,98499,98498,196997,37.35898971557617,6.378889286704535e-05
98699,98700,98699,197399,37.420153856277466,6.294496154533116e-05
98899,98900,98899,197799,37.47979497909546,6.211518222798223e-05
99099,99100,99099,198199,37.54805874824524,6.128381441590894e-05
99299,99300,99299,198599,37.61007595062256,6.0467151899641244e-05
99499,99500,99499,198999,37.66990780830383,5.966680186815877e-05
99700,99701,99700,199401,37.73011302947998,5.887957321171497e-05
99900,99901,99900,199801,37.790013790130615,5.8105150948722326e-05
100100,100101,100100,200201,37.84955286979675,5.7336257043037044e-05
100300,100301,100300,200601,37.91429781913757,5.6582861504167654e-05
100501,100502,100501,201003,37.97379779815674,5.584283652914116e-05
100701,100702,100701,201403,38.050381660461426,5.511720330360962e-05
100901,100902,100901,201803,38.11131691932678,5.440586890368439e-05
101101,101102,101101,202203,38.171793937683105,5.370455596587546e-05
101301,101302,101301,202603,38.232303857803345,5.300214814511839e-05
101502,101503,101502,203005,38.29396891593933,5.230988910939091e-05
101702,101703,101702,203405,38.35495090484619,5.164113340159465e-05
101902,101903,101902,203805,38.41509389877319,5.098268983141891e-05
102102,102103,102102,204205,38.47502374649048,5.033136035485895e-05
102302,102303,102302,204605,38.538670778274536,4.968291970495641e-05
102503,102504,102503,205007,38.60185694694519,4.9039978373801967e-05
102703,102704,102703,205407,38.6640567779541,4.841448018030458e-05
102903,102904,102903,205807,38.724607944488525,4.779731643772772e-05
103103,103104,103103,206207,38.79421901702881,4.718193771009914e-05
103303,103304,103303,206607,38.86729693412781,4.656798449963186e-05
103504,103505,103504,207009,38.931734800338745,4.596012323952167e-05
103704,103705,103704,207409,38.99436593055725,4.5362270301787345e-05
103904,103905,103904,207809,39.0641028881073,4.476877423596486e-05
104104,104105,104104,208209,39.124178886413574,4.418007522984389e-05
104304,104305,104304,208609,39.18551588058472,4.359678135619597e-05
104505,104506,104505,209011,39.24861478805542,4.302084883661207e-05
104705,104706,104705,209411,39.30854082107544,4.2454754744606647e-05
104905,104906,104905,209811,39.368504762649536,4.1894119348474885e-05
105105,105106,105105,210211,39.42807388305664,4.134734380362787e-05
105305,105306,105305,210611,39.49134373664856,4.0810808497345947e-05
105506,105507,105506,211013,39.560030937194824,4.0274739708349363e-05
105706,105707,105706,211413,39.62084984779358,3.974816206506211e-05
105906,105907,105906,211813,39.68134570121765,3.923246554957875e-05
106106,106107,106106,212213,39.74094080924988,3.872214455492361e-05
106306,106307,106306,212613,39.80156898498535,3.821798367002212e-05
106507,106508,106507,213015,39.862539768218994,3.772278860044604e-05
106707,106708,106707,213415,39.92196202278137,3.724096755943991e-05
106907,106908,106907,213815,39.982202768325806,3.676667704662083e-05
107107,107108,107107,214215,40.05090093612671,3.6291062343616e-05
107307,107308,107307,214615,40.11375594139099,3.582170345720955e-05
107508,107509,107508,215017,40.1730637550354,3.53671612117223e-05
107708,107709,107708,215417,40.234827756881714,3.492178029743362e-05
107908,107909,107908,215817,40.294973850250244,3.4474854288589036e-05
108108,108109,108108,216217,40.35436487197876,3.40294995071156e-05
108308,108309,108308,216617,40.41771864891052,3.3591607353848384e-05
108509,108510,108509,217019,40.477025747299194,3.315898945917218e-05
108709,108710,108709,217419,40.54208183288574,3.273263239382966e-05
108909,108910,108909,217819,40.60425591468811,3.2309032001612506e-05
109109,109110,109109,218219,40.663909912109375,3.188638286560343e-05
109309,109310,109309,218619,40.72731685638428,3.146923261258838e-05
109510,109511,109510,219021,40.78778600692749,3.1055075627444526e-05
109710,109711,109710,219421,40.84722280502319,3.06483763686686e-05
109910,109911,109910,219821,40.91623401641846,3.0250342983088576e-05
110110,110111,110110,220221,40.99052381515503,2.9851965056713734e-05
110310,110311,110310,220621,41.06473779678345,2.9453946396981197e-05
110511,110512,110511,221023,41.12474966049194,2.906447969107026e-05
110711,110712,110711,221423,41.18628406524658,2.8685361672851316e-05
110911,110912,110911,221823,41.24617075920105,2.8309791881153772e-05
111111,111112,111111,222223,41.30719065666199,2.793519868376379e-05
111311,111312,111311,222623,41.36850690841675,2.756709385061219e-05
111512,111513,111512,223025,41.42861270904541,2.7209345144369468e-05
111712,111713,111712,223425,41.489858865737915,2.6856382755677513e-05
111912,111913,111912,223825,41.559897899627686,2.6500766470475935e-05
112112,112113,112112,224225,41.62149977684021,2.6152504592056777e-05
112312,112313,112312,224625,41.68115782737732,2.5819325671295058e-05
112513,112514,112513,225027,41.74170184135437,2.5489445060157117e-05
112713,112714,112713,225427,41.80459499359131,2.5158092247333167e-05
112913,112914,112913,225827,41.86544680595398,2.483022924094265e-05
113113,113114,113113,226227,41.92523980140686,2.4510038193581392e-05
113313,113314,113313,226627,41.985302686691284,2.419587332316833e-05
113514,113515,113514,227029,42.05528783798218,2.3885442286206356e-05
113714,113715,113714,227429,42.11510491371155,2.3580706848808053e-05
113914,113915,113914,227829,42.175896883010864,2.327710824570571e-05
114114,114115,114114,228229,42.239330768585205,2.2973227534980313e-05
114314,114315,114314,228629,42.30159068107605,2.2674804915710805e-05
114515,114516,114515,229031,42.361777782440186,2.238453946885797e-05
114715,114716,114715,229431,42.421462059020996,2.2099449084474933e-05
114915,114916,114915,229831,42.4836049079895,2.180977521247195e-05
115115,115116,115115,230231,42.54961895942688,2.1519500463285077e-05
115315,115316,115315,230631,42.61103582382202,2.1238677804018657e-05
115516,115517,115516,231033,42.671281814575195,2.0962494835235708e-05
115716,115717,115716,231433,42.7308988571167,2.0687329974705248e-05
115916,115917,115916,231833,42.79102063179016,2.041431648426385e-05
116116,116117,116116,232233,42.85270094871521,2.014596851656732e-05
116316,116317,116316,232633,42.91355800628662,1.988266146999009e-05
116517,116518,116517,233035,42.97365188598633,1.962033701367244e-05
116717,116718,116717,233435,43.0461368560791,1.9359956486047953e-05
116917,116918,116917,233835,43.123414754867554,1.910567367206094e-05
117117,117118,117117,234235,43.19151592254639,1.8858412497266025e-05
117317,117318,117317,234635,43.2505247592926,1.8614066529843346e-05
117518,117519,117518,235037,43.31029295921326,1.8371253627111054e-05
117718,117719,117718,235437,43.3689227104187,1.8132783849439717e-05
117918,117919,117918,235837,43.429646730422974,1.789673532767881e-05
118118,118119,118118,236237,43.49250793457031,1.766461490286039e-05
118318,118319,118318,236637,43.55985999107361,1.743852663848573e-05
118519,118520,118519,237039,43.6204948425293,1.7216707430073667e-05
118719,118720,118719,237439,43.68128776550293,1.6997802784941326e-05
118919,118920,118919,237839,43.75149965286255,1.6779103041475532e-05
119119,119120,119119,238239,43.81121373176575,1.6564321561972023e-05
119319,119320,119319,238639,43.886295795440674,1.6356685286522123e-05
119520,119521,119520,239041,43.966556787490845,1.6151432781057944e-05
119720,119721,119720,239441,44.04910063743591,1.5945612527305607e-05
119920,119921,119920,239841,44.11272597312927,1.5739866418091707e-05
120120,120121,120120,240241,44.172802686691284,1.553851433457343e-05
120320,120321,120320,240641,44.2318058013916,1.5341289814167193e-05
120521,120522,120521,241043,44.29466986656189,1.5144882344943706e-05
120721,120722,120721,241443,44.35399675369263,1.4949704941051995e-05
120921,120922,120921,241843,44.414384841918945,1.4755043955947428e-05
121121,121122,121121,242243,44.47479605674744,1.4562447467048299e-05
121321,121322,121321,242643,44.53909182548523,1.4372106761909459e-05
121522,121523,121522,243045,44.600366830825806,1.4184032568775834e-05
121722,121723,121722,243445,44.65978980064392,1.4000548234215654e-05
121922,121923,121922,243845,44.720109701156616,1.3818528370447301e-05
122122,122123,122122,244245,44.77963185310364,1.3637848930070931e-05
122322,122323,122322,244645,44.84082889556885,1.346016461261688e-05
122523,122524,122523,245047,44.90179777145386,1.3284685446248557e-05
122723,122724,122723,245447,44.96177887916565,1.3111916551545706e-05
122923,122924,122923,245847,45.02664875984192,1.2940464068257475e-05
123123,123124,123123,246247,45.08845901489258,1.2772285486469118e-05
123323,123324,123323,246647,45.14738988876343,1.2608320098172464e-05
123524,123525,123524,247049,45.219958782196045,1.2446292583172009e-05
123724,123725,123724,247449,45.29409980773926,1.2286311093599653e-05
123924,123925,123924,247849,45.356268644332886,1.212859376112078e-05
124124,124125,124124,248249,45.41667890548706,1.197567135851732e-05
124324,124325,124324,248649,45.476961612701416,1.1826469258359274e-05
124525,124526,124525,249051,45.546366930007935,1.16768822811991e-05
124725,124726,124725,249451,45.60671281814575,1.1528104328762432e-05
124925,124926,124925,249851,45.6670196056366,1.1381546194638878e-05
125125,125126,125125,250251,45.72658085823059,1.1238571386144452e-05
125325,125326,125325,250651,45.788230895996094,1.1097406986620853e-05
125526,125527,125526,251053,45.84754991531372,1.0955261815643842e-05
125726,125727,125726,251453,45.90619397163391,1.0814539096459148e-05
125926,125927,125926,251853,45.96526575088501,1.0675868479583636e-05
126126,126127,126126,252253,46.032530784606934,1.0538860674751363e-05
126326,126327,126326,252653,46.094796657562256,1.040318660931943e-05
126527,126528,126527,253055,46.15490365028381,1.0268598696375037e-05
126727,126728,126727,253455,46.21890878677368,1.0135279140182757e-05
126927,126928,126927,253855,46.27927088737488,1.0002281435417993e-05
127127,127128,127127,254255,46.338499784469604,9.871722723459605e-06
127327,127328,127327,254655,46.402169704437256,9.744002680000372e-06
127528,127529,127528,255057,46.46312093734741,9.61665289956283e-06
127728,127729,127728,255457,46.524186849594116,9.489892778628001e-06
127928,127929,127928,255857,46.588220834732056,9.364846366372176e-06
128128,128129,128128,256257,46.64966678619385,9.243442205259841e-06
128328,128329,128328,256657,46.710991859436035,9.12367042457294e-06
128529,128530,128529,257059,46.77103590965271,9.003295915835782e-06
128729,128730,128729,257459,46.83199882507324,8.88562893484679e-06
128929,128930,128929,257859,46.8933207988739,8.771650341437249e-06
129129,129130,129129,258259,46.955169677734375,8.659843149925473e-06
129329,129330,129329,258659,47.02410173416138,8.54787266385816e-06
129530,129531,129530,259061,47.09418702125549,8.436113866643165e-06
129730,129731,129730,259461,47.154953956604004,8.32801029647945e-06
129930,129931,129930,259861,47.21739387512207,8.222559849159845e-06
130130,130131,130130,260261,47.27873373031616,8.11831464853367e-06
130330,130331,130330,260661,47.34968090057373,8.014772111331724e-06
130531,130532,130531,261063,47.43169569969177,7.91168205984678e-06
130731,130732,130731,261463,47.49445462226868,7.810640273877008e-06
130931,130932,130931,261863,47.55974292755127,7.711617353754715e-06
131131,131132,131131,262263,47.63801193237305,7.614713840505814e-06
131331,131332,131331,262663,47.70688486099243,7.518567731952333e-06
131532,131533,131532,263065,47.77128767967224,7.4209399919042546e-06
131732,131733,131732,263465,47.83075189590454,7.323895286212233e-06
131932,131933,131932,263865,47.892345905303955,7.229769122956267e-06
132132,132133,132132,264265,47.95261788368225,7.138375794736244e-06
132332,132333,132332,264665,48.01800179481506,7.046717227891322e-06
132533,132534,132533,265067,48.09047985076904,6.953719171646285e-06
132733,132734,132733,265467,48.15100693702698,6.86255131019586e-06
132933,132934,132933,265867,48.21178865432739,6.773653189719054e-06
133133,133134,133133,266267,48.27247166633606,6.685829351678706e-06
133333,133334,133333,266667,48.331542015075684,6.598275845722372e-06
133534,133535,133534,267069,48.39093995094299,6.511316376804007e-06
133734,133735,133734,267469,48.45172381401062,6.426538597378519e-06
133934,133935,133934,267869,48.5146267414093,6.342950500301896e-06
134134,134135,134134,268269,48.58068585395813,6.260024005570409e-06
134334,134335,134334,268669,48.64064002037048,6.178153318738682e-06
134535,134536,134535,269071,48.70200490951538,6.097140053088602e-06
134735,134736,134735,269471,48.762115716934204,6.017931854360804e-06
134935,134936,134935,269871,48.82332491874695,5.940626116836509e-06
135135,135136,135135,270271,48.885751724243164,5.8649880954584645e-06
135335,135336,135335,270671,48.947041034698486,5.79002498268552e-06
135536,135537,135536,271073,49.00969696044922,5.715211775086579e-06
135736,135737,135736,271473,49.08655071258545,5.642488123792656e-06
135936,135937,135936,271873,49.1610586643219,5.572112908137876e-06
136136,136137,136136,272273,49.238494873046875,5.502890415650309e-06
136336,136337,136336,272673,49.30309987068176,5.4332172146445835e-06
136537,136538,136537,273075,49.36418104171753,5.36324690683766e-06
136737,136738,136737,273475,49.425548791885376,5.29555988049713e-06
136937,136938,136937,273875,49.49917697906494,5.229951966662565e-06
137137,137138,137137,274275,49.582589864730835,5.164772931214835e-06
137337,137338,137337,274675,49.645219802856445,5.099144547466333e-06
137538,137539,137538,275077,49.710747957229614,5.03319326224279e-06
137738,137739,137738,275477,49.773003816604614,4.968439750193433e-06
137938,137939,137938,275877,49.83520174026489,4.904971023017556e-06
138138,138139,138138,276277,49.89748668670654,4.8425071157005245e-06
138338,138339,138338,276677,49.960121870040894,4.780337490587529e-06
138539,138540,138539,277079,50.030799865722656,4.717899547625745e-06
138739,138740,138739,277479,50.0931499004364,4.656403717616764e-06
138939,138940,138939,277879,50.15567684173584,4.596001507415269e-06
139139,139140,139139,278279,50.217352867126465,4.5365244405257544e-06
139339,139340,139339,278679,50.27994966506958,4.477411346521915e-06
139540,139541,139540,279081,50.344873905181885,4.418341416871295e-06
139740,139741,139740,279481,50.40745782852173,4.360684891394473e-06
139940,139941,139940,279881,50.46904182434082,4.304246028507933e-06
140140,140141,140140,280281,50.5456109046936,4.248564247995627e-06
140340,140341,140340,280681,50.61003279685974,4.193591393814858e-06
140541,140542,140541,281083,50.67338967323303,4.139229228976016e-06
140741,140742,140741,281483,50.736163854599,4.086548298739797e-06
140941,140942,140941,281883,50.798152923583984,4.03532747944773e-06
141141,141142,141141,282283,50.86064887046814,3.984594220651304e-06
141341,141342,141341,282683,50.92532682418823,3.933951906301062e-06
141542,141543,141542,283085,50.987836837768555,3.883895986929403e-06
141742,141743,141742,283485,51.05851483345032,3.835469243612382e-06
141942,141943,141942,283885,51.11996579170227,3.7879403018177495e-06
142142,142143,142142,284285,51.18251180648804,3.740481095173814e-06
142342,142343,142342,284685,51.24501395225525,3.693041010992595e-06
142543,142544,142543,285087,51.30893898010254,3.646088954879403e-06
142743,142744,142743,285487,51.37893891334534,3.600401307003214e-06
142943,142944,142943,285887,51.44209384918213,3.5551678471800976e-06
143143,143144,143143,286287,51.50591993331909,3.5099594176301056e-06
143343,143344,143343,286687,51.57579493522644,3.4649756250481164e-06
143544,143545,143544,287089,51.65611171722412,3.420150384363263e-06
143744,143745,143744,287489,51.730748891830444,3.3761523250988917e-06
143944,143945,143944,287889,51.792627811431885,3.3329406729572125e-06
144144,144145,144144,288289,51.85452890396118,3.290064197314144e-06
144344,144345,144344,288689,51.9156129360199,3.2472210970613423e-06
144545,144546,144545,289091,51.97831869125366,3.204534554643172e-06
144745,144746,144745,289491,52.0505108833313,3.1628178548410484e-06
144945,144946,144945,289891,52.11395883560181,3.1218451767060057e-06
145145,145146,145145,290291,52.17653679847717,3.0811733251195294e-06
145345,145346,145345,290691,52.23960590362549,3.0407507982479615e-06
145546,145547,145546,291093,52.30375671386719,3.001078858145176e-06
145746,145747,145746,291493,52.36700081825256,2.9626735072299912e-06
145946,145947,145946,291893,52.427663803100586,2.9245379736346688e-06
146146,146147,146146,292293,52.48917078971863,2.8865134397707923e-06
146346,146347,146346,292693,52.55846571922302,2.849297883626035e-06
146547,146548,146547,293095,52.61917281150818,2.8129249391549343e-06
146747,146748,146747,293495,52.6798939704895,2.777302146417527e-06
146947,146948,146947,293895,52.74266481399536,2.7419292369919155e-06
147147,147148,147147,294295,52.8097448348999,2.7068802920729257e-06
147347,147348,147347,294695,52.87354493141174,2.6725383248930564e-06
147548,147549,147548,295097,52.93374800682068,2.638854531680487e-06
147748,147749,147748,295497,52.99685478210449,2.6057969797990767e-06
147948,147949,147948,295897,53.067662715911865,2.5729477897224153e-06
148148,148149,148148,296297,53.1274778842926,2.5402633075014834e-06
148348,148349,148348,296697,53.18883991241455,2.5079049522177933e-06
148549,148550,148549,297099,53.24907684326172,2.476136025799737e-06
148749,148750,148749,297499,53.30963182449341,2.4452260116823235e-06
148949,148950,148949,297899,53.36964392662048,2.4143571316762967e-06
149149,149150,149149,298299,53.4293167591095,2.3832745014154056e-06
149349,149350,149349,298699,53.489238023757935,2.3524776276886625e-06
149550,149551,149550,299101,53.560263872146606,2.3222773307274835e-06
149750,149751,149750,299501,53.623634815216064,2.2927824916195944e-06
149950,149951,149950,299901,53.68368577957153,2.2633046514341802e-06
150150,150151,150150,300301,53.75056791305542,2.233761261888304e-06
150350,150351,150350,300701,53.823171854019165,2.204743523057599e-06
150551,150552,150551,301103,53.892369747161865,2.176259129767353e-06
150751,150752,150751,301503,53.95189571380615,2.148072818259588e-06
150951,150952,150951,301903,54.01576280593872,2.1199573870360405e-06
151151,151152,151151,302303,54.0836067199707,2.092202735698951e-06
151351,151352,151351,302703,54.14453196525574,2.0649519007327967e-06
151552,151553,151552,303105,54.20456290245056,2.038084486924125e-06
151752,151753,151752,303505,54.267946004867554,2.0117552351323047e-06
151952,151953,151952,303905,54.32860088348389,1.9857548265499217e-06
152152,152153,152152,304305,54.3891327381134,1.9601379698214323e-06
152352,152353,152352,304705,54.448476791381836,1.93512459629048e-06
152553,152554,152553,305107,54.509888887405396,1.9106915127102578e-06
152753,152754,152753,305507,54.575562953948975,1.886714272826311e-06
152953,152954,152953,305907,54.63675379753113,1.8627299201078509e-06
153153,153154,153153,306307,54.69654870033264,1.8389731052285115e-06
153353,153354,153353,306707,54.7558867931366,1.815951511223215e-06
153554,153555,153554,307109,54.81662678718567,1.793509352821652e-06
153754,153755,153754,307509,54.87687683105469,1.771288074652469e-06
153954,153955,153954,307909,54.936954736709595,1.748938889953805e-06
154154,154155,154154,308309,54.996731758117676,1.7267110426722498e-06
154354,154355,154354,308709,55.06560182571411,1.7049668350902972e-06
154555,154556,154555,309111,55.12768578529358,1.6837136711172876e-06
154755,154756,154755,309511,55.187920808792114,1.6627795349463743e-06
154955,154956,154955,309911,55.24683976173401,1.641667787480338e-06
155155,155156,155155,310311,55.307506799697876,1.6205305030376032e-06
155355,155356,155355,310711,55.36838674545288,1.5997622493536874e-06
155556,155557,155556,311113,55.430370807647705,1.5793052671669733e-06
155756,155757,155756,311513,55.48920679092407,1.5590695929271191e-06
155956,155957,155956,311913,55.55509567260742,1.5388243093847645e-06
156156,156157,156156,312313,55.61346483230591,1.5187644885157856e-06
156356,156357,156356,312713,55.67162275314331,1.4990445061076293e-06
156557,156558,156557,313115,55.73058199882507,1.4794910115911802e-06
156757,156758,156757,313515,55.788310050964355,1.4602146897990975e-06
156957,156958,156957,313915,55.84657001495361,1.4411500162480282e-06
157157,157158,157157,314315,55.92092967033386,1.422385633275846e-06
157357,157358,157357,314715,55.991414070129395,1.4040512143322632e-06
157558,157559,157558,315117,56.06198978424072,1.3860666070618404e-06
157758,157759,157758,315517,56.12020564079285,1.368401535398108e-06
157958,157959,157958,315917,56.17799973487854,1.3508324281528885e-06
158158,158159,158158,316317,56.235511779785156,1.3335530931028398e-06
158358,158359,158358,316717,56.29626774787903,1.316793952292029e-06
158559,158560,158559,317119,56.356281757354736,1.300329485565827e-06
158759,158760,158759,317519,56.415931940078735,1.283996167354821e-06
158959,158960,158959,317919,56.47360587120056,1.2676646165800633e-06
159159,159160,159159,318319,56.53683376312256,1.25165266315491e-06
159359,159360,159359,318719,56.599350690841675,1.2361798902373522e-06
159560,159561,159560,319121,56.65918588638306,1.2209033524791474e-06
159760,159761,159760,319521,56.71827673912048,1.2056296236478967e-06
159960,159961,159960,319921,56.77606391906738,1.190341052165116e-06
160160,160161,160160,320321,56.834030866622925,1.1752693185250995e-06
160360,160361,160360,320721,56.89381289482117,1.1604782089536489e-06
160561,160562,160561,321123,56.956806898117065,1.1457857039362884e-06
160761,160762,160761,321523,57.01985573768616,1.131234488928252e-06
160961,160962,160961,321923,57.07897186279297,1.1167431080956844e-06
161161,161162,161161,322323,57.136884927749634,1.1023542060902663e-06
161361,161362,161361,322723,57.19827580451965,1.0881325836548938e-06
161562,161563,161562,323125,57.2576117515564,1.0740668182164666e-06
161762,161763,161762,323525,57.315521001815796,1.0602150423936037e-06
161962,161963,161962,323925,57.37256193161011,1.0463866135990375e-06
162162,162163,162162,324325,57.431970834732056,1.0327121590505122e-06
162362,162363,162362,324725,57.48894691467285,1.0193771925717172e-06
162563,162564,162563,325127,57.553565979003906,1.0061992302395457e-06
162763,162764,162763,325527,57.612422943115234,9.931070773009517e-07
162963,162964,162963,325927,57.669928789138794,9.801370792048226e-07
163163,163164,163163,326327,57.72789978981018,9.67535781638883e-07
163363,163364,163363,326727,57.78707671165466,9.552442733616229e-07
163564,163565,163564,327129,57.84712195396423,9.429610079340143e-07
163764,163765,163764,327529,57.90556073188782,9.308083047756543e-07
163964,163965,163964,327929,57.96312594413757,9.189327350413245e-07
164164,164165,164164,328329,58.03810095787048,9.074089474913384e-07
164364,164365,164364,328729,58.11135983467102,8.960465478113089e-07
164565,164566,164565,329131,58.17171382904053,8.846701086735691e-07
164765,164766,164765,329531,58.236202001571655,8.734887753219937e-07
164965,164966,164965,329931,58.30508065223694,8.62492197246098e-07
165165,165166,165165,330331,58.36454486846924,8.516846471160357e-07
165365,165366,165365,330731,58.424694776535034,8.410797225687716e-07
165566,165567,165566,331133,58.48463988304138,8.305437919108827e-07
165766,165767,165766,331533,58.55148983001709,8.200733313725215e-07
165966,165967,165966,331933,58.61307883262634,8.096620286572932e-07
166166,166167,166166,332333,58.672852993011475,7.994789688250922e-07
166366,166367,166366,332733,58.733152866363525,7.895131555253986e-07
166567,166568,166567,333135,58.79424476623535,7.795112268536304e-07
166767,166768,166767,333535,58.854344844818115,7.695090999328867e-07
166967,166968,166967,333935,58.91391587257385,7.596304554481433e-07
167167,167168,167167,334335,58.975557804107666,7.499883839230843e-07
167367,167368,167367,334735,59.04400181770325,7.404336427758975e-07
167568,167569,167568,335137,59.105830907821655,7.307938460227386e-07
167768,167769,167768,335537,59.16838192939758,7.212766163665938e-07
167968,167969,167968,335937,59.22900986671448,7.119506513262573e-07
168168,168169,168168,336337,59.28995084762573,7.027814072030042e-07
168368,168369,168368,336737,59.351645946502686,6.936857911989809e-07
168569,168570,168569,337139,59.41222882270813,6.846197383240841e-07
168769,168770,168769,337539,59.474448919296265,6.757604887183849e-07
168969,168970,168969,337939,59.53952169418335,6.671213132957595e-07
169169,169170,169169,338339,59.601072788238525,6.586428742558714e-07
169369,169370,169369,338739,59.66215491294861,6.502269373174994e-07
169570,169571,169570,339141,59.72314190864563,6.418453016865293e-07
169770,169771,169770,339541,59.78239893913269,6.336639828602979e-07
169970,169971,169970,339941,59.84087681770325,6.257014113464206e-07
170170,170171,170170,340341,59.90053200721741,6.179362636613606e-07
170370,170371,170370,340741,59.9603316783905,6.102394559995958e-07
170571,170572,170571,341143,60.02673673629761,6.024935308915762e-07
170771,170772,170771,341543,60.089582681655884,5.948616954224373e-07
170971,170972,170971,341943,60.160029888153076,5.874504584502186e-07
171171,171172,171171,342343,60.23397088050842,5.802639811988597e-07
171371,171372,171371,342743,60.29550886154175,5.731128522499426e-07
171572,171573,171572,343145,60.35413980484009,5.658446915831294e-07
171772,171773,171772,343545,60.41728377342224,5.586594208061028e-07
171972,171973,171972,343945,60.47794985771179,5.516666896027404e-07
172172,172173,172172,344345,60.54065275192261,5.44809824612287e-07
172372,172373,172372,344745,60.60131788253784,5.379444549209167e-07
172573,172574,172573,345147,60.66133666038513,5.310236546010064e-07
172773,172774,172773,345547,60.72070670127869,5.242006534608068e-07
172973,172974,172973,345947,60.78043985366821,5.17480967287459e-07
173173,173174,173173,346347,60.841118812561035,5.108417534121768e-07
173373,173374,173373,346747,60.90516185760498,5.042424987648239e-07
173574,173575,173574,347149,60.976810932159424,4.976596913049939e-07
173774,173775,173774,347549,61.04982876777649,4.912061132788909e-07
173974,173975,173974,347949,61.11187791824341,4.848600815213234e-07
174174,174175,174174,348349,61.172563791275024,4.786043908529564e-07
174374,174375,174374,348749,61.233882904052734,4.724246854445593e-07
174575,174576,174575,349151,61.297812938690186,4.6628649103876314e-07
174775,174776,174775,349551,61.36579895019531,4.6028536766352673e-07
174975,174976,174975,349951,61.430842876434326,4.5442540031962536e-07
175175,175176,175175,350351,61.493780851364136,4.486662322018489e-07
175375,175376,175375,350751,61.563384771347046,4.429340211126801e-07
175576,175577,175576,351153,61.62601971626282,4.371969877166193e-07
175776,175777,175776,351553,61.688098669052124,4.316257988846358e-07
175976,175977,175976,351953,61.750359773635864,4.262826729148975e-07
176176,176177,176176,352353,61.811625957489014,4.210493994299217e-07
176376,176377,176376,352753,61.87491989135742,4.157573416715212e-07
176577,176578,176577,353155,61.938326835632324,4.104236325823518e-07
176777,176778,176777,353555,62.002076864242554,4.052512745619879e-07
176977,176978,176977,353955,62.07077193260193,4.002335371804569e-07
177177,177178,177177,354355,62.13396382331848,3.952737100979377e-07
177377,177378,177377,354755,62.19641184806824,3.903161444109756e-07
177578,177579,177578,355157,62.26505398750305,3.853512111404058e-07
177778,177779,177778,355557,62.34135389328003,3.8045461642645474e-07
177978,177979,177978,355957,62.412214040756226,3.756242191030937e-07
178178,178179,178178,356357,62.474151849746704,3.7087068143957036e-07
178378,178379,178378,356757,62.54298281669617,3.661680159886707e-07
178579,178580,178579,357159,62.60648488998413,3.614389773281601e-07
178779,178780,178779,357559,62.669455766677856,3.567449036002454e-07
178979,178980,178979,357959,62.7307448387146,3.5214573737304166e-07
179179,179180,179179,358359,62.79183077812195,3.476381096307733e-07
179379,179380,179379,358759,62.853513956069946,3.431408229135755e-07
179580,179581,179580,359161,62.92089605331421,3.386343021941778e-07
179780,179781,179780,359561,62.98424768447876,3.342458396868161e-07
179980,179981,179980,359961,63.053616762161255,3.2996860727917556e-07
180180,180181,180180,360361,63.123408794403076,3.2572614196233787e-07
180380,180381,180380,360761,63.187368869781494,3.214879246781353e-07
180581,180582,180581,361163,63.25515294075012,3.173100086722686e-07
180781,180782,180781,361563,63.321457862854004,3.132918228668646e-07
180981,180982,180981,361963,63.38478899002075,3.093481077540065e-07
181181,181182,181181,362363,63.4469678401947,3.054066366150126e-07
181381,181382,181381,362763,63.51300573348999,3.0150281054007786e-07
181582,181583,181582,363165,63.58309888839722,2.9766746455967676e-07
181782,181783,181782,363565,63.646214962005615,2.9393251325970226e-07
181982,181983,181982,363965,63.7078058719635,2.902615914449767e-07
182182,182183,182182,364365,63.769644021987915,2.866387313383574e-07
182382,182383,182382,364765,63.83152794837952,2.8304402320318553e-07
182583,182584,182583,365167,63.894386768341064,2.79463195030544e-07
182783,182784,182783,365567,63.956339836120605,2.7597202730253195e-07
182983,182984,182983,365967,64.03209090232849,2.725656016599168e-07
183183,183184,183183,366367,64.09457278251648,2.6918522515797925e-07
183383,183384,183383,366767,64.1571409702301,2.657850886548911e-07
183584,183585,183584,367169,64.2197036743164,2.6239189046436764e-07
183784,183785,183784,367569,64.28181886672974,2.5910270184870646e-07
183984,183985,183984,367969,64.34269165992737,2.558698754155164e-07
184184,184185,184184,368369,64.41018986701965,2.526216409068788e-07
184384,184385,184384,368769,64.48366475105286,2.4937226475776374e-07
184585,184586,184585,369171,64.55963587760925,2.4616163454001323e-07
184785,184786,184785,369571,64.6213538646698,2.430220285434953e-07
184985,184986,184985,369971,64.68664884567261,2.3990199264264543e-07
185185,185186,185185,370371,64.74654269218445,2.3679800730692766e-07
185385,185386,185385,370771,64.80782794952393,2.3374992317239174e-07
185586,185587,185586,371173,64.86886978149414,2.3075584844544786e-07
185786,185787,185786,371573,64.9288158416748,2.2780786566789327e-07
185986,185987,185986,371973,64.99002981185913,2.2487366378109202e-07
186186,186187,186186,372373,65.05838894844055,2.2197879234654386e-07
186386,186387,186386,372773,65.11838889122009,2.19142646845246e-07
186587,186588,186587,373175,65.17802286148071,2.1634846850792098e-07
186787,186788,186787,373575,65.2383668422699,2.1361475189357947e-07
186987,186988,186987,373975,65.29953169822693,2.1091119254978668e-07
187187,187188,187187,374375,65.35990881919861,2.08228818787683e-07
187387,187388,187387,374775,65.41930079460144,2.0559249209179393e-07
187588,187589,187588,375177,65.47995686531067,2.0302445857150853e-07
187788,187789,187788,375577,65.5450439453125,2.0053782900678585e-07
187988,187989,187988,375977,65.60585379600525,1.980610660771319e-07
188188,188189,188188,376377,65.66565680503845,1.9557087916446244e-07
188388,188389,188388,376777,65.72573280334473,1.931128232628215e-07
188589,188590,188589,377179,65.78593373298645,1.9071416011678247e-07
188789,188790,188789,377579,65.84458589553833,1.8837164937829967e-07
188989,188990,188989,377979,65.9072687625885,1.8602450286028056e-07
189189,189190,189189,378379,65.96752285957336,1.8367237760799064e-07
189389,189390,189389,378779,66.03352189064026,1.813507448119563e-07
189590,189591,189590,379181,66.09423589706421,1.7906443323206803e-07
189790,189791,189790,379581,66.15466976165771,1.7681787160434122e-07
189990,189991,189990,379981,66.21747875213623,1.7457407381226337e-07
190190,190191,190190,380381,66.27755379676819,1.7233343619771274e-07
190390,190391,190390,380781,66.339430809021,1.701135962645282e-07
190591,190592,190591,381183,66.40091800689697,1.6791120691909394e-07
190791,190792,190791,381583,66.46028065681458,1.657496984649122e-07
190991,190992,190991,381983,66.52766799926758,1.6361929877227506e-07
191191,191192,191191,382383,66.60428285598755,1.6151612481616844e-07
191391,191392,191391,382783,66.67480492591858,1.594374761313716e-07
191592,191593,191592,383185,66.73496603965759,1.5737710509995908e-07
191792,191793,191792,383585,66.79504895210266,1.553552481558247e-07
191992,191993,191992,383985,66.8544819355011,1.5335383015895235e-07
192192,192193,192192,384385,66.91520166397095,1.5137711944338506e-07
192392,192393,192392,384785,66.97679996490479,1.494476857872407e-07
192593,192594,192593,385187,67.04678392410278,1.4756529137405865e-07
192793,192794,192793,385587,67.10744667053223,1.4571558904610506e-07
192993,192994,192993,385987,67.16641879081726,1.438552775562191e-07
193193,193194,193193,386387,67.22728395462036,1.4200736732755282e-07
193393,193394,193393,386787,67.28616786003113,1.402206265505515e-07
193594,193595,193594,387189,67.3452160358429,1.38487841259072e-07
193794,193795,193794,387589,67.41273593902588,1.3677925045925167e-07
193994,193995,193994,387989,67.47072887420654,1.3505679888684066e-07
194194,194195,194194,388389,67.53550171852112,1.3333945257277157e-07
194394,194395,194394,388789,67.5959689617157,1.3165881002515542e-07
194595,194596,194595,389191,67.65608668327332,1.3001269738221647e-07
194795,194796,194795,389591,67.71608281135559,1.2839786550831146e-07
194995,194996,194995,389991,67.77418184280396,1.267846978808963e-07
195195,195196,195195,390391,67.8316798210144,1.2516574577409197e-07
195395,195396,195395,390791,67.88878798484802,1.235539017118894e-07
195596,195597,195596,391193,67.94821786880493,1.2196787488171025e-07
195796,195797,195796,391593,68.01076579093933,1.2042646442762324e-07
195996,195997,195996,391993,68.07212281227112,1.1889282713378138e-07
196196,196197,196196,392393,68.13036894798279,1.1735389490475789e-07
196396,196397,196396,392793,68.18715071678162,1.1583263875314402e-07
196597,196598,196597,393195,68.24531674385071,1.143396542600712e-07
196797,196798,196797,393595,68.30553984642029,1.1287178909428801e-07
196997,196998,196997,393995,68.36324572563171,1.1140457339744957e-07
197197,197198,197197,394395,68.42155861854553,1.0995729019477146e-07
197397,197398,197397,394795,68.47958397865295,1.0855053616836268e-07
197598,197599,197598,395197,68.54426598548889,1.0716217891046946e-07
197798,197799,197798,395597,68.60455083847046,1.0578118339393362e-07
197998,197999,197998,395997,68.66564083099365,1.044090346227869e-07
198198,198199,198198,396397,68.73851490020752,1.0307312692123835e-07
198398,198399,198398,396797,68.80732679367065,1.0177676074940671e-07
198599,198600,198599,397199,68.86567974090576,1.0049481413669124e-07
198799,198800,198799,397599,68.92366576194763,9.922729371176391e-08
198999,199000,198999,397999,68.98159885406494,9.796925448788079e-08
199199,199200,199199,398399,69.04638171195984,9.673107976383111e-08
199399,199400,199399,398799,69.10658097267151,9.552364641923907e-08
199600,199601,199600,399201,69.1683099269867,9.433914868353828e-08
199800,199801,199800,399601,69.2270028591156,9.317096573598365e-08
200000,200001,200000,400001,69.28586792945862,9.20000982116779e-08


==> plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-aai.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0013942718505859375,30.358106049564984
100,309,0,309,1.3257431983947754,0.6507547624690679
200,609,0,609,2.8780300617218018,0.4182419742677393
300,909,0,909,4.388712167739868,0.3110699759547583
400,1209,0,1209,5.709566354751587,0.2465004680819078
501,1512,0,1512,6.936438083648682,0.20282738540711617
601,1885,0,1885,8.291751146316528,0.12622544045254913
701,2238,0,2238,9.883986234664917,0.07743810430328488
801,2602,0,2602,11.418199062347412,0.05325129915661818
901,2986,0,2986,12.78946828842163,0.04345792423451749
1001,3371,0,3371,14.251145362854004,0.0365011017767492
1101,3773,0,3773,15.607449054718018,0.0354375508873495
1201,4160,0,4160,17.138273000717163,0.02981484593213899
1301,4560,0,4560,18.95812702178955,0.02905896039873752
1401,4960,0,4960,20.28397512435913,0.026356620340761645
1502,5364,0,5364,21.7161762714386,0.025706961200401265
1602,5763,0,5763,23.441672325134277,0.025053600169154467
1702,6163,0,6163,24.93668508529663,0.02332565854780266
1802,6563,0,6563,27.31739616394043,0.022801049042980723
1902,6963,0,6963,28.759879112243652,0.022284665871272702
2002,7363,0,7363,30.785332918167114,0.02177763200369444
2102,7763,0,7763,32.381479263305664,0.021281419981965796
2202,8163,0,8163,33.93050813674927,0.020799524693982878
2302,8563,0,8563,35.49981212615967,0.020333657755180683
2402,8963,0,8963,36.82053804397583,0.01988131965592813
2503,9367,0,9367,38.088961124420166,0.019438349041856744
2603,9767,0,9767,39.32350301742554,0.01901171937323965
2703,10167,0,10167,40.66910910606384,0.018597009783050882
2803,10567,0,10567,42.108487129211426,0.018196952675144953
2903,10967,0,10967,43.49486517906189,0.017809676412902122
3003,11367,0,11367,44.94133400917053,0.017432966796540564
3103,11767,0,11767,47.342814207077026,0.01706720342611169
3203,12167,0,12167,49.65823006629944,0.016709862949451176
3303,12567,0,12567,51.03801608085632,0.016360531159521505
3403,12967,0,12967,52.678218364715576,0.016022328460370227
3504,13371,0,13371,54.107999324798584,0.01569015604597771
3604,13771,0,13771,55.499009132385254,0.015368212120845071
3704,14171,0,14171,56.8081111907959,0.015052928956088172
3804,14571,0,14571,58.17817521095276,0.014744764608116728
3904,14971,0,14971,59.618213176727295,0.014444478515888088
4004,15371,0,15371,61.146820068359375,0.014152361288010229
4104,15771,0,15771,63.08996510505676,0.013868448132787412
4204,16171,0,16171,64.53096914291382,0.013591314333172278
4304,16571,0,16571,65.94555902481079,0.013320199854744336
4404,16971,0,16971,67.32756114006042,0.013057116876893376
4505,17375,0,17375,68.8132700920105,0.012799273959925184
4605,17775,0,17775,70.14143991470337,0.012549457965282505
4705,18175,0,18175,71.50015616416931,0.01230467586786776
4805,18575,0,18575,72.81968116760254,0.012065379068085394
4905,18975,0,18975,74.06960320472717,0.011832570205677932
5005,19375,0,19375,75.44185018539429,0.011606891903434615
5105,19775,0,19775,76.82581233978271,0.011386065924475428
5205,20175,0,20175,78.1908061504364,0.01116838840480713
5305,20575,0,20575,79.5469081401825,0.010955288799765128
5405,20975,0,20975,80.77636909484863,0.010748463182153674
5506,21379,0,21379,82.18384099006653,0.010545310546435979
5606,21779,0,21779,83.42752814292908,0.010347920470839137
5706,22179,0,22179,84.71753025054932,0.010153940681293728
5806,22579,0,22579,86.02191829681396,0.009963913005620021
5906,22979,0,22979,87.30474519729614,0.009777287850303287
6006,23379,0,23379,88.60146617889404,0.009594540981701814
6106,23779,0,23779,89.86962723731995,0.009416719337336383
6206,24179,0,24179,91.21616315841675,0.00924273978820138
6306,24579,0,24579,92.51898527145386,0.009071119409911205
6406,24979,0,24979,93.78722715377808,0.008901789677730688
6507,25383,0,25383,95.0853180885315,0.008734038825469009
6607,25783,0,25783,96.28937220573425,0.008572474705299152
6707,26183,0,26183,97.67125606536865,0.008414866243460033
6807,26583,0,26583,99.01777625083923,0.008259313311634483
6907,26983,0,26983,100.27417421340942,0.008105748721700437
7007,27383,0,27383,101.58654713630676,0.007955529562193248
7107,27783,0,27783,102.97901010513306,0.00780919373545589
7207,28183,0,28183,104.21745729446411,0.007665904501052503
7307,28583,0,28583,105.60704112052917,0.007524905359377179
7407,28983,0,28983,107.01325631141663,0.007386490077686376
7508,29387,0,29387,108.37999510765076,0.007250190828197828
7608,29787,0,29787,109.7057740688324,0.00711877034482702
7708,30187,0,30187,111.00402808189392,0.006990152600426185
7808,30587,0,30587,112.38723921775818,0.0068636568236796975
7908,30987,0,30987,113.90844798088074,0.006739364849018432
8008,31387,0,31387,115.51555132865906,0.006617919916156095
8108,31787,0,31787,117.07736229896545,0.0064998319003776615
8208,32187,0,32187,118.48056435585022,0.006384874047414578
8308,32587,0,32587,119.9318950176239,0.006272224513318704
8408,32987,0,32987,121.46299719810486,0.006161140168506875
8509,33391,0,33391,123.33060503005981,0.006050297776820639
8609,33791,0,33791,124.80073428153992,0.005942584381552453
8709,34191,0,34191,126.07985925674438,0.005837946296906162
8809,34591,0,34591,127.42879509925842,0.0057364884452167945
8909,34991,0,34991,128.8494062423706,0.005636856477054728
9009,35391,0,35391,130.11250925064087,0.0055379537288795895
9109,35791,0,35791,132.27751326560974,0.005440027801509376
9209,36191,0,36191,133.93895316123962,0.005344026836957584
9309,36591,0,36591,135.36651420593262,0.005250470711951127
9409,36991,0,36991,137.55284023284912,0.005159039462309007
9510,37395,0,37395,139.10367727279663,0.005068065405467702
9610,37795,0,37795,140.5872540473938,0.004979015991549589
9710,38195,0,38195,142.466046333313,0.0048912152740051
9810,38595,0,38595,144.0951201915741,0.004805089934748792
9910,38995,0,38995,145.5192632675171,0.004720842512797192
10010,39395,0,39395,146.92554330825806,0.004638331629492168
10110,39795,0,39795,148.28331017494202,0.00455714383273268
10210,40195,0,40195,149.83534002304077,0.004477098057683501
10310,40595,0,40595,151.33019018173218,0.004398417688785877
10410,40995,0,40995,152.90133905410767,0.004321374983913718
10511,41399,0,41399,154.7786841392517,0.004245192040503568
10611,41799,0,41799,156.38902711868286,0.004171260805560101
10711,42199,0,42199,157.9491412639618,0.00409882913631162
10811,42599,0,42599,159.3759651184082,0.004028015348708646
10911,42999,0,42999,161.26487016677856,0.003958854471329461
11011,43399,0,43399,163.67064428329468,0.0038911650450352843
11111,43799,0,43799,165.07705807685852,0.0038246051275886463
11211,44199,0,44199,166.37035632133484,0.0037590367662733385
11311,44599,0,44599,167.8639690876007,0.00369465623117031
11411,44999,0,44999,169.2154951095581,0.003631865694224254
11512,45403,0,45403,170.75410723686218,0.0035702213362157386
11612,45803,0,45803,172.03366017341614,0.0035105026751957396
11712,46203,0,46203,173.37079334259033,0.003451427439638342
11812,46603,0,46603,174.75291109085083,0.0033928517413217797
11912,47003,0,47003,176.1000051498413,0.0033352398661281664
12012,47403,0,47403,177.38842105865479,0.0032791838094821807
12112,47803,0,47803,178.6816382408142,0.0032247140975964557
12212,48203,0,48203,179.97429704666138,0.0031711376312158323
12312,48603,0,48603,181.26625418663025,0.0031179053308697043
12412,49003,0,49003,182.53753113746643,0.0030651788633711853
12513,49407,0,49407,183.87928128242493,0.003012973807248253
12613,49807,0,49807,185.3775680065155,0.0029625165749871617
12713,50207,0,50207,187.05910921096802,0.0029130463650657106
12813,50607,0,50607,188.68206310272217,0.0028641723864838153
12913,51007,0,51007,190.28484296798706,0.0028158049214479413
13013,51407,0,51407,191.79163312911987,0.002768097981770114
13113,51807,0,51807,193.80993723869324,0.0027212577206088785
13213,52207,0,52207,195.33388113975525,0.0026753701200842896
13313,52607,0,52607,196.73185205459595,0.0026304417093238703
13413,53007,0,53007,198.085853099823,0.002586291247923236
13514,53411,0,53411,199.6228699684143,0.0025423106232928968
13614,53811,0,53811,201.05761098861694,0.002499527268664444
13714,54211,0,54211,202.51929116249084,0.00245769199844635
13814,54611,0,54611,203.83179712295532,0.002416732630308154
13914,55011,0,55011,205.2480161190033,0.0023764348375698912
14014,55411,0,55411,206.5768129825592,0.0023367048497196204
14114,55811,0,55811,208.0562460422516,0.0022978003691479444
14214,56211,0,56211,209.41531205177307,0.0022598911054391158
14314,56611,0,56611,210.74947214126587,0.0022227212480486606
14414,57011,0,57011,212.01885223388672,0.0021859738234900426
14515,57415,0,57415,213.3082091808319,0.002149392905430431
14615,57815,0,57815,214.62981820106506,0.002114000215870793
14715,58215,0,58215,216.12208199501038,0.0020795752259138273
14815,58615,0,58615,217.40436124801636,0.002045863870732177
14915,59015,0,59015,218.6551992893219,0.002012520976274969
15015,59415,0,59415,219.98070120811462,0.0019795682034044327
15115,59815,0,59815,221.35109496116638,0.0019472168721430191
15215,60215,0,60215,222.71408009529114,0.0019155840479106873
15315,60615,0,60615,224.15484523773193,0.0018846100571719632
15415,61015,0,61015,225.46359515190125,0.0018541948417008939
15516,61419,0,61419,226.86920428276062,0.0018238410209070722
15616,61819,0,61819,228.1631453037262,0.0017941188364593
15716,62219,0,62219,229.4073121547699,0.0017648020716875535
15816,62619,0,62619,230.861102104187,0.0017360344126222406
15916,63019,0,63019,232.12626099586487,0.001707866608355096
16016,63419,0,63419,233.42491221427917,0.0016801305389868557
16116,63819,0,63819,234.73857617378235,0.0016526024271049096
16216,64219,0,64219,236.0356583595276,0.001625364637911422
16316,64619,0,64619,237.28669428825378,0.0015986457495929147
16416,65019,0,65019,238.64607095718384,0.0015724954517711436
16517,65423,0,65423,239.87859725952148,0.0015465410373268294
16617,65823,0,65823,241.20359706878662,0.0015211622597440433
16717,66223,0,66223,242.7109191417694,0.0014961524371583706
16817,66623,0,66623,244.05299019813538,0.0014716815971164174
16917,67023,0,67023,245.46382212638855,0.0014477048721005556
17017,67423,0,67423,246.72404313087463,0.0014240937809227533
17117,67823,0,67823,247.64771127700806,0.0014008621205052457
17217,68223,0,68223,248.84257912635803,0.0013780778521612666
17317,68623,0,68623,250.26639008522034,0.0013557930380092102
17417,69023,0,69023,251.44510221481323,0.0013339893755452302
17518,69427,0,69427,252.66408228874207,0.001312318321097196
17618,69827,0,69827,253.9125370979309,0.0012911466345974076
17718,70227,0,70227,255.10173511505127,0.0012703533072887887
17818,70627,0,70627,256.12733817100525,0.0012499921720609162
17918,71027,0,71027,257.325168132782,0.0012301403507880093
18018,71427,0,71427,258.43595814704895,0.0012107402047670326
18118,71827,0,71827,259.45753812789917,0.0011916346730938452
18218,72227,0,72227,260.50616431236267,0.0011727029709069719
18318,72627,0,72627,261.6184639930725,0.0011539753824583846
18418,73027,0,73027,262.6610600948334,0.0011356046604891988
18519,73431,0,73431,263.7278881072998,0.0011175134924743734
18619,73831,0,73831,264.8621871471405,0.0010999862408079823
18719,74231,0,74231,265.91029024124146,0.0010826272468067338
18819,74631,0,74631,267.03843927383423,0.0010653470201187137
18919,75031,0,75031,268.4012773036957,0.001048252511288985
19019,75431,0,75431,270.01831912994385,0.001031521089464909
19119,75831,0,75831,271.2057421207428,0.0010151868380032882
19219,76231,0,76231,272.3089520931244,0.0009991272976077434
19319,76631,0,76631,273.45073318481445,0.0009832007547621177
19419,77031,0,77031,274.58428621292114,0.0009673938704916476
19520,77435,0,77435,275.9043519496918,0.0009516409683803534
19620,77835,0,77835,277.00987005233765,0.0009363404548170853
19720,78235,0,78235,278.05911111831665,0.000921362703504236
19820,78635,0,78635,279.1259319782257,0.0009066758120257018
19920,79035,0,79035,280.2930450439453,0.0008922464749570341
20020,79435,0,79435,281.3099613189697,0.0008780581871527938
20120,79835,0,79835,282.8442039489746,0.0008641098500179282
20220,80235,0,80235,284.25258326530457,0.0008503922100089217
20320,80635,0,80635,285.46898913383484,0.0008368883175660513
20420,81035,0,81035,286.63552618026733,0.0008236042699702059
20521,81439,0,81439,288.07090520858765,0.0008104537164871062
20621,81839,0,81839,289.33183097839355,0.0007977362436747548
20721,82239,0,82239,290.3971881866455,0.0007853094526995712
20821,82639,0,82639,291.45324420928955,0.0007730861722539401
20921,83039,0,83039,292.6145761013031,0.0007609877975096041
21021,83439,0,83439,293.65397334098816,0.0007490204622297301
21121,83839,0,83839,294.7806692123413,0.0007372819971865592
21221,84239,0,84239,295.90140318870544,0.0007258527384648382
21321,84639,0,84639,297.01545429229736,0.0007146963311767857
21421,85039,0,85039,298.20522904396057,0.0007036754498273726
21522,85443,0,85443,299.24672627449036,0.0006925984689575183
21622,85843,0,85843,300.29191422462463,0.0006817427362606502
21722,86243,0,86243,301.3416311740875,0.0006711226004206478
21822,86643,0,86643,302.4089353084564,0.0006607801966491446
21922,87043,0,87043,303.4068253040314,0.000650636868992007
22022,87443,0,87443,304.42526721954346,0.0006405776058091096
22122,87843,0,87843,305.44574427604675,0.0006305722331827804
22222,88243,0,88243,306.5190739631653,0.0006206730587145202
22322,88643,0,88643,307.6278340816498,0.000610945042903948
22422,89043,0,89043,308.6482470035553,0.0006014150101720749
22523,89447,0,89447,309.64598321914673,0.0005919631910887146
22623,89847,0,89847,310.64476323127747,0.0005827343039487044
22723,90247,0,90247,311.70755195617676,0.0005736218683153639
22823,90647,0,90647,312.76607608795166,0.0005646507357322053
22923,91047,0,91047,313.82152223587036,0.0005558550042906865
23023,91447,0,91447,314.9217641353607,0.0005472343501870208
23123,91847,0,91847,316.0132031440735,0.0005387492039469365
23223,92247,0,92247,317.15062713623047,0.0005303746919463805
23323,92647,0,92647,318.3307251930237,0.0005221246244921503
23423,93047,0,93047,319.39635396003723,0.0005140231809636976
23524,93451,0,93451,320.46302318573,0.0005059808989078129
23624,93851,0,93851,321.4664011001587,0.0004981260379678544
23724,94251,0,94251,322.4534749984741,0.0004903765375955209
23824,94651,0,94651,323.44416403770447,0.0004827800708702784
23924,95051,0,95051,324.4483850002289,0.0004753641784925095
24024,95451,0,95451,325.439893245697,0.00046810511835460847
24124,95851,0,95851,326.4390251636505,0.0004609444542536899
24224,96251,0,96251,327.4278492927551,0.00045385860043912845
24324,96651,0,96651,328.4334282875061,0.00044688021003721617
24424,97051,0,97051,329.4233720302582,0.00044005081923466935
24525,97455,0,97455,330.4420852661133,0.0004333080267294898
24625,97855,0,97855,331.44218015670776,0.0004267498640150915
24725,98255,0,98255,332.4462089538574,0.000420273870148551
24825,98655,0,98655,333.43499517440796,0.0004138666777851403
24925,99055,0,99055,334.4527630805969,0.0004075487951987757
25025,99455,0,99455,335.4453649520874,0.0004013435912567003
25125,99855,0,99855,336.4456181526184,0.0003952591876055962
25225,100255,0,100255,337.4488501548767,0.00038926910819748805
25325,100655,0,100655,338.44034814834595,0.0003833427975293865
25425,101055,0,101055,339.4847753047943,0.0003774772172054246
25526,101459,0,101459,340.48418712615967,0.00037163947874811824
25626,101859,0,101859,341.48699736595154,0.0003659729725449927
25726,102259,0,102259,342.5179831981659,0.00036040546811693037
25826,102659,0,102659,343.5232219696045,0.00035490869049088346
25926,103059,0,103059,344.5140151977539,0.00034947369577205525
26026,103459,0,103459,345.5404930114746,0.0003441142167159695
26126,103859,0,103859,346.5290632247925,0.00033884478743114696
26226,104259,0,104259,347.5746190547943,0.00033366565119359153
26326,104659,0,104659,348.6023211479187,0.0003285623625134495
26426,105059,0,105059,349.65351819992065,0.00032353980652274715
26527,105463,0,105463,350.68159198760986,0.0003185604267722937
26627,105863,0,105863,351.6799590587616,0.00031371933830147517
26727,106263,0,106263,352.67128920555115,0.0003089547111937232
26827,106663,0,106663,353.6594431400299,0.0003042546872309285
26927,107063,0,107063,354.6641652584076,0.00029962096264257146
27027,107463,0,107463,355.65529322624207,0.00029506827443446815
27127,107863,0,107863,356.79106616973877,0.0002906055792065784
27227,108263,0,108263,357.886372089386,0.00028622549208219496
27327,108663,0,108663,358.9966812133789,0.0002819159369750738
27427,109063,0,109063,360.0048770904541,0.0002776670474268531
27528,109467,0,109467,361.075434923172,0.00027344288370076257
27628,109867,0,109867,362.10153007507324,0.00026934092248323907
27728,110267,0,110267,363.19413924217224,0.00026532895146723313
27828,110667,0,110667,364.3256850242615,0.00026138777792272333
27928,111067,0,111067,365.410117149353,0.0002574923490464453
28028,111467,0,111467,366.4783601760864,0.00025363063438622717
28128,111867,0,111867,367.58180022239685,0.0002498173679740786
28228,112267,0,112267,368.6898012161255,0.0002460785476639138
28328,112667,0,112667,369.73567509651184,0.0002424193866919694
28428,113067,0,113067,370.7259042263031,0.00023881403962149264
28529,113471,0,113471,371.74574422836304,0.00023520226694484332
28629,113871,0,113871,372.7768371105194,0.00023165407319258353
28729,114271,0,114271,373.84909415245056,0.00022814869049691638
28829,114671,0,114671,374.92775416374207,0.0002247076484011169
28929,115071,0,115071,376.01430010795593,0.00022133124997030147
29029,115471,0,115471,377.0426800251007,0.00021800847619289274
29129,115871,0,115871,378.12698698043823,0.00021473409427183202
29229,116271,0,116271,379.18932127952576,0.0002115068493260824
29329,116671,0,116671,380.28385305404663,0.00020832828602043848
29429,117071,0,117071,381.3401322364807,0.0002052019016221952
29530,117475,0,117475,382.4307670593262,0.0002020917180155017
29630,117875,0,117875,383.4690160751343,0.000199056694005001
29730,118275,0,118275,384.591924905777,0.00019606859155655275
29830,118675,0,118675,385.64229011535645,0.00019312579891759497
29930,119075,0,119075,386.6971802711487,0.0001902261216503937
30030,119475,0,119475,387.89540219306946,0.00018736527897840997
30130,119875,0,119875,389.1136722564697,0.00018453992392629458
30230,120275,0,120275,390.2558591365814,0.0001817618848748329
30330,120675,0,120675,391.4258060455322,0.0001790473959149819
30430,121075,0,121075,392.5677082538605,0.00017639893568001098
30531,121479,0,121479,394.2540521621704,0.00017377634308344243
30631,121879,0,121879,395.8938159942627,0.00017121008402431486
30731,122279,0,122279,397.1998071670532,0.00016866265796159258
30831,122679,0,122679,398.25563621520996,0.00016614825333388303
30931,123079,0,123079,399.4763581752777,0.0001636862735752721
31031,123479,0,123479,400.57799315452576,0.00016127849224959907
31131,123879,0,123879,401.90285897254944,0.000158911661910389
31231,124279,0,124279,403.03972911834717,0.000156566337465703
31331,124679,0,124679,404.0527353286743,0.00015423878029110062
31431,125079,0,125079,405.0433671474457,0.00015194383854620188
31532,125483,0,125483,406.05002617836,0.00014967728225045984
31632,125883,0,125883,406.9705812931061,0.00014748141364491927
31732,126283,0,126283,407.7231001853943,0.0001453236496155613
31832,126683,0,126683,408.81299805641174,0.00014318577820739394
31932,127083,0,127083,409.85258316993713,0.0001410630636861738
32032,127483,0,127483,410.917592048645,0.00013896495685249098
32132,127883,0,127883,411.94422221183777,0.00013690068219397215
32232,128283,0,128283,413.0728142261505,0.00013487394860806374
32332,128683,0,128683,414.21441411972046,0.00013288422901165894
32432,129083,0,129083,415.2850432395935,0.00013092481030741037
32533,129487,0,129487,416.303524017334,0.00012897076579163302
32633,129887,0,129887,417.32983922958374,0.00012706354815131054
32733,130287,0,130287,418.4362292289734,0.00012517977678015444
32833,130687,0,130687,419.4902651309967,0.00012332019549503957
32933,131087,0,131087,420.50152707099915,0.00012149010101979144
33033,131487,0,131487,421.6357972621918,0.00011969138451786213
33133,131887,0,131887,422.889475107193,0.00011792744669814292
33233,132287,0,132287,423.99755120277405,0.00011619614486706059
33333,132687,0,132687,425.22660303115845,0.00011448422249397478
33433,133087,0,133087,426.55300307273865,0.00011279029892638291
33534,133491,0,133491,428.3420422077179,0.00011110764052425343
33634,133891,0,133891,429.65023922920227,0.00010947545315292079
33734,134291,0,134291,430.98934412002563,0.00010788322633093137
33834,134691,0,134691,432.1551170349121,0.00010632222575153737
33934,135091,0,135091,433.7206072807312,0.00010477778169075889
34034,135491,0,135491,435.2484230995178,0.00010325130623508456
34134,135891,0,135891,436.99455404281616,0.00010174668960357438
34234,136291,0,136291,438.0871322154999,0.00010026908442009072
34334,136691,0,136691,439.2035140991211,9.882425639087327e-05
34434,137091,0,137091,440.3708510398865,9.740489934607251e-05
34535,137495,0,137495,442.57846331596375,9.598480524907882e-05
34635,137895,0,137895,444.6038911342621,9.459384537432654e-05
34735,138295,0,138295,446.07711720466614,9.321669210295596e-05
34835,138695,0,138695,447.1051902770996,9.186034875953142e-05
34935,139095,0,139095,448.11547207832336,9.052982550168082e-05
35035,139495,0,139495,449.10090708732605,8.92164727620526e-05
35135,139895,0,139895,450.098441362381,8.791907397811734e-05
35235,140295,0,140295,451.09479117393494,8.663904547262731e-05
35335,140695,0,140695,452.0951783657074,8.537736021308555e-05
35435,141095,0,141095,453.0814073085785,8.413637141505549e-05
35536,141499,0,141499,454.1009750366211,8.290218088452492e-05
35636,141899,0,141899,455.08919501304626,8.169775599583504e-05
35736,142299,0,142299,456.1527841091156,8.050980248098726e-05
35836,142699,0,142699,457.1680529117584,7.933879789632287e-05
35936,143099,0,143099,458.1706962585449,7.818308111840444e-05
36036,143499,0,143499,459.1510121822357,7.704229695343715e-05
36136,143899,0,143899,460.1360182762146,7.59171165284166e-05
36236,144299,0,144299,461.13270711898804,7.48103105131684e-05
36336,144699,0,144699,462.12735414505005,7.372422598790913e-05
36436,145099,0,145099,463.12385416030884,7.265879187829862e-05
36537,145503,0,145503,464.1199150085449,7.160137565200747e-05
36637,145903,0,145903,465.1146080493927,7.057174588152417e-05
36737,146303,0,146303,466.1013660430908,6.955945952849099e-05
36837,146703,0,146703,467.1002140045166,6.856652057333526e-05
36937,147103,0,147103,468.0889720916748,6.759265262571435e-05
37037,147503,0,147503,469.0820610523224,6.663467672217817e-05
37137,147903,0,147903,470.06203722953796,6.568809940505057e-05
37237,148303,0,148303,471.05312609672546,6.475095377543622e-05
37337,148703,0,148703,472.03926706314087,6.382472233856275e-05
37437,149103,0,149103,473.0179052352905,6.291342747488348e-05
37538,149507,0,149507,474.0270850658417,6.200868654269514e-05
37638,149907,0,149907,475.36258912086487,6.112581513221243e-05
37738,150307,0,150307,476.5173201560974,6.0251812479518895e-05
37838,150707,0,150707,477.52821230888367,5.938581968737049e-05
37938,151107,0,151107,478.5801191329956,5.853082032565416e-05
38038,151507,0,151507,480.0252311229706,5.769017168739846e-05
38138,151907,0,151907,481.16616010665894,5.686502208912203e-05
38238,152307,0,152307,482.3984282016754,5.605363998276093e-05
38338,152707,0,152707,483.63373017311096,5.525336418396882e-05
38438,153107,0,153107,484.94600009918213,5.446326214701382e-05
38539,153511,0,153511,486.29078912734985,5.367594125777318e-05
38639,153911,0,153911,487.6389229297638,5.2907840519948476e-05
38739,154311,0,154311,489.18898725509644,5.2151945661753104e-05
38839,154711,0,154711,490.29198932647705,5.1407917682869146e-05
38939,155111,0,155111,491.3472549915314,5.067568178899403e-05
39039,155511,0,155511,492.4073541164398,4.9954439275361084e-05
39139,155911,0,155911,493.49091601371765,4.924334693885037e-05
39239,156311,0,156311,494.7532353401184,4.8541978607420313e-05
39339,156711,0,156711,496.2634479999542,4.7851136506433944e-05
39439,157111,0,157111,497.4674801826477,4.7171751473896564e-05
39540,157515,0,157515,498.54406905174255,4.6498403011874585e-05
39640,157915,0,157915,499.63926219940186,4.5842853010942615e-05
39740,158315,0,158315,500.63603711128235,4.5196447928530915e-05
39840,158715,0,158715,501.64628314971924,4.455746233899277e-05
39940,159115,0,159115,502.6616430282593,4.39266923026386e-05
40040,159515,0,159515,503.6896412372589,4.330722491081732e-05
40140,159915,0,159915,504.7260551452637,4.2700188223661464e-05
40240,160315,0,160315,505.7306101322174,4.210478121716521e-05
40340,160715,0,160715,506.73683619499207,4.151688057124669e-05
40440,161115,0,161115,507.72879815101624,4.0933794901470184e-05
40541,161519,0,161519,508.7896182537079,4.035038955071414e-05
40641,161919,0,161919,509.8320822715759,3.9781410389822186e-05
40741,162319,0,162319,510.88662910461426,3.922359090576307e-05
40841,162719,0,162719,511.9524390697479,3.8676209565013035e-05
40941,163119,0,163119,513.0294530391693,3.8135728513416286e-05
41041,163519,0,163519,514.0424020290375,3.759931452240164e-05
41141,163919,0,163919,515.0468881130219,3.706755012762417e-05
41241,164319,0,164319,516.2123100757599,3.654310401692769e-05
41341,164719,0,164719,517.511214017868,3.602930826266534e-05
41441,165119,0,165119,518.7000062465668,3.552630053197368e-05
41542,165523,0,165523,519.7183301448822,3.502700887585216e-05
41642,165923,0,165923,520.775562286377,3.453848331963569e-05
41742,166323,0,166323,521.9549460411072,3.40545464973837e-05
41842,166723,0,166723,523.1511561870575,3.357609857912339e-05
41942,167123,0,167123,524.4625062942505,3.3105104687177495e-05
42042,167523,0,167523,525.88605427742,3.2643058733740716e-05
42142,167923,0,167923,527.1354732513428,3.218981763336597e-05
42242,168323,0,168323,528.4549281597137,3.174405997224603e-05
42342,168723,0,168723,529.6390731334686,3.130387613325087e-05
42442,169123,0,169123,530.8285531997681,3.086769732740725e-05
42543,169527,0,169527,531.9804141521454,3.0431192242622897e-05
42643,169927,0,169927,533.6264822483063,3.0004304201570393e-05
42743,170327,0,170327,534.8456251621246,2.958485139992288e-05
42843,170727,0,170727,536.2514982223511,2.9173888324019765e-05
42943,171127,0,171127,537.317253112793,2.8770464179708746e-05
43043,171527,0,171527,538.321542263031,2.8372448808121058e-05
43143,171927,0,171927,539.3156542778015,2.797807427382608e-05
43243,172327,0,172327,540.2998111248016,2.7588125409690452e-05
43343,172727,0,172727,541.3872423171997,2.720448877470487e-05
43443,173127,0,173127,542.4823281764984,2.682870052336601e-05
43544,173531,0,173531,543.7519881725311,2.645593846849383e-05
43644,173931,0,173931,544.8588061332703,2.6091094352291837e-05
43744,174331,0,174331,545.8787310123444,2.572785873359281e-05
43844,174731,0,174731,546.9218912124634,2.5366970880339185e-05
43944,175131,0,175131,548.0383841991425,2.5010573177106722e-05
44044,175531,0,175531,549.1710162162781,2.4661525675845345e-05
44144,175931,0,175931,550.2923800945282,2.4320668474522675e-05
44244,176331,0,176331,551.43421626091,2.3986592352350425e-05
44344,176731,0,176731,552.7863461971283,2.3657501962508774e-05
44444,177131,0,177131,554.0807480812073,2.3332351584105995e-05
44545,177535,0,177535,555.1927480697632,2.3008363738438773e-05
44645,177935,0,177935,556.395188331604,2.2692614418630773e-05
44745,178335,0,178335,557.4989211559296,2.2382231538718818e-05
44845,178735,0,178735,558.7036671638489,2.207622470308336e-05
44945,179135,0,179135,560.014847278595,2.1774014121078972e-05
45045,179535,0,179535,561.5879452228546,2.1474766996474042e-05
45145,179935,0,179935,562.8088240623474,2.1178689104366647e-05
45245,180335,0,180335,564.090968132019,2.0886337825348448e-05
45345,180735,0,180735,565.5297381877899,2.0598172496271158e-05
45445,181135,0,181135,566.6878509521484,2.0315056016407612e-05
45546,181539,0,181539,567.7800121307373,2.0034041301974822e-05
45646,181939,0,181939,568.9753642082214,1.9760409854259747e-05
45746,182339,0,182339,569.9647040367126,1.949068917943313e-05
45846,182739,0,182739,571.4102830886841,1.9224465537906003e-05
45946,183139,0,183139,572.5167112350464,1.896201192914267e-05
46046,183539,0,183539,573.6434030532837,1.8703711456500528e-05
46146,183939,0,183939,574.9623260498047,1.8449640067827e-05
46246,184339,0,184339,576.0870361328125,1.8199343147451876e-05
46346,184739,0,184739,577.1256680488586,1.7952264618032697e-05
46446,185139,0,185139,578.3857641220093,1.770799472806867e-05
46547,185543,0,185543,579.4220821857452,1.7464743831697954e-05
46647,185943,0,185943,580.5141031742096,1.722776873860336e-05
46747,186343,0,186343,581.3292181491852,1.6994910254835852e-05
46847,186743,0,186743,582.6953721046448,1.6765650870970367e-05
46947,187143,0,187143,583.9828500747681,1.6539186208977222e-05
47047,187543,0,187543,585.1963651180267,1.6315300860420997e-05
47147,187943,0,187943,586.4084820747375,1.6094185032023962e-05
47247,188343,0,188343,588.0410380363464,1.5876555508977693e-05
47347,188743,0,188743,589.2095663547516,1.5662663687851418e-05
47447,189143,0,189143,590.3033990859985,1.545228607945765e-05
47548,189547,0,189547,591.5232892036438,1.5243089138493048e-05
47648,189947,0,189947,592.6011960506439,1.5038979476610688e-05
47748,190347,0,190347,593.6105592250824,1.4838164235708716e-05
47848,190747,0,190747,594.6183032989502,1.4640945891980317e-05
47948,191147,0,191147,595.7158432006836,1.4447278005491406e-05
48048,191547,0,191547,596.7931661605835,1.4256848524202011e-05
48148,191947,0,191947,597.8204391002655,1.40689802950577e-05
48248,192347,0,192347,598.8248331546783,1.3883157446564332e-05
48348,192747,0,192747,599.8229801654816,1.36992177439814e-05
48448,193147,0,193147,600.8519032001495,1.351729771919296e-05
48549,193551,0,193551,601.9680330753326,1.3335837044536997e-05
48649,193951,0,193951,603.0528712272644,1.3158729742192206e-05
48749,194351,0,194351,604.0618481636047,1.2984057736325511e-05
48849,194751,0,194751,605.0527131557465,1.2811695616457415e-05
48949,195151,0,195151,606.0559799671173,1.264148639817577e-05
49049,195551,0,195551,607.0398392677307,1.2473403608076921e-05
49149,195951,0,195951,608.0317831039429,1.2307708479639038e-05
49249,196351,0,196351,609.0545401573181,1.214448625758407e-05
49349,196751,0,196751,610.0444111824036,1.1983733834179065e-05
49449,197151,0,197151,611.0636131763458,1.1825016208866703e-05
49550,197555,0,197555,612.0737330913544,1.1666644093359632e-05
49650,197955,0,197955,613.1485161781311,1.1511657256007075e-05
49750,198355,0,198355,614.1764721870422,1.135903485513368e-05
49850,198755,0,198755,615.1814641952515,1.1209135438638551e-05
49950,199155,0,199155,616.2290060520172,1.1062057889284107e-05
50050,199555,0,199555,617.2373633384705,1.0917302462094327e-05
50150,199955,0,199955,618.2452793121338,1.0774230643912528e-05
50250,200355,0,200355,619.2969691753387,1.063253491129586e-05
50350,200755,0,200755,620.2837240695953,1.0492483734337304e-05
50450,201155,0,201155,621.3276801109314,1.035474516791634e-05
50551,201559,0,201559,622.3290610313416,1.021822903828198e-05
50651,201959,0,201959,623.3441913127899,1.0085594708426323e-05
50751,202359,0,202359,624.3804280757904,9.954836535181103e-06
50851,202759,0,202759,625.3796589374542,9.825650048544928e-06
50951,203159,0,203159,626.3680601119995,9.697939698790288e-06
51051,203559,0,203559,627.3758492469788,9.571945114533722e-06
51151,203959,0,203959,628.4409573078156,9.447695721932687e-06
51251,204359,0,204359,629.5014071464539,9.324911077350676e-06
51351,204759,0,204759,630.578152179718,9.203035696461605e-06
51451,205159,0,205159,631.6558091640472,9.081650478476648e-06
51552,205563,0,205563,632.6903390884399,8.95962500118488e-06
51652,205963,0,205963,633.6959891319275,8.83985127087238e-06
51752,206363,0,206363,634.7289042472839,8.721849220794106e-06
51852,206763,0,206763,635.7285680770874,8.606096806631979e-06
51952,207163,0,207163,636.8051381111145,8.492665965099632e-06
52052,207563,0,207563,637.824969291687,8.381225596827836e-06
52152,207963,0,207963,638.8321640491486,8.271369276637015e-06
52252,208363,0,208363,639.8122990131378,8.16279965861016e-06
52352,208763,0,208763,640.8534829616547,8.055561275217626e-06
52452,209163,0,209163,641.8400650024414,7.949936598108902e-06
52553,209567,0,209567,642.8706271648407,7.845095367950762e-06
52653,209967,0,209967,643.8680372238159,7.742903785998902e-06
52753,210367,0,210367,644.8584632873535,7.642040998701366e-06
52853,210767,0,210767,645.9236991405487,7.5420329193684395e-06
52953,211167,0,211167,646.9664182662964,7.443137799215738e-06
53053,211567,0,211567,647.9657912254333,7.345820028657914e-06
53153,211967,0,211967,649.0217311382294,7.250603728363687e-06
53253,212367,0,212367,650.0586552619934,7.15766801946621e-06
53353,212767,0,212767,651.1012892723083,7.066473656269929e-06
53453,213167,0,213167,652.1935620307922,6.976346024624254e-06
53554,213571,0,213571,653.1913640499115,6.885916108395203e-06
53654,213971,0,213971,654.2576770782471,6.797099124601739e-06
53754,214371,0,214371,655.274697303772,6.7093271483412155e-06
53854,214771,0,214771,656.8361930847168,6.623070481088954e-06
53954,215171,0,215171,658.0087883472443,6.53819019410309e-06
54054,215571,0,215571,659.430251121521,6.454413882037678e-06
54154,215971,0,215971,660.6212720870972,6.371480296821456e-06
54254,216371,0,216371,662.3938090801239,6.28926962026742e-06
54354,216771,0,216771,664.0144181251526,6.2080586569873455e-06
54454,217171,0,217171,665.5412590503693,6.128068291095267e-06
54555,217575,0,217575,667.1645832061768,6.0485804600161595e-06
54655,217975,0,217975,668.675594329834,5.970969770861281e-06
54755,218375,0,218375,670.4293601512909,5.894223568229561e-06
54855,218775,0,218775,672.3742399215698,5.8180816778302945e-06
54955,219175,0,219175,674.3033351898193,5.742671881943044e-06
55055,219575,0,219575,675.4915812015533,5.6682689975973985e-06
55155,219975,0,219975,676.6361591815948,5.595117891605344e-06
55255,220375,0,220375,677.817877292633,5.523516138411069e-06
55355,220775,0,220775,678.9796681404114,5.4533916387236665e-06
55455,221175,0,221175,680.1013350486755,5.3845500601115786e-06
55556,221579,0,221579,681.5626201629639,5.316129703487026e-06
55656,221979,0,221979,682.7532021999359,5.249403219276246e-06
55756,222379,0,222379,683.8975882530212,5.1836920378081895e-06
55856,222779,0,222779,685.2395482063293,5.119123136614227e-06
55956,223179,0,223179,686.351056098938,5.0555465323844834e-06
56056,223579,0,223579,687.3846471309662,4.992782080638137e-06
56156,223979,0,223979,688.4062051773071,4.930689948811121e-06
56256,224379,0,224379,689.4379193782806,4.869135102791936e-06
56356,224779,0,224779,690.4742381572723,4.808255019351345e-06
56456,225179,0,225179,691.5622591972351,4.748228341129539e-06
56557,225583,0,225583,692.6293942928314,4.6885234610329356e-06
56657,225983,0,225983,693.6982400417328,4.630248797921739e-06
56757,226383,0,226383,694.799173116684,4.572668913662691e-06
56857,226783,0,226783,696.5837690830231,4.5156219338936226e-06
56957,227183,0,227183,698.0538511276245,4.459127358579368e-06
57057,227583,0,227583,699.2839541435242,4.40331125808424e-06
57157,227983,0,227983,700.9476132392883,4.348128492884911e-06
57257,228383,0,228383,702.1238760948181,4.293644517479232e-06
57357,228783,0,228783,703.341824054718,4.239798075609552e-06
57457,229183,0,229183,705.2493031024933,4.186517036364248e-06
57558,229587,0,229587,707.4480082988739,4.133340724856987e-06
57658,229987,0,229987,708.9408671855927,4.08139716676382e-06
57758,230387,0,230387,710.06059217453,4.030204162088082e-06
57858,230787,0,230787,711.6056010723114,3.9798110550305215e-06
57958,231187,0,231187,712.9833152294159,3.930221550922501e-06
58058,231587,0,231587,714.3864681720734,3.881311482298429e-06
58158,231987,0,231987,715.4723660945892,3.8332331369600245e-06
58258,232387,0,232387,716.6452369689941,3.7859352843292656e-06
58358,232787,0,232787,717.9499592781067,3.7394264613393535e-06
58458,233187,0,233187,719.4845969676971,3.693740422425617e-06
58559,233591,0,233591,720.7327680587769,3.648286751095104e-06
58659,233991,0,233991,721.9344301223755,3.6038327363250865e-06
58759,234391,0,234391,723.1373450756073,3.5598468900574956e-06
58859,234791,0,234791,724.2824430465698,3.5162069556923925e-06
58959,235191,0,235191,725.3549811840057,3.4729135677940472e-06
59059,235591,0,235591,726.4161510467529,3.430090824602499e-06
59159,235991,0,235991,727.7118473052979,3.387621914787003e-06
59259,236391,0,236391,728.9871249198914,3.345561302183569e-06
59359,236791,0,236791,730.4741811752319,3.3039740340263686e-06
59459,237191,0,237191,731.8067572116852,3.2627825045956263e-06
59560,237595,0,237595,733.1149852275848,3.2217623468362737e-06
59660,237995,0,237995,734.2683219909668,3.181754183696677e-06
59760,238395,0,238395,736.1057043075562,3.142352294922836e-06
59860,238795,0,238795,737.6260652542114,3.103545859882017e-06
59960,239195,0,239195,739.3872129917145,3.0652456821621016e-06
60060,239595,0,239595,740.919536113739,3.0273166125728335e-06
60160,239995,0,239995,742.6512761116028,2.989867056676196e-06
60260,240395,0,240395,743.8366949558258,2.952888321344867e-06
60360,240795,0,240795,745.287709236145,2.916320135033591e-06
60460,241195,0,241195,746.3824801445007,2.8802413999003536e-06
60561,241599,0,241599,747.4534063339233,2.8442250376086884e-06
60661,241999,0,241999,748.7622570991516,2.8089741283178198e-06
60761,242399,0,242399,749.8771481513977,2.7742600313758343e-06
60861,242799,0,242799,751.5456392765045,2.740040262608529e-06
60961,243199,0,243199,752.7018442153931,2.706389367869176e-06
61061,243599,0,243599,753.783370256424,2.6733382121301483e-06
61161,243999,0,243999,754.8596611022949,2.64069991370476e-06
61261,244399,0,244399,755.9157192707062,2.6084546714155837e-06
61361,244799,0,244799,756.9667780399323,2.5766848069360984e-06
61461,245199,0,245199,757.9608690738678,2.5452902395189833e-06
61562,245603,0,245603,759.0303871631622,2.5140911161542614e-06
61662,246003,0,246003,760.0438132286072,2.4837238245520025e-06
61762,246403,0,246403,761.0542650222778,2.4537474279728738e-06
61862,246803,0,246803,762.0401840209961,2.4242513185264145e-06
61962,247203,0,247203,763.0221741199493,2.395082194623818e-06
62062,247603,0,247603,764.1599049568176,2.3661778989874117e-06
62162,248003,0,248003,765.2604939937592,2.3377148662151028e-06
62262,248403,0,248403,766.2949151992798,2.3096265637023976e-06
62362,248803,0,248803,767.34334897995,2.281808213590547e-06
62462,249203,0,249203,768.3266880512238,2.2543788736567392e-06
62563,249607,0,249607,769.3407561779022,2.2267855488598186e-06
62663,250007,0,250007,770.4326503276825,2.199669948610493e-06
62763,250407,0,250407,771.4548561573029,2.1727766477733587e-06
62863,250807,0,250807,772.442223072052,2.1462690757759383e-06
62963,251207,0,251207,773.7432081699371,2.120178255857176e-06
63063,251607,0,251607,774.8062152862549,2.09454822417445e-06
63163,252007,0,252007,775.901123046875,2.0693017110775478e-06
63263,252407,0,252407,777.0236222743988,2.0443749484881163e-06
63363,252807,0,252807,778.0860903263092,2.0197617907224266e-06
63463,253207,0,253207,779.3427550792694,1.995493427360685e-06
63564,253611,0,253611,780.266520023346,1.97139229558571e-06
63664,254011,0,254011,781.0719332695007,1.9479418001527857e-06
63764,254411,0,254411,782.030641078949,1.924834509294109e-06
63864,254811,0,254811,783.0867431163788,1.9020028983841408e-06
63964,255211,0,255211,784.1868510246277,1.8793923292913581e-06
64064,255611,0,255611,785.2005131244659,1.8570328049087636e-06
64164,256011,0,256011,786.2473940849304,1.8349743397947918e-06
64264,256411,0,256411,787.372935295105,1.8132793296433024e-06
64364,256811,0,256811,788.4433310031891,1.7919418038348578e-06
64464,257211,0,257211,789.5576272010803,1.770918113164439e-06
64565,257615,0,257615,790.6588661670685,1.7499264036300537e-06
64665,258015,0,258015,791.7803702354431,1.7293333319452015e-06
64765,258415,0,258415,793.0903232097626,1.7089253274686808e-06
64865,258815,0,258815,794.1923530101776,1.6887238647171406e-06
64965,259215,0,259215,795.3986873626709,1.6687428933357523e-06
65065,259615,0,259615,796.4649271965027,1.6489829100005038e-06
65165,260015,0,260015,797.6697173118591,1.6293824477856277e-06
65265,260415,0,260415,798.7960503101349,1.6099276506428023e-06
65365,260815,0,260815,800.0661461353302,1.5905814654011146e-06
65465,261215,0,261215,801.3166501522064,1.5714139668683233e-06
65566,261619,0,261619,802.565092086792,1.5522837876226608e-06
65666,262019,0,262019,803.6415331363678,1.5336400666136054e-06
65766,262419,0,262419,804.6969132423401,1.515300850471348e-06
65866,262819,0,262819,805.6872119903564,1.497245275117191e-06
65966,263219,0,263219,806.6691403388977,1.4794424086375368e-06
66066,263619,0,263619,807.6774272918701,1.4618707073977875e-06
66166,264019,0,264019,808.6544580459595,1.4445520582828496e-06
66266,264419,0,264419,809.6196253299713,1.4274704444059194e-06
66366,264819,0,264819,810.8162460327148,1.4106444234349605e-06
66466,265219,0,265219,812.0272421836853,1.3940132227299357e-06
66567,265623,0,265623,813.1285643577576,1.3774039578916548e-06
66667,266023,0,266023,814.1375563144684,1.3611191454388932e-06
66767,266423,0,266423,815.2245512008667,1.345021182879363e-06
66867,266823,0,266823,816.2662572860718,1.3291447259736833e-06
66967,267223,0,267223,817.2963471412659,1.3135000798574967e-06
67067,267623,0,267623,818.3205161094666,1.2981024415150494e-06
67167,268023,0,268023,819.3667030334473,1.2829156725181327e-06
67267,268423,0,268423,820.4118509292603,1.2679262483326907e-06
67367,268823,0,268823,821.4513032436371,1.2531132991180455e-06
67467,269223,0,269223,822.4573440551758,1.2384682144442457e-06
67568,269627,0,269627,823.543799161911,1.2238452451863084e-06
67668,270027,0,270027,824.5630550384521,1.2095152150899361e-06
67768,270427,0,270427,825.6330552101135,1.1953278996768847e-06
67868,270827,0,270827,826.7277760505676,1.1812585198159799e-06
67968,271227,0,271227,827.7762720584869,1.1673167802833678e-06
68068,271627,0,271627,828.8376371860504,1.1534990541942596e-06
68168,272027,0,272027,829.8604590892792,1.1398314220677187e-06
68268,272427,0,272427,830.921168088913,1.1263105672165294e-06
68368,272827,0,272827,832.1719479560852,1.1129489175853223e-06
68468,273227,0,273227,833.3938670158386,1.0997318978161957e-06
68569,273631,0,273631,834.5086162090302,1.0865303243533404e-06
68669,274031,0,274031,835.5781490802765,1.0736133538596146e-06
68769,274431,0,274431,836.6413171291351,1.0608614281135875e-06
68869,274831,0,274831,837.6496601104736,1.0483012593675632e-06
68969,275231,0,275231,838.7254812717438,1.0359412601086447e-06
69069,275631,0,275631,839.8014409542084,1.023789525530111e-06
69169,276031,0,276031,840.9427199363708,1.011842107933497e-06
69269,276431,0,276431,842.0674731731415,1.0000944219321423e-06
69369,276831,0,276831,843.6644041538239,9.885471379049085e-07
69469,277231,0,277231,845.1625919342041,9.7718955479878e-07
69570,277635,0,277635,846.3538012504578,9.659094887044727e-07
69670,278035,0,278035,847.9398510456085,9.54903046785818e-07
69770,278435,0,278435,849.4691061973572,9.4404678818232e-07
69870,278835,0,278835,850.8184220790863,9.333108626545276e-07
69970,279235,0,279235,851.8698239326477,9.226982245004449e-07
70070,279635,0,279635,852.946702003479,9.121918523054026e-07
70170,280035,0,280035,854.1681931018829,9.017904365217595e-07
70270,280435,0,280435,855.3023171424866,8.914867277509191e-07
70370,280835,0,280835,856.3659851551056,8.812657899412108e-07
70470,281235,0,281235,857.4272072315216,8.711361565196021e-07
70571,281639,0,281639,858.5804421901703,8.609867966318388e-07
70671,282039,0,282039,859.6804389953613,8.510431707216438e-07
70771,282439,0,282439,860.7975351810455,8.411976006039792e-07
70871,282839,0,282839,861.8751800060272,8.314646398451331e-07
70971,283239,0,283239,863.0477240085602,8.218384883031475e-07
71071,283639,0,283639,864.5447962284088,8.123209272154853e-07
71171,284039,0,284039,866.1464612483978,8.029165958653523e-07
71271,284439,0,284439,867.525475025177,7.936242012795865e-07
71371,284839,0,284839,868.6835091114044,7.84454986341409e-07
71471,285239,0,285239,870.0586512088776,7.754000674016833e-07
71572,285643,0,285643,871.2820842266083,7.663821814855323e-07
71672,286043,0,286043,872.5120582580566,7.575649461618619e-07
71772,286443,0,286443,873.7398200035095,7.488728451730774e-07
71872,286843,0,286843,875.0853471755981,7.40303613269805e-07
71972,287243,0,287243,876.5599811077118,7.31869071489858e-07
72072,287643,0,287643,877.7067613601685,7.235787411459034e-07
72172,288043,0,288043,878.8241751194,7.154153025248268e-07
72272,288443,0,288443,879.9004542827606,7.073797434443381e-07
72372,288843,0,288843,881.0113611221313,6.994405857970477e-07
72472,289243,0,289243,882.0724651813507,6.91596409795027e-07
72573,289647,0,289647,883.2885921001434,6.837521241815563e-07
72673,290047,0,290047,884.7426149845123,6.76063614227455e-07
72773,290447,0,290447,885.9948070049286,6.684365460551952e-07
72873,290847,0,290847,887.1287441253662,6.608606357052393e-07
72973,291247,0,291247,888.4719820022583,6.533201527392151e-07
73073,291647,0,291647,889.6597559452057,6.458129668715352e-07
73173,292047,0,292047,890.8027250766754,6.383510968567983e-07
73273,292447,0,292447,892.1578443050385,6.309498024153505e-07
73373,292847,0,292847,893.4214472770691,6.236311401905401e-07
73473,293247,0,293247,894.4731872081757,6.164007865978117e-07
73574,293651,0,293651,895.5479040145874,6.09187964875479e-07
73674,294051,0,294051,896.8453812599182,6.021311735914442e-07
73774,294451,0,294451,897.9569911956787,5.951524542427206e-07
73874,294851,0,294851,899.3481891155243,5.88257375420663e-07
73974,295251,0,295251,900.7169382572174,5.814451520660815e-07
74074,295651,0,295651,901.9344160556793,5.747191750822218e-07
74174,296051,0,296051,902.990195274353,5.680764583261537e-07
74274,296451,0,296451,904.2461459636688,5.615087542563483e-07
74374,296851,0,296851,905.4452481269836,5.550197064147841e-07
74474,297251,0,297251,906.6694593429565,5.48611636532368e-07
74575,297655,0,297655,907.8476431369781,5.422367302184988e-07
74675,298055,0,298055,909.0447070598602,5.360308924718053e-07
74775,298455,0,298455,910.2183620929718,5.299344190555424e-07
74875,298855,0,298855,911.2995183467865,5.23939895091956e-07
74975,299255,0,299255,912.4112451076508,5.180314380096783e-07
75075,299655,0,299655,913.4860689640045,5.121924579850823e-07
75175,300055,0,300055,914.8848240375519,5.064118452941054e-07
75275,300455,0,300455,916.0268442630768,5.006896168826657e-07
75375,300855,0,300855,917.0905940532684,4.950239922248364e-07
75475,301255,0,301255,918.136744260788,4.894208573032311e-07
75576,301659,0,301659,919.264083147049,4.838201304410442e-07
75676,302059,0,302059,920.3298633098602,4.783333177991947e-07
75776,302459,0,302459,921.3424220085144,4.728986537459399e-07
75876,302859,0,302859,922.3772192001343,4.675228480748712e-07
75976,303259,0,303259,923.3843071460724,4.6220236043669274e-07
76076,303659,0,303659,924.3918220996857,4.56942263802604e-07
76176,304059,0,304059,925.3893821239471,4.5173454659227366e-07
76276,304459,0,304459,926.3973910808563,4.465713470526085e-07
76376,304859,0,304859,927.3936371803284,4.4145151777678366e-07
76476,305259,0,305259,928.4042851924896,4.3637294947482686e-07
76577,305663,0,305663,929.409585237503,4.3129788306002076e-07
76677,306063,0,306063,930.4236512184143,4.2633601200510203e-07
76777,306463,0,306463,931.4365103244781,4.2144866600397913e-07
76877,306863,0,306863,932.4453852176666,4.166373875156341e-07
76977,307263,0,307263,933.4628882408142,4.119053954311408e-07
77077,307663,0,307663,934.5746963024139,4.072453579507207e-07
77177,308063,0,308063,936.0996351242065,4.026567022653564e-07
77277,308463,0,308463,937.7437093257904,3.9813683556749264e-07
77377,308863,0,308863,938.8904850482941,3.936821479100894e-07
77477,309263,0,309263,939.9566671848297,3.8929141694876395e-07
77578,309667,0,309667,940.9691932201385,3.849181033926139e-07
77678,310067,0,310067,942.0533401966095,3.806434913733557e-07
77778,310467,0,310467,943.1178741455078,3.764251248863545e-07
77878,310867,0,310867,944.1489191055298,3.7225677148854326e-07
77978,311267,0,311267,945.3985750675201,3.681427430983257e-07
78078,311667,0,311667,946.6487441062927,3.6407689873230597e-07
78178,312067,0,312067,947.7825500965118,3.600605246330963e-07
78278,312467,0,312467,948.9133801460266,3.560850307839211e-07
78378,312867,0,312867,950.0206341743469,3.5214890799133697e-07
78478,313267,0,313267,951.1887900829315,3.482481584211923e-07
78579,313671,0,313671,952.3502221107483,3.4434168574921477e-07
78679,314071,0,314071,953.6887972354889,3.4050992210492806e-07
78779,314471,0,314471,955.1924362182617,3.3671034773279705e-07
78879,314871,0,314871,956.8400461673737,3.3294519206690856e-07
78979,315271,0,315271,957.9179210662842,3.292108782800375e-07
79079,315671,0,315671,959.1221830844879,3.2550911060341167e-07
79179,316071,0,316071,960.2934482097626,3.218395227398407e-07
79279,316471,0,316471,961.3661522865295,3.1820662474047363e-07
79379,316871,0,316871,962.3666622638702,3.1461431271844557e-07
79479,317271,0,317271,963.3950293064117,3.1106163730826524e-07
79580,317675,0,317675,964.5986909866333,3.0752429550424507e-07
79680,318075,0,318075,966.1613349914551,3.040672379606385e-07
79780,318475,0,318475,967.7474451065063,3.0066529580455973e-07
79880,318875,0,318875,969.2014091014862,2.973142055404846e-07
79980,319275,0,319275,970.7110960483551,2.9401600084151916e-07
80080,319675,0,319675,971.8899283409119,2.9076673490048286e-07
80180,320075,0,320075,972.9514880180359,2.875612438718773e-07
80280,320475,0,320475,974.9245312213898,2.8439378976916807e-07
80380,320875,0,320875,977.3543212413788,2.812588848199686e-07
80480,321275,0,321275,980.0509810447693,2.781559329971361e-07
80581,321679,0,321679,982.0676741600037,2.7504706398147847e-07
80681,322079,0,322079,983.5015389919281,2.71999773485749e-07
80781,322479,0,322479,985.3971531391144,2.689769071097198e-07
80881,322879,0,322879,988.3764650821686,2.6598275593857814e-07
80981,323279,0,323279,989.6701080799103,2.6301675240739e-07
81081,323679,0,323679,991.2975442409515,2.600799408329081e-07
81181,324079,0,324079,993.1775691509247,2.571725825193734e-07
81281,324479,0,324479,995.2193410396576,2.5429492924187986e-07
81381,324879,0,324879,996.4848623275757,2.51446044277539e-07
81481,325279,0,325279,997.5870652198792,2.486218261936775e-07
81582,325683,0,325683,998.7318289279938,2.4579569633958043e-07
81682,326083,0,326083,999.8632659912109,2.430193904617974e-07
81782,326483,0,326483,1001.394195318222,2.4026697880435034e-07
81882,326883,0,326883,1002.6235539913177,2.3753980555745512e-07
81982,327283,0,327283,1003.8423261642456,2.3483703164491856e-07
82082,327683,0,327683,1005.1575553417206,2.3216298191340907e-07
82182,328083,0,328083,1006.3331582546234,2.2951926401383224e-07
82282,328483,0,328483,1007.4084672927856,2.269087968593467e-07
82382,328883,0,328883,1008.6117062568665,2.2433209792170738e-07
82482,329283,0,329283,1010.1392540931702,2.2179468603730744e-07
82583,329687,0,329687,1011.2276751995087,2.1926664651152742e-07
82683,330087,0,330087,1012.7358913421631,2.1680084153062058e-07
82783,330487,0,330487,1013.8506863117218,2.1436801665210095e-07
82883,330887,0,330887,1015.1302771568298,2.119662457054118e-07
82983,331287,0,331287,1016.5265882015228,2.0959815876851192e-07
83083,331687,0,331687,1018.1083650588989,2.0726120171785138e-07
83183,332087,0,332087,1019.9863741397858,2.0495843331358286e-07
83283,332487,0,332487,1021.4649641513824,2.026877893109564e-07
83383,332887,0,332887,1022.6689400672913,2.0045176143843585e-07
83483,333287,0,333287,1023.9901113510132,1.982443994630695e-07
83584,333691,0,333691,1025.205542087555,1.9604628638782837e-07
83684,334091,0,334091,1026.5016911029816,1.9389606439804818e-07
83784,334491,0,334491,1027.9447782039642,1.9176870427346846e-07
83884,334891,0,334891,1029.1786050796509,1.8966417403643064e-07
83984,335291,0,335291,1030.8003282546997,1.8757449454631704e-07
84084,335691,0,335691,1031.9380910396576,1.8550118310140662e-07
84184,336091,0,336091,1033.0166010856628,1.8344146101589218e-07
84284,336491,0,336491,1034.3357932567596,1.81398277875427e-07
84384,336891,0,336891,1035.4633440971375,1.7937110694401527e-07
84484,337291,0,337291,1036.5045862197876,1.7736662695707541e-07
84585,337695,0,337695,1037.5681290626526,1.7536400398700696e-07
84685,338095,0,338095,1038.6069691181183,1.7340465970212296e-07
84785,338495,0,338495,1039.6131031513214,1.7146955118389847e-07
84885,338895,0,338895,1040.6616671085358,1.6955452625618653e-07
84985,339295,0,339295,1041.6590151786804,1.6766379965195107e-07
85085,339695,0,339695,1043.002869129181,1.6579624741978435e-07
85185,340095,0,340095,1044.4244811534882,1.6395272018562886e-07
85285,340495,0,340495,1046.1672821044922,1.6213430741596268e-07
85385,340895,0,340895,1048.534559249878,1.603423493146407e-07
85485,341295,0,341295,1050.0151982307434,1.5857443262925334e-07
85586,341699,0,341699,1051.1447081565857,1.5681517234473405e-07
85686,342099,0,342099,1052.274167060852,1.5509986516961643e-07
85786,342499,0,342499,1053.4609920978546,1.534089002977632e-07
85886,342899,0,342899,1054.474314212799,1.5174556034614455e-07
85986,343299,0,343299,1055.7289361953735,1.5010475247312503e-07
86086,343699,0,343699,1057.9921810626984,1.4848430850428215e-07
86186,344099,0,344099,1060.2575380802155,1.4688344504131224e-07
86286,344499,0,344499,1062.8989062309265,1.4529864449529885e-07
86386,344899,0,344899,1064.1817650794983,1.4372807903555653e-07
86486,345299,0,345299,1065.7103242874146,1.4217254855254989e-07
86587,345703,0,345703,1067.0061461925507,1.4061428989036337e-07
86687,346103,0,346103,1068.5022420883179,1.3908225498039293e-07
86787,346503,0,346503,1070.105339050293,1.3756139940271955e-07
86887,346903,0,346903,1071.1293580532074,1.3604743285176824e-07
86987,347303,0,347303,1072.156372308731,1.3454252422643153e-07
87087,347703,0,347703,1073.3452022075653,1.3304926794014083e-07
87187,348103,0,348103,1074.3824472427368,1.3156623749083803e-07
87287,348503,0,348503,1075.4003932476044,1.3009773316822023e-07
87387,348903,0,348903,1076.4065861701965,1.286464938143749e-07
87487,349303,0,349303,1077.437441110611,1.2721104614696963e-07
87588,349707,0,349707,1078.4747912883759,1.2577966178835254e-07
87688,350107,0,350107,1079.4963171482086,1.2438094387859732e-07
87788,350507,0,350507,1080.5023410320282,1.229991935762216e-07
87888,350907,0,350907,1081.5497682094574,1.2163643110099446e-07
87988,351307,0,351307,1082.6328670978546,1.2029139293048514e-07
88088,351707,0,351707,1083.8623220920563,1.1896061635752625e-07
88188,352107,0,352107,1084.8975591659546,1.1764813733733752e-07
88288,352507,0,352507,1085.9750430583954,1.1635133451015061e-07
88388,352907,0,352907,1087.1409599781036,1.1506990649353804e-07
88488,353307,0,353307,1088.2605140209198,1.13806669551508e-07
88589,353711,0,353711,1089.3632380962372,1.1254841742980241e-07
88689,354111,0,354111,1090.4624450206757,1.1131851544271273e-07
88789,354511,0,354511,1091.5379860401154,1.101063177997413e-07
88889,354911,0,354911,1092.62313914299,1.0890621649539111e-07
88989,355311,0,355311,1093.7232131958008,1.0771832314092281e-07
89089,355711,0,355711,1094.8296341896057,1.0654335374651037e-07
89189,356111,0,356111,1096.1392612457275,1.053759700281656e-07
89289,356511,0,356511,1097.2922360897064,1.0421716900829841e-07
89389,356911,0,356911,1098.3739030361176,1.0306856991339264e-07
89489,357311,0,357311,1099.5771770477295,1.0192665470982408e-07
89590,357715,0,357715,1101.0182111263275,1.0078184585451295e-07
89690,358115,0,358115,1102.718159198761,9.965863869115317e-08
89790,358515,0,358515,1104.093513250351,9.854282207238429e-08
89890,358915,0,358915,1105.4410872459412,9.743925169987752e-08
89990,359315,0,359315,1106.5551590919495,9.63467050150379e-08
90090,359715,0,359715,1107.7799799442291,9.526257018720066e-08
90190,360115,0,360115,1108.785926103592,9.419193935644718e-08
90290,360515,0,360515,1109.8138873577118,9.313354786771865e-08
90390,360915,0,360915,1110.8434171676636,9.208467522870625e-08
90490,361315,0,361315,1111.88347530365,9.10512516981325e-08
90591,361719,0,361719,1112.9739980697632,9.002063463121937e-08
90691,362119,0,362119,1114.0708799362183,8.901403308725061e-08
90791,362519,0,362519,1115.128065109253,8.802473281360776e-08
90891,362919,0,362919,1116.166395187378,8.704841692783936e-08
90991,363319,0,363319,1117.1768102645874,8.608767001960605e-08
91091,363719,0,363719,1118.1964461803436,8.514478683632309e-08
91191,364119,0,364119,1119.2165212631226,8.421453346511235e-08
91291,364519,0,364519,1120.2221901416779,8.32975128501969e-08
91391,364919,0,364919,1121.2344102859497,8.239677103729871e-08
91491,365319,0,365319,1122.2495033740997,8.150406982451709e-08
91592,365723,0,365723,1123.7854890823364,8.061479824915943e-08
91692,366123,0,366123,1124.9350662231445,7.974387422840997e-08
91792,366523,0,366523,1126.3274581432343,7.887948789447006e-08
91892,366923,0,366923,1127.3863141536713,7.802711139763855e-08
91992,367323,0,367323,1128.514074087143,7.718147819396633e-08
92092,367723,0,367723,1129.5837752819061,7.634159550578226e-08
92192,368123,0,368123,1130.6263892650604,7.551134497436577e-08
92292,368523,0,368523,1131.6822383403778,7.468767356755495e-08
92392,368923,0,368923,1132.8006372451782,7.387189050439875e-08
92492,369323,0,369323,1133.9880361557007,7.306421831716721e-08
92593,369727,0,369727,1135.0615921020508,7.225596467286293e-08
92693,370127,0,370127,1136.1750662326813,7.14622812174851e-08
92793,370527,0,370527,1137.2107751369476,7.06759930821609e-08
92893,370927,0,370927,1138.326689004898,6.989677117076018e-08
92993,371327,0,371327,1139.4300472736359,6.912612654031898e-08
93093,371727,0,371727,1140.6457750797272,6.836331134107448e-08
93193,372127,0,372127,1141.8034522533417,6.761064901178e-08
93293,372527,0,372527,1142.8753521442413,6.68670578513105e-08
93393,372927,0,372927,1143.9127690792084,6.613454563806163e-08
93493,373327,0,373327,1144.9707782268524,6.541222325576293e-08
93594,373731,0,373731,1146.0220091342926,6.46940292654225e-08
93694,374131,0,374131,1147.1108300685883,6.39936951211201e-08
93794,374531,0,374531,1148.1831641197205,6.330341616316238e-08
93894,374931,0,374931,1149.2012090682983,6.262325789121572e-08
93994,375331,0,375331,1150.2771520614624,6.195165795092965e-08
94094,375731,0,375731,1151.2844462394714,6.12889114372425e-08
94194,376131,0,376131,1152.2869460582733,6.063332235305462e-08
94294,376531,0,376531,1153.309261083603,5.9984956998014e-08
94394,376931,0,376931,1154.3012590408325,5.934233531774784e-08
94494,377331,0,377331,1155.3132452964783,5.870491644438914e-08
94595,377735,0,377735,1156.320237159729,5.80657044164055e-08
94695,378135,0,378135,1157.3337421417236,5.743674085479315e-08
94795,378535,0,378535,1158.3331441879272,5.6812004998798084e-08
94895,378935,0,378935,1159.349106311798,5.6191289592457075e-08
94995,379335,0,379335,1160.3232700824738,5.557543491370609e-08
95095,379735,0,379735,1161.3079252243042,5.496442636523241e-08
95195,380135,0,380135,1162.2878692150116,5.435870121136235e-08
95295,380535,0,380535,1163.2618160247803,5.375852331662496e-08
95395,380935,0,380935,1164.24946808815,5.316373849877799e-08
95495,381335,0,381335,1165.23513007164,5.2574931379234836e-08
95596,381739,0,381739,1166.2439930438995,5.1985933236070685e-08
95696,382139,0,382139,1167.22824716568,5.140887452552616e-08
95796,382539,0,382539,1168.2298302650452,5.083780943217572e-08
95896,382939,0,382939,1169.1600761413574,5.027314531429729e-08
95996,383339,0,383339,1169.8720932006836,4.971497222426046e-08
96096,383739,0,383739,1171.0124940872192,4.9164000644309835e-08
96196,384139,0,384139,1171.7770371437073,4.862067011163972e-08
96296,384539,0,384539,1172.5745720863342,4.80850914426928e-08
96396,384939,0,384939,1173.7295711040497,4.755767303250286e-08
96496,385339,0,385339,1174.8598430156708,4.703757639862222e-08
96597,385743,0,385743,1175.966480255127,4.651979405712348e-08
96697,386143,0,386143,1176.7894961833954,4.601303013606069e-08
96797,386543,0,386543,1177.5492541790009,4.551266894616704e-08
96897,386943,0,386943,1178.3781323432922,4.5017193642435716e-08
96997,387343,0,387343,1179.352536201477,4.452738903731044e-08
97097,387743,0,387743,1180.275621175766,4.4042361795700234e-08
97197,388143,0,388143,1181.02214717865,4.356238542056959e-08
97297,388543,0,388543,1181.7586982250214,4.308732859046706e-08
97397,388943,0,388943,1182.6723272800446,4.2616768134765095e-08
97497,389343,0,389343,1183.4478282928467,4.215118823121505e-08
97598,389747,0,389747,1184.644632101059,4.1685124613830125e-08
97698,390147,0,390147,1185.362755060196,4.1228433487632625e-08
97798,390547,0,390547,1186.058223247528,4.077539389436083e-08
97898,390947,0,390947,1186.8260741233826,4.032631789071949e-08
97998,391347,0,391347,1187.5545053482056,3.988070972476413e-08
98098,391747,0,391747,1188.2228801250458,3.943868396650517e-08
98198,392147,0,392147,1188.8985600471497,3.9000731195867856e-08
98298,392547,0,392547,1189.647919178009,3.856680814685892e-08
98398,392947,0,392947,1190.3186831474304,3.8138081893172694e-08
98498,393347,0,393347,1190.9794092178345,3.7714119863253e-08
98599,393751,0,393751,1191.686457157135,3.729179949919601e-08
98699,394151,0,394151,1192.3494062423706,3.687899354533666e-08
98799,394551,0,394551,1193.0217730998993,3.64720343999125e-08
98899,394951,0,394951,1193.7159841060638,3.607072189358274e-08
98999,395351,0,395351,1194.3831901550293,3.5675037623247156e-08
99099,395751,0,395751,1195.0449483394623,3.528507681533561e-08
99199,396151,0,396151,1195.72380900383,3.49004885007863e-08
99299,396551,0,396551,1196.4018700122833,3.452136691670143e-08
99399,396951,0,396951,1197.2123210430145,3.414743518920771e-08
99499,397351,0,397351,1198.0194561481476,3.377871398734246e-08
99600,397755,0,397755,1198.7835252285004,3.341149102622366e-08
99700,398155,0,398155,1199.5125889778137,3.3052810473139837e-08
99800,398555,0,398555,1200.3517112731934,3.269894022201112e-08
99900,398955,0,398955,1201.065805196762,3.234938905480299e-08
100000,399355,0,399355,1201.8951790332794,3.2003996086682737e-08


==> plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-aaii.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0007729530334472656,30.358106049564984
100,252,0,252,0.7068758010864258,0.2584702496066637
200,504,0,504,1.379183053970337,0.10025228889566092
300,757,0,757,2.0684399604797363,0.05354232784000942
400,1007,0,1007,2.7371439933776855,0.04118183074080015
501,1259,0,1259,3.395610809326172,0.03212008761769572
601,1511,0,1511,4.045492887496948,0.026550400741840233
701,1761,0,1761,4.715965032577515,0.022253473456958668
801,2013,0,2013,5.367310047149658,0.017617868455366646
901,2262,0,2262,6.01697301864624,0.014662611161370801
1001,2512,0,2512,6.672208786010742,0.011962667368031256
1101,2760,0,2760,7.313669919967651,0.009501045770622368
1201,3013,0,3013,7.967495918273926,0.007629167055048466
1301,3263,0,3263,8.737348794937134,0.0060928937607256884
1401,3513,0,3513,9.461069107055664,0.005125194375011903
1502,3764,0,3764,10.340143918991089,0.0043152279799267045
1602,4003,0,4003,11.070133924484253,0.0038042693624838367
1702,4249,0,4249,11.953434944152832,0.003289468275864946
1802,4498,0,4498,12.598495960235596,0.0027370060050925966
1902,4742,0,4742,13.230838060379028,0.0024009989456067883
2002,4970,0,4970,13.843727111816406,0.0022620802558184962
2102,5220,0,5220,14.467022180557251,0.001993849435343263
2202,5468,0,5468,15.116336822509766,0.0017790620894565959
2302,5694,0,5694,15.739657878875732,0.001686982584417212
2402,5921,0,5921,16.355583906173706,0.0016136342708067159
2503,6141,0,6141,16.98948097229004,0.001568348894393168
2603,6353,0,6353,17.605875968933105,0.0015383013425077706
2703,6569,0,6569,18.21681308746338,0.0014969245093177557
2803,6778,0,6778,18.826438903808594,0.0014692927979711983
2903,6978,0,6978,19.452043056488037,0.001455371015657392
3003,7178,0,7178,20.071763038635254,0.0014414202912371972
3103,7378,0,7378,20.69378399848938,0.0014291242240314893
3203,7578,0,7578,21.33190894126892,0.0014173919844090417
3303,7778,0,7778,21.9515221118927,0.0014059351458918633
3403,7982,0,7982,22.565647840499878,0.0013896522951835479
3504,8204,0,8204,23.191898107528687,0.0013468770142071734
3604,8424,0,8424,23.808932065963745,0.001309703265807277
3704,8627,0,8627,24.419151782989502,0.0012950370323156109
3804,8827,0,8827,25.123759031295776,0.0012839912619955068
3904,9027,0,9027,25.743422985076904,0.0012736515872593822
4004,9227,0,9227,26.345382928848267,0.001263644071159475
4104,9427,0,9427,27.023279190063477,0.0012538186059952879
4204,9627,0,9627,27.67383599281311,0.0012440576751176337
4304,9827,0,9827,28.302362203598022,0.0012344217955391433
4404,10027,0,10027,28.927103996276855,0.0012248451385586648
4505,10229,0,10229,29.636065006256104,0.001215275785555544
4605,10429,0,10429,30.24572992324829,0.0012058541351347418
4705,10629,0,10629,30.847866773605347,0.0011965243775971769
4805,10829,0,10829,31.444740772247314,0.001187239629111943
4905,11029,0,11029,32.08491492271423,0.0011780640177723562
5005,11229,0,11229,32.70137095451355,0.0011689179926348255
5105,11429,0,11429,33.402997970581055,0.0011598643366503097
5205,11629,0,11629,34.11725378036499,0.0011508732958342587
5305,11829,0,11829,34.7608699798584,0.0011419386771410434
5405,12029,0,12029,35.388041973114014,0.0011330806723231933
5506,12231,0,12231,36.04432415962219,0.0011241863769342836
5606,12431,0,12431,36.71251893043518,0.0011154487440146873
5706,12631,0,12631,37.392329931259155,0.0011067594856848282
5806,12831,0,12831,38.04498314857483,0.001098148373770333
5906,13031,0,13031,38.713518142700195,0.0010895849939988825
6006,13231,0,13231,39.416255950927734,0.0010811070554585178
6106,13431,0,13431,40.02256679534912,0.0010726725806420659
6206,13631,0,13631,40.651983976364136,0.0010643270736202508
6306,13831,0,13831,41.260719776153564,0.0010560548511251823
6406,14031,0,14031,41.85399913787842,0.0010478504535294789
6507,14233,0,14233,42.456090211868286,0.0010396539829893715
6607,14433,0,14433,43.06252908706665,0.0010316157105679075
6707,14633,0,14633,43.66241788864136,0.0010236619342892095
6807,14833,0,14833,44.25987887382507,0.001015788713083205
6907,15033,0,15033,44.86520981788635,0.00100800942591253
7007,15233,0,15233,45.46085000038147,0.0010002993147332677
7107,15433,0,15433,46.065337896347046,0.0009926842602501259
7207,15633,0,15633,46.67070198059082,0.000985136917510493
7307,15833,0,15833,47.28620481491089,0.000977677415512971
7407,16033,0,16033,47.888723850250244,0.0009703001268882239
7508,16235,0,16235,48.49437499046326,0.0009629107201948288
7608,16435,0,16435,49.11427092552185,0.0009556840689592388
7708,16635,0,16635,49.71981501579285,0.0009485176226957701
7808,16835,0,16835,50.322710037231445,0.0009414199962282755
7908,17035,0,17035,50.922971963882446,0.0009343843112065706
8008,17235,0,17235,51.60275197029114,0.0009274205350711474
8108,17435,0,17435,52.29482293128967,0.0009204924942285719
8208,17635,0,17635,52.92790985107422,0.0009136286913271874
8308,17835,0,17835,53.54347109794617,0.0009068068343480386
8408,18035,0,18035,54.163559913635254,0.0009000270090566092
8509,18237,0,18237,54.77231001853943,0.0008932266933670874
8609,18437,0,18437,55.382158041000366,0.000886526134108414
8709,18637,0,18637,55.991092920303345,0.0008798703917080213
8809,18837,0,18837,56.60236191749573,0.0008732388405790019
8909,19037,0,19037,57.206937074661255,0.0008666458561685062
9009,19237,0,19237,57.81745886802673,0.0008600793249633281
9109,19437,0,19437,58.43125891685486,0.0008535567535819349
9209,19637,0,19637,59.035927057266235,0.0008470499035956939
9309,19837,0,19837,59.6563560962677,0.0008405847965517346
9409,20037,0,20037,60.292248010635376,0.0008341569660013585
9510,20239,0,20239,60.92379283905029,0.0008276910640619939
9610,20439,0,20439,61.55014705657959,0.0008213421525889225
9710,20639,0,20639,62.31665515899658,0.0008150230559175037
9810,20839,0,20839,62.911009073257446,0.0008087508388999406
9910,21039,0,21039,63.513838052749634,0.0008025177898582031
10010,21239,0,21239,64.13097286224365,0.0007963358147768895
10110,21439,0,21439,64.72679400444031,0.0007901961507791906
10210,21639,0,21639,65.32241296768188,0.0007841150761982164
10310,21839,0,21839,65.91669201850891,0.0007780758068359257
10410,22039,0,22039,66.52472400665283,0.0007720959792644743
10511,22241,0,22241,67.17713212966919,0.0007661133807162037
10611,22441,0,22441,67.78945517539978,0.0007602381962508519
10711,22641,0,22641,68.48090076446533,0.0007544339932959039
10811,22841,0,22841,69.11091899871826,0.0007486817152696908
10911,23041,0,23041,69.73817896842957,0.0007429864672240095
11011,23241,0,23241,70.42927098274231,0.0007373467912476561
11111,23441,0,23441,71.06552910804749,0.0007317670519517288
11211,23641,0,23641,71.68601393699646,0.0007262271186072409
11311,23841,0,23841,72.29236507415771,0.0007207458053562501
11411,24041,0,24041,72.92595195770264,0.0007153041910518533
11512,24243,0,24243,73.53457403182983,0.0007098528903494391
11612,24443,0,24443,74.16267585754395,0.0007045043948059424
11712,24643,0,24643,74.78318214416504,0.0006991866902834604
11812,24843,0,24843,75.46767592430115,0.0006939131820039643
11912,25043,0,25043,76.08375287055969,0.0006886686979943295
12012,25243,0,25243,76.69523692131042,0.0006834596379482868
12112,25443,0,25443,77.32318997383118,0.0006782810810842254
12212,25643,0,25643,78.02672100067139,0.000673140277194275
12312,25843,0,25843,78.77969694137573,0.0006680172446606728
12412,26043,0,26043,79.38611793518066,0.000662933542348563
12513,26245,0,26245,79.99329781532288,0.0006578274647383251
12613,26445,0,26445,80.62433791160583,0.000652794812909588
12713,26645,0,26645,81.32913303375244,0.0006478020725564155
12813,26845,0,26845,82.02087187767029,0.0006428315891682619
12913,27045,0,27045,82.64428114891052,0.0006378926848420316
13013,27245,0,27245,83.23762512207031,0.0006329784244122047
13113,27445,0,27445,83.8675229549408,0.0006280947899234017
13213,27645,0,27645,84.46443295478821,0.0006232334516178511
13313,27845,0,27845,85.07261896133423,0.0006184054021369296
13413,28045,0,28045,85.69485807418823,0.0006135939992542019
13514,28247,0,28247,86.30983996391296,0.0006087694716298938
13614,28447,0,28447,86.92777490615845,0.0006040247923667176
13714,28647,0,28647,87.54356002807617,0.0005993051498557232
13814,28847,0,28847,88.17477989196777,0.0005946281900220586
13914,29047,0,29047,88.80349683761597,0.0005899840208390282
14014,29247,0,29247,89.41207098960876,0.000585378590315593
14114,29447,0,29447,90.02428913116455,0.0005808136705156818
14214,29647,0,29647,90.63132500648499,0.0005762942964938985
14314,29847,0,29847,91.3162739276886,0.0005718093606579084
14414,30047,0,30047,92.07652187347412,0.0005673766887800034
14515,30249,0,30249,92.73198795318604,0.00056293813812618
14615,30449,0,30449,93.40262389183044,0.0005585868011223772
14715,30649,0,30649,94.00507497787476,0.0005542857290798216
14815,30849,0,30849,94.6109938621521,0.000550023656887512
14915,31049,0,31049,95.27486681938171,0.0005458078546689329
15015,31249,0,31249,95.9251799583435,0.0005416327920443533
15115,31449,0,31449,96.57166314125061,0.0005375001520164296
15215,31649,0,31649,97.1998028755188,0.0005334065235919501
15315,31849,0,31849,97.79765820503235,0.0005293572486470912
15415,32049,0,32049,98.41478300094604,0.0005253385886448999
15516,32251,0,32251,99.02612209320068,0.0005213237067526812
15616,32451,0,32451,99.63762593269348,0.0005173861963796446
15716,32651,0,32651,100.24147510528564,0.0005134822703219745
15816,32851,0,32851,100.85399985313416,0.0005096197051733007
15916,33051,0,33051,101.46249198913574,0.0005057893169031855
16016,33251,0,33251,102.08565616607666,0.0005019918295248721
16116,33451,0,33451,102.71265888214111,0.0004982251305301748
16216,33651,0,33651,103.32244896888733,0.0004944885121008328
16316,33851,0,33851,103.92506384849548,0.0004907738364088092
16416,34051,0,34051,104.5291359424591,0.0004870877120369311
16517,34253,0,34253,105.15603685379028,0.0004833804984239596
16617,34453,0,34453,105.76220202445984,0.0004797330493777302
16717,34653,0,34653,106.38558197021484,0.00047610690183506405
16817,34853,0,34853,107.0181450843811,0.00047249765018663955
16917,35053,0,35053,107.63880181312561,0.00046891116119504323
17017,35253,0,35253,108.25740599632263,0.0004653437519083225
17117,35453,0,35453,108.8708701133728,0.0004617962528859499
17217,35653,0,35653,109.49806594848633,0.0004582701824303153
17317,35853,0,35853,110.10927200317383,0.0004547687604330165
17417,36053,0,36053,110.71548795700073,0.00045128437346690533
17518,36255,0,36255,111.32962989807129,0.0004477930877810582
17618,36455,0,36455,111.92428708076477,0.0004443591892495973
17718,36655,0,36655,112.51942491531372,0.0004409497955571983
17818,36855,0,36855,113.1193459033966,0.00043757055722700626
17918,37055,0,37055,113.72715997695923,0.0004342176166511042
18018,37255,0,37255,114.32560300827026,0.0004308949137895955
18118,37455,0,37455,114.93120408058167,0.00042760332710377433
18218,37655,0,37655,115.53678894042969,0.00042434238597930545
18318,37855,0,37855,116.15500116348267,0.00042111320081761756
18418,38055,0,38055,116.75652003288269,0.00041791849634199103
18519,38257,0,38257,117.36364793777466,0.0004147187089950228
18619,38457,0,38457,117.97554397583008,0.00041158695939104884
18719,38657,0,38657,118.5896828174591,0.00040848647394878436
18819,38857,0,38857,119.19590187072754,0.0004054158580496927
18919,39057,0,39057,119.81007409095764,0.00040237907853972726
19019,39257,0,39257,120.41503691673279,0.0003993730556905505
19119,39457,0,39457,121.01978802680969,0.00039639367435427065
19219,39657,0,39657,121.63254976272583,0.0003934434677054196
19319,39857,0,39857,122.25486993789673,0.000390520311579414
19419,40057,0,40057,123.06004595756531,0.0003876191080762832
19520,40259,0,40259,124.00348687171936,0.00038471360769292426
19620,40459,0,40459,125.04608678817749,0.00038185600423155724
19720,40659,0,40659,125.7197630405426,0.0003790185753043543
19820,40859,0,40859,126.36906003952026,0.0003761996412252371
19920,41059,0,41059,127.01756119728088,0.00037339614998068137
20020,41259,0,41259,127.63852381706238,0.0003706095186496348
20120,41459,0,41459,128.44525694847107,0.00036783803027635596
20220,41659,0,41659,129.08334493637085,0.0003650780506977404
20320,41859,0,41859,129.73592400550842,0.00036233235838273846
20420,42059,0,42059,130.82493495941162,0.0003595999505905372
20521,42261,0,42261,131.6005699634552,0.00035684891179602193
20621,42461,0,42461,132.5287380218506,0.00035413872752315277
20721,42661,0,42661,133.20463490486145,0.0003514401796663164
20821,42861,0,42861,133.88311386108398,0.0003487530584537215
20921,43061,0,43061,134.52379488945007,0.000346081288205072
21021,43261,0,43261,135.18935203552246,0.00034342336890239445
21121,43461,0,43461,135.89525699615479,0.00034077988080391633
21221,43661,0,43661,136.65432691574097,0.0003381552792047508
21321,43861,0,43861,137.36546206474304,0.0003355467871620267
21421,44061,0,44061,138.07551217079163,0.0003329575301029765
21522,44263,0,44263,138.70357704162598,0.0003303631338765218
21622,44463,0,44463,139.35773015022278,0.00032781345143755296
21722,44663,0,44663,139.9798698425293,0.00032528533403602115
21822,44863,0,44863,140.7370171546936,0.0003227793365833121
21922,45063,0,45063,141.43171310424805,0.0003202933986150201
22022,45263,0,45263,142.08801198005676,0.000317831510223095
22122,45463,0,45463,142.7682821750641,0.00031539237131079754
22222,45663,0,45663,143.39924502372742,0.0003129730274493356
22322,45863,0,45863,144.02545309066772,0.00031057877397405227
22422,46063,0,46063,144.72197794914246,0.0003082062989425342
22523,46265,0,46265,145.39064407348633,0.0003058305658265321
22623,46465,0,46465,146.12807703018188,0.0003035012625069254
22723,46665,0,46665,146.7635350227356,0.0003011931708341892
22823,46865,0,46865,147.68794298171997,0.00029890485815325295
22923,47065,0,47065,148.56560683250427,0.0002966392754110865
23023,47265,0,47265,149.20667695999146,0.00029439297729068104
23123,47465,0,47465,149.8996069431305,0.0002921666178834573
23223,47665,0,47665,150.5553379058838,0.0002899609204899502
23323,47865,0,47865,151.18448686599731,0.00028777152786029403
23423,48065,0,48065,151.7739119529724,0.00028560086598337047
23524,48267,0,48267,152.3808250427246,0.000283425415367278
23624,48467,0,48467,152.98989009857178,0.000281285343596098
23724,48667,0,48667,153.58051991462708,0.0002791592651166682
23824,48867,0,48867,154.1827688217163,0.0002770474455131497
23924,49067,0,49067,154.76696491241455,0.0002749457655943594
24024,49267,0,49267,155.35586786270142,0.00027285720725492697
24124,49467,0,49467,155.94023084640503,0.0002707794414598029
24224,49667,0,49667,156.54836511611938,0.0002687110015026959
24324,49867,0,49867,157.17590594291687,0.0002666549878073356
24424,50067,0,50067,157.80360388755798,0.0002646084946306814
24525,50269,0,50269,158.4638729095459,0.00026255316257905217
24625,50469,0,50469,159.09524393081665,0.00026052936999974456
24725,50669,0,50669,159.7210569381714,0.0002585174985078759
24825,50869,0,50869,160.3486888408661,0.0002565168249625047
24925,51069,0,51069,160.9927899837494,0.0002545306146038231
25025,51269,0,51269,161.66569900512695,0.00025255617540901286
25125,51469,0,51469,162.28719091415405,0.0002505970022365586
25225,51669,0,51669,162.91463804244995,0.0002486523651083687
25325,51869,0,51869,163.51620507240295,0.0002467210610026379
25425,52069,0,52069,164.22326493263245,0.00024480671153083547
25526,52271,0,52271,164.84002995491028,0.0002428889403873808
25626,52471,0,52471,165.44886994361877,0.00024100508276690637
25726,52671,0,52671,166.03661704063416,0.00023913762345952072
25826,52871,0,52871,166.62563395500183,0.00023728854733783952
25926,53071,0,53071,167.22940492630005,0.0002354548191160929
26026,53271,0,53271,167.8174810409546,0.00023364082907492137
26126,53471,0,53471,168.407870054245,0.00023184394983657023
26226,53671,0,53671,169.0115568637848,0.00023006583114829995
26326,53871,0,53871,169.62092685699463,0.00022830774893845568
26426,54071,0,54071,170.21799397468567,0.0002265672500330913
26527,54273,0,54273,170.82471919059753,0.00022483005704650977
26627,54473,0,54473,171.44301295280457,0.0002231283912994526
26727,54673,0,54673,172.0834128856659,0.0002214447442247862
26827,54873,0,54873,172.78787899017334,0.00021977843527910056
26927,55073,0,55073,173.40511107444763,0.0002181304824832683
27027,55273,0,55273,174.017569065094,0.0002164967824813005
27127,55473,0,55473,174.62448596954346,0.00021488007347808178
27227,55673,0,55673,175.2231800556183,0.00021327745909552535
27327,55873,0,55873,175.83118319511414,0.00021168733259085756
27427,56073,0,56073,176.430006980896,0.00021011134181499002
27528,56275,0,56275,177.13954091072083,0.00020853148852802478
27628,56475,0,56475,177.8225531578064,0.00020697657033605182
27728,56675,0,56675,178.44165992736816,0.00020543276352366958
27828,56875,0,56875,179.04805397987366,0.00020389906726857066
27928,57075,0,57075,179.6666579246521,0.00020237301150427867
28028,57275,0,57275,180.32892894744873,0.00020085728865357745
28128,57475,0,57475,180.98265194892883,0.00019934892810812715
28228,57675,0,57675,181.78625893592834,0.0001978494083934189
28328,57875,0,57875,182.4686357975006,0.00019635774952518771
28428,58075,0,58075,183.16277885437012,0.00019487328990784112
28529,58277,0,58277,183.69937586784363,0.00019338311135536077
28629,58477,0,58477,184.4154748916626,0.00019191532079112776
28729,58677,0,58677,185.1088740825653,0.00019045551933789047
28829,58877,0,58877,185.76232290267944,0.00018900433314244754
28929,59077,0,59077,186.46609687805176,0.00018756345769059362
29029,59277,0,59277,187.20150804519653,0.00018613002286098547
29129,59477,0,59477,187.8998510837555,0.00018470874899264813
29229,59677,0,59677,188.77955985069275,0.00018329699709438766
29329,59877,0,59877,189.4547038078308,0.00018189626234066733
29429,60077,0,60077,190.1146490573883,0.0001805079591626119
29530,60279,0,60279,190.98282194137573,0.00017911792327088473
29630,60479,0,60479,191.62425088882446,0.00017775347981368876
29730,60679,0,60679,192.2395088672638,0.0001764021671225788
29830,60879,0,60879,193.16676497459412,0.00017506414447812418
29930,61079,0,61079,193.83730506896973,0.00017373841390050366
30030,61279,0,61279,194.43358898162842,0.0001724277115588337
30130,61479,0,61479,195.04026198387146,0.000171128725403631
30230,61679,0,61679,195.9217610359192,0.0001698440874122675
30330,61879,0,61879,196.54260778427124,0.000168572193476397
30430,62079,0,62079,197.39280009269714,0.0001673121741196704
30531,62281,0,62281,198.16310501098633,0.0001660523094134607
30631,62481,0,62481,198.8099970817566,0.0001648160222200106
30731,62681,0,62681,199.5168640613556,0.00016358943784135465
30831,62881,0,62881,200.25389003753662,0.00016237289954352757
30931,63081,0,63081,201.07305097579956,0.00016116625916700667
31031,63281,0,63281,201.73207998275757,0.00015996645778294533
31131,63481,0,63481,202.53593707084656,0.00015877595923150073
31231,63681,0,63681,203.30050611495972,0.00015759139816969936
31331,63881,0,63881,204.01559400558472,0.0001564142936334903
31431,64081,0,64081,204.6910331249237,0.0001552431025456382
31532,64283,0,64283,205.38644194602966,0.00015406606266292033
31632,64483,0,64483,206.16119813919067,0.00015290577696838527
31732,64683,0,64683,206.8336479663849,0.00015175066717090682
31832,64883,0,64883,207.48850893974304,0.0001506006285510276
31932,65083,0,65083,208.1568660736084,0.00014945552988276822
32032,65283,0,65283,208.81217408180237,0.00014831700517161893
32132,65483,0,65483,209.48066782951355,0.00014718225070919924
32232,65683,0,65683,210.13635087013245,0.00014605507968210675
32332,65883,0,65883,211.01289010047913,0.00014493339219364977
32432,66083,0,66083,212.05531120300293,0.0001438178336584473
32533,66285,0,66285,212.81058502197266,0.00014269831289686962
32633,66485,0,66485,213.45252513885498,0.0001415968044264991
32733,66685,0,66685,214.10069704055786,0.0001405012898246268
32833,66885,0,66885,214.7384729385376,0.00013941327057696726
32933,67085,0,67085,215.3522801399231,0.00013833313920478258
33033,67285,0,67285,216.0153510570526,0.00013725971375036042
33133,67485,0,67485,216.64478588104248,0.00013619581661395767
33233,67685,0,67685,217.26382207870483,0.00013513927122535697
33333,67885,0,67885,217.90499210357666,0.00013409201003752486
33433,68085,0,68085,218.5293607711792,0.00013305408727889813
33534,68287,0,68287,219.17728400230408,0.0001320157740428634
33634,68487,0,68487,219.82823181152344,0.00013099710551960124
33734,68687,0,68687,220.4589581489563,0.00012998883125896088
33834,68887,0,68887,221.08950805664062,0.00012899001029243267
33934,69087,0,69087,221.70202708244324,0.00012800127891324502
34034,69287,0,69287,222.319561958313,0.0001270232414831008
34134,69487,0,69487,222.96285009384155,0.00012605360841796571
34234,69687,0,69687,223.58916878700256,0.00012509486854965992
34334,69887,0,69887,224.19584107398987,0.00012414464919178382
34434,70087,0,70087,224.82733297348022,0.00012320314742889858
34535,70289,0,70289,225.46966886520386,0.00012226112923271603
34635,70489,0,70489,226.1762239933014,0.00012133680648015636
34735,70689,0,70689,226.83656287193298,0.00012041901537431509
34835,70889,0,70889,227.51425004005432,0.00011950850479196048
34935,71089,0,71089,228.1524360179901,0.00011860512871200248
35035,71289,0,71289,228.91786694526672,0.00011770768612362751
35135,71489,0,71489,229.5420789718628,0.00011681771815507912
35235,71689,0,71689,230.23105096817017,0.00011593301479817612
35335,71889,0,71889,231.04729080200195,0.00011505544979761924
35435,72089,0,72089,231.74563097953796,0.00011418384359810981
35536,72291,0,72291,232.54534602165222,0.0001133095489306335
35636,72491,0,72491,233.21299290657043,0.00011244948311060167
35736,72691,0,72691,233.90584087371826,0.00011159541376238941
35836,72891,0,72891,234.55936694145203,0.0001107461648523344
35936,73091,0,73091,235.1596920490265,0.00010990178311003876
36036,73291,0,73291,235.84373879432678,0.0001090631414045197
36136,73491,0,73491,236.52281188964844,0.00010822854079998133
36236,73691,0,73691,237.12053084373474,0.00010739963142051337
36336,73891,0,73891,237.74765801429749,0.00010657504426321588
36436,74091,0,74091,238.374449968338,0.00010575581804849181
36537,74293,0,74293,238.96523809432983,0.00010493379840527903
36637,74493,0,74493,239.59968495368958,0.00010412550051366789
36737,74693,0,74693,240.2002251148224,0.00010332243979409745
36837,74893,0,74893,240.80988788604736,0.00010252545337754673
36937,75093,0,75093,241.39804697036743,0.00010173432290030916
37037,75293,0,75293,242.01562809944153,0.0001009493166840781
37137,75493,0,75493,242.61565494537354,0.00010017200392660194
37237,75693,0,75693,243.22374606132507,9.940053450249466e-05
37337,75893,0,75893,243.85982012748718,9.863714322880651e-05
37437,76093,0,76093,244.49518489837646,9.788101101211603e-05
37538,76295,0,76295,245.11855578422546,9.712488764820541e-05
37638,76495,0,76495,245.7154791355133,9.638388637943132e-05
37738,76695,0,76695,246.32887601852417,9.565107724430238e-05
37838,76895,0,76895,246.92242574691772,9.492526967449331e-05
37938,77095,0,77095,247.50263285636902,9.420701735260339e-05
38038,77295,0,77295,248.08391284942627,9.349657348637701e-05
38138,77495,0,77495,248.67868208885193,9.27929926563787e-05
38238,77695,0,77695,249.25940895080566,9.209739344045966e-05
38338,77895,0,77895,249.88612699508667,9.140795839302996e-05
38438,78095,0,78095,250.56012296676636,9.072596785544364e-05
38539,78297,0,78297,251.21732711791992,9.004364332352874e-05
38639,78497,0,78497,251.81299996376038,8.937434065194356e-05
38739,78697,0,78697,252.43141198158264,8.871057595504296e-05
38839,78897,0,78897,253.07039999961853,8.805266715968323e-05
38939,79097,0,79097,253.6945059299469,8.739938172311207e-05
39039,79297,0,79297,254.31948900222778,8.675059852876052e-05
39139,79497,0,79497,254.92196106910706,8.610691571864104e-05
39239,79697,0,79697,255.5321409702301,8.546657782203729e-05
39339,79897,0,79897,256.195280790329,8.483061418949398e-05
39439,80097,0,80097,256.8293960094452,8.419787432410362e-05
39540,80299,0,80299,257.47469997406006,8.356234376145117e-05
39640,80499,0,80499,258.125501871109,8.293637639645695e-05
39740,80699,0,80699,258.8050570487976,8.231374234293663e-05
39840,80899,0,80899,259.4195258617401,8.169351300950722e-05
39940,81099,0,81099,260.04206705093384,8.107650554352536e-05
40040,81299,0,81299,260.66415309906006,8.046241694219585e-05
40140,81499,0,81499,261.2646269798279,7.98510604664737e-05
40240,81699,0,81699,261.9257950782776,7.924378465520752e-05
40340,81899,0,81899,262.5607581138611,7.863918892009517e-05
40440,82099,0,82099,263.1705138683319,7.803881410523735e-05
40541,82301,0,82301,263.7903528213501,7.743649762678876e-05
40641,82501,0,82501,264.40058279037476,7.68442771565698e-05
40741,82701,0,82701,264.99062395095825,7.625654710508454e-05
40841,82901,0,82901,265.61910700798035,7.56739784998458e-05
40941,83101,0,83101,266.2294268608093,7.509581080976655e-05
41041,83301,0,83301,266.8148009777069,7.452269962300603e-05
41141,83501,0,83501,267.4017128944397,7.395508657068421e-05
41241,83701,0,83701,268.0309760570526,7.339225578271027e-05
41341,83901,0,83901,268.67869997024536,7.283539553671882e-05
41441,84101,0,84101,269.3540539741516,7.228343188734343e-05
41542,84303,0,84303,269.99715209007263,7.173144985901524e-05
41642,84503,0,84503,270.59252095222473,7.119026673264571e-05
41742,84703,0,84703,271.19855213165283,7.065427020085051e-05
41842,84903,0,84903,271.79841685295105,7.012284916203294e-05
41942,85103,0,85103,272.4300081729889,6.95964589360568e-05
42042,85303,0,85303,273.0467550754547,6.907440714732261e-05
42142,85503,0,85503,273.6844160556793,6.855638698617058e-05
42242,85703,0,85703,274.32533288002014,6.80431143177364e-05
42342,85903,0,85903,274.9689657688141,6.753313055557815e-05
42442,86103,0,86103,275.6555781364441,6.70273378896746e-05
42543,86305,0,86305,276.33174085617065,6.652000189465398e-05
42643,86505,0,86505,276.98042702674866,6.602093227357179e-05
42743,86705,0,86705,277.6614999771118,6.552520530361839e-05
42843,86905,0,86905,278.33678579330444,6.503285457849874e-05
42943,87105,0,87105,278.96060013771057,6.454311424559498e-05
43043,87305,0,87305,279.57845306396484,6.405622852978978e-05
43143,87505,0,87505,280.1980059146881,6.357231000006421e-05
43243,87705,0,87705,280.81048488616943,6.30905376468477e-05
43343,87905,0,87905,281.42666387557983,6.261183045847129e-05
43443,88105,0,88105,282.06085777282715,6.213498541749344e-05
43544,88307,0,88307,282.6765968799591,6.165612881598858e-05
43644,88507,0,88507,283.3594660758972,6.118418804801787e-05
43744,88707,0,88707,283.9830777645111,6.071441210752756e-05
43844,88907,0,88907,284.6134331226349,6.0246894393600237e-05
43944,89107,0,89107,285.24489402770996,5.978196655349359e-05
44044,89307,0,89307,285.87508511543274,5.931910077149472e-05
44144,89507,0,89507,286.51080298423767,5.885893744758608e-05
44244,89707,0,89707,287.1990110874176,5.8402172021352594e-05
44344,89907,0,89907,287.83762407302856,5.794768852772707e-05
44444,90107,0,90107,288.53836584091187,5.749721344987527e-05
44545,90309,0,90309,289.262423992157,5.7045629493327914e-05
44645,90509,0,90509,289.8851897716522,5.660194787177847e-05
44745,90709,0,90709,290.50241208076477,5.616229602226952e-05
44845,90909,0,90909,291.0987560749054,5.572664853885232e-05
44945,91109,0,91109,291.7102429866791,5.529468902648988e-05
45045,91309,0,91309,292.3205590248108,5.4866811065071414e-05
45145,91509,0,91509,292.9358232021332,5.4443009773984783e-05
45245,91709,0,91709,293.55915904045105,5.4022748027274466e-05
45345,91909,0,91909,294.15739011764526,5.360716837731729e-05
45445,92109,0,92109,294.79322600364685,5.319489721805407e-05
45546,92311,0,92311,295.43519592285156,5.278286028414498e-05
45646,92511,0,92511,296.0567879676819,5.2379017355885644e-05
45746,92711,0,92711,296.6551458835602,5.197894037279224e-05
45846,92911,0,92911,297.2536828517914,5.1582810622158925e-05
45946,93111,0,93111,297.8995678424835,5.11908045861562e-05
46046,93311,0,93311,298.51045989990234,5.080248123445317e-05
46146,93511,0,93511,299.10808801651,5.0417963484566186e-05
46246,93711,0,93711,299.7077341079712,5.00375611458384e-05
46346,93911,0,93911,300.32214307785034,4.9660322960779094e-05
46446,94111,0,94111,300.92493891716003,4.928711397785531e-05
46547,94313,0,94313,301.5496509075165,4.891326095647499e-05
46647,94513,0,94513,302.1861639022827,4.854621146598419e-05
46747,94713,0,94713,302.86983919143677,4.8182061776829455e-05
46847,94913,0,94913,303.47004103660583,4.782059564788464e-05
46947,95113,0,95113,304.0695197582245,4.746137469564154e-05
47047,95313,0,95313,304.69054889678955,4.7104603874885286e-05
47147,95513,0,95513,305.32476592063904,4.674986780861241e-05
47247,95713,0,95713,305.9562039375305,4.6396996463405836e-05
47347,95913,0,95913,306.5839729309082,4.604667994954013e-05
47447,96113,0,96113,307.2306728363037,4.569773493930747e-05
47548,96315,0,96315,307.89585518836975,4.5347664953674166e-05
47648,96515,0,96515,308.5352210998535,4.5003088292862485e-05
47748,96715,0,96715,309.1831338405609,4.466034906287146e-05
47848,96915,0,96915,309.99512100219727,4.4319712501454125e-05
47948,97115,0,97115,310.65628600120544,4.398129134801827e-05
48048,97315,0,97315,311.27326583862305,4.364476471695583e-05
48148,97515,0,97515,311.8998010158539,4.331041428687018e-05
48248,97715,0,97715,312.5549690723419,4.297856902932587e-05
48348,97915,0,97915,313.21011090278625,4.264866143459578e-05
48448,98115,0,98115,313.82904505729675,4.232188980734421e-05
48549,98317,0,98317,314.4438910484314,4.199404269397213e-05
48649,98517,0,98517,315.0822739601135,4.167231678516772e-05
48749,98717,0,98717,315.7777590751648,4.135353619686628e-05
48849,98917,0,98917,316.4194600582123,4.103765035766239e-05
48949,99117,0,99117,317.07096695899963,4.072460522226543e-05
49049,99317,0,99317,317.8059220314026,4.041472521671458e-05
49149,99517,0,99517,318.4816040992737,4.010799105812023e-05
49249,99717,0,99717,319.095666885376,3.980424415389728e-05
49349,99917,0,99917,319.7405378818512,3.950404639026843e-05
49449,100117,0,100117,320.3455801010132,3.920660413744864e-05
49550,100319,0,100319,320.94023394584656,3.890971781278493e-05
49650,100519,0,100519,321.54556488990784,3.8618810463466516e-05
49750,100719,0,100719,322.34872603416443,3.833077829905268e-05
49850,100919,0,100919,323.21276807785034,3.804564711144888e-05
49950,101119,0,101119,324.30821895599365,3.776331453170784e-05
50050,101319,0,101319,325.0324831008911,3.74833523510667e-05
50150,101519,0,101519,325.7647190093994,3.720584587137094e-05
50250,101719,0,101719,326.41942501068115,3.693062042191386e-05
50350,101919,0,101919,327.32740783691406,3.6657228163448914e-05
50450,102119,0,102119,328.15406799316406,3.638614125525189e-05
50551,102321,0,102321,328.7749660015106,3.611373987522251e-05
50651,102521,0,102521,329.3693277835846,3.5845807319357395e-05
50751,102721,0,102721,329.99326491355896,3.557933648513148e-05
50851,102921,0,102921,330.5853319168091,3.531413109097836e-05
50951,103121,0,103121,331.17602801322937,3.5050145076216006e-05
51051,103321,0,103321,331.76759099960327,3.478745295010657e-05
51151,103521,0,103521,332.3749289512634,3.452575653460189e-05
51251,103721,0,103721,332.983766078949,3.4265168029987166e-05
51351,103921,0,103921,333.6047978401184,3.40060196903115e-05
51451,104121,0,104121,334.2046089172363,3.374763791811429e-05
51552,104323,0,104323,335.0697548389435,3.348840966315586e-05
51652,104523,0,104523,335.6807837486267,3.323298358861103e-05
51752,104723,0,104723,336.28847885131836,3.297895696371409e-05
51852,104923,0,104923,336.89856576919556,3.2726515890778106e-05
51952,105123,0,105123,337.4913430213928,3.2475800655501076e-05
52052,105323,0,105323,338.0805058479309,3.2226532196011374e-05
52152,105523,0,105523,338.67868280410767,3.197916099323629e-05
52252,105723,0,105723,339.2710859775543,3.1733638745644914e-05
52352,105923,0,105923,339.8845360279083,3.148976793595069e-05
52452,106123,0,106123,340.49234890937805,3.1248287381188036e-05
52553,106325,0,106325,341.12679386138916,3.100603446358872e-05
52653,106525,0,106525,341.7794859409332,3.076850288402706e-05
52753,106725,0,106725,342.4600830078125,3.053310549363389e-05
52853,106925,0,106925,343.1286928653717,3.0299879882048615e-05
52953,107125,0,107125,343.75484013557434,3.006870365520377e-05
53053,107325,0,107325,344.3911271095276,2.9839857335849676e-05
53153,107525,0,107525,345.0135941505432,2.96130264010156e-05
53253,107725,0,107725,345.67022705078125,2.9388338746368155e-05
53353,107925,0,107925,346.2984688282013,2.9165943396633036e-05
53453,108125,0,108125,347.0047130584717,2.894542443994101e-05
53554,108327,0,108327,347.67646312713623,2.872511028379031e-05
53654,108527,0,108527,348.3052759170532,2.8508766216073827e-05
53754,108727,0,108727,349.03134989738464,2.829443008010574e-05
53854,108927,0,108927,349.7788710594177,2.808189275915651e-05
53954,109127,0,109127,350.5026822090149,2.7871104825364495e-05
54054,109327,0,109327,351.2570948600769,2.766174664941889e-05
54154,109527,0,109527,351.94405794143677,2.7453971265987298e-05
54254,109727,0,109727,352.67224407196045,2.7247401868772074e-05
54354,109927,0,109927,353.3786470890045,2.7041950610316864e-05
54454,110127,0,110127,354.1697189807892,2.6837934531089925e-05
54555,110329,0,110329,354.8905348777771,2.663257074141629e-05
54655,110529,0,110529,355.7283329963684,2.6430587780569974e-05
54755,110729,0,110729,356.44058299064636,2.6229535317192693e-05
54855,110929,0,110929,357.15073680877686,2.6029552013235097e-05
54955,111129,0,111129,357.88414216041565,2.5830518181817362e-05
55055,111329,0,111329,358.59960985183716,2.5632764911201122e-05
55155,111529,0,111529,359.30150294303894,2.5435883324491686e-05
55255,111729,0,111729,359.9685220718384,2.524017673636083e-05
55355,111929,0,111929,360.7099299430847,2.5045689120942454e-05
55455,112129,0,112129,361.39246582984924,2.4852206539384386e-05
55556,112331,0,112331,362.1593589782715,2.465826036784896e-05
55656,112531,0,112531,362.8707129955292,2.446730537766309e-05
55756,112731,0,112731,363.4994339942932,2.4277777723184916e-05
55856,112931,0,112931,364.1788420677185,2.4089521978280944e-05
55956,113131,0,113131,364.8579430580139,2.3902691575340915e-05
56056,113331,0,113331,365.48497104644775,2.371708484704446e-05
56156,113531,0,113531,366.1555299758911,2.3533050676478333e-05
56256,113731,0,113731,366.83223700523376,2.3350381624040462e-05
56356,113931,0,113931,367.4798810482025,2.3169202588273757e-05
56456,114131,0,114131,368.22042083740234,2.2989720401696376e-05
56557,114333,0,114333,368.92000579833984,2.2809910362262673e-05
56657,114533,0,114533,369.6110751628876,2.263383417133118e-05
56757,114733,0,114733,370.26581597328186,2.2459352328843787e-05
56857,114933,0,114933,370.9637858867645,2.2286755196490683e-05
56957,115133,0,115133,371.5862760543823,2.2115940830902616e-05
57057,115333,0,115333,372.16930413246155,2.1947049590799025e-05
57157,115533,0,115533,372.76252007484436,2.177979208049645e-05
57257,115733,0,115733,373.36372780799866,2.1614417351885568e-05
57357,115933,0,115933,373.9700779914856,2.145071925963538e-05
57457,116133,0,116133,374.5914099216461,2.128859423325382e-05
57558,116335,0,116335,375.20637488365173,2.112667422998877e-05
57658,116535,0,116535,375.85319805145264,2.0967699516192574e-05
57758,116735,0,116735,376.52798891067505,2.0810408758386963e-05
57858,116935,0,116935,377.1757791042328,2.065448158127986e-05
57958,117135,0,117135,377.8636348247528,2.049993181781727e-05
58058,117335,0,117335,378.57864594459534,2.0346614991395484e-05
58158,117535,0,117535,379.2965569496155,2.0194704858145192e-05
58258,117735,0,117735,379.95403504371643,2.0043783640262423e-05
58358,117935,0,117935,380.6011619567871,1.9894032141978684e-05
58458,118135,0,118135,381.24692392349243,1.97454291394858e-05
58559,118337,0,118337,381.8853528499603,1.9596158221805785e-05
58659,118537,0,118537,382.5211970806122,1.9449516101442805e-05
58759,118737,0,118737,383.27076411247253,1.9303652319141874e-05
58859,118937,0,118937,383.9805829524994,1.915872212089755e-05
58959,119137,0,119137,384.7412528991699,1.9014558244743635e-05
59059,119337,0,119337,385.4037010669708,1.887126195748468e-05
59159,119537,0,119537,386.03964400291443,1.872860522796255e-05
59259,119737,0,119737,386.69029784202576,1.8586901452993914e-05
59359,119937,0,119937,387.32730197906494,1.844584041925176e-05
59459,120137,0,120137,387.9417657852173,1.830559611170457e-05
59560,120339,0,120339,388.69621205329895,1.816488629364249e-05
59660,120539,0,120539,389.3617830276489,1.8026267040952264e-05
59760,120739,0,120739,390.0135669708252,1.7888733357865932e-05
59860,120939,0,120939,390.7386939525604,1.775211442151869e-05
59960,121139,0,121139,391.394238948822,1.761658564471472e-05
60060,121339,0,121339,392.0378839969635,1.748204897797837e-05
60160,121539,0,121539,392.74437403678894,1.7348803819419792e-05
60260,121739,0,121739,393.43798875808716,1.7216544850927023e-05
60360,121939,0,121939,394.1121201515198,1.708563634181421e-05
60460,122139,0,122139,394.86521792411804,1.6955945053165952e-05
60561,122341,0,122341,395.5207929611206,1.6826160028791547e-05
60661,122541,0,122541,396.1546711921692,1.669910615911218e-05
60761,122741,0,122741,396.7959179878235,1.6573212706128094e-05
60861,122941,0,122941,397.4983940124512,1.6448708926825412e-05
60961,123141,0,123141,398.19069480895996,1.632541848389529e-05
61061,123341,0,123341,398.87851119041443,1.6203436570302123e-05
61161,123541,0,123541,399.4818859100342,1.6082518029769993e-05
61261,123741,0,123741,400.10635900497437,1.5962891772901577e-05
61361,123941,0,123941,400.8191831111908,1.5844194950537758e-05
61461,124141,0,124141,401.4544150829315,1.5726544734975448e-05
61562,124343,0,124343,402.094398021698,1.5608769900655392e-05
61662,124543,0,124543,402.78393602371216,1.5492878980594764e-05
61762,124743,0,124743,403.46703696250916,1.5377941291400723e-05
61862,124943,0,124943,404.11604404449463,1.5263701389698473e-05
61962,125143,0,125143,404.74460101127625,1.5150199649539458e-05
62062,125343,0,125343,405.46997594833374,1.5037328438538426e-05
62162,125543,0,125543,406.1849138736725,1.4925154827623717e-05
62262,125743,0,125743,406.835618019104,1.4813441117636205e-05
62362,125943,0,125943,407.48988103866577,1.4702409965936642e-05
62462,126143,0,126143,408.08847093582153,1.4591840478928431e-05
62563,126345,0,126345,408.69754791259766,1.4480683365918852e-05
62663,126545,0,126545,409.3220510482788,1.437126738197788e-05
62763,126745,0,126745,409.9333429336548,1.4262276009837356e-05
62863,126945,0,126945,410.53281903266907,1.4153877784041205e-05
62963,127145,0,127145,411.1538031101227,1.4046001156033034e-05
63063,127345,0,127345,411.765949010849,1.3938722739015937e-05
63163,127545,0,127545,412.37078499794006,1.383191018574915e-05
63263,127745,0,127745,412.9565329551697,1.3725779572735748e-05
63363,127945,0,127945,413.54607486724854,1.3620141684758081e-05
63463,128145,0,128145,414.1534368991852,1.3515190282173448e-05
63564,128347,0,128347,414.7744948863983,1.3409850173584944e-05
63664,128547,0,128547,415.39181113243103,1.3306187645815762e-05
63764,128747,0,128747,416.02448987960815,1.3203371994691153e-05
63864,128947,0,128947,416.64029908180237,1.3101283465909305e-05
63964,129147,0,129147,417.2598338127136,1.3000090630357126e-05
64064,129347,0,129347,417.86910581588745,1.2899767113116023e-05
64164,129547,0,129547,418.47745513916016,1.2800416166629442e-05
64264,129747,0,129747,419.0674910545349,1.270190393674691e-05
64364,129947,0,129947,419.6441309452057,1.2604462067721216e-05
64464,130147,0,130147,420.24226999282837,1.2507878208588994e-05
64565,130349,0,130349,420.84535694122314,1.2411269890918923e-05
64665,130549,0,130549,421.42707991600037,1.2316659628862083e-05
64765,130749,0,130749,422.024973154068,1.2222819263759922e-05
64865,130949,0,130949,422.65682888031006,1.2129922600918836e-05
64965,131149,0,131149,423.28590989112854,1.2037853611787515e-05
65065,131349,0,131349,423.9060218334198,1.1946580965315364e-05
65165,131549,0,131549,424.5155670642853,1.1856065136206761e-05
65265,131749,0,131749,425.11040210723877,1.1766353708199098e-05
65365,131949,0,131949,425.72669291496277,1.167724871246685e-05
65465,132149,0,132149,426.32280802726746,1.1588947343439148e-05
65566,132351,0,132351,426.9393699169159,1.1500438385053332e-05
65666,132551,0,132551,427.55221819877625,1.1413423254379055e-05
65766,132751,0,132751,428.14381289482117,1.1327170441942158e-05
65866,132951,0,132951,428.74916100502014,1.1241518259173395e-05
65966,133151,0,133151,429.34031319618225,1.1156506329348e-05
66066,133351,0,133351,429.9369249343872,1.1072097398836292e-05
66166,133551,0,133551,430.5435938835144,1.0988308526350402e-05
66266,133751,0,133751,431.25048184394836,1.0904986088647595e-05
66366,133951,0,133951,432.14616084098816,1.0822277263820602e-05
66466,134151,0,134151,432.98023080825806,1.0739992642320685e-05
66567,134353,0,134353,433.89529180526733,1.0657363612103514e-05
66667,134553,0,134553,434.7601239681244,1.0576102336443649e-05
66767,134753,0,134753,435.61061787605286,1.0495182742941092e-05
66867,134953,0,134953,436.48784494400024,1.0414793228570489e-05
66967,135153,0,135153,437.2382950782776,1.033483385346973e-05
67067,135353,0,135353,438.016685962677,1.0255339052786068e-05
67167,135553,0,135553,438.812735080719,1.0176337895995188e-05
67267,135753,0,135753,439.623899936676,1.0097875100640438e-05
67367,135953,0,135953,440.42767214775085,1.0019865868934044e-05
67467,136153,0,136153,441.2257149219513,9.942464363251308e-06
67568,136355,0,136355,442.0674271583557,9.864838208106528e-06
67668,136555,0,136555,442.8186628818512,9.788552321385637e-06
67768,136755,0,136755,443.45524311065674,9.71298748709938e-06
67868,136955,0,136955,444.15042209625244,9.637984877770238e-06
67968,137155,0,137155,444.8312158584595,9.563667522618277e-06
68068,137355,0,137355,445.4767370223999,9.490071452886143e-06
68168,137555,0,137555,446.1261591911316,9.417143965723027e-06
68268,137755,0,137755,446.8735947608948,9.344881027881366e-06
68368,137955,0,137955,447.5651981830597,9.273424073879207e-06
68468,138155,0,138155,448.29535007476807,9.202581376413858e-06
68569,138357,0,138357,448.9791600704193,9.131791870563843e-06
68669,138557,0,138557,449.65449810028076,9.062507289409087e-06
68769,138757,0,138757,450.3195080757141,8.99387642718576e-06
68869,138957,0,138957,451.04637908935547,8.926021546686734e-06
68969,139157,0,139157,451.65922498703003,8.858878998736708e-06
69069,139357,0,139357,452.3623070716858,8.792442734339651e-06
69169,139557,0,139557,453.01997208595276,8.726668729635766e-06
69269,139757,0,139757,453.6280961036682,8.661604176695646e-06
69369,139957,0,139957,454.29483699798584,8.597111507336238e-06
69469,140157,0,140157,454.9539740085602,8.533243973006507e-06
69570,140359,0,140359,455.69319200515747,8.46926274520164e-06
69670,140559,0,140559,456.34978795051575,8.4064320740932e-06
69770,140759,0,140759,457.05005288124084,8.34413592844067e-06
69870,140959,0,140959,457.71186685562134,8.282209224020744e-06
69970,141159,0,141159,458.3615128993988,8.220716244237576e-06
70070,141359,0,141359,459.0150001049042,8.15960579700872e-06
70170,141559,0,141559,459.7156238555908,8.09882843162136e-06
70270,141759,0,141759,460.3523588180542,8.038352925438101e-06
70370,141959,0,141959,461.07253408432007,7.978231898212134e-06
70470,142159,0,142159,461.7345688343048,7.918350513493208e-06
70571,142361,0,142361,462.36542105674744,7.85816125301329e-06
70671,142561,0,142561,462.99021792411804,7.798913813381822e-06
70771,142761,0,142761,463.58568596839905,7.739923909181886e-06
70871,142961,0,142961,464.1959738731384,7.681304821705222e-06
70971,143161,0,143161,464.78199100494385,7.622960271769597e-06
71071,143361,0,143361,465.41716980934143,7.564964713800656e-06
71171,143561,0,143561,466.07135701179504,7.507363479542707e-06
71271,143761,0,143761,466.72151613235474,7.450142415256025e-06
71371,143961,0,143961,467.3684720993042,7.393285777399734e-06
71471,144161,0,144161,467.9876379966736,7.336921548769119e-06
71572,144363,0,144363,468.75275015830994,7.280381105019782e-06
71672,144563,0,144563,469.4639639854431,7.224857186431219e-06
71772,144763,0,144763,470.1030521392822,7.1698837072445935e-06
71872,144963,0,144963,470.8810999393463,7.115334130268065e-06
71972,145163,0,145163,471.53812289237976,7.06132749647829e-06
72072,145363,0,145363,472.2201430797577,7.007825944211396e-06
72172,145563,0,145563,472.8610529899597,6.954835793758115e-06
72272,145763,0,145763,473.5195698738098,6.902340738013492e-06
72372,145963,0,145963,474.2089421749115,6.850390865927634e-06
72472,146163,0,146163,474.8682041168213,6.798900524696962e-06
72573,146365,0,146365,475.5143837928772,6.74738038507656e-06
72673,146565,0,146565,476.1572799682617,6.69686324770728e-06
72773,146765,0,146765,476.83115100860596,6.646771911011553e-06
72873,146965,0,146965,477.6176450252533,6.59717745652697e-06
72973,147165,0,147165,478.25211811065674,6.547943306296499e-06
73073,147365,0,147365,478.98289585113525,6.499128352094346e-06
73173,147565,0,147565,479.6576318740845,6.450697382032735e-06
73273,147765,0,147765,480.2871301174164,6.402620827333474e-06
73373,147965,0,147965,480.88256192207336,6.354853803882367e-06
73473,148165,0,148165,481.577898979187,6.307454005809182e-06
73574,148367,0,148367,482.31625390052795,6.259831382669664e-06
73674,148567,0,148567,483.3391628265381,6.212946624938324e-06
73774,148767,0,148767,484.07390999794006,6.166366123968573e-06
73874,148967,0,148967,484.69056582450867,6.119968230353549e-06
73974,149167,0,149167,485.3141529560089,6.073843096076162e-06
74074,149367,0,149367,485.92646503448486,6.027884190548463e-06
74174,149567,0,149567,486.52882409095764,5.9821171241385404e-06
74274,149767,0,149767,487.1366078853607,5.936552718669297e-06
74374,149967,0,149967,487.72609305381775,5.891190427785493e-06
74474,150167,0,150167,488.3263759613037,5.845976198538585e-06
74575,150369,0,150369,488.9737629890442,5.800565718091956e-06
74675,150569,0,150569,489.57557702064514,5.7558369132181936e-06
74775,150769,0,150769,490.1651918888092,5.711324993775308e-06
74875,150969,0,150969,490.840900182724,5.667149355843167e-06
74975,151169,0,151169,491.4607789516449,5.623223486844825e-06
75075,151369,0,151369,492.05795884132385,5.579632484490381e-06
75175,151569,0,151569,492.65349102020264,5.536366216019064e-06
75275,151769,0,151769,493.2597119808197,5.493438410783094e-06
75375,151969,0,151969,493.8481459617615,5.450842567026544e-06
75475,152169,0,152169,494.43840193748474,5.408634446041755e-06
75576,152371,0,152371,495.0362501144409,5.366330496517034e-06
75676,152571,0,152571,495.6350929737091,5.324802466985541e-06
75776,152771,0,152771,496.2743270397186,5.28367961591007e-06
75876,152971,0,152971,496.9093029499054,5.242884052922791e-06
75976,153171,0,153171,497.5529668331146,5.2025006269278264e-06
76076,153371,0,153371,498.2955551147461,5.162474070247018e-06
76176,153571,0,153571,499.0639429092407,5.122827011812248e-06
76276,153771,0,153771,499.75546002388,5.083569693792328e-06
76376,153971,0,153971,500.3991689682007,5.044715217185312e-06
76476,154171,0,154171,501.2404658794403,5.006207089397427e-06
76577,154373,0,154373,501.93090415000916,4.967732215366245e-06
76677,154573,0,154573,502.7770380973816,4.9300297651013014e-06
76777,154773,0,154773,503.51630687713623,4.892667429254642e-06
76877,154973,0,154973,504.1841480731964,4.855714931500125e-06
76977,155173,0,155173,504.89077496528625,4.81908439921022e-06
77077,155373,0,155373,505.5897150039673,4.782801293762221e-06
77177,155573,0,155573,506.27947998046875,4.7468190984422e-06
77277,155773,0,155773,507.09723591804504,4.711136634652969e-06
77377,155973,0,155973,508.0875689983368,4.6757064895309695e-06
77477,156173,0,156173,508.8962061405182,4.640550846775455e-06
77578,156375,0,156375,509.8362228870392,4.605259714452819e-06
77678,156575,0,156575,510.79137897491455,4.570538505013441e-06
77778,156775,0,156775,511.4780170917511,4.536058643988779e-06
77878,156975,0,156975,512.1315879821777,4.50176351097292e-06
77978,157175,0,157175,512.7893800735474,4.467706645686447e-06
78078,157375,0,157375,513.5007028579712,4.433828506148469e-06
78178,157575,0,157575,514.1695308685303,4.400166848662369e-06
78278,157775,0,157775,515.1405999660492,4.36670054666082e-06
78378,157975,0,157975,516.1388289928436,4.333439773565808e-06
78478,158175,0,158175,516.914244890213,4.30035366528698e-06
78579,158377,0,158377,517.6172490119934,4.26717338839268e-06
78679,158577,0,158577,518.3363630771637,4.234506444369769e-06
78779,158777,0,158777,519.1833038330078,4.2020341075590146e-06
78879,158977,0,158977,519.8516170978546,4.169817229262236e-06
78979,159177,0,159177,520.5025520324707,4.137784507893257e-06
79079,159377,0,159377,521.1632080078125,4.106001278618e-06
79179,159577,0,159577,522.0002980232239,4.074449252982557e-06
79279,159777,0,159777,522.7276520729065,4.043145921149018e-06
79379,159977,0,159977,523.5685591697693,4.012080752675307e-06
79479,160177,0,160177,524.7420680522919,3.981317666105197e-06
79580,160379,0,160379,525.4439549446106,3.950496040725624e-06
79680,160579,0,160579,526.1651358604431,3.920276808071134e-06
79780,160779,0,160779,526.845675945282,3.890383427832657e-06
79880,160979,0,160979,527.5440559387207,3.8607737059271235e-06
79980,161179,0,161179,528.1611189842224,3.831512068940237e-06
80080,161379,0,161379,528.833398103714,3.8025453023885537e-06
80180,161579,0,161579,529.48384308815,3.7739078379104337e-06
80280,161779,0,161779,530.4195849895477,3.7455753286746114e-06
80380,161979,0,161979,531.1123919487,3.7175551393393335e-06
80480,162179,0,162179,531.7630319595337,3.68980297314952e-06
80581,162381,0,162381,532.4402461051941,3.662076834574067e-06
80681,162581,0,162581,533.0767920017242,3.6348709231321e-06
80781,162781,0,162781,533.6986210346222,3.607906757920782e-06
80881,162981,0,162981,534.315672159195,3.5811925187506002e-06
80981,163181,0,163181,534.914351940155,3.5546783979919598e-06
81081,163381,0,163381,535.5051209926605,3.5283876305968027e-06
81181,163581,0,163581,536.0958080291748,3.5022651556287515e-06
81281,163781,0,163781,536.7111728191376,3.476330539603092e-06
81381,163981,0,163981,537.3039548397064,3.4505516904251232e-06
81481,164181,0,164181,537.8951139450073,3.4249350964786683e-06
81582,164383,0,164383,538.5337378978729,3.399182405427791e-06
81682,164583,0,164583,539.1522009372711,3.3738407379563757e-06
81782,164783,0,164783,539.7673690319061,3.3486130951712232e-06
81882,164983,0,164983,540.3566768169403,3.323494234062731e-06
81982,165183,0,165183,540.9868788719177,3.2985329460532954e-06
82082,165383,0,165383,541.6059498786926,3.2736639603264874e-06
82182,165583,0,165583,542.2150871753693,3.248929878597313e-06
82282,165783,0,165783,542.8452107906342,3.224321037993892e-06
82382,165983,0,165983,543.4570989608765,3.199843142208055e-06
82482,166183,0,166183,544.0671417713165,3.1754777956940448e-06
82583,166385,0,166385,544.6755578517914,3.151042886154563e-06
82683,166585,0,166585,545.286041021347,3.1269674225249115e-06
82783,166785,0,166785,545.8747789859772,3.1030502698863703e-06
82883,166985,0,166985,546.4670519828796,3.0793172371672937e-06
82983,167185,0,167185,547.0766189098358,3.055729893422786e-06
83083,167385,0,167385,547.6598899364471,3.0323502903909136e-06
83183,167585,0,167585,548.2589540481567,3.0091515024766936e-06
83283,167785,0,167785,548.8459329605103,2.986155210052376e-06
83383,167985,0,167985,549.4396591186523,2.963356847060609e-06
83483,168185,0,168185,550.0195660591125,2.9407802042907966e-06
83584,168387,0,168387,550.605908870697,2.918170619569536e-06
83684,168587,0,168587,551.191731929779,2.8960151440899013e-06
83784,168787,0,168787,551.7786328792572,2.874061410343222e-06
83884,168987,0,168987,552.3727450370789,2.85231843241691e-06
83984,169187,0,169187,552.9603190422058,2.8308037674667108e-06
84084,169387,0,169387,553.5554180145264,2.8094754450873076e-06
84184,169587,0,169587,554.1372790336609,2.7883687710220772e-06
84284,169787,0,169787,554.7185111045837,2.767452767990027e-06
84384,169987,0,169987,555.3015899658203,2.7467214645459015e-06
84484,170187,0,170187,555.8983118534088,2.72615933508333e-06
84585,170389,0,170389,556.4948379993439,2.705571511941965e-06
84685,170589,0,170589,557.0769329071045,2.685309433290966e-06
84785,170789,0,170789,557.6723310947418,2.665194921709819e-06
84885,170989,0,170989,558.2541718482971,2.645208115197551e-06
84985,171189,0,171189,558.8372559547424,2.6253184580682564e-06
85085,171389,0,171389,559.4406979084015,2.605566462832908e-06
85185,171589,0,171589,560.0951619148254,2.585904061393184e-06
85285,171789,0,171789,560.7126569747925,2.566345352638161e-06
85385,171989,0,171989,561.3095240592957,2.5468993078231486e-06
85485,172189,0,172189,561.9271218776703,2.5275594877472443e-06
85586,172391,0,172391,562.5450518131256,2.508113175755994e-06
85686,172591,0,172591,563.1670877933502,2.488984446413225e-06
85786,172791,0,172791,563.7580919265747,2.46994892586167e-06
85886,172991,0,172991,564.3616309165955,2.451017548838693e-06
85986,173191,0,173191,564.9477660655975,2.4322055746942683e-06
86086,173391,0,173391,565.5448288917542,2.413491154492168e-06
86186,173591,0,173591,566.1716830730438,2.3948986978617078e-06
86286,173791,0,173791,566.7796580791473,2.3764150333947072e-06
86386,173991,0,173991,567.3714711666107,2.3580481831241218e-06
86486,174191,0,174191,567.9748778343201,2.339794836447996e-06
86587,174393,0,174393,568.5997200012207,2.321495051495372e-06
86687,174593,0,174593,569.2078640460968,2.3034812661446043e-06
86787,174793,0,174793,569.8030829429626,2.2856068311588078e-06
86887,174993,0,174993,570.4031829833984,2.2678613479223647e-06
86987,175193,0,175193,571.0293021202087,2.250253911743942e-06
87087,175393,0,175393,571.629312992096,2.232804458135173e-06
87187,175593,0,175593,572.2268528938293,2.215495589391987e-06
87287,175793,0,175793,572.8286700248718,2.1983557392862455e-06
87387,175993,0,175993,573.4384250640869,2.1813796435135547e-06
87487,176193,0,176193,574.0209710597992,2.1645688755179054e-06
87588,176395,0,176395,574.6137809753418,2.147755829317943e-06
87688,176595,0,176595,575.2253239154816,2.1312924838890866e-06
87788,176795,0,176795,575.8048748970032,2.1149801759977623e-06
87888,176995,0,176995,576.3926179409027,2.0988379535929303e-06
87988,177195,0,177195,576.9907479286194,2.082858702918764e-06
88088,177395,0,177395,577.5803310871124,2.0670354740016958e-06
88188,177595,0,177595,578.197338104248,2.0513756143699444e-06
88288,177795,0,177795,578.7861199378967,2.035858888402486e-06
88388,177995,0,177995,579.3867688179016,2.020494909856002e-06
88488,178195,0,178195,579.9717991352081,2.0052747932716198e-06
88589,178397,0,178397,580.5732569694519,1.9900508459123435e-06
88689,178597,0,178597,581.1855340003967,1.9750985379851917e-06
88789,178797,0,178797,581.7794480323792,1.9602906551972216e-06
88889,178997,0,178997,582.3756411075592,1.945596151435756e-06
88989,179197,0,179197,582.9636399745941,1.9310241467658295e-06
89089,179397,0,179397,583.5594608783722,1.9165712747214978e-06
89189,179597,0,179597,584.2747828960419,1.9022216891742925e-06
89289,179797,0,179797,584.9579257965088,1.887975560370724e-06
89389,179997,0,179997,585.7207617759705,1.8738260539184176e-06
89489,180197,0,180197,586.5515367984772,1.8597684035906994e-06
89590,180399,0,180399,587.3266041278839,1.8456527108642321e-06
89690,180599,0,180599,588.3229150772095,1.8317665243006394e-06
89790,180799,0,180799,589.0684008598328,1.8179468026736838e-06
89890,180999,0,180999,589.6977269649506,1.8042040416748932e-06
89990,181199,0,181199,590.4895720481873,1.7905314581199996e-06
90090,181399,0,181399,591.3753180503845,1.776931842160697e-06
90190,181599,0,181599,592.0639729499817,1.7634158459338296e-06
90290,181799,0,181799,592.8882579803467,1.7499692914795147e-06
90390,181999,0,181999,593.499354839325,1.7366111646817009e-06
90490,182199,0,182199,594.1284260749817,1.7233476500255928e-06
90591,182401,0,182401,594.7257721424103,1.710049434287031e-06
90691,182601,0,182601,595.3474910259247,1.6969704935572674e-06
90791,182801,0,182801,595.9379539489746,1.6840096149626877e-06
90891,183001,0,183001,596.5566971302032,1.6711520777234454e-06
90991,183201,0,183201,597.1538910865784,1.6584066526467182e-06
91091,183401,0,183401,597.7538540363312,1.645783710156191e-06
91191,183601,0,183601,598.3675048351288,1.633280882331549e-06
91291,183801,0,183801,598.9858827590942,1.6209014746470676e-06
91391,184001,0,184001,599.5942988395691,1.6086441137379897e-06
91491,184201,0,184201,600.1933560371399,1.596509742104133e-06
91592,184403,0,184403,600.8179559707642,1.5843787362078483e-06
91692,184603,0,184603,601.425598859787,1.5724946821974035e-06
91792,184803,0,184803,602.0334300994873,1.5607202830781737e-06
91892,185003,0,185003,602.6386139392853,1.5490663500186797e-06
91992,185203,0,185203,603.2656409740448,1.5375209073907825e-06
92092,185403,0,185403,603.8959879875183,1.5260812466214766e-06
92192,185603,0,185603,604.5085701942444,1.5147506325257688e-06
92292,185803,0,185803,605.126219034195,1.5035130687255285e-06
92392,186003,0,186003,605.7266299724579,1.4923692652286187e-06
92492,186203,0,186203,606.3310580253601,1.4813166098323629e-06
92593,186405,0,186405,606.9500200748444,1.4702379345534065e-06
92693,186605,0,186605,607.5604820251465,1.459335993350903e-06
92793,186805,0,186805,608.1909618377686,1.4485156785497143e-06
92893,187005,0,187005,608.811802148819,1.437755459854486e-06
92993,187205,0,187205,609.4189748764038,1.4270543735565689e-06
93093,187405,0,187405,610.0142540931702,1.4164150710628116e-06
93193,187605,0,187605,610.6045770645142,1.4058248629781644e-06
93293,187805,0,187805,611.20228099823,1.395291249509511e-06
93393,188005,0,188005,611.8114049434662,1.3848043912678075e-06
93493,188205,0,188205,612.4165670871735,1.3743634345532688e-06
93594,188407,0,188407,613.0349559783936,1.3638681824790274e-06
93694,188607,0,188607,613.6392419338226,1.3535277450155348e-06
93794,188807,0,188807,614.2417321205139,1.3432236341376245e-06
93894,189007,0,189007,614.8418719768524,1.3329751419255003e-06
93994,189207,0,189207,615.4455499649048,1.3227798818890784e-06
94094,189407,0,189407,616.0512890815735,1.3126353530357905e-06
94194,189607,0,189607,616.6510980129242,1.3025547539576348e-06
94294,189807,0,189807,617.2606341838837,1.2925397849867724e-06
94394,190007,0,190007,617.8822209835052,1.2825915753454641e-06
94494,190207,0,190207,618.4849500656128,1.2727206850032e-06
94595,190409,0,190409,619.0867660045624,1.2628334451157749e-06
94695,190609,0,190609,619.6870319843292,1.2531183974701988e-06
94795,190809,0,190809,620.2983071804047,1.2434959456660206e-06
94895,191009,0,191009,620.9165308475494,1.2339553454112062e-06
94995,191209,0,191209,621.5151998996735,1.2245015662122534e-06
95095,191409,0,191409,622.119304895401,1.2151416319119495e-06
95195,191609,0,191609,622.7104949951172,1.2058636528237055e-06
95295,191809,0,191809,623.2983779907227,1.1966755125647558e-06
95395,192009,0,192009,623.8850340843201,1.1875720422037863e-06
95495,192209,0,192209,624.489984035492,1.178548265083279e-06
95596,192411,0,192411,625.0832901000977,1.1695183919269834e-06
95696,192611,0,192611,625.6753380298615,1.1606571934457763e-06
95796,192811,0,192811,626.2768361568451,1.1518652626813492e-06
95896,193011,0,193011,626.906594991684,1.1431520471685178e-06
95996,193211,0,193211,627.5283739566803,1.1345122821810895e-06
96096,193411,0,193411,628.1312749385834,1.1259423518478545e-06
96196,193611,0,193611,628.7546439170837,1.1174488074276777e-06
96296,193811,0,193811,629.3544399738312,1.109021561821781e-06
96396,194011,0,194011,629.9657537937164,1.1006638273926115e-06
96496,194211,0,194211,630.5774290561676,1.0923722907727755e-06
96597,194413,0,194413,631.1818768978119,1.0840583368099956e-06
96697,194613,0,194613,631.7842519283295,1.075881840308675e-06
96797,194813,0,194813,632.3880798816681,1.0677634112301208e-06
96897,195013,0,195013,633.0047340393066,1.0596883876249186e-06
96997,195213,0,195213,633.5937559604645,1.051663210002239e-06
97097,195413,0,195413,634.185035943985,1.0436860946132034e-06
97197,195613,0,195613,634.7786450386047,1.035747017504654e-06
97297,195813,0,195813,635.3675577640533,1.0278549296860162e-06
97397,196013,0,196013,635.9553279876709,1.0200052089645967e-06
97497,196213,0,196213,636.548975944519,1.0121943544906185e-06
97598,196415,0,196415,637.1539199352264,1.0043523179938854e-06
97698,196615,0,196615,637.7392871379852,9.966326188669086e-07
97798,196815,0,196815,638.3265841007233,9.889522774418954e-07
97898,197015,0,197015,638.9100549221039,9.813222441203943e-07
97998,197215,0,197215,639.5118458271027,9.737394366816385e-07
98098,197415,0,197415,640.1088230609894,9.662046130810569e-07
98198,197615,0,197615,640.7085750102997,9.587290081837911e-07
98298,197815,0,197815,641.3140740394592,9.513035387357513e-07
98398,198015,0,198015,641.9098289012909,9.439384114206126e-07
98498,198215,0,198215,642.5046610832214,9.366322869161767e-07
98599,198417,0,198417,643.1066329479218,9.293146885608845e-07
98699,198617,0,198617,643.7138249874115,9.221294159223128e-07
98799,198817,0,198817,644.3119428157806,9.150099619610875e-07
98899,199017,0,199017,644.9177448749542,9.079534592504279e-07
98999,199217,0,199217,645.5203168392181,9.009640445539038e-07
99099,199417,0,199417,646.1035780906677,8.940445639886966e-07
99199,199617,0,199617,646.6888709068298,8.871930218869844e-07
99299,199817,0,199817,647.27774477005,8.804185973959066e-07
99399,200017,0,200017,647.8891589641571,8.737119264510185e-07
99499,200217,0,200217,648.5291268825531,8.670821048970407e-07
99600,200419,0,200419,649.14275598526,8.604598341583776e-07
99700,200619,0,200619,649.7710380554199,8.539735896117068e-07
99800,200819,0,200819,650.3901538848877,8.475539440632675e-07
99900,201019,0,201019,651.0035009384155,8.41203786902975e-07
100000,201219,0,201219,651.6190719604492,8.349147262165961e-07


==> plot_data/quadratic_minimax_problem_n500_alpha00001/iflex-jsym.tex <==
iterations,numFevals,numproxgevals,numoperatorevals,times,performance
0,1,0,1,0.0026328563690185547,30.358106049564984
100,306,0,306,14.320288896560669,0.9422502041522252
200,619,0,619,27.078051805496216,0.6454136351145678
300,942,0,942,39.46141576766968,0.5019972146039132
400,1286,0,1286,51.95039200782776,0.43140873841620175
501,1619,0,1619,66.2687919139862,0.30496679106112357
601,1944,0,1944,79.18061375617981,0.18817142900277187
701,2262,0,2262,92.19059681892395,0.15371379297272325
801,2579,0,2579,104.54784774780273,0.12338554112716502
901,2894,0,2894,117.20402669906616,0.08221709423217131
1001,3237,0,3237,130.38253784179688,0.06984434218493957
1101,3561,0,3561,143.53513193130493,0.06010246580473832
1201,3898,0,3898,156.12393069267273,0.047199717744222616
1301,4221,0,4221,168.42241096496582,0.04086055685802822
1401,4544,0,4544,180.83590483665466,0.03746282103789143
1502,4890,0,4890,193.27395677566528,0.03298771243418722
1602,5256,0,5256,205.75885581970215,0.030609032513997284
1702,5608,0,5608,218.09506678581238,0.027487031735449835
1802,5950,0,5950,230.6181778907776,0.020729467353265186
1902,6262,0,6262,244.77308678627014,0.016411253938967335
2002,6566,0,6566,257.7110116481781,0.014535583141738168
2102,6924,0,6924,270.39437794685364,0.013081551052449453
2202,7258,0,7258,283.3077030181885,0.01253580897335412
2302,7616,0,7616,297.29773783683777,0.011474476867663135
2402,8018,0,8018,311.64810490608215,0.011022913812834226
2503,8424,0,8424,323.96124792099,0.010595203571808329
2603,8827,0,8827,336.60743594169617,0.01027737539856765
2703,9203,0,9203,349.1094739437103,0.009619172677001865
2803,9575,0,9575,363.7211458683014,0.009170373933208886
2903,9970,0,9970,377.47912979125977,0.008889484050902249
3003,10350,0,10350,390.5671308040619,0.008616093915275026
3103,10748,0,10748,402.9129958152771,0.008305742516016706
3203,11148,0,11148,415.49212884902954,0.008060462809686189
3303,11548,0,11548,427.90462589263916,0.007827010149757493
3403,11948,0,11948,441.50829577445984,0.007600005517303026
3504,12352,0,12352,454.07040572166443,0.007377068571289519
3604,12721,0,12721,466.48176193237305,0.006934409501450845
3704,13105,0,13105,480.4797348976135,0.006671262425635498
3804,13484,0,13484,493.051894903183,0.0064036368258757834
3904,13887,0,13887,505.90757870674133,0.0062162913644169746
4004,14287,0,14287,519.415755033493,0.0060527692799498874
4104,14688,0,14688,532.2386207580566,0.005888929265942775
4204,15090,0,15090,545.2517008781433,0.005745148820044792
4304,15458,0,15458,557.7466368675232,0.005544341333481691
4404,15859,0,15859,570.2446918487549,0.005401691863294874
4505,16267,0,16267,583.5146317481995,0.005264399318165443
4605,16667,0,16667,596.2369027137756,0.005137824160175279
4705,17055,0,17055,609.0616450309753,0.004967653676811899
4805,17408,0,17408,622.1610238552094,0.004760483722098519
4905,17808,0,17808,635.0699429512024,0.004644044355785966
5005,18180,0,18180,647.6781597137451,0.004533124046759345
5105,18584,0,18584,661.5949869155884,0.004425196115630989
5205,18984,0,18984,674.1957459449768,0.004323504846899951
5305,19386,0,19386,688.3045749664307,0.004218546758477948
5405,19786,0,19786,701.8029727935791,0.004117843277968966
5506,20190,0,20190,715.7630977630615,0.004022398318283946
5606,20606,0,20606,728.1963038444519,0.00393091013479318
5706,21010,0,21010,740.8697829246521,0.0038533633795048007
5806,21365,0,21365,753.4239187240601,0.003726492113100608
5906,21747,0,21747,766.8110547065735,0.003625610447392005
6006,22154,0,22154,779.6448328495026,0.0035434126392202715
6106,22521,0,22521,792.4005868434906,0.0034732136208631805
6206,22922,0,22922,804.9844448566437,0.0034003347687246084
6306,23268,0,23268,817.6081347465515,0.003330482374597922
6406,23668,0,23668,830.8294508457184,0.0032464377800249748
6507,24080,0,24080,844.0932068824768,0.003177920281810571
6607,24483,0,24483,857.4227876663208,0.003114156893866665
6707,24848,0,24848,870.7252368927002,0.0030232935387433262
6807,25237,0,25237,884.1292088031769,0.0029530785144706866
6907,25629,0,25629,897.6164417266846,0.0028837659394432146
7007,25996,0,25996,910.8111429214478,0.0028135980733120704
7107,26340,0,26340,924.1725697517395,0.002779390401043439
7207,26734,0,26734,937.2359910011292,0.0027224226840900155
7307,27130,0,27130,950.429780960083,0.0026730402817795595
7407,27489,0,27489,964.0635948181152,0.0026310161955881654
7508,27845,0,27845,977.4715876579285,0.0025825858740462834
7608,28243,0,28243,990.6157388687134,0.002528906891232298
7708,28647,0,28647,1003.7907519340515,0.0024790644118429985
7808,29034,0,29034,1018.2161557674408,0.0024329172547202602
7908,29415,0,29415,1033.5922708511353,0.0023814944757358397
8008,29815,0,29815,1047.6484627723694,0.002333865148872729
8108,30226,0,30226,1061.5310850143433,0.002286652378843076
8208,30619,0,30619,1075.2793338298798,0.0022533649811338164
8308,31012,0,31012,1089.0825889110565,0.0022152277147825016
8408,31419,0,31419,1101.9019718170166,0.0021729502222565637
8509,31825,0,31825,1115.6117010116577,0.0021345489793878755
8609,32182,0,32182,1129.381561756134,0.0020578318140581004
8709,32520,0,32520,1142.8710677623749,0.002020681228389821
8809,32921,0,32921,1158.062005996704,0.001984076473889116
8909,33321,0,33321,1170.9583506584167,0.0019495324044025732
9009,33714,0,33714,1184.101893901825,0.0019117539977271398
9109,34115,0,34115,1197.4933869838715,0.0018802119638683995
9209,34523,0,34523,1210.7037768363953,0.0018478231295097627
9309,34923,0,34923,1223.86079788208,0.0018151816746560902
9409,35323,0,35323,1236.7886867523193,0.001785075383718616
9510,35693,0,35693,1250.95831990242,0.001750890860639731
9610,36061,0,36061,1264.3509788513184,0.0017260215747920834
9710,36462,0,36462,1277.2281339168549,0.0016970871431886921
9810,36863,0,36863,1290.1840069293976,0.0016687473787766263
9910,37248,0,37248,1302.8961129188538,0.0016387053062096035
10010,37626,0,37626,1315.112049818039,0.0015991861080642167
10110,38030,0,38030,1329.5293889045715,0.001572717378416053
10210,38439,0,38439,1342.9929978847504,0.0015473764092206392
10310,38841,0,38841,1355.0766327381134,0.0015231332080212032
10410,39203,0,39203,1367.1157848834991,0.0014926783972053364
10511,39614,0,39614,1379.3518829345703,0.0014589677200493845
10611,40033,0,40033,1391.9240798950195,0.0014336658423230527
10711,40443,0,40443,1407.3018009662628,0.0014126628104428258
10811,40849,0,40849,1420.2639198303223,0.0013896365840841676
10911,41249,0,41249,1435.9298989772797,0.0013697459903100231
11011,41650,0,41650,1449.1853036880493,0.001351024386897269
11111,42050,0,42050,1462.6232538223267,0.001331738889948267
11211,42440,0,42440,1476.052875995636,0.0013131124619855164
11311,42841,0,42841,1488.8200318813324,0.0012938310456183768
11411,43232,0,43232,1502.3149619102478,0.0012732451084010836
11512,43636,0,43636,1515.7867438793182,0.0012554015228936448
11612,44039,0,44039,1528.7091567516327,0.0012353780352350962
11712,44439,0,44439,1542.1411938667297,0.0012171475796690988
11812,44842,0,44842,1555.3097338676453,0.0012000052203734396
11912,45242,0,45242,1568.1469719409943,0.001182460501693055
12012,45649,0,45649,1581.4098329544067,0.0011663032102492224
12112,46050,0,46050,1594.4399118423462,0.0011494719563772899
12212,46456,0,46456,1609.2976748943329,0.001132723206714369
12312,46856,0,46856,1623.9189157485962,0.0011170926976670154
12412,47259,0,47259,1638.1216268539429,0.0011011919814463591
12513,47663,0,47663,1654.0793499946594,0.0010859361579843802
12613,48065,0,48065,1669.9881646633148,0.0010721755351631563
12713,48465,0,48465,1682.8820819854736,0.0010568730436232136
12813,48865,0,48865,1695.256404876709,0.001041453670032459
12913,49265,0,49265,1705.6983397006989,0.001027166286410131
13013,49665,0,49665,1716.2093250751495,0.0010135892301770537
13113,50067,0,50067,1726.5059387683868,0.0009991442060019596
13213,50467,0,50467,1736.7197387218475,0.0009852861658181111
13313,50867,0,50867,1747.8129708766937,0.0009719468480550609
13413,51267,0,51267,1758.6908700466156,0.0009601337440435346
13514,51675,0,51675,1769.4830548763275,0.000946612122085883
13614,52011,0,52011,1780.5671517848969,0.0009271237410040231
13714,52402,0,52402,1791.445071697235,0.000907199593501205
13814,52802,0,52802,1801.578617811203,0.0008916422030383128
13914,53239,0,53239,1811.9286658763885,0.0008783760194220778
14014,53719,0,53719,1822.5408608913422,0.0008661778610022733
14114,54123,0,54123,1832.587462902069,0.0008539540801192267
14214,54523,0,54523,1842.6651289463043,0.0008418467849681847
14314,54923,0,54923,1852.7770779132843,0.0008299138528635405
14414,55323,0,55323,1862.8224167823792,0.0008156513884347599
14515,55727,0,55727,1873.1323509216309,0.0008032012308447868
14615,56151,0,56151,1883.000331878662,0.000794606684711435
14715,56566,0,56566,1893.0025007724762,0.000783648597672953
14815,56931,0,56931,1903.6007947921753,0.0007718833450045091
14915,57331,0,57331,1913.9983139038086,0.0007593463922832501
15015,57731,0,57731,1924.0168859958649,0.0007390001595945756
15115,58131,0,58131,1933.8897268772125,0.0007204871710550149
15215,58531,0,58531,1943.8463339805603,0.0007098726301379159
15315,58931,0,58931,1953.8134589195251,0.0007006559230223607
15415,59331,0,59331,1966.0064158439636,0.0006900433427787053
15516,59735,0,59735,1976.5860648155212,0.0006814299631436453
15616,60135,0,60135,1986.741266965866,0.00067218983020765
15716,60538,0,60538,1996.8994617462158,0.0006592218163309039
15816,60938,0,60938,2007.127644777298,0.0006494569607892599
15916,61339,0,61339,2017.1052479743958,0.0006393652583115093
16016,61740,0,61740,2027.4574139118195,0.0006314554294007589
16116,62140,0,62140,2038.113273859024,0.0006242061074775746
16216,62540,0,62540,2049.5724079608917,0.0006198007037450807
16316,62943,0,62943,2060.2774288654327,0.0006112244860067309
16416,63343,0,63343,2070.4109008312225,0.0006033667849436786
16517,63752,0,63752,2081.179081916809,0.0005958126018257389
16617,64152,0,64152,2091.878425836563,0.0005884304076770148
16717,64560,0,64560,2103.9045197963715,0.0005807329723163746
16817,64960,0,64960,2114.2978649139404,0.000572434739333991
16917,65360,0,65360,2124.975908756256,0.0005645859132482295
17017,65775,0,65775,2137.437141895294,0.0005550983510809038
17117,66177,0,66177,2149.628495693207,0.0005506704438528659
17217,66577,0,66577,2161.1236548423767,0.0005460777058542842
17317,66997,0,66997,2173.260134935379,0.0005390892578602638
17417,67397,0,67397,2185.1960220336914,0.0005325580499249493
17518,67801,0,67801,2195.550178050995,0.0005256167183984047
17618,68239,0,68239,2205.8031108379364,0.0005163361818477986
17718,68712,0,68712,2215.7998719215393,0.0005059529496340252
17818,69113,0,69113,2225.64341878891,0.0004970593989266672
17918,69513,0,69513,2235.604395866394,0.000490409209747679
18018,69914,0,69914,2246.724880695343,0.00048408129955181676
18118,70314,0,70314,2259.1571867465973,0.0004779228277252532
18218,70711,0,70711,2271.1914498806,0.0004712955836481078
18318,71108,0,71108,2281.9602658748627,0.0004650416142208705
18418,71508,0,71508,2291.9779546260834,0.0004588579804950263
18519,71923,0,71923,2302.2331619262695,0.0004530204673623569
18619,72323,0,72323,2312.353904724121,0.00044759037349184546
18719,72723,0,72723,2322.512184858322,0.0004420890566590109
18819,73128,0,73128,2332.6552879810333,0.0004367747293393769
18919,73485,0,73485,2342.8513708114624,0.00043254697721018426
19019,73889,0,73889,2353.4478499889374,0.00042765332796154573
19119,74289,0,74289,2365.029685020447,0.00042268659756135237
19219,74692,0,74692,2375.327740907669,0.0004181894881244355
19319,75093,0,75093,2385.458564758301,0.00041259586685208526
19419,75493,0,75493,2395.5801708698273,0.00040745441649334043
19520,75914,0,75914,2405.8247170448303,0.0004011222259599184
19620,76314,0,76314,2416.0710949897766,0.0003908954558087201
19720,76714,0,76714,2429.1064398288727,0.00038646913196544954
19820,77114,0,77114,2441.77351975441,0.0003837312889559713
19920,77605,0,77605,2454.6682097911835,0.00037901970647472667
20020,78028,0,78028,2465.947621822357,0.00037337793501585775
20120,78428,0,78428,2477.3179309368134,0.00036709534095047484
20220,78828,0,78828,2488.0166709423065,0.0003592615084853481
20320,79254,0,79254,2498.3813309669495,0.0003540389496825915
20420,79753,0,79753,2508.406221628189,0.00034979435996740707
20521,80245,0,80245,2518.6325948238373,0.0003455421829862938
20621,80645,0,80645,2528.718903064728,0.00034109566144315434
20721,81045,0,81045,2538.859433889389,0.0003370433598572845
20821,81445,0,81445,2549.1613688468933,0.0003328912296929974
20921,81845,0,81845,2559.236934900284,0.00032824005876116324
21021,82245,0,82245,2569.1069428920746,0.0003222839904480631
21121,82645,0,82645,2580.5283436775208,0.0003149735616087853
21221,83045,0,83045,2592.5516879558563,0.0003094166758643336
21321,83445,0,83445,2603.307413816452,0.0003056853573100172
21421,83867,0,83867,2613.49449801445,0.0003035396969177266
21522,84278,0,84278,2623.5829129219055,0.0003002678940075171
21622,84722,0,84722,2633.5474138259888,0.0002972424011706127
21722,85123,0,85123,2643.5911927223206,0.0002927944542119663
21822,85520,0,85520,2653.8582026958466,0.0002886471003959103
21922,85920,0,85920,2663.8333439826965,0.0002842087046260646
22022,86325,0,86325,2674.5096328258514,0.0002801494043541774
22122,86725,0,86725,2684.714166879654,0.0002765273536950806
22222,87127,0,87127,2694.6676077842712,0.00027331854256015955
22322,87527,0,87527,2706.027328014374,0.0002703982739312082
22422,87938,0,87938,2716.852288007736,0.0002671699642845657
22523,88342,0,88342,2727.6057438850403,0.00026393392202295754
22623,88739,0,88739,2737.629264831543,0.00026054968150296783
22723,89083,0,89083,2747.581135749817,0.00025739168438893874
22823,89462,0,89462,2757.754903793335,0.0002546240611557995
22923,89863,0,89863,2767.790071964264,0.00025135567755494404
23023,90278,0,90278,2777.8962817192078,0.0002481322576717506
23123,90678,0,90678,2787.796170949936,0.00024436314245598764
23223,91069,0,91069,2797.9175169467926,0.00023944502471971656
23323,91469,0,91469,2808.1920037269592,0.00023644915138251903
23423,91878,0,91878,2818.3492867946625,0.0002336891765335185
23524,92282,0,92282,2828.6790556907654,0.0002313167001717177
23624,92685,0,92685,2840.067464828491,0.00022747135636723886
23724,93018,0,93018,2851.958416700363,0.00022256793569638532
23824,93415,0,93415,2864.5241808891296,0.0002197736223251733
23924,93874,0,93874,2877.2504897117615,0.00021676343303387948
24024,94281,0,94281,2890.878970861435,0.00021460278266645765
24124,94681,0,94681,2903.4709787368774,0.0002121725598343107
24224,95097,0,95097,2914.8310227394104,0.00020995755189278845
24324,95501,0,95501,2925.0266468524933,0.0002073447719691021
24424,95904,0,95904,2935.1892297267914,0.00020485085406243838
24525,96308,0,96308,2945.5024378299713,0.00020234842124037587
24625,96708,0,96708,2955.6885879039764,0.00019990870849697433
24725,97126,0,97126,2965.9204998016357,0.00019757604451493875
24825,97526,0,97526,2976.485944747925,0.00019519605992010454
24925,97927,0,97927,2987.0093989372253,0.00019278623540830374
25025,98328,0,98328,2997.2754468917847,0.00019027273379862935
25125,98728,0,98728,3007.46142578125,0.00018782146487290562
25225,99136,0,99136,3017.6086568832397,0.00018545885317105474
25325,99536,0,99536,3027.7731597423553,0.00018343074029495042
25425,99936,0,99936,3037.852336883545,0.00018121262467681127
25526,100355,0,100355,3048.353572845459,0.00017885030901587144
25626,100755,0,100755,3058.483521938324,0.00017744250239785196
25726,101155,0,101155,3068.516399860382,0.00017620022457903863
25826,101555,0,101555,3078.8042690753937,0.00017432231954308343
25926,101955,0,101955,3088.941330909729,0.00017235473907902421
26026,102360,0,102360,3099.06387090683,0.0001703375897657138
26126,102760,0,102760,3109.594944000244,0.00016824277805839092
26226,103160,0,103160,3119.785757780075,0.00016613215877260622
26326,103577,0,103577,3129.8505227565765,0.00016417944210684837
26426,103977,0,103977,3140.1339190006256,0.0001621673380239702
26527,104381,0,104381,3150.4823989868164,0.00016014291144940578
26627,104782,0,104782,3161.9972388744354,0.00015807519639960568
26727,105182,0,105182,3172.9561138153076,0.00015596637564836035
26827,105582,0,105582,3184.272752761841,0.00015365815470126724
26927,106003,0,106003,3197.077116727829,0.0001520655123490817
27027,106445,0,106445,3209.068366765976,0.00015073270353364255
27127,106845,0,106845,3221.616997718811,0.00014921545296488274
27227,107251,0,107251,3231.8350188732147,0.00014734865759007267
27327,107658,0,107658,3242.047626018524,0.00014577787942409172
27427,108058,0,108058,3252.392695903778,0.0001442151355241795
27528,108462,0,108462,3262.63801074028,0.00014258573622551632
27628,108862,0,108862,3272.9561710357666,0.00013992986611692052
27728,109262,0,109262,3284.481151819229,0.0001379309281835918
27828,109662,0,109662,3296.6992888450623,0.00013624660496959026
27928,110062,0,110062,3307.9787929058075,0.00013472107999085067
28028,110470,0,110470,3318.666251897812,0.00013307307705188572
28128,110868,0,110868,3328.813841819763,0.00013097885779502112
28228,111268,0,111268,3339.798820734024,0.00012944935322995203
28328,111668,0,111668,3350.0267357826233,0.00012794100022306263
28428,112068,0,112068,3360.3446147441864,0.00012643371187944367
28529,112484,0,112484,3370.85897397995,0.0001251510589176902
28629,112886,0,112886,3381.0274329185486,0.0001237224753678505
28729,113288,0,113288,3391.111303806305,0.00012234700531482272
28829,113688,0,113688,3401.552274942398,0.00012105308878328524
28929,114094,0,114094,3411.7404396533966,0.00011984130612321805
29029,114494,0,114494,3421.843284845352,0.00011831028544112074
29129,114897,0,114897,3432.0412769317627,0.000116863388425639
29229,115297,0,115297,3442.1782598495483,0.0001155090881472452
29329,115697,0,115697,3453.0048887729645,0.00011435749326729027
29429,116104,0,116104,3463.918296813965,0.00011275102387235703
29530,116508,0,116508,3475.3084738254547,0.00011137631688930513
29630,116911,0,116911,3486.5675337314606,0.00010994599303183763
29730,117311,0,117311,3497.7788178920746,0.00010868704086356126
29830,117715,0,117715,3508.458199739456,0.00010749132585568326
29930,118108,0,118108,3518.988511800766,0.00010573523422980514
30030,118470,0,118470,3530.6023547649384,0.00010427149020952374
30130,118902,0,118902,3542.5246357917786,0.00010238439144053656
30230,119328,0,119328,3552.650099992752,0.00010120286543551357
30330,119728,0,119728,3563.0353558063507,0.00010016376256316201
30430,120128,0,120128,3574.745941877365,9.899154154943003e-05
30531,120532,0,120532,3587.2326788902283,9.783412763344362e-05
30631,120932,0,120932,3600.6748719215393,9.670266493882557e-05
30731,121332,0,121332,3611.5405728816986,9.556820637225997e-05
30831,121732,0,121732,3622.702734708786,9.451937675865648e-05
30931,122137,0,122137,3634.2105967998505,9.345792122304126e-05
31031,122537,0,122537,3645.1981859207153,9.224222854676652e-05
31131,122937,0,122937,3657.150510787964,9.089501189611666e-05
31231,123339,0,123339,3671.5934069156647,8.982681197707944e-05
31331,123739,0,123739,3684.3202769756317,8.880867559191539e-05
31431,124139,0,124139,3695.6493859291077,8.782861827264184e-05
31532,124567,0,124567,3707.0144877433777,8.685378806724268e-05
31632,124971,0,124971,3717.607852935791,8.568056820440973e-05
31732,125425,0,125425,3727.92174577713,8.456313465542205e-05
31832,125905,0,125905,3738.064008951187,8.356591233946333e-05
31932,126305,0,126305,3748.341814994812,8.257840044893502e-05
32032,126705,0,126705,3758.713833808899,8.167460515263254e-05
32132,127105,0,127105,3770.195755004883,8.07903865550202e-05
32232,127504,0,127504,3780.9095590114594,7.982945388256612e-05
32332,127904,0,127904,3791.4729838371277,7.887673167716399e-05
32432,128304,0,128304,3801.6878888607025,7.797824808701287e-05
32533,128724,0,128724,3811.8930938243866,7.705514441986566e-05
32633,129124,0,129124,3822.077381849289,7.602862569224201e-05
32733,129524,0,129524,3833.0901918411255,7.517930967801706e-05
32833,129924,0,129924,3844.7061858177185,7.433557134709314e-05
32933,130320,0,130320,3855.539563894272,7.340595561279589e-05
33033,130720,0,130720,3865.6352648735046,7.24778667596786e-05
33133,131120,0,131120,3875.800526857376,7.155545381974582e-05
33233,131537,0,131537,3885.8442759513855,7.078417101927625e-05
33333,131937,0,131937,3896.709077835083,6.999728209802592e-05
33433,132337,0,132337,3907.623962879181,6.93934668221286e-05
33534,132760,0,132760,3917.9817748069763,6.853028539667494e-05
33634,133160,0,133160,3928.254852771759,6.778675541907926e-05
33734,133560,0,133560,3940.9250617027283,6.736134291238419e-05
33834,133966,0,133966,3954.983341693878,6.67157720353266e-05
33934,134366,0,134366,3968.4900019168854,6.602598143685546e-05
34034,134774,0,134774,3980.8073558807373,6.54221366098861e-05
34134,135206,0,135206,3991.9372317790985,6.453727229134149e-05
34234,135617,0,135617,4002.3161787986755,6.396465409845194e-05
34334,136017,0,136017,4013.07923579216,6.320597244996557e-05
34434,136417,0,136417,4025.0460538864136,6.238717770196551e-05
34535,136824,0,136824,4035.7009868621826,6.163485949844837e-05
34635,137224,0,137224,4045.6716380119324,6.091563171089057e-05
34735,137624,0,137624,4055.7392678260803,6.020143165021511e-05
34835,138034,0,138034,4066.73597574234,5.9561336599476496e-05
34935,138434,0,138434,4077.6231570243835,5.892966210536418e-05
35035,138834,0,138834,4087.7863857746124,5.8444390828926566e-05
35135,139234,0,139234,4097.93643283844,5.7903114351401115e-05
35235,139634,0,139634,4108.184392929077,5.714054849741641e-05
35335,140057,0,140057,4119.116251707077,5.6164668673561406e-05
35435,140479,0,140479,4129.350229024887,5.567728491481927e-05
35536,140883,0,140883,4140.04344701767,5.5098798203238274e-05
35636,141283,0,141283,4150.725972890854,5.4577777657216226e-05
35736,141683,0,141683,4161.557512760162,5.393398063107944e-05
35836,142083,0,142083,4172.361981868744,5.328298949773998e-05
35936,142483,0,142483,4182.935382843018,5.2694614917925634e-05
36036,142883,0,142883,4196.078763008118,5.2115032567726434e-05
36136,143283,0,143283,4206.873333930969,5.152686108950694e-05
36236,143683,0,143683,4218.458694934845,5.08969942216297e-05
36336,144083,0,144083,4228.7423667907715,5.0269390135097306e-05
36436,144483,0,144483,4238.797570705414,4.965012760690812e-05
36537,144916,0,144916,4248.8703808784485,4.899587551565599e-05
36637,145316,0,145316,4260.735287904739,4.836202742050014e-05
36737,145732,0,145732,4271.326268911362,4.778087015953832e-05
36837,146193,0,146193,4282.098360776901,4.724512062706605e-05
36937,146655,0,146655,4292.295848846436,4.6840877385218866e-05
37037,147069,0,147069,4302.525901079178,4.639659651361963e-05
37137,147493,0,147493,4312.62343287468,4.588819103869085e-05
37237,147893,0,147893,4322.5288026332855,4.536320075098226e-05
37337,148293,0,148293,4332.695277690887,4.481017225825197e-05
37437,148693,0,148693,4342.5907208919525,4.41078841408741e-05
37538,149097,0,149097,4352.70111489296,4.358566571676771e-05
37638,149497,0,149497,4363.154179811478,4.313335671503863e-05
37738,149919,0,149919,4373.512731790543,4.2716110020942954e-05
37838,150319,0,150319,4383.948361873627,4.2194737723441915e-05
37938,150715,0,150715,4393.886861085892,4.161033947365209e-05
38038,151123,0,151123,4403.9251227378845,4.113552616975659e-05
38138,151523,0,151523,4413.91786980629,4.06857486244519e-05
38238,151923,0,151923,4423.733615875244,4.030817032521562e-05
38338,152330,0,152330,4433.726512908936,3.97464528722631e-05
38438,152738,0,152738,4443.656572818756,3.932924176513749e-05
38539,153145,0,153145,4453.900458812714,3.8934127746041905e-05
38639,153545,0,153545,4463.75693488121,3.839332190384249e-05
38739,153945,0,153945,4474.878427743912,3.784860045309609e-05
38839,154346,0,154346,4486.6213257312775,3.71868576988942e-05
38939,154767,0,154767,4496.968081951141,3.6708971579778275e-05
39039,155171,0,155171,4507.167531013489,3.63115642901297e-05
39139,155571,0,155571,4516.9626569747925,3.5907477202159014e-05
39239,155971,0,155971,4526.734974861145,3.548819613236401e-05
39339,156371,0,156371,4536.79537987709,3.5078287986173454e-05
39439,156789,0,156789,4546.592157840729,3.459846285166222e-05
39540,157193,0,157193,4556.453375816345,3.413088614416957e-05
39640,157593,0,157593,4567.030353784561,3.371303340880087e-05
39740,157993,0,157993,4579.504422903061,3.3268258139279165e-05
39840,158405,0,158405,4589.299461841583,3.271433058919915e-05
39940,158813,0,158813,4599.260725021362,3.2461090072945196e-05
40040,159267,0,159267,4609.4146900177,3.2058850385841914e-05
40140,159667,0,159667,4619.198193788528,3.168800467911144e-05
40240,160071,0,160071,4629.182372808456,3.129020721717123e-05
40340,160471,0,160471,4638.985112667084,3.0928661935873606e-05
40440,160872,0,160872,4649.4882798194885,3.0562911023019355e-05
40541,161276,0,161276,4659.480014801025,3.0187697024666925e-05
40641,161679,0,161679,4669.531934976578,2.9848702079798598e-05
40741,162079,0,162079,4680.510471820831,2.9519568518714734e-05
40841,162479,0,162479,4692.447855710983,2.9175100383889804e-05
40941,162879,0,162879,4703.369692802429,2.882527263320823e-05
41041,163281,0,163281,4714.25435590744,2.851200088929682e-05
41141,163683,0,163683,4725.569247961044,2.8203158722222263e-05
41241,164083,0,164083,4735.730828046799,2.7885697857660244e-05
41341,164490,0,164490,4746.959768772125,2.7575361468084376e-05
41441,164890,0,164890,4758.149640798569,2.729608407853401e-05
41542,165343,0,165343,4769.049248933792,2.706331452754166e-05
41642,165764,0,165764,4780.049454689026,2.6660154793363547e-05
41742,166164,0,166164,4791.22819185257,2.628852459491141e-05
41842,166576,0,166576,4802.465106964111,2.595007146490731e-05
41942,167020,0,167020,4813.324889659882,2.5655526130181784e-05
42042,167420,0,167420,4823.83212685585,2.532965838536584e-05
42142,167820,0,167820,4834.477093696594,2.5031770030239653e-05
42242,168262,0,168262,4845.29097867012,2.4824594205915403e-05
42342,168712,0,168712,4855.489416837692,2.4554693324789405e-05
42442,169112,0,169112,4865.652290821075,2.424994326827886e-05
42543,169516,0,169516,4876.939782857895,2.3946943791369842e-05
42643,169916,0,169916,4887.544286966324,2.368230508305363e-05
42743,170316,0,170316,4897.634063720703,2.3424852048576904e-05
42843,170718,0,170718,4907.549701690674,2.315500117887978e-05
42943,171124,0,171124,4918.015922784805,2.2866906003554736e-05
43043,171524,0,171524,4928.2339408397675,2.261205958635084e-05
43143,171924,0,171924,4939.7607617378235,2.234806716367232e-05
43243,172324,0,172324,4951.0381598472595,2.206940008733229e-05
43343,172752,0,172752,4961.478968858719,2.1830336340416323e-05
43443,173165,0,173165,4972.182922840118,2.156746679860404e-05
43544,173569,0,173569,4982.675860881805,2.1324232292795074e-05
43644,173971,0,173971,4993.014811754227,2.1086319392166087e-05
43744,174371,0,174371,5003.6672167778015,2.0849303813133373e-05
43844,174771,0,174771,5014.8869388103485,2.0618252988014274e-05
43944,175171,0,175171,5025.874874830246,2.0428074471604026e-05
44044,175579,0,175579,5035.892442703247,2.0216628712791705e-05
44144,175979,0,175979,5045.915585041046,2.001200989623607e-05
44244,176379,0,176379,5056.712639808655,1.978816457252913e-05
44344,176780,0,176780,5068.182596683502,1.95670079437613e-05
44444,177180,0,177180,5078.4361798763275,1.9349374272162423e-05
44545,177584,0,177584,5089.130698919296,1.9138829147075982e-05
44645,177989,0,177989,5099.708534955978,1.8971141035306394e-05
44745,178389,0,178389,5111.08406496048,1.8753997904304344e-05
44845,178789,0,178789,5122.096751689911,1.8525506379824143e-05
44945,179186,0,179186,5133.39354968071,1.829022230647906e-05
45045,179587,0,179587,5144.344250679016,1.8091986684099703e-05
45145,179987,0,179987,5154.312718868256,1.7881846006866393e-05
45245,180387,0,180387,5164.798399925232,1.768224702491259e-05
45345,180787,0,180787,5174.792721748352,1.7460532900104204e-05
45445,181187,0,181187,5184.948194742203,1.723242316174815e-05
45546,181591,0,181591,5196.3235738277435,1.7025631880332628e-05
45646,182010,0,182010,5206.863363742828,1.6876316522709253e-05
45746,182451,0,182451,5217.5674369335175,1.6710999324673394e-05
45846,182862,0,182862,5228.484987735748,1.6531766342470556e-05
45946,183262,0,183262,5239.077036857605,1.638838835223355e-05
46046,183662,0,183662,5249.284647941589,1.6250863947252408e-05
46146,184062,0,184062,5259.31104683876,1.611922120852518e-05
46246,184493,0,184493,5269.318282842636,1.5985157267241232e-05
46346,184912,0,184912,5279.40225481987,1.5776588784033497e-05
46446,185394,0,185394,5290.089840888977,1.5569814480015045e-05
46547,185861,0,185861,5300.253712892532,1.530581284839792e-05
46647,186286,0,186286,5310.498909950256,1.50648802651523e-05
46747,186687,0,186687,5320.58917093277,1.4858430871343398e-05
46847,187087,0,187087,5330.54723405838,1.4687276132686402e-05
46947,187487,0,187487,5341.5915858745575,1.4532423666935653e-05
47047,187887,0,187887,5352.701686859131,1.4470956239492378e-05
47147,188287,0,188287,5363.631676912308,1.4238108624375247e-05
47247,188687,0,188687,5374.274030685425,1.3830366697500005e-05
47347,189087,0,189087,5385.685078859329,1.3597156015712433e-05
47447,189487,0,189487,5395.71701669693,1.342528667369465e-05
47548,189892,0,189892,5405.864633798599,1.3258520744842657e-05
47648,190292,0,190292,5416.042627811432,1.3116190288640837e-05
47748,190744,0,190744,5426.035094022751,1.2980172541237682e-05
47848,191194,0,191194,5436.215679883957,1.2788036334922801e-05
47948,191598,0,191598,5448.63534283638,1.2637215632115302e-05
48048,191998,0,191998,5459.430818080902,1.2477754383523048e-05
48148,192398,0,192398,5469.444789886475,1.2299972777150304e-05
48248,192798,0,192798,5479.482694864273,1.2136605585952214e-05
48348,193214,0,193214,5489.866908788681,1.1971081094836657e-05
48448,193614,0,193614,5502.103098869324,1.1844461754963386e-05
48549,194060,0,194060,5512.12437081337,1.171528405790925e-05
48649,194462,0,194462,5522.228287935257,1.1554897354792769e-05
48749,194862,0,194862,5533.769217014313,1.1414597292951774e-05
48849,195265,0,195265,5544.9055688381195,1.125880700614873e-05
48949,195665,0,195665,5555.437716960907,1.1139675995979238e-05
49049,196065,0,196065,5565.4607038497925,1.1020432295072243e-05
49149,196481,0,196481,5575.610279798508,1.0900187352281154e-05
49249,196881,0,196881,5585.649618864059,1.0769889276972745e-05
49349,197281,0,197281,5595.685715913773,1.064627372715248e-05
49449,197681,0,197681,5606.304788827896,1.0525563523899414e-05
49550,198085,0,198085,5616.7632439136505,1.042187113519763e-05
49650,198537,0,198537,5626.851796865463,1.0313348509871162e-05
49750,198943,0,198943,5636.912987709045,1.0186057078732708e-05
49850,199343,0,199343,5647.164335727692,1.0083348773931497e-05
49950,199743,0,199743,5657.734130859375,9.980630424658256e-06
50050,200143,0,200143,5668.735941886902,9.888773482690802e-06
50150,200561,0,200561,5679.965418815613,9.804023609915965e-06
50250,201024,0,201024,5690.150532722473,9.682444694856837e-06
50350,201445,0,201445,5700.1978487968445,9.581215447898793e-06
50450,201845,0,201845,5710.442479848862,9.465698092260571e-06
50551,202311,0,202311,5720.719299793243,9.35394046232098e-06
50651,202736,0,202736,5730.787453889847,9.306934794413667e-06
50751,203147,0,203147,5741.022821903229,9.231362089064466e-06
50851,203551,0,203551,5752.605818748474,9.113591110249482e-06
50951,203951,0,203951,5763.109275817871,9.007051101234301e-06
51051,204351,0,204351,5773.987378835678,8.902272761549182e-06
51151,204753,0,204753,5784.817870855331,8.799943891521851e-06
51251,205153,0,205153,5794.966627836227,8.69876722801585e-06
51351,205553,0,205553,5805.464652061462,8.596302981169532e-06
51451,205955,0,205955,5817.167312860489,8.495105583119697e-06
51552,206359,0,206359,5828.283645868301,8.399346704903733e-06
51652,206769,0,206769,5839.159593820572,8.314394151670704e-06
51752,207188,0,207188,5849.95116186142,8.214676671364452e-06
51852,207616,0,207616,5860.731780767441,8.1229090312935e-06
51952,208016,0,208016,5871.957078933716,8.02623165788817e-06
52052,208416,0,208416,5883.588018894196,7.934131364352607e-06
52152,208820,0,208820,5894.94437289238,7.843330498326725e-06
52252,209220,0,209220,5906.955757856369,7.750954060909387e-06
52352,209620,0,209620,5917.639263868332,7.665023734343951e-06
52452,210035,0,210035,5928.709703922272,7.593378375188449e-06
52553,210441,0,210441,5940.192176818848,7.4942685379516696e-06
52653,210841,0,210841,5951.48242688179,7.40790571840286e-06
52753,211251,0,211251,5963.860898017883,7.33135323530711e-06
52853,211651,0,211651,5975.599026918411,7.244134373062369e-06
52953,212051,0,212051,5987.012977838516,7.168177194264008e-06
53053,212466,0,212466,5998.409687757492,7.113549694973732e-06
53153,212878,0,212878,6009.582151889801,7.026998430259692e-06
53253,213278,0,213278,6020.208327770233,6.9467247210828205e-06
53353,213678,0,213678,6030.79859995842,6.870113439326289e-06
53453,214078,0,214078,6041.498998880386,6.7959071784617575e-06
53554,214484,0,214484,6052.552349805832,6.723883966941916e-06
53654,214884,0,214884,6063.074895858765,6.6492067379089875e-06
53754,215291,0,215291,6073.579252958298,6.5721755472975515e-06
53854,215690,0,215690,6083.956429004669,6.495893647372448e-06
53954,216090,0,216090,6094.240772724152,6.423023420075878e-06
54054,216490,0,216490,6104.384328842163,6.352718985421361e-06
54154,216928,0,216928,6114.748403787613,6.288196511592228e-06
54254,217330,0,217330,6125.165185928345,6.216683548407225e-06
54354,217740,0,217740,6135.669550657272,6.121262803207672e-06
54454,218160,0,218160,6146.052115917206,6.082028683836774e-06
54555,218564,0,218564,6156.599954843521,6.0399517114100855e-06
54655,218964,0,218964,6168.407337903976,5.988628870417393e-06
54755,219398,0,219398,6178.977984905243,5.927141694345715e-06
54855,219816,0,219816,6189.519851922989,5.827774635370873e-06
54955,220216,0,220216,6201.0712077617645,5.737545491409928e-06
55055,220616,0,220616,6211.939050912857,5.6389711550402334e-06
55155,221021,0,221021,6224.002977848053,5.548474276971407e-06
55255,221421,0,221421,6234.610040664673,5.493797967710033e-06
55355,221821,0,221821,6245.74210691452,5.439645830606562e-06
55455,222237,0,222237,6256.538938760757,5.380789089292857e-06
55556,222641,0,222641,6267.344523906708,5.313852258092505e-06
55656,223041,0,223041,6278.137974977493,5.2500186030035825e-06
55756,223441,0,223441,6289.188262939453,5.1881383030339805e-06
55856,223841,0,223841,6299.9364647865295,5.129711487413517e-06
55956,224241,0,224241,6309.912473678589,5.073067050438757e-06
56056,224648,0,224648,6319.856200933456,5.016830084648336e-06
56156,225048,0,225048,6329.745715856552,4.960453306234759e-06
56256,225448,0,225448,6339.912431716919,4.903677984941614e-06
56356,225848,0,225848,6350.583124876022,4.85097982085289e-06
56456,226290,0,226290,6361.1688277721405,4.79741280558138e-06
56557,226709,0,226709,6373.889014005661,4.730011937986839e-06
56657,227126,0,227126,6386.898291826248,4.689971952161236e-06
56757,227526,0,227526,6398.329894781113,4.647048172052899e-06
56857,227926,0,227926,6409.246228933334,4.59694095657292e-06
56957,228326,0,228326,6419.943177938461,4.547556612461091e-06
57057,228726,0,228726,6429.844078779221,4.5128033713149055e-06
57157,229150,0,229150,6439.95091676712,4.4533364064090605e-06
57257,229550,0,229550,6451.639367818832,4.3973023300702936e-06
57357,229950,0,229950,6462.413186073303,4.347810297784083e-06
57457,230373,0,230373,6472.433758974075,4.304443452209902e-06
57558,230777,0,230777,6482.479736089706,4.268014115320721e-06
57658,231200,0,231200,6492.521454811096,4.216705319764031e-06
57758,231600,0,231600,6503.987907648087,4.167996597655336e-06
57858,232000,0,232000,6514.406795978546,4.1226949198811136e-06
57958,232400,0,232400,6524.448867797852,4.078679981304765e-06
58058,232800,0,232800,6534.88875079155,4.035813166370459e-06
58158,233210,0,233210,6545.798992872238,3.992801917373896e-06
58258,233610,0,233610,6557.050982713699,3.943799626549921e-06
58358,234019,0,234019,6567.040434837341,3.897027019152542e-06
58458,234419,0,234419,6578.073345899582,3.855001292252268e-06
58559,234823,0,234823,6589.431523799896,3.8132994025712006e-06
58659,235223,0,235223,6603.872560739517,3.774602791944578e-06
58759,235650,0,235650,6615.565088033676,3.739124529237241e-06
58859,236050,0,236050,6628.239198923111,3.693208533509167e-06
58959,236450,0,236450,6639.196997880936,3.6500253698180134e-06
59059,236855,0,236855,6649.345595836639,3.6092819017486706e-06
59159,237255,0,237255,6659.30327296257,3.5712072976781485e-06
59259,237655,0,237655,6669.114847898483,3.535824461703461e-06
59359,238079,0,238079,6679.057107925415,3.5094123836806934e-06
59459,238486,0,238486,6690.341347694397,3.460350696653848e-06
59560,238890,0,238890,6701.551258802414,3.4172713765374545e-06
59660,239290,0,239290,6711.54962182045,3.3788963853607173e-06
59760,239716,0,239716,6721.513408899307,3.344416751750773e-06
59860,240116,0,240116,6731.665677785873,3.308377530628277e-06
59960,240516,0,240516,6741.886015892029,3.274083711519252e-06
60060,240941,0,240941,6751.941395998001,3.2399277962230358e-06
60160,241341,0,241341,6762.607656955719,3.2022356680261435e-06
60260,241741,0,241741,6774.9292578697205,3.166124679701199e-06
60360,242141,0,242141,6785.641284704208,3.1308050751517447e-06
60460,242544,0,242544,6795.748785734177,3.0978318385399927e-06
60561,242955,0,242955,6806.00492477417,3.061141955773735e-06
60661,243357,0,243357,6815.982434749603,3.026342263944977e-06
60761,243757,0,243757,6826.462989807129,2.993669256996373e-06
60861,244157,0,244157,6836.800254821777,2.9598728633145336e-06
60961,244557,0,244557,6846.862382650375,2.9269927671491856e-06
61061,244971,0,244971,6856.974760770798,2.9008338717312994e-06
61161,245392,0,245392,6867.0651977062225,2.866866387957142e-06
61261,245812,0,245812,6878.759229898453,2.8345821190155197e-06
61361,246263,0,246263,6889.680304765701,2.798538181405236e-06
61461,246720,0,246720,6901.035206794739,2.7749687384301106e-06
61562,247192,0,247192,6912.522010803223,2.7419974410638376e-06
61662,247614,0,247614,6923.924127817154,2.7071891868517793e-06
61762,248014,0,248014,6935.175519943237,2.6747138328648107e-06
61862,248414,0,248414,6946.560245990753,2.64419654839792e-06
61962,248814,0,248814,6956.7614488601685,2.6139010502765676e-06
62062,249214,0,249214,6966.744277954102,2.58320113449307e-06
62162,249614,0,249614,6980.967495918274,2.5623865649745302e-06
62262,250017,0,250017,6991.685698747635,2.5313798309933523e-06
62362,250417,0,250417,7130.561433792114,2.50325161168091e-06
62462,250817,0,250817,7144.060402870178,2.4760799122340626e-06
62563,251221,0,251221,7155.007926940918,2.4505143242134578e-06
62663,251653,0,251653,7165.424834012985,2.4272100381258585e-06
62763,252056,0,252056,7176.063416719437,2.398698182750731e-06
62863,252458,0,252458,7185.893605709076,2.3712131526833173e-06
62963,252859,0,252859,7195.947855710983,2.3486279402466145e-06
63063,253259,0,253259,7206.729133844376,2.3240627763563196e-06
63163,253659,0,253659,7220.108228683472,2.2993386098569537e-06
63263,254060,0,254060,7230.194826841354,2.276323700992765e-06
63363,254543,0,254543,7241.748633861542,2.2529113228515458e-06
63463,254957,0,254957,7253.03680896759,2.232512906693952e-06
63564,255362,0,255362,7266.5976939201355,2.2089413419983377e-06
63664,255778,0,255778,7279.514303922653,2.1873171095272813e-06
63764,256178,0,256178,7290.438591003418,2.1648694720531835e-06
63864,256578,0,256578,7300.657102823257,2.1422366969407022e-06
63964,256978,0,256978,7310.928555011749,2.1170639269188167e-06
64064,257408,0,257408,7320.9234828948975,2.0943110712389345e-06
64164,257808,0,257808,7330.89550280571,2.0726780639948353e-06
64264,258208,0,258208,7340.797921895981,2.04850974175818e-06
64364,258616,0,258616,7350.848154783249,2.024432043531637e-06
64464,259016,0,259016,7364.275927782059,2.0007855480485393e-06
64565,259420,0,259420,7377.339048862457,1.974744178672659e-06
64665,259844,0,259844,7390.293400764465,1.9507496269949372e-06
64765,260244,0,260244,7401.330806970596,1.930336787223596e-06
64865,260644,0,260644,7415.548991918564,1.910082060219956e-06
64965,261044,0,261044,7426.118906736374,1.8904970211509851e-06
65065,261447,0,261447,7437.03723692894,1.876005256229634e-06
65165,261878,0,261878,7447.495055675507,1.8538447316420386e-06
65265,262278,0,262278,7458.0891127586365,1.8336837005698339e-06
65365,262696,0,262696,7468.440954685211,1.8151394535474332e-06
65465,263096,0,263096,7478.9291298389435,1.7971553648884543e-06
65566,263500,0,263500,7489.011496782303,1.7806875709085267e-06
65666,263918,0,263918,7498.96933889389,1.7669135680824723e-06
65766,264331,0,264331,7510.030032873154,1.744163940637864e-06
65866,264731,0,264731,7519.963414907455,1.7237721992891986e-06
65966,265130,0,265130,7530.952185869217,1.7036444515446634e-06
66066,265536,0,265536,7541.562170743942,1.6843442642963872e-06
66166,265949,0,265949,7551.472735881805,1.6668151650154212e-06
66266,266377,0,266377,7561.252680778503,1.6518713371833432e-06
66366,266788,0,266788,7572.763526916504,1.6281155395410053e-06
66466,267188,0,267188,7582.582846879959,1.6075401053360116e-06
66567,267592,0,267592,7593.745565891266,1.5885363300896434e-06
66667,267992,0,267992,7604.767908811569,1.5712863993797225e-06
66767,268393,0,268393,7689.023098707199,1.555194061089775e-06
66867,268793,0,268793,7727.548644781113,1.5396609228738053e-06
66967,269197,0,269197,7765.137663841248,1.5240343036482317e-06
67067,269597,0,269597,7786.671293973923,1.5070412711410389e-06
67167,269997,0,269997,13520.848861932755,1.49084890704183e-06
67267,270397,0,270397,13536.916369915009,1.4754826628343498e-06
67367,270797,0,270797,13553.955519914627,1.4611579781155318e-06
67467,271231,0,271231,13569.34403681755,1.4458233604153994e-06
67568,271700,0,271700,13582.381492853165,1.4287637620475838e-06
67668,272100,0,272100,13593.752383947372,1.4177748333950488e-06
67768,272500,0,272500,13605.308815717697,1.4049215332131361e-06
67868,272900,0,272900,13617.487741947174,1.392096204809855e-06
67968,273300,0,273300,13628.88274884224,1.3790095081733934e-06
68068,273728,0,273728,13642.253819704056,1.3669564816260645e-06
68168,274134,0,274134,13657.66178202629,1.3505213695926098e-06
68268,274534,0,274534,13673.149640798569,1.3342109382112987e-06
68368,274995,0,274995,13688.408628940582,1.3180577277775576e-06
68468,275442,0,275442,13705.88222694397,1.3074120288244478e-06
68569,275851,0,275851,13725.300395965576,1.2999680212634706e-06
68669,276269,0,276269,13744.52787399292,1.2836178587190838e-06
68769,276669,0,276669,13758.534643888474,1.268964885444587e-06
68869,277069,0,277069,13771.22844696045,1.2543004083205812e-06
68969,277469,0,277469,13784.803527832031,1.2398659073653343e-06
69069,277881,0,277881,13797.879735946655,1.2264720414525902e-06
69169,278284,0,278284,13811.065168857574,1.2092716782662362e-06
69269,278703,0,278703,13825.623783826828,1.1974524783488282e-06
69369,279103,0,279103,13838.348809957504,1.184253505406977e-06
69469,279503,0,279503,13851.021616697311,1.1712390022266077e-06
69570,279907,0,279907,13862.672761678696,1.1593639503684127e-06
69670,280345,0,280345,13873.935953855515,1.1487286153379232e-06
69770,280759,0,280759,13885.218297719955,1.1344217395285738e-06
69870,281159,0,281159,13897.184917926788,1.1212149625672243e-06
69970,281559,0,281559,13911.443629741669,1.1080076491003522e-06
70070,281960,0,281960,13926.943417787552,1.0961625287842646e-06
70170,282360,0,282360,13942.243999958038,1.0846008796971656e-06
70270,282760,0,282760,13955.086726903915,1.0746970309398854e-06
70370,283187,0,283187,13967.901709079742,1.0620794082976127e-06
70470,283587,0,283587,13980.773181915283,1.0493442228658675e-06
70571,283991,0,283991,13992.7038667202,1.0375099782643808e-06
70671,284392,0,284392,14005.466857910156,1.0248599846607567e-06
70771,284792,0,284792,14019.3892557621,1.014312930603419e-06
70871,285192,0,285192,14030.500526666641,1.0037112377102884e-06
70971,285610,0,285610,14041.964143753052,9.934929753541923e-07
71071,286010,0,286010,14054.321960926056,9.822915458035683e-07
71171,286410,0,286410,14068.522819757462,9.714335854496573e-07
71271,286810,0,286810,14082.440248012543,9.607674601155528e-07
71371,287210,0,287210,14094.670219898224,9.503172500976728e-07
71471,287610,0,287610,14106.438518047333,9.404897529081387e-07
71572,288014,0,288014,14119.649853944778,9.311205670874974e-07
71672,288414,0,288414,14132.96973490715,9.220211514355736e-07
71772,288814,0,288814,14145.083048820496,9.126129770836336e-07
71872,289214,0,289214,14158.40751695633,9.032076703395716e-07
71972,289614,0,289614,14170.334521770477,8.942279281489675e-07
72072,290015,0,290015,14182.575288057327,8.87471195931216e-07
72172,290515,0,290515,14194.954794883728,8.773176528154345e-07
72272,290947,0,290947,14208.546563863754,8.655670815112437e-07
72372,291428,0,291428,14222.928004741669,8.549343884997848e-07
72472,291849,0,291849,14235.797130823135,8.479533777361922e-07
72573,292253,0,292253,14252.268322706223,8.418179992999328e-07
72673,292698,0,292698,14265.629841804504,8.350570126896555e-07
72773,293117,0,293117,14280.819965839386,8.242434816989671e-07
72873,293514,0,293514,14295.005631923676,8.139683184143849e-07
72973,293914,0,293914,14309.32589006424,8.045617516330923e-07
73073,294314,0,294314,14323.935647964478,7.952322657820172e-07
73173,294714,0,294714,14338.203241825104,7.858214065760654e-07
73273,295114,0,295114,14352.457570075989,7.767373945643967e-07
73373,295514,0,295514,14368.482233762741,7.678185060952507e-07
73473,295914,0,295914,14383.405756950378,7.594382372447948e-07
73574,296318,0,296318,14397.946604013443,7.514702004921488e-07
73674,296718,0,296718,14412.02955698967,7.437714201643554e-07
73774,297138,0,297138,14426.891326904297,7.353525296978136e-07
73874,297541,0,297541,14441.375842809677,7.263531540251491e-07
73974,297969,0,297969,14457.22301697731,7.191228186840203e-07
74074,298369,0,298369,14475.915849924088,7.120889985653659e-07
74174,298769,0,298769,14494.93766093254,7.0553340125369e-07
74274,299169,0,299169,14513.349521875381,7.007026550264617e-07
74374,299624,0,299624,14527.48746085167,6.939705682312843e-07
74474,300031,0,300031,14543.621475696564,6.855232692009365e-07
74575,300435,0,300435,14558.459505796432,6.774329822591194e-07
74675,300837,0,300837,14573.223762750626,6.697861440130672e-07
74775,301237,0,301237,14588.678036928177,6.629175666633251e-07
74875,301637,0,301637,14608.348542928696,6.558758916042579e-07
74975,302041,0,302041,14630.481372833252,6.498660706007343e-07
75075,302462,0,302462,14651.259255886078,6.417244851779826e-07
75175,302862,0,302862,14670.681910037994,6.346398648875173e-07
75275,303262,0,303262,14693.138034820557,6.273273656076201e-07
75375,303662,0,303662,14706.855571985245,6.194985338664273e-07
75475,304064,0,304064,14719.816530942917,6.13419376632122e-07
75576,304496,0,304496,14732.505197763443,6.075625611295174e-07
75676,304901,0,304901,14745.017341852188,6.002225062382942e-07
75776,305301,0,305301,14757.829218626022,5.934851523102857e-07
75876,305701,0,305701,14774.6754758358,5.867866997059162e-07
75976,306101,0,306101,14790.541660785675,5.800908044501054e-07
76076,306501,0,306501,14807.441243886948,5.73919536913779e-07
76176,306950,0,306950,14823.933819770813,5.678116931486469e-07
76276,307434,0,307434,14840.250585794449,5.612638310598383e-07
76376,307865,0,307865,14857.061288833618,5.560733937588856e-07
76476,308265,0,308265,14873.82907485962,5.501119444480241e-07
76577,308669,0,308669,14890.514155864716,5.442978147499882e-07
76677,309069,0,309069,14906.996808767319,5.402596204110269e-07
76777,309518,0,309518,14924.000007867813,5.346879130915806e-07
76877,309926,0,309926,14940.519862890244,5.278699462468655e-07
76977,310326,0,310326,14957.031074047089,5.218951092492117e-07
77077,310726,0,310726,14973.550788879395,5.158469368598607e-07
77177,311130,0,311130,14990.335552930832,5.088374433608189e-07
77277,311541,0,311541,15006.907369852066,5.035118510622414e-07
77377,311945,0,311945,15023.258351802826,4.977021864274098e-07
77477,312345,0,312345,15039.512373924255,4.916639482090588e-07
77578,312749,0,312749,15056.167650699615,4.854509161007306e-07
77678,313149,0,313149,15072.95151591301,4.797117836780916e-07
77778,313549,0,313549,15088.963807821274,4.7428393513668223e-07
77878,313957,0,313957,15105.553271055222,4.6897264606878285e-07
77978,314357,0,314357,15122.103750944138,4.6413865153820304e-07
78078,314770,0,314770,15138.665925741196,4.5914903812422647e-07
78178,315170,0,315170,15154.932953834534,4.5414992110568997e-07
78278,315570,0,315570,15171.452276945114,4.4943835264549854e-07
78378,315988,0,315988,15187.96973991394,4.4499629192246506e-07
78478,316407,0,316407,15204.842444896698,4.3949225538393664e-07
78579,316878,0,316878,15221.982729911804,4.345183240074859e-07
78679,317282,0,317282,15239.508748054504,4.303521129268585e-07
78779,317683,0,317683,15256.003060817719,4.2574616101850916e-07
78879,318083,0,318083,15273.175028800964,4.21505218328016e-07
78979,318483,0,318483,15289.970846891403,4.173612784536854e-07
79079,318892,0,318892,15307.035054683685,4.1443764543620156e-07
79179,319337,0,319337,15323.880649805069,4.094211563940876e-07
79279,319739,0,319739,15340.597425937653,4.038078363650969e-07
79379,320182,0,320182,15357.499654769897,3.9902838209812533e-07
79479,320664,0,320664,15374.752733945847,3.9448349885476335e-07
79580,321102,0,321102,15392.51977968216,3.891285586136519e-07
79680,321507,0,321507,15410.16709971428,3.84089359355555e-07
79780,321907,0,321907,15426.948192834854,3.797560853945233e-07
79880,322307,0,322307,15443.900880813599,3.756121146322568e-07
79980,322707,0,322707,15460.600098848343,3.715657574812282e-07
80080,323107,0,323107,15477.9101998806,3.6767188433199283e-07
80180,323507,0,323507,15494.746936798096,3.6392048599851405e-07
80280,323907,0,323907,15511.463689804077,3.602224026294866e-07
80380,324307,0,324307,15528.675112962723,3.564930832136617e-07
80480,324707,0,324707,15545.68844795227,3.528303165499225e-07
80581,325111,0,325111,15563.515948057175,3.4924023064370487e-07
80681,325524,0,325524,15580.531557798386,3.4636115532735223e-07
80781,325954,0,325954,15597.711624860764,3.422439203479064e-07
80881,326354,0,326354,15614.396297931671,3.3789223370687146e-07
80981,326763,0,326763,15630.945016860962,3.335605072101008e-07
81081,327201,0,327201,15647.489248991013,3.3075578551367555e-07
81181,327601,0,327601,15664.085426807404,3.2838897827818514e-07
81281,328019,0,328019,15681.095537900925,3.2608050332692496e-07
81381,328439,0,328439,15697.12857580185,3.2189219070497296e-07
81481,328839,0,328839,15713.816102743149,3.1807258685682894e-07
81582,329243,0,329243,15730.892192840576,3.14409486510509e-07
81682,329643,0,329643,15747.568557739258,3.1066246421252924e-07
81782,330051,0,330051,15764.288004875183,3.074906172809023e-07
81882,330451,0,330451,15780.870626688004,3.04441798144283e-07
81982,330855,0,330855,15797.601193904877,3.0202495326455546e-07
82082,331279,0,331279,15814.234801769257,2.9846763208428665e-07
82182,331676,0,331676,15831.199179887772,2.94995138107707e-07
82282,332076,0,332076,15848.009873867035,2.918066030655304e-07
82382,332476,0,332476,15864.786816835403,2.8876057885118127e-07
82482,332882,0,332882,15881.775674819946,2.860998905169654e-07
82583,333298,0,333298,15898.745918989182,2.827582593916247e-07
82683,333699,0,333699,15915.604249715805,2.7977353284147384e-07
82783,334099,0,334099,15932.408201932907,2.765792351863162e-07
82883,334499,0,334499,15949.421532869339,2.7360545274271834e-07
82983,334899,0,334899,15966.025629758835,2.7054016602564795e-07
83083,335299,0,335299,15982.772310972214,2.6798631277379294e-07
83183,335757,0,335757,15999.643648862839,2.6523193443771547e-07
83283,336250,0,336250,16016.479781866074,2.621573813908726e-07
83383,336745,0,336745,16033.590453863144,2.590850120427256e-07
83483,337241,0,337241,16050.816306829453,2.562374233320243e-07
83584,337736,0,337736,16068.222395896912,2.53458372030281e-07
83684,338215,0,338215,16085.04884505272,2.506637856501577e-07
83784,338696,0,338696,16101.972738742828,2.4784400479645475e-07
83884,339097,0,339097,16118.709660768509,2.448674848434284e-07
83984,339525,0,339525,16135.287276029587,2.418252576458208e-07
84084,339925,0,339925,16151.915331840515,2.3867454824098213e-07
84184,340325,0,340325,16169.202194929123,2.359511116835448e-07
84284,340734,0,340734,16185.988778829575,2.3328835527590855e-07
84384,341134,0,341134,16202.230846881866,2.3076378069014194e-07
84484,341534,0,341534,16218.659557819366,2.2837747000064633e-07
84585,341938,0,341938,16236.057975053787,2.2591220803122445e-07
84685,342377,0,342377,16252.586108922958,2.2396951318741884e-07
84785,342877,0,342877,16267.785552740097,2.2149524486498983e-07
84885,343380,0,343380,16284.205383777618,2.1899449686308108e-07
84985,343832,0,343832,16300.064196825027,2.1713427169819043e-07
85085,344248,0,344248,16316.123724937439,2.154409562675113e-07
85185,344706,0,344706,16332.763937950134,2.1353890787340823e-07
85285,345200,0,345200,16349.411043643951,2.1114031245006489e-07
85385,345640,0,345640,16366.239155769348,2.0874209721395754e-07
85485,346040,0,346040,16383.222201824188,2.0637902316607376e-07
85586,346444,0,346444,16400.042165994644,2.046094066943201e-07
85686,346859,0,346859,16416.112982034683,2.028735283106159e-07
85786,347264,0,347264,16432.788405895233,2.0103497378850287e-07
85886,347664,0,347664,16449.090122938156,1.9961059726473524e-07
85986,348086,0,348086,16466.05198574066,1.9806146225771726e-07
86086,348505,0,348505,16482.262558937073,1.9561544431576993e-07
86186,348905,0,348905,16499.094829797745,1.930673473588112e-07
86286,349305,0,349305,16516.336216688156,1.9083836136289953e-07
86386,349709,0,349709,16534.15461587906,1.8873195617643762e-07
86486,350109,0,350109,16551.135371923447,1.8710201358036535e-07
86587,350519,0,350519,16568.91496706009,1.8539982823435127e-07
86687,350919,0,350919,16586.203938007355,1.8326534947126e-07
86787,351319,0,351319,16603.823423862457,1.8118767333990246e-07
86887,351719,0,351719,16620.884287834167,1.7917378827190804e-07
86987,352119,0,352119,16638.07405781746,1.7732601758255137e-07
87087,352519,0,352519,16655.144119024277,1.7538805637834614e-07
87187,352985,0,352985,16672.50740671158,1.737603785673645e-07
87287,353440,0,353440,16689.468461036682,1.7221584895567955e-07
87387,353863,0,353863,16706.5229036808,1.707209838437113e-07
87487,354263,0,354263,16723.08661198616,1.6902631863167814e-07
87588,354667,0,354667,16740.323824882507,1.6728170094151757e-07
87688,355067,0,355067,16757.690091848373,1.657573651539669e-07
87788,355514,0,355514,16776.09467983246,1.6427934822956142e-07
87888,355945,0,355945,16793.92746067047,1.627308768062199e-07
87988,356351,0,356351,16811.043840885162,1.6110324294089615e-07
88088,356751,0,356751,16828.059235811234,1.5924636943165983e-07
88188,357151,0,357151,16845.4700217247,1.5731866937904354e-07
88288,357568,0,357568,16862.34520292282,1.5539723384327008e-07
88388,357971,0,357971,16880.007618665695,1.5398715530114612e-07
88488,358371,0,358371,16898.052629947662,1.5217727109014406e-07
88589,358775,0,358775,16915.517234802246,1.5038642783770023e-07
88689,359175,0,359175,16932.700761795044,1.4863392079053175e-07
88789,359575,0,359575,16949.62714290619,1.4709615472948048e-07
88889,359977,0,359977,16966.819042682648,1.455396173100678e-07
88989,360382,0,360382,16984.018115758896,1.439819304890888e-07
89089,360787,0,360787,17001.55196595192,1.4228767331729662e-07
89189,361187,0,361187,17019.219342708588,1.4066312597793106e-07
89289,361587,0,361587,17036.408198833466,1.3916439167062391e-07
89389,361987,0,361987,17054.144582748413,1.379253727489247e-07
89489,362387,0,362387,17071.531824827194,1.368161311848869e-07
89590,362804,0,362804,17088.654189825058,1.353605519336311e-07
89690,363256,0,363256,17105.430329799652,1.3387712132779978e-07
89790,363701,0,363701,17123.17912697792,1.327709024862888e-07
89890,364114,0,364114,17140.46694779396,1.3150209759042126e-07
89990,364532,0,364532,17157.56935596466,1.3032675377304123e-07
90090,364934,0,364934,17174.648664712906,1.29400077243808e-07
90190,365334,0,365334,17192.081341981888,1.279356217571168e-07
90290,365748,0,365748,17209.251225709915,1.2707389063520447e-07
90390,366181,0,366181,17226.056595802307,1.259065728011688e-07
90490,366581,0,366581,17242.819936037064,1.2493621866819186e-07
90591,367002,0,367002,17261.044704914093,1.2399903018416328e-07
90691,367433,0,367433,17278.481316804886,1.2326620963531135e-07
90791,367833,0,367833,17295.92996096611,1.2243363673608862e-07
90891,368238,0,368238,17312.655117750168,1.2102962702048405e-07
90991,368640,0,368640,17329.281161785126,1.1976138359055542e-07
91091,369041,0,369041,17345.455058813095,1.1822056662051088e-07
91191,369443,0,369443,17361.95388174057,1.1689271676808044e-07
91291,369861,0,369861,17379.132032871246,1.1537227964015238e-07
91391,370264,0,370264,17396.153426885605,1.1392061361549021e-07
91491,370684,0,370684,17412.776926994324,1.1264337098703756e-07
91592,371108,0,371108,17429.691930770874,1.1149437938877706e-07
91692,371535,0,371535,17446.73506784439,1.1039117110305343e-07
91792,371944,0,371944,17463.094883680344,1.0890570621879834e-07
91892,372344,0,372344,17479.03117275238,1.0729389654525857e-07
91992,372744,0,372744,17496.186893701553,1.05738724185194e-07
92092,373144,0,373144,17512.594274044037,1.0456754405039415e-07
92192,373544,0,373544,17529.171110868454,1.028736637099955e-07
92292,373960,0,373960,17546.419762849808,1.0163406373658878e-07
92392,374360,0,374360,17564.352607011795,1.0030289196989211e-07
92492,374760,0,374760,17582.7334856987,9.897487515309336e-08
92593,375164,0,375164,17599.372788906097,9.783715943127147e-08
92693,375564,0,375564,17617.12578368187,9.667751589724215e-08
92793,375966,0,375966,17634.536660909653,9.560029585819874e-08
92893,376371,0,376371,17651.800632715225,9.455122189411496e-08
92993,376771,0,376771,17668.337813854218,9.337249570503426e-08
93093,377171,0,377171,17681.81037592888,9.22761964931805e-08
93193,377571,0,377571,17695.392057657242,9.122577444106852e-08
93293,377971,0,377971,17708.77663588524,9.020938987365484e-08
93393,378384,0,378384,17722.003447055817,8.920535041894006e-08
93493,378788,0,378788,17735.109533786774,8.831238772031648e-08
93594,379194,0,379194,17748.75566482544,8.73212530230848e-08
93694,379594,0,379594,17762.190478801727,8.637855423286896e-08
93794,379994,0,379994,17775.79851269722,8.536823367375284e-08
93894,380394,0,380394,17789.278181791306,8.436178907311676e-08
93994,380794,0,380794,17805.15885591507,8.340601180925517e-08
94094,381194,0,381194,17821.749264717102,8.231095117754788e-08
94194,381615,0,381615,17835.33438181877,8.105766452754393e-08
94294,382113,0,382113,17848.44676876068,8.013904983480435e-08
94394,382601,0,382601,17861.709520816803,7.93252911613184e-08
94494,383004,0,383004,17875.14972281456,7.875180334942952e-08
94595,383408,0,383408,17888.945774793625,7.826334029299435e-08
94695,383840,0,383840,17902.4111058712,7.775483079943193e-08
94795,384280,0,384280,17916.2815618515,7.679651502061278e-08
94895,384694,0,384694,17929.83689069748,7.596205631416066e-08
94995,385126,0,385126,17943.207675933838,7.546981869082434e-08
95095,385526,0,385526,17956.707291841507,7.472680046823974e-08
95195,385926,0,385926,17969.968990802765,7.388964166495848e-08
95295,386406,0,386406,17985.697425842285,7.307055152554242e-08
95395,386817,0,386817,17996.419474840164,7.201780177284061e-08
95495,387220,0,387220,18007.262611865997,7.102241643398086e-08
95596,387624,0,387624,18018.515835762024,7.035566402068843e-08
95696,388024,0,388024,18031.36367583275,6.978037938714585e-08
95796,388432,0,388432,18043.81618285179,6.933841058515675e-08
95896,388856,0,388856,18057.566844940186,6.876210875288444e-08
95996,389256,0,389256,18068.235913991928,6.810695865575518e-08
96096,389656,0,389656,18079.848688840866,6.753140383169205e-08
96196,390056,0,390056,18092.22718477249,6.70249430207126e-08
96296,390500,0,390500,18105.638551712036,6.639047896165022e-08
96396,390905,0,390905,18116.820812940598,6.585455484940558e-08
96496,391305,0,391305,18128.1346449852,6.515855170302506e-08
96597,391709,0,391709,18146.03696680069,6.464788551669323e-08
96697,392109,0,392109,18161.011561870575,6.417162443421299e-08
96797,392535,0,392535,18174.816218852997,6.354100933537149e-08
96897,392935,0,392935,18188.594550848007,6.286098475133281e-08
96997,393335,0,393335,18202.861769914627,6.206026187324512e-08
97097,393735,0,393735,18216.9926776886,6.133779357180541e-08
97197,394135,0,394135,18229.39980006218,6.060462598415631e-08
97297,394535,0,394535,18245.975040912628,5.975711297133548e-08
97397,394995,0,394995,18258.029283761978,5.912935533763928e-08
97497,395395,0,395395,18269.730046987534,5.840521111852311e-08
97598,395799,0,395799,18281.18526005745,5.7663745639994564e-08
97698,396199,0,396199,18292.800553798676,5.696699191693378e-08
97798,396599,0,396599,18304.58425593376,5.6319752510952725e-08
97898,396999,0,396999,18316.264544010162,5.5671567286123847e-08
97998,397399,0,397399,18329.473797798157,5.501351813452079e-08
98098,397799,0,397799,18343.167600870132,5.456995590938496e-08
98198,398199,0,398199,18359.76096892357,5.420247371377915e-08
98298,398599,0,398599,18372.703540802002,5.348344135530575e-08
98398,398999,0,398999,18385.13614487648,5.274857482142117e-08
98498,399399,0,399399,18397.37694168091,5.217998129385823e-08
98599,399803,0,399803,18409.859637975693,5.171315126473708e-08
98699,400280,0,400280,18421.979474782944,5.109606705686943e-08
98799,400690,0,400690,18433.848405838013,5.036346200305783e-08
98899,401175,0,401175,18445.617862939835,4.973823201808809e-08
98999,401635,0,401635,18457.574733018875,4.916140360743018e-08
99099,402070,0,402070,18469.481784820557,4.8682400601033e-08
99199,402492,0,402492,18481.356375694275,4.803456827132368e-08
99299,402892,0,402892,18493.98102402687,4.7317108423285936e-08
99399,403292,0,403292,18507.821284770966,4.663701697501625e-08
99499,403692,0,403692,18519.195009946823,4.6120049341829064e-08
99600,404100,0,404100,18532.40629673004,4.547682688458229e-08
99700,404500,0,404500,18543.96808075905,4.489454433830025e-08
99800,404903,0,404903,18557.293793916702,4.4330824546781934e-08
99900,405325,0,405325,18568.5245718956,4.3876470418214795e-08
100000,405740,0,405740,18579.303149700165,4.342412912807868e-08

